JevAgentHarness: Benchmarking, Deploying and Training Decision Models That Share Control with LLMs

Large language model (LLM) agents now fix software, operate computers and serve customers, but their harnesses, the programs that run them, call a large LLM at every step, which makes long tasks slow and costly. Most of these calls end in a multiple-choice decision, such as which tool to call next. Decision models such as Jev answer these questions directly, at a fraction of an LLM call's time and price. We ask how a harness can delegate these decisions to a decision model with little loss of success. To evaluate decision models in agentic tasks, we build AgentDecisionBench, which tests them from isolated questions up to control of a running agent, on public benchmarks and our DecisionGym environment. The decision model most accurate on isolated questions solved only 69.5% of agent tasks, and without a fitted confidence threshold, delegating tool choices lowered success by 19.0 points. Building on these findings, we then design JevAgentHarness, which fits this threshold for each choice on the agent's own trajectories and lets the LLM decide below it. Because existing decision models never see the states an agent reaches after its own mistakes, we train AgentDecision-4B, an open 4B model, on such states with Jev's answers as labels. On tasks unlike its training data, the agent solved 91.5% of them with AgentDecision-4B and 82.0% with Jev. On tasks like their training data, 4B models trained this way made agents 81.1-89.0% cheaper and up to 2.5 times faster, without losing 3 or more points of task success. The models, data, and harness will be released at https://github.com/JevAgentHarness/JevAgentHarness.

==> figures/fig_levels.tex <==
\definecolor{rkNavy}{HTML}{2B3A55}   \definecolor{rkGrey}{HTML}{5C6476}   \definecolor{rkRule}{HTML}{DCE1E9}
\definecolor{lvStatic}{HTML}{E4DACA} \definecolor{lvStaticE}{HTML}{B6A486}
\definecolor{lvSame}{HTML}{F8E2A6}   \definecolor{lvSameE}{HTML}{C9972F}
\definecolor{lvLive}{HTML}{BCD3F0}   \definecolor{lvLiveE}{HTML}{5A88C8}
\definecolor{lvCard}{HTML}{FBFAF7}
\providecolor{hdOurs}{HTML}{7D58B0}%
\colorlet{lvOurs}{hdOurs!50}\colorlet{lvOursE}{hdOurs}\colorlet{lvOursT}{hdOurs!85!black}
\providecommand{\lvB}{\fontsize{7}{8.3}\selectfont\rmfamily}
\providecommand{\lvH}{\fontsize{8.5}{10}\selectfont\rmfamily\bfseries\itshape}
\providecommand{\lvHs}{\fontsize{7.5}{9}\selectfont\rmfamily\bfseries\itshape}%
\providecommand{\lvI}{\fontsize{7}{8.3}\selectfont\rmfamily\itshape}
\providecommand{\lvP}{\fontsize{7}{8.3}\selectfont\rmfamily\bfseries}
\providecommand{\lvS}{0.155}%
\def\lvHasE{0}\def\lvHasA{0}\def\lvHasO{0}\def\lvHasJ{0}
\def\lvExtraCore{1}
\def\lvHasG{0}%
\ifcsname jevres@e28/l3/success\endcsname\def\lvHasA{1}\fi%
\edef\lvExtra{\the\numexpr\lvExtraCore+\lvHasG+\lvHasA\relax}
\ifnum\lvExtra>0 \def\lvPitch{3.0}\def\lvHalf{1.15}\def\lvBandH{1.35}\else\def\lvPitch{3.6}\def\lvHalf{1.3}\def\lvBandH{1.65}\fi
\pgfmathsetmacro\lvBot{32.6-(\lvExtra+7)*\lvPitch-1.4}%
\edef\lvNOurs{\the\numexpr1+\lvHasA+\lvHasG\relax}%
\providecommand{\lvBar}[5]{%
  \pgfmathsetmacro\lvw{max(\res{#3}*\lvS,0.35)}%
  \draw[fill=#4, draw=#5, line width=0.35pt, rounded corners=0.45pt] (#1,#2-\lvHalf) rectangle ({#1+\lvw},#2+\lvHalf);
  \pgfmathtruncatemacro\lvin{greater(\res{#3},39.95)}%
  \ifnum\lvin=1 \node[font=\lvB, text=rkNavy, anchor=east] at ({#1+\lvw-0.55},#2-0.05) {\res{#3}};%
  \else \node[font=\lvB, text=rkNavy, anchor=west] at ({#1+\lvw+0.6},#2-0.05) {\res{#3}};\fi}
\def\lvU{0}
\providecommand{\lvRowK}[4]{%
  \ifnum\lvU=1 \node[font=\lvB, text=lvOursT, anchor=east] at (19.6,\lvY-0.05) {#1};%
  \else\node[font=\lvB, text=rkNavy, anchor=east] at (19.6,\lvY-0.05) {#1};\fi
  \ifnum\lvU=1 \lvBar{21}{\lvY}{#2}{lvOurs}{lvOursE}\else\lvBar{21}{\lvY}{#2}{lvStatic}{lvStaticE}\fi
  \ifnum\lvU=1 \lvBar{40}{\lvY}{#3}{lvOurs}{lvOursE}\else\lvBar{40}{\lvY}{#3}{lvSame}{lvSameE}\fi
  \xdef\lvStMax{\fpeval{max(\lvStMax,\res{#2})}}\xdef\lvStMin{\fpeval{min(\lvStMin,\res{#2})}}%
  \xdef\lvCoMax{\fpeval{max(\lvCoMax,\res{#3})}}\xdef\lvCoMin{\fpeval{min(\lvCoMin,\res{#3})}}%
  \ifcsname jevres@#4\endcsname
    \ifnum\lvU=1 \lvBar{59}{\lvY}{#4}{lvOurs}{lvOursE}\else\lvBar{59}{\lvY}{#4}{lvLive}{lvLiveE}\fi
    \xdef\lvLiMax{\fpeval{max(\lvLiMax,\res{#4})}}\xdef\lvLiMin{\fpeval{min(\lvLiMin,\res{#4})}}%
  \else
    \node[font=\lvB, text=rkGrey, anchor=west] at (59.6,\lvY-0.05) {--};\gdef\lvAnyDash{1}%
  \fi
  \pgfmathsetmacro\lvYn{\lvY-\lvPitch}\xdef\lvY{\lvYn}}
\providecommand{\lvRow}[2]{\lvRowK{#1}{explore/startlux_live/#2/e1_acc}{explore/startlux_live/#2/corpus_acc}{explore/startlux_live/#2/live_success}}
\providecommand{\lvRowS}[3]{\ifcsname jevres@e21/#3/l2/all\endcsname\lvRowK{#1}{#2}{e21/#3/l2/all}{e21/#3/l3/success}\fi}%
\providecommand{\lvGap}[1]{\pgfmathsetmacro\lvYn{\lvY-#1}\xdef\lvY{\lvYn}}%
\ifdefined\lvDefsOnly\else
\ifdefined\lvBodyOnly\else
\begin{figure}[t]
\centering
\fi
\gdef\lvAnyDash{0}%
\def\lvY{32.6}\def\lvStMax{0}\def\lvStMin{100}\def\lvCoMax{0}\def\lvCoMin{100}\def\lvLiMax{0}\def\lvLiMin{100}%
\makebox[\columnwidth]{%
\begin{tikzpicture}[jevfig]
\foreach \x/\l/\h/\e in {21/L1/Isolated/lvStaticE,
    40/L2/Step-level/lvSameE,
    59/L3/Task-level/lvLiveE} {
  \draw[draw=rkRule, line width=0.45pt, fill=lvCard, rounded corners=1.6mm] (\x-1.1,\lvBot-5.0) rectangle (\x+17.4,47.4);
  \node[font=\lvH, text=rkNavy, anchor=base] at (\x+7.75,43.4) {\l};
  \node[font=\lvHs, text=rkNavy, anchor=base] at (\x+7.75,40.3) {\h};}
\foreach \x in {21,40,59} {
  \foreach \t in {0,50,100} {\draw[rkRule, line width=0.4pt] ({\x+\t*\lvS},\lvBot-1.4) -- ({\x+\t*\lvS},35.4);}
  \foreach \t in {50,100} {\node[font=\lvB, text=rkGrey, anchor=base] at ({\x+\t*\lvS},\lvBot-4.0) {\t};}}
\foreach \x in {38.65, 57.65} {
  \fill[white] (\x,44.4) circle (1.45);
  \draw[rkNavy!70, line width=0.6pt, line cap=round, line join=round] (\x-0.35,45.1) -- (\x+0.35,44.4) -- (\x-0.35,43.7);}
\fill[hdOurs!8, rounded corners=0.8mm] (-1.7,{32.6-(\lvNOurs-1)*\lvPitch-\lvBandH}) rectangle (76.7,32.6+\lvBandH);
\gdef\lvU{1}%
\lvRowS{\textbf{\modeltext{}-4B}}{e12/e12/e1/acc/toolchoice}{e12}
\ifnum\lvHasA=1 \lvRowK{\textbf{\modeltext{}-0.8B}}{e28/l1/tool}{e28/l2/all}{e28/l3/success}\fi
\gdef\lvU{0}%
\lvGap{0.6}
\lvRowS{\jev{}}{explore/startlux_live/jev/e1_acc}{jev}
\lvRowS{OpenAI Decisions}{e15/oaidec/e1_acc}{oaidec}
\lvGap{0.8}
\lvRowS{OpenJev-27B}{e15/openjevhf/e1_acc}{openjevhf}
\lvRowS{StartLux-27B}{explore/startlux_live/sl27b/e1_acc}{sl27b}
\lvRowS{StartLux-9B}{explore/startlux_live/sl9b/e1_acc}{sl9b}
\lvRowS{StartLux-4B}{explore/startlux_live/sl4b/e1_acc}{sl4b}
\lvRowS{Intern-Decision-4B}{explore/startlux_live/intern/e1_acc}{intern}
\foreach \x/\g/\e in {21/{\fpeval{round(\lvStMax-\lvStMin,1)}}/lvStaticE,
    40/{\fpeval{round(\lvCoMax-\lvCoMin,1)}}/lvSameE,
    59/{\fpeval{round(\lvLiMax-\lvLiMin,1)}}/lvLiveE} {
  \node[font=\lvP, text=\e!75!black, anchor=base] at (\x+7.75,37.0) {spread \g\,pt};}
\end{tikzpicture}}
\ifdefined\lvBodyOnly\else
\caption[Evaluation levels]{\textbf{Similar on fixed questions, far apart inside the agent.} L1: tool-choice
accuracy (\%) on \res{diff/e1/bfcl_tool_select/n} BFCL items; L2: accuracy at the \res{e21/corpus/occurrences} states
recorded from live runs on \res{e21/corpus/tasks} shifted \gym{} tasks (renamed tools, added distractors, new task
kinds); L3: task success (\%) when the model picks every tool on \res{e21/rl/l3/n} shifted tasks (agent LLM Flash,
which alone solved \res{e21/llm_only/l3/success}\%\ifnum\lvAnyDash=1; --: no live run\fi). Spread: best minus worst
model. $^\ast$Ours, trained on states of \gym{}'s unshifted generator (App.~\ref{app:levels}).}
\label{fig:levels}\label{fig:slope}
\end{figure}
\fi
\fi


==> generated/coverage.tex <==
\makeatletter
\providecommand{\res}[1]{\ifcsname jevres@#1\endcsname\csname jevres@#1\endcsname\else\tbd\fi}
\providecommand{\defres}[2]{\expandafter\def\csname jevres@#1\endcsname{#2}}
\defres{cov/ask/act/occurrences}{4{,}565}
\defres{cov/ask/act/tasks}{200}
\defres{cov/ask/after_off_plan/occurrences}{386}
\defres{cov/ask/after_off_plan/tasks}{57}
\defres{cov/ask/all/occurrences}{5{,}314}
\defres{cov/ask/all/tasks}{200}
\defres{cov/ask/ask_now/occurrences}{582}
\defres{cov/ask/ask_now/tasks}{100}
\defres{cov/ask/ask_only/occurrences}{267}
\defres{cov/ask/ask_only/tasks}{100}
\defres{cov/ask/ask_optional/occurrences}{167}
\defres{cov/ask/ask_optional/tasks}{25}
\defres{cov/ask/base/act/acc}{54.9}
\defres{cov/ask/base/act/over_ask}{1.5}
\defres{cov/ask/base/after_off_plan/acc}{26.7}
\defres{cov/ask/base/all/acc}{50.1}
\defres{cov/ask/base/ask_now/acc}{47.3}
\defres{cov/ask/base/ask_now/acted}{258}
\defres{cov/ask/base/ask_now/asked}{264}
\defres{cov/ask/base/ask_now/failed}{0}
\defres{cov/ask/base/ask_now/finished}{4}
\defres{cov/ask/base/ask_now/other_acceptable}{27}
\defres{cov/ask/base/ask_now/other_wrong}{29}
\defres{cov/ask/base/ask_only/acc}{24.0}
\defres{cov/ask/base/ask_only/acted}{166}
\defres{cov/ask/base/ask_only/asked}{96}
\defres{cov/ask/base/ask_only/failed}{0}
\defres{cov/ask/base/ask_only/finished}{1}
\defres{cov/ask/base/ask_only/other_acceptable}{0}
\defres{cov/ask/base/ask_only/other_wrong}{4}
\defres{cov/ask/base/ask_optional/acc}{60.2}
\defres{cov/ask/intern/act/acc}{76.1}
\defres{cov/ask/intern/act/over_ask}{1.4}
\defres{cov/ask/intern/after_off_plan/acc}{47.6}
\defres{cov/ask/intern/all/acc}{75.2}
\defres{cov/ask/intern/ask_now/acc}{59.6}
\defres{cov/ask/intern/ask_now/acted}{166}
\defres{cov/ask/intern/ask_now/asked}{120}
\defres{cov/ask/intern/ask_now/failed}{0}
\defres{cov/ask/intern/ask_now/finished}{1}
\defres{cov/ask/intern/ask_now/other_acceptable}{269}
\defres{cov/ask/intern/ask_now/other_wrong}{26}
\defres{cov/ask/intern/ask_only/acc}{25.0}
\defres{cov/ask/intern/ask_only/acted}{164}
\defres{cov/ask/intern/ask_only/asked}{100}
\defres{cov/ask/intern/ask_only/failed}{0}
\defres{cov/ask/intern/ask_only/finished}{1}
\defres{cov/ask/intern/ask_only/other_acceptable}{0}
\defres{cov/ask/intern/ask_only/other_wrong}{2}
\defres{cov/ask/intern/ask_optional/acc}{86.3}
\defres{cov/ask/jev/act/acc}{94.2}
\defres{cov/ask/jev/act/over_ask}{1.2}
\defres{cov/ask/jev/after_off_plan/acc}{81.5}
\defres{cov/ask/jev/all/acc}{91.5}
\defres{cov/ask/jev/ask_now/acc}{64.4}
\defres{cov/ask/jev/ask_now/acted}{162}
\defres{cov/ask/jev/ask_now/asked}{270}
\defres{cov/ask/jev/ask_now/failed}{0}
\defres{cov/ask/jev/ask_now/finished}{2}
\defres{cov/ask/jev/ask_now/other_acceptable}{148}
\defres{cov/ask/jev/ask_now/other_wrong}{0}
\defres{cov/ask/jev/ask_only/acc}{27.0}
\defres{cov/ask/jev/ask_only/acted}{162}
\defres{cov/ask/jev/ask_only/asked}{105}
\defres{cov/ask/jev/ask_only/failed}{0}
\defres{cov/ask/jev/ask_only/finished}{0}
\defres{cov/ask/jev/ask_only/other_acceptable}{0}
\defres{cov/ask/jev/ask_only/other_wrong}{0}
\defres{cov/ask/jev/ask_optional/acc}{100.0}
\defres{cov/ask/rl/act/acc}{98.9}
\defres{cov/ask/rl/act/over_ask}{0.8}
\defres{cov/ask/rl/after_off_plan/acc}{94.7}
\defres{cov/ask/rl/all/acc}{99.2}
\defres{cov/ask/rl/ask_now/acc}{100.0}
\defres{cov/ask/rl/ask_now/acted}{0}
\defres{cov/ask/rl/ask_now/asked}{503}
\defres{cov/ask/rl/ask_now/failed}{0}
\defres{cov/ask/rl/ask_now/finished}{0}
\defres{cov/ask/rl/ask_now/other_acceptable}{79}
\defres{cov/ask/rl/ask_now/other_wrong}{0}
\defres{cov/ask/rl/ask_only/acc}{100.0}
\defres{cov/ask/rl/ask_only/acted}{0}
\defres{cov/ask/rl/ask_only/asked}{267}
\defres{cov/ask/rl/ask_only/failed}{0}
\defres{cov/ask/rl/ask_only/finished}{0}
\defres{cov/ask/rl/ask_only/other_acceptable}{0}
\defres{cov/ask/rl/ask_only/other_wrong}{0}
\defres{cov/ask/rl/ask_optional/acc}{100.0}
\defres{cov/ask/sft_v1/act/acc}{98.9}
\defres{cov/ask/sft_v1/act/over_ask}{0.8}
\defres{cov/ask/sft_v1/after_off_plan/acc}{93.8}
\defres{cov/ask/sft_v1/all/acc}{99.2}
\defres{cov/ask/sft_v1/ask_now/acc}{100.0}
\defres{cov/ask/sft_v1/ask_now/acted}{0}
\defres{cov/ask/sft_v1/ask_now/asked}{581}
\defres{cov/ask/sft_v1/ask_now/failed}{0}
\defres{cov/ask/sft_v1/ask_now/finished}{0}
\defres{cov/ask/sft_v1/ask_now/other_acceptable}{1}
\defres{cov/ask/sft_v1/ask_now/other_wrong}{0}
\defres{cov/ask/sft_v1/ask_only/acc}{100.0}
\defres{cov/ask/sft_v1/ask_only/acted}{0}
\defres{cov/ask/sft_v1/ask_only/asked}{267}
\defres{cov/ask/sft_v1/ask_only/failed}{0}
\defres{cov/ask/sft_v1/ask_only/finished}{0}
\defres{cov/ask/sft_v1/ask_only/other_acceptable}{0}
\defres{cov/ask/sft_v1/ask_only/other_wrong}{0}
\defres{cov/ask/sft_v1/ask_optional/acc}{100.0}
\defres{cov/ask/sl0.8b/act/acc}{53.1}
\defres{cov/ask/sl0.8b/act/over_ask}{8.5}
\defres{cov/ask/sl0.8b/after_off_plan/acc}{31.5}
\defres{cov/ask/sl0.8b/all/acc}{48.3}
\defres{cov/ask/sl0.8b/ask_now/acc}{49.4}
\defres{cov/ask/sl0.8b/ask_now/acted}{279}
\defres{cov/ask/sl0.8b/ask_now/asked}{301}
\defres{cov/ask/sl0.8b/ask_now/failed}{0}
\defres{cov/ask/sl0.8b/ask_now/finished}{0}
\defres{cov/ask/sl0.8b/ask_now/other_acceptable}{1}
\defres{cov/ask/sl0.8b/ask_now/other_wrong}{1}
\defres{cov/ask/sl0.8b/ask_only/acc}{25.0}
\defres{cov/ask/sl0.8b/ask_only/acted}{167}
\defres{cov/ask/sl0.8b/ask_only/asked}{100}
\defres{cov/ask/sl0.8b/ask_only/failed}{0}
\defres{cov/ask/sl0.8b/ask_only/finished}{0}
\defres{cov/ask/sl0.8b/ask_only/other_acceptable}{0}
\defres{cov/ask/sl0.8b/ask_only/other_wrong}{0}
\defres{cov/ask/sl0.8b/ask_optional/acc}{60.2}
\defres{cov/ask/sl27b/act/acc}{98.7}
\defres{cov/ask/sl27b/act/over_ask}{0.7}
\defres{cov/ask/sl27b/after_off_plan/acc}{85.1}
\defres{cov/ask/sl27b/all/acc}{93.9}
\defres{cov/ask/sl27b/ask_now/acc}{63.4}
\defres{cov/ask/sl27b/ask_now/acted}{165}
\defres{cov/ask/sl27b/ask_now/asked}{102}
\defres{cov/ask/sl27b/ask_now/failed}{0}
\defres{cov/ask/sl27b/ask_now/finished}{2}
\defres{cov/ask/sl27b/ask_now/other_acceptable}{313}
\defres{cov/ask/sl27b/ask_now/other_wrong}{0}
\defres{cov/ask/sl27b/ask_only/acc}{26.0}
\defres{cov/ask/sl27b/ask_only/acted}{165}
\defres{cov/ask/sl27b/ask_only/asked}{102}
\defres{cov/ask/sl27b/ask_only/failed}{0}
\defres{cov/ask/sl27b/ask_only/finished}{0}
\defres{cov/ask/sl27b/ask_only/other_acceptable}{0}
\defres{cov/ask/sl27b/ask_only/other_wrong}{0}
\defres{cov/ask/sl27b/ask_optional/acc}{100.0}
\defres{cov/ask/sl2b/act/acc}{69.7}
\defres{cov/ask/sl2b/act/over_ask}{1.1}
\defres{cov/ask/sl2b/after_off_plan/acc}{47.2}
\defres{cov/ask/sl2b/all/acc}{68.4}
\defres{cov/ask/sl2b/ask_now/acc}{61.8}
\defres{cov/ask/sl2b/ask_now/acted}{169}
\defres{cov/ask/sl2b/ask_now/asked}{137}
\defres{cov/ask/sl2b/ask_now/failed}{0}
\defres{cov/ask/sl2b/ask_now/finished}{1}
\defres{cov/ask/sl2b/ask_now/other_acceptable}{260}
\defres{cov/ask/sl2b/ask_now/other_wrong}{15}
\defres{cov/ask/sl2b/ask_only/acc}{27.0}
\defres{cov/ask/sl2b/ask_only/acted}{161}
\defres{cov/ask/sl2b/ask_only/asked}{105}
\defres{cov/ask/sl2b/ask_only/failed}{0}
\defres{cov/ask/sl2b/ask_only/finished}{1}
\defres{cov/ask/sl2b/ask_only/other_acceptable}{0}
\defres{cov/ask/sl2b/ask_only/other_wrong}{0}
\defres{cov/ask/sl2b/ask_optional/acc}{82.1}
\defres{cov/ask/sl4b/act/acc}{91.3}
\defres{cov/ask/sl4b/act/over_ask}{0.3}
\defres{cov/ask/sl4b/after_off_plan/acc}{76.8}
\defres{cov/ask/sl4b/all/acc}{89.1}
\defres{cov/ask/sl4b/ask_now/acc}{84.1}
\defres{cov/ask/sl4b/ask_now/acted}{109}
\defres{cov/ask/sl4b/ask_now/asked}{156}
\defres{cov/ask/sl4b/ask_now/failed}{0}
\defres{cov/ask/sl4b/ask_now/finished}{2}
\defres{cov/ask/sl4b/ask_now/other_acceptable}{310}
\defres{cov/ask/sl4b/ask_now/other_wrong}{5}
\defres{cov/ask/sl4b/ask_only/acc}{47.0}
\defres{cov/ask/sl4b/ask_only/acted}{109}
\defres{cov/ask/sl4b/ask_only/asked}{156}
\defres{cov/ask/sl4b/ask_only/failed}{0}
\defres{cov/ask/sl4b/ask_only/finished}{0}
\defres{cov/ask/sl4b/ask_only/other_acceptable}{0}
\defres{cov/ask/sl4b/ask_only/other_wrong}{2}
\defres{cov/ask/sl4b/ask_optional/acc}{66.1}
\defres{cov/ask/sl9b/act/acc}{91.8}
\defres{cov/ask/sl9b/act/over_ask}{0.9}
\defres{cov/ask/sl9b/after_off_plan/acc}{74.3}
\defres{cov/ask/sl9b/all/acc}{91.8}
\defres{cov/ask/sl9b/ask_now/acc}{87.1}
\defres{cov/ask/sl9b/ask_now/acted}{105}
\defres{cov/ask/sl9b/ask_now/asked}{162}
\defres{cov/ask/sl9b/ask_now/failed}{0}
\defres{cov/ask/sl9b/ask_now/finished}{3}
\defres{cov/ask/sl9b/ask_now/other_acceptable}{311}
\defres{cov/ask/sl9b/ask_now/other_wrong}{1}
\defres{cov/ask/sl9b/ask_only/acc}{50.0}
\defres{cov/ask/sl9b/ask_only/acted}{105}
\defres{cov/ask/sl9b/ask_only/asked}{162}
\defres{cov/ask/sl9b/ask_only/failed}{0}
\defres{cov/ask/sl9b/ask_only/finished}{0}
\defres{cov/ask/sl9b/ask_only/other_acceptable}{0}
\defres{cov/ask/sl9b/ask_only/other_wrong}{0}
\defres{cov/ask/sl9b/ask_optional/acc}{98.9}
\defres{cov/ask/v2/act/acc}{99.2}
\defres{cov/ask/v2/act/over_ask}{0.6}
\defres{cov/ask/v2/after_off_plan/acc}{95.0}
\defres{cov/ask/v2/all/acc}{99.4}
\defres{cov/ask/v2/ask_now/acc}{100.0}
\defres{cov/ask/v2/ask_now/acted}{0}
\defres{cov/ask/v2/ask_now/asked}{582}
\defres{cov/ask/v2/ask_now/failed}{0}
\defres{cov/ask/v2/ask_now/finished}{0}
\defres{cov/ask/v2/ask_now/other_acceptable}{0}
\defres{cov/ask/v2/ask_now/other_wrong}{0}
\defres{cov/ask/v2/ask_only/acc}{100.0}
\defres{cov/ask/v2/ask_only/acted}{0}
\defres{cov/ask/v2/ask_only/asked}{267}
\defres{cov/ask/v2/ask_only/failed}{0}
\defres{cov/ask/v2/ask_only/finished}{0}
\defres{cov/ask/v2/ask_only/other_acceptable}{0}
\defres{cov/ask/v2/ask_only/other_wrong}{0}
\defres{cov/ask/v2/ask_optional/acc}{100.0}
\defres{cov/gate/stop/flash_intern/all/false_veto}{28.6}
\defres{cov/gate/stop/flash_intern/all/n}{695}
\defres{cov/gate/stop/flash_intern/all/right}{695}
\defres{cov/gate/stop/flash_intern/all/vetoed_right}{199}
\defres{cov/gate/stop/flash_intern/all/vetoed_wrong}{0}
\defres{cov/gate/stop/flash_intern/all/wrong}{0}
\defres{cov/gate/stop/flash_intern/episodes/accepted_right}{458}
\defres{cov/gate/stop/flash_intern/episodes/blocked}{40}
\defres{cov/gate/stop/flash_intern/episodes/blocked_then_success}{38}
\defres{cov/gate/stop/flash_intern/episodes/caught}{0}
\defres{cov/gate/stop/flash_intern/episodes/caught_then_success}{0}
\defres{cov/gate/stop/flash_intern/episodes/wrong_accepted}{0}
\defres{cov/gate/stop/flash_intern/first/false_veto}{8.0}
\defres{cov/gate/stop/flash_intern/first/n}{498}
\defres{cov/gate/stop/flash_intern/first/right}{498}
\defres{cov/gate/stop/flash_intern/first/vetoed_right}{40}
\defres{cov/gate/stop/flash_intern/first/vetoed_wrong}{0}
\defres{cov/gate/stop/flash_intern/first/wrong}{0}
\defres{cov/gate/stop/flash_intern/premature}{0}
\defres{cov/gate/stop/flash_jev/all/false_veto}{17.3}
\defres{cov/gate/stop/flash_jev/all/n}{600}
\defres{cov/gate/stop/flash_jev/all/right}{600}
\defres{cov/gate/stop/flash_jev/all/vetoed_right}{104}
\defres{cov/gate/stop/flash_jev/all/vetoed_wrong}{0}
\defres{cov/gate/stop/flash_jev/all/wrong}{0}
\defres{cov/gate/stop/flash_jev/episodes/accepted_right}{462}
\defres{cov/gate/stop/flash_jev/episodes/blocked}{37}
\defres{cov/gate/stop/flash_jev/episodes/blocked_then_success}{34}
\defres{cov/gate/stop/flash_jev/episodes/caught}{0}
\defres{cov/gate/stop/flash_jev/episodes/caught_then_success}{0}
\defres{cov/gate/stop/flash_jev/episodes/wrong_accepted}{0}
\defres{cov/gate/stop/flash_jev/first/false_veto}{7.4}
\defres{cov/gate/stop/flash_jev/first/n}{499}
\defres{cov/gate/stop/flash_jev/first/right}{499}
\defres{cov/gate/stop/flash_jev/first/vetoed_right}{37}
\defres{cov/gate/stop/flash_jev/first/vetoed_wrong}{0}
\defres{cov/gate/stop/flash_jev/first/wrong}{0}
\defres{cov/gate/stop/flash_jev/premature}{0}
\defres{cov/gate/stop/flash_lite/all/false_veto}{20.7}
\defres{cov/gate/stop/flash_lite/all/n}{251}
\defres{cov/gate/stop/flash_lite/all/right}{251}
\defres{cov/gate/stop/flash_lite/all/vetoed_right}{52}
\defres{cov/gate/stop/flash_lite/all/vetoed_wrong}{0}
\defres{cov/gate/stop/flash_lite/all/wrong}{0}
\defres{cov/gate/stop/flash_lite/episodes/accepted_right}{194}
\defres{cov/gate/stop/flash_lite/episodes/blocked}{6}
\defres{cov/gate/stop/flash_lite/episodes/blocked_then_success}{5}
\defres{cov/gate/stop/flash_lite/episodes/caught}{0}
\defres{cov/gate/stop/flash_lite/episodes/caught_then_success}{0}
\defres{cov/gate/stop/flash_lite/episodes/wrong_accepted}{0}
\defres{cov/gate/stop/flash_lite/first/false_veto}{3.0}
\defres{cov/gate/stop/flash_lite/first/n}{200}
\defres{cov/gate/stop/flash_lite/first/right}{200}
\defres{cov/gate/stop/flash_lite/first/vetoed_right}{6}
\defres{cov/gate/stop/flash_lite/first/vetoed_wrong}{0}
\defres{cov/gate/stop/flash_lite/first/wrong}{0}
\defres{cov/gate/stop/flash_lite/premature}{0}
\defres{cov/gate/stop/lite_intern/all/auroc}{0.64}
\defres{cov/gate/stop/lite_intern/all/false_veto}{69.3}
\defres{cov/gate/stop/lite_intern/all/n}{2{,}199}
\defres{cov/gate/stop/lite_intern/all/recall}{94.0}
\defres{cov/gate/stop/lite_intern/all/right}{1{,}261}
\defres{cov/gate/stop/lite_intern/all/vetoed_right}{874}
\defres{cov/gate/stop/lite_intern/all/vetoed_wrong}{882}
\defres{cov/gate/stop/lite_intern/all/wrong}{938}
\defres{cov/gate/stop/lite_intern/episodes/accepted_right}{347}
\defres{cov/gate/stop/lite_intern/episodes/blocked}{58}
\defres{cov/gate/stop/lite_intern/episodes/blocked_then_success}{26}
\defres{cov/gate/stop/lite_intern/episodes/caught}{61}
\defres{cov/gate/stop/lite_intern/episodes/caught_then_success}{14}
\defres{cov/gate/stop/lite_intern/episodes/wrong_accepted}{34}
\defres{cov/gate/stop/lite_intern/first/auroc}{0.89}
\defres{cov/gate/stop/lite_intern/first/false_veto}{14.3}
\defres{cov/gate/stop/lite_intern/first/n}{500}
\defres{cov/gate/stop/lite_intern/first/recall}{64.2}
\defres{cov/gate/stop/lite_intern/first/right}{405}
\defres{cov/gate/stop/lite_intern/first/vetoed_right}{58}
\defres{cov/gate/stop/lite_intern/first/vetoed_wrong}{61}
\defres{cov/gate/stop/lite_intern/first/wrong}{95}
\defres{cov/gate/stop/lite_intern/premature}{0}
\defres{cov/gate/stop/lite_jev/all/auroc}{0.81}
\defres{cov/gate/stop/lite_jev/all/false_veto}{47.0}
\defres{cov/gate/stop/lite_jev/all/n}{1{,}639}
\defres{cov/gate/stop/lite_jev/all/recall}{95.5}
\defres{cov/gate/stop/lite_jev/all/right}{774}
\defres{cov/gate/stop/lite_jev/all/vetoed_right}{364}
\defres{cov/gate/stop/lite_jev/all/vetoed_wrong}{826}
\defres{cov/gate/stop/lite_jev/all/wrong}{865}
\defres{cov/gate/stop/lite_jev/episodes/accepted_right}{401}
\defres{cov/gate/stop/lite_jev/episodes/blocked}{14}
\defres{cov/gate/stop/lite_jev/episodes/blocked_then_success}{5}
\defres{cov/gate/stop/lite_jev/episodes/caught}{52}
\defres{cov/gate/stop/lite_jev/episodes/caught_then_success}{4}
\defres{cov/gate/stop/lite_jev/episodes/wrong_accepted}{33}
\defres{cov/gate/stop/lite_jev/first/auroc}{0.96}
\defres{cov/gate/stop/lite_jev/first/false_veto}{3.4}
\defres{cov/gate/stop/lite_jev/first/n}{500}
\defres{cov/gate/stop/lite_jev/first/recall}{61.2}
\defres{cov/gate/stop/lite_jev/first/right}{415}
\defres{cov/gate/stop/lite_jev/first/vetoed_right}{14}
\defres{cov/gate/stop/lite_jev/first/vetoed_wrong}{52}
\defres{cov/gate/stop/lite_jev/first/wrong}{85}
\defres{cov/gate/stop/lite_jev/premature}{0}
\defres{cov/gate/stop/lite_random/all/auroc}{0.47}
\defres{cov/gate/stop/lite_random/all/false_veto}{31.1}
\defres{cov/gate/stop/lite_random/all/n}{287}
\defres{cov/gate/stop/lite_random/all/recall}{26.1}
\defres{cov/gate/stop/lite_random/all/right}{241}
\defres{cov/gate/stop/lite_random/all/vetoed_right}{75}
\defres{cov/gate/stop/lite_random/all/vetoed_wrong}{12}
\defres{cov/gate/stop/lite_random/all/wrong}{46}
\defres{cov/gate/stop/lite_random/episodes/accepted_right}{112}
\defres{cov/gate/stop/lite_random/episodes/blocked}{55}
\defres{cov/gate/stop/lite_random/episodes/blocked_then_success}{52}
\defres{cov/gate/stop/lite_random/episodes/caught}{10}
\defres{cov/gate/stop/lite_random/episodes/caught_then_success}{2}
\defres{cov/gate/stop/lite_random/episodes/wrong_accepted}{23}
\defres{cov/gate/stop/lite_random/first/auroc}{0.49}
\defres{cov/gate/stop/lite_random/first/false_veto}{32.9}
\defres{cov/gate/stop/lite_random/first/n}{200}
\defres{cov/gate/stop/lite_random/first/recall}{30.3}
\defres{cov/gate/stop/lite_random/first/right}{167}
\defres{cov/gate/stop/lite_random/first/vetoed_right}{55}
\defres{cov/gate/stop/lite_random/first/vetoed_wrong}{10}
\defres{cov/gate/stop/lite_random/first/wrong}{33}
\defres{cov/gate/stop/lite_random/premature}{0}
\defres{cov/gate/stop/n_all}{5{,}671}
\defres{cov/gate/stop/premature}{0}
\defres{cov/gate/tool/dm/state_changing/n}{1{,}601}
\defres{cov/gate/tool/dm/state_changing/wrong}{0}
\defres{cov/gate/tool/flash_intern/false_veto}{4.5}
\defres{cov/gate/tool/flash_intern/n}{1{,}532}
\defres{cov/gate/tool/flash_intern/right}{1{,}528}
\defres{cov/gate/tool/flash_intern/state_changing/n}{401}
\defres{cov/gate/tool/flash_intern/state_changing/right}{401}
\defres{cov/gate/tool/flash_intern/state_changing/right_vetoed}{3}
\defres{cov/gate/tool/flash_intern/state_changing/wrong}{0}
\defres{cov/gate/tool/flash_intern/state_changing/wrong_vetoed}{0}
\defres{cov/gate/tool/flash_intern/verdict/detour/n}{4}
\defres{cov/gate/tool/flash_intern/verdict/detour/vetoed}{3}
\defres{cov/gate/tool/flash_intern/vetoed_right}{68}
\defres{cov/gate/tool/flash_intern/vetoed_wrong}{3}
\defres{cov/gate/tool/flash_intern/wrong}{4}
\defres{cov/gate/tool/flash_jev/false_veto}{2.0}
\defres{cov/gate/tool/flash_jev/n}{1{,}501}
\defres{cov/gate/tool/flash_jev/right}{1{,}500}
\defres{cov/gate/tool/flash_jev/state_changing/n}{400}
\defres{cov/gate/tool/flash_jev/state_changing/right}{400}
\defres{cov/gate/tool/flash_jev/state_changing/right_vetoed}{1}
\defres{cov/gate/tool/flash_jev/state_changing/wrong}{0}
\defres{cov/gate/tool/flash_jev/state_changing/wrong_vetoed}{0}
\defres{cov/gate/tool/flash_jev/verdict/detour/n}{1}
\defres{cov/gate/tool/flash_jev/verdict/detour/vetoed}{1}
\defres{cov/gate/tool/flash_jev/vetoed_right}{30}
\defres{cov/gate/tool/flash_jev/vetoed_wrong}{1}
\defres{cov/gate/tool/flash_jev/wrong}{1}
\defres{cov/gate/tool/flash_lite/auroc}{0.84}
\defres{cov/gate/tool/flash_lite/false_veto}{10.2}
\defres{cov/gate/tool/flash_lite/n}{1{,}603}
\defres{cov/gate/tool/flash_lite/recall}{78.9}
\defres{cov/gate/tool/flash_lite/right}{1{,}584}
\defres{cov/gate/tool/flash_lite/state_changing/n}{407}
\defres{cov/gate/tool/flash_lite/state_changing/right}{405}
\defres{cov/gate/tool/flash_lite/state_changing/right_vetoed}{17}
\defres{cov/gate/tool/flash_lite/state_changing/wrong}{2}
\defres{cov/gate/tool/flash_lite/state_changing/wrong_vetoed}{2}
\defres{cov/gate/tool/flash_lite/verdict/detour/n}{17}
\defres{cov/gate/tool/flash_lite/verdict/detour/vetoed}{13}
\defres{cov/gate/tool/flash_lite/verdict/fatal/n}{2}
\defres{cov/gate/tool/flash_lite/verdict/fatal/vetoed}{2}
\defres{cov/gate/tool/flash_lite/vetoed_right}{162}
\defres{cov/gate/tool/flash_lite/vetoed_wrong}{15}
\defres{cov/gate/tool/flash_lite/wrong}{19}
\defres{cov/gate/tool/lite_intern/auroc}{0.96}
\defres{cov/gate/tool/lite_intern/false_veto}{3.0}
\defres{cov/gate/tool/lite_intern/n}{1{,}510}
\defres{cov/gate/tool/lite_intern/recall}{53.3}
\defres{cov/gate/tool/lite_intern/right}{1{,}465}
\defres{cov/gate/tool/lite_intern/state_changing/n}{400}
\defres{cov/gate/tool/lite_intern/state_changing/right}{400}
\defres{cov/gate/tool/lite_intern/state_changing/right_vetoed}{2}
\defres{cov/gate/tool/lite_intern/state_changing/wrong}{0}
\defres{cov/gate/tool/lite_intern/state_changing/wrong_vetoed}{0}
\defres{cov/gate/tool/lite_intern/verdict/detour/n}{15}
\defres{cov/gate/tool/lite_intern/verdict/detour/vetoed}{13}
\defres{cov/gate/tool/lite_intern/verdict/wrong_answer/n}{30}
\defres{cov/gate/tool/lite_intern/verdict/wrong_answer/vetoed}{11}
\defres{cov/gate/tool/lite_intern/vetoed_right}{44}
\defres{cov/gate/tool/lite_intern/vetoed_wrong}{24}
\defres{cov/gate/tool/lite_intern/wrong}{45}
\defres{cov/gate/tool/lite_jev/auroc}{0.97}
\defres{cov/gate/tool/lite_jev/false_veto}{1.3}
\defres{cov/gate/tool/lite_jev/n}{1{,}514}
\defres{cov/gate/tool/lite_jev/recall}{64.3}
\defres{cov/gate/tool/lite_jev/right}{1{,}472}
\defres{cov/gate/tool/lite_jev/state_changing/n}{400}
\defres{cov/gate/tool/lite_jev/state_changing/right}{400}
\defres{cov/gate/tool/lite_jev/state_changing/right_vetoed}{0}
\defres{cov/gate/tool/lite_jev/state_changing/wrong}{0}
\defres{cov/gate/tool/lite_jev/state_changing/wrong_vetoed}{0}
\defres{cov/gate/tool/lite_jev/verdict/detour/n}{11}
\defres{cov/gate/tool/lite_jev/verdict/detour/vetoed}{4}
\defres{cov/gate/tool/lite_jev/verdict/wrong_answer/n}{31}
\defres{cov/gate/tool/lite_jev/verdict/wrong_answer/vetoed}{23}
\defres{cov/gate/tool/lite_jev/vetoed_right}{19}
\defres{cov/gate/tool/lite_jev/vetoed_wrong}{27}
\defres{cov/gate/tool/lite_jev/wrong}{42}
\makeatother


==> generated/data_stats.tex <==
\makeatletter
\providecommand{\res}[1]{\ifcsname jevres@#1\endcsname\csname jevres@#1\endcsname\else\tbd\fi}
\providecommand{\defres}[2]{\expandafter\def\csname jevres@#1\endcsname{#2}}
\defres{data_stats/jevgym_eval/by_family/clarify/n}{250}
\defres{data_stats/jevgym_eval/by_family/clarify/plan_steps_median}{5.0}
\defres{data_stats/jevgym_eval/by_family/multi/n}{250}
\defres{data_stats/jevgym_eval/by_family/multi/plan_steps_median}{10.0}
\defres{data_stats/jevgym_eval/largest_plan_share}{24.8}
\defres{data_stats/jevgym_eval/n_distinct_plans}{11}
\defres{data_stats/jevgym_eval/n_families}{2}
\defres{data_stats/jevgym_eval/n_plan_tools}{7}
\defres{data_stats/jevgym_eval/n_tasks}{500}
\defres{data_stats/jevgym_eval/plan_calls_mean}{6.5}
\defres{data_stats/jevgym_eval/plan_calls_median}{6.5}
\defres{data_stats/jevgym_eval/plan_steps_max}{10}
\defres{data_stats/jevgym_eval/plan_steps_mean}{7.5}
\defres{data_stats/jevgym_eval/plan_steps_median}{7.5}
\defres{data_stats/jevgym_eval/plan_steps_min}{5}
\defres{data_stats/jevgym_eval/plan_steps_p90}{10.0}
\defres{data_stats/jevgym_eval/population}{PREREG\_A7\_STAGE2 A7.2 (a): stage2\_jevgym.yaml seeds 300000-300499}
\defres{data_stats/jevgym_eval/tools_offered_median}{69}
\makeatother


==> generated/difficulty.tex <==
\makeatletter
\providecommand{\res}[1]{\ifcsname jevres@#1\endcsname\csname jevres@#1\endcsname\else\tbd\fi}
\providecommand{\defres}[2]{\expandafter\def\csname jevres@#1\endcsname{#2}}
\defres{diff/c/after_off_plan/base/acc}{26.7}
\defres{diff/c/after_off_plan/base/ci/hi}{33.5}
\defres{diff/c/after_off_plan/base/ci/lo}{19.9}
\defres{diff/c/after_off_plan/intern/acc}{47.6}
\defres{diff/c/after_off_plan/intern/ci/hi}{57.1}
\defres{diff/c/after_off_plan/intern/ci/lo}{37.4}
\defres{diff/c/after_off_plan/jev/acc}{81.5}
\defres{diff/c/after_off_plan/jev/ci/hi}{88.1}
\defres{diff/c/after_off_plan/jev/ci/lo}{74.4}
\defres{diff/c/after_off_plan/n}{386}
\defres{diff/c/after_off_plan/offshelf/max}{85.1}
\defres{diff/c/after_off_plan/offshelf/max_model}{StartLux-27B}
\defres{diff/c/after_off_plan/offshelf/min}{31.5}
\defres{diff/c/after_off_plan/offshelf/min_model}{StartLux-0.8B}
\defres{diff/c/after_off_plan/rl/acc}{94.7}
\defres{diff/c/after_off_plan/rl/ci/hi}{98.3}
\defres{diff/c/after_off_plan/rl/ci/lo}{90.1}
\defres{diff/c/after_off_plan/sft_v1/acc}{93.8}
\defres{diff/c/after_off_plan/sft_v1/ci/hi}{97.6}
\defres{diff/c/after_off_plan/sft_v1/ci/lo}{89.3}
\defres{diff/c/after_off_plan/sl0.8b/acc}{31.5}
\defres{diff/c/after_off_plan/sl0.8b/ci/hi}{39.3}
\defres{diff/c/after_off_plan/sl0.8b/ci/lo}{23.7}
\defres{diff/c/after_off_plan/sl27b/acc}{85.1}
\defres{diff/c/after_off_plan/sl27b/ci/hi}{91.0}
\defres{diff/c/after_off_plan/sl27b/ci/lo}{78.1}
\defres{diff/c/after_off_plan/sl2b/acc}{47.2}
\defres{diff/c/after_off_plan/sl2b/ci/hi}{55.4}
\defres{diff/c/after_off_plan/sl2b/ci/lo}{38.6}
\defres{diff/c/after_off_plan/sl4b/acc}{76.8}
\defres{diff/c/after_off_plan/sl4b/ci/hi}{84.9}
\defres{diff/c/after_off_plan/sl4b/ci/lo}{67.7}
\defres{diff/c/after_off_plan/sl9b/acc}{74.3}
\defres{diff/c/after_off_plan/sl9b/ci/hi}{82.8}
\defres{diff/c/after_off_plan/sl9b/ci/lo}{64.9}
\defres{diff/c/after_off_plan/spread}{63.2}
\defres{diff/c/after_off_plan/tasks}{57}
\defres{diff/c/after_off_plan/v2/acc}{95.0}
\defres{diff/c/after_off_plan/v2/ci/hi}{98.2}
\defres{diff/c/after_off_plan/v2/ci/lo}{90.8}
\defres{diff/c/all/base/acc}{50.1}
\defres{diff/c/all/base/ci/hi}{52.5}
\defres{diff/c/all/base/ci/lo}{48.0}
\defres{diff/c/all/intern/acc}{75.2}
\defres{diff/c/all/intern/ci/hi}{77.1}
\defres{diff/c/all/intern/ci/lo}{73.2}
\defres{diff/c/all/jev/acc}{91.5}
\defres{diff/c/all/jev/ci/hi}{92.9}
\defres{diff/c/all/jev/ci/lo}{90.0}
\defres{diff/c/all/llm/acc}{99.9}
\defres{diff/c/all/llm/ci/hi}{100.0}
\defres{diff/c/all/llm/ci/lo}{99.8}
\defres{diff/c/all/n}{5{,}314}
\defres{diff/c/all/offshelf/max}{93.9}
\defres{diff/c/all/offshelf/max_model}{StartLux-27B}
\defres{diff/c/all/offshelf/min}{48.3}
\defres{diff/c/all/offshelf/min_model}{StartLux-0.8B}
\defres{diff/c/all/rl/acc}{99.2}
\defres{diff/c/all/rl/ci/hi}{99.8}
\defres{diff/c/all/rl/ci/lo}{98.4}
\defres{diff/c/all/sft_v1/acc}{99.2}
\defres{diff/c/all/sft_v1/ci/hi}{99.8}
\defres{diff/c/all/sft_v1/ci/lo}{98.4}
\defres{diff/c/all/sl0.8b/acc}{48.3}
\defres{diff/c/all/sl0.8b/ci/hi}{51.1}
\defres{diff/c/all/sl0.8b/ci/lo}{45.9}
\defres{diff/c/all/sl27b/acc}{93.9}
\defres{diff/c/all/sl27b/ci/hi}{95.1}
\defres{diff/c/all/sl27b/ci/lo}{92.7}
\defres{diff/c/all/sl2b/acc}{68.4}
\defres{diff/c/all/sl2b/ci/hi}{70.3}
\defres{diff/c/all/sl2b/ci/lo}{66.6}
\defres{diff/c/all/sl4b/acc}{89.1}
\defres{diff/c/all/sl4b/ci/hi}{90.8}
\defres{diff/c/all/sl4b/ci/lo}{87.4}
\defres{diff/c/all/sl9b/acc}{91.8}
\defres{diff/c/all/sl9b/ci/hi}{93.5}
\defres{diff/c/all/sl9b/ci/lo}{90.0}
\defres{diff/c/all/spread}{50.9}
\defres{diff/c/all/tasks}{200}
\defres{diff/c/all/v2/acc}{99.4}
\defres{diff/c/all/v2/ci/hi}{99.8}
\defres{diff/c/all/v2/ci/lo}{98.7}
\defres{diff/c/ask_gold/base/acc}{47.3}
\defres{diff/c/ask_gold/base/ci/hi}{54.6}
\defres{diff/c/ask_gold/base/ci/lo}{39.7}
\defres{diff/c/ask_gold/intern/acc}{59.6}
\defres{diff/c/ask_gold/intern/ci/hi}{66.8}
\defres{diff/c/ask_gold/intern/ci/lo}{51.9}
\defres{diff/c/ask_gold/jev/acc}{64.4}
\defres{diff/c/ask_gold/jev/ci/hi}{71.2}
\defres{diff/c/ask_gold/jev/ci/lo}{56.8}
\defres{diff/c/ask_gold/llm/acc}{100.0}
\defres{diff/c/ask_gold/llm/ci/hi}{100.0}
\defres{diff/c/ask_gold/llm/ci/lo}{100.0}
\defres{diff/c/ask_gold/n}{582}
\defres{diff/c/ask_gold/offshelf/max}{87.1}
\defres{diff/c/ask_gold/offshelf/max_model}{StartLux-9B}
\defres{diff/c/ask_gold/offshelf/min}{49.4}
\defres{diff/c/ask_gold/offshelf/min_model}{StartLux-0.8B}
\defres{diff/c/ask_gold/rl/acc}{100.0}
\defres{diff/c/ask_gold/rl/ci/hi}{100.0}
\defres{diff/c/ask_gold/rl/ci/lo}{100.0}
\defres{diff/c/ask_gold/sft_v1/acc}{100.0}
\defres{diff/c/ask_gold/sft_v1/ci/hi}{100.0}
\defres{diff/c/ask_gold/sft_v1/ci/lo}{100.0}
\defres{diff/c/ask_gold/sl0.8b/acc}{49.4}
\defres{diff/c/ask_gold/sl0.8b/ci/hi}{56.5}
\defres{diff/c/ask_gold/sl0.8b/ci/lo}{42.2}
\defres{diff/c/ask_gold/sl27b/acc}{63.4}
\defres{diff/c/ask_gold/sl27b/ci/hi}{70.4}
\defres{diff/c/ask_gold/sl27b/ci/lo}{55.7}
\defres{diff/c/ask_gold/sl2b/acc}{61.8}
\defres{diff/c/ask_gold/sl2b/ci/hi}{68.8}
\defres{diff/c/ask_gold/sl2b/ci/lo}{54.0}
\defres{diff/c/ask_gold/sl4b/acc}{84.1}
\defres{diff/c/ask_gold/sl4b/ci/hi}{87.7}
\defres{diff/c/ask_gold/sl4b/ci/lo}{79.9}
\defres{diff/c/ask_gold/sl9b/acc}{87.1}
\defres{diff/c/ask_gold/sl9b/ci/hi}{89.7}
\defres{diff/c/ask_gold/sl9b/ci/lo}{84.4}
\defres{diff/c/ask_gold/spread}{50.6}
\defres{diff/c/ask_gold/tasks}{100}
\defres{diff/c/ask_gold/v2/acc}{100.0}
\defres{diff/c/ask_gold/v2/ci/hi}{100.0}
\defres{diff/c/ask_gold/v2/ci/lo}{100.0}
\defres{diff/c/finish_gold/base/acc}{99.4}
\defres{diff/c/finish_gold/intern/acc}{98.5}
\defres{diff/c/finish_gold/jev/acc}{97.7}
\defres{diff/c/finish_gold/llm/acc}{100.0}
\defres{diff/c/finish_gold/n}{603}
\defres{diff/c/finish_gold/offshelf/max}{98.6}
\defres{diff/c/finish_gold/offshelf/max_model}{StartLux-27B}
\defres{diff/c/finish_gold/offshelf/min}{74.7}
\defres{diff/c/finish_gold/offshelf/min_model}{StartLux-2B}
\defres{diff/c/finish_gold/rl/acc}{99.2}
\defres{diff/c/finish_gold/sft_v1/acc}{99.2}
\defres{diff/c/finish_gold/sl0.8b/acc}{97.5}
\defres{diff/c/finish_gold/sl27b/acc}{98.6}
\defres{diff/c/finish_gold/sl2b/acc}{74.7}
\defres{diff/c/finish_gold/sl4b/acc}{97.8}
\defres{diff/c/finish_gold/sl9b/acc}{98.1}
\defres{diff/c/finish_gold/spread}{24.5}
\defres{diff/c/finish_gold/tasks}{200}
\defres{diff/c/finish_gold/v2/acc}{99.2}
\defres{diff/c/hard/base/acc}{39.9}
\defres{diff/c/hard/base/ci/hi}{45.6}
\defres{diff/c/hard/base/ci/lo}{34.5}
\defres{diff/c/hard/intern/acc}{55.7}
\defres{diff/c/hard/intern/ci/hi}{61.7}
\defres{diff/c/hard/intern/ci/lo}{49.3}
\defres{diff/c/hard/jev/acc}{69.4}
\defres{diff/c/hard/jev/ci/hi}{74.9}
\defres{diff/c/hard/jev/ci/lo}{63.5}
\defres{diff/c/hard/llm/acc}{100.0}
\defres{diff/c/hard/llm/ci/hi}{100.0}
\defres{diff/c/hard/llm/ci/lo}{100.0}
\defres{diff/c/hard/n}{957}
\defres{diff/c/hard/offshelf/max}{82.7}
\defres{diff/c/hard/offshelf/max_model}{StartLux-9B}
\defres{diff/c/hard/offshelf/min}{42.7}
\defres{diff/c/hard/offshelf/min_model}{StartLux-0.8B}
\defres{diff/c/hard/rl/acc}{98.2}
\defres{diff/c/hard/rl/ci/hi}{99.3}
\defres{diff/c/hard/rl/ci/lo}{96.8}
\defres{diff/c/hard/sft_v1/acc}{98.0}
\defres{diff/c/hard/sft_v1/ci/hi}{99.2}
\defres{diff/c/hard/sft_v1/ci/lo}{96.5}
\defres{diff/c/hard/sl0.8b/acc}{42.7}
\defres{diff/c/hard/sl0.8b/ci/hi}{47.8}
\defres{diff/c/hard/sl0.8b/ci/lo}{37.3}
\defres{diff/c/hard/sl27b/acc}{71.2}
\defres{diff/c/hard/sl27b/ci/hi}{76.6}
\defres{diff/c/hard/sl27b/ci/lo}{65.2}
\defres{diff/c/hard/sl2b/acc}{56.2}
\defres{diff/c/hard/sl2b/ci/hi}{62.2}
\defres{diff/c/hard/sl2b/ci/lo}{50.5}
\defres{diff/c/hard/sl4b/acc}{81.7}
\defres{diff/c/hard/sl4b/ci/hi}{85.7}
\defres{diff/c/hard/sl4b/ci/lo}{77.6}
\defres{diff/c/hard/sl9b/acc}{82.7}
\defres{diff/c/hard/sl9b/ci/hi}{86.3}
\defres{diff/c/hard/sl9b/ci/lo}{78.8}
\defres{diff/c/hard/spread}{55.5}
\defres{diff/c/hard/tasks}{135}
\defres{diff/c/hard/v2/acc}{98.2}
\defres{diff/c/hard/v2/ci/hi}{99.3}
\defres{diff/c/hard/v2/ci/lo}{96.9}
\defres{diff/c/llm_states/base/acc}{54.4}
\defres{diff/c/llm_states/intern/acc}{76.3}
\defres{diff/c/llm_states/jev/acc}{92.0}
\defres{diff/c/llm_states/llm/acc}{99.9}
\defres{diff/c/llm_states/n}{1{,}498}
\defres{diff/c/llm_states/offshelf/max}{92.9}
\defres{diff/c/llm_states/offshelf/max_model}{StartLux-9B}
\defres{diff/c/llm_states/offshelf/min}{52.1}
\defres{diff/c/llm_states/offshelf/min_model}{StartLux-0.8B}
\defres{diff/c/llm_states/rl/acc}{100.0}
\defres{diff/c/llm_states/sft_v1/acc}{100.0}
\defres{diff/c/llm_states/sl0.8b/acc}{52.1}
\defres{diff/c/llm_states/sl27b/acc}{92.6}
\defres{diff/c/llm_states/sl2b/acc}{73.7}
\defres{diff/c/llm_states/sl4b/acc}{89.6}
\defres{diff/c/llm_states/sl9b/acc}{92.9}
\defres{diff/c/llm_states/spread}{47.9}
\defres{diff/c/llm_states/tasks}{200}
\defres{diff/c/llm_states/v2/acc}{100.0}
\defres{diff/c/long_history/base/acc}{81.2}
\defres{diff/c/long_history/intern/acc}{93.5}
\defres{diff/c/long_history/jev/acc}{96.5}
\defres{diff/c/long_history/llm/acc}{100.0}
\defres{diff/c/long_history/n}{770}
\defres{diff/c/long_history/offshelf/max}{96.8}
\defres{diff/c/long_history/offshelf/max_model}{StartLux-27B}
\defres{diff/c/long_history/offshelf/min}{71.9}
\defres{diff/c/long_history/offshelf/min_model}{StartLux-0.8B}
\defres{diff/c/long_history/rl/acc}{97.0}
\defres{diff/c/long_history/sft_v1/acc}{97.0}
\defres{diff/c/long_history/sl0.8b/acc}{71.9}
\defres{diff/c/long_history/sl27b/acc}{96.8}
\defres{diff/c/long_history/sl2b/acc}{72.8}
\defres{diff/c/long_history/sl4b/acc}{95.1}
\defres{diff/c/long_history/sl9b/acc}{94.5}
\defres{diff/c/long_history/spread}{25.1}
\defres{diff/c/long_history/tasks}{104}
\defres{diff/c/long_history/v2/acc}{97.0}
\defres{diff/c/state_change_trap/base/acc}{91.0}
\defres{diff/c/state_change_trap/intern/acc}{89.4}
\defres{diff/c/state_change_trap/jev/acc}{100.0}
\defres{diff/c/state_change_trap/llm/acc}{99.9}
\defres{diff/c/state_change_trap/n}{1{,}339}
\defres{diff/c/state_change_trap/offshelf/max}{100.0}
\defres{diff/c/state_change_trap/offshelf/max_model}{Jev}
\defres{diff/c/state_change_trap/offshelf/min}{83.2}
\defres{diff/c/state_change_trap/offshelf/min_model}{StartLux-0.8B}
\defres{diff/c/state_change_trap/rl/acc}{100.0}
\defres{diff/c/state_change_trap/sft_v1/acc}{100.0}
\defres{diff/c/state_change_trap/sl0.8b/acc}{83.2}
\defres{diff/c/state_change_trap/sl27b/acc}{100.0}
\defres{diff/c/state_change_trap/sl2b/acc}{98.0}
\defres{diff/c/state_change_trap/sl4b/acc}{100.0}
\defres{diff/c/state_change_trap/sl9b/acc}{99.8}
\defres{diff/c/state_change_trap/spread}{16.8}
\defres{diff/c/state_change_trap/tasks}{200}
\defres{diff/c/state_change_trap/v2/acc}{99.8}
\defres{diff/ceiling/stage1_flash/fail_final_answer}{0}
\defres{diff/ceiling/stage1_flash/fail_final_answer_n}{0}
\defres{diff/ceiling/stage1_flash/fail_lookalike}{0}
\defres{diff/ceiling/stage1_flash/fail_premature}{0}
\defres{diff/ceiling/stage1_flash/failures}{1}
\defres{diff/ceiling/stage1_flash/success}{99.8}
\defres{diff/ceiling/stage1_flash/tool_acc}{99.8}
\defres{diff/ceiling/stage1_lite/fail_final_answer}{98}
\defres{diff/ceiling/stage1_lite/fail_final_answer_n}{97}
\defres{diff/ceiling/stage1_lite/fail_lookalike}{1}
\defres{diff/ceiling/stage1_lite/fail_premature}{0}
\defres{diff/ceiling/stage1_lite/failures}{99}
\defres{diff/ceiling/stage1_lite/success}{80.2}
\defres{diff/ceiling/stage1_lite/tool_acc}{99.0}
\defres{diff/ceiling/stage2_flash/fail_final_answer}{0}
\defres{diff/ceiling/stage2_flash/fail_final_answer_n}{0}
\defres{diff/ceiling/stage2_flash/fail_lookalike}{0}
\defres{diff/ceiling/stage2_flash/fail_premature}{0}
\defres{diff/ceiling/stage2_flash/failures}{3}
\defres{diff/ceiling/stage2_flash/success}{99.4}
\defres{diff/ceiling/stage2_flash/tool_acc}{99.6}
\defres{diff/e1/bfcl_arguments/base/acc}{70.5}
\defres{diff/e1/bfcl_arguments/intern/acc}{71.2}
\defres{diff/e1/bfcl_arguments/jev/acc}{89.6}
\defres{diff/e1/bfcl_arguments/llm/acc}{96.3}
\defres{diff/e1/bfcl_arguments/n}{1{,}949}
\defres{diff/e1/bfcl_arguments/rl/acc}{85.0}
\defres{diff/e1/bfcl_arguments/sft_v1/acc}{85.5}
\defres{diff/e1/bfcl_arguments/sl0.8b/acc}{67.1}
\defres{diff/e1/bfcl_arguments/sl27b/acc}{89.1}
\defres{diff/e1/bfcl_arguments/sl2b/acc}{73.1}
\defres{diff/e1/bfcl_arguments/sl4b/acc}{81.2}
\defres{diff/e1/bfcl_arguments/sl9b/acc}{81.0}
\defres{diff/e1/bfcl_arguments/spread}{22.5}
\defres{diff/e1/bfcl_irrelevance/base/acc}{70.0}
\defres{diff/e1/bfcl_irrelevance/intern/acc}{67.8}
\defres{diff/e1/bfcl_irrelevance/jev/acc}{74.1}
\defres{diff/e1/bfcl_irrelevance/llm/acc}{55.1}
\defres{diff/e1/bfcl_irrelevance/n}{370}
\defres{diff/e1/bfcl_irrelevance/rl/acc}{84.9}
\defres{diff/e1/bfcl_irrelevance/sft_v1/acc}{85.7}
\defres{diff/e1/bfcl_irrelevance/sl0.8b/acc}{69.5}
\defres{diff/e1/bfcl_irrelevance/sl27b/acc}{76.5}
\defres{diff/e1/bfcl_irrelevance/sl2b/acc}{77.8}
\defres{diff/e1/bfcl_irrelevance/sl4b/acc}{79.2}
\defres{diff/e1/bfcl_irrelevance/sl9b/acc}{81.1}
\defres{diff/e1/bfcl_irrelevance/spread}{17.0}
\defres{diff/e1/bfcl_live_arguments/base/acc}{66.5}
\defres{diff/e1/bfcl_live_arguments/intern/acc}{65.2}
\defres{diff/e1/bfcl_live_arguments/jev/acc}{89.0}
\defres{diff/e1/bfcl_live_arguments/llm/acc}{94.2}
\defres{diff/e1/bfcl_live_arguments/n}{1{,}033}
\defres{diff/e1/bfcl_live_arguments/rl/acc}{81.5}
\defres{diff/e1/bfcl_live_arguments/sft_v1/acc}{82.0}
\defres{diff/e1/bfcl_live_arguments/sl0.8b/acc}{60.6}
\defres{diff/e1/bfcl_live_arguments/sl27b/acc}{87.4}
\defres{diff/e1/bfcl_live_arguments/sl2b/acc}{68.3}
\defres{diff/e1/bfcl_live_arguments/sl4b/acc}{79.0}
\defres{diff/e1/bfcl_live_arguments/sl9b/acc}{76.6}
\defres{diff/e1/bfcl_live_arguments/spread}{28.4}
\defres{diff/e1/bfcl_multi_tool/base/acc}{95.7}
\defres{diff/e1/bfcl_multi_tool/intern/acc}{97.0}
\defres{diff/e1/bfcl_multi_tool/jev/acc}{96.8}
\defres{diff/e1/bfcl_multi_tool/llm/acc}{97.8}
\defres{diff/e1/bfcl_multi_tool/n}{372}
\defres{diff/e1/bfcl_multi_tool/rl/acc}{91.7}
\defres{diff/e1/bfcl_multi_tool/sft_v1/acc}{87.9}
\defres{diff/e1/bfcl_multi_tool/sl0.8b/acc}{97.8}
\defres{diff/e1/bfcl_multi_tool/sl27b/acc}{97.6}
\defres{diff/e1/bfcl_multi_tool/sl2b/acc}{96.2}
\defres{diff/e1/bfcl_multi_tool/sl4b/acc}{97.6}
\defres{diff/e1/bfcl_multi_tool/sl9b/acc}{97.0}
\defres{diff/e1/bfcl_multi_tool/spread}{6.2}
\defres{diff/e1/bfcl_tool_select/base/acc}{87.5}
\defres{diff/e1/bfcl_tool_select/intern/acc}{88.2}
\defres{diff/e1/bfcl_tool_select/jev/acc}{89.9}
\defres{diff/e1/bfcl_tool_select/llm/acc}{84.2}
\defres{diff/e1/bfcl_tool_select/n}{1{,}114}
\defres{diff/e1/bfcl_tool_select/rl/acc}{88.4}
\defres{diff/e1/bfcl_tool_select/sft_v1/acc}{86.9}
\defres{diff/e1/bfcl_tool_select/sl0.8b/acc}{88.2}
\defres{diff/e1/bfcl_tool_select/sl27b/acc}{90.8}
\defres{diff/e1/bfcl_tool_select/sl2b/acc}{89.9}
\defres{diff/e1/bfcl_tool_select/sl4b/acc}{91.3}
\defres{diff/e1/bfcl_tool_select/sl9b/acc}{92.2}
\defres{diff/e1/bfcl_tool_select/spread}{3.9}
\defres{diff/e1/when2call/base/acc}{53.9}
\defres{diff/e1/when2call/intern/acc}{60.1}
\defres{diff/e1/when2call/jev/acc}{75.4}
\defres{diff/e1/when2call/llm/acc}{42.1}
\defres{diff/e1/when2call/n}{928}
\defres{diff/e1/when2call/rl/acc}{54.0}
\defres{diff/e1/when2call/sft_v1/acc}{53.3}
\defres{diff/e1/when2call/sl0.8b/acc}{54.2}
\defres{diff/e1/when2call/sl27b/acc}{81.2}
\defres{diff/e1/when2call/sl2b/acc}{64.1}
\defres{diff/e1/when2call/sl4b/acc}{77.4}
\defres{diff/e1/when2call/sl9b/acc}{78.1}
\defres{diff/e1/when2call/spread}{27.3}
\defres{diff/e1/when2call_noncall/base/acc}{32.6}
\defres{diff/e1/when2call_noncall/intern/acc}{48.2}
\defres{diff/e1/when2call_noncall/jev/acc}{69.4}
\defres{diff/e1/when2call_noncall/llm/acc}{0.0}
\defres{diff/e1/when2call_noncall/n}{599}
\defres{diff/e1/when2call_noncall/rl/acc}{83.6}
\defres{diff/e1/when2call_noncall/sft_v1/acc}{82.6}
\defres{diff/e1/when2call_noncall/sl0.8b/acc}{44.9}
\defres{diff/e1/when2call_noncall/sl27b/acc}{80.8}
\defres{diff/e1/when2call_noncall/sl2b/acc}{58.3}
\defres{diff/e1/when2call_noncall/sl4b/acc}{75.8}
\defres{diff/e1/when2call_noncall/sl9b/acc}{71.8}
\defres{diff/e1/when2call_noncall/spread}{38.7}
\defres{diff/s1/flash/tp/all/intern/acc}{91.1}
\defres{diff/s1/flash/tp/all/jev/acc}{100.0}
\defres{diff/s1/flash/tp/all/llm/acc}{100.0}
\defres{diff/s1/flash/tp/all/n}{1{,}492}
\defres{diff/s1/flash/tp/copy/intern/acc}{92.2}
\defres{diff/s1/flash/tp/copy/jev/acc}{100.0}
\defres{diff/s1/flash/tp/copy/llm/acc}{100.0}
\defres{diff/s1/flash/tp/copy/n}{797}
\defres{diff/s1/flash/tp/many_candidates/intern/acc}{79.7}
\defres{diff/s1/flash/tp/many_candidates/jev/acc}{100.0}
\defres{diff/s1/flash/tp/many_candidates/llm/acc}{100.0}
\defres{diff/s1/flash/tp/many_candidates/n}{449}
\defres{diff/s1/flash/ts/all/intern/acc}{68.6}
\defres{diff/s1/flash/ts/all/jev/acc}{93.0}
\defres{diff/s1/flash/ts/all/llm/acc}{99.8}
\defres{diff/s1/flash/ts/all/n}{1{,}693}
\defres{diff/s1/flash/ts/ask_gold/intern/acc}{72.5}
\defres{diff/s1/flash/ts/ask_gold/jev/acc}{77.7}
\defres{diff/s1/flash/ts/ask_gold/llm/acc}{100.0}
\defres{diff/s1/flash/ts/ask_gold/n}{410}
\defres{diff/s1/flash_lite/tp/all/intern/acc}{81.6}
\defres{diff/s1/flash_lite/tp/all/jev/acc}{100.0}
\defres{diff/s1/flash_lite/tp/all/llm/acc}{100.0}
\defres{diff/s1/flash_lite/tp/all/n}{1{,}674}
\defres{diff/s1/flash_lite/tp/copy/intern/acc}{78.0}
\defres{diff/s1/flash_lite/tp/copy/jev/acc}{100.0}
\defres{diff/s1/flash_lite/tp/copy/llm/acc}{100.0}
\defres{diff/s1/flash_lite/tp/copy/n}{950}
\defres{diff/s1/flash_lite/tp/many_candidates/intern/acc}{61.2}
\defres{diff/s1/flash_lite/tp/many_candidates/jev/acc}{100.0}
\defres{diff/s1/flash_lite/tp/many_candidates/llm/acc}{100.0}
\defres{diff/s1/flash_lite/tp/many_candidates/n}{633}
\defres{diff/s1/flash_lite/ts/all/intern/acc}{72.6}
\defres{diff/s1/flash_lite/ts/all/jev/acc}{90.5}
\defres{diff/s1/flash_lite/ts/all/llm/acc}{98.3}
\defres{diff/s1/flash_lite/ts/all/n}{1{,}393}
\defres{diff/s1/flash_lite/ts/ask_gold/intern/acc}{67.7}
\defres{diff/s1/flash_lite/ts/ask_gold/jev/acc}{73.0}
\defres{diff/s1/flash_lite/ts/ask_gold/llm/acc}{97.6}
\defres{diff/s1/flash_lite/ts/ask_gold/n}{436}
\defres{diff/stress/grpo/success}{60.0}
\defres{diff/stress/grpo/tool_acc}{93.9}
\defres{diff/stress/grpo_i15/success}{62.5}
\defres{diff/stress/grpo_i15/tool_acc}{94.9}
\defres{diff/stress/opd/success}{65.0}
\defres{diff/stress/opd/tool_acc}{93.9}
\defres{diff/stress/opd_i12/success}{66.5}
\defres{diff/stress/opd_i12/tool_acc}{94.7}
\defres{diff/stress/refs_intern/success}{11.5}
\defres{diff/stress/refs_intern/tool_acc}{61.1}
\defres{diff/stress/refs_jev/success}{49.0}
\defres{diff/stress/refs_jev/tool_acc}{69.1}
\defres{diff/stress/sft_v2/success}{71.5}
\defres{diff/stress/sft_v2/tool_acc}{95.4}
\defres{diff/t2/tp/all/base/acc}{71.3}
\defres{diff/t2/tp/all/intern/acc}{77.2}
\defres{diff/t2/tp/all/jev/acc}{90.0}
\defres{diff/t2/tp/all/n}{4{,}023}
\defres{diff/t2/tp/all/rl/acc}{85.9}
\defres{diff/t2/tp/many_candidates/base/acc}{66.6}
\defres{diff/t2/tp/many_candidates/intern/acc}{74.3}
\defres{diff/t2/tp/many_candidates/jev/acc}{84.0}
\defres{diff/t2/tp/many_candidates/n}{2{,}635}
\defres{diff/t2/tp/many_candidates/rl/acc}{76.9}
\defres{diff/t2/ts/all/base/acc}{41.1}
\defres{diff/t2/ts/all/intern/acc}{42.1}
\defres{diff/t2/ts/all/jev/acc}{59.9}
\defres{diff/t2/ts/all/n}{19{,}934}
\defres{diff/t2/ts/all/rl/acc}{53.7}
\defres{diff/t2/ts/non_majority/base/acc}{37.9}
\defres{diff/t2/ts/non_majority/intern/acc}{59.9}
\defres{diff/t2/ts/non_majority/jev/acc}{51.0}
\defres{diff/t2/ts/non_majority/n}{8{,}283}
\defres{diff/t2/ts/non_majority/rl/acc}{50.7}
\makeatother


==> generated/drift.tex <==
\makeatletter
\providecommand{\res}[1]{\ifcsname jevres@#1\endcsname\csname jevres@#1\endcsname\else\tbd\fi}
\providecommand{\defres}[2]{\expandafter\def\csname jevres@#1\endcsname{#2}}
\defres{drift/base/acc/after_off_plan}{0.0}
\defres{drift/base/acc/after_off_plan/n}{137}
\defres{drift/base/acc/all}{30.9}
\defres{drift/base/acc/all/n}{324}
\defres{drift/base/acc/executed_all}{30.9}
\defres{drift/base/acc/executed_all/n}{324}
\defres{drift/base/acc/in_c}{48.6}
\defres{drift/base/acc/in_c/n}{144}
\defres{drift/base/acc/in_c_after_off_plan}{0.0}
\defres{drift/base/acc/in_c_after_off_plan/n}{1}
\defres{drift/base/acc/in_c_on_plan}{49.0}
\defres{drift/base/acc/in_c_on_plan/n}{143}
\defres{drift/base/acc/novel}{16.7}
\defres{drift/base/acc/novel/n}{180}
\defres{drift/base/acc/novel_after_off_plan}{0.0}
\defres{drift/base/acc/novel_after_off_plan/n}{136}
\defres{drift/base/acc/novel_on_plan}{68.2}
\defres{drift/base/acc/novel_on_plan/n}{44}
\defres{drift/base/acc/on_plan}{53.5}
\defres{drift/base/acc/on_plan/n}{187}
\defres{drift/base/ask/acc}{56.2}
\defres{drift/base/ask/acted}{3.1}
\defres{drift/base/ask/acted/n}{2}
\defres{drift/base/ask/acted_of_wrong}{7.1}
\defres{drift/base/ask/n}{64}
\defres{drift/base/askearly/share}{13.0}
\defres{drift/base/askearly/tasks}{13}
\defres{drift/base/c/acc}{50.1}
\defres{drift/base/c/ask_acc}{47.3}
\defres{drift/base/c/mustask_acc}{24.0}
\defres{drift/base/conf/right}{68.8}
\defres{drift/base/conf/wrong}{52.0}
\defres{drift/base/faith/agree}{97.2}
\defres{drift/base/faith/live}{48.6}
\defres{drift/base/faith/lr_ow}{1}
\defres{drift/base/faith/lw_or}{0}
\defres{drift/base/faith/n}{144}
\defres{drift/base/faith/offline}{47.9}
\defres{drift/base/faith/sign_p}{1.000}
\defres{drift/base/first/conseq/recoverable/n}{14}
\defres{drift/base/first/conseq/recoverable/recovered}{0.0}
\defres{drift/base/first/conseq/recoverable/share}{16.1}
\defres{drift/base/first/conseq/recoverable/tasks}{14.0}
\defres{drift/base/first/conseq/write/n}{73}
\defres{drift/base/first/conseq/write/recovered}{0.0}
\defres{drift/base/first/conseq/write/share}{83.9}
\defres{drift/base/first/conseq/write/tasks}{73.0}
\defres{drift/base/first/failed}{87}
\defres{drift/base/first/failed_with_wrong}{100.0}
\defres{drift/base/first/in_c}{73.0}
\defres{drift/base/first/in_c/n}{73}
\defres{drift/base/first/inc_offline_right}{0.0}
\defres{drift/base/first/inc_offline_right/n}{0}
\defres{drift/base/first/inc_same_answer/n}{70}
\defres{drift/base/first/irreversible}{73.0}
\defres{drift/base/first/irreversible/n}{73}
\defres{drift/base/first/irreversible_of_failed}{83.9}
\defres{drift/base/first/none}{13.0}
\defres{drift/base/first/none/n}{13}
\defres{drift/base/first/novel}{14.0}
\defres{drift/base/first/novel/n}{14}
\defres{drift/base/first/recovered}{0.0}
\defres{drift/base/first/recovered/n}{0}
\defres{drift/base/first/step_le1}{87.4}
\defres{drift/base/first/step_median}{1}
\defres{drift/base/first/top_type}{wrong core tool}
\defres{drift/base/first/top_type/share}{83.9}
\defres{drift/base/first/type/act_before_ask/n}{2}
\defres{drift/base/first/type/act_before_ask/share}{2.3}
\defres{drift/base/first/type/act_before_ask/tasks}{2.0}
\defres{drift/base/first/type/lookalike_gold/n}{5}
\defres{drift/base/first/type/lookalike_gold/share}{5.7}
\defres{drift/base/first/type/lookalike_gold/tasks}{5.0}
\defres{drift/base/first/type/lookalike_other/n}{2}
\defres{drift/base/first/type/lookalike_other/share}{2.3}
\defres{drift/base/first/type/lookalike_other/tasks}{2.0}
\defres{drift/base/first/type/unneeded_question/n}{5}
\defres{drift/base/first/type/unneeded_question/share}{5.7}
\defres{drift/base/first/type/unneeded_question/tasks}{5.0}
\defres{drift/base/first/type/wrong_core_tool/n}{73}
\defres{drift/base/first/type/wrong_core_tool/share}{83.9}
\defres{drift/base/first/type/wrong_core_tool/tasks}{73.0}
\defres{drift/base/first/with_wrong/n}{87}
\defres{drift/base/gate/05/failed_first_below}{39.1}
\defres{drift/base/gate/05/right_below}{15.0}
\defres{drift/base/gate/05/wrong_below}{47.8}
\defres{drift/base/gate/09/failed_first_below}{100.0}
\defres{drift/base/gate/09/right_below}{100.0}
\defres{drift/base/gate/09/wrong_below}{100.0}
\defres{drift/base/gate/failed_first_below}{100.0}
\defres{drift/base/gate/jev/failed_first_below}{100.0}
\defres{drift/base/gate/jev/right_below}{100.0}
\defres{drift/base/gate/jev/wrong_below}{100.0}
\defres{drift/base/gate/n_wrong}{224}
\defres{drift/base/gate/right_below}{100.0}
\defres{drift/base/gate/source}{jev}
\defres{drift/base/gate/tau}{1.00}
\defres{drift/base/gate/wrong_below}{100.0}
\defres{drift/base/live/n}{100}
\defres{drift/base/live/success}{13.0}
\defres{drift/base/loss/compounding}{14.0}
\defres{drift/base/loss/irreversible}{73.0}
\defres{drift/base/loss/no_wrong_choice}{0.0}
\defres{drift/base/loss/total}{87.0}
\defres{drift/base/mustask/acc}{100.0}
\defres{drift/base/mustask/acted}{0.0}
\defres{drift/base/mustask/acted/n}{0}
\defres{drift/base/mustask/n}{12}
\defres{drift/base/mustask/step_median}{0}
\defres{drift/base/mustask/tasks}{12}
\defres{drift/base/states/inc_share}{44.4}
\defres{drift/base/states/n}{324}
\defres{drift/base/states/novel_offplan_share}{42.0}
\defres{drift/base/states/novel_onplan_share}{13.6}
\defres{drift/base/states/novel_share}{55.6}
\defres{drift/base/states/offplan_share}{42.3}
\defres{drift/c/ask/occurrences}{582}
\defres{drift/c/ask/share}{11.0}
\defres{drift/c/ask/tasks}{100}
\defres{drift/c/mustask/occurrences}{267}
\defres{drift/c/mustask/share}{5.0}
\defres{drift/c/mustask/tasks}{100}
\defres{drift/c/occurrences}{5{,}314}
\defres{drift/c/questions}{3{,}939}
\defres{drift/e12/acc/after_off_plan/n}{0}
\defres{drift/e12/acc/all}{100.0}
\defres{drift/e12/acc/all/n}{1{,}500}
\defres{drift/e12/acc/executed_all}{100.0}
\defres{drift/e12/acc/executed_all/n}{1{,}500}
\defres{drift/e12/acc/in_c}{100.0}
\defres{drift/e12/acc/in_c/n}{735}
\defres{drift/e12/acc/in_c_after_off_plan/n}{0}
\defres{drift/e12/acc/in_c_on_plan}{100.0}
\defres{drift/e12/acc/in_c_on_plan/n}{735}
\defres{drift/e12/acc/novel}{100.0}
\defres{drift/e12/acc/novel/n}{765}
\defres{drift/e12/acc/novel_after_off_plan/n}{0}
\defres{drift/e12/acc/novel_on_plan}{100.0}
\defres{drift/e12/acc/novel_on_plan/n}{765}
\defres{drift/e12/acc/on_plan}{100.0}
\defres{drift/e12/acc/on_plan/n}{1{,}500}
\defres{drift/e12/ask/acc}{100.0}
\defres{drift/e12/ask/acted}{0.0}
\defres{drift/e12/ask/acted/n}{0}
\defres{drift/e12/ask/n}{100}
\defres{drift/e12/askearly/share}{0.0}
\defres{drift/e12/askearly/tasks}{0}
\defres{drift/e12/c/acc}{99.1}
\defres{drift/e12/c/ask_acc}{99.9}
\defres{drift/e12/c/mustask_acc}{99.7}
\defres{drift/e12/conf/right}{97.7}
\defres{drift/e12/faith/agree}{100.0}
\defres{drift/e12/faith/live}{100.0}
\defres{drift/e12/faith/lr_ow}{0}
\defres{drift/e12/faith/lw_or}{0}
\defres{drift/e12/faith/n}{735}
\defres{drift/e12/faith/offline}{100.0}
\defres{drift/e12/first/failed}{0}
\defres{drift/e12/first/in_c}{0.0}
\defres{drift/e12/first/in_c/n}{0}
\defres{drift/e12/first/inc_offline_right/n}{0}
\defres{drift/e12/first/inc_same_answer/n}{0}
\defres{drift/e12/first/irreversible}{0.0}
\defres{drift/e12/first/irreversible/n}{0}
\defres{drift/e12/first/none}{100.0}
\defres{drift/e12/first/none/n}{200}
\defres{drift/e12/first/novel}{0.0}
\defres{drift/e12/first/novel/n}{0}
\defres{drift/e12/first/recovered/n}{0}
\defres{drift/e12/first/with_wrong/n}{0}
\defres{drift/e12/gate/05/right_below}{0.0}
\defres{drift/e12/gate/09/right_below}{6.6}
\defres{drift/e12/gate/jev/right_below}{100.0}
\defres{drift/e12/gate/n_wrong}{0}
\defres{drift/e12/gate/right_below}{100.0}
\defres{drift/e12/gate/source}{jev}
\defres{drift/e12/gate/tau}{1.00}
\defres{drift/e12/live/n}{200}
\defres{drift/e12/live/success}{100.0}
\defres{drift/e12/loss/compounding}{0.0}
\defres{drift/e12/loss/irreversible}{0.0}
\defres{drift/e12/loss/no_wrong_choice}{0.0}
\defres{drift/e12/loss/total}{0.0}
\defres{drift/e12/mustask/acc}{100.0}
\defres{drift/e12/mustask/acted}{0.0}
\defres{drift/e12/mustask/acted/n}{0}
\defres{drift/e12/mustask/n}{50}
\defres{drift/e12/mustask/step_median}{1}
\defres{drift/e12/mustask/tasks}{50}
\defres{drift/e12/states/inc_share}{49.0}
\defres{drift/e12/states/n}{1{,}500}
\defres{drift/e12/states/novel_offplan_share}{0.0}
\defres{drift/e12/states/novel_onplan_share}{51.0}
\defres{drift/e12/states/novel_share}{51.0}
\defres{drift/e12/states/offplan_share}{0.0}
\defres{drift/e12c/acc/after_off_plan/n}{0}
\defres{drift/e12c/acc/all}{100.0}
\defres{drift/e12c/acc/all/n}{1{,}500}
\defres{drift/e12c/acc/executed_all}{100.0}
\defres{drift/e12c/acc/executed_all/n}{1{,}500}
\defres{drift/e12c/acc/in_c}{100.0}
\defres{drift/e12c/acc/in_c/n}{722}
\defres{drift/e12c/acc/in_c_after_off_plan/n}{0}
\defres{drift/e12c/acc/in_c_on_plan}{100.0}
\defres{drift/e12c/acc/in_c_on_plan/n}{722}
\defres{drift/e12c/acc/novel}{100.0}
\defres{drift/e12c/acc/novel/n}{778}
\defres{drift/e12c/acc/novel_after_off_plan/n}{0}
\defres{drift/e12c/acc/novel_on_plan}{100.0}
\defres{drift/e12c/acc/novel_on_plan/n}{778}
\defres{drift/e12c/acc/on_plan}{100.0}
\defres{drift/e12c/acc/on_plan/n}{1{,}500}
\defres{drift/e12c/ask/acc}{100.0}
\defres{drift/e12c/ask/acted}{0.0}
\defres{drift/e12c/ask/acted/n}{0}
\defres{drift/e12c/ask/n}{100}
\defres{drift/e12c/askearly/share}{0.0}
\defres{drift/e12c/askearly/tasks}{0}
\defres{drift/e12c/c/acc}{99.6}
\defres{drift/e12c/c/ask_acc}{100.0}
\defres{drift/e12c/c/mustask_acc}{100.0}
\defres{drift/e12c/conf/right}{95.9}
\defres{drift/e12c/faith/agree}{100.0}
\defres{drift/e12c/faith/live}{100.0}
\defres{drift/e12c/faith/lr_ow}{0}
\defres{drift/e12c/faith/lw_or}{0}
\defres{drift/e12c/faith/n}{722}
\defres{drift/e12c/faith/offline}{100.0}
\defres{drift/e12c/first/failed}{0}
\defres{drift/e12c/first/in_c}{0.0}
\defres{drift/e12c/first/in_c/n}{0}
\defres{drift/e12c/first/inc_offline_right/n}{0}
\defres{drift/e12c/first/inc_same_answer/n}{0}
\defres{drift/e12c/first/irreversible}{0.0}
\defres{drift/e12c/first/irreversible/n}{0}
\defres{drift/e12c/first/none}{100.0}
\defres{drift/e12c/first/none/n}{200}
\defres{drift/e12c/first/novel}{0.0}
\defres{drift/e12c/first/novel/n}{0}
\defres{drift/e12c/first/recovered/n}{0}
\defres{drift/e12c/first/with_wrong/n}{0}
\defres{drift/e12c/gate/05/right_below}{0.0}
\defres{drift/e12c/gate/09/right_below}{9.1}
\defres{drift/e12c/gate/jev/right_below}{100.0}
\defres{drift/e12c/gate/n_wrong}{0}
\defres{drift/e12c/gate/right_below}{100.0}
\defres{drift/e12c/gate/source}{jev}
\defres{drift/e12c/gate/tau}{1.00}
\defres{drift/e12c/live/n}{200}
\defres{drift/e12c/live/success}{100.0}
\defres{drift/e12c/loss/compounding}{0.0}
\defres{drift/e12c/loss/irreversible}{0.0}
\defres{drift/e12c/loss/no_wrong_choice}{0.0}
\defres{drift/e12c/loss/total}{0.0}
\defres{drift/e12c/mustask/acc}{100.0}
\defres{drift/e12c/mustask/acted}{0.0}
\defres{drift/e12c/mustask/acted/n}{0}
\defres{drift/e12c/mustask/n}{50}
\defres{drift/e12c/mustask/step_median}{1}
\defres{drift/e12c/mustask/tasks}{50}
\defres{drift/e12c/states/inc_share}{48.1}
\defres{drift/e12c/states/n}{1{,}500}
\defres{drift/e12c/states/novel_offplan_share}{0.0}
\defres{drift/e12c/states/novel_onplan_share}{51.9}
\defres{drift/e12c/states/novel_share}{51.9}
\defres{drift/e12c/states/offplan_share}{0.0}
\defres{drift/e14a/acc/after_off_plan/n}{0}
\defres{drift/e14a/acc/all}{100.0}
\defres{drift/e14a/acc/all/n}{1{,}500}
\defres{drift/e14a/acc/executed_all}{100.0}
\defres{drift/e14a/acc/executed_all/n}{1{,}500}
\defres{drift/e14a/acc/in_c}{100.0}
\defres{drift/e14a/acc/in_c/n}{715}
\defres{drift/e14a/acc/in_c_after_off_plan/n}{0}
\defres{drift/e14a/acc/in_c_on_plan}{100.0}
\defres{drift/e14a/acc/in_c_on_plan/n}{715}
\defres{drift/e14a/acc/novel}{100.0}
\defres{drift/e14a/acc/novel/n}{785}
\defres{drift/e14a/acc/novel_after_off_plan/n}{0}
\defres{drift/e14a/acc/novel_on_plan}{100.0}
\defres{drift/e14a/acc/novel_on_plan/n}{785}
\defres{drift/e14a/acc/on_plan}{100.0}
\defres{drift/e14a/acc/on_plan/n}{1{,}500}
\defres{drift/e14a/ask/acc}{100.0}
\defres{drift/e14a/ask/acted}{0.0}
\defres{drift/e14a/ask/acted/n}{0}
\defres{drift/e14a/ask/n}{100}
\defres{drift/e14a/askearly/share}{0.0}
\defres{drift/e14a/askearly/tasks}{0}
\defres{drift/e14a/c/acc}{99.2}
\defres{drift/e14a/c/ask_acc}{100.0}
\defres{drift/e14a/c/mustask_acc}{100.0}
\defres{drift/e14a/conf/right}{100.0}
\defres{drift/e14a/faith/agree}{100.0}
\defres{drift/e14a/faith/live}{100.0}
\defres{drift/e14a/faith/lr_ow}{0}
\defres{drift/e14a/faith/lw_or}{0}
\defres{drift/e14a/faith/n}{715}
\defres{drift/e14a/faith/offline}{100.0}
\defres{drift/e14a/first/failed}{0}
\defres{drift/e14a/first/in_c}{0.0}
\defres{drift/e14a/first/in_c/n}{0}
\defres{drift/e14a/first/inc_offline_right/n}{0}
\defres{drift/e14a/first/inc_same_answer/n}{0}
\defres{drift/e14a/first/irreversible}{0.0}
\defres{drift/e14a/first/irreversible/n}{0}
\defres{drift/e14a/first/none}{100.0}
\defres{drift/e14a/first/none/n}{200}
\defres{drift/e14a/first/novel}{0.0}
\defres{drift/e14a/first/novel/n}{0}
\defres{drift/e14a/first/recovered/n}{0}
\defres{drift/e14a/first/with_wrong/n}{0}
\defres{drift/e14a/gate/05/right_below}{0.0}
\defres{drift/e14a/gate/09/right_below}{0.0}
\defres{drift/e14a/gate/jev/right_below}{45.5}
\defres{drift/e14a/gate/n_wrong}{0}
\defres{drift/e14a/gate/own/right_below}{16.8}
\defres{drift/e14a/gate/right_below}{16.8}
\defres{drift/e14a/gate/source}{own}
\defres{drift/e14a/gate/tau}{1.00}
\defres{drift/e14a/live/n}{200}
\defres{drift/e14a/live/success}{100.0}
\defres{drift/e14a/loss/compounding}{0.0}
\defres{drift/e14a/loss/irreversible}{0.0}
\defres{drift/e14a/loss/no_wrong_choice}{0.0}
\defres{drift/e14a/loss/total}{0.0}
\defres{drift/e14a/mustask/acc}{100.0}
\defres{drift/e14a/mustask/acted}{0.0}
\defres{drift/e14a/mustask/acted/n}{0}
\defres{drift/e14a/mustask/n}{50}
\defres{drift/e14a/mustask/step_median}{1}
\defres{drift/e14a/mustask/tasks}{50}
\defres{drift/e14a/states/inc_share}{47.7}
\defres{drift/e14a/states/n}{1{,}500}
\defres{drift/e14a/states/novel_offplan_share}{0.0}
\defres{drift/e14a/states/novel_onplan_share}{52.3}
\defres{drift/e14a/states/novel_share}{52.3}
\defres{drift/e14a/states/offplan_share}{0.0}
\defres{drift/e14g/acc/after_off_plan/n}{0}
\defres{drift/e14g/acc/all}{11.1}
\defres{drift/e14g/acc/all/n}{225}
\defres{drift/e14g/acc/executed_all}{11.1}
\defres{drift/e14g/acc/executed_all/n}{225}
\defres{drift/e14g/acc/in_c}{11.5}
\defres{drift/e14g/acc/in_c/n}{217}
\defres{drift/e14g/acc/in_c_after_off_plan/n}{0}
\defres{drift/e14g/acc/in_c_on_plan}{11.5}
\defres{drift/e14g/acc/in_c_on_plan/n}{217}
\defres{drift/e14g/acc/novel}{0.0}
\defres{drift/e14g/acc/novel/n}{8}
\defres{drift/e14g/acc/novel_after_off_plan/n}{0}
\defres{drift/e14g/acc/novel_on_plan}{0.0}
\defres{drift/e14g/acc/novel_on_plan/n}{8}
\defres{drift/e14g/acc/on_plan}{11.1}
\defres{drift/e14g/acc/on_plan/n}{225}
\defres{drift/e14g/ask/acc}{33.3}
\defres{drift/e14g/ask/acted}{66.7}
\defres{drift/e14g/ask/acted/n}{50}
\defres{drift/e14g/ask/acted_of_wrong}{100.0}
\defres{drift/e14g/ask/n}{75}
\defres{drift/e14g/askearly/share}{0.0}
\defres{drift/e14g/askearly/tasks}{0}
\defres{drift/e14g/c/acc}{23.9}
\defres{drift/e14g/c/ask_acc}{25.0}
\defres{drift/e14g/c/mustask_acc}{25.0}
\defres{drift/e14g/conf/right}{57.7}
\defres{drift/e14g/conf/wrong}{77.7}
\defres{drift/e14g/faith/agree}{100.0}
\defres{drift/e14g/faith/live}{11.5}
\defres{drift/e14g/faith/lr_ow}{0}
\defres{drift/e14g/faith/lw_or}{0}
\defres{drift/e14g/faith/n}{217}
\defres{drift/e14g/faith/offline}{11.5}
\defres{drift/e14g/first/conseq/write/n}{200}
\defres{drift/e14g/first/conseq/write/recovered}{0.0}
\defres{drift/e14g/first/conseq/write/share}{100.0}
\defres{drift/e14g/first/conseq/write/tasks}{100.0}
\defres{drift/e14g/first/failed}{200}
\defres{drift/e14g/first/failed_with_wrong}{100.0}
\defres{drift/e14g/first/in_c}{96.0}
\defres{drift/e14g/first/in_c/n}{192}
\defres{drift/e14g/first/inc_offline_right}{0.0}
\defres{drift/e14g/first/inc_offline_right/n}{0}
\defres{drift/e14g/first/inc_same_answer/n}{192}
\defres{drift/e14g/first/irreversible}{100.0}
\defres{drift/e14g/first/irreversible/n}{200}
\defres{drift/e14g/first/irreversible_of_failed}{100.0}
\defres{drift/e14g/first/none}{0.0}
\defres{drift/e14g/first/none/n}{0}
\defres{drift/e14g/first/novel}{4.0}
\defres{drift/e14g/first/novel/n}{8}
\defres{drift/e14g/first/recovered}{0.0}
\defres{drift/e14g/first/recovered/n}{0}
\defres{drift/e14g/first/step_le1}{100.0}
\defres{drift/e14g/first/step_median}{0}
\defres{drift/e14g/first/top_type}{wrong core tool}
\defres{drift/e14g/first/top_type/share}{62.5}
\defres{drift/e14g/first/type/act_before_ask/n}{75}
\defres{drift/e14g/first/type/act_before_ask/share}{37.5}
\defres{drift/e14g/first/type/act_before_ask/tasks}{37.5}
\defres{drift/e14g/first/type/wrong_core_tool/n}{125}
\defres{drift/e14g/first/type/wrong_core_tool/share}{62.5}
\defres{drift/e14g/first/type/wrong_core_tool/tasks}{62.5}
\defres{drift/e14g/first/with_wrong/n}{200}
\defres{drift/e14g/gate/05/failed_first_below}{5.0}
\defres{drift/e14g/gate/05/right_below}{0.0}
\defres{drift/e14g/gate/05/wrong_below}{5.0}
\defres{drift/e14g/gate/09/failed_first_below}{63.0}
\defres{drift/e14g/gate/09/right_below}{100.0}
\defres{drift/e14g/gate/09/wrong_below}{63.0}
\defres{drift/e14g/gate/failed_first_below}{100.0}
\defres{drift/e14g/gate/jev/failed_first_below}{100.0}
\defres{drift/e14g/gate/jev/right_below}{100.0}
\defres{drift/e14g/gate/jev/wrong_below}{100.0}
\defres{drift/e14g/gate/n_wrong}{200}
\defres{drift/e14g/gate/own/failed_first_below}{100.0}
\defres{drift/e14g/gate/own/right_below}{100.0}
\defres{drift/e14g/gate/own/wrong_below}{100.0}
\defres{drift/e14g/gate/right_below}{100.0}
\defres{drift/e14g/gate/source}{own}
\defres{drift/e14g/gate/tau}{$\infty$}
\defres{drift/e14g/gate/wrong_below}{100.0}
\defres{drift/e14g/live/n}{200}
\defres{drift/e14g/live/success}{0.0}
\defres{drift/e14g/loss/compounding}{0.0}
\defres{drift/e14g/loss/irreversible}{100.0}
\defres{drift/e14g/loss/no_wrong_choice}{0.0}
\defres{drift/e14g/loss/total}{100.0}
\defres{drift/e14g/mustask/acc}{100.0}
\defres{drift/e14g/mustask/acted}{0.0}
\defres{drift/e14g/mustask/acted/n}{0}
\defres{drift/e14g/mustask/n}{25}
\defres{drift/e14g/mustask/step_median}{0}
\defres{drift/e14g/mustask/tasks}{25}
\defres{drift/e14g/states/inc_share}{96.4}
\defres{drift/e14g/states/n}{225}
\defres{drift/e14g/states/novel_offplan_share}{0.0}
\defres{drift/e14g/states/novel_onplan_share}{3.6}
\defres{drift/e14g/states/novel_share}{3.6}
\defres{drift/e14g/states/offplan_share}{0.0}
\defres{drift/intern/acc/after_off_plan}{43.9}
\defres{drift/intern/acc/after_off_plan/n}{264}
\defres{drift/intern/acc/all}{65.7}
\defres{drift/intern/acc/all/n}{925}
\defres{drift/intern/acc/executed_all}{65.7}
\defres{drift/intern/acc/executed_all/n}{925}
\defres{drift/intern/acc/in_c}{65.7}
\defres{drift/intern/acc/in_c/n}{925}
\defres{drift/intern/acc/in_c_after_off_plan}{43.9}
\defres{drift/intern/acc/in_c_after_off_plan/n}{264}
\defres{drift/intern/acc/in_c_on_plan}{74.4}
\defres{drift/intern/acc/in_c_on_plan/n}{661}
\defres{drift/intern/acc/novel/n}{0}
\defres{drift/intern/acc/novel_after_off_plan/n}{0}
\defres{drift/intern/acc/novel_on_plan/n}{0}
\defres{drift/intern/acc/on_plan}{74.4}
\defres{drift/intern/acc/on_plan/n}{661}
\defres{drift/intern/ask/acc}{65.0}
\defres{drift/intern/ask/acted}{29.4}
\defres{drift/intern/ask/acted/n}{53}
\defres{drift/intern/ask/acted_of_wrong}{84.1}
\defres{drift/intern/ask/n}{180}
\defres{drift/intern/askearly/share}{5.0}
\defres{drift/intern/askearly/tasks}{10}
\defres{drift/intern/c/acc}{75.2}
\defres{drift/intern/c/ask_acc}{59.6}
\defres{drift/intern/c/mustask_acc}{25.0}
\defres{drift/intern/conf/right}{80.6}
\defres{drift/intern/conf/wrong}{70.4}
\defres{drift/intern/faith/agree}{100.0}
\defres{drift/intern/faith/live}{65.7}
\defres{drift/intern/faith/lr_ow}{0}
\defres{drift/intern/faith/lw_or}{0}
\defres{drift/intern/faith/n}{925}
\defres{drift/intern/faith/offline}{65.7}
\defres{drift/intern/first/conseq/recoverable/n}{50}
\defres{drift/intern/first/conseq/recoverable/recovered}{44.0}
\defres{drift/intern/first/conseq/recoverable/share}{29.6}
\defres{drift/intern/first/conseq/recoverable/tasks}{25.0}
\defres{drift/intern/first/conseq/write/n}{119}
\defres{drift/intern/first/conseq/write/recovered}{0.0}
\defres{drift/intern/first/conseq/write/share}{70.4}
\defres{drift/intern/first/conseq/write/tasks}{59.5}
\defres{drift/intern/first/failed}{147}
\defres{drift/intern/first/failed_with_wrong}{100.0}
\defres{drift/intern/first/in_c}{84.5}
\defres{drift/intern/first/in_c/n}{169}
\defres{drift/intern/first/inc_offline_right}{0.0}
\defres{drift/intern/first/inc_offline_right/n}{0}
\defres{drift/intern/first/inc_same_answer/n}{169}
\defres{drift/intern/first/irreversible}{59.5}
\defres{drift/intern/first/irreversible/n}{119}
\defres{drift/intern/first/irreversible_of_failed}{81.0}
\defres{drift/intern/first/none}{15.5}
\defres{drift/intern/first/none/n}{31}
\defres{drift/intern/first/novel}{0.0}
\defres{drift/intern/first/novel/n}{0}
\defres{drift/intern/first/recovered}{13.0}
\defres{drift/intern/first/recovered/n}{22}
\defres{drift/intern/first/step_le1}{51.5}
\defres{drift/intern/first/step_median}{1}
\defres{drift/intern/first/top_type}{wrong core tool}
\defres{drift/intern/first/top_type/share}{49.7}
\defres{drift/intern/first/type/act_before_ask/n}{55}
\defres{drift/intern/first/type/act_before_ask/share}{32.5}
\defres{drift/intern/first/type/act_before_ask/tasks}{27.5}
\defres{drift/intern/first/type/lookalike_gold/n}{20}
\defres{drift/intern/first/type/lookalike_gold/share}{11.8}
\defres{drift/intern/first/type/lookalike_gold/tasks}{10.0}
\defres{drift/intern/first/type/lookalike_other/n}{2}
\defres{drift/intern/first/type/lookalike_other/share}{1.2}
\defres{drift/intern/first/type/lookalike_other/tasks}{1.0}
\defres{drift/intern/first/type/unneeded_question/n}{8}
\defres{drift/intern/first/type/unneeded_question/share}{4.7}
\defres{drift/intern/first/type/unneeded_question/tasks}{4.0}
\defres{drift/intern/first/type/wrong_core_tool/n}{84}
\defres{drift/intern/first/type/wrong_core_tool/share}{49.7}
\defres{drift/intern/first/type/wrong_core_tool/tasks}{42.0}
\defres{drift/intern/first/with_wrong/n}{169}
\defres{drift/intern/gate/05/failed_first_below}{3.4}
\defres{drift/intern/gate/05/right_below}{1.8}
\defres{drift/intern/gate/05/wrong_below}{9.5}
\defres{drift/intern/gate/09/failed_first_below}{66.7}
\defres{drift/intern/gate/09/right_below}{60.9}
\defres{drift/intern/gate/09/wrong_below}{82.0}
\defres{drift/intern/gate/failed_first_below}{100.0}
\defres{drift/intern/gate/jev/failed_first_below}{100.0}
\defres{drift/intern/gate/jev/right_below}{100.0}
\defres{drift/intern/gate/jev/wrong_below}{100.0}
\defres{drift/intern/gate/n_wrong}{317}
\defres{drift/intern/gate/own/failed_first_below}{100.0}
\defres{drift/intern/gate/own/right_below}{100.0}
\defres{drift/intern/gate/own/wrong_below}{100.0}
\defres{drift/intern/gate/right_below}{100.0}
\defres{drift/intern/gate/source}{own}
\defres{drift/intern/gate/tau}{$\infty$}
\defres{drift/intern/gate/wrong_below}{100.0}
\defres{drift/intern/live/n}{200}
\defres{drift/intern/live/success}{26.5}
\defres{drift/intern/loss/compounding}{14.0}
\defres{drift/intern/loss/irreversible}{59.5}
\defres{drift/intern/loss/no_wrong_choice}{0.0}
\defres{drift/intern/loss/total}{73.5}
\defres{drift/intern/mustask/acc}{31.6}
\defres{drift/intern/mustask/acted}{65.8}
\defres{drift/intern/mustask/acted/n}{52}
\defres{drift/intern/mustask/n}{79}
\defres{drift/intern/mustask/step_median}{2}
\defres{drift/intern/mustask/tasks}{78}
\defres{drift/intern/states/inc_share}{100.0}
\defres{drift/intern/states/n}{925}
\defres{drift/intern/states/novel_offplan_share}{0.0}
\defres{drift/intern/states/novel_onplan_share}{0.0}
\defres{drift/intern/states/novel_share}{0.0}
\defres{drift/intern/states/offplan_share}{28.5}
\defres{drift/jev/acc/after_off_plan}{82.0}
\defres{drift/jev/acc/after_off_plan/n}{122}
\defres{drift/jev/acc/all}{95.1}
\defres{drift/jev/acc/all/n}{1{,}391}
\defres{drift/jev/acc/executed_all}{95.1}
\defres{drift/jev/acc/executed_all/n}{1{,}391}
\defres{drift/jev/acc/in_c}{95.1}
\defres{drift/jev/acc/in_c/n}{1{,}391}
\defres{drift/jev/acc/in_c_after_off_plan}{82.0}
\defres{drift/jev/acc/in_c_after_off_plan/n}{122}
\defres{drift/jev/acc/in_c_on_plan}{96.4}
\defres{drift/jev/acc/in_c_on_plan/n}{1{,}269}
\defres{drift/jev/acc/novel/n}{0}
\defres{drift/jev/acc/novel_after_off_plan/n}{0}
\defres{drift/jev/acc/novel_on_plan/n}{0}
\defres{drift/jev/acc/on_plan}{96.4}
\defres{drift/jev/acc/on_plan/n}{1{,}269}
\defres{drift/jev/ask/acc}{90.3}
\defres{drift/jev/ask/acted}{9.7}
\defres{drift/jev/ask/acted/n}{9}
\defres{drift/jev/ask/acted_of_wrong}{100.0}
\defres{drift/jev/ask/n}{93}
\defres{drift/jev/askearly/share}{12.5}
\defres{drift/jev/askearly/tasks}{25}
\defres{drift/jev/c/acc}{91.5}
\defres{drift/jev/c/ask_acc}{64.4}
\defres{drift/jev/c/mustask_acc}{27.0}
\defres{drift/jev/conf/right}{93.4}
\defres{drift/jev/conf/wrong}{63.8}
\defres{drift/jev/faith/agree}{99.3}
\defres{drift/jev/faith/live}{95.1}
\defres{drift/jev/faith/lr_ow}{4}
\defres{drift/jev/faith/lw_or}{1}
\defres{drift/jev/faith/n}{1{,}391}
\defres{drift/jev/faith/offline}{94.9}
\defres{drift/jev/faith/sign_p}{0.375}
\defres{drift/jev/first/conseq/recoverable/n}{12}
\defres{drift/jev/first/conseq/recoverable/recovered}{100.0}
\defres{drift/jev/first/conseq/recoverable/share}{26.1}
\defres{drift/jev/first/conseq/recoverable/tasks}{6.0}
\defres{drift/jev/first/conseq/write/n}{34}
\defres{drift/jev/first/conseq/write/recovered}{0.0}
\defres{drift/jev/first/conseq/write/share}{73.9}
\defres{drift/jev/first/conseq/write/tasks}{17.0}
\defres{drift/jev/first/failed}{34}
\defres{drift/jev/first/failed_with_wrong}{100.0}
\defres{drift/jev/first/in_c}{23.0}
\defres{drift/jev/first/in_c/n}{46}
\defres{drift/jev/first/inc_offline_right}{0.0}
\defres{drift/jev/first/inc_offline_right/n}{0}
\defres{drift/jev/first/inc_same_answer/n}{45}
\defres{drift/jev/first/irreversible}{17.0}
\defres{drift/jev/first/irreversible/n}{34}
\defres{drift/jev/first/irreversible_of_failed}{100.0}
\defres{drift/jev/first/none}{77.0}
\defres{drift/jev/first/none/n}{154}
\defres{drift/jev/first/novel}{0.0}
\defres{drift/jev/first/novel/n}{0}
\defres{drift/jev/first/recovered}{26.1}
\defres{drift/jev/first/recovered/n}{12}
\defres{drift/jev/first/step_le1}{80.4}
\defres{drift/jev/first/step_median}{1}
\defres{drift/jev/first/top_type}{wrong core tool}
\defres{drift/jev/first/top_type/share}{58.7}
\defres{drift/jev/first/type/act_before_ask/n}{9}
\defres{drift/jev/first/type/act_before_ask/share}{19.6}
\defres{drift/jev/first/type/act_before_ask/tasks}{4.5}
\defres{drift/jev/first/type/lookalike_other/n}{1}
\defres{drift/jev/first/type/lookalike_other/share}{2.2}
\defres{drift/jev/first/type/lookalike_other/tasks}{0.5}
\defres{drift/jev/first/type/unneeded_question/n}{9}
\defres{drift/jev/first/type/unneeded_question/share}{19.6}
\defres{drift/jev/first/type/unneeded_question/tasks}{4.5}
\defres{drift/jev/first/type/wrong_core_tool/n}{27}
\defres{drift/jev/first/type/wrong_core_tool/share}{58.7}
\defres{drift/jev/first/type/wrong_core_tool/tasks}{13.5}
\defres{drift/jev/first/with_wrong/n}{46}
\defres{drift/jev/gate/05/failed_first_below}{0.0}
\defres{drift/jev/gate/05/right_below}{1.1}
\defres{drift/jev/gate/05/wrong_below}{20.6}
\defres{drift/jev/gate/09/failed_first_below}{73.5}
\defres{drift/jev/gate/09/right_below}{18.9}
\defres{drift/jev/gate/09/wrong_below}{86.8}
\defres{drift/jev/gate/failed_first_below}{97.1}
\defres{drift/jev/gate/jev/failed_first_below}{97.1}
\defres{drift/jev/gate/jev/right_below}{60.3}
\defres{drift/jev/gate/jev/wrong_below}{98.5}
\defres{drift/jev/gate/n_wrong}{68}
\defres{drift/jev/gate/own/failed_first_below}{97.1}
\defres{drift/jev/gate/own/right_below}{60.3}
\defres{drift/jev/gate/own/wrong_below}{98.5}
\defres{drift/jev/gate/right_below}{60.3}
\defres{drift/jev/gate/source}{own}
\defres{drift/jev/gate/tau}{1.00}
\defres{drift/jev/gate/wrong_below}{98.5}
\defres{drift/jev/live/n}{200}
\defres{drift/jev/live/success}{83.0}
\defres{drift/jev/loss/compounding}{0.0}
\defres{drift/jev/loss/irreversible}{17.0}
\defres{drift/jev/loss/no_wrong_choice}{0.0}
\defres{drift/jev/loss/total}{17.0}
\defres{drift/jev/mustask/acc}{73.5}
\defres{drift/jev/mustask/acted}{26.5}
\defres{drift/jev/mustask/acted/n}{9}
\defres{drift/jev/mustask/n}{34}
\defres{drift/jev/mustask/step_median}{0}
\defres{drift/jev/mustask/tasks}{34}
\defres{drift/jev/states/inc_share}{100.0}
\defres{drift/jev/states/n}{1{,}391}
\defres{drift/jev/states/novel_offplan_share}{0.0}
\defres{drift/jev/states/novel_onplan_share}{0.0}
\defres{drift/jev/states/novel_share}{0.0}
\defres{drift/jev/states/offplan_share}{8.8}
\defres{drift/jev_tau}{1.00}
\defres{drift/kendall/novel_after_off_plan_share_vs_live}{-0.49}
\defres{drift/kendall/novel_on_plan_share_vs_live}{0.50}
\defres{drift/kendall/novel_share_vs_live}{0.13}
\defres{drift/match/intern}{100.0}
\defres{drift/match/intern/n}{925}
\defres{drift/match/jev}{100.0}
\defres{drift/match/jev/n}{1{,}391}
\defres{drift/match/llm_only}{100.0}
\defres{drift/match/llm_only/n}{1{,}498}
\defres{drift/match/rl}{100.0}
\defres{drift/match/rl/n}{1{,}500}
\defres{drift/n_models}{18}
\defres{drift/oaidec/acc/after_off_plan}{55.6}
\defres{drift/oaidec/acc/after_off_plan/n}{248}
\defres{drift/oaidec/acc/all}{87.4}
\defres{drift/oaidec/acc/all/n}{1{,}466}
\defres{drift/oaidec/acc/executed_all}{87.4}
\defres{drift/oaidec/acc/executed_all/n}{1{,}466}
\defres{drift/oaidec/acc/in_c}{92.3}
\defres{drift/oaidec/acc/in_c/n}{613}
\defres{drift/oaidec/acc/in_c_after_off_plan}{60.0}
\defres{drift/oaidec/acc/in_c_after_off_plan/n}{5}
\defres{drift/oaidec/acc/in_c_on_plan}{92.6}
\defres{drift/oaidec/acc/in_c_on_plan/n}{608}
\defres{drift/oaidec/acc/novel}{83.9}
\defres{drift/oaidec/acc/novel/n}{853}
\defres{drift/oaidec/acc/novel_after_off_plan}{55.6}
\defres{drift/oaidec/acc/novel_after_off_plan/n}{243}
\defres{drift/oaidec/acc/novel_on_plan}{95.2}
\defres{drift/oaidec/acc/novel_on_plan/n}{610}
\defres{drift/oaidec/acc/on_plan}{93.9}
\defres{drift/oaidec/acc/on_plan/n}{1{,}218}
\defres{drift/oaidec/ask/acc}{88.8}
\defres{drift/oaidec/ask/acted}{11.2}
\defres{drift/oaidec/ask/acted/n}{11}
\defres{drift/oaidec/ask/acted_of_wrong}{100.0}
\defres{drift/oaidec/ask/n}{98}
\defres{drift/oaidec/askearly/share}{11.0}
\defres{drift/oaidec/askearly/tasks}{22}
\defres{drift/oaidec/c/acc}{90.9}
\defres{drift/oaidec/c/ask_acc}{75.9}
\defres{drift/oaidec/c/mustask_acc}{38.5}
\defres{drift/oaidec/conf/right}{73.4}
\defres{drift/oaidec/conf/wrong}{50.4}
\defres{drift/oaidec/faith/agree}{100.0}
\defres{drift/oaidec/faith/live}{92.3}
\defres{drift/oaidec/faith/lr_ow}{0}
\defres{drift/oaidec/faith/lw_or}{0}
\defres{drift/oaidec/faith/n}{613}
\defres{drift/oaidec/faith/offline}{92.3}
\defres{drift/oaidec/first/conseq/finish/n}{1}
\defres{drift/oaidec/first/conseq/finish/recovered}{0.0}
\defres{drift/oaidec/first/conseq/finish/share}{1.4}
\defres{drift/oaidec/first/conseq/finish/tasks}{0.5}
\defres{drift/oaidec/first/conseq/recoverable/n}{39}
\defres{drift/oaidec/first/conseq/recoverable/recovered}{79.5}
\defres{drift/oaidec/first/conseq/recoverable/share}{52.7}
\defres{drift/oaidec/first/conseq/recoverable/tasks}{19.5}
\defres{drift/oaidec/first/conseq/write/n}{34}
\defres{drift/oaidec/first/conseq/write/recovered}{0.0}
\defres{drift/oaidec/first/conseq/write/share}{45.9}
\defres{drift/oaidec/first/conseq/write/tasks}{17.0}
\defres{drift/oaidec/first/failed}{43}
\defres{drift/oaidec/first/failed_with_wrong}{100.0}
\defres{drift/oaidec/first/in_c}{22.5}
\defres{drift/oaidec/first/in_c/n}{45}
\defres{drift/oaidec/first/inc_offline_right}{0.0}
\defres{drift/oaidec/first/inc_offline_right/n}{0}
\defres{drift/oaidec/first/inc_same_answer/n}{45}
\defres{drift/oaidec/first/irreversible}{17.5}
\defres{drift/oaidec/first/irreversible/n}{35}
\defres{drift/oaidec/first/irreversible_of_failed}{81.4}
\defres{drift/oaidec/first/none}{63.0}
\defres{drift/oaidec/first/none/n}{126}
\defres{drift/oaidec/first/novel}{14.5}
\defres{drift/oaidec/first/novel/n}{29}
\defres{drift/oaidec/first/recovered}{41.9}
\defres{drift/oaidec/first/recovered/n}{31}
\defres{drift/oaidec/first/step_le1}{60.8}
\defres{drift/oaidec/first/step_median}{1}
\defres{drift/oaidec/first/top_type}{wrong core tool}
\defres{drift/oaidec/first/top_type/share}{52.7}
\defres{drift/oaidec/first/type/act_before_ask/n}{11}
\defres{drift/oaidec/first/type/act_before_ask/share}{14.9}
\defres{drift/oaidec/first/type/act_before_ask/tasks}{5.5}
\defres{drift/oaidec/first/type/finished_too_early/n}{1}
\defres{drift/oaidec/first/type/finished_too_early/share}{1.4}
\defres{drift/oaidec/first/type/finished_too_early/tasks}{0.5}
\defres{drift/oaidec/first/type/lookalike_other/n}{14}
\defres{drift/oaidec/first/type/lookalike_other/share}{18.9}
\defres{drift/oaidec/first/type/lookalike_other/tasks}{7.0}
\defres{drift/oaidec/first/type/unneeded_question/n}{9}
\defres{drift/oaidec/first/type/unneeded_question/share}{12.2}
\defres{drift/oaidec/first/type/unneeded_question/tasks}{4.5}
\defres{drift/oaidec/first/type/wrong_core_tool/n}{39}
\defres{drift/oaidec/first/type/wrong_core_tool/share}{52.7}
\defres{drift/oaidec/first/type/wrong_core_tool/tasks}{19.5}
\defres{drift/oaidec/first/with_wrong/n}{74}
\defres{drift/oaidec/gate/05/failed_first_below}{32.6}
\defres{drift/oaidec/gate/05/right_below}{18.4}
\defres{drift/oaidec/gate/05/wrong_below}{54.9}
\defres{drift/oaidec/gate/09/failed_first_below}{86.0}
\defres{drift/oaidec/gate/09/right_below}{66.6}
\defres{drift/oaidec/gate/09/wrong_below}{92.9}
\defres{drift/oaidec/gate/failed_first_below}{100.0}
\defres{drift/oaidec/gate/jev/failed_first_below}{100.0}
\defres{drift/oaidec/gate/jev/right_below}{96.5}
\defres{drift/oaidec/gate/jev/wrong_below}{100.0}
\defres{drift/oaidec/gate/n_wrong}{184}
\defres{drift/oaidec/gate/right_below}{96.5}
\defres{drift/oaidec/gate/source}{jev}
\defres{drift/oaidec/gate/tau}{1.00}
\defres{drift/oaidec/gate/wrong_below}{100.0}
\defres{drift/oaidec/live/n}{200}
\defres{drift/oaidec/live/success}{78.5}
\defres{drift/oaidec/loss/compounding}{4.0}
\defres{drift/oaidec/loss/irreversible}{17.5}
\defres{drift/oaidec/loss/no_wrong_choice}{0.0}
\defres{drift/oaidec/loss/total}{21.5}
\defres{drift/oaidec/mustask/acc}{71.1}
\defres{drift/oaidec/mustask/acted}{28.9}
\defres{drift/oaidec/mustask/acted/n}{11}
\defres{drift/oaidec/mustask/n}{38}
\defres{drift/oaidec/mustask/step_median}{0}
\defres{drift/oaidec/mustask/tasks}{38}
\defres{drift/oaidec/states/inc_share}{41.8}
\defres{drift/oaidec/states/n}{1{,}466}
\defres{drift/oaidec/states/novel_offplan_share}{16.6}
\defres{drift/oaidec/states/novel_onplan_share}{41.6}
\defres{drift/oaidec/states/novel_share}{58.2}
\defres{drift/oaidec/states/offplan_share}{16.9}
\defres{drift/openjev/acc/after_off_plan}{38.3}
\defres{drift/openjev/acc/after_off_plan/n}{493}
\defres{drift/openjev/acc/all}{75.9}
\defres{drift/openjev/acc/all/n}{1{,}650}
\defres{drift/openjev/acc/executed_all}{75.9}
\defres{drift/openjev/acc/executed_all/n}{1{,}650}
\defres{drift/openjev/acc/in_c}{91.3}
\defres{drift/openjev/acc/in_c/n}{677}
\defres{drift/openjev/acc/in_c_after_off_plan/n}{0}
\defres{drift/openjev/acc/in_c_on_plan}{91.3}
\defres{drift/openjev/acc/in_c_on_plan/n}{677}
\defres{drift/openjev/acc/novel}{65.3}
\defres{drift/openjev/acc/novel/n}{973}
\defres{drift/openjev/acc/novel_after_off_plan}{38.3}
\defres{drift/openjev/acc/novel_after_off_plan/n}{493}
\defres{drift/openjev/acc/novel_on_plan}{92.9}
\defres{drift/openjev/acc/novel_on_plan/n}{480}
\defres{drift/openjev/acc/on_plan}{92.0}
\defres{drift/openjev/acc/on_plan/n}{1{,}157}
\defres{drift/openjev/ask/acc}{74.7}
\defres{drift/openjev/ask/acted}{25.3}
\defres{drift/openjev/ask/acted/n}{50}
\defres{drift/openjev/ask/acted_of_wrong}{100.0}
\defres{drift/openjev/ask/n}{198}
\defres{drift/openjev/askearly/share}{1.0}
\defres{drift/openjev/askearly/tasks}{2}
\defres{drift/openjev/c/acc}{91.1}
\defres{drift/openjev/c/ask_acc}{87.5}
\defres{drift/openjev/c/mustask_acc}{50.0}
\defres{drift/openjev/conf/right}{90.4}
\defres{drift/openjev/conf/wrong}{82.3}
\defres{drift/openjev/faith/agree}{96.9}
\defres{drift/openjev/faith/live}{91.3}
\defres{drift/openjev/faith/lr_ow}{8}
\defres{drift/openjev/faith/lw_or}{7}
\defres{drift/openjev/faith/n}{677}
\defres{drift/openjev/faith/offline}{91.1}
\defres{drift/openjev/faith/sign_p}{1.000}
\defres{drift/openjev/first/conseq/recoverable/n}{25}
\defres{drift/openjev/first/conseq/recoverable/recovered}{48.0}
\defres{drift/openjev/first/conseq/recoverable/share}{26.9}
\defres{drift/openjev/first/conseq/recoverable/tasks}{12.5}
\defres{drift/openjev/first/conseq/write/n}{68}
\defres{drift/openjev/first/conseq/write/recovered}{8.8}
\defres{drift/openjev/first/conseq/write/share}{73.1}
\defres{drift/openjev/first/conseq/write/tasks}{34.0}
\defres{drift/openjev/first/failed}{75}
\defres{drift/openjev/first/failed_with_wrong}{100.0}
\defres{drift/openjev/first/in_c}{29.5}
\defres{drift/openjev/first/in_c/n}{59}
\defres{drift/openjev/first/inc_offline_right}{11.9}
\defres{drift/openjev/first/inc_offline_right/n}{7}
\defres{drift/openjev/first/inc_same_answer/n}{47}
\defres{drift/openjev/first/irreversible}{34.0}
\defres{drift/openjev/first/irreversible/n}{68}
\defres{drift/openjev/first/irreversible_of_failed}{82.7}
\defres{drift/openjev/first/none}{53.5}
\defres{drift/openjev/first/none/n}{107}
\defres{drift/openjev/first/novel}{17.0}
\defres{drift/openjev/first/novel/n}{34}
\defres{drift/openjev/first/recovered}{19.4}
\defres{drift/openjev/first/recovered/n}{18}
\defres{drift/openjev/first/step_le1}{5.4}
\defres{drift/openjev/first/step_median}{2}
\defres{drift/openjev/first/top_type}{changed state before asking}
\defres{drift/openjev/first/top_type/share}{53.8}
\defres{drift/openjev/first/type/act_before_ask/n}{50}
\defres{drift/openjev/first/type/act_before_ask/share}{53.8}
\defres{drift/openjev/first/type/act_before_ask/tasks}{25.0}
\defres{drift/openjev/first/type/lookalike_gold/n}{9}
\defres{drift/openjev/first/type/lookalike_gold/share}{9.7}
\defres{drift/openjev/first/type/lookalike_gold/tasks}{4.5}
\defres{drift/openjev/first/type/lookalike_other/n}{8}
\defres{drift/openjev/first/type/lookalike_other/share}{8.6}
\defres{drift/openjev/first/type/lookalike_other/tasks}{4.0}
\defres{drift/openjev/first/type/unneeded_question/n}{2}
\defres{drift/openjev/first/type/unneeded_question/share}{2.2}
\defres{drift/openjev/first/type/unneeded_question/tasks}{1.0}
\defres{drift/openjev/first/type/unrelated/n}{4}
\defres{drift/openjev/first/type/unrelated/share}{4.3}
\defres{drift/openjev/first/type/unrelated/tasks}{2.0}
\defres{drift/openjev/first/type/wrong_core_tool/n}{20}
\defres{drift/openjev/first/type/wrong_core_tool/share}{21.5}
\defres{drift/openjev/first/type/wrong_core_tool/tasks}{10.0}
\defres{drift/openjev/first/with_wrong/n}{93}
\defres{drift/openjev/gate/05/failed_first_below}{9.3}
\defres{drift/openjev/gate/05/right_below}{1.2}
\defres{drift/openjev/gate/05/wrong_below}{5.8}
\defres{drift/openjev/gate/09/failed_first_below}{34.7}
\defres{drift/openjev/gate/09/right_below}{31.0}
\defres{drift/openjev/gate/09/wrong_below}{52.4}
\defres{drift/openjev/gate/failed_first_below}{100.0}
\defres{drift/openjev/gate/jev/failed_first_below}{100.0}
\defres{drift/openjev/gate/jev/right_below}{100.0}
\defres{drift/openjev/gate/jev/wrong_below}{100.0}
\defres{drift/openjev/gate/n_wrong}{397}
\defres{drift/openjev/gate/right_below}{100.0}
\defres{drift/openjev/gate/source}{jev}
\defres{drift/openjev/gate/tau}{1.00}
\defres{drift/openjev/gate/wrong_below}{100.0}
\defres{drift/openjev/live/n}{200}
\defres{drift/openjev/live/success}{62.5}
\defres{drift/openjev/loss/compounding}{6.5}
\defres{drift/openjev/loss/irreversible}{31.0}
\defres{drift/openjev/loss/no_wrong_choice}{0.0}
\defres{drift/openjev/loss/total}{37.5}
\defres{drift/openjev/mustask/acc}{49.0}
\defres{drift/openjev/mustask/acted}{51.0}
\defres{drift/openjev/mustask/acted/n}{50}
\defres{drift/openjev/mustask/n}{98}
\defres{drift/openjev/mustask/step_median}{2}
\defres{drift/openjev/mustask/tasks}{98}
\defres{drift/openjev/states/inc_share}{41.0}
\defres{drift/openjev/states/n}{1{,}650}
\defres{drift/openjev/states/novel_offplan_share}{29.9}
\defres{drift/openjev/states/novel_onplan_share}{29.1}
\defres{drift/openjev/states/novel_share}{59.0}
\defres{drift/openjev/states/offplan_share}{29.9}
\defres{drift/openjevhf/acc/after_off_plan}{100.0}
\defres{drift/openjevhf/acc/after_off_plan/n}{1}
\defres{drift/openjevhf/acc/all}{94.5}
\defres{drift/openjevhf/acc/all/n}{1{,}353}
\defres{drift/openjevhf/acc/executed_all}{94.5}
\defres{drift/openjevhf/acc/executed_all/n}{1{,}353}
\defres{drift/openjevhf/acc/in_c}{92.0}
\defres{drift/openjevhf/acc/in_c/n}{736}
\defres{drift/openjevhf/acc/in_c_after_off_plan/n}{0}
\defres{drift/openjevhf/acc/in_c_on_plan}{92.0}
\defres{drift/openjevhf/acc/in_c_on_plan/n}{736}
\defres{drift/openjevhf/acc/novel}{97.4}
\defres{drift/openjevhf/acc/novel/n}{617}
\defres{drift/openjevhf/acc/novel_after_off_plan}{100.0}
\defres{drift/openjevhf/acc/novel_after_off_plan/n}{1}
\defres{drift/openjevhf/acc/novel_on_plan}{97.4}
\defres{drift/openjevhf/acc/novel_on_plan/n}{616}
\defres{drift/openjevhf/acc/on_plan}{94.5}
\defres{drift/openjevhf/acc/on_plan/n}{1{,}352}
\defres{drift/openjevhf/ask/acc}{63.0}
\defres{drift/openjevhf/ask/acted}{37.0}
\defres{drift/openjevhf/ask/acted/n}{74}
\defres{drift/openjevhf/ask/acted_of_wrong}{100.0}
\defres{drift/openjevhf/ask/n}{200}
\defres{drift/openjevhf/askearly/share}{0.0}
\defres{drift/openjevhf/askearly/tasks}{0}
\defres{drift/openjevhf/c/acc}{92.4}
\defres{drift/openjevhf/c/ask_acc}{63.5}
\defres{drift/openjevhf/c/mustask_acc}{26.0}
\defres{drift/openjevhf/conf/right}{98.6}
\defres{drift/openjevhf/conf/wrong}{91.9}
\defres{drift/openjevhf/faith/agree}{100.0}
\defres{drift/openjevhf/faith/live}{92.0}
\defres{drift/openjevhf/faith/lr_ow}{0}
\defres{drift/openjevhf/faith/lw_or}{0}
\defres{drift/openjevhf/faith/n}{736}
\defres{drift/openjevhf/faith/offline}{92.0}
\defres{drift/openjevhf/first/conseq/recoverable/n}{1}
\defres{drift/openjevhf/first/conseq/recoverable/recovered}{100.0}
\defres{drift/openjevhf/first/conseq/recoverable/share}{1.3}
\defres{drift/openjevhf/first/conseq/recoverable/tasks}{0.5}
\defres{drift/openjevhf/first/conseq/write/n}{74}
\defres{drift/openjevhf/first/conseq/write/recovered}{0.0}
\defres{drift/openjevhf/first/conseq/write/share}{98.7}
\defres{drift/openjevhf/first/conseq/write/tasks}{37.0}
\defres{drift/openjevhf/first/failed}{74}
\defres{drift/openjevhf/first/failed_with_wrong}{100.0}
\defres{drift/openjevhf/first/in_c}{29.5}
\defres{drift/openjevhf/first/in_c/n}{59}
\defres{drift/openjevhf/first/inc_offline_right}{0.0}
\defres{drift/openjevhf/first/inc_offline_right/n}{0}
\defres{drift/openjevhf/first/inc_same_answer/n}{59}
\defres{drift/openjevhf/first/irreversible}{37.0}
\defres{drift/openjevhf/first/irreversible/n}{74}
\defres{drift/openjevhf/first/irreversible_of_failed}{100.0}
\defres{drift/openjevhf/first/none}{62.5}
\defres{drift/openjevhf/first/none/n}{125}
\defres{drift/openjevhf/first/novel}{8.0}
\defres{drift/openjevhf/first/novel/n}{16}
\defres{drift/openjevhf/first/recovered}{1.3}
\defres{drift/openjevhf/first/recovered/n}{1}
\defres{drift/openjevhf/first/step_le1}{0.0}
\defres{drift/openjevhf/first/step_median}{2}
\defres{drift/openjevhf/first/top_type}{changed state before asking}
\defres{drift/openjevhf/first/top_type/share}{98.7}
\defres{drift/openjevhf/first/type/act_before_ask/n}{74}
\defres{drift/openjevhf/first/type/act_before_ask/share}{98.7}
\defres{drift/openjevhf/first/type/act_before_ask/tasks}{37.0}
\defres{drift/openjevhf/first/type/wrong_core_tool/n}{1}
\defres{drift/openjevhf/first/type/wrong_core_tool/share}{1.3}
\defres{drift/openjevhf/first/type/wrong_core_tool/tasks}{0.5}
\defres{drift/openjevhf/first/with_wrong/n}{75}
\defres{drift/openjevhf/gate/05/failed_first_below}{0.0}
\defres{drift/openjevhf/gate/05/right_below}{0.0}
\defres{drift/openjevhf/gate/05/wrong_below}{1.3}
\defres{drift/openjevhf/gate/09/failed_first_below}{25.7}
\defres{drift/openjevhf/gate/09/right_below}{2.6}
\defres{drift/openjevhf/gate/09/wrong_below}{26.7}
\defres{drift/openjevhf/gate/failed_first_below}{100.0}
\defres{drift/openjevhf/gate/jev/failed_first_below}{100.0}
\defres{drift/openjevhf/gate/jev/right_below}{99.1}
\defres{drift/openjevhf/gate/jev/wrong_below}{100.0}
\defres{drift/openjevhf/gate/n_wrong}{75}
\defres{drift/openjevhf/gate/right_below}{99.1}
\defres{drift/openjevhf/gate/source}{jev}
\defres{drift/openjevhf/gate/tau}{1.00}
\defres{drift/openjevhf/gate/wrong_below}{100.0}
\defres{drift/openjevhf/live/n}{200}
\defres{drift/openjevhf/live/success}{63.0}
\defres{drift/openjevhf/loss/compounding}{0.0}
\defres{drift/openjevhf/loss/irreversible}{37.0}
\defres{drift/openjevhf/loss/no_wrong_choice}{0.0}
\defres{drift/openjevhf/loss/total}{37.0}
\defres{drift/openjevhf/mustask/acc}{26.0}
\defres{drift/openjevhf/mustask/acted}{74.0}
\defres{drift/openjevhf/mustask/acted/n}{74}
\defres{drift/openjevhf/mustask/n}{100}
\defres{drift/openjevhf/mustask/step_median}{2}
\defres{drift/openjevhf/mustask/tasks}{100}
\defres{drift/openjevhf/states/inc_share}{54.4}
\defres{drift/openjevhf/states/n}{1{,}353}
\defres{drift/openjevhf/states/novel_offplan_share}{0.1}
\defres{drift/openjevhf/states/novel_onplan_share}{45.5}
\defres{drift/openjevhf/states/novel_share}{45.6}
\defres{drift/openjevhf/states/offplan_share}{0.1}
\defres{drift/pred/base/pred}{21.8}
\defres{drift/pred/base/pred/err}{+8.8}
\defres{drift/pred/base/pred_earlyask}{30.0}
\defres{drift/pred/base/pred_earlyask/err}{+17.0}
\defres{drift/pred/base/pred_llm}{18.0}
\defres{drift/pred/base/pred_llm/err}{+5.0}
\defres{drift/pred/base/pred_onplan}{23.0}
\defres{drift/pred/base/pred_onplan/err}{+10.0}
\defres{drift/pred/e12/pred}{99.8}
\defres{drift/pred/e12/pred/err}{-0.2}
\defres{drift/pred/e12/pred_earlyask}{99.8}
\defres{drift/pred/e12/pred_earlyask/err}{-0.2}
\defres{drift/pred/e12/pred_llm}{100.0}
\defres{drift/pred/e12/pred_llm/err}{+0.0}
\defres{drift/pred/e12/pred_onplan}{100.0}
\defres{drift/pred/e12/pred_onplan/err}{+0.0}
\defres{drift/pred/e12c/pred}{99.8}
\defres{drift/pred/e12c/pred/err}{-0.2}
\defres{drift/pred/e12c/pred_earlyask}{99.8}
\defres{drift/pred/e12c/pred_earlyask/err}{-0.2}
\defres{drift/pred/e12c/pred_llm}{99.5}
\defres{drift/pred/e12c/pred_llm/err}{-0.5}
\defres{drift/pred/e12c/pred_onplan}{99.9}
\defres{drift/pred/e12c/pred_onplan/err}{-0.1}
\defres{drift/pred/e14a/pred}{99.4}
\defres{drift/pred/e14a/pred/err}{-0.6}
\defres{drift/pred/e14a/pred_earlyask}{99.4}
\defres{drift/pred/e14a/pred_earlyask/err}{-0.6}
\defres{drift/pred/e14a/pred_llm}{98.0}
\defres{drift/pred/e14a/pred_llm/err}{-2.0}
\defres{drift/pred/e14a/pred_onplan}{99.5}
\defres{drift/pred/e14a/pred_onplan/err}{-0.5}
\defres{drift/pred/e14g/pred}{0.0}
\defres{drift/pred/e14g/pred/err}{+0.0}
\defres{drift/pred/e14g/pred_earlyask}{0.0}
\defres{drift/pred/e14g/pred_earlyask/err}{+0.0}
\defres{drift/pred/e14g/pred_llm}{0.0}
\defres{drift/pred/e14g/pred_llm/err}{+0.0}
\defres{drift/pred/e14g/pred_onplan}{0.0}
\defres{drift/pred/e14g/pred_onplan/err}{+0.0}
\defres{drift/pred/intern/pred}{42.9}
\defres{drift/pred/intern/pred/err}{+16.4}
\defres{drift/pred/intern/pred_earlyask}{44.9}
\defres{drift/pred/intern/pred_earlyask/err}{+18.4}
\defres{drift/pred/intern/pred_llm}{32.5}
\defres{drift/pred/intern/pred_llm/err}{+6.0}
\defres{drift/pred/intern/pred_onplan}{43.1}
\defres{drift/pred/intern/pred_onplan/err}{+16.6}
\defres{drift/pred/jev/pred}{72.9}
\defres{drift/pred/jev/pred/err}{-10.1}
\defres{drift/pred/jev/pred_earlyask}{80.0}
\defres{drift/pred/jev/pred_earlyask/err}{-3.0}
\defres{drift/pred/jev/pred_llm}{63.5}
\defres{drift/pred/jev/pred_llm/err}{-19.5}
\defres{drift/pred/jev/pred_onplan}{73.4}
\defres{drift/pred/jev/pred_onplan/err}{-9.6}
\defres{drift/pred/kendall/all/cmean}{0.78}
\defres{drift/pred/kendall/all/mustask}{0.72}
\defres{drift/pred/kendall/all/n}{18}
\defres{drift/pred/kendall/all/pred}{0.83}
\defres{drift/pred/kendall/all/pred_earlyask}{0.84}
\defres{drift/pred/kendall/all/pred_llm}{0.83}
\defres{drift/pred/kendall/all/pred_onplan}{0.83}
\defres{drift/pred/kendall/offtheshelf/cmean}{0.54}
\defres{drift/pred/kendall/offtheshelf/mustask}{0.26}
\defres{drift/pred/kendall/offtheshelf/n}{10}
\defres{drift/pred/kendall/offtheshelf/pred}{0.63}
\defres{drift/pred/kendall/offtheshelf/pred_earlyask}{0.63}
\defres{drift/pred/kendall/offtheshelf/pred_llm}{0.57}
\defres{drift/pred/kendall/offtheshelf/pred_onplan}{0.63}
\defres{drift/pred/mae/all/pred}{8.3}
\defres{drift/pred/mae/all/pred_earlyask}{9.0}
\defres{drift/pred/mae/all/pred_llm}{7.0}
\defres{drift/pred/mae/all/pred_onplan}{8.6}
\defres{drift/pred/mae/offtheshelf/pred}{14.0}
\defres{drift/pred/mae/offtheshelf/pred_earlyask}{14.4}
\defres{drift/pred/mae/offtheshelf/pred_llm}{11.7}
\defres{drift/pred/mae/offtheshelf/pred_onplan}{14.5}
\defres{drift/pred/oaidec/pred}{77.4}
\defres{drift/pred/oaidec/pred/err}{-1.1}
\defres{drift/pred/oaidec/pred_earlyask}{80.1}
\defres{drift/pred/oaidec/pred_earlyask/err}{+1.6}
\defres{drift/pred/oaidec/pred_llm}{67.0}
\defres{drift/pred/oaidec/pred_llm/err}{-11.5}
\defres{drift/pred/oaidec/pred_onplan}{77.9}
\defres{drift/pred/oaidec/pred_onplan/err}{-0.6}
\defres{drift/pred/openjev/pred}{71.5}
\defres{drift/pred/openjev/pred/err}{+9.0}
\defres{drift/pred/openjev/pred_earlyask}{71.5}
\defres{drift/pred/openjev/pred_earlyask/err}{+9.0}
\defres{drift/pred/openjev/pred_llm}{67.0}
\defres{drift/pred/openjev/pred_llm/err}{+4.5}
\defres{drift/pred/openjev/pred_onplan}{72.6}
\defres{drift/pred/openjev/pred_onplan/err}{+10.1}
\defres{drift/pred/openjevhf/pred}{75.6}
\defres{drift/pred/openjevhf/pred/err}{+12.6}
\defres{drift/pred/openjevhf/pred_earlyask}{75.6}
\defres{drift/pred/openjevhf/pred_earlyask/err}{+12.6}
\defres{drift/pred/openjevhf/pred_llm}{63.0}
\defres{drift/pred/openjevhf/pred_llm/err}{+0.0}
\defres{drift/pred/openjevhf/pred_onplan}{76.6}
\defres{drift/pred/openjevhf/pred_onplan/err}{+13.6}
\defres{drift/pred/rl/pred}{100.0}
\defres{drift/pred/rl/pred/err}{+0.0}
\defres{drift/pred/rl/pred_earlyask}{100.0}
\defres{drift/pred/rl/pred_earlyask/err}{+0.0}
\defres{drift/pred/rl/pred_llm}{100.0}
\defres{drift/pred/rl/pred_llm/err}{+0.0}
\defres{drift/pred/rl/pred_onplan}{100.0}
\defres{drift/pred/rl/pred_onplan/err}{+0.0}
\defres{drift/pred/sft_v1/pred}{100.0}
\defres{drift/pred/sft_v1/pred/err}{+0.0}
\defres{drift/pred/sft_v1/pred_earlyask}{100.0}
\defres{drift/pred/sft_v1/pred_earlyask/err}{+0.0}
\defres{drift/pred/sft_v1/pred_llm}{100.0}
\defres{drift/pred/sft_v1/pred_llm/err}{+0.0}
\defres{drift/pred/sft_v1/pred_onplan}{100.0}
\defres{drift/pred/sft_v1/pred_onplan/err}{+0.0}
\defres{drift/pred/sl0.8b/pred}{63.7}
\defres{drift/pred/sl0.8b/pred/err}{+46.2}
\defres{drift/pred/sl0.8b/pred_earlyask}{72.1}
\defres{drift/pred/sl0.8b/pred_earlyask/err}{+54.6}
\defres{drift/pred/sl0.8b/pred_llm}{59.5}
\defres{drift/pred/sl0.8b/pred_llm/err}{+42.0}
\defres{drift/pred/sl0.8b/pred_onplan}{64.4}
\defres{drift/pred/sl0.8b/pred_onplan/err}{+46.9}
\defres{drift/pred/sl27b/pred}{78.9}
\defres{drift/pred/sl27b/pred/err}{+15.9}
\defres{drift/pred/sl27b/pred_earlyask}{78.9}
\defres{drift/pred/sl27b/pred_earlyask/err}{+15.9}
\defres{drift/pred/sl27b/pred_llm}{63.0}
\defres{drift/pred/sl27b/pred_llm/err}{+0.0}
\defres{drift/pred/sl27b/pred_onplan}{79.6}
\defres{drift/pred/sl27b/pred_onplan/err}{+16.6}
\defres{drift/pred/sl2b/pred}{24.5}
\defres{drift/pred/sl2b/pred/err}{+18.0}
\defres{drift/pred/sl2b/pred_earlyask}{25.2}
\defres{drift/pred/sl2b/pred_earlyask/err}{+18.8}
\defres{drift/pred/sl2b/pred_llm}{18.0}
\defres{drift/pred/sl2b/pred_llm/err}{+11.5}
\defres{drift/pred/sl2b/pred_onplan}{27.3}
\defres{drift/pred/sl2b/pred_onplan/err}{+20.8}
\defres{drift/pred/sl4b/pred}{67.4}
\defres{drift/pred/sl4b/pred/err}{+7.4}
\defres{drift/pred/sl4b/pred_earlyask}{67.4}
\defres{drift/pred/sl4b/pred_earlyask/err}{+7.4}
\defres{drift/pred/sl4b/pred_llm}{51.0}
\defres{drift/pred/sl4b/pred_llm/err}{-9.0}
\defres{drift/pred/sl4b/pred_onplan}{68.2}
\defres{drift/pred/sl4b/pred_onplan/err}{+8.3}
\defres{drift/pred/sl9b/pred}{71.0}
\defres{drift/pred/sl9b/pred/err}{-3.0}
\defres{drift/pred/sl9b/pred_earlyask}{71.0}
\defres{drift/pred/sl9b/pred_earlyask/err}{-3.0}
\defres{drift/pred/sl9b/pred_llm}{60.5}
\defres{drift/pred/sl9b/pred_llm/err}{-13.5}
\defres{drift/pred/sl9b/pred_onplan}{72.4}
\defres{drift/pred/sl9b/pred_onplan/err}{-1.6}
\defres{drift/pred/v2/pred}{99.9}
\defres{drift/pred/v2/pred/err}{-0.1}
\defres{drift/pred/v2/pred_earlyask}{99.9}
\defres{drift/pred/v2/pred_earlyask/err}{-0.1}
\defres{drift/pred/v2/pred_llm}{99.5}
\defres{drift/pred/v2/pred_llm/err}{-0.5}
\defres{drift/pred/v2/pred_onplan}{99.9}
\defres{drift/pred/v2/pred_onplan/err}{-0.1}
\defres{drift/rl/acc/after_off_plan/n}{0}
\defres{drift/rl/acc/all}{100.0}
\defres{drift/rl/acc/all/n}{1{,}500}
\defres{drift/rl/acc/executed_all}{100.0}
\defres{drift/rl/acc/executed_all/n}{1{,}500}
\defres{drift/rl/acc/in_c}{100.0}
\defres{drift/rl/acc/in_c/n}{1{,}500}
\defres{drift/rl/acc/in_c_after_off_plan/n}{0}
\defres{drift/rl/acc/in_c_on_plan}{100.0}
\defres{drift/rl/acc/in_c_on_plan/n}{1{,}500}
\defres{drift/rl/acc/novel/n}{0}
\defres{drift/rl/acc/novel_after_off_plan/n}{0}
\defres{drift/rl/acc/novel_on_plan/n}{0}
\defres{drift/rl/acc/on_plan}{100.0}
\defres{drift/rl/acc/on_plan/n}{1{,}500}
\defres{drift/rl/ask/acc}{100.0}
\defres{drift/rl/ask/acted}{0.0}
\defres{drift/rl/ask/acted/n}{0}
\defres{drift/rl/ask/n}{109}
\defres{drift/rl/askearly/share}{0.0}
\defres{drift/rl/askearly/tasks}{0}
\defres{drift/rl/c/acc}{99.2}
\defres{drift/rl/c/ask_acc}{100.0}
\defres{drift/rl/c/mustask_acc}{100.0}
\defres{drift/rl/conf/right}{99.9}
\defres{drift/rl/faith/agree}{99.8}
\defres{drift/rl/faith/live}{100.0}
\defres{drift/rl/faith/lr_ow}{0}
\defres{drift/rl/faith/lw_or}{0}
\defres{drift/rl/faith/n}{1{,}500}
\defres{drift/rl/faith/offline}{100.0}
\defres{drift/rl/first/failed}{0}
\defres{drift/rl/first/in_c}{0.0}
\defres{drift/rl/first/in_c/n}{0}
\defres{drift/rl/first/inc_offline_right/n}{0}
\defres{drift/rl/first/inc_same_answer/n}{0}
\defres{drift/rl/first/irreversible}{0.0}
\defres{drift/rl/first/irreversible/n}{0}
\defres{drift/rl/first/none}{100.0}
\defres{drift/rl/first/none/n}{200}
\defres{drift/rl/first/novel}{0.0}
\defres{drift/rl/first/novel/n}{0}
\defres{drift/rl/first/recovered/n}{0}
\defres{drift/rl/first/with_wrong/n}{0}
\defres{drift/rl/gate/05/right_below}{0.1}
\defres{drift/rl/gate/09/right_below}{0.2}
\defres{drift/rl/gate/jev/right_below}{35.3}
\defres{drift/rl/gate/n_wrong}{0}
\defres{drift/rl/gate/own/right_below}{0.0}
\defres{drift/rl/gate/right_below}{0.0}
\defres{drift/rl/gate/source}{own}
\defres{drift/rl/gate/tau}{0.50}
\defres{drift/rl/live/n}{200}
\defres{drift/rl/live/success}{100.0}
\defres{drift/rl/loss/compounding}{0.0}
\defres{drift/rl/loss/irreversible}{0.0}
\defres{drift/rl/loss/no_wrong_choice}{0.0}
\defres{drift/rl/loss/total}{0.0}
\defres{drift/rl/mustask/acc}{100.0}
\defres{drift/rl/mustask/acted}{0.0}
\defres{drift/rl/mustask/acted/n}{0}
\defres{drift/rl/mustask/n}{54}
\defres{drift/rl/mustask/step_median}{2}
\defres{drift/rl/mustask/tasks}{54}
\defres{drift/rl/states/inc_share}{100.0}
\defres{drift/rl/states/n}{1{,}500}
\defres{drift/rl/states/novel_offplan_share}{0.0}
\defres{drift/rl/states/novel_onplan_share}{0.0}
\defres{drift/rl/states/novel_share}{0.0}
\defres{drift/rl/states/offplan_share}{0.0}
\defres{drift/sft_v1/acc/after_off_plan/n}{0}
\defres{drift/sft_v1/acc/all}{100.0}
\defres{drift/sft_v1/acc/all/n}{750}
\defres{drift/sft_v1/acc/executed_all}{100.0}
\defres{drift/sft_v1/acc/executed_all/n}{750}
\defres{drift/sft_v1/acc/in_c}{100.0}
\defres{drift/sft_v1/acc/in_c/n}{360}
\defres{drift/sft_v1/acc/in_c_after_off_plan/n}{0}
\defres{drift/sft_v1/acc/in_c_on_plan}{100.0}
\defres{drift/sft_v1/acc/in_c_on_plan/n}{360}
\defres{drift/sft_v1/acc/novel}{100.0}
\defres{drift/sft_v1/acc/novel/n}{390}
\defres{drift/sft_v1/acc/novel_after_off_plan/n}{0}
\defres{drift/sft_v1/acc/novel_on_plan}{100.0}
\defres{drift/sft_v1/acc/novel_on_plan/n}{390}
\defres{drift/sft_v1/acc/on_plan}{100.0}
\defres{drift/sft_v1/acc/on_plan/n}{750}
\defres{drift/sft_v1/ask/acc}{100.0}
\defres{drift/sft_v1/ask/acted}{0.0}
\defres{drift/sft_v1/ask/acted/n}{0}
\defres{drift/sft_v1/ask/n}{50}
\defres{drift/sft_v1/askearly/share}{0.0}
\defres{drift/sft_v1/askearly/tasks}{0}
\defres{drift/sft_v1/c/acc}{99.2}
\defres{drift/sft_v1/c/ask_acc}{100.0}
\defres{drift/sft_v1/c/mustask_acc}{100.0}
\defres{drift/sft_v1/conf/right}{100.0}
\defres{drift/sft_v1/faith/agree}{100.0}
\defres{drift/sft_v1/faith/live}{100.0}
\defres{drift/sft_v1/faith/lr_ow}{0}
\defres{drift/sft_v1/faith/lw_or}{0}
\defres{drift/sft_v1/faith/n}{360}
\defres{drift/sft_v1/faith/offline}{100.0}
\defres{drift/sft_v1/first/failed}{0}
\defres{drift/sft_v1/first/in_c}{0.0}
\defres{drift/sft_v1/first/in_c/n}{0}
\defres{drift/sft_v1/first/inc_offline_right/n}{0}
\defres{drift/sft_v1/first/inc_same_answer/n}{0}
\defres{drift/sft_v1/first/irreversible}{0.0}
\defres{drift/sft_v1/first/irreversible/n}{0}
\defres{drift/sft_v1/first/none}{100.0}
\defres{drift/sft_v1/first/none/n}{100}
\defres{drift/sft_v1/first/novel}{0.0}
\defres{drift/sft_v1/first/novel/n}{0}
\defres{drift/sft_v1/first/recovered/n}{0}
\defres{drift/sft_v1/first/with_wrong/n}{0}
\defres{drift/sft_v1/gate/05/right_below}{0.0}
\defres{drift/sft_v1/gate/09/right_below}{0.0}
\defres{drift/sft_v1/gate/jev/right_below}{3.6}
\defres{drift/sft_v1/gate/n_wrong}{0}
\defres{drift/sft_v1/gate/right_below}{3.6}
\defres{drift/sft_v1/gate/source}{jev}
\defres{drift/sft_v1/gate/tau}{1.00}
\defres{drift/sft_v1/live/n}{100}
\defres{drift/sft_v1/live/success}{100.0}
\defres{drift/sft_v1/loss/compounding}{0.0}
\defres{drift/sft_v1/loss/irreversible}{0.0}
\defres{drift/sft_v1/loss/no_wrong_choice}{0.0}
\defres{drift/sft_v1/loss/total}{0.0}
\defres{drift/sft_v1/mustask/acc}{100.0}
\defres{drift/sft_v1/mustask/acted}{0.0}
\defres{drift/sft_v1/mustask/acted/n}{0}
\defres{drift/sft_v1/mustask/n}{25}
\defres{drift/sft_v1/mustask/step_median}{2}
\defres{drift/sft_v1/mustask/tasks}{25}
\defres{drift/sft_v1/states/inc_share}{48.0}
\defres{drift/sft_v1/states/n}{750}
\defres{drift/sft_v1/states/novel_offplan_share}{0.0}
\defres{drift/sft_v1/states/novel_onplan_share}{52.0}
\defres{drift/sft_v1/states/novel_share}{52.0}
\defres{drift/sft_v1/states/offplan_share}{0.0}
\defres{drift/sl0.8b/acc/after_off_plan}{2.0}
\defres{drift/sl0.8b/acc/after_off_plan/n}{767}
\defres{drift/sl0.8b/acc/all}{19.8}
\defres{drift/sl0.8b/acc/all/n}{1{,}145}
\defres{drift/sl0.8b/acc/executed_all}{19.8}
\defres{drift/sl0.8b/acc/executed_all/n}{1{,}145}
\defres{drift/sl0.8b/acc/in_c}{52.1}
\defres{drift/sl0.8b/acc/in_c/n}{284}
\defres{drift/sl0.8b/acc/in_c_after_off_plan}{0.0}
\defres{drift/sl0.8b/acc/in_c_after_off_plan/n}{5}
\defres{drift/sl0.8b/acc/in_c_on_plan}{53.0}
\defres{drift/sl0.8b/acc/in_c_on_plan/n}{279}
\defres{drift/sl0.8b/acc/novel}{9.2}
\defres{drift/sl0.8b/acc/novel/n}{861}
\defres{drift/sl0.8b/acc/novel_after_off_plan}{2.0}
\defres{drift/sl0.8b/acc/novel_after_off_plan/n}{762}
\defres{drift/sl0.8b/acc/novel_on_plan}{64.6}
\defres{drift/sl0.8b/acc/novel_on_plan/n}{99}
\defres{drift/sl0.8b/acc/on_plan}{56.1}
\defres{drift/sl0.8b/acc/on_plan/n}{378}
\defres{drift/sl0.8b/ask/acc}{100.0}
\defres{drift/sl0.8b/ask/acted}{0.0}
\defres{drift/sl0.8b/ask/acted/n}{0}
\defres{drift/sl0.8b/ask/n}{75}
\defres{drift/sl0.8b/askearly/share}{12.5}
\defres{drift/sl0.8b/askearly/tasks}{25}
\defres{drift/sl0.8b/c/acc}{48.3}
\defres{drift/sl0.8b/c/ask_acc}{49.4}
\defres{drift/sl0.8b/c/mustask_acc}{25.0}
\defres{drift/sl0.8b/conf/right}{56.7}
\defres{drift/sl0.8b/conf/wrong}{47.9}
\defres{drift/sl0.8b/faith/agree}{100.0}
\defres{drift/sl0.8b/faith/live}{52.1}
\defres{drift/sl0.8b/faith/lr_ow}{0}
\defres{drift/sl0.8b/faith/lw_or}{0}
\defres{drift/sl0.8b/faith/n}{284}
\defres{drift/sl0.8b/faith/offline}{52.1}
\defres{drift/sl0.8b/first/conseq/recoverable/n}{110}
\defres{drift/sl0.8b/first/conseq/recoverable/recovered}{0.9}
\defres{drift/sl0.8b/first/conseq/recoverable/share}{66.3}
\defres{drift/sl0.8b/first/conseq/recoverable/tasks}{55.0}
\defres{drift/sl0.8b/first/conseq/write/n}{56}
\defres{drift/sl0.8b/first/conseq/write/recovered}{0.0}
\defres{drift/sl0.8b/first/conseq/write/share}{33.7}
\defres{drift/sl0.8b/first/conseq/write/tasks}{28.0}
\defres{drift/sl0.8b/first/failed}{165}
\defres{drift/sl0.8b/first/failed_with_wrong}{100.0}
\defres{drift/sl0.8b/first/in_c}{65.5}
\defres{drift/sl0.8b/first/in_c/n}{131}
\defres{drift/sl0.8b/first/inc_offline_right}{0.0}
\defres{drift/sl0.8b/first/inc_offline_right/n}{0}
\defres{drift/sl0.8b/first/inc_same_answer/n}{131}
\defres{drift/sl0.8b/first/irreversible}{28.0}
\defres{drift/sl0.8b/first/irreversible/n}{56}
\defres{drift/sl0.8b/first/irreversible_of_failed}{33.9}
\defres{drift/sl0.8b/first/none}{17.0}
\defres{drift/sl0.8b/first/none/n}{34}
\defres{drift/sl0.8b/first/novel}{17.5}
\defres{drift/sl0.8b/first/novel/n}{35}
\defres{drift/sl0.8b/first/recovered}{0.6}
\defres{drift/sl0.8b/first/recovered/n}{1}
\defres{drift/sl0.8b/first/step_le1}{90.4}
\defres{drift/sl0.8b/first/step_median}{0}
\defres{drift/sl0.8b/first/top_type}{unneeded question}
\defres{drift/sl0.8b/first/top_type/share}{65.7}
\defres{drift/sl0.8b/first/type/lookalike_other/n}{1}
\defres{drift/sl0.8b/first/type/lookalike_other/share}{0.6}
\defres{drift/sl0.8b/first/type/lookalike_other/tasks}{0.5}
\defres{drift/sl0.8b/first/type/unneeded_question/n}{109}
\defres{drift/sl0.8b/first/type/unneeded_question/share}{65.7}
\defres{drift/sl0.8b/first/type/unneeded_question/tasks}{54.5}
\defres{drift/sl0.8b/first/type/wrong_core_tool/n}{56}
\defres{drift/sl0.8b/first/type/wrong_core_tool/share}{33.7}
\defres{drift/sl0.8b/first/type/wrong_core_tool/tasks}{28.0}
\defres{drift/sl0.8b/first/with_wrong/n}{166}
\defres{drift/sl0.8b/gate/05/failed_first_below}{58.2}
\defres{drift/sl0.8b/gate/05/right_below}{33.5}
\defres{drift/sl0.8b/gate/05/wrong_below}{57.1}
\defres{drift/sl0.8b/gate/09/failed_first_below}{100.0}
\defres{drift/sl0.8b/gate/09/right_below}{94.7}
\defres{drift/sl0.8b/gate/09/wrong_below}{100.0}
\defres{drift/sl0.8b/gate/failed_first_below}{100.0}
\defres{drift/sl0.8b/gate/jev/failed_first_below}{100.0}
\defres{drift/sl0.8b/gate/jev/right_below}{100.0}
\defres{drift/sl0.8b/gate/jev/wrong_below}{100.0}
\defres{drift/sl0.8b/gate/n_wrong}{918}
\defres{drift/sl0.8b/gate/right_below}{100.0}
\defres{drift/sl0.8b/gate/source}{jev}
\defres{drift/sl0.8b/gate/tau}{1.00}
\defres{drift/sl0.8b/gate/wrong_below}{100.0}
\defres{drift/sl0.8b/live/n}{200}
\defres{drift/sl0.8b/live/success}{17.5}
\defres{drift/sl0.8b/loss/compounding}{54.5}
\defres{drift/sl0.8b/loss/irreversible}{28.0}
\defres{drift/sl0.8b/loss/no_wrong_choice}{0.0}
\defres{drift/sl0.8b/loss/total}{82.5}
\defres{drift/sl0.8b/mustask/acc}{100.0}
\defres{drift/sl0.8b/mustask/acted}{0.0}
\defres{drift/sl0.8b/mustask/acted/n}{0}
\defres{drift/sl0.8b/mustask/n}{25}
\defres{drift/sl0.8b/mustask/step_median}{0}
\defres{drift/sl0.8b/mustask/tasks}{25}
\defres{drift/sl0.8b/states/inc_share}{24.8}
\defres{drift/sl0.8b/states/n}{1{,}145}
\defres{drift/sl0.8b/states/novel_offplan_share}{66.6}
\defres{drift/sl0.8b/states/novel_onplan_share}{8.6}
\defres{drift/sl0.8b/states/novel_share}{75.2}
\defres{drift/sl0.8b/states/offplan_share}{67.0}
\defres{drift/sl27b/acc/after_off_plan/n}{0}
\defres{drift/sl27b/acc/all}{94.5}
\defres{drift/sl27b/acc/all/n}{1{,}352}
\defres{drift/sl27b/acc/executed_all}{94.5}
\defres{drift/sl27b/acc/executed_all/n}{1{,}352}
\defres{drift/sl27b/acc/in_c}{92.1}
\defres{drift/sl27b/acc/in_c/n}{746}
\defres{drift/sl27b/acc/in_c_after_off_plan/n}{0}
\defres{drift/sl27b/acc/in_c_on_plan}{92.1}
\defres{drift/sl27b/acc/in_c_on_plan/n}{746}
\defres{drift/sl27b/acc/novel}{97.5}
\defres{drift/sl27b/acc/novel/n}{606}
\defres{drift/sl27b/acc/novel_after_off_plan/n}{0}
\defres{drift/sl27b/acc/novel_on_plan}{97.5}
\defres{drift/sl27b/acc/novel_on_plan/n}{606}
\defres{drift/sl27b/acc/on_plan}{94.5}
\defres{drift/sl27b/acc/on_plan/n}{1{,}352}
\defres{drift/sl27b/ask/acc}{63.0}
\defres{drift/sl27b/ask/acted}{37.0}
\defres{drift/sl27b/ask/acted/n}{74}
\defres{drift/sl27b/ask/acted_of_wrong}{100.0}
\defres{drift/sl27b/ask/n}{200}
\defres{drift/sl27b/askearly/share}{0.0}
\defres{drift/sl27b/askearly/tasks}{0}
\defres{drift/sl27b/c/acc}{93.9}
\defres{drift/sl27b/c/ask_acc}{63.4}
\defres{drift/sl27b/c/mustask_acc}{26.0}
\defres{drift/sl27b/conf/right}{98.0}
\defres{drift/sl27b/conf/wrong}{82.1}
\defres{drift/sl27b/faith/agree}{100.0}
\defres{drift/sl27b/faith/live}{92.1}
\defres{drift/sl27b/faith/lr_ow}{0}
\defres{drift/sl27b/faith/lw_or}{0}
\defres{drift/sl27b/faith/n}{746}
\defres{drift/sl27b/faith/offline}{92.1}
\defres{drift/sl27b/first/conseq/write/n}{74}
\defres{drift/sl27b/first/conseq/write/recovered}{0.0}
\defres{drift/sl27b/first/conseq/write/share}{100.0}
\defres{drift/sl27b/first/conseq/write/tasks}{37.0}
\defres{drift/sl27b/first/failed}{74}
\defres{drift/sl27b/first/failed_with_wrong}{100.0}
\defres{drift/sl27b/first/in_c}{29.5}
\defres{drift/sl27b/first/in_c/n}{59}
\defres{drift/sl27b/first/inc_offline_right}{0.0}
\defres{drift/sl27b/first/inc_offline_right/n}{0}
\defres{drift/sl27b/first/inc_same_answer/n}{59}
\defres{drift/sl27b/first/irreversible}{37.0}
\defres{drift/sl27b/first/irreversible/n}{74}
\defres{drift/sl27b/first/irreversible_of_failed}{100.0}
\defres{drift/sl27b/first/none}{63.0}
\defres{drift/sl27b/first/none/n}{126}
\defres{drift/sl27b/first/novel}{7.5}
\defres{drift/sl27b/first/novel/n}{15}
\defres{drift/sl27b/first/recovered}{0.0}
\defres{drift/sl27b/first/recovered/n}{0}
\defres{drift/sl27b/first/step_le1}{0.0}
\defres{drift/sl27b/first/step_median}{2}
\defres{drift/sl27b/first/top_type}{changed state before asking}
\defres{drift/sl27b/first/top_type/share}{100.0}
\defres{drift/sl27b/first/type/act_before_ask/n}{74}
\defres{drift/sl27b/first/type/act_before_ask/share}{100.0}
\defres{drift/sl27b/first/type/act_before_ask/tasks}{37.0}
\defres{drift/sl27b/first/with_wrong/n}{74}
\defres{drift/sl27b/gate/05/failed_first_below}{1.4}
\defres{drift/sl27b/gate/05/right_below}{0.0}
\defres{drift/sl27b/gate/05/wrong_below}{1.4}
\defres{drift/sl27b/gate/09/failed_first_below}{62.2}
\defres{drift/sl27b/gate/09/right_below}{3.4}
\defres{drift/sl27b/gate/09/wrong_below}{62.2}
\defres{drift/sl27b/gate/failed_first_below}{100.0}
\defres{drift/sl27b/gate/jev/failed_first_below}{100.0}
\defres{drift/sl27b/gate/jev/right_below}{100.0}
\defres{drift/sl27b/gate/jev/wrong_below}{100.0}
\defres{drift/sl27b/gate/n_wrong}{74}
\defres{drift/sl27b/gate/right_below}{100.0}
\defres{drift/sl27b/gate/source}{jev}
\defres{drift/sl27b/gate/tau}{1.00}
\defres{drift/sl27b/gate/wrong_below}{100.0}
\defres{drift/sl27b/live/n}{200}
\defres{drift/sl27b/live/success}{63.0}
\defres{drift/sl27b/loss/compounding}{0.0}
\defres{drift/sl27b/loss/irreversible}{37.0}
\defres{drift/sl27b/loss/no_wrong_choice}{0.0}
\defres{drift/sl27b/loss/total}{37.0}
\defres{drift/sl27b/mustask/acc}{26.0}
\defres{drift/sl27b/mustask/acted}{74.0}
\defres{drift/sl27b/mustask/acted/n}{74}
\defres{drift/sl27b/mustask/n}{100}
\defres{drift/sl27b/mustask/step_median}{2}
\defres{drift/sl27b/mustask/tasks}{100}
\defres{drift/sl27b/states/inc_share}{55.2}
\defres{drift/sl27b/states/n}{1{,}352}
\defres{drift/sl27b/states/novel_offplan_share}{0.0}
\defres{drift/sl27b/states/novel_onplan_share}{44.8}
\defres{drift/sl27b/states/novel_share}{44.8}
\defres{drift/sl27b/states/offplan_share}{0.0}
\defres{drift/sl2b/acc/after_off_plan}{14.6}
\defres{drift/sl2b/acc/after_off_plan/n}{144}
\defres{drift/sl2b/acc/all}{58.7}
\defres{drift/sl2b/acc/all/n}{755}
\defres{drift/sl2b/acc/executed_all}{58.7}
\defres{drift/sl2b/acc/executed_all/n}{755}
\defres{drift/sl2b/acc/in_c}{73.9}
\defres{drift/sl2b/acc/in_c/n}{514}
\defres{drift/sl2b/acc/in_c_after_off_plan}{0.0}
\defres{drift/sl2b/acc/in_c_after_off_plan/n}{2}
\defres{drift/sl2b/acc/in_c_on_plan}{74.2}
\defres{drift/sl2b/acc/in_c_on_plan/n}{512}
\defres{drift/sl2b/acc/novel}{26.1}
\defres{drift/sl2b/acc/novel/n}{241}
\defres{drift/sl2b/acc/novel_after_off_plan}{14.8}
\defres{drift/sl2b/acc/novel_after_off_plan/n}{142}
\defres{drift/sl2b/acc/novel_on_plan}{42.4}
\defres{drift/sl2b/acc/novel_on_plan/n}{99}
\defres{drift/sl2b/acc/on_plan}{69.1}
\defres{drift/sl2b/acc/on_plan/n}{611}
\defres{drift/sl2b/ask/acc}{66.1}
\defres{drift/sl2b/ask/acted}{30.5}
\defres{drift/sl2b/ask/acted/n}{54}
\defres{drift/sl2b/ask/acted_of_wrong}{90.0}
\defres{drift/sl2b/ask/n}{177}
\defres{drift/sl2b/askearly/share}{1.0}
\defres{drift/sl2b/askearly/tasks}{2}
\defres{drift/sl2b/c/acc}{68.4}
\defres{drift/sl2b/c/ask_acc}{61.8}
\defres{drift/sl2b/c/mustask_acc}{27.0}
\defres{drift/sl2b/conf/right}{58.0}
\defres{drift/sl2b/conf/wrong}{57.1}
\defres{drift/sl2b/faith/agree}{100.0}
\defres{drift/sl2b/faith/live}{73.9}
\defres{drift/sl2b/faith/lr_ow}{0}
\defres{drift/sl2b/faith/lw_or}{0}
\defres{drift/sl2b/faith/n}{514}
\defres{drift/sl2b/faith/offline}{73.9}
\defres{drift/sl2b/first/conseq/recoverable/n}{23}
\defres{drift/sl2b/first/conseq/recoverable/recovered}{8.7}
\defres{drift/sl2b/first/conseq/recoverable/share}{12.2}
\defres{drift/sl2b/first/conseq/recoverable/tasks}{11.5}
\defres{drift/sl2b/first/conseq/write/n}{166}
\defres{drift/sl2b/first/conseq/write/recovered}{0.0}
\defres{drift/sl2b/first/conseq/write/share}{87.8}
\defres{drift/sl2b/first/conseq/write/tasks}{83.0}
\defres{drift/sl2b/first/failed}{187}
\defres{drift/sl2b/first/failed_with_wrong}{100.0}
\defres{drift/sl2b/first/in_c}{66.0}
\defres{drift/sl2b/first/in_c/n}{132}
\defres{drift/sl2b/first/inc_offline_right}{0.0}
\defres{drift/sl2b/first/inc_offline_right/n}{0}
\defres{drift/sl2b/first/inc_same_answer/n}{132}
\defres{drift/sl2b/first/irreversible}{83.0}
\defres{drift/sl2b/first/irreversible/n}{166}
\defres{drift/sl2b/first/irreversible_of_failed}{88.8}
\defres{drift/sl2b/first/none}{5.5}
\defres{drift/sl2b/first/none/n}{11}
\defres{drift/sl2b/first/novel}{28.5}
\defres{drift/sl2b/first/novel/n}{57}
\defres{drift/sl2b/first/recovered}{1.1}
\defres{drift/sl2b/first/recovered/n}{2}
\defres{drift/sl2b/first/step_le1}{32.8}
\defres{drift/sl2b/first/step_median}{2}
\defres{drift/sl2b/first/top_type}{wrong core tool}
\defres{drift/sl2b/first/top_type/share}{65.6}
\defres{drift/sl2b/first/type/act_before_ask/n}{58}
\defres{drift/sl2b/first/type/act_before_ask/share}{30.7}
\defres{drift/sl2b/first/type/act_before_ask/tasks}{29.0}
\defres{drift/sl2b/first/type/lookalike_gold/n}{4}
\defres{drift/sl2b/first/type/lookalike_gold/share}{2.1}
\defres{drift/sl2b/first/type/lookalike_gold/tasks}{2.0}
\defres{drift/sl2b/first/type/unneeded_question/n}{3}
\defres{drift/sl2b/first/type/unneeded_question/share}{1.6}
\defres{drift/sl2b/first/type/unneeded_question/tasks}{1.5}
\defres{drift/sl2b/first/type/wrong_core_tool/n}{124}
\defres{drift/sl2b/first/type/wrong_core_tool/share}{65.6}
\defres{drift/sl2b/first/type/wrong_core_tool/tasks}{62.0}
\defres{drift/sl2b/first/with_wrong/n}{189}
\defres{drift/sl2b/gate/05/failed_first_below}{29.9}
\defres{drift/sl2b/gate/05/right_below}{41.3}
\defres{drift/sl2b/gate/05/wrong_below}{41.3}
\defres{drift/sl2b/gate/09/failed_first_below}{96.3}
\defres{drift/sl2b/gate/09/right_below}{88.9}
\defres{drift/sl2b/gate/09/wrong_below}{97.8}
\defres{drift/sl2b/gate/failed_first_below}{100.0}
\defres{drift/sl2b/gate/jev/failed_first_below}{100.0}
\defres{drift/sl2b/gate/jev/right_below}{100.0}
\defres{drift/sl2b/gate/jev/wrong_below}{100.0}
\defres{drift/sl2b/gate/n_wrong}{312}
\defres{drift/sl2b/gate/right_below}{100.0}
\defres{drift/sl2b/gate/source}{jev}
\defres{drift/sl2b/gate/tau}{1.00}
\defres{drift/sl2b/gate/wrong_below}{100.0}
\defres{drift/sl2b/live/n}{200}
\defres{drift/sl2b/live/success}{6.5}
\defres{drift/sl2b/loss/compounding}{10.5}
\defres{drift/sl2b/loss/irreversible}{83.0}
\defres{drift/sl2b/loss/no_wrong_choice}{0.0}
\defres{drift/sl2b/loss/total}{93.5}
\defres{drift/sl2b/mustask/acc}{33.3}
\defres{drift/sl2b/mustask/acted}{66.7}
\defres{drift/sl2b/mustask/acted/n}{52}
\defres{drift/sl2b/mustask/n}{78}
\defres{drift/sl2b/mustask/step_median}{2}
\defres{drift/sl2b/mustask/tasks}{78}
\defres{drift/sl2b/states/inc_share}{68.1}
\defres{drift/sl2b/states/n}{755}
\defres{drift/sl2b/states/novel_offplan_share}{18.8}
\defres{drift/sl2b/states/novel_onplan_share}{13.1}
\defres{drift/sl2b/states/novel_share}{31.9}
\defres{drift/sl2b/states/offplan_share}{19.1}
\defres{drift/sl4b/acc/after_off_plan}{66.7}
\defres{drift/sl4b/acc/after_off_plan/n}{30}
\defres{drift/sl4b/acc/all}{92.4}
\defres{drift/sl4b/acc/all/n}{1{,}232}
\defres{drift/sl4b/acc/executed_all}{92.4}
\defres{drift/sl4b/acc/executed_all/n}{1{,}232}
\defres{drift/sl4b/acc/in_c}{89.0}
\defres{drift/sl4b/acc/in_c/n}{683}
\defres{drift/sl4b/acc/in_c_after_off_plan/n}{0}
\defres{drift/sl4b/acc/in_c_on_plan}{89.0}
\defres{drift/sl4b/acc/in_c_on_plan/n}{683}
\defres{drift/sl4b/acc/novel}{96.5}
\defres{drift/sl4b/acc/novel/n}{549}
\defres{drift/sl4b/acc/novel_after_off_plan}{66.7}
\defres{drift/sl4b/acc/novel_after_off_plan/n}{30}
\defres{drift/sl4b/acc/novel_on_plan}{98.3}
\defres{drift/sl4b/acc/novel_on_plan/n}{519}
\defres{drift/sl4b/acc/on_plan}{93.0}
\defres{drift/sl4b/acc/on_plan/n}{1{,}202}
\defres{drift/sl4b/ask/acc}{72.1}
\defres{drift/sl4b/ask/acted}{27.9}
\defres{drift/sl4b/ask/acted/n}{53}
\defres{drift/sl4b/ask/acted_of_wrong}{100.0}
\defres{drift/sl4b/ask/n}{190}
\defres{drift/sl4b/askearly/share}{0.0}
\defres{drift/sl4b/askearly/tasks}{0}
\defres{drift/sl4b/c/acc}{89.1}
\defres{drift/sl4b/c/ask_acc}{84.1}
\defres{drift/sl4b/c/mustask_acc}{47.0}
\defres{drift/sl4b/conf/right}{86.8}
\defres{drift/sl4b/conf/wrong}{64.0}
\defres{drift/sl4b/faith/agree}{100.0}
\defres{drift/sl4b/faith/live}{89.0}
\defres{drift/sl4b/faith/lr_ow}{0}
\defres{drift/sl4b/faith/lw_or}{0}
\defres{drift/sl4b/faith/n}{683}
\defres{drift/sl4b/faith/offline}{89.0}
\defres{drift/sl4b/first/conseq/recoverable/n}{14}
\defres{drift/sl4b/first/conseq/recoverable/recovered}{28.6}
\defres{drift/sl4b/first/conseq/recoverable/share}{16.7}
\defres{drift/sl4b/first/conseq/recoverable/tasks}{7.0}
\defres{drift/sl4b/first/conseq/write/n}{70}
\defres{drift/sl4b/first/conseq/write/recovered}{0.0}
\defres{drift/sl4b/first/conseq/write/share}{83.3}
\defres{drift/sl4b/first/conseq/write/tasks}{35.0}
\defres{drift/sl4b/first/failed}{80}
\defres{drift/sl4b/first/failed_with_wrong}{100.0}
\defres{drift/sl4b/first/in_c}{37.5}
\defres{drift/sl4b/first/in_c/n}{75}
\defres{drift/sl4b/first/inc_offline_right}{0.0}
\defres{drift/sl4b/first/inc_offline_right/n}{0}
\defres{drift/sl4b/first/inc_same_answer/n}{75}
\defres{drift/sl4b/first/irreversible}{35.0}
\defres{drift/sl4b/first/irreversible/n}{70}
\defres{drift/sl4b/first/irreversible_of_failed}{87.5}
\defres{drift/sl4b/first/none}{58.0}
\defres{drift/sl4b/first/none/n}{116}
\defres{drift/sl4b/first/novel}{4.5}
\defres{drift/sl4b/first/novel/n}{9}
\defres{drift/sl4b/first/recovered}{4.8}
\defres{drift/sl4b/first/recovered/n}{4}
\defres{drift/sl4b/first/step_le1}{36.9}
\defres{drift/sl4b/first/step_median}{2}
\defres{drift/sl4b/first/top_type}{changed state before asking}
\defres{drift/sl4b/first/top_type/share}{63.1}
\defres{drift/sl4b/first/type/act_before_ask/n}{53}
\defres{drift/sl4b/first/type/act_before_ask/share}{63.1}
\defres{drift/sl4b/first/type/act_before_ask/tasks}{26.5}
\defres{drift/sl4b/first/type/wrong_core_tool/n}{31}
\defres{drift/sl4b/first/type/wrong_core_tool/share}{36.9}
\defres{drift/sl4b/first/type/wrong_core_tool/tasks}{15.5}
\defres{drift/sl4b/first/with_wrong/n}{84}
\defres{drift/sl4b/gate/05/failed_first_below}{26.2}
\defres{drift/sl4b/gate/05/right_below}{2.3}
\defres{drift/sl4b/gate/05/wrong_below}{34.0}
\defres{drift/sl4b/gate/09/failed_first_below}{68.8}
\defres{drift/sl4b/gate/09/right_below}{43.1}
\defres{drift/sl4b/gate/09/wrong_below}{73.4}
\defres{drift/sl4b/gate/failed_first_below}{100.0}
\defres{drift/sl4b/gate/jev/failed_first_below}{100.0}
\defres{drift/sl4b/gate/jev/right_below}{100.0}
\defres{drift/sl4b/gate/jev/wrong_below}{100.0}
\defres{drift/sl4b/gate/n_wrong}{94}
\defres{drift/sl4b/gate/own/failed_first_below}{100.0}
\defres{drift/sl4b/gate/own/right_below}{75.3}
\defres{drift/sl4b/gate/own/wrong_below}{100.0}
\defres{drift/sl4b/gate/right_below}{75.3}
\defres{drift/sl4b/gate/source}{own}
\defres{drift/sl4b/gate/tau}{0.9756}
\defres{drift/sl4b/gate/wrong_below}{100.0}
\defres{drift/sl4b/live/n}{200}
\defres{drift/sl4b/live/success}{60.0}
\defres{drift/sl4b/loss/compounding}{5.0}
\defres{drift/sl4b/loss/irreversible}{35.0}
\defres{drift/sl4b/loss/no_wrong_choice}{0.0}
\defres{drift/sl4b/loss/total}{40.0}
\defres{drift/sl4b/mustask/acc}{41.1}
\defres{drift/sl4b/mustask/acted}{58.9}
\defres{drift/sl4b/mustask/acted/n}{53}
\defres{drift/sl4b/mustask/n}{90}
\defres{drift/sl4b/mustask/step_median}{2}
\defres{drift/sl4b/mustask/tasks}{90}
\defres{drift/sl4b/states/inc_share}{55.4}
\defres{drift/sl4b/states/n}{1{,}232}
\defres{drift/sl4b/states/novel_offplan_share}{2.4}
\defres{drift/sl4b/states/novel_onplan_share}{42.1}
\defres{drift/sl4b/states/novel_share}{44.6}
\defres{drift/sl4b/states/offplan_share}{2.4}
\defres{drift/sl9b/acc/after_off_plan}{0.0}
\defres{drift/sl9b/acc/after_off_plan/n}{25}
\defres{drift/sl9b/acc/all}{94.6}
\defres{drift/sl9b/acc/all/n}{1{,}416}
\defres{drift/sl9b/acc/executed_all}{94.6}
\defres{drift/sl9b/acc/executed_all/n}{1{,}416}
\defres{drift/sl9b/acc/in_c}{94.7}
\defres{drift/sl9b/acc/in_c/n}{739}
\defres{drift/sl9b/acc/in_c_after_off_plan/n}{0}
\defres{drift/sl9b/acc/in_c_on_plan}{94.7}
\defres{drift/sl9b/acc/in_c_on_plan/n}{739}
\defres{drift/sl9b/acc/novel}{94.4}
\defres{drift/sl9b/acc/novel/n}{677}
\defres{drift/sl9b/acc/novel_after_off_plan}{0.0}
\defres{drift/sl9b/acc/novel_after_off_plan/n}{25}
\defres{drift/sl9b/acc/novel_on_plan}{98.0}
\defres{drift/sl9b/acc/novel_on_plan/n}{652}
\defres{drift/sl9b/acc/on_plan}{96.3}
\defres{drift/sl9b/acc/on_plan/n}{1{,}391}
\defres{drift/sl9b/ask/acc}{75.0}
\defres{drift/sl9b/ask/acted}{25.0}
\defres{drift/sl9b/ask/acted/n}{50}
\defres{drift/sl9b/ask/acted_of_wrong}{100.0}
\defres{drift/sl9b/ask/n}{200}
\defres{drift/sl9b/askearly/share}{0.0}
\defres{drift/sl9b/askearly/tasks}{0}
\defres{drift/sl9b/c/acc}{91.8}
\defres{drift/sl9b/c/ask_acc}{87.1}
\defres{drift/sl9b/c/mustask_acc}{50.0}
\defres{drift/sl9b/conf/right}{90.6}
\defres{drift/sl9b/conf/wrong}{69.8}
\defres{drift/sl9b/faith/agree}{100.0}
\defres{drift/sl9b/faith/live}{94.7}
\defres{drift/sl9b/faith/lr_ow}{0}
\defres{drift/sl9b/faith/lw_or}{0}
\defres{drift/sl9b/faith/n}{739}
\defres{drift/sl9b/faith/offline}{94.7}
\defres{drift/sl9b/first/conseq/recoverable/n}{1}
\defres{drift/sl9b/first/conseq/recoverable/recovered}{0.0}
\defres{drift/sl9b/first/conseq/recoverable/share}{1.9}
\defres{drift/sl9b/first/conseq/recoverable/tasks}{0.5}
\defres{drift/sl9b/first/conseq/write/n}{51}
\defres{drift/sl9b/first/conseq/write/recovered}{0.0}
\defres{drift/sl9b/first/conseq/write/share}{98.1}
\defres{drift/sl9b/first/conseq/write/tasks}{25.5}
\defres{drift/sl9b/first/failed}{52}
\defres{drift/sl9b/first/failed_with_wrong}{100.0}
\defres{drift/sl9b/first/in_c}{19.5}
\defres{drift/sl9b/first/in_c/n}{39}
\defres{drift/sl9b/first/inc_offline_right}{0.0}
\defres{drift/sl9b/first/inc_offline_right/n}{0}
\defres{drift/sl9b/first/inc_same_answer/n}{39}
\defres{drift/sl9b/first/irreversible}{25.5}
\defres{drift/sl9b/first/irreversible/n}{51}
\defres{drift/sl9b/first/irreversible_of_failed}{98.1}
\defres{drift/sl9b/first/none}{74.0}
\defres{drift/sl9b/first/none/n}{148}
\defres{drift/sl9b/first/novel}{6.5}
\defres{drift/sl9b/first/novel/n}{13}
\defres{drift/sl9b/first/recovered}{0.0}
\defres{drift/sl9b/first/recovered/n}{0}
\defres{drift/sl9b/first/step_le1}{1.9}
\defres{drift/sl9b/first/step_median}{2}
\defres{drift/sl9b/first/top_type}{changed state before asking}
\defres{drift/sl9b/first/top_type/share}{96.2}
\defres{drift/sl9b/first/type/act_before_ask/n}{50}
\defres{drift/sl9b/first/type/act_before_ask/share}{96.2}
\defres{drift/sl9b/first/type/act_before_ask/tasks}{25.0}
\defres{drift/sl9b/first/type/unneeded_question/n}{1}
\defres{drift/sl9b/first/type/unneeded_question/share}{1.9}
\defres{drift/sl9b/first/type/unneeded_question/tasks}{0.5}
\defres{drift/sl9b/first/type/wrong_core_tool/n}{1}
\defres{drift/sl9b/first/type/wrong_core_tool/share}{1.9}
\defres{drift/sl9b/first/type/wrong_core_tool/tasks}{0.5}
\defres{drift/sl9b/first/with_wrong/n}{52}
\defres{drift/sl9b/gate/05/failed_first_below}{7.7}
\defres{drift/sl9b/gate/05/right_below}{0.2}
\defres{drift/sl9b/gate/05/wrong_below}{13.0}
\defres{drift/sl9b/gate/09/failed_first_below}{75.0}
\defres{drift/sl9b/gate/09/right_below}{35.1}
\defres{drift/sl9b/gate/09/wrong_below}{83.1}
\defres{drift/sl9b/gate/failed_first_below}{100.0}
\defres{drift/sl9b/gate/jev/failed_first_below}{100.0}
\defres{drift/sl9b/gate/jev/right_below}{100.0}
\defres{drift/sl9b/gate/jev/wrong_below}{100.0}
\defres{drift/sl9b/gate/n_wrong}{77}
\defres{drift/sl9b/gate/right_below}{100.0}
\defres{drift/sl9b/gate/source}{jev}
\defres{drift/sl9b/gate/tau}{1.00}
\defres{drift/sl9b/gate/wrong_below}{100.0}
\defres{drift/sl9b/live/n}{200}
\defres{drift/sl9b/live/success}{74.0}
\defres{drift/sl9b/loss/compounding}{0.5}
\defres{drift/sl9b/loss/irreversible}{25.5}
\defres{drift/sl9b/loss/no_wrong_choice}{0.0}
\defres{drift/sl9b/loss/total}{26.0}
\defres{drift/sl9b/mustask/acc}{50.0}
\defres{drift/sl9b/mustask/acted}{50.0}
\defres{drift/sl9b/mustask/acted/n}{50}
\defres{drift/sl9b/mustask/n}{100}
\defres{drift/sl9b/mustask/step_median}{2}
\defres{drift/sl9b/mustask/tasks}{100}
\defres{drift/sl9b/states/inc_share}{52.2}
\defres{drift/sl9b/states/n}{1{,}416}
\defres{drift/sl9b/states/novel_offplan_share}{1.8}
\defres{drift/sl9b/states/novel_onplan_share}{46.0}
\defres{drift/sl9b/states/novel_share}{47.8}
\defres{drift/sl9b/states/offplan_share}{1.8}
\defres{drift/v2/acc/after_off_plan/n}{0}
\defres{drift/v2/acc/all}{100.0}
\defres{drift/v2/acc/all/n}{1{,}500}
\defres{drift/v2/acc/executed_all}{100.0}
\defres{drift/v2/acc/executed_all/n}{1{,}500}
\defres{drift/v2/acc/in_c}{100.0}
\defres{drift/v2/acc/in_c/n}{746}
\defres{drift/v2/acc/in_c_after_off_plan/n}{0}
\defres{drift/v2/acc/in_c_on_plan}{100.0}
\defres{drift/v2/acc/in_c_on_plan/n}{746}
\defres{drift/v2/acc/novel}{100.0}
\defres{drift/v2/acc/novel/n}{754}
\defres{drift/v2/acc/novel_after_off_plan/n}{0}
\defres{drift/v2/acc/novel_on_plan}{100.0}
\defres{drift/v2/acc/novel_on_plan/n}{754}
\defres{drift/v2/acc/on_plan}{100.0}
\defres{drift/v2/acc/on_plan/n}{1{,}500}
\defres{drift/v2/ask/acc}{100.0}
\defres{drift/v2/ask/acted}{0.0}
\defres{drift/v2/ask/acted/n}{0}
\defres{drift/v2/ask/n}{100}
\defres{drift/v2/askearly/share}{0.0}
\defres{drift/v2/askearly/tasks}{0}
\defres{drift/v2/c/acc}{99.4}
\defres{drift/v2/c/ask_acc}{100.0}
\defres{drift/v2/c/mustask_acc}{100.0}
\defres{drift/v2/conf/right}{100.0}
\defres{drift/v2/faith/agree}{100.0}
\defres{drift/v2/faith/live}{100.0}
\defres{drift/v2/faith/lr_ow}{0}
\defres{drift/v2/faith/lw_or}{0}
\defres{drift/v2/faith/n}{746}
\defres{drift/v2/faith/offline}{100.0}
\defres{drift/v2/first/failed}{0}
\defres{drift/v2/first/in_c}{0.0}
\defres{drift/v2/first/in_c/n}{0}
\defres{drift/v2/first/inc_offline_right/n}{0}
\defres{drift/v2/first/inc_same_answer/n}{0}
\defres{drift/v2/first/irreversible}{0.0}
\defres{drift/v2/first/irreversible/n}{0}
\defres{drift/v2/first/none}{100.0}
\defres{drift/v2/first/none/n}{200}
\defres{drift/v2/first/novel}{0.0}
\defres{drift/v2/first/novel/n}{0}
\defres{drift/v2/first/recovered/n}{0}
\defres{drift/v2/first/with_wrong/n}{0}
\defres{drift/v2/gate/05/right_below}{0.0}
\defres{drift/v2/gate/09/right_below}{0.0}
\defres{drift/v2/gate/jev/right_below}{100.0}
\defres{drift/v2/gate/n_wrong}{0}
\defres{drift/v2/gate/own/right_below}{1.7}
\defres{drift/v2/gate/right_below}{1.7}
\defres{drift/v2/gate/source}{own}
\defres{drift/v2/gate/tau}{0.9987}
\defres{drift/v2/live/n}{200}
\defres{drift/v2/live/success}{100.0}
\defres{drift/v2/loss/compounding}{0.0}
\defres{drift/v2/loss/irreversible}{0.0}
\defres{drift/v2/loss/no_wrong_choice}{0.0}
\defres{drift/v2/loss/total}{0.0}
\defres{drift/v2/mustask/acc}{100.0}
\defres{drift/v2/mustask/acted}{0.0}
\defres{drift/v2/mustask/acted/n}{0}
\defres{drift/v2/mustask/n}{50}
\defres{drift/v2/mustask/step_median}{1}
\defres{drift/v2/mustask/tasks}{50}
\defres{drift/v2/states/inc_share}{49.7}
\defres{drift/v2/states/n}{1{,}500}
\defres{drift/v2/states/novel_offplan_share}{0.0}
\defres{drift/v2/states/novel_onplan_share}{50.3}
\defres{drift/v2/states/novel_share}{50.3}
\defres{drift/v2/states/offplan_share}{0.0}
\makeatother


==> generated/e11_alfworld.tex <==
\makeatletter
\providecommand{\res}[1]{\ifcsname jevres@#1\endcsname\csname jevres@#1\endcsname\else\tbd\fi}
\providecommand{\defres}[2]{\expandafter\def\csname jevres@#1\endcsname{#2}}
\defres{e11/cal/flash_acc}{40.5}
\defres{e11/cal/model_acc}{71.0}
\defres{e11/cal_games}{48}
\defres{e11/cal_paired}{711}
\defres{e11/cascade/acc}{64.6}
\defres{e11/cascade/cost_k}{0.0}
\defres{e11/cascade/coverage}{100.0}
\defres{e11/cascade/delta}{+4.3}
\defres{e11/cascade/delta_ci/hi}{+10.7}
\defres{e11/cascade/delta_ci/lo}{-2.1}
\defres{e11/cascade/llm_calls}{0.0}
\defres{e11/cascade/losses}{7}
\defres{e11/cascade/n}{140}
\defres{e11/cascade/saving}{89.0}
\defres{e11/cascade/saving_api}{100.0}
\defres{e11/cascade/saving_ci/hi}{91.4}
\defres{e11/cascade/saving_ci/lo}{85.6}
\defres{e11/cascade/saving_q_s2_4}{89.9}
\defres{e11/cascade/saving_q_zero}{100.0}
\defres{e11/cascade/status}{run}
\defres{e11/cascade/steps}{12.1}
\defres{e11/cascade/success}{95.0}
\defres{e11/cascade/wall_mean}{18.2}
\defres{e11/cascade/wall_median}{13.7}
\defres{e11/cascade/wins}{13}
\defres{e11/data/dev_rows}{965}
\defres{e11/data/fallback_dropped}{1{,}742}
\defres{e11/data/flash_games}{360}
\defres{e11/data/off_plan_share}{78.1}
\defres{e11/data/scripted_games}{600}
\defres{e11/data/train_games}{540}
\defres{e11/data/train_rows}{9{,}159}
\defres{e11/label}{exploratory (E11)}
\defres{e11/llm_only/cost_k}{19.4}
\defres{e11/llm_only/llm_acc}{46.4}
\defres{e11/llm_only/n}{140}
\defres{e11/llm_only/steps}{13.1}
\defres{e11/llm_only/success}{90.7}
\defres{e11/llm_only/wall_mean}{37.0}
\defres{e11/llm_only/wall_median}{25.4}
\defres{e11/n_games}{140}
\defres{e11/offline/base/dev/acc}{45.4}
\defres{e11/offline/base/dev/ece}{0.516}
\defres{e11/offline/base/dev_flash/acc}{39.0}
\defres{e11/offline/base/dev_flash/ece}{0.576}
\defres{e11/offline/base/dev_off_plan/acc}{46.2}
\defres{e11/offline/base/dev_off_plan/ece}{0.504}
\defres{e11/offline/trained/dev/acc}{84.7}
\defres{e11/offline/trained/dev/ece}{0.026}
\defres{e11/offline/trained/dev_flash/acc}{81.5}
\defres{e11/offline/trained/dev_flash/ece}{0.047}
\defres{e11/offline/trained/dev_off_plan/acc}{88.1}
\defres{e11/offline/trained/dev_off_plan/ece}{0.029}
\defres{e11/replace/acc}{64.7}
\defres{e11/replace/cost_k}{0.0}
\defres{e11/replace/coverage}{100.0}
\defres{e11/replace/delta}{+5.0}
\defres{e11/replace/delta_ci/hi}{+11.4}
\defres{e11/replace/delta_ci/lo}{-0.7}
\defres{e11/replace/llm_calls}{0.0}
\defres{e11/replace/losses}{6}
\defres{e11/replace/n}{140}
\defres{e11/replace/saving}{89.0}
\defres{e11/replace/saving_api}{100.0}
\defres{e11/replace/saving_ci/hi}{91.4}
\defres{e11/replace/saving_ci/lo}{85.6}
\defres{e11/replace/saving_q_s2_4}{89.9}
\defres{e11/replace/saving_q_zero}{100.0}
\defres{e11/replace/status}{run}
\defres{e11/replace/steps}{12.1}
\defres{e11/replace/success}{95.7}
\defres{e11/replace/wall_mean}{17.9}
\defres{e11/replace/wall_median}{14.5}
\defres{e11/replace/wins}{13}
\defres{e11/spend/gemini}{11.61}
\defres{e11/tariff/host_usd_h}{1.624}
\defres{e11/tariff/q}{0.00213}
\defres{e11/tau}{0.12}
\defres{e11/train/minutes}{158}
\defres{e11/trained/acc}{64.6}
\defres{e11/trained/cost_k}{0.0}
\defres{e11/trained/coverage}{100.0}
\defres{e11/trained/delta}{+4.3}
\defres{e11/trained/delta_ci/hi}{+10.7}
\defres{e11/trained/delta_ci/lo}{-2.1}
\defres{e11/trained/llm_calls}{0.0}
\defres{e11/trained/losses}{7}
\defres{e11/trained/n}{140}
\defres{e11/trained/saving}{89.0}
\defres{e11/trained/saving_api}{100.0}
\defres{e11/trained/saving_ci/hi}{91.4}
\defres{e11/trained/saving_ci/lo}{85.6}
\defres{e11/trained/saving_q_s2_4}{89.9}
\defres{e11/trained/saving_q_zero}{100.0}
\defres{e11/trained/status}{run}
\defres{e11/trained/steps}{12.1}
\defres{e11/trained/success}{95.0}
\defres{e11/trained/wall_mean}{18.2}
\defres{e11/trained/wall_median}{13.7}
\defres{e11/trained/wins}{13}
\makeatother


==> generated/e12_train.tex <==
\makeatletter
\providecommand{\res}[1]{\ifcsname jevres@#1\endcsname\csname jevres@#1\endcsname\else\tbd\fi}
\providecommand{\defres}[2]{\expandafter\def\csname jevres@#1\endcsname{#2}}
\defres{e12/audit/e1/exact}{0}
\defres{e12/audit/e1/ngram}{175}
\defres{e12/audit/e1dev/exact}{0}
\defres{e12/audit/e1dev/ngram}{14}
\defres{e12/audit/items}{485}
\defres{e12/audit/publictestpools/exact}{2}
\defres{e12/audit/publictestpools/ngram}{205}
\defres{e12/audit/units}{207}
\defres{e12/audit/unitsall}{19{,}909}
\defres{e12/c/delta}{-0.1}
\defres{e12/c/delta/hi}{+0.1}
\defres{e12/c/delta/lo}{-0.3}
\defres{e12/c/n}{5{,}314}
\defres{e12/c/ni}{yes}
\defres{e12/c/offplan/delta}{-3.1}
\defres{e12/c/offplan/hi}{-0.1}
\defres{e12/c/offplan/lo}{-7.4}
\defres{e12/data/bfclargs}{2{,}000}
\defres{e12/data/bfclnone}{500}
\defres{e12/data/bfcltool}{1{,}500}
\defres{e12/data/dev}{1{,}000}
\defres{e12/data/new}{7{,}000}
\defres{e12/data/replay}{7{,}000}
\defres{e12/data/total}{14{,}000}
\defres{e12/data/w2cask}{1{,}000}
\defres{e12/data/w2ccall}{1{,}000}
\defres{e12/data/w2ccannot}{1{,}000}
\defres{e12/e1/delta/all}{+6.3}
\defres{e12/e1/delta/all/hi}{+7.5}
\defres{e12/e1/delta/all/lo}{+5.1}
\defres{e12/e1/delta/args}{+5.5}
\defres{e12/e1/delta/args/hi}{+7.0}
\defres{e12/e1/delta/args/lo}{+3.9}
\defres{e12/e1/delta/toolchoice}{+0.9}
\defres{e12/e1/delta/toolchoice/hi}{+2.7}
\defres{e12/e1/delta/toolchoice/lo}{-0.9}
\defres{e12/e1/delta/w2c}{+14.5}
\defres{e12/e1/delta/w2c/hi}{+17.9}
\defres{e12/e1/delta/w2c/lo}{+11.2}
\defres{e12/e12/c/acc}{99.1}
\defres{e12/e12/c/ask}{99.9}
\defres{e12/e12/c/offplan}{91.7}
\defres{e12/e12/e1/acc}{85.1}
\defres{e12/e12/e1/acc/args}{90.5}
\defres{e12/e12/e1/acc/toolchoice}{89.3}
\defres{e12/e12/e1/acc/w2c}{68.5}
\defres{e12/e12/e1/usdk}{0.1397}
\defres{e12/e12/e1/usdkadj}{0.0914}
\defres{e12/e12/e1/w2c/askt}{74.8}
\defres{e12/e12/e1/w2c/call}{59.6}
\defres{e12/e12/e1/w2c/sayi}{72.4}
\defres{e12/e12/live/n}{200}
\defres{e12/e12/live/own}{100.0}
\defres{e12/e12/live/success}{100.0}
\defres{e12/e12/live/usdep}{0.0145}
\defres{e12/e12/pubdev/devargs/acc}{96.0}
\defres{e12/e12/pubdev/devtool/acc}{97.7}
\defres{e12/e12/pubdev/devw2c/acc}{96.7}
\defres{e12/e12/v1/dev/acc}{99.7}
\defres{e12/e12/v1/devknockout/acc}{99.8}
\defres{e12/e12/v1/devrecovery/acc}{99.8}
\defres{e12/fast/e12/agree}{99.6}
\defres{e12/fast/e12/c1/msdec}{28.8}
\defres{e12/fast/e12/c1/p50}{40}
\defres{e12/fast/e12/c1/usdkwall}{0.0180}
\defres{e12/fast/e12/c4/msdec}{23.8}
\defres{e12/fast/e12/c4/p50}{186}
\defres{e12/fast/e12/c4/usdkwall}{0.0148}
\defres{e12/fast/e12/gb}{8.0}
\defres{e12/fast/e12/msdec}{23.8}
\defres{e12/fast/e12/usdke9}{0.0592}
\defres{e12/fast/e12/usdkserved}{0.1397}
\defres{e12/fast/e12/usdkwall}{0.0148}
\defres{e12/fast/e12c/agree}{99.8}
\defres{e12/fast/e12c/c1/msdec}{46.2}
\defres{e12/fast/e12c/c1/p50}{79}
\defres{e12/fast/e12c/c1/usdkwall}{0.0288}
\defres{e12/fast/e12c/c4/msdec}{39.5}
\defres{e12/fast/e12c/c4/p50}{306}
\defres{e12/fast/e12c/c4/usdkwall}{0.0246}
\defres{e12/fast/e12c/gb}{8.4}
\defres{e12/fast/e12c/msdec}{39.5}
\defres{e12/fast/e12c/usdke9}{0.0983}
\defres{e12/fast/e12c/usdkserved}{0.2946}
\defres{e12/fast/e12c/usdkwall}{0.0246}
\defres{e12/fast/frozen/agree}{99.8}
\defres{e12/fast/frozen/c1/msdec}{28.8}
\defres{e12/fast/frozen/c1/p50}{40}
\defres{e12/fast/frozen/c1/usdkwall}{0.0180}
\defres{e12/fast/frozen/c4/msdec}{23.7}
\defres{e12/fast/frozen/c4/p50}{184}
\defres{e12/fast/frozen/c4/usdkwall}{0.0147}
\defres{e12/fast/frozen/gb}{8.0}
\defres{e12/fast/frozen/msdec}{23.7}
\defres{e12/fast/frozen/usdke9}{0.0589}
\defres{e12/fast/frozen/usdkserved}{0.0934}
\defres{e12/fast/frozen/usdkwall}{0.0147}
\defres{e12/fast/startlux4b/agree}{96.3}
\defres{e12/fast/startlux4b/c1/msdec}{46.9}
\defres{e12/fast/startlux4b/c1/p50}{79}
\defres{e12/fast/startlux4b/c1/usdkwall}{0.0292}
\defres{e12/fast/startlux4b/c4/msdec}{39.8}
\defres{e12/fast/startlux4b/c4/p50}{310}
\defres{e12/fast/startlux4b/c4/usdkwall}{0.0248}
\defres{e12/fast/startlux4b/gb}{9.3}
\defres{e12/fast/startlux4b/msdec}{39.8}
\defres{e12/fast/startlux4b/usdke9}{0.0990}
\defres{e12/fast/startlux4b/usdkserved}{0.0524}
\defres{e12/fast/startlux4b/usdkwall}{0.0248}
\defres{e12/front}{no}
\defres{e12/front/changed}{no}
\defres{e12/front/hostadj}{no}
\defres{e12/frozen/c/acc}{99.2}
\defres{e12/frozen/c/ask}{100.0}
\defres{e12/frozen/c/offplan}{94.7}
\defres{e12/frozen/e1/acc}{78.8}
\defres{e12/frozen/e1/acc/args}{85.0}
\defres{e12/frozen/e1/acc/toolchoice}{88.4}
\defres{e12/frozen/e1/acc/w2c}{54.0}
\defres{e12/frozen/e1/usdk}{0.0934}
\defres{e12/frozen/live/n}{200}
\defres{e12/frozen/live/own}{100.0}
\defres{e12/frozen/live/success}{100.0}
\defres{e12/frozen/live/usdep}{0.0145}
\defres{e12/frozen/pubdev/devargs/acc}{90.8}
\defres{e12/frozen/pubdev/devtool/acc}{93.0}
\defres{e12/frozen/pubdev/devw2c/acc}{67.1}
\defres{e12/frozen/v1/dev/acc}{99.7}
\defres{e12/frozen/v1/devknockout/acc}{99.7}
\defres{e12/frozen/v1/devrecovery/acc}{99.8}
\defres{e12/gpuh}{8.4}
\defres{e12/jev/live/n}{200}
\defres{e12/jev/live/own}{91.0}
\defres{e12/jev/live/success}{83.0}
\defres{e12/jev/live/usdep}{0.0144}
\defres{e12/live/vs/frozen}{+0.0}
\defres{e12/live/vs/frozen/hi}{+1.9}
\defres{e12/live/vs/frozen/lo}{-1.9}
\defres{e12/live/vs/jev}{+17.0}
\defres{e12/live/vs/jev/hi}{+22.8}
\defres{e12/live/vs/jev/lo}{+12.1}
\defres{e12/rehost/agree}{99.8}
\defres{e12/rehost/usdk}{0.1428}
\defres{e12/spend}{2.93}
\defres{e12/train/min}{146}
\defres{e12b/e12b/heldout/op/acc}{91.0}
\defres{e12b/e12b/heldout/op/n}{600}
\defres{e12b/e12b/heldout/tp/acc}{98.7}
\defres{e12b/e12b/heldout/tp/n}{225}
\defres{e12b/e12b/heldout/tsother/acc}{100.0}
\defres{e12b/e12b/heldout/tsother/n}{225}
\defres{e12b/e7dfrozen/heldout/op/acc}{76.5}
\defres{e12b/e7dfrozen/heldout/tp/acc}{95.1}
\defres{e12b/e7dfrozen/heldout/tsother/acc}{91.6}
\defres{e12b/e7dtier/heldout/op/acc}{95.3}
\defres{e12b/e7dtier/heldout/tp/acc}{98.2}
\defres{e12b/e7dtier/heldout/tsother/acc}{100.0}
\defres{e12b/frozen/heldout/op/acc}{76.5}
\defres{e12b/frozen/heldout/op/n}{600}
\defres{e12b/frozen/heldout/tp/acc}{95.1}
\defres{e12b/frozen/heldout/tp/n}{225}
\defres{e12b/frozen/heldout/tsother/acc}{91.6}
\defres{e12b/frozen/heldout/tsother/n}{225}
\defres{e12b/train/min}{74}
\defres{e12c/c/delta}{+0.4}
\defres{e12c/c/delta/hi}{+1.0}
\defres{e12c/c/delta/lo}{+0.0}
\defres{e12c/c/ni}{yes}
\defres{e12c/c/vssl4b}{+10.5}
\defres{e12c/c/vssl4b/hi}{+12.2}
\defres{e12c/c/vssl4b/lo}{+8.8}
\defres{e12c/e1/beatssl4b}{yes}
\defres{e12c/e1/vs/frozen/all}{+6.7}
\defres{e12c/e1/vs/frozen/all/hi}{+8.1}
\defres{e12c/e1/vs/frozen/all/lo}{+5.4}
\defres{e12c/e1/vs/frozen/args}{+6.9}
\defres{e12c/e1/vs/frozen/args/hi}{+8.6}
\defres{e12c/e1/vs/frozen/args/lo}{+5.3}
\defres{e12c/e1/vs/frozen/toolchoice}{+1.1}
\defres{e12c/e1/vs/frozen/toolchoice/hi}{+2.8}
\defres{e12c/e1/vs/frozen/toolchoice/lo}{-0.6}
\defres{e12c/e1/vs/frozen/w2c}{+13.1}
\defres{e12c/e1/vs/frozen/w2c/hi}{+17.3}
\defres{e12c/e1/vs/frozen/w2c/lo}{+9.2}
\defres{e12c/e1/vs/jev/all}{-0.9}
\defres{e12c/e1/vs/jev/all/hi}{+0.2}
\defres{e12c/e1/vs/jev/all/lo}{-2.1}
\defres{e12c/e1/vs/jev/args}{+2.3}
\defres{e12c/e1/vs/jev/args/hi}{+3.7}
\defres{e12c/e1/vs/jev/args/lo}{+0.9}
\defres{e12c/e1/vs/jev/toolchoice}{-0.4}
\defres{e12c/e1/vs/jev/toolchoice/hi}{+0.7}
\defres{e12c/e1/vs/jev/toolchoice/lo}{-1.6}
\defres{e12c/e1/vs/jev/w2c}{-8.3}
\defres{e12c/e1/vs/jev/w2c/hi}{-5.2}
\defres{e12c/e1/vs/jev/w2c/lo}{-11.5}
\defres{e12c/e1/vs/sl4b/all}{+2.3}
\defres{e12c/e1/vs/sl4b/all/hi}{+3.6}
\defres{e12c/e1/vs/sl4b/all/lo}{+1.1}
\defres{e12c/e1/vs/sl4b/args}{+10.7}
\defres{e12c/e1/vs/sl4b/args/hi}{+12.6}
\defres{e12c/e1/vs/sl4b/args/lo}{+8.8}
\defres{e12c/e1/vs/sl4b/toolchoice}{-1.8}
\defres{e12c/e1/vs/sl4b/toolchoice/hi}{-0.6}
\defres{e12c/e1/vs/sl4b/toolchoice/lo}{-3.1}
\defres{e12c/e1/vs/sl4b/w2c}{-10.2}
\defres{e12c/e1/vs/sl4b/w2c/hi}{-7.1}
\defres{e12c/e1/vs/sl4b/w2c/lo}{-13.5}
\defres{e12c/e12c/c/acc}{99.6}
\defres{e12c/e12c/c/ask}{100.0}
\defres{e12c/e12c/c/offplan}{96.1}
\defres{e12c/e12c/e1/acc}{85.5}
\defres{e12c/e12c/e1/acc/args}{91.9}
\defres{e12c/e12c/e1/acc/toolchoice}{89.5}
\defres{e12c/e12c/e1/acc/w2c}{67.1}
\defres{e12c/e12c/e1/usdk}{0.2946}
\defres{e12c/e12c/live/n}{200}
\defres{e12c/e12c/live/success}{100.0}
\defres{e12c/e12c/pubdev/devargs/acc}{98.0}
\defres{e12c/e12c/pubdev/devtool/acc}{97.7}
\defres{e12c/e12c/pubdev/devw2c/acc}{97.3}
\defres{e12c/e12c/v1/dev/acc}{99.5}
\defres{e12c/e12c/v1/devknockout/acc}{99.7}
\defres{e12c/e12c/v1/devrecovery/acc}{99.2}
\defres{e12c/frozen/c/acc}{99.2}
\defres{e12c/frozen/c/ask}{100.0}
\defres{e12c/frozen/c/offplan}{94.7}
\defres{e12c/frozen/e1/acc}{78.8}
\defres{e12c/frozen/e1/acc/args}{85.0}
\defres{e12c/frozen/e1/acc/toolchoice}{88.4}
\defres{e12c/frozen/e1/acc/w2c}{54.0}
\defres{e12c/frozen/e1/usdk}{0.0934}
\defres{e12c/frozen/live/n}{200}
\defres{e12c/frozen/live/success}{100.0}
\defres{e12c/gpuh}{7.1}
\defres{e12c/jev/e1/acc}{86.4}
\defres{e12c/jev/e1/acc/args}{89.6}
\defres{e12c/jev/e1/acc/toolchoice}{89.9}
\defres{e12c/jev/e1/acc/w2c}{75.4}
\defres{e12c/jev/e1/usdk}{0.0163}
\defres{e12c/jev/live/n}{200}
\defres{e12c/jev/live/success}{83.0}
\defres{e12c/live/vs/frozen}{+0.0}
\defres{e12c/live/vs/frozen/hi}{+1.9}
\defres{e12c/live/vs/frozen/lo}{-1.9}
\defres{e12c/live/vs/jev}{+17.0}
\defres{e12c/live/vs/jev/hi}{+22.8}
\defres{e12c/live/vs/jev/lo}{+12.1}
\defres{e12c/live/vs/sl4b}{+40.0}
\defres{e12c/live/vs/sl4b/hi}{+46.9}
\defres{e12c/live/vs/sl4b/lo}{+33.2}
\defres{e12c/sel/ep1/devprefix}{89.6}
\defres{e12c/sel/ep1/v1dev}{99.5}
\defres{e12c/sel/ep2/devprefix}{87.9}
\defres{e12c/sel/ep2/v1dev}{99.5}
\defres{e12c/sel/epoch}{1}
\defres{e12c/sl4b/c/acc}{89.1}
\defres{e12c/sl4b/c/ask}{84.1}
\defres{e12c/sl4b/c/offplan}{76.8}
\defres{e12c/sl4b/e1/acc}{83.1}
\defres{e12c/sl4b/e1/acc/args}{81.2}
\defres{e12c/sl4b/e1/acc/toolchoice}{91.3}
\defres{e12c/sl4b/e1/acc/w2c}{77.4}
\defres{e12c/sl4b/e1/usdk}{0.0524}
\defres{e12c/sl4b/live/n}{200}
\defres{e12c/sl4b/live/success}{60.0}
\defres{e12c/smoke/sperstep}{47.8}
\defres{e12c/spend}{2.92}
\defres{e12c/train/min}{270}
\makeatother


==> generated/e13_llms.tex <==
\makeatletter
\providecommand{\res}[1]{\ifcsname jevres@#1\endcsname\csname jevres@#1\endcsname\else\tbd\fi}
\providecommand{\defres}[2]{\expandafter\def\csname jevres@#1\endcsname{#2}}
\defres{e13/claude/name}{Claude Haiku 4.5}
\defres{e13/claude/runner}{collaborator}
\defres{e13/claude/seeds}{311200--311299}
\defres{e13/claude/state}{not run}
\defres{e13/deepseek/name}{DeepSeek-V4-Flash}
\defres{e13/deepseek/runner}{collaborator}
\defres{e13/deepseek/seeds}{311100--311199}
\defres{e13/deepseek/state}{not run}
\defres{e13/luna/cal/ntasks}{100}
\defres{e13/luna/cal/op/coverage}{100.0}
\defres{e13/luna/cal/op/llmaccall}{95.3}
\defres{e13/luna/cal/op/n}{911}
\defres{e13/luna/cal/op/s1accall}{100.0}
\defres{e13/luna/cal/toolparams/coverage}{90.2}
\defres{e13/luna/cal/toolparams/llmaccall}{100.0}
\defres{e13/luna/cal/toolparams/n}{4469}
\defres{e13/luna/cal/toolparams/s1accall}{97.2}
\defres{e13/luna/cal/toolparams/s1acctaken}{100.0}
\defres{e13/luna/cal/toolparams/tau}{0.61}
\defres{e13/luna/cal/toolselect/coverage}{100.0}
\defres{e13/luna/cal/toolselect/llmaccall}{98.5}
\defres{e13/luna/cal/toolselect/n}{2790}
\defres{e13/luna/cal/toolselect/s1accall}{99.9}
\defres{e13/luna/cal/toolselect/s1acctaken}{99.9}
\defres{e13/luna/cal/toolselect/tau}{0.49}
\defres{e13/luna/cap}{65}
\defres{e13/luna/cap_jev}{5}
\defres{e13/luna/cap_llm}{60}
\defres{e13/luna/date}{2026-10-07}
\defres{e13/luna/diag/alltools/cachedshare}{78.6}
\defres{e13/luna/diag/alltools/calls}{4}
\defres{e13/luna/diag/alltools/callshare}{0.2}
\defres{e13/luna/diag/alltools/hitcalls}{4}
\defres{e13/luna/diag/alltools/tokenshare}{0.4}
\defres{e13/luna/diag/gap_k}{20.1}
\defres{e13/luna/diag/jev_k}{13.7}
\defres{e13/luna/diag/jevshareofgap}{68}
\defres{e13/luna/diag/llm_k}{9.1}
\defres{e13/luna/diag/llm_ref_k}{2.7}
\defres{e13/luna/diag/notools/cachedshare}{0.3}
\defres{e13/luna/diag/notools/calls}{255}
\defres{e13/luna/diag/notools/callshare}{12.0}
\defres{e13/luna/diag/notools/hitcalls}{1}
\defres{e13/luna/diag/notools/tokenshare}{13.4}
\defres{e13/luna/diag/onetool/cachedshare}{0.7}
\defres{e13/luna/diag/onetool/calls}{1861}
\defres{e13/luna/diag/onetool/callshare}{87.8}
\defres{e13/luna/diag/onetool/hitcalls}{18}
\defres{e13/luna/diag/onetool/tokenshare}{86.2}
\defres{e13/luna/diag/perfectfix_k}{15.2}
\defres{e13/luna/diag/perfectfix_llm_k}{1.4}
\defres{e13/luna/diag/perfectfix_ratio}{5.6}
\defres{e13/luna/diag/ratio}{8.4}
\defres{e13/luna/diag/writesurcharge_k/jevrefit}{2.1}
\defres{e13/luna/diag/writesurcharge_k/llmonly}{0.2}
\defres{e13/luna/jev_refit/acc}{97.7}
\defres{e13/luna/jev_refit/acc_accepted}{99.1}
\defres{e13/luna/jev_refit/cached_share}{0.9}
\defres{e13/luna/jev_refit/cost_api_k}{22.8}
\defres{e13/luna/jev_refit/cost_k}{22.8}
\defres{e13/luna/jev_refit/cost_ref_k}{2.7}
\defres{e13/luna/jev_refit/coverage}{82.0}
\defres{e13/luna/jev_refit/delta}{+38.0}
\defres{e13/luna/jev_refit/delta_ci/hi}{+50.0}
\defres{e13/luna/jev_refit/delta_ci/lo}{+26.0}
\defres{e13/luna/jev_refit/fail/askfinish}{8}
\defres{e13/luna/jev_refit/fail/n}{17}
\defres{e13/luna/jev_refit/fail/other}{0}
\defres{e13/luna/jev_refit/fail/wrongtotal}{8}
\defres{e13/luna/jev_refit/fail/wrongwrite}{1}
\defres{e13/luna/jev_refit/fig_delta}{+38.0}
\defres{e13/luna/jev_refit/fig_saving}{-737}
\defres{e13/luna/jev_refit/form/itemized/n}{98}
\defres{e13/luna/jev_refit/form/itemized/share}{98.0}
\defres{e13/luna/jev_refit/form/itemized/success}{84.7}
\defres{e13/luna/jev_refit/form/none/n}{2}
\defres{e13/luna/jev_refit/form/none/share}{2.0}
\defres{e13/luna/jev_refit/form/none/success}{0.0}
\defres{e13/luna/jev_refit/form/number/n}{0}
\defres{e13/luna/jev_refit/form/number/share}{0.0}
\defres{e13/luna/jev_refit/form/sentence/n}{0}
\defres{e13/luna/jev_refit/form/sentence/share}{0.0}
\defres{e13/luna/jev_refit/losses}{6}
\defres{e13/luna/jev_refit/n}{100}
\defres{e13/luna/jev_refit/n_dropped}{0}
\defres{e13/luna/jev_refit/newcombe/hi}{+48.9}
\defres{e13/luna/jev_refit/newcombe/lo}{+25.4}
\defres{e13/luna/jev_refit/op_acc}{100.0}
\defres{e13/luna/jev_refit/op_acc_accepted}{100.0}
\defres{e13/luna/jev_refit/op_accepted_wrong}{0}
\defres{e13/luna/jev_refit/op_coverage}{100.0}
\defres{e13/luna/jev_refit/op_n}{1182}
\defres{e13/luna/jev_refit/reflection_fired}{7.0}
\defres{e13/luna/jev_refit/saving}{-737.4}
\defres{e13/luna/jev_refit/saving_api}{-737.4}
\defres{e13/luna/jev_refit/saving_ci/hi}{-672.2}
\defres{e13/luna/jev_refit/saving_ci/lo}{-814.1}
\defres{e13/luna/jev_refit/state}{run}
\defres{e13/luna/jev_refit/steps}{37.5}
\defres{e13/luna/jev_refit/success}{83.0}
\defres{e13/luna/jev_refit/success_ref}{45.0}
\defres{e13/luna/jev_refit/tool_params/acc}{97.0}
\defres{e13/luna/jev_refit/tool_params/acc_accepted}{99.2}
\defres{e13/luna/jev_refit/tool_params/coverage}{70.9}
\defres{e13/luna/jev_refit/tool_select/acc}{98.8}
\defres{e13/luna/jev_refit/tool_select/acc_accepted}{98.9}
\defres{e13/luna/jev_refit/tool_select/coverage}{99.9}
\defres{e13/luna/jev_refit/wall_mean}{67.4}
\defres{e13/luna/jev_refit/wall_median}{65.4}
\defres{e13/luna/jev_refit/wall_ref_mean}{53.9}
\defres{e13/luna/jev_refit/wall_ref_median}{62.3}
\defres{e13/luna/jev_refit/wins}{44}
\defres{e13/luna/lat/jevrefit/extra}{13.6}
\defres{e13/luna/lat/jevrefit/extratail}{-2.8}
\defres{e13/luna/lat/jevrefit/s1}{32.6}
\defres{e13/luna/lat/jevrefit/s2}{32.9}
\defres{e13/luna/lat/jevrefit/s2tail}{2.2}
\defres{e13/luna/lat/jevrefit/tailshareofextra}{-20}
\defres{e13/luna/lat/jevrefit/wall}{67.4}
\defres{e13/luna/lat/llmonly/s1}{0.0}
\defres{e13/luna/lat/llmonly/s2}{52.6}
\defres{e13/luna/lat/llmonly/s2tail}{5.0}
\defres{e13/luna/lat/llmonly/wall}{53.9}
\defres{e13/luna/llm_only/cached_share}{95.5}
\defres{e13/luna/llm_only/cost_k}{2.7}
\defres{e13/luna/llm_only/fail/askfinish}{0}
\defres{e13/luna/llm_only/fail/n}{55}
\defres{e13/luna/llm_only/fail/other}{0}
\defres{e13/luna/llm_only/fail/wrongtotal}{11}
\defres{e13/luna/llm_only/fail/wrongwrite}{44}
\defres{e13/luna/llm_only/form/itemized/n}{56}
\defres{e13/luna/llm_only/form/itemized/share}{56.0}
\defres{e13/luna/llm_only/form/itemized/success}{80.4}
\defres{e13/luna/llm_only/form/none/n}{44}
\defres{e13/luna/llm_only/form/none/share}{44.0}
\defres{e13/luna/llm_only/form/none/success}{0.0}
\defres{e13/luna/llm_only/form/number/n}{0}
\defres{e13/luna/llm_only/form/number/share}{0.0}
\defres{e13/luna/llm_only/form/sentence/n}{0}
\defres{e13/luna/llm_only/form/sentence/share}{0.0}
\defres{e13/luna/llm_only/n}{100}
\defres{e13/luna/llm_only/steps}{29.1}
\defres{e13/luna/llm_only/success}{45.0}
\defres{e13/luna/llm_only/wall_mean}{53.9}
\defres{e13/luna/llm_only/wall_median}{62.3}
\defres{e13/luna/name}{GPT-6-Luna}
\defres{e13/luna/route}{openai\_responses}
\defres{e13/luna/runner}{local}
\defres{e13/luna/seeds}{311000--311099}
\defres{e13/luna/setting/answer_style}{itemized}
\defres{e13/luna/setting/families}{multi}
\defres{e13/luna/setting/max_steps}{45}
\defres{e13/luna/setting/multi_customers}{12}
\defres{e13/luna/setting/n}{100}
\defres{e13/luna/setting/n_distractors}{60}
\defres{e13/luna/setting/noise_lines}{20}
\defres{e13/luna/setting/rule}{tier}
\defres{e13/luna/setting/seed0}{311000}
\defres{e13/luna/spend}{3.65}
\defres{e13/luna/spend_jev}{2.19}
\defres{e13/luna/spend_llm}{1.46}
\defres{e13/luna/state}{run}
\defres{e13/n_llms_run}{1}
\makeatother


==> generated/e14_small.tex <==
\makeatletter
\providecommand{\res}[1]{\ifcsname jevres@#1\endcsname\csname jevres@#1\endcsname\else\tbd\fi}
\providecommand{\defres}[2]{\expandafter\def\csname jevres@#1\endcsname{#2}}
\defres{cov/ask/e14a/ask_now/acc}{100.0}
\defres{cov/ask/e14ag/ask_now/acc}{100.0}
\defres{cov/ask/e14g/ask_now/acc}{25.0}
\defres{e14/4b/cal/tp/casc}{99.9}
\defres{e14/4b/cal/tp/cov}{77.5}
\defres{e14/4b/cal/tp/llm}{100.0}
\defres{e14/4b/cal/tp/s1acc}{99.9}
\defres{e14/4b/cal/tp/tau}{1}
\defres{e14/4b/cal/tp/taugap}{1.2e-7}
\defres{e14/4b/cal/ts/casc}{100.0}
\defres{e14/4b/cal/ts/cov}{100.0}
\defres{e14/4b/cal/ts/llm}{100.0}
\defres{e14/4b/cal/ts/s1acc}{100.0}
\defres{e14/4b/cal/ts/tau}{0.5}
\defres{e14/4b/cal/ts/taugap}{5.0e-1}
\defres{e14/a/c/acc}{99.2}
\defres{e14/a/c/ask}{100.0}
\defres{e14/a/c/ece}{0.011}
\defres{e14/a/c/offplan}{94.1}
\defres{e14/a/c/vse14g/all}{75.3}
\defres{e14/a/c/vse14g/all/hi}{76.5}
\defres{e14/a/c/vse14g/all/lo}{73.9}
\defres{e14/a/c/vse14g/ask}{75.0}
\defres{e14/a/c/vse14g/ask/hi}{83.0}
\defres{e14/a/c/vse14g/ask/lo}{66.0}
\defres{e14/a/c/vse14g/offplan}{71.7}
\defres{e14/a/c/vse14g/offplan/hi}{78.9}
\defres{e14/a/c/vse14g/offplan/lo}{64.3}
\defres{e14/a/c/vse5mc1/all}{0.6}
\defres{e14/a/c/vse5mc1/all/hi}{0.9}
\defres{e14/a/c/vse5mc1/all/lo}{0.4}
\defres{e14/a/c/vse5mc1/ask}{0.0}
\defres{e14/a/c/vse5mc1/ask/hi}{0.0}
\defres{e14/a/c/vse5mc1/ask/lo}{0.0}
\defres{e14/a/c/vse5mc1/offplan}{1.9}
\defres{e14/a/c/vse5mc1/offplan/hi}{4.4}
\defres{e14/a/c/vse5mc1/offplan/lo}{0.1}
\defres{e14/a/c/vse5q06/all}{0.1}
\defres{e14/a/c/vse5q06/all/hi}{0.3}
\defres{e14/a/c/vse5q06/all/lo}{$-$0.2}
\defres{e14/a/c/vse5q06/ask}{0.0}
\defres{e14/a/c/vse5q06/ask/hi}{0.0}
\defres{e14/a/c/vse5q06/ask/lo}{0.0}
\defres{e14/a/c/vse5q06/offplan}{5.4}
\defres{e14/a/c/vse5q06/offplan/hi}{10.7}
\defres{e14/a/c/vse5q06/offplan/lo}{1.1}
\defres{e14/a/c/vsrl/all}{0.0}
\defres{e14/a/c/vsrl/all/hi}{0.2}
\defres{e14/a/c/vsrl/all/lo}{$-$0.2}
\defres{e14/a/c/vsrl/ask}{0.0}
\defres{e14/a/c/vsrl/ask/hi}{0.0}
\defres{e14/a/c/vsrl/ask/lo}{0.0}
\defres{e14/a/c/vsrl/offplan}{$-$0.6}
\defres{e14/a/c/vsrl/offplan/hi}{0.7}
\defres{e14/a/c/vsrl/offplan/lo}{$-$2.2}
\defres{e14/a/c/vssftv1/all}{0.0}
\defres{e14/a/c/vssftv1/all/hi}{0.2}
\defres{e14/a/c/vssftv1/all/lo}{$-$0.1}
\defres{e14/a/c/vssftv1/ask}{0.0}
\defres{e14/a/c/vssftv1/ask/hi}{0.0}
\defres{e14/a/c/vssftv1/ask/lo}{0.0}
\defres{e14/a/c/vssftv1/offplan}{0.3}
\defres{e14/a/c/vssftv1/offplan/hi}{2.1}
\defres{e14/a/c/vssftv1/offplan/lo}{$-$1.5}
\defres{e14/a/c/vssl08/all}{50.9}
\defres{e14/a/c/vssl08/all/hi}{53.3}
\defres{e14/a/c/vssl08/all/lo}{48.0}
\defres{e14/a/c/vssl08/ask}{50.6}
\defres{e14/a/c/vssl08/ask/hi}{57.8}
\defres{e14/a/c/vssl08/ask/lo}{43.5}
\defres{e14/a/c/vssl08/offplan}{62.6}
\defres{e14/a/c/vssl08/offplan/hi}{71.2}
\defres{e14/a/c/vssl08/offplan/lo}{54.2}
\defres{e14/a/cal/tp/casc}{100.0}
\defres{e14/a/cal/tp/cov}{78.8}
\defres{e14/a/cal/tp/llm}{100.0}
\defres{e14/a/cal/tp/s1acc}{100.0}
\defres{e14/a/cal/tp/tau}{1}
\defres{e14/a/cal/tp/taugap}{1.1e-12}
\defres{e14/a/cal/ts/casc}{100.0}
\defres{e14/a/cal/ts/cov}{80.0}
\defres{e14/a/cal/ts/llm}{100.0}
\defres{e14/a/cal/ts/s1acc}{100.0}
\defres{e14/a/cal/ts/tau}{1}
\defres{e14/a/cal/ts/taugap}{2.3e-10}
\defres{e14/a/e1/acc}{67.8}
\defres{e14/a/e1/args}{70.1}
\defres{e14/a/e1/front}{no}
\defres{e14/a/e1/lat}{239}
\defres{e14/a/e1/toolchoice}{80.5}
\defres{e14/a/e1/usdk}{0.12}
\defres{e14/a/e1/vsrl}{$-$11.0}
\defres{e14/a/e1/vssl08}{$-$2.2}
\defres{e14/a/e1/w2c}{47.4}
\defres{e14/a/fig4b/corpus_acc}{99.2}
\defres{e14/a/fig4b/e1_acc}{80.5}
\defres{e14/a/fig4b/live_success}{100.0}
\defres{e14/a/l1/usdk}{0.12}
\defres{e14/a/l1/usdk_wall}{0.032}
\defres{e14/a/live/api}{0.0145}
\defres{e14/a/live/n}{200}
\defres{e14/a/live/own}{100.0}
\defres{e14/a/live/steps}{7.5}
\defres{e14/a/live/success}{100.0}
\defres{e14/a/live/vsfrozen}{0.0}
\defres{e14/a/live/vsfrozen/hi}{1.9}
\defres{e14/a/live/vsfrozen/lo}{$-$1.9}
\defres{e14/a/live/vsjev}{17.0}
\defres{e14/a/live/vsjev/hi}{22.8}
\defres{e14/a/live/vsjev/lo}{12.1}
\defres{e14/a/live/vssl08b}{82.5}
\defres{e14/a/live/vssl08b/hi}{87.1}
\defres{e14/a/live/vssl08b/lo}{76.3}
\defres{e14/a/saved}{64.2}
\defres{e14/a/sets/bank}{57.2}
\defres{e14/a/sets/clinc}{54.0}
\defres{e14/a/sets/mean}{51.1}
\defres{e14/a/sets/td}{42.1}
\defres{e14/a/train/devbase}{39.1}
\defres{e14/a/train/devcal}{99.7}
\defres{e14/a/train/devece}{0.002}
\defres{e14/a/train/epoch1/dev}{99.7}
\defres{e14/a/train/epoch1/minutes}{59}
\defres{e14/a/train/epoch2/dev}{99.7}
\defres{e14/a/train/epoch2/minutes}{57}
\defres{e14/a/train/epochs}{2}
\defres{e14/a/train/mem}{6.3}
\defres{e14/a/train/minutes}{132}
\defres{e14/a/train/records}{14{,}787}
\defres{e14/a/train/selected}{1}
\defres{e14/a/v1/acc}{99.7}
\defres{e14/a/v1/ece}{0.001}
\defres{e14/a/v1/ko}{100.0}
\defres{e14/a/v1/rec}{99.7}
\defres{e14/a/v1/stop}{99.3}
\defres{e14/a/v1/tp}{100.0}
\defres{e14/a/v1/ts}{99.8}
\defres{e14/ag/c/acc}{99.1}
\defres{e14/ag/c/ask}{100.0}
\defres{e14/ag/c/ece}{0.013}
\defres{e14/ag/c/offplan}{92.7}
\defres{e14/ag/c/vse5mc1/all}{0.5}
\defres{e14/ag/c/vse5mc1/all/hi}{0.8}
\defres{e14/ag/c/vse5mc1/all/lo}{0.3}
\defres{e14/ag/c/vse5mc1/ask}{0.0}
\defres{e14/ag/c/vse5mc1/ask/hi}{0.0}
\defres{e14/ag/c/vse5mc1/ask/lo}{0.0}
\defres{e14/ag/c/vse5mc1/offplan}{0.4}
\defres{e14/ag/c/vse5mc1/offplan/hi}{3.0}
\defres{e14/ag/c/vse5mc1/offplan/lo}{$-$1.7}
\defres{e14/ag/c/vse5q06/all}{$-$0.0}
\defres{e14/ag/c/vse5q06/all/hi}{0.2}
\defres{e14/ag/c/vse5q06/all/lo}{$-$0.4}
\defres{e14/ag/c/vse5q06/ask}{0.0}
\defres{e14/ag/c/vse5q06/ask/hi}{0.0}
\defres{e14/ag/c/vse5q06/ask/lo}{0.0}
\defres{e14/ag/c/vse5q06/offplan}{4.0}
\defres{e14/ag/c/vse5q06/offplan/hi}{9.5}
\defres{e14/ag/c/vse5q06/offplan/lo}{$-$0.8}
\defres{e14/ag/c/vsrl/all}{$-$0.1}
\defres{e14/ag/c/vsrl/all/hi}{0.1}
\defres{e14/ag/c/vsrl/all/lo}{$-$0.3}
\defres{e14/ag/c/vsrl/ask}{0.0}
\defres{e14/ag/c/vsrl/ask/hi}{0.0}
\defres{e14/ag/c/vsrl/ask/lo}{0.0}
\defres{e14/ag/c/vsrl/offplan}{$-$2.0}
\defres{e14/ag/c/vsrl/offplan/hi}{$-$0.4}
\defres{e14/ag/c/vsrl/offplan/lo}{$-$4.0}
\defres{e14/ag/c/vssftv1/all}{$-$0.1}
\defres{e14/ag/c/vssftv1/all/hi}{0.1}
\defres{e14/ag/c/vssftv1/all/lo}{$-$0.2}
\defres{e14/ag/c/vssftv1/ask}{0.0}
\defres{e14/ag/c/vssftv1/ask/hi}{0.0}
\defres{e14/ag/c/vssftv1/ask/lo}{0.0}
\defres{e14/ag/c/vssftv1/offplan}{$-$1.1}
\defres{e14/ag/c/vssftv1/offplan/hi}{1.0}
\defres{e14/ag/c/vssftv1/offplan/lo}{$-$3.3}
\defres{e14/ag/c/vssl08/all}{50.8}
\defres{e14/ag/c/vssl08/all/hi}{53.3}
\defres{e14/ag/c/vssl08/all/lo}{47.9}
\defres{e14/ag/c/vssl08/ask}{50.6}
\defres{e14/ag/c/vssl08/ask/hi}{57.8}
\defres{e14/ag/c/vssl08/ask/lo}{43.5}
\defres{e14/ag/c/vssl08/offplan}{61.2}
\defres{e14/ag/c/vssl08/offplan/hi}{70.3}
\defres{e14/ag/c/vssl08/offplan/lo}{52.2}
\defres{e14/ag/cal/tp/casc}{100.0}
\defres{e14/ag/cal/tp/cov}{70.0}
\defres{e14/ag/cal/tp/llm}{100.0}
\defres{e14/ag/cal/tp/s1acc}{100.0}
\defres{e14/ag/cal/tp/tau}{1}
\defres{e14/ag/cal/tp/taugap}{5.8e-12}
\defres{e14/ag/cal/ts/casc}{100.0}
\defres{e14/ag/cal/ts/cov}{90.0}
\defres{e14/ag/cal/ts/llm}{100.0}
\defres{e14/ag/cal/ts/s1acc}{100.0}
\defres{e14/ag/cal/ts/tau}{0.9998}
\defres{e14/ag/cal/ts/taugap}{1.6e-4}
\defres{e14/ag/e1/acc}{68.8}
\defres{e14/ag/e1/args}{68.9}
\defres{e14/ag/e1/front}{no}
\defres{e14/ag/e1/lat}{236}
\defres{e14/ag/e1/toolchoice}{84.8}
\defres{e14/ag/e1/usdk}{0.100}
\defres{e14/ag/e1/vsrl}{$-$9.9}
\defres{e14/ag/e1/vssl08}{$-$1.2}
\defres{e14/ag/e1/w2c}{49.5}
\defres{e14/ag/fig4b/corpus_acc}{99.1}
\defres{e14/ag/fig4b/e1_acc}{84.8}
\defres{e14/ag/l1/usdk}{0.100}
\defres{e14/ag/l1/usdk_wall}{0.026}
\defres{e14/ag/sets/bank}{71.8}
\defres{e14/ag/sets/clinc}{75.8}
\defres{e14/ag/sets/mean}{69.4}
\defres{e14/ag/sets/td}{60.6}
\defres{e14/ag/train/devbase}{39.3}
\defres{e14/ag/train/devcal}{99.7}
\defres{e14/ag/train/devece}{0.002}
\defres{e14/ag/train/epoch1/dev}{99.7}
\defres{e14/ag/train/epoch1/minutes}{71}
\defres{e14/ag/train/epochs}{1}
\defres{e14/ag/train/mem}{6.3}
\defres{e14/ag/train/minutes}{83}
\defres{e14/ag/train/records}{27{,}137}
\defres{e14/ag/train/selected}{1}
\defres{e14/ag/v1/acc}{99.7}
\defres{e14/ag/v1/ece}{0.002}
\defres{e14/ag/v1/ko}{100.0}
\defres{e14/ag/v1/rec}{99.7}
\defres{e14/ag/v1/stop}{99.3}
\defres{e14/ag/v1/tp}{99.9}
\defres{e14/ag/v1/ts}{99.8}
\defres{e14/b/a/api}{13.56}
\defres{e14/b/a/argcov}{86.4}
\defres{e14/b/a/q}{1.86}
\defres{e14/b/a/s1s}{1.3}
\defres{e14/b/a/s2call}{0.76}
\defres{e14/b/a/s2s}{2.7}
\defres{e14/b/a/success}{100.0}
\defres{e14/b/a/toolcov}{85.5}
\defres{e14/b/a/tot}{15.42}
\defres{e14/b/a/tot9}{16.13}
\defres{e14/b/a/totown}{14.95}
\defres{e14/b/a/wall}{4.1}
\defres{e14/b/hf4b/api}{5.82}
\defres{e14/b/hf4b/argcov}{85.5}
\defres{e14/b/hf4b/q}{4.33}
\defres{e14/b/hf4b/s1s}{3.9}
\defres{e14/b/hf4b/s2call}{1.68}
\defres{e14/b/hf4b/s2s}{5.1}
\defres{e14/b/hf4b/success}{100.0}
\defres{e14/b/hf4b/toolcov}{100.0}
\defres{e14/b/hf4b/tot}{10.15}
\defres{e14/b/hf4b/tot9}{11.80}
\defres{e14/b/hf4b/totown}{9.05}
\defres{e14/b/hf4b/tottariff}{10.20}
\defres{e14/b/hf4b/wall}{9.6}
\defres{e14/b/llm/api}{43.12}
\defres{e14/b/llm/q}{0.00}
\defres{e14/b/llm/s1s}{0.0}
\defres{e14/b/llm/s2call}{1.55}
\defres{e14/b/llm/s2s}{11.7}
\defres{e14/b/llm/success}{99.5}
\defres{e14/b/llm/toolcov}{0.0}
\defres{e14/b/llm/tot}{43.12}
\defres{e14/b/llm/tot9}{43.12}
\defres{e14/b/llm/totown}{43.12}
\defres{e14/b/llm/wall}{13.6}
\defres{e14/b/n}{200}
\defres{e14/b/vshf4b/saving}{$-$51.9}
\defres{e14/b/vshf4b/saving/hi}{$-$41.4}
\defres{e14/b/vshf4b/saving/lo}{$-$63.3}
\defres{e14/b/vshf4b/saving_api}{$-$132.9}
\defres{e14/b/vshf4b/saving_tariff}{$-$51.2}
\defres{e14/b/vshf4b/success}{0.0}
\defres{e14/b/vshf4b/success/hi}{1.9}
\defres{e14/b/vshf4b/success/lo}{$-$1.9}
\defres{e14/b/vshf4b/wall}{$-$5.5}
\defres{e14/b/vsllm/saving}{64.2}
\defres{e14/b/vsllm/saving/hi}{66.0}
\defres{e14/b/vsllm/saving/lo}{62.4}
\defres{e14/b/vsllm/saving_api}{68.5}
\defres{e14/b/vsllm/success}{0.5}
\defres{e14/b/vsllm/success/hi}{2.8}
\defres{e14/b/vsllm/success/lo}{$-$1.4}
\defres{e14/b/vsllm/wall}{$-$9.5}
\defres{e14/base/sets/bank}{7.0}
\defres{e14/base/sets/clinc}{19.6}
\defres{e14/base/sets/mean}{20.8}
\defres{e14/base/sets/td}{35.9}
\defres{e14/e1/amg}{15.5}
\defres{e14/e1/amg/args}{28.3}
\defres{e14/e1/amg/args/hi}{30.6}
\defres{e14/e1/amg/args/lo}{26.1}
\defres{e14/e1/amg/hi}{17.2}
\defres{e14/e1/amg/lo}{13.7}
\defres{e14/e1/amg/toolchoice}{$-$1.3}
\defres{e14/e1/amg/toolchoice/hi}{1.3}
\defres{e14/e1/amg/toolchoice/lo}{$-$4.0}
\defres{e14/e1/amg/w2c}{8.7}
\defres{e14/e1/amg/w2c/hi}{13.6}
\defres{e14/e1/amg/w2c/lo}{3.9}
\defres{e14/e1cost/a/v1/e9}{0.12}
\defres{e14/e1cost/a/v1/lat}{239}
\defres{e14/e1cost/a/v1/wall}{0.032}
\defres{e14/e1cost/a/v1/walls}{203}
\defres{e14/e1cost/ag/v1/e9}{0.100}
\defres{e14/e1cost/ag/v1/lat}{236}
\defres{e14/e1cost/ag/v1/wall}{0.026}
\defres{e14/e1cost/ag/v1/walls}{166}
\defres{e14/e1cost/g/v1/e9}{0.100}
\defres{e14/e1cost/g/v1/lat}{235}
\defres{e14/e1cost/g/v1/wall}{0.026}
\defres{e14/e1cost/g/v1/walls}{166}
\defres{e14/engine/check}{failed}
\defres{e14/engine/dev/maxdp}{0.044}
\defres{e14/engine/dev/n}{2{,}377}
\defres{e14/engine/dev/same}{2{,}377}
\defres{e14/engine/dev/v1s}{162}
\defres{e14/engine/dev/v2s}{182}
\defres{e14/engine/e1dev/flips}{1}
\defres{e14/engine/e1dev/n}{299}
\defres{e14/g/c/acc}{23.9}
\defres{e14/g/c/ask}{25.0}
\defres{e14/g/c/ece}{0.530}
\defres{e14/g/c/offplan}{22.4}
\defres{e14/g/c/vse5mc1/all}{$-$74.6}
\defres{e14/g/c/vse5mc1/all/hi}{$-$73.2}
\defres{e14/g/c/vse5mc1/all/lo}{$-$76.0}
\defres{e14/g/c/vse5mc1/ask}{$-$75.0}
\defres{e14/g/c/vse5mc1/ask/hi}{$-$66.0}
\defres{e14/g/c/vse5mc1/ask/lo}{$-$83.0}
\defres{e14/g/c/vse5mc1/offplan}{$-$69.8}
\defres{e14/g/c/vse5mc1/offplan/hi}{$-$61.4}
\defres{e14/g/c/vse5mc1/offplan/lo}{$-$77.8}
\defres{e14/g/c/vse5q06/all}{$-$75.2}
\defres{e14/g/c/vse5q06/all/hi}{$-$73.8}
\defres{e14/g/c/vse5q06/all/lo}{$-$76.5}
\defres{e14/g/c/vse5q06/ask}{$-$75.0}
\defres{e14/g/c/vse5q06/ask/hi}{$-$66.0}
\defres{e14/g/c/vse5q06/ask/lo}{$-$83.0}
\defres{e14/g/c/vse5q06/offplan}{$-$66.3}
\defres{e14/g/c/vse5q06/offplan/hi}{$-$55.4}
\defres{e14/g/c/vse5q06/offplan/lo}{$-$76.2}
\defres{e14/g/c/vsrl/all}{$-$75.3}
\defres{e14/g/c/vsrl/all/hi}{$-$73.9}
\defres{e14/g/c/vsrl/all/lo}{$-$76.5}
\defres{e14/g/c/vsrl/ask}{$-$75.0}
\defres{e14/g/c/vsrl/ask/hi}{$-$66.0}
\defres{e14/g/c/vsrl/ask/lo}{$-$83.0}
\defres{e14/g/c/vsrl/offplan}{$-$72.3}
\defres{e14/g/c/vsrl/offplan/hi}{$-$64.7}
\defres{e14/g/c/vsrl/offplan/lo}{$-$79.7}
\defres{e14/g/c/vssftv1/all}{$-$75.2}
\defres{e14/g/c/vssftv1/all/hi}{$-$73.9}
\defres{e14/g/c/vssftv1/all/lo}{$-$76.5}
\defres{e14/g/c/vssftv1/ask}{$-$75.0}
\defres{e14/g/c/vssftv1/ask/hi}{$-$66.0}
\defres{e14/g/c/vssftv1/ask/lo}{$-$83.0}
\defres{e14/g/c/vssftv1/offplan}{$-$71.4}
\defres{e14/g/c/vssftv1/offplan/hi}{$-$63.7}
\defres{e14/g/c/vssftv1/offplan/lo}{$-$78.7}
\defres{e14/g/c/vssl08/all}{$-$24.4}
\defres{e14/g/c/vssl08/all/hi}{$-$22.0}
\defres{e14/g/c/vssl08/all/lo}{$-$26.8}
\defres{e14/g/c/vssl08/ask}{$-$24.4}
\defres{e14/g/c/vssl08/ask/hi}{$-$19.4}
\defres{e14/g/c/vssl08/ask/lo}{$-$29.6}
\defres{e14/g/c/vssl08/offplan}{$-$9.1}
\defres{e14/g/c/vssl08/offplan/hi}{$-$0.8}
\defres{e14/g/c/vssl08/offplan/lo}{$-$17.0}
\defres{e14/g/cal/tp/casc}{100.0}
\defres{e14/g/cal/tp/cov}{0.0}
\defres{e14/g/cal/tp/llm}{100.0}
\defres{e14/g/cal/tp/tau}{always defers}
\defres{e14/g/cal/ts/casc}{100.0}
\defres{e14/g/cal/ts/cov}{0.0}
\defres{e14/g/cal/ts/llm}{100.0}
\defres{e14/g/cal/ts/tau}{always defers}
\defres{e14/g/e1/acc}{52.3}
\defres{e14/g/e1/args}{41.9}
\defres{e14/g/e1/front}{no}
\defres{e14/g/e1/lat}{235}
\defres{e14/g/e1/toolchoice}{81.8}
\defres{e14/g/e1/usdk}{0.100}
\defres{e14/g/e1/vsrl}{$-$26.5}
\defres{e14/g/e1/vssl08}{$-$17.7}
\defres{e14/g/e1/w2c}{38.7}
\defres{e14/g/fig4b/corpus_acc}{23.9}
\defres{e14/g/fig4b/e1_acc}{81.8}
\defres{e14/g/fig4b/live_success}{0.0}
\defres{e14/g/l1/usdk}{0.100}
\defres{e14/g/l1/usdk_wall}{0.026}
\defres{e14/g/live/api}{0.0007}
\defres{e14/g/live/n}{200}
\defres{e14/g/live/own}{6.2}
\defres{e14/g/live/steps}{1.1}
\defres{e14/g/live/success}{0.0}
\defres{e14/g/live/vse14a}{$-$100.0}
\defres{e14/g/live/vse14a/hi}{$-$97.3}
\defres{e14/g/live/vse14a/lo}{$-$100.0}
\defres{e14/g/live/vsfrozen}{$-$100.0}
\defres{e14/g/live/vsfrozen/hi}{$-$97.3}
\defres{e14/g/live/vsfrozen/lo}{$-$100.0}
\defres{e14/g/live/vsjev}{$-$83.0}
\defres{e14/g/live/vsjev/hi}{$-$76.9}
\defres{e14/g/live/vsjev/lo}{$-$87.6}
\defres{e14/g/live/vssl08b}{$-$17.5}
\defres{e14/g/live/vssl08b/hi}{$-$12.5}
\defres{e14/g/live/vssl08b/lo}{$-$23.4}
\defres{e14/g/reproduced}{yes}
\defres{e14/g/sets/bank}{75.0}
\defres{e14/g/sets/clinc}{73.6}
\defres{e14/g/sets/mean}{69.6}
\defres{e14/g/sets/td}{60.2}
\defres{e14/g/train/devbase}{35.2}
\defres{e14/g/train/devcal}{86.5}
\defres{e14/g/train/devece}{0.040}
\defres{e14/g/train/epoch1/dev}{86.5}
\defres{e14/g/train/epoch1/minutes}{13}
\defres{e14/g/train/epochs}{1}
\defres{e14/g/train/mem}{5.2}
\defres{e14/g/train/minutes}{14}
\defres{e14/g/train/records}{12{,}078}
\defres{e14/g/train/selected}{1}
\defres{e14/g/v1/acc}{39.6}
\defres{e14/g/v1/ece}{0.248}
\defres{e14/g/v1/ko}{82.0}
\defres{e14/g/v1/rec}{40.8}
\defres{e14/g/v1/stop}{50.7}
\defres{e14/g/v1/tp}{33.1}
\defres{e14/g/v1/ts}{37.2}
\defres{e14/gpuh}{6.5}
\defres{e14/lat/4b/c1/p50}{319}
\defres{e14/lat/4b/c1/p90}{443}
\defres{e14/lat/4b/c1/step}{381}
\defres{e14/lat/4b/c4/p50}{879}
\defres{e14/lat/4b/c4/p90}{1298}
\defres{e14/lat/4b/c4/step}{1727}
\defres{e14/lat/4b/mem}{22.0}
\defres{e14/lat/a/c1/p50}{91}
\defres{e14/lat/a/c1/p90}{118}
\defres{e14/lat/a/c1/speedup}{3.5}
\defres{e14/lat/a/c1/step}{153}
\defres{e14/lat/a/c4/p50}{203}
\defres{e14/lat/a/c4/p90}{386}
\defres{e14/lat/a/c4/speedup}{4.3}
\defres{e14/lat/a/c4/step}{372}
\defres{e14/lat/a/mem}{2.4}
\defres{e14/lat/g/c1/p50}{91}
\defres{e14/lat/g/c1/p90}{118}
\defres{e14/lat/g/c1/speedup}{3.5}
\defres{e14/lat/g/c1/step}{153}
\defres{e14/lat/g/c4/p50}{207}
\defres{e14/lat/g/c4/p90}{377}
\defres{e14/lat/g/c4/speedup}{4.2}
\defres{e14/lat/g/c4/step}{387}
\defres{e14/lat/g/mem}{2.4}
\defres{e14/reading/i_usable_confidences/e14a}{did not hold}
\defres{e14/reading/i_usable_confidences/e14ag}{did not hold}
\defres{e14/reading/i_usable_confidences/e14g}{did not hold}
\defres{e14/reading/ii_near_4b_at_fraction_of_cost/e14a}{did not hold}
\defres{e14/reading/iii_fixed_questions_misrank/AvsG}{did not hold}
\defres{e14/ref/e1n}{3{,}991}
\defres{e14/ref/flash/e1acc}{88.1}
\defres{e14/ref/flash/e1toolchoice}{90.3}
\defres{e14/ref/flash/e1usdk}{0.81}
\defres{e14/ref/jev/e1acc}{86.4}
\defres{e14/ref/jev/e1toolchoice}{89.9}
\defres{e14/ref/jev/e1usdk}{0.016}
\defres{e14/ref/jev/live}{83.0}
\defres{e14/ref/jev/livewall}{7.3}
\defres{e14/ref/mc1/c/acc}{98.6}
\defres{e14/ref/mc1/c/ask}{100.0}
\defres{e14/ref/mc1/c/offplan}{92.3}
\defres{e14/ref/q06/c/acc}{99.1}
\defres{e14/ref/q06/c/ask}{100.0}
\defres{e14/ref/q06/c/offplan}{88.7}
\defres{e14/ref/q06/offplan_vs_rl}{$-$6.0}
\defres{e14/ref/rl/c/acc}{99.2}
\defres{e14/ref/rl/c/ask}{100.0}
\defres{e14/ref/rl/c/offplan}{94.7}
\defres{e14/ref/rl/e1acc}{78.8}
\defres{e14/ref/rl/e1toolchoice}{88.4}
\defres{e14/ref/rl/e1usdk}{0.093}
\defres{e14/ref/rl/live}{100.0}
\defres{e14/ref/rl/livewall}{8.8}
\defres{e14/ref/sftv1/c/acc}{99.2}
\defres{e14/ref/sftv1/c/ask}{100.0}
\defres{e14/ref/sftv1/c/offplan}{93.8}
\defres{e14/ref/sl08/c/acc}{48.3}
\defres{e14/ref/sl08/c/ask}{49.4}
\defres{e14/ref/sl08/c/offplan}{31.5}
\defres{e14/ref/sl08/e1acc}{70.0}
\defres{e14/ref/sl08/e1toolchoice}{88.2}
\defres{e14/ref/sl08/e1usdk}{0.013}
\defres{e14/ref/sl08/live}{17.5}
\defres{e14/ref/sl08/livewall}{7.7}
\defres{e14/spend}{5.82}
\defres{e9/e14a/acc}{67.8}
\defres{e9/e14a/acc/args}{70.1}
\defres{e9/e14a/acc/toolchoice}{80.5}
\defres{e9/e14a/acc/w2c}{47.4}
\defres{e9/e14a/costvsjev}{7.6}
\defres{e9/e14a/front}{no}
\defres{e9/e14a/gapfrozen}{-11.0}
\defres{e9/e14a/gapfrozenabs}{11.0}
\defres{e9/e14a/gapjev}{-18.6}
\defres{e9/e14a/gapjevabs}{18.6}
\defres{e9/e14a/gapsl4b}{-15.4}
\defres{e9/e14a/gapsl4babs}{15.4}
\defres{e9/e14a/lat}{239}
\defres{e9/e14a/lg}{-3.9096}
\defres{e9/e14a/usdk}{0.12}
\defres{e9/e14ag/acc}{68.8}
\defres{e9/e14ag/acc/args}{68.9}
\defres{e9/e14ag/acc/toolchoice}{84.8}
\defres{e9/e14ag/acc/w2c}{49.5}
\defres{e9/e14ag/costvsjev}{6.1}
\defres{e9/e14ag/front}{no}
\defres{e9/e14ag/gapfrozen}{-9.9}
\defres{e9/e14ag/gapfrozenabs}{9.9}
\defres{e9/e14ag/gapjev}{-17.6}
\defres{e9/e14ag/gapjevabs}{17.6}
\defres{e9/e14ag/gapsl4b}{-14.3}
\defres{e9/e14ag/gapsl4babs}{14.3}
\defres{e9/e14ag/lat}{236}
\defres{e9/e14ag/lg}{-4.0011}
\defres{e9/e14ag/usdk}{0.100}
\defres{e9/e14g/acc}{52.3}
\defres{e9/e14g/acc/args}{41.9}
\defres{e9/e14g/acc/toolchoice}{81.8}
\defres{e9/e14g/acc/w2c}{38.7}
\defres{e9/e14g/costvsjev}{6.1}
\defres{e9/e14g/front}{no}
\defres{e9/e14g/gapfrozen}{-26.5}
\defres{e9/e14g/gapfrozenabs}{26.5}
\defres{e9/e14g/gapjev}{-34.1}
\defres{e9/e14g/gapjevabs}{34.1}
\defres{e9/e14g/gapsl4b}{-30.9}
\defres{e9/e14g/gapsl4babs}{30.9}
\defres{e9/e14g/lat}{235}
\defres{e9/e14g/lg}{-4.0011}
\defres{e9/e14g/usdk}{0.100}
\defres{e9/front14/first}{sl08b}
\defres{e9/front14/n}{3}
\defres{e9/front14/rest}{jev,flash}
\defres{explore/startlux_live/e14a/live_n}{200}
\defres{explore/startlux_live/e14a/live_success}{100.0}
\defres{explore/startlux_live/e14g/live_n}{200}
\defres{explore/startlux_live/e14g/live_success}{0.0}
\defres{stage2_rl/e14a/corpus_acc}{99.2}
\defres{stage2_rl/e14ag/corpus_acc}{99.1}
\defres{stage2_rl/e14g/corpus_acc}{23.9}
\makeatother


==> generated/e15_baselines.tex <==
\makeatletter
\providecommand{\res}[1]{\ifcsname jevres@#1\endcsname\csname jevres@#1\endcsname\else\tbd\fi}
\providecommand{\defres}[2]{\expandafter\def\csname jevres@#1\endcsname{#2}}
\defres{e15/bosun/corpus_acc}{36.3}
\defres{e15/bosun/corpus_acc_ask}{49.2}
\defres{e15/bosun/corpus_acc_offplan}{29.5}
\defres{e15/bosun/corpus_vs_frozen}{$-$62.9}
\defres{e15/bosun/corpus_vs_frozen/hi}{$-$61.5}
\defres{e15/bosun/corpus_vs_frozen/lo}{$-$64.2}
\defres{e15/bosun/corpus_vs_jev}{$-$55.2}
\defres{e15/bosun/corpus_vs_jev/hi}{$-$53.0}
\defres{e15/bosun/corpus_vs_jev/lo}{$-$57.3}
\defres{e15/bosun/e1_acc}{85.8}
\defres{e15/bosun/e1_vs_jev}{$-$4.1}
\defres{e15/bosun/ece}{0.290}
\defres{e15/bosun/l1/errors}{0}
\defres{e15/bosun/l1/refusals}{0}
\defres{e15/bosun/l2/errors}{0}
\defres{e15/bosun/l2/refusals}{0}
\defres{e15/bosun/live}{no}
\defres{e15/bosun/livecell}{--}
\defres{e15/bosun/meanconf}{60.6}
\defres{e15/bosun/occacc}{34.3}
\defres{e15/clef/e1_acc}{86.3}
\defres{e15/clef/e1_vs_jev}{$-$3.7}
\defres{e15/clef/l1/errors}{0}
\defres{e15/clef/l1/refusals}{0}
\defres{e15/clef/live}{no}
\defres{e15/clef/livecell}{--}
\defres{e15/clefflash/corpus_acc}{47.7}
\defres{e15/clefflash/corpus_acc_ask}{25.0}
\defres{e15/clefflash/corpus_acc_offplan}{48.8}
\defres{e15/clefflash/corpus_vs_frozen}{$-$51.5}
\defres{e15/clefflash/corpus_vs_frozen/hi}{$-$49.1}
\defres{e15/clefflash/corpus_vs_frozen/lo}{$-$53.7}
\defres{e15/clefflash/corpus_vs_jev}{$-$43.8}
\defres{e15/clefflash/corpus_vs_jev/hi}{$-$42.0}
\defres{e15/clefflash/corpus_vs_jev/lo}{$-$45.4}
\defres{e15/clefflash/e1_acc}{87.5}
\defres{e15/clefflash/e1_vs_jev}{$-$2.4}
\defres{e15/clefflash/ece}{0.252}
\defres{e15/clefflash/l1/errors}{0}
\defres{e15/clefflash/l1/refusals}{0}
\defres{e15/clefflash/l2/errors}{0}
\defres{e15/clefflash/l2/refusals}{0}
\defres{e15/clefflash/live}{no}
\defres{e15/clefflash/livecell}{--}
\defres{e15/clefflash/meanconf}{74.4}
\defres{e15/clefflash/occacc}{49.2}
\defres{e15/clm/corpus_acc}{11.9}
\defres{e15/clm/corpus_acc_ask}{36.2}
\defres{e15/clm/corpus_acc_offplan}{5.1}
\defres{e15/clm/corpus_vs_frozen}{$-$87.3}
\defres{e15/clm/corpus_vs_frozen/hi}{$-$85.3}
\defres{e15/clm/corpus_vs_frozen/lo}{$-$89.2}
\defres{e15/clm/corpus_vs_jev}{$-$79.5}
\defres{e15/clm/corpus_vs_jev/hi}{$-$77.3}
\defres{e15/clm/corpus_vs_jev/lo}{$-$81.6}
\defres{e15/clm/e1_acc}{71.0}
\defres{e15/clm/e1_vs_jev}{$-$18.9}
\defres{e15/clm/ece}{0.371}
\defres{e15/clm/l1/errors}{0}
\defres{e15/clm/l1/refusals}{0}
\defres{e15/clm/l2/errors}{0}
\defres{e15/clm/l2/refusals}{0}
\defres{e15/clm/live}{no}
\defres{e15/clm/livecell}{--}
\defres{e15/clm/meanconf}{48.1}
\defres{e15/clm/occacc}{11.0}
\defres{e15/decider/corpus_acc}{63.2}
\defres{e15/decider/corpus_acc_ask}{57.8}
\defres{e15/decider/corpus_acc_offplan}{43.8}
\defres{e15/decider/corpus_vs_frozen}{$-$36.0}
\defres{e15/decider/corpus_vs_frozen/hi}{$-$33.4}
\defres{e15/decider/corpus_vs_frozen/lo}{$-$38.4}
\defres{e15/decider/corpus_vs_jev}{$-$28.2}
\defres{e15/decider/corpus_vs_jev/hi}{$-$25.3}
\defres{e15/decider/corpus_vs_jev/lo}{$-$31.0}
\defres{e15/decider/e1_acc}{90.8}
\defres{e15/decider/e1_vs_jev}{0.9}
\defres{e15/decider/ece}{0.261}
\defres{e15/decider/l1/errors}{0}
\defres{e15/decider/l1/refusals}{0}
\defres{e15/decider/l2/errors}{0}
\defres{e15/decider/l2/refusals}{0}
\defres{e15/decider/live}{no}
\defres{e15/decider/livecell}{--}
\defres{e15/decider/meanconf}{84.1}
\defres{e15/decider/occacc}{60.1}
\defres{e15/gpuh}{8.8}
\defres{e15/imajev/corpus_acc}{76.9}
\defres{e15/imajev/corpus_acc_ask}{49.0}
\defres{e15/imajev/corpus_acc_offplan}{64.1}
\defres{e15/imajev/corpus_vs_frozen}{$-$22.3}
\defres{e15/imajev/corpus_vs_frozen/hi}{$-$20.1}
\defres{e15/imajev/corpus_vs_frozen/lo}{$-$24.4}
\defres{e15/imajev/corpus_vs_jev}{$-$14.5}
\defres{e15/imajev/corpus_vs_jev/hi}{$-$13.0}
\defres{e15/imajev/corpus_vs_jev/lo}{$-$16.1}
\defres{e15/imajev/e1_acc}{87.9}
\defres{e15/imajev/e1_vs_jev}{$-$2.1}
\defres{e15/imajev/ece}{0.095}
\defres{e15/imajev/l1/errors}{0}
\defres{e15/imajev/l1/refusals}{0}
\defres{e15/imajev/l2/errors}{0}
\defres{e15/imajev/l2/refusals}{0}
\defres{e15/imajev/live}{no}
\defres{e15/imajev/livecell}{--}
\defres{e15/imajev/meanconf}{78.0}
\defres{e15/imajev/occacc}{79.1}
\defres{e15/jevk5/corpus_acc}{65.0}
\defres{e15/jevk5/corpus_acc_ask}{60.0}
\defres{e15/jevk5/corpus_acc_offplan}{50.0}
\defres{e15/jevk5/corpus_vs_frozen}{$-$34.2}
\defres{e15/jevk5/corpus_vs_frozen/hi}{$-$31.7}
\defres{e15/jevk5/corpus_vs_frozen/lo}{$-$36.6}
\defres{e15/jevk5/corpus_vs_jev}{$-$26.5}
\defres{e15/jevk5/corpus_vs_jev/hi}{$-$23.6}
\defres{e15/jevk5/corpus_vs_jev/lo}{$-$29.4}
\defres{e15/jevk5/e1_acc}{86.4}
\defres{e15/jevk5/e1_vs_jev}{$-$3.5}
\defres{e15/jevk5/ece}{0.228}
\defres{e15/jevk5/l1/errors}{0}
\defres{e15/jevk5/l1/refusals}{0}
\defres{e15/jevk5/l2/errors}{0}
\defres{e15/jevk5/l2/refusals}{0}
\defres{e15/jevk5/live}{no}
\defres{e15/jevk5/livecell}{--}
\defres{e15/jevk5/meanconf}{84.5}
\defres{e15/jevk5/occacc}{61.7}
\defres{e15/kendall/corpus_vs_live_all_rows}{0.62}
\defres{e15/kendall/e1_vs_corpus_all_rows}{0.56}
\defres{e15/kendall/e1_vs_live_all_rows}{0.04}
\defres{e15/kendall/holds}{yes}
\defres{e15/kendall/n_rows_all_three}{11}
\defres{e15/kendall/n_rows_static_common}{19}
\defres{e15/kendall/notrained/common_live}{0.54}
\defres{e15/kendall/notrained/holds}{yes}
\defres{e15/kendall/notrained/n}{10}
\defres{e15/kendall/notrained/n_static_common}{18}
\defres{e15/kendall/notrained/static_common}{0.63}
\defres{e15/kendall/notrained/static_live}{0.18}
\defres{e15/kendall/offtheshelf/common_live}{0.54}
\defres{e15/kendall/offtheshelf/holds}{yes}
\defres{e15/kendall/offtheshelf/n}{10}
\defres{e15/kendall/offtheshelf/n_static_common}{18}
\defres{e15/kendall/offtheshelf/static_common}{0.63}
\defres{e15/kendall/offtheshelf/static_live}{0.18}
\defres{e15/kendallold/corpus_vs_live_all_rows}{0.71}
\defres{e15/kendallold/e1_vs_corpus_all_rows}{0.30}
\defres{e15/kendallold/e1_vs_live_all_rows}{0.15}
\defres{e15/kendallold/holds}{yes}
\defres{e15/kendallold/n_rows_all_three}{8}
\defres{e15/kendallold/n_rows_static_common}{8}
\defres{e15/laya/corpus_acc}{11.0}
\defres{e15/laya/corpus_acc_ask}{1.5}
\defres{e15/laya/corpus_acc_offplan}{13.2}
\defres{e15/laya/corpus_vs_frozen}{$-$88.2}
\defres{e15/laya/corpus_vs_frozen/hi}{$-$86.5}
\defres{e15/laya/corpus_vs_frozen/lo}{$-$89.8}
\defres{e15/laya/corpus_vs_jev}{$-$80.5}
\defres{e15/laya/corpus_vs_jev/hi}{$-$78.5}
\defres{e15/laya/corpus_vs_jev/lo}{$-$82.5}
\defres{e15/laya/e1_acc}{79.8}
\defres{e15/laya/e1_vs_jev}{$-$10.1}
\defres{e15/laya/ece}{0.303}
\defres{e15/laya/l1/errors}{0}
\defres{e15/laya/l1/refusals}{0}
\defres{e15/laya/l2/errors}{0}
\defres{e15/laya/l2/refusals}{0}
\defres{e15/laya/live}{no}
\defres{e15/laya/livecell}{--}
\defres{e15/laya/meanconf}{41.5}
\defres{e15/laya/occacc}{11.2}
\defres{e15/n/models}{12}
\defres{e15/oaidec/api_cost}{0.0163}
\defres{e15/oaidec/corpus_acc}{90.9}
\defres{e15/oaidec/corpus_acc_ask}{75.9}
\defres{e15/oaidec/corpus_acc_offplan}{74.3}
\defres{e15/oaidec/corpus_vs_frozen}{$-$8.3}
\defres{e15/oaidec/corpus_vs_frozen/hi}{$-$6.9}
\defres{e15/oaidec/corpus_vs_frozen/lo}{$-$9.7}
\defres{e15/oaidec/corpus_vs_jev}{$-$0.5}
\defres{e15/oaidec/corpus_vs_jev/hi}{0.5}
\defres{e15/oaidec/corpus_vs_jev/lo}{$-$1.5}
\defres{e15/oaidec/e1_acc}{90.6}
\defres{e15/oaidec/e1_vs_jev}{0.6}
\defres{e15/oaidec/ece}{0.193}
\defres{e15/oaidec/l1/errors}{0}
\defres{e15/oaidec/l1/refusals}{10}
\defres{e15/oaidec/l2/errors}{0}
\defres{e15/oaidec/l2/refusals}{0}
\defres{e15/oaidec/l3/refusals}{0}
\defres{e15/oaidec/live}{yes}
\defres{e15/oaidec/live_n}{200}
\defres{e15/oaidec/live_success}{78.5}
\defres{e15/oaidec/live_vs_jev}{$-$4.5}
\defres{e15/oaidec/live_vs_jev/hi}{1.9}
\defres{e15/oaidec/live_vs_jev/lo}{$-$10.9}
\defres{e15/oaidec/livecell}{78.5}
\defres{e15/oaidec/meanconf}{73.2}
\defres{e15/oaidec/occacc}{92.5}
\defres{e15/oaidec/own_acc}{87.0}
\defres{e15/oaidec/steps}{7.4}
\defres{e15/openjev/api_cost}{0.0210}
\defres{e15/openjev/corpus_acc}{91.1}
\defres{e15/openjev/corpus_acc_ask}{87.5}
\defres{e15/openjev/corpus_acc_offplan}{82.4}
\defres{e15/openjev/corpus_vs_frozen}{$-$8.1}
\defres{e15/openjev/corpus_vs_frozen/hi}{$-$6.8}
\defres{e15/openjev/corpus_vs_frozen/lo}{$-$9.6}
\defres{e15/openjev/corpus_vs_jev}{$-$0.4}
\defres{e15/openjev/corpus_vs_jev/hi}{0.9}
\defres{e15/openjev/corpus_vs_jev/lo}{$-$1.6}
\defres{e15/openjev/e1_acc}{91.2}
\defres{e15/openjev/e1_vs_jev}{1.3}
\defres{e15/openjev/ece}{0.030}
\defres{e15/openjev/l1/errors}{0}
\defres{e15/openjev/l1/refusals}{0}
\defres{e15/openjev/l2/errors}{0}
\defres{e15/openjev/l2/refusals}{0}
\defres{e15/openjev/l3/refusals}{0}
\defres{e15/openjev/live}{yes}
\defres{e15/openjev/live_n}{200}
\defres{e15/openjev/live_success}{62.5}
\defres{e15/openjev/live_vs_jev}{$-$20.5}
\defres{e15/openjev/live_vs_jev/hi}{$-$14.8}
\defres{e15/openjev/live_vs_jev/lo}{$-$26.2}
\defres{e15/openjev/livecell}{62.5}
\defres{e15/openjev/meanconf}{90.6}
\defres{e15/openjev/occacc}{91.9}
\defres{e15/openjev/own_acc}{83.0}
\defres{e15/openjev/steps}{8.3}
\defres{e15/openjevhf/api_cost}{0.0133}
\defres{e15/openjevhf/corpus_acc}{92.4}
\defres{e15/openjevhf/corpus_acc_ask}{63.5}
\defres{e15/openjevhf/corpus_acc_offplan}{80.1}
\defres{e15/openjevhf/corpus_vs_frozen}{$-$6.8}
\defres{e15/openjevhf/corpus_vs_frozen/hi}{$-$5.5}
\defres{e15/openjevhf/corpus_vs_frozen/lo}{$-$8.1}
\defres{e15/openjevhf/corpus_vs_jev}{0.9}
\defres{e15/openjevhf/corpus_vs_jev/hi}{1.8}
\defres{e15/openjevhf/corpus_vs_jev/lo}{0.1}
\defres{e15/openjevhf/e1_acc}{90.2}
\defres{e15/openjevhf/e1_vs_jev}{0.3}
\defres{e15/openjevhf/ece}{0.021}
\defres{e15/openjevhf/l1/errors}{0}
\defres{e15/openjevhf/l1/refusals}{0}
\defres{e15/openjevhf/l2/errors}{0}
\defres{e15/openjevhf/l2/refusals}{0}
\defres{e15/openjevhf/l3/refusals}{0}
\defres{e15/openjevhf/live}{yes}
\defres{e15/openjevhf/live_n}{200}
\defres{e15/openjevhf/live_success}{63.0}
\defres{e15/openjevhf/live_vs_jev}{$-$20.0}
\defres{e15/openjevhf/live_vs_jev/hi}{$-$14.4}
\defres{e15/openjevhf/live_vs_jev/lo}{$-$25.7}
\defres{e15/openjevhf/livecell}{63.0}
\defres{e15/openjevhf/meanconf}{96.1}
\defres{e15/openjevhf/occacc}{94.5}
\defres{e15/openjevhf/own_acc}{87.6}
\defres{e15/openjevhf/steps}{6.8}
\defres{e15/spend/gemini}{9.93}
\defres{e15/spend/openai}{1.13}
\defres{e15/spread/all/live}{93.5}
\defres{e15/spread/notrained/live}{76.5}
\defres{e15/spread/offtheshelf/live}{76.5}
\defres{e15/verdict/corpus_acc}{19.0}
\defres{e15/verdict/corpus_acc_ask}{0.0}
\defres{e15/verdict/corpus_acc_offplan}{22.1}
\defres{e15/verdict/corpus_vs_frozen}{$-$80.2}
\defres{e15/verdict/corpus_vs_frozen/hi}{$-$79.0}
\defres{e15/verdict/corpus_vs_frozen/lo}{$-$81.2}
\defres{e15/verdict/corpus_vs_jev}{$-$72.4}
\defres{e15/verdict/corpus_vs_jev/hi}{$-$71.0}
\defres{e15/verdict/corpus_vs_jev/lo}{$-$73.9}
\defres{e15/verdict/e1_acc}{78.3}
\defres{e15/verdict/e1_vs_jev}{$-$11.7}
\defres{e15/verdict/ece}{0.148}
\defres{e15/verdict/l1/errors}{11}
\defres{e15/verdict/l1/refusals}{0}
\defres{e15/verdict/l2/errors}{0}
\defres{e15/verdict/l2/refusals}{0}
\defres{e15/verdict/live}{no}
\defres{e15/verdict/livecell}{--}
\defres{e15/verdict/meanconf}{31.5}
\defres{e15/verdict/occacc}{19.6}
\defres{e9/bosun/acc}{63.3}
\defres{e9/bosun/acc/args}{56.4}
\defres{e9/bosun/acc/toolchoice}{85.8}
\defres{e9/bosun/acc/w2c}{50.8}
\defres{e9/bosun/costvsjev}{8.0}
\defres{e9/bosun/front}{no}
\defres{e9/bosun/frontall}{no}
\defres{e9/bosun/gapfrozen}{-15.4}
\defres{e9/bosun/gapjev}{-23.1}
\defres{e9/bosun/lat}{361}
\defres{e9/bosun/lg}{-3.8870}
\defres{e9/bosun/usdk}{0.13}
\defres{e9/clef/acc}{84.0}
\defres{e9/clef/acc/args}{88.8}
\defres{e9/clef/acc/toolchoice}{86.3}
\defres{e9/clef/acc/w2c}{71.3}
\defres{e9/clef/costvsjev}{41}
\defres{e9/clef/front}{no}
\defres{e9/clef/frontall}{no}
\defres{e9/clef/gapfrozen}{+5.3}
\defres{e9/clef/gapjev}{-2.4}
\defres{e9/clef/lat}{1{,}578}
\defres{e9/clef/lg}{-3.1743}
\defres{e9/clef/usdk}{0.67}
\defres{e9/clefflash/acc}{81.4}
\defres{e9/clefflash/acc/args}{85.1}
\defres{e9/clefflash/acc/toolchoice}{87.5}
\defres{e9/clefflash/acc/w2c}{66.2}
\defres{e9/clefflash/costvsjev}{6.7}
\defres{e9/clefflash/front}{no}
\defres{e9/clefflash/frontall}{no}
\defres{e9/clefflash/gapfrozen}{+2.6}
\defres{e9/clefflash/gapjev}{-5.0}
\defres{e9/clefflash/lat}{249}
\defres{e9/clefflash/lg}{-3.9640}
\defres{e9/clefflash/usdk}{0.11}
\defres{e9/clm/acc}{46.2}
\defres{e9/clm/acc/args}{41.1}
\defres{e9/clm/acc/toolchoice}{71.0}
\defres{e9/clm/acc/w2c}{27.0}
\defres{e9/clm/costvsjev}{1.9}
\defres{e9/clm/front}{no}
\defres{e9/clm/frontall}{no}
\defres{e9/clm/gapfrozen}{-32.5}
\defres{e9/clm/gapjev}{-40.2}
\defres{e9/clm/lat}{80}
\defres{e9/clm/lg}{-4.5037}
\defres{e9/clm/usdk}{0.031}
\defres{e9/decider/acc}{79.3}
\defres{e9/decider/acc/args}{76.9}
\defres{e9/decider/acc/toolchoice}{90.8}
\defres{e9/decider/acc/w2c}{70.4}
\defres{e9/decider/costvsjev}{3.3}
\defres{e9/decider/front}{no}
\defres{e9/decider/frontall}{no}
\defres{e9/decider/gapfrozen}{+0.5}
\defres{e9/decider/gapjev}{-7.1}
\defres{e9/decider/lat}{100}
\defres{e9/decider/lg}{-4.2686}
\defres{e9/decider/usdk}{0.054}
\defres{e9/front15/changed}{no}
\defres{e9/front15/first}{sl08b}
\defres{e9/front15/n}{3}
\defres{e9/front15/rest}{jev,flash}
\defres{e9/imajev/acc}{78.9}
\defres{e9/imajev/acc/args}{77.6}
\defres{e9/imajev/acc/toolchoice}{87.9}
\defres{e9/imajev/acc/w2c}{70.6}
\defres{e9/imajev/costvsjev}{70}
\defres{e9/imajev/front}{no}
\defres{e9/imajev/frontall}{no}
\defres{e9/imajev/gapfrozen}{+0.1}
\defres{e9/imajev/gapjev}{-7.5}
\defres{e9/imajev/lat}{2{,}874}
\defres{e9/imajev/lg}{-2.9432}
\defres{e9/imajev/usdk}{1.1}
\defres{e9/jevk5/acc}{70.3}
\defres{e9/jevk5/acc/args}{62.4}
\defres{e9/jevk5/acc/toolchoice}{86.4}
\defres{e9/jevk5/acc/w2c}{67.3}
\defres{e9/jevk5/costvsjev}{2.9}
\defres{e9/jevk5/front}{no}
\defres{e9/jevk5/frontall}{no}
\defres{e9/jevk5/gapfrozen}{-8.5}
\defres{e9/jevk5/gapjev}{-16.1}
\defres{e9/jevk5/lat}{111}
\defres{e9/jevk5/lg}{-4.3221}
\defres{e9/jevk5/usdk}{0.048}
\defres{e9/laya/acc}{49.4}
\defres{e9/laya/acc/args}{39.8}
\defres{e9/laya/acc/toolchoice}{79.8}
\defres{e9/laya/acc/w2c}{32.9}
\defres{e9/laya/costvsjev}{2.3}
\defres{e9/laya/front}{no}
\defres{e9/laya/frontall}{no}
\defres{e9/laya/gapfrozen}{-29.4}
\defres{e9/laya/gapjev}{-37.0}
\defres{e9/laya/lat}{90}
\defres{e9/laya/lg}{-4.4320}
\defres{e9/laya/usdk}{0.037}
\defres{e9/oaidec/acc}{79.2}
\defres{e9/oaidec/acc/args}{81.4}
\defres{e9/oaidec/acc/toolchoice}{90.6}
\defres{e9/oaidec/acc/w2c}{60.7}
\defres{e9/oaidec/costvsjev}{1.7}
\defres{e9/oaidec/front}{no}
\defres{e9/oaidec/frontall}{no}
\defres{e9/oaidec/gapfrozen}{+0.4}
\defres{e9/oaidec/gapjev}{-7.2}
\defres{e9/oaidec/lat}{158}
\defres{e9/oaidec/lg}{-4.5619}
\defres{e9/oaidec/usdk}{0.027}
\defres{e9/openjev/acc}{78.8}
\defres{e9/openjev/acc/args}{79.8}
\defres{e9/openjev/acc/toolchoice}{91.2}
\defres{e9/openjev/acc/w2c}{62.0}
\defres{e9/openjev/costvsjev}{5.6}
\defres{e9/openjev/front}{no}
\defres{e9/openjev/frontall}{no}
\defres{e9/openjev/gapfrozen}{+0.1}
\defres{e9/openjev/gapjev}{-7.6}
\defres{e9/openjev/lat}{244}
\defres{e9/openjev/lg}{-4.0421}
\defres{e9/openjev/usdk}{0.091}
\defres{e9/openjevhf/acc}{82.7}
\defres{e9/openjevhf/acc/args}{81.6}
\defres{e9/openjevhf/acc/toolchoice}{90.2}
\defres{e9/openjevhf/acc/w2c}{76.2}
\defres{e9/openjevhf/costvsjev}{15}
\defres{e9/openjevhf/front}{no}
\defres{e9/openjevhf/frontall}{no}
\defres{e9/openjevhf/gapfrozen}{+4.0}
\defres{e9/openjevhf/gapjev}{-3.7}
\defres{e9/openjevhf/lat}{542}
\defres{e9/openjevhf/lg}{-3.6231}
\defres{e9/openjevhf/usdk}{0.24}
\defres{e9/verdict/acc}{47.2}
\defres{e9/verdict/acc/args}{34.9}
\defres{e9/verdict/acc/toolchoice}{78.3}
\defres{e9/verdict/acc/w2c}{35.5}
\defres{e9/verdict/costvsjev}{1.3}
\defres{e9/verdict/front}{no}
\defres{e9/verdict/frontall}{no}
\defres{e9/verdict/gapfrozen}{-31.6}
\defres{e9/verdict/gapjev}{-39.2}
\defres{e9/verdict/lat}{53}
\defres{e9/verdict/lg}{-4.6608}
\defres{e9/verdict/usdk}{0.022}
\makeatother


==> generated/e16_best_open.tex <==
\makeatletter
\providecommand{\res}[1]{\ifcsname jevres@#1\endcsname\csname jevres@#1\endcsname\else\tbd\fi}
\providecommand{\defres}[2]{\expandafter\def\csname jevres@#1\endcsname{#2}}
\defres{e16/a/best_open/l1}{no}
\defres{e16/a/best_open/l1/gap}{$-$3.4}
\defres{e16/a/best_open/l1/gapabs}{3.4}
\defres{e16/a/best_open/l1/model}{StartLux-27B (Q8\_0)}
\defres{e16/a/best_open/l2}{yes}
\defres{e16/a/best_open/l2/gap}{+5.2}
\defres{e16/a/best_open/l2/gapabs}{5.2}
\defres{e16/a/best_open/l2/model}{StartLux-27B (Q8\_0)}
\defres{e16/a/best_open/l3}{yes}
\defres{e16/a/best_open/l3/gap}{+26.0}
\defres{e16/a/best_open/l3/gapabs}{26.0}
\defres{e16/a/best_open/l3/model}{StartLux-9B}
\defres{e16/a/c/acc}{99.1}
\defres{e16/a/c/ask}{100.0}
\defres{e16/a/c/avail}{yes}
\defres{e16/a/c/delta}{$-$0.1}
\defres{e16/a/c/delta/hi}{+0.2}
\defres{e16/a/c/delta/lo}{$-$0.3}
\defres{e16/a/c/n}{5{,}314}
\defres{e16/a/c/ni}{yes}
\defres{e16/a/c/offplan}{93.5}
\defres{e16/a/c/offplan/delta}{$-$1.2}
\defres{e16/a/c/offplan/hi}{+1.3}
\defres{e16/a/c/offplan/lo}{$-$5.2}
\defres{e16/a/c/vsbestopen}{+5.2}
\defres{e16/a/c/vsbestopen/hi}{+6.2}
\defres{e16/a/c/vsbestopen/lo}{+4.2}
\defres{e16/a/e1/acc}{84.3}
\defres{e16/a/e1/acc/args}{90.1}
\defres{e16/a/e1/acc/hi}{85.4}
\defres{e16/a/e1/acc/lo}{83.2}
\defres{e16/a/e1/acc/toolchoice}{88.8}
\defres{e16/a/e1/acc/w2c}{66.9}
\defres{e16/a/e1/avail}{yes}
\defres{e16/a/e1/lat}{260}
\defres{e16/a/e1/usdk}{0.0909}
\defres{e16/a/e1/vs/bestopen/all}{$-$3.4}
\defres{e16/a/e1/vs/bestopen/all/abs}{3.4}
\defres{e16/a/e1/vs/bestopen/all/hi}{$-$2.2}
\defres{e16/a/e1/vs/bestopen/all/lo}{$-$4.5}
\defres{e16/a/e1/vs/bestopen/args}{+1.0}
\defres{e16/a/e1/vs/bestopen/args/abs}{1.0}
\defres{e16/a/e1/vs/bestopen/args/hi}{+2.5}
\defres{e16/a/e1/vs/bestopen/args/lo}{$-$0.4}
\defres{e16/a/e1/vs/bestopen/toolchoice}{$-$2.0}
\defres{e16/a/e1/vs/bestopen/toolchoice/abs}{2.0}
\defres{e16/a/e1/vs/bestopen/toolchoice/hi}{$-$0.2}
\defres{e16/a/e1/vs/bestopen/toolchoice/lo}{$-$3.8}
\defres{e16/a/e1/vs/bestopen/w2c}{$-$14.3}
\defres{e16/a/e1/vs/bestopen/w2c/abs}{14.3}
\defres{e16/a/e1/vs/bestopen/w2c/hi}{$-$11.1}
\defres{e16/a/e1/vs/bestopen/w2c/lo}{$-$17.6}
\defres{e16/a/e1/vs/e12/all}{$-$0.7}
\defres{e16/a/e1/vs/e12/all/abs}{0.7}
\defres{e16/a/e1/vs/e12/all/hi}{+0.1}
\defres{e16/a/e1/vs/e12/all/lo}{$-$1.6}
\defres{e16/a/e1/vs/e12/args}{$-$0.4}
\defres{e16/a/e1/vs/e12/args/abs}{0.4}
\defres{e16/a/e1/vs/e12/args/hi}{+0.7}
\defres{e16/a/e1/vs/e12/args/lo}{$-$1.4}
\defres{e16/a/e1/vs/e12/toolchoice}{$-$0.5}
\defres{e16/a/e1/vs/e12/toolchoice/abs}{0.5}
\defres{e16/a/e1/vs/e12/toolchoice/hi}{+1.0}
\defres{e16/a/e1/vs/e12/toolchoice/lo}{$-$2.1}
\defres{e16/a/e1/vs/e12/w2c}{$-$1.6}
\defres{e16/a/e1/vs/e12/w2c/abs}{1.6}
\defres{e16/a/e1/vs/e12/w2c/hi}{+0.8}
\defres{e16/a/e1/vs/e12/w2c/lo}{$-$4.0}
\defres{e16/a/e1/vs/frozen/all}{+5.6}
\defres{e16/a/e1/vs/frozen/all/abs}{5.6}
\defres{e16/a/e1/vs/frozen/all/hi}{+6.8}
\defres{e16/a/e1/vs/frozen/all/lo}{+4.4}
\defres{e16/a/e1/vs/frozen/args}{+5.1}
\defres{e16/a/e1/vs/frozen/args/abs}{5.1}
\defres{e16/a/e1/vs/frozen/args/hi}{+6.5}
\defres{e16/a/e1/vs/frozen/args/lo}{+3.7}
\defres{e16/a/e1/vs/frozen/toolchoice}{+0.4}
\defres{e16/a/e1/vs/frozen/toolchoice/abs}{0.4}
\defres{e16/a/e1/vs/frozen/toolchoice/hi}{+2.1}
\defres{e16/a/e1/vs/frozen/toolchoice/lo}{$-$1.3}
\defres{e16/a/e1/vs/frozen/w2c}{+12.9}
\defres{e16/a/e1/vs/frozen/w2c/abs}{12.9}
\defres{e16/a/e1/vs/frozen/w2c/hi}{+16.7}
\defres{e16/a/e1/vs/frozen/w2c/lo}{+9.2}
\defres{e16/a/e1/vs/jev/all}{$-$2.1}
\defres{e16/a/e1/vs/jev/all/abs}{2.1}
\defres{e16/a/e1/vs/jev/all/hi}{$-$1.0}
\defres{e16/a/e1/vs/jev/all/lo}{$-$3.2}
\defres{e16/a/e1/vs/jev/args}{+0.5}
\defres{e16/a/e1/vs/jev/args/abs}{0.5}
\defres{e16/a/e1/vs/jev/args/hi}{+2.0}
\defres{e16/a/e1/vs/jev/args/lo}{$-$1.0}
\defres{e16/a/e1/vs/jev/toolchoice}{$-$1.2}
\defres{e16/a/e1/vs/jev/toolchoice/abs}{1.2}
\defres{e16/a/e1/vs/jev/toolchoice/hi}{+0.5}
\defres{e16/a/e1/vs/jev/toolchoice/lo}{$-$3.0}
\defres{e16/a/e1/vs/jev/w2c}{$-$8.5}
\defres{e16/a/e1/vs/jev/w2c/abs}{8.5}
\defres{e16/a/e1/vs/jev/w2c/hi}{$-$5.3}
\defres{e16/a/e1/vs/jev/w2c/lo}{$-$11.6}
\defres{e16/a/e1/vs/sl27b/all}{$-$3.4}
\defres{e16/a/e1/vs/sl27b/all/abs}{3.4}
\defres{e16/a/e1/vs/sl27b/all/hi}{$-$2.2}
\defres{e16/a/e1/vs/sl27b/all/lo}{$-$4.5}
\defres{e16/a/e1/vs/sl27b/args}{+1.0}
\defres{e16/a/e1/vs/sl27b/args/abs}{1.0}
\defres{e16/a/e1/vs/sl27b/args/hi}{+2.5}
\defres{e16/a/e1/vs/sl27b/args/lo}{$-$0.4}
\defres{e16/a/e1/vs/sl27b/toolchoice}{$-$2.0}
\defres{e16/a/e1/vs/sl27b/toolchoice/abs}{2.0}
\defres{e16/a/e1/vs/sl27b/toolchoice/hi}{$-$0.2}
\defres{e16/a/e1/vs/sl27b/toolchoice/lo}{$-$3.8}
\defres{e16/a/e1/vs/sl27b/w2c}{$-$14.3}
\defres{e16/a/e1/vs/sl27b/w2c/abs}{14.3}
\defres{e16/a/e1/vs/sl27b/w2c/hi}{$-$11.1}
\defres{e16/a/e1/vs/sl27b/w2c/lo}{$-$17.6}
\defres{e16/a/e1/vs/sl4b/all}{+1.2}
\defres{e16/a/e1/vs/sl4b/all/abs}{1.2}
\defres{e16/a/e1/vs/sl4b/all/hi}{+2.4}
\defres{e16/a/e1/vs/sl4b/all/lo}{$-$0.1}
\defres{e16/a/e1/vs/sl4b/args}{+8.9}
\defres{e16/a/e1/vs/sl4b/args/abs}{8.9}
\defres{e16/a/e1/vs/sl4b/args/hi}{+10.7}
\defres{e16/a/e1/vs/sl4b/args/lo}{+7.0}
\defres{e16/a/e1/vs/sl4b/toolchoice}{$-$2.5}
\defres{e16/a/e1/vs/sl4b/toolchoice/abs}{2.5}
\defres{e16/a/e1/vs/sl4b/toolchoice/hi}{$-$0.9}
\defres{e16/a/e1/vs/sl4b/toolchoice/lo}{$-$4.1}
\defres{e16/a/e1/vs/sl4b/w2c}{$-$10.5}
\defres{e16/a/e1/vs/sl4b/w2c/abs}{10.5}
\defres{e16/a/e1/vs/sl4b/w2c/hi}{$-$7.2}
\defres{e16/a/e1/vs/sl4b/w2c/lo}{$-$13.7}
\defres{e16/a/e1/vs/sl9b/all}{+0.9}
\defres{e16/a/e1/vs/sl9b/all/abs}{0.9}
\defres{e16/a/e1/vs/sl9b/all/hi}{+2.1}
\defres{e16/a/e1/vs/sl9b/all/lo}{$-$0.4}
\defres{e16/a/e1/vs/sl9b/args}{+9.1}
\defres{e16/a/e1/vs/sl9b/args/abs}{9.1}
\defres{e16/a/e1/vs/sl9b/args/hi}{+10.9}
\defres{e16/a/e1/vs/sl9b/args/lo}{+7.4}
\defres{e16/a/e1/vs/sl9b/toolchoice}{$-$3.4}
\defres{e16/a/e1/vs/sl9b/toolchoice/abs}{3.4}
\defres{e16/a/e1/vs/sl9b/toolchoice/hi}{$-$1.7}
\defres{e16/a/e1/vs/sl9b/toolchoice/lo}{$-$5.1}
\defres{e16/a/e1/vs/sl9b/w2c}{$-$11.2}
\defres{e16/a/e1/vs/sl9b/w2c/abs}{11.2}
\defres{e16/a/e1/vs/sl9b/w2c/hi}{$-$8.1}
\defres{e16/a/e1/vs/sl9b/w2c/lo}{$-$14.2}
\defres{e16/a/e1/w2c/askt}{66.9}
\defres{e16/a/e1/w2c/call}{69.3}
\defres{e16/a/e1/w2c/sayi}{64.6}
\defres{e16/a/live/avail}{yes}
\defres{e16/a/live/gate}{yes}
\defres{e16/a/live/n}{200}
\defres{e16/a/live/own}{99.9}
\defres{e16/a/live/steps}{7.5}
\defres{e16/a/live/success}{100.0}
\defres{e16/a/live/usdep}{0.0145}
\defres{e16/a/live/vs/bestopen}{+26.0}
\defres{e16/a/live/vs/bestopen/hi}{+32.5}
\defres{e16/a/live/vs/bestopen/lo}{+20.1}
\defres{e16/a/live/vs/frozen}{+0.0}
\defres{e16/a/live/vs/frozen/hi}{+1.9}
\defres{e16/a/live/vs/frozen/lo}{$-$1.9}
\defres{e16/a/live/vs/jev}{+17.0}
\defres{e16/a/live/vs/jev/hi}{+22.8}
\defres{e16/a/live/vs/jev/lo}{+12.1}
\defres{e16/a/live/walls}{11}
\defres{e16/a/name}{AgentDecision-4B (mixed+)}
\defres{e16/a/sel/ep1/devprefix}{87.2}
\defres{e16/a/sel/ep1/v1dev}{99.7}
\defres{e16/a/sel/ep2/devprefix}{87.2}
\defres{e16/a/sel/ep2/v1dev}{99.7}
\defres{e16/a/sel/epoch}{2}
\defres{e16/a/train/min}{145}
\defres{e16/a/train/setting}{nogc\_3072}
\defres{e16/audit/items}{485}
\defres{e16/audit/units}{207}
\defres{e16/b/best_open/l1}{no}
\defres{e16/b/best_open/l1/gap}{$-$2.9}
\defres{e16/b/best_open/l1/gapabs}{2.9}
\defres{e16/b/best_open/l1/model}{StartLux-27B (Q8\_0)}
\defres{e16/b/best_open/l2}{yes}
\defres{e16/b/best_open/l2/gap}{+5.4}
\defres{e16/b/best_open/l2/gapabs}{5.4}
\defres{e16/b/best_open/l2/model}{StartLux-27B (Q8\_0)}
\defres{e16/b/best_open/l3}{yes}
\defres{e16/b/best_open/l3/gap}{+26.0}
\defres{e16/b/best_open/l3/gapabs}{26.0}
\defres{e16/b/best_open/l3/model}{StartLux-9B}
\defres{e16/b/c/acc}{99.3}
\defres{e16/b/c/ask}{100.0}
\defres{e16/b/c/avail}{yes}
\defres{e16/b/c/delta}{+0.1}
\defres{e16/b/c/delta/hi}{+0.4}
\defres{e16/b/c/delta/lo}{$-$0.1}
\defres{e16/b/c/n}{5{,}314}
\defres{e16/b/c/ni}{yes}
\defres{e16/b/c/offplan}{95.0}
\defres{e16/b/c/offplan/delta}{+0.3}
\defres{e16/b/c/offplan/hi}{+1.9}
\defres{e16/b/c/offplan/lo}{$-$1.0}
\defres{e16/b/c/vsbestopen}{+5.4}
\defres{e16/b/c/vsbestopen/hi}{+6.3}
\defres{e16/b/c/vsbestopen/lo}{+4.4}
\defres{e16/b/e1/acc}{84.8}
\defres{e16/b/e1/acc/args}{91.9}
\defres{e16/b/e1/acc/hi}{85.9}
\defres{e16/b/e1/acc/lo}{83.7}
\defres{e16/b/e1/acc/toolchoice}{90.0}
\defres{e16/b/e1/acc/w2c}{63.6}
\defres{e16/b/e1/avail}{yes}
\defres{e16/b/e1/lat}{604}
\defres{e16/b/e1/usdk}{0.2404}
\defres{e16/b/e1/vs/bestopen/all}{$-$2.9}
\defres{e16/b/e1/vs/bestopen/all/abs}{2.9}
\defres{e16/b/e1/vs/bestopen/all/hi}{$-$1.7}
\defres{e16/b/e1/vs/bestopen/all/lo}{$-$4.0}
\defres{e16/b/e1/vs/bestopen/args}{+2.9}
\defres{e16/b/e1/vs/bestopen/args/abs}{2.9}
\defres{e16/b/e1/vs/bestopen/args/hi}{+4.2}
\defres{e16/b/e1/vs/bestopen/args/lo}{+1.6}
\defres{e16/b/e1/vs/bestopen/toolchoice}{$-$0.7}
\defres{e16/b/e1/vs/bestopen/toolchoice/abs}{0.7}
\defres{e16/b/e1/vs/bestopen/toolchoice/hi}{+1.0}
\defres{e16/b/e1/vs/bestopen/toolchoice/lo}{$-$2.4}
\defres{e16/b/e1/vs/bestopen/w2c}{$-$17.7}
\defres{e16/b/e1/vs/bestopen/w2c/abs}{17.7}
\defres{e16/b/e1/vs/bestopen/w2c/hi}{$-$14.1}
\defres{e16/b/e1/vs/bestopen/w2c/lo}{$-$21.1}
\defres{e16/b/e1/vs/e12c/all}{$-$0.7}
\defres{e16/b/e1/vs/e12c/all/abs}{0.7}
\defres{e16/b/e1/vs/e12c/all/hi}{+0.4}
\defres{e16/b/e1/vs/e12c/all/lo}{$-$1.7}
\defres{e16/b/e1/vs/e12c/args}{+0.1}
\defres{e16/b/e1/vs/e12c/args/abs}{0.1}
\defres{e16/b/e1/vs/e12c/args/hi}{+1.1}
\defres{e16/b/e1/vs/e12c/args/lo}{$-$1.1}
\defres{e16/b/e1/vs/e12c/toolchoice}{+0.5}
\defres{e16/b/e1/vs/e12c/toolchoice/abs}{0.5}
\defres{e16/b/e1/vs/e12c/toolchoice/hi}{+1.9}
\defres{e16/b/e1/vs/e12c/toolchoice/lo}{$-$0.8}
\defres{e16/b/e1/vs/e12c/w2c}{$-$3.6}
\defres{e16/b/e1/vs/e12c/w2c/abs}{3.6}
\defres{e16/b/e1/vs/e12c/w2c/hi}{+0.0}
\defres{e16/b/e1/vs/e12c/w2c/lo}{$-$6.9}
\defres{e16/b/e1/vs/frozen/all}{+6.1}
\defres{e16/b/e1/vs/frozen/all/abs}{6.1}
\defres{e16/b/e1/vs/frozen/all/hi}{+7.5}
\defres{e16/b/e1/vs/frozen/all/lo}{+4.6}
\defres{e16/b/e1/vs/frozen/args}{+6.9}
\defres{e16/b/e1/vs/frozen/args/abs}{6.9}
\defres{e16/b/e1/vs/frozen/args/hi}{+8.5}
\defres{e16/b/e1/vs/frozen/args/lo}{+5.3}
\defres{e16/b/e1/vs/frozen/toolchoice}{+1.6}
\defres{e16/b/e1/vs/frozen/toolchoice/abs}{1.6}
\defres{e16/b/e1/vs/frozen/toolchoice/hi}{+3.4}
\defres{e16/b/e1/vs/frozen/toolchoice/lo}{$-$0.2}
\defres{e16/b/e1/vs/frozen/w2c}{+9.6}
\defres{e16/b/e1/vs/frozen/w2c/abs}{9.6}
\defres{e16/b/e1/vs/frozen/w2c/hi}{+14.7}
\defres{e16/b/e1/vs/frozen/w2c/lo}{+4.5}
\defres{e16/b/e1/vs/jev/all}{$-$1.6}
\defres{e16/b/e1/vs/jev/all/abs}{1.6}
\defres{e16/b/e1/vs/jev/all/hi}{$-$0.5}
\defres{e16/b/e1/vs/jev/all/lo}{$-$2.8}
\defres{e16/b/e1/vs/jev/args}{+2.4}
\defres{e16/b/e1/vs/jev/args/abs}{2.4}
\defres{e16/b/e1/vs/jev/args/hi}{+3.7}
\defres{e16/b/e1/vs/jev/args/lo}{+0.9}
\defres{e16/b/e1/vs/jev/toolchoice}{+0.1}
\defres{e16/b/e1/vs/jev/toolchoice/abs}{0.1}
\defres{e16/b/e1/vs/jev/toolchoice/hi}{+1.5}
\defres{e16/b/e1/vs/jev/toolchoice/lo}{$-$1.4}
\defres{e16/b/e1/vs/jev/w2c}{$-$11.9}
\defres{e16/b/e1/vs/jev/w2c/abs}{11.9}
\defres{e16/b/e1/vs/jev/w2c/hi}{$-$8.4}
\defres{e16/b/e1/vs/jev/w2c/lo}{$-$15.5}
\defres{e16/b/e1/vs/sl27b/all}{$-$2.9}
\defres{e16/b/e1/vs/sl27b/all/abs}{2.9}
\defres{e16/b/e1/vs/sl27b/all/hi}{$-$1.7}
\defres{e16/b/e1/vs/sl27b/all/lo}{$-$4.0}
\defres{e16/b/e1/vs/sl27b/args}{+2.9}
\defres{e16/b/e1/vs/sl27b/args/abs}{2.9}
\defres{e16/b/e1/vs/sl27b/args/hi}{+4.2}
\defres{e16/b/e1/vs/sl27b/args/lo}{+1.6}
\defres{e16/b/e1/vs/sl27b/toolchoice}{$-$0.7}
\defres{e16/b/e1/vs/sl27b/toolchoice/abs}{0.7}
\defres{e16/b/e1/vs/sl27b/toolchoice/hi}{+1.0}
\defres{e16/b/e1/vs/sl27b/toolchoice/lo}{$-$2.4}
\defres{e16/b/e1/vs/sl27b/w2c}{$-$17.7}
\defres{e16/b/e1/vs/sl27b/w2c/abs}{17.7}
\defres{e16/b/e1/vs/sl27b/w2c/hi}{$-$14.1}
\defres{e16/b/e1/vs/sl27b/w2c/lo}{$-$21.1}
\defres{e16/b/e1/vs/sl4b/all}{+1.7}
\defres{e16/b/e1/vs/sl4b/all/abs}{1.7}
\defres{e16/b/e1/vs/sl4b/all/hi}{+3.0}
\defres{e16/b/e1/vs/sl4b/all/lo}{+0.5}
\defres{e16/b/e1/vs/sl4b/args}{+10.7}
\defres{e16/b/e1/vs/sl4b/args/abs}{10.7}
\defres{e16/b/e1/vs/sl4b/args/hi}{+12.4}
\defres{e16/b/e1/vs/sl4b/args/lo}{+8.9}
\defres{e16/b/e1/vs/sl4b/toolchoice}{$-$1.3}
\defres{e16/b/e1/vs/sl4b/toolchoice/abs}{1.3}
\defres{e16/b/e1/vs/sl4b/toolchoice/hi}{+0.1}
\defres{e16/b/e1/vs/sl4b/toolchoice/lo}{$-$2.7}
\defres{e16/b/e1/vs/sl4b/w2c}{$-$13.8}
\defres{e16/b/e1/vs/sl4b/w2c/abs}{13.8}
\defres{e16/b/e1/vs/sl4b/w2c/hi}{$-$10.5}
\defres{e16/b/e1/vs/sl4b/w2c/lo}{$-$17.0}
\defres{e16/b/e1/vs/sl9b/all}{+1.4}
\defres{e16/b/e1/vs/sl9b/all/abs}{1.4}
\defres{e16/b/e1/vs/sl9b/all/hi}{+2.6}
\defres{e16/b/e1/vs/sl9b/all/lo}{+0.2}
\defres{e16/b/e1/vs/sl9b/args}{+11.0}
\defres{e16/b/e1/vs/sl9b/args/abs}{11.0}
\defres{e16/b/e1/vs/sl9b/args/hi}{+12.6}
\defres{e16/b/e1/vs/sl9b/args/lo}{+9.3}
\defres{e16/b/e1/vs/sl9b/toolchoice}{$-$2.2}
\defres{e16/b/e1/vs/sl9b/toolchoice/abs}{2.2}
\defres{e16/b/e1/vs/sl9b/toolchoice/hi}{$-$0.7}
\defres{e16/b/e1/vs/sl9b/toolchoice/lo}{$-$3.7}
\defres{e16/b/e1/vs/sl9b/w2c}{$-$14.5}
\defres{e16/b/e1/vs/sl9b/w2c/abs}{14.5}
\defres{e16/b/e1/vs/sl9b/w2c/hi}{$-$11.6}
\defres{e16/b/e1/vs/sl9b/w2c/lo}{$-$17.5}
\defres{e16/b/e1/w2c/askt}{14.3}
\defres{e16/b/e1/w2c/call}{93.6}
\defres{e16/b/e1/w2c/sayi}{73.3}
\defres{e16/b/live/avail}{yes}
\defres{e16/b/live/gate}{yes}
\defres{e16/b/live/n}{200}
\defres{e16/b/live/own}{100.0}
\defres{e16/b/live/steps}{7.5}
\defres{e16/b/live/success}{100.0}
\defres{e16/b/live/usdep}{0.0145}
\defres{e16/b/live/vs/bestopen}{+26.0}
\defres{e16/b/live/vs/bestopen/hi}{+32.5}
\defres{e16/b/live/vs/bestopen/lo}{+20.1}
\defres{e16/b/live/vs/frozen}{+0.0}
\defres{e16/b/live/vs/frozen/hi}{+1.9}
\defres{e16/b/live/vs/frozen/lo}{$-$1.9}
\defres{e16/b/live/vs/jev}{+17.0}
\defres{e16/b/live/vs/jev/hi}{+22.8}
\defres{e16/b/live/vs/jev/lo}{+12.1}
\defres{e16/b/live/walls}{22}
\defres{e16/b/name}{StartLux-9B (mixed)}
\defres{e16/b/plan}{run}
\defres{e16/b/plan/epochs}{2}
\defres{e16/b/plan/minperepoch}{205}
\defres{e16/b/sel/ep1/devprefix}{86.9}
\defres{e16/b/sel/ep1/v1dev}{99.7}
\defres{e16/b/sel/ep2/devprefix}{87.9}
\defres{e16/b/sel/ep2/v1dev}{99.8}
\defres{e16/b/sel/epoch}{2}
\defres{e16/b/train/epochs}{2}
\defres{e16/b/train/min}{303}
\defres{e16/b/train/setting}{gc\_3072}
\defres{e16/best_open/l1/model}{StartLux-27B (Q8\_0)}
\defres{e16/best_open/l1/value}{87.7}
\defres{e16/best_open/l2/model}{StartLux-27B (Q8\_0)}
\defres{e16/best_open/l2/value}{93.9}
\defres{e16/best_open/l3/model}{StartLux-9B}
\defres{e16/best_open/l3/value}{74.0}
\defres{e16/data/bfclargs}{2{,}600}
\defres{e16/data/bfclnone}{1{,}000}
\defres{e16/data/bfcltool}{1{,}892}
\defres{e16/data/new}{13{,}992}
\defres{e16/data/replay}{13{,}992}
\defres{e16/data/total}{27{,}984}
\defres{e16/data/units}{11{,}392}
\defres{e16/data/w2cask}{3{,}000}
\defres{e16/data/w2ccall}{2{,}500}
\defres{e16/data/w2ccannot}{3{,}000}
\defres{e16/fast/e16a/agree}{99.6}
\defres{e16/fast/e16a/c1/p50}{20}
\defres{e16/fast/e16a/c1/usdkwall}{0.0080}
\defres{e16/fast/e16a/c4/p50}{56}
\defres{e16/fast/e16a/c4/usdkwall}{0.0047}
\defres{e16/fast/e16a/gb}{8.0}
\defres{e16/fast/e16a/msdec}{7.5}
\defres{e16/fast/e16a/usdke9}{0.0188}
\defres{e16/fast/e16a/usdkwall}{0.0047}
\defres{e16/fast/e16b/agree}{99.9}
\defres{e16/fast/e16b/c1/p50}{50}
\defres{e16/fast/e16b/c1/usdkwall}{0.0204}
\defres{e16/fast/e16b/c4/p50}{171}
\defres{e16/fast/e16b/c4/usdkwall}{0.0140}
\defres{e16/fast/e16b/gb}{17.9}
\defres{e16/fast/e16b/msdec}{22.5}
\defres{e16/fast/e16b/usdke9}{0.0560}
\defres{e16/fast/e16b/usdkwall}{0.0140}
\defres{e16/fast/frozen/agree}{99.8}
\defres{e16/fast/frozen/c1/p50}{20}
\defres{e16/fast/frozen/c1/usdkwall}{0.0082}
\defres{e16/fast/frozen/c4/p50}{56}
\defres{e16/fast/frozen/c4/usdkwall}{0.0047}
\defres{e16/fast/frozen/gb}{8.0}
\defres{e16/fast/frozen/msdec}{7.5}
\defres{e16/fast/frozen/usdke9}{0.0188}
\defres{e16/fast/frozen/usdkwall}{0.0047}
\defres{e16/gpuh}{10.2}
\defres{e16/host/type}{g6e.2xlarge}
\defres{e16/rehost/agree}{99.8}
\defres{e16/rehost/factor}{1.01}
\defres{e16/rehost/usdk}{0.0925}
\defres{e16/row/bosun/l1}{63.3}
\defres{e16/row/bosun/l2}{36.3}
\defres{e16/row/bosun/l2ask}{49.2}
\defres{e16/row/clef/l1}{84.0}
\defres{e16/row/clefflash/l1}{81.4}
\defres{e16/row/clefflash/l2}{47.7}
\defres{e16/row/clefflash/l2ask}{25.0}
\defres{e16/row/clm/l1}{46.2}
\defres{e16/row/clm/l2}{11.9}
\defres{e16/row/clm/l2ask}{36.2}
\defres{e16/row/decider/l1}{79.3}
\defres{e16/row/decider/l2}{63.2}
\defres{e16/row/decider/l2ask}{57.8}
\defres{e16/row/e12/l1}{85.1}
\defres{e16/row/e12/l2}{99.1}
\defres{e16/row/e12/l2ask}{99.9}
\defres{e16/row/e12/l3}{100.0}
\defres{e16/row/e12c/l1}{85.5}
\defres{e16/row/e12c/l2}{99.6}
\defres{e16/row/e12c/l2ask}{100.0}
\defres{e16/row/e12c/l3}{100.0}
\defres{e16/row/frozen/l1}{78.8}
\defres{e16/row/frozen/l2}{99.2}
\defres{e16/row/frozen/l2ask}{100.0}
\defres{e16/row/frozen/l3}{100.0}
\defres{e16/row/imajev/l1}{78.9}
\defres{e16/row/imajev/l2}{76.9}
\defres{e16/row/imajev/l2ask}{49.0}
\defres{e16/row/intern/l1}{73.4}
\defres{e16/row/intern/l2}{75.2}
\defres{e16/row/intern/l2ask}{59.6}
\defres{e16/row/intern/l3}{26.5}
\defres{e16/row/jevk5/l1}{70.3}
\defres{e16/row/jevk5/l2}{65.0}
\defres{e16/row/jevk5/l2ask}{60.0}
\defres{e16/row/laya/l1}{49.4}
\defres{e16/row/laya/l2}{11.0}
\defres{e16/row/laya/l2ask}{1.5}
\defres{e16/row/openjev/l1}{78.8}
\defres{e16/row/openjev/l2}{91.1}
\defres{e16/row/openjev/l2ask}{87.5}
\defres{e16/row/openjev/l3}{62.5}
\defres{e16/row/openjevhf/l1}{82.7}
\defres{e16/row/openjevhf/l2}{92.4}
\defres{e16/row/openjevhf/l2ask}{63.5}
\defres{e16/row/openjevhf/l3}{63.0}
\defres{e16/row/sl08b/l1}{70.0}
\defres{e16/row/sl08b/l2}{48.3}
\defres{e16/row/sl08b/l2ask}{49.4}
\defres{e16/row/sl08b/l3}{17.5}
\defres{e16/row/sl27b/l1}{87.7}
\defres{e16/row/sl27b/l2}{93.9}
\defres{e16/row/sl27b/l2ask}{63.4}
\defres{e16/row/sl27b/l3}{63.0}
\defres{e16/row/sl2b/l1}{75.7}
\defres{e16/row/sl2b/l2}{68.4}
\defres{e16/row/sl2b/l2ask}{61.8}
\defres{e16/row/sl2b/l3}{6.5}
\defres{e16/row/sl4b/l1}{83.1}
\defres{e16/row/sl4b/l2}{89.1}
\defres{e16/row/sl4b/l2ask}{84.1}
\defres{e16/row/sl4b/l3}{60.0}
\defres{e16/row/sl9b/l1}{83.4}
\defres{e16/row/sl9b/l2}{91.8}
\defres{e16/row/sl9b/l2ask}{87.1}
\defres{e16/row/sl9b/l3}{74.0}
\defres{e16/row/verdict/l1}{47.2}
\defres{e16/row/verdict/l2}{19.0}
\defres{e16/row/verdict/l2ask}{0.0}
\defres{e16/spend}{5.85}
\makeatother


==> generated/e17_e18.tex <==
\makeatletter
\providecommand{\res}[1]{\ifcsname jevres@#1\endcsname\csname jevres@#1\endcsname\else\tbd\fi}
\providecommand{\defres}[2]{\expandafter\def\csname jevres@#1\endcsname{#2}}
\defres{e17/e18f/c/acc}{99.1}
\defres{e17/e18f/c/ask}{100.0}
\defres{e17/e18f/c/ece}{0.012}
\defres{e17/e18f/c/offplan}{86.2}
\defres{e17/e18f/c/vshead/all}{$-$0.1}
\defres{e17/e18f/c/vshead/all/hi}{0.2}
\defres{e17/e18f/c/vshead/all/lo}{$-$0.3}
\defres{e17/e18f/c/vshead/ask}{0.0}
\defres{e17/e18f/c/vshead/ask/hi}{0.0}
\defres{e17/e18f/c/vshead/ask/lo}{0.0}
\defres{e17/e18f/c/vshead/offplan}{$-$8.0}
\defres{e17/e18f/c/vshead/offplan/hi}{$-$2.6}
\defres{e17/e18f/c/vshead/offplan/lo}{$-$14.0}
\defres{e17/e18f/c/vsrl/all}{$-$0.1}
\defres{e17/e18f/c/vsrl/all/hi}{0.4}
\defres{e17/e18f/c/vsrl/all/lo}{$-$0.4}
\defres{e17/e18f/c/vsrl/ask}{0.0}
\defres{e17/e18f/c/vsrl/ask/hi}{0.0}
\defres{e17/e18f/c/vsrl/ask/lo}{0.0}
\defres{e17/e18f/c/vsrl/offplan}{$-$8.6}
\defres{e17/e18f/c/vsrl/offplan/hi}{$-$2.9}
\defres{e17/e18f/c/vsrl/offplan/lo}{$-$14.8}
\defres{e17/e18f/c/vssftv1/all}{$-$0.0}
\defres{e17/e18f/c/vssftv1/all/hi}{0.4}
\defres{e17/e18f/c/vssftv1/all/lo}{$-$0.3}
\defres{e17/e18f/c/vssftv1/ask}{0.0}
\defres{e17/e18f/c/vssftv1/ask/hi}{0.0}
\defres{e17/e18f/c/vssftv1/ask/lo}{0.0}
\defres{e17/e18f/c/vssftv1/offplan}{$-$7.6}
\defres{e17/e18f/c/vssftv1/offplan/hi}{$-$1.8}
\defres{e17/e18f/c/vssftv1/offplan/lo}{$-$14.0}
\defres{e17/e18f/v1/acc}{99.7}
\defres{e17/e18f/v1/ece}{0.002}
\defres{e17/e18f/v1/ko}{100.0}
\defres{e17/e18f/v1/rec}{99.7}
\defres{e17/e18f/v1/stop}{99.3}
\defres{e17/e18f/v1/tp}{99.9}
\defres{e17/e18f/v1/ts}{99.9}
\defres{e17/fourb/cal/tp/acc}{99.9}
\defres{e17/fourb/cal/tp/casc}{99.9}
\defres{e17/fourb/cal/tp/clean}{no}
\defres{e17/fourb/cal/tp/cov}{77.5}
\defres{e17/fourb/cal/tp/errors}{1}
\defres{e17/fourb/cal/tp/llmacc}{100.0}
\defres{e17/fourb/cal/tp/n}{1{,}328}
\defres{e17/fourb/cal/tp/tau}{0.999999880791}
\defres{e17/fourb/cal/tp/taushort}{1.0000}
\defres{e17/fourb/cal/ts/acc}{100.0}
\defres{e17/fourb/cal/ts/casc}{100.0}
\defres{e17/fourb/cal/ts/clean}{yes}
\defres{e17/fourb/cal/ts/cov}{100.0}
\defres{e17/fourb/cal/ts/errors}{0}
\defres{e17/fourb/cal/ts/llmacc}{100.0}
\defres{e17/fourb/cal/ts/n}{1{,}125}
\defres{e17/fourb/cal/ts/tau}{0.499999999998}
\defres{e17/fourb/cal/ts/taushort}{0.5000}
\defres{e17/gen/c/acc}{99.0}
\defres{e17/gen/c/ask}{100.0}
\defres{e17/gen/c/ece}{0.014}
\defres{e17/gen/c/offplan}{92.3}
\defres{e17/gen/c/vshead/all}{$-$0.2}
\defres{e17/gen/c/vshead/all/hi}{$-$0.0}
\defres{e17/gen/c/vshead/all/lo}{$-$0.4}
\defres{e17/gen/c/vshead/ask}{0.0}
\defres{e17/gen/c/vshead/ask/hi}{0.0}
\defres{e17/gen/c/vshead/ask/lo}{0.0}
\defres{e17/gen/c/vshead/offplan}{$-$1.8}
\defres{e17/gen/c/vshead/offplan/hi}{$-$0.2}
\defres{e17/gen/c/vshead/offplan/lo}{$-$3.6}
\defres{e17/gen/c/vsrl/all}{$-$0.2}
\defres{e17/gen/c/vsrl/all/hi}{0.0}
\defres{e17/gen/c/vsrl/all/lo}{$-$0.5}
\defres{e17/gen/c/vsrl/ask}{0.0}
\defres{e17/gen/c/vsrl/ask/hi}{0.0}
\defres{e17/gen/c/vsrl/ask/lo}{0.0}
\defres{e17/gen/c/vsrl/offplan}{$-$2.4}
\defres{e17/gen/c/vsrl/offplan/hi}{$-$0.8}
\defres{e17/gen/c/vsrl/offplan/lo}{$-$4.4}
\defres{e17/gen/c/vssftv1/all}{$-$0.2}
\defres{e17/gen/c/vssftv1/all/hi}{$-$0.0}
\defres{e17/gen/c/vssftv1/all/lo}{$-$0.4}
\defres{e17/gen/c/vssftv1/ask}{0.0}
\defres{e17/gen/c/vssftv1/ask/hi}{0.0}
\defres{e17/gen/c/vssftv1/ask/lo}{0.0}
\defres{e17/gen/c/vssftv1/offplan}{$-$1.5}
\defres{e17/gen/c/vssftv1/offplan/hi}{0.7}
\defres{e17/gen/c/vssftv1/offplan/lo}{$-$3.6}
\defres{e17/gen/cal/tp/acc}{100.0}
\defres{e17/gen/cal/tp/casc}{100.0}
\defres{e17/gen/cal/tp/clean}{yes}
\defres{e17/gen/cal/tp/cov}{88.5}
\defres{e17/gen/cal/tp/errors}{0}
\defres{e17/gen/cal/tp/llmacc}{100.0}
\defres{e17/gen/cal/tp/n}{1{,}328}
\defres{e17/gen/cal/tp/tau}{0.999673485756}
\defres{e17/gen/cal/tp/taushort}{0.9997}
\defres{e17/gen/cal/ts/acc}{100.0}
\defres{e17/gen/cal/ts/casc}{100.0}
\defres{e17/gen/cal/ts/clean}{yes}
\defres{e17/gen/cal/ts/cov}{100.0}
\defres{e17/gen/cal/ts/errors}{0}
\defres{e17/gen/cal/ts/llmacc}{100.0}
\defres{e17/gen/cal/ts/n}{1{,}125}
\defres{e17/gen/cal/ts/tau}{0.999619071672}
\defres{e17/gen/cal/ts/taushort}{0.9996}
\defres{e17/gen/train/epochs}{1}
\defres{e17/gen/train/loss}{0.377}
\defres{e17/gen/train/mem}{17.4}
\defres{e17/gen/train/minutes}{52}
\defres{e17/gen/train/setting}{nogc_6144}
\defres{e17/gen/train/sperstep}{22.7}
\defres{e17/gen/v1/acc}{99.7}
\defres{e17/gen/v1/ece}{0.001}
\defres{e17/gen/v1/ko}{100.0}
\defres{e17/gen/v1/rec}{99.5}
\defres{e17/gen/v1/stop}{99.3}
\defres{e17/gen/v1/tp}{100.0}
\defres{e17/gen/v1/ts}{99.7}
\defres{e17/genraw/v1/acc}{99.7}
\defres{e17/genraw/v1/ece}{0.032}
\defres{e17/genraw/v1/ko}{100.0}
\defres{e17/genraw/v1/rec}{99.5}
\defres{e17/genraw/v1/stop}{99.3}
\defres{e17/genraw/v1/tp}{100.0}
\defres{e17/genraw/v1/ts}{99.7}
\defres{e17/gpuhours}{5.7}
\defres{e17/head/c/acc}{99.2}
\defres{e17/head/c/ask}{100.0}
\defres{e17/head/c/ece}{0.011}
\defres{e17/head/c/offplan}{94.1}
\defres{e17/head/cal/tp/acc}{100.0}
\defres{e17/head/cal/tp/casc}{100.0}
\defres{e17/head/cal/tp/clean}{yes}
\defres{e17/head/cal/tp/cov}{78.8}
\defres{e17/head/cal/tp/errors}{0}
\defres{e17/head/cal/tp/llmacc}{100.0}
\defres{e17/head/cal/tp/n}{1{,}328}
\defres{e17/head/cal/tp/tau}{0.999999999999}
\defres{e17/head/cal/tp/taushort}{1.0000}
\defres{e17/head/cal/ts/acc}{100.0}
\defres{e17/head/cal/ts/casc}{100.0}
\defres{e17/head/cal/ts/clean}{yes}
\defres{e17/head/cal/ts/cov}{80.0}
\defres{e17/head/cal/ts/errors}{0}
\defres{e17/head/cal/ts/llmacc}{100.0}
\defres{e17/head/cal/ts/n}{1{,}125}
\defres{e17/head/cal/ts/tau}{0.999999999765}
\defres{e17/head/cal/ts/taushort}{1.0000}
\defres{e17/head/v1/acc}{99.7}
\defres{e17/head/v1/ece}{0.001}
\defres{e17/head/v1/ko}{100.0}
\defres{e17/head/v1/rec}{99.7}
\defres{e17/head/v1/stop}{99.3}
\defres{e17/head/v1/tp}{100.0}
\defres{e17/head/v1/ts}{99.8}
\defres{e17/lat/fourb/c1/p50}{318}
\defres{e17/lat/fourb/c1/p90}{441}
\defres{e17/lat/fourb/c1/s1step}{377}
\defres{e17/lat/fourb/c4/p50}{875}
\defres{e17/lat/fourb/c4/p90}{1305}
\defres{e17/lat/fourb/c4/s1step}{1714}
\defres{e17/lat/fourb/mem}{22.0}
\defres{e17/lat/gen/c1/p50}{247}
\defres{e17/lat/gen/c1/p90}{348}
\defres{e17/lat/gen/c1/s1step}{487}
\defres{e17/lat/gen/c4/p50}{796}
\defres{e17/lat/gen/c4/p90}{1061}
\defres{e17/lat/gen/c4/s1step}{1531}
\defres{e17/lat/gen/mem}{4.5}
\defres{e17/lat/gen/speedup/c1}{1.3}
\defres{e17/lat/gen/speedup/c4}{1.1}
\defres{e17/lat/head/c1/p50}{92}
\defres{e17/lat/head/c1/p90}{119}
\defres{e17/lat/head/c1/s1step}{157}
\defres{e17/lat/head/c4/p50}{204}
\defres{e17/lat/head/c4/p90}{377}
\defres{e17/lat/head/c4/s1step}{384}
\defres{e17/lat/head/mem}{2.5}
\defres{e17/lat/head/speedup/c1}{3.5}
\defres{e17/lat/head/speedup/c4}{4.3}
\defres{e17/lat/head/vsgen/c1}{2.7}
\defres{e17/lat/head/vsgen/c4}{3.9}
\defres{e17/reading/tp}{the one-token read-out}
\defres{e17/reading/ts}{the one-token read-out}
\defres{e17/rl/c/acc}{99.2}
\defres{e17/rl/c/ask}{100.0}
\defres{e17/rl/c/ece}{0.010}
\defres{e17/rl/c/offplan}{94.7}
\defres{e17/rows}{16{,}902}
\defres{e17/sft_v1/c/acc}{99.2}
\defres{e17/sft_v1/c/ask}{100.0}
\defres{e17/sft_v1/c/ece}{0.011}
\defres{e17/sft_v1/c/offplan}{93.8}
\defres{e17/spend}{0.66}
\defres{e18/c/a/accacc}{100.0}
\defres{e18/c/a/accerr}{0}
\defres{e18/c/a/cov}{78.0}
\defres{e18/c/a/defacc}{94.6}
\defres{e18/c/a/llm/accwrongllmright}{0}
\defres{e18/c/a/llm/cascacc}{100.0}
\defres{e18/c/a/llm/deferred}{327}
\defres{e18/c/a/llm/deferredright}{100.0}
\defres{e18/c/a/llm/n}{1{,}498}
\defres{e18/c/a/n}{5{,}314}
\defres{e18/c/areplace/accacc}{98.8}
\defres{e18/c/areplace/accerr}{63}
\defres{e18/c/areplace/cov}{100.0}
\defres{e18/c/areplace/llm/accwrongllmright}{4}
\defres{e18/c/areplace/llm/cascacc}{99.8}
\defres{e18/c/areplace/llm/deferred}{0}
\defres{e18/c/areplace/llm/n}{1{,}498}
\defres{e18/c/areplace/n}{5{,}314}
\defres{e18/c/e18/accacc}{99.1}
\defres{e18/c/e18/accerr}{46}
\defres{e18/c/e18/cov}{98.5}
\defres{e18/c/e18/defacc}{78.5}
\defres{e18/c/e18/llm/accwrongllmright}{1}
\defres{e18/c/e18/llm/cascacc}{100.0}
\defres{e18/c/e18/llm/deferred}{6}
\defres{e18/c/e18/llm/deferredright}{100.0}
\defres{e18/c/e18/llm/n}{1{,}498}
\defres{e18/c/e18/n}{5{,}314}
\defres{e18/c/e18f/accacc}{98.8}
\defres{e18/c/e18f/accerr}{63}
\defres{e18/c/e18f/cov}{100.0}
\defres{e18/c/e18f/llm/accwrongllmright}{0}
\defres{e18/c/e18f/llm/cascacc}{100.0}
\defres{e18/c/e18f/llm/deferred}{0}
\defres{e18/c/e18f/llm/n}{1{,}498}
\defres{e18/c/e18f/n}{5{,}314}
\defres{e18/c/gen/accacc}{98.7}
\defres{e18/c/gen/accerr}{66}
\defres{e18/c/gen/cov}{98.4}
\defres{e18/c/gen/defacc}{86.9}
\defres{e18/c/gen/llm/accwrongllmright}{1}
\defres{e18/c/gen/llm/cascacc}{100.0}
\defres{e18/c/gen/llm/deferred}{11}
\defres{e18/c/gen/llm/deferredright}{100.0}
\defres{e18/c/gen/llm/n}{1{,}498}
\defres{e18/c/gen/n}{5{,}314}
\defres{e18/c/rl/accacc}{98.9}
\defres{e18/c/rl/accerr}{57}
\defres{e18/c/rl/cov}{99.9}
\defres{e18/c/rl/defacc}{0.0}
\defres{e18/c/rl/llm/accwrongllmright}{0}
\defres{e18/c/rl/llm/cascacc}{100.0}
\defres{e18/c/rl/llm/deferred}{0}
\defres{e18/c/rl/llm/n}{1{,}498}
\defres{e18/c/rl/n}{5{,}314}
\defres{e18/f/cal/tp/acc}{99.5}
\defres{e18/f/cal/tp/accacc}{99.8}
\defres{e18/f/cal/tp/cov}{99.2}
\defres{e18/f/cal/tp/defacc}{63.6}
\defres{e18/f/cal/tp/deferred}{11}
\defres{e18/f/cal/tp/n}{1{,}328}
\defres{e18/f/cal/ts/acc}{99.7}
\defres{e18/f/cal/ts/accacc}{99.7}
\defres{e18/f/cal/ts/cov}{100.0}
\defres{e18/f/cal/ts/deferred}{0}
\defres{e18/f/cal/ts/n}{1{,}125}
\defres{e18/f/dev/tp/acc}{100.0}
\defres{e18/f/dev/tp/accacc}{100.0}
\defres{e18/f/dev/tp/cov}{100.0}
\defres{e18/f/dev/tp/deferred}{0}
\defres{e18/f/dev/tp/n}{824}
\defres{e18/f/dev/ts/acc}{99.9}
\defres{e18/f/dev/ts/accacc}{99.9}
\defres{e18/f/dev/ts/cov}{100.0}
\defres{e18/f/dev/ts/deferred}{0}
\defres{e18/f/dev/ts/n}{668}
\defres{e18/f/train/devcal}{99.7}
\defres{e18/f/train/epoch1/dev}{99.7}
\defres{e18/f/train/minutes}{84}
\defres{e18/f/train/records}{16{,}707}
\defres{e18/final/api}{3.29}
\defres{e18/final/argcov}{98.7}
\defres{e18/final/e14/api}{13.56}
\defres{e18/final/e14/argcov}{86.4}
\defres{e18/final/e14/q}{1.86}
\defres{e18/final/e14/s1s}{1.35}
\defres{e18/final/e14/s2calls}{3.60}
\defres{e18/final/e14/s2s}{2.74}
\defres{e18/final/e14/success}{100.0}
\defres{e18/final/e14/toolcov}{85.5}
\defres{e18/final/e14/tot}{15.42}
\defres{e18/final/e14/tote9}{16.13}
\defres{e18/final/e14/wall}{4.1}
\defres{e18/final/errored}{0}
\defres{e18/final/hf4b/api}{5.82}
\defres{e18/final/hf4b/argcov}{85.5}
\defres{e18/final/hf4b/q}{4.33}
\defres{e18/final/hf4b/s1s}{3.93}
\defres{e18/final/hf4b/s2calls}{3.04}
\defres{e18/final/hf4b/s2s}{5.11}
\defres{e18/final/hf4b/success}{100.0}
\defres{e18/final/hf4b/toolcov}{100.0}
\defres{e18/final/hf4b/tot}{10.15}
\defres{e18/final/hf4b/tote9}{11.80}
\defres{e18/final/hf4b/wall}{9.6}
\defres{e18/final/llm/api}{43.12}
\defres{e18/final/llm/q}{0.00}
\defres{e18/final/llm/s1s}{0.00}
\defres{e18/final/llm/s2calls}{7.53}
\defres{e18/final/llm/s2s}{11.68}
\defres{e18/final/llm/success}{99.5}
\defres{e18/final/llm/toolcov}{0.0}
\defres{e18/final/llm/tot}{43.12}
\defres{e18/final/llm/tote9}{43.12}
\defres{e18/final/llm/wall}{13.6}
\defres{e18/final/n}{200}
\defres{e18/final/q}{1.34}
\defres{e18/final/s1s}{1.43}
\defres{e18/final/s2calls}{1.51}
\defres{e18/final/s2s}{1.52}
\defres{e18/final/saving_vs_e14}{70.0}
\defres{e18/final/saving_vs_e14/e9}{68.1}
\defres{e18/final/saving_vs_e14/hi}{71.8}
\defres{e18/final/saving_vs_e14/lo}{68.0}
\defres{e18/final/saving_vs_hf4b}{54.4}
\defres{e18/final/saving_vs_hf4b/e9}{56.4}
\defres{e18/final/saving_vs_hf4b/hi}{57.5}
\defres{e18/final/saving_vs_hf4b/lo}{51.0}
\defres{e18/final/saving_vs_llm}{89.3}
\defres{e18/final/saving_vs_llm/e9}{88.1}
\defres{e18/final/saving_vs_llm/hi}{89.8}
\defres{e18/final/saving_vs_llm/lo}{88.7}
\defres{e18/final/success}{100.0}
\defres{e18/final/time_saving_vs_e14}{27.8}
\defres{e18/final/time_saving_vs_hf4b}{69.0}
\defres{e18/final/time_saving_vs_llm}{78.1}
\defres{e18/final/toolcov}{100.0}
\defres{e18/final/tot}{4.63}
\defres{e18/final/tote9}{5.14}
\defres{e18/final/vse14/success}{0.0}
\defres{e18/final/vse14/success/hi}{1.9}
\defres{e18/final/vse14/success/lo}{$-$1.9}
\defres{e18/final/vse14/wall}{$-$1.15}
\defres{e18/final/vshf4b/success}{0.0}
\defres{e18/final/vshf4b/success/hi}{1.9}
\defres{e18/final/vshf4b/success/lo}{$-$1.9}
\defres{e18/final/vshf4b/wall}{$-$6.62}
\defres{e18/final/vsllm/success}{0.5}
\defres{e18/final/vsllm/success/hi}{2.8}
\defres{e18/final/vsllm/success/lo}{$-$1.4}
\defres{e18/final/vsllm/wall}{$-$10.61}
\defres{e18/final/wall}{3.0}
\defres{e18/head/logloss}{0.022}
\defres{e18/head/n}{2{,}453}
\defres{e18/head/positives}{15}
\defres{e18/head/tp/covinsample}{51.4}
\defres{e18/head/tp/k}{0.0035}
\defres{e18/head/tp/kpct}{0.35}
\defres{e18/head/tp/llmright}{1{,}244}
\defres{e18/head/tp/n}{1{,}328}
\defres{e18/head/tp/posdeferred}{11}
\defres{e18/head/tp/positives}{12}
\defres{e18/head/tp/refright}{1{,}313}
\defres{e18/head/tp/tau}{0.9965}
\defres{e18/head/ts/covinsample}{99.7}
\defres{e18/head/ts/k}{0.0058}
\defres{e18/head/ts/kpct}{0.58}
\defres{e18/head/ts/llmright}{1{,}125}
\defres{e18/head/ts/n}{1{,}125}
\defres{e18/head/ts/posdeferred}{2}
\defres{e18/head/ts/positives}{3}
\defres{e18/head/ts/refright}{1{,}122}
\defres{e18/head/ts/tau}{0.9942}
\defres{e18/head/w0}{3.40}
\defres{e18/head/w1}{1.29}
\defres{e18/head/w2}{0.33}
\defres{e18/head/w3}{-1.08}
\defres{e18/reading/c}{does not hold}
\defres{e18/reading/live}{holds}
\defres{e18/reading/live/delta}{0.5}
\makeatother


==> generated/e19_hard_random.tex <==
\makeatletter
\providecommand{\res}[1]{\ifcsname jevres@#1\endcsname\csname jevres@#1\endcsname\else\tbd\fi}
\providecommand{\defres}[2]{\expandafter\def\csname jevres@#1\endcsname{#2}}
\defres{e19/cal/ntasks}{20}
\defres{e19/cal/op/coverage}{12.9}
\defres{e19/cal/op/llmaccall}{100.0}
\defres{e19/cal/op/n}{240}
\defres{e19/cal/op/s1accall}{87.1}
\defres{e19/cal/op/s1acctaken}{100.0}
\defres{e19/cal/toolparams/coverage}{90.0}
\defres{e19/cal/toolparams/llmaccall}{100.0}
\defres{e19/cal/toolparams/npaired}{1200}
\defres{e19/cal/toolparams/s1accall}{99.1}
\defres{e19/cal/toolparams/s1acctaken}{100.0}
\defres{e19/cal/toolparams/tau}{0.98623}
\defres{e19/cal/toolselect/coverage}{20.0}
\defres{e19/cal/toolselect/llmaccall}{100.0}
\defres{e19/cal/toolselect/npaired}{740}
\defres{e19/cal/toolselect/s1accall}{95.7}
\defres{e19/cal/toolselect/s1acctaken}{100.0}
\defres{e19/cal/toolselect/tau}{0.99995}
\defres{e19/cap}{62}
\defres{e19/ext/llm_only/success}{80.0}
\defres{e19/ext/llm_only/wall_mean}{81.4}
\defres{e19/ext/n}{20}
\defres{e19/ext/rl_random/cost_k}{283.1}
\defres{e19/ext/rl_random/cost_ref_k}{264.8}
\defres{e19/ext/rl_random/delta}{+0.0}
\defres{e19/ext/rl_random/delta_ci/hi}{+15.0}
\defres{e19/ext/rl_random/delta_ci/lo}{-15.0}
\defres{e19/ext/rl_random/fig_delta}{+0.0}
\defres{e19/ext/rl_random/fig_saving}{-7}
\defres{e19/ext/rl_random/losses}{1}
\defres{e19/ext/rl_random/n}{20}
\defres{e19/ext/rl_random/n_dropped}{0}
\defres{e19/ext/rl_random/saving}{-6.9}
\defres{e19/ext/rl_random/saving_ci/hi}{-0.2}
\defres{e19/ext/rl_random/saving_ci/lo}{-13.1}
\defres{e19/ext/rl_random/success}{80.0}
\defres{e19/ext/rl_random/success_ref}{80.0}
\defres{e19/ext/rl_random/wall_mean}{340.2}
\defres{e19/ext/rl_random/wins}{1}
\defres{e19/ext/seed0}{310780}
\defres{e19/ext/spend}{5.42}
\defres{e19/first/llm_only/success}{83.9}
\defres{e19/first/llm_only/wall_mean}{73.4}
\defres{e19/first/n}{180}
\defres{e19/first/rl_random/cost_k}{276.9}
\defres{e19/first/rl_random/cost_ref_k}{264.3}
\defres{e19/first/rl_random/delta}{+1.1}
\defres{e19/first/rl_random/delta_ci/hi}{+7.2}
\defres{e19/first/rl_random/delta_ci/lo}{-5.0}
\defres{e19/first/rl_random/fig_delta}{+1.1}
\defres{e19/first/rl_random/fig_saving}{-5}
\defres{e19/first/rl_random/losses}{15}
\defres{e19/first/rl_random/n}{180}
\defres{e19/first/rl_random/n_dropped}{0}
\defres{e19/first/rl_random/saving}{-4.8}
\defres{e19/first/rl_random/saving_ci/hi}{-2.5}
\defres{e19/first/rl_random/saving_ci/lo}{-7.0}
\defres{e19/first/rl_random/success}{85.0}
\defres{e19/first/rl_random/success_ref}{83.9}
\defres{e19/first/rl_random/wall_mean}{394.9}
\defres{e19/first/rl_random/wins}{17}
\defres{e19/first/seed0}{310600}
\defres{e19/first/spend}{47.80}
\defres{e19/lat/llmonly/s1}{0.0}
\defres{e19/lat/llmonly/s2}{70.7}
\defres{e19/lat/llmonly/s2-toolselect-gemini/n}{7401}
\defres{e19/lat/llmonly/s2-toolselect-gemini/over}{565}
\defres{e19/lat/llmonly/s2-toolselect-gemini/p50}{1.15}
\defres{e19/lat/llmonly/s2-toolselect-gemini/p90}{4.02}
\defres{e19/lat/llmonly/s2-toolselect-gemini/tailshare}{30.9}
\defres{e19/lat/llmonly/s2tail}{22.9}
\defres{e19/lat/llmonly/wall}{74.2}
\defres{e19/lat/rlrandom/extra}{315.2}
\defres{e19/lat/rlrandom/extratail}{-13.1}
\defres{e19/lat/rlrandom/s1}{336.5}
\defres{e19/lat/rlrandom/s2}{48.4}
\defres{e19/lat/rlrandom/s2-reflection-gemini/n}{1019}
\defres{e19/lat/rlrandom/s2-reflection-gemini/over}{23}
\defres{e19/lat/rlrandom/s2-reflection-gemini/p50}{1.15}
\defres{e19/lat/rlrandom/s2-reflection-gemini/p90}{1.49}
\defres{e19/lat/rlrandom/s2-reflection-gemini/tailshare}{0.9}
\defres{e19/lat/rlrandom/s2-toolparams-1tool-gemini/n}{1357}
\defres{e19/lat/rlrandom/s2-toolparams-1tool-gemini/over}{43}
\defres{e19/lat/rlrandom/s2-toolparams-1tool-gemini/p50}{0.78}
\defres{e19/lat/rlrandom/s2-toolparams-1tool-gemini/p90}{1.52}
\defres{e19/lat/rlrandom/s2-toolparams-1tool-gemini/tailshare}{0.9}
\defres{e19/lat/rlrandom/s2-toolselect-gemini/n}{5035}
\defres{e19/lat/rlrandom/s2-toolselect-gemini/over}{36}
\defres{e19/lat/rlrandom/s2-toolselect-gemini/p50}{1.00}
\defres{e19/lat/rlrandom/s2-toolselect-gemini/p90}{1.45}
\defres{e19/lat/rlrandom/s2-toolselect-gemini/tailshare}{0.8}
\defres{e19/lat/rlrandom/s2tail}{9.8}
\defres{e19/lat/rlrandom/tailshareofextra}{-4}
\defres{e19/lat/rlrandom/wall}{389.4}
\defres{e19/llm_only/cost_k}{264.3}
\defres{e19/llm_only/fail/askfinish}{0}
\defres{e19/llm_only/fail/n}{33}
\defres{e19/llm_only/fail/other}{0}
\defres{e19/llm_only/fail/wrongtotal}{33}
\defres{e19/llm_only/fail/wrongwrite}{0}
\defres{e19/llm_only/form/itemized/n}{200}
\defres{e19/llm_only/form/itemized/share}{100.0}
\defres{e19/llm_only/form/itemized/success}{83.5}
\defres{e19/llm_only/form/none/n}{0}
\defres{e19/llm_only/form/none/share}{0.0}
\defres{e19/llm_only/form/number/n}{0}
\defres{e19/llm_only/form/number/share}{0.0}
\defres{e19/llm_only/form/sentence/n}{0}
\defres{e19/llm_only/form/sentence/share}{0.0}
\defres{e19/llm_only/n}{200}
\defres{e19/llm_only/success}{83.5}
\defres{e19/llm_only/wall_mean}{74.2}
\defres{e19/llm_only/wall_median}{63.2}
\defres{e19/pilot/n}{60}
\defres{e19/pilot/success}{46.7}
\defres{e19/rl_random/acc}{99.0}
\defres{e19/rl_random/acc_accepted}{100.0}
\defres{e19/rl_random/cost_api_k}{266.1}
\defres{e19/rl_random/cost_k}{277.5}
\defres{e19/rl_random/cost_ref_k}{264.3}
\defres{e19/rl_random/coverage}{43.4}
\defres{e19/rl_random/delta}{+1.0}
\defres{e19/rl_random/delta_ci/hi}{+7.0}
\defres{e19/rl_random/delta_ci/lo}{-4.5}
\defres{e19/rl_random/diag/earlyfinishbymodel}{0}
\defres{e19/rl_random/diag/failsbymodel}{4}
\defres{e19/rl_random/diag/wrongwritebymodel}{0}
\defres{e19/rl_random/fail/askfinish}{0}
\defres{e19/rl_random/fail/n}{31}
\defres{e19/rl_random/fail/other}{0}
\defres{e19/rl_random/fail/wrongtotal}{31}
\defres{e19/rl_random/fail/wrongwrite}{0}
\defres{e19/rl_random/fig_delta}{+1.0}
\defres{e19/rl_random/fig_saving}{-5}
\defres{e19/rl_random/form/itemized/n}{200}
\defres{e19/rl_random/form/itemized/share}{100.0}
\defres{e19/rl_random/form/itemized/success}{84.5}
\defres{e19/rl_random/form/none/n}{0}
\defres{e19/rl_random/form/none/share}{0.0}
\defres{e19/rl_random/form/number/n}{0}
\defres{e19/rl_random/form/number/share}{0.0}
\defres{e19/rl_random/form/sentence/n}{0}
\defres{e19/rl_random/form/sentence/share}{0.0}
\defres{e19/rl_random/losses}{16}
\defres{e19/rl_random/n}{200}
\defres{e19/rl_random/n_dropped}{0}
\defres{e19/rl_random/newcombe/hi}{+6.9}
\defres{e19/rl_random/newcombe/lo}{-4.9}
\defres{e19/rl_random/op_acc}{96.6}
\defres{e19/rl_random/op_acc_accepted}{100.0}
\defres{e19/rl_random/op_accepted_wrong}{0}
\defres{e19/rl_random/op_coverage}{33.4}
\defres{e19/rl_random/op_n}{2400}
\defres{e19/rl_random/reflection_fired}{14.2}
\defres{e19/rl_random/saving}{-5.0}
\defres{e19/rl_random/saving_api}{-0.7}
\defres{e19/rl_random/saving_ci/hi}{-2.8}
\defres{e19/rl_random/saving_ci/lo}{-7.1}
\defres{e19/rl_random/saving_q_s24}{-1.4}
\defres{e19/rl_random/saving_q_zero}{-0.7}
\defres{e19/rl_random/state}{run}
\defres{e19/rl_random/success}{84.5}
\defres{e19/rl_random/success_ref}{83.5}
\defres{e19/rl_random/tool_params/acc}{99.1}
\defres{e19/rl_random/tool_params/acc_accepted}{100.0}
\defres{e19/rl_random/tool_params/coverage}{65.2}
\defres{e19/rl_random/tool_select/acc}{98.9}
\defres{e19/rl_random/tool_select/acc_accepted}{100.0}
\defres{e19/rl_random/tool_select/coverage}{32.0}
\defres{e19/rl_random/vs_tier/cost_k}{266.1}
\defres{e19/rl_random/vs_tier/cost_ref_k}{229.6}
\defres{e19/rl_random/vs_tier/delta}{+3.0}
\defres{e19/rl_random/vs_tier/delta_ci/hi}{+9.5}
\defres{e19/rl_random/vs_tier/delta_ci/lo}{-3.5}
\defres{e19/rl_random/vs_tier/fig_delta}{+3.0}
\defres{e19/rl_random/vs_tier/fig_saving}{-16}
\defres{e19/rl_random/vs_tier/losses}{20}
\defres{e19/rl_random/vs_tier/n}{200}
\defres{e19/rl_random/vs_tier/n_dropped}{0}
\defres{e19/rl_random/vs_tier/newcombe/hi}{+9.8}
\defres{e19/rl_random/vs_tier/newcombe/lo}{-3.8}
\defres{e19/rl_random/vs_tier/saving}{-15.9}
\defres{e19/rl_random/vs_tier/saving_ci/hi}{-14.4}
\defres{e19/rl_random/vs_tier/saving_ci/lo}{-17.4}
\defres{e19/rl_random/vs_tier/success}{84.5}
\defres{e19/rl_random/vs_tier/success_ref}{81.5}
\defres{e19/rl_random/vs_tier/wall_ref_mean}{327.2}
\defres{e19/rl_random/vs_tier/wins}{26}
\defres{e19/rl_random/wall_mean}{389.4}
\defres{e19/rl_random/wall_median}{389.9}
\defres{e19/rl_random/wall_ref_mean}{74.2}
\defres{e19/rl_random/wall_ref_median}{63.2}
\defres{e19/rl_random/wins}{18}
\defres{e19/route}{gemini}
\defres{e19/setting/answer_style}{itemized}
\defres{e19/setting/families}{multi}
\defres{e19/setting/max_steps}{45}
\defres{e19/setting/multi_customers}{12}
\defres{e19/setting/n}{200}
\defres{e19/setting/n_distractors}{60}
\defres{e19/setting/noise_lines}{20}
\defres{e19/setting/rule}{tier}
\defres{e19/setting/seed0}{310600}
\defres{e19/spend}{53.79}
\defres{e19/tariff/host_usd_h}{1.212}
\defres{e19/tariff/q}{0.01144}
\makeatother


==> generated/e20_ensembles.tex <==
\makeatletter
\providecommand{\res}[1]{\ifcsname jevres@#1\endcsname\csname jevres@#1\endcsname\else\tbd\fi}
\providecommand{\defres}[2]{\expandafter\def\csname jevres@#1\endcsname{#2}}
\defres{e20/a/c/hosted/gate/accacc}{95.9}
\defres{e20/a/c/hosted/gate/cov}{88.2}
\defres{e20/a/c/hosted/gate/devcov}{92.6}
\defres{e20/a/c/hosted/gate/deverr}{113}
\defres{e20/a/c/hosted/gate/err}{103}
\defres{e20/a/c/hosted/gate/k}{2}
\defres{e20/a/c/hosted/gate/m}{2}
\defres{e20/a/c/hosted/gate/mustacc_n}{128}
\defres{e20/a/c/hosted/gate/musterr}{72}
\defres{e20/a/c/hosted/gate/own/e14a}{0}
\defres{e20/a/c/hosted/gate/own/jev}{101}
\defres{e20/a/c/hosted/gate/own/oaidec}{158}
\defres{e20/a/c/hosted/gate/own/rl}{0}
\defres{e20/a/c/hosted/gate/pred}{79.9}
\defres{e20/a/c/hosted/majority/acc}{92.2}
\defres{e20/a/c/hosted/majority/devacc}{91.6}
\defres{e20/a/c/hosted/majority/k}{2}
\defres{e20/a/c/hosted/majority/must}{31.5}
\defres{e20/a/c/hosted/majority/pred}{75.0}
\defres{e20/a/c/hosted/single/acc}{90.6}
\defres{e20/a/c/hosted/single/must}{37.3}
\defres{e20/a/c/hosted/single/name}{OpenAI Decisions API}
\defres{e20/a/c/hosted/single/pred}{77.5}
\defres{e20/a/c/hosted/weighted/acc}{92.2}
\defres{e20/a/c/hosted/weighted/devacc}{91.6}
\defres{e20/a/c/hosted/weighted/k}{2}
\defres{e20/a/c/hosted/weighted/must}{31.5}
\defres{e20/a/c/hosted/weighted/pred}{75.0}
\defres{e20/a/c/mixed/gate/accacc}{99.9}
\defres{e20/a/c/mixed/gate/cov}{99.0}
\defres{e20/a/c/mixed/gate/devcov}{98.7}
\defres{e20/a/c/mixed/gate/deverr}{9}
\defres{e20/a/c/mixed/gate/err}{3}
\defres{e20/a/c/mixed/gate/k}{2}
\defres{e20/a/c/mixed/gate/m}{2}
\defres{e20/a/c/mixed/gate/mustacc_n}{144}
\defres{e20/a/c/mixed/gate/musterr}{0}
\defres{e20/a/c/mixed/gate/own/e12c}{1}
\defres{e20/a/c/mixed/gate/own/e14a}{16}
\defres{e20/a/c/mixed/gate/own/e16b}{5}
\defres{e20/a/c/mixed/gate/own/rl}{11}
\defres{e20/a/c/mixed/gate/pred}{100.0}
\defres{e20/a/c/mixed/majority/acc}{99.5}
\defres{e20/a/c/mixed/majority/devacc}{99.3}
\defres{e20/a/c/mixed/majority/k}{5}
\defres{e20/a/c/mixed/majority/must}{100.0}
\defres{e20/a/c/mixed/majority/pred}{99.1}
\defres{e20/a/c/mixed/single/acc}{99.9}
\defres{e20/a/c/mixed/single/must}{100.0}
\defres{e20/a/c/mixed/single/name}{StartLux-4B + our recipe (E12c)}
\defres{e20/a/c/mixed/single/pred}{99.5}
\defres{e20/a/c/mixed/weighted/acc}{99.6}
\defres{e20/a/c/mixed/weighted/devacc}{99.4}
\defres{e20/a/c/mixed/weighted/k}{5}
\defres{e20/a/c/mixed/weighted/must}{100.0}
\defres{e20/a/c/mixed/weighted/pred}{99.1}
\defres{e20/a/c/ots/gate/accacc}{97.5}
\defres{e20/a/c/ots/gate/cov}{88.8}
\defres{e20/a/c/ots/gate/devcov}{87.7}
\defres{e20/a/c/ots/gate/deverr}{48}
\defres{e20/a/c/ots/gate/err}{63}
\defres{e20/a/c/ots/gate/k}{4}
\defres{e20/a/c/ots/gate/m}{4}
\defres{e20/a/c/ots/gate/mustacc_n}{113}
\defres{e20/a/c/ots/gate/musterr}{61}
\defres{e20/a/c/ots/gate/own/e14a}{0}
\defres{e20/a/c/ots/gate/own/openjev}{110}
\defres{e20/a/c/ots/gate/own/openjevhf}{70}
\defres{e20/a/c/ots/gate/own/rl}{0}
\defres{e20/a/c/ots/gate/own/sl27b}{50}
\defres{e20/a/c/ots/gate/own/sl9b}{59}
\defres{e20/a/c/ots/gate/pred}{86.1}
\defres{e20/a/c/ots/majority/acc}{94.9}
\defres{e20/a/c/ots/majority/devacc}{94.9}
\defres{e20/a/c/ots/majority/k}{2}
\defres{e20/a/c/ots/majority/must}{47.3}
\defres{e20/a/c/ots/majority/pred}{81.0}
\defres{e20/a/c/ots/single/acc}{93.9}
\defres{e20/a/c/ots/single/must}{25.5}
\defres{e20/a/c/ots/single/name}{StartLux-27B}
\defres{e20/a/c/ots/single/pred}{78.5}
\defres{e20/a/c/ots/weighted/acc}{94.9}
\defres{e20/a/c/ots/weighted/devacc}{94.9}
\defres{e20/a/c/ots/weighted/k}{2}
\defres{e20/a/c/ots/weighted/must}{47.3}
\defres{e20/a/c/ots/weighted/pred}{81.0}
\defres{e20/a/c/pair/acc}{99.7}
\defres{e20/a/c/pair/cov}{88.4}
\defres{e20/a/c/pair/err}{1}
\defres{e20/a/c/pair/gpred}{100.0}
\defres{e20/a/c/pair/must}{100.0}
\defres{e20/a/c/pair/pred}{100.0}
\defres{e20/a/c/ref/e14a/acc}{99.5}
\defres{e20/a/c/ref/e14a/cov}{78.2}
\defres{e20/a/c/ref/e14a/err}{0}
\defres{e20/a/c/ref/e14a/gpred}{100.0}
\defres{e20/a/c/ref/e14a/must}{100.0}
\defres{e20/a/c/ref/e14a/pred}{99.5}
\defres{e20/a/c/ref/rl/acc}{99.7}
\defres{e20/a/c/ref/rl/cov}{100.0}
\defres{e20/a/c/ref/rl/err}{12}
\defres{e20/a/c/ref/rl/gpred}{100.0}
\defres{e20/a/c/ref/rl/must}{100.0}
\defres{e20/a/c/ref/rl/pred}{100.0}
\defres{e20/a/c/sweep/0/cov}{88.2}
\defres{e20/a/c/sweep/0/err}{103}
\defres{e20/a/c/sweep/0/jev}{101}
\defres{e20/a/c/sweep/0/oaidec}{158}
\defres{e20/a/c/sweep/05/cov}{76.1}
\defres{e20/a/c/sweep/05/err}{82}
\defres{e20/a/c/sweep/05/jev}{62}
\defres{e20/a/c/sweep/05/oaidec}{110}
\defres{e20/a/c/sweep/07/cov}{55.5}
\defres{e20/a/c/sweep/07/err}{56}
\defres{e20/a/c/sweep/07/jev}{39}
\defres{e20/a/c/sweep/07/oaidec}{66}
\defres{e20/a/c/sweep/09/cov}{25.6}
\defres{e20/a/c/sweep/09/err}{21}
\defres{e20/a/c/sweep/09/jev}{1}
\defres{e20/a/c/sweep/09/oaidec}{19}
\defres{e20/a/c/sweep/095/cov}{14.7}
\defres{e20/a/c/sweep/095/err}{14}
\defres{e20/a/c/sweep/095/jev}{0}
\defres{e20/a/c/sweep/095/oaidec}{13}
\defres{e20/a/c/sweep/099/cov}{4.3}
\defres{e20/a/c/sweep/099/err}{0}
\defres{e20/a/c/sweep/099/jev}{0}
\defres{e20/a/c/sweep/099/oaidec}{2}
\defres{e20/a/c/sweep/1/cov}{1.3}
\defres{e20/a/c/sweep/1/err}{0}
\defres{e20/a/c/sweep/1/jev}{0}
\defres{e20/a/c/sweep/1/oaidec}{1}
\defres{e20/a/c/test_tasks}{108}
\defres{e20/a/c/test_units}{2{,}821}
\defres{e20/a/corr/all/jac}{24.9}
\defres{e20/a/corr/all/jacind}{7.1}
\defres{e20/a/corr/all/must/best}{StartLux-27B}
\defres{e20/a/corr/all/must/besterr}{165}
\defres{e20/a/corr/all/must/bestshared}{165}
\defres{e20/a/corr/all/must/failall}{39}
\defres{e20/a/corr/all/must/failhalf}{63}
\defres{e20/a/corr/all/must/failnone}{0}
\defres{e20/a/corr/all/must/n}{267}
\defres{e20/a/corr/all/n_models}{18}
\defres{e20/a/corr/all/ratio}{1.8}
\defres{e20/a/corr/all/samewrong}{73}
\defres{e20/a/corr/must27b/both}{162}
\defres{e20/a/corr/must27b/erra}{164}
\defres{e20/a/corr/must27b/errb}{165}
\defres{e20/a/corr/must27b/same}{162}
\defres{e20/a/corr/top6/jac}{43.8}
\defres{e20/a/corr/top6/jacind}{3.3}
\defres{e20/a/corr/top6/must/best}{StartLux-27B}
\defres{e20/a/corr/top6/must/besterr}{165}
\defres{e20/a/corr/top6/must/bestshared}{130}
\defres{e20/a/corr/top6/must/failall}{39}
\defres{e20/a/corr/top6/must/failhalf}{59}
\defres{e20/a/corr/top6/must/failnone}{37}
\defres{e20/a/corr/top6/must/n}{267}
\defres{e20/a/corr/top6/n_models}{6}
\defres{e20/a/corr/top6/ratio}{13.4}
\defres{e20/a/corr/top6/samewrong}{86}
\defres{e20/a/hard/all/gateacc}{100.0}
\defres{e20/a/hard/all/gatecov}{94.1}
\defres{e20/a/hard/all/gateerr}{0}
\defres{e20/a/hard/all/jev}{100.0}
\defres{e20/a/hard/all/n}{392}
\defres{e20/a/hard/all/rl}{94.1}
\defres{e20/a/hard/all/tasks}{91}
\defres{e20/a/hard/all/vote}{95.2}
\defres{e20/a/hard/common}{392}
\defres{e20/a/hard/other/gateacc}{100.0}
\defres{e20/a/hard/other/gatecov}{99.0}
\defres{e20/a/hard/other/gateerr}{0}
\defres{e20/a/hard/other/jev}{100.0}
\defres{e20/a/hard/other/n}{295}
\defres{e20/a/hard/other/rl}{99.0}
\defres{e20/a/hard/other/tasks}{91}
\defres{e20/a/hard/other/vote}{99.0}
\defres{e20/a/hard/tier/gateacc}{100.0}
\defres{e20/a/hard/tier/gatecov}{79.4}
\defres{e20/a/hard/tier/gateerr}{0}
\defres{e20/a/hard/tier/jev}{100.0}
\defres{e20/a/hard/tier/n}{97}
\defres{e20/a/hard/tier/rl}{79.4}
\defres{e20/a/hard/tier/tasks}{61}
\defres{e20/a/hard/tier/vote}{83.5}
\defres{e20/a/l1/hosted/gate/accacc}{87.5}
\defres{e20/a/l1/hosted/gate/cov}{86.8}
\defres{e20/a/l1/hosted/gate/devcov}{87.0}
\defres{e20/a/l1/hosted/gate/deverr}{176}
\defres{e20/a/l1/hosted/gate/err}{224}
\defres{e20/a/l1/hosted/gate/k}{2}
\defres{e20/a/l1/hosted/gate/m}{2}
\defres{e20/a/l1/hosted/gate/own/e14a}{537}
\defres{e20/a/l1/hosted/gate/own/jev}{164}
\defres{e20/a/l1/hosted/gate/own/oaidec}{311}
\defres{e20/a/l1/hosted/gate/own/rl}{350}
\defres{e20/a/l1/hosted/majority/acc}{84.1}
\defres{e20/a/l1/hosted/majority/args}{87.9}
\defres{e20/a/l1/hosted/majority/devacc}{86.0}
\defres{e20/a/l1/hosted/majority/k}{2}
\defres{e20/a/l1/hosted/majority/toolchoice}{88.4}
\defres{e20/a/l1/hosted/majority/w2c}{71.5}
\defres{e20/a/l1/hosted/single/acc}{85.6}
\defres{e20/a/l1/hosted/single/args}{88.5}
\defres{e20/a/l1/hosted/single/name}{Jev}
\defres{e20/a/l1/hosted/single/toolchoice}{87.7}
\defres{e20/a/l1/hosted/single/w2c}{77.4}
\defres{e20/a/l1/hosted/weighted/acc}{84.1}
\defres{e20/a/l1/hosted/weighted/args}{87.9}
\defres{e20/a/l1/hosted/weighted/devacc}{86.0}
\defres{e20/a/l1/hosted/weighted/k}{2}
\defres{e20/a/l1/hosted/weighted/toolchoice}{88.4}
\defres{e20/a/l1/hosted/weighted/w2c}{71.5}
\defres{e20/a/l1/mixed/gate/accacc}{96.0}
\defres{e20/a/l1/mixed/gate/cov}{68.6}
\defres{e20/a/l1/mixed/gate/devcov}{69.6}
\defres{e20/a/l1/mixed/gate/deverr}{36}
\defres{e20/a/l1/mixed/gate/err}{57}
\defres{e20/a/l1/mixed/gate/k}{7}
\defres{e20/a/l1/mixed/gate/m}{7}
\defres{e20/a/l1/mixed/gate/own/clef}{122}
\defres{e20/a/l1/mixed/gate/own/e12}{77}
\defres{e20/a/l1/mixed/gate/own/e12c}{71}
\defres{e20/a/l1/mixed/gate/own/e14a}{403}
\defres{e20/a/l1/mixed/gate/own/e16a}{82}
\defres{e20/a/l1/mixed/gate/own/e16b}{116}
\defres{e20/a/l1/mixed/gate/own/jev}{69}
\defres{e20/a/l1/mixed/gate/own/rl}{307}
\defres{e20/a/l1/mixed/gate/own/sl27b}{55}
\defres{e20/a/l1/mixed/majority/acc}{87.8}
\defres{e20/a/l1/mixed/majority/args}{91.0}
\defres{e20/a/l1/mixed/majority/devacc}{90.0}
\defres{e20/a/l1/mixed/majority/k}{6}
\defres{e20/a/l1/mixed/majority/toolchoice}{88.4}
\defres{e20/a/l1/mixed/majority/w2c}{80.5}
\defres{e20/a/l1/mixed/single/acc}{87.7}
\defres{e20/a/l1/mixed/single/args}{88.5}
\defres{e20/a/l1/mixed/single/name}{StartLux-27B}
\defres{e20/a/l1/mixed/single/toolchoice}{89.1}
\defres{e20/a/l1/mixed/single/w2c}{84.3}
\defres{e20/a/l1/mixed/weighted/acc}{88.0}
\defres{e20/a/l1/mixed/weighted/args}{91.4}
\defres{e20/a/l1/mixed/weighted/devacc}{90.0}
\defres{e20/a/l1/mixed/weighted/k}{6}
\defres{e20/a/l1/mixed/weighted/toolchoice}{88.6}
\defres{e20/a/l1/mixed/weighted/w2c}{80.5}
\defres{e20/a/l1/ots/gate/accacc}{93.4}
\defres{e20/a/l1/ots/gate/cov}{68.9}
\defres{e20/a/l1/ots/gate/devcov}{70.1}
\defres{e20/a/l1/ots/gate/deverr}{77}
\defres{e20/a/l1/ots/gate/err}{94}
\defres{e20/a/l1/ots/gate/k}{8}
\defres{e20/a/l1/ots/gate/m}{8}
\defres{e20/a/l1/ots/gate/own/clef}{122}
\defres{e20/a/l1/ots/gate/own/clefflash}{165}
\defres{e20/a/l1/ots/gate/own/e14a}{404}
\defres{e20/a/l1/ots/gate/own/jev}{70}
\defres{e20/a/l1/ots/gate/own/oaidec}{164}
\defres{e20/a/l1/ots/gate/own/openjevhf}{141}
\defres{e20/a/l1/ots/gate/own/rl}{307}
\defres{e20/a/l1/ots/gate/own/sl27b}{57}
\defres{e20/a/l1/ots/gate/own/sl4b}{118}
\defres{e20/a/l1/ots/gate/own/sl9b}{102}
\defres{e20/a/l1/ots/majority/acc}{86.4}
\defres{e20/a/l1/ots/majority/args}{89.4}
\defres{e20/a/l1/ots/majority/devacc}{88.4}
\defres{e20/a/l1/ots/majority/k}{4}
\defres{e20/a/l1/ots/majority/toolchoice}{87.2}
\defres{e20/a/l1/ots/majority/w2c}{79.3}
\defres{e20/a/l1/ots/single/acc}{87.7}
\defres{e20/a/l1/ots/single/args}{88.5}
\defres{e20/a/l1/ots/single/name}{StartLux-27B}
\defres{e20/a/l1/ots/single/toolchoice}{89.1}
\defres{e20/a/l1/ots/single/w2c}{84.3}
\defres{e20/a/l1/ots/weighted/acc}{86.4}
\defres{e20/a/l1/ots/weighted/args}{89.2}
\defres{e20/a/l1/ots/weighted/devacc}{88.5}
\defres{e20/a/l1/ots/weighted/k}{5}
\defres{e20/a/l1/ots/weighted/toolchoice}{87.7}
\defres{e20/a/l1/ots/weighted/w2c}{79.1}
\defres{e20/a/l1/pair/acc}{78.9}
\defres{e20/a/l1/pair/cov}{80.3}
\defres{e20/a/l1/pair/err}{156}
\defres{e20/a/l1/ref/e14a/acc}{67.4}
\defres{e20/a/l1/ref/e14a/cov}{33.8}
\defres{e20/a/l1/ref/e14a/err}{191}
\defres{e20/a/l1/ref/rl/acc}{78.2}
\defres{e20/a/l1/ref/rl/cov}{99.9}
\defres{e20/a/l1/ref/rl/err}{450}
\defres{e20/a/l1/sweep/0/cov}{86.8}
\defres{e20/a/l1/sweep/0/err}{224}
\defres{e20/a/l1/sweep/0/jev}{164}
\defres{e20/a/l1/sweep/0/oaidec}{311}
\defres{e20/a/l1/sweep/05/cov}{74.8}
\defres{e20/a/l1/sweep/05/err}{143}
\defres{e20/a/l1/sweep/05/jev}{98}
\defres{e20/a/l1/sweep/05/oaidec}{208}
\defres{e20/a/l1/sweep/07/cov}{65.2}
\defres{e20/a/l1/sweep/07/err}{94}
\defres{e20/a/l1/sweep/07/jev}{55}
\defres{e20/a/l1/sweep/07/oaidec}{153}
\defres{e20/a/l1/sweep/09/cov}{50.8}
\defres{e20/a/l1/sweep/09/err}{52}
\defres{e20/a/l1/sweep/09/jev}{22}
\defres{e20/a/l1/sweep/09/oaidec}{76}
\defres{e20/a/l1/sweep/095/cov}{43.3}
\defres{e20/a/l1/sweep/095/err}{31}
\defres{e20/a/l1/sweep/095/jev}{15}
\defres{e20/a/l1/sweep/095/oaidec}{48}
\defres{e20/a/l1/sweep/099/cov}{29.0}
\defres{e20/a/l1/sweep/099/err}{10}
\defres{e20/a/l1/sweep/099/jev}{8}
\defres{e20/a/l1/sweep/099/oaidec}{19}
\defres{e20/a/l1/sweep/1/cov}{21.0}
\defres{e20/a/l1/sweep/1/err}{4}
\defres{e20/a/l1/sweep/1/jev}{6}
\defres{e20/a/l1/sweep/1/oaidec}{12}
\defres{e20/a/l1/test_units}{2{,}069}
\defres{e20/a/transfer/hosted/majority/c_members_on_l1}{84.1}
\defres{e20/a/transfer/hosted/majority/l1_members_on_c}{92.3}
\defres{e20/a/transfer/hosted/weighted/c_members_on_l1}{84.1}
\defres{e20/a/transfer/hosted/weighted/l1_members_on_c}{92.3}
\defres{e20/a/transfer/mixed/majority/c_members_on_l1}{83.8}
\defres{e20/a/transfer/mixed/weighted/c_members_on_l1}{84.4}
\defres{e20/a/transfer/ots/majority/c_members_on_l1}{84.8}
\defres{e20/a/transfer/ots/weighted/c_members_on_l1}{84.8}
\defres{e20/cal/agree/arg/acc}{91.9}
\defres{e20/cal/agree/arg/agree}{75.7}
\defres{e20/cal/agree/arg/cov}{50.2}
\defres{e20/cal/agree/arg/err}{0}
\defres{e20/cal/agree/arg/n}{1{,}328}
\defres{e20/cal/agree/arg/tau}{0.99}
\defres{e20/cal/agree/tool/acc}{94.9}
\defres{e20/cal/agree/tool/agree}{89.5}
\defres{e20/cal/agree/tool/cov}{0.0}
\defres{e20/cal/agree/tool/err}{0}
\defres{e20/cal/agree/tool/n}{1{,}125}
\defres{e20/cal/agree/tool/tau}{$\infty$}
\defres{e20/cal/facts/arg/agree}{90.8}
\defres{e20/cal/facts/arg/agree99}{666}
\defres{e20/cal/facts/arg/agree99wrong}{0}
\defres{e20/cal/facts/arg/agreeacc}{95.5}
\defres{e20/cal/facts/arg/jev/acc}{95.8}
\defres{e20/cal/facts/arg/jev/conf1}{870}
\defres{e20/cal/facts/arg/jev/conf1wrong}{0}
\defres{e20/cal/facts/arg/llm}{93.7}
\defres{e20/cal/facts/arg/n}{1{,}328}
\defres{e20/cal/facts/arg/oaidec/acc}{86.8}
\defres{e20/cal/facts/arg/oaidec/conf1}{626}
\defres{e20/cal/facts/arg/oaidec/conf1wrong}{12}
\defres{e20/cal/facts/tool/agree}{89.5}
\defres{e20/cal/facts/tool/agree99}{49}
\defres{e20/cal/facts/tool/agree99wrong}{2}
\defres{e20/cal/facts/tool/agreeacc}{95.6}
\defres{e20/cal/facts/tool/jev/acc}{94.2}
\defres{e20/cal/facts/tool/jev/conf1}{353}
\defres{e20/cal/facts/tool/jev/conf1wrong}{1}
\defres{e20/cal/facts/tool/llm}{100.0}
\defres{e20/cal/facts/tool/n}{1{,}125}
\defres{e20/cal/facts/tool/oaidec/acc}{93.7}
\defres{e20/cal/facts/tool/oaidec/conf1}{34}
\defres{e20/cal/facts/tool/oaidec/conf1wrong}{3}
\defres{e20/cal/oaidec/arg/acc}{86.8}
\defres{e20/cal/oaidec/arg/cov}{0.0}
\defres{e20/cal/oaidec/arg/err}{0}
\defres{e20/cal/oaidec/arg/n}{1{,}328}
\defres{e20/cal/oaidec/arg/tau}{$\infty$}
\defres{e20/cal/oaidec/tool/acc}{93.7}
\defres{e20/cal/oaidec/tool/cov}{0.0}
\defres{e20/cal/oaidec/tool/err}{0}
\defres{e20/cal/oaidec/tool/n}{1{,}125}
\defres{e20/cal/oaidec/tool/tau}{$\infty$}
\defres{e20/live/agree/status}{not run}
\defres{e20/live/oaidec/status}{not run}
\defres{e20/spend/gemini}{0.00}
\defres{e20/spend/jev}{0.21}
\defres{e20/spend/openai}{0.33}
\makeatother


==> generated/e21_shift.tex <==
\makeatletter
\providecommand{\res}[1]{\ifcsname jevres@#1\endcsname\csname jevres@#1\endcsname\else\tbd\fi}
\providecommand{\defres}[2]{\expandafter\def\csname jevres@#1\endcsname{#2}}
\defres{e21/base/in/c}{50.1}
\defres{e21/base/in/live}{13.0}
\defres{e21/base/l2/all}{52.9}
\defres{e21/base/l2/askany}{60.8}
\defres{e21/base/l2/genkind}{47.6}
\defres{e21/base/l2/mustask}{27.6}
\defres{e21/base/l2/newkind}{65.1}
\defres{e21/base/l2/offplan}{79.8}
\defres{e21/base/l2/renamed}{44.7}
\defres{e21/base/l2/vs_jev}{$-$38.9}
\defres{e21/base/l2/vs_jev/hi}{$-$34.5}
\defres{e21/base/l2/vs_jev/lo}{$-$43.4}
\defres{e21/base/l2/vs_rl}{$-$45.7}
\defres{e21/base/l2/vs_rl/hi}{$-$41.9}
\defres{e21/base/l2/vs_rl/lo}{$-$49.5}
\defres{e21/base/l3/kind/clarify.ask_after_lookup}{45.0}
\defres{e21/base/l3/kind/clarify.ask_twice}{0.0}
\defres{e21/base/l3/kind/clarify.method}{0.0}
\defres{e21/base/l3/kind/clarify.name}{0.0}
\defres{e21/base/l3/kind/clarify.order}{90.0}
\defres{e21/base/l3/kind/clarify.speed}{0.0}
\defres{e21/base/l3/kind/multi}{0.0}
\defres{e21/base/l3/kind/notify}{0.0}
\defres{e21/base/l3/n}{200}
\defres{e21/base/l3/newkind}{15.0}
\defres{e21/base/l3/own}{40.5}
\defres{e21/base/l3/success}{13.5}
\defres{e21/base/l3/usd}{0.0033}
\defres{e21/base/l3/vs_jev}{$-$68.5}
\defres{e21/base/l3/vs_jev/hi}{$-$61.2}
\defres{e21/base/l3/vs_jev/lo}{$-$74.2}
\defres{e21/base/l3/vs_llm_only}{$-$86.5}
\defres{e21/base/l3/vs_llm_only/hi}{$-$80.8}
\defres{e21/base/l3/vs_llm_only/lo}{$-$90.6}
\defres{e21/corpus/all/n}{1{,}250}
\defres{e21/corpus/all/tasks}{100}
\defres{e21/corpus/askany/n}{263}
\defres{e21/corpus/askany/tasks}{60}
\defres{e21/corpus/genkind/n}{943}
\defres{e21/corpus/genkind/tasks}{70}
\defres{e21/corpus/mustask/n}{100}
\defres{e21/corpus/mustask/tasks}{60}
\defres{e21/corpus/newkind/n}{307}
\defres{e21/corpus/newkind/tasks}{30}
\defres{e21/corpus/occurrences}{1{,}250}
\defres{e21/corpus/offplan/n}{81}
\defres{e21/corpus/offplan/tasks}{25}
\defres{e21/corpus/options}{129}
\defres{e21/corpus/questions}{1{,}093}
\defres{e21/corpus/renamed/n}{1{,}069}
\defres{e21/corpus/renamed/tasks}{100}
\defres{e21/corpus/tasks}{100}
\defres{e21/e12/in/c}{99.1}
\defres{e21/e12/in/live}{100.0}
\defres{e21/e12/l2/all}{94.9}
\defres{e21/e12/l2/askany}{90.9}
\defres{e21/e12/l2/cost_distraction}{0.1}
\defres{e21/e12/l2/cost_distraction/hi}{1.1}
\defres{e21/e12/l2/cost_distraction/lo}{$-$0.9}
\defres{e21/e12/l2/cost_surface}{3.7}
\defres{e21/e12/l2/cost_surface/hi}{5.3}
\defres{e21/e12/l2/cost_surface/lo}{2.2}
\defres{e21/e12/l2/genkind}{95.3}
\defres{e21/e12/l2/mustask}{67.4}
\defres{e21/e12/l2/newkind}{93.7}
\defres{e21/e12/l2/nodist}{95.0}
\defres{e21/e12/l2/nosurf}{98.5}
\defres{e21/e12/l2/offplan}{98.4}
\defres{e21/e12/l2/renamed}{93.8}
\defres{e21/e12/l2/vs_jev}{3.1}
\defres{e21/e12/l2/vs_jev/hi}{4.6}
\defres{e21/e12/l2/vs_jev/lo}{1.6}
\defres{e21/e12/l2/vs_rl}{$-$3.7}
\defres{e21/e12/l2/vs_rl/hi}{$-$2.5}
\defres{e21/e12/l2/vs_rl/lo}{$-$5.0}
\defres{e21/e12/l3/kind/clarify.ask_after_lookup}{30.0}
\defres{e21/e12/l3/kind/clarify.ask_twice}{95.0}
\defres{e21/e12/l3/kind/clarify.method}{100.0}
\defres{e21/e12/l3/kind/clarify.name}{100.0}
\defres{e21/e12/l3/kind/clarify.order}{100.0}
\defres{e21/e12/l3/kind/clarify.speed}{95.0}
\defres{e21/e12/l3/kind/multi}{98.3}
\defres{e21/e12/l3/kind/notify}{100.0}
\defres{e21/e12/l3/n}{200}
\defres{e21/e12/l3/newkind}{75.0}
\defres{e21/e12/l3/own}{95.5}
\defres{e21/e12/l3/success}{91.5}
\defres{e21/e12/l3/usd}{0.0161}
\defres{e21/e12/l3/vs_jev}{9.5}
\defres{e21/e12/l3/vs_jev/hi}{16.4}
\defres{e21/e12/l3/vs_jev/lo}{2.5}
\defres{e21/e12/l3/vs_llm_only}{$-$8.5}
\defres{e21/e12/l3/vs_llm_only/hi}{$-$4.9}
\defres{e21/e12/l3/vs_llm_only/lo}{$-$13.2}
\defres{e21/e12c/in/c}{99.6}
\defres{e21/e12c/in/live}{100.0}
\defres{e21/e12c/l2/all}{98.5}
\defres{e21/e12c/l2/askany}{100.0}
\defres{e21/e12c/l2/cost_distraction}{$-$0.8}
\defres{e21/e12c/l2/cost_distraction/hi}{$-$0.2}
\defres{e21/e12c/l2/cost_distraction/lo}{$-$1.4}
\defres{e21/e12c/l2/cost_surface}{1.4}
\defres{e21/e12c/l2/cost_surface/hi}{2.3}
\defres{e21/e12c/l2/cost_surface/lo}{0.6}
\defres{e21/e12c/l2/genkind}{100.0}
\defres{e21/e12c/l2/mustask}{100.0}
\defres{e21/e12c/l2/newkind}{94.9}
\defres{e21/e12c/l2/nodist}{97.7}
\defres{e21/e12c/l2/nosurf}{99.9}
\defres{e21/e12c/l2/offplan}{100.0}
\defres{e21/e12c/l2/renamed}{98.0}
\defres{e21/e12c/l2/vs_jev}{6.7}
\defres{e21/e12c/l2/vs_jev/hi}{8.9}
\defres{e21/e12c/l2/vs_jev/lo}{4.6}
\defres{e21/e12c/l2/vs_rl}{$-$0.1}
\defres{e21/e12c/l2/vs_rl/hi}{1.1}
\defres{e21/e12c/l2/vs_rl/lo}{$-$1.4}
\defres{e21/e12c/l3/kind/clarify.ask_after_lookup}{85.0}
\defres{e21/e12c/l3/kind/clarify.ask_twice}{100.0}
\defres{e21/e12c/l3/kind/clarify.method}{100.0}
\defres{e21/e12c/l3/kind/clarify.name}{100.0}
\defres{e21/e12c/l3/kind/clarify.order}{100.0}
\defres{e21/e12c/l3/kind/clarify.speed}{95.0}
\defres{e21/e12c/l3/kind/multi}{100.0}
\defres{e21/e12c/l3/kind/notify}{100.0}
\defres{e21/e12c/l3/n}{200}
\defres{e21/e12c/l3/newkind}{95.0}
\defres{e21/e12c/l3/own}{97.1}
\defres{e21/e12c/l3/success}{98.0}
\defres{e21/e12c/l3/usd}{0.0190}
\defres{e21/e12c/l3/vs_jev}{16.0}
\defres{e21/e12c/l3/vs_jev/hi}{22.0}
\defres{e21/e12c/l3/vs_jev/lo}{10.4}
\defres{e21/e12c/l3/vs_llm_only}{$-$2.0}
\defres{e21/e12c/l3/vs_llm_only/hi}{0.2}
\defres{e21/e12c/l3/vs_llm_only/lo}{$-$5.0}
\defres{e21/e14a/in/c}{99.2}
\defres{e21/e14a/in/live}{100.0}
\defres{e21/e14a/l2/all}{73.2}
\defres{e21/e14a/l2/askany}{81.3}
\defres{e21/e14a/l2/cost_distraction}{$-$2.6}
\defres{e21/e14a/l2/cost_distraction/hi}{$-$1.2}
\defres{e21/e14a/l2/cost_distraction/lo}{$-$4.0}
\defres{e21/e14a/l2/cost_surface}{21.9}
\defres{e21/e14a/l2/cost_surface/hi}{24.9}
\defres{e21/e14a/l2/cost_surface/lo}{18.9}
\defres{e21/e14a/l2/genkind}{76.4}
\defres{e21/e14a/l2/mustask}{77.2}
\defres{e21/e14a/l2/newkind}{65.9}
\defres{e21/e14a/l2/nodist}{70.7}
\defres{e21/e14a/l2/nosurf}{95.1}
\defres{e21/e14a/l2/offplan}{72.4}
\defres{e21/e14a/l2/renamed}{68.1}
\defres{e21/e14a/l2/vs_jev}{$-$18.5}
\defres{e21/e14a/l2/vs_jev/hi}{$-$14.9}
\defres{e21/e14a/l2/vs_jev/lo}{$-$22.2}
\defres{e21/e14a/l2/vs_rl}{$-$25.4}
\defres{e21/e14a/l2/vs_rl/hi}{$-$22.1}
\defres{e21/e14a/l2/vs_rl/lo}{$-$28.8}
\defres{e21/e14a/l3/kind/clarify.ask_after_lookup}{0.0}
\defres{e21/e14a/l3/kind/clarify.ask_twice}{0.0}
\defres{e21/e14a/l3/kind/clarify.method}{100.0}
\defres{e21/e14a/l3/kind/clarify.name}{75.0}
\defres{e21/e14a/l3/kind/clarify.order}{0.0}
\defres{e21/e14a/l3/kind/clarify.speed}{0.0}
\defres{e21/e14a/l3/kind/multi}{0.0}
\defres{e21/e14a/l3/kind/notify}{0.0}
\defres{e21/e14a/l3/n}{200}
\defres{e21/e14a/l3/newkind}{0.0}
\defres{e21/e14a/l3/own}{42.7}
\defres{e21/e14a/l3/success}{17.5}
\defres{e21/e14a/l3/usd}{0.0408}
\defres{e21/e14a/l3/vs_jev}{$-$64.5}
\defres{e21/e14a/l3/vs_jev/hi}{$-$55.0}
\defres{e21/e14a/l3/vs_jev/lo}{$-$72.0}
\defres{e21/e14a/l3/vs_llm_only}{$-$82.5}
\defres{e21/e14a/l3/vs_llm_only/hi}{$-$76.3}
\defres{e21/e14a/l3/vs_llm_only/lo}{$-$87.1}
\defres{e21/gpu/hours}{11.1}
\defres{e21/intern/in/c}{75.2}
\defres{e21/intern/in/live}{26.5}
\defres{e21/intern/l2/all}{75.9}
\defres{e21/intern/l2/askany}{73.6}
\defres{e21/intern/l2/cost_distraction}{1.9}
\defres{e21/intern/l2/cost_distraction/hi}{4.4}
\defres{e21/intern/l2/cost_distraction/lo}{$-$0.5}
\defres{e21/intern/l2/cost_surface}{0.6}
\defres{e21/intern/l2/cost_surface/hi}{3.2}
\defres{e21/intern/l2/cost_surface/lo}{$-$2.1}
\defres{e21/intern/l2/genkind}{74.7}
\defres{e21/intern/l2/mustask}{33.9}
\defres{e21/intern/l2/newkind}{78.8}
\defres{e21/intern/l2/nodist}{77.8}
\defres{e21/intern/l2/nosurf}{76.6}
\defres{e21/intern/l2/offplan}{83.4}
\defres{e21/intern/l2/renamed}{71.4}
\defres{e21/intern/l2/vs_jev}{$-$15.9}
\defres{e21/intern/l2/vs_jev/hi}{$-$13.2}
\defres{e21/intern/l2/vs_jev/lo}{$-$18.4}
\defres{e21/intern/l2/vs_rl}{$-$22.7}
\defres{e21/intern/l2/vs_rl/hi}{$-$19.7}
\defres{e21/intern/l2/vs_rl/lo}{$-$25.6}
\defres{e21/intern/l3/kind/clarify.ask_after_lookup}{45.0}
\defres{e21/intern/l3/kind/clarify.ask_twice}{40.0}
\defres{e21/intern/l3/kind/clarify.method}{5.0}
\defres{e21/intern/l3/kind/clarify.name}{60.0}
\defres{e21/intern/l3/kind/clarify.order}{55.0}
\defres{e21/intern/l3/kind/clarify.speed}{0.0}
\defres{e21/intern/l3/kind/multi}{30.0}
\defres{e21/intern/l3/kind/notify}{45.0}
\defres{e21/intern/l3/n}{200}
\defres{e21/intern/l3/newkind}{43.3}
\defres{e21/intern/l3/own}{65.1}
\defres{e21/intern/l3/success}{34.0}
\defres{e21/intern/l3/usd}{0.0128}
\defres{e21/intern/l3/vs_jev}{$-$48.0}
\defres{e21/intern/l3/vs_jev/hi}{$-$40.4}
\defres{e21/intern/l3/vs_jev/lo}{$-$54.6}
\defres{e21/intern/l3/vs_llm_only}{$-$66.0}
\defres{e21/intern/l3/vs_llm_only/hi}{$-$58.9}
\defres{e21/intern/l3/vs_llm_only/lo}{$-$72.2}
\defres{e21/jev/in/c}{91.5}
\defres{e21/jev/in/live}{83.0}
\defres{e21/jev/l2/all}{91.8}
\defres{e21/jev/l2/askany}{88.7}
\defres{e21/jev/l2/cost_distraction}{0.1}
\defres{e21/jev/l2/cost_distraction/hi}{0.9}
\defres{e21/jev/l2/cost_distraction/lo}{$-$0.6}
\defres{e21/jev/l2/cost_surface}{$-$2.8}
\defres{e21/jev/l2/cost_surface/hi}{$-$1.5}
\defres{e21/jev/l2/cost_surface/lo}{$-$4.1}
\defres{e21/jev/l2/genkind}{90.2}
\defres{e21/jev/l2/mustask}{58.3}
\defres{e21/jev/l2/newkind}{95.6}
\defres{e21/jev/l2/nodist}{91.9}
\defres{e21/jev/l2/nosurf}{89.0}
\defres{e21/jev/l2/offplan}{94.4}
\defres{e21/jev/l2/renamed}{90.2}
\defres{e21/jev/l2/vs_rl}{$-$6.8}
\defres{e21/jev/l2/vs_rl/hi}{$-$5.0}
\defres{e21/jev/l2/vs_rl/lo}{$-$8.6}
\defres{e21/jev/l3/kind/clarify.ask_after_lookup}{100.0}
\defres{e21/jev/l3/kind/clarify.ask_twice}{95.0}
\defres{e21/jev/l3/kind/clarify.method}{25.0}
\defres{e21/jev/l3/kind/clarify.name}{100.0}
\defres{e21/jev/l3/kind/clarify.order}{100.0}
\defres{e21/jev/l3/kind/clarify.speed}{0.0}
\defres{e21/jev/l3/kind/multi}{100.0}
\defres{e21/jev/l3/kind/notify}{100.0}
\defres{e21/jev/l3/n}{200}
\defres{e21/jev/l3/newkind}{98.3}
\defres{e21/jev/l3/own}{87.3}
\defres{e21/jev/l3/success}{82.0}
\defres{e21/jev/l3/usd}{0.0167}
\defres{e21/jev/l3/vs_llm_only}{$-$18.0}
\defres{e21/jev/l3/vs_llm_only/hi}{$-$12.9}
\defres{e21/jev/l3/vs_llm_only/lo}{$-$23.9}
\defres{e21/kendall/c_vs_l2}{0.56}
\defres{e21/kendall/c_vs_l2/n}{11}
\defres{e21/kendall/c_vs_l3}{0.55}
\defres{e21/kendall/c_vs_l3/n}{11}
\defres{e21/kendall/l2_vs_l3}{0.84}
\defres{e21/kendall/l2_vs_l3/n}{11}
\defres{e21/kendall/l2_vs_l3_ladder}{0.88}
\defres{e21/kendall/l2_vs_l3_ladder/n}{13}
\defres{e21/kendall/live_vs_l3}{0.49}
\defres{e21/kendall/live_vs_l3/n}{11}
\defres{e21/lead/cost_distraction/diff}{$-$1.8}
\defres{e21/lead/cost_distraction/offshelf_mean}{0.9}
\defres{e21/lead/cost_distraction/trained_mean}{$-$0.9}
\defres{e21/lead/cost_surface/diff}{7.2}
\defres{e21/lead/cost_surface/offshelf_mean}{$-$0.2}
\defres{e21/lead/cost_surface/trained_mean}{7.0}
\defres{e21/lead/in_c/gap}{5.7}
\defres{e21/lead/in_c/keeps}{yes}
\defres{e21/lead/in_c/offshelf}{StartLux-27B (Q8\_0)}
\defres{e21/lead/in_c/trained}{StartLux-4B (mixed)}
\defres{e21/lead/in_live/gap}{17.0}
\defres{e21/lead/in_live/keeps}{yes}
\defres{e21/lead/in_live/offshelf}{Jev}
\defres{e21/lead/in_live/trained}{AgentDecision-4B}
\defres{e21/lead/l2_all/gap}{3.9}
\defres{e21/lead/l2_all/keeps}{yes}
\defres{e21/lead/l2_all/offshelf}{StartLux-27B (Q8\_0)}
\defres{e21/lead/l2_all/trained}{AgentDecision-4B}
\defres{e21/lead/l2_genkind/gap}{5.7}
\defres{e21/lead/l2_genkind/keeps}{yes}
\defres{e21/lead/l2_genkind/offshelf}{StartLux-27B (Q8\_0)}
\defres{e21/lead/l2_genkind/trained}{StartLux-4B (mixed)}
\defres{e21/lead/l2_mustask/gap}{35.0}
\defres{e21/lead/l2_mustask/keeps}{yes}
\defres{e21/lead/l2_mustask/offshelf}{StartLux-27B (Q8\_0)}
\defres{e21/lead/l2_mustask/trained}{StartLux-4B (mixed)}
\defres{e21/lead/l2_newkind/gap}{3.6}
\defres{e21/lead/l2_newkind/keeps}{yes}
\defres{e21/lead/l2_newkind/offshelf}{StartLux-27B (Q8\_0)}
\defres{e21/lead/l2_newkind/trained}{AgentDecision-4B}
\defres{e21/lead/l2_offplan/gap}{1.6}
\defres{e21/lead/l2_offplan/keeps}{yes}
\defres{e21/lead/l2_offplan/offshelf}{StartLux-27B (Q8\_0)}
\defres{e21/lead/l2_offplan/trained}{StartLux-4B (mixed)}
\defres{e21/lead/l2_renamed/gap}{4.6}
\defres{e21/lead/l2_renamed/keeps}{yes}
\defres{e21/lead/l2_renamed/offshelf}{StartLux-27B (Q8\_0)}
\defres{e21/lead/l2_renamed/trained}{AgentDecision-4B}
\defres{e21/lead/l3/gap}{16.0}
\defres{e21/lead/l3/keeps}{yes}
\defres{e21/lead/l3/offshelf}{Jev}
\defres{e21/lead/l3/trained}{StartLux-4B (mixed)}
\defres{e21/lead/l3_newkind/gap}{$-$3.3}
\defres{e21/lead/l3_newkind/keeps}{no}
\defres{e21/lead/l3_newkind/offshelf}{Jev}
\defres{e21/lead/l3_newkind/trained}{AgentDecision-4B}
\defres{e21/llm_only/in/live}{99.5}
\defres{e21/llm_only/l3/kind/clarify.ask_after_lookup}{100.0}
\defres{e21/llm_only/l3/kind/clarify.ask_twice}{100.0}
\defres{e21/llm_only/l3/kind/clarify.method}{100.0}
\defres{e21/llm_only/l3/kind/clarify.name}{100.0}
\defres{e21/llm_only/l3/kind/clarify.order}{100.0}
\defres{e21/llm_only/l3/kind/clarify.speed}{100.0}
\defres{e21/llm_only/l3/kind/multi}{100.0}
\defres{e21/llm_only/l3/kind/notify}{100.0}
\defres{e21/llm_only/l3/n}{200}
\defres{e21/llm_only/l3/newkind}{100.0}
\defres{e21/llm_only/l3/success}{100.0}
\defres{e21/llm_only/l3/usd}{0.0535}
\defres{e21/llm_only/l3/vs_jev}{18.0}
\defres{e21/llm_only/l3/vs_jev/hi}{23.9}
\defres{e21/llm_only/l3/vs_jev/lo}{12.9}
\defres{e21/oaidec/in/c}{90.9}
\defres{e21/oaidec/in/live}{78.5}
\defres{e21/oaidec/l2/all}{86.1}
\defres{e21/oaidec/l2/askany}{83.6}
\defres{e21/oaidec/l2/cost_distraction}{2.7}
\defres{e21/oaidec/l2/cost_distraction/hi}{4.4}
\defres{e21/oaidec/l2/cost_distraction/lo}{0.8}
\defres{e21/oaidec/l2/cost_surface}{0.6}
\defres{e21/oaidec/l2/cost_surface/hi}{2.3}
\defres{e21/oaidec/l2/cost_surface/lo}{$-$1.0}
\defres{e21/oaidec/l2/genkind}{86.7}
\defres{e21/oaidec/l2/mustask}{41.7}
\defres{e21/oaidec/l2/newkind}{84.8}
\defres{e21/oaidec/l2/nodist}{88.8}
\defres{e21/oaidec/l2/nosurf}{86.8}
\defres{e21/oaidec/l2/offplan}{95.8}
\defres{e21/oaidec/l2/renamed}{83.4}
\defres{e21/oaidec/l2/vs_jev}{$-$5.7}
\defres{e21/oaidec/l2/vs_jev/hi}{$-$3.9}
\defres{e21/oaidec/l2/vs_jev/lo}{$-$7.7}
\defres{e21/oaidec/l2/vs_rl}{$-$12.5}
\defres{e21/oaidec/l2/vs_rl/hi}{$-$10.4}
\defres{e21/oaidec/l2/vs_rl/lo}{$-$14.7}
\defres{e21/oaidec/l3/kind/clarify.ask_after_lookup}{100.0}
\defres{e21/oaidec/l3/kind/clarify.ask_twice}{50.0}
\defres{e21/oaidec/l3/kind/clarify.method}{30.0}
\defres{e21/oaidec/l3/kind/clarify.name}{90.0}
\defres{e21/oaidec/l3/kind/clarify.order}{90.0}
\defres{e21/oaidec/l3/kind/clarify.speed}{20.0}
\defres{e21/oaidec/l3/kind/multi}{65.0}
\defres{e21/oaidec/l3/kind/notify}{85.0}
\defres{e21/oaidec/l3/n}{200}
\defres{e21/oaidec/l3/newkind}{78.3}
\defres{e21/oaidec/l3/own}{76.5}
\defres{e21/oaidec/l3/success}{66.0}
\defres{e21/oaidec/l3/usd}{0.0229}
\defres{e21/oaidec/l3/vs_jev}{$-$16.0}
\defres{e21/oaidec/l3/vs_jev/hi}{$-$9.5}
\defres{e21/oaidec/l3/vs_jev/lo}{$-$22.5}
\defres{e21/oaidec/l3/vs_llm_only}{$-$34.0}
\defres{e21/oaidec/l3/vs_llm_only/hi}{$-$27.5}
\defres{e21/oaidec/l3/vs_llm_only/lo}{$-$40.8}
\defres{e21/openjevhf/in/c}{92.4}
\defres{e21/openjevhf/in/live}{63.0}
\defres{e21/openjevhf/l2/all}{92.4}
\defres{e21/openjevhf/l2/askany}{88.3}
\defres{e21/openjevhf/l2/cost_distraction}{$-$0.0}
\defres{e21/openjevhf/l2/cost_distraction/hi}{0.6}
\defres{e21/openjevhf/l2/cost_distraction/lo}{$-$0.7}
\defres{e21/openjevhf/l2/cost_surface}{$-$0.1}
\defres{e21/openjevhf/l2/cost_surface/hi}{0.9}
\defres{e21/openjevhf/l2/cost_surface/lo}{$-$1.2}
\defres{e21/openjevhf/l2/genkind}{91.6}
\defres{e21/openjevhf/l2/mustask}{58.3}
\defres{e21/openjevhf/l2/newkind}{94.3}
\defres{e21/openjevhf/l2/nodist}{92.4}
\defres{e21/openjevhf/l2/nosurf}{92.2}
\defres{e21/openjevhf/l2/offplan}{92.6}
\defres{e21/openjevhf/l2/renamed}{91.1}
\defres{e21/openjevhf/l2/vs_jev}{0.6}
\defres{e21/openjevhf/l2/vs_jev/hi}{1.6}
\defres{e21/openjevhf/l2/vs_jev/lo}{$-$0.4}
\defres{e21/openjevhf/l2/vs_rl}{$-$6.2}
\defres{e21/openjevhf/l2/vs_rl/hi}{$-$4.4}
\defres{e21/openjevhf/l2/vs_rl/lo}{$-$8.0}
\defres{e21/openjevhf/l3/kind/clarify.ask_after_lookup}{95.0}
\defres{e21/openjevhf/l3/kind/clarify.ask_twice}{50.0}
\defres{e21/openjevhf/l3/kind/clarify.method}{0.0}
\defres{e21/openjevhf/l3/kind/clarify.name}{100.0}
\defres{e21/openjevhf/l3/kind/clarify.order}{50.0}
\defres{e21/openjevhf/l3/kind/clarify.speed}{0.0}
\defres{e21/openjevhf/l3/kind/multi}{100.0}
\defres{e21/openjevhf/l3/kind/notify}{100.0}
\defres{e21/openjevhf/l3/n}{200}
\defres{e21/openjevhf/l3/newkind}{81.7}
\defres{e21/openjevhf/l3/own}{89.8}
\defres{e21/openjevhf/l3/success}{69.5}
\defres{e21/openjevhf/l3/usd}{0.0154}
\defres{e21/openjevhf/l3/vs_jev}{$-$12.5}
\defres{e21/openjevhf/l3/vs_jev/hi}{$-$7.8}
\defres{e21/openjevhf/l3/vs_jev/lo}{$-$17.3}
\defres{e21/openjevhf/l3/vs_llm_only}{$-$30.5}
\defres{e21/openjevhf/l3/vs_llm_only/hi}{$-$24.2}
\defres{e21/openjevhf/l3/vs_llm_only/lo}{$-$37.2}
\defres{e21/rl/in/c}{99.2}
\defres{e21/rl/in/live}{100.0}
\defres{e21/rl/l2/all}{98.6}
\defres{e21/rl/l2/askany}{97.4}
\defres{e21/rl/l2/cost_distraction}{$-$0.2}
\defres{e21/rl/l2/cost_distraction/hi}{0.7}
\defres{e21/rl/l2/cost_distraction/lo}{$-$1.1}
\defres{e21/rl/l2/cost_surface}{1.1}
\defres{e21/rl/l2/cost_surface/hi}{2.1}
\defres{e21/rl/l2/cost_surface/lo}{0.2}
\defres{e21/rl/l2/genkind}{98.3}
\defres{e21/rl/l2/mustask}{90.8}
\defres{e21/rl/l2/newkind}{99.3}
\defres{e21/rl/l2/nodist}{98.3}
\defres{e21/rl/l2/nosurf}{99.7}
\defres{e21/rl/l2/offplan}{99.2}
\defres{e21/rl/l2/renamed}{98.3}
\defres{e21/rl/l2/vs_jev}{6.8}
\defres{e21/rl/l2/vs_jev/hi}{8.6}
\defres{e21/rl/l2/vs_jev/lo}{5.0}
\defres{e21/rl/l3/kind/clarify.ask_after_lookup}{85.0}
\defres{e21/rl/l3/kind/clarify.ask_twice}{100.0}
\defres{e21/rl/l3/kind/clarify.method}{90.0}
\defres{e21/rl/l3/kind/clarify.name}{100.0}
\defres{e21/rl/l3/kind/clarify.order}{100.0}
\defres{e21/rl/l3/kind/clarify.speed}{85.0}
\defres{e21/rl/l3/kind/multi}{100.0}
\defres{e21/rl/l3/kind/notify}{100.0}
\defres{e21/rl/l3/n}{200}
\defres{e21/rl/l3/newkind}{95.0}
\defres{e21/rl/l3/own}{98.0}
\defres{e21/rl/l3/success}{96.0}
\defres{e21/rl/l3/usd}{0.0169}
\defres{e21/rl/l3/vs_jev}{14.0}
\defres{e21/rl/l3/vs_jev/hi}{19.8}
\defres{e21/rl/l3/vs_jev/lo}{8.6}
\defres{e21/rl/l3/vs_llm_only}{$-$4.0}
\defres{e21/rl/l3/vs_llm_only/hi}{$-$1.3}
\defres{e21/rl/l3/vs_llm_only/lo}{$-$7.7}
\defres{e21/sft_v1/in/c}{99.2}
\defres{e21/sft_v1/in/live}{100.0}
\defres{e21/sft_v1/l2/all}{98.4}
\defres{e21/sft_v1/l2/askany}{98.6}
\defres{e21/sft_v1/l2/genkind}{99.1}
\defres{e21/sft_v1/l2/mustask}{95.0}
\defres{e21/sft_v1/l2/newkind}{96.8}
\defres{e21/sft_v1/l2/offplan}{99.2}
\defres{e21/sft_v1/l2/renamed}{98.1}
\defres{e21/sft_v1/l2/vs_jev}{6.6}
\defres{e21/sft_v1/l2/vs_jev/hi}{8.7}
\defres{e21/sft_v1/l2/vs_jev/lo}{4.6}
\defres{e21/sft_v1/l2/vs_rl}{$-$0.2}
\defres{e21/sft_v1/l2/vs_rl/hi}{0.9}
\defres{e21/sft_v1/l2/vs_rl/lo}{$-$1.2}
\defres{e21/sft_v1/l3/kind/clarify.ask_after_lookup}{60.0}
\defres{e21/sft_v1/l3/kind/clarify.ask_twice}{100.0}
\defres{e21/sft_v1/l3/kind/clarify.method}{100.0}
\defres{e21/sft_v1/l3/kind/clarify.name}{100.0}
\defres{e21/sft_v1/l3/kind/clarify.order}{100.0}
\defres{e21/sft_v1/l3/kind/clarify.speed}{100.0}
\defres{e21/sft_v1/l3/kind/multi}{100.0}
\defres{e21/sft_v1/l3/kind/notify}{100.0}
\defres{e21/sft_v1/l3/n}{200}
\defres{e21/sft_v1/l3/newkind}{86.7}
\defres{e21/sft_v1/l3/own}{96.8}
\defres{e21/sft_v1/l3/success}{96.0}
\defres{e21/sft_v1/l3/usd}{0.0164}
\defres{e21/sft_v1/l3/vs_jev}{14.0}
\defres{e21/sft_v1/l3/vs_jev/hi}{20.4}
\defres{e21/sft_v1/l3/vs_jev/lo}{7.7}
\defres{e21/sft_v1/l3/vs_llm_only}{$-$4.0}
\defres{e21/sft_v1/l3/vs_llm_only/hi}{$-$1.3}
\defres{e21/sft_v1/l3/vs_llm_only/lo}{$-$7.7}
\defres{e21/sl27b/in/c}{93.9}
\defres{e21/sl27b/in/live}{63.0}
\defres{e21/sl27b/l2/all}{94.7}
\defres{e21/sl27b/l2/askany}{90.4}
\defres{e21/sl27b/l2/genkind}{94.3}
\defres{e21/sl27b/l2/mustask}{65.0}
\defres{e21/sl27b/l2/newkind}{95.6}
\defres{e21/sl27b/l2/offplan}{98.4}
\defres{e21/sl27b/l2/renamed}{93.8}
\defres{e21/sl27b/l2/vs_jev}{3.0}
\defres{e21/sl27b/l2/vs_jev/hi}{4.5}
\defres{e21/sl27b/l2/vs_jev/lo}{1.5}
\defres{e21/sl27b/l2/vs_rl}{$-$3.9}
\defres{e21/sl27b/l2/vs_rl/hi}{$-$2.4}
\defres{e21/sl27b/l2/vs_rl/lo}{$-$5.3}
\defres{e21/sl27b/l3/kind/clarify.ask_after_lookup}{100.0}
\defres{e21/sl27b/l3/kind/clarify.ask_twice}{87.5}
\defres{e21/sl27b/l3/kind/clarify.method}{0.0}
\defres{e21/sl27b/l3/kind/clarify.name}{100.0}
\defres{e21/sl27b/l3/kind/clarify.order}{76.5}
\defres{e21/sl27b/l3/kind/clarify.speed}{41.2}
\defres{e21/sl27b/l3/kind/multi}{100.0}
\defres{e21/sl27b/l3/kind/notify}{100.0}
\defres{e21/sl27b/l3/n}{164}
\defres{e21/sl27b/l3/newkind}{95.9}
\defres{e21/sl27b/l3/own}{92.6}
\defres{e21/sl27b/l3/success}{79.9}
\defres{e21/sl27b/l3/usd}{0.0159}
\defres{e21/sl27b/l3/vs_jev}{$-$1.8}
\defres{e21/sl27b/l3/vs_jev/hi}{3.3}
\defres{e21/sl27b/l3/vs_jev/lo}{$-$7.1}
\defres{e21/sl27b/l3/vs_llm_only}{$-$20.1}
\defres{e21/sl27b/l3/vs_llm_only/hi}{$-$14.2}
\defres{e21/sl27b/l3/vs_llm_only/lo}{$-$26.9}
\defres{e21/sl4b/in/c}{89.1}
\defres{e21/sl4b/in/live}{60.0}
\defres{e21/sl4b/l2/all}{86.5}
\defres{e21/sl4b/l2/askany}{81.4}
\defres{e21/sl4b/l2/cost_distraction}{$-$0.0}
\defres{e21/sl4b/l2/cost_distraction/hi}{1.2}
\defres{e21/sl4b/l2/cost_distraction/lo}{$-$1.3}
\defres{e21/sl4b/l2/cost_surface}{1.6}
\defres{e21/sl4b/l2/cost_surface/hi}{3.5}
\defres{e21/sl4b/l2/cost_surface/lo}{$-$0.1}
\defres{e21/sl4b/l2/genkind}{86.9}
\defres{e21/sl4b/l2/mustask}{36.7}
\defres{e21/sl4b/l2/newkind}{85.6}
\defres{e21/sl4b/l2/nodist}{86.5}
\defres{e21/sl4b/l2/nosurf}{88.2}
\defres{e21/sl4b/l2/offplan}{87.8}
\defres{e21/sl4b/l2/renamed}{84.1}
\defres{e21/sl4b/l2/vs_jev}{$-$5.2}
\defres{e21/sl4b/l2/vs_jev/hi}{$-$3.4}
\defres{e21/sl4b/l2/vs_jev/lo}{$-$7.2}
\defres{e21/sl4b/l2/vs_rl}{$-$12.1}
\defres{e21/sl4b/l2/vs_rl/hi}{$-$9.6}
\defres{e21/sl4b/l2/vs_rl/lo}{$-$14.7}
\defres{e21/sl4b/l3/kind/clarify.ask_after_lookup}{10.0}
\defres{e21/sl4b/l3/kind/clarify.ask_twice}{15.0}
\defres{e21/sl4b/l3/kind/clarify.method}{0.0}
\defres{e21/sl4b/l3/kind/clarify.name}{95.0}
\defres{e21/sl4b/l3/kind/clarify.order}{35.0}
\defres{e21/sl4b/l3/kind/clarify.speed}{0.0}
\defres{e21/sl4b/l3/kind/multi}{91.7}
\defres{e21/sl4b/l3/kind/notify}{60.0}
\defres{e21/sl4b/l3/n}{200}
\defres{e21/sl4b/l3/newkind}{28.3}
\defres{e21/sl4b/l3/own}{80.7}
\defres{e21/sl4b/l3/success}{49.0}
\defres{e21/sl4b/l3/usd}{0.0135}
\defres{e21/sl4b/l3/vs_jev}{$-$33.0}
\defres{e21/sl4b/l3/vs_jev/hi}{$-$26.2}
\defres{e21/sl4b/l3/vs_jev/lo}{$-$39.3}
\defres{e21/sl4b/l3/vs_llm_only}{$-$51.0}
\defres{e21/sl4b/l3/vs_llm_only/hi}{$-$43.9}
\defres{e21/sl4b/l3/vs_llm_only/lo}{$-$57.8}
\defres{e21/sl9b/in/c}{91.8}
\defres{e21/sl9b/in/live}{74.0}
\defres{e21/sl9b/l2/all}{90.9}
\defres{e21/sl9b/l2/askany}{87.9}
\defres{e21/sl9b/l2/cost_distraction}{0.7}
\defres{e21/sl9b/l2/cost_distraction/hi}{1.5}
\defres{e21/sl9b/l2/cost_distraction/lo}{0.0}
\defres{e21/sl9b/l2/cost_surface}{$-$0.9}
\defres{e21/sl9b/l2/cost_surface/hi}{$-$0.0}
\defres{e21/sl9b/l2/cost_surface/lo}{$-$1.8}
\defres{e21/sl9b/l2/genkind}{90.8}
\defres{e21/sl9b/l2/mustask}{55.0}
\defres{e21/sl9b/l2/newkind}{91.0}
\defres{e21/sl9b/l2/nodist}{91.6}
\defres{e21/sl9b/l2/nosurf}{89.9}
\defres{e21/sl9b/l2/offplan}{96.4}
\defres{e21/sl9b/l2/renamed}{89.6}
\defres{e21/sl9b/l2/vs_jev}{$-$0.9}
\defres{e21/sl9b/l2/vs_jev/hi}{0.5}
\defres{e21/sl9b/l2/vs_jev/lo}{$-$2.3}
\defres{e21/sl9b/l2/vs_rl}{$-$7.7}
\defres{e21/sl9b/l2/vs_rl/hi}{$-$5.8}
\defres{e21/sl9b/l2/vs_rl/lo}{$-$9.8}
\defres{e21/sl9b/l3/kind/clarify.ask_after_lookup}{90.0}
\defres{e21/sl9b/l3/kind/clarify.ask_twice}{15.0}
\defres{e21/sl9b/l3/kind/clarify.method}{0.0}
\defres{e21/sl9b/l3/kind/clarify.name}{100.0}
\defres{e21/sl9b/l3/kind/clarify.order}{95.0}
\defres{e21/sl9b/l3/kind/clarify.speed}{0.0}
\defres{e21/sl9b/l3/kind/multi}{100.0}
\defres{e21/sl9b/l3/kind/notify}{95.0}
\defres{e21/sl9b/l3/n}{200}
\defres{e21/sl9b/l3/newkind}{66.7}
\defres{e21/sl9b/l3/own}{87.5}
\defres{e21/sl9b/l3/success}{69.5}
\defres{e21/sl9b/l3/usd}{0.0147}
\defres{e21/sl9b/l3/vs_jev}{$-$12.5}
\defres{e21/sl9b/l3/vs_jev/hi}{$-$7.8}
\defres{e21/sl9b/l3/vs_jev/lo}{$-$17.3}
\defres{e21/sl9b/l3/vs_llm_only}{$-$30.5}
\defres{e21/sl9b/l3/vs_llm_only/hi}{$-$24.2}
\defres{e21/sl9b/l3/vs_llm_only/lo}{$-$37.2}
\defres{e21/spend/gemini}{61.87}
\defres{e21/spend/gemini_host}{36.71}
\defres{e21/spend/gemini_local}{25.15}
\defres{e21/spend/jev}{0.84}
\defres{e21/spend/openai}{1.23}
\makeatother


==> generated/e21b_shift_cascade.tex <==
\makeatletter
\providecommand{\res}[1]{\ifcsname jevres@#1\endcsname\csname jevres@#1\endcsname\else\tbd\fi}
\providecommand{\defres}[2]{\expandafter\def\csname jevres@#1\endcsname{#2}}
\defres{e21b/e12/acc_wrong_arg}{0}
\defres{e21b/e12/acc_wrong_tool}{22}
\defres{e21b/e12/api_k}{12.4}
\defres{e21b/e12/argcov}{62.2}
\defres{e21b/e12/cal/argcov}{83.7}
\defres{e21b/e12/cal/toolcov}{100.0}
\defres{e21b/e12/delta}{$-$7.5}
\defres{e21b/e12/delta_ci/hi}{$-$4.0}
\defres{e21b/e12/delta_ci/lo}{$-$12.0}
\defres{e21b/e12/errored}{0}
\defres{e21b/e12/genkinds}{99.3}
\defres{e21b/e12/handed_back}{0.0}
\defres{e21b/e12/in/argcov}{92.3}
\defres{e21b/e12/in/success}{100.0}
\defres{e21b/e12/in/toolcov}{100.0}
\defres{e21b/e12/llm_calls}{4.3}
\defres{e21b/e12/losses}{15}
\defres{e21b/e12/mustask/n}{82}
\defres{e21b/e12/mustask/taken}{82}
\defres{e21b/e12/mustask/wrong}{2}
\defres{e21b/e12/n}{200}
\defres{e21b/e12/newkinds}{76.7}
\defres{e21b/e12/ni/hi}{$-$4.6}
\defres{e21b/e12/ni/lo}{$-$12.0}
\defres{e21b/e12/ni/p}{1.000}
\defres{e21b/e12/ni/verdict}{not shown}
\defres{e21b/e12/ref_success}{100.0}
\defres{e21b/e12/ref_wall}{8.0}
\defres{e21b/e12/replace/delta}{+1.0}
\defres{e21b/e12/replace/success}{91.5}
\defres{e21b/e12/saving}{69.7}
\defres{e21b/e12/saving_api}{76.8}
\defres{e21b/e12/saving_ci/hi}{71.6}
\defres{e21b/e12/saving_ci/lo}{67.9}
\defres{e21b/e12/steps}{6.4}
\defres{e21b/e12/success}{92.5}
\defres{e21b/e12/taken_arg}{1039}
\defres{e21b/e12/taken_tool}{1272}
\defres{e21b/e12/tau/arg}{0.995873}
\defres{e21b/e12/tau/tool}{0.445030}
\defres{e21b/e12/toolcov}{100.0}
\defres{e21b/e12/usd_k}{16.2}
\defres{e21b/e12/wall}{8.4}
\defres{e21b/e12/wall_median}{6.0}
\defres{e21b/e12/wins}{0}
\defres{e21b/e12_in/acc_wrong_arg}{0}
\defres{e21b/e12_in/acc_wrong_tool}{0}
\defres{e21b/e12_in/api_k}{3.5}
\defres{e21b/e12_in/argcov}{92.3}
\defres{e21b/e12_in/delta}{+0.5}
\defres{e21b/e12_in/delta_ci/hi}{+2.8}
\defres{e21b/e12_in/delta_ci/lo}{$-$1.4}
\defres{e21b/e12_in/errored}{0}
\defres{e21b/e12_in/handed_back}{0.0}
\defres{e21b/e12_in/llm_calls}{1.8}
\defres{e21b/e12_in/losses}{0}
\defres{e21b/e12_in/mustask/n}{50}
\defres{e21b/e12_in/mustask/taken}{50}
\defres{e21b/e12_in/mustask/wrong}{0}
\defres{e21b/e12_in/n}{200}
\defres{e21b/e12_in/ni/hi}{+2.8}
\defres{e21b/e12_in/ni/lo}{$-$1.4}
\defres{e21b/e12_in/ni/p}{0.002}
\defres{e21b/e12_in/ni/verdict}{non-inferior}
\defres{e21b/e12_in/ref_success}{99.5}
\defres{e21b/e12_in/ref_wall}{13.6}
\defres{e21b/e12_in/saving}{86.3}
\defres{e21b/e12_in/saving_api}{91.9}
\defres{e21b/e12_in/saving_ci/hi}{86.7}
\defres{e21b/e12_in/saving_ci/lo}{85.8}
\defres{e21b/e12_in/steps}{7.5}
\defres{e21b/e12_in/success}{100.0}
\defres{e21b/e12_in/taken_arg}{1962}
\defres{e21b/e12_in/taken_tool}{1500}
\defres{e21b/e12_in/toolcov}{100.0}
\defres{e21b/e12_in/usd_k}{5.9}
\defres{e21b/e12_in/wall}{5.4}
\defres{e21b/e12_in/wall_median}{6.2}
\defres{e21b/e12_in/wins}{1}
\defres{e21b/e18/acc_wrong_arg}{61}
\defres{e21b/e18/acc_wrong_tool}{383}
\defres{e21b/e18/api_k}{37.1}
\defres{e21b/e18/argcov}{56.6}
\defres{e21b/e18/deferred_llm_acc}{97.9}
\defres{e21b/e18/delta}{$-$35.5}
\defres{e21b/e18/delta_ci/hi}{$-$28.9}
\defres{e21b/e18/delta_ci/lo}{$-$42.3}
\defres{e21b/e18/errored}{0}
\defres{e21b/e18/genkinds}{62.9}
\defres{e21b/e18/handed_back}{32.8}
\defres{e21b/e18/in/argcov}{98.7}
\defres{e21b/e18/in/success}{100.0}
\defres{e21b/e18/in/toolcov}{100.0}
\defres{e21b/e18/llm_calls}{6.1}
\defres{e21b/e18/losses}{71}
\defres{e21b/e18/mustask/n}{146}
\defres{e21b/e18/mustask/taken}{139}
\defres{e21b/e18/mustask/wrong}{33}
\defres{e21b/e18/n}{200}
\defres{e21b/e18/newkinds}{68.3}
\defres{e21b/e18/ni/hi}{$-$29.2}
\defres{e21b/e18/ni/lo}{$-$42.3}
\defres{e21b/e18/ni/p}{1.000}
\defres{e21b/e18/ni/verdict}{not shown}
\defres{e21b/e18/ref_success}{100.0}
\defres{e21b/e18/ref_wall}{8.0}
\defres{e21b/e18/replace/delta}{+47.0}
\defres{e21b/e18/replace/success}{17.5}
\defres{e21b/e18/saving}{24.8}
\defres{e21b/e18/saving_api}{30.7}
\defres{e21b/e18/saving_ci/hi}{32.1}
\defres{e21b/e18/saving_ci/lo}{17.1}
\defres{e21b/e18/steps}{7.3}
\defres{e21b/e18/success}{64.5}
\defres{e21b/e18/taken_arg}{446}
\defres{e21b/e18/taken_tool}{984}
\defres{e21b/e18/toolcov}{67.2}
\defres{e21b/e18/usd_k}{40.3}
\defres{e21b/e18/wall}{7.0}
\defres{e21b/e18/wall_median}{5.0}
\defres{e21b/e18/wins}{0}
\defres{e21b/n_ref}{200}
\defres{e21b/ref/success}{100.0}
\defres{e21b/ref/usd_k}{53.5}
\defres{e21b/ref/wall}{8.0}
\defres{e21b/rl/acc_wrong_arg}{17}
\defres{e21b/rl/acc_wrong_tool}{62}
\defres{e21b/rl/api_k}{14.6}
\defres{e21b/rl/argcov}{58.9}
\defres{e21b/rl/deferred_llm_acc}{100.0}
\defres{e21b/rl/delta}{$-$6.0}
\defres{e21b/rl/delta_ci/hi}{$-$2.8}
\defres{e21b/rl/delta_ci/lo}{$-$10.2}
\defres{e21b/rl/errored}{0}
\defres{e21b/rl/genkinds}{95.0}
\defres{e21b/rl/handed_back}{0.4}
\defres{e21b/rl/in/argcov}{85.5}
\defres{e21b/rl/in/success}{100.0}
\defres{e21b/rl/in/toolcov}{100.0}
\defres{e21b/rl/llm_calls}{5.0}
\defres{e21b/rl/losses}{12}
\defres{e21b/rl/mustask/n}{113}
\defres{e21b/rl/mustask/taken}{113}
\defres{e21b/rl/mustask/wrong}{7}
\defres{e21b/rl/n}{200}
\defres{e21b/rl/newkinds}{91.7}
\defres{e21b/rl/ni/hi}{$-$3.5}
\defres{e21b/rl/ni/lo}{$-$10.2}
\defres{e21b/rl/ni/p}{0.993}
\defres{e21b/rl/ni/verdict}{not shown}
\defres{e21b/rl/ref_success}{100.0}
\defres{e21b/rl/ref_wall}{8.0}
\defres{e21b/rl/replace/delta}{$-$2.0}
\defres{e21b/rl/replace/success}{96.0}
\defres{e21b/rl/saving}{64.8}
\defres{e21b/rl/saving_api}{72.8}
\defres{e21b/rl/saving_ci/hi}{67.8}
\defres{e21b/rl/saving_ci/lo}{60.9}
\defres{e21b/rl/steps}{6.9}
\defres{e21b/rl/success}{94.0}
\defres{e21b/rl/taken_arg}{959}
\defres{e21b/rl/taken_tool}{1364}
\defres{e21b/rl/toolcov}{99.6}
\defres{e21b/rl/usd_k}{18.9}
\defres{e21b/rl/wall}{9.5}
\defres{e21b/rl/wall_median}{7.0}
\defres{e21b/rl/wins}{0}
\defres{e21b/spend/gemini}{13.70}
\defres{e21b/tariff}{1.624}
\makeatother


==> generated/e22_tau2.tex <==
\makeatletter
\providecommand{\res}[1]{\ifcsname jevres@#1\endcsname\csname jevres@#1\endcsname\else\tbd\fi}
\providecommand{\defres}[2]{\expandafter\def\csname jevres@#1\endcsname{#2}}
\defres{e22/airline/e22_final/calls}{12.53}
\defres{e22/airline/e22_final/cost_k}{81.03}
\defres{e22/airline/e22_final/delta}{-12.5}
\defres{e22/airline/e22_final/hi}{-1.2}
\defres{e22/airline/e22_final/lcb}{-22.5}
\defres{e22/airline/e22_final/llmfree}{0.9}
\defres{e22/airline/e22_final/lo}{-25.0}
\defres{e22/airline/e22_final/losses}{5}
\defres{e22/airline/e22_final/n}{20}
\defres{e22/airline/e22_final/ni}{no}
\defres{e22/airline/e22_final/p}{1.000}
\defres{e22/airline/e22_final/pair/ni}{no}
\defres{e22/airline/e22_final/pair/p}{0.921}
\defres{e22/airline/e22_final/pairs}{80}
\defres{e22/airline/e22_final/passk}{35.0}
\defres{e22/airline/e22_final/refagree}{\tbd}
\defres{e22/airline/e22_final/saving}{2.5}
\defres{e22/airline/e22_final/saving_api}{3.6}
\defres{e22/airline/e22_final/saving_e9}{1.6}
\defres{e22/airline/e22_final/saving_hi}{10.3}
\defres{e22/airline/e22_final/saving_lo}{-4.5}
\defres{e22/airline/e22_final/success}{57.5}
\defres{e22/airline/e22_final/time_saving}{-34.8}
\defres{e22/airline/e22_final/tpcov}{25.7}
\defres{e22/airline/e22_final/wall_mean}{27.4}
\defres{e22/airline/e22_final/wins}{0}
\defres{e22/airline/e22_tau05/calls}{8.32}
\defres{e22/airline/e22_tau05/cost_k}{58.72}
\defres{e22/airline/e22_tau05/delta}{-6.2}
\defres{e22/airline/e22_tau05/hi}{+1.2}
\defres{e22/airline/e22_tau05/lcb}{-12.5}
\defres{e22/airline/e22_tau05/llmfree}{35.2}
\defres{e22/airline/e22_tau05/lo}{-15.0}
\defres{e22/airline/e22_tau05/losses}{2}
\defres{e22/airline/e22_tau05/n}{20}
\defres{e22/airline/e22_tau05/ni}{no}
\defres{e22/airline/e22_tau05/p}{0.926}
\defres{e22/airline/e22_tau05/pair/ni}{no}
\defres{e22/airline/e22_tau05/pair/p}{0.629}
\defres{e22/airline/e22_tau05/pairs}{80}
\defres{e22/airline/e22_tau05/passk}{30.0}
\defres{e22/airline/e22_tau05/refagree}{64.8}
\defres{e22/airline/e22_tau05/saving}{29.4}
\defres{e22/airline/e22_tau05/saving_api}{30.4}
\defres{e22/airline/e22_tau05/saving_e9}{28.4}
\defres{e22/airline/e22_tau05/saving_hi}{37.5}
\defres{e22/airline/e22_tau05/saving_lo}{21.0}
\defres{e22/airline/e22_tau05/success}{63.7}
\defres{e22/airline/e22_tau05/time_saving}{-49.1}
\defres{e22/airline/e22_tau05/tpcov}{49.8}
\defres{e22/airline/e22_tau05/wall_mean}{30.3}
\defres{e22/airline/e22_tau05/wins}{0}
\defres{e22/airline/llm_only/calls}{12.79}
\defres{e22/airline/llm_only/cost_k}{83.13}
\defres{e22/airline/llm_only/passk}{50.0}
\defres{e22/airline/llm_only/success}{70.0}
\defres{e22/airline/llm_only/wall_mean}{20.4}
\defres{e22/audit/coverage}{71.5}
\defres{e22/audit/fail/listed}{100}
\defres{e22/audit/fail/match}{100}
\defres{e22/audit/fail/match_listed_pct}{100.0}
\defres{e22/audit/fail/n}{100}
\defres{e22/audit/fail/ref_agree_pct}{93.8}
\defres{e22/audit/fail/ref_n}{97}
\defres{e22/audit/fail/toollabels}{100}
\defres{e22/audit/labelled}{7{,}116}
\defres{e22/audit/succ/listed}{42}
\defres{e22/audit/succ/match}{37}
\defres{e22/audit/succ/match_listed_pct}{88.1}
\defres{e22/audit/succ/n}{100}
\defres{e22/audit/succ/ref_agree_pct}{75.0}
\defres{e22/audit/succ/ref_n}{48}
\defres{e22/audit/succ/toollabels}{67}
\defres{e22/data/dev_records}{2{,}940}
\defres{e22/data/episodes}{832}
\defres{e22/data/fit_records}{11{,}096}
\defres{e22/data/states}{9{,}959}
\defres{e22/dev/tool_params/acc}{95.5}
\defres{e22/dev/tool_params/cov}{49.8}
\defres{e22/dev/tool_params/wrong}{0}
\defres{e22/dev/tool_select/acc}{84.6}
\defres{e22/dev/tool_select/cov}{13.3}
\defres{e22/dev/tool_select/wrong}{0}
\defres{e22/diag/e22_final/emitted}{111}
\defres{e22/diag/e22_final/s1_s}{7.9}
\defres{e22/diag/e22_final/tasks_lost}{22}
\defres{e22/diag/e22_final/tasks_lost_noemit}{13}
\defres{e22/diag/e22_final/writes}{3}
\defres{e22/diag/e22_tau05/emitted}{1{,}141}
\defres{e22/diag/e22_tau05/s1_s}{13.0}
\defres{e22/diag/e22_tau05/tasks_lost}{20}
\defres{e22/diag/e22_tau05/tasks_lost_noemit}{0}
\defres{e22/diag/e22_tau05/writes}{70}
\defres{e22/diag/noise_sd}{3.6}
\defres{e22/gpu/hours}{5.4}
\defres{e22/k}{4}
\defres{e22/pooled/e22_final/calls}{11.30}
\defres{e22/pooled/e22_final/cost_k}{73.70}
\defres{e22/pooled/e22_final/delta}{-12.1}
\defres{e22/pooled/e22_final/hi}{-5.4}
\defres{e22/pooled/e22_final/lcb}{-17.9}
\defres{e22/pooled/e22_final/llmfree}{3.9}
\defres{e22/pooled/e22_final/lo}{-19.2}
\defres{e22/pooled/e22_final/losses}{12}
\defres{e22/pooled/e22_final/n}{60}
\defres{e22/pooled/e22_final/ni}{no}
\defres{e22/pooled/e22_final/p}{0.979}
\defres{e22/pooled/e22_final/pair/ni}{no}
\defres{e22/pooled/e22_final/pair/p}{0.986}
\defres{e22/pooled/e22_final/pairs}{240}
\defres{e22/pooled/e22_final/passk}{31.7}
\defres{e22/pooled/e22_final/refagree}{87.5}
\defres{e22/pooled/e22_final/saving}{4.6}
\defres{e22/pooled/e22_final/saving_api}{5.8}
\defres{e22/pooled/e22_final/saving_e9}{3.6}
\defres{e22/pooled/e22_final/saving_hi}{8.4}
\defres{e22/pooled/e22_final/saving_lo}{0.8}
\defres{e22/pooled/e22_final/success}{54.2}
\defres{e22/pooled/e22_final/time_saving}{-35.8}
\defres{e22/pooled/e22_final/tpcov}{21.0}
\defres{e22/pooled/e22_final/wall_mean}{26.9}
\defres{e22/pooled/e22_final/wins}{2}
\defres{e22/pooled/e22_tau05/calls}{7.45}
\defres{e22/pooled/e22_tau05/cost_k}{53.09}
\defres{e22/pooled/e22_tau05/delta}{-7.1}
\defres{e22/pooled/e22_tau05/hi}{-0.4}
\defres{e22/pooled/e22_tau05/lcb}{-12.9}
\defres{e22/pooled/e22_tau05/llmfree}{39.0}
\defres{e22/pooled/e22_tau05/lo}{-13.8}
\defres{e22/pooled/e22_tau05/losses}{7}
\defres{e22/pooled/e22_tau05/n}{60}
\defres{e22/pooled/e22_tau05/ni}{no}
\defres{e22/pooled/e22_tau05/p}{0.654}
\defres{e22/pooled/e22_tau05/pair/ni}{no}
\defres{e22/pooled/e22_tau05/pair/p}{0.725}
\defres{e22/pooled/e22_tau05/pairs}{240}
\defres{e22/pooled/e22_tau05/passk}{25.0}
\defres{e22/pooled/e22_tau05/refagree}{80.0}
\defres{e22/pooled/e22_tau05/saving}{31.3}
\defres{e22/pooled/e22_tau05/saving_api}{32.5}
\defres{e22/pooled/e22_tau05/saving_e9}{30.3}
\defres{e22/pooled/e22_tau05/saving_hi}{35.2}
\defres{e22/pooled/e22_tau05/saving_lo}{27.4}
\defres{e22/pooled/e22_tau05/success}{59.2}
\defres{e22/pooled/e22_tau05/time_saving}{-41.0}
\defres{e22/pooled/e22_tau05/tpcov}{56.2}
\defres{e22/pooled/e22_tau05/wall_mean}{28.0}
\defres{e22/pooled/e22_tau05/wins}{3}
\defres{e22/pooled/llm_only/calls}{11.95}
\defres{e22/pooled/llm_only/cost_k}{77.25}
\defres{e22/pooled/llm_only/passk}{40.0}
\defres{e22/pooled/llm_only/success}{66.2}
\defres{e22/pooled/llm_only/wall_mean}{19.8}
\defres{e22/q_cents}{0.09}
\defres{e22/retail/e22_final/calls}{10.69}
\defres{e22/retail/e22_final/cost_k}{70.04}
\defres{e22/retail/e22_final/delta}{-11.9}
\defres{e22/retail/e22_final/hi}{-3.8}
\defres{e22/retail/e22_final/lcb}{-19.4}
\defres{e22/retail/e22_final/llmfree}{5.6}
\defres{e22/retail/e22_final/lo}{-20.6}
\defres{e22/retail/e22_final/losses}{7}
\defres{e22/retail/e22_final/n}{40}
\defres{e22/retail/e22_final/ni}{no}
\defres{e22/retail/e22_final/p}{0.857}
\defres{e22/retail/e22_final/pair/ni}{no}
\defres{e22/retail/e22_final/pair/p}{0.955}
\defres{e22/retail/e22_final/pairs}{160}
\defres{e22/retail/e22_final/passk}{30.0}
\defres{e22/retail/e22_final/refagree}{87.5}
\defres{e22/retail/e22_final/saving}{5.8}
\defres{e22/retail/e22_final/saving_api}{7.0}
\defres{e22/retail/e22_final/saving_e9}{4.7}
\defres{e22/retail/e22_final/saving_hi}{9.9}
\defres{e22/retail/e22_final/saving_lo}{1.7}
\defres{e22/retail/e22_final/success}{52.5}
\defres{e22/retail/e22_final/time_saving}{-36.4}
\defres{e22/retail/e22_final/tpcov}{20.6}
\defres{e22/retail/e22_final/wall_mean}{26.7}
\defres{e22/retail/e22_final/wins}{2}
\defres{e22/retail/e22_tau05/calls}{7.01}
\defres{e22/retail/e22_tau05/cost_k}{50.27}
\defres{e22/retail/e22_tau05/delta}{-7.5}
\defres{e22/retail/e22_tau05/hi}{+1.9}
\defres{e22/retail/e22_tau05/lcb}{-15.6}
\defres{e22/retail/e22_tau05/llmfree}{41.0}
\defres{e22/retail/e22_tau05/lo}{-16.9}
\defres{e22/retail/e22_tau05/losses}{5}
\defres{e22/retail/e22_tau05/n}{40}
\defres{e22/retail/e22_tau05/ni}{no}
\defres{e22/retail/e22_tau05/p}{0.560}
\defres{e22/retail/e22_tau05/pair/ni}{no}
\defres{e22/retail/e22_tau05/pair/p}{0.706}
\defres{e22/retail/e22_tau05/pairs}{160}
\defres{e22/retail/e22_tau05/passk}{22.5}
\defres{e22/retail/e22_tau05/refagree}{86.4}
\defres{e22/retail/e22_tau05/saving}{32.4}
\defres{e22/retail/e22_tau05/saving_api}{33.6}
\defres{e22/retail/e22_tau05/saving_e9}{31.3}
\defres{e22/retail/e22_tau05/saving_hi}{36.2}
\defres{e22/retail/e22_tau05/saving_lo}{28.4}
\defres{e22/retail/e22_tau05/success}{56.9}
\defres{e22/retail/e22_tau05/time_saving}{-36.8}
\defres{e22/retail/e22_tau05/tpcov}{59.8}
\defres{e22/retail/e22_tau05/wall_mean}{26.8}
\defres{e22/retail/e22_tau05/wins}{3}
\defres{e22/retail/llm_only/calls}{11.54}
\defres{e22/retail/llm_only/cost_k}{74.32}
\defres{e22/retail/llm_only/passk}{35.0}
\defres{e22/retail/llm_only/success}{64.4}
\defres{e22/retail/llm_only/wall_mean}{19.6}
\defres{e22/spend/gemini}{120.69}
\defres{e22/tau/tool_params}{0.9980}
\defres{e22/tau/tool_select}{0.9945}
\defres{e22/train/base_acc}{36.1}
\defres{e22/train/dev_acc}{89.9}
\defres{e22/train/epochs}{2}
\makeatother


==> generated/e23_alfworld_unseen.tex <==
\makeatletter
\providecommand{\res}[1]{\ifcsname jevres@#1\endcsname\csname jevres@#1\endcsname\else\tbd\fi}
\providecommand{\defres}[2]{\expandafter\def\csname jevres@#1\endcsname{#2}}
\defres{e23/cascade/acc}{63.0}
\defres{e23/cascade/cost_k}{0.1}
\defres{e23/cascade/coverage}{99.4}
\defres{e23/cascade/deferred_llm_acc}{0.0}
\defres{e23/cascade/delta}{+0.7}
\defres{e23/cascade/delta_ci/hi}{+8.2}
\defres{e23/cascade/delta_ci/lo}{-6.7}
\defres{e23/cascade/llm_calls}{0.1}
\defres{e23/cascade/losses}{13}
\defres{e23/cascade/n}{134}
\defres{e23/cascade/ni/hi}{+8.7}
\defres{e23/cascade/ni/lo}{-7.1}
\defres{e23/cascade/ni/p}{0.175}
\defres{e23/cascade/ni/verdict}{not shown}
\defres{e23/cascade/ni/yes}{no}
\defres{e23/cascade/saving}{92.0}
\defres{e23/cascade/saving_api}{99.6}
\defres{e23/cascade/saving_ci/hi}{93.6}
\defres{e23/cascade/saving_ci/lo}{89.7}
\defres{e23/cascade/saving_q_s2_4}{90.5}
\defres{e23/cascade/saving_q_zero}{99.6}
\defres{e23/cascade/status}{run}
\defres{e23/cascade/steps}{16.4}
\defres{e23/cascade/success}{89.6}
\defres{e23/cascade/taken/mean_conf}{0.79}
\defres{e23/cascade/taken/n}{2{,}178}
\defres{e23/cascade/taken/n_deferred}{13}
\defres{e23/cascade/taken/n_gold}{2{,}178}
\defres{e23/cascade/taken/n_wrong}{805}
\defres{e23/cascade/taken/wrong_share}{37.0}
\defres{e23/cascade/wall_mean}{18.2}
\defres{e23/cascade/wall_median}{12.5}
\defres{e23/cascade/wins}{14}
\defres{e23/host/hours}{0.74}
\defres{e23/label}{exploratory (E23)}
\defres{e23/llm_only/cost_k}{21.5}
\defres{e23/llm_only/llm_acc}{36.9}
\defres{e23/llm_only/n}{134}
\defres{e23/llm_only/steps}{14.8}
\defres{e23/llm_only/success}{88.8}
\defres{e23/llm_only/wall_mean}{35.1}
\defres{e23/llm_only/wall_median}{22.7}
\defres{e23/n_games}{134}
\defres{e23/n_scenes}{4}
\defres{e23/pilot_contact/n}{5}
\defres{e23/replace/acc}{62.6}
\defres{e23/replace/cost_k}{0.0}
\defres{e23/replace/coverage}{100.0}
\defres{e23/replace/delta}{-0.7}
\defres{e23/replace/delta_ci/hi}{+7.5}
\defres{e23/replace/delta_ci/lo}{-8.2}
\defres{e23/replace/llm_calls}{0.0}
\defres{e23/replace/losses}{15}
\defres{e23/replace/n}{134}
\defres{e23/replace/ni/hi}{+7.4}
\defres{e23/replace/ni/lo}{-8.9}
\defres{e23/replace/ni/p}{0.301}
\defres{e23/replace/ni/verdict}{not shown}
\defres{e23/replace/ni/yes}{no}
\defres{e23/replace/saving}{92.4}
\defres{e23/replace/saving_api}{100.0}
\defres{e23/replace/saving_ci/hi}{93.9}
\defres{e23/replace/saving_ci/lo}{90.2}
\defres{e23/replace/saving_q_s2_4}{90.9}
\defres{e23/replace/saving_q_zero}{100.0}
\defres{e23/replace/status}{run}
\defres{e23/replace/steps}{16.7}
\defres{e23/replace/success}{88.1}
\defres{e23/replace/taken/mean_conf}{0.78}
\defres{e23/replace/taken/n}{2{,}239}
\defres{e23/replace/taken/n_deferred}{0}
\defres{e23/replace/taken/n_gold}{2{,}239}
\defres{e23/replace/taken/n_wrong}{838}
\defres{e23/replace/taken/wrong_share}{37.4}
\defres{e23/replace/wall_mean}{18.8}
\defres{e23/replace/wall_median}{12.9}
\defres{e23/replace/wins}{14}
\defres{e23/seen/cascade/ni/p}{0.014}
\defres{e23/seen/cascade/ni/verdict}{non-inferior}
\defres{e23/seen/replace/ni/p}{0.007}
\defres{e23/seen/replace/ni/verdict}{non-inferior}
\defres{e23/seen_change/cascade}{-5.4}
\defres{e23/seen_change/llm_only}{-1.9}
\defres{e23/seen_change/replace}{-7.7}
\defres{e23/spend/gemini}{2.90}
\defres{e23/tariff/host_usd_h}{1.212}
\defres{e23/tariff/q}{0.00163}
\defres{e23/tau}{0.12}
\defres{e23/type/clean/cascade}{94}
\defres{e23/type/clean/llm_only}{68}
\defres{e23/type/clean/n}{31}
\defres{e23/type/clean/replace}{90}
\defres{e23/type/cool/cascade}{86}
\defres{e23/type/cool/llm_only}{90}
\defres{e23/type/cool/n}{21}
\defres{e23/type/cool/replace}{86}
\defres{e23/type/heat/cascade}{96}
\defres{e23/type/heat/llm_only}{87}
\defres{e23/type/heat/n}{23}
\defres{e23/type/heat/replace}{91}
\defres{e23/type/light/cascade}{78}
\defres{e23/type/light/llm_only}{100}
\defres{e23/type/light/n}{18}
\defres{e23/type/light/replace}{78}
\defres{e23/type/simple/cascade}{88}
\defres{e23/type/simple/llm_only}{100}
\defres{e23/type/simple/n}{24}
\defres{e23/type/simple/replace}{88}
\defres{e23/type/two/cascade}{94}
\defres{e23/type/two/llm_only}{100}
\defres{e23/type/two/n}{17}
\defres{e23/type/two/replace}{94}
\makeatother


==> generated/e24_public_l2.tex <==
\makeatletter
\providecommand{\res}[1]{\ifcsname jevres@#1\endcsname\csname jevres@#1\endcsname\else\tbd\fi}
\providecommand{\defres}[2]{\expandafter\def\csname jevres@#1\endcsname{#2}}
\defres{e24/alf/n/dropped}{469}
\defres{e24/alf/n/games}{274}
\defres{e24/alf/n/questions}{3{,}263}
\defres{e24/alf/n/seen/games}{140}
\defres{e24/alf/n/seen/states}{1{,}660}
\defres{e24/alf/n/states}{3{,}355}
\defres{e24/alf/n/steps}{3{,}824}
\defres{e24/alf/n/unseen/games}{134}
\defres{e24/alf/n/unseen/states}{1{,}695}
\defres{e24/alf/seen/off_plan_share}{87.0}
\defres{e24/alf/seen/options_median}{31}
\defres{e24/alf/seen/set/acceptable}{8.3}
\defres{e24/alf/seen/set/acceptable_share}{25.4}
\defres{e24/alf/seen/set/lenient}{4.7}
\defres{e24/alf/seen/set/options}{33.2}
\defres{e24/alf/unseen/off_plan_share}{89.5}
\defres{e24/alf/unseen/options_median}{28}
\defres{e24/alf/unseen/set/acceptable}{3.9}
\defres{e24/alf/unseen/set/acceptable_share}{15.0}
\defres{e24/alf/unseen/set/lenient}{3.0}
\defres{e24/alf/unseen/set/options}{25.9}
\defres{e24/e11/errors}{0}
\defres{e24/e11/mean_conf}{81.8}
\defres{e24/e11/pooled/acceptable}{92.8}
\defres{e24/e11/pooled/acceptable/hi}{94.1}
\defres{e24/e11/pooled/acceptable/lo}{91.3}
\defres{e24/e11/pooled/after_off_plan}{96.9}
\defres{e24/e11/pooled/lenient}{88.6}
\defres{e24/e11/pooled/logged}{79.8}
\defres{e24/e11/pooled/on_plan}{66.8}
\defres{e24/e11/pooled/strict}{84.5}
\defres{e24/e11/pooled/tt/clean}{93.8}
\defres{e24/e11/pooled/tt/cool}{94.3}
\defres{e24/e11/pooled/tt/heat}{91.7}
\defres{e24/e11/pooled/tt/look}{90.7}
\defres{e24/e11/pooled/tt/pick2}{97.0}
\defres{e24/e11/pooled/tt/place}{89.3}
\defres{e24/e11/seen/acceptable}{93.9}
\defres{e24/e11/seen/acceptable/hi}{95.5}
\defres{e24/e11/seen/acceptable/lo}{92.1}
\defres{e24/e11/seen/after_off_plan}{97.6}
\defres{e24/e11/seen/lenient}{89.2}
\defres{e24/e11/seen/logged}{79.2}
\defres{e24/e11/seen/on_plan}{69.4}
\defres{e24/e11/seen/strict}{83.2}
\defres{e24/e11/seen/tt/clean}{94.1}
\defres{e24/e11/seen/tt/cool}{94.1}
\defres{e24/e11/seen/tt/heat}{93.5}
\defres{e24/e11/seen/tt/look}{90.2}
\defres{e24/e11/seen/tt/pick2}{97.2}
\defres{e24/e11/seen/tt/place}{93.0}
\defres{e24/e11/seen_to_unseen}{-2.4}
\defres{e24/e11/unseen/acceptable}{91.5}
\defres{e24/e11/unseen/acceptable/hi}{93.5}
\defres{e24/e11/unseen/acceptable/lo}{89.4}
\defres{e24/e11/unseen/after_off_plan}{96.1}
\defres{e24/e11/unseen/lenient}{87.9}
\defres{e24/e11/unseen/logged}{80.5}
\defres{e24/e11/unseen/on_plan}{64.1}
\defres{e24/e11/unseen/strict}{85.9}
\defres{e24/e11/unseen/tt/clean}{93.5}
\defres{e24/e11/unseen/tt/cool}{94.5}
\defres{e24/e11/unseen/tt/heat}{90.4}
\defres{e24/e11/unseen/tt/look}{91.0}
\defres{e24/e11/unseen/tt/pick2}{96.9}
\defres{e24/e11/unseen/tt/place}{84.1}
\defres{e24/e12/errors}{0}
\defres{e24/e12/mean_conf}{94.8}
\defres{e24/e12/pooled/acceptable}{64.7}
\defres{e24/e12/pooled/acceptable/hi}{67.7}
\defres{e24/e12/pooled/acceptable/lo}{61.6}
\defres{e24/e12/pooled/after_off_plan}{69.5}
\defres{e24/e12/pooled/lenient}{57.6}
\defres{e24/e12/pooled/logged}{46.5}
\defres{e24/e12/pooled/on_plan}{31.1}
\defres{e24/e12/pooled/strict}{46.9}
\defres{e24/e12/pooled/tt/clean}{60.9}
\defres{e24/e12/pooled/tt/cool}{55.1}
\defres{e24/e12/pooled/tt/heat}{59.5}
\defres{e24/e12/pooled/tt/look}{38.5}
\defres{e24/e12/pooled/tt/pick2}{83.4}
\defres{e24/e12/pooled/tt/place}{80.1}
\defres{e24/e12/seen/acceptable}{66.5}
\defres{e24/e12/seen/acceptable/hi}{70.9}
\defres{e24/e12/seen/acceptable/lo}{61.7}
\defres{e24/e12/seen/after_off_plan}{72.2}
\defres{e24/e12/seen/lenient}{59.2}
\defres{e24/e12/seen/logged}{47.4}
\defres{e24/e12/seen/on_plan}{31.9}
\defres{e24/e12/seen/strict}{47.7}
\defres{e24/e12/seen/tt/clean}{63.6}
\defres{e24/e12/seen/tt/cool}{49.2}
\defres{e24/e12/seen/tt/heat}{57.8}
\defres{e24/e12/seen/tt/look}{38.7}
\defres{e24/e12/seen/tt/pick2}{83.9}
\defres{e24/e12/seen/tt/place}{83.4}
\defres{e24/e12/seen_to_unseen}{-3.6}
\defres{e24/e12/tau2/args/airline}{86.4}
\defres{e24/e12/tau2/args/pooled}{89.1}
\defres{e24/e12/tau2/args/retail}{90.0}
\defres{e24/e12/tau2/call/airline}{38.5}
\defres{e24/e12/tau2/call/pooled}{53.4}
\defres{e24/e12/tau2/call/retail}{58.0}
\defres{e24/e12/tau2/tool/airline}{45.3}
\defres{e24/e12/tau2/tool/airline/hi}{62.7}
\defres{e24/e12/tau2/tool/airline/lo}{29.2}
\defres{e24/e12/tau2/tool/pooled}{62.7}
\defres{e24/e12/tau2/tool/pooled/hi}{71.0}
\defres{e24/e12/tau2/tool/pooled/lo}{53.7}
\defres{e24/e12/tau2/tool/retail}{68.2}
\defres{e24/e12/tau2/tool/retail/hi}{77.4}
\defres{e24/e12/tau2/tool/retail/lo}{58.4}
\defres{e24/e12/tau2/wrong_write/airline}{10.2}
\defres{e24/e12/tau2/wrong_write/pooled}{9.7}
\defres{e24/e12/tau2/wrong_write/retail}{9.6}
\defres{e24/e12/unseen/acceptable}{62.9}
\defres{e24/e12/unseen/acceptable/hi}{66.6}
\defres{e24/e12/unseen/acceptable/lo}{58.8}
\defres{e24/e12/unseen/after_off_plan}{66.9}
\defres{e24/e12/unseen/lenient}{55.8}
\defres{e24/e12/unseen/logged}{45.5}
\defres{e24/e12/unseen/on_plan}{30.2}
\defres{e24/e12/unseen/strict}{45.9}
\defres{e24/e12/unseen/tt/clean}{58.6}
\defres{e24/e12/unseen/tt/cool}{62.2}
\defres{e24/e12/unseen/tt/heat}{60.7}
\defres{e24/e12/unseen/tt/look}{38.4}
\defres{e24/e12/unseen/tt/pick2}{82.6}
\defres{e24/e12/unseen/tt/place}{75.3}
\defres{e24/e14a/errors}{0}
\defres{e24/e14a/mean_conf}{92.4}
\defres{e24/e14a/pooled/acceptable}{48.8}
\defres{e24/e14a/pooled/acceptable/hi}{51.4}
\defres{e24/e14a/pooled/acceptable/lo}{46.1}
\defres{e24/e14a/pooled/after_off_plan}{47.8}
\defres{e24/e14a/pooled/lenient}{38.8}
\defres{e24/e14a/pooled/logged}{30.6}
\defres{e24/e14a/pooled/on_plan}{44.3}
\defres{e24/e14a/pooled/strict}{30.2}
\defres{e24/e14a/pooled/tt/clean}{39.4}
\defres{e24/e14a/pooled/tt/cool}{37.4}
\defres{e24/e14a/pooled/tt/heat}{51.2}
\defres{e24/e14a/pooled/tt/look}{42.3}
\defres{e24/e14a/pooled/tt/pick2}{53.5}
\defres{e24/e14a/pooled/tt/place}{65.4}
\defres{e24/e14a/seen/acceptable}{49.2}
\defres{e24/e14a/seen/acceptable/hi}{52.8}
\defres{e24/e14a/seen/acceptable/lo}{45.2}
\defres{e24/e14a/seen/after_off_plan}{47.6}
\defres{e24/e14a/seen/lenient}{38.5}
\defres{e24/e14a/seen/logged}{30.8}
\defres{e24/e14a/seen/on_plan}{45.3}
\defres{e24/e14a/seen/strict}{30.6}
\defres{e24/e14a/seen/tt/clean}{41.3}
\defres{e24/e14a/seen/tt/cool}{33.6}
\defres{e24/e14a/seen/tt/heat}{50.8}
\defres{e24/e14a/seen/tt/look}{46.8}
\defres{e24/e14a/seen/tt/pick2}{54.0}
\defres{e24/e14a/seen/tt/place}{63.3}
\defres{e24/e14a/seen_to_unseen}{-0.8}
\defres{e24/e14a/tau2/args/airline}{73.1}
\defres{e24/e14a/tau2/args/pooled}{64.5}
\defres{e24/e14a/tau2/args/retail}{61.8}
\defres{e24/e14a/tau2/call/airline}{16.9}
\defres{e24/e14a/tau2/call/pooled}{24.0}
\defres{e24/e14a/tau2/call/retail}{26.3}
\defres{e24/e14a/tau2/tool/airline}{39.2}
\defres{e24/e14a/tau2/tool/airline/hi}{65.2}
\defres{e24/e14a/tau2/tool/airline/lo}{14.4}
\defres{e24/e14a/tau2/tool/pooled}{61.8}
\defres{e24/e14a/tau2/tool/pooled/hi}{71.6}
\defres{e24/e14a/tau2/tool/pooled/lo}{50.7}
\defres{e24/e14a/tau2/tool/retail}{68.9}
\defres{e24/e14a/tau2/tool/retail/hi}{78.2}
\defres{e24/e14a/tau2/tool/retail/lo}{58.9}
\defres{e24/e14a/tau2/wrong_write/airline}{14.3}
\defres{e24/e14a/tau2/wrong_write/pooled}{16.1}
\defres{e24/e14a/tau2/wrong_write/retail}{16.6}
\defres{e24/e14a/unseen/acceptable}{48.4}
\defres{e24/e14a/unseen/acceptable/hi}{52.0}
\defres{e24/e14a/unseen/acceptable/lo}{44.8}
\defres{e24/e14a/unseen/after_off_plan}{47.9}
\defres{e24/e14a/unseen/lenient}{39.1}
\defres{e24/e14a/unseen/logged}{30.4}
\defres{e24/e14a/unseen/on_plan}{43.2}
\defres{e24/e14a/unseen/strict}{29.8}
\defres{e24/e14a/unseen/tt/clean}{37.8}
\defres{e24/e14a/unseen/tt/cool}{42.1}
\defres{e24/e14a/unseen/tt/heat}{51.5}
\defres{e24/e14a/unseen/tt/look}{39.1}
\defres{e24/e14a/unseen/tt/pick2}{52.9}
\defres{e24/e14a/unseen/tt/place}{68.5}
\defres{e24/e22/tau2/args/airline}{92.4}
\defres{e24/e22/tau2/args/pooled}{92.1}
\defres{e24/e22/tau2/args/retail}{92.0}
\defres{e24/e22/tau2/call/airline}{39.8}
\defres{e24/e22/tau2/call/pooled}{42.7}
\defres{e24/e22/tau2/call/retail}{43.6}
\defres{e24/e22/tau2/tool/airline}{45.2}
\defres{e24/e22/tau2/tool/airline/hi}{59.4}
\defres{e24/e22/tau2/tool/airline/lo}{29.4}
\defres{e24/e22/tau2/tool/pooled}{46.6}
\defres{e24/e22/tau2/tool/pooled/hi}{54.0}
\defres{e24/e22/tau2/tool/pooled/lo}{39.2}
\defres{e24/e22/tau2/tool/retail}{47.0}
\defres{e24/e22/tau2/tool/retail/hi}{56.1}
\defres{e24/e22/tau2/tool/retail/lo}{38.6}
\defres{e24/e22/tau2/wrong_write/airline}{4.7}
\defres{e24/e22/tau2/wrong_write/pooled}{4.6}
\defres{e24/e22/tau2/wrong_write/retail}{4.6}
\defres{e24/flash/pooled/acceptable}{80.9}
\defres{e24/flash/pooled/acceptable/hi}{83.8}
\defres{e24/flash/pooled/acceptable/lo}{78.2}
\defres{e24/flash/pooled/after_off_plan}{85.3}
\defres{e24/flash/pooled/lenient}{73.3}
\defres{e24/flash/pooled/logged}{58.7}
\defres{e24/flash/pooled/on_plan}{54.9}
\defres{e24/flash/pooled/strict}{58.7}
\defres{e24/flash/pooled/tt/clean}{70.6}
\defres{e24/flash/pooled/tt/cool}{72.0}
\defres{e24/flash/pooled/tt/heat}{82.1}
\defres{e24/flash/pooled/tt/look}{80.5}
\defres{e24/flash/pooled/tt/pick2}{94.2}
\defres{e24/flash/pooled/tt/place}{88.3}
\defres{e24/flash/seen/acceptable}{81.1}
\defres{e24/flash/seen/acceptable/hi}{84.6}
\defres{e24/flash/seen/acceptable/lo}{77.1}
\defres{e24/flash/seen/after_off_plan}{87.1}
\defres{e24/flash/seen/lenient}{74.9}
\defres{e24/flash/seen/logged}{59.6}
\defres{e24/flash/seen/on_plan}{49.0}
\defres{e24/flash/seen/strict}{59.3}
\defres{e24/flash/seen/tt/clean}{74.3}
\defres{e24/flash/seen/tt/cool}{67.1}
\defres{e24/flash/seen/tt/heat}{79.7}
\defres{e24/flash/seen/tt/look}{80.3}
\defres{e24/flash/seen/tt/pick2}{95.5}
\defres{e24/flash/seen/tt/place}{87.5}
\defres{e24/flash/tau2/args/airline}{97.0}
\defres{e24/flash/tau2/args/pooled}{98.1}
\defres{e24/flash/tau2/args/retail}{98.4}
\defres{e24/flash/tau2/call/airline}{38.4}
\defres{e24/flash/tau2/call/pooled}{46.0}
\defres{e24/flash/tau2/call/retail}{48.4}
\defres{e24/flash/tau2/tool/airline}{41.0}
\defres{e24/flash/tau2/tool/airline/hi}{55.2}
\defres{e24/flash/tau2/tool/airline/lo}{25.9}
\defres{e24/flash/tau2/tool/pooled}{47.7}
\defres{e24/flash/tau2/tool/pooled/hi}{55.1}
\defres{e24/flash/tau2/tool/pooled/lo}{40.1}
\defres{e24/flash/tau2/tool/retail}{49.8}
\defres{e24/flash/tau2/tool/retail/hi}{58.4}
\defres{e24/flash/tau2/tool/retail/lo}{41.6}
\defres{e24/flash/tau2/wrong_write/airline}{4.6}
\defres{e24/flash/tau2/wrong_write/pooled}{4.0}
\defres{e24/flash/tau2/wrong_write/retail}{3.8}
\defres{e24/flash/unseen/acceptable}{80.8}
\defres{e24/flash/unseen/acceptable/hi}{84.8}
\defres{e24/flash/unseen/acceptable/lo}{76.3}
\defres{e24/flash/unseen/after_off_plan}{83.6}
\defres{e24/flash/unseen/lenient}{71.7}
\defres{e24/flash/unseen/logged}{57.7}
\defres{e24/flash/unseen/on_plan}{60.9}
\defres{e24/flash/unseen/strict}{58.1}
\defres{e24/flash/unseen/tt/clean}{67.4}
\defres{e24/flash/unseen/tt/cool}{77.8}
\defres{e24/flash/unseen/tt/heat}{83.8}
\defres{e24/flash/unseen/tt/look}{80.6}
\defres{e24/flash/unseen/tt/pick2}{92.4}
\defres{e24/flash/unseen/tt/place}{89.5}
\defres{e24/host_hours}{6.7}
\defres{e24/jev/errors}{0}
\defres{e24/jev/mean_conf}{67.5}
\defres{e24/jev/pooled/acceptable}{67.9}
\defres{e24/jev/pooled/acceptable/hi}{70.9}
\defres{e24/jev/pooled/acceptable/lo}{64.8}
\defres{e24/jev/pooled/after_off_plan}{70.1}
\defres{e24/jev/pooled/lenient}{60.1}
\defres{e24/jev/pooled/logged}{49.6}
\defres{e24/jev/pooled/on_plan}{46.7}
\defres{e24/jev/pooled/strict}{49.0}
\defres{e24/jev/pooled/tt/clean}{64.8}
\defres{e24/jev/pooled/tt/cool}{60.4}
\defres{e24/jev/pooled/tt/heat}{63.1}
\defres{e24/jev/pooled/tt/look}{35.0}
\defres{e24/jev/pooled/tt/pick2}{88.2}
\defres{e24/jev/pooled/tt/place}{83.2}
\defres{e24/jev/seen/acceptable}{70.5}
\defres{e24/jev/seen/acceptable/hi}{74.7}
\defres{e24/jev/seen/acceptable/lo}{65.8}
\defres{e24/jev/seen/after_off_plan}{73.4}
\defres{e24/jev/seen/lenient}{61.6}
\defres{e24/jev/seen/logged}{50.2}
\defres{e24/jev/seen/on_plan}{49.6}
\defres{e24/jev/seen/strict}{49.7}
\defres{e24/jev/seen/tt/clean}{67.1}
\defres{e24/jev/seen/tt/cool}{57.1}
\defres{e24/jev/seen/tt/heat}{66.0}
\defres{e24/jev/seen/tt/look}{32.5}
\defres{e24/jev/seen/tt/pick2}{87.5}
\defres{e24/jev/seen/tt/place}{87.2}
\defres{e24/jev/seen_to_unseen}{-5.2}
\defres{e24/jev/tau2/args/airline}{90.9}
\defres{e24/jev/tau2/args/pooled}{91.3}
\defres{e24/jev/tau2/args/retail}{91.4}
\defres{e24/jev/tau2/call/airline}{35.7}
\defres{e24/jev/tau2/call/pooled}{46.1}
\defres{e24/jev/tau2/call/retail}{49.4}
\defres{e24/jev/tau2/tool/airline}{42.8}
\defres{e24/jev/tau2/tool/airline/hi}{59.2}
\defres{e24/jev/tau2/tool/airline/lo}{27.0}
\defres{e24/jev/tau2/tool/pooled}{52.0}
\defres{e24/jev/tau2/tool/pooled/hi}{59.9}
\defres{e24/jev/tau2/tool/pooled/lo}{43.9}
\defres{e24/jev/tau2/tool/retail}{54.9}
\defres{e24/jev/tau2/tool/retail/hi}{63.6}
\defres{e24/jev/tau2/tool/retail/lo}{46.7}
\defres{e24/jev/tau2/wrong_write/airline}{5.8}
\defres{e24/jev/tau2/wrong_write/pooled}{5.2}
\defres{e24/jev/tau2/wrong_write/retail}{5.1}
\defres{e24/jev/unseen/acceptable}{65.3}
\defres{e24/jev/unseen/acceptable/hi}{69.4}
\defres{e24/jev/unseen/acceptable/lo}{61.0}
\defres{e24/jev/unseen/after_off_plan}{66.8}
\defres{e24/jev/unseen/lenient}{58.5}
\defres{e24/jev/unseen/logged}{49.0}
\defres{e24/jev/unseen/on_plan}{43.6}
\defres{e24/jev/unseen/strict}{48.3}
\defres{e24/jev/unseen/tt/clean}{62.9}
\defres{e24/jev/unseen/tt/cool}{64.4}
\defres{e24/jev/unseen/tt/heat}{61.1}
\defres{e24/jev/unseen/tt/look}{36.8}
\defres{e24/jev/unseen/tt/pick2}{89.2}
\defres{e24/jev/unseen/tt/place}{77.5}
\defres{e24/kendall/acceptable/across}{1.00}
\defres{e24/kendall/acceptable/across/n}{3}
\defres{e24/kendall/acceptable/within/e11}{0.08}
\defres{e24/kendall/acceptable/within/e11/n}{12}
\defres{e24/kendall/acceptable/within/jev}{0.07}
\defres{e24/kendall/acceptable/within/jev/n}{6}
\defres{e24/kendall/acceptable/within/pooled}{0.49}
\defres{e24/kendall/acceptable/within/pooled/n}{18}
\defres{e24/kendall/alf_tau2}{-0.43}
\defres{e24/kendall/alf_tau2/n}{8}
\defres{e24/kendall/strict/across}{0.33}
\defres{e24/kendall/strict/across/n}{3}
\defres{e24/kendall/strict/within/e11}{-0.38}
\defres{e24/kendall/strict/within/e11/n}{12}
\defres{e24/kendall/strict/within/jev}{0.07}
\defres{e24/kendall/strict/within/jev/n}{6}
\defres{e24/kendall/strict/within/pooled}{0.31}
\defres{e24/kendall/strict/within/pooled/n}{18}
\defres{e24/live/e11/seen/cascade}{95.0}
\defres{e24/live/e11/seen/replace}{95.7}
\defres{e24/live/e11/unseen/cascade}{89.6}
\defres{e24/live/e11/unseen/replace}{88.1}
\defres{e24/live/flash/seen}{90.7}
\defres{e24/live/flash/unseen}{88.8}
\defres{e24/live/jev/seen/cascade}{91.4}
\defres{e24/live/jev/seen/replace}{27.1}
\defres{e24/oaidec/errors}{0}
\defres{e24/oaidec/mean_conf}{55.1}
\defres{e24/oaidec/pooled/acceptable}{68.2}
\defres{e24/oaidec/pooled/acceptable/hi}{71.1}
\defres{e24/oaidec/pooled/acceptable/lo}{65.2}
\defres{e24/oaidec/pooled/after_off_plan}{71.7}
\defres{e24/oaidec/pooled/lenient}{60.0}
\defres{e24/oaidec/pooled/logged}{48.4}
\defres{e24/oaidec/pooled/on_plan}{41.4}
\defres{e24/oaidec/pooled/strict}{48.1}
\defres{e24/oaidec/pooled/tt/clean}{62.0}
\defres{e24/oaidec/pooled/tt/cool}{60.0}
\defres{e24/oaidec/pooled/tt/heat}{60.2}
\defres{e24/oaidec/pooled/tt/look}{54.1}
\defres{e24/oaidec/pooled/tt/pick2}{85.3}
\defres{e24/oaidec/pooled/tt/place}{81.3}
\defres{e24/oaidec/seen/acceptable}{72.0}
\defres{e24/oaidec/seen/acceptable/hi}{75.9}
\defres{e24/oaidec/seen/acceptable/lo}{67.6}
\defres{e24/oaidec/seen/after_off_plan}{75.8}
\defres{e24/oaidec/seen/lenient}{62.9}
\defres{e24/oaidec/seen/logged}{50.4}
\defres{e24/oaidec/seen/on_plan}{45.7}
\defres{e24/oaidec/seen/strict}{49.7}
\defres{e24/oaidec/seen/tt/clean}{65.7}
\defres{e24/oaidec/seen/tt/cool}{58.4}
\defres{e24/oaidec/seen/tt/heat}{63.8}
\defres{e24/oaidec/seen/tt/look}{60.0}
\defres{e24/oaidec/seen/tt/pick2}{85.7}
\defres{e24/oaidec/seen/tt/place}{85.3}
\defres{e24/oaidec/seen_to_unseen}{-7.8}
\defres{e24/oaidec/tau2/args/airline}{87.3}
\defres{e24/oaidec/tau2/args/pooled}{90.2}
\defres{e24/oaidec/tau2/args/retail}{91.1}
\defres{e24/oaidec/tau2/call/airline}{24.8}
\defres{e24/oaidec/tau2/call/pooled}{34.8}
\defres{e24/oaidec/tau2/call/retail}{37.9}
\defres{e24/oaidec/tau2/tool/airline}{31.5}
\defres{e24/oaidec/tau2/tool/airline/hi}{44.2}
\defres{e24/oaidec/tau2/tool/airline/lo}{19.9}
\defres{e24/oaidec/tau2/tool/pooled}{37.7}
\defres{e24/oaidec/tau2/tool/pooled/hi}{44.9}
\defres{e24/oaidec/tau2/tool/pooled/lo}{30.4}
\defres{e24/oaidec/tau2/tool/retail}{39.6}
\defres{e24/oaidec/tau2/tool/retail/hi}{48.6}
\defres{e24/oaidec/tau2/tool/retail/lo}{31.7}
\defres{e24/oaidec/tau2/wrong_write/airline}{3.1}
\defres{e24/oaidec/tau2/wrong_write/pooled}{3.3}
\defres{e24/oaidec/tau2/wrong_write/retail}{3.4}
\defres{e24/oaidec/unseen/acceptable}{64.2}
\defres{e24/oaidec/unseen/acceptable/hi}{68.3}
\defres{e24/oaidec/unseen/acceptable/lo}{59.8}
\defres{e24/oaidec/unseen/after_off_plan}{67.7}
\defres{e24/oaidec/unseen/lenient}{56.9}
\defres{e24/oaidec/unseen/logged}{46.2}
\defres{e24/oaidec/unseen/on_plan}{36.9}
\defres{e24/oaidec/unseen/strict}{46.4}
\defres{e24/oaidec/unseen/tt/clean}{58.8}
\defres{e24/oaidec/unseen/tt/cool}{62.0}
\defres{e24/oaidec/unseen/tt/heat}{57.8}
\defres{e24/oaidec/unseen/tt/look}{49.8}
\defres{e24/oaidec/unseen/tt/pick2}{84.8}
\defres{e24/oaidec/unseen/tt/place}{75.5}
\defres{e24/qwen4b/errors}{0}
\defres{e24/qwen4b/mean_conf}{96.4}
\defres{e24/qwen4b/pooled/acceptable}{61.1}
\defres{e24/qwen4b/pooled/acceptable/hi}{63.8}
\defres{e24/qwen4b/pooled/acceptable/lo}{58.3}
\defres{e24/qwen4b/pooled/after_off_plan}{64.5}
\defres{e24/qwen4b/pooled/lenient}{53.8}
\defres{e24/qwen4b/pooled/logged}{41.9}
\defres{e24/qwen4b/pooled/on_plan}{37.1}
\defres{e24/qwen4b/pooled/strict}{42.5}
\defres{e24/qwen4b/pooled/tt/clean}{54.3}
\defres{e24/qwen4b/pooled/tt/cool}{50.1}
\defres{e24/qwen4b/pooled/tt/heat}{55.8}
\defres{e24/qwen4b/pooled/tt/look}{40.8}
\defres{e24/qwen4b/pooled/tt/pick2}{80.1}
\defres{e24/qwen4b/pooled/tt/place}{77.1}
\defres{e24/qwen4b/seen/acceptable}{64.7}
\defres{e24/qwen4b/seen/acceptable/hi}{68.2}
\defres{e24/qwen4b/seen/acceptable/lo}{60.7}
\defres{e24/qwen4b/seen/after_off_plan}{70.0}
\defres{e24/qwen4b/seen/lenient}{57.4}
\defres{e24/qwen4b/seen/logged}{45.0}
\defres{e24/qwen4b/seen/on_plan}{40.4}
\defres{e24/qwen4b/seen/strict}{45.8}
\defres{e24/qwen4b/seen/tt/clean}{59.6}
\defres{e24/qwen4b/seen/tt/cool}{50.6}
\defres{e24/qwen4b/seen/tt/heat}{58.9}
\defres{e24/qwen4b/seen/tt/look}{45.4}
\defres{e24/qwen4b/seen/tt/pick2}{79.2}
\defres{e24/qwen4b/seen/tt/place}{78.5}
\defres{e24/qwen4b/seen_to_unseen}{-7.4}
\defres{e24/qwen4b/tau2/args/airline}{85.6}
\defres{e24/qwen4b/tau2/args/pooled}{86.7}
\defres{e24/qwen4b/tau2/args/retail}{87.1}
\defres{e24/qwen4b/tau2/call/airline}{30.2}
\defres{e24/qwen4b/tau2/call/pooled}{48.1}
\defres{e24/qwen4b/tau2/call/retail}{53.7}
\defres{e24/qwen4b/tau2/tool/airline}{40.4}
\defres{e24/qwen4b/tau2/tool/airline/hi}{59.3}
\defres{e24/qwen4b/tau2/tool/airline/lo}{22.5}
\defres{e24/qwen4b/tau2/tool/pooled}{59.2}
\defres{e24/qwen4b/tau2/tool/pooled/hi}{68.1}
\defres{e24/qwen4b/tau2/tool/pooled/lo}{49.9}
\defres{e24/qwen4b/tau2/tool/retail}{65.1}
\defres{e24/qwen4b/tau2/tool/retail/hi}{75.1}
\defres{e24/qwen4b/tau2/tool/retail/lo}{55.5}
\defres{e24/qwen4b/tau2/wrong_write/airline}{7.7}
\defres{e24/qwen4b/tau2/wrong_write/pooled}{9.0}
\defres{e24/qwen4b/tau2/wrong_write/retail}{9.4}
\defres{e24/qwen4b/unseen/acceptable}{57.3}
\defres{e24/qwen4b/unseen/acceptable/hi}{61.4}
\defres{e24/qwen4b/unseen/acceptable/lo}{53.0}
\defres{e24/qwen4b/unseen/after_off_plan}{59.1}
\defres{e24/qwen4b/unseen/lenient}{50.1}
\defres{e24/qwen4b/unseen/logged}{38.6}
\defres{e24/qwen4b/unseen/on_plan}{33.5}
\defres{e24/qwen4b/unseen/strict}{39.0}
\defres{e24/qwen4b/unseen/tt/clean}{49.6}
\defres{e24/qwen4b/unseen/tt/cool}{49.6}
\defres{e24/qwen4b/unseen/tt/heat}{53.6}
\defres{e24/qwen4b/unseen/tt/look}{37.6}
\defres{e24/qwen4b/unseen/tt/pick2}{81.5}
\defres{e24/qwen4b/unseen/tt/place}{75.1}
\defres{e24/reading/lead_over_offshelf}{+20.0}
\defres{e24/reading/lead_over_transfer}{+28.1}
\defres{e24/reading/spread}{44.0}
\defres{e24/sl27b/errors}{0}
\defres{e24/sl27b/mean_conf}{66.2}
\defres{e24/sl27b/pooled/acceptable}{70.7}
\defres{e24/sl27b/pooled/acceptable/hi}{73.3}
\defres{e24/sl27b/pooled/acceptable/lo}{68.0}
\defres{e24/sl27b/pooled/after_off_plan}{74.8}
\defres{e24/sl27b/pooled/lenient}{65.4}
\defres{e24/sl27b/pooled/logged}{54.3}
\defres{e24/sl27b/pooled/on_plan}{37.1}
\defres{e24/sl27b/pooled/strict}{55.2}
\defres{e24/sl27b/pooled/tt/clean}{63.7}
\defres{e24/sl27b/pooled/tt/cool}{67.3}
\defres{e24/sl27b/pooled/tt/heat}{56.5}
\defres{e24/sl27b/pooled/tt/look}{72.1}
\defres{e24/sl27b/pooled/tt/pick2}{85.9}
\defres{e24/sl27b/pooled/tt/place}{78.2}
\defres{e24/sl27b/seen/acceptable}{73.1}
\defres{e24/sl27b/seen/acceptable/hi}{76.3}
\defres{e24/sl27b/seen/acceptable/lo}{69.6}
\defres{e24/sl27b/seen/after_off_plan}{77.0}
\defres{e24/sl27b/seen/lenient}{67.2}
\defres{e24/sl27b/seen/logged}{55.4}
\defres{e24/sl27b/seen/on_plan}{41.8}
\defres{e24/sl27b/seen/strict}{55.7}
\defres{e24/sl27b/seen/tt/clean}{69.2}
\defres{e24/sl27b/seen/tt/cool}{67.3}
\defres{e24/sl27b/seen/tt/heat}{54.4}
\defres{e24/sl27b/seen/tt/look}{68.1}
\defres{e24/sl27b/seen/tt/pick2}{87.4}
\defres{e24/sl27b/seen/tt/place}{80.7}
\defres{e24/sl27b/seen_to_unseen}{-4.8}
\defres{e24/sl27b/tau2/args/airline}{88.9}
\defres{e24/sl27b/tau2/args/pooled}{88.8}
\defres{e24/sl27b/tau2/args/retail}{88.8}
\defres{e24/sl27b/tau2/call/airline}{40.9}
\defres{e24/sl27b/tau2/call/pooled}{48.9}
\defres{e24/sl27b/tau2/call/retail}{51.4}
\defres{e24/sl27b/tau2/tool/airline}{43.5}
\defres{e24/sl27b/tau2/tool/airline/hi}{60.2}
\defres{e24/sl27b/tau2/tool/airline/lo}{27.1}
\defres{e24/sl27b/tau2/tool/pooled}{51.6}
\defres{e24/sl27b/tau2/tool/pooled/hi}{59.3}
\defres{e24/sl27b/tau2/tool/pooled/lo}{43.8}
\defres{e24/sl27b/tau2/tool/retail}{54.2}
\defres{e24/sl27b/tau2/tool/retail/hi}{62.6}
\defres{e24/sl27b/tau2/tool/retail/lo}{45.5}
\defres{e24/sl27b/tau2/wrong_write/airline}{7.5}
\defres{e24/sl27b/tau2/wrong_write/pooled}{5.4}
\defres{e24/sl27b/tau2/wrong_write/retail}{4.7}
\defres{e24/sl27b/unseen/acceptable}{68.2}
\defres{e24/sl27b/unseen/acceptable/hi}{72.0}
\defres{e24/sl27b/unseen/acceptable/lo}{64.1}
\defres{e24/sl27b/unseen/after_off_plan}{72.7}
\defres{e24/sl27b/unseen/lenient}{63.6}
\defres{e24/sl27b/unseen/logged}{53.1}
\defres{e24/sl27b/unseen/on_plan}{32.2}
\defres{e24/sl27b/unseen/strict}{54.7}
\defres{e24/sl27b/unseen/tt/clean}{59.0}
\defres{e24/sl27b/unseen/tt/cool}{67.2}
\defres{e24/sl27b/unseen/tt/heat}{58.0}
\defres{e24/sl27b/unseen/tt/look}{74.9}
\defres{e24/sl27b/unseen/tt/pick2}{83.8}
\defres{e24/sl27b/unseen/tt/place}{74.7}
\defres{e24/sl4b/errors}{0}
\defres{e24/sl4b/mean_conf}{60.8}
\defres{e24/sl4b/pooled/acceptable}{66.5}
\defres{e24/sl4b/pooled/acceptable/hi}{69.6}
\defres{e24/sl4b/pooled/acceptable/lo}{63.5}
\defres{e24/sl4b/pooled/after_off_plan}{69.1}
\defres{e24/sl4b/pooled/lenient}{59.3}
\defres{e24/sl4b/pooled/logged}{48.0}
\defres{e24/sl4b/pooled/on_plan}{45.1}
\defres{e24/sl4b/pooled/strict}{47.6}
\defres{e24/sl4b/pooled/tt/clean}{61.6}
\defres{e24/sl4b/pooled/tt/cool}{51.3}
\defres{e24/sl4b/pooled/tt/heat}{50.4}
\defres{e24/sl4b/pooled/tt/look}{52.7}
\defres{e24/sl4b/pooled/tt/pick2}{90.4}
\defres{e24/sl4b/pooled/tt/place}{84.4}
\defres{e24/sl4b/seen/acceptable}{69.2}
\defres{e24/sl4b/seen/acceptable/hi}{73.5}
\defres{e24/sl4b/seen/acceptable/lo}{64.4}
\defres{e24/sl4b/seen/after_off_plan}{72.0}
\defres{e24/sl4b/seen/lenient}{61.7}
\defres{e24/sl4b/seen/logged}{49.8}
\defres{e24/sl4b/seen/on_plan}{47.6}
\defres{e24/sl4b/seen/strict}{49.0}
\defres{e24/sl4b/seen/tt/clean}{65.4}
\defres{e24/sl4b/seen/tt/cool}{50.2}
\defres{e24/sl4b/seen/tt/heat}{45.2}
\defres{e24/sl4b/seen/tt/look}{57.3}
\defres{e24/sl4b/seen/tt/pick2}{91.2}
\defres{e24/sl4b/seen/tt/place}{86.2}
\defres{e24/sl4b/seen_to_unseen}{-5.6}
\defres{e24/sl4b/tau2/args/airline}{71.2}
\defres{e24/sl4b/tau2/args/pooled}{79.8}
\defres{e24/sl4b/tau2/args/retail}{82.5}
\defres{e24/sl4b/tau2/call/airline}{32.6}
\defres{e24/sl4b/tau2/call/pooled}{48.0}
\defres{e24/sl4b/tau2/call/retail}{52.8}
\defres{e24/sl4b/tau2/tool/airline}{41.7}
\defres{e24/sl4b/tau2/tool/airline/hi}{58.1}
\defres{e24/sl4b/tau2/tool/airline/lo}{26.2}
\defres{e24/sl4b/tau2/tool/pooled}{59.2}
\defres{e24/sl4b/tau2/tool/pooled/hi}{67.3}
\defres{e24/sl4b/tau2/tool/pooled/lo}{50.9}
\defres{e24/sl4b/tau2/tool/retail}{64.7}
\defres{e24/sl4b/tau2/tool/retail/hi}{73.4}
\defres{e24/sl4b/tau2/tool/retail/lo}{55.6}
\defres{e24/sl4b/tau2/wrong_write/airline}{7.9}
\defres{e24/sl4b/tau2/wrong_write/pooled}{8.9}
\defres{e24/sl4b/tau2/wrong_write/retail}{9.2}
\defres{e24/sl4b/unseen/acceptable}{63.6}
\defres{e24/sl4b/unseen/acceptable/hi}{67.7}
\defres{e24/sl4b/unseen/acceptable/lo}{59.4}
\defres{e24/sl4b/unseen/after_off_plan}{66.3}
\defres{e24/sl4b/unseen/lenient}{56.8}
\defres{e24/sl4b/unseen/logged}{46.0}
\defres{e24/sl4b/unseen/on_plan}{42.5}
\defres{e24/sl4b/unseen/strict}{46.1}
\defres{e24/sl4b/unseen/tt/clean}{58.4}
\defres{e24/sl4b/unseen/tt/cool}{52.6}
\defres{e24/sl4b/unseen/tt/heat}{54.1}
\defres{e24/sl4b/unseen/tt/look}{49.4}
\defres{e24/sl4b/unseen/tt/pick2}{89.3}
\defres{e24/sl4b/unseen/tt/place}{81.8}
\defres{e24/sl9b/errors}{0}
\defres{e24/sl9b/mean_conf}{65.9}
\defres{e24/sl9b/pooled/acceptable}{72.8}
\defres{e24/sl9b/pooled/acceptable/hi}{75.5}
\defres{e24/sl9b/pooled/acceptable/lo}{70.1}
\defres{e24/sl9b/pooled/after_off_plan}{74.0}
\defres{e24/sl9b/pooled/lenient}{65.6}
\defres{e24/sl9b/pooled/logged}{54.2}
\defres{e24/sl9b/pooled/on_plan}{54.4}
\defres{e24/sl9b/pooled/strict}{55.0}
\defres{e24/sl9b/pooled/tt/clean}{70.2}
\defres{e24/sl9b/pooled/tt/cool}{65.4}
\defres{e24/sl9b/pooled/tt/heat}{64.4}
\defres{e24/sl9b/pooled/tt/look}{56.6}
\defres{e24/sl9b/pooled/tt/pick2}{89.5}
\defres{e24/sl9b/pooled/tt/place}{83.6}
\defres{e24/sl9b/seen/acceptable}{74.9}
\defres{e24/sl9b/seen/acceptable/hi}{78.2}
\defres{e24/sl9b/seen/acceptable/lo}{71.0}
\defres{e24/sl9b/seen/after_off_plan}{76.7}
\defres{e24/sl9b/seen/lenient}{67.8}
\defres{e24/sl9b/seen/logged}{55.6}
\defres{e24/sl9b/seen/on_plan}{52.0}
\defres{e24/sl9b/seen/strict}{55.6}
\defres{e24/sl9b/seen/tt/clean}{72.5}
\defres{e24/sl9b/seen/tt/cool}{65.8}
\defres{e24/sl9b/seen/tt/heat}{65.9}
\defres{e24/sl9b/seen/tt/look}{55.6}
\defres{e24/sl9b/seen/tt/pick2}{89.2}
\defres{e24/sl9b/seen/tt/place}{84.5}
\defres{e24/sl9b/seen_to_unseen}{-4.2}
\defres{e24/sl9b/tau2/args/airline}{89.5}
\defres{e24/sl9b/tau2/args/pooled}{93.0}
\defres{e24/sl9b/tau2/args/retail}{94.1}
\defres{e24/sl9b/tau2/call/airline}{41.5}
\defres{e24/sl9b/tau2/call/pooled}{55.2}
\defres{e24/sl9b/tau2/call/retail}{59.5}
\defres{e24/sl9b/tau2/tool/airline}{44.6}
\defres{e24/sl9b/tau2/tool/airline/hi}{61.4}
\defres{e24/sl9b/tau2/tool/airline/lo}{28.6}
\defres{e24/sl9b/tau2/tool/pooled}{59.3}
\defres{e24/sl9b/tau2/tool/pooled/hi}{67.1}
\defres{e24/sl9b/tau2/tool/pooled/lo}{51.1}
\defres{e24/sl9b/tau2/tool/retail}{63.9}
\defres{e24/sl9b/tau2/tool/retail/hi}{72.7}
\defres{e24/sl9b/tau2/tool/retail/lo}{55.3}
\defres{e24/sl9b/tau2/wrong_write/airline}{6.1}
\defres{e24/sl9b/tau2/wrong_write/pooled}{7.6}
\defres{e24/sl9b/tau2/wrong_write/retail}{8.1}
\defres{e24/sl9b/unseen/acceptable}{70.6}
\defres{e24/sl9b/unseen/acceptable/hi}{74.5}
\defres{e24/sl9b/unseen/acceptable/lo}{66.6}
\defres{e24/sl9b/unseen/after_off_plan}{71.3}
\defres{e24/sl9b/unseen/lenient}{63.3}
\defres{e24/sl9b/unseen/logged}{52.7}
\defres{e24/sl9b/unseen/on_plan}{56.9}
\defres{e24/sl9b/unseen/strict}{54.3}
\defres{e24/sl9b/unseen/tt/clean}{68.1}
\defres{e24/sl9b/unseen/tt/cool}{64.9}
\defres{e24/sl9b/unseen/tt/heat}{63.3}
\defres{e24/sl9b/unseen/tt/look}{57.3}
\defres{e24/sl9b/unseen/tt/pick2}{89.9}
\defres{e24/sl9b/unseen/tt/place}{82.4}
\defres{e24/spend/jev}{0.44}
\defres{e24/spend/oaidec}{0.82}
\defres{e24/tau2/n/questions}{1{,}867}
\defres{e24/tau2/n/states}{422}
\defres{e24/tau2/n/tasks}{46}
\makeatother


==> generated/e25_harnesses.tex <==
\makeatletter
\providecommand{\res}[1]{\ifcsname jevres@#1\endcsname\csname jevres@#1\endcsname\else\tbd\fi}
\providecommand{\defres}[2]{\expandafter\def\csname jevres@#1\endcsname{#2}}
\defres{e25/margin}{3}
\defres{e25/tb/n_common}{89}
\defres{e25/tb/n_left_out}{0}
\defres{e25/tb/baseline/n}{89}
\defres{e25/tb/baseline/success}{42.7}
\defres{e25/tb/baseline/cost_usd}{0.5103}
\defres{e25/tb/baseline/wall_mean_s}{257}
\defres{e25/tb/baseline/wall_median_s}{121}
\defres{e25/tb/baseline/taken_share}{0.0}
\defres{e25/tb/baseline/requests_mean}{36.5}
\defres{e25/tb/baseline/steps_mean}{38.5}
\defres{e25/tb/jev_router/n}{89}
\defres{e25/tb/jev_router/success}{50.6}
\defres{e25/tb/jev_router/cost_usd}{0.4611}
\defres{e25/tb/jev_router/wall_mean_s}{260}
\defres{e25/tb/jev_router/wall_median_s}{120}
\defres{e25/tb/jev_router/taken_share}{12.4}
\defres{e25/tb/jev_router/requests_mean}{37.1}
\defres{e25/tb/jev_router/steps_mean}{38.2}
\defres{e25/tb/jev_router/jev_answer_share}{88.7}
\defres{e25/tb/jev_router/route_rule_share}{11.1}
\defres{e25/tb/jev_router/route_error_share}{0.2}
\defres{e25/tb/jev_router/route_cheap_share}{12.5}
\defres{e25/tb/jev_router/jev_cost_usd}{0.00252}
\defres{e25/tb/jev_router/jev_s_per_task}{6.2}
\defres{e25/tb/jev_router/delta}{$+$7.9}
\defres{e25/tb/jev_router/delta_lo}{$-$1.1}
\defres{e25/tb/jev_router/delta_hi}{$+$16.9}
\defres{e25/tb/jev_router/saving}{9.6}
\defres{e25/tb/jev_router/saving_lo}{-13.6}
\defres{e25/tb/jev_router/saving_hi}{27.5}
\defres{e25/tb/jev_router/time_saving}{-1.0}
\defres{e25/tb/jev_router/cost_change}{$-$9.6}
\defres{e25/tb/jev_router/time_change}{$+$1.0}
\defres{e25/tb/jev_router/time_more}{1.0}
\defres{e25/tb/jev_router/time_saving_lo}{-19.6}
\defres{e25/tb/jev_router/time_saving_hi}{15.3}
\defres{e25/tb/jev_router/median_time_saving}{0.6}
\defres{e25/tb/jev_router/cheaper_share}{55}
\defres{e25/tb/jev_router/faster_share}{49}
\defres{e25/tb/jev_router/wins}{12}
\defres{e25/tb/jev_router/losses}{5}
\defres{e25/tb/jev_router/ni_p}{0.012}
\defres{e25/tb/jev_router/ni}{yes}
\defres{e25/tb/jev_router/lo}{$-$1.3}
\defres{e25/tb/jev_router/hi}{$+$17.6}
\defres{e25/tb/jev_router/cc/n}{83}
\defres{e25/tb/jev_router/cc/delta}{$+$8.4}
\defres{e25/tb/jev_router/cc/saving}{10.5}
\defres{e25/tb/jev_router/cc/time_saving}{-4.6}
\defres{e25/tb/jev_router/cc/ni_p}{0.013}
\defres{e25/tb/jev_router/cc/ni}{yes}
\defres{e25/tb/always_cheap/n}{89}
\defres{e25/tb/always_cheap/success}{36.0}
\defres{e25/tb/always_cheap/cost_usd}{0.1484}
\defres{e25/tb/always_cheap/wall_mean_s}{336}
\defres{e25/tb/always_cheap/wall_median_s}{150}
\defres{e25/tb/always_cheap/taken_share}{100.0}
\defres{e25/tb/always_cheap/requests_mean}{49.8}
\defres{e25/tb/always_cheap/steps_mean}{50.6}
\defres{e25/tb/always_cheap/delta}{$-$6.7}
\defres{e25/tb/always_cheap/delta_lo}{$-$16.9}
\defres{e25/tb/always_cheap/delta_hi}{$+$3.4}
\defres{e25/tb/always_cheap/saving}{70.9}
\defres{e25/tb/always_cheap/saving_lo}{61.8}
\defres{e25/tb/always_cheap/saving_hi}{78.0}
\defres{e25/tb/always_cheap/time_saving}{-30.5}
\defres{e25/tb/always_cheap/cost_change}{$-$70.9}
\defres{e25/tb/always_cheap/time_change}{$+$30.5}
\defres{e25/tb/always_cheap/time_more}{30.5}
\defres{e25/tb/always_cheap/time_saving_lo}{-60.4}
\defres{e25/tb/always_cheap/time_saving_hi}{-6.2}
\defres{e25/tb/always_cheap/median_time_saving}{-24.7}
\defres{e25/tb/always_cheap/cheaper_share}{80}
\defres{e25/tb/always_cheap/faster_share}{36}
\defres{e25/tb/always_cheap/wins}{9}
\defres{e25/tb/always_cheap/losses}{15}
\defres{e25/tb/always_cheap/ni_p}{0.761}
\defres{e25/tb/always_cheap/ni}{no}
\defres{e25/tb/always_cheap/lo}{$-$17.8}
\defres{e25/tb/always_cheap/hi}{$+$4.2}
\defres{e25/tb/always_cheap/cc/n}{84}
\defres{e25/tb/always_cheap/cc/delta}{$-$8.3}
\defres{e25/tb/always_cheap/cc/saving}{71.2}
\defres{e25/tb/always_cheap/cc/time_saving}{-26.6}
\defres{e25/tb/always_cheap/cc/ni_p}{0.831}
\defres{e25/tb/always_cheap/cc/ni}{no}
\defres{e25/tb/baseline_on_router_tasks/n}{89}
\defres{e25/tb/baseline_on_router_tasks/success}{42.7}
\defres{e25/tb/baseline_on_router_tasks/cost_usd}{0.5103}
\defres{e25/tb/baseline_on_router_tasks/wall_mean_s}{257}
\defres{e25/tb/baseline_on_router_tasks/wall_median_s}{121}
\defres{e25/tb/baseline_on_router_tasks/taken_share}{0.0}
\defres{e25/tb/baseline_on_router_tasks/requests_mean}{36.5}
\defres{e25/tb/baseline_on_router_tasks/steps_mean}{38.5}
\defres{e25/tb/jev_router_defect/n}{74}
\defres{e25/tb/jev_router_defect/success}{18.9}
\defres{e25/tb/jev_router_defect/signature_errors}{51}
\defres{e25/swe/n_common}{100}
\defres{e25/swe/n_left_out}{0}
\defres{e25/swe/baseline/n}{100}
\defres{e25/swe/baseline/success}{63.0}
\defres{e25/swe/baseline/cost_usd}{0.2605}
\defres{e25/swe/baseline/wall_mean_s}{110}
\defres{e25/swe/baseline/wall_median_s}{98}
\defres{e25/swe/baseline/taken_share}{0.0}
\defres{e25/swe/baseline/steps_mean}{29.3}
\defres{e25/swe/jev_router/n}{100}
\defres{e25/swe/jev_router/success}{57.0}
\defres{e25/swe/jev_router/cost_usd}{0.2403}
\defres{e25/swe/jev_router/wall_mean_s}{124}
\defres{e25/swe/jev_router/wall_median_s}{106}
\defres{e25/swe/jev_router/taken_share}{23.2}
\defres{e25/swe/jev_router/requests_mean}{33.4}
\defres{e25/swe/jev_router/steps_mean}{33.4}
\defres{e25/swe/jev_router/jev_answer_share}{100.0}
\defres{e25/swe/jev_router/route_rule_share}{0.0}
\defres{e25/swe/jev_router/route_error_share}{0.0}
\defres{e25/swe/jev_router/route_cheap_share}{23.2}
\defres{e25/swe/jev_router/jev_cost_usd}{0.00309}
\defres{e25/swe/jev_router/jev_s_per_task}{7.5}
\defres{e25/swe/jev_router/delta}{$-$6.0}
\defres{e25/swe/jev_router/delta_lo}{$-$12.0}
\defres{e25/swe/jev_router/delta_hi}{$+$0.0}
\defres{e25/swe/jev_router/saving}{7.7}
\defres{e25/swe/jev_router/saving_lo}{-1.9}
\defres{e25/swe/jev_router/saving_hi}{16.3}
\defres{e25/swe/jev_router/time_saving}{-12.7}
\defres{e25/swe/jev_router/cost_change}{$-$7.7}
\defres{e25/swe/jev_router/time_change}{$+$12.7}
\defres{e25/swe/jev_router/time_more}{12.7}
\defres{e25/swe/jev_router/time_saving_lo}{-27.1}
\defres{e25/swe/jev_router/time_saving_hi}{-0.1}
\defres{e25/swe/jev_router/median_time_saving}{-8.6}
\defres{e25/swe/jev_router/cheaper_share}{59}
\defres{e25/swe/jev_router/faster_share}{34}
\defres{e25/swe/jev_router/wins}{2}
\defres{e25/swe/jev_router/losses}{8}
\defres{e25/swe/jev_router/ni_p}{0.848}
\defres{e25/swe/jev_router/ni}{no}
\defres{e25/swe/jev_router/lo}{$-$13.4}
\defres{e25/swe/jev_router/hi}{$+$0.2}
\defres{e25/swe/jev_router/cc/n}{100}
\defres{e25/swe/jev_router/cc/delta}{$-$6.0}
\defres{e25/swe/jev_router/cc/saving}{7.7}
\defres{e25/swe/jev_router/cc/time_saving}{-12.7}
\defres{e25/swe/jev_router/cc/ni_p}{0.848}
\defres{e25/swe/jev_router/cc/ni}{no}
\defres{e25/swe/always_cheap/n}{100}
\defres{e25/swe/always_cheap/success}{28.0}
\defres{e25/swe/always_cheap/cost_usd}{0.0813}
\defres{e25/swe/always_cheap/wall_mean_s}{102}
\defres{e25/swe/always_cheap/wall_median_s}{98}
\defres{e25/swe/always_cheap/taken_share}{100.0}
\defres{e25/swe/always_cheap/steps_mean}{44.2}
\defres{e25/swe/always_cheap/delta}{$-$35.0}
\defres{e25/swe/always_cheap/delta_lo}{$-$45.0}
\defres{e25/swe/always_cheap/delta_hi}{$-$25.0}
\defres{e25/swe/always_cheap/saving}{68.8}
\defres{e25/swe/always_cheap/saving_lo}{64.3}
\defres{e25/swe/always_cheap/saving_hi}{72.6}
\defres{e25/swe/always_cheap/time_saving}{7.5}
\defres{e25/swe/always_cheap/cost_change}{$-$68.8}
\defres{e25/swe/always_cheap/time_change}{$-$7.5}
\defres{e25/swe/always_cheap/time_more}{-7.5}
\defres{e25/swe/always_cheap/time_saving_lo}{-3.0}
\defres{e25/swe/always_cheap/time_saving_hi}{17.6}
\defres{e25/swe/always_cheap/median_time_saving}{-0.5}
\defres{e25/swe/always_cheap/cheaper_share}{95}
\defres{e25/swe/always_cheap/faster_share}{49}
\defres{e25/swe/always_cheap/wins}{2}
\defres{e25/swe/always_cheap/losses}{37}
\defres{e25/swe/always_cheap/ni_p}{1.000}
\defres{e25/swe/always_cheap/ni}{no}
\defres{e25/swe/always_cheap/lo}{$-$45.3}
\defres{e25/swe/always_cheap/hi}{$-$24.9}
\defres{e25/swe/always_cheap/cc/n}{100}
\defres{e25/swe/always_cheap/cc/delta}{$-$35.0}
\defres{e25/swe/always_cheap/cc/saving}{68.8}
\defres{e25/swe/always_cheap/cc/time_saving}{7.5}
\defres{e25/swe/always_cheap/cc/ni_p}{1.000}
\defres{e25/swe/always_cheap/cc/ni}{no}
\defres{e25/swe/baseline_on_router_tasks/n}{100}
\defres{e25/swe/baseline_on_router_tasks/success}{63.0}
\defres{e25/swe/baseline_on_router_tasks/cost_usd}{0.2605}
\defres{e25/swe/baseline_on_router_tasks/wall_mean_s}{110}
\defres{e25/swe/baseline_on_router_tasks/wall_median_s}{98}
\defres{e25/swe/baseline_on_router_tasks/taken_share}{0.0}
\defres{e25/swe/baseline_on_router_tasks/steps_mean}{29.3}
\makeatother


==> generated/e27_small_shift.tex <==
\makeatletter
\providecommand{\res}[1]{\ifcsname jevres@#1\endcsname\csname jevres@#1\endcsname\else\tbd\fi}
\providecommand{\defres}[2]{\expandafter\def\csname jevres@#1\endcsname{#2}}
\defres{e27/data/augstates}{2{,}552}
\defres{e27/data/s_records}{14{,}787}
\defres{e27/data/sp_records}{31{,}689}
\defres{e27/data/states}{5{,}168}
\defres{e27/lat/4b/c1/p50}{155}
\defres{e27/lat/4b/c1/p90}{183}
\defres{e27/lat/4b/c1/step}{213}
\defres{e27/lat/4b/c4/p50}{318}
\defres{e27/lat/4b/c4/p90}{526}
\defres{e27/lat/4b/c4/step}{593}
\defres{e27/lat/4b/mem}{22.6}
\defres{e27/lat/sel/c1/p50}{69}
\defres{e27/lat/sel/c1/p90}{72}
\defres{e27/lat/sel/c1/speedup}{2.2}
\defres{e27/lat/sel/c1/step}{131}
\defres{e27/lat/sel/c4/p50}{120}
\defres{e27/lat/sel/c4/p90}{199}
\defres{e27/lat/sel/c4/speedup}{2.6}
\defres{e27/lat/sel/c4/step}{201}
\defres{e27/lat/sel/mem}{2.6}
\defres{e27/ref/e12/c}{99.1}
\defres{e27/ref/e12/l1}{85.1}
\defres{e27/ref/e12/l2}{94.9}
\defres{e27/ref/e12/l2mustask}{67.4}
\defres{e27/ref/e12/l3}{91.5}
\defres{e27/ref/e12/l3genkinds}{98.6}
\defres{e27/ref/e12/l3genkinds_n}{140}
\defres{e27/ref/e12/l3in}{100.0}
\defres{e27/ref/e12/l3newkinds}{75.0}
\defres{e27/ref/e12/l3newkinds_n}{60}
\defres{e27/ref/e12/surfcost}{+3.7}
\defres{e27/ref/e12/surfcost_abs}{3.7}
\defres{e27/ref/e14a/c}{99.2}
\defres{e27/ref/e14a/l1}{67.8}
\defres{e27/ref/e14a/l2}{73.2}
\defres{e27/ref/e14a/l2mustask}{77.2}
\defres{e27/ref/e14a/l3}{17.5}
\defres{e27/ref/e14a/l3genkinds}{25.0}
\defres{e27/ref/e14a/l3genkinds_n}{140}
\defres{e27/ref/e14a/l3in}{100.0}
\defres{e27/ref/e14a/l3newkinds}{0.0}
\defres{e27/ref/e14a/l3newkinds_n}{60}
\defres{e27/ref/e14a/surfcost}{+21.9}
\defres{e27/ref/e14a/surfcost_abs}{21.9}
\defres{e27/ref/llm_only/l3}{100.0}
\defres{e27/ref/llm_only/l3genkinds}{100.0}
\defres{e27/ref/llm_only/l3genkinds_n}{140}
\defres{e27/ref/llm_only/l3newkinds}{100.0}
\defres{e27/ref/llm_only/l3newkinds_n}{60}
\defres{e27/ref/rl/c}{99.2}
\defres{e27/ref/rl/l1}{78.8}
\defres{e27/ref/rl/l2}{98.6}
\defres{e27/ref/rl/l2mustask}{90.8}
\defres{e27/ref/rl/l3}{96.0}
\defres{e27/ref/rl/l3genkinds}{96.4}
\defres{e27/ref/rl/l3genkinds_n}{140}
\defres{e27/ref/rl/l3in}{100.0}
\defres{e27/ref/rl/l3newkinds}{95.0}
\defres{e27/ref/rl/l3newkinds_n}{60}
\defres{e27/ref/rl/surfcost}{+1.1}
\defres{e27/ref/rl/surfcost_abs}{1.1}
\defres{e27/s/l1/acc}{67.7}
\defres{e27/s/l1/lat}{215}
\defres{e27/s/l1/tool}{77.2}
\defres{e27/s/l1/usdk}{0.092}
\defres{e27/s/l1/vs_e14a}{$-$0.0}
\defres{e27/s/l2/all}{93.7}
\defres{e27/s/l2/mustask}{77.2}
\defres{e27/s/l2/mustask_vs_e12}{+9.9}
\defres{e27/s/l2/newkind}{88.4}
\defres{e27/s/l2/offplan}{99.2}
\defres{e27/s/l2/renamed}{93.2}
\defres{e27/s/l2/surfcost}{+1.6}
\defres{e27/s/l2/surfcost_abs}{1.6}
\defres{e27/s/l2/vs_e14a}{+20.4}
\defres{e27/s/l2in/all}{98.8}
\defres{e27/s/l2in/offplan}{92.2}
\defres{e27/s/l2in/vs_e14a_lo}{$-$0.6}
\defres{e27/s/l3/genkinds}{82.9}
\defres{e27/s/l3/genkinds_n}{140}
\defres{e27/s/l3/kind/clarify_ask_after_lookup}{100.0}
\defres{e27/s/l3/kind/clarify_ask_twice}{0.0}
\defres{e27/s/l3/kind/clarify_method}{100.0}
\defres{e27/s/l3/kind/clarify_name}{100.0}
\defres{e27/s/l3/kind/clarify_order}{100.0}
\defres{e27/s/l3/kind/clarify_speed}{0.0}
\defres{e27/s/l3/kind/multi}{93.3}
\defres{e27/s/l3/kind/notify}{40.0}
\defres{e27/s/l3/n}{200}
\defres{e27/s/l3/newkinds}{46.7}
\defres{e27/s/l3/newkinds_n}{60}
\defres{e27/s/l3/own}{90.1}
\defres{e27/s/l3/success}{72.0}
\defres{e27/s/l3/usd_k}{14.87}
\defres{e27/s/l3/vs_e12}{$-$19.5}
\defres{e27/s/l3/vs_e12_lo}{$-$27.1}
\defres{e27/s/l3/wall}{5.9}
\defres{e27/s/train/mem}{7.3}
\defres{e27/s/train/minutes}{40}
\defres{e27/s/train/records}{14{,}787}
\defres{e27/sel/cal/argscov}{77.8}
\defres{e27/sel/cal/toolcov}{50.0}
\defres{e27/sel/final_in/argcov}{89.0}
\defres{e27/sel/final_in/argstaken}{959}
\defres{e27/sel/final_in/argswrong}{0}
\defres{e27/sel/final_in/delta}{$-$0.5}
\defres{e27/sel/final_in/errored}{0}
\defres{e27/sel/final_in/handed}{51.5}
\defres{e27/sel/final_in/losses}{2}
\defres{e27/sel/final_in/mustask_taken}{6}
\defres{e27/sel/final_in/mustask_wrong}{0}
\defres{e27/sel/final_in/n}{200}
\defres{e27/sel/final_in/ni}{not shown}
\defres{e27/sel/final_in/ni_p}{0.059}
\defres{e27/sel/final_in/ref}{99.5}
\defres{e27/sel/final_in/refusd_k}{43.12}
\defres{e27/sel/final_in/refwall}{13.6}
\defres{e27/sel/final_in/refwall_median}{8.9}
\defres{e27/sel/final_in/saving}{30.3}
\defres{e27/sel/final_in/saving_api}{37.1}
\defres{e27/sel/final_in/success}{99.0}
\defres{e27/sel/final_in/toolcov}{48.5}
\defres{e27/sel/final_in/tooltaken}{727}
\defres{e27/sel/final_in/toolwrong}{0}
\defres{e27/sel/final_in/usd_k}{30.05}
\defres{e27/sel/final_in/wall}{6.5}
\defres{e27/sel/final_in/wall_median}{4.8}
\defres{e27/sel/final_in/wins}{1}
\defres{e27/sel/final_shift/argcov}{71.3}
\defres{e27/sel/final_shift/argstaken}{271}
\defres{e27/sel/final_shift/argswrong}{0}
\defres{e27/sel/final_shift/delta}{+0.0}
\defres{e27/sel/final_shift/errored}{0}
\defres{e27/sel/final_shift/handed}{72.3}
\defres{e27/sel/final_shift/losses}{0}
\defres{e27/sel/final_shift/mustask_taken}{0}
\defres{e27/sel/final_shift/mustask_wrong}{0}
\defres{e27/sel/final_shift/n}{200}
\defres{e27/sel/final_shift/ni}{non-inferior}
\defres{e27/sel/final_shift/ni_p}{0.002}
\defres{e27/sel/final_shift/ref}{100.0}
\defres{e27/sel/final_shift/refusd_k}{53.52}
\defres{e27/sel/final_shift/refwall}{8.0}
\defres{e27/sel/final_shift/refwall_median}{6.6}
\defres{e27/sel/final_shift/saving}{6.0}
\defres{e27/sel/final_shift/saving_api}{12.9}
\defres{e27/sel/final_shift/success}{100.0}
\defres{e27/sel/final_shift/toolcov}{27.7}
\defres{e27/sel/final_shift/tooltaken}{365}
\defres{e27/sel/final_shift/toolwrong}{0}
\defres{e27/sel/final_shift/usd_k}{50.30}
\defres{e27/sel/final_shift/wall}{8.1}
\defres{e27/sel/final_shift/wall_median}{6.1}
\defres{e27/sel/final_shift/wins}{0}
\defres{e27/sel/l1/acc}{77.2}
\defres{e27/sel/l1/lat}{215}
\defres{e27/sel/l1/tool}{83.2}
\defres{e27/sel/l1/usdk}{0.091}
\defres{e27/sel/l1/vs_e14a}{+9.5}
\defres{e27/sel/l2/all}{96.3}
\defres{e27/sel/l2/mustask}{93.9}
\defres{e27/sel/l2/mustask_vs_e12}{+26.5}
\defres{e27/sel/l2/newkind}{88.1}
\defres{e27/sel/l2/offplan}{100.0}
\defres{e27/sel/l2/renamed}{95.5}
\defres{e27/sel/l2/surfcost}{$-$1.7}
\defres{e27/sel/l2/surfcost_abs}{1.7}
\defres{e27/sel/l2/vs_e14a}{+23.1}
\defres{e27/sel/l2in/all}{99.2}
\defres{e27/sel/l2in/offplan}{94.6}
\defres{e27/sel/l2in/vs_e14a_lo}{$-$0.1}
\defres{e27/sel/l3/genkinds}{100.0}
\defres{e27/sel/l3/genkinds_n}{140}
\defres{e27/sel/l3/kind/clarify_ask_after_lookup}{100.0}
\defres{e27/sel/l3/kind/clarify_ask_twice}{0.0}
\defres{e27/sel/l3/kind/clarify_method}{100.0}
\defres{e27/sel/l3/kind/clarify_name}{100.0}
\defres{e27/sel/l3/kind/clarify_order}{100.0}
\defres{e27/sel/l3/kind/clarify_speed}{100.0}
\defres{e27/sel/l3/kind/multi}{100.0}
\defres{e27/sel/l3/kind/notify}{0.0}
\defres{e27/sel/l3/n}{200}
\defres{e27/sel/l3/newkinds}{33.3}
\defres{e27/sel/l3/newkinds_n}{60}
\defres{e27/sel/l3/own}{95.0}
\defres{e27/sel/l3/success}{80.0}
\defres{e27/sel/l3/usd_k}{16.05}
\defres{e27/sel/l3/vs_e12}{$-$11.5}
\defres{e27/sel/l3/vs_e12_lo}{$-$18.6}
\defres{e27/sel/l3/wall}{6.6}
\defres{e27/sel/l3in/n}{200}
\defres{e27/sel/l3in/success}{100.0}
\defres{e27/sel/reading/holdsundershift}{no}
\defres{e27/sel/reading/keepsc}{yes}
\defres{e27/sel/reading/keepsindomain}{no}
\defres{e27/sel/reading/l2holds}{yes}
\defres{e27/sel/reading/l3holds}{no}
\defres{e27/sel/train/mem}{7.2}
\defres{e27/sel/train/minutes}{48}
\defres{e27/sel/train/records}{31{,}689}
\defres{e27/sp/l1/acc}{77.2}
\defres{e27/sp/l1/lat}{215}
\defres{e27/sp/l1/tool}{83.2}
\defres{e27/sp/l1/usdk}{0.091}
\defres{e27/sp/l1/vs_e14a}{+9.5}
\defres{e27/sp/l2/all}{96.3}
\defres{e27/sp/l2/mustask}{93.9}
\defres{e27/sp/l2/mustask_vs_e12}{+26.5}
\defres{e27/sp/l2/newkind}{88.1}
\defres{e27/sp/l2/offplan}{100.0}
\defres{e27/sp/l2/renamed}{95.5}
\defres{e27/sp/l2/surfcost}{$-$1.7}
\defres{e27/sp/l2/surfcost_abs}{1.7}
\defres{e27/sp/l2/vs_e14a}{+23.1}
\defres{e27/sp/l2in/all}{99.2}
\defres{e27/sp/l2in/offplan}{94.6}
\defres{e27/sp/l2in/vs_e14a_lo}{$-$0.1}
\defres{e27/sp/l3/genkinds}{100.0}
\defres{e27/sp/l3/genkinds_n}{140}
\defres{e27/sp/l3/kind/clarify_ask_after_lookup}{100.0}
\defres{e27/sp/l3/kind/clarify_ask_twice}{0.0}
\defres{e27/sp/l3/kind/clarify_method}{100.0}
\defres{e27/sp/l3/kind/clarify_name}{100.0}
\defres{e27/sp/l3/kind/clarify_order}{100.0}
\defres{e27/sp/l3/kind/clarify_speed}{100.0}
\defres{e27/sp/l3/kind/multi}{100.0}
\defres{e27/sp/l3/kind/notify}{0.0}
\defres{e27/sp/l3/n}{200}
\defres{e27/sp/l3/newkinds}{33.3}
\defres{e27/sp/l3/newkinds_n}{60}
\defres{e27/sp/l3/own}{95.0}
\defres{e27/sp/l3/success}{80.0}
\defres{e27/sp/l3/usd_k}{16.05}
\defres{e27/sp/l3/vs_e12}{$-$11.5}
\defres{e27/sp/l3/vs_e12_lo}{$-$18.6}
\defres{e27/sp/l3/wall}{6.6}
\defres{e27/sp/train/mem}{7.2}
\defres{e27/sp/train/minutes}{48}
\defres{e27/sp/train/records}{31{,}689}
\defres{e27/spend/gemini}{24.07}
\defres{e27/vocab/augwords}{193}
\defres{e27/vocab/overlap}{0}
\defres{e9/e27s/acc}{67.7}
\defres{e9/e27s/acc/args}{70.2}
\defres{e9/e27s/acc/toolchoice}{77.2}
\defres{e9/e27s/acc/w2c}{51.1}
\defres{e9/e27s/costvsjev}{5.6}
\defres{e9/e27s/front}{no}
\defres{e9/e27s/gapfrozen}{-11.0}
\defres{e9/e27s/gapfrozenabs}{11.0}
\defres{e9/e27s/gapjev}{-18.7}
\defres{e9/e27s/gapjevabs}{18.7}
\defres{e9/e27s/gapsl4b}{-15.4}
\defres{e9/e27s/gapsl4babs}{15.4}
\defres{e9/e27s/lat}{215}
\defres{e9/e27s/lg}{-4.0369}
\defres{e9/e27s/usdk}{0.092}
\defres{e9/e27sel/acc}{77.2}
\defres{e9/e27sel/acc/args}{89.1}
\defres{e9/e27sel/acc/toolchoice}{83.2}
\defres{e9/e27sel/acc/w2c}{45.3}
\defres{e9/e27sel/costvsjev}{5.6}
\defres{e9/e27sel/front}{no}
\defres{e9/e27sel/gapfrozen}{-1.5}
\defres{e9/e27sel/gapfrozenabs}{1.5}
\defres{e9/e27sel/gapjev}{-9.1}
\defres{e9/e27sel/gapjevabs}{9.1}
\defres{e9/e27sel/gapsl4b}{-5.9}
\defres{e9/e27sel/gapsl4babs}{5.9}
\defres{e9/e27sel/lat}{215}
\defres{e9/e27sel/lg}{-4.0410}
\defres{e9/e27sel/usdk}{0.091}
\defres{e9/e27sp/acc}{77.2}
\defres{e9/e27sp/acc/args}{89.1}
\defres{e9/e27sp/acc/toolchoice}{83.2}
\defres{e9/e27sp/acc/w2c}{45.3}
\defres{e9/e27sp/costvsjev}{5.6}
\defres{e9/e27sp/front}{no}
\defres{e9/e27sp/gapfrozen}{-1.5}
\defres{e9/e27sp/gapfrozenabs}{1.5}
\defres{e9/e27sp/gapjev}{-9.1}
\defres{e9/e27sp/gapjevabs}{9.1}
\defres{e9/e27sp/gapsl4b}{-5.9}
\defres{e9/e27sp/gapsl4babs}{5.9}
\defres{e9/e27sp/lat}{215}
\defres{e9/e27sp/lg}{-4.0410}
\defres{e9/e27sp/usdk}{0.091}
\makeatother


==> generated/e28_sl08b.tex <==
\makeatletter
\providecommand{\res}[1]{\ifcsname jevres@#1\endcsname\csname jevres@#1\endcsname\else\tbd\fi}
\providecommand{\defres}[2]{\expandafter\def\csname jevres@#1\endcsname{#2}}
\defres{e28/base/l1/acc}{70.0}
\defres{e28/base/l1/lat}{17}
\defres{e28/base/l1/tool}{88.2}
\defres{e28/base/l1/usdk}{0.013}
\defres{e28/base/l2/all}{51.7}
\defres{e28/base/l2/genkind}{47.3}
\defres{e28/base/l2/mustask}{27.2}
\defres{e28/base/l2/newkind}{61.8}
\defres{e28/base/l2/offplan}{66.0}
\defres{e28/base/l2/renamed}{46.2}
\defres{e28/base/l2/surfcost}{+5.7}
\defres{e28/base/l2/vs_e12_all}{$-$43.2}
\defres{e28/base/l2/vs_e12_mustask}{$-$40.1}
\defres{e28/base/l2/vs_e12c_all}{$-$46.8}
\defres{e28/base/l2/vs_e12c_mustask}{$-$72.8}
\defres{e28/base/l2/vs_e27sp_all}{$-$44.7}
\defres{e28/base/l2/vs_e27sp_mustask}{$-$66.7}
\defres{e28/base/l2/vs_sl4b_all}{$-$34.9}
\defres{e28/base/l2/vs_sl4b_mustask}{$-$9.4}
\defres{e28/base/l2in/all}{48.3}
\defres{e28/base/l2in/offplan}{31.5}
\defres{e28/base/l3/errored}{0}
\defres{e28/base/l3/genkinds}{4.3}
\defres{e28/base/l3/genkinds_n}{140}
\defres{e28/base/l3/n}{200}
\defres{e28/base/l3/newkinds}{33.3}
\defres{e28/base/l3/newkinds_n}{60}
\defres{e28/base/l3/own}{36.6}
\defres{e28/base/l3/success}{13.0}
\defres{e28/base/l3/usd_k}{25.68}
\defres{e28/base/l3/vs_e12}{$-$78.5}
\defres{e28/base/l3/vs_e12_hi}{$-$69.4}
\defres{e28/base/l3/vs_e12_lo}{$-$84.9}
\defres{e28/base/l3/vs_e12c}{$-$85.0}
\defres{e28/base/l3/vs_e12c_hi}{$-$78.2}
\defres{e28/base/l3/vs_e12c_lo}{$-$89.5}
\defres{e28/base/l3/vs_e14a}{$-$4.5}
\defres{e28/base/l3/vs_e14a_hi}{+3.2}
\defres{e28/base/l3/vs_e14a_lo}{$-$12.1}
\defres{e28/base/l3/vs_e27sp}{$-$67.0}
\defres{e28/base/l3/vs_e27sp_hi}{$-$59.6}
\defres{e28/base/l3/vs_e27sp_lo}{$-$72.8}
\defres{e28/base/l3/vs_llm_only}{$-$87.0}
\defres{e28/base/l3/vs_llm_only_hi}{$-$81.3}
\defres{e28/base/l3/vs_llm_only_lo}{$-$91.0}
\defres{e28/base/l3/vs_sl4b}{$-$36.0}
\defres{e28/base/l3/vs_sl4b_hi}{$-$26.6}
\defres{e28/base/l3/vs_sl4b_lo}{$-$44.5}
\defres{e28/base/l3/wall}{10.6}
\defres{e28/base/l3in/n}{200}
\defres{e28/base/l3in/success}{17.5}
\defres{e28/cal/argscov}{47.1}
\defres{e28/cal/toolcov}{40.0}
\defres{e28/data/agentrows}{7{,}000}
\defres{e28/data/augrows}{3{,}463}
\defres{e28/data/augstates}{2{,}014}
\defres{e28/data/publicrows}{7{,}000}
\defres{e28/data/rows}{14{,}000}
\defres{e28/data/states}{4{,}063}
\defres{e28/final_in/argcov}{66.9}
\defres{e28/final_in/argswrong}{0}
\defres{e28/final_in/delta}{+0.5}
\defres{e28/final_in/errored}{0}
\defres{e28/final_in/losses}{0}
\defres{e28/final_in/n}{200}
\defres{e28/final_in/ni}{non-inferior}
\defres{e28/final_in/ni_p}{0.002}
\defres{e28/final_in/ref}{99.5}
\defres{e28/final_in/refs1s}{0.0}
\defres{e28/final_in/refs2call}{1.55}
\defres{e28/final_in/refs2s}{11.7}
\defres{e28/final_in/refusd_k}{43.12}
\defres{e28/final_in/refwall}{13.6}
\defres{e28/final_in/s1s}{2.4}
\defres{e28/final_in/s2call}{1.93}
\defres{e28/final_in/s2s}{12.4}
\defres{e28/final_in/saving}{$-$6.0}
\defres{e28/final_in/saving_api}{9.6}
\defres{e28/final_in/success}{100.0}
\defres{e28/final_in/toolcov}{35.9}
\defres{e28/final_in/toolwrong}{0}
\defres{e28/final_in/usd_k}{45.72}
\defres{e28/final_in/wall}{14.9}
\defres{e28/final_in/wins}{1}
\defres{e28/final_shift/argcov}{31.9}
\defres{e28/final_shift/argswrong}{2}
\defres{e28/final_shift/delta}{$-$2.0}
\defres{e28/final_shift/errored}{0}
\defres{e28/final_shift/losses}{4}
\defres{e28/final_shift/n}{200}
\defres{e28/final_shift/ni}{not shown}
\defres{e28/final_shift/ni_p}{0.306}
\defres{e28/final_shift/ref}{100.0}
\defres{e28/final_shift/refs1s}{0.0}
\defres{e28/final_shift/refs2call}{1.20}
\defres{e28/final_shift/refs2s}{7.9}
\defres{e28/final_shift/refusd_k}{53.52}
\defres{e28/final_shift/refwall}{8.0}
\defres{e28/final_shift/s1s}{2.2}
\defres{e28/final_shift/s2call}{3.51}
\defres{e28/final_shift/s2s}{20.9}
\defres{e28/final_shift/saving}{13.2}
\defres{e28/final_shift/saving_api}{33.2}
\defres{e28/final_shift/success}{98.0}
\defres{e28/final_shift/toolcov}{61.7}
\defres{e28/final_shift/toolwrong}{6}
\defres{e28/final_shift/usd_k}{46.48}
\defres{e28/final_shift/wall}{23.8}
\defres{e28/final_shift/wins}{0}
\defres{e28/host/hours}{4.37}
\defres{e28/l1/acc}{80.5}
\defres{e28/l1/acc/args}{87.2}
\defres{e28/l1/acc/toolchoice}{87.1}
\defres{e28/l1/acc/w2c}{58.3}
\defres{e28/l1/acc_vendor}{80.8}
\defres{e28/l1/lat}{18}
\defres{e28/l1/lat_own}{456}
\defres{e28/l1/tool}{87.1}
\defres{e28/l1/usdk}{0.010}
\defres{e28/l1/usdk_basis}{vendor}
\defres{e28/l1/usdk_own}{0.179}
\defres{e28/l1/vs_base}{+10.5}
\defres{e28/l1/vs_base_hi}{+11.9}
\defres{e28/l1/vs_base_lo}{+9.1}
\defres{e28/l1/vs_e12}{$-$4.6}
\defres{e28/l1/vs_e12_hi}{$-$3.5}
\defres{e28/l1/vs_e12_lo}{$-$5.8}
\defres{e28/l1/vs_e12c}{$-$5.0}
\defres{e28/l1/vs_e12c_hi}{$-$4.0}
\defres{e28/l1/vs_e12c_lo}{$-$6.1}
\defres{e28/l1/vs_e27sp}{+3.2}
\defres{e28/l1/vs_e27sp_hi}{+4.3}
\defres{e28/l1/vs_e27sp_lo}{+2.1}
\defres{e28/l2/all}{95.6}
\defres{e28/l2/genkind}{97.8}
\defres{e28/l2/mustask}{93.5}
\defres{e28/l2/newkind}{90.5}
\defres{e28/l2/offplan}{97.4}
\defres{e28/l2/renamed}{94.8}
\defres{e28/l2/surfcost}{+1.2}
\defres{e28/l2/vs_e12_all}{+0.8}
\defres{e28/l2/vs_e12_mustask}{+26.1}
\defres{e28/l2/vs_e12c_all}{$-$2.8}
\defres{e28/l2/vs_e12c_mustask}{$-$6.5}
\defres{e28/l2/vs_e27sp_all}{$-$0.7}
\defres{e28/l2/vs_e27sp_mustask}{$-$0.4}
\defres{e28/l2/vs_sl08b_all}{+43.9}
\defres{e28/l2/vs_sl08b_mustask}{+66.2}
\defres{e28/l2/vs_sl4b_all}{+9.1}
\defres{e28/l2/vs_sl4b_mustask}{+56.8}
\defres{e28/l2in/all}{98.5}
\defres{e28/l2in/offplan}{90.0}
\defres{e28/l2in/vs_base}{+50.1}
\defres{e28/l2in/vs_base_hi}{+52.6}
\defres{e28/l2in/vs_base_lo}{+47.2}
\defres{e28/l2in/vs_e12c}{$-$1.2}
\defres{e28/l2in/vs_e12c_hi}{$-$0.5}
\defres{e28/l2in/vs_e12c_lo}{$-$2.0}
\defres{e28/l2in/vs_e27sp}{$-$0.7}
\defres{e28/l2in/vs_e27sp_hi}{$-$0.4}
\defres{e28/l2in/vs_e27sp_lo}{$-$1.2}
\defres{e28/l2in/vs_rl}{$-$0.7}
\defres{e28/l2in/vs_rl_hi}{$-$0.3}
\defres{e28/l2in/vs_rl_lo}{$-$1.2}
\defres{e28/l3/errored}{0}
\defres{e28/l3/genkinds}{96.4}
\defres{e28/l3/genkinds_n}{140}
\defres{e28/l3/n}{200}
\defres{e28/l3/newkinds}{48.3}
\defres{e28/l3/newkinds_n}{60}
\defres{e28/l3/own}{89.8}
\defres{e28/l3/success}{82.0}
\defres{e28/l3/usd_k}{16.90}
\defres{e28/l3/vs_e12}{$-$9.5}
\defres{e28/l3/vs_e12_hi}{$-$5.0}
\defres{e28/l3/vs_e12_lo}{$-$14.5}
\defres{e28/l3/vs_e12c}{$-$16.0}
\defres{e28/l3/vs_e12c_hi}{$-$10.8}
\defres{e28/l3/vs_e12c_lo}{$-$21.8}
\defres{e28/l3/vs_e14a}{+64.5}
\defres{e28/l3/vs_e14a_hi}{+70.4}
\defres{e28/l3/vs_e14a_lo}{+57.0}
\defres{e28/l3/vs_e27sp}{+2.0}
\defres{e28/l3/vs_e27sp_hi}{+9.3}
\defres{e28/l3/vs_e27sp_lo}{$-$5.3}
\defres{e28/l3/vs_llm_only}{$-$18.0}
\defres{e28/l3/vs_llm_only_hi}{$-$12.9}
\defres{e28/l3/vs_llm_only_lo}{$-$23.9}
\defres{e28/l3/vs_sl4b}{+33.0}
\defres{e28/l3/vs_sl4b_hi}{+39.9}
\defres{e28/l3/vs_sl4b_lo}{+25.6}
\defres{e28/l3/wall}{8.1}
\defres{e28/l3in/n}{200}
\defres{e28/l3in/own}{100.0}
\defres{e28/l3in/success}{100.0}
\defres{e28/reading/holdsundershift}{no}
\defres{e28/reading/keepsc}{no}
\defres{e28/reading/keepsindomain}{no}
\defres{e28/reading/l2holds}{yes}
\defres{e28/reading/l3holds}{no}
\defres{e28/ref/e12/l1/acc}{85.1}
\defres{e28/ref/e12/l1/lat}{344}
\defres{e28/ref/e12/l1/tool}{89.3}
\defres{e28/ref/e12/l1/usdk}{0.140}
\defres{e28/ref/e12/l2/all}{94.9}
\defres{e28/ref/e12/l2/genkind}{95.3}
\defres{e28/ref/e12/l2/mustask}{67.4}
\defres{e28/ref/e12/l2/newkind}{93.7}
\defres{e28/ref/e12/l2/offplan}{98.4}
\defres{e28/ref/e12/l2/renamed}{93.8}
\defres{e28/ref/e12/l2/surfcost}{+3.7}
\defres{e28/ref/e12/l2in/all}{99.1}
\defres{e28/ref/e12/l3/n}{200}
\defres{e28/ref/e12/l3/success}{91.5}
\defres{e28/ref/e12/l3in/success}{100.0}
\defres{e28/ref/e12c/l1/acc}{85.5}
\defres{e28/ref/e12c/l1/lat}{713}
\defres{e28/ref/e12c/l1/tool}{89.5}
\defres{e28/ref/e12c/l1/usdk}{0.295}
\defres{e28/ref/e12c/l2/all}{98.5}
\defres{e28/ref/e12c/l2/genkind}{100.0}
\defres{e28/ref/e12c/l2/mustask}{100.0}
\defres{e28/ref/e12c/l2/newkind}{94.9}
\defres{e28/ref/e12c/l2/offplan}{100.0}
\defres{e28/ref/e12c/l2/renamed}{98.0}
\defres{e28/ref/e12c/l2/surfcost}{+1.4}
\defres{e28/ref/e12c/l2in/all}{99.6}
\defres{e28/ref/e12c/l2in/offplan}{96.1}
\defres{e28/ref/e12c/l3/n}{200}
\defres{e28/ref/e12c/l3/success}{98.0}
\defres{e28/ref/e12c/l3in/success}{100.0}
\defres{e28/ref/e14a/l2/all}{73.2}
\defres{e28/ref/e14a/l2/genkind}{76.4}
\defres{e28/ref/e14a/l2/mustask}{77.2}
\defres{e28/ref/e14a/l2/newkind}{65.9}
\defres{e28/ref/e14a/l2/offplan}{72.4}
\defres{e28/ref/e14a/l2/renamed}{68.1}
\defres{e28/ref/e14a/l2/surfcost}{+21.9}
\defres{e28/ref/e14a/l3/n}{200}
\defres{e28/ref/e14a/l3/success}{17.5}
\defres{e28/ref/e27sp/final_in/ni_p}{0.059}
\defres{e28/ref/e27sp/final_in/ref}{99.5}
\defres{e28/ref/e27sp/final_in/saving}{30.3}
\defres{e28/ref/e27sp/final_in/success}{99.0}
\defres{e28/ref/e27sp/final_in/toolcov}{48.5}
\defres{e28/ref/e27sp/final_in/wall}{6.5}
\defres{e28/ref/e27sp/final_shift/ni_p}{0.002}
\defres{e28/ref/e27sp/final_shift/ref}{100.0}
\defres{e28/ref/e27sp/final_shift/saving}{6.0}
\defres{e28/ref/e27sp/final_shift/success}{100.0}
\defres{e28/ref/e27sp/final_shift/toolcov}{27.7}
\defres{e28/ref/e27sp/final_shift/wall}{8.1}
\defres{e28/ref/e27sp/l1/acc}{77.2}
\defres{e28/ref/e27sp/l1/lat}{215}
\defres{e28/ref/e27sp/l1/tool}{83.2}
\defres{e28/ref/e27sp/l1/usdk}{0.091}
\defres{e28/ref/e27sp/l2/all}{96.3}
\defres{e28/ref/e27sp/l2/genkind}{99.8}
\defres{e28/ref/e27sp/l2/mustask}{93.9}
\defres{e28/ref/e27sp/l2/newkind}{88.1}
\defres{e28/ref/e27sp/l2/offplan}{100.0}
\defres{e28/ref/e27sp/l2/renamed}{95.5}
\defres{e28/ref/e27sp/l2/surfcost}{$-$1.7}
\defres{e28/ref/e27sp/l2in/all}{99.2}
\defres{e28/ref/e27sp/l2in/offplan}{94.6}
\defres{e28/ref/e27sp/l3/n}{200}
\defres{e28/ref/e27sp/l3/success}{80.0}
\defres{e28/ref/e27sp/l3in/n}{200}
\defres{e28/ref/e27sp/l3in/success}{100.0}
\defres{e28/ref/jev/l1/acc}{86.4}
\defres{e28/ref/jev/l1/lat}{206}
\defres{e28/ref/jev/l1/usdk}{0.016}
\defres{e28/ref/llm_only/l3/n}{200}
\defres{e28/ref/llm_only/l3/success}{100.0}
\defres{e28/ref/rl/l1/acc}{78.8}
\defres{e28/ref/rl/l1/lat}{268}
\defres{e28/ref/rl/l1/usdk}{0.093}
\defres{e28/ref/rl/l2/all}{98.6}
\defres{e28/ref/rl/l2/genkind}{98.3}
\defres{e28/ref/rl/l2/mustask}{90.8}
\defres{e28/ref/rl/l2/newkind}{99.3}
\defres{e28/ref/rl/l2/offplan}{99.2}
\defres{e28/ref/rl/l2/renamed}{98.3}
\defres{e28/ref/rl/l2/surfcost}{+1.1}
\defres{e28/ref/rl/l2in/all}{99.2}
\defres{e28/ref/rl/l2in/offplan}{94.7}
\defres{e28/ref/rl/l3/n}{200}
\defres{e28/ref/rl/l3/success}{96.0}
\defres{e28/ref/sl4b/l1/acc}{83.1}
\defres{e28/ref/sl4b/l1/lat}{111}
\defres{e28/ref/sl4b/l1/usdk}{0.052}
\defres{e28/ref/sl4b/l2/all}{86.5}
\defres{e28/ref/sl4b/l2/genkind}{86.9}
\defres{e28/ref/sl4b/l2/mustask}{36.7}
\defres{e28/ref/sl4b/l2/newkind}{85.6}
\defres{e28/ref/sl4b/l2/offplan}{87.8}
\defres{e28/ref/sl4b/l2/renamed}{84.1}
\defres{e28/ref/sl4b/l2/surfcost}{+1.6}
\defres{e28/ref/sl4b/l3/n}{200}
\defres{e28/ref/sl4b/l3/success}{49.0}
\defres{e28/spend/gemini}{26.65}
\defres{e28/train/epoch}{2}
\defres{e28/train/minutes}{28}
\defres{e28/train/setting}{nogc\_3072}
\defres{e28/vocab/augwords}{193}
\defres{e28/vocab/e21words}{1011}
\defres{e28/vocab/overlap}{0}
\defres{e9/e28/acc}{80.5}
\defres{e9/e28/acc/args}{87.2}
\defres{e9/e28/acc/toolchoice}{87.1}
\defres{e9/e28/acc/w2c}{58.3}
\defres{e9/e28/basis}{vendor}
\defres{e9/e28/lat}{18}
\defres{e9/e28/lat_own}{456}
\defres{e9/e28/lg}{-4.9970}
\defres{e9/e28/lg_own}{-3.7481}
\defres{e9/e28/usdk}{0.010}
\defres{e9/e28/usdk_own}{0.18}
\makeatother


==> generated/e29_port.tex <==
\makeatletter
\providecommand{\res}[1]{\ifcsname jevres@#1\endcsname\csname jevres@#1\endcsname\else\tbd\fi}
\providecommand{\defres}[2]{\expandafter\def\csname jevres@#1\endcsname{#2}}
\defres{e29/gate/mswe/agree_fast}{7.8}
\defres{e29/gate/mswe/agree_self}{15.1}
\defres{e29/gate/mswe/auroc}{0.70}
\defres{e29/gate/mswe/jevfast_agree_fast}{8.8}
\defres{e29/gate/mswe/jevfast_agree_self}{15.9}
\defres{e29/gate/mswe/jevfast_share}{72.8}
\defres{e29/gate/mswe/routed_agree_fast}{44.4}
\defres{e29/gate/mswe/routed_agree_self}{33.3}
\defres{e29/gate/mswe/same_tool_fast}{99.6}
\defres{e29/gate/mswe/same_tool_self}{99.0}
\defres{e29/gate/mswe/sim_share}{2.4}
\defres{e29/gate/mswe/steps}{735}
\defres{e29/gate/mswe/tasks}{20}
\defres{e29/gate/mswe/tau}{0.990}
\defres{e29/gate/tb/agree_fast}{36.9}
\defres{e29/gate/tb/agree_self}{60.4}
\defres{e29/gate/tb/auroc}{0.52}
\defres{e29/gate/tb/jevfast_agree_fast}{40.7}
\defres{e29/gate/tb/jevfast_agree_self}{65.0}
\defres{e29/gate/tb/jevfast_share}{65.8}
\defres{e29/gate/tb/routed_agree_fast}{--}
\defres{e29/gate/tb/routed_agree_self}{--}
\defres{e29/gate/tb/same_tool_fast}{77.0}
\defres{e29/gate/tb/same_tool_self}{96.3}
\defres{e29/gate/tb/sim_share}{0.0}
\defres{e29/gate/tb/steps}{187}
\defres{e29/gate/tb/tasks}{10}
\defres{e29/gate/tb/tau}{none}
\defres{e29/go/decision}{no-go}
\defres{e29/go/mswe/drop}{0}
\defres{e29/go/mswe/saving}{10.7}
\defres{e29/go/tb/saving}{0.0}
\defres{e29/leaks/checks}{9}
\defres{e29/leaks/max_files}{0}
\defres{e29/mswe/status}{not run (no-go)}
\defres{e29/pilot/mswe/cached}{91.3}
\defres{e29/pilot/mswe/cached_ref}{91.5}
\defres{e29/pilot/mswe/cc_delta}{0.0}
\defres{e29/pilot/mswe/cc_n}{30}
\defres{e29/pilot/mswe/cc_ni_p}{0.577}
\defres{e29/pilot/mswe/cost}{0.0459}
\defres{e29/pilot/mswe/cost_ref}{0.0514}
\defres{e29/pilot/mswe/decisions}{42.3}
\defres{e29/pilot/mswe/delta}{0.0}
\defres{e29/pilot/mswe/delta_hi}{+13.3}
\defres{e29/pilot/mswe/delta_lo}{-13.3}
\defres{e29/pilot/mswe/dm_cost}{0.0057}
\defres{e29/pilot/mswe/dm_latency}{8.1}
\defres{e29/pilot/mswe/fail_open}{0}
\defres{e29/pilot/mswe/fast_share}{0.7}
\defres{e29/pilot/mswe/losses}{2}
\defres{e29/pilot/mswe/median_time}{361}
\defres{e29/pilot/mswe/median_time_ref}{325}
\defres{e29/pilot/mswe/median_time_saving}{-11.2}
\defres{e29/pilot/mswe/n}{30}
\defres{e29/pilot/mswe/ni}{no}
\defres{e29/pilot/mswe/ni_p}{0.577}
\defres{e29/pilot/mswe/ref_success}{70.0}
\defres{e29/pilot/mswe/saving}{10.7}
\defres{e29/pilot/mswe/saving_hi}{42.2}
\defres{e29/pilot/mswe/saving_lo}{-62.9}
\defres{e29/pilot/mswe/segment_len}{1.5}
\defres{e29/pilot/mswe/segments_capped}{0.0}
\defres{e29/pilot/mswe/segments_per_task}{0.2}
\defres{e29/pilot/mswe/success}{70.0}
\defres{e29/pilot/mswe/time}{561}
\defres{e29/pilot/mswe/time_ref}{543}
\defres{e29/pilot/mswe/time_saving}{-3.3}
\defres{e29/pilot/mswe/waited}{1.06}
\defres{e29/pilot/mswe/wins}{2}
\defres{e29/pilot/tb/status}{the gate kept every step on the strong LLM}
\defres{e29/spend/cap}{300}
\defres{e29/spend/total}{13.38}
\defres{e29/swea/status}{not run (no-go)}
\defres{e29/tb/status}{not run (no-go)}
\makeatother


==> generated/e29b_route.tex <==
\makeatletter
\providecommand{\res}[1]{\ifcsname jevres@#1\endcsname\csname jevres@#1\endcsname\else\tbd\fi}
\providecommand{\defres}[2]{\expandafter\def\csname jevres@#1\endcsname{#2}}
\defres{e29b/gate/mswe/ans_edit_n}{90}
\defres{e29b/gate/mswe/ans_edit_ro}{44.4}
\defres{e29b/gate/mswe/ans_finish_n}{18}
\defres{e29b/gate/mswe/ans_finish_ro}{11.1}
\defres{e29b/gate/mswe/ans_inspect_n}{531}
\defres{e29b/gate/mswe/ans_inspect_ro}{53.7}
\defres{e29b/gate/mswe/ans_run_n}{70}
\defres{e29b/gate/mswe/ans_run_ro}{22.9}
\defres{e29b/gate/mswe/auroc}{0.70}
\defres{e29b/gate/mswe/base_rate}{48.4}
\defres{e29b/gate/mswe/eligible}{531}
\defres{e29b/gate/mswe/eligible_precision}{53.7}
\defres{e29b/gate/mswe/fast_ro_when_not}{25.5}
\defres{e29b/gate/mswe/fast_ro_when_ro}{70.5}
\defres{e29b/gate/mswe/guard_sim}{100.0}
\defres{e29b/gate/mswe/implied_share}{0.8}
\defres{e29b/gate/mswe/precision}{100.0}
\defres{e29b/gate/mswe/recall}{1.7}
\defres{e29b/gate/mswe/ro_cost_share}{41.9}
\defres{e29b/gate/mswe/routed}{6}
\defres{e29b/gate/mswe/routed_cost_share}{0.3}
\defres{e29b/gate/mswe/sim_saving}{0.1}
\defres{e29b/gate/mswe/steps}{709}
\defres{e29b/gate/mswe/tasks}{20}
\defres{e29b/gate/mswe/tau}{0.980}
\defres{e29b/gate/tb/ans_edit_n}{66}
\defres{e29b/gate/tb/ans_edit_ro}{25.8}
\defres{e29b/gate/tb/ans_finish_n}{2}
\defres{e29b/gate/tb/ans_finish_ro}{0.0}
\defres{e29b/gate/tb/ans_inspect_n}{98}
\defres{e29b/gate/tb/ans_inspect_ro}{25.5}
\defres{e29b/gate/tb/ans_run_n}{39}
\defres{e29b/gate/tb/ans_run_ro}{23.1}
\defres{e29b/gate/tb/auroc}{0.56}
\defres{e29b/gate/tb/base_rate}{24.9}
\defres{e29b/gate/tb/eligible}{98}
\defres{e29b/gate/tb/eligible_precision}{25.5}
\defres{e29b/gate/tb/fast_ro_when_not}{9.1}
\defres{e29b/gate/tb/fast_ro_when_ro}{60.8}
\defres{e29b/gate/tb/guard_sim}{75.0}
\defres{e29b/gate/tb/implied_share}{2.0}
\defres{e29b/gate/tb/precision}{100.0}
\defres{e29b/gate/tb/recall}{7.8}
\defres{e29b/gate/tb/ro_cost_share}{14.1}
\defres{e29b/gate/tb/routed}{4}
\defres{e29b/gate/tb/routed_cost_share}{0.6}
\defres{e29b/gate/tb/sim_saving}{0.5}
\defres{e29b/gate/tb/steps}{205}
\defres{e29b/gate/tb/tasks}{10}
\defres{e29b/gate/tb/tau}{0.920}
\defres{e29b/go/decision}{no-go}
\defres{e29b/go/mswe/drop}{0}
\defres{e29b/go/mswe/saving}{-21.1}
\defres{e29b/go/tb/drop}{2}
\defres{e29b/go/tb/saving}{15.5}
\defres{e29b/leaks/checks}{9}
\defres{e29b/leaks/max_files}{0}
\defres{e29b/mswe/status}{not run (no-go)}
\defres{e29b/pilot/mswe/cached}{91.1}
\defres{e29b/pilot/mswe/cached_ref}{91.5}
\defres{e29b/pilot/mswe/cc_delta}{0.0}
\defres{e29b/pilot/mswe/cc_n}{30}
\defres{e29b/pilot/mswe/cc_ni_p}{0.774}
\defres{e29b/pilot/mswe/cost}{0.0470}
\defres{e29b/pilot/mswe/cost_ref}{0.0388}
\defres{e29b/pilot/mswe/decisions}{41.5}
\defres{e29b/pilot/mswe/delta}{0.0}
\defres{e29b/pilot/mswe/delta_hi}{+10.0}
\defres{e29b/pilot/mswe/delta_lo}{-10.0}
\defres{e29b/pilot/mswe/dm_cost}{0.0055}
\defres{e29b/pilot/mswe/dm_latency}{7.8}
\defres{e29b/pilot/mswe/fail_open}{0}
\defres{e29b/pilot/mswe/fast_call_share}{1.2}
\defres{e29b/pilot/mswe/fast_share}{1.2}
\defres{e29b/pilot/mswe/guard_accept}{15}
\defres{e29b/pilot/mswe/guard_reject}{0}
\defres{e29b/pilot/mswe/guard_reject_cost}{0.0000}
\defres{e29b/pilot/mswe/guard_reject_share}{0.0}
\defres{e29b/pilot/mswe/losses}{1}
\defres{e29b/pilot/mswe/median_time}{312}
\defres{e29b/pilot/mswe/median_time_ref}{288}
\defres{e29b/pilot/mswe/median_time_saving}{-8.3}
\defres{e29b/pilot/mswe/n}{30}
\defres{e29b/pilot/mswe/ni}{no}
\defres{e29b/pilot/mswe/ni_p}{0.774}
\defres{e29b/pilot/mswe/ref_success}{66.7}
\defres{e29b/pilot/mswe/saving}{-21.1}
\defres{e29b/pilot/mswe/saving_hi}{16.5}
\defres{e29b/pilot/mswe/saving_lo}{-76.1}
\defres{e29b/pilot/mswe/segment_len}{1.1}
\defres{e29b/pilot/mswe/segments_capped}{0.0}
\defres{e29b/pilot/mswe/segments_per_task}{0.5}
\defres{e29b/pilot/mswe/steps}{41.5}
\defres{e29b/pilot/mswe/success}{66.7}
\defres{e29b/pilot/mswe/time}{497}
\defres{e29b/pilot/mswe/time_ref}{469}
\defres{e29b/pilot/mswe/time_saving}{-6.0}
\defres{e29b/pilot/mswe/waited}{1.24}
\defres{e29b/pilot/mswe/wins}{1}
\defres{e29b/pilot/tb/cached}{85.1}
\defres{e29b/pilot/tb/cached_ref}{81.8}
\defres{e29b/pilot/tb/cc_delta}{-7.1}
\defres{e29b/pilot/tb/cc_n}{28}
\defres{e29b/pilot/tb/cc_ni_p}{0.702}
\defres{e29b/pilot/tb/cost}{0.4668}
\defres{e29b/pilot/tb/cost_ref}{0.5524}
\defres{e29b/pilot/tb/decisions}{36.3}
\defres{e29b/pilot/tb/delta}{-7.1}
\defres{e29b/pilot/tb/delta_hi}{+10.7}
\defres{e29b/pilot/tb/delta_lo}{-25.0}
\defres{e29b/pilot/tb/dm_cost}{0.0033}
\defres{e29b/pilot/tb/dm_latency}{7.2}
\defres{e29b/pilot/tb/fail_open}{0}
\defres{e29b/pilot/tb/fast_call_share}{10.3}
\defres{e29b/pilot/tb/fast_share}{6.2}
\defres{e29b/pilot/tb/guard_accept}{63}
\defres{e29b/pilot/tb/guard_reject}{46}
\defres{e29b/pilot/tb/guard_reject_cost}{0.0051}
\defres{e29b/pilot/tb/guard_reject_share}{42.2}
\defres{e29b/pilot/tb/losses}{4}
\defres{e29b/pilot/tb/median_time}{126}
\defres{e29b/pilot/tb/median_time_ref}{166}
\defres{e29b/pilot/tb/median_time_saving}{24.0}
\defres{e29b/pilot/tb/n}{28}
\defres{e29b/pilot/tb/ni}{no}
\defres{e29b/pilot/tb/ni_p}{0.702}
\defres{e29b/pilot/tb/ref_success}{53.6}
\defres{e29b/pilot/tb/saving}{15.5}
\defres{e29b/pilot/tb/saving_hi}{34.9}
\defres{e29b/pilot/tb/saving_lo}{-2.4}
\defres{e29b/pilot/tb/segment_len}{2.0}
\defres{e29b/pilot/tb/segments_capped}{15.6}
\defres{e29b/pilot/tb/segments_per_task}{1.1}
\defres{e29b/pilot/tb/steps}{36.3}
\defres{e29b/pilot/tb/success}{46.4}
\defres{e29b/pilot/tb/time}{225}
\defres{e29b/pilot/tb/time_ref}{247}
\defres{e29b/pilot/tb/time_saving}{8.8}
\defres{e29b/pilot/tb/waited}{4.53}
\defres{e29b/pilot/tb/wins}{2}
\defres{e29b/spend/cap}{250}
\defres{e29b/spend/total}{38.59}
\defres{e29b/spend/with_e29}{51.97}
\defres{e29b/swea/status}{not run (no-go)}
\defres{e29b/tb/status}{not run (no-go)}
\makeatother


==> generated/e30_cost.tex <==
\makeatletter
\providecommand{\res}[1]{\ifcsname jevres@#1\endcsname\csname jevres@#1\endcsname\else\tbd\fi}
\providecommand{\defres}[2]{\expandafter\def\csname jevres@#1\endcsname{#2}}
\defres{e30/clefflash/ref}{81.4}
\defres{e30/decider/acc}{79.4}
\defres{e30/decider/agree}{99.0}
\defres{e30/decider/bf16/acc}{79.3}
\defres{e30/decider/bf16/agree}{99.8}
\defres{e30/decider/bf16/conc}{64}
\defres{e30/decider/bf16/dps}{29.0}
\defres{e30/decider/bf16/lat_p50}{53}
\defres{e30/decider/bf16/lat_p90}{96}
\defres{e30/decider/bf16/lg}{-5.1133}
\defres{e30/decider/bf16/usdk}{0.0077}
\defres{e30/decider/conc}{64}
\defres{e30/decider/dacc}{+0.1}
\defres{e30/decider/dps}{37.1}
\defres{e30/decider/engine}{vLLM}
\defres{e30/decider/flag}{none}
\defres{e30/decider/fp8/acc}{79.4}
\defres{e30/decider/fp8/agree}{99.0}
\defres{e30/decider/fp8/conc}{64}
\defres{e30/decider/fp8/dps}{37.1}
\defres{e30/decider/fp8/lat_p50}{39}
\defres{e30/decider/fp8/lat_p90}{66}
\defres{e30/decider/fp8/lg}{-5.2201}
\defres{e30/decider/fp8/usdk}{0.0060}
\defres{e30/decider/lat_p50}{39}
\defres{e30/decider/lat_p90}{66}
\defres{e30/decider/lg}{-5.2201}
\defres{e30/decider/prec}{FP8}
\defres{e30/decider/ref}{79.3}
\defres{e30/decider/usdk}{0.0060}
\defres{e30/decider/vse9}{9.0}
\defres{e30/e12/acc}{84.8}
\defres{e30/e12/agree}{98.6}
\defres{e30/e12/bf16/acc}{85.2}
\defres{e30/e12/bf16/agree}{99.6}
\defres{e30/e12/bf16/conc}{64}
\defres{e30/e12/bf16/dps}{37.8}
\defres{e30/e12/bf16/lat_p50}{45}
\defres{e30/e12/bf16/lat_p90}{73}
\defres{e30/e12/bf16/lg}{-5.2284}
\defres{e30/e12/bf16/usdk}{0.0059}
\defres{e30/e12/conc}{256}
\defres{e30/e12/dacc}{-0.3}
\defres{e30/e12/dps}{50.2}
\defres{e30/e12/engine}{vLLM}
\defres{e30/e12/flag}{none}
\defres{e30/e12/fp8/acc}{84.8}
\defres{e30/e12/fp8/agree}{98.6}
\defres{e30/e12/fp8/conc}{256}
\defres{e30/e12/fp8/dps}{50.2}
\defres{e30/e12/fp8/lat_p50}{31}
\defres{e30/e12/fp8/lat_p90}{52}
\defres{e30/e12/fp8/lg}{-5.3513}
\defres{e30/e12/fp8/usdk}{0.0045}
\defres{e30/e12/lat_p50}{31}
\defres{e30/e12/lat_p90}{52}
\defres{e30/e12/lg}{-5.3513}
\defres{e30/e12/prec}{FP8}
\defres{e30/e12/ref}{85.1}
\defres{e30/e12/usdk}{0.0045}
\defres{e30/e12/vse9}{31}
\defres{e30/e12c/acc}{85.5}
\defres{e30/e12c/agree}{98.7}
\defres{e30/e12c/bf16/acc}{85.5}
\defres{e30/e12c/bf16/agree}{99.9}
\defres{e30/e12c/bf16/conc}{64}
\defres{e30/e12c/bf16/dps}{23.4}
\defres{e30/e12c/bf16/lat_p50}{58}
\defres{e30/e12c/bf16/lat_p90}{99}
\defres{e30/e12c/bf16/lg}{-5.0193}
\defres{e30/e12c/bf16/usdk}{0.0096}
\defres{e30/e12c/conc}{64}
\defres{e30/e12c/dacc}{+0.0}
\defres{e30/e12c/dps}{30.3}
\defres{e30/e12c/engine}{vLLM}
\defres{e30/e12c/flag}{none}
\defres{e30/e12c/fp8/acc}{85.5}
\defres{e30/e12c/fp8/agree}{98.7}
\defres{e30/e12c/fp8/conc}{64}
\defres{e30/e12c/fp8/dps}{30.3}
\defres{e30/e12c/fp8/lat_p50}{45}
\defres{e30/e12c/fp8/lat_p90}{70}
\defres{e30/e12c/fp8/lg}{-5.1317}
\defres{e30/e12c/fp8/usdk}{0.0074}
\defres{e30/e12c/lat_p50}{45}
\defres{e30/e12c/lat_p90}{70}
\defres{e30/e12c/lg}{-5.1317}
\defres{e30/e12c/prec}{FP8}
\defres{e30/e12c/ref}{85.5}
\defres{e30/e12c/usdk}{0.0074}
\defres{e30/e12c/vse9}{39}
\defres{e30/e27sp/acc}{77.3}
\defres{e30/e27sp/agree}{99.8}
\defres{e30/e27sp/bf16/acc}{77.3}
\defres{e30/e27sp/bf16/agree}{99.8}
\defres{e30/e27sp/bf16/conc}{16}
\defres{e30/e27sp/bf16/dps}{26.7}
\defres{e30/e27sp/bf16/lat_p50}{60}
\defres{e30/e27sp/bf16/lat_p90}{63}
\defres{e30/e27sp/bf16/lg}{-5.0777}
\defres{e30/e27sp/bf16/usdk}{0.0084}
\defres{e30/e27sp/conc}{16}
\defres{e30/e27sp/dacc}{+0.1}
\defres{e30/e27sp/dps}{26.7}
\defres{e30/e27sp/engine}{serve\_jev (scoring head)}
\defres{e30/e27sp/flag}{none}
\defres{e30/e27sp/lat_p50}{60}
\defres{e30/e27sp/lat_p90}{63}
\defres{e30/e27sp/lg}{-5.0777}
\defres{e30/e27sp/prec}{BF16}
\defres{e30/e27sp/ref}{77.2}
\defres{e30/e27sp/usdk}{0.0084}
\defres{e30/e27sp/vse9}{11}
\defres{e30/e28/acc}{80.5}
\defres{e30/e28/agree}{98.3}
\defres{e30/e28/bf16/acc}{80.5}
\defres{e30/e28/bf16/agree}{99.9}
\defres{e30/e28/bf16/conc}{64}
\defres{e30/e28/bf16/dps}{114}
\defres{e30/e28/bf16/lat_p50}{31}
\defres{e30/e28/bf16/lat_p90}{34}
\defres{e30/e28/bf16/lg}{-5.7067}
\defres{e30/e28/bf16/usdk}{0.0020}
\defres{e30/e28/conc}{64}
\defres{e30/e28/dacc}{-0.0}
\defres{e30/e28/dps}{122}
\defres{e30/e28/engine}{vLLM}
\defres{e30/e28/flag}{none}
\defres{e30/e28/fp8/acc}{80.5}
\defres{e30/e28/fp8/agree}{98.3}
\defres{e30/e28/fp8/conc}{64}
\defres{e30/e28/fp8/dps}{122}
\defres{e30/e28/fp8/lat_p50}{27}
\defres{e30/e28/fp8/lat_p90}{30}
\defres{e30/e28/fp8/lg}{-5.7387}
\defres{e30/e28/fp8/usdk}{0.0018}
\defres{e30/e28/lat_p50}{27}
\defres{e30/e28/lat_p90}{30}
\defres{e30/e28/lg}{-5.7387}
\defres{e30/e28/prec}{FP8}
\defres{e30/e28/ref}{80.5}
\defres{e30/e28/usdk}{0.0018}
\defres{e30/e28/vse9}{5.5}
\defres{e30/front/first}{sl08b}
\defres{e30/front/n}{6}
\defres{e30/front/rest}{ours08,ours,jev,sl27b,flash}
\defres{e30/imajev/ref}{78.9}
\defres{e30/intern/acc}{73.5}
\defres{e30/intern/agree}{97.1}
\defres{e30/intern/bf16/acc}{73.4}
\defres{e30/intern/bf16/agree}{99.4}
\defres{e30/intern/bf16/conc}{64}
\defres{e30/intern/bf16/dps}{13.6}
\defres{e30/intern/bf16/lat_p50}{83}
\defres{e30/intern/bf16/lat_p90}{172}
\defres{e30/intern/bf16/lg}{-4.7842}
\defres{e30/intern/bf16/usdk}{0.016}
\defres{e30/intern/conc}{64}
\defres{e30/intern/dacc}{+0.1}
\defres{e30/intern/dps}{18.0}
\defres{e30/intern/engine}{vLLM}
\defres{e30/intern/flag}{none}
\defres{e30/intern/fp8/acc}{73.5}
\defres{e30/intern/fp8/agree}{97.1}
\defres{e30/intern/fp8/conc}{64}
\defres{e30/intern/fp8/dps}{18.0}
\defres{e30/intern/fp8/lat_p50}{61}
\defres{e30/intern/fp8/lat_p90}{125}
\defres{e30/intern/fp8/lg}{-4.9062}
\defres{e30/intern/fp8/usdk}{0.012}
\defres{e30/intern/lat_p50}{61}
\defres{e30/intern/lat_p90}{125}
\defres{e30/intern/lg}{-4.9062}
\defres{e30/intern/prec}{FP8}
\defres{e30/intern/ref}{73.4}
\defres{e30/intern/usdk}{0.012}
\defres{e30/intern/vse9}{3.1}
\defres{e30/jevk5/acc}{70.1}
\defres{e30/jevk5/agree}{96.4}
\defres{e30/jevk5/bf16/acc}{70.3}
\defres{e30/jevk5/bf16/agree}{99.4}
\defres{e30/jevk5/bf16/conc}{64}
\defres{e30/jevk5/bf16/dps}{19.3}
\defres{e30/jevk5/bf16/lat_p50}{63}
\defres{e30/jevk5/bf16/lat_p90}{154}
\defres{e30/jevk5/bf16/lg}{-4.9355}
\defres{e30/jevk5/bf16/usdk}{0.012}
\defres{e30/jevk5/conc}{64}
\defres{e30/jevk5/dacc}{-0.2}
\defres{e30/jevk5/dps}{25.1}
\defres{e30/jevk5/engine}{vLLM}
\defres{e30/jevk5/flag}{none}
\defres{e30/jevk5/fp8/acc}{70.1}
\defres{e30/jevk5/fp8/agree}{96.4}
\defres{e30/jevk5/fp8/conc}{64}
\defres{e30/jevk5/fp8/dps}{25.1}
\defres{e30/jevk5/fp8/lat_p50}{46}
\defres{e30/jevk5/fp8/lat_p90}{105}
\defres{e30/jevk5/fp8/lg}{-5.0511}
\defres{e30/jevk5/fp8/usdk}{0.0089}
\defres{e30/jevk5/lat_p50}{46}
\defres{e30/jevk5/lat_p90}{105}
\defres{e30/jevk5/lg}{-5.0511}
\defres{e30/jevk5/prec}{FP8}
\defres{e30/jevk5/ref}{70.3}
\defres{e30/jevk5/usdk}{0.0089}
\defres{e30/jevk5/vse9}{5.4}
\defres{e30/jevk5v02/acc}{72.7}
\defres{e30/jevk5v02/agree}{87.3}
\defres{e30/jevk5v02/bf16/acc}{73.1}
\defres{e30/jevk5v02/bf16/agree}{86.7}
\defres{e30/jevk5v02/bf16/conc}{64}
\defres{e30/jevk5v02/bf16/dps}{18.6}
\defres{e30/jevk5v02/bf16/lat_p50}{64}
\defres{e30/jevk5v02/bf16/lat_p90}{153}
\defres{e30/jevk5v02/bf16/lg}{-4.9194}
\defres{e30/jevk5v02/bf16/usdk}{0.012}
\defres{e30/jevk5v02/conc}{64}
\defres{e30/jevk5v02/dacc}{+2.4}
\defres{e30/jevk5v02/dps}{24.6}
\defres{e30/jevk5v02/engine}{vLLM}
\defres{e30/jevk5v02/flag}{agreement 87.3 \% $<$ 95 \%}
\defres{e30/jevk5v02/fp8/acc}{72.7}
\defres{e30/jevk5v02/fp8/agree}{87.3}
\defres{e30/jevk5v02/fp8/conc}{64}
\defres{e30/jevk5v02/fp8/dps}{24.6}
\defres{e30/jevk5v02/fp8/lat_p50}{47}
\defres{e30/jevk5v02/fp8/lat_p90}{108}
\defres{e30/jevk5v02/fp8/lg}{-5.0413}
\defres{e30/jevk5v02/fp8/usdk}{0.0091}
\defres{e30/jevk5v02/lat_p50}{47}
\defres{e30/jevk5v02/lat_p90}{108}
\defres{e30/jevk5v02/lg}{-5.0413}
\defres{e30/jevk5v02/prec}{FP8}
\defres{e30/jevk5v02/ref}{70.3}
\defres{e30/jevk5v02/usdk}{0.0091}
\defres{e30/jevk5v02/vse9}{5.3}
\defres{e30/meta/conc}{64 and 256}
\defres{e30/meta/engine}{vLLM}
\defres{e30/meta/fp8kept}{all of them}
\defres{e30/meta/fp8maxdiff}{0.6}
\defres{e30/meta/fp8n}{12}
\defres{e30/meta/gpu}{NVIDIA L4 24 GB}
\defres{e30/meta/hosth}{8.0}
\defres{e30/meta/instance}{g6.xlarge}
\defres{e30/meta/latn}{1{,}000}
\defres{e30/meta/llama}{llama.cpp}
\defres{e30/meta/margin}{1}
\defres{e30/meta/maxdiff}{0.7}
\defres{e30/meta/maxdiff_same}{0.7}
\defres{e30/meta/minagree}{96.1}
\defres{e30/meta/minagree_same}{96.1}
\defres{e30/meta/models}{15}
\defres{e30/meta/n}{3{,}991}
\defres{e30/meta/nlowagree}{0}
\defres{e30/meta/nsame}{15}
\defres{e30/meta/nvllm}{11}
\defres{e30/meta/price_h}{0.8048}
\defres{e30/meta/samefor}{every model}
\defres{e30/meta/version}{0.31.0}
\defres{e30/openjev/acc}{79.1}
\defres{e30/openjev/agree}{96.1}
\defres{e30/openjev/conc}{64}
\defres{e30/openjev/dacc}{+0.3}
\defres{e30/openjev/dps}{45.0}
\defres{e30/openjev/engine}{its own image (g6e.xlarge)}
\defres{e30/openjev/flag}{none}
\defres{e30/openjev/fp8/acc}{79.1}
\defres{e30/openjev/fp8/agree}{96.1}
\defres{e30/openjev/fp8/conc}{64}
\defres{e30/openjev/fp8/dps}{45.0}
\defres{e30/openjev/fp8/lat_p50}{144}
\defres{e30/openjev/fp8/lat_p90}{162}
\defres{e30/openjev/fp8/lg}{-4.9400}
\defres{e30/openjev/fp8/usdk}{0.011}
\defres{e30/openjev/gpu}{NVIDIA L40S 48 GB}
\defres{e30/openjev/instance}{g6e.xlarge}
\defres{e30/openjev/lat_p50}{144}
\defres{e30/openjev/lat_p90}{162}
\defres{e30/openjev/lg}{-4.9400}
\defres{e30/openjev/prec}{FP8}
\defres{e30/openjev/price_h}{1.861}
\defres{e30/openjev/ref}{78.8}
\defres{e30/openjev/usdk}{0.011}
\defres{e30/openjev/vse9}{7.9}
\defres{e30/openjevhf/acc}{83.0}
\defres{e30/openjevhf/agree}{98.4}
\defres{e30/openjevhf/conc}{8}
\defres{e30/openjevhf/dacc}{+0.3}
\defres{e30/openjevhf/dps}{1.3}
\defres{e30/openjevhf/engine}{llama.cpp}
\defres{e30/openjevhf/flag}{none}
\defres{e30/openjevhf/lat_p50}{744}
\defres{e30/openjevhf/lat_p90}{1{,}231}
\defres{e30/openjevhf/lg}{-3.7507}
\defres{e30/openjevhf/prec}{Q4\_K\_M}
\defres{e30/openjevhf/q4_k_m/acc}{83.0}
\defres{e30/openjevhf/q4_k_m/agree}{98.4}
\defres{e30/openjevhf/q4_k_m/conc}{8}
\defres{e30/openjevhf/q4_k_m/dps}{1.3}
\defres{e30/openjevhf/q4_k_m/lat_p50}{744}
\defres{e30/openjevhf/q4_k_m/lat_p90}{1{,}231}
\defres{e30/openjevhf/q4_k_m/lg}{-3.7507}
\defres{e30/openjevhf/q4_k_m/usdk}{0.18}
\defres{e30/openjevhf/ref}{82.7}
\defres{e30/openjevhf/usdk}{0.18}
\defres{e30/openjevhf/vse9}{1.4}
\defres{e30/rl/acc}{78.6}
\defres{e30/rl/agree}{98.5}
\defres{e30/rl/bf16/acc}{78.8}
\defres{e30/rl/bf16/agree}{99.8}
\defres{e30/rl/bf16/conc}{64}
\defres{e30/rl/bf16/dps}{37.5}
\defres{e30/rl/bf16/lat_p50}{45}
\defres{e30/rl/bf16/lat_p90}{75}
\defres{e30/rl/bf16/lg}{-5.2242}
\defres{e30/rl/bf16/usdk}{0.0060}
\defres{e30/rl/conc}{256}
\defres{e30/rl/dacc}{-0.2}
\defres{e30/rl/dps}{50.2}
\defres{e30/rl/engine}{vLLM}
\defres{e30/rl/flag}{none}
\defres{e30/rl/fp8/acc}{78.6}
\defres{e30/rl/fp8/agree}{98.5}
\defres{e30/rl/fp8/conc}{256}
\defres{e30/rl/fp8/dps}{50.2}
\defres{e30/rl/fp8/lat_p50}{31}
\defres{e30/rl/fp8/lat_p90}{52}
\defres{e30/rl/fp8/lg}{-5.3512}
\defres{e30/rl/fp8/usdk}{0.0045}
\defres{e30/rl/lat_p50}{31}
\defres{e30/rl/lat_p90}{52}
\defres{e30/rl/lg}{-5.3512}
\defres{e30/rl/prec}{FP8}
\defres{e30/rl/ref}{78.8}
\defres{e30/rl/usdk}{0.0045}
\defres{e30/rl/vse9}{21}
\defres{e30/sl0.8b/acc}{69.3}
\defres{e30/sl0.8b/agree}{96.9}
\defres{e30/sl0.8b/bf16/acc}{69.9}
\defres{e30/sl0.8b/bf16/agree}{99.1}
\defres{e30/sl0.8b/bf16/conc}{64}
\defres{e30/sl0.8b/bf16/dps}{122}
\defres{e30/sl0.8b/bf16/lat_p50}{35}
\defres{e30/sl0.8b/bf16/lat_p90}{37}
\defres{e30/sl0.8b/bf16/lg}{-5.7377}
\defres{e30/sl0.8b/bf16/usdk}{0.0018}
\defres{e30/sl0.8b/conc}{64}
\defres{e30/sl0.8b/dacc}{-0.7}
\defres{e30/sl0.8b/dps}{131}
\defres{e30/sl0.8b/engine}{vLLM}
\defres{e30/sl0.8b/flag}{none}
\defres{e30/sl0.8b/fp8/acc}{69.3}
\defres{e30/sl0.8b/fp8/agree}{96.9}
\defres{e30/sl0.8b/fp8/conc}{64}
\defres{e30/sl0.8b/fp8/dps}{131}
\defres{e30/sl0.8b/fp8/lat_p50}{32}
\defres{e30/sl0.8b/fp8/lat_p90}{34}
\defres{e30/sl0.8b/fp8/lg}{-5.7690}
\defres{e30/sl0.8b/fp8/usdk}{0.0017}
\defres{e30/sl0.8b/lat_p50}{32}
\defres{e30/sl0.8b/lat_p90}{34}
\defres{e30/sl0.8b/lg}{-5.7690}
\defres{e30/sl0.8b/prec}{FP8}
\defres{e30/sl0.8b/ref}{70.0}
\defres{e30/sl0.8b/usdk}{0.0017}
\defres{e30/sl0.8b/vse9}{7.6}
\defres{e30/sl27b/acc}{87.5}
\defres{e30/sl27b/agree}{98.4}
\defres{e30/sl27b/conc}{8}
\defres{e30/sl27b/dacc}{-0.2}
\defres{e30/sl27b/dps}{1.3}
\defres{e30/sl27b/engine}{llama.cpp}
\defres{e30/sl27b/flag}{none}
\defres{e30/sl27b/lat_p50}{649}
\defres{e30/sl27b/lat_p90}{1{,}224}
\defres{e30/sl27b/lg}{-3.7801}
\defres{e30/sl27b/prec}{Q4\_K\_M}
\defres{e30/sl27b/q4_k_m/acc}{87.5}
\defres{e30/sl27b/q4_k_m/agree}{98.4}
\defres{e30/sl27b/q4_k_m/conc}{8}
\defres{e30/sl27b/q4_k_m/dps}{1.3}
\defres{e30/sl27b/q4_k_m/lat_p50}{649}
\defres{e30/sl27b/q4_k_m/lat_p90}{1{,}224}
\defres{e30/sl27b/q4_k_m/lg}{-3.7801}
\defres{e30/sl27b/q4_k_m/usdk}{0.17}
\defres{e30/sl27b/ref}{87.7}
\defres{e30/sl27b/usdk}{0.17}
\defres{e30/sl27b/vse9}{6.6}
\defres{e30/sl2b/acc}{76.0}
\defres{e30/sl2b/agree}{97.4}
\defres{e30/sl2b/bf16/acc}{75.9}
\defres{e30/sl2b/bf16/agree}{99.4}
\defres{e30/sl2b/bf16/conc}{64}
\defres{e30/sl2b/bf16/dps}{65.2}
\defres{e30/sl2b/bf16/lat_p50}{37}
\defres{e30/sl2b/bf16/lat_p90}{40}
\defres{e30/sl2b/bf16/lg}{-5.4649}
\defres{e30/sl2b/bf16/usdk}{0.0034}
\defres{e30/sl2b/conc}{64}
\defres{e30/sl2b/dacc}{+0.3}
\defres{e30/sl2b/dps}{81.6}
\defres{e30/sl2b/engine}{vLLM}
\defres{e30/sl2b/flag}{none}
\defres{e30/sl2b/fp8/acc}{76.0}
\defres{e30/sl2b/fp8/agree}{97.4}
\defres{e30/sl2b/fp8/conc}{64}
\defres{e30/sl2b/fp8/dps}{81.6}
\defres{e30/sl2b/fp8/lat_p50}{34}
\defres{e30/sl2b/fp8/lat_p90}{36}
\defres{e30/sl2b/fp8/lg}{-5.5625}
\defres{e30/sl2b/fp8/usdk}{0.0027}
\defres{e30/sl2b/lat_p50}{34}
\defres{e30/sl2b/lat_p90}{36}
\defres{e30/sl2b/lg}{-5.5625}
\defres{e30/sl2b/prec}{FP8}
\defres{e30/sl2b/ref}{75.7}
\defres{e30/sl2b/usdk}{0.0027}
\defres{e30/sl2b/vse9}{8.0}
\defres{e30/sl4b/acc}{83.0}
\defres{e30/sl4b/agree}{98.6}
\defres{e30/sl4b/bf16/acc}{83.1}
\defres{e30/sl4b/bf16/agree}{99.7}
\defres{e30/sl4b/bf16/conc}{64}
\defres{e30/sl4b/bf16/dps}{25.3}
\defres{e30/sl4b/bf16/lat_p50}{56}
\defres{e30/sl4b/bf16/lat_p90}{98}
\defres{e30/sl4b/bf16/lg}{-5.0535}
\defres{e30/sl4b/bf16/usdk}{0.0088}
\defres{e30/sl4b/conc}{64}
\defres{e30/sl4b/dacc}{-0.1}
\defres{e30/sl4b/dps}{33.0}
\defres{e30/sl4b/engine}{vLLM}
\defres{e30/sl4b/flag}{none}
\defres{e30/sl4b/fp8/acc}{83.0}
\defres{e30/sl4b/fp8/agree}{98.6}
\defres{e30/sl4b/fp8/conc}{64}
\defres{e30/sl4b/fp8/dps}{33.0}
\defres{e30/sl4b/fp8/lat_p50}{44}
\defres{e30/sl4b/fp8/lat_p90}{69}
\defres{e30/sl4b/fp8/lg}{-5.1696}
\defres{e30/sl4b/fp8/usdk}{0.0068}
\defres{e30/sl4b/lat_p50}{44}
\defres{e30/sl4b/lat_p90}{69}
\defres{e30/sl4b/lg}{-5.1696}
\defres{e30/sl4b/prec}{FP8}
\defres{e30/sl4b/ref}{83.1}
\defres{e30/sl4b/usdk}{0.0068}
\defres{e30/sl4b/vse9}{7.7}
\defres{e30/sl9b/acc}{83.3}
\defres{e30/sl9b/agree}{98.7}
\defres{e30/sl9b/bf16/acc}{83.5}
\defres{e30/sl9b/bf16/agree}{99.8}
\defres{e30/sl9b/bf16/conc}{64}
\defres{e30/sl9b/bf16/dps}{12.9}
\defres{e30/sl9b/bf16/lat_p50}{99}
\defres{e30/sl9b/bf16/lat_p90}{195}
\defres{e30/sl9b/bf16/lg}{-4.7611}
\defres{e30/sl9b/bf16/usdk}{0.017}
\defres{e30/sl9b/conc}{64}
\defres{e30/sl9b/dacc}{-0.1}
\defres{e30/sl9b/dps}{19.5}
\defres{e30/sl9b/engine}{vLLM}
\defres{e30/sl9b/flag}{none}
\defres{e30/sl9b/fp8/acc}{83.3}
\defres{e30/sl9b/fp8/agree}{98.7}
\defres{e30/sl9b/fp8/conc}{64}
\defres{e30/sl9b/fp8/dps}{19.5}
\defres{e30/sl9b/fp8/lat_p50}{66}
\defres{e30/sl9b/fp8/lat_p90}{118}
\defres{e30/sl9b/fp8/lg}{-4.9414}
\defres{e30/sl9b/fp8/usdk}{0.011}
\defres{e30/sl9b/lat_p50}{66}
\defres{e30/sl9b/lat_p90}{118}
\defres{e30/sl9b/lg}{-4.9414}
\defres{e30/sl9b/prec}{FP8}
\defres{e30/sl9b/ref}{83.4}
\defres{e30/sl9b/usdk}{0.011}
\defres{e30/sl9b/vse9}{7.3}
\makeatother


==> generated/e31_rl_only.tex <==
\makeatletter
\providecommand{\res}[1]{\ifcsname jevres@#1\endcsname\csname jevres@#1\endcsname\else\tbd\fi}
\providecommand{\defres}[2]{\expandafter\def\csname jevres@#1\endcsname{#2}}
\defres{e31/ref/base/c/acc}{50.1}
\defres{e31/ref/base/l1/acc}{71.4}
\defres{e31/ref/base/l2/all}{52.9}
\defres{e31/ref/base/l2/mustask}{27.6}
\defres{e31/ref/base/l2/wrong}{655}
\defres{e31/ref/base/l2/wrong_finish}{215}
\defres{e31/ref/base/l2/wrong_finish_share}{33}
\defres{e31/ref/base/l3/success}{13.5}
\defres{e31/ref/base/v1dev/acc}{70.1}
\defres{e31/ref/base/v1dev/recovery}{66.3}
\defres{e31/ref/rl/c/acc}{99.2}
\defres{e31/ref/rl/l1/acc}{78.8}
\defres{e31/ref/rl/l2/all}{98.6}
\defres{e31/ref/rl/l2/mustask}{90.8}
\defres{e31/ref/rl/l3/success}{96.0}
\defres{e31/ref/rl/v1dev/acc}{99.7}
\defres{e31/ref/rl/v1dev/recovery}{99.8}
\defres{e31/ref/sft_v1/c/acc}{99.2}
\defres{e31/ref/sft_v1/l1/acc}{78.4}
\defres{e31/ref/sft_v1/l2/all}{98.4}
\defres{e31/ref/sft_v1/l2/mustask}{95.0}
\defres{e31/ref/sft_v1/l3/success}{96.0}
\defres{e31/ref/sft_v1/v1dev/acc}{99.7}
\defres{e31/ref/sft_v1/v1dev/recovery}{99.8}
\defres{e31/rlonly/api_usd}{21.34}
\defres{e31/rlonly/c/acc}{48.5}
\defres{e31/rlonly/c/offplan}{25.2}
\defres{e31/rlonly/c/vs_base}{-1.6}
\defres{e31/rlonly/c/vs_base/hi}{-0.9}
\defres{e31/rlonly/c/vs_base/lo}{-2.4}
\defres{e31/rlonly/decisions}{9,608}
\defres{e31/rlonly/decisions_made}{9,429}
\defres{e31/rlonly/decisions_made_share}{98.1}
\defres{e31/rlonly/eval/0/rl_ts_assist_k3}{31.2}
\defres{e31/rlonly/eval/0/rl_ts_params_replace}{12.5}
\defres{e31/rlonly/eval/10/rl_ts_assist_k3}{25.0}
\defres{e31/rlonly/eval/10/rl_ts_params_replace}{12.5}
\defres{e31/rlonly/eval/15/rl_ts_assist_k3}{35.4}
\defres{e31/rlonly/eval/15/rl_ts_params_replace}{12.5}
\defres{e31/rlonly/gemini_usd}{22.24}
\defres{e31/rlonly/gpu_h}{1.6}
\defres{e31/rlonly/gpu_min}{96}
\defres{e31/rlonly/host_h}{2.6}
\defres{e31/rlonly/iterations}{15}
\defres{e31/rlonly/kl_max}{0.88}
\defres{e31/rlonly/l1/acc}{71.4}
\defres{e31/rlonly/l1/vs_base}{+0.0}
\defres{e31/rlonly/l1/vs_base/hi}{+0.4}
\defres{e31/rlonly/l1/vs_base/lo}{-0.4}
\defres{e31/rlonly/l2/all}{50.2}
\defres{e31/rlonly/l2/genkind}{44.8}
\defres{e31/rlonly/l2/mustask}{27.6}
\defres{e31/rlonly/l2/newkind}{62.7}
\defres{e31/rlonly/l2/offplan}{76.2}
\defres{e31/rlonly/l2/renamed}{41.7}
\defres{e31/rlonly/l2/vs_base}{-2.7}
\defres{e31/rlonly/l2/vs_base/hi}{-1.2}
\defres{e31/rlonly/l2/vs_base/lo}{-4.1}
\defres{e31/rlonly/l2/vs_rl}{-48.4}
\defres{e31/rlonly/l2/vs_rl/hi}{-44.1}
\defres{e31/rlonly/l2/vs_rl/lo}{-52.9}
\defres{e31/rlonly/l2/vs_sft_v1}{-48.3}
\defres{e31/rlonly/l2/vs_sft_v1/hi}{-43.9}
\defres{e31/rlonly/l2/vs_sft_v1/lo}{-52.7}
\defres{e31/rlonly/l2/wrong}{705}
\defres{e31/rlonly/l2/wrong_finish}{331}
\defres{e31/rlonly/l2/wrong_finish_share}{47}
\defres{e31/rlonly/l3/gemini_usd}{0.88}
\defres{e31/rlonly/l3/n}{200}
\defres{e31/rlonly/l3/own}{40.0}
\defres{e31/rlonly/l3/success}{11.5}
\defres{e31/rlonly/l3/vs_base}{-2.0}
\defres{e31/rlonly/l3/vs_base/hi}{+1.7}
\defres{e31/rlonly/l3/vs_base/lo}{-5.8}
\defres{e31/rlonly/l3/vs_rl}{-84.5}
\defres{e31/rlonly/l3/vs_rl/hi}{-78.1}
\defres{e31/rlonly/l3/vs_rl/lo}{-88.7}
\defres{e31/rlonly/l3/vs_sft_v1}{-84.5}
\defres{e31/rlonly/l3/vs_sft_v1/hi}{-77.7}
\defres{e31/rlonly/l3/vs_sft_v1/lo}{-89.0}
\defres{e31/rlonly/live_usd}{0.89}
\defres{e31/rlonly/matches_sft}{0}
\defres{e31/rlonly/no_update_iters}{0}
\defres{e31/rlonly/peak_gpu_gb}{30}
\defres{e31/rlonly/share/c}{-3}
\defres{e31/rlonly/share/l1}{0}
\defres{e31/rlonly/share/l2}{-6}
\defres{e31/rlonly/share/l3}{-2}
\defres{e31/rlonly/share/mustask}{0}
\defres{e31/rlonly/stopped_early}{0}
\defres{e31/rlonly/train/dec_acc_first3}{70.4}
\defres{e31/rlonly/train/dec_acc_last3}{80.3}
\defres{e31/rlonly/train/success_first3}{38.0}
\defres{e31/rlonly/train/success_last3}{39.6}
\defres{e31/rlonly/updated}{3,274}
\defres{e31/rlonly/v1/dec_acc}{96.0}
\defres{e31/rlonly/v1/train_success}{80.4}
\defres{e31/rlonly/v1/updated}{5,882}
\defres{e31/rlonly/v1/zero_std_share}{60.0}
\defres{e31/rlonly/v1dev/acc}{65.8}
\defres{e31/rlonly/v1dev/recovery}{62.0}
\defres{e31/rlonly/zero_std_share}{75.0}
\makeatother


==> generated/e4_swe.tex <==
\makeatletter
\providecommand{\res}[1]{\ifcsname jevres@#1\endcsname\csname jevres@#1\endcsname\else\tbd\fi}
\providecommand{\defres}[2]{\expandafter\def\csname jevres@#1\endcsname{#2}}
\defres{e4/always_deep/cost_usd}{0.0411}
\defres{e4/always_deep/deep_call_s}{9.5}
\defres{e4/always_deep/fast_call_s}{--}
\defres{e4/always_deep/fast_share}{0.0}
\defres{e4/always_deep/limits_exceeded}{0}
\defres{e4/always_deep/llm_calls}{40.1}
\defres{e4/always_deep/llm_cost_usd}{0.0411}
\defres{e4/always_deep/n}{100}
\defres{e4/always_deep/resolved}{81}
\defres{e4/always_deep/s1_call_s}{--}
\defres{e4/always_deep/s1_cost_usd}{0.0000}
\defres{e4/always_deep/steps}{40.1}
\defres{e4/always_deep/success}{81.0}
\defres{e4/always_deep/wall_mean_s}{399}
\defres{e4/always_deep/wall_median_s}{238}
\defres{e4/always_fast/cost_usd}{0.0108}
\defres{e4/always_fast/deep_call_s}{--}
\defres{e4/always_fast/fast_call_s}{5.3}
\defres{e4/always_fast/fast_share}{100.0}
\defres{e4/always_fast/limits_exceeded}{0}
\defres{e4/always_fast/llm_calls}{46.9}
\defres{e4/always_fast/llm_cost_usd}{0.0108}
\defres{e4/always_fast/n}{100}
\defres{e4/always_fast/resolved}{78}
\defres{e4/always_fast/s1_call_s}{--}
\defres{e4/always_fast/s1_cost_usd}{0.0000}
\defres{e4/always_fast/steps}{46.9}
\defres{e4/always_fast/success}{78.0}
\defres{e4/always_fast/vs_deep/delta}{$-$3}
\defres{e4/always_fast/vs_deep/losses}{6}
\defres{e4/always_fast/vs_deep/saving_pct}{73.7}
\defres{e4/always_fast/vs_deep/time_all/d_median_s}{$-$59.3}
\defres{e4/always_fast/vs_deep/time_cosolved/d_median_s}{$-$38.6}
\defres{e4/always_fast/vs_deep/time_cosolved/n}{75}
\defres{e4/always_fast/vs_deep/time_saving_pct}{31.8}
\defres{e4/always_fast/vs_deep/wins}{3}
\defres{e4/always_fast/wall_mean_s}{272}
\defres{e4/always_fast/wall_median_s}{187}
\defres{e4/dev/always_deep/fast_share}{0.0}
\defres{e4/dev/always_deep/resolved}{36}
\defres{e4/dev/always_fast/fast_share}{100.0}
\defres{e4/dev/always_fast/resolved}{34}
\defres{e4/dev/jevagent_t050/fast_share}{21.4}
\defres{e4/dev/jevagent_t050/resolved}{38}
\defres{e4/dev/jevagent_t060/fast_share}{39.0}
\defres{e4/dev/jevagent_t060/resolved}{38}
\defres{e4/dev/jevagent_t070/fast_share}{72.8}
\defres{e4/dev/jevagent_t070/resolved}{33}
\defres{e4/jevagent/cost_usd}{0.0324}
\defres{e4/jevagent/deep_call_s}{10.3}
\defres{e4/jevagent/fast_call_s}{4.1}
\defres{e4/jevagent/fast_share}{23.5}
\defres{e4/jevagent/limits_exceeded}{0}
\defres{e4/jevagent/llm_calls}{37.4}
\defres{e4/jevagent/llm_cost_usd}{0.0291}
\defres{e4/jevagent/n}{100}
\defres{e4/jevagent/resolved}{81}
\defres{e4/jevagent/s1_call_s}{0.19}
\defres{e4/jevagent/s1_cost_usd}{0.0033}
\defres{e4/jevagent/steps}{37.4}
\defres{e4/jevagent/success}{81.0}
\defres{e4/jevagent/vs_deep/delta}{$+$0}
\defres{e4/jevagent/vs_deep/losses}{3}
\defres{e4/jevagent/vs_deep/saving_pct}{21.3}
\defres{e4/jevagent/vs_deep/time_all/d_median_s}{$-$21.9}
\defres{e4/jevagent/vs_deep/time_cosolved/d_median_s}{$-$25.8}
\defres{e4/jevagent/vs_deep/time_cosolved/n}{78}
\defres{e4/jevagent/vs_deep/time_saving_pct}{11.3}
\defres{e4/jevagent/vs_deep/wins}{3}
\defres{e4/jevagent/wall_mean_s}{354}
\defres{e4/jevagent/wall_median_s}{219}
\defres{e4/n_dev}{45}
\defres{e4/n_eval}{100}
\defres{e4/tau}{0.50}
\makeatother


==> generated/e4b_swe.tex <==
\makeatletter
\providecommand{\res}[1]{\ifcsname jevres@#1\endcsname\csname jevres@#1\endcsname\else\tbd\fi}
\providecommand{\defres}[2]{\expandafter\def\csname jevres@#1\endcsname{#2}}
\defres{e4b/always_deep/cost_usd}{1.0164}
\defres{e4b/always_deep/deep_call_s}{8.6}
\defres{e4b/always_deep/fast_call_s}{--}
\defres{e4b/always_deep/fast_share}{0.0}
\defres{e4b/always_deep/limits_exceeded}{24}
\defres{e4b/always_deep/llm_calls}{93.6}
\defres{e4b/always_deep/llm_cost_usd}{1.0164}
\defres{e4b/always_deep/n}{100}
\defres{e4b/always_deep/resolved}{70}
\defres{e4b/always_deep/s1_call_s}{--}
\defres{e4b/always_deep/s1_cost_usd}{0.0000}
\defres{e4b/always_deep/steps}{93.6}
\defres{e4b/always_deep/success}{70.0}
\defres{e4b/always_deep/wall_mean_s}{886}
\defres{e4b/always_deep/wall_median_s}{907}
\defres{e4b/always_fast/cost_usd}{0.6597}
\defres{e4b/always_fast/deep_call_s}{--}
\defres{e4b/always_fast/fast_call_s}{7.2}
\defres{e4b/always_fast/fast_share}{100.0}
\defres{e4b/always_fast/limits_exceeded}{3}
\defres{e4b/always_fast/llm_calls}{70.1}
\defres{e4b/always_fast/llm_cost_usd}{0.6597}
\defres{e4b/always_fast/n}{50}
\defres{e4b/always_fast/resolved}{40}
\defres{e4b/always_fast/s1_call_s}{--}
\defres{e4b/always_fast/s1_cost_usd}{0.0000}
\defres{e4b/always_fast/steps}{70.1}
\defres{e4b/always_fast/success}{80.0}
\defres{e4b/always_fast/vs_deep/delta}{$+$4}
\defres{e4b/always_fast/vs_deep/losses}{2}
\defres{e4b/always_fast/vs_deep/saving_pct}{36.2}
\defres{e4b/always_fast/vs_deep/time_all/d_median_s}{$-$271.7}
\defres{e4b/always_fast/vs_deep/time_cosolved/d_median_s}{$-$332.7}
\defres{e4b/always_fast/vs_deep/time_cosolved/n}{34}
\defres{e4b/always_fast/vs_deep/time_saving_pct}{35.3}
\defres{e4b/always_fast/vs_deep/wins}{6}
\defres{e4b/always_fast/wall_mean_s}{558}
\defres{e4b/always_fast/wall_median_s}{537}
\defres{e4b/jevagent/cost_usd}{0.9448}
\defres{e4b/jevagent/deep_call_s}{8.0}
\defres{e4b/jevagent/fast_call_s}{7.5}
\defres{e4b/jevagent/fast_share}{21.6}
\defres{e4b/jevagent/limits_exceeded}{17}
\defres{e4b/jevagent/llm_calls}{83.1}
\defres{e4b/jevagent/llm_cost_usd}{0.9376}
\defres{e4b/jevagent/n}{100}
\defres{e4b/jevagent/resolved}{75}
\defres{e4b/jevagent/s1_call_s}{0.18}
\defres{e4b/jevagent/s1_cost_usd}{0.0071}
\defres{e4b/jevagent/steps}{83.1}
\defres{e4b/jevagent/success}{75.0}
\defres{e4b/jevagent/vs_deep/delta}{$+$5}
\defres{e4b/jevagent/vs_deep/losses}{3}
\defres{e4b/jevagent/vs_deep/saving_pct}{7.0}
\defres{e4b/jevagent/vs_deep/time_all/d_median_s}{$-$123.3}
\defres{e4b/jevagent/vs_deep/time_cosolved/d_median_s}{$-$120.5}
\defres{e4b/jevagent/vs_deep/time_cosolved/n}{67}
\defres{e4b/jevagent/vs_deep/time_saving_pct}{17.8}
\defres{e4b/jevagent/vs_deep/wins}{8}
\defres{e4b/jevagent/wall_mean_s}{728}
\defres{e4b/jevagent/wall_median_s}{721}
\defres{e4b/n_dev}{30}
\defres{e4b/n_eval}{100}
\makeatother


==> generated/e4r_swe.tex <==
\makeatletter
\providecommand{\res}[1]{\ifcsname jevres@#1\endcsname\csname jevres@#1\endcsname\else\tbd\fi}
\providecommand{\defres}[2]{\expandafter\def\csname jevres@#1\endcsname{#2}}
\defres{e4r/always_deep/cost_usd}{0.0397}
\defres{e4r/always_deep/errors}{0}
\defres{e4r/always_deep/fast_share}{0.0}
\defres{e4r/always_deep/limits_exceeded}{1}
\defres{e4r/always_deep/llm_cost_usd}{0.0397}
\defres{e4r/always_deep/n}{300}
\defres{e4r/always_deep/resolved}{232}
\defres{e4r/always_deep/s1_cost_usd}{0.0000}
\defres{e4r/always_deep/steps}{39.2}
\defres{e4r/always_deep/success}{77.3}
\defres{e4r/always_deep/wall_mean_s}{457}
\defres{e4r/always_deep/wall_median_s}{315}
\defres{e4r/always_fast/cost_usd}{0.0116}
\defres{e4r/always_fast/errors}{0}
\defres{e4r/always_fast/fast_share}{100.0}
\defres{e4r/always_fast/limits_exceeded}{0}
\defres{e4r/always_fast/llm_cost_usd}{0.0116}
\defres{e4r/always_fast/n}{300}
\defres{e4r/always_fast/resolved}{227}
\defres{e4r/always_fast/s1_cost_usd}{0.0000}
\defres{e4r/always_fast/steps}{47.3}
\defres{e4r/always_fast/success}{75.7}
\defres{e4r/always_fast/vs_deep/d_resolved}{$-$5}
\defres{e4r/always_fast/vs_deep/delta}{$-$1.7}
\defres{e4r/always_fast/vs_deep/delta_hi}{$+$1.7}
\defres{e4r/always_fast/vs_deep/delta_lo}{$-$5.0}
\defres{e4r/always_fast/vs_deep/losses}{15}
\defres{e4r/always_fast/vs_deep/n}{300}
\defres{e4r/always_fast/vs_deep/ni}{no}
\defres{e4r/always_fast/vs_deep/ni_p}{0.229}
\defres{e4r/always_fast/vs_deep/saving_hi}{74.3}
\defres{e4r/always_fast/vs_deep/saving_lo}{66.5}
\defres{e4r/always_fast/vs_deep/saving_pct}{70.7}
\defres{e4r/always_fast/vs_deep/tango_hi}{$+$1.7}
\defres{e4r/always_fast/vs_deep/tango_lo}{$-$5.2}
\defres{e4r/always_fast/vs_deep/time_cosolved/d_median_s}{$-$62.1}
\defres{e4r/always_fast/vs_deep/time_cosolved/n}{217}
\defres{e4r/always_fast/vs_deep/time_saving_hi}{34.1}
\defres{e4r/always_fast/vs_deep/time_saving_lo}{21.0}
\defres{e4r/always_fast/vs_deep/time_saving_pct}{27.9}
\defres{e4r/always_fast/vs_deep/wins}{10}
\defres{e4r/always_fast/wall_mean_s}{330}
\defres{e4r/always_fast/wall_median_s}{228}
\defres{e4r/e4/always_deep/cost_usd}{0.0411}
\defres{e4r/e4/always_deep/errors}{0}
\defres{e4r/e4/always_deep/fast_share}{0.0}
\defres{e4r/e4/always_deep/limits_exceeded}{0}
\defres{e4r/e4/always_deep/llm_cost_usd}{0.0411}
\defres{e4r/e4/always_deep/n}{100}
\defres{e4r/e4/always_deep/resolved}{81}
\defres{e4r/e4/always_deep/s1_cost_usd}{0.0000}
\defres{e4r/e4/always_deep/steps}{40.1}
\defres{e4r/e4/always_deep/success}{81.0}
\defres{e4r/e4/always_deep/wall_mean_s}{399}
\defres{e4r/e4/always_deep/wall_median_s}{238}
\defres{e4r/e4/always_fast/cost_usd}{0.0108}
\defres{e4r/e4/always_fast/errors}{0}
\defres{e4r/e4/always_fast/fast_share}{100.0}
\defres{e4r/e4/always_fast/limits_exceeded}{0}
\defres{e4r/e4/always_fast/llm_cost_usd}{0.0108}
\defres{e4r/e4/always_fast/n}{100}
\defres{e4r/e4/always_fast/resolved}{78}
\defres{e4r/e4/always_fast/s1_cost_usd}{0.0000}
\defres{e4r/e4/always_fast/steps}{46.9}
\defres{e4r/e4/always_fast/success}{78.0}
\defres{e4r/e4/always_fast/vs_deep/d_resolved}{$-$3}
\defres{e4r/e4/always_fast/vs_deep/delta}{$-$3.0}
\defres{e4r/e4/always_fast/vs_deep/delta_hi}{$+$3.0}
\defres{e4r/e4/always_fast/vs_deep/delta_lo}{$-$9.0}
\defres{e4r/e4/always_fast/vs_deep/losses}{6}
\defres{e4r/e4/always_fast/vs_deep/n}{100}
\defres{e4r/e4/always_fast/vs_deep/ni}{no}
\defres{e4r/e4/always_fast/vs_deep/ni_p}{0.571}
\defres{e4r/e4/always_fast/vs_deep/saving_hi}{78.0}
\defres{e4r/e4/always_fast/vs_deep/saving_lo}{68.0}
\defres{e4r/e4/always_fast/vs_deep/saving_pct}{73.7}
\defres{e4r/e4/always_fast/vs_deep/tango_hi}{$+$3.4}
\defres{e4r/e4/always_fast/vs_deep/tango_lo}{$-$10.0}
\defres{e4r/e4/always_fast/vs_deep/time_cosolved/d_median_s}{$-$38.6}
\defres{e4r/e4/always_fast/vs_deep/time_cosolved/n}{75}
\defres{e4r/e4/always_fast/vs_deep/time_saving_hi}{41.0}
\defres{e4r/e4/always_fast/vs_deep/time_saving_lo}{21.0}
\defres{e4r/e4/always_fast/vs_deep/time_saving_pct}{31.8}
\defres{e4r/e4/always_fast/vs_deep/wins}{3}
\defres{e4r/e4/always_fast/wall_mean_s}{272}
\defres{e4r/e4/always_fast/wall_median_s}{187}
\defres{e4r/e4/jevagent/cost_usd}{0.0324}
\defres{e4r/e4/jevagent/errors}{0}
\defres{e4r/e4/jevagent/fast_share}{23.5}
\defres{e4r/e4/jevagent/limits_exceeded}{0}
\defres{e4r/e4/jevagent/llm_cost_usd}{0.0291}
\defres{e4r/e4/jevagent/n}{100}
\defres{e4r/e4/jevagent/resolved}{81}
\defres{e4r/e4/jevagent/s1_cost_usd}{0.0033}
\defres{e4r/e4/jevagent/steps}{37.4}
\defres{e4r/e4/jevagent/success}{81.0}
\defres{e4r/e4/jevagent/vs_deep/d_resolved}{$+$0}
\defres{e4r/e4/jevagent/vs_deep/delta}{$+$0.0}
\defres{e4r/e4/jevagent/vs_deep/delta_hi}{$+$5.0}
\defres{e4r/e4/jevagent/vs_deep/delta_lo}{$-$5.0}
\defres{e4r/e4/jevagent/vs_deep/losses}{3}
\defres{e4r/e4/jevagent/vs_deep/n}{100}
\defres{e4r/e4/jevagent/vs_deep/ni}{no}
\defres{e4r/e4/jevagent/vs_deep/ni_p}{0.135}
\defres{e4r/e4/jevagent/vs_deep/saving_hi}{32.5}
\defres{e4r/e4/jevagent/vs_deep/saving_lo}{8.5}
\defres{e4r/e4/jevagent/vs_deep/saving_pct}{21.3}
\defres{e4r/e4/jevagent/vs_deep/tango_hi}{$+$5.9}
\defres{e4r/e4/jevagent/vs_deep/tango_lo}{$-$5.9}
\defres{e4r/e4/jevagent/vs_deep/time_cosolved/d_median_s}{$-$25.8}
\defres{e4r/e4/jevagent/vs_deep/time_cosolved/n}{78}
\defres{e4r/e4/jevagent/vs_deep/time_saving_hi}{20.2}
\defres{e4r/e4/jevagent/vs_deep/time_saving_lo}{2.0}
\defres{e4r/e4/jevagent/vs_deep/time_saving_pct}{11.3}
\defres{e4r/e4/jevagent/vs_deep/wins}{3}
\defres{e4r/e4/jevagent/wall_mean_s}{354}
\defres{e4r/e4/jevagent/wall_median_s}{219}
\defres{e4r/e4/n_eval}{100}
\defres{e4r/ext/always_deep/cost_usd}{0.0389}
\defres{e4r/ext/always_deep/errors}{0}
\defres{e4r/ext/always_deep/fast_share}{0.0}
\defres{e4r/ext/always_deep/limits_exceeded}{1}
\defres{e4r/ext/always_deep/llm_cost_usd}{0.0389}
\defres{e4r/ext/always_deep/n}{200}
\defres{e4r/ext/always_deep/resolved}{151}
\defres{e4r/ext/always_deep/s1_cost_usd}{0.0000}
\defres{e4r/ext/always_deep/steps}{38.7}
\defres{e4r/ext/always_deep/success}{75.5}
\defres{e4r/ext/always_deep/wall_mean_s}{486}
\defres{e4r/ext/always_deep/wall_median_s}{347}
\defres{e4r/ext/always_fast/cost_usd}{0.0120}
\defres{e4r/ext/always_fast/errors}{0}
\defres{e4r/ext/always_fast/fast_share}{100.0}
\defres{e4r/ext/always_fast/limits_exceeded}{0}
\defres{e4r/ext/always_fast/llm_cost_usd}{0.0120}
\defres{e4r/ext/always_fast/n}{200}
\defres{e4r/ext/always_fast/resolved}{149}
\defres{e4r/ext/always_fast/s1_cost_usd}{0.0000}
\defres{e4r/ext/always_fast/steps}{47.5}
\defres{e4r/ext/always_fast/success}{74.5}
\defres{e4r/ext/always_fast/vs_deep/d_resolved}{$-$2}
\defres{e4r/ext/always_fast/vs_deep/delta}{$-$1.0}
\defres{e4r/ext/always_fast/vs_deep/delta_hi}{$+$3.0}
\defres{e4r/ext/always_fast/vs_deep/delta_lo}{$-$5.0}
\defres{e4r/ext/always_fast/vs_deep/losses}{9}
\defres{e4r/ext/always_fast/vs_deep/n}{200}
\defres{e4r/ext/always_fast/vs_deep/ni}{no}
\defres{e4r/ext/always_fast/vs_deep/ni_p}{0.176}
\defres{e4r/ext/always_fast/vs_deep/saving_hi}{73.8}
\defres{e4r/ext/always_fast/vs_deep/saving_lo}{63.4}
\defres{e4r/ext/always_fast/vs_deep/saving_pct}{69.1}
\defres{e4r/ext/always_fast/vs_deep/tango_hi}{$+$3.2}
\defres{e4r/ext/always_fast/vs_deep/tango_lo}{$-$5.3}
\defres{e4r/ext/always_fast/vs_deep/time_cosolved/d_median_s}{$-$70.4}
\defres{e4r/ext/always_fast/vs_deep/time_cosolved/n}{142}
\defres{e4r/ext/always_fast/vs_deep/time_saving_hi}{34.3}
\defres{e4r/ext/always_fast/vs_deep/time_saving_lo}{17.4}
\defres{e4r/ext/always_fast/vs_deep/time_saving_pct}{26.3}
\defres{e4r/ext/always_fast/vs_deep/wins}{7}
\defres{e4r/ext/always_fast/wall_mean_s}{359}
\defres{e4r/ext/always_fast/wall_median_s}{244}
\defres{e4r/ext/jevagent/cost_usd}{0.0370}
\defres{e4r/ext/jevagent/errors}{0}
\defres{e4r/ext/jevagent/fast_share}{21.7}
\defres{e4r/ext/jevagent/limits_exceeded}{1}
\defres{e4r/ext/jevagent/llm_cost_usd}{0.0336}
\defres{e4r/ext/jevagent/n}{200}
\defres{e4r/ext/jevagent/resolved}{148}
\defres{e4r/ext/jevagent/s1_cost_usd}{0.0034}
\defres{e4r/ext/jevagent/steps}{39.5}
\defres{e4r/ext/jevagent/success}{74.0}
\defres{e4r/ext/jevagent/vs_deep/d_resolved}{$-$3}
\defres{e4r/ext/jevagent/vs_deep/delta}{$-$1.5}
\defres{e4r/ext/jevagent/vs_deep/delta_hi}{$+$2.0}
\defres{e4r/ext/jevagent/vs_deep/delta_lo}{$-$5.0}
\defres{e4r/ext/jevagent/vs_deep/losses}{9}
\defres{e4r/ext/jevagent/vs_deep/n}{200}
\defres{e4r/ext/jevagent/vs_deep/ni}{no}
\defres{e4r/ext/jevagent/vs_deep/ni_p}{0.240}
\defres{e4r/ext/jevagent/vs_deep/saving_hi}{16.9}
\defres{e4r/ext/jevagent/vs_deep/saving_lo}{$-$8.5}
\defres{e4r/ext/jevagent/vs_deep/saving_pct}{4.8}
\defres{e4r/ext/jevagent/vs_deep/tango_hi}{$+$2.6}
\defres{e4r/ext/jevagent/vs_deep/tango_lo}{$-$5.8}
\defres{e4r/ext/jevagent/vs_deep/time_cosolved/d_median_s}{$-$13.5}
\defres{e4r/ext/jevagent/vs_deep/time_cosolved/n}{142}
\defres{e4r/ext/jevagent/vs_deep/time_saving_hi}{10.4}
\defres{e4r/ext/jevagent/vs_deep/time_saving_lo}{$-$6.9}
\defres{e4r/ext/jevagent/vs_deep/time_saving_pct}{2.0}
\defres{e4r/ext/jevagent/vs_deep/wins}{6}
\defres{e4r/ext/jevagent/wall_mean_s}{476}
\defres{e4r/ext/jevagent/wall_median_s}{317}
\defres{e4r/ext/n_eval}{200}
\defres{e4r/jevagent/cost_usd}{0.0355}
\defres{e4r/jevagent/errors}{0}
\defres{e4r/jevagent/fast_share}{22.3}
\defres{e4r/jevagent/limits_exceeded}{1}
\defres{e4r/jevagent/llm_cost_usd}{0.0321}
\defres{e4r/jevagent/n}{300}
\defres{e4r/jevagent/resolved}{229}
\defres{e4r/jevagent/s1_cost_usd}{0.0033}
\defres{e4r/jevagent/steps}{38.8}
\defres{e4r/jevagent/success}{76.3}
\defres{e4r/jevagent/vs_deep/d_resolved}{$-$3}
\defres{e4r/jevagent/vs_deep/delta}{$-$1.0}
\defres{e4r/jevagent/vs_deep/delta_hi}{$+$2.0}
\defres{e4r/jevagent/vs_deep/delta_lo}{$-$4.0}
\defres{e4r/jevagent/vs_deep/losses}{12}
\defres{e4r/jevagent/vs_deep/n}{300}
\defres{e4r/jevagent/vs_deep/ni}{no}
\defres{e4r/jevagent/vs_deep/ni_p}{0.108}
\defres{e4r/jevagent/vs_deep/saving_hi}{19.5}
\defres{e4r/jevagent/vs_deep/saving_lo}{0.4}
\defres{e4r/jevagent/vs_deep/saving_pct}{10.5}
\defres{e4r/jevagent/vs_deep/tango_hi}{$+$2.2}
\defres{e4r/jevagent/vs_deep/tango_lo}{$-$4.3}
\defres{e4r/jevagent/vs_deep/time_cosolved/d_median_s}{$-$17.4}
\defres{e4r/jevagent/vs_deep/time_cosolved/n}{220}
\defres{e4r/jevagent/vs_deep/time_saving_hi}{11.1}
\defres{e4r/jevagent/vs_deep/time_saving_lo}{$-$2.4}
\defres{e4r/jevagent/vs_deep/time_saving_pct}{4.7}
\defres{e4r/jevagent/vs_deep/wins}{9}
\defres{e4r/jevagent/wall_mean_s}{436}
\defres{e4r/jevagent/wall_median_s}{301}
\defres{e4r/margin}{3}
\defres{e4r/n_eval}{300}
\defres{e4r/n_ext}{200}
\defres{e4r/n_rep}{100}
\defres{e4r/spend/key_usage}{17.61}
\defres{e4r/spend/logged_eval}{17.59}
\defres{e4r/spend/logged_smoke}{0.02}
\defres{e4r/spend/logged_total}{17.61}
\defres{e4r/tau}{0.50}
\makeatother


==> generated/e6a.tex <==
\makeatletter
\providecommand{\res}[1]{\ifcsname jevres@#1\endcsname\csname jevres@#1\endcsname\else\tbd\fi}
\providecommand{\defres}[2]{\expandafter\def\csname jevres@#1\endcsname{#2}}
\defres{e6a/assist/acc}{37.5}
\defres{e6a/assist/cost_k}{52.0}
\defres{e6a/assist/cost_usd}{0.0520}
\defres{e6a/assist/coverage}{0.0}
\defres{e6a/assist/delta}{-40.7}
\defres{e6a/assist/delta_ci/hi}{-32.1}
\defres{e6a/assist/delta_ci/lo}{-49.3}
\defres{e6a/assist/llm_calls}{30.0}
\defres{e6a/assist/losses}{58}
\defres{e6a/assist/n}{140}
\defres{e6a/assist/n_dropped}{0}
\defres{e6a/assist/s1_calls}{30.0}
\defres{e6a/assist/saving}{-182.0}
\defres{e6a/assist/saving_ci/hi}{-122.6}
\defres{e6a/assist/saving_ci/lo}{-267.3}
\defres{e6a/assist/status}{run}
\defres{e6a/assist/steps}{30.0}
\defres{e6a/assist/success}{50.7}
\defres{e6a/assist/wall_mean}{57.1}
\defres{e6a/assist/wall_median}{53.1}
\defres{e6a/assist/wins}{1}
\defres{e6a/cal_games}{48}
\defres{e6a/cal_paired}{707}
\defres{e6a/cascade/acc}{73.5}
\defres{e6a/cascade/cost_k}{15.9}
\defres{e6a/cascade/cost_usd}{0.0159}
\defres{e6a/cascade/coverage}{23.3}
\defres{e6a/cascade/delta}{+0.0}
\defres{e6a/cascade/delta_ci/hi}{+3.6}
\defres{e6a/cascade/delta_ci/lo}{-4.3}
\defres{e6a/cascade/llm_calls}{10.1}
\defres{e6a/cascade/losses}{4}
\defres{e6a/cascade/n}{140}
\defres{e6a/cascade/n_dropped}{0}
\defres{e6a/cascade/s1_calls}{13.2}
\defres{e6a/cascade/saving}{14.0}
\defres{e6a/cascade/saving_ci/hi}{28.2}
\defres{e6a/cascade/saving_ci/lo}{-2.8}
\defres{e6a/cascade/status}{run}
\defres{e6a/cascade/steps}{13.2}
\defres{e6a/cascade/success}{91.4}
\defres{e6a/cascade/wall_mean}{22.3}
\defres{e6a/cascade/wall_median}{12.9}
\defres{e6a/cascade/wins}{4}
\defres{e6a/label}{exploratory (E6a)}
\defres{e6a/llm_only/cost_k}{18.4}
\defres{e6a/llm_only/cost_usd}{0.0184}
\defres{e6a/llm_only/llm_acc}{46.7}
\defres{e6a/llm_only/n}{140}
\defres{e6a/llm_only/steps}{12.7}
\defres{e6a/llm_only/success}{91.4}
\defres{e6a/llm_only/wall_mean}{24.1}
\defres{e6a/llm_only/wall_median}{13.7}
\defres{e6a/n_games}{140}
\defres{e6a/replace/acc}{17.7}
\defres{e6a/replace/cost_k}{1.7}
\defres{e6a/replace/cost_usd}{0.0017}
\defres{e6a/replace/coverage}{100.0}
\defres{e6a/replace/delta}{-64.3}
\defres{e6a/replace/delta_ci/hi}{-56.4}
\defres{e6a/replace/delta_ci/lo}{-72.1}
\defres{e6a/replace/llm_calls}{0.0}
\defres{e6a/replace/losses}{90}
\defres{e6a/replace/n}{140}
\defres{e6a/replace/n_dropped}{0}
\defres{e6a/replace/s1_calls}{40.5}
\defres{e6a/replace/saving}{90.7}
\defres{e6a/replace/saving_ci/hi}{92.6}
\defres{e6a/replace/saving_ci/lo}{88.0}
\defres{e6a/replace/status}{run}
\defres{e6a/replace/steps}{40.5}
\defres{e6a/replace/success}{27.1}
\defres{e6a/replace/wall_mean}{18.7}
\defres{e6a/replace/wall_median}{19.8}
\defres{e6a/replace/wins}{0}
\defres{e6a/spend/gemini}{13.55}
\defres{e6a/spend/jev}{0.542}
\defres{e6a/spend/total}{14.09}
\defres{e6a/tau}{0.95}
\makeatother


==> generated/e6b.tex <==
\makeatletter
\providecommand{\res}[1]{\ifcsname jevres@#1\endcsname\csname jevres@#1\endcsname\else\tbd\fi}
\providecommand{\defres}[2]{\expandafter\def\csname jevres@#1\endcsname{#2}}
\defres{e6b/cap}{150}
\defres{e6b/count/cells}{9}
\defres{e6b/count/run}{9}
\defres{e6b/mr_cascade/acc}{76.2}
\defres{e6b/mr_cascade/acted}{54.4}
\defres{e6b/mr_cascade/acted_kind}{decided}
\defres{e6b/mr_cascade/cost_k}{49.0}
\defres{e6b/mr_cascade/cost_ref_k}{40.7}
\defres{e6b/mr_cascade/coverage}{54.4}
\defres{e6b/mr_cascade/delta}{+0.0}
\defres{e6b/mr_cascade/delta_ci/hi}{+1.5}
\defres{e6b/mr_cascade/delta_ci/lo}{-1.5}
\defres{e6b/mr_cascade/fig_delta}{+0.0}
\defres{e6b/mr_cascade/fig_saving}{-21}
\defres{e6b/mr_cascade/losses}{1}
\defres{e6b/mr_cascade/n}{200}
\defres{e6b/mr_cascade/n_dropped}{0}
\defres{e6b/mr_cascade/ref}{llm\_only}
\defres{e6b/mr_cascade/s1_acc_all}{57.2}
\defres{e6b/mr_cascade/saving}{-20.5}
\defres{e6b/mr_cascade/saving_ci/hi}{-17.2}
\defres{e6b/mr_cascade/saving_ci/lo}{-24.0}
\defres{e6b/mr_cascade/state}{exploratory}
\defres{e6b/mr_cascade/success}{99.5}
\defres{e6b/mr_cascade/success_ref}{99.5}
\defres{e6b/mr_cascade/vcode}{3}
\defres{e6b/mr_cascade/verdict}{no saving}
\defres{e6b/mr_cascade/wall_s}{15.2}
\defres{e6b/mr_cascade/wins}{1}
\defres{e6b/mr_trigger/acc}{24.8}
\defres{e6b/mr_trigger/acted}{0.0}
\defres{e6b/mr_trigger/acted_kind}{fired}
\defres{e6b/mr_trigger/cost_k}{41.0}
\defres{e6b/mr_trigger/cost_ref_k}{40.7}
\defres{e6b/mr_trigger/coverage}{100.0}
\defres{e6b/mr_trigger/delta}{+0.0}
\defres{e6b/mr_trigger/delta_ci/hi}{+0.0}
\defres{e6b/mr_trigger/delta_ci/lo}{+0.0}
\defres{e6b/mr_trigger/fig_delta}{+0.0}
\defres{e6b/mr_trigger/fig_saving}{-1}
\defres{e6b/mr_trigger/losses}{0}
\defres{e6b/mr_trigger/n}{200}
\defres{e6b/mr_trigger/n_dropped}{0}
\defres{e6b/mr_trigger/ref}{llm\_only}
\defres{e6b/mr_trigger/saving}{-0.9}
\defres{e6b/mr_trigger/saving_ci/hi}{-0.2}
\defres{e6b/mr_trigger/saving_ci/lo}{-1.6}
\defres{e6b/mr_trigger/state}{exploratory}
\defres{e6b/mr_trigger/success}{99.5}
\defres{e6b/mr_trigger/success_ref}{99.5}
\defres{e6b/mr_trigger/vcode}{3}
\defres{e6b/mr_trigger/verdict}{no saving}
\defres{e6b/mr_trigger/wall_s}{14.2}
\defres{e6b/mr_trigger/wins}{0}
\defres{e6b/mw_cascade/acc}{100.0}
\defres{e6b/mw_cascade/acted}{44.0}
\defres{e6b/mw_cascade/acted_kind}{decided}
\defres{e6b/mw_cascade/cost_k}{60.2}
\defres{e6b/mw_cascade/cost_ref_k}{40.7}
\defres{e6b/mw_cascade/coverage}{44.0}
\defres{e6b/mw_cascade/delta}{-1.0}
\defres{e6b/mw_cascade/delta_ci/hi}{+1.0}
\defres{e6b/mw_cascade/delta_ci/lo}{-3.0}
\defres{e6b/mw_cascade/fig_delta}{-1.0}
\defres{e6b/mw_cascade/fig_saving}{-48}
\defres{e6b/mw_cascade/llm_acc_deferred}{67.5}
\defres{e6b/mw_cascade/losses}{3}
\defres{e6b/mw_cascade/n}{200}
\defres{e6b/mw_cascade/n_dropped}{0}
\defres{e6b/mw_cascade/ref}{llm\_only}
\defres{e6b/mw_cascade/s1_acc_all}{69.1}
\defres{e6b/mw_cascade/saving}{-48.1}
\defres{e6b/mw_cascade/saving_ci/hi}{-43.4}
\defres{e6b/mw_cascade/saving_ci/lo}{-52.5}
\defres{e6b/mw_cascade/state}{exploratory}
\defres{e6b/mw_cascade/success}{98.5}
\defres{e6b/mw_cascade/success_ref}{99.5}
\defres{e6b/mw_cascade/vcode}{3}
\defres{e6b/mw_cascade/verdict}{no saving}
\defres{e6b/mw_cascade/wall_s}{19.8}
\defres{e6b/mw_cascade/wins}{1}
\defres{e6b/mw_guard/acc}{96.8}
\defres{e6b/mw_guard/acted}{0.0}
\defres{e6b/mw_guard/acted_kind}{vetoed}
\defres{e6b/mw_guard/cost_k}{65.2}
\defres{e6b/mw_guard/cost_ref_k}{40.7}
\defres{e6b/mw_guard/coverage}{0.0}
\defres{e6b/mw_guard/delta}{+0.0}
\defres{e6b/mw_guard/delta_ci/hi}{+0.0}
\defres{e6b/mw_guard/delta_ci/lo}{+0.0}
\defres{e6b/mw_guard/fig_delta}{+0.0}
\defres{e6b/mw_guard/fig_saving}{-60}
\defres{e6b/mw_guard/losses}{0}
\defres{e6b/mw_guard/n}{200}
\defres{e6b/mw_guard/n_dropped}{0}
\defres{e6b/mw_guard/ref}{llm\_only}
\defres{e6b/mw_guard/saving}{-60.3}
\defres{e6b/mw_guard/saving_ci/hi}{-55.1}
\defres{e6b/mw_guard/saving_ci/lo}{-65.1}
\defres{e6b/mw_guard/state}{exploratory}
\defres{e6b/mw_guard/success}{99.5}
\defres{e6b/mw_guard/success_ref}{99.5}
\defres{e6b/mw_guard/vcode}{3}
\defres{e6b/mw_guard/verdict}{no saving}
\defres{e6b/mw_guard/wall_s}{24.4}
\defres{e6b/mw_guard/wins}{0}
\defres{e6b/ref/llm_only/cost_k}{40.7}
\defres{e6b/ref/llm_only/n}{200}
\defres{e6b/ref/llm_only/success}{99.5}
\defres{e6b/ref/small_only/cost_k}{9.8}
\defres{e6b/ref/small_only/n}{200}
\defres{e6b/ref/small_only/success}{85.0}
\defres{e6b/rf_cascade/acc}{100.0}
\defres{e6b/rf_cascade/acted}{6.4}
\defres{e6b/rf_cascade/acted_kind}{decided}
\defres{e6b/rf_cascade/cost_k}{51.0}
\defres{e6b/rf_cascade/cost_ref_k}{40.7}
\defres{e6b/rf_cascade/coverage}{6.4}
\defres{e6b/rf_cascade/delta}{+0.5}
\defres{e6b/rf_cascade/delta_ci/hi}{+1.5}
\defres{e6b/rf_cascade/delta_ci/lo}{+0.0}
\defres{e6b/rf_cascade/fig_delta}{+0.5}
\defres{e6b/rf_cascade/fig_saving}{-25}
\defres{e6b/rf_cascade/llm_acc_deferred}{100.0}
\defres{e6b/rf_cascade/losses}{0}
\defres{e6b/rf_cascade/n}{200}
\defres{e6b/rf_cascade/n_dropped}{0}
\defres{e6b/rf_cascade/ref}{llm\_only}
\defres{e6b/rf_cascade/s1_acc_all}{77.6}
\defres{e6b/rf_cascade/saving}{-25.4}
\defres{e6b/rf_cascade/saving_ci/hi}{-23.7}
\defres{e6b/rf_cascade/saving_ci/lo}{-27.1}
\defres{e6b/rf_cascade/state}{exploratory}
\defres{e6b/rf_cascade/success}{100.0}
\defres{e6b/rf_cascade/success_ref}{99.5}
\defres{e6b/rf_cascade/vcode}{3}
\defres{e6b/rf_cascade/verdict}{no saving}
\defres{e6b/rf_cascade/wall_s}{22.2}
\defres{e6b/rf_cascade/wins}{1}
\defres{e6b/rt_cascade/acc}{100.0}
\defres{e6b/rt_cascade/acted}{5.5}
\defres{e6b/rt_cascade/acted_kind}{decided}
\defres{e6b/rt_cascade/cost_k}{20.9}
\defres{e6b/rt_cascade/cost_ref_k}{9.8}
\defres{e6b/rt_cascade/coverage}{5.5}
\defres{e6b/rt_cascade/delta}{-4.0}
\defres{e6b/rt_cascade/delta_ci/hi}{+0.0}
\defres{e6b/rt_cascade/delta_ci/lo}{-8.0}
\defres{e6b/rt_cascade/fig_delta}{-4.0}
\defres{e6b/rt_cascade/fig_saving}{-113}
\defres{e6b/rt_cascade/flash/delta}{-18.5}
\defres{e6b/rt_cascade/flash/n}{200}
\defres{e6b/rt_cascade/flash/saving}{48.7}
\defres{e6b/rt_cascade/llm_acc_deferred}{96.2}
\defres{e6b/rt_cascade/losses}{12}
\defres{e6b/rt_cascade/n}{200}
\defres{e6b/rt_cascade/n_dropped}{0}
\defres{e6b/rt_cascade/ref}{small\_only}
\defres{e6b/rt_cascade/s1_acc_all}{90.6}
\defres{e6b/rt_cascade/saving}{-113.1}
\defres{e6b/rt_cascade/saving_ci/hi}{-104.5}
\defres{e6b/rt_cascade/saving_ci/lo}{-121.6}
\defres{e6b/rt_cascade/state}{exploratory}
\defres{e6b/rt_cascade/success}{81.0}
\defres{e6b/rt_cascade/success_ref}{85.0}
\defres{e6b/rt_cascade/vcode}{4}
\defres{e6b/rt_cascade/verdict}{costs success}
\defres{e6b/rt_cascade/wall_s}{11.2}
\defres{e6b/rt_cascade/wins}{4}
\defres{e6b/spend}{92.74}
\defres{e6b/st_cascade/acc}{100.0}
\defres{e6b/st_cascade/acted}{94.2}
\defres{e6b/st_cascade/acted_kind}{decided}
\defres{e6b/st_cascade/cost_k}{41.0}
\defres{e6b/st_cascade/cost_ref_k}{40.7}
\defres{e6b/st_cascade/coverage}{94.2}
\defres{e6b/st_cascade/delta}{+0.0}
\defres{e6b/st_cascade/delta_ci/hi}{+0.0}
\defres{e6b/st_cascade/delta_ci/lo}{+0.0}
\defres{e6b/st_cascade/fig_delta}{+0.0}
\defres{e6b/st_cascade/fig_saving}{-1}
\defres{e6b/st_cascade/llm_acc_deferred}{100.0}
\defres{e6b/st_cascade/losses}{0}
\defres{e6b/st_cascade/n}{200}
\defres{e6b/st_cascade/n_dropped}{0}
\defres{e6b/st_cascade/overrode}{0.0}
\defres{e6b/st_cascade/ref}{llm\_only}
\defres{e6b/st_cascade/s1_acc_all}{98.9}
\defres{e6b/st_cascade/saving}{-0.7}
\defres{e6b/st_cascade/saving_ci/hi}{-0.1}
\defres{e6b/st_cascade/saving_ci/lo}{-1.4}
\defres{e6b/st_cascade/state}{exploratory}
\defres{e6b/st_cascade/success}{99.5}
\defres{e6b/st_cascade/success_ref}{99.5}
\defres{e6b/st_cascade/vcode}{3}
\defres{e6b/st_cascade/verdict}{no saving}
\defres{e6b/st_cascade/wall_s}{13.6}
\defres{e6b/st_cascade/wins}{0}
\defres{e6b/tp_assist/acc}{98.8}
\defres{e6b/tp_assist/acted}{100.0}
\defres{e6b/tp_assist/acted_kind}{shortlist}
\defres{e6b/tp_assist/binding}{65.6}
\defres{e6b/tp_assist/cost_k}{37.1}
\defres{e6b/tp_assist/cost_ref_k}{40.7}
\defres{e6b/tp_assist/coverage}{0.0}
\defres{e6b/tp_assist/delta}{+0.0}
\defres{e6b/tp_assist/delta_ci/hi}{+0.0}
\defres{e6b/tp_assist/delta_ci/lo}{+0.0}
\defres{e6b/tp_assist/fig_delta}{+0.0}
\defres{e6b/tp_assist/fig_saving}{9}
\defres{e6b/tp_assist/losses}{0}
\defres{e6b/tp_assist/n}{200}
\defres{e6b/tp_assist/n_dropped}{0}
\defres{e6b/tp_assist/recall_k}{98.8}
\defres{e6b/tp_assist/ref}{llm\_only}
\defres{e6b/tp_assist/s1_acc_all}{95.2}
\defres{e6b/tp_assist/saving}{8.9}
\defres{e6b/tp_assist/saving_ci/hi}{10.2}
\defres{e6b/tp_assist/saving_ci/lo}{7.7}
\defres{e6b/tp_assist/state}{exploratory}
\defres{e6b/tp_assist/success}{99.5}
\defres{e6b/tp_assist/success_ref}{99.5}
\defres{e6b/tp_assist/vcode}{1}
\defres{e6b/tp_assist/verdict}{takes over safely}
\defres{e6b/tp_assist/wall_s}{14.8}
\defres{e6b/tp_assist/wins}{0}
\defres{e6b/tp_guard/acc}{93.8}
\defres{e6b/tp_guard/acted}{6.3}
\defres{e6b/tp_guard/acted_kind}{vetoed}
\defres{e6b/tp_guard/cost_k}{43.4}
\defres{e6b/tp_guard/cost_ref_k}{40.7}
\defres{e6b/tp_guard/coverage}{0.0}
\defres{e6b/tp_guard/delta}{+0.0}
\defres{e6b/tp_guard/delta_ci/hi}{+0.0}
\defres{e6b/tp_guard/delta_ci/lo}{+0.0}
\defres{e6b/tp_guard/fig_delta}{+0.0}
\defres{e6b/tp_guard/fig_saving}{-7}
\defres{e6b/tp_guard/losses}{0}
\defres{e6b/tp_guard/n}{200}
\defres{e6b/tp_guard/n_dropped}{0}
\defres{e6b/tp_guard/ref}{llm\_only}
\defres{e6b/tp_guard/saving}{-6.7}
\defres{e6b/tp_guard/saving_ci/hi}{-4.7}
\defres{e6b/tp_guard/saving_ci/lo}{-9.0}
\defres{e6b/tp_guard/state}{exploratory}
\defres{e6b/tp_guard/success}{99.5}
\defres{e6b/tp_guard/success_ref}{99.5}
\defres{e6b/tp_guard/vcode}{3}
\defres{e6b/tp_guard/verdict}{no saving}
\defres{e6b/tp_guard/veto_llm_was_wrong}{0.0}
\defres{e6b/tp_guard/veto_on_other}{100.0}
\defres{e6b/tp_guard/veto_tool_changed}{32.9}
\defres{e6b/tp_guard/wall_s}{16.5}
\defres{e6b/tp_guard/wins}{0}
\makeatother


==> generated/e6c.tex <==
\makeatletter
\providecommand{\res}[1]{\ifcsname jevres@#1\endcsname\csname jevres@#1\endcsname\else\tbd\fi}
\providecommand{\defres}[2]{\expandafter\def\csname jevres@#1\endcsname{#2}}
\defres{e6c/guard/acc}{65.5}
\defres{e6c/guard/cost_k}{35.7}
\defres{e6c/guard/cost_usd}{0.0357}
\defres{e6c/guard/coverage}{46.5}
\defres{e6c/guard/delta}{-0.7}
\defres{e6c/guard/delta_ci/hi}{+2.9}
\defres{e6c/guard/delta_ci/lo}{-4.3}
\defres{e6c/guard/executed_acc}{39.7}
\defres{e6c/guard/llm_calls}{22.1}
\defres{e6c/guard/losses}{4}
\defres{e6c/guard/n}{140}
\defres{e6c/guard/n_dropped}{0}
\defres{e6c/guard/proposal_acc}{44.6}
\defres{e6c/guard/rewrite_acc}{17.1}
\defres{e6c/guard/rewrite_same}{24.7}
\defres{e6c/guard/s1_calls}{15.1}
\defres{e6c/guard/saving}{-86.7}
\defres{e6c/guard/saving_ci/hi}{-56.6}
\defres{e6c/guard/saving_ci/lo}{-127.4}
\defres{e6c/guard/status}{run}
\defres{e6c/guard/steps}{15.1}
\defres{e6c/guard/success}{90.0}
\defres{e6c/guard/verdict}{no saving}
\defres{e6c/guard/veto_precision}{72.4}
\defres{e6c/guard/veto_recall}{60.8}
\defres{e6c/guard/vetoed}{46.5}
\defres{e6c/guard/vetoes_per_episode}{7.02}
\defres{e6c/guard/wall_mean}{56.9}
\defres{e6c/guard/wall_median}{36.1}
\defres{e6c/guard/wins}{3}
\defres{e6c/label}{exploratory (E6c)}
\defres{e6c/llm_only/cost_k}{19.1}
\defres{e6c/llm_only/cost_usd}{0.0191}
\defres{e6c/llm_only/llm_acc}{45.7}
\defres{e6c/llm_only/n}{140}
\defres{e6c/llm_only/steps}{13.0}
\defres{e6c/llm_only/success}{90.7}
\defres{e6c/llm_only/wall_mean}{37.2}
\defres{e6c/llm_only/wall_median}{24.6}
\defres{e6c/n_games}{140}
\defres{e6c/spend/gemini}{7.65}
\defres{e6c/spend/jev}{0.056}
\defres{e6c/spend/total}{7.70}
\defres{e6c/tau}{0.5}
\makeatother


==> generated/e6d.tex <==
\makeatletter
\providecommand{\res}[1]{\ifcsname jevres@#1\endcsname\csname jevres@#1\endcsname\else\tbd\fi}
\providecommand{\defres}[2]{\expandafter\def\csname jevres@#1\endcsname{#2}}
\defres{e6d/cap}{120}
\defres{e6d/count/cells}{7}
\defres{e6d/count/run}{7}
\defres{e6d/mr_guard/acc}{58.7}
\defres{e6d/mr_guard/acted}{41.2}
\defres{e6d/mr_guard/acted_kind}{vetoed}
\defres{e6d/mr_guard/cost_k}{38.2}
\defres{e6d/mr_guard/cost_ref_k}{16.0}
\defres{e6d/mr_guard/coverage}{0.0}
\defres{e6d/mr_guard/delta}{+0.0}
\defres{e6d/mr_guard/delta_ci/hi}{+0.0}
\defres{e6d/mr_guard/delta_ci/lo}{+0.0}
\defres{e6d/mr_guard/fig_delta}{+0.0}
\defres{e6d/mr_guard/fig_saving}{-140}
\defres{e6d/mr_guard/final_covers}{65.8}
\defres{e6d/mr_guard/llm_store_rate}{0.0}
\defres{e6d/mr_guard/losses}{0}
\defres{e6d/mr_guard/n}{200}
\defres{e6d/mr_guard/n_dropped}{0}
\defres{e6d/mr_guard/ref}{llm\_only}
\defres{e6d/mr_guard/saving}{-139.8}
\defres{e6d/mr_guard/saving_ci/hi}{-130.9}
\defres{e6d/mr_guard/saving_ci/lo}{-148.7}
\defres{e6d/mr_guard/state}{exploratory}
\defres{e6d/mr_guard/success}{100.0}
\defres{e6d/mr_guard/success_ref}{100.0}
\defres{e6d/mr_guard/vcode}{3}
\defres{e6d/mr_guard/verdict}{no saving}
\defres{e6d/mr_guard/veto_precision}{30.0}
\defres{e6d/mr_guard/wall_s}{16.5}
\defres{e6d/mr_guard/wins}{0}
\defres{e6d/mw_assist/acc}{69.3}
\defres{e6d/mw_assist/acted}{100.0}
\defres{e6d/mw_assist/acted_kind}{advised}
\defres{e6d/mw_assist/cost_k}{27.8}
\defres{e6d/mw_assist/cost_ref_k}{16.0}
\defres{e6d/mw_assist/coverage}{0.0}
\defres{e6d/mw_assist/delta}{+0.0}
\defres{e6d/mw_assist/delta_ci/hi}{+0.0}
\defres{e6d/mw_assist/delta_ci/lo}{+0.0}
\defres{e6d/mw_assist/fig_delta}{+0.0}
\defres{e6d/mw_assist/fig_saving}{-74}
\defres{e6d/mw_assist/followed}{2.7}
\defres{e6d/mw_assist/llm_final_acc}{33.4}
\defres{e6d/mw_assist/losses}{0}
\defres{e6d/mw_assist/n}{200}
\defres{e6d/mw_assist/n_dropped}{0}
\defres{e6d/mw_assist/ref}{llm\_only}
\defres{e6d/mw_assist/saving}{-74.2}
\defres{e6d/mw_assist/saving_ci/hi}{-69.2}
\defres{e6d/mw_assist/saving_ci/lo}{-79.1}
\defres{e6d/mw_assist/state}{exploratory}
\defres{e6d/mw_assist/success}{100.0}
\defres{e6d/mw_assist/success_ref}{100.0}
\defres{e6d/mw_assist/vcode}{3}
\defres{e6d/mw_assist/verdict}{no saving}
\defres{e6d/mw_assist/wall_s}{14.2}
\defres{e6d/mw_assist/wins}{0}
\defres{e6d/ref/llm_only/cost_k}{16.0}
\defres{e6d/ref/llm_only/n}{200}
\defres{e6d/ref/llm_only/success}{100.0}
\defres{e6d/ref/small_only (e6d_modes_routing)/cost_k}{9.8}
\defres{e6d/ref/small_only (e6d_modes_routing)/n}{200}
\defres{e6d/ref/small_only (e6d_modes_routing)/success}{83.5}
\defres{e6d/ref/small_only/cost_k}{2.5}
\defres{e6d/ref/small_only/n}{200}
\defres{e6d/ref/small_only/success}{25.5}
\defres{e6d/rf_assist/acc}{69.0}
\defres{e6d/rf_assist/acted}{100.0}
\defres{e6d/rf_assist/acted_kind}{advised}
\defres{e6d/rf_assist/cost_k}{26.4}
\defres{e6d/rf_assist/cost_ref_k}{16.0}
\defres{e6d/rf_assist/coverage}{0.0}
\defres{e6d/rf_assist/delta}{-0.5}
\defres{e6d/rf_assist/delta_ci/hi}{+0.0}
\defres{e6d/rf_assist/delta_ci/lo}{-1.5}
\defres{e6d/rf_assist/fig_delta}{-0.5}
\defres{e6d/rf_assist/fig_saving}{-66}
\defres{e6d/rf_assist/followed}{69.1}
\defres{e6d/rf_assist/llm_final_acc}{99.9}
\defres{e6d/rf_assist/losses}{1}
\defres{e6d/rf_assist/n}{200}
\defres{e6d/rf_assist/n_dropped}{0}
\defres{e6d/rf_assist/ref}{llm\_only}
\defres{e6d/rf_assist/saving}{-65.7}
\defres{e6d/rf_assist/saving_ci/hi}{-61.1}
\defres{e6d/rf_assist/saving_ci/lo}{-70.5}
\defres{e6d/rf_assist/state}{exploratory}
\defres{e6d/rf_assist/success}{99.5}
\defres{e6d/rf_assist/success_ref}{100.0}
\defres{e6d/rf_assist/vcode}{3}
\defres{e6d/rf_assist/verdict}{no saving}
\defres{e6d/rf_assist/wall_s}{14.1}
\defres{e6d/rf_assist/wins}{0}
\defres{e6d/rf_guard/acc}{100.0}
\defres{e6d/rf_guard/acted}{90.9}
\defres{e6d/rf_guard/acted_kind}{vetoed}
\defres{e6d/rf_guard/cost_k}{25.7}
\defres{e6d/rf_guard/cost_ref_k}{16.0}
\defres{e6d/rf_guard/coverage}{0.0}
\defres{e6d/rf_guard/delta}{+0.0}
\defres{e6d/rf_guard/delta_ci/hi}{+0.0}
\defres{e6d/rf_guard/delta_ci/lo}{+0.0}
\defres{e6d/rf_guard/fig_delta}{+0.0}
\defres{e6d/rf_guard/fig_saving}{-61}
\defres{e6d/rf_guard/llm_store_rate}{0.8}
\defres{e6d/rf_guard/losses}{0}
\defres{e6d/rf_guard/n}{200}
\defres{e6d/rf_guard/n_dropped}{0}
\defres{e6d/rf_guard/ref}{llm\_only}
\defres{e6d/rf_guard/saving}{-61.2}
\defres{e6d/rf_guard/saving_ci/hi}{-56.6}
\defres{e6d/rf_guard/saving_ci/lo}{-65.6}
\defres{e6d/rf_guard/state}{exploratory}
\defres{e6d/rf_guard/success}{100.0}
\defres{e6d/rf_guard/success_ref}{100.0}
\defres{e6d/rf_guard/vcode}{3}
\defres{e6d/rf_guard/verdict}{no saving}
\defres{e6d/rf_guard/veto_precision}{100.0}
\defres{e6d/rf_guard/wall_s}{12.8}
\defres{e6d/rf_guard/wins}{0}
\defres{e6d/rt_assist/acc}{92.8}
\defres{e6d/rt_assist/acted}{100.0}
\defres{e6d/rt_assist/acted_kind}{advised}
\defres{e6d/rt_assist/cost_k}{12.8}
\defres{e6d/rt_assist/cost_ref_k}{9.8}
\defres{e6d/rt_assist/coverage}{0.0}
\defres{e6d/rt_assist/delta}{-2.0}
\defres{e6d/rt_assist/delta_ci/hi}{+2.0}
\defres{e6d/rt_assist/delta_ci/lo}{-6.0}
\defres{e6d/rt_assist/fig_delta}{-2.0}
\defres{e6d/rt_assist/fig_saving}{-31}
\defres{e6d/rt_assist/followed}{92.7}
\defres{e6d/rt_assist/llm_final_acc}{97.5}
\defres{e6d/rt_assist/losses}{11}
\defres{e6d/rt_assist/n}{200}
\defres{e6d/rt_assist/n_dropped}{0}
\defres{e6d/rt_assist/ref}{small\_only}
\defres{e6d/rt_assist/saving}{-31.0}
\defres{e6d/rt_assist/saving_ci/hi}{-28.2}
\defres{e6d/rt_assist/saving_ci/lo}{-33.9}
\defres{e6d/rt_assist/state}{exploratory}
\defres{e6d/rt_assist/success}{81.5}
\defres{e6d/rt_assist/success_ref}{83.5}
\defres{e6d/rt_assist/vcode}{3}
\defres{e6d/rt_assist/verdict}{no saving}
\defres{e6d/rt_assist/wall_s}{11.9}
\defres{e6d/rt_assist/wins}{7}
\defres{e6d/rt_guard/acc}{100.0}
\defres{e6d/rt_guard/acted}{95.8}
\defres{e6d/rt_guard/acted_kind}{vetoed}
\defres{e6d/rt_guard/cost_k}{12.0}
\defres{e6d/rt_guard/cost_ref_k}{9.8}
\defres{e6d/rt_guard/coverage}{0.0}
\defres{e6d/rt_guard/delta}{+0.0}
\defres{e6d/rt_guard/delta_ci/hi}{+4.0}
\defres{e6d/rt_guard/delta_ci/lo}{-4.0}
\defres{e6d/rt_guard/fig_delta}{+0.0}
\defres{e6d/rt_guard/fig_saving}{-23}
\defres{e6d/rt_guard/llm_store_rate}{20.4}
\defres{e6d/rt_guard/losses}{8}
\defres{e6d/rt_guard/n}{200}
\defres{e6d/rt_guard/n_dropped}{0}
\defres{e6d/rt_guard/ref}{small\_only}
\defres{e6d/rt_guard/saving}{-22.6}
\defres{e6d/rt_guard/saving_ci/hi}{-20.9}
\defres{e6d/rt_guard/saving_ci/lo}{-24.3}
\defres{e6d/rt_guard/state}{exploratory}
\defres{e6d/rt_guard/success}{83.5}
\defres{e6d/rt_guard/success_ref}{83.5}
\defres{e6d/rt_guard/vcode}{3}
\defres{e6d/rt_guard/verdict}{no saving}
\defres{e6d/rt_guard/veto_precision}{100.0}
\defres{e6d/rt_guard/wall_s}{11.1}
\defres{e6d/rt_guard/wins}{8}
\defres{e6d/spend}{40.57}
\defres{e6d/st_assist/acc}{99.3}
\defres{e6d/st_assist/acted}{100.0}
\defres{e6d/st_assist/acted_kind}{advised}
\defres{e6d/st_assist/cost_k}{18.6}
\defres{e6d/st_assist/cost_ref_k}{16.0}
\defres{e6d/st_assist/coverage}{0.0}
\defres{e6d/st_assist/delta}{+0.0}
\defres{e6d/st_assist/delta_ci/hi}{+0.0}
\defres{e6d/st_assist/delta_ci/lo}{+0.0}
\defres{e6d/st_assist/fig_delta}{+0.0}
\defres{e6d/st_assist/fig_saving}{-17}
\defres{e6d/st_assist/followed}{99.3}
\defres{e6d/st_assist/llm_final_acc}{100.0}
\defres{e6d/st_assist/losses}{0}
\defres{e6d/st_assist/n}{200}
\defres{e6d/st_assist/n_dropped}{0}
\defres{e6d/st_assist/ref}{llm\_only}
\defres{e6d/st_assist/saving}{-16.7}
\defres{e6d/st_assist/saving_ci/hi}{-13.7}
\defres{e6d/st_assist/saving_ci/lo}{-19.8}
\defres{e6d/st_assist/state}{exploratory}
\defres{e6d/st_assist/success}{100.0}
\defres{e6d/st_assist/success_ref}{100.0}
\defres{e6d/st_assist/vcode}{3}
\defres{e6d/st_assist/verdict}{no saving}
\defres{e6d/st_assist/wall_s}{9.2}
\defres{e6d/st_assist/wins}{0}
\makeatother


==> generated/e6e.tex <==
\makeatletter
\providecommand{\res}[1]{\ifcsname jevres@#1\endcsname\csname jevres@#1\endcsname\else\tbd\fi}
\providecommand{\defres}[2]{\expandafter\def\csname jevres@#1\endcsname{#2}}
\defres{e6e/cap}{60}
\defres{e6e/count/cells}{5}
\defres{e6e/count/run}{5}
\defres{e6e/mr_replace/acc}{57.2}
\defres{e6e/mr_replace/acted}{100.0}
\defres{e6e/mr_replace/acted_kind}{decided}
\defres{e6e/mr_replace/cost_k}{17.8}
\defres{e6e/mr_replace/cost_ref_k}{16.0}
\defres{e6e/mr_replace/coverage}{100.0}
\defres{e6e/mr_replace/delta}{+0.5}
\defres{e6e/mr_replace/delta_ci/hi}{+1.5}
\defres{e6e/mr_replace/delta_ci/lo}{+0.0}
\defres{e6e/mr_replace/equals}{assist with k = 1}
\defres{e6e/mr_replace/fig_delta}{+0.5}
\defres{e6e/mr_replace/fig_saving}{-11}
\defres{e6e/mr_replace/final_covers}{68.6}
\defres{e6e/mr_replace/losses}{0}
\defres{e6e/mr_replace/n}{200}
\defres{e6e/mr_replace/n_dropped}{0}
\defres{e6e/mr_replace/ref}{llm\_only}
\defres{e6e/mr_replace/saving}{-11.1}
\defres{e6e/mr_replace/saving_ci/hi}{-8.4}
\defres{e6e/mr_replace/saving_ci/lo}{-13.9}
\defres{e6e/mr_replace/state}{exploratory}
\defres{e6e/mr_replace/success}{100.0}
\defres{e6e/mr_replace/success_ref}{99.5}
\defres{e6e/mr_replace/vcode}{3}
\defres{e6e/mr_replace/verdict}{no saving}
\defres{e6e/mr_replace/wall_s}{8.8}
\defres{e6e/mr_replace/wins}{1}
\defres{e6e/mw_replace/acc}{69.4}
\defres{e6e/mw_replace/acted}{100.0}
\defres{e6e/mw_replace/acted_kind}{decided}
\defres{e6e/mw_replace/cost_k}{23.7}
\defres{e6e/mw_replace/cost_ref_k}{16.0}
\defres{e6e/mw_replace/coverage}{100.0}
\defres{e6e/mw_replace/delta}{+0.5}
\defres{e6e/mw_replace/delta_ci/hi}{+1.5}
\defres{e6e/mw_replace/delta_ci/lo}{+0.0}
\defres{e6e/mw_replace/equals}{trigger at tau = 0.5}
\defres{e6e/mw_replace/fig_delta}{+0.5}
\defres{e6e/mw_replace/fig_saving}{-47}
\defres{e6e/mw_replace/gold_positive_rate}{67.9}
\defres{e6e/mw_replace/losses}{0}
\defres{e6e/mw_replace/model_yes_rate}{98.5}
\defres{e6e/mw_replace/n}{200}
\defres{e6e/mw_replace/n_dropped}{0}
\defres{e6e/mw_replace/ref}{llm\_only}
\defres{e6e/mw_replace/saving}{-47.4}
\defres{e6e/mw_replace/saving_ci/hi}{-42.4}
\defres{e6e/mw_replace/saving_ci/lo}{-53.1}
\defres{e6e/mw_replace/state}{exploratory}
\defres{e6e/mw_replace/success}{100.0}
\defres{e6e/mw_replace/success_ref}{99.5}
\defres{e6e/mw_replace/vcode}{3}
\defres{e6e/mw_replace/verdict}{no saving}
\defres{e6e/mw_replace/wall_s}{9.1}
\defres{e6e/mw_replace/wins}{1}
\defres{e6e/ref/llm_only/cost_k}{16.0}
\defres{e6e/ref/llm_only/n}{200}
\defres{e6e/ref/llm_only/success}{99.5}
\defres{e6e/ref/small_only/cost_k}{9.8}
\defres{e6e/ref/small_only/n}{200}
\defres{e6e/ref/small_only/success}{80.0}
\defres{e6e/rf_replace/acc}{99.9}
\defres{e6e/rf_replace/acted}{100.0}
\defres{e6e/rf_replace/acted_kind}{decided}
\defres{e6e/rf_replace/cost_k}{17.2}
\defres{e6e/rf_replace/cost_ref_k}{16.0}
\defres{e6e/rf_replace/coverage}{100.0}
\defres{e6e/rf_replace/delta}{-0.5}
\defres{e6e/rf_replace/delta_ci/hi}{+0.0}
\defres{e6e/rf_replace/delta_ci/lo}{-1.5}
\defres{e6e/rf_replace/equals}{trigger at tau = 0.5}
\defres{e6e/rf_replace/fig_delta}{-0.5}
\defres{e6e/rf_replace/fig_saving}{-7}
\defres{e6e/rf_replace/gold_positive_rate}{0.1}
\defres{e6e/rf_replace/losses}{1}
\defres{e6e/rf_replace/model_yes_rate}{14.0}
\defres{e6e/rf_replace/n}{200}
\defres{e6e/rf_replace/n_dropped}{0}
\defres{e6e/rf_replace/ref}{llm\_only}
\defres{e6e/rf_replace/saving}{-7.2}
\defres{e6e/rf_replace/saving_ci/hi}{-4.6}
\defres{e6e/rf_replace/saving_ci/lo}{-9.8}
\defres{e6e/rf_replace/state}{exploratory}
\defres{e6e/rf_replace/success}{99.0}
\defres{e6e/rf_replace/success_ref}{99.5}
\defres{e6e/rf_replace/vcode}{3}
\defres{e6e/rf_replace/verdict}{no saving}
\defres{e6e/rf_replace/wall_s}{10.4}
\defres{e6e/rf_replace/wins}{0}
\defres{e6e/rt_replace/acc}{97.8}
\defres{e6e/rt_replace/acted}{100.0}
\defres{e6e/rt_replace/acted_kind}{decided}
\defres{e6e/rt_replace/cost_k}{10.4}
\defres{e6e/rt_replace/cost_ref_k}{9.8}
\defres{e6e/rt_replace/coverage}{100.0}
\defres{e6e/rt_replace/delta}{+4.0}
\defres{e6e/rt_replace/delta_ci/hi}{+7.5}
\defres{e6e/rt_replace/delta_ci/lo}{+0.5}
\defres{e6e/rt_replace/equals}{trigger at tau = 0.5}
\defres{e6e/rt_replace/fig_delta}{+4.0}
\defres{e6e/rt_replace/fig_saving}{-7}
\defres{e6e/rt_replace/flash/delta}{-15.5}
\defres{e6e/rt_replace/flash/n}{200}
\defres{e6e/rt_replace/flash/saving}{34.9}
\defres{e6e/rt_replace/gold_positive_rate}{2.2}
\defres{e6e/rt_replace/losses}{3}
\defres{e6e/rt_replace/model_yes_rate}{4.6}
\defres{e6e/rt_replace/n}{200}
\defres{e6e/rt_replace/n_dropped}{0}
\defres{e6e/rt_replace/ref}{small\_only}
\defres{e6e/rt_replace/saving}{-6.7}
\defres{e6e/rt_replace/saving_ci/hi}{-5.3}
\defres{e6e/rt_replace/saving_ci/lo}{-8.2}
\defres{e6e/rt_replace/state}{exploratory}
\defres{e6e/rt_replace/success}{84.0}
\defres{e6e/rt_replace/success_ref}{80.0}
\defres{e6e/rt_replace/vcode}{3}
\defres{e6e/rt_replace/verdict}{no saving}
\defres{e6e/rt_replace/wall_s}{6.8}
\defres{e6e/rt_replace/wins}{11}
\defres{e6e/spend}{22.65}
\defres{e6e/st_replace/acc}{98.1}
\defres{e6e/st_replace/acted}{100.0}
\defres{e6e/st_replace/acted_kind}{decided}
\defres{e6e/st_replace/cost_k}{17.1}
\defres{e6e/st_replace/cost_ref_k}{16.0}
\defres{e6e/st_replace/coverage}{100.0}
\defres{e6e/st_replace/delta}{+0.5}
\defres{e6e/st_replace/delta_ci/hi}{+1.5}
\defres{e6e/st_replace/delta_ci/lo}{+0.0}
\defres{e6e/st_replace/equals}{cascade at tau = 0.5}
\defres{e6e/st_replace/fig_delta}{+0.5}
\defres{e6e/st_replace/fig_saving}{-7}
\defres{e6e/st_replace/gold_positive_rate}{14.9}
\defres{e6e/st_replace/losses}{0}
\defres{e6e/st_replace/model_yes_rate}{13.0}
\defres{e6e/st_replace/n}{200}
\defres{e6e/st_replace/n_dropped}{0}
\defres{e6e/st_replace/overrode}{2.1}
\defres{e6e/st_replace/ref}{llm\_only}
\defres{e6e/st_replace/saving}{-6.8}
\defres{e6e/st_replace/saving_ci/hi}{-3.4}
\defres{e6e/st_replace/saving_ci/lo}{-10.8}
\defres{e6e/st_replace/state}{exploratory}
\defres{e6e/st_replace/success}{100.0}
\defres{e6e/st_replace/success_ref}{99.5}
\defres{e6e/st_replace/vcode}{3}
\defres{e6e/st_replace/verdict}{no saving}
\defres{e6e/st_replace/wall_s}{9.8}
\defres{e6e/st_replace/wins}{1}
\makeatother


==> generated/e6f.tex <==
\makeatletter
\providecommand{\res}[1]{\ifcsname jevres@#1\endcsname\csname jevres@#1\endcsname\else\tbd\fi}
\providecommand{\defres}[2]{\expandafter\def\csname jevres@#1\endcsname{#2}}
\defres{e6f/count/cells}{3}
\defres{e6f/count/run}{3}
\defres{e6f/jev_action_trigger/acc}{67.1}
\defres{e6f/jev_action_trigger/acted}{74.9}
\defres{e6f/jev_action_trigger/acted_kind}{fired}
\defres{e6f/jev_action_trigger/always/broke}{49}
\defres{e6f/jev_action_trigger/always/cost_k}{50.9}
\defres{e6f/jev_action_trigger/always/cost_ref_k}{19.6}
\defres{e6f/jev_action_trigger/always/cost_share}{69.7}
\defres{e6f/jev_action_trigger/always/delta}{-2.9}
\defres{e6f/jev_action_trigger/always/delta_ci/hi}{+0.0}
\defres{e6f/jev_action_trigger/always/delta_ci/lo}{-6.4}
\defres{e6f/jev_action_trigger/always/effect_share}{75.0}
\defres{e6f/jev_action_trigger/always/fig_delta}{-2.9}
\defres{e6f/jev_action_trigger/always/fig_saving}{-160}
\defres{e6f/jev_action_trigger/always/fix_share}{300.0}
\defres{e6f/jev_action_trigger/always/fixed}{3}
\defres{e6f/jev_action_trigger/always/n}{140}
\defres{e6f/jev_action_trigger/always/n_dropped}{0}
\defres{e6f/jev_action_trigger/always/n_proposals}{2007}
\defres{e6f/jev_action_trigger/always/net_fix_share}{30.4}
\defres{e6f/jev_action_trigger/always/net_fixed}{-46}
\defres{e6f/jev_action_trigger/always/saving}{-159.5}
\defres{e6f/jev_action_trigger/always/saving_ci/hi}{-127.4}
\defres{e6f/jev_action_trigger/always/saving_ci/lo}{-202.3}
\defres{e6f/jev_action_trigger/always/success}{87.9}
\defres{e6f/jev_action_trigger/always/success_ref}{90.7}
\defres{e6f/jev_action_trigger/always/tva_delta}{+0.7}
\defres{e6f/jev_action_trigger/broke}{23}
\defres{e6f/jev_action_trigger/changed}{7.9}
\defres{e6f/jev_action_trigger/confirmed_right}{438}
\defres{e6f/jev_action_trigger/confirmed_wrong}{888}
\defres{e6f/jev_action_trigger/cost_k}{41.4}
\defres{e6f/jev_action_trigger/cost_ref_k}{19.6}
\defres{e6f/jev_action_trigger/coverage}{100.0}
\defres{e6f/jev_action_trigger/delta}{-2.1}
\defres{e6f/jev_action_trigger/delta_ci/hi}{+2.1}
\defres{e6f/jev_action_trigger/delta_ci/lo}{-6.4}
\defres{e6f/jev_action_trigger/fig_delta}{-2.1}
\defres{e6f/jev_action_trigger/fig_saving}{-111}
\defres{e6f/jev_action_trigger/fixed}{9}
\defres{e6f/jev_action_trigger/losses}{6}
\defres{e6f/jev_action_trigger/n}{140}
\defres{e6f/jev_action_trigger/n_dropped}{0}
\defres{e6f/jev_action_trigger/n_proposals}{1920}
\defres{e6f/jev_action_trigger/n_verified}{1439}
\defres{e6f/jev_action_trigger/net_fixed}{-14}
\defres{e6f/jev_action_trigger/proposal_wrong}{59.8}
\defres{e6f/jev_action_trigger/reply_no_call}{0}
\defres{e6f/jev_action_trigger/revised_right}{0}
\defres{e6f/jev_action_trigger/revised_wrong}{81}
\defres{e6f/jev_action_trigger/right_verified}{59.7}
\defres{e6f/jev_action_trigger/saving}{-111.2}
\defres{e6f/jev_action_trigger/saving_ci/hi}{-79.6}
\defres{e6f/jev_action_trigger/saving_ci/lo}{-148.3}
\defres{e6f/jev_action_trigger/state}{exploratory}
\defres{e6f/jev_action_trigger/success}{88.6}
\defres{e6f/jev_action_trigger/success_ref}{90.7}
\defres{e6f/jev_action_trigger/tau}{0.5}
\defres{e6f/jev_action_trigger/vcode}{3}
\defres{e6f/jev_action_trigger/verdict}{no saving}
\defres{e6f/jev_action_trigger/verified}{74.9}
\defres{e6f/jev_action_trigger/wall_s}{139.0}
\defres{e6f/jev_action_trigger/wins}{3}
\defres{e6f/jev_action_trigger/wrong_verified}{85.2}
\defres{e6f/ref/alfworld/cost_k}{19.6}
\defres{e6f/ref/alfworld/n}{140}
\defres{e6f/ref/alfworld/success}{90.7}
\defres{e6f/ref/jevgym/cost_k}{42.2}
\defres{e6f/ref/jevgym/n}{100}
\defres{e6f/ref/jevgym/success}{100.0}
\defres{e6f/spend/gemini}{43.55}
\defres{e6f/spend/jev}{0.12}
\defres{e6f/tp_trigger/acc}{100.0}
\defres{e6f/tp_trigger/acted}{0.0}
\defres{e6f/tp_trigger/acted_kind}{fired}
\defres{e6f/tp_trigger/always/broke}{1}
\defres{e6f/tp_trigger/always/cost_k}{58.3}
\defres{e6f/tp_trigger/always/cost_ref_k}{42.2}
\defres{e6f/tp_trigger/always/cost_share}{3.3}
\defres{e6f/tp_trigger/always/delta}{+0.0}
\defres{e6f/tp_trigger/always/delta_ci/hi}{+0.0}
\defres{e6f/tp_trigger/always/delta_ci/lo}{+0.0}
\defres{e6f/tp_trigger/always/fig_delta}{+0.0}
\defres{e6f/tp_trigger/always/fig_saving}{-38}
\defres{e6f/tp_trigger/always/fixed}{0}
\defres{e6f/tp_trigger/always/n}{100}
\defres{e6f/tp_trigger/always/n_dropped}{0}
\defres{e6f/tp_trigger/always/n_proposals}{751}
\defres{e6f/tp_trigger/always/net_fix_share}{-0.0}
\defres{e6f/tp_trigger/always/net_fixed}{-1}
\defres{e6f/tp_trigger/always/saving}{-38.1}
\defres{e6f/tp_trigger/always/saving_ci/hi}{-35.1}
\defres{e6f/tp_trigger/always/saving_ci/lo}{-41.0}
\defres{e6f/tp_trigger/always/success}{100.0}
\defres{e6f/tp_trigger/always/success_ref}{100.0}
\defres{e6f/tp_trigger/always/tva_delta}{+0.0}
\defres{e6f/tp_trigger/broke}{0}
\defres{e6f/tp_trigger/confirmed_right}{0}
\defres{e6f/tp_trigger/confirmed_wrong}{0}
\defres{e6f/tp_trigger/cost_k}{42.7}
\defres{e6f/tp_trigger/cost_ref_k}{42.2}
\defres{e6f/tp_trigger/coverage}{100.0}
\defres{e6f/tp_trigger/delta}{+0.0}
\defres{e6f/tp_trigger/delta_ci/hi}{+0.0}
\defres{e6f/tp_trigger/delta_ci/lo}{+0.0}
\defres{e6f/tp_trigger/fig_delta}{+0.0}
\defres{e6f/tp_trigger/fig_saving}{-1}
\defres{e6f/tp_trigger/fixed}{0}
\defres{e6f/tp_trigger/losses}{0}
\defres{e6f/tp_trigger/n}{100}
\defres{e6f/tp_trigger/n_dropped}{0}
\defres{e6f/tp_trigger/n_proposals}{750}
\defres{e6f/tp_trigger/n_verified}{0}
\defres{e6f/tp_trigger/net_fixed}{0}
\defres{e6f/tp_trigger/proposal_wrong}{0.0}
\defres{e6f/tp_trigger/reply_no_call}{0}
\defres{e6f/tp_trigger/revised_right}{0}
\defres{e6f/tp_trigger/revised_wrong}{0}
\defres{e6f/tp_trigger/right_verified}{0.0}
\defres{e6f/tp_trigger/saving}{-1.2}
\defres{e6f/tp_trigger/saving_ci/hi}{0.3}
\defres{e6f/tp_trigger/saving_ci/lo}{-2.8}
\defres{e6f/tp_trigger/state}{exploratory}
\defres{e6f/tp_trigger/success}{100.0}
\defres{e6f/tp_trigger/success_ref}{100.0}
\defres{e6f/tp_trigger/tau}{0.9}
\defres{e6f/tp_trigger/vcode}{3}
\defres{e6f/tp_trigger/verdict}{no saving}
\defres{e6f/tp_trigger/verified}{0.0}
\defres{e6f/tp_trigger/wall_s}{53.2}
\defres{e6f/tp_trigger/wins}{0}
\defres{e6f/ts_trigger/acc}{86.3}
\defres{e6f/ts_trigger/acted}{13.7}
\defres{e6f/ts_trigger/acted_kind}{fired}
\defres{e6f/ts_trigger/always/broke}{0}
\defres{e6f/ts_trigger/always/cost_k}{81.2}
\defres{e6f/ts_trigger/always/cost_ref_k}{42.2}
\defres{e6f/ts_trigger/always/cost_share}{15.3}
\defres{e6f/ts_trigger/always/delta}{+0.0}
\defres{e6f/ts_trigger/always/delta_ci/hi}{+0.0}
\defres{e6f/ts_trigger/always/delta_ci/lo}{+0.0}
\defres{e6f/ts_trigger/always/fig_delta}{+0.0}
\defres{e6f/ts_trigger/always/fig_saving}{-93}
\defres{e6f/ts_trigger/always/fixed}{0}
\defres{e6f/ts_trigger/always/n}{100}
\defres{e6f/ts_trigger/always/n_dropped}{0}
\defres{e6f/ts_trigger/always/n_proposals}{750}
\defres{e6f/ts_trigger/always/net_fixed}{0}
\defres{e6f/ts_trigger/always/saving}{-92.6}
\defres{e6f/ts_trigger/always/saving_ci/hi}{-89.8}
\defres{e6f/ts_trigger/always/saving_ci/lo}{-95.5}
\defres{e6f/ts_trigger/always/success}{100.0}
\defres{e6f/ts_trigger/always/success_ref}{100.0}
\defres{e6f/ts_trigger/always/tva_delta}{+0.0}
\defres{e6f/ts_trigger/broke}{0}
\defres{e6f/ts_trigger/changed}{0.0}
\defres{e6f/ts_trigger/confirmed_right}{103}
\defres{e6f/ts_trigger/confirmed_wrong}{0}
\defres{e6f/ts_trigger/cost_k}{48.2}
\defres{e6f/ts_trigger/cost_ref_k}{42.2}
\defres{e6f/ts_trigger/coverage}{100.0}
\defres{e6f/ts_trigger/delta}{+0.0}
\defres{e6f/ts_trigger/delta_ci/hi}{+0.0}
\defres{e6f/ts_trigger/delta_ci/lo}{+0.0}
\defres{e6f/ts_trigger/fig_delta}{+0.0}
\defres{e6f/ts_trigger/fig_saving}{-14}
\defres{e6f/ts_trigger/fixed}{0}
\defres{e6f/ts_trigger/losses}{0}
\defres{e6f/ts_trigger/n}{100}
\defres{e6f/ts_trigger/n_dropped}{0}
\defres{e6f/ts_trigger/n_proposals}{750}
\defres{e6f/ts_trigger/n_verified}{103}
\defres{e6f/ts_trigger/net_fixed}{0}
\defres{e6f/ts_trigger/proposal_wrong}{0.0}
\defres{e6f/ts_trigger/reply_no_call}{0}
\defres{e6f/ts_trigger/revised_right}{0}
\defres{e6f/ts_trigger/revised_wrong}{0}
\defres{e6f/ts_trigger/right_verified}{13.7}
\defres{e6f/ts_trigger/saving}{-14.2}
\defres{e6f/ts_trigger/saving_ci/hi}{-11.3}
\defres{e6f/ts_trigger/saving_ci/lo}{-17.4}
\defres{e6f/ts_trigger/state}{exploratory}
\defres{e6f/ts_trigger/success}{100.0}
\defres{e6f/ts_trigger/success_ref}{100.0}
\defres{e6f/ts_trigger/tau}{0.5}
\defres{e6f/ts_trigger/vcode}{3}
\defres{e6f/ts_trigger/verdict}{no saving}
\defres{e6f/ts_trigger/verified}{13.7}
\defres{e6f/ts_trigger/wall_s}{58.2}
\defres{e6f/ts_trigger/wins}{0}
\makeatother


==> generated/e7_hard.tex <==
\makeatletter
\providecommand{\res}[1]{\ifcsname jevres@#1\endcsname\csname jevres@#1\endcsname\else\tbd\fi}
\providecommand{\defres}[2]{\expandafter\def\csname jevres@#1\endcsname{#2}}
\defres{e7/cap}{150}
\defres{e7/jevagent_best/acc}{99.7}
\defres{e7/jevagent_best/acc_accepted}{100.0}
\defres{e7/jevagent_best/cost_api_k}{55.7}
\defres{e7/jevagent_best/cost_k}{55.7}
\defres{e7/jevagent_best/cost_ref_k}{59.4}
\defres{e7/jevagent_best/coverage}{66.2}
\defres{e7/jevagent_best/delta}{-1.5}
\defres{e7/jevagent_best/delta_ci/hi}{+4.5}
\defres{e7/jevagent_best/delta_ci/lo}{-7.5}
\defres{e7/jevagent_best/fail/askfinish}{0}
\defres{e7/jevagent_best/fail/n}{27}
\defres{e7/jevagent_best/fail/other}{0}
\defres{e7/jevagent_best/fail/wrongtotal}{27}
\defres{e7/jevagent_best/fail/wrongwrite}{0}
\defres{e7/jevagent_best/fig_delta}{-1.5}
\defres{e7/jevagent_best/fig_saving}{6}
\defres{e7/jevagent_best/losses}{19}
\defres{e7/jevagent_best/n}{200}
\defres{e7/jevagent_best/n_dropped}{0}
\defres{e7/jevagent_best/newcombe/hi}{+4.5}
\defres{e7/jevagent_best/newcombe/lo}{-7.5}
\defres{e7/jevagent_best/op_acc}{99.7}
\defres{e7/jevagent_best/op_acc_accepted}{100.0}
\defres{e7/jevagent_best/op_accepted_wrong}{0}
\defres{e7/jevagent_best/op_coverage}{56.3}
\defres{e7/jevagent_best/op_n}{2009}
\defres{e7/jevagent_best/reflection_fired}{6.5}
\defres{e7/jevagent_best/saving}{6.2}
\defres{e7/jevagent_best/saving_api}{6.2}
\defres{e7/jevagent_best/saving_ci/hi}{8.0}
\defres{e7/jevagent_best/saving_ci/lo}{4.4}
\defres{e7/jevagent_best/state}{run}
\defres{e7/jevagent_best/success}{86.5}
\defres{e7/jevagent_best/success_ref}{88.0}
\defres{e7/jevagent_best/tool_params/acc}{99.7}
\defres{e7/jevagent_best/tool_params/acc_accepted}{100.0}
\defres{e7/jevagent_best/tool_params/coverage}{69.7}
\defres{e7/jevagent_best/tool_select/acc}{99.8}
\defres{e7/jevagent_best/tool_select/acc_accepted}{100.0}
\defres{e7/jevagent_best/tool_select/coverage}{62.5}
\defres{e7/jevagent_best/wall_mean}{47.6}
\defres{e7/jevagent_best/wall_median}{46.9}
\defres{e7/jevagent_best/wall_ref_mean}{33.1}
\defres{e7/jevagent_best/wall_ref_median}{32.5}
\defres{e7/jevagent_best/wins}{16}
\defres{e7/jevagent_best_rl/acc}{95.5}
\defres{e7/jevagent_best_rl/acc_accepted}{96.2}
\defres{e7/jevagent_best_rl/cost_api_k}{10.0}
\defres{e7/jevagent_best_rl/cost_k}{18.2}
\defres{e7/jevagent_best_rl/cost_ref_k}{59.4}
\defres{e7/jevagent_best_rl/coverage}{77.6}
\defres{e7/jevagent_best_rl/delta}{-85.0}
\defres{e7/jevagent_best_rl/delta_ci/hi}{-79.5}
\defres{e7/jevagent_best_rl/delta_ci/lo}{-90.0}
\defres{e7/jevagent_best_rl/fail/askfinish}{37}
\defres{e7/jevagent_best_rl/fail/n}{194}
\defres{e7/jevagent_best_rl/fail/other}{0}
\defres{e7/jevagent_best_rl/fail/wrongtotal}{5}
\defres{e7/jevagent_best_rl/fail/wrongwrite}{152}
\defres{e7/jevagent_best_rl/fig_delta}{-85.0}
\defres{e7/jevagent_best_rl/fig_saving}{69}
\defres{e7/jevagent_best_rl/losses}{171}
\defres{e7/jevagent_best_rl/n}{200}
\defres{e7/jevagent_best_rl/n_dropped}{0}
\defres{e7/jevagent_best_rl/newcombe/hi}{-78.7}
\defres{e7/jevagent_best_rl/newcombe/lo}{-89.2}
\defres{e7/jevagent_best_rl/op_acc}{81.6}
\defres{e7/jevagent_best_rl/op_acc_accepted}{81.7}
\defres{e7/jevagent_best_rl/op_accepted_wrong}{160}
\defres{e7/jevagent_best_rl/op_coverage}{99.9}
\defres{e7/jevagent_best_rl/op_n}{877}
\defres{e7/jevagent_best_rl/reflection_fired}{3.6}
\defres{e7/jevagent_best_rl/saving}{69.4}
\defres{e7/jevagent_best_rl/saving_api}{83.2}
\defres{e7/jevagent_best_rl/saving_ci/hi}{71.7}
\defres{e7/jevagent_best_rl/saving_ci/lo}{67.0}
\defres{e7/jevagent_best_rl/saving_q_s24}{79.9}
\defres{e7/jevagent_best_rl/saving_q_zero}{83.2}
\defres{e7/jevagent_best_rl/state}{run}
\defres{e7/jevagent_best_rl/success}{3.0}
\defres{e7/jevagent_best_rl/success_ref}{88.0}
\defres{e7/jevagent_best_rl/tool_params/acc}{97.4}
\defres{e7/jevagent_best_rl/tool_params/acc_accepted}{99.8}
\defres{e7/jevagent_best_rl/tool_params/coverage}{64.0}
\defres{e7/jevagent_best_rl/tool_select/acc}{92.6}
\defres{e7/jevagent_best_rl/tool_select/acc_accepted}{92.6}
\defres{e7/jevagent_best_rl/tool_select/coverage}{99.9}
\defres{e7/jevagent_best_rl/wall_mean}{60.5}
\defres{e7/jevagent_best_rl/wall_median}{48.0}
\defres{e7/jevagent_best_rl/wall_ref_mean}{33.1}
\defres{e7/jevagent_best_rl/wall_ref_median}{32.5}
\defres{e7/jevagent_best_rl/wins}{1}
\defres{e7/llm_only/cost_k}{59.4}
\defres{e7/llm_only/fail/askfinish}{0}
\defres{e7/llm_only/fail/n}{24}
\defres{e7/llm_only/fail/other}{0}
\defres{e7/llm_only/fail/wrongtotal}{24}
\defres{e7/llm_only/fail/wrongwrite}{0}
\defres{e7/llm_only/n}{200}
\defres{e7/llm_only/success}{88.0}
\defres{e7/llm_only/wall_mean}{33.1}
\defres{e7/llm_only/wall_median}{32.5}
\defres{e7/pilot/n}{30}
\defres{e7/pilot/success}{76.7}
\defres{e7/setting/families}{multi}
\defres{e7/setting/max_steps}{45}
\defres{e7/setting/multi_customers}{10}
\defres{e7/setting/n}{200}
\defres{e7/setting/n_distractors}{60}
\defres{e7/setting/noise_lines}{20}
\defres{e7/setting/rule}{tier}
\defres{e7/setting/seed0}{310000}
\defres{e7/spend}{43.01}
\defres{e7/spend_pilot}{17.75}
\defres{e7/tariff/host_usd_h}{2.448}
\defres{e7/tariff/q}{0.00821}
\makeatother


==> generated/e7b_hard.tex <==
\makeatletter
\providecommand{\res}[1]{\ifcsname jevres@#1\endcsname\csname jevres@#1\endcsname\else\tbd\fi}
\providecommand{\defres}[2]{\expandafter\def\csname jevres@#1\endcsname{#2}}
\defres{e7b/cap}{60}
\defres{e7b/jevagent_best/acc}{99.6}
\defres{e7b/jevagent_best/acc_accepted}{100.0}
\defres{e7b/jevagent_best/cost_api_k}{69.9}
\defres{e7b/jevagent_best/cost_k}{69.9}
\defres{e7b/jevagent_best/cost_ref_k}{73.3}
\defres{e7b/jevagent_best/coverage}{65.7}
\defres{e7b/jevagent_best/delta}{+3.5}
\defres{e7b/jevagent_best/delta_ci/hi}{+11.5}
\defres{e7b/jevagent_best/delta_ci/lo}{-4.5}
\defres{e7b/jevagent_best/fail/askfinish}{0}
\defres{e7b/jevagent_best/fail/n}{61}
\defres{e7b/jevagent_best/fail/other}{0}
\defres{e7b/jevagent_best/fail/wrongtotal}{61}
\defres{e7b/jevagent_best/fail/wrongwrite}{0}
\defres{e7b/jevagent_best/fig_delta}{+3.5}
\defres{e7b/jevagent_best/fig_saving}{5}
\defres{e7b/jevagent_best/losses}{31}
\defres{e7b/jevagent_best/n}{200}
\defres{e7b/jevagent_best/n_dropped}{0}
\defres{e7b/jevagent_best/newcombe/hi}{+11.6}
\defres{e7b/jevagent_best/newcombe/lo}{-4.7}
\defres{e7b/jevagent_best/op_acc}{99.8}
\defres{e7b/jevagent_best/op_acc_accepted}{100.0}
\defres{e7b/jevagent_best/op_accepted_wrong}{0}
\defres{e7b/jevagent_best/op_coverage}{58.1}
\defres{e7b/jevagent_best/op_n}{2411}
\defres{e7b/jevagent_best/reflection_fired}{5.6}
\defres{e7b/jevagent_best/saving}{4.6}
\defres{e7b/jevagent_best/saving_api}{4.6}
\defres{e7b/jevagent_best/saving_ci/hi}{6.1}
\defres{e7b/jevagent_best/saving_ci/lo}{3.1}
\defres{e7b/jevagent_best/state}{run}
\defres{e7b/jevagent_best/success}{69.5}
\defres{e7b/jevagent_best/success_ref}{66.0}
\defres{e7b/jevagent_best/tool_params/acc}{99.6}
\defres{e7b/jevagent_best/tool_params/acc_accepted}{100.0}
\defres{e7b/jevagent_best/tool_params/coverage}{70.5}
\defres{e7b/jevagent_best/tool_select/acc}{99.6}
\defres{e7b/jevagent_best/tool_select/acc_accepted}{100.0}
\defres{e7b/jevagent_best/tool_select/coverage}{60.4}
\defres{e7b/jevagent_best/wall_mean}{71.5}
\defres{e7b/jevagent_best/wall_median}{70.3}
\defres{e7b/jevagent_best/wall_ref_mean}{41.6}
\defres{e7b/jevagent_best/wall_ref_median}{40.6}
\defres{e7b/jevagent_best/wins}{38}
\defres{e7b/jevagent_best_rl/acc}{95.2}
\defres{e7b/jevagent_best_rl/acc_accepted}{96.2}
\defres{e7b/jevagent_best_rl/cost_api_k}{12.4}
\defres{e7b/jevagent_best_rl/cost_k}{22.3}
\defres{e7b/jevagent_best_rl/cost_ref_k}{73.3}
\defres{e7b/jevagent_best_rl/coverage}{75.7}
\defres{e7b/jevagent_best_rl/delta}{-65.5}
\defres{e7b/jevagent_best_rl/delta_ci/hi}{-59.0}
\defres{e7b/jevagent_best_rl/delta_ci/lo}{-72.0}
\defres{e7b/jevagent_best_rl/fail/askfinish}{25}
\defres{e7b/jevagent_best_rl/fail/n}{199}
\defres{e7b/jevagent_best_rl/fail/other}{0}
\defres{e7b/jevagent_best_rl/fail/wrongtotal}{5}
\defres{e7b/jevagent_best_rl/fail/wrongwrite}{169}
\defres{e7b/jevagent_best_rl/fig_delta}{-65.5}
\defres{e7b/jevagent_best_rl/fig_saving}{70}
\defres{e7b/jevagent_best_rl/losses}{131}
\defres{e7b/jevagent_best_rl/n}{200}
\defres{e7b/jevagent_best_rl/n_dropped}{0}
\defres{e7b/jevagent_best_rl/newcombe/hi}{-58.3}
\defres{e7b/jevagent_best_rl/newcombe/lo}{-71.7}
\defres{e7b/jevagent_best_rl/op_acc}{81.5}
\defres{e7b/jevagent_best_rl/op_acc_accepted}{81.5}
\defres{e7b/jevagent_best_rl/op_accepted_wrong}{177}
\defres{e7b/jevagent_best_rl/op_coverage}{100.0}
\defres{e7b/jevagent_best_rl/op_n}{957}
\defres{e7b/jevagent_best_rl/reflection_fired}{3.5}
\defres{e7b/jevagent_best_rl/saving}{69.5}
\defres{e7b/jevagent_best_rl/saving_api}{83.1}
\defres{e7b/jevagent_best_rl/saving_ci/hi}{72.2}
\defres{e7b/jevagent_best_rl/saving_ci/lo}{66.8}
\defres{e7b/jevagent_best_rl/saving_q_s24}{80.4}
\defres{e7b/jevagent_best_rl/saving_q_zero}{83.1}
\defres{e7b/jevagent_best_rl/state}{run}
\defres{e7b/jevagent_best_rl/success}{0.5}
\defres{e7b/jevagent_best_rl/success_ref}{66.0}
\defres{e7b/jevagent_best_rl/tool_params/acc}{96.9}
\defres{e7b/jevagent_best_rl/tool_params/acc_accepted}{100.0}
\defres{e7b/jevagent_best_rl/tool_params/coverage}{61.0}
\defres{e7b/jevagent_best_rl/tool_select/acc}{92.6}
\defres{e7b/jevagent_best_rl/tool_select/acc_accepted}{92.6}
\defres{e7b/jevagent_best_rl/tool_select/coverage}{100.0}
\defres{e7b/jevagent_best_rl/wall_mean}{59.3}
\defres{e7b/jevagent_best_rl/wall_median}{38.7}
\defres{e7b/jevagent_best_rl/wall_ref_mean}{41.6}
\defres{e7b/jevagent_best_rl/wall_ref_median}{40.6}
\defres{e7b/jevagent_best_rl/wins}{0}
\defres{e7b/lat/jevagentbest/extra}{29.9}
\defres{e7b/lat/jevagentbest/extratail}{8.2}
\defres{e7b/lat/jevagentbest/s1}{22.5}
\defres{e7b/lat/jevagentbest/s2}{45.6}
\defres{e7b/lat/jevagentbest/s2-reflection-Google/n}{406}
\defres{e7b/lat/jevagentbest/s2-reflection-Google/over}{4}
\defres{e7b/lat/jevagentbest/s2-reflection-Google/p50}{1.36}
\defres{e7b/lat/jevagentbest/s2-reflection-Google/p90}{1.59}
\defres{e7b/lat/jevagentbest/s2-reflection-Google/tailshare}{0.4}
\defres{e7b/lat/jevagentbest/s2-toolparams-1tool-Google/n}{2216}
\defres{e7b/lat/jevagentbest/s2-toolparams-1tool-Google/over}{230}
\defres{e7b/lat/jevagentbest/s2-toolparams-1tool-Google/p50}{1.31}
\defres{e7b/lat/jevagentbest/s2-toolparams-1tool-Google/p90}{5.10}
\defres{e7b/lat/jevagentbest/s2-toolparams-1tool-Google/tailshare}{10.9}
\defres{e7b/lat/jevagentbest/s2-toolparams-1tool-GoogleAIStudio/n}{9}
\defres{e7b/lat/jevagentbest/s2-toolparams-1tool-GoogleAIStudio/over}{9}
\defres{e7b/lat/jevagentbest/s2-toolparams-1tool-GoogleAIStudio/p50}{11.98}
\defres{e7b/lat/jevagentbest/s2-toolparams-1tool-GoogleAIStudio/p90}{12.53}
\defres{e7b/lat/jevagentbest/s2-toolparams-1tool-GoogleAIStudio/tailshare}{0.8}
\defres{e7b/lat/jevagentbest/s2-toolselect-Google/n}{2928}
\defres{e7b/lat/jevagentbest/s2-toolselect-Google/over}{6}
\defres{e7b/lat/jevagentbest/s2-toolselect-Google/p50}{0.98}
\defres{e7b/lat/jevagentbest/s2-toolselect-Google/p90}{1.30}
\defres{e7b/lat/jevagentbest/s2-toolselect-Google/tailshare}{0.4}
\defres{e7b/lat/jevagentbest/s2tail}{9.0}
\defres{e7b/lat/jevagentbest/tailshareofextra}{27}
\defres{e7b/lat/jevagentbest/wall}{71.5}
\defres{e7b/lat/jevagentbestrl/extra}{17.7}
\defres{e7b/lat/jevagentbestrl/extratail}{6.0}
\defres{e7b/lat/jevagentbestrl/s1}{39.8}
\defres{e7b/lat/jevagentbestrl/s2}{17.9}
\defres{e7b/lat/jevagentbestrl/s2-reflection-Google/n}{95}
\defres{e7b/lat/jevagentbestrl/s2-reflection-Google/over}{0}
\defres{e7b/lat/jevagentbestrl/s2-reflection-Google/p50}{1.56}
\defres{e7b/lat/jevagentbestrl/s2-reflection-Google/p90}{1.77}
\defres{e7b/lat/jevagentbestrl/s2-reflection-Google/tailshare}{0.0}
\defres{e7b/lat/jevagentbestrl/s2-toolparams-1tool-Google/n}{1364}
\defres{e7b/lat/jevagentbestrl/s2-toolparams-1tool-Google/over}{181}
\defres{e7b/lat/jevagentbestrl/s2-toolparams-1tool-Google/p50}{1.32}
\defres{e7b/lat/jevagentbestrl/s2-toolparams-1tool-Google/p90}{5.54}
\defres{e7b/lat/jevagentbestrl/s2-toolparams-1tool-Google/tailshare}{10.7}
\defres{e7b/lat/jevagentbestrl/s2-toolparams-1tool-GoogleAIStudio/n}{7}
\defres{e7b/lat/jevagentbestrl/s2-toolparams-1tool-GoogleAIStudio/over}{7}
\defres{e7b/lat/jevagentbestrl/s2-toolparams-1tool-GoogleAIStudio/p50}{11.84}
\defres{e7b/lat/jevagentbestrl/s2-toolparams-1tool-GoogleAIStudio/p90}{15.07}
\defres{e7b/lat/jevagentbestrl/s2-toolparams-1tool-GoogleAIStudio/tailshare}{0.8}
\defres{e7b/lat/jevagentbestrl/s2tail}{6.8}
\defres{e7b/lat/jevagentbestrl/tailshareofextra}{34}
\defres{e7b/lat/jevagentbestrl/wall}{59.3}
\defres{e7b/lat/llmonly/s1}{0.0}
\defres{e7b/lat/llmonly/s2}{38.9}
\defres{e7b/lat/llmonly/s2-toolselect-Google/n}{7397}
\defres{e7b/lat/llmonly/s2-toolselect-Google/over}{17}
\defres{e7b/lat/llmonly/s2-toolselect-Google/p50}{0.97}
\defres{e7b/lat/llmonly/s2-toolselect-Google/p90}{1.18}
\defres{e7b/lat/llmonly/s2-toolselect-Google/tailshare}{1.2}
\defres{e7b/lat/llmonly/s2-toolselect-GoogleAIStudio/n}{3}
\defres{e7b/lat/llmonly/s2-toolselect-GoogleAIStudio/over}{3}
\defres{e7b/lat/llmonly/s2-toolselect-GoogleAIStudio/p50}{17.77}
\defres{e7b/lat/llmonly/s2-toolselect-GoogleAIStudio/p90}{18.50}
\defres{e7b/lat/llmonly/s2-toolselect-GoogleAIStudio/tailshare}{0.6}
\defres{e7b/lat/llmonly/s2tail}{0.8}
\defres{e7b/lat/llmonly/wall}{41.6}
\defres{e7b/llm_only/cost_k}{73.3}
\defres{e7b/llm_only/fail/askfinish}{0}
\defres{e7b/llm_only/fail/n}{68}
\defres{e7b/llm_only/fail/other}{0}
\defres{e7b/llm_only/fail/wrongtotal}{68}
\defres{e7b/llm_only/fail/wrongwrite}{0}
\defres{e7b/llm_only/n}{200}
\defres{e7b/llm_only/success}{66.0}
\defres{e7b/llm_only/wall_mean}{41.6}
\defres{e7b/llm_only/wall_median}{40.6}
\defres{e7b/pilot/n}{60}
\defres{e7b/pilot/success}{46.7}
\defres{e7b/setting/families}{multi}
\defres{e7b/setting/max_steps}{45}
\defres{e7b/setting/multi_customers}{12}
\defres{e7b/setting/n}{200}
\defres{e7b/setting/n_distractors}{60}
\defres{e7b/setting/noise_lines}{20}
\defres{e7b/setting/rule}{tier}
\defres{e7b/setting/seed0}{310200}
\defres{e7b/spend}{31.47}
\defres{e7b/tariff/host_usd_h}{2.448}
\defres{e7b/tariff/q}{0.00992}
\makeatother


==> generated/e7c_cal.tex <==
\makeatletter
\providecommand{\res}[1]{\ifcsname jevres@#1\endcsname\csname jevres@#1\endcsname\else\tbd\fi}
\providecommand{\defres}[2]{\expandafter\def\csname jevres@#1\endcsname{#2}}
\defres{e7c/cal/jev/errored}{0}
\defres{e7c/cal/jev/ntasks}{100}
\defres{e7c/cal/jev/op/coverage}{99.5}
\defres{e7c/cal/jev/op/llmaccall}{100.0}
\defres{e7c/cal/jev/op/llmacctaken}{100.0}
\defres{e7c/cal/jev/op/n}{1200}
\defres{e7c/cal/jev/op/s1accall}{100.0}
\defres{e7c/cal/jev/op/s1acctaken}{100.0}
\defres{e7c/cal/jev/op/tau}{0.91}
\defres{e7c/cal/jev/toolparams/coverage}{80.2}
\defres{e7c/cal/jev/toolparams/llmaccall}{100.0}
\defres{e7c/cal/jev/toolparams/llmacctaken}{100.0}
\defres{e7c/cal/jev/toolparams/n}{5998}
\defres{e7c/cal/jev/toolparams/s1accall}{97.4}
\defres{e7c/cal/jev/toolparams/s1acctaken}{100.0}
\defres{e7c/cal/jev/toolparams/tau}{0.87}
\defres{e7c/cal/jev/toolselect/coverage}{90.1}
\defres{e7c/cal/jev/toolselect/llmaccall}{100.0}
\defres{e7c/cal/jev/toolselect/llmacctaken}{100.0}
\defres{e7c/cal/jev/toolselect/n}{3699}
\defres{e7c/cal/jev/toolselect/s1accall}{99.8}
\defres{e7c/cal/jev/toolselect/s1acctaken}{100.0}
\defres{e7c/cal/jev/toolselect/tau}{0.91}
\defres{e7c/cal/rl4b/errored}{9}
\defres{e7c/cal/rl4b/ntasks}{100}
\defres{e7c/cal/rl4b/op/coverage}{0.0}
\defres{e7c/cal/rl4b/op/llmaccall}{100.0}
\defres{e7c/cal/rl4b/op/llmacctaken}{--}
\defres{e7c/cal/rl4b/op/n}{1153}
\defres{e7c/cal/rl4b/op/s1accall}{81.1}
\defres{e7c/cal/rl4b/op/s1acctaken}{--}
\defres{e7c/cal/rl4b/op/tau}{always defer}
\defres{e7c/cal/rl4b/toolparams/coverage}{62.9}
\defres{e7c/cal/rl4b/toolparams/llmaccall}{100.0}
\defres{e7c/cal/rl4b/toolparams/llmacctaken}{100.0}
\defres{e7c/cal/rl4b/toolparams/n}{5781}
\defres{e7c/cal/rl4b/toolparams/s1accall}{94.8}
\defres{e7c/cal/rl4b/toolparams/s1acctaken}{100.0}
\defres{e7c/cal/rl4b/toolparams/tau}{1}
\defres{e7c/cal/rl4b/toolselect/coverage}{0.0}
\defres{e7c/cal/rl4b/toolselect/llmaccall}{100.0}
\defres{e7c/cal/rl4b/toolselect/llmacctaken}{--}
\defres{e7c/cal/rl4b/toolselect/n}{3561}
\defres{e7c/cal/rl4b/toolselect/s1accall}{86.5}
\defres{e7c/cal/rl4b/toolselect/s1acctaken}{--}
\defres{e7c/cal/rl4b/toolselect/tau}{always defer}
\defres{e7c/cal/seeds}{5300--5399}
\defres{e7c/cal/spend}{14.97}
\makeatother


==> generated/e7c_hard.tex <==
\makeatletter
\providecommand{\res}[1]{\ifcsname jevres@#1\endcsname\csname jevres@#1\endcsname\else\tbd\fi}
\providecommand{\defres}[2]{\expandafter\def\csname jevres@#1\endcsname{#2}}
\defres{e7c/cal/jevrefit/toolparams/coverage}{80.2}
\defres{e7c/cal/jevrefit/toolparams/tau}{0.87}
\defres{e7c/cal/jevrefit/toolselect/coverage}{90.1}
\defres{e7c/cal/jevrefit/toolselect/tau}{0.91}
\defres{e7c/cal/rlrefit/toolparams/coverage}{62.9}
\defres{e7c/cal/rlrefit/toolparams/tau}{1}
\defres{e7c/cal/rlrefit/toolselect/coverage}{0.0}
\defres{e7c/cal/rlrefit/toolselect/tau}{always defer}
\defres{e7c/cap}{90}
\defres{e7c/jev_refit/acc}{97.8}
\defres{e7c/jev_refit/acc_accepted}{99.5}
\defres{e7c/jev_refit/cost_api_k}{181.4}
\defres{e7c/jev_refit/cost_k}{181.4}
\defres{e7c/jev_refit/cost_ref_k}{262.9}
\defres{e7c/jev_refit/coverage}{76.6}
\defres{e7c/jev_refit/delta}{-23.0}
\defres{e7c/jev_refit/delta_ci/hi}{-11.0}
\defres{e7c/jev_refit/delta_ci/lo}{-35.0}
\defres{e7c/jev_refit/fail/askfinish}{0}
\defres{e7c/jev_refit/fail/n}{81}
\defres{e7c/jev_refit/fail/other}{0}
\defres{e7c/jev_refit/fail/wrongtotal}{81}
\defres{e7c/jev_refit/fail/wrongwrite}{0}
\defres{e7c/jev_refit/fig_delta}{-23.0}
\defres{e7c/jev_refit/fig_saving}{31}
\defres{e7c/jev_refit/form/itemized/n}{26}
\defres{e7c/jev_refit/form/itemized/share}{26.0}
\defres{e7c/jev_refit/form/itemized/success}{61.5}
\defres{e7c/jev_refit/form/none/n}{0}
\defres{e7c/jev_refit/form/none/share}{0.0}
\defres{e7c/jev_refit/form/number/n}{74}
\defres{e7c/jev_refit/form/number/share}{74.0}
\defres{e7c/jev_refit/form/number/success}{4.1}
\defres{e7c/jev_refit/form/sentence/n}{0}
\defres{e7c/jev_refit/form/sentence/share}{0.0}
\defres{e7c/jev_refit/losses}{34}
\defres{e7c/jev_refit/n}{100}
\defres{e7c/jev_refit/n_dropped}{0}
\defres{e7c/jev_refit/newcombe/hi}{-10.3}
\defres{e7c/jev_refit/newcombe/lo}{-34.7}
\defres{e7c/jev_refit/op_acc}{99.9}
\defres{e7c/jev_refit/op_acc_accepted}{100.0}
\defres{e7c/jev_refit/op_accepted_wrong}{0}
\defres{e7c/jev_refit/op_coverage}{99.3}
\defres{e7c/jev_refit/op_n}{1200}
\defres{e7c/jev_refit/reflection_fired}{5.3}
\defres{e7c/jev_refit/saving}{31.0}
\defres{e7c/jev_refit/saving_api}{31.0}
\defres{e7c/jev_refit/saving_ci/hi}{31.7}
\defres{e7c/jev_refit/saving_ci/lo}{30.3}
\defres{e7c/jev_refit/state}{run}
\defres{e7c/jev_refit/success}{19.0}
\defres{e7c/jev_refit/success_ref}{42.0}
\defres{e7c/jev_refit/tool_params/acc}{97.0}
\defres{e7c/jev_refit/tool_params/acc_accepted}{99.5}
\defres{e7c/jev_refit/tool_params/coverage}{64.1}
\defres{e7c/jev_refit/tool_select/acc}{99.1}
\defres{e7c/jev_refit/tool_select/acc_accepted}{99.4}
\defres{e7c/jev_refit/tool_select/coverage}{96.7}
\defres{e7c/jev_refit/wall_mean}{118.3}
\defres{e7c/jev_refit/wall_median}{114.4}
\defres{e7c/jev_refit/wall_ref_mean}{66.6}
\defres{e7c/jev_refit/wall_ref_median}{64.9}
\defres{e7c/jev_refit/wins}{11}
\defres{e7c/lat/jevrefit/extra}{51.7}
\defres{e7c/lat/jevrefit/extratail}{21.7}
\defres{e7c/lat/jevrefit/s1}{37.9}
\defres{e7c/lat/jevrefit/s2}{64.1}
\defres{e7c/lat/jevrefit/s2-reflection-gemini/n}{193}
\defres{e7c/lat/jevrefit/s2-reflection-gemini/over}{33}
\defres{e7c/lat/jevrefit/s2-reflection-gemini/p50}{1.40}
\defres{e7c/lat/jevrefit/s2-reflection-gemini/p90}{8.19}
\defres{e7c/lat/jevrefit/s2-reflection-gemini/tailshare}{2.8}
\defres{e7c/lat/jevrefit/s2-toolparams-1tool-gemini/n}{2205}
\defres{e7c/lat/jevrefit/s2-toolparams-1tool-gemini/over}{345}
\defres{e7c/lat/jevrefit/s2-toolparams-1tool-gemini/p50}{1.05}
\defres{e7c/lat/jevrefit/s2-toolparams-1tool-gemini/p90}{6.97}
\defres{e7c/lat/jevrefit/s2-toolparams-1tool-gemini/tailshare}{25.5}
\defres{e7c/lat/jevrefit/s2-toolselect-gemini/n}{125}
\defres{e7c/lat/jevrefit/s2-toolselect-gemini/over}{21}
\defres{e7c/lat/jevrefit/s2-toolselect-gemini/p50}{1.45}
\defres{e7c/lat/jevrefit/s2-toolselect-gemini/p90}{8.72}
\defres{e7c/lat/jevrefit/s2-toolselect-gemini/tailshare}{2.0}
\defres{e7c/lat/jevrefit/s2tail}{35.9}
\defres{e7c/lat/jevrefit/tailshareofextra}{42}
\defres{e7c/lat/jevrefit/wall}{118.3}
\defres{e7c/lat/llmonly/s1}{0.0}
\defres{e7c/lat/llmonly/s2}{62.0}
\defres{e7c/lat/llmonly/s2-toolselect-gemini/n}{3700}
\defres{e7c/lat/llmonly/s2-toolselect-gemini/over}{147}
\defres{e7c/lat/llmonly/s2-toolselect-gemini/p50}{1.20}
\defres{e7c/lat/llmonly/s2-toolselect-gemini/p90}{2.34}
\defres{e7c/lat/llmonly/s2-toolselect-gemini/tailshare}{21.3}
\defres{e7c/lat/llmonly/s2tail}{14.2}
\defres{e7c/lat/llmonly/wall}{66.6}
\defres{e7c/llm_only/cost_k}{262.9}
\defres{e7c/llm_only/fail/askfinish}{0}
\defres{e7c/llm_only/fail/n}{58}
\defres{e7c/llm_only/fail/other}{0}
\defres{e7c/llm_only/fail/wrongtotal}{58}
\defres{e7c/llm_only/fail/wrongwrite}{0}
\defres{e7c/llm_only/form/itemized/n}{51}
\defres{e7c/llm_only/form/itemized/share}{51.0}
\defres{e7c/llm_only/form/itemized/success}{82.4}
\defres{e7c/llm_only/form/none/n}{0}
\defres{e7c/llm_only/form/none/share}{0.0}
\defres{e7c/llm_only/form/number/n}{31}
\defres{e7c/llm_only/form/number/share}{31.0}
\defres{e7c/llm_only/form/number/success}{0.0}
\defres{e7c/llm_only/form/sentence/n}{18}
\defres{e7c/llm_only/form/sentence/share}{18.0}
\defres{e7c/llm_only/form/sentence/success}{0.0}
\defres{e7c/llm_only/n}{100}
\defres{e7c/llm_only/success}{42.0}
\defres{e7c/llm_only/wall_mean}{66.6}
\defres{e7c/llm_only/wall_median}{64.9}
\defres{e7c/pilot/n}{60}
\defres{e7c/pilot/success}{46.7}
\defres{e7c/rl_refit/state}{not run}
\defres{e7c/route}{gemini}
\defres{e7c/setting/families}{multi}
\defres{e7c/setting/max_steps}{45}
\defres{e7c/setting/multi_customers}{12}
\defres{e7c/setting/n}{100}
\defres{e7c/setting/n_distractors}{60}
\defres{e7c/setting/noise_lines}{20}
\defres{e7c/setting/rule}{tier}
\defres{e7c/setting/seed0}{310400}
\defres{e7c/spend}{0.00}
\makeatother


==> generated/e7d_tier.tex <==
\makeatletter
\providecommand{\res}[1]{\ifcsname jevres@#1\endcsname\csname jevres@#1\endcsname\else\tbd\fi}
\providecommand{\defres}[2]{\expandafter\def\csname jevres@#1\endcsname{#2}}
\defres{e7d/c/delta}{-0.1}
\defres{e7d/c/delta_ci/hi}{+0.1}
\defres{e7d/c/delta_ci/lo}{-0.4}
\defres{e7d/cal/ntasks}{20}
\defres{e7d/check/toolparams/agree}{100.0}
\defres{e7d/check/toolparams/n}{300}
\defres{e7d/check/toolselect/agree}{100.0}
\defres{e7d/check/toolselect/n}{185}
\defres{e7d/frozen/c/acc}{99.2}
\defres{e7d/frozen/cal/op/coverage}{0.0}
\defres{e7d/frozen/cal/op/s1accall}{79.2}
\defres{e7d/frozen/cal/toolparams/coverage}{70.1}
\defres{e7d/frozen/cal/toolparams/s1accall}{94.8}
\defres{e7d/frozen/cal/toolparams/s1acctaken}{100.0}
\defres{e7d/frozen/cal/toolparams/tau}{1}
\defres{e7d/frozen/cal/toolselect/coverage}{0.0}
\defres{e7d/frozen/cal/toolselect/s1accall}{85.8}
\defres{e7d/frozen/cal/toolselect/s1acctaken}{--}
\defres{e7d/frozen/cal/toolselect/tau}{always defer}
\defres{e7d/frozen/heldout/op/acc}{76.5}
\defres{e7d/frozen/heldout/op/n}{600}
\defres{e7d/frozen/heldout/tp/acc}{95.1}
\defres{e7d/frozen/heldout/tp/n}{225}
\defres{e7d/frozen/heldout/tsother/acc}{91.6}
\defres{e7d/frozen/heldout/tsother/n}{225}
\defres{e7d/frozen/v1/acc}{99.7}
\defres{e7d/tier/c/acc}{99.1}
\defres{e7d/tier/cal/op/coverage}{42.1}
\defres{e7d/tier/cal/op/s1accall}{96.7}
\defres{e7d/tier/cal/toolparams/coverage}{90.0}
\defres{e7d/tier/cal/toolparams/s1accall}{99.4}
\defres{e7d/tier/cal/toolparams/s1acctaken}{100.0}
\defres{e7d/tier/cal/toolparams/tau}{0.9929}
\defres{e7d/tier/cal/toolselect/coverage}{50.0}
\defres{e7d/tier/cal/toolselect/s1accall}{98.5}
\defres{e7d/tier/cal/toolselect/s1acctaken}{100.0}
\defres{e7d/tier/cal/toolselect/tau}{0.9999}
\defres{e7d/tier/heldout/op/acc}{95.3}
\defres{e7d/tier/heldout/op/n}{600}
\defres{e7d/tier/heldout/tp/acc}{98.2}
\defres{e7d/tier/heldout/tp/n}{225}
\defres{e7d/tier/heldout/tsother/acc}{100.0}
\defres{e7d/tier/heldout/tsother/n}{225}
\makeatother


==> generated/e7e_hard.tex <==
\makeatletter
\providecommand{\res}[1]{\ifcsname jevres@#1\endcsname\csname jevres@#1\endcsname\else\tbd\fi}
\providecommand{\defres}[2]{\expandafter\def\csname jevres@#1\endcsname{#2}}
\defres{e7e/cap}{60}
\defres{e7e/jev_refit/acc}{97.5}
\defres{e7e/jev_refit/acc_accepted}{99.2}
\defres{e7e/jev_refit/cost_api_k}{183.8}
\defres{e7e/jev_refit/cost_k}{183.8}
\defres{e7e/jev_refit/cost_ref_k}{264.6}
\defres{e7e/jev_refit/coverage}{76.5}
\defres{e7e/jev_refit/delta}{+2.0}
\defres{e7e/jev_refit/delta_ci/hi}{+10.0}
\defres{e7e/jev_refit/delta_ci/lo}{-6.0}
\defres{e7e/jev_refit/fail/askfinish}{0}
\defres{e7e/jev_refit/fail/n}{11}
\defres{e7e/jev_refit/fail/other}{0}
\defres{e7e/jev_refit/fail/wrongtotal}{11}
\defres{e7e/jev_refit/fail/wrongwrite}{0}
\defres{e7e/jev_refit/fig_delta}{+2.0}
\defres{e7e/jev_refit/fig_saving}{31}
\defres{e7e/jev_refit/form/itemized/n}{100}
\defres{e7e/jev_refit/form/itemized/share}{100.0}
\defres{e7e/jev_refit/form/itemized/success}{89.0}
\defres{e7e/jev_refit/form/none/n}{0}
\defres{e7e/jev_refit/form/none/share}{0.0}
\defres{e7e/jev_refit/form/number/n}{0}
\defres{e7e/jev_refit/form/number/share}{0.0}
\defres{e7e/jev_refit/form/sentence/n}{0}
\defres{e7e/jev_refit/form/sentence/share}{0.0}
\defres{e7e/jev_refit/losses}{7}
\defres{e7e/jev_refit/n}{100}
\defres{e7e/jev_refit/n_dropped}{0}
\defres{e7e/jev_refit/newcombe/hi}{+10.4}
\defres{e7e/jev_refit/newcombe/lo}{-6.4}
\defres{e7e/jev_refit/op_acc}{100.0}
\defres{e7e/jev_refit/op_acc_accepted}{100.0}
\defres{e7e/jev_refit/op_accepted_wrong}{0}
\defres{e7e/jev_refit/op_coverage}{99.6}
\defres{e7e/jev_refit/op_n}{1200}
\defres{e7e/jev_refit/reflection_fired}{4.9}
\defres{e7e/jev_refit/saving}{30.5}
\defres{e7e/jev_refit/saving_api}{30.5}
\defres{e7e/jev_refit/saving_ci/hi}{31.3}
\defres{e7e/jev_refit/saving_ci/lo}{29.8}
\defres{e7e/jev_refit/state}{run}
\defres{e7e/jev_refit/success}{89.0}
\defres{e7e/jev_refit/success_ref}{87.0}
\defres{e7e/jev_refit/tool_params/acc}{96.7}
\defres{e7e/jev_refit/tool_params/acc_accepted}{99.3}
\defres{e7e/jev_refit/tool_params/coverage}{64.0}
\defres{e7e/jev_refit/tool_select/acc}{98.8}
\defres{e7e/jev_refit/tool_select/acc_accepted}{99.2}
\defres{e7e/jev_refit/tool_select/coverage}{96.3}
\defres{e7e/jev_refit/wall_mean}{104.1}
\defres{e7e/jev_refit/wall_median}{103.6}
\defres{e7e/jev_refit/wall_ref_mean}{63.5}
\defres{e7e/jev_refit/wall_ref_median}{63.2}
\defres{e7e/jev_refit/wins}{9}
\defres{e7e/lat/jevrefit/extra}{40.6}
\defres{e7e/lat/jevrefit/extratail}{11.4}
\defres{e7e/lat/jevrefit/s1}{35.7}
\defres{e7e/lat/jevrefit/s2}{56.5}
\defres{e7e/lat/jevrefit/s2-reflection-gemini/n}{178}
\defres{e7e/lat/jevrefit/s2-reflection-gemini/over}{21}
\defres{e7e/lat/jevrefit/s2-reflection-gemini/p50}{1.31}
\defres{e7e/lat/jevrefit/s2-reflection-gemini/p90}{5.95}
\defres{e7e/lat/jevrefit/s2-reflection-gemini/tailshare}{2.1}
\defres{e7e/lat/jevrefit/s2-toolparams-1tool-gemini/n}{2217}
\defres{e7e/lat/jevrefit/s2-toolparams-1tool-gemini/over}{289}
\defres{e7e/lat/jevrefit/s2-toolparams-1tool-gemini/p50}{0.97}
\defres{e7e/lat/jevrefit/s2-toolparams-1tool-gemini/p90}{6.18}
\defres{e7e/lat/jevrefit/s2-toolparams-1tool-gemini/tailshare}{22.7}
\defres{e7e/lat/jevrefit/s2-toolselect-gemini/n}{138}
\defres{e7e/lat/jevrefit/s2-toolselect-gemini/over}{17}
\defres{e7e/lat/jevrefit/s2-toolselect-gemini/p50}{1.31}
\defres{e7e/lat/jevrefit/s2-toolselect-gemini/p90}{5.71}
\defres{e7e/lat/jevrefit/s2-toolselect-gemini/tailshare}{2.0}
\defres{e7e/lat/jevrefit/s2tail}{27.9}
\defres{e7e/lat/jevrefit/tailshareofextra}{28}
\defres{e7e/lat/jevrefit/wall}{104.1}
\defres{e7e/lat/llmonly/s1}{0.0}
\defres{e7e/lat/llmonly/s2}{59.2}
\defres{e7e/lat/llmonly/s2-toolselect-gemini/n}{3700}
\defres{e7e/lat/llmonly/s2-toolselect-gemini/over}{175}
\defres{e7e/lat/llmonly/s2-toolselect-gemini/p50}{1.07}
\defres{e7e/lat/llmonly/s2-toolselect-gemini/p90}{2.03}
\defres{e7e/lat/llmonly/s2-toolselect-gemini/tailshare}{26.0}
\defres{e7e/lat/llmonly/s2tail}{16.5}
\defres{e7e/lat/llmonly/wall}{63.5}
\defres{e7e/llm_only/cost_k}{264.6}
\defres{e7e/llm_only/fail/askfinish}{0}
\defres{e7e/llm_only/fail/n}{13}
\defres{e7e/llm_only/fail/other}{0}
\defres{e7e/llm_only/fail/wrongtotal}{13}
\defres{e7e/llm_only/fail/wrongwrite}{0}
\defres{e7e/llm_only/form/itemized/n}{100}
\defres{e7e/llm_only/form/itemized/share}{100.0}
\defres{e7e/llm_only/form/itemized/success}{87.0}
\defres{e7e/llm_only/form/none/n}{0}
\defres{e7e/llm_only/form/none/share}{0.0}
\defres{e7e/llm_only/form/number/n}{0}
\defres{e7e/llm_only/form/number/share}{0.0}
\defres{e7e/llm_only/form/sentence/n}{0}
\defres{e7e/llm_only/form/sentence/share}{0.0}
\defres{e7e/llm_only/n}{100}
\defres{e7e/llm_only/success}{87.0}
\defres{e7e/llm_only/wall_mean}{63.5}
\defres{e7e/llm_only/wall_median}{63.2}
\defres{e7e/pilot/n}{60}
\defres{e7e/pilot/success}{46.7}
\defres{e7e/rl_refit/state}{not run}
\defres{e7e/route}{gemini}
\defres{e7e/setting/families}{multi}
\defres{e7e/setting/max_steps}{45}
\defres{e7e/setting/multi_customers}{12}
\defres{e7e/setting/n}{100}
\defres{e7e/setting/n_distractors}{60}
\defres{e7e/setting/noise_lines}{20}
\defres{e7e/setting/rule}{tier}
\defres{e7e/setting/seed0}{310500}
\defres{e7e/spend}{45.75}
\makeatother


==> generated/e7f_hard.tex <==
\makeatletter
\providecommand{\res}[1]{\ifcsname jevres@#1\endcsname\csname jevres@#1\endcsname\else\tbd\fi}
\providecommand{\defres}[2]{\expandafter\def\csname jevres@#1\endcsname{#2}}
\defres{e7f/cap}{115}
\defres{e7f/ext/llm_only/success}{87.5}
\defres{e7f/ext/llm_only/wall_mean}{84.7}
\defres{e7f/ext/n}{120}
\defres{e7f/ext/rl_tier/cost_k}{251.7}
\defres{e7f/ext/rl_tier/cost_ref_k}{264.6}
\defres{e7f/ext/rl_tier/delta}{-2.5}
\defres{e7f/ext/rl_tier/delta_ci/hi}{+5.8}
\defres{e7f/ext/rl_tier/delta_ci/lo}{-10.8}
\defres{e7f/ext/rl_tier/fig_delta}{-2.5}
\defres{e7f/ext/rl_tier/fig_saving}{5}
\defres{e7f/ext/rl_tier/losses}{15}
\defres{e7f/ext/rl_tier/n}{120}
\defres{e7f/ext/rl_tier/n_dropped}{0}
\defres{e7f/ext/rl_tier/saving}{4.9}
\defres{e7f/ext/rl_tier/saving_ci/hi}{7.9}
\defres{e7f/ext/rl_tier/saving_ci/lo}{1.9}
\defres{e7f/ext/rl_tier/success}{85.0}
\defres{e7f/ext/rl_tier/success_ref}{87.5}
\defres{e7f/ext/rl_tier/wall_mean}{321.3}
\defres{e7f/ext/rl_tier/wins}{12}
\defres{e7f/ext/seed0}{310680}
\defres{e7f/ext/spend}{59.14}
\defres{e7f/first/llm_only/success}{77.5}
\defres{e7f/first/llm_only/wall_mean}{58.4}
\defres{e7f/first/n}{80}
\defres{e7f/first/rl_tier/cost_k}{254.9}
\defres{e7f/first/rl_tier/cost_ref_k}{263.9}
\defres{e7f/first/rl_tier/delta}{-1.2}
\defres{e7f/first/rl_tier/delta_ci/hi}{+8.8}
\defres{e7f/first/rl_tier/delta_ci/lo}{-12.5}
\defres{e7f/first/rl_tier/fig_delta}{-1.2}
\defres{e7f/first/rl_tier/fig_saving}{3}
\defres{e7f/first/rl_tier/losses}{10}
\defres{e7f/first/rl_tier/n}{80}
\defres{e7f/first/rl_tier/n_dropped}{0}
\defres{e7f/first/rl_tier/saving}{3.4}
\defres{e7f/first/rl_tier/saving_ci/hi}{6.9}
\defres{e7f/first/rl_tier/saving_ci/lo}{0.0}
\defres{e7f/first/rl_tier/success}{76.2}
\defres{e7f/first/rl_tier/success_ref}{77.5}
\defres{e7f/first/rl_tier/wall_mean}{336.0}
\defres{e7f/first/rl_tier/wins}{9}
\defres{e7f/first/seed0}{310600}
\defres{e7f/first/spend}{39.64}
\defres{e7f/lat/llmonly/s1}{0.0}
\defres{e7f/lat/llmonly/s2}{70.7}
\defres{e7f/lat/llmonly/s2-toolselect-gemini/n}{7401}
\defres{e7f/lat/llmonly/s2-toolselect-gemini/over}{565}
\defres{e7f/lat/llmonly/s2-toolselect-gemini/p50}{1.15}
\defres{e7f/lat/llmonly/s2-toolselect-gemini/p90}{4.02}
\defres{e7f/lat/llmonly/s2-toolselect-gemini/tailshare}{30.9}
\defres{e7f/lat/llmonly/s2tail}{22.9}
\defres{e7f/lat/llmonly/wall}{74.2}
\defres{e7f/lat/rltier/extra}{253.0}
\defres{e7f/lat/rltier/extratail}{22.9}
\defres{e7f/lat/rltier/s1}{232.3}
\defres{e7f/lat/rltier/s2}{86.0}
\defres{e7f/lat/rltier/s2-reflection-gemini/n}{669}
\defres{e7f/lat/rltier/s2-reflection-gemini/over}{170}
\defres{e7f/lat/rltier/s2-reflection-gemini/p50}{1.65}
\defres{e7f/lat/rltier/s2-reflection-gemini/p90}{8.25}
\defres{e7f/lat/rltier/s2-reflection-gemini/tailshare}{2.2}
\defres{e7f/lat/rltier/s2-toolparams-1tool-gemini/n}{2159}
\defres{e7f/lat/rltier/s2-toolparams-1tool-gemini/over}{506}
\defres{e7f/lat/rltier/s2-toolparams-1tool-gemini/p50}{1.46}
\defres{e7f/lat/rltier/s2-toolparams-1tool-gemini/p90}{7.47}
\defres{e7f/lat/rltier/s2-toolparams-1tool-gemini/tailshare}{6.0}
\defres{e7f/lat/rltier/s2-toolselect-gemini/n}{3494}
\defres{e7f/lat/rltier/s2-toolselect-gemini/over}{441}
\defres{e7f/lat/rltier/s2-toolselect-gemini/p50}{1.21}
\defres{e7f/lat/rltier/s2-toolselect-gemini/p90}{5.81}
\defres{e7f/lat/rltier/s2-toolselect-gemini/tailshare}{5.8}
\defres{e7f/lat/rltier/s2tail}{45.8}
\defres{e7f/lat/rltier/tailshareofextra}{9}
\defres{e7f/lat/rltier/wall}{327.2}
\defres{e7f/llm_only/cost_k}{264.3}
\defres{e7f/llm_only/fail/askfinish}{0}
\defres{e7f/llm_only/fail/n}{33}
\defres{e7f/llm_only/fail/other}{0}
\defres{e7f/llm_only/fail/wrongtotal}{33}
\defres{e7f/llm_only/fail/wrongwrite}{0}
\defres{e7f/llm_only/form/itemized/n}{200}
\defres{e7f/llm_only/form/itemized/share}{100.0}
\defres{e7f/llm_only/form/itemized/success}{83.5}
\defres{e7f/llm_only/form/none/n}{0}
\defres{e7f/llm_only/form/none/share}{0.0}
\defres{e7f/llm_only/form/number/n}{0}
\defres{e7f/llm_only/form/number/share}{0.0}
\defres{e7f/llm_only/form/sentence/n}{0}
\defres{e7f/llm_only/form/sentence/share}{0.0}
\defres{e7f/llm_only/n}{200}
\defres{e7f/llm_only/success}{83.5}
\defres{e7f/llm_only/wall_mean}{74.2}
\defres{e7f/llm_only/wall_median}{63.2}
\defres{e7f/pilot/n}{60}
\defres{e7f/pilot/success}{46.7}
\defres{e7f/rl_frozen_refit/state}{not run}
\defres{e7f/rl_tier/acc}{98.9}
\defres{e7f/rl_tier/acc_accepted}{100.0}
\defres{e7f/rl_tier/cost_api_k}{229.6}
\defres{e7f/rl_tier/cost_k}{253.0}
\defres{e7f/rl_tier/cost_ref_k}{264.3}
\defres{e7f/rl_tier/coverage}{58.7}
\defres{e7f/rl_tier/delta}{-2.0}
\defres{e7f/rl_tier/delta_ci/hi}{+4.5}
\defres{e7f/rl_tier/delta_ci/lo}{-8.5}
\defres{e7f/rl_tier/diag/earlyfinishbymodel}{2}
\defres{e7f/rl_tier/diag/failsbymodel}{15}
\defres{e7f/rl_tier/diag/wrongwritebymodel}{0}
\defres{e7f/rl_tier/fail/askfinish}{2}
\defres{e7f/rl_tier/fail/n}{37}
\defres{e7f/rl_tier/fail/other}{0}
\defres{e7f/rl_tier/fail/wrongtotal}{35}
\defres{e7f/rl_tier/fail/wrongwrite}{0}
\defres{e7f/rl_tier/fig_delta}{-2.0}
\defres{e7f/rl_tier/fig_saving}{4}
\defres{e7f/rl_tier/form/itemized/n}{200}
\defres{e7f/rl_tier/form/itemized/share}{100.0}
\defres{e7f/rl_tier/form/itemized/success}{81.5}
\defres{e7f/rl_tier/form/none/n}{0}
\defres{e7f/rl_tier/form/none/share}{0.0}
\defres{e7f/rl_tier/form/number/n}{0}
\defres{e7f/rl_tier/form/number/share}{0.0}
\defres{e7f/rl_tier/form/sentence/n}{0}
\defres{e7f/rl_tier/form/sentence/share}{0.0}
\defres{e7f/rl_tier/losses}{25}
\defres{e7f/rl_tier/n}{200}
\defres{e7f/rl_tier/n_dropped}{0}
\defres{e7f/rl_tier/newcombe/hi}{+4.8}
\defres{e7f/rl_tier/newcombe/lo}{-8.8}
\defres{e7f/rl_tier/op_acc}{96.3}
\defres{e7f/rl_tier/op_acc_accepted}{100.0}
\defres{e7f/rl_tier/op_accepted_wrong}{0}
\defres{e7f/rl_tier/op_coverage}{51.6}
\defres{e7f/rl_tier/op_n}{2398}
\defres{e7f/rl_tier/reflection_fired}{9.3}
\defres{e7f/rl_tier/saving}{4.3}
\defres{e7f/rl_tier/saving_api}{13.1}
\defres{e7f/rl_tier/saving_ci/hi}{6.6}
\defres{e7f/rl_tier/saving_ci/lo}{2.1}
\defres{e7f/rl_tier/saving_q_s24}{12.4}
\defres{e7f/rl_tier/saving_q_zero}{13.1}
\defres{e7f/rl_tier/state}{run}
\defres{e7f/rl_tier/success}{81.5}
\defres{e7f/rl_tier/success_ref}{83.5}
\defres{e7f/rl_tier/tool_params/acc}{99.3}
\defres{e7f/rl_tier/tool_params/acc_accepted}{100.0}
\defres{e7f/rl_tier/tool_params/coverage}{65.9}
\defres{e7f/rl_tier/tool_select/acc}{98.5}
\defres{e7f/rl_tier/tool_select/acc_accepted}{99.9}
\defres{e7f/rl_tier/tool_select/coverage}{52.7}
\defres{e7f/rl_tier/wall_mean}{327.2}
\defres{e7f/rl_tier/wall_median}{325.8}
\defres{e7f/rl_tier/wall_ref_mean}{74.2}
\defres{e7f/rl_tier/wall_ref_median}{63.2}
\defres{e7f/rl_tier/wins}{21}
\defres{e7f/route}{gemini}
\defres{e7f/setting/answer_style}{itemized}
\defres{e7f/setting/families}{multi}
\defres{e7f/setting/max_steps}{45}
\defres{e7f/setting/multi_customers}{12}
\defres{e7f/setting/n}{200}
\defres{e7f/setting/n_distractors}{60}
\defres{e7f/setting/noise_lines}{20}
\defres{e7f/setting/rule}{tier}
\defres{e7f/setting/seed0}{310600}
\defres{e7f/spend}{99.67}
\defres{e7f/tariff/host_usd_h}{2.448}
\defres{e7f/tariff/q}{0.02340}
\makeatother


==> generated/e8_gates.tex <==
\makeatletter
\providecommand{\res}[1]{\ifcsname jevres@#1\endcsname\csname jevres@#1\endcsname\else\tbd\fi}
\providecommand{\defres}[2]{\expandafter\def\csname jevres@#1\endcsname{#2}}
\defres{e8/V}{1}
\defres{e8/cap}{40}
\defres{e8/n}{1{,}000}
\defres{e8/ntasks}{150}
\defres{e8/spend}{2.49}
\defres{e8/toolparams/dc}{0.0034}
\defres{e8/toolparams/dlms}{696}
\defres{e8/toolparams/g1/auroc}{0.89}
\defres{e8/toolparams/g1/cov}{73}
\defres{e8/toolparams/g1/latms}{208}
\defres{e8/toolparams/g1/save}{59}
\defres{e8/toolparams/g1/savefree}{59}
\defres{e8/toolparams/g1/saveheld}{1}
\defres{e8/toolparams/g1/sel50}{100.0}
\defres{e8/toolparams/g1/sel90}{97.1}
\defres{e8/toolparams/g1g3/auroc}{0.94}
\defres{e8/toolparams/g1g3/cov}{88}
\defres{e8/toolparams/g1g3/latms}{310}
\defres{e8/toolparams/g1g3/save}{81}
\defres{e8/toolparams/g1g3/savefree}{81}
\defres{e8/toolparams/g1g3/saveheld}{81}
\defres{e8/toolparams/g1g3/sel50}{100.0}
\defres{e8/toolparams/g1g3/sel90}{98.0}
\defres{e8/toolparams/g1g4/auroc}{0.88}
\defres{e8/toolparams/g1g4/cov}{73}
\defres{e8/toolparams/g1g4/latms}{$-$246}
\defres{e8/toolparams/g1g4/save}{48}
\defres{e8/toolparams/g1g4/savefree}{59}
\defres{e8/toolparams/g1g4/saveheld}{48}
\defres{e8/toolparams/g1g4/sel50}{100.0}
\defres{e8/toolparams/g1g4/sel90}{96.9}
\defres{e8/toolparams/g1g4v/auroc}{0.97}
\defres{e8/toolparams/g1g4v/cov}{73}
\defres{e8/toolparams/g1g4v/latms}{$-$246}
\defres{e8/toolparams/g1g4v/save}{48}
\defres{e8/toolparams/g1g4v/savefree}{59}
\defres{e8/toolparams/g1g4v/saveheld}{15}
\defres{e8/toolparams/g1g4v/sel50}{100.0}
\defres{e8/toolparams/g1g4v/sel90}{99.5}
\defres{e8/toolparams/g1tau/auroc}{0.89}
\defres{e8/toolparams/g1tau/cov}{73}
\defres{e8/toolparams/g1tau/latms}{208}
\defres{e8/toolparams/g1tau/save}{59}
\defres{e8/toolparams/g1tau/savefree}{59}
\defres{e8/toolparams/g1tau/saveheld}{59}
\defres{e8/toolparams/g1tau/sel50}{100.0}
\defres{e8/toolparams/g1tau/sel90}{97.1}
\defres{e8/toolparams/g2/auroc}{0.88}
\defres{e8/toolparams/g2/cov}{74}
\defres{e8/toolparams/g2/latms}{225}
\defres{e8/toolparams/g2/save}{62}
\defres{e8/toolparams/g2/savefree}{62}
\defres{e8/toolparams/g2/saveheld}{10}
\defres{e8/toolparams/g2/sel50}{100.0}
\defres{e8/toolparams/g2/sel90}{96.9}
\defres{e8/toolparams/g3/auroc}{0.83}
\defres{e8/toolparams/g3/cov}{68}
\defres{e8/toolparams/g3/latms}{52}
\defres{e8/toolparams/g3/save}{63}
\defres{e8/toolparams/g3/savefree}{64}
\defres{e8/toolparams/g3/saveheld}{45}
\defres{e8/toolparams/g3/sel50}{100.0}
\defres{e8/toolparams/g3/sel90}{96.7}
\defres{e8/toolparams/g3cost}{0.00005}
\defres{e8/toolparams/g3ms}{206}
\defres{e8/toolparams/g4/auroc}{0.50}
\defres{e8/toolparams/g4/cov}{0}
\defres{e8/toolparams/g4/latms}{$-$1881}
\defres{e8/toolparams/g4/save}{$-$49}
\defres{e8/toolparams/g4/savefree}{$-$2}
\defres{e8/toolparams/g4/saveheld}{$-$49}
\defres{e8/toolparams/g4/sel50}{95.6}
\defres{e8/toolparams/g4/sel90}{95.6}
\defres{e8/toolparams/g4cost}{0.0016}
\defres{e8/toolparams/g4ms}{1658}
\defres{e8/toolparams/g4overdc}{0.47}
\defres{e8/toolparams/g4v/auroc}{0.92}
\defres{e8/toolparams/g4v/cov}{0}
\defres{e8/toolparams/g4v/latms}{$-$1881}
\defres{e8/toolparams/g4v/save}{$-$49}
\defres{e8/toolparams/g4v/savefree}{$-$2}
\defres{e8/toolparams/g4v/saveheld}{$-$75}
\defres{e8/toolparams/g4v/sel50}{99.4}
\defres{e8/toolparams/g4v/sel90}{99.4}
\defres{e8/toolparams/g5/auroc}{1.00}
\defres{e8/toolparams/g5/cov}{0}
\defres{e8/toolparams/g5/latms}{0}
\defres{e8/toolparams/g5/save}{$-$2}
\defres{e8/toolparams/g5/savefree}{$-$2}
\defres{e8/toolparams/g5/saveheld}{$-$2}
\defres{e8/toolparams/g5/sel50}{100.0}
\defres{e8/toolparams/g5/sel90}{100.0}
\defres{e8/toolparams/llmacc}{100.0}
\defres{e8/toolparams/n}{500}
\defres{e8/toolparams/nwrong}{22}
\defres{e8/toolparams/perfect/cov}{96}
\defres{e8/toolparams/perfect/latms}{448}
\defres{e8/toolparams/perfect/save}{95}
\defres{e8/toolparams/perfect/savefree}{95}
\defres{e8/toolparams/perfect/saveheld}{95}
\defres{e8/toolparams/perfect/sel50}{100.0}
\defres{e8/toolparams/perfect/sel90}{100.0}
\defres{e8/toolparams/s1acc}{95.6}
\defres{e8/toolselect/dc}{0.0057}
\defres{e8/toolselect/dlms}{1160}
\defres{e8/toolselect/g1/auroc}{0.74}
\defres{e8/toolselect/g1/cov}{33}
\defres{e8/toolselect/g1/latms}{170}
\defres{e8/toolselect/g1/save}{28}
\defres{e8/toolselect/g1/savefree}{28}
\defres{e8/toolselect/g1/saveheld}{$-$1}
\defres{e8/toolselect/g1/sel50}{97.8}
\defres{e8/toolselect/g1/sel90}{95.3}
\defres{e8/toolselect/g1g3/auroc}{0.75}
\defres{e8/toolselect/g1g3/cov}{40}
\defres{e8/toolselect/g1g3/latms}{128}
\defres{e8/toolselect/g1g3/save}{33}
\defres{e8/toolselect/g1g3/savefree}{34}
\defres{e8/toolselect/g1g3/saveheld}{$-$21}
\defres{e8/toolselect/g1g3/sel50}{97.3}
\defres{e8/toolselect/g1g3/sel90}{96.2}
\defres{e8/toolselect/g1g4/auroc}{0.67}
\defres{e8/toolselect/g1g4/cov}{33}
\defres{e8/toolselect/g1g4/latms}{$-$1108}
\defres{e8/toolselect/g1g4/save}{$-$8}
\defres{e8/toolselect/g1g4/savefree}{28}
\defres{e8/toolselect/g1g4/saveheld}{$-$8}
\defres{e8/toolselect/g1g4/sel50}{96.9}
\defres{e8/toolselect/g1g4/sel90}{94.3}
\defres{e8/toolselect/g1g4v/auroc}{0.79}
\defres{e8/toolselect/g1g4v/cov}{33}
\defres{e8/toolselect/g1g4v/latms}{$-$1108}
\defres{e8/toolselect/g1g4v/save}{$-$8}
\defres{e8/toolselect/g1g4v/savefree}{28}
\defres{e8/toolselect/g1g4v/saveheld}{$-$8}
\defres{e8/toolselect/g1g4v/sel50}{98.0}
\defres{e8/toolselect/g1g4v/sel90}{96.4}
\defres{e8/toolselect/g1tau/auroc}{0.74}
\defres{e8/toolselect/g1tau/cov}{33}
\defres{e8/toolselect/g1tau/latms}{170}
\defres{e8/toolselect/g1tau/save}{28}
\defres{e8/toolselect/g1tau/savefree}{28}
\defres{e8/toolselect/g1tau/saveheld}{28}
\defres{e8/toolselect/g1tau/sel50}{97.8}
\defres{e8/toolselect/g1tau/sel90}{95.3}
\defres{e8/toolselect/g2/auroc}{0.73}
\defres{e8/toolselect/g2/cov}{38}
\defres{e8/toolselect/g2/latms}{224}
\defres{e8/toolselect/g2/save}{33}
\defres{e8/toolselect/g2/savefree}{33}
\defres{e8/toolselect/g2/saveheld}{$-$25}
\defres{e8/toolselect/g2/sel50}{97.4}
\defres{e8/toolselect/g2/sel90}{95.3}
\defres{e8/toolselect/g3/auroc}{0.73}
\defres{e8/toolselect/g3/cov}{31}
\defres{e8/toolselect/g3/latms}{$-$35}
\defres{e8/toolselect/g3/save}{25}
\defres{e8/toolselect/g3/savefree}{26}
\defres{e8/toolselect/g3/saveheld}{$-$27}
\defres{e8/toolselect/g3/sel50}{96.8}
\defres{e8/toolselect/g3/sel90}{96.2}
\defres{e8/toolselect/g3cost}{0.00005}
\defres{e8/toolselect/g3ms}{203}
\defres{e8/toolselect/g4/auroc}{0.50}
\defres{e8/toolselect/g4/cov}{0}
\defres{e8/toolselect/g4/latms}{$-$2005}
\defres{e8/toolselect/g4/save}{$-$60}
\defres{e8/toolselect/g4/savefree}{$-$2}
\defres{e8/toolselect/g4/saveheld}{$-$60}
\defres{e8/toolselect/g4/sel50}{94.0}
\defres{e8/toolselect/g4/sel90}{94.0}
\defres{e8/toolselect/g4cost}{0.0033}
\defres{e8/toolselect/g4ms}{1781}
\defres{e8/toolselect/g4overdc}{0.58}
\defres{e8/toolselect/g4v/auroc}{0.69}
\defres{e8/toolselect/g4v/cov}{0}
\defres{e8/toolselect/g4v/latms}{$-$2005}
\defres{e8/toolselect/g4v/save}{$-$60}
\defres{e8/toolselect/g4v/savefree}{$-$2}
\defres{e8/toolselect/g4v/saveheld}{$-$60}
\defres{e8/toolselect/g4v/sel50}{96.3}
\defres{e8/toolselect/g4v/sel90}{96.3}
\defres{e8/toolselect/g5/auroc}{0.93}
\defres{e8/toolselect/g5/cov}{0}
\defres{e8/toolselect/g5/latms}{0}
\defres{e8/toolselect/g5/save}{$-$2}
\defres{e8/toolselect/g5/savefree}{$-$2}
\defres{e8/toolselect/g5/saveheld}{$-$2}
\defres{e8/toolselect/g5/sel50}{100.0}
\defres{e8/toolselect/g5/sel90}{96.8}
\defres{e8/toolselect/llmacc}{100.0}
\defres{e8/toolselect/n}{500}
\defres{e8/toolselect/nwrong}{30}
\defres{e8/toolselect/perfect/cov}{94}
\defres{e8/toolselect/perfect/latms}{862}
\defres{e8/toolselect/perfect/save}{91}
\defres{e8/toolselect/perfect/savefree}{91}
\defres{e8/toolselect/perfect/saveheld}{91}
\defres{e8/toolselect/perfect/sel50}{100.0}
\defres{e8/toolselect/perfect/sel90}{100.0}
\defres{e8/toolselect/s1acc}{94.0}
\makeatother


==> generated/e9_frontier.tex <==
\makeatletter
\providecommand{\res}[1]{\ifcsname jevres@#1\endcsname\csname jevres@#1\endcsname\else\tbd\fi}
\providecommand{\defres}[2]{\expandafter\def\csname jevres@#1\endcsname{#2}}
\defres{e9/base/acc}{71.4}
\defres{e9/base/acc/args}{70.5}
\defres{e9/base/acc/toolchoice}{87.5}
\defres{e9/base/acc/w2c}{53.9}
\defres{e9/base/front}{no}
\defres{e9/base/lat}{266}
\defres{e9/base/lg}{-4.0316}
\defres{e9/base/usdk}{0.093}
\defres{e9/bestdm/gap}{-0.4}
\defres{e9/bestdm/gaphi}{+0.5}
\defres{e9/bestdm/gaplo}{-1.3}
\defres{e9/bestdm/model}{StartLux-27B}
\defres{e9/bm25/acc}{39.4}
\defres{e9/bm25/acc/args}{31.5}
\defres{e9/bm25/acc/toolchoice}{61.4}
\defres{e9/bm25/acc/w2c}{29.5}
\defres{e9/bm25/front}{no}
\defres{e9/bm25/lat}{1}
\defres{e9/bm25/usdk}{0}
\defres{e9/cap}{30}
\defres{e9/cheapest/flash/model}{none}
\defres{e9/cheapest/flashfc/model}{\jev{}}
\defres{e9/cheapest/flashfc/ratio}{45}
\defres{e9/cheapest/lite/model}{\jev{}}
\defres{e9/cheapest/lite/ratio}{11}
\defres{e9/cheapest/litelabel/model}{\jev{}}
\defres{e9/cheapest/litelabel/ratio}{8.4}
\defres{e9/check/flash/acc}{91.6}
\defres{e9/check/flash/lat}{1{,}122}
\defres{e9/check/flash/usdk}{0.81}
\defres{e9/check/jev/acc}{91.3}
\defres{e9/check/jev/lat}{202}
\defres{e9/check/jev/usdk}{0.017}
\defres{e9/check/jev/vs/flash/gap}{-0.3}
\defres{e9/check/jev/vs/flash/gapabs}{0.3}
\defres{e9/check/jev/vs/flash/gaphi}{+2.0}
\defres{e9/check/jev/vs/flash/gaplo}{-2.7}
\defres{e9/check/jev/vs/flash/ratio}{48}
\defres{e9/check/jev/vs/lite/gap}{+5.0}
\defres{e9/check/jev/vs/lite/gapabs}{5.0}
\defres{e9/check/jev/vs/lite/gaphi}{+8.0}
\defres{e9/check/jev/vs/lite/gaplo}{+1.7}
\defres{e9/check/jev/vs/lite/ratio}{11}
\defres{e9/check/jev/vs/luna/gap}{+6.7}
\defres{e9/check/jev/vs/luna/gapabs}{6.7}
\defres{e9/check/jev/vs/luna/gaphi}{+10.0}
\defres{e9/check/jev/vs/luna/gaplo}{+3.7}
\defres{e9/check/jev/vs/luna/ratio}{2.6}
\defres{e9/check/jev/vs/sol/gap}{+0.7}
\defres{e9/check/jev/vs/sol/gapabs}{0.7}
\defres{e9/check/jev/vs/sol/gaphi}{+3.3}
\defres{e9/check/jev/vs/sol/gaplo}{-2.0}
\defres{e9/check/jev/vs/sol/ratio}{54}
\defres{e9/check/jevfront}{yes}
\defres{e9/check/lite/acc}{86.3}
\defres{e9/check/lite/lat}{767}
\defres{e9/check/lite/usdk}{0.19}
\defres{e9/check/luna/acc}{84.6}
\defres{e9/check/luna/lat}{1{,}147}
\defres{e9/check/luna/usdk}{0.044}
\defres{e9/check/n}{299}
\defres{e9/check/sol/acc}{90.6}
\defres{e9/check/sol/lat}{2{,}322}
\defres{e9/check/sol/usdk}{0.91}
\defres{e9/e12/acc}{85.1}
\defres{e9/e12/acc/args}{90.5}
\defres{e9/e12/acc/toolchoice}{89.3}
\defres{e9/e12/acc/w2c}{68.5}
\defres{e9/e12/costvsjev}{8.6}
\defres{e9/e12/front}{no}
\defres{e9/e12/frontadj}{no}
\defres{e9/e12/gapfrozen}{+6.3}
\defres{e9/e12/gapfrozenabs}{6.3}
\defres{e9/e12/gapjev}{-1.3}
\defres{e9/e12/gapjevabs}{1.3}
\defres{e9/e12/gapsl4b}{+1.9}
\defres{e9/e12/gapsl4babs}{1.9}
\defres{e9/e12/lat}{344}
\defres{e9/e12/lg}{-3.8549}
\defres{e9/e12/lgadj}{-4.0392}
\defres{e9/e12/usdk}{0.14}
\defres{e9/e12/usdk_hostadj}{0.091}
\defres{e9/e12/usdkadj}{0.091}
\defres{e9/e12c/acc}{85.5}
\defres{e9/e12c/acc/args}{91.9}
\defres{e9/e12c/acc/toolchoice}{89.5}
\defres{e9/e12c/acc/w2c}{67.1}
\defres{e9/e12c/costvsjev}{18}
\defres{e9/e12c/front}{no}
\defres{e9/e12c/frontadj}{no}
\defres{e9/e12c/gapfrozen}{+6.7}
\defres{e9/e12c/gapfrozenabs}{6.7}
\defres{e9/e12c/gapjev}{-0.9}
\defres{e9/e12c/gapjevabs}{0.9}
\defres{e9/e12c/gapsl4b}{+2.3}
\defres{e9/e12c/gapsl4babs}{2.3}
\defres{e9/e12c/lat}{713}
\defres{e9/e12c/lg}{-3.5307}
\defres{e9/e12c/lgadj}{-3.7151}
\defres{e9/e12c/usdk}{0.29}
\defres{e9/e12c/usdk_hostadj}{0.19}
\defres{e9/e12c/usdkadj}{0.19}
\defres{e9/e16a/acc}{84.3}
\defres{e9/e16a/acc/args}{90.1}
\defres{e9/e16a/acc/toolchoice}{88.8}
\defres{e9/e16a/acc/w2c}{66.9}
\defres{e9/e16a/costvsjev}{5.6}
\defres{e9/e16a/front}{no}
\defres{e9/e16a/frontadj}{no}
\defres{e9/e16a/gapfrozen}{+5.6}
\defres{e9/e16a/gapfrozenabs}{5.6}
\defres{e9/e16a/gapjev}{-2.1}
\defres{e9/e16a/gapjevabs}{2.1}
\defres{e9/e16a/gapsl4b}{+1.2}
\defres{e9/e16a/gapsl4babs}{1.2}
\defres{e9/e16a/lat}{260}
\defres{e9/e16a/lg}{-4.0414}
\defres{e9/e16a/lgadj}{-4.0373}
\defres{e9/e16a/usdk}{0.091}
\defres{e9/e16a/usdk_hostadj}{0.092}
\defres{e9/e16a/usdkadj}{0.092}
\defres{e9/e16b/acc}{84.8}
\defres{e9/e16b/acc/args}{91.9}
\defres{e9/e16b/acc/toolchoice}{90.0}
\defres{e9/e16b/acc/w2c}{63.6}
\defres{e9/e16b/costvsjev}{15}
\defres{e9/e16b/front}{no}
\defres{e9/e16b/frontadj}{no}
\defres{e9/e16b/gapfrozen}{+6.1}
\defres{e9/e16b/gapfrozenabs}{6.1}
\defres{e9/e16b/gapjev}{-1.6}
\defres{e9/e16b/gapjevabs}{1.6}
\defres{e9/e16b/gapsl4b}{+1.7}
\defres{e9/e16b/gapsl4babs}{1.7}
\defres{e9/e16b/lat}{604}
\defres{e9/e16b/lg}{-3.6191}
\defres{e9/e16b/lgadj}{-3.6149}
\defres{e9/e16b/usdk}{0.24}
\defres{e9/e16b/usdk_hostadj}{0.24}
\defres{e9/e16b/usdkadj}{0.24}
\defres{e9/embed/acc}{51.7}
\defres{e9/embed/acc/args}{40.0}
\defres{e9/embed/acc/toolchoice}{79.3}
\defres{e9/embed/acc/w2c}{43.2}
\defres{e9/embed/front}{no}
\defres{e9/embed/lat}{196}
\defres{e9/embed/lg}{-4.5910}
\defres{e9/embed/usdk}{0.026}
\defres{e9/flash/acc}{88.1}
\defres{e9/flash/acc/args}{93.6}
\defres{e9/flash/acc/toolchoice}{90.3}
\defres{e9/flash/acc/w2c}{74.0}
\defres{e9/flash/front}{yes}
\defres{e9/flash/lat}{2{,}570}
\defres{e9/flash/lg}{-3.0911}
\defres{e9/flash/usdk}{0.81}
\defres{e9/flashfc/acc}{78.7}
\defres{e9/flashfc/acc/args}{96.3}
\defres{e9/flashfc/acc/toolchoice}{84.2}
\defres{e9/flashfc/acc/w2c}{35.2}
\defres{e9/flashfc/front}{no}
\defres{e9/flashfc/lat}{884}
\defres{e9/flashfc/lg}{-3.1384}
\defres{e9/flashfc/usdk}{0.73}
\defres{e9/front/dm}{2}
\defres{e9/front/first}{sl08b}
\defres{e9/front/llm}{1}
\defres{e9/front/n}{3}
\defres{e9/front/onlydm}{yes}
\defres{e9/front/rest}{jev,flash}
\defres{e9/front12/changed}{no}
\defres{e9/front12/first}{sl08b}
\defres{e9/front12/n}{3}
\defres{e9/front12/rest}{jev,flash}
\defres{e9/front16/changed}{no}
\defres{e9/front16/first}{sl08b}
\defres{e9/front16/n}{3}
\defres{e9/front16/rest}{jev,flash}
\defres{e9/gemma/acc}{80.2}
\defres{e9/gemma/acc/args}{87.4}
\defres{e9/gemma/acc/toolchoice}{89.1}
\defres{e9/gemma/acc/w2c}{54.4}
\defres{e9/gemma/front}{no}
\defres{e9/gemma/lat}{1{,}739}
\defres{e9/gpu/usdh}{2.24}
\defres{e9/intern/acc}{73.4}
\defres{e9/intern/acc/args}{71.2}
\defres{e9/intern/acc/toolchoice}{88.2}
\defres{e9/intern/acc/w2c}{60.1}
\defres{e9/intern/front}{no}
\defres{e9/intern/lat}{91}
\defres{e9/intern/lg}{-4.4101}
\defres{e9/intern/usdk}{0.039}
\defres{e9/jev/acc}{86.4}
\defres{e9/jev/acc/args}{89.6}
\defres{e9/jev/acc/toolchoice}{89.9}
\defres{e9/jev/acc/w2c}{75.4}
\defres{e9/jev/front}{yes}
\defres{e9/jev/lat}{206}
\defres{e9/jev/lg}{-4.7877}
\defres{e9/jev/usdk}{0.016}
\defres{e9/jev/vs/flash/gap}{-1.7}
\defres{e9/jev/vs/flash/gapabs}{1.7}
\defres{e9/jev/vs/flash/gaphi}{-0.9}
\defres{e9/jev/vs/flash/gaplo}{-2.6}
\defres{e9/jev/vs/flash/ratio}{50}
\defres{e9/jev/vs/flashfc/gap}{+7.7}
\defres{e9/jev/vs/flashfc/gapabs}{7.7}
\defres{e9/jev/vs/flashfc/gaphi}{+9.0}
\defres{e9/jev/vs/flashfc/gaplo}{+6.2}
\defres{e9/jev/vs/flashfc/ratio}{45}
\defres{e9/jev/vs/lite/gap}{+3.1}
\defres{e9/jev/vs/lite/gapabs}{3.1}
\defres{e9/jev/vs/lite/gaphi}{+4.0}
\defres{e9/jev/vs/lite/gaplo}{+2.0}
\defres{e9/jev/vs/lite/ratio}{11}
\defres{e9/jev/vs/litelabel/gap}{+2.3}
\defres{e9/jev/vs/litelabel/gapabs}{2.3}
\defres{e9/jev/vs/litelabel/gaphi}{+3.2}
\defres{e9/jev/vs/litelabel/gaplo}{+1.3}
\defres{e9/jev/vs/litelabel/ratio}{8.4}
\defres{e9/lite/acc}{83.3}
\defres{e9/lite/acc/args}{89.0}
\defres{e9/lite/acc/toolchoice}{90.7}
\defres{e9/lite/acc/w2c}{62.6}
\defres{e9/lite/front}{no}
\defres{e9/lite/lat}{681}
\defres{e9/lite/lg}{-3.7302}
\defres{e9/lite/usdk}{0.19}
\defres{e9/litelabel/acc}{84.1}
\defres{e9/litelabel/acc/args}{89.7}
\defres{e9/litelabel/acc/toolchoice}{90.4}
\defres{e9/litelabel/acc/w2c}{64.9}
\defres{e9/litelabel/front}{no}
\defres{e9/litelabel/lat}{582}
\defres{e9/litelabel/lg}{-3.8655}
\defres{e9/litelabel/usdk}{0.14}
\defres{e9/n}{3{,}991}
\defres{e9/n/args}{1{,}949}
\defres{e9/n/toolchoice}{1{,}114}
\defres{e9/n/w2c}{928}
\defres{e9/rl/acc}{78.8}
\defres{e9/rl/acc/args}{85.0}
\defres{e9/rl/acc/toolchoice}{88.4}
\defres{e9/rl/acc/w2c}{54.0}
\defres{e9/rl/front}{no}
\defres{e9/rl/lat}{268}
\defres{e9/rl/lg}{-4.0296}
\defres{e9/rl/usdk}{0.093}
\defres{e9/sens/token_tariff/front/dm}{3}
\defres{e9/sens/token_tariff/front/n}{4}
\defres{e9/sens/token_tariff/jevfront}{no}
\defres{e9/sens/token_tariff/onlydm}{yes}
\defres{e9/sens/zero/front/dm}{1}
\defres{e9/sens/zero/front/n}{2}
\defres{e9/sens/zero/jevfront}{no}
\defres{e9/sens/zero/onlydm}{yes}
\defres{e9/sftv1/acc}{78.4}
\defres{e9/sftv1/acc/args}{85.5}
\defres{e9/sftv1/acc/toolchoice}{86.9}
\defres{e9/sftv1/acc/w2c}{53.3}
\defres{e9/sftv1/front}{no}
\defres{e9/sftv1/lat}{270}
\defres{e9/sftv1/lg}{-4.0252}
\defres{e9/sftv1/usdk}{0.094}
\defres{e9/sl0.8b/acc}{70.0}
\defres{e9/sl0.8b/acc/args}{67.1}
\defres{e9/sl0.8b/acc/toolchoice}{88.2}
\defres{e9/sl0.8b/acc/w2c}{54.2}
\defres{e9/sl0.8b/front}{yes}
\defres{e9/sl0.8b/lat}{17}
\defres{e9/sl0.8b/lg}{-4.8970}
\defres{e9/sl0.8b/usdk}{0.013}
\defres{e9/sl27b/acc}{87.7}
\defres{e9/sl27b/acc/args}{89.1}
\defres{e9/sl27b/acc/toolchoice}{90.8}
\defres{e9/sl27b/acc/w2c}{81.2}
\defres{e9/sl27b/front}{no}
\defres{e9/sl27b/lat}{2{,}689}
\defres{e9/sl27b/lg}{-2.9617}
\defres{e9/sl27b/usdk}{1.1}
\defres{e9/sl2b/acc}{75.7}
\defres{e9/sl2b/acc/args}{73.1}
\defres{e9/sl2b/acc/toolchoice}{89.9}
\defres{e9/sl2b/acc/w2c}{64.1}
\defres{e9/sl2b/front}{no}
\defres{e9/sl2b/lat}{50}
\defres{e9/sl2b/lg}{-4.6622}
\defres{e9/sl2b/usdk}{0.022}
\defres{e9/sl4b/acc}{83.1}
\defres{e9/sl4b/acc/args}{81.2}
\defres{e9/sl4b/acc/toolchoice}{91.3}
\defres{e9/sl4b/acc/w2c}{77.4}
\defres{e9/sl4b/front}{no}
\defres{e9/sl4b/lat}{111}
\defres{e9/sl4b/lg}{-4.2810}
\defres{e9/sl4b/usdk}{0.052}
\defres{e9/sl9b/acc}{83.4}
\defres{e9/sl9b/acc/args}{81.0}
\defres{e9/sl9b/acc/toolchoice}{92.2}
\defres{e9/sl9b/acc/w2c}{78.1}
\defres{e9/sl9b/front}{no}
\defres{e9/sl9b/lat}{182}
\defres{e9/sl9b/lg}{-4.0811}
\defres{e9/sl9b/usdk}{0.083}
\defres{e9/spend}{0.59}
\defres{e9/tfidf/acc}{39.9}
\defres{e9/tfidf/acc/args}{31.6}
\defres{e9/tfidf/acc/toolchoice}{62.3}
\defres{e9/tfidf/acc/w2c}{30.4}
\defres{e9/tfidf/front}{no}
\defres{e9/tfidf/lat}{1}
\defres{e9/tfidf/usdk}{0}
\defres{e9/tokrate/rl}{0.094}
\defres{e9/tokrate/sl4b}{0.043}
\makeatother


==> generated/economics.tex <==
\makeatletter
\providecommand{\res}[1]{\ifcsname jevres@#1\endcsname\csname jevres@#1\endcsname\else\tbd\fi}
\providecommand{\defres}[2]{\expandafter\def\csname jevres@#1\endcsname{#2}}
\defres{econ/best_single/abs_ratio/astra}{7.4}
\defres{econ/best_single/abs_ratio/sol}{1.3}
\defres{econ/best_single/abs_savings/astra}{0.0577}
\defres{econ/best_single/abs_savings/frozen}{0.00775}
\defres{econ/best_single/abs_savings/sol}{0.00987}
\defres{econ/best_single/abs_savings_ci/astra/hi}{0.0628}
\defres{econ/best_single/abs_savings_ci/astra/lo}{0.0528}
\defres{econ/best_single/abs_savings_ci/frozen/hi}{0.00849}
\defres{econ/best_single/abs_savings_ci/frozen/lo}{0.00704}
\defres{econ/best_single/abs_savings_ci/sol/hi}{0.0108}
\defres{econ/best_single/abs_savings_ci/sol/lo}{0.00897}
\defres{econ/best_single/calllat/mean}{7.92}
\defres{econ/best_single/calllat/mean_diff}{+1.12}
\defres{econ/best_single/calllat/mean_diff_ci/hi}{+1.29}
\defres{econ/best_single/calllat/mean_diff_ci/lo}{+0.92}
\defres{econ/best_single/calllat/median}{8.08}
\defres{econ/best_single/calllat/median_diff}{+1.07}
\defres{econ/best_single/calllat/median_diff_ci/hi}{+1.33}
\defres{econ/best_single/calllat/median_diff_ci/lo}{-0.24}
\defres{econ/best_single/calllat/ratio}{1.16}
\defres{econ/best_single/calllat/ref_mean}{6.80}
\defres{econ/best_single/calllat/ref_median}{7.01}
\defres{econ/best_single/concurrency}{8}
\defres{econ/best_single/cost/astra}{0.215}
\defres{econ/best_single/cost/frozen}{0.0335}
\defres{econ/best_single/cost/sol}{0.0425}
\defres{econ/best_single/lgcost/frozen}{-1.4744}
\defres{econ/best_single/n}{500}
\defres{econ/best_single/rel_change/astra}{+2.4}
\defres{econ/best_single/rel_change/sol}{+0.1}
\defres{econ/best_single/s2_share/astra}{99.5}
\defres{econ/best_single/s2_share/frozen}{96.6}
\defres{econ/best_single/s2_share/sol}{97.3}
\defres{econ/best_single/savings/astra}{21.2}
\defres{econ/best_single/savings/frozen}{18.8}
\defres{econ/best_single/savings/sol}{18.9}
\defres{econ/best_single/savings_ci/astra/hi}{22.8}
\defres{econ/best_single/savings_ci/astra/lo}{19.6}
\defres{econ/best_single/savings_ci/frozen/hi}{20.3}
\defres{econ/best_single/savings_ci/frozen/lo}{17.2}
\defres{econ/best_single/savings_ci/sol/hi}{20.4}
\defres{econ/best_single/savings_ci/sol/lo}{17.3}
\defres{econ/best_single/wall/mean}{7.61}
\defres{econ/best_single/wall/mean_diff}{+0.78}
\defres{econ/best_single/wall/mean_diff_ci/hi}{+0.97}
\defres{econ/best_single/wall/mean_diff_ci/lo}{+0.59}
\defres{econ/best_single/wall/median}{7.58}
\defres{econ/best_single/wall/median_diff}{+0.53}
\defres{econ/best_single/wall/median_diff_ci/hi}{+1.05}
\defres{econ/best_single/wall/median_diff_ci/lo}{-0.70}
\defres{econ/best_single/wall/ratio}{1.11}
\defres{econ/best_single/wall/ref_mean}{6.83}
\defres{econ/best_single/wall/ref_median}{7.05}
\defres{econ/jevagent_best/abs_ratio/astra}{7.2}
\defres{econ/jevagent_best/abs_ratio/sol}{1.3}
\defres{econ/jevagent_best/abs_savings/astra}{0.122}
\defres{econ/jevagent_best/abs_savings/frozen}{0.0168}
\defres{econ/jevagent_best/abs_savings/sol}{0.0218}
\defres{econ/jevagent_best/abs_savings_ci/astra/hi}{0.129}
\defres{econ/jevagent_best/abs_savings_ci/astra/lo}{0.114}
\defres{econ/jevagent_best/abs_savings_ci/frozen/hi}{0.0179}
\defres{econ/jevagent_best/abs_savings_ci/frozen/lo}{0.0157}
\defres{econ/jevagent_best/abs_savings_ci/sol/hi}{0.0231}
\defres{econ/jevagent_best/abs_savings_ci/sol/lo}{0.0204}
\defres{econ/jevagent_best/calllat/mean}{9.35}
\defres{econ/jevagent_best/calllat/mean_diff}{+2.54}
\defres{econ/jevagent_best/calllat/mean_diff_ci/hi}{+2.89}
\defres{econ/jevagent_best/calllat/mean_diff_ci/lo}{+2.22}
\defres{econ/jevagent_best/calllat/median}{10.09}
\defres{econ/jevagent_best/calllat/median_diff}{+3.08}
\defres{econ/jevagent_best/calllat/median_diff_ci/hi}{+3.69}
\defres{econ/jevagent_best/calllat/median_diff_ci/lo}{+2.68}
\defres{econ/jevagent_best/calllat/ratio}{1.37}
\defres{econ/jevagent_best/calllat/ref_mean}{6.80}
\defres{econ/jevagent_best/calllat/ref_median}{7.01}
\defres{econ/jevagent_best/concurrency}{8}
\defres{econ/jevagent_best/cost/astra}{0.151}
\defres{econ/jevagent_best/cost/frozen}{0.0245}
\defres{econ/jevagent_best/cost/sol}{0.0306}
\defres{econ/jevagent_best/lgcost/frozen}{-1.6112}
\defres{econ/jevagent_best/n}{500}
\defres{econ/jevagent_best/rel_change/astra}{+3.8}
\defres{econ/jevagent_best/rel_change/sol}{+0.9}
\defres{econ/jevagent_best/s2_share/astra}{98.9}
\defres{econ/jevagent_best/s2_share/frozen}{93.1}
\defres{econ/jevagent_best/s2_share/sol}{94.4}
\defres{econ/jevagent_best/savings/astra}{44.6}
\defres{econ/jevagent_best/savings/frozen}{40.7}
\defres{econ/jevagent_best/savings/sol}{41.6}
\defres{econ/jevagent_best/savings_ci/astra/hi}{46.3}
\defres{econ/jevagent_best/savings_ci/astra/lo}{42.7}
\defres{econ/jevagent_best/savings_ci/frozen/hi}{42.5}
\defres{econ/jevagent_best/savings_ci/frozen/lo}{38.9}
\defres{econ/jevagent_best/savings_ci/sol/hi}{43.3}
\defres{econ/jevagent_best/savings_ci/sol/lo}{39.8}
\defres{econ/jevagent_best/wall/mean}{9.21}
\defres{econ/jevagent_best/wall/mean_diff}{+2.39}
\defres{econ/jevagent_best/wall/mean_diff_ci/hi}{+2.73}
\defres{econ/jevagent_best/wall/mean_diff_ci/lo}{+2.07}
\defres{econ/jevagent_best/wall/median}{10.00}
\defres{econ/jevagent_best/wall/median_diff}{+2.95}
\defres{econ/jevagent_best/wall/median_diff_ci/hi}{+3.17}
\defres{econ/jevagent_best/wall/median_diff_ci/lo}{+1.84}
\defres{econ/jevagent_best/wall/ratio}{1.35}
\defres{econ/jevagent_best/wall/ref_mean}{6.83}
\defres{econ/jevagent_best/wall/ref_median}{7.05}
\defres{econ/jevagent_best_rl/abs_ratio/astra}{6.9}
\defres{econ/jevagent_best_rl/abs_ratio/sol}{1.3}
\defres{econ/jevagent_best_rl/abs_savings/astra}{0.233}
\defres{econ/jevagent_best_rl/abs_savings/frozen}{0.0335}
\defres{econ/jevagent_best_rl/abs_savings/sol}{0.0428}
\defres{econ/jevagent_best_rl/abs_savings_ci/astra/hi}{0.239}
\defres{econ/jevagent_best_rl/abs_savings_ci/astra/lo}{0.226}
\defres{econ/jevagent_best_rl/abs_savings_ci/frozen/hi}{0.0345}
\defres{econ/jevagent_best_rl/abs_savings_ci/frozen/lo}{0.0325}
\defres{econ/jevagent_best_rl/abs_savings_ci/sol/hi}{0.044}
\defres{econ/jevagent_best_rl/abs_savings_ci/sol/lo}{0.0415}
\defres{econ/jevagent_best_rl/calllat/mean}{9.77}
\defres{econ/jevagent_best_rl/calllat/mean_diff}{+2.97}
\defres{econ/jevagent_best_rl/calllat/mean_diff_ci/hi}{+3.42}
\defres{econ/jevagent_best_rl/calllat/mean_diff_ci/lo}{+2.52}
\defres{econ/jevagent_best_rl/calllat/median}{8.43}
\defres{econ/jevagent_best_rl/calllat/median_diff}{+1.42}
\defres{econ/jevagent_best_rl/calllat/median_diff_ci/hi}{+3.01}
\defres{econ/jevagent_best_rl/calllat/median_diff_ci/lo}{+0.78}
\defres{econ/jevagent_best_rl/calllat/ratio}{1.44}
\defres{econ/jevagent_best_rl/calllat/ref_mean}{6.80}
\defres{econ/jevagent_best_rl/calllat/ref_median}{7.01}
\defres{econ/jevagent_best_rl/concurrency}{4}
\defres{econ/jevagent_best_rl/cost/astra}{0.0399}
\defres{econ/jevagent_best_rl/cost/frozen}{0.00779}
\defres{econ/jevagent_best_rl/cost/sol}{0.00955}
\defres{econ/jevagent_best_rl/lgcost/frozen}{-2.1082}
\defres{econ/jevagent_best_rl/n}{500}
\defres{econ/jevagent_best_rl/rel_change/astra}{+4.2}
\defres{econ/jevagent_best_rl/rel_change/sol}{+0.6}
\defres{econ/jevagent_best_rl/s2_share/astra}{95.1}
\defres{econ/jevagent_best_rl/s2_share/frozen}{74.8}
\defres{econ/jevagent_best_rl/s2_share/sol}{79.5}
\defres{econ/jevagent_best_rl/savings/astra}{85.4}
\defres{econ/jevagent_best_rl/savings/frozen}{81.1}
\defres{econ/jevagent_best_rl/savings/sol}{81.7}
\defres{econ/jevagent_best_rl/savings_ci/astra/hi}{85.8}
\defres{econ/jevagent_best_rl/savings_ci/astra/lo}{84.9}
\defres{econ/jevagent_best_rl/savings_ci/frozen/hi}{81.6}
\defres{econ/jevagent_best_rl/savings_ci/frozen/lo}{80.7}
\defres{econ/jevagent_best_rl/savings_ci/sol/hi}{82.2}
\defres{econ/jevagent_best_rl/savings_ci/sol/lo}{81.3}
\defres{econ/jevagent_best_rl/tariff_q}{0.00196}
\defres{econ/jevagent_best_rl/wall/mean}{10.21}
\defres{econ/jevagent_best_rl/wall/mean_diff}{+3.38}
\defres{econ/jevagent_best_rl/wall/mean_diff_ci/hi}{+3.95}
\defres{econ/jevagent_best_rl/wall/mean_diff_ci/lo}{+2.85}
\defres{econ/jevagent_best_rl/wall/median}{9.10}
\defres{econ/jevagent_best_rl/wall/median_diff}{+2.05}
\defres{econ/jevagent_best_rl/wall/median_diff_ci/hi}{+3.77}
\defres{econ/jevagent_best_rl/wall/median_diff_ci/lo}{+0.93}
\defres{econ/jevagent_best_rl/wall/ratio}{1.50}
\defres{econ/jevagent_best_rl/wall/ref_mean}{6.83}
\defres{econ/jevagent_best_rl/wall/ref_median}{7.05}
\defres{econ/jevagent_best_sl4b/abs_ratio/astra}{-13.3}
\defres{econ/jevagent_best_sl4b/abs_ratio/sol}{1.3}
\defres{econ/jevagent_best_sl4b/abs_savings/astra}{0.00793}
\defres{econ/jevagent_best_sl4b/abs_savings/frozen}{-0.000594}
\defres{econ/jevagent_best_sl4b/abs_savings/sol}{-0.000777}
\defres{econ/jevagent_best_sl4b/abs_savings_ci/astra/hi}{0.0107}
\defres{econ/jevagent_best_sl4b/abs_savings_ci/astra/lo}{0.0052}
\defres{econ/jevagent_best_sl4b/abs_savings_ci/frozen/hi}{-0.000179}
\defres{econ/jevagent_best_sl4b/abs_savings_ci/frozen/lo}{-0.00101}
\defres{econ/jevagent_best_sl4b/abs_savings_ci/sol/hi}{-0.000271}
\defres{econ/jevagent_best_sl4b/abs_savings_ci/sol/lo}{-0.00129}
\defres{econ/jevagent_best_sl4b/calllat/mean}{13.81}
\defres{econ/jevagent_best_sl4b/calllat/mean_diff}{+7.01}
\defres{econ/jevagent_best_sl4b/calllat/mean_diff_ci/hi}{+7.51}
\defres{econ/jevagent_best_sl4b/calllat/mean_diff_ci/lo}{+6.51}
\defres{econ/jevagent_best_sl4b/calllat/median}{15.74}
\defres{econ/jevagent_best_sl4b/calllat/median_diff}{+8.73}
\defres{econ/jevagent_best_sl4b/calllat/median_diff_ci/hi}{+9.27}
\defres{econ/jevagent_best_sl4b/calllat/median_diff_ci/lo}{+4.69}
\defres{econ/jevagent_best_sl4b/calllat/ratio}{2.03}
\defres{econ/jevagent_best_sl4b/calllat/ref_mean}{6.80}
\defres{econ/jevagent_best_sl4b/calllat/ref_median}{7.01}
\defres{econ/jevagent_best_sl4b/concurrency}{4}
\defres{econ/jevagent_best_sl4b/cost/astra}{0.265}
\defres{econ/jevagent_best_sl4b/cost/frozen}{0.0419}
\defres{econ/jevagent_best_sl4b/cost/sol}{0.0531}
\defres{econ/jevagent_best_sl4b/lgcost/frozen}{-1.3779}
\defres{econ/jevagent_best_sl4b/n}{500}
\defres{econ/jevagent_best_sl4b/rel_change/astra}{+4.3}
\defres{econ/jevagent_best_sl4b/rel_change/sol}{-0.0}
\defres{econ/jevagent_best_sl4b/s2_share/astra}{99.2}
\defres{econ/jevagent_best_sl4b/s2_share/frozen}{94.8}
\defres{econ/jevagent_best_sl4b/s2_share/sol}{95.9}
\defres{econ/jevagent_best_sl4b/savings/astra}{2.9}
\defres{econ/jevagent_best_sl4b/savings/frozen}{-1.4}
\defres{econ/jevagent_best_sl4b/savings/sol}{-1.5}
\defres{econ/jevagent_best_sl4b/savings_ci/astra/hi}{3.8}
\defres{econ/jevagent_best_sl4b/savings_ci/astra/lo}{1.9}
\defres{econ/jevagent_best_sl4b/savings_ci/frozen/hi}{-0.4}
\defres{econ/jevagent_best_sl4b/savings_ci/frozen/lo}{-2.5}
\defres{econ/jevagent_best_sl4b/savings_ci/sol/hi}{-0.5}
\defres{econ/jevagent_best_sl4b/savings_ci/sol/lo}{-2.5}
\defres{econ/jevagent_best_sl4b/tariff_q}{0.00217}
\defres{econ/jevagent_best_sl4b/wall/mean}{13.99}
\defres{econ/jevagent_best_sl4b/wall/mean_diff}{+7.17}
\defres{econ/jevagent_best_sl4b/wall/mean_diff_ci/hi}{+7.67}
\defres{econ/jevagent_best_sl4b/wall/mean_diff_ci/lo}{+6.67}
\defres{econ/jevagent_best_sl4b/wall/median}{15.93}
\defres{econ/jevagent_best_sl4b/wall/median_diff}{+8.88}
\defres{econ/jevagent_best_sl4b/wall/median_diff_ci/hi}{+9.48}
\defres{econ/jevagent_best_sl4b/wall/median_diff_ci/lo}{+4.78}
\defres{econ/jevagent_best_sl4b/wall/ratio}{2.05}
\defres{econ/jevagent_best_sl4b/wall/ref_mean}{6.83}
\defres{econ/jevagent_best_sl4b/wall/ref_median}{7.05}
\defres{econ/jevagent_best_v2/abs_ratio/astra}{9.7}
\defres{econ/jevagent_best_v2/abs_ratio/sol}{1.4}
\defres{econ/jevagent_best_v2/abs_savings/astra}{0.219}
\defres{econ/jevagent_best_v2/abs_savings/frozen}{0.0226}
\defres{econ/jevagent_best_v2/abs_savings/sol}{0.0317}
\defres{econ/jevagent_best_v2/abs_savings_ci/astra/hi}{0.226}
\defres{econ/jevagent_best_v2/abs_savings_ci/astra/lo}{0.212}
\defres{econ/jevagent_best_v2/abs_savings_ci/frozen/hi}{0.0237}
\defres{econ/jevagent_best_v2/abs_savings_ci/frozen/lo}{0.0216}
\defres{econ/jevagent_best_v2/abs_savings_ci/sol/hi}{0.033}
\defres{econ/jevagent_best_v2/abs_savings_ci/sol/lo}{0.0305}
\defres{econ/jevagent_best_v2/calllat/mean}{22.58}
\defres{econ/jevagent_best_v2/calllat/mean_diff}{+15.78}
\defres{econ/jevagent_best_v2/calllat/mean_diff_ci/hi}{+16.46}
\defres{econ/jevagent_best_v2/calllat/mean_diff_ci/lo}{+15.11}
\defres{econ/jevagent_best_v2/calllat/median}{21.41}
\defres{econ/jevagent_best_v2/calllat/median_diff}{+14.40}
\defres{econ/jevagent_best_v2/calllat/median_diff_ci/hi}{+22.68}
\defres{econ/jevagent_best_v2/calllat/median_diff_ci/lo}{+8.21}
\defres{econ/jevagent_best_v2/calllat/ratio}{3.32}
\defres{econ/jevagent_best_v2/calllat/ref_mean}{6.80}
\defres{econ/jevagent_best_v2/calllat/ref_median}{7.01}
\defres{econ/jevagent_best_v2/concurrency}{4}
\defres{econ/jevagent_best_v2/cost/astra}{0.0535}
\defres{econ/jevagent_best_v2/cost/frozen}{0.0187}
\defres{econ/jevagent_best_v2/cost/sol}{0.0206}
\defres{econ/jevagent_best_v2/lgcost/frozen}{-1.7292}
\defres{econ/jevagent_best_v2/n}{500}
\defres{econ/jevagent_best_v2/rel_change/astra}{+25.5}
\defres{econ/jevagent_best_v2/rel_change/sol}{+5.8}
\defres{econ/jevagent_best_v2/s2_share/astra}{76.9}
\defres{econ/jevagent_best_v2/s2_share/frozen}{33.8}
\defres{econ/jevagent_best_v2/s2_share/sol}{40.0}
\defres{econ/jevagent_best_v2/savings/astra}{80.4}
\defres{econ/jevagent_best_v2/savings/frozen}{54.8}
\defres{econ/jevagent_best_v2/savings/sol}{60.7}
\defres{econ/jevagent_best_v2/savings_ci/astra/hi}{80.8}
\defres{econ/jevagent_best_v2/savings_ci/astra/lo}{79.9}
\defres{econ/jevagent_best_v2/savings_ci/frozen/hi}{55.8}
\defres{econ/jevagent_best_v2/savings_ci/frozen/lo}{53.8}
\defres{econ/jevagent_best_v2/savings_ci/sol/hi}{61.4}
\defres{econ/jevagent_best_v2/savings_ci/sol/lo}{59.8}
\defres{econ/jevagent_best_v2/tariff_q}{0.0124}
\defres{econ/jevagent_best_v2/wall/mean}{22.79}
\defres{econ/jevagent_best_v2/wall/mean_diff}{+15.96}
\defres{econ/jevagent_best_v2/wall/mean_diff_ci/hi}{+16.65}
\defres{econ/jevagent_best_v2/wall/mean_diff_ci/lo}{+15.27}
\defres{econ/jevagent_best_v2/wall/median}{23.64}
\defres{econ/jevagent_best_v2/wall/median_diff}{+16.59}
\defres{econ/jevagent_best_v2/wall/median_diff_ci/hi}{+23.05}
\defres{econ/jevagent_best_v2/wall/median_diff_ci/lo}{+8.30}
\defres{econ/jevagent_best_v2/wall/ratio}{3.34}
\defres{econ/jevagent_best_v2/wall/ref_mean}{6.83}
\defres{econ/jevagent_best_v2/wall/ref_median}{7.05}
\defres{econ/jevagent_best_x/abs_ratio/astra}{11.8}
\defres{econ/jevagent_best_x/abs_ratio/sol}{2.8}
\defres{econ/jevagent_best_x/abs_savings/astra}{-0.00499}
\defres{econ/jevagent_best_x/abs_savings/frozen}{-0.000423}
\defres{econ/jevagent_best_x/abs_savings/sol}{-0.00118}
\defres{econ/jevagent_best_x/abs_savings_ci/astra/hi}{-0.00381}
\defres{econ/jevagent_best_x/abs_savings_ci/astra/lo}{-0.00621}
\defres{econ/jevagent_best_x/abs_savings_ci/frozen/hi}{-0.000395}
\defres{econ/jevagent_best_x/abs_savings_ci/frozen/lo}{-0.000451}
\defres{econ/jevagent_best_x/abs_savings_ci/sol/hi}{-0.00096}
\defres{econ/jevagent_best_x/abs_savings_ci/sol/lo}{-0.00141}
\defres{econ/jevagent_best_x/calllat/mean}{37.45}
\defres{econ/jevagent_best_x/calllat/mean_diff}{+3.92}
\defres{econ/jevagent_best_x/calllat/mean_diff_ci/hi}{+5.04}
\defres{econ/jevagent_best_x/calllat/mean_diff_ci/lo}{+2.69}
\defres{econ/jevagent_best_x/calllat/median}{40.09}
\defres{econ/jevagent_best_x/calllat/median_diff}{+4.62}
\defres{econ/jevagent_best_x/calllat/median_diff_ci/hi}{+8.21}
\defres{econ/jevagent_best_x/calllat/median_diff_ci/lo}{+2.17}
\defres{econ/jevagent_best_x/calllat/ratio}{1.12}
\defres{econ/jevagent_best_x/calllat/ref_mean}{33.53}
\defres{econ/jevagent_best_x/calllat/ref_median}{35.47}
\defres{econ/jevagent_best_x/concurrency}{8}
\defres{econ/jevagent_best_x/cost/astra}{0.133}
\defres{econ/jevagent_best_x/cost/frozen}{0.00246}
\defres{econ/jevagent_best_x/cost/sol}{0.0224}
\defres{econ/jevagent_best_x/lgcost/frozen}{-2.6097}
\defres{econ/jevagent_best_x/n}{500}
\defres{econ/jevagent_best_x/rel_change/astra}{+16.9}
\defres{econ/jevagent_best_x/rel_change/sol}{+15.2}
\defres{econ/jevagent_best_x/s2_share/astra}{99.7}
\defres{econ/jevagent_best_x/s2_share/frozen}{85.3}
\defres{econ/jevagent_best_x/s2_share/sol}{98.4}
\defres{econ/jevagent_best_x/savings/astra}{-3.9}
\defres{econ/jevagent_best_x/savings/frozen}{-20.8}
\defres{econ/jevagent_best_x/savings/sol}{-5.6}
\defres{econ/jevagent_best_x/savings_ci/astra/hi}{-3.0}
\defres{econ/jevagent_best_x/savings_ci/astra/lo}{-4.9}
\defres{econ/jevagent_best_x/savings_ci/frozen/hi}{-19.6}
\defres{econ/jevagent_best_x/savings_ci/frozen/lo}{-22.0}
\defres{econ/jevagent_best_x/savings_ci/sol/hi}{-4.5}
\defres{econ/jevagent_best_x/savings_ci/sol/lo}{-6.7}
\defres{econ/jevagent_best_x/wall/mean}{37.82}
\defres{econ/jevagent_best_x/wall/mean_diff}{+4.02}
\defres{econ/jevagent_best_x/wall/mean_diff_ci/hi}{+5.33}
\defres{econ/jevagent_best_x/wall/mean_diff_ci/lo}{+2.61}
\defres{econ/jevagent_best_x/wall/median}{40.52}
\defres{econ/jevagent_best_x/wall/median_diff}{+5.01}
\defres{econ/jevagent_best_x/wall/median_diff_ci/hi}{+8.88}
\defres{econ/jevagent_best_x/wall/median_diff_ci/lo}{+2.67}
\defres{econ/jevagent_best_x/wall/ratio}{1.12}
\defres{econ/jevagent_best_x/wall/ref_mean}{33.80}
\defres{econ/jevagent_best_x/wall/ref_median}{35.51}
\defres{econ/jevagent_default/abs_ratio/astra}{7.5}
\defres{econ/jevagent_default/abs_ratio/sol}{1.3}
\defres{econ/jevagent_default/abs_savings/astra}{0.0559}
\defres{econ/jevagent_default/abs_savings/frozen}{0.00748}
\defres{econ/jevagent_default/abs_savings/sol}{0.00952}
\defres{econ/jevagent_default/abs_savings_ci/astra/hi}{0.0608}
\defres{econ/jevagent_default/abs_savings_ci/astra/lo}{0.0512}
\defres{econ/jevagent_default/abs_savings_ci/frozen/hi}{0.00819}
\defres{econ/jevagent_default/abs_savings_ci/frozen/lo}{0.0068}
\defres{econ/jevagent_default/abs_savings_ci/sol/hi}{0.0104}
\defres{econ/jevagent_default/abs_savings_ci/sol/lo}{0.00866}
\defres{econ/jevagent_default/calllat/mean}{7.96}
\defres{econ/jevagent_default/calllat/mean_diff}{+1.16}
\defres{econ/jevagent_default/calllat/mean_diff_ci/hi}{+1.33}
\defres{econ/jevagent_default/calllat/mean_diff_ci/lo}{+0.96}
\defres{econ/jevagent_default/calllat/median}{8.07}
\defres{econ/jevagent_default/calllat/median_diff}{+1.06}
\defres{econ/jevagent_default/calllat/median_diff_ci/hi}{+1.33}
\defres{econ/jevagent_default/calllat/median_diff_ci/lo}{-0.16}
\defres{econ/jevagent_default/calllat/ratio}{1.17}
\defres{econ/jevagent_default/calllat/ref_mean}{6.80}
\defres{econ/jevagent_default/calllat/ref_median}{7.01}
\defres{econ/jevagent_default/concurrency}{8}
\defres{econ/jevagent_default/cost/astra}{0.217}
\defres{econ/jevagent_default/cost/frozen}{0.0338}
\defres{econ/jevagent_default/cost/sol}{0.0428}
\defres{econ/jevagent_default/lgcost/frozen}{-1.4708}
\defres{econ/jevagent_default/n}{500}
\defres{econ/jevagent_default/rel_change/astra}{+2.4}
\defres{econ/jevagent_default/rel_change/sol}{+0.1}
\defres{econ/jevagent_default/s2_share/astra}{99.5}
\defres{econ/jevagent_default/s2_share/frozen}{96.7}
\defres{econ/jevagent_default/s2_share/sol}{97.4}
\defres{econ/jevagent_default/savings/astra}{20.5}
\defres{econ/jevagent_default/savings/frozen}{18.1}
\defres{econ/jevagent_default/savings/sol}{18.2}
\defres{econ/jevagent_default/savings_ci/astra/hi}{22.0}
\defres{econ/jevagent_default/savings_ci/astra/lo}{19.0}
\defres{econ/jevagent_default/savings_ci/frozen/hi}{19.6}
\defres{econ/jevagent_default/savings_ci/frozen/lo}{16.6}
\defres{econ/jevagent_default/savings_ci/sol/hi}{19.7}
\defres{econ/jevagent_default/savings_ci/sol/lo}{16.7}
\defres{econ/jevagent_default/wall/mean}{7.67}
\defres{econ/jevagent_default/wall/mean_diff}{+0.84}
\defres{econ/jevagent_default/wall/mean_diff_ci/hi}{+1.02}
\defres{econ/jevagent_default/wall/mean_diff_ci/lo}{+0.65}
\defres{econ/jevagent_default/wall/median}{7.72}
\defres{econ/jevagent_default/wall/median_diff}{+0.67}
\defres{econ/jevagent_default/wall/median_diff_ci/hi}{+1.04}
\defres{econ/jevagent_default/wall/median_diff_ci/lo}{-0.47}
\defres{econ/jevagent_default/wall/ratio}{1.12}
\defres{econ/jevagent_default/wall/ref_mean}{6.83}
\defres{econ/jevagent_default/wall/ref_median}{7.05}
\defres{econ/jevagent_minus_tool/abs_ratio/astra}{0.4}
\defres{econ/jevagent_minus_tool/abs_ratio/sol}{0.3}
\defres{econ/jevagent_minus_tool/abs_savings/astra}{-0.000166}
\defres{econ/jevagent_minus_tool/abs_savings/frozen}{-0.000429}
\defres{econ/jevagent_minus_tool/abs_savings/sol}{-0.000137}
\defres{econ/jevagent_minus_tool/abs_savings_ci/astra/hi}{0.00392}
\defres{econ/jevagent_minus_tool/abs_savings_ci/astra/lo}{-0.00522}
\defres{econ/jevagent_minus_tool/abs_savings_ci/frozen/hi}{0.000194}
\defres{econ/jevagent_minus_tool/abs_savings_ci/frozen/lo}{-0.0012}
\defres{econ/jevagent_minus_tool/abs_savings_ci/sol/hi}{0.000679}
\defres{econ/jevagent_minus_tool/abs_savings_ci/sol/lo}{-0.00114}
\defres{econ/jevagent_minus_tool/calllat/mean}{8.32}
\defres{econ/jevagent_minus_tool/calllat/mean_diff}{+2.25}
\defres{econ/jevagent_minus_tool/calllat/mean_diff_ci/hi}{+2.51}
\defres{econ/jevagent_minus_tool/calllat/mean_diff_ci/lo}{+1.96}
\defres{econ/jevagent_minus_tool/calllat/median}{9.47}
\defres{econ/jevagent_minus_tool/calllat/median_diff}{+2.58}
\defres{econ/jevagent_minus_tool/calllat/median_diff_ci/hi}{+3.69}
\defres{econ/jevagent_minus_tool/calllat/median_diff_ci/lo}{+1.69}
\defres{econ/jevagent_minus_tool/calllat/ratio}{1.37}
\defres{econ/jevagent_minus_tool/calllat/ref_mean}{6.08}
\defres{econ/jevagent_minus_tool/calllat/ref_median}{6.89}
\defres{econ/jevagent_minus_tool/concurrency}{8}
\defres{econ/jevagent_minus_tool/cost/astra}{0.27}
\defres{econ/jevagent_minus_tool/cost/frozen}{0.0413}
\defres{econ/jevagent_minus_tool/cost/sol}{0.0519}
\defres{econ/jevagent_minus_tool/lgcost/frozen}{-1.3838}
\defres{econ/jevagent_minus_tool/n}{200}
\defres{econ/jevagent_minus_tool/rel_change/astra}{+1.0}
\defres{econ/jevagent_minus_tool/rel_change/sol}{+0.8}
\defres{econ/jevagent_minus_tool/s2_share/astra}{99.9}
\defres{econ/jevagent_minus_tool/s2_share/frozen}{99.2}
\defres{econ/jevagent_minus_tool/s2_share/sol}{99.3}
\defres{econ/jevagent_minus_tool/savings/astra}{-0.1}
\defres{econ/jevagent_minus_tool/savings/frozen}{-1.0}
\defres{econ/jevagent_minus_tool/savings/sol}{-0.3}
\defres{econ/jevagent_minus_tool/savings_ci/astra/hi}{1.4}
\defres{econ/jevagent_minus_tool/savings_ci/astra/lo}{-1.9}
\defres{econ/jevagent_minus_tool/savings_ci/frozen/hi}{0.5}
\defres{econ/jevagent_minus_tool/savings_ci/frozen/lo}{-3.0}
\defres{econ/jevagent_minus_tool/savings_ci/sol/hi}{1.3}
\defres{econ/jevagent_minus_tool/savings_ci/sol/lo}{-2.2}
\defres{econ/jevagent_minus_tool/wall/mean}{8.26}
\defres{econ/jevagent_minus_tool/wall/mean_diff}{+2.16}
\defres{econ/jevagent_minus_tool/wall/mean_diff_ci/hi}{+2.43}
\defres{econ/jevagent_minus_tool/wall/mean_diff_ci/lo}{+1.87}
\defres{econ/jevagent_minus_tool/wall/median}{9.27}
\defres{econ/jevagent_minus_tool/wall/median_diff}{+2.34}
\defres{econ/jevagent_minus_tool/wall/median_diff_ci/hi}{+3.58}
\defres{econ/jevagent_minus_tool/wall/median_diff_ci/lo}{+1.58}
\defres{econ/jevagent_minus_tool/wall/ratio}{1.35}
\defres{econ/jevagent_minus_tool/wall/ref_mean}{6.10}
\defres{econ/jevagent_minus_tool/wall/ref_median}{6.93}
\defres{econ/llm_only/calllat/mean}{6.80}
\defres{econ/llm_only/calllat/median}{7.01}
\defres{econ/llm_only/concurrency}{8}
\defres{econ/llm_only/cost/astra}{0.273}
\defres{econ/llm_only/cost/frozen}{0.0413}
\defres{econ/llm_only/cost/sol}{0.0523}
\defres{econ/llm_only/lgcost/frozen}{-1.3841}
\defres{econ/llm_only/n}{500}
\defres{econ/llm_only/s2_share/astra}{100.0}
\defres{econ/llm_only/s2_share/frozen}{100.0}
\defres{econ/llm_only/s2_share/sol}{100.0}
\defres{econ/llm_only/wall/mean}{6.83}
\defres{econ/llm_only/wall/median}{7.05}
\defres{econ/llm_only_x/calllat/mean}{33.53}
\defres{econ/llm_only_x/calllat/median}{35.47}
\defres{econ/llm_only_x/concurrency}{8}
\defres{econ/llm_only_x/cost/astra}{0.128}
\defres{econ/llm_only_x/cost/frozen}{0.00203}
\defres{econ/llm_only_x/cost/sol}{0.0212}
\defres{econ/llm_only_x/lgcost/frozen}{-2.6918}
\defres{econ/llm_only_x/n}{500}
\defres{econ/llm_only_x/s2_share/astra}{100.0}
\defres{econ/llm_only_x/s2_share/frozen}{100.0}
\defres{econ/llm_only_x/s2_share/sol}{100.0}
\defres{econ/llm_only_x/wall/mean}{33.80}
\defres{econ/llm_only_x/wall/median}{35.51}
\defres{econ/llm_only_xsmall/abs_savings/frozen}{0.00153}
\defres{econ/llm_only_xsmall/abs_savings_ci/frozen/hi}{0.00159}
\defres{econ/llm_only_xsmall/abs_savings_ci/frozen/lo}{0.00147}
\defres{econ/llm_only_xsmall/calllat/mean}{23.39}
\defres{econ/llm_only_xsmall/calllat/mean_diff}{-10.15}
\defres{econ/llm_only_xsmall/calllat/mean_diff_ci/hi}{-8.54}
\defres{econ/llm_only_xsmall/calllat/mean_diff_ci/lo}{-11.79}
\defres{econ/llm_only_xsmall/calllat/median}{22.25}
\defres{econ/llm_only_xsmall/calllat/median_diff}{-13.22}
\defres{econ/llm_only_xsmall/calllat/median_diff_ci/hi}{-3.98}
\defres{econ/llm_only_xsmall/calllat/median_diff_ci/lo}{-15.09}
\defres{econ/llm_only_xsmall/calllat/ratio}{0.70}
\defres{econ/llm_only_xsmall/calllat/ref_mean}{33.53}
\defres{econ/llm_only_xsmall/calllat/ref_median}{35.47}
\defres{econ/llm_only_xsmall/concurrency}{8}
\defres{econ/llm_only_xsmall/cost/frozen}{0.000503}
\defres{econ/llm_only_xsmall/lgcost/frozen}{-3.2987}
\defres{econ/llm_only_xsmall/n}{500}
\defres{econ/llm_only_xsmall/s2_share/frozen}{100.0}
\defres{econ/llm_only_xsmall/savings/frozen}{75.3}
\defres{econ/llm_only_xsmall/savings_ci/frozen/hi}{75.7}
\defres{econ/llm_only_xsmall/savings_ci/frozen/lo}{74.8}
\defres{econ/llm_only_xsmall/wall/mean}{24.04}
\defres{econ/llm_only_xsmall/wall/mean_diff}{-9.76}
\defres{econ/llm_only_xsmall/wall/mean_diff_ci/hi}{-7.93}
\defres{econ/llm_only_xsmall/wall/mean_diff_ci/lo}{-11.58}
\defres{econ/llm_only_xsmall/wall/median}{22.44}
\defres{econ/llm_only_xsmall/wall/median_diff}{-13.07}
\defres{econ/llm_only_xsmall/wall/median_diff_ci/hi}{-3.80}
\defres{econ/llm_only_xsmall/wall/median_diff_ci/lo}{-14.95}
\defres{econ/llm_only_xsmall/wall/ratio}{0.71}
\defres{econ/llm_only_xsmall/wall/ref_mean}{33.80}
\defres{econ/llm_only_xsmall/wall/ref_median}{35.51}
\defres{econ/meta/n_boot}{10{,}000}
\defres{econ/meta/n_checks}{61}
\defres{econ/meta/reasoning_tokens}{0}
\defres{econ/meta/seed}{0}
\defres{econ/price/astra/cached}{1.00}
\defres{econ/price/astra/input}{10.00}
\defres{econ/price/astra/model}{gpt-6-astra}
\defres{econ/price/astra/output}{50.00}
\defres{econ/price/frozen/deepseek/deepseek-v4-flash/cached}{0.0056}
\defres{econ/price/frozen/deepseek/deepseek-v4-flash/input}{0.0280}
\defres{econ/price/frozen/deepseek/deepseek-v4-flash/output}{0.0560}
\defres{econ/price/frozen/deepseek/deepseek-v4-pro/cached}{0.0174}
\defres{econ/price/frozen/deepseek/deepseek-v4-pro/input}{0.2088}
\defres{econ/price/frozen/deepseek/deepseek-v4-pro/output}{0.4176}
\defres{econ/price/frozen/gemini-3.5-flash/cached}{0.1500}
\defres{econ/price/frozen/gemini-3.5-flash/input}{1.5000}
\defres{econ/price/frozen/gemini-3.5-flash/output}{9.0000}
\defres{econ/price/sol/cached}{0.10}
\defres{econ/price/sol/input}{2.00}
\defres{econ/price/sol/model}{gpt-6.1-sol}
\defres{econ/price/sol/output}{10.00}
\makeatother


==> generated/explore.tex <==
\makeatletter
\providecommand{\res}[1]{\ifcsname jevres@#1\endcsname\csname jevres@#1\endcsname\else\tbd\fi}
\providecommand{\defres}[2]{\expandafter\def\csname jevres@#1\endcsname{#2}}
\defres{explore/startlux_live/frozen/api_cost}{0.0145}
\defres{explore/startlux_live/frozen/corpus_acc}{99.2}
\defres{explore/startlux_live/frozen/e1_acc}{88.4}
\defres{explore/startlux_live/frozen/e1_vs_jev_ci/hi}{0.3}
\defres{explore/startlux_live/frozen/e1_vs_jev_ci/lo}{$-$3.4}
\defres{explore/startlux_live/frozen/e1_vs_jev}{$-$1.5}
\defres{explore/startlux_live/frozen/live_n}{200}
\defres{explore/startlux_live/frozen/live_success}{100.0}
\defres{explore/startlux_live/frozen/live_vs_jev_ci/hi}{22.8}
\defres{explore/startlux_live/frozen/live_vs_jev_ci/lo}{12.1}
\defres{explore/startlux_live/frozen/live_vs_jev}{17.0}
\defres{explore/startlux_live/frozen/own_acc}{100.0}
\defres{explore/startlux_live/frozen/steps}{7.5}
\defres{explore/startlux_live/intern/api_cost}{0.0080}
\defres{explore/startlux_live/intern/corpus_acc}{75.2}
\defres{explore/startlux_live/intern/e1_acc}{88.2}
\defres{explore/startlux_live/intern/e1_vs_jev_ci/hi}{$-$0.5}
\defres{explore/startlux_live/intern/e1_vs_jev_ci/lo}{$-$2.9}
\defres{explore/startlux_live/intern/e1_vs_jev}{$-$1.7}
\defres{explore/startlux_live/intern/live_n}{200}
\defres{explore/startlux_live/intern/live_success}{26.5}
\defres{explore/startlux_live/intern/live_vs_jev_ci/hi}{$-$49.0}
\defres{explore/startlux_live/intern/live_vs_jev_ci/lo}{$-$62.8}
\defres{explore/startlux_live/intern/live_vs_jev}{$-$56.5}
\defres{explore/startlux_live/intern/own_acc}{62.2}
\defres{explore/startlux_live/intern/steps}{4.6}
\defres{explore/startlux_live/jev/api_cost}{0.0144}
\defres{explore/startlux_live/jev/corpus_acc}{91.5}
\defres{explore/startlux_live/jev/e1_acc}{89.9}
\defres{explore/startlux_live/jev/live_n}{200}
\defres{explore/startlux_live/jev/live_success}{83.0}
\defres{explore/startlux_live/jev/own_acc}{91.0}
\defres{explore/startlux_live/jev/steps}{7.0}
\defres{explore/startlux_live/kendall/corpus_acc}{1.00}
\defres{explore/startlux_live/kendall/corpus_vs_live_all_rows}{0.71}
\defres{explore/startlux_live/kendall/e1_acc}{0.60}
\defres{explore/startlux_live/kendall/e1_vs_live_all_rows}{0.15}
\defres{explore/startlux_live/kendall/live_success}{0.60}
\defres{explore/startlux_live/kendall/own_acc}{0.80}
\defres{explore/startlux_live/sl0.8b/api_cost}{0.0143}
\defres{explore/startlux_live/sl0.8b/corpus_acc}{48.3}
\defres{explore/startlux_live/sl0.8b/e1_acc}{88.2}
\defres{explore/startlux_live/sl0.8b/e1_vs_jev_ci/hi}{$-$0.3}
\defres{explore/startlux_live/sl0.8b/e1_vs_jev_ci/lo}{$-$3.2}
\defres{explore/startlux_live/sl0.8b/e1_vs_jev}{$-$1.7}
\defres{explore/startlux_live/sl0.8b/live_n}{200}
\defres{explore/startlux_live/sl0.8b/live_success}{17.5}
\defres{explore/startlux_live/sl0.8b/live_vs_jev_ci/hi}{$-$58.1}
\defres{explore/startlux_live/sl0.8b/live_vs_jev_ci/lo}{$-$71.4}
\defres{explore/startlux_live/sl0.8b/live_vs_jev}{$-$65.5}
\defres{explore/startlux_live/sl0.8b/own_acc}{35.8}
\defres{explore/startlux_live/sl0.8b/steps}{7.0}
\defres{explore/startlux_live/sl27b/api_cost}{0.0133}
\defres{explore/startlux_live/sl27b/corpus_acc}{93.9}
\defres{explore/startlux_live/sl27b/e1_acc}{90.8}
\defres{explore/startlux_live/sl27b/e1_vs_jev_ci/hi}{2.1}
\defres{explore/startlux_live/sl27b/e1_vs_jev_ci/lo}{$-$0.5}
\defres{explore/startlux_live/sl27b/e1_vs_jev}{0.8}
\defres{explore/startlux_live/sl27b/live_n}{200}
\defres{explore/startlux_live/sl27b/live_success}{63.0}
\defres{explore/startlux_live/sl27b/live_vs_jev_ci/hi}{$-$14.4}
\defres{explore/startlux_live/sl27b/live_vs_jev_ci/lo}{$-$25.7}
\defres{explore/startlux_live/sl27b/live_vs_jev}{$-$20.0}
\defres{explore/startlux_live/sl27b/own_acc}{87.7}
\defres{explore/startlux_live/sl27b/steps}{6.8}
\defres{explore/startlux_live/sl2b/api_cost}{0.0049}
\defres{explore/startlux_live/sl2b/corpus_acc}{68.4}
\defres{explore/startlux_live/sl2b/e1_acc}{89.9}
\defres{explore/startlux_live/sl2b/e1_vs_jev_ci/hi}{1.5}
\defres{explore/startlux_live/sl2b/e1_vs_jev_ci/lo}{$-$1.5}
\defres{explore/startlux_live/sl2b/e1_vs_jev}{0.0}
\defres{explore/startlux_live/sl2b/live_n}{200}
\defres{explore/startlux_live/sl2b/live_success}{6.5}
\defres{explore/startlux_live/sl2b/live_vs_jev_ci/hi}{$-$69.4}
\defres{explore/startlux_live/sl2b/live_vs_jev_ci/lo}{$-$81.7}
\defres{explore/startlux_live/sl2b/live_vs_jev}{$-$76.5}
\defres{explore/startlux_live/sl2b/own_acc}{59.5}
\defres{explore/startlux_live/sl2b/steps}{3.8}
\defres{explore/startlux_live/sl4b/api_cost}{0.0116}
\defres{explore/startlux_live/sl4b/corpus_acc}{89.1}
\defres{explore/startlux_live/sl4b/e1_acc}{91.3}
\defres{explore/startlux_live/sl4b/e1_vs_jev_ci/hi}{2.6}
\defres{explore/startlux_live/sl4b/e1_vs_jev_ci/lo}{0.1}
\defres{explore/startlux_live/sl4b/e1_vs_jev}{1.3}
\defres{explore/startlux_live/sl4b/live_n}{200}
\defres{explore/startlux_live/sl4b/live_success}{60.0}
\defres{explore/startlux_live/sl4b/live_vs_jev_ci/hi}{$-$17.0}
\defres{explore/startlux_live/sl4b/live_vs_jev_ci/lo}{$-$28.9}
\defres{explore/startlux_live/sl4b/live_vs_jev}{$-$23.0}
\defres{explore/startlux_live/sl4b/own_acc}{81.6}
\defres{explore/startlux_live/sl4b/steps}{6.2}
\defres{explore/startlux_live/sl9b/api_cost}{0.0142}
\defres{explore/startlux_live/sl9b/corpus_acc}{91.8}
\defres{explore/startlux_live/sl9b/e1_acc}{92.2}
\defres{explore/startlux_live/sl9b/e1_vs_jev_ci/hi}{3.4}
\defres{explore/startlux_live/sl9b/e1_vs_jev_ci/lo}{1.1}
\defres{explore/startlux_live/sl9b/e1_vs_jev}{2.2}
\defres{explore/startlux_live/sl9b/live_n}{200}
\defres{explore/startlux_live/sl9b/live_success}{74.0}
\defres{explore/startlux_live/sl9b/live_vs_jev_ci/hi}{$-$4.9}
\defres{explore/startlux_live/sl9b/live_vs_jev_ci/lo}{$-$13.3}
\defres{explore/startlux_live/sl9b/live_vs_jev}{$-$9.0}
\defres{explore/startlux_live/sl9b/own_acc}{91.0}
\defres{explore/startlux_live/sl9b/steps}{7.1}
\defres{explore/telecom_rl/gonogo/decision}{no-go}
\defres{explore/telecom_rl/gonogo/n_val_tasks}{10}
\defres{explore/telecom_rl/gonogo/r1/go}{no}
\defres{explore/telecom_rl/gonogo/r1/max_repeats}{0}
\defres{explore/telecom_rl/gonogo/r1/n_tasks}{5}
\defres{explore/telecom_rl/gonogo/r1/s1_calls}{80}
\defres{explore/telecom_rl/gonogo/r1/too_many_errors}{3}
\defres{explore/telecom_rl/gonogo/r1/tool_errors}{37}
\defres{explore/telecom_rl/gonogo/r1/ts_decisions}{70}
\defres{explore/telecom_rl/gonogo/r1/unknown_tool_calls}{36}
\defres{explore/telecom_rl/gonogo/r2/go}{no}
\defres{explore/telecom_rl/gonogo/r2/max_repeats}{23}
\defres{explore/telecom_rl/gonogo/r2/n_tasks}{5}
\defres{explore/telecom_rl/gonogo/r2/s1_calls}{167}
\defres{explore/telecom_rl/gonogo/r2/too_many_errors}{0}
\defres{explore/telecom_rl/gonogo/r2/tool_errors}{0}
\defres{explore/telecom_rl/gonogo/r2/ts_decisions}{118}
\defres{explore/telecom_rl/gonogo/r2/unknown_tool_calls}{0}
\defres{explore/telecom_rl/gonogo/rounds}{2}
\defres{explore/telecom_rl/gonogo/spend}{1.79}
\makeatother


==> generated/failure_audit.tex <==
\makeatletter
\providecommand{\res}[1]{\ifcsname jevres@#1\endcsname\csname jevres@#1\endcsname\else\tbd\fi}
\providecommand{\defres}[2]{\expandafter\def\csname jevres@#1\endcsname{#2}}
\defres{audit/base/fail/split_after_reflection}{14}
\defres{audit/base/success/no_reflection_no_split}{83}
\defres{audit/base/success/no_reflection_split}{1}
\defres{audit/base/success/no_split}{282}
\defres{audit/base/success/split_after_reflection}{119}
\defres{audit/base/success/split_before_reflection}{1}
\defres{audit/base_n/fail}{14}
\defres{audit/base_n/success}{486}
\defres{audit/case/defer/llm_tool}{\texttt{ask\_user}}
\defres{audit/case/defer/n_steps}{5}
\defres{audit/case/defer/s1_conf}{0.99}
\defres{audit/case/defer/s1_tool}{\texttt{refund}}
\defres{audit/case/defer/seed}{300034}
\defres{audit/case/defer/step}{3}
\defres{audit/case/defer/variant}{method}
\defres{audit/case/fail/cascade/accepted}{accepted}
\defres{audit/case/fail/cascade/s1_conf}{1.00}
\defres{audit/case/fail/cascade/s1_tool}{\texttt{cancel\_order}}
\defres{audit/case/fail/div_step}{4}
\defres{audit/case/fail/div_tool}{\texttt{ask\_user}}
\defres{audit/case/fail/first_fire}{2}
\defres{audit/case/fail/profile/accepted}{deferred}
\defres{audit/case/fail/profile/s1_conf}{0.66}
\defres{audit/case/fail/profile/s1_tool}{\texttt{cancel\_order}}
\defres{audit/case/fail/seed}{300080}
\defres{audit/case/fail/split_step}{4}
\defres{audit/case/fail/variant}{order}
\defres{audit/consistent}{no}
\defres{audit/fail/div_by_llm}{10}
\defres{audit/fail/div_by_s1_arg}{0}
\defres{audit/fail/div_by_s1_tool}{4}
\defres{audit/fail/div_step_median}{3.0}
\defres{audit/fail/diverged}{14}
\defres{audit/fail/fatal_by_llm}{10}
\defres{audit/fail/fatal_by_s1}{4}
\defres{audit/fail/fatal_tool/refund}{14}
\defres{audit/fail/fired_any}{14}
\defres{audit/fail/fired_before_div}{14}
\defres{audit/fail/label/accepted_system_1_tool_choice_after_a_reflection}{4}
\defres{audit/fail/label/llm_choice_after_a_reflection}{10}
\defres{audit/fail/n}{14}
\defres{audit/fail/no_reflection_split}{0}
\defres{audit/fail/no_split}{0}
\defres{audit/fail/premature_finish}{0}
\defres{audit/fail/s1_err_any}{4}
\defres{audit/fail/s1_err_arg}{0}
\defres{audit/fail/s1_err_tool}{4}
\defres{audit/fail/split_accept_flip}{13}
\defres{audit/fail/split_after_reflection}{14}
\defres{audit/fail/split_before_reflection}{0}
\defres{audit/fail/split_s1_same_tool}{14}
\defres{audit/fail/success}{0}
\defres{audit/fail/term_budget}{0}
\defres{audit/fail/term_strict}{14}
\defres{audit/fail/unclear}{0}
\defres{audit/fail_cascade/div_by_llm}{0}
\defres{audit/fail_cascade/div_by_s1_arg}{0}
\defres{audit/fail_cascade/div_by_s1_tool}{0}
\defres{audit/fail_cascade/diverged}{0}
\defres{audit/fail_cascade/fatal_by_llm}{0}
\defres{audit/fail_cascade/fatal_by_s1}{0}
\defres{audit/fail_cascade/label/no_divergence}{14}
\defres{audit/fail_cascade/n}{14}
\defres{audit/fail_cascade/premature_finish}{0}
\defres{audit/fail_cascade/s1_err_any}{0}
\defres{audit/fail_cascade/s1_err_arg}{0}
\defres{audit/fail_cascade/s1_err_tool}{0}
\defres{audit/fail_cascade/success}{14}
\defres{audit/fail_cascade/term_budget}{0}
\defres{audit/fail_cascade/term_strict}{0}
\defres{audit/fail_cascade/unclear}{0}
\defres{audit/fail_llm/div_by_llm}{1}
\defres{audit/fail_llm/div_by_s1_arg}{0}
\defres{audit/fail_llm/div_by_s1_tool}{0}
\defres{audit/fail_llm/div_step_median}{4.0}
\defres{audit/fail_llm/diverged}{1}
\defres{audit/fail_llm/fatal_by_llm}{1}
\defres{audit/fail_llm/fatal_by_s1}{0}
\defres{audit/fail_llm/fatal_tool/refund}{1}
\defres{audit/fail_llm/label/llm_choice}{1}
\defres{audit/fail_llm/label/no_divergence}{13}
\defres{audit/fail_llm/n}{14}
\defres{audit/fail_llm/premature_finish}{0}
\defres{audit/fail_llm/s1_err_any}{0}
\defres{audit/fail_llm/s1_err_arg}{0}
\defres{audit/fail_llm/s1_err_tool}{0}
\defres{audit/fail_llm/success}{13}
\defres{audit/fail_llm/term_budget}{0}
\defres{audit/fail_llm/term_strict}{1}
\defres{audit/fail_llm/unclear}{0}
\defres{audit/match/div_by_llm}{0}
\defres{audit/match/div_by_s1_arg}{0}
\defres{audit/match/div_by_s1_tool}{0}
\defres{audit/match/diverged}{0}
\defres{audit/match/fatal_by_llm}{0}
\defres{audit/match/fatal_by_s1}{0}
\defres{audit/match/fired_any}{12}
\defres{audit/match/fired_before_div}{0}
\defres{audit/match/label/no_divergence}{14}
\defres{audit/match/n}{14}
\defres{audit/match/no_reflection_split}{0}
\defres{audit/match/no_split}{12}
\defres{audit/match/premature_finish}{0}
\defres{audit/match/s1_err_any}{0}
\defres{audit/match/s1_err_arg}{0}
\defres{audit/match/s1_err_tool}{0}
\defres{audit/match/split_accept_flip}{0}
\defres{audit/match/split_after_reflection}{0}
\defres{audit/match/split_before_reflection}{0}
\defres{audit/match/split_s1_same_tool}{0}
\defres{audit/match/success}{14}
\defres{audit/match/term_budget}{0}
\defres{audit/match/term_strict}{0}
\defres{audit/match/unclear}{0}
\defres{audit/match_cascade/div_by_llm}{0}
\defres{audit/match_cascade/div_by_s1_arg}{0}
\defres{audit/match_cascade/div_by_s1_tool}{0}
\defres{audit/match_cascade/diverged}{0}
\defres{audit/match_cascade/fatal_by_llm}{0}
\defres{audit/match_cascade/fatal_by_s1}{0}
\defres{audit/match_cascade/label/no_divergence}{14}
\defres{audit/match_cascade/n}{14}
\defres{audit/match_cascade/premature_finish}{0}
\defres{audit/match_cascade/s1_err_any}{0}
\defres{audit/match_cascade/s1_err_arg}{0}
\defres{audit/match_cascade/s1_err_tool}{0}
\defres{audit/match_cascade/success}{14}
\defres{audit/match_cascade/term_budget}{0}
\defres{audit/match_cascade/term_strict}{0}
\defres{audit/match_cascade/unclear}{0}
\defres{audit/n_failures}{14}
\defres{audit/reading}{these counts do not identify how the failures arose}
\defres{audit/success_all/div_by_llm}{9}
\defres{audit/success_all/div_by_s1_arg}{0}
\defres{audit/success_all/div_by_s1_tool}{0}
\defres{audit/success_all/div_step_median}{3.0}
\defres{audit/success_all/diverged}{9}
\defres{audit/success_all/fatal_by_llm}{0}
\defres{audit/success_all/fatal_by_s1}{0}
\defres{audit/success_all/fired_any}{402}
\defres{audit/success_all/fired_before_div}{9}
\defres{audit/success_all/label/llm_choice_after_a_reflection}{9}
\defres{audit/success_all/label/no_divergence}{477}
\defres{audit/success_all/n}{486}
\defres{audit/success_all/no_reflection_split}{1}
\defres{audit/success_all/no_split}{282}
\defres{audit/success_all/premature_finish}{0}
\defres{audit/success_all/s1_err_any}{0}
\defres{audit/success_all/s1_err_arg}{0}
\defres{audit/success_all/s1_err_tool}{0}
\defres{audit/success_all/split_accept_flip}{110}
\defres{audit/success_all/split_after_reflection}{119}
\defres{audit/success_all/split_before_reflection}{1}
\defres{audit/success_all/split_s1_same_tool}{114}
\defres{audit/success_all/success}{486}
\defres{audit/success_all/term_budget}{0}
\defres{audit/success_all/term_strict}{0}
\defres{audit/success_all/unclear}{0}
\defres{audit/tau}{1.00}
\makeatother


==> generated/fig1_episode.tex <==
\makeatletter
\providecommand{\res}[1]{\ifcsname jevres@#1\endcsname\csname jevres@#1\endcsname\else\tbd\fi}
\providecommand{\defres}[2]{\expandafter\def\csname jevres@#1\endcsname{#2}}
\defres{fig1/accept/chosen}{cancel\_order}
\defres{fig1/accept/conf}{1.00}
\defres{fig1/accept/llm_calls}{0}
\defres{fig1/accept/n_args_model}{2}
\defres{fig1/accept/n_more}{66}
\defres{fig1/accept/opt/1/name}{cancel\_order}
\defres{fig1/accept/opt/1/p}{1.00}
\defres{fig1/accept/opt/1/pnum}{0.9999}
\defres{fig1/accept/opt/2/name}{verify\_identity}
\defres{fig1/accept/opt/2/p}{$<$0.01}
\defres{fig1/accept/opt/2/pnum}{0.0000}
\defres{fig1/accept/opt/3/name}{get\_shipping\_zones}
\defres{fig1/accept/opt/3/p}{$<$0.01}
\defres{fig1/accept/opt/3/pnum}{0.0000}
\defres{fig1/accept/step}{4}
\defres{fig1/cost/s1}{0.00011}
\defres{fig1/cost/s2}{0.0042}
\defres{fig1/cost_ratio}{40}
\defres{fig1/defer/chosen}{ask\_user}
\defres{fig1/defer/conf}{0.62}
\defres{fig1/defer/llm_calls}{1}
\defres{fig1/defer/n_more}{66}
\defres{fig1/defer/opt/1/name}{ask\_user}
\defres{fig1/defer/opt/1/p}{0.63}
\defres{fig1/defer/opt/1/pnum}{0.6300}
\defres{fig1/defer/opt/2/name}{cancel\_order}
\defres{fig1/defer/opt/2/p}{0.37}
\defres{fig1/defer/opt/2/pnum}{0.3700}
\defres{fig1/defer/opt/3/name}{verify\_identity}
\defres{fig1/defer/opt/3/p}{$<$0.01}
\defres{fig1/defer/opt/3/pnum}{0.0000}
\defres{fig1/defer/step}{3}
\defres{fig1/latency/s1}{223}
\defres{fig1/latency/s2}{809}
\defres{fig1/latency_ratio}{3.6}
\defres{fig1/n_by_model}{2}
\defres{fig1/n_options}{69}
\defres{fig1/n_steps}{5}
\defres{fig1/seed}{300000}
\defres{fig1/step/1/by}{s2}
\defres{fig1/step/1/tool}{find\_user}
\defres{fig1/step/2/by}{s1}
\defres{fig1/step/2/tool}{get\_orders}
\defres{fig1/step/3/by}{s2}
\defres{fig1/step/3/tool}{ask\_user}
\defres{fig1/step/4/by}{s1}
\defres{fig1/step/4/tool}{cancel\_order}
\defres{fig1/step/5/by}{s2}
\defres{fig1/step/5/tool}{finish}
\defres{fig1/task}{The customer Jia Haddad asked us to cancel their pending order.}
\defres{fig1/task_id}{jevgym-clarify-300000-d60-near-strict}
\defres{fig1/tauhat}{1.00}
\makeatother


==> generated/hard_ni.tex <==
\makeatletter
\providecommand{\defres}[2]{\expandafter\def\csname jevres@#1\endcsname{#2}}
\defres{hardni/margin}{3}
\defres{hardni/e11/n}{140}
\defres{hardni/e11/wins}{13}
\defres{hardni/e11/losses}{7}
\defres{hardni/e11/delta}{$+$4.3}
\defres{hardni/e11/lo}{$-$2.1}
\defres{hardni/e11/hi}{$+$11.1}
\defres{hardni/e11/p}{0.014}
\defres{hardni/e11/ni}{yes}
\defres{hardni/e13_luna/n}{100}
\defres{hardni/e13_luna/wins}{44}
\defres{hardni/e13_luna/losses}{6}
\defres{hardni/e13_luna/delta}{$+$38.0}
\defres{hardni/e13_luna/lo}{$+$25.8}
\defres{hardni/e13_luna/hi}{$+$49.2}
\defres{hardni/e13_luna/p}{0.000}
\defres{hardni/e13_luna/ni}{yes}
\defres{hardni/e19/n}{200}
\defres{hardni/e19/wins}{18}
\defres{hardni/e19/losses}{16}
\defres{hardni/e19/delta}{$+$1.0}
\defres{hardni/e19/lo}{$-$4.9}
\defres{hardni/e19/hi}{$+$6.9}
\defres{hardni/e19/p}{0.091}
\defres{hardni/e19/ni}{no}
\defres{hardni/e23/n}{134}
\defres{hardni/e23/wins}{14}
\defres{hardni/e23/losses}{13}
\defres{hardni/e23/delta}{$+$0.7}
\defres{hardni/e23/lo}{$-$7.1}
\defres{hardni/e23/hi}{$+$8.7}
\defres{hardni/e23/p}{0.175}
\defres{hardni/e23/ni}{no}
\defres{hardni/e4/n}{100}
\defres{hardni/e4/wins}{3}
\defres{hardni/e4/losses}{3}
\defres{hardni/e4/delta}{$+$0.0}
\defres{hardni/e4/lo}{$-$5.9}
\defres{hardni/e4/hi}{$+$5.9}
\defres{hardni/e4/p}{0.135}
\defres{hardni/e4/ni}{no}
\defres{hardni/e4b/n}{100}
\defres{hardni/e4b/wins}{8}
\defres{hardni/e4b/losses}{3}
\defres{hardni/e4b/delta}{$+$5.0}
\defres{hardni/e4b/lo}{$-$1.7}
\defres{hardni/e4b/hi}{$+$12.5}
\defres{hardni/e4b/p}{0.012}
\defres{hardni/e4b/ni}{yes}
\defres{hardni/e4r/n}{300}
\defres{hardni/e4r/wins}{9}
\defres{hardni/e4r/losses}{12}
\defres{hardni/e4r/delta}{$-$1.0}
\defres{hardni/e4r/lo}{$-$4.3}
\defres{hardni/e4r/hi}{$+$2.2}
\defres{hardni/e4r/p}{0.108}
\defres{hardni/e4r/ni}{no}
\defres{hardni/e6a/n}{140}
\defres{hardni/e6a/wins}{4}
\defres{hardni/e6a/losses}{4}
\defres{hardni/e6a/delta}{$+$0.0}
\defres{hardni/e6a/lo}{$-$4.7}
\defres{hardni/e6a/hi}{$+$4.7}
\defres{hardni/e6a/p}{0.092}
\defres{hardni/e6a/ni}{no}
\defres{hardni/e7b_jev/n}{200}
\defres{hardni/e7b_jev/wins}{38}
\defres{hardni/e7b_jev/losses}{31}
\defres{hardni/e7b_jev/delta}{$+$3.5}
\defres{hardni/e7b_jev/lo}{$-$4.7}
\defres{hardni/e7b_jev/hi}{$+$11.7}
\defres{hardni/e7b_jev/p}{0.061}
\defres{hardni/e7b_jev/ni}{no}
\defres{hardni/e7b_rl/n}{200}
\defres{hardni/e7b_rl/wins}{0}
\defres{hardni/e7b_rl/losses}{131}
\defres{hardni/e7b_rl/delta}{$-$65.5}
\defres{hardni/e7b_rl/lo}{$-$71.7}
\defres{hardni/e7b_rl/hi}{$-$58.7}
\defres{hardni/e7b_rl/p}{1.000}
\defres{hardni/e7b_rl/ni}{no}
\defres{hardni/e7e_jev/n}{100}
\defres{hardni/e7e_jev/wins}{9}
\defres{hardni/e7e_jev/losses}{7}
\defres{hardni/e7e_jev/delta}{$+$2.0}
\defres{hardni/e7e_jev/lo}{$-$6.3}
\defres{hardni/e7e_jev/hi}{$+$10.5}
\defres{hardni/e7e_jev/p}{0.117}
\defres{hardni/e7e_jev/ni}{no}
\defres{hardni/e7f/n}{200}
\defres{hardni/e7f/wins}{21}
\defres{hardni/e7f/losses}{25}
\defres{hardni/e7f/delta}{$-$2.0}
\defres{hardni/e7f/lo}{$-$8.8}
\defres{hardni/e7f/hi}{$+$4.8}
\defres{hardni/e7f/p}{0.402}
\defres{hardni/e7f/ni}{no}
\makeatother


==> generated/harness_final.tex <==
\makeatletter
\providecommand{\res}[1]{\ifcsname jevres@#1\endcsname\csname jevres@#1\endcsname\else\tbd\fi}
\providecommand{\defres}[2]{\expandafter\def\csname jevres@#1\endcsname{#2}}
\defres{hf/arg_coverage}{85.4}
\defres{hf/bench/cross/v0/new/4/flips}{2}
\defres{hf/bench/cross/v0/new/4/questions}{1811}
\defres{hf/bench/cross/v0/new/8/flips}{2}
\defres{hf/bench/cross/v0/new/8/questions}{1811}
\defres{hf/bench/cross/v0p/new/1/flips}{0}
\defres{hf/bench/cross/v0p/new/1/questions}{281}
\defres{hf/bench/cross/v0p/old/1/flips}{0}
\defres{hf/bench/cross/v0p/old/1/questions}{381}
\defres{hf/bench/cross/v2/new/1/flips}{0}
\defres{hf/bench/cross/v2/new/1/questions}{281}
\defres{hf/bench/cross/v2/new/2/flips}{2}
\defres{hf/bench/cross/v2/new/2/questions}{1811}
\defres{hf/bench/cross/v2/new/4/flips}{2}
\defres{hf/bench/cross/v2/new/4/questions}{1811}
\defres{hf/bench/cross/v2/new/8/flips}{2}
\defres{hf/bench/cross/v2/new/8/questions}{1811}
\defres{hf/bench/cross/v2/old/4/flips}{2}
\defres{hf/bench/cross/v2/old/4/questions}{2461}
\defres{hf/bench/cross/v2p/new/1/flips}{0}
\defres{hf/bench/cross/v2p/new/1/questions}{281}
\defres{hf/bench/v0/new/c4/eps_per_gpu_h}{659}
\defres{hf/bench/v0/new/c4/flips}{1}
\defres{hf/bench/v0/new/c4/flips_vs_dist}{904}
\defres{hf/bench/v0/new/c4/questions}{1811}
\defres{hf/bench/v0/new/c4/requests_ep}{14.0}
\defres{hf/bench/v0/new/c4/s1_ms_step}{2440}
\defres{hf/bench/v0/new/c4/s1_s_ep}{18.30}
\defres{hf/bench/v0/new/c4/wall_s_ep}{21.63}
\defres{hf/bench/v0/new/c8/eps_per_gpu_h}{662}
\defres{hf/bench/v0/new/c8/flips}{1}
\defres{hf/bench/v0/new/c8/flips_vs_dist}{904}
\defres{hf/bench/v0/new/c8/questions}{1811}
\defres{hf/bench/v0/new/c8/requests_ep}{14.0}
\defres{hf/bench/v0/new/c8/s1_ms_step}{5206}
\defres{hf/bench/v0/new/c8/s1_s_ep}{39.04}
\defres{hf/bench/v0/new/c8/wall_s_ep}{42.38}
\defres{hf/bench/v0/old/c1/eps_per_gpu_h}{585}
\defres{hf/bench/v0/old/c1/flips}{0}
\defres{hf/bench/v0/old/c1/flips_vs_dist}{140}
\defres{hf/bench/v0/old/c1/questions}{381}
\defres{hf/bench/v0/old/c1/requests_ep}{15.2}
\defres{hf/bench/v0/old/c1/s1_ms_step}{648}
\defres{hf/bench/v0/old/c1/s1_s_ep}{3.24}
\defres{hf/bench/v0/old/c1/wall_s_ep}{6.15}
\defres{hf/bench/v0/old/c4/eps_per_gpu_h}{666}
\defres{hf/bench/v0/old/c4/flips}{1}
\defres{hf/bench/v0/old/c4/flips_vs_dist}{903}
\defres{hf/bench/v0/old/c4/questions}{2461}
\defres{hf/bench/v0/old/c4/requests_ep}{24.6}
\defres{hf/bench/v0/old/c4/s1_ms_step}{2409}
\defres{hf/bench/v0/old/c4/s1_s_ep}{18.07}
\defres{hf/bench/v0/old/c4/wall_s_ep}{21.40}
\defres{hf/bench/v0/old/c8/eps_per_gpu_h}{668}
\defres{hf/bench/v0/old/c8/flips}{1}
\defres{hf/bench/v0/old/c8/flips_vs_dist}{903}
\defres{hf/bench/v0/old/c8/questions}{2461}
\defres{hf/bench/v0/old/c8/requests_ep}{24.6}
\defres{hf/bench/v0/old/c8/s1_ms_step}{5166}
\defres{hf/bench/v0/old/c8/s1_s_ep}{38.74}
\defres{hf/bench/v0/old/c8/wall_s_ep}{42.08}
\defres{hf/bench/v0p/new/c1/eps_per_gpu_h}{591}
\defres{hf/bench/v0p/new/c1/flips}{0}
\defres{hf/bench/v0p/new/c1/flips_vs_dist}{140}
\defres{hf/bench/v0p/new/c1/questions}{281}
\defres{hf/bench/v0p/new/c1/requests_ep}{9.0}
\defres{hf/bench/v0p/new/c1/s1_ms_step}{637}
\defres{hf/bench/v0p/new/c1/s1_s_ep}{3.19}
\defres{hf/bench/v0p/new/c1/wall_s_ep}{6.09}
\defres{hf/bench/v0p/old/c1/eps_per_gpu_h}{580}
\defres{hf/bench/v0p/old/c1/flips}{0}
\defres{hf/bench/v0p/old/c1/flips_vs_dist}{140}
\defres{hf/bench/v0p/old/c1/questions}{381}
\defres{hf/bench/v0p/old/c1/requests_ep}{15.2}
\defres{hf/bench/v0p/old/c1/s1_ms_step}{659}
\defres{hf/bench/v0p/old/c1/s1_s_ep}{3.30}
\defres{hf/bench/v0p/old/c1/wall_s_ep}{6.20}
\defres{hf/bench/v2/new/c1/eps_per_gpu_h}{694}
\defres{hf/bench/v2/new/c1/flips}{0}
\defres{hf/bench/v2/new/c1/flips_vs_dist}{140}
\defres{hf/bench/v2/new/c1/questions}{281}
\defres{hf/bench/v2/new/c1/requests_ep}{9.0}
\defres{hf/bench/v2/new/c1/s1_ms_step}{455}
\defres{hf/bench/v2/new/c1/s1_s_ep}{2.28}
\defres{hf/bench/v2/new/c1/wall_s_ep}{5.18}
\defres{hf/bench/v2/new/c2/eps_per_gpu_h}{777}
\defres{hf/bench/v2/new/c2/flips}{3}
\defres{hf/bench/v2/new/c2/flips_vs_dist}{905}
\defres{hf/bench/v2/new/c2/questions}{1811}
\defres{hf/bench/v2/new/c2/requests_ep}{14.0}
\defres{hf/bench/v2/new/c2/s1_ms_step}{784}
\defres{hf/bench/v2/new/c2/s1_s_ep}{5.88}
\defres{hf/bench/v2/new/c2/wall_s_ep}{9.21}
\defres{hf/bench/v2/new/c4/eps_per_gpu_h}{919}
\defres{hf/bench/v2/new/c4/flips}{3}
\defres{hf/bench/v2/new/c4/flips_vs_dist}{905}
\defres{hf/bench/v2/new/c4/questions}{1811}
\defres{hf/bench/v2/new/c4/requests_ep}{14.0}
\defres{hf/bench/v2/new/c4/s1_ms_step}{1623}
\defres{hf/bench/v2/new/c4/s1_s_ep}{12.17}
\defres{hf/bench/v2/new/c4/wall_s_ep}{15.50}
\defres{hf/bench/v2/new/c8/eps_per_gpu_h}{934}
\defres{hf/bench/v2/new/c8/flips}{3}
\defres{hf/bench/v2/new/c8/flips_vs_dist}{905}
\defres{hf/bench/v2/new/c8/questions}{1811}
\defres{hf/bench/v2/new/c8/requests_ep}{14.0}
\defres{hf/bench/v2/new/c8/s1_ms_step}{3564}
\defres{hf/bench/v2/new/c8/s1_s_ep}{26.73}
\defres{hf/bench/v2/new/c8/wall_s_ep}{30.06}
\defres{hf/bench/v2/old/c4/eps_per_gpu_h}{878}
\defres{hf/bench/v2/old/c4/flips}{3}
\defres{hf/bench/v2/old/c4/flips_vs_dist}{905}
\defres{hf/bench/v2/old/c4/questions}{2461}
\defres{hf/bench/v2/old/c4/requests_ep}{24.6}
\defres{hf/bench/v2/old/c4/s1_ms_step}{1719}
\defres{hf/bench/v2/old/c4/s1_s_ep}{12.89}
\defres{hf/bench/v2/old/c4/wall_s_ep}{16.23}
\defres{hf/bench/v2p/new/c1/eps_per_gpu_h}{691}
\defres{hf/bench/v2p/new/c1/flips}{0}
\defres{hf/bench/v2p/new/c1/flips_vs_dist}{140}
\defres{hf/bench/v2p/new/c1/questions}{281}
\defres{hf/bench/v2p/new/c1/requests_ep}{9.0}
\defres{hf/bench/v2p/new/c1/s1_ms_step}{460}
\defres{hf/bench/v2p/new/c1/s1_s_ep}{2.30}
\defres{hf/bench/v2p/new/c1/wall_s_ep}{5.21}
\defres{hf/cache_hit_share}{37.6}
\defres{hf/conc}{8}
\defres{hf/cost/harness_final}{0.0078}
\defres{hf/cost/llm_only}{0.0434}
\defres{hf/cost/q}{0.00192}
\defres{hf/cost/saving}{82.1}
\defres{hf/cost/saving_ci/hi}{82.7}
\defres{hf/cost/saving_ci/lo}{81.5}
\defres{hf/cost/saving_no_tariff}{86.6}
\defres{hf/diag/jev/s1_requests}{21.2}
\defres{hf/diag/jev/s1_requests_per_step}{2.81}
\defres{hf/diag/jev/s1_s}{4.26}
\defres{hf/diag/jev/s2_calls}{5.37}
\defres{hf/diag/jev/s2_s}{5.09}
\defres{hf/diag/jev/wall_s}{9.21}
\defres{hf/diag/llm_only/s1_requests}{0.0}
\defres{hf/diag/llm_only/s1_requests_per_step}{0.00}
\defres{hf/diag/llm_only/s1_s}{0.00}
\defres{hf/diag/llm_only/s2_calls}{7.52}
\defres{hf/diag/llm_only/s2_s}{6.80}
\defres{hf/diag/llm_only/wall_s}{6.83}
\defres{hf/diag/rl/busy}{97.3}
\defres{hf/diag/rl/queue_ms}{199}
\defres{hf/diag/rl/queue_share}{66.1}
\defres{hf/diag/rl/reflection_fired}{0}
\defres{hf/diag/rl/reflection_pmax}{0.40}
\defres{hf/diag/rl/reflection_questions}{3250}
\defres{hf/diag/rl/s1_requests}{24.6}
\defres{hf/diag/rl/s1_requests_per_step}{3.28}
\defres{hf/diag/rl/s1_s}{7.40}
\defres{hf/diag/rl/s2_calls}{3.03}
\defres{hf/diag/rl/s2_s}{2.37}
\defres{hf/diag/rl/service_ms}{102}
\defres{hf/diag/rl/ts_service_ms}{220}
\defres{hf/diag/rl/wall_s}{10.21}
\defres{hf/model_s/delta}{+13.62}
\defres{hf/model_s/delta_ci/hi}{+14.93}
\defres{hf/model_s/delta_ci/lo}{+12.16}
\defres{hf/model_s/harness_final}{22.05}
\defres{hf/model_s/llm_only}{8.43}
\defres{hf/n}{200}
\defres{hf/positions/v0_new/forwards_step}{4.4}
\defres{hf/positions/v0_new/gflop_step}{20658}
\defres{hf/positions/v0_new/per_step}{2680}
\defres{hf/positions/v0_new/requests_step}{1.86}
\defres{hf/positions/v0_old/forwards_step}{5.3}
\defres{hf/positions/v0_old/gflop_step}{19286}
\defres{hf/positions/v0_old/per_step}{2534}
\defres{hf/positions/v0_old/requests_step}{3.28}
\defres{hf/positions/v2_new/forwards_step}{4.4}
\defres{hf/positions/v2_new/gflop_step}{13985}
\defres{hf/positions/v2_new/per_step}{1924}
\defres{hf/positions/v2_new/requests_step}{1.86}
\defres{hf/queue_share}{76.3}
\defres{hf/s1_requests}{14.00}
\defres{hf/s1_s}{16.41}
\defres{hf/s2_calls/harness_final}{3.05}
\defres{hf/s2_calls/llm_only}{7.52}
\defres{hf/s2_s}{5.63}
\defres{hf/success/delta}{+0.5}
\defres{hf/success/delta_ci/hi}{+1.5}
\defres{hf/success/delta_ci/lo}{+0.0}
\defres{hf/success/harness_final}{100.0}
\defres{hf/success/llm_only}{99.5}
\defres{hf/tariff/host_usd_h}{1.624}
\defres{hf/tariff/q}{0.00192}
\defres{hf/tariff/q_s24}{0.00196}
\defres{hf/tool_coverage}{100.0}
\defres{hf/wall_s/delta}{+13.69}
\defres{hf/wall_s/delta_ci/hi}{+15.13}
\defres{hf/wall_s/delta_ci/lo}{+12.08}
\defres{hf/wall_s/harness_final}{22.39}
\defres{hf/wall_s/llm_only}{8.70}
\defres{hf/wall_s/median/harness_final}{20.72}
\defres{hf/wall_s/median/llm_only}{8.94}
\defres{hf/wall_s/saving}{-157.4}
\defres{hf_ded/arg_coverage}{85.5}
\defres{hf_ded/cache_hit_share}{37.6}
\defres{hf_ded/conc}{1}
\defres{hf_ded/cost/harness_final}{0.0102}
\defres{hf_ded/cost/llm_only}{0.0431}
\defres{hf_ded/cost/q}{0.00438}
\defres{hf_ded/cost/saving}{76.3}
\defres{hf_ded/cost/saving_ci/hi}{77.1}
\defres{hf_ded/cost/saving_ci/lo}{75.6}
\defres{hf_ded/cost/saving_no_tariff}{86.5}
\defres{hf_ded/model_s/delta}{-2.64}
\defres{hf_ded/model_s/delta_ci/hi}{-0.44}
\defres{hf_ded/model_s/delta_ci/lo}{-5.16}
\defres{hf_ded/model_s/harness_final}{9.04}
\defres{hf_ded/model_s/llm_only}{11.68}
\defres{hf_ded/n}{200}
\defres{hf_ded/queue_share}{0.0}
\defres{hf_ded/s1_requests}{14.00}
\defres{hf_ded/s1_s}{3.93}
\defres{hf_ded/s2_calls/harness_final}{3.04}
\defres{hf_ded/s2_calls/llm_only}{7.53}
\defres{hf_ded/s2_s}{5.11}
\defres{hf_ded/success/delta}{+0.5}
\defres{hf_ded/success/delta_ci/hi}{+1.5}
\defres{hf_ded/success/delta_ci/lo}{+0.0}
\defres{hf_ded/success/harness_final}{100.0}
\defres{hf_ded/success/llm_only}{99.5}
\defres{hf_ded/tariff/host_usd_h}{1.624}
\defres{hf_ded/tariff/q}{0.00438}
\defres{hf_ded/tariff/q_s24}{0.00196}
\defres{hf_ded/tool_coverage}{100.0}
\defres{hf_ded/wall_s/delta}{-4.00}
\defres{hf_ded/wall_s/delta_ci/hi}{-0.61}
\defres{hf_ded/wall_s/delta_ci/lo}{-7.98}
\defres{hf_ded/wall_s/harness_final}{9.59}
\defres{hf_ded/wall_s/llm_only}{13.59}
\defres{hf_ded/wall_s/median/harness_final}{7.89}
\defres{hf_ded/wall_s/median/llm_only}{8.87}
\defres{hf_ded/wall_s/saving}{29.4}
\makeatother


==> generated/leakage.tex <==
\makeatletter
\providecommand{\res}[1]{\ifcsname jevres@#1\endcsname\csname jevres@#1\endcsname\else\tbd\fi}
\providecommand{\defres}[2]{\expandafter\def\csname jevres@#1\endcsname{#2}}
\defres{leak/canary/wire}{absent}
\defres{leak/jev/responses}{192{,}326}
\defres{leak/jev/snapshot}{typesafe/jev-1.13-20260917}
\defres{leak/jev/snapshots_n}{1}
\defres{leak/jevgym/first_commit}{2026-09-30}
\defres{leak/opd/budget}{8}
\defres{leak/opd/dev_hi}{1{,}047}
\defres{leak/opd/dev_lo}{1{,}000}
\defres{leak/opd/drawn}{864}
\defres{leak/opd/iterations}{24}
\defres{leak/opd/lr}{5{\times}10^{-5}}
\defres{leak/opd/pool_hi}{43{,}999}
\defres{leak/opd/pool_lo}{40{,}000}
\defres{leak/opd/tasks_per_iter}{36}
\defres{leak/opd/teacher_usd}{0.38}
\defres{leak/rescore/base/all}{50.1}
\defres{leak/rescore/base/only_exact}{95.3}
\defres{leak/rescore/base/only_masked}{40.5}
\defres{leak/rescore/base/only_near80}{80.0}
\defres{leak/rescore/base/only_near90}{95.3}
\defres{leak/rescore/base/without_exact}{48.3}
\defres{leak/rescore/base/without_exact/delta}{-1.8}
\defres{leak/rescore/base/without_masked}{54.4}
\defres{leak/rescore/base/without_masked/delta}{+4.3}
\defres{leak/rescore/base/without_near80}{44.9}
\defres{leak/rescore/base/without_near80/delta}{-5.2}
\defres{leak/rescore/base/without_near90}{48.3}
\defres{leak/rescore/base/without_near90/delta}{-1.8}
\defres{leak/rescore/intern/all}{75.2}
\defres{leak/rescore/intern/only_exact}{93.0}
\defres{leak/rescore/intern/only_masked}{73.2}
\defres{leak/rescore/intern/only_near80}{92.5}
\defres{leak/rescore/intern/only_near90}{93.0}
\defres{leak/rescore/intern/without_exact}{74.2}
\defres{leak/rescore/intern/without_exact/delta}{-1.0}
\defres{leak/rescore/intern/without_masked}{74.1}
\defres{leak/rescore/intern/without_masked/delta}{-1.1}
\defres{leak/rescore/intern/without_near80}{71.3}
\defres{leak/rescore/intern/without_near80/delta}{-4.0}
\defres{leak/rescore/intern/without_near90}{74.2}
\defres{leak/rescore/intern/without_near90/delta}{-1.0}
\defres{leak/rescore/jev/all}{91.5}
\defres{leak/rescore/jev/only_exact}{100.0}
\defres{leak/rescore/jev/only_masked}{93.6}
\defres{leak/rescore/jev/only_near80}{96.5}
\defres{leak/rescore/jev/only_near90}{100.0}
\defres{leak/rescore/jev/without_exact}{90.9}
\defres{leak/rescore/jev/without_exact/delta}{-0.6}
\defres{leak/rescore/jev/without_masked}{89.4}
\defres{leak/rescore/jev/without_masked/delta}{-2.0}
\defres{leak/rescore/jev/without_near80}{89.3}
\defres{leak/rescore/jev/without_near80/delta}{-2.1}
\defres{leak/rescore/jev/without_near90}{90.9}
\defres{leak/rescore/jev/without_near90/delta}{-0.6}
\defres{leak/rescore/rl/all}{99.2}
\defres{leak/rescore/rl/only_exact}{100.0}
\defres{leak/rescore/rl/only_masked}{100.0}
\defres{leak/rescore/rl/only_near80}{100.0}
\defres{leak/rescore/rl/only_near90}{100.0}
\defres{leak/rescore/rl/without_exact}{99.2}
\defres{leak/rescore/rl/without_exact/delta}{+0.0}
\defres{leak/rescore/rl/without_masked}{99.0}
\defres{leak/rescore/rl/without_masked/delta}{-0.2}
\defres{leak/rescore/rl/without_near80}{99.1}
\defres{leak/rescore/rl/without_near80/delta}{-0.1}
\defres{leak/rescore/rl/without_near90}{99.2}
\defres{leak/rescore/rl/without_near90/delta}{+0.0}
\defres{leak/rescore/sft_v1/all}{99.2}
\defres{leak/rescore/sft_v1/only_exact}{100.0}
\defres{leak/rescore/sft_v1/only_masked}{100.0}
\defres{leak/rescore/sft_v1/only_near80}{100.0}
\defres{leak/rescore/sft_v1/only_near90}{100.0}
\defres{leak/rescore/sft_v1/without_exact}{99.2}
\defres{leak/rescore/sft_v1/without_exact/delta}{+0.0}
\defres{leak/rescore/sft_v1/without_masked}{99.0}
\defres{leak/rescore/sft_v1/without_masked/delta}{-0.2}
\defres{leak/rescore/sft_v1/without_near80}{99.1}
\defres{leak/rescore/sft_v1/without_near80/delta}{-0.1}
\defres{leak/rescore/sft_v1/without_near90}{99.2}
\defres{leak/rescore/sft_v1/without_near90/delta}{+0.0}
\defres{leak/rescore/sl0.8b/all}{48.3}
\defres{leak/rescore/sl0.8b/only_exact}{100.0}
\defres{leak/rescore/sl0.8b/only_masked}{36.6}
\defres{leak/rescore/sl0.8b/only_near80}{82.4}
\defres{leak/rescore/sl0.8b/only_near90}{100.0}
\defres{leak/rescore/sl0.8b/without_exact}{46.6}
\defres{leak/rescore/sl0.8b/without_exact/delta}{-1.8}
\defres{leak/rescore/sl0.8b/without_masked}{52.7}
\defres{leak/rescore/sl0.8b/without_masked/delta}{+4.3}
\defres{leak/rescore/sl0.8b/without_near80}{42.7}
\defres{leak/rescore/sl0.8b/without_near80/delta}{-5.6}
\defres{leak/rescore/sl0.8b/without_near90}{46.6}
\defres{leak/rescore/sl0.8b/without_near90/delta}{-1.8}
\defres{leak/rescore/sl27b/all}{93.9}
\defres{leak/rescore/sl27b/only_exact}{100.0}
\defres{leak/rescore/sl27b/only_masked}{96.6}
\defres{leak/rescore/sl27b/only_near80}{100.0}
\defres{leak/rescore/sl27b/only_near90}{100.0}
\defres{leak/rescore/sl27b/without_exact}{93.5}
\defres{leak/rescore/sl27b/without_exact/delta}{-0.4}
\defres{leak/rescore/sl27b/without_masked}{92.6}
\defres{leak/rescore/sl27b/without_masked/delta}{-1.3}
\defres{leak/rescore/sl27b/without_near80}{92.1}
\defres{leak/rescore/sl27b/without_near80/delta}{-1.8}
\defres{leak/rescore/sl27b/without_near90}{93.5}
\defres{leak/rescore/sl27b/without_near90/delta}{-0.4}
\defres{leak/rescore/sl2b/all}{68.4}
\defres{leak/rescore/sl2b/only_exact}{97.7}
\defres{leak/rescore/sl2b/only_masked}{79.6}
\defres{leak/rescore/sl2b/only_near80}{93.1}
\defres{leak/rescore/sl2b/only_near90}{97.7}
\defres{leak/rescore/sl2b/without_exact}{67.3}
\defres{leak/rescore/sl2b/without_exact/delta}{-1.2}
\defres{leak/rescore/sl2b/without_masked}{63.5}
\defres{leak/rescore/sl2b/without_masked/delta}{-5.0}
\defres{leak/rescore/sl2b/without_near80}{64.6}
\defres{leak/rescore/sl2b/without_near80/delta}{-3.9}
\defres{leak/rescore/sl2b/without_near90}{67.3}
\defres{leak/rescore/sl2b/without_near90/delta}{-1.2}
\defres{leak/rescore/sl4b/all}{89.1}
\defres{leak/rescore/sl4b/only_exact}{97.7}
\defres{leak/rescore/sl4b/only_masked}{88.0}
\defres{leak/rescore/sl4b/only_near80}{88.3}
\defres{leak/rescore/sl4b/only_near90}{97.7}
\defres{leak/rescore/sl4b/without_exact}{88.6}
\defres{leak/rescore/sl4b/without_exact/delta}{-0.5}
\defres{leak/rescore/sl4b/without_masked}{89.8}
\defres{leak/rescore/sl4b/without_masked/delta}{+0.6}
\defres{leak/rescore/sl4b/without_near80}{88.6}
\defres{leak/rescore/sl4b/without_near80/delta}{-0.5}
\defres{leak/rescore/sl4b/without_near90}{88.6}
\defres{leak/rescore/sl4b/without_near90/delta}{-0.5}
\defres{leak/rescore/sl9b/all}{91.8}
\defres{leak/rescore/sl9b/only_exact}{100.0}
\defres{leak/rescore/sl9b/only_masked}{95.5}
\defres{leak/rescore/sl9b/only_near80}{99.8}
\defres{leak/rescore/sl9b/only_near90}{100.0}
\defres{leak/rescore/sl9b/without_exact}{91.2}
\defres{leak/rescore/sl9b/without_exact/delta}{-0.6}
\defres{leak/rescore/sl9b/without_masked}{89.9}
\defres{leak/rescore/sl9b/without_masked/delta}{-1.9}
\defres{leak/rescore/sl9b/without_near80}{89.6}
\defres{leak/rescore/sl9b/without_near80/delta}{-2.2}
\defres{leak/rescore/sl9b/without_near90}{91.2}
\defres{leak/rescore/sl9b/without_near90/delta}{-0.6}
\defres{leak/rescore/v2/all}{99.4}
\defres{leak/rescore/v2/only_exact}{100.0}
\defres{leak/rescore/v2/only_masked}{100.0}
\defres{leak/rescore/v2/only_near80}{100.0}
\defres{leak/rescore/v2/only_near90}{100.0}
\defres{leak/rescore/v2/without_exact}{99.3}
\defres{leak/rescore/v2/without_exact/delta}{+0.0}
\defres{leak/rescore/v2/without_masked}{99.2}
\defres{leak/rescore/v2/without_masked/delta}{-0.2}
\defres{leak/rescore/v2/without_near80}{99.3}
\defres{leak/rescore/v2/without_near80/delta}{-0.1}
\defres{leak/rescore/v2/without_near90}{99.3}
\defres{leak/rescore/v2/without_near90/delta}{+0.0}
\defres{leak/seeds/eval/n}{1{,}250}
\defres{leak/seeds/overlap}{0}
\defres{leak/seeds/overlap_registered}{0}
\defres{leak/seeds/reconstruction/identical}{yes}
\defres{leak/seeds/reconstruction/n}{240}
\defres{leak/seeds/train/max}{72{,}999}
\defres{leak/seeds/train/min}{10{,}000}
\defres{leak/seeds/train_files/n}{2{,}898}
\defres{leak/seeds/train_pools/n}{14{,}000}
\defres{leak/spec/baseline/instruction_dup}{23.8}
\defres{leak/spec/corpus/instruction_dup}{43.5}
\defres{leak/spec/corpus/orders_dup}{0.0}
\defres{leak/spec/corpus/plan_dup}{0}
\defres{leak/spec/corpus/pool_plan_dup}{0}
\defres{leak/spec/corpus/target_dup}{0.0}
\defres{leak/spec/corpus/world_dup}{0}
\defres{leak/spec/n_pool_tasks}{14{,}000}
\defres{leak/spec/n_train_tasks}{2{,}898}
\defres{leak/spec/spare/instruction_dup}{44.0}
\defres{leak/spec/spare/orders_dup}{0.0}
\defres{leak/spec/spare/plan_dup}{0}
\defres{leak/spec/spare/pool_plan_dup}{0}
\defres{leak/spec/spare/target_dup}{0.0}
\defres{leak/spec/spare/world_dup}{0}
\defres{leak/spec/stage1/instruction_dup}{45.4}
\defres{leak/spec/stage1/orders_dup}{0.0}
\defres{leak/spec/stage1/plan_dup}{0}
\defres{leak/spec/stage1/pool_plan_dup}{0}
\defres{leak/spec/stage1/target_dup}{0.0}
\defres{leak/spec/stage1/world_dup}{0}
\defres{leak/spec/stage2/instruction_dup}{43.2}
\defres{leak/spec/stage2/orders_dup}{0.0}
\defres{leak/spec/stage2/plan_dup}{0}
\defres{leak/spec/stage2/pool_plan_dup}{0}
\defres{leak/spec/stage2/target_dup}{0.2}
\defres{leak/spec/stage2/world_dup}{0}
\defres{leak/state/c/exact/occ}{174}
\defres{leak/state/c/exact/rate}{3.3}
\defres{leak/state/c/exact/tasks}{43}
\defres{leak/state/c/masked/rate}{32.1}
\defres{leak/state/c/maxj/median}{0.31}
\defres{leak/state/c/n_occ}{5{,}314}
\defres{leak/state/c/near80/rate}{10.4}
\defres{leak/state/c/near90/rate}{3.3}
\defres{leak/state/c/spec_step_dup}{0}
\defres{leak/state/c/train_states}{5{,}173}
\defres{leak/state/c/within/exact/rate}{2.6}
\defres{leak/state/c/within/masked/rate}{37.4}
\defres{leak/state/c/within/maxj/median}{0.32}
\defres{leak/state/c/within/near80/rate}{10.4}
\defres{leak/state/c/within/near90/rate}{2.6}
\defres{leak/static/n_eval_texts}{6{,}687}
\defres{leak/static/v0-replay-when2call/exact}{0}
\defres{leak/static/v0-replay-when2call/ngram8}{15}
\defres{leak/static/v1-replay-when2call/exact}{0}
\defres{leak/static/v1-replay-when2call/ngram8}{0}
\defres{leak/static/v1-train-jevgym/exact}{0}
\defres{leak/static/v1-train-jevgym/ngram8}{0}
\defres{leak/tau2/exact}{0}
\defres{leak/tau2/maxj}{0.04}
\defres{leak/tau2/n_states}{18{,}782}
\defres{leak/tau2/near80}{0}
\defres{leak/teacher/entries}{7{,}552}
\defres{leak/teacher/matched}{7{,}552}
\defres{leak/teacher/unmatched}{0}
\makeatother


==> generated/module_map.tex <==
\makeatletter
\providecommand{\res}[1]{\ifcsname jevres@#1\endcsname\csname jevres@#1\endcsname\else\tbd\fi}
\providecommand{\defres}[2]{\expandafter\def\csname jevres@#1\endcsname{#2}}
\defres{mm/best/flash/action/vcode}{0}
\defres{mm/best/flash/action/verdict}{not run}
\defres{mm/best/flash/memory_read/acted}{100.0}
\defres{mm/best/flash/memory_read/delta}{+0.0}
\defres{mm/best/flash/memory_read/fig_delta}{+0.0}
\defres{mm/best/flash/memory_read/fig_saving}{-5}
\defres{mm/best/flash/memory_read/mode}{assist}
\defres{mm/best/flash/memory_read/row}{jev\_mem}
\defres{mm/best/flash/memory_read/saving}{-4.8}
\defres{mm/best/flash/memory_read/vcode}{3}
\defres{mm/best/flash/memory_read/verdict}{no saving}
\defres{mm/best/flash/memory_write/acted}{99.5}
\defres{mm/best/flash/memory_write/delta}{-1.0}
\defres{mm/best/flash/memory_write/fig_delta}{-1.0}
\defres{mm/best/flash/memory_write/fig_saving}{-39}
\defres{mm/best/flash/memory_write/mode}{trigger}
\defres{mm/best/flash/memory_write/row}{jev\_memw}
\defres{mm/best/flash/memory_write/saving}{-38.9}
\defres{mm/best/flash/memory_write/vcode}{3}
\defres{mm/best/flash/memory_write/verdict}{no saving}
\defres{mm/best/flash/reflection/acted}{13.9}
\defres{mm/best/flash/reflection/delta}{+0.0}
\defres{mm/best/flash/reflection/fig_delta}{+0.0}
\defres{mm/best/flash/reflection/fig_saving}{1}
\defres{mm/best/flash/reflection/mode}{trigger}
\defres{mm/best/flash/reflection/row}{jev\_reflect\_trigger}
\defres{mm/best/flash/reflection/saving}{0.9}
\defres{mm/best/flash/reflection/vcode}{1}
\defres{mm/best/flash/reflection/verdict}{takes over safely}
\defres{mm/best/flash/routing/acted}{10.1}
\defres{mm/best/flash/routing/delta}{+0.6}
\defres{mm/best/flash/routing/fig_delta}{+0.6}
\defres{mm/best/flash/routing/fig_saving}{-36}
\defres{mm/best/flash/routing/mode}{trigger}
\defres{mm/best/flash/routing/reg}{C4}
\defres{mm/best/flash/routing/row}{jev\_route\_tau0.4}
\defres{mm/best/flash/routing/saving}{-36.2}
\defres{mm/best/flash/routing/vcode}{3}
\defres{mm/best/flash/routing/verdict}{no saving}
\defres{mm/best/flash/stop/acted}{0.0}
\defres{mm/best/flash/stop/delta}{+0.0}
\defres{mm/best/flash/stop/fig_delta}{+0.0}
\defres{mm/best/flash/stop/fig_saving}{0}
\defres{mm/best/flash/stop/mode}{trigger}
\defres{mm/best/flash/stop/row}{jev\_stop\_trigger}
\defres{mm/best/flash/stop/saving}{-0.1}
\defres{mm/best/flash/stop/vcode}{3}
\defres{mm/best/flash/stop/verdict}{no saving}
\defres{mm/best/flash/tool_params/acted}{20.8}
\defres{mm/best/flash/tool_params/delta}{+0.0}
\defres{mm/best/flash/tool_params/fig_delta}{+0.0}
\defres{mm/best/flash/tool_params/fig_saving}{14}
\defres{mm/best/flash/tool_params/mode}{cascade}
\defres{mm/best/flash/tool_params/reg}{C1F}
\defres{mm/best/flash/tool_params/row}{jev\_ts\_cascade\_tauhat}
\defres{mm/best/flash/tool_params/saving}{14.2}
\defres{mm/best/flash/tool_params/vcode}{1}
\defres{mm/best/flash/tool_params/verdict}{takes over safely}
\defres{mm/best/flash/tool_select/acted}{27.2}
\defres{mm/best/flash/tool_select/delta}{+0.0}
\defres{mm/best/flash/tool_select/fig_delta}{+0.0}
\defres{mm/best/flash/tool_select/fig_saving}{14}
\defres{mm/best/flash/tool_select/mode}{cascade}
\defres{mm/best/flash/tool_select/reg}{C1F}
\defres{mm/best/flash/tool_select/row}{jev\_ts\_cascade\_tauhat}
\defres{mm/best/flash/tool_select/saving}{14.2}
\defres{mm/best/flash/tool_select/vcode}{1}
\defres{mm/best/flash/tool_select/verdict}{takes over safely}
\defres{mm/best/lite/action/vcode}{0}
\defres{mm/best/lite/action/verdict}{not run}
\defres{mm/best/lite/memory_read/vcode}{0}
\defres{mm/best/lite/memory_read/verdict}{not run}
\defres{mm/best/lite/memory_write/vcode}{0}
\defres{mm/best/lite/memory_write/verdict}{not run}
\defres{mm/best/lite/reflection/acted}{14.8}
\defres{mm/best/lite/reflection/delta}{+1.8}
\defres{mm/best/lite/reflection/fig_delta}{+1.8}
\defres{mm/best/lite/reflection/fig_saving}{-2}
\defres{mm/best/lite/reflection/mode}{trigger}
\defres{mm/best/lite/reflection/reg}{C5}
\defres{mm/best/lite/reflection/row}{jev\_reflect\_trigger\_s2lite}
\defres{mm/best/lite/reflection/saving}{-1.9}
\defres{mm/best/lite/reflection/vcode}{3}
\defres{mm/best/lite/reflection/verdict}{no saving}
\defres{mm/best/lite/routing/acted}{10.1}
\defres{mm/best/lite/routing/delta}{+0.6}
\defres{mm/best/lite/routing/fig_delta}{+0.6}
\defres{mm/best/lite/routing/fig_saving}{-36}
\defres{mm/best/lite/routing/mode}{trigger}
\defres{mm/best/lite/routing/reg}{C4}
\defres{mm/best/lite/routing/row}{jev\_route\_tau0.4}
\defres{mm/best/lite/routing/saving}{-36.2}
\defres{mm/best/lite/routing/vcode}{3}
\defres{mm/best/lite/routing/verdict}{no saving}
\defres{mm/best/lite/stop/acted}{72.6}
\defres{mm/best/lite/stop/delta}{+1.6}
\defres{mm/best/lite/stop/fig_delta}{+1.6}
\defres{mm/best/lite/stop/fig_saving}{-32}
\defres{mm/best/lite/stop/mode}{guard}
\defres{mm/best/lite/stop/reg}{C6L}
\defres{mm/best/lite/stop/row}{jev\_stop\_guard\_s2lite}
\defres{mm/best/lite/stop/saving}{-32.1}
\defres{mm/best/lite/stop/vcode}{3}
\defres{mm/best/lite/stop/verdict}{no saving}
\defres{mm/best/lite/tool_params/acted}{0.0}
\defres{mm/best/lite/tool_params/delta}{+1.0}
\defres{mm/best/lite/tool_params/fig_delta}{+1.0}
\defres{mm/best/lite/tool_params/fig_saving}{0}
\defres{mm/best/lite/tool_params/mode}{cascade}
\defres{mm/best/lite/tool_params/reg}{C1L}
\defres{mm/best/lite/tool_params/row}{jev\_ts\_cascade\_tau0.9\_s2lite}
\defres{mm/best/lite/tool_params/saving}{0.2}
\defres{mm/best/lite/tool_params/vcode}{2}
\defres{mm/best/lite/tool_params/verdict}{mixed}
\defres{mm/best/lite/tool_select/acted}{0.0}
\defres{mm/best/lite/tool_select/delta}{+1.0}
\defres{mm/best/lite/tool_select/fig_delta}{+1.0}
\defres{mm/best/lite/tool_select/fig_saving}{0}
\defres{mm/best/lite/tool_select/mode}{cascade}
\defres{mm/best/lite/tool_select/reg}{C1L}
\defres{mm/best/lite/tool_select/row}{jev\_ts\_cascade\_tau0.9\_s2lite}
\defres{mm/best/lite/tool_select/saving}{0.2}
\defres{mm/best/lite/tool_select/vcode}{2}
\defres{mm/best/lite/tool_select/verdict}{mixed}
\defres{mm/cell/flash/action/assist/state}{not run}
\defres{mm/cell/flash/action/assist/vcode}{0}
\defres{mm/cell/flash/action/assist/verdict}{not run}
\defres{mm/cell/flash/action/cascade/state}{not run}
\defres{mm/cell/flash/action/cascade/vcode}{0}
\defres{mm/cell/flash/action/cascade/verdict}{not run}
\defres{mm/cell/flash/action/guard/state}{not run}
\defres{mm/cell/flash/action/guard/vcode}{0}
\defres{mm/cell/flash/action/guard/verdict}{not run}
\defres{mm/cell/flash/action/replace/state}{not run}
\defres{mm/cell/flash/action/replace/vcode}{0}
\defres{mm/cell/flash/action/replace/verdict}{not run}
\defres{mm/cell/flash/action/trigger/state}{not run}
\defres{mm/cell/flash/action/trigger/vcode}{0}
\defres{mm/cell/flash/action/trigger/verdict}{not run}
\defres{mm/cell/flash/memory_read/assist/acted}{100.0}
\defres{mm/cell/flash/memory_read/assist/delta}{+0.0}
\defres{mm/cell/flash/memory_read/assist/fig_delta}{+0.0}
\defres{mm/cell/flash/memory_read/assist/fig_saving}{-5}
\defres{mm/cell/flash/memory_read/assist/joint}{1}
\defres{mm/cell/flash/memory_read/assist/n}{200}
\defres{mm/cell/flash/memory_read/assist/row}{jev\_mem}
\defres{mm/cell/flash/memory_read/assist/saving}{-4.8}
\defres{mm/cell/flash/memory_read/assist/state}{run}
\defres{mm/cell/flash/memory_read/assist/vcode}{3}
\defres{mm/cell/flash/memory_read/assist/verdict}{no saving}
\defres{mm/cell/flash/memory_read/cascade/state}{not run}
\defres{mm/cell/flash/memory_read/cascade/vcode}{0}
\defres{mm/cell/flash/memory_read/cascade/verdict}{not run}
\defres{mm/cell/flash/memory_read/guard/state}{not run}
\defres{mm/cell/flash/memory_read/guard/vcode}{0}
\defres{mm/cell/flash/memory_read/guard/verdict}{not run}
\defres{mm/cell/flash/memory_read/replace/equiv}{assist}
\defres{mm/cell/flash/memory_read/replace/state}{not run}
\defres{mm/cell/flash/memory_read/replace/vcode}{0}
\defres{mm/cell/flash/memory_read/replace/verdict}{not run}
\defres{mm/cell/flash/memory_read/trigger/state}{not run}
\defres{mm/cell/flash/memory_read/trigger/vcode}{0}
\defres{mm/cell/flash/memory_read/trigger/verdict}{not run}
\defres{mm/cell/flash/memory_write/assist/state}{not run}
\defres{mm/cell/flash/memory_write/assist/vcode}{0}
\defres{mm/cell/flash/memory_write/assist/verdict}{not run}
\defres{mm/cell/flash/memory_write/cascade/state}{not run}
\defres{mm/cell/flash/memory_write/cascade/vcode}{0}
\defres{mm/cell/flash/memory_write/cascade/verdict}{not run}
\defres{mm/cell/flash/memory_write/guard/state}{not run}
\defres{mm/cell/flash/memory_write/guard/vcode}{0}
\defres{mm/cell/flash/memory_write/guard/verdict}{not run}
\defres{mm/cell/flash/memory_write/replace/equiv}{trigger}
\defres{mm/cell/flash/memory_write/replace/state}{not run}
\defres{mm/cell/flash/memory_write/replace/vcode}{0}
\defres{mm/cell/flash/memory_write/replace/verdict}{not run}
\defres{mm/cell/flash/memory_write/trigger/acted}{99.5}
\defres{mm/cell/flash/memory_write/trigger/delta}{-1.0}
\defres{mm/cell/flash/memory_write/trigger/fig_delta}{-1.0}
\defres{mm/cell/flash/memory_write/trigger/fig_saving}{-39}
\defres{mm/cell/flash/memory_write/trigger/joint}{0}
\defres{mm/cell/flash/memory_write/trigger/n}{200}
\defres{mm/cell/flash/memory_write/trigger/row}{jev\_memw}
\defres{mm/cell/flash/memory_write/trigger/saving}{-38.9}
\defres{mm/cell/flash/memory_write/trigger/state}{run}
\defres{mm/cell/flash/memory_write/trigger/vcode}{3}
\defres{mm/cell/flash/memory_write/trigger/verdict}{no saving}
\defres{mm/cell/flash/reflection/assist/state}{not run}
\defres{mm/cell/flash/reflection/assist/vcode}{0}
\defres{mm/cell/flash/reflection/assist/verdict}{not run}
\defres{mm/cell/flash/reflection/cascade/state}{not run}
\defres{mm/cell/flash/reflection/cascade/vcode}{0}
\defres{mm/cell/flash/reflection/cascade/verdict}{not run}
\defres{mm/cell/flash/reflection/guard/state}{not run}
\defres{mm/cell/flash/reflection/guard/vcode}{0}
\defres{mm/cell/flash/reflection/guard/verdict}{not run}
\defres{mm/cell/flash/reflection/replace/equiv}{trigger}
\defres{mm/cell/flash/reflection/replace/state}{not run}
\defres{mm/cell/flash/reflection/replace/vcode}{0}
\defres{mm/cell/flash/reflection/replace/verdict}{not run}
\defres{mm/cell/flash/reflection/trigger/acted}{13.9}
\defres{mm/cell/flash/reflection/trigger/alt_vcode}{3}
\defres{mm/cell/flash/reflection/trigger/alt_verdict}{no saving}
\defres{mm/cell/flash/reflection/trigger/delta}{+0.0}
\defres{mm/cell/flash/reflection/trigger/fig_delta}{+0.0}
\defres{mm/cell/flash/reflection/trigger/fig_saving}{1}
\defres{mm/cell/flash/reflection/trigger/joint}{0}
\defres{mm/cell/flash/reflection/trigger/n}{200}
\defres{mm/cell/flash/reflection/trigger/row}{jev\_reflect\_trigger}
\defres{mm/cell/flash/reflection/trigger/saving}{0.9}
\defres{mm/cell/flash/reflection/trigger/state}{run}
\defres{mm/cell/flash/reflection/trigger/vcode}{1}
\defres{mm/cell/flash/reflection/trigger/verdict}{takes over safely}
\defres{mm/cell/flash/routing/assist/state}{not run}
\defres{mm/cell/flash/routing/assist/vcode}{0}
\defres{mm/cell/flash/routing/assist/verdict}{not run}
\defres{mm/cell/flash/routing/cascade/state}{not run}
\defres{mm/cell/flash/routing/cascade/vcode}{0}
\defres{mm/cell/flash/routing/cascade/verdict}{not run}
\defres{mm/cell/flash/routing/guard/state}{not run}
\defres{mm/cell/flash/routing/guard/vcode}{0}
\defres{mm/cell/flash/routing/guard/verdict}{not run}
\defres{mm/cell/flash/routing/replace/equiv}{trigger}
\defres{mm/cell/flash/routing/replace/state}{not run}
\defres{mm/cell/flash/routing/replace/vcode}{0}
\defres{mm/cell/flash/routing/replace/verdict}{not run}
\defres{mm/cell/flash/routing/trigger/acted}{10.1}
\defres{mm/cell/flash/routing/trigger/delta}{+0.6}
\defres{mm/cell/flash/routing/trigger/fig_delta}{+0.6}
\defres{mm/cell/flash/routing/trigger/fig_saving}{-36}
\defres{mm/cell/flash/routing/trigger/joint}{0}
\defres{mm/cell/flash/routing/trigger/n}{500}
\defres{mm/cell/flash/routing/trigger/reg}{C4}
\defres{mm/cell/flash/routing/trigger/row}{jev\_route\_tau0.4}
\defres{mm/cell/flash/routing/trigger/saving}{-36.2}
\defres{mm/cell/flash/routing/trigger/state}{run}
\defres{mm/cell/flash/routing/trigger/vcode}{3}
\defres{mm/cell/flash/routing/trigger/verdict}{no saving}
\defres{mm/cell/flash/stop/assist/state}{not run}
\defres{mm/cell/flash/stop/assist/vcode}{0}
\defres{mm/cell/flash/stop/assist/verdict}{not run}
\defres{mm/cell/flash/stop/cascade/state}{not run}
\defres{mm/cell/flash/stop/cascade/vcode}{0}
\defres{mm/cell/flash/stop/cascade/verdict}{not run}
\defres{mm/cell/flash/stop/guard/acted}{17.3}
\defres{mm/cell/flash/stop/guard/delta}{-0.6}
\defres{mm/cell/flash/stop/guard/fig_delta}{-0.6}
\defres{mm/cell/flash/stop/guard/fig_saving}{-6}
\defres{mm/cell/flash/stop/guard/joint}{0}
\defres{mm/cell/flash/stop/guard/n}{500}
\defres{mm/cell/flash/stop/guard/reg}{C6F}
\defres{mm/cell/flash/stop/guard/row}{jev\_stop\_guard}
\defres{mm/cell/flash/stop/guard/saving}{-6.2}
\defres{mm/cell/flash/stop/guard/state}{run}
\defres{mm/cell/flash/stop/guard/vcode}{3}
\defres{mm/cell/flash/stop/guard/verdict}{no saving}
\defres{mm/cell/flash/stop/replace/equiv}{cascade}
\defres{mm/cell/flash/stop/replace/state}{not run}
\defres{mm/cell/flash/stop/replace/vcode}{0}
\defres{mm/cell/flash/stop/replace/verdict}{not run}
\defres{mm/cell/flash/stop/trigger/acted}{0.0}
\defres{mm/cell/flash/stop/trigger/delta}{+0.0}
\defres{mm/cell/flash/stop/trigger/fig_delta}{+0.0}
\defres{mm/cell/flash/stop/trigger/fig_saving}{0}
\defres{mm/cell/flash/stop/trigger/joint}{0}
\defres{mm/cell/flash/stop/trigger/n}{200}
\defres{mm/cell/flash/stop/trigger/row}{jev\_stop\_trigger}
\defres{mm/cell/flash/stop/trigger/saving}{-0.1}
\defres{mm/cell/flash/stop/trigger/state}{run}
\defres{mm/cell/flash/stop/trigger/vcode}{3}
\defres{mm/cell/flash/stop/trigger/verdict}{no saving}
\defres{mm/cell/flash/tool_params/assist/state}{not run}
\defres{mm/cell/flash/tool_params/assist/vcode}{0}
\defres{mm/cell/flash/tool_params/assist/verdict}{not run}
\defres{mm/cell/flash/tool_params/cascade/acted}{20.8}
\defres{mm/cell/flash/tool_params/cascade/coverage}{20.8}
\defres{mm/cell/flash/tool_params/cascade/delta}{+0.0}
\defres{mm/cell/flash/tool_params/cascade/fig_delta}{+0.0}
\defres{mm/cell/flash/tool_params/cascade/fig_saving}{14}
\defres{mm/cell/flash/tool_params/cascade/joint}{1}
\defres{mm/cell/flash/tool_params/cascade/n}{500}
\defres{mm/cell/flash/tool_params/cascade/reg}{C1F}
\defres{mm/cell/flash/tool_params/cascade/row}{jev\_ts\_cascade\_tauhat}
\defres{mm/cell/flash/tool_params/cascade/saving}{14.2}
\defres{mm/cell/flash/tool_params/cascade/state}{run}
\defres{mm/cell/flash/tool_params/cascade/vcode}{1}
\defres{mm/cell/flash/tool_params/cascade/verdict}{takes over safely}
\defres{mm/cell/flash/tool_params/guard/state}{not run}
\defres{mm/cell/flash/tool_params/guard/vcode}{0}
\defres{mm/cell/flash/tool_params/guard/verdict}{not run}
\defres{mm/cell/flash/tool_params/replace/acted}{85.7}
\defres{mm/cell/flash/tool_params/replace/coverage}{85.7}
\defres{mm/cell/flash/tool_params/replace/delta}{-20.0}
\defres{mm/cell/flash/tool_params/replace/fig_delta}{-20.0}
\defres{mm/cell/flash/tool_params/replace/fig_saving}{88}
\defres{mm/cell/flash/tool_params/replace/joint}{1}
\defres{mm/cell/flash/tool_params/replace/n}{200}
\defres{mm/cell/flash/tool_params/replace/row}{jev\_ts\_params\_replace}
\defres{mm/cell/flash/tool_params/replace/saving}{88.1}
\defres{mm/cell/flash/tool_params/replace/state}{run}
\defres{mm/cell/flash/tool_params/replace/vcode}{4}
\defres{mm/cell/flash/tool_params/replace/verdict}{costs success}
\defres{mm/cell/flash/tool_params/trigger/state}{not run}
\defres{mm/cell/flash/tool_params/trigger/vcode}{0}
\defres{mm/cell/flash/tool_params/trigger/verdict}{not run}
\defres{mm/cell/flash/tool_select/assist/acted}{100.0}
\defres{mm/cell/flash/tool_select/assist/delta}{-7.8}
\defres{mm/cell/flash/tool_select/assist/fig_delta}{-7.8}
\defres{mm/cell/flash/tool_select/assist/fig_saving}{54}
\defres{mm/cell/flash/tool_select/assist/joint}{0}
\defres{mm/cell/flash/tool_select/assist/n}{500}
\defres{mm/cell/flash/tool_select/assist/reg}{C2F}
\defres{mm/cell/flash/tool_select/assist/row}{jev\_ts\_assist\_k3}
\defres{mm/cell/flash/tool_select/assist/saving}{53.7}
\defres{mm/cell/flash/tool_select/assist/state}{run}
\defres{mm/cell/flash/tool_select/assist/vcode}{4}
\defres{mm/cell/flash/tool_select/assist/verdict}{costs success}
\defres{mm/cell/flash/tool_select/cascade/acted}{27.2}
\defres{mm/cell/flash/tool_select/cascade/coverage}{27.2}
\defres{mm/cell/flash/tool_select/cascade/delta}{+0.0}
\defres{mm/cell/flash/tool_select/cascade/fig_delta}{+0.0}
\defres{mm/cell/flash/tool_select/cascade/fig_saving}{14}
\defres{mm/cell/flash/tool_select/cascade/joint}{1}
\defres{mm/cell/flash/tool_select/cascade/n}{500}
\defres{mm/cell/flash/tool_select/cascade/reg}{C1F}
\defres{mm/cell/flash/tool_select/cascade/row}{jev\_ts\_cascade\_tauhat}
\defres{mm/cell/flash/tool_select/cascade/saving}{14.2}
\defres{mm/cell/flash/tool_select/cascade/state}{run}
\defres{mm/cell/flash/tool_select/cascade/vcode}{1}
\defres{mm/cell/flash/tool_select/cascade/verdict}{takes over safely}
\defres{mm/cell/flash/tool_select/guard/acted}{2.1}
\defres{mm/cell/flash/tool_select/guard/delta}{+0.0}
\defres{mm/cell/flash/tool_select/guard/fig_delta}{+0.0}
\defres{mm/cell/flash/tool_select/guard/fig_saving}{0}
\defres{mm/cell/flash/tool_select/guard/joint}{0}
\defres{mm/cell/flash/tool_select/guard/n}{200}
\defres{mm/cell/flash/tool_select/guard/row}{jev\_ts\_guard}
\defres{mm/cell/flash/tool_select/guard/saving}{-0.2}
\defres{mm/cell/flash/tool_select/guard/state}{run}
\defres{mm/cell/flash/tool_select/guard/vcode}{3}
\defres{mm/cell/flash/tool_select/guard/verdict}{no saving}
\defres{mm/cell/flash/tool_select/replace/acted}{100.0}
\defres{mm/cell/flash/tool_select/replace/coverage}{100.0}
\defres{mm/cell/flash/tool_select/replace/delta}{-19.0}
\defres{mm/cell/flash/tool_select/replace/fig_delta}{-19.0}
\defres{mm/cell/flash/tool_select/replace/fig_saving}{67}
\defres{mm/cell/flash/tool_select/replace/joint}{0}
\defres{mm/cell/flash/tool_select/replace/n}{200}
\defres{mm/cell/flash/tool_select/replace/row}{jev\_ts\_replace}
\defres{mm/cell/flash/tool_select/replace/saving}{67.0}
\defres{mm/cell/flash/tool_select/replace/state}{run}
\defres{mm/cell/flash/tool_select/replace/vcode}{4}
\defres{mm/cell/flash/tool_select/replace/verdict}{costs success}
\defres{mm/cell/flash/tool_select/trigger/state}{not run}
\defres{mm/cell/flash/tool_select/trigger/vcode}{0}
\defres{mm/cell/flash/tool_select/trigger/verdict}{not run}
\defres{mm/cell/lite/action/assist/state}{not run}
\defres{mm/cell/lite/action/assist/vcode}{0}
\defres{mm/cell/lite/action/assist/verdict}{not run}
\defres{mm/cell/lite/action/cascade/state}{not run}
\defres{mm/cell/lite/action/cascade/vcode}{0}
\defres{mm/cell/lite/action/cascade/verdict}{not run}
\defres{mm/cell/lite/action/guard/state}{not run}
\defres{mm/cell/lite/action/guard/vcode}{0}
\defres{mm/cell/lite/action/guard/verdict}{not run}
\defres{mm/cell/lite/action/replace/state}{not run}
\defres{mm/cell/lite/action/replace/vcode}{0}
\defres{mm/cell/lite/action/replace/verdict}{not run}
\defres{mm/cell/lite/action/trigger/state}{not run}
\defres{mm/cell/lite/action/trigger/vcode}{0}
\defres{mm/cell/lite/action/trigger/verdict}{not run}
\defres{mm/cell/lite/memory_read/assist/state}{not run}
\defres{mm/cell/lite/memory_read/assist/vcode}{0}
\defres{mm/cell/lite/memory_read/assist/verdict}{not run}
\defres{mm/cell/lite/memory_read/cascade/state}{not run}
\defres{mm/cell/lite/memory_read/cascade/vcode}{0}
\defres{mm/cell/lite/memory_read/cascade/verdict}{not run}
\defres{mm/cell/lite/memory_read/guard/state}{not run}
\defres{mm/cell/lite/memory_read/guard/vcode}{0}
\defres{mm/cell/lite/memory_read/guard/verdict}{not run}
\defres{mm/cell/lite/memory_read/replace/equiv}{assist}
\defres{mm/cell/lite/memory_read/replace/state}{not run}
\defres{mm/cell/lite/memory_read/replace/vcode}{0}
\defres{mm/cell/lite/memory_read/replace/verdict}{not run}
\defres{mm/cell/lite/memory_read/trigger/state}{not run}
\defres{mm/cell/lite/memory_read/trigger/vcode}{0}
\defres{mm/cell/lite/memory_read/trigger/verdict}{not run}
\defres{mm/cell/lite/memory_write/assist/state}{not run}
\defres{mm/cell/lite/memory_write/assist/vcode}{0}
\defres{mm/cell/lite/memory_write/assist/verdict}{not run}
\defres{mm/cell/lite/memory_write/cascade/state}{not run}
\defres{mm/cell/lite/memory_write/cascade/vcode}{0}
\defres{mm/cell/lite/memory_write/cascade/verdict}{not run}
\defres{mm/cell/lite/memory_write/guard/state}{not run}
\defres{mm/cell/lite/memory_write/guard/vcode}{0}
\defres{mm/cell/lite/memory_write/guard/verdict}{not run}
\defres{mm/cell/lite/memory_write/replace/equiv}{trigger}
\defres{mm/cell/lite/memory_write/replace/state}{not run}
\defres{mm/cell/lite/memory_write/replace/vcode}{0}
\defres{mm/cell/lite/memory_write/replace/verdict}{not run}
\defres{mm/cell/lite/memory_write/trigger/state}{not run}
\defres{mm/cell/lite/memory_write/trigger/vcode}{0}
\defres{mm/cell/lite/memory_write/trigger/verdict}{not run}
\defres{mm/cell/lite/reflection/assist/state}{not run}
\defres{mm/cell/lite/reflection/assist/vcode}{0}
\defres{mm/cell/lite/reflection/assist/verdict}{not run}
\defres{mm/cell/lite/reflection/cascade/state}{not run}
\defres{mm/cell/lite/reflection/cascade/vcode}{0}
\defres{mm/cell/lite/reflection/cascade/verdict}{not run}
\defres{mm/cell/lite/reflection/guard/state}{not run}
\defres{mm/cell/lite/reflection/guard/vcode}{0}
\defres{mm/cell/lite/reflection/guard/verdict}{not run}
\defres{mm/cell/lite/reflection/replace/equiv}{trigger}
\defres{mm/cell/lite/reflection/replace/state}{not run}
\defres{mm/cell/lite/reflection/replace/vcode}{0}
\defres{mm/cell/lite/reflection/replace/verdict}{not run}
\defres{mm/cell/lite/reflection/trigger/acted}{14.8}
\defres{mm/cell/lite/reflection/trigger/delta}{+1.8}
\defres{mm/cell/lite/reflection/trigger/fig_delta}{+1.8}
\defres{mm/cell/lite/reflection/trigger/fig_saving}{-2}
\defres{mm/cell/lite/reflection/trigger/joint}{0}
\defres{mm/cell/lite/reflection/trigger/n}{500}
\defres{mm/cell/lite/reflection/trigger/reg}{C5}
\defres{mm/cell/lite/reflection/trigger/row}{jev\_reflect\_trigger\_s2lite}
\defres{mm/cell/lite/reflection/trigger/saving}{-1.9}
\defres{mm/cell/lite/reflection/trigger/state}{run}
\defres{mm/cell/lite/reflection/trigger/vcode}{3}
\defres{mm/cell/lite/reflection/trigger/verdict}{no saving}
\defres{mm/cell/lite/routing/assist/state}{not run}
\defres{mm/cell/lite/routing/assist/vcode}{0}
\defres{mm/cell/lite/routing/assist/verdict}{not run}
\defres{mm/cell/lite/routing/cascade/state}{not run}
\defres{mm/cell/lite/routing/cascade/vcode}{0}
\defres{mm/cell/lite/routing/cascade/verdict}{not run}
\defres{mm/cell/lite/routing/guard/state}{not run}
\defres{mm/cell/lite/routing/guard/vcode}{0}
\defres{mm/cell/lite/routing/guard/verdict}{not run}
\defres{mm/cell/lite/routing/replace/equiv}{trigger}
\defres{mm/cell/lite/routing/replace/state}{not run}
\defres{mm/cell/lite/routing/replace/vcode}{0}
\defres{mm/cell/lite/routing/replace/verdict}{not run}
\defres{mm/cell/lite/routing/trigger/acted}{10.1}
\defres{mm/cell/lite/routing/trigger/delta}{+0.6}
\defres{mm/cell/lite/routing/trigger/fig_delta}{+0.6}
\defres{mm/cell/lite/routing/trigger/fig_saving}{-36}
\defres{mm/cell/lite/routing/trigger/joint}{0}
\defres{mm/cell/lite/routing/trigger/n}{500}
\defres{mm/cell/lite/routing/trigger/reg}{C4}
\defres{mm/cell/lite/routing/trigger/row}{jev\_route\_tau0.4}
\defres{mm/cell/lite/routing/trigger/saving}{-36.2}
\defres{mm/cell/lite/routing/trigger/state}{run}
\defres{mm/cell/lite/routing/trigger/vcode}{3}
\defres{mm/cell/lite/routing/trigger/verdict}{no saving}
\defres{mm/cell/lite/stop/assist/state}{not run}
\defres{mm/cell/lite/stop/assist/vcode}{0}
\defres{mm/cell/lite/stop/assist/verdict}{not run}
\defres{mm/cell/lite/stop/cascade/state}{not run}
\defres{mm/cell/lite/stop/cascade/vcode}{0}
\defres{mm/cell/lite/stop/cascade/verdict}{not run}
\defres{mm/cell/lite/stop/guard/acted}{72.6}
\defres{mm/cell/lite/stop/guard/delta}{+1.6}
\defres{mm/cell/lite/stop/guard/fig_delta}{+1.6}
\defres{mm/cell/lite/stop/guard/fig_saving}{-32}
\defres{mm/cell/lite/stop/guard/joint}{0}
\defres{mm/cell/lite/stop/guard/n}{500}
\defres{mm/cell/lite/stop/guard/reg}{C6L}
\defres{mm/cell/lite/stop/guard/row}{jev\_stop\_guard\_s2lite}
\defres{mm/cell/lite/stop/guard/saving}{-32.1}
\defres{mm/cell/lite/stop/guard/state}{run}
\defres{mm/cell/lite/stop/guard/vcode}{3}
\defres{mm/cell/lite/stop/guard/verdict}{no saving}
\defres{mm/cell/lite/stop/replace/equiv}{cascade}
\defres{mm/cell/lite/stop/replace/state}{not run}
\defres{mm/cell/lite/stop/replace/vcode}{0}
\defres{mm/cell/lite/stop/replace/verdict}{not run}
\defres{mm/cell/lite/stop/trigger/state}{not run}
\defres{mm/cell/lite/stop/trigger/vcode}{0}
\defres{mm/cell/lite/stop/trigger/verdict}{not run}
\defres{mm/cell/lite/tool_params/assist/state}{not run}
\defres{mm/cell/lite/tool_params/assist/vcode}{0}
\defres{mm/cell/lite/tool_params/assist/verdict}{not run}
\defres{mm/cell/lite/tool_params/cascade/acted}{0.0}
\defres{mm/cell/lite/tool_params/cascade/coverage}{0.0}
\defres{mm/cell/lite/tool_params/cascade/delta}{+1.0}
\defres{mm/cell/lite/tool_params/cascade/fig_delta}{+1.0}
\defres{mm/cell/lite/tool_params/cascade/fig_saving}{0}
\defres{mm/cell/lite/tool_params/cascade/joint}{1}
\defres{mm/cell/lite/tool_params/cascade/n}{500}
\defres{mm/cell/lite/tool_params/cascade/reg}{C1L}
\defres{mm/cell/lite/tool_params/cascade/row}{jev\_ts\_cascade\_tau0.9\_s2lite}
\defres{mm/cell/lite/tool_params/cascade/saving}{0.2}
\defres{mm/cell/lite/tool_params/cascade/state}{run}
\defres{mm/cell/lite/tool_params/cascade/vcode}{2}
\defres{mm/cell/lite/tool_params/cascade/verdict}{mixed}
\defres{mm/cell/lite/tool_params/guard/state}{not run}
\defres{mm/cell/lite/tool_params/guard/vcode}{0}
\defres{mm/cell/lite/tool_params/guard/verdict}{not run}
\defres{mm/cell/lite/tool_params/replace/state}{not run}
\defres{mm/cell/lite/tool_params/replace/vcode}{0}
\defres{mm/cell/lite/tool_params/replace/verdict}{not run}
\defres{mm/cell/lite/tool_params/trigger/state}{not run}
\defres{mm/cell/lite/tool_params/trigger/vcode}{0}
\defres{mm/cell/lite/tool_params/trigger/verdict}{not run}
\defres{mm/cell/lite/tool_select/assist/acted}{100.0}
\defres{mm/cell/lite/tool_select/assist/delta}{-3.4}
\defres{mm/cell/lite/tool_select/assist/fig_delta}{-3.4}
\defres{mm/cell/lite/tool_select/assist/fig_saving}{52}
\defres{mm/cell/lite/tool_select/assist/joint}{0}
\defres{mm/cell/lite/tool_select/assist/n}{500}
\defres{mm/cell/lite/tool_select/assist/reg}{C2L}
\defres{mm/cell/lite/tool_select/assist/row}{jev\_ts\_assist\_k3\_s2lite}
\defres{mm/cell/lite/tool_select/assist/saving}{52.0}
\defres{mm/cell/lite/tool_select/assist/state}{run}
\defres{mm/cell/lite/tool_select/assist/vcode}{4}
\defres{mm/cell/lite/tool_select/assist/verdict}{costs success}
\defres{mm/cell/lite/tool_select/cascade/acted}{0.0}
\defres{mm/cell/lite/tool_select/cascade/coverage}{0.0}
\defres{mm/cell/lite/tool_select/cascade/delta}{+1.0}
\defres{mm/cell/lite/tool_select/cascade/fig_delta}{+1.0}
\defres{mm/cell/lite/tool_select/cascade/fig_saving}{0}
\defres{mm/cell/lite/tool_select/cascade/joint}{1}
\defres{mm/cell/lite/tool_select/cascade/n}{500}
\defres{mm/cell/lite/tool_select/cascade/reg}{C1L}
\defres{mm/cell/lite/tool_select/cascade/row}{jev\_ts\_cascade\_tau0.9\_s2lite}
\defres{mm/cell/lite/tool_select/cascade/saving}{0.2}
\defres{mm/cell/lite/tool_select/cascade/state}{run}
\defres{mm/cell/lite/tool_select/cascade/vcode}{2}
\defres{mm/cell/lite/tool_select/cascade/verdict}{mixed}
\defres{mm/cell/lite/tool_select/guard/acted}{3.0}
\defres{mm/cell/lite/tool_select/guard/delta}{+4.5}
\defres{mm/cell/lite/tool_select/guard/fig_delta}{+4.5}
\defres{mm/cell/lite/tool_select/guard/fig_saving}{-7}
\defres{mm/cell/lite/tool_select/guard/joint}{0}
\defres{mm/cell/lite/tool_select/guard/n}{200}
\defres{mm/cell/lite/tool_select/guard/row}{jev\_ts\_guard\_s2lite}
\defres{mm/cell/lite/tool_select/guard/saving}{-6.7}
\defres{mm/cell/lite/tool_select/guard/state}{run}
\defres{mm/cell/lite/tool_select/guard/vcode}{3}
\defres{mm/cell/lite/tool_select/guard/verdict}{no saving}
\defres{mm/cell/lite/tool_select/replace/state}{not run}
\defres{mm/cell/lite/tool_select/replace/vcode}{0}
\defres{mm/cell/lite/tool_select/replace/verdict}{not run}
\defres{mm/cell/lite/tool_select/trigger/state}{not run}
\defres{mm/cell/lite/tool_select/trigger/vcode}{0}
\defres{mm/cell/lite/tool_select/trigger/verdict}{not run}
\defres{mm/count/flash/costs}{3}
\defres{mm/count/flash/equivalent}{0}
\defres{mm/count/flash/mixed}{0}
\defres{mm/count/flash/no_saving}{6}
\defres{mm/count/flash/not_implemented}{0}
\defres{mm/count/flash/not_run}{28}
\defres{mm/count/flash/pairs}{40}
\defres{mm/count/flash/run}{12}
\defres{mm/count/flash/safe}{3}
\defres{mm/count/flash/same_rule}{5}
\defres{mm/count/flash/undefined}{0}
\defres{mm/count/flash/valid}{40}
\defres{mm/count/lite/costs}{1}
\defres{mm/count/lite/equivalent}{0}
\defres{mm/count/lite/mixed}{2}
\defres{mm/count/lite/no_saving}{4}
\defres{mm/count/lite/not_implemented}{0}
\defres{mm/count/lite/not_run}{33}
\defres{mm/count/lite/pairs}{40}
\defres{mm/count/lite/run}{7}
\defres{mm/count/lite/safe}{0}
\defres{mm/count/lite/same_rule}{5}
\defres{mm/count/lite/undefined}{0}
\defres{mm/count/lite/valid}{40}
\defres{mm/memory_read/assist/jev_mem/acc}{57.6}
\defres{mm/memory_read/assist/jev_mem/accepted_acc}{57.6}
\defres{mm/memory_read/assist/jev_mem/acted}{100.0}
\defres{mm/memory_read/assist/jev_mem/acted_kind}{shortlist}
\defres{mm/memory_read/assist/jev_mem/cost_k}{42.6}
\defres{mm/memory_read/assist/jev_mem/cost_ref_k}{40.6}
\defres{mm/memory_read/assist/jev_mem/delta}{+0.0}
\defres{mm/memory_read/assist/jev_mem/delta_ci/hi}{+0.0}
\defres{mm/memory_read/assist/jev_mem/delta_ci/lo}{+0.0}
\defres{mm/memory_read/assist/jev_mem/fig_delta}{+0.0}
\defres{mm/memory_read/assist/jev_mem/fig_saving}{-5}
\defres{mm/memory_read/assist/jev_mem/n}{200}
\defres{mm/memory_read/assist/jev_mem/n_dropped}{0}
\defres{mm/memory_read/assist/jev_mem/s1_acc}{57.6}
\defres{mm/memory_read/assist/jev_mem/saving}{-4.8}
\defres{mm/memory_read/assist/jev_mem/saving_ci/hi}{-3.3}
\defres{mm/memory_read/assist/jev_mem/saving_ci/lo}{-6.2}
\defres{mm/memory_read/assist/jev_mem/status}{descriptive}
\defres{mm/memory_read/assist/jev_mem/success}{100.0}
\defres{mm/memory_read/assist/jev_mem/success_ref}{100.0}
\defres{mm/memory_read/assist/jev_mem/vcode}{3}
\defres{mm/memory_read/assist/jev_mem/verdict}{no saving}
\defres{mm/memory_write/always/mem_always/cost_k}{55.4}
\defres{mm/memory_write/always/mem_always/cost_ref_k}{40.6}
\defres{mm/memory_write/always/mem_always/delta}{-2.0}
\defres{mm/memory_write/always/mem_always/delta_ci/hi}{-0.5}
\defres{mm/memory_write/always/mem_always/delta_ci/lo}{-4.0}
\defres{mm/memory_write/always/mem_always/fig_delta}{-2.0}
\defres{mm/memory_write/always/mem_always/fig_saving}{-36}
\defres{mm/memory_write/always/mem_always/n}{200}
\defres{mm/memory_write/always/mem_always/n_dropped}{0}
\defres{mm/memory_write/always/mem_always/saving}{-36.3}
\defres{mm/memory_write/always/mem_always/saving_ci/hi}{-29.7}
\defres{mm/memory_write/always/mem_always/saving_ci/lo}{-44.0}
\defres{mm/memory_write/always/mem_always/status}{descriptive}
\defres{mm/memory_write/always/mem_always/success}{98.0}
\defres{mm/memory_write/always/mem_always/success_ref}{100.0}
\defres{mm/memory_write/llm/mem_llm_gate/cost_k}{64.8}
\defres{mm/memory_write/llm/mem_llm_gate/cost_ref_k}{40.6}
\defres{mm/memory_write/llm/mem_llm_gate/delta}{+0.0}
\defres{mm/memory_write/llm/mem_llm_gate/delta_ci/hi}{+0.0}
\defres{mm/memory_write/llm/mem_llm_gate/delta_ci/lo}{+0.0}
\defres{mm/memory_write/llm/mem_llm_gate/fig_delta}{+0.0}
\defres{mm/memory_write/llm/mem_llm_gate/fig_saving}{-60}
\defres{mm/memory_write/llm/mem_llm_gate/n}{200}
\defres{mm/memory_write/llm/mem_llm_gate/n_dropped}{0}
\defres{mm/memory_write/llm/mem_llm_gate/saving}{-59.6}
\defres{mm/memory_write/llm/mem_llm_gate/saving_ci/hi}{-54.5}
\defres{mm/memory_write/llm/mem_llm_gate/saving_ci/lo}{-64.2}
\defres{mm/memory_write/llm/mem_llm_gate/status}{descriptive}
\defres{mm/memory_write/llm/mem_llm_gate/success}{100.0}
\defres{mm/memory_write/llm/mem_llm_gate/success_ref}{100.0}
\defres{mm/memory_write/trigger/heuristic_memw/acc}{63.9}
\defres{mm/memory_write/trigger/heuristic_memw/accepted_acc}{63.9}
\defres{mm/memory_write/trigger/heuristic_memw/acted}{92.2}
\defres{mm/memory_write/trigger/heuristic_memw/acted_kind}{fired}
\defres{mm/memory_write/trigger/heuristic_memw/cost_k}{51.7}
\defres{mm/memory_write/trigger/heuristic_memw/cost_ref_k}{40.9}
\defres{mm/memory_write/trigger/heuristic_memw/delta}{-2.5}
\defres{mm/memory_write/trigger/heuristic_memw/delta_ci/hi}{-0.5}
\defres{mm/memory_write/trigger/heuristic_memw/delta_ci/lo}{-5.0}
\defres{mm/memory_write/trigger/heuristic_memw/fig_delta}{-2.5}
\defres{mm/memory_write/trigger/heuristic_memw/fig_saving}{-26}
\defres{mm/memory_write/trigger/heuristic_memw/n}{200}
\defres{mm/memory_write/trigger/heuristic_memw/n_dropped}{0}
\defres{mm/memory_write/trigger/heuristic_memw/s1_acc}{63.9}
\defres{mm/memory_write/trigger/heuristic_memw/saving}{-26.3}
\defres{mm/memory_write/trigger/heuristic_memw/saving_ci/hi}{-22.7}
\defres{mm/memory_write/trigger/heuristic_memw/saving_ci/lo}{-30.1}
\defres{mm/memory_write/trigger/heuristic_memw/status}{descriptive}
\defres{mm/memory_write/trigger/heuristic_memw/success}{97.5}
\defres{mm/memory_write/trigger/heuristic_memw/success_ref}{100.0}
\defres{mm/memory_write/trigger/heuristic_memw/vcode}{3}
\defres{mm/memory_write/trigger/heuristic_memw/verdict}{no saving}
\defres{mm/memory_write/trigger/jev_mem/acc}{69.2}
\defres{mm/memory_write/trigger/jev_mem/accepted_acc}{69.2}
\defres{mm/memory_write/trigger/jev_mem/acted}{100.0}
\defres{mm/memory_write/trigger/jev_mem/acted_kind}{fired}
\defres{mm/memory_write/trigger/jev_mem/cost_k}{42.6}
\defres{mm/memory_write/trigger/jev_mem/cost_ref_k}{40.6}
\defres{mm/memory_write/trigger/jev_mem/delta}{+0.0}
\defres{mm/memory_write/trigger/jev_mem/delta_ci/hi}{+0.0}
\defres{mm/memory_write/trigger/jev_mem/delta_ci/lo}{+0.0}
\defres{mm/memory_write/trigger/jev_mem/fig_delta}{+0.0}
\defres{mm/memory_write/trigger/jev_mem/fig_saving}{-5}
\defres{mm/memory_write/trigger/jev_mem/n}{200}
\defres{mm/memory_write/trigger/jev_mem/n_dropped}{0}
\defres{mm/memory_write/trigger/jev_mem/s1_acc}{69.2}
\defres{mm/memory_write/trigger/jev_mem/saving}{-4.8}
\defres{mm/memory_write/trigger/jev_mem/saving_ci/hi}{-3.3}
\defres{mm/memory_write/trigger/jev_mem/saving_ci/lo}{-6.2}
\defres{mm/memory_write/trigger/jev_mem/status}{descriptive}
\defres{mm/memory_write/trigger/jev_mem/success}{100.0}
\defres{mm/memory_write/trigger/jev_mem/success_ref}{100.0}
\defres{mm/memory_write/trigger/jev_mem/vcode}{3}
\defres{mm/memory_write/trigger/jev_mem/verdict}{no saving}
\defres{mm/memory_write/trigger/jev_memw/acc}{69.2}
\defres{mm/memory_write/trigger/jev_memw/accepted_acc}{69.2}
\defres{mm/memory_write/trigger/jev_memw/acted}{99.5}
\defres{mm/memory_write/trigger/jev_memw/acted_kind}{fired}
\defres{mm/memory_write/trigger/jev_memw/cost_k}{56.9}
\defres{mm/memory_write/trigger/jev_memw/cost_ref_k}{40.9}
\defres{mm/memory_write/trigger/jev_memw/delta}{-1.0}
\defres{mm/memory_write/trigger/jev_memw/delta_ci/hi}{+0.0}
\defres{mm/memory_write/trigger/jev_memw/delta_ci/lo}{-2.5}
\defres{mm/memory_write/trigger/jev_memw/fig_delta}{-1.0}
\defres{mm/memory_write/trigger/jev_memw/fig_saving}{-39}
\defres{mm/memory_write/trigger/jev_memw/n}{200}
\defres{mm/memory_write/trigger/jev_memw/n_dropped}{0}
\defres{mm/memory_write/trigger/jev_memw/s1_acc}{69.2}
\defres{mm/memory_write/trigger/jev_memw/saving}{-38.9}
\defres{mm/memory_write/trigger/jev_memw/saving_ci/hi}{-35.5}
\defres{mm/memory_write/trigger/jev_memw/saving_ci/lo}{-42.2}
\defres{mm/memory_write/trigger/jev_memw/status}{descriptive}
\defres{mm/memory_write/trigger/jev_memw/success}{99.0}
\defres{mm/memory_write/trigger/jev_memw/success_ref}{100.0}
\defres{mm/memory_write/trigger/jev_memw/vcode}{3}
\defres{mm/memory_write/trigger/jev_memw/verdict}{no saving}
\defres{mm/memory_write/trigger/ratem_memw/acc}{67.4}
\defres{mm/memory_write/trigger/ratem_memw/accepted_acc}{67.4}
\defres{mm/memory_write/trigger/ratem_memw/acted}{99.4}
\defres{mm/memory_write/trigger/ratem_memw/acted_kind}{fired}
\defres{mm/memory_write/trigger/ratem_memw/cost_k}{55.6}
\defres{mm/memory_write/trigger/ratem_memw/cost_ref_k}{40.9}
\defres{mm/memory_write/trigger/ratem_memw/delta}{-1.5}
\defres{mm/memory_write/trigger/ratem_memw/delta_ci/hi}{+0.0}
\defres{mm/memory_write/trigger/ratem_memw/delta_ci/lo}{-3.5}
\defres{mm/memory_write/trigger/ratem_memw/fig_delta}{-1.5}
\defres{mm/memory_write/trigger/ratem_memw/fig_saving}{-36}
\defres{mm/memory_write/trigger/ratem_memw/n}{200}
\defres{mm/memory_write/trigger/ratem_memw/n_dropped}{0}
\defres{mm/memory_write/trigger/ratem_memw/s1_acc}{67.4}
\defres{mm/memory_write/trigger/ratem_memw/saving}{-35.8}
\defres{mm/memory_write/trigger/ratem_memw/saving_ci/hi}{-31.9}
\defres{mm/memory_write/trigger/ratem_memw/saving_ci/lo}{-40.0}
\defres{mm/memory_write/trigger/ratem_memw/status}{descriptive}
\defres{mm/memory_write/trigger/ratem_memw/success}{98.5}
\defres{mm/memory_write/trigger/ratem_memw/success_ref}{100.0}
\defres{mm/memory_write/trigger/ratem_memw/vcode}{3}
\defres{mm/memory_write/trigger/ratem_memw/verdict}{no saving}
\defres{mm/reflection/always/reflect_always-e2c/cost_k}{67.7}
\defres{mm/reflection/always/reflect_always-e2c/cost_ref_k}{40.9}
\defres{mm/reflection/always/reflect_always-e2c/delta}{-2.5}
\defres{mm/reflection/always/reflect_always-e2c/delta_ci/hi}{-0.5}
\defres{mm/reflection/always/reflect_always-e2c/delta_ci/lo}{-5.0}
\defres{mm/reflection/always/reflect_always-e2c/fig_delta}{-2.5}
\defres{mm/reflection/always/reflect_always-e2c/fig_saving}{-65}
\defres{mm/reflection/always/reflect_always-e2c/n}{200}
\defres{mm/reflection/always/reflect_always-e2c/n_dropped}{0}
\defres{mm/reflection/always/reflect_always-e2c/saving}{-65.3}
\defres{mm/reflection/always/reflect_always-e2c/saving_ci/hi}{-59.6}
\defres{mm/reflection/always/reflect_always-e2c/saving_ci/lo}{-70.9}
\defres{mm/reflection/always/reflect_always-e2c/status}{replicate}
\defres{mm/reflection/always/reflect_always-e2c/success}{97.5}
\defres{mm/reflection/always/reflect_always-e2c/success_ref}{100.0}
\defres{mm/reflection/always/reflect_always/cost_k}{73.1}
\defres{mm/reflection/always/reflect_always/cost_ref_k}{40.6}
\defres{mm/reflection/always/reflect_always/delta}{-4.0}
\defres{mm/reflection/always/reflect_always/delta_ci/hi}{-1.5}
\defres{mm/reflection/always/reflect_always/delta_ci/lo}{-7.0}
\defres{mm/reflection/always/reflect_always/fig_delta}{-4.0}
\defres{mm/reflection/always/reflect_always/fig_saving}{-80}
\defres{mm/reflection/always/reflect_always/n}{200}
\defres{mm/reflection/always/reflect_always/n_dropped}{0}
\defres{mm/reflection/always/reflect_always/saving}{-80.0}
\defres{mm/reflection/always/reflect_always/saving_ci/hi}{-73.1}
\defres{mm/reflection/always/reflect_always/saving_ci/lo}{-87.9}
\defres{mm/reflection/always/reflect_always/status}{descriptive}
\defres{mm/reflection/always/reflect_always/success}{96.0}
\defres{mm/reflection/always/reflect_always/success_ref}{100.0}
\defres{mm/reflection/always/reflect_always_s2lite/cost_k}{14.3}
\defres{mm/reflection/always/reflect_always_s2lite/cost_ref_k}{9.8}
\defres{mm/reflection/always/reflect_always_s2lite/delta}{+8.5}
\defres{mm/reflection/always/reflect_always_s2lite/delta_ci/hi}{+13.0}
\defres{mm/reflection/always/reflect_always_s2lite/delta_ci/lo}{+4.0}
\defres{mm/reflection/always/reflect_always_s2lite/fig_delta}{+8.5}
\defres{mm/reflection/always/reflect_always_s2lite/fig_saving}{-46}
\defres{mm/reflection/always/reflect_always_s2lite/n}{200}
\defres{mm/reflection/always/reflect_always_s2lite/n_dropped}{0}
\defres{mm/reflection/always/reflect_always_s2lite/saving}{-46.4}
\defres{mm/reflection/always/reflect_always_s2lite/saving_ci/hi}{-42.7}
\defres{mm/reflection/always/reflect_always_s2lite/saving_ci/lo}{-49.9}
\defres{mm/reflection/always/reflect_always_s2lite/status}{descriptive}
\defres{mm/reflection/always/reflect_always_s2lite/success}{89.5}
\defres{mm/reflection/always/reflect_always_s2lite/success_ref}{81.0}
\defres{mm/reflection/trigger/heuristic_reflect_trigger/acc}{100.0}
\defres{mm/reflection/trigger/heuristic_reflect_trigger/accepted_acc}{100.0}
\defres{mm/reflection/trigger/heuristic_reflect_trigger/acted}{0.1}
\defres{mm/reflection/trigger/heuristic_reflect_trigger/acted_kind}{fired}
\defres{mm/reflection/trigger/heuristic_reflect_trigger/cost_k}{40.7}
\defres{mm/reflection/trigger/heuristic_reflect_trigger/cost_ref_k}{40.9}
\defres{mm/reflection/trigger/heuristic_reflect_trigger/delta}{+0.0}
\defres{mm/reflection/trigger/heuristic_reflect_trigger/delta_ci/hi}{+0.0}
\defres{mm/reflection/trigger/heuristic_reflect_trigger/delta_ci/lo}{+0.0}
\defres{mm/reflection/trigger/heuristic_reflect_trigger/fig_delta}{+0.0}
\defres{mm/reflection/trigger/heuristic_reflect_trigger/fig_saving}{1}
\defres{mm/reflection/trigger/heuristic_reflect_trigger/n}{200}
\defres{mm/reflection/trigger/heuristic_reflect_trigger/n_dropped}{0}
\defres{mm/reflection/trigger/heuristic_reflect_trigger/s1_acc}{100.0}
\defres{mm/reflection/trigger/heuristic_reflect_trigger/saving}{0.6}
\defres{mm/reflection/trigger/heuristic_reflect_trigger/saving_ci/hi}{1.3}
\defres{mm/reflection/trigger/heuristic_reflect_trigger/saving_ci/lo}{-0.1}
\defres{mm/reflection/trigger/heuristic_reflect_trigger/status}{descriptive}
\defres{mm/reflection/trigger/heuristic_reflect_trigger/success}{100.0}
\defres{mm/reflection/trigger/heuristic_reflect_trigger/success_ref}{100.0}
\defres{mm/reflection/trigger/heuristic_reflect_trigger/vcode}{2}
\defres{mm/reflection/trigger/heuristic_reflect_trigger/verdict}{mixed}
\defres{mm/reflection/trigger/heuristic_reflect_trigger_s2lite/acc}{97.3}
\defres{mm/reflection/trigger/heuristic_reflect_trigger_s2lite/accepted_acc}{97.3}
\defres{mm/reflection/trigger/heuristic_reflect_trigger_s2lite/acted}{0.2}
\defres{mm/reflection/trigger/heuristic_reflect_trigger_s2lite/acted_kind}{fired}
\defres{mm/reflection/trigger/heuristic_reflect_trigger_s2lite/cost_k}{9.7}
\defres{mm/reflection/trigger/heuristic_reflect_trigger_s2lite/cost_ref_k}{9.7}
\defres{mm/reflection/trigger/heuristic_reflect_trigger_s2lite/delta}{+1.5}
\defres{mm/reflection/trigger/heuristic_reflect_trigger_s2lite/delta_ci/hi}{+4.5}
\defres{mm/reflection/trigger/heuristic_reflect_trigger_s2lite/delta_ci/lo}{-1.5}
\defres{mm/reflection/trigger/heuristic_reflect_trigger_s2lite/fig_delta}{+1.5}
\defres{mm/reflection/trigger/heuristic_reflect_trigger_s2lite/fig_saving}{0}
\defres{mm/reflection/trigger/heuristic_reflect_trigger_s2lite/n}{200}
\defres{mm/reflection/trigger/heuristic_reflect_trigger_s2lite/n_dropped}{0}
\defres{mm/reflection/trigger/heuristic_reflect_trigger_s2lite/s1_acc}{97.3}
\defres{mm/reflection/trigger/heuristic_reflect_trigger_s2lite/saving}{-0.3}
\defres{mm/reflection/trigger/heuristic_reflect_trigger_s2lite/saving_ci/hi}{0.1}
\defres{mm/reflection/trigger/heuristic_reflect_trigger_s2lite/saving_ci/lo}{-0.7}
\defres{mm/reflection/trigger/heuristic_reflect_trigger_s2lite/status}{descriptive}
\defres{mm/reflection/trigger/heuristic_reflect_trigger_s2lite/success}{83.0}
\defres{mm/reflection/trigger/heuristic_reflect_trigger_s2lite/success_ref}{81.5}
\defres{mm/reflection/trigger/heuristic_reflect_trigger_s2lite/vcode}{3}
\defres{mm/reflection/trigger/heuristic_reflect_trigger_s2lite/verdict}{no saving}
\defres{mm/reflection/trigger/jev_reflect_trigger-e2c/acc}{100.0}
\defres{mm/reflection/trigger/jev_reflect_trigger-e2c/accepted_acc}{100.0}
\defres{mm/reflection/trigger/jev_reflect_trigger-e2c/acted}{14.1}
\defres{mm/reflection/trigger/jev_reflect_trigger-e2c/acted_kind}{fired}
\defres{mm/reflection/trigger/jev_reflect_trigger-e2c/cost_k}{42.9}
\defres{mm/reflection/trigger/jev_reflect_trigger-e2c/cost_ref_k}{40.9}
\defres{mm/reflection/trigger/jev_reflect_trigger-e2c/delta}{+0.0}
\defres{mm/reflection/trigger/jev_reflect_trigger-e2c/delta_ci/hi}{+0.0}
\defres{mm/reflection/trigger/jev_reflect_trigger-e2c/delta_ci/lo}{+0.0}
\defres{mm/reflection/trigger/jev_reflect_trigger-e2c/fig_delta}{+0.0}
\defres{mm/reflection/trigger/jev_reflect_trigger-e2c/fig_saving}{-5}
\defres{mm/reflection/trigger/jev_reflect_trigger-e2c/n}{200}
\defres{mm/reflection/trigger/jev_reflect_trigger-e2c/n_dropped}{0}
\defres{mm/reflection/trigger/jev_reflect_trigger-e2c/s1_acc}{100.0}
\defres{mm/reflection/trigger/jev_reflect_trigger-e2c/saving}{-4.8}
\defres{mm/reflection/trigger/jev_reflect_trigger-e2c/saving_ci/hi}{-3.8}
\defres{mm/reflection/trigger/jev_reflect_trigger-e2c/saving_ci/lo}{-5.8}
\defres{mm/reflection/trigger/jev_reflect_trigger-e2c/status}{replicate}
\defres{mm/reflection/trigger/jev_reflect_trigger-e2c/success}{100.0}
\defres{mm/reflection/trigger/jev_reflect_trigger-e2c/success_ref}{100.0}
\defres{mm/reflection/trigger/jev_reflect_trigger-e2c/vcode}{3}
\defres{mm/reflection/trigger/jev_reflect_trigger-e2c/verdict}{no saving}
\defres{mm/reflection/trigger/jev_reflect_trigger/acc}{100.0}
\defres{mm/reflection/trigger/jev_reflect_trigger/accepted_acc}{100.0}
\defres{mm/reflection/trigger/jev_reflect_trigger/acted}{13.9}
\defres{mm/reflection/trigger/jev_reflect_trigger/acted_kind}{fired}
\defres{mm/reflection/trigger/jev_reflect_trigger/cost_k}{40.3}
\defres{mm/reflection/trigger/jev_reflect_trigger/cost_ref_k}{40.6}
\defres{mm/reflection/trigger/jev_reflect_trigger/delta}{+0.0}
\defres{mm/reflection/trigger/jev_reflect_trigger/delta_ci/hi}{+0.0}
\defres{mm/reflection/trigger/jev_reflect_trigger/delta_ci/lo}{+0.0}
\defres{mm/reflection/trigger/jev_reflect_trigger/fig_delta}{+0.0}
\defres{mm/reflection/trigger/jev_reflect_trigger/fig_saving}{1}
\defres{mm/reflection/trigger/jev_reflect_trigger/fresh/acc}{99.7}
\defres{mm/reflection/trigger/jev_reflect_trigger/fresh/accepted_acc}{99.7}
\defres{mm/reflection/trigger/jev_reflect_trigger/fresh/acted}{14.3}
\defres{mm/reflection/trigger/jev_reflect_trigger/fresh/acted_kind}{fired}
\defres{mm/reflection/trigger/jev_reflect_trigger/fresh/cost_k}{41.3}
\defres{mm/reflection/trigger/jev_reflect_trigger/fresh/cost_ref_k}{40.9}
\defres{mm/reflection/trigger/jev_reflect_trigger/fresh/delta}{-1.0}
\defres{mm/reflection/trigger/jev_reflect_trigger/fresh/fig_delta}{-1.0}
\defres{mm/reflection/trigger/jev_reflect_trigger/fresh/fig_saving}{-1}
\defres{mm/reflection/trigger/jev_reflect_trigger/fresh/n}{200}
\defres{mm/reflection/trigger/jev_reflect_trigger/fresh/n_dropped}{0}
\defres{mm/reflection/trigger/jev_reflect_trigger/fresh/s1_acc}{99.7}
\defres{mm/reflection/trigger/jev_reflect_trigger/fresh/saving}{-1.0}
\defres{mm/reflection/trigger/jev_reflect_trigger/fresh/success}{98.5}
\defres{mm/reflection/trigger/jev_reflect_trigger/fresh/success_ref}{99.5}
\defres{mm/reflection/trigger/jev_reflect_trigger/fresh/verdict}{no saving}
\defres{mm/reflection/trigger/jev_reflect_trigger/n}{200}
\defres{mm/reflection/trigger/jev_reflect_trigger/n_dropped}{0}
\defres{mm/reflection/trigger/jev_reflect_trigger/s1_acc}{100.0}
\defres{mm/reflection/trigger/jev_reflect_trigger/saving}{0.9}
\defres{mm/reflection/trigger/jev_reflect_trigger/saving_ci/hi}{1.7}
\defres{mm/reflection/trigger/jev_reflect_trigger/saving_ci/lo}{0.0}
\defres{mm/reflection/trigger/jev_reflect_trigger/status}{descriptive}
\defres{mm/reflection/trigger/jev_reflect_trigger/success}{100.0}
\defres{mm/reflection/trigger/jev_reflect_trigger/success_ref}{100.0}
\defres{mm/reflection/trigger/jev_reflect_trigger/vcode}{1}
\defres{mm/reflection/trigger/jev_reflect_trigger/verdict}{takes over safely}
\defres{mm/reflection/trigger/jev_reflect_trigger_s2lite/acc}{83.5}
\defres{mm/reflection/trigger/jev_reflect_trigger_s2lite/accepted_acc}{83.5}
\defres{mm/reflection/trigger/jev_reflect_trigger_s2lite/acted}{14.8}
\defres{mm/reflection/trigger/jev_reflect_trigger_s2lite/acted_kind}{fired}
\defres{mm/reflection/trigger/jev_reflect_trigger_s2lite/cost_k}{9.9}
\defres{mm/reflection/trigger/jev_reflect_trigger_s2lite/cost_ref_k}{9.7}
\defres{mm/reflection/trigger/jev_reflect_trigger_s2lite/delta}{+1.8}
\defres{mm/reflection/trigger/jev_reflect_trigger_s2lite/delta_ci/hi}{+5.0}
\defres{mm/reflection/trigger/jev_reflect_trigger_s2lite/delta_ci/lo}{-1.4}
\defres{mm/reflection/trigger/jev_reflect_trigger_s2lite/fig_delta}{+1.8}
\defres{mm/reflection/trigger/jev_reflect_trigger_s2lite/fig_saving}{-2}
\defres{mm/reflection/trigger/jev_reflect_trigger_s2lite/n}{500}
\defres{mm/reflection/trigger/jev_reflect_trigger_s2lite/n_dropped}{0}
\defres{mm/reflection/trigger/jev_reflect_trigger_s2lite/reg}{C5}
\defres{mm/reflection/trigger/jev_reflect_trigger_s2lite/s1_acc}{83.5}
\defres{mm/reflection/trigger/jev_reflect_trigger_s2lite/saving}{-1.9}
\defres{mm/reflection/trigger/jev_reflect_trigger_s2lite/saving_ci/hi}{-0.1}
\defres{mm/reflection/trigger/jev_reflect_trigger_s2lite/saving_ci/lo}{-5.1}
\defres{mm/reflection/trigger/jev_reflect_trigger_s2lite/status}{registered}
\defres{mm/reflection/trigger/jev_reflect_trigger_s2lite/success}{83.0}
\defres{mm/reflection/trigger/jev_reflect_trigger_s2lite/success_ref}{81.2}
\defres{mm/reflection/trigger/jev_reflect_trigger_s2lite/vcode}{3}
\defres{mm/reflection/trigger/jev_reflect_trigger_s2lite/verdict}{no saving}
\defres{mm/reflection/trigger/jev_reflect_trigger_s2lite_e2b-e2b/acc}{97.3}
\defres{mm/reflection/trigger/jev_reflect_trigger_s2lite_e2b-e2b/accepted_acc}{97.3}
\defres{mm/reflection/trigger/jev_reflect_trigger_s2lite_e2b-e2b/acted}{14.0}
\defres{mm/reflection/trigger/jev_reflect_trigger_s2lite_e2b-e2b/acted_kind}{fired}
\defres{mm/reflection/trigger/jev_reflect_trigger_s2lite_e2b-e2b/cost_k}{9.8}
\defres{mm/reflection/trigger/jev_reflect_trigger_s2lite_e2b-e2b/cost_ref_k}{9.8}
\defres{mm/reflection/trigger/jev_reflect_trigger_s2lite_e2b-e2b/delta}{+3.5}
\defres{mm/reflection/trigger/jev_reflect_trigger_s2lite_e2b-e2b/delta_ci/hi}{+7.5}
\defres{mm/reflection/trigger/jev_reflect_trigger_s2lite_e2b-e2b/delta_ci/lo}{-0.5}
\defres{mm/reflection/trigger/jev_reflect_trigger_s2lite_e2b-e2b/fig_delta}{+3.5}
\defres{mm/reflection/trigger/jev_reflect_trigger_s2lite_e2b-e2b/fig_saving}{0}
\defres{mm/reflection/trigger/jev_reflect_trigger_s2lite_e2b-e2b/n}{200}
\defres{mm/reflection/trigger/jev_reflect_trigger_s2lite_e2b-e2b/n_dropped}{0}
\defres{mm/reflection/trigger/jev_reflect_trigger_s2lite_e2b-e2b/s1_acc}{97.3}
\defres{mm/reflection/trigger/jev_reflect_trigger_s2lite_e2b-e2b/saving}{-0.2}
\defres{mm/reflection/trigger/jev_reflect_trigger_s2lite_e2b-e2b/saving_ci/hi}{0.6}
\defres{mm/reflection/trigger/jev_reflect_trigger_s2lite_e2b-e2b/saving_ci/lo}{-1.0}
\defres{mm/reflection/trigger/jev_reflect_trigger_s2lite_e2b-e2b/status}{replicate}
\defres{mm/reflection/trigger/jev_reflect_trigger_s2lite_e2b-e2b/success}{84.5}
\defres{mm/reflection/trigger/jev_reflect_trigger_s2lite_e2b-e2b/success_ref}{81.0}
\defres{mm/reflection/trigger/jev_reflect_trigger_s2lite_e2b-e2b/vcode}{3}
\defres{mm/reflection/trigger/jev_reflect_trigger_s2lite_e2b-e2b/verdict}{no saving}
\defres{mm/reflection/trigger/rate10_reflect_trigger/acc}{100.0}
\defres{mm/reflection/trigger/rate10_reflect_trigger/accepted_acc}{100.0}
\defres{mm/reflection/trigger/rate10_reflect_trigger/acted}{8.7}
\defres{mm/reflection/trigger/rate10_reflect_trigger/acted_kind}{fired}
\defres{mm/reflection/trigger/rate10_reflect_trigger/cost_k}{42.3}
\defres{mm/reflection/trigger/rate10_reflect_trigger/cost_ref_k}{40.9}
\defres{mm/reflection/trigger/rate10_reflect_trigger/delta}{+0.0}
\defres{mm/reflection/trigger/rate10_reflect_trigger/delta_ci/hi}{+0.0}
\defres{mm/reflection/trigger/rate10_reflect_trigger/delta_ci/lo}{+0.0}
\defres{mm/reflection/trigger/rate10_reflect_trigger/fig_delta}{+0.0}
\defres{mm/reflection/trigger/rate10_reflect_trigger/fig_saving}{-3}
\defres{mm/reflection/trigger/rate10_reflect_trigger/n}{200}
\defres{mm/reflection/trigger/rate10_reflect_trigger/n_dropped}{0}
\defres{mm/reflection/trigger/rate10_reflect_trigger/s1_acc}{100.0}
\defres{mm/reflection/trigger/rate10_reflect_trigger/saving}{-3.4}
\defres{mm/reflection/trigger/rate10_reflect_trigger/saving_ci/hi}{-2.3}
\defres{mm/reflection/trigger/rate10_reflect_trigger/saving_ci/lo}{-4.6}
\defres{mm/reflection/trigger/rate10_reflect_trigger/status}{descriptive}
\defres{mm/reflection/trigger/rate10_reflect_trigger/success}{100.0}
\defres{mm/reflection/trigger/rate10_reflect_trigger/success_ref}{100.0}
\defres{mm/reflection/trigger/rate10_reflect_trigger/vcode}{3}
\defres{mm/reflection/trigger/rate10_reflect_trigger/verdict}{no saving}
\defres{mm/reflection/trigger/rate10_reflect_trigger_s2lite/acc}{89.3}
\defres{mm/reflection/trigger/rate10_reflect_trigger_s2lite/accepted_acc}{89.3}
\defres{mm/reflection/trigger/rate10_reflect_trigger_s2lite/acted}{9.5}
\defres{mm/reflection/trigger/rate10_reflect_trigger_s2lite/acted_kind}{fired}
\defres{mm/reflection/trigger/rate10_reflect_trigger_s2lite/cost_k}{10.0}
\defres{mm/reflection/trigger/rate10_reflect_trigger_s2lite/cost_ref_k}{9.7}
\defres{mm/reflection/trigger/rate10_reflect_trigger_s2lite/delta}{+5.5}
\defres{mm/reflection/trigger/rate10_reflect_trigger_s2lite/delta_ci/hi}{+10.0}
\defres{mm/reflection/trigger/rate10_reflect_trigger_s2lite/delta_ci/lo}{+1.5}
\defres{mm/reflection/trigger/rate10_reflect_trigger_s2lite/fig_delta}{+5.5}
\defres{mm/reflection/trigger/rate10_reflect_trigger_s2lite/fig_saving}{-3}
\defres{mm/reflection/trigger/rate10_reflect_trigger_s2lite/n}{200}
\defres{mm/reflection/trigger/rate10_reflect_trigger_s2lite/n_dropped}{0}
\defres{mm/reflection/trigger/rate10_reflect_trigger_s2lite/s1_acc}{89.3}
\defres{mm/reflection/trigger/rate10_reflect_trigger_s2lite/saving}{-3.3}
\defres{mm/reflection/trigger/rate10_reflect_trigger_s2lite/saving_ci/hi}{-2.3}
\defres{mm/reflection/trigger/rate10_reflect_trigger_s2lite/saving_ci/lo}{-4.3}
\defres{mm/reflection/trigger/rate10_reflect_trigger_s2lite/status}{descriptive}
\defres{mm/reflection/trigger/rate10_reflect_trigger_s2lite/success}{87.0}
\defres{mm/reflection/trigger/rate10_reflect_trigger_s2lite/success_ref}{81.5}
\defres{mm/reflection/trigger/rate10_reflect_trigger_s2lite/vcode}{3}
\defres{mm/reflection/trigger/rate10_reflect_trigger_s2lite/verdict}{no saving}
\defres{mm/reflection/trigger/rate30_reflect_trigger/acc}{99.8}
\defres{mm/reflection/trigger/rate30_reflect_trigger/accepted_acc}{99.8}
\defres{mm/reflection/trigger/rate30_reflect_trigger/acted}{30.2}
\defres{mm/reflection/trigger/rate30_reflect_trigger/acted_kind}{fired}
\defres{mm/reflection/trigger/rate30_reflect_trigger/cost_k}{46.1}
\defres{mm/reflection/trigger/rate30_reflect_trigger/cost_ref_k}{40.9}
\defres{mm/reflection/trigger/rate30_reflect_trigger/delta}{-1.0}
\defres{mm/reflection/trigger/rate30_reflect_trigger/delta_ci/hi}{+0.0}
\defres{mm/reflection/trigger/rate30_reflect_trigger/delta_ci/lo}{-2.5}
\defres{mm/reflection/trigger/rate30_reflect_trigger/fig_delta}{-1.0}
\defres{mm/reflection/trigger/rate30_reflect_trigger/fig_saving}{-13}
\defres{mm/reflection/trigger/rate30_reflect_trigger/n}{200}
\defres{mm/reflection/trigger/rate30_reflect_trigger/n_dropped}{0}
\defres{mm/reflection/trigger/rate30_reflect_trigger/s1_acc}{99.8}
\defres{mm/reflection/trigger/rate30_reflect_trigger/saving}{-12.5}
\defres{mm/reflection/trigger/rate30_reflect_trigger/saving_ci/hi}{-10.3}
\defres{mm/reflection/trigger/rate30_reflect_trigger/saving_ci/lo}{-15.0}
\defres{mm/reflection/trigger/rate30_reflect_trigger/status}{descriptive}
\defres{mm/reflection/trigger/rate30_reflect_trigger/success}{99.0}
\defres{mm/reflection/trigger/rate30_reflect_trigger/success_ref}{100.0}
\defres{mm/reflection/trigger/rate30_reflect_trigger/vcode}{3}
\defres{mm/reflection/trigger/rate30_reflect_trigger/verdict}{no saving}
\defres{mm/reflection/trigger/rate30_reflect_trigger_s2lite/acc}{70.1}
\defres{mm/reflection/trigger/rate30_reflect_trigger_s2lite/accepted_acc}{70.1}
\defres{mm/reflection/trigger/rate30_reflect_trigger_s2lite/acted}{29.3}
\defres{mm/reflection/trigger/rate30_reflect_trigger_s2lite/acted_kind}{fired}
\defres{mm/reflection/trigger/rate30_reflect_trigger_s2lite/cost_k}{10.6}
\defres{mm/reflection/trigger/rate30_reflect_trigger_s2lite/cost_ref_k}{9.7}
\defres{mm/reflection/trigger/rate30_reflect_trigger_s2lite/delta}{+6.5}
\defres{mm/reflection/trigger/rate30_reflect_trigger_s2lite/delta_ci/hi}{+11.5}
\defres{mm/reflection/trigger/rate30_reflect_trigger_s2lite/delta_ci/lo}{+2.0}
\defres{mm/reflection/trigger/rate30_reflect_trigger_s2lite/fig_delta}{+6.5}
\defres{mm/reflection/trigger/rate30_reflect_trigger_s2lite/fig_saving}{-10}
\defres{mm/reflection/trigger/rate30_reflect_trigger_s2lite/n}{200}
\defres{mm/reflection/trigger/rate30_reflect_trigger_s2lite/n_dropped}{0}
\defres{mm/reflection/trigger/rate30_reflect_trigger_s2lite/s1_acc}{70.1}
\defres{mm/reflection/trigger/rate30_reflect_trigger_s2lite/saving}{-9.7}
\defres{mm/reflection/trigger/rate30_reflect_trigger_s2lite/saving_ci/hi}{-7.8}
\defres{mm/reflection/trigger/rate30_reflect_trigger_s2lite/saving_ci/lo}{-11.6}
\defres{mm/reflection/trigger/rate30_reflect_trigger_s2lite/status}{descriptive}
\defres{mm/reflection/trigger/rate30_reflect_trigger_s2lite/success}{88.0}
\defres{mm/reflection/trigger/rate30_reflect_trigger_s2lite/success_ref}{81.5}
\defres{mm/reflection/trigger/rate30_reflect_trigger_s2lite/vcode}{3}
\defres{mm/reflection/trigger/rate30_reflect_trigger_s2lite/verdict}{no saving}
\defres{mm/reflection/trigger/rate50_reflect_trigger/acc}{99.7}
\defres{mm/reflection/trigger/rate50_reflect_trigger/accepted_acc}{99.7}
\defres{mm/reflection/trigger/rate50_reflect_trigger/acted}{49.5}
\defres{mm/reflection/trigger/rate50_reflect_trigger/acted_kind}{fired}
\defres{mm/reflection/trigger/rate50_reflect_trigger/cost_k}{50.7}
\defres{mm/reflection/trigger/rate50_reflect_trigger/cost_ref_k}{40.9}
\defres{mm/reflection/trigger/rate50_reflect_trigger/delta}{-1.5}
\defres{mm/reflection/trigger/rate50_reflect_trigger/delta_ci/hi}{+0.0}
\defres{mm/reflection/trigger/rate50_reflect_trigger/delta_ci/lo}{-3.5}
\defres{mm/reflection/trigger/rate50_reflect_trigger/fig_delta}{-1.5}
\defres{mm/reflection/trigger/rate50_reflect_trigger/fig_saving}{-24}
\defres{mm/reflection/trigger/rate50_reflect_trigger/n}{200}
\defres{mm/reflection/trigger/rate50_reflect_trigger/n_dropped}{0}
\defres{mm/reflection/trigger/rate50_reflect_trigger/s1_acc}{99.7}
\defres{mm/reflection/trigger/rate50_reflect_trigger/saving}{-24.0}
\defres{mm/reflection/trigger/rate50_reflect_trigger/saving_ci/hi}{-20.7}
\defres{mm/reflection/trigger/rate50_reflect_trigger/saving_ci/lo}{-27.2}
\defres{mm/reflection/trigger/rate50_reflect_trigger/status}{descriptive}
\defres{mm/reflection/trigger/rate50_reflect_trigger/success}{98.5}
\defres{mm/reflection/trigger/rate50_reflect_trigger/success_ref}{100.0}
\defres{mm/reflection/trigger/rate50_reflect_trigger/vcode}{3}
\defres{mm/reflection/trigger/rate50_reflect_trigger/verdict}{no saving}
\defres{mm/reflection/trigger/rate50_reflect_trigger_s2lite/acc}{50.3}
\defres{mm/reflection/trigger/rate50_reflect_trigger_s2lite/accepted_acc}{50.3}
\defres{mm/reflection/trigger/rate50_reflect_trigger_s2lite/acted}{50.1}
\defres{mm/reflection/trigger/rate50_reflect_trigger_s2lite/acted_kind}{fired}
\defres{mm/reflection/trigger/rate50_reflect_trigger_s2lite/cost_k}{11.6}
\defres{mm/reflection/trigger/rate50_reflect_trigger_s2lite/cost_ref_k}{9.7}
\defres{mm/reflection/trigger/rate50_reflect_trigger_s2lite/delta}{+8.5}
\defres{mm/reflection/trigger/rate50_reflect_trigger_s2lite/delta_ci/hi}{+13.5}
\defres{mm/reflection/trigger/rate50_reflect_trigger_s2lite/delta_ci/lo}{+4.0}
\defres{mm/reflection/trigger/rate50_reflect_trigger_s2lite/fig_delta}{+8.5}
\defres{mm/reflection/trigger/rate50_reflect_trigger_s2lite/fig_saving}{-19}
\defres{mm/reflection/trigger/rate50_reflect_trigger_s2lite/n}{200}
\defres{mm/reflection/trigger/rate50_reflect_trigger_s2lite/n_dropped}{0}
\defres{mm/reflection/trigger/rate50_reflect_trigger_s2lite/s1_acc}{50.3}
\defres{mm/reflection/trigger/rate50_reflect_trigger_s2lite/saving}{-19.5}
\defres{mm/reflection/trigger/rate50_reflect_trigger_s2lite/saving_ci/hi}{-17.0}
\defres{mm/reflection/trigger/rate50_reflect_trigger_s2lite/saving_ci/lo}{-21.8}
\defres{mm/reflection/trigger/rate50_reflect_trigger_s2lite/status}{descriptive}
\defres{mm/reflection/trigger/rate50_reflect_trigger_s2lite/success}{90.0}
\defres{mm/reflection/trigger/rate50_reflect_trigger_s2lite/success_ref}{81.5}
\defres{mm/reflection/trigger/rate50_reflect_trigger_s2lite/vcode}{3}
\defres{mm/reflection/trigger/rate50_reflect_trigger_s2lite/verdict}{no saving}
\defres{mm/reflection/trigger/ratem_reflect_trigger_s2lite/acc}{83.6}
\defres{mm/reflection/trigger/ratem_reflect_trigger_s2lite/accepted_acc}{83.6}
\defres{mm/reflection/trigger/ratem_reflect_trigger_s2lite/acted}{14.7}
\defres{mm/reflection/trigger/ratem_reflect_trigger_s2lite/acted_kind}{fired}
\defres{mm/reflection/trigger/ratem_reflect_trigger_s2lite/cost_k}{10.3}
\defres{mm/reflection/trigger/ratem_reflect_trigger_s2lite/cost_ref_k}{9.7}
\defres{mm/reflection/trigger/ratem_reflect_trigger_s2lite/delta}{+4.2}
\defres{mm/reflection/trigger/ratem_reflect_trigger_s2lite/delta_ci/hi}{+7.4}
\defres{mm/reflection/trigger/ratem_reflect_trigger_s2lite/delta_ci/lo}{+1.0}
\defres{mm/reflection/trigger/ratem_reflect_trigger_s2lite/fig_delta}{+4.2}
\defres{mm/reflection/trigger/ratem_reflect_trigger_s2lite/fig_saving}{-6}
\defres{mm/reflection/trigger/ratem_reflect_trigger_s2lite/n}{500}
\defres{mm/reflection/trigger/ratem_reflect_trigger_s2lite/n_dropped}{0}
\defres{mm/reflection/trigger/ratem_reflect_trigger_s2lite/s1_acc}{83.6}
\defres{mm/reflection/trigger/ratem_reflect_trigger_s2lite/saving}{-5.9}
\defres{mm/reflection/trigger/ratem_reflect_trigger_s2lite/saving_ci/hi}{-5.0}
\defres{mm/reflection/trigger/ratem_reflect_trigger_s2lite/saving_ci/lo}{-6.8}
\defres{mm/reflection/trigger/ratem_reflect_trigger_s2lite/status}{descriptive}
\defres{mm/reflection/trigger/ratem_reflect_trigger_s2lite/success}{85.4}
\defres{mm/reflection/trigger/ratem_reflect_trigger_s2lite/success_ref}{81.2}
\defres{mm/reflection/trigger/ratem_reflect_trigger_s2lite/vcode}{3}
\defres{mm/reflection/trigger/ratem_reflect_trigger_s2lite/verdict}{no saving}
\defres{mm/reflection/trigger/s2self_reflect_trigger/acc}{100.0}
\defres{mm/reflection/trigger/s2self_reflect_trigger/accepted_acc}{100.0}
\defres{mm/reflection/trigger/s2self_reflect_trigger/acted}{2.4}
\defres{mm/reflection/trigger/s2self_reflect_trigger/acted_kind}{fired}
\defres{mm/reflection/trigger/s2self_reflect_trigger/cost_k}{52.8}
\defres{mm/reflection/trigger/s2self_reflect_trigger/cost_ref_k}{40.9}
\defres{mm/reflection/trigger/s2self_reflect_trigger/delta}{+0.0}
\defres{mm/reflection/trigger/s2self_reflect_trigger/delta_ci/hi}{+0.0}
\defres{mm/reflection/trigger/s2self_reflect_trigger/delta_ci/lo}{+0.0}
\defres{mm/reflection/trigger/s2self_reflect_trigger/fig_delta}{+0.0}
\defres{mm/reflection/trigger/s2self_reflect_trigger/fig_saving}{-29}
\defres{mm/reflection/trigger/s2self_reflect_trigger/n}{200}
\defres{mm/reflection/trigger/s2self_reflect_trigger/n_dropped}{0}
\defres{mm/reflection/trigger/s2self_reflect_trigger/s1_acc}{100.0}
\defres{mm/reflection/trigger/s2self_reflect_trigger/saving}{-29.0}
\defres{mm/reflection/trigger/s2self_reflect_trigger/saving_ci/hi}{-27.6}
\defres{mm/reflection/trigger/s2self_reflect_trigger/saving_ci/lo}{-30.4}
\defres{mm/reflection/trigger/s2self_reflect_trigger/status}{descriptive}
\defres{mm/reflection/trigger/s2self_reflect_trigger/success}{100.0}
\defres{mm/reflection/trigger/s2self_reflect_trigger/success_ref}{100.0}
\defres{mm/reflection/trigger/s2self_reflect_trigger/vcode}{3}
\defres{mm/reflection/trigger/s2self_reflect_trigger/verdict}{no saving}
\defres{mm/reflection/trigger/s2self_reflect_trigger_s2lite/acc}{97.4}
\defres{mm/reflection/trigger/s2self_reflect_trigger_s2lite/accepted_acc}{97.4}
\defres{mm/reflection/trigger/s2self_reflect_trigger_s2lite/acted}{0.2}
\defres{mm/reflection/trigger/s2self_reflect_trigger_s2lite/acted_kind}{fired}
\defres{mm/reflection/trigger/s2self_reflect_trigger_s2lite/cost_k}{12.2}
\defres{mm/reflection/trigger/s2self_reflect_trigger_s2lite/cost_ref_k}{9.7}
\defres{mm/reflection/trigger/s2self_reflect_trigger_s2lite/delta}{+2.5}
\defres{mm/reflection/trigger/s2self_reflect_trigger_s2lite/delta_ci/hi}{+6.0}
\defres{mm/reflection/trigger/s2self_reflect_trigger_s2lite/delta_ci/lo}{-0.5}
\defres{mm/reflection/trigger/s2self_reflect_trigger_s2lite/fig_delta}{+2.5}
\defres{mm/reflection/trigger/s2self_reflect_trigger_s2lite/fig_saving}{-26}
\defres{mm/reflection/trigger/s2self_reflect_trigger_s2lite/n}{200}
\defres{mm/reflection/trigger/s2self_reflect_trigger_s2lite/n_dropped}{0}
\defres{mm/reflection/trigger/s2self_reflect_trigger_s2lite/s1_acc}{97.4}
\defres{mm/reflection/trigger/s2self_reflect_trigger_s2lite/saving}{-25.8}
\defres{mm/reflection/trigger/s2self_reflect_trigger_s2lite/saving_ci/hi}{-24.6}
\defres{mm/reflection/trigger/s2self_reflect_trigger_s2lite/saving_ci/lo}{-27.0}
\defres{mm/reflection/trigger/s2self_reflect_trigger_s2lite/status}{descriptive}
\defres{mm/reflection/trigger/s2self_reflect_trigger_s2lite/success}{84.0}
\defres{mm/reflection/trigger/s2self_reflect_trigger_s2lite/success_ref}{81.5}
\defres{mm/reflection/trigger/s2self_reflect_trigger_s2lite/vcode}{3}
\defres{mm/reflection/trigger/s2self_reflect_trigger_s2lite/verdict}{no saving}
\defres{mm/routing/trigger/heuristic_route/acc}{97.8}
\defres{mm/routing/trigger/heuristic_route/accepted_acc}{97.8}
\defres{mm/routing/trigger/heuristic_route/acted}{0.3}
\defres{mm/routing/trigger/heuristic_route/acted_kind}{fired}
\defres{mm/routing/trigger/heuristic_route/cost_k}{9.8}
\defres{mm/routing/trigger/heuristic_route/cost_ref_k}{9.7}
\defres{mm/routing/trigger/heuristic_route/delta}{+2.0}
\defres{mm/routing/trigger/heuristic_route/delta_ci/hi}{+5.0}
\defres{mm/routing/trigger/heuristic_route/delta_ci/lo}{-1.0}
\defres{mm/routing/trigger/heuristic_route/fig_delta}{+2.0}
\defres{mm/routing/trigger/heuristic_route/fig_saving}{-1}
\defres{mm/routing/trigger/heuristic_route/flash/delta}{-16.5}
\defres{mm/routing/trigger/heuristic_route/flash/delta_ci/hi}{-11.5}
\defres{mm/routing/trigger/heuristic_route/flash/delta_ci/lo}{-21.5}
\defres{mm/routing/trigger/heuristic_route/flash/fig_delta}{-16.5}
\defres{mm/routing/trigger/heuristic_route/flash/fig_saving}{76}
\defres{mm/routing/trigger/heuristic_route/flash/n}{200}
\defres{mm/routing/trigger/heuristic_route/flash/saving}{76.0}
\defres{mm/routing/trigger/heuristic_route/flash/saving_ci/hi}{76.4}
\defres{mm/routing/trigger/heuristic_route/flash/saving_ci/lo}{75.6}
\defres{mm/routing/trigger/heuristic_route/n}{200}
\defres{mm/routing/trigger/heuristic_route/n_dropped}{0}
\defres{mm/routing/trigger/heuristic_route/s1_acc}{97.8}
\defres{mm/routing/trigger/heuristic_route/saving}{-1.3}
\defres{mm/routing/trigger/heuristic_route/saving_ci/hi}{-0.3}
\defres{mm/routing/trigger/heuristic_route/saving_ci/lo}{-2.4}
\defres{mm/routing/trigger/heuristic_route/status}{descriptive}
\defres{mm/routing/trigger/heuristic_route/success}{83.5}
\defres{mm/routing/trigger/heuristic_route/success_ref}{81.5}
\defres{mm/routing/trigger/heuristic_route/vcode}{3}
\defres{mm/routing/trigger/heuristic_route/verdict}{no saving}
\defres{mm/routing/trigger/jev_route_tau0.2-e2c/acc}{98.7}
\defres{mm/routing/trigger/jev_route_tau0.2-e2c/accepted_acc}{98.7}
\defres{mm/routing/trigger/jev_route_tau0.2-e2c/acted}{59.4}
\defres{mm/routing/trigger/jev_route_tau0.2-e2c/acted_kind}{fired}
\defres{mm/routing/trigger/jev_route_tau0.2-e2c/cost_k}{30.9}
\defres{mm/routing/trigger/jev_route_tau0.2-e2c/cost_ref_k}{9.7}
\defres{mm/routing/trigger/jev_route_tau0.2-e2c/delta}{+14.5}
\defres{mm/routing/trigger/jev_route_tau0.2-e2c/delta_ci/hi}{+19.5}
\defres{mm/routing/trigger/jev_route_tau0.2-e2c/delta_ci/lo}{+10.0}
\defres{mm/routing/trigger/jev_route_tau0.2-e2c/fig_delta}{+14.5}
\defres{mm/routing/trigger/jev_route_tau0.2-e2c/fig_saving}{-218}
\defres{mm/routing/trigger/jev_route_tau0.2-e2c/flash/delta}{-4.0}
\defres{mm/routing/trigger/jev_route_tau0.2-e2c/flash/delta_ci/hi}{-1.5}
\defres{mm/routing/trigger/jev_route_tau0.2-e2c/flash/delta_ci/lo}{-7.0}
\defres{mm/routing/trigger/jev_route_tau0.2-e2c/flash/fig_delta}{-4.0}
\defres{mm/routing/trigger/jev_route_tau0.2-e2c/flash/fig_saving}{25}
\defres{mm/routing/trigger/jev_route_tau0.2-e2c/flash/n}{200}
\defres{mm/routing/trigger/jev_route_tau0.2-e2c/flash/saving}{24.6}
\defres{mm/routing/trigger/jev_route_tau0.2-e2c/flash/saving_ci/hi}{27.3}
\defres{mm/routing/trigger/jev_route_tau0.2-e2c/flash/saving_ci/lo}{21.9}
\defres{mm/routing/trigger/jev_route_tau0.2-e2c/n}{200}
\defres{mm/routing/trigger/jev_route_tau0.2-e2c/n_dropped}{0}
\defres{mm/routing/trigger/jev_route_tau0.2-e2c/s1_acc}{98.7}
\defres{mm/routing/trigger/jev_route_tau0.2-e2c/saving}{-217.8}
\defres{mm/routing/trigger/jev_route_tau0.2-e2c/saving_ci/hi}{-204.2}
\defres{mm/routing/trigger/jev_route_tau0.2-e2c/saving_ci/lo}{-231.7}
\defres{mm/routing/trigger/jev_route_tau0.2-e2c/status}{replicate}
\defres{mm/routing/trigger/jev_route_tau0.2-e2c/success}{96.0}
\defres{mm/routing/trigger/jev_route_tau0.2-e2c/success_ref}{81.5}
\defres{mm/routing/trigger/jev_route_tau0.2-e2c/vcode}{3}
\defres{mm/routing/trigger/jev_route_tau0.2-e2c/verdict}{no saving}
\defres{mm/routing/trigger/jev_route_tau0.2/acc}{99.0}
\defres{mm/routing/trigger/jev_route_tau0.2/accepted_acc}{99.0}
\defres{mm/routing/trigger/jev_route_tau0.2/acted}{59.6}
\defres{mm/routing/trigger/jev_route_tau0.2/acted_kind}{fired}
\defres{mm/routing/trigger/jev_route_tau0.2/cost_k}{29.1}
\defres{mm/routing/trigger/jev_route_tau0.2/cost_ref_k}{9.8}
\defres{mm/routing/trigger/jev_route_tau0.2/delta}{+15.0}
\defres{mm/routing/trigger/jev_route_tau0.2/delta_ci/hi}{+20.0}
\defres{mm/routing/trigger/jev_route_tau0.2/delta_ci/lo}{+10.5}
\defres{mm/routing/trigger/jev_route_tau0.2/fig_delta}{+15.0}
\defres{mm/routing/trigger/jev_route_tau0.2/fig_saving}{-198}
\defres{mm/routing/trigger/jev_route_tau0.2/flash/delta}{-3.0}
\defres{mm/routing/trigger/jev_route_tau0.2/flash/delta_ci/hi}{-1.0}
\defres{mm/routing/trigger/jev_route_tau0.2/flash/delta_ci/lo}{-5.5}
\defres{mm/routing/trigger/jev_route_tau0.2/flash/fig_delta}{-3.0}
\defres{mm/routing/trigger/jev_route_tau0.2/flash/fig_saving}{28}
\defres{mm/routing/trigger/jev_route_tau0.2/flash/n}{200}
\defres{mm/routing/trigger/jev_route_tau0.2/flash/saving}{28.4}
\defres{mm/routing/trigger/jev_route_tau0.2/flash/saving_ci/hi}{31.3}
\defres{mm/routing/trigger/jev_route_tau0.2/flash/saving_ci/lo}{25.6}
\defres{mm/routing/trigger/jev_route_tau0.2/n}{200}
\defres{mm/routing/trigger/jev_route_tau0.2/n_dropped}{0}
\defres{mm/routing/trigger/jev_route_tau0.2/s1_acc}{99.0}
\defres{mm/routing/trigger/jev_route_tau0.2/saving}{-198.0}
\defres{mm/routing/trigger/jev_route_tau0.2/saving_ci/hi}{-183.1}
\defres{mm/routing/trigger/jev_route_tau0.2/saving_ci/lo}{-212.6}
\defres{mm/routing/trigger/jev_route_tau0.2/status}{descriptive}
\defres{mm/routing/trigger/jev_route_tau0.2/success}{97.0}
\defres{mm/routing/trigger/jev_route_tau0.2/success_ref}{82.0}
\defres{mm/routing/trigger/jev_route_tau0.2/vcode}{3}
\defres{mm/routing/trigger/jev_route_tau0.2/verdict}{no saving}
\defres{mm/routing/trigger/jev_route_tau0.4-e2c/acc}{97.5}
\defres{mm/routing/trigger/jev_route_tau0.4-e2c/accepted_acc}{97.5}
\defres{mm/routing/trigger/jev_route_tau0.4-e2c/acted}{9.7}
\defres{mm/routing/trigger/jev_route_tau0.4-e2c/acted_kind}{fired}
\defres{mm/routing/trigger/jev_route_tau0.4-e2c/cost_k}{12.9}
\defres{mm/routing/trigger/jev_route_tau0.4-e2c/cost_ref_k}{9.7}
\defres{mm/routing/trigger/jev_route_tau0.4-e2c/delta}{+1.5}
\defres{mm/routing/trigger/jev_route_tau0.4-e2c/delta_ci/hi}{+4.5}
\defres{mm/routing/trigger/jev_route_tau0.4-e2c/delta_ci/lo}{-1.5}
\defres{mm/routing/trigger/jev_route_tau0.4-e2c/fig_delta}{+1.5}
\defres{mm/routing/trigger/jev_route_tau0.4-e2c/fig_saving}{-33}
\defres{mm/routing/trigger/jev_route_tau0.4-e2c/flash/delta}{-17.0}
\defres{mm/routing/trigger/jev_route_tau0.4-e2c/flash/delta_ci/hi}{-12.0}
\defres{mm/routing/trigger/jev_route_tau0.4-e2c/flash/delta_ci/lo}{-22.0}
\defres{mm/routing/trigger/jev_route_tau0.4-e2c/flash/fig_delta}{-17.0}
\defres{mm/routing/trigger/jev_route_tau0.4-e2c/flash/fig_saving}{68}
\defres{mm/routing/trigger/jev_route_tau0.4-e2c/flash/n}{200}
\defres{mm/routing/trigger/jev_route_tau0.4-e2c/flash/saving}{68.4}
\defres{mm/routing/trigger/jev_route_tau0.4-e2c/flash/saving_ci/hi}{69.4}
\defres{mm/routing/trigger/jev_route_tau0.4-e2c/flash/saving_ci/lo}{67.3}
\defres{mm/routing/trigger/jev_route_tau0.4-e2c/n}{200}
\defres{mm/routing/trigger/jev_route_tau0.4-e2c/n_dropped}{0}
\defres{mm/routing/trigger/jev_route_tau0.4-e2c/s1_acc}{97.5}
\defres{mm/routing/trigger/jev_route_tau0.4-e2c/saving}{-33.3}
\defres{mm/routing/trigger/jev_route_tau0.4-e2c/saving_ci/hi}{-29.4}
\defres{mm/routing/trigger/jev_route_tau0.4-e2c/saving_ci/lo}{-37.4}
\defres{mm/routing/trigger/jev_route_tau0.4-e2c/status}{replicate}
\defres{mm/routing/trigger/jev_route_tau0.4-e2c/success}{83.0}
\defres{mm/routing/trigger/jev_route_tau0.4-e2c/success_ref}{81.5}
\defres{mm/routing/trigger/jev_route_tau0.4-e2c/vcode}{3}
\defres{mm/routing/trigger/jev_route_tau0.4-e2c/verdict}{no saving}
\defres{mm/routing/trigger/jev_route_tau0.4/acc}{97.3}
\defres{mm/routing/trigger/jev_route_tau0.4/accepted_acc}{97.3}
\defres{mm/routing/trigger/jev_route_tau0.4/acted}{10.1}
\defres{mm/routing/trigger/jev_route_tau0.4/acted_kind}{fired}
\defres{mm/routing/trigger/jev_route_tau0.4/cost_k}{13.4}
\defres{mm/routing/trigger/jev_route_tau0.4/cost_ref_k}{9.8}
\defres{mm/routing/trigger/jev_route_tau0.4/delta}{+0.6}
\defres{mm/routing/trigger/jev_route_tau0.4/delta_ci/hi}{+2.8}
\defres{mm/routing/trigger/jev_route_tau0.4/delta_ci/lo}{-1.6}
\defres{mm/routing/trigger/jev_route_tau0.4/fig_delta}{+0.6}
\defres{mm/routing/trigger/jev_route_tau0.4/fig_saving}{-36}
\defres{mm/routing/trigger/jev_route_tau0.4/flash/delta}{-18.4}
\defres{mm/routing/trigger/jev_route_tau0.4/flash/delta_ci/hi}{-15.0}
\defres{mm/routing/trigger/jev_route_tau0.4/flash/delta_ci/lo}{-22.0}
\defres{mm/routing/trigger/jev_route_tau0.4/flash/fig_delta}{-18.4}
\defres{mm/routing/trigger/jev_route_tau0.4/flash/fig_saving}{67}
\defres{mm/routing/trigger/jev_route_tau0.4/flash/n}{500}
\defres{mm/routing/trigger/jev_route_tau0.4/flash/saving}{67.3}
\defres{mm/routing/trigger/jev_route_tau0.4/flash/saving_ci/hi}{68.0}
\defres{mm/routing/trigger/jev_route_tau0.4/flash/saving_ci/lo}{66.5}
\defres{mm/routing/trigger/jev_route_tau0.4/n}{500}
\defres{mm/routing/trigger/jev_route_tau0.4/n_dropped}{0}
\defres{mm/routing/trigger/jev_route_tau0.4/reg}{C4}
\defres{mm/routing/trigger/jev_route_tau0.4/s1_acc}{97.3}
\defres{mm/routing/trigger/jev_route_tau0.4/saving}{-36.2}
\defres{mm/routing/trigger/jev_route_tau0.4/saving_ci/hi}{-33.3}
\defres{mm/routing/trigger/jev_route_tau0.4/saving_ci/lo}{-39.3}
\defres{mm/routing/trigger/jev_route_tau0.4/status}{registered}
\defres{mm/routing/trigger/jev_route_tau0.4/success}{81.4}
\defres{mm/routing/trigger/jev_route_tau0.4/success_ref}{80.8}
\defres{mm/routing/trigger/jev_route_tau0.4/vcode}{3}
\defres{mm/routing/trigger/jev_route_tau0.4/verdict}{no saving}
\defres{mm/routing/trigger/jev_route_tau0.5/acc}{97.8}
\defres{mm/routing/trigger/jev_route_tau0.5/accepted_acc}{97.8}
\defres{mm/routing/trigger/jev_route_tau0.5/acted}{5.0}
\defres{mm/routing/trigger/jev_route_tau0.5/acted_kind}{fired}
\defres{mm/routing/trigger/jev_route_tau0.5/cost_k}{11.5}
\defres{mm/routing/trigger/jev_route_tau0.5/cost_ref_k}{9.7}
\defres{mm/routing/trigger/jev_route_tau0.5/delta}{+3.0}
\defres{mm/routing/trigger/jev_route_tau0.5/delta_ci/hi}{+6.5}
\defres{mm/routing/trigger/jev_route_tau0.5/delta_ci/lo}{-0.5}
\defres{mm/routing/trigger/jev_route_tau0.5/fig_delta}{+3.0}
\defres{mm/routing/trigger/jev_route_tau0.5/fig_saving}{-19}
\defres{mm/routing/trigger/jev_route_tau0.5/flash/delta}{-15.5}
\defres{mm/routing/trigger/jev_route_tau0.5/flash/delta_ci/hi}{-10.5}
\defres{mm/routing/trigger/jev_route_tau0.5/flash/delta_ci/lo}{-20.5}
\defres{mm/routing/trigger/jev_route_tau0.5/flash/fig_delta}{-15.5}
\defres{mm/routing/trigger/jev_route_tau0.5/flash/fig_saving}{72}
\defres{mm/routing/trigger/jev_route_tau0.5/flash/n}{200}
\defres{mm/routing/trigger/jev_route_tau0.5/flash/saving}{71.8}
\defres{mm/routing/trigger/jev_route_tau0.5/flash/saving_ci/hi}{72.3}
\defres{mm/routing/trigger/jev_route_tau0.5/flash/saving_ci/lo}{71.4}
\defres{mm/routing/trigger/jev_route_tau0.5/n}{200}
\defres{mm/routing/trigger/jev_route_tau0.5/n_dropped}{0}
\defres{mm/routing/trigger/jev_route_tau0.5/s1_acc}{97.8}
\defres{mm/routing/trigger/jev_route_tau0.5/saving}{-18.8}
\defres{mm/routing/trigger/jev_route_tau0.5/saving_ci/hi}{-16.3}
\defres{mm/routing/trigger/jev_route_tau0.5/saving_ci/lo}{-21.3}
\defres{mm/routing/trigger/jev_route_tau0.5/status}{descriptive}
\defres{mm/routing/trigger/jev_route_tau0.5/success}{84.5}
\defres{mm/routing/trigger/jev_route_tau0.5/success_ref}{81.5}
\defres{mm/routing/trigger/jev_route_tau0.5/vcode}{3}
\defres{mm/routing/trigger/jev_route_tau0.5/verdict}{no saving}
\defres{mm/routing/trigger/jev_route_tau0.6-e2c/acc}{97.6}
\defres{mm/routing/trigger/jev_route_tau0.6-e2c/accepted_acc}{97.6}
\defres{mm/routing/trigger/jev_route_tau0.6-e2c/acted}{0.1}
\defres{mm/routing/trigger/jev_route_tau0.6-e2c/acted_kind}{fired}
\defres{mm/routing/trigger/jev_route_tau0.6-e2c/cost_k}{10.1}
\defres{mm/routing/trigger/jev_route_tau0.6-e2c/cost_ref_k}{9.7}
\defres{mm/routing/trigger/jev_route_tau0.6-e2c/delta}{+0.5}
\defres{mm/routing/trigger/jev_route_tau0.6-e2c/delta_ci/hi}{+3.5}
\defres{mm/routing/trigger/jev_route_tau0.6-e2c/delta_ci/lo}{-2.5}
\defres{mm/routing/trigger/jev_route_tau0.6-e2c/fig_delta}{+0.5}
\defres{mm/routing/trigger/jev_route_tau0.6-e2c/fig_saving}{-4}
\defres{mm/routing/trigger/jev_route_tau0.6-e2c/flash/delta}{-18.0}
\defres{mm/routing/trigger/jev_route_tau0.6-e2c/flash/delta_ci/hi}{-13.0}
\defres{mm/routing/trigger/jev_route_tau0.6-e2c/flash/delta_ci/lo}{-23.5}
\defres{mm/routing/trigger/jev_route_tau0.6-e2c/flash/fig_delta}{-18.0}
\defres{mm/routing/trigger/jev_route_tau0.6-e2c/flash/fig_saving}{75}
\defres{mm/routing/trigger/jev_route_tau0.6-e2c/flash/n}{200}
\defres{mm/routing/trigger/jev_route_tau0.6-e2c/flash/saving}{75.4}
\defres{mm/routing/trigger/jev_route_tau0.6-e2c/flash/saving_ci/hi}{75.7}
\defres{mm/routing/trigger/jev_route_tau0.6-e2c/flash/saving_ci/lo}{75.0}
\defres{mm/routing/trigger/jev_route_tau0.6-e2c/n}{200}
\defres{mm/routing/trigger/jev_route_tau0.6-e2c/n_dropped}{0}
\defres{mm/routing/trigger/jev_route_tau0.6-e2c/s1_acc}{97.6}
\defres{mm/routing/trigger/jev_route_tau0.6-e2c/saving}{-3.9}
\defres{mm/routing/trigger/jev_route_tau0.6-e2c/saving_ci/hi}{-3.1}
\defres{mm/routing/trigger/jev_route_tau0.6-e2c/saving_ci/lo}{-4.9}
\defres{mm/routing/trigger/jev_route_tau0.6-e2c/status}{replicate}
\defres{mm/routing/trigger/jev_route_tau0.6-e2c/success}{82.0}
\defres{mm/routing/trigger/jev_route_tau0.6-e2c/success_ref}{81.5}
\defres{mm/routing/trigger/jev_route_tau0.6-e2c/vcode}{3}
\defres{mm/routing/trigger/jev_route_tau0.6-e2c/verdict}{no saving}
\defres{mm/routing/trigger/jev_route_tau0.6/acc}{97.7}
\defres{mm/routing/trigger/jev_route_tau0.6/accepted_acc}{97.7}
\defres{mm/routing/trigger/jev_route_tau0.6/acted}{0.0}
\defres{mm/routing/trigger/jev_route_tau0.6/acted_kind}{fired}
\defres{mm/routing/trigger/jev_route_tau0.6/cost_k}{10.1}
\defres{mm/routing/trigger/jev_route_tau0.6/cost_ref_k}{9.8}
\defres{mm/routing/trigger/jev_route_tau0.6/delta}{+1.0}
\defres{mm/routing/trigger/jev_route_tau0.6/delta_ci/hi}{+4.0}
\defres{mm/routing/trigger/jev_route_tau0.6/delta_ci/lo}{-2.0}
\defres{mm/routing/trigger/jev_route_tau0.6/fig_delta}{+1.0}
\defres{mm/routing/trigger/jev_route_tau0.6/fig_saving}{-3}
\defres{mm/routing/trigger/jev_route_tau0.6/flash/delta}{-17.0}
\defres{mm/routing/trigger/jev_route_tau0.6/flash/delta_ci/hi}{-12.0}
\defres{mm/routing/trigger/jev_route_tau0.6/flash/delta_ci/lo}{-22.0}
\defres{mm/routing/trigger/jev_route_tau0.6/flash/fig_delta}{-17.0}
\defres{mm/routing/trigger/jev_route_tau0.6/flash/fig_saving}{75}
\defres{mm/routing/trigger/jev_route_tau0.6/flash/n}{200}
\defres{mm/routing/trigger/jev_route_tau0.6/flash/saving}{75.2}
\defres{mm/routing/trigger/jev_route_tau0.6/flash/saving_ci/hi}{75.5}
\defres{mm/routing/trigger/jev_route_tau0.6/flash/saving_ci/lo}{74.8}
\defres{mm/routing/trigger/jev_route_tau0.6/n}{200}
\defres{mm/routing/trigger/jev_route_tau0.6/n_dropped}{0}
\defres{mm/routing/trigger/jev_route_tau0.6/s1_acc}{97.7}
\defres{mm/routing/trigger/jev_route_tau0.6/saving}{-3.3}
\defres{mm/routing/trigger/jev_route_tau0.6/saving_ci/hi}{-2.8}
\defres{mm/routing/trigger/jev_route_tau0.6/saving_ci/lo}{-3.9}
\defres{mm/routing/trigger/jev_route_tau0.6/status}{descriptive}
\defres{mm/routing/trigger/jev_route_tau0.6/success}{83.0}
\defres{mm/routing/trigger/jev_route_tau0.6/success_ref}{82.0}
\defres{mm/routing/trigger/jev_route_tau0.6/vcode}{3}
\defres{mm/routing/trigger/jev_route_tau0.6/verdict}{no saving}
\defres{mm/routing/trigger/jev_route_tau0.8-e2c/acc}{97.9}
\defres{mm/routing/trigger/jev_route_tau0.8-e2c/accepted_acc}{97.9}
\defres{mm/routing/trigger/jev_route_tau0.8-e2c/acted}{0.0}
\defres{mm/routing/trigger/jev_route_tau0.8-e2c/acted_kind}{fired}
\defres{mm/routing/trigger/jev_route_tau0.8-e2c/cost_k}{10.1}
\defres{mm/routing/trigger/jev_route_tau0.8-e2c/cost_ref_k}{9.7}
\defres{mm/routing/trigger/jev_route_tau0.8-e2c/delta}{+2.5}
\defres{mm/routing/trigger/jev_route_tau0.8-e2c/delta_ci/hi}{+6.0}
\defres{mm/routing/trigger/jev_route_tau0.8-e2c/delta_ci/lo}{-1.0}
\defres{mm/routing/trigger/jev_route_tau0.8-e2c/fig_delta}{+2.5}
\defres{mm/routing/trigger/jev_route_tau0.8-e2c/fig_saving}{-4}
\defres{mm/routing/trigger/jev_route_tau0.8-e2c/flash/delta}{-16.0}
\defres{mm/routing/trigger/jev_route_tau0.8-e2c/flash/delta_ci/hi}{-11.0}
\defres{mm/routing/trigger/jev_route_tau0.8-e2c/flash/delta_ci/lo}{-21.0}
\defres{mm/routing/trigger/jev_route_tau0.8-e2c/flash/fig_delta}{-16.0}
\defres{mm/routing/trigger/jev_route_tau0.8-e2c/flash/fig_saving}{75}
\defres{mm/routing/trigger/jev_route_tau0.8-e2c/flash/n}{200}
\defres{mm/routing/trigger/jev_route_tau0.8-e2c/flash/saving}{75.4}
\defres{mm/routing/trigger/jev_route_tau0.8-e2c/flash/saving_ci/hi}{75.7}
\defres{mm/routing/trigger/jev_route_tau0.8-e2c/flash/saving_ci/lo}{75.1}
\defres{mm/routing/trigger/jev_route_tau0.8-e2c/n}{200}
\defres{mm/routing/trigger/jev_route_tau0.8-e2c/n_dropped}{0}
\defres{mm/routing/trigger/jev_route_tau0.8-e2c/s1_acc}{97.9}
\defres{mm/routing/trigger/jev_route_tau0.8-e2c/saving}{-3.7}
\defres{mm/routing/trigger/jev_route_tau0.8-e2c/saving_ci/hi}{-3.2}
\defres{mm/routing/trigger/jev_route_tau0.8-e2c/saving_ci/lo}{-4.1}
\defres{mm/routing/trigger/jev_route_tau0.8-e2c/status}{replicate}
\defres{mm/routing/trigger/jev_route_tau0.8-e2c/success}{84.0}
\defres{mm/routing/trigger/jev_route_tau0.8-e2c/success_ref}{81.5}
\defres{mm/routing/trigger/jev_route_tau0.8-e2c/vcode}{3}
\defres{mm/routing/trigger/jev_route_tau0.8-e2c/verdict}{no saving}
\defres{mm/routing/trigger/jev_route_tau0.8/acc}{97.9}
\defres{mm/routing/trigger/jev_route_tau0.8/accepted_acc}{97.9}
\defres{mm/routing/trigger/jev_route_tau0.8/acted}{0.0}
\defres{mm/routing/trigger/jev_route_tau0.8/acted_kind}{fired}
\defres{mm/routing/trigger/jev_route_tau0.8/cost_k}{10.1}
\defres{mm/routing/trigger/jev_route_tau0.8/cost_ref_k}{9.8}
\defres{mm/routing/trigger/jev_route_tau0.8/delta}{+2.0}
\defres{mm/routing/trigger/jev_route_tau0.8/delta_ci/hi}{+5.5}
\defres{mm/routing/trigger/jev_route_tau0.8/delta_ci/lo}{-1.5}
\defres{mm/routing/trigger/jev_route_tau0.8/fig_delta}{+2.0}
\defres{mm/routing/trigger/jev_route_tau0.8/fig_saving}{-3}
\defres{mm/routing/trigger/jev_route_tau0.8/flash/delta}{-16.0}
\defres{mm/routing/trigger/jev_route_tau0.8/flash/delta_ci/hi}{-11.0}
\defres{mm/routing/trigger/jev_route_tau0.8/flash/delta_ci/lo}{-21.0}
\defres{mm/routing/trigger/jev_route_tau0.8/flash/fig_delta}{-16.0}
\defres{mm/routing/trigger/jev_route_tau0.8/flash/fig_saving}{75}
\defres{mm/routing/trigger/jev_route_tau0.8/flash/n}{200}
\defres{mm/routing/trigger/jev_route_tau0.8/flash/saving}{75.2}
\defres{mm/routing/trigger/jev_route_tau0.8/flash/saving_ci/hi}{75.5}
\defres{mm/routing/trigger/jev_route_tau0.8/flash/saving_ci/lo}{74.8}
\defres{mm/routing/trigger/jev_route_tau0.8/n}{200}
\defres{mm/routing/trigger/jev_route_tau0.8/n_dropped}{0}
\defres{mm/routing/trigger/jev_route_tau0.8/s1_acc}{97.9}
\defres{mm/routing/trigger/jev_route_tau0.8/saving}{-3.4}
\defres{mm/routing/trigger/jev_route_tau0.8/saving_ci/hi}{-2.8}
\defres{mm/routing/trigger/jev_route_tau0.8/saving_ci/lo}{-4.0}
\defres{mm/routing/trigger/jev_route_tau0.8/status}{descriptive}
\defres{mm/routing/trigger/jev_route_tau0.8/success}{84.0}
\defres{mm/routing/trigger/jev_route_tau0.8/success_ref}{82.0}
\defres{mm/routing/trigger/jev_route_tau0.8/vcode}{3}
\defres{mm/routing/trigger/jev_route_tau0.8/verdict}{no saving}
\defres{mm/routing/trigger/lite_route-e2c/acc}{97.8}
\defres{mm/routing/trigger/lite_route-e2c/accepted_acc}{97.8}
\defres{mm/routing/trigger/lite_route-e2c/acted}{5.8}
\defres{mm/routing/trigger/lite_route-e2c/acted_kind}{fired}
\defres{mm/routing/trigger/lite_route-e2c/cost_k}{14.2}
\defres{mm/routing/trigger/lite_route-e2c/cost_ref_k}{9.7}
\defres{mm/routing/trigger/lite_route-e2c/delta}{+2.5}
\defres{mm/routing/trigger/lite_route-e2c/delta_ci/hi}{+6.0}
\defres{mm/routing/trigger/lite_route-e2c/delta_ci/lo}{-1.0}
\defres{mm/routing/trigger/lite_route-e2c/fig_delta}{+2.5}
\defres{mm/routing/trigger/lite_route-e2c/fig_saving}{-47}
\defres{mm/routing/trigger/lite_route-e2c/flash/delta}{-16.0}
\defres{mm/routing/trigger/lite_route-e2c/flash/delta_ci/hi}{-11.0}
\defres{mm/routing/trigger/lite_route-e2c/flash/delta_ci/lo}{-21.0}
\defres{mm/routing/trigger/lite_route-e2c/flash/fig_delta}{-16.0}
\defres{mm/routing/trigger/lite_route-e2c/flash/fig_saving}{65}
\defres{mm/routing/trigger/lite_route-e2c/flash/n}{200}
\defres{mm/routing/trigger/lite_route-e2c/flash/saving}{65.2}
\defres{mm/routing/trigger/lite_route-e2c/flash/saving_ci/hi}{66.1}
\defres{mm/routing/trigger/lite_route-e2c/flash/saving_ci/lo}{64.2}
\defres{mm/routing/trigger/lite_route-e2c/n}{200}
\defres{mm/routing/trigger/lite_route-e2c/n_dropped}{0}
\defres{mm/routing/trigger/lite_route-e2c/s1_acc}{97.8}
\defres{mm/routing/trigger/lite_route-e2c/saving}{-46.7}
\defres{mm/routing/trigger/lite_route-e2c/saving_ci/hi}{-43.0}
\defres{mm/routing/trigger/lite_route-e2c/saving_ci/lo}{-50.5}
\defres{mm/routing/trigger/lite_route-e2c/status}{replicate}
\defres{mm/routing/trigger/lite_route-e2c/success}{84.0}
\defres{mm/routing/trigger/lite_route-e2c/success_ref}{81.5}
\defres{mm/routing/trigger/lite_route-e2c/vcode}{3}
\defres{mm/routing/trigger/lite_route-e2c/verdict}{no saving}
\defres{mm/routing/trigger/lite_route/acc}{97.9}
\defres{mm/routing/trigger/lite_route/accepted_acc}{97.9}
\defres{mm/routing/trigger/lite_route/acted}{6.4}
\defres{mm/routing/trigger/lite_route/acted_kind}{fired}
\defres{mm/routing/trigger/lite_route/cost_k}{14.4}
\defres{mm/routing/trigger/lite_route/cost_ref_k}{9.8}
\defres{mm/routing/trigger/lite_route/delta}{+3.0}
\defres{mm/routing/trigger/lite_route/delta_ci/hi}{+6.0}
\defres{mm/routing/trigger/lite_route/delta_ci/lo}{+0.0}
\defres{mm/routing/trigger/lite_route/fig_delta}{+3.0}
\defres{mm/routing/trigger/lite_route/fig_saving}{-48}
\defres{mm/routing/trigger/lite_route/flash/delta}{-15.0}
\defres{mm/routing/trigger/lite_route/flash/delta_ci/hi}{-10.5}
\defres{mm/routing/trigger/lite_route/flash/delta_ci/lo}{-20.0}
\defres{mm/routing/trigger/lite_route/flash/fig_delta}{-15.0}
\defres{mm/routing/trigger/lite_route/flash/fig_saving}{64}
\defres{mm/routing/trigger/lite_route/flash/n}{200}
\defres{mm/routing/trigger/lite_route/flash/saving}{64.5}
\defres{mm/routing/trigger/lite_route/flash/saving_ci/hi}{65.5}
\defres{mm/routing/trigger/lite_route/flash/saving_ci/lo}{63.5}
\defres{mm/routing/trigger/lite_route/n}{200}
\defres{mm/routing/trigger/lite_route/n_dropped}{0}
\defres{mm/routing/trigger/lite_route/s1_acc}{97.9}
\defres{mm/routing/trigger/lite_route/saving}{-47.8}
\defres{mm/routing/trigger/lite_route/saving_ci/hi}{-43.8}
\defres{mm/routing/trigger/lite_route/saving_ci/lo}{-51.9}
\defres{mm/routing/trigger/lite_route/status}{descriptive}
\defres{mm/routing/trigger/lite_route/success}{85.0}
\defres{mm/routing/trigger/lite_route/success_ref}{82.0}
\defres{mm/routing/trigger/lite_route/vcode}{3}
\defres{mm/routing/trigger/lite_route/verdict}{no saving}
\defres{mm/routing/trigger/randscore_route_tau0.2/acc}{97.8}
\defres{mm/routing/trigger/randscore_route_tau0.2/accepted_acc}{97.8}
\defres{mm/routing/trigger/randscore_route_tau0.2/acted}{78.5}
\defres{mm/routing/trigger/randscore_route_tau0.2/acted_kind}{fired}
\defres{mm/routing/trigger/randscore_route_tau0.2/cost_k}{33.8}
\defres{mm/routing/trigger/randscore_route_tau0.2/cost_ref_k}{9.7}
\defres{mm/routing/trigger/randscore_route_tau0.2/delta}{+15.0}
\defres{mm/routing/trigger/randscore_route_tau0.2/delta_ci/hi}{+20.0}
\defres{mm/routing/trigger/randscore_route_tau0.2/delta_ci/lo}{+10.0}
\defres{mm/routing/trigger/randscore_route_tau0.2/fig_delta}{+15.0}
\defres{mm/routing/trigger/randscore_route_tau0.2/fig_saving}{-248}
\defres{mm/routing/trigger/randscore_route_tau0.2/flash/delta}{-3.5}
\defres{mm/routing/trigger/randscore_route_tau0.2/flash/delta_ci/hi}{-1.0}
\defres{mm/routing/trigger/randscore_route_tau0.2/flash/delta_ci/lo}{-6.0}
\defres{mm/routing/trigger/randscore_route_tau0.2/flash/fig_delta}{-3.5}
\defres{mm/routing/trigger/randscore_route_tau0.2/flash/fig_saving}{18}
\defres{mm/routing/trigger/randscore_route_tau0.2/flash/n}{200}
\defres{mm/routing/trigger/randscore_route_tau0.2/flash/saving}{17.5}
\defres{mm/routing/trigger/randscore_route_tau0.2/flash/saving_ci/hi}{19.3}
\defres{mm/routing/trigger/randscore_route_tau0.2/flash/saving_ci/lo}{15.9}
\defres{mm/routing/trigger/randscore_route_tau0.2/n}{200}
\defres{mm/routing/trigger/randscore_route_tau0.2/n_dropped}{0}
\defres{mm/routing/trigger/randscore_route_tau0.2/s1_acc}{97.8}
\defres{mm/routing/trigger/randscore_route_tau0.2/saving}{-247.6}
\defres{mm/routing/trigger/randscore_route_tau0.2/saving_ci/hi}{-239.4}
\defres{mm/routing/trigger/randscore_route_tau0.2/saving_ci/lo}{-255.8}
\defres{mm/routing/trigger/randscore_route_tau0.2/status}{descriptive}
\defres{mm/routing/trigger/randscore_route_tau0.2/success}{96.5}
\defres{mm/routing/trigger/randscore_route_tau0.2/success_ref}{81.5}
\defres{mm/routing/trigger/randscore_route_tau0.2/vcode}{3}
\defres{mm/routing/trigger/randscore_route_tau0.2/verdict}{no saving}
\defres{mm/routing/trigger/randscore_route_tau0.4/acc}{98.1}
\defres{mm/routing/trigger/randscore_route_tau0.4/accepted_acc}{98.1}
\defres{mm/routing/trigger/randscore_route_tau0.4/acted}{58.6}
\defres{mm/routing/trigger/randscore_route_tau0.4/acted_kind}{fired}
\defres{mm/routing/trigger/randscore_route_tau0.4/cost_k}{28.9}
\defres{mm/routing/trigger/randscore_route_tau0.4/cost_ref_k}{9.7}
\defres{mm/routing/trigger/randscore_route_tau0.4/delta}{+12.5}
\defres{mm/routing/trigger/randscore_route_tau0.4/delta_ci/hi}{+17.5}
\defres{mm/routing/trigger/randscore_route_tau0.4/delta_ci/lo}{+8.0}
\defres{mm/routing/trigger/randscore_route_tau0.4/fig_delta}{+12.5}
\defres{mm/routing/trigger/randscore_route_tau0.4/fig_saving}{-197}
\defres{mm/routing/trigger/randscore_route_tau0.4/flash/delta}{-6.0}
\defres{mm/routing/trigger/randscore_route_tau0.4/flash/delta_ci/hi}{-3.0}
\defres{mm/routing/trigger/randscore_route_tau0.4/flash/delta_ci/lo}{-9.5}
\defres{mm/routing/trigger/randscore_route_tau0.4/flash/fig_delta}{-6.0}
\defres{mm/routing/trigger/randscore_route_tau0.4/flash/fig_saving}{29}
\defres{mm/routing/trigger/randscore_route_tau0.4/flash/n}{200}
\defres{mm/routing/trigger/randscore_route_tau0.4/flash/saving}{29.5}
\defres{mm/routing/trigger/randscore_route_tau0.4/flash/saving_ci/hi}{31.6}
\defres{mm/routing/trigger/randscore_route_tau0.4/flash/saving_ci/lo}{27.3}
\defres{mm/routing/trigger/randscore_route_tau0.4/n}{200}
\defres{mm/routing/trigger/randscore_route_tau0.4/n_dropped}{0}
\defres{mm/routing/trigger/randscore_route_tau0.4/s1_acc}{98.1}
\defres{mm/routing/trigger/randscore_route_tau0.4/saving}{-197.4}
\defres{mm/routing/trigger/randscore_route_tau0.4/saving_ci/hi}{-187.7}
\defres{mm/routing/trigger/randscore_route_tau0.4/saving_ci/lo}{-206.9}
\defres{mm/routing/trigger/randscore_route_tau0.4/status}{descriptive}
\defres{mm/routing/trigger/randscore_route_tau0.4/success}{94.0}
\defres{mm/routing/trigger/randscore_route_tau0.4/success_ref}{81.5}
\defres{mm/routing/trigger/randscore_route_tau0.4/vcode}{3}
\defres{mm/routing/trigger/randscore_route_tau0.4/verdict}{no saving}
\defres{mm/routing/trigger/randscore_route_tau0.6/acc}{97.5}
\defres{mm/routing/trigger/randscore_route_tau0.6/accepted_acc}{97.5}
\defres{mm/routing/trigger/randscore_route_tau0.6/acted}{37.5}
\defres{mm/routing/trigger/randscore_route_tau0.6/acted_kind}{fired}
\defres{mm/routing/trigger/randscore_route_tau0.6/cost_k}{21.6}
\defres{mm/routing/trigger/randscore_route_tau0.6/cost_ref_k}{9.7}
\defres{mm/routing/trigger/randscore_route_tau0.6/delta}{+6.5}
\defres{mm/routing/trigger/randscore_route_tau0.6/delta_ci/hi}{+10.5}
\defres{mm/routing/trigger/randscore_route_tau0.6/delta_ci/lo}{+2.5}
\defres{mm/routing/trigger/randscore_route_tau0.6/fig_delta}{+6.5}
\defres{mm/routing/trigger/randscore_route_tau0.6/fig_saving}{-122}
\defres{mm/routing/trigger/randscore_route_tau0.6/flash/delta}{-12.0}
\defres{mm/routing/trigger/randscore_route_tau0.6/flash/delta_ci/hi}{-7.5}
\defres{mm/routing/trigger/randscore_route_tau0.6/flash/delta_ci/lo}{-16.5}
\defres{mm/routing/trigger/randscore_route_tau0.6/flash/fig_delta}{-12.0}
\defres{mm/routing/trigger/randscore_route_tau0.6/flash/fig_saving}{47}
\defres{mm/routing/trigger/randscore_route_tau0.6/flash/n}{200}
\defres{mm/routing/trigger/randscore_route_tau0.6/flash/saving}{47.3}
\defres{mm/routing/trigger/randscore_route_tau0.6/flash/saving_ci/hi}{49.2}
\defres{mm/routing/trigger/randscore_route_tau0.6/flash/saving_ci/lo}{45.4}
\defres{mm/routing/trigger/randscore_route_tau0.6/n}{200}
\defres{mm/routing/trigger/randscore_route_tau0.6/n_dropped}{0}
\defres{mm/routing/trigger/randscore_route_tau0.6/s1_acc}{97.5}
\defres{mm/routing/trigger/randscore_route_tau0.6/saving}{-122.2}
\defres{mm/routing/trigger/randscore_route_tau0.6/saving_ci/hi}{-113.8}
\defres{mm/routing/trigger/randscore_route_tau0.6/saving_ci/lo}{-130.6}
\defres{mm/routing/trigger/randscore_route_tau0.6/status}{descriptive}
\defres{mm/routing/trigger/randscore_route_tau0.6/success}{88.0}
\defres{mm/routing/trigger/randscore_route_tau0.6/success_ref}{81.5}
\defres{mm/routing/trigger/randscore_route_tau0.6/vcode}{3}
\defres{mm/routing/trigger/randscore_route_tau0.6/verdict}{no saving}
\defres{mm/routing/trigger/randscore_route_tau0.8/acc}{97.8}
\defres{mm/routing/trigger/randscore_route_tau0.8/accepted_acc}{97.8}
\defres{mm/routing/trigger/randscore_route_tau0.8/acted}{19.9}
\defres{mm/routing/trigger/randscore_route_tau0.8/acted_kind}{fired}
\defres{mm/routing/trigger/randscore_route_tau0.8/cost_k}{15.9}
\defres{mm/routing/trigger/randscore_route_tau0.8/cost_ref_k}{9.7}
\defres{mm/routing/trigger/randscore_route_tau0.8/delta}{+5.5}
\defres{mm/routing/trigger/randscore_route_tau0.8/delta_ci/hi}{+9.5}
\defres{mm/routing/trigger/randscore_route_tau0.8/delta_ci/lo}{+2.0}
\defres{mm/routing/trigger/randscore_route_tau0.8/fig_delta}{+5.5}
\defres{mm/routing/trigger/randscore_route_tau0.8/fig_saving}{-64}
\defres{mm/routing/trigger/randscore_route_tau0.8/flash/delta}{-13.0}
\defres{mm/routing/trigger/randscore_route_tau0.8/flash/delta_ci/hi}{-8.5}
\defres{mm/routing/trigger/randscore_route_tau0.8/flash/delta_ci/lo}{-17.5}
\defres{mm/routing/trigger/randscore_route_tau0.8/flash/fig_delta}{-13.0}
\defres{mm/routing/trigger/randscore_route_tau0.8/flash/fig_saving}{61}
\defres{mm/routing/trigger/randscore_route_tau0.8/flash/n}{200}
\defres{mm/routing/trigger/randscore_route_tau0.8/flash/saving}{61.1}
\defres{mm/routing/trigger/randscore_route_tau0.8/flash/saving_ci/hi}{62.6}
\defres{mm/routing/trigger/randscore_route_tau0.8/flash/saving_ci/lo}{59.6}
\defres{mm/routing/trigger/randscore_route_tau0.8/n}{200}
\defres{mm/routing/trigger/randscore_route_tau0.8/n_dropped}{0}
\defres{mm/routing/trigger/randscore_route_tau0.8/s1_acc}{97.8}
\defres{mm/routing/trigger/randscore_route_tau0.8/saving}{-64.0}
\defres{mm/routing/trigger/randscore_route_tau0.8/saving_ci/hi}{-57.6}
\defres{mm/routing/trigger/randscore_route_tau0.8/saving_ci/lo}{-70.4}
\defres{mm/routing/trigger/randscore_route_tau0.8/status}{descriptive}
\defres{mm/routing/trigger/randscore_route_tau0.8/success}{87.0}
\defres{mm/routing/trigger/randscore_route_tau0.8/success_ref}{81.5}
\defres{mm/routing/trigger/randscore_route_tau0.8/vcode}{3}
\defres{mm/routing/trigger/randscore_route_tau0.8/verdict}{no saving}
\defres{mm/routing/trigger/rate10_route/acc}{97.5}
\defres{mm/routing/trigger/rate10_route/accepted_acc}{97.5}
\defres{mm/routing/trigger/rate10_route/acted}{11.3}
\defres{mm/routing/trigger/rate10_route/acted_kind}{fired}
\defres{mm/routing/trigger/rate10_route/cost_k}{13.2}
\defres{mm/routing/trigger/rate10_route/cost_ref_k}{9.7}
\defres{mm/routing/trigger/rate10_route/delta}{+1.5}
\defres{mm/routing/trigger/rate10_route/delta_ci/hi}{+4.5}
\defres{mm/routing/trigger/rate10_route/delta_ci/lo}{-1.5}
\defres{mm/routing/trigger/rate10_route/fig_delta}{+1.5}
\defres{mm/routing/trigger/rate10_route/fig_saving}{-36}
\defres{mm/routing/trigger/rate10_route/flash/delta}{-17.0}
\defres{mm/routing/trigger/rate10_route/flash/delta_ci/hi}{-12.0}
\defres{mm/routing/trigger/rate10_route/flash/delta_ci/lo}{-22.0}
\defres{mm/routing/trigger/rate10_route/flash/fig_delta}{-17.0}
\defres{mm/routing/trigger/rate10_route/flash/fig_saving}{68}
\defres{mm/routing/trigger/rate10_route/flash/n}{200}
\defres{mm/routing/trigger/rate10_route/flash/saving}{67.9}
\defres{mm/routing/trigger/rate10_route/flash/saving_ci/hi}{69.2}
\defres{mm/routing/trigger/rate10_route/flash/saving_ci/lo}{66.5}
\defres{mm/routing/trigger/rate10_route/n}{200}
\defres{mm/routing/trigger/rate10_route/n_dropped}{0}
\defres{mm/routing/trigger/rate10_route/s1_acc}{97.5}
\defres{mm/routing/trigger/rate10_route/saving}{-35.5}
\defres{mm/routing/trigger/rate10_route/saving_ci/hi}{-30.5}
\defres{mm/routing/trigger/rate10_route/saving_ci/lo}{-40.8}
\defres{mm/routing/trigger/rate10_route/status}{descriptive}
\defres{mm/routing/trigger/rate10_route/success}{83.0}
\defres{mm/routing/trigger/rate10_route/success_ref}{81.5}
\defres{mm/routing/trigger/rate10_route/vcode}{3}
\defres{mm/routing/trigger/rate10_route/verdict}{no saving}
\defres{mm/routing/trigger/rate30_route/acc}{97.4}
\defres{mm/routing/trigger/rate30_route/accepted_acc}{97.4}
\defres{mm/routing/trigger/rate30_route/acted}{31.0}
\defres{mm/routing/trigger/rate30_route/acted_kind}{fired}
\defres{mm/routing/trigger/rate30_route/cost_k}{19.3}
\defres{mm/routing/trigger/rate30_route/cost_ref_k}{9.7}
\defres{mm/routing/trigger/rate30_route/delta}{+5.0}
\defres{mm/routing/trigger/rate30_route/delta_ci/hi}{+10.0}
\defres{mm/routing/trigger/rate30_route/delta_ci/lo}{+0.5}
\defres{mm/routing/trigger/rate30_route/fig_delta}{+5.0}
\defres{mm/routing/trigger/rate30_route/fig_saving}{-99}
\defres{mm/routing/trigger/rate30_route/flash/delta}{-13.5}
\defres{mm/routing/trigger/rate30_route/flash/delta_ci/hi}{-9.0}
\defres{mm/routing/trigger/rate30_route/flash/delta_ci/lo}{-18.5}
\defres{mm/routing/trigger/rate30_route/flash/fig_delta}{-13.5}
\defres{mm/routing/trigger/rate30_route/flash/fig_saving}{53}
\defres{mm/routing/trigger/rate30_route/flash/n}{200}
\defres{mm/routing/trigger/rate30_route/flash/saving}{52.8}
\defres{mm/routing/trigger/rate30_route/flash/saving_ci/hi}{54.6}
\defres{mm/routing/trigger/rate30_route/flash/saving_ci/lo}{51.0}
\defres{mm/routing/trigger/rate30_route/n}{200}
\defres{mm/routing/trigger/rate30_route/n_dropped}{0}
\defres{mm/routing/trigger/rate30_route/s1_acc}{97.4}
\defres{mm/routing/trigger/rate30_route/saving}{-99.0}
\defres{mm/routing/trigger/rate30_route/saving_ci/hi}{-91.7}
\defres{mm/routing/trigger/rate30_route/saving_ci/lo}{-106.3}
\defres{mm/routing/trigger/rate30_route/status}{descriptive}
\defres{mm/routing/trigger/rate30_route/success}{86.5}
\defres{mm/routing/trigger/rate30_route/success_ref}{81.5}
\defres{mm/routing/trigger/rate30_route/vcode}{3}
\defres{mm/routing/trigger/rate30_route/verdict}{no saving}
\defres{mm/routing/trigger/rate50_route/acc}{97.0}
\defres{mm/routing/trigger/rate50_route/accepted_acc}{97.0}
\defres{mm/routing/trigger/rate50_route/acted}{51.3}
\defres{mm/routing/trigger/rate50_route/acted_kind}{fired}
\defres{mm/routing/trigger/rate50_route/cost_k}{25.5}
\defres{mm/routing/trigger/rate50_route/cost_ref_k}{9.7}
\defres{mm/routing/trigger/rate50_route/delta}{+7.5}
\defres{mm/routing/trigger/rate50_route/delta_ci/hi}{+12.5}
\defres{mm/routing/trigger/rate50_route/delta_ci/lo}{+3.0}
\defres{mm/routing/trigger/rate50_route/fig_delta}{+7.5}
\defres{mm/routing/trigger/rate50_route/fig_saving}{-163}
\defres{mm/routing/trigger/rate50_route/flash/delta}{-11.0}
\defres{mm/routing/trigger/rate50_route/flash/delta_ci/hi}{-7.0}
\defres{mm/routing/trigger/rate50_route/flash/delta_ci/lo}{-15.5}
\defres{mm/routing/trigger/rate50_route/flash/fig_delta}{-11.0}
\defres{mm/routing/trigger/rate50_route/flash/fig_saving}{38}
\defres{mm/routing/trigger/rate50_route/flash/n}{200}
\defres{mm/routing/trigger/rate50_route/flash/saving}{37.6}
\defres{mm/routing/trigger/rate50_route/flash/saving_ci/hi}{39.6}
\defres{mm/routing/trigger/rate50_route/flash/saving_ci/lo}{35.5}
\defres{mm/routing/trigger/rate50_route/n}{200}
\defres{mm/routing/trigger/rate50_route/n_dropped}{0}
\defres{mm/routing/trigger/rate50_route/s1_acc}{97.0}
\defres{mm/routing/trigger/rate50_route/saving}{-163.1}
\defres{mm/routing/trigger/rate50_route/saving_ci/hi}{-155.0}
\defres{mm/routing/trigger/rate50_route/saving_ci/lo}{-171.6}
\defres{mm/routing/trigger/rate50_route/status}{descriptive}
\defres{mm/routing/trigger/rate50_route/success}{89.0}
\defres{mm/routing/trigger/rate50_route/success_ref}{81.5}
\defres{mm/routing/trigger/rate50_route/vcode}{3}
\defres{mm/routing/trigger/rate50_route/verdict}{no saving}
\defres{mm/routing/trigger/ratem_route/acc}{97.7}
\defres{mm/routing/trigger/ratem_route/accepted_acc}{97.7}
\defres{mm/routing/trigger/ratem_route/acted}{4.8}
\defres{mm/routing/trigger/ratem_route/acted_kind}{fired}
\defres{mm/routing/trigger/ratem_route/cost_k}{11.4}
\defres{mm/routing/trigger/ratem_route/cost_ref_k}{9.7}
\defres{mm/routing/trigger/ratem_route/delta}{+2.0}
\defres{mm/routing/trigger/ratem_route/delta_ci/hi}{+5.5}
\defres{mm/routing/trigger/ratem_route/delta_ci/lo}{-1.0}
\defres{mm/routing/trigger/ratem_route/fig_delta}{+2.0}
\defres{mm/routing/trigger/ratem_route/fig_saving}{-17}
\defres{mm/routing/trigger/ratem_route/flash/delta}{-16.5}
\defres{mm/routing/trigger/ratem_route/flash/delta_ci/hi}{-11.5}
\defres{mm/routing/trigger/ratem_route/flash/delta_ci/lo}{-21.5}
\defres{mm/routing/trigger/ratem_route/flash/fig_delta}{-16.5}
\defres{mm/routing/trigger/ratem_route/flash/fig_saving}{72}
\defres{mm/routing/trigger/ratem_route/flash/n}{200}
\defres{mm/routing/trigger/ratem_route/flash/saving}{72.3}
\defres{mm/routing/trigger/ratem_route/flash/saving_ci/hi}{73.3}
\defres{mm/routing/trigger/ratem_route/flash/saving_ci/lo}{71.1}
\defres{mm/routing/trigger/ratem_route/n}{200}
\defres{mm/routing/trigger/ratem_route/n_dropped}{0}
\defres{mm/routing/trigger/ratem_route/s1_acc}{97.7}
\defres{mm/routing/trigger/ratem_route/saving}{-17.0}
\defres{mm/routing/trigger/ratem_route/saving_ci/hi}{-13.0}
\defres{mm/routing/trigger/ratem_route/saving_ci/lo}{-21.2}
\defres{mm/routing/trigger/ratem_route/status}{descriptive}
\defres{mm/routing/trigger/ratem_route/success}{83.5}
\defres{mm/routing/trigger/ratem_route/success_ref}{81.5}
\defres{mm/routing/trigger/ratem_route/vcode}{3}
\defres{mm/routing/trigger/ratem_route/verdict}{no saving}
\defres{mm/routing/trigger/s2self_route/acc}{97.6}
\defres{mm/routing/trigger/s2self_route/accepted_acc}{97.6}
\defres{mm/routing/trigger/s2self_route/acted}{1.3}
\defres{mm/routing/trigger/s2self_route/acted_kind}{fired}
\defres{mm/routing/trigger/s2self_route/cost_k}{22.6}
\defres{mm/routing/trigger/s2self_route/cost_ref_k}{9.7}
\defres{mm/routing/trigger/s2self_route/delta}{+1.0}
\defres{mm/routing/trigger/s2self_route/delta_ci/hi}{+4.0}
\defres{mm/routing/trigger/s2self_route/delta_ci/lo}{-1.5}
\defres{mm/routing/trigger/s2self_route/fig_delta}{+1.0}
\defres{mm/routing/trigger/s2self_route/fig_saving}{-133}
\defres{mm/routing/trigger/s2self_route/flash/delta}{-17.5}
\defres{mm/routing/trigger/s2self_route/flash/delta_ci/hi}{-12.5}
\defres{mm/routing/trigger/s2self_route/flash/delta_ci/lo}{-23.0}
\defres{mm/routing/trigger/s2self_route/flash/fig_delta}{-17.5}
\defres{mm/routing/trigger/s2self_route/flash/fig_saving}{45}
\defres{mm/routing/trigger/s2self_route/flash/n}{200}
\defres{mm/routing/trigger/s2self_route/flash/saving}{44.7}
\defres{mm/routing/trigger/s2self_route/flash/saving_ci/hi}{45.5}
\defres{mm/routing/trigger/s2self_route/flash/saving_ci/lo}{43.9}
\defres{mm/routing/trigger/s2self_route/n}{200}
\defres{mm/routing/trigger/s2self_route/n_dropped}{0}
\defres{mm/routing/trigger/s2self_route/s1_acc}{97.6}
\defres{mm/routing/trigger/s2self_route/saving}{-133.2}
\defres{mm/routing/trigger/s2self_route/saving_ci/hi}{-127.8}
\defres{mm/routing/trigger/s2self_route/saving_ci/lo}{-138.3}
\defres{mm/routing/trigger/s2self_route/status}{descriptive}
\defres{mm/routing/trigger/s2self_route/success}{82.5}
\defres{mm/routing/trigger/s2self_route/success_ref}{81.5}
\defres{mm/routing/trigger/s2self_route/vcode}{3}
\defres{mm/routing/trigger/s2self_route/verdict}{no saving}
\defres{mm/stop/guard/heuristic_stop_guard/acc}{100.0}
\defres{mm/stop/guard/heuristic_stop_guard/accepted_acc}{100.0}
\defres{mm/stop/guard/heuristic_stop_guard/acted}{0.0}
\defres{mm/stop/guard/heuristic_stop_guard/acted_kind}{vetoed}
\defres{mm/stop/guard/heuristic_stop_guard/cost_k}{40.5}
\defres{mm/stop/guard/heuristic_stop_guard/cost_ref_k}{40.9}
\defres{mm/stop/guard/heuristic_stop_guard/delta}{+0.0}
\defres{mm/stop/guard/heuristic_stop_guard/delta_ci/hi}{+0.0}
\defres{mm/stop/guard/heuristic_stop_guard/delta_ci/lo}{+0.0}
\defres{mm/stop/guard/heuristic_stop_guard/fig_delta}{+0.0}
\defres{mm/stop/guard/heuristic_stop_guard/fig_saving}{1}
\defres{mm/stop/guard/heuristic_stop_guard/n}{200}
\defres{mm/stop/guard/heuristic_stop_guard/n_dropped}{0}
\defres{mm/stop/guard/heuristic_stop_guard/s1_acc}{100.0}
\defres{mm/stop/guard/heuristic_stop_guard/saving}{1.1}
\defres{mm/stop/guard/heuristic_stop_guard/saving_ci/hi}{1.8}
\defres{mm/stop/guard/heuristic_stop_guard/saving_ci/lo}{0.4}
\defres{mm/stop/guard/heuristic_stop_guard/status}{descriptive}
\defres{mm/stop/guard/heuristic_stop_guard/success}{100.0}
\defres{mm/stop/guard/heuristic_stop_guard/success_ref}{100.0}
\defres{mm/stop/guard/heuristic_stop_guard/vcode}{2}
\defres{mm/stop/guard/heuristic_stop_guard/verdict}{mixed}
\defres{mm/stop/guard/heuristic_stop_guard_s2lite/acc}{86.5}
\defres{mm/stop/guard/heuristic_stop_guard_s2lite/accepted_acc}{86.5}
\defres{mm/stop/guard/heuristic_stop_guard_s2lite/acted}{0.0}
\defres{mm/stop/guard/heuristic_stop_guard_s2lite/acted_kind}{vetoed}
\defres{mm/stop/guard/heuristic_stop_guard_s2lite/cost_k}{9.7}
\defres{mm/stop/guard/heuristic_stop_guard_s2lite/cost_ref_k}{9.7}
\defres{mm/stop/guard/heuristic_stop_guard_s2lite/delta}{+5.0}
\defres{mm/stop/guard/heuristic_stop_guard_s2lite/delta_ci/hi}{+8.5}
\defres{mm/stop/guard/heuristic_stop_guard_s2lite/delta_ci/lo}{+1.5}
\defres{mm/stop/guard/heuristic_stop_guard_s2lite/fig_delta}{+5.0}
\defres{mm/stop/guard/heuristic_stop_guard_s2lite/fig_saving}{0}
\defres{mm/stop/guard/heuristic_stop_guard_s2lite/n}{200}
\defres{mm/stop/guard/heuristic_stop_guard_s2lite/n_dropped}{0}
\defres{mm/stop/guard/heuristic_stop_guard_s2lite/s1_acc}{86.5}
\defres{mm/stop/guard/heuristic_stop_guard_s2lite/saving}{-0.1}
\defres{mm/stop/guard/heuristic_stop_guard_s2lite/saving_ci/hi}{0.3}
\defres{mm/stop/guard/heuristic_stop_guard_s2lite/saving_ci/lo}{-0.5}
\defres{mm/stop/guard/heuristic_stop_guard_s2lite/status}{descriptive}
\defres{mm/stop/guard/heuristic_stop_guard_s2lite/success}{86.5}
\defres{mm/stop/guard/heuristic_stop_guard_s2lite/success_ref}{81.5}
\defres{mm/stop/guard/heuristic_stop_guard_s2lite/vcode}{3}
\defres{mm/stop/guard/heuristic_stop_guard_s2lite/verdict}{no saving}
\defres{mm/stop/guard/jev_stop_guard-e2c/acc}{89.3}
\defres{mm/stop/guard/jev_stop_guard-e2c/accepted_acc}{89.3}
\defres{mm/stop/guard/jev_stop_guard-e2c/acted}{10.7}
\defres{mm/stop/guard/jev_stop_guard-e2c/acted_kind}{vetoed}
\defres{mm/stop/guard/jev_stop_guard-e2c/cost_k}{42.1}
\defres{mm/stop/guard/jev_stop_guard-e2c/cost_ref_k}{40.9}
\defres{mm/stop/guard/jev_stop_guard-e2c/delta}{+0.0}
\defres{mm/stop/guard/jev_stop_guard-e2c/delta_ci/hi}{+0.0}
\defres{mm/stop/guard/jev_stop_guard-e2c/delta_ci/lo}{+0.0}
\defres{mm/stop/guard/jev_stop_guard-e2c/fig_delta}{+0.0}
\defres{mm/stop/guard/jev_stop_guard-e2c/fig_saving}{-3}
\defres{mm/stop/guard/jev_stop_guard-e2c/n}{200}
\defres{mm/stop/guard/jev_stop_guard-e2c/n_dropped}{0}
\defres{mm/stop/guard/jev_stop_guard-e2c/s1_acc}{89.3}
\defres{mm/stop/guard/jev_stop_guard-e2c/saving}{-2.9}
\defres{mm/stop/guard/jev_stop_guard-e2c/saving_ci/hi}{-1.6}
\defres{mm/stop/guard/jev_stop_guard-e2c/saving_ci/lo}{-4.4}
\defres{mm/stop/guard/jev_stop_guard-e2c/status}{replicate}
\defres{mm/stop/guard/jev_stop_guard-e2c/success}{100.0}
\defres{mm/stop/guard/jev_stop_guard-e2c/success_ref}{100.0}
\defres{mm/stop/guard/jev_stop_guard-e2c/vcode}{3}
\defres{mm/stop/guard/jev_stop_guard-e2c/verdict}{no saving}
\defres{mm/stop/guard/jev_stop_guard/acc}{82.7}
\defres{mm/stop/guard/jev_stop_guard/accepted_acc}{82.7}
\defres{mm/stop/guard/jev_stop_guard/acted}{17.3}
\defres{mm/stop/guard/jev_stop_guard/acted_kind}{vetoed}
\defres{mm/stop/guard/jev_stop_guard/cost_k}{43.3}
\defres{mm/stop/guard/jev_stop_guard/cost_ref_k}{40.8}
\defres{mm/stop/guard/jev_stop_guard/delta}{-0.6}
\defres{mm/stop/guard/jev_stop_guard/delta_ci/hi}{+0.0}
\defres{mm/stop/guard/jev_stop_guard/delta_ci/lo}{-1.4}
\defres{mm/stop/guard/jev_stop_guard/fig_delta}{-0.6}
\defres{mm/stop/guard/jev_stop_guard/fig_saving}{-6}
\defres{mm/stop/guard/jev_stop_guard/n}{500}
\defres{mm/stop/guard/jev_stop_guard/n_dropped}{0}
\defres{mm/stop/guard/jev_stop_guard/reg}{C6F}
\defres{mm/stop/guard/jev_stop_guard/s1_acc}{82.7}
\defres{mm/stop/guard/jev_stop_guard/saving}{-6.2}
\defres{mm/stop/guard/jev_stop_guard/saving_ci/hi}{-4.0}
\defres{mm/stop/guard/jev_stop_guard/saving_ci/lo}{-9.1}
\defres{mm/stop/guard/jev_stop_guard/status}{registered}
\defres{mm/stop/guard/jev_stop_guard/success}{99.2}
\defres{mm/stop/guard/jev_stop_guard/success_ref}{99.8}
\defres{mm/stop/guard/jev_stop_guard/vcode}{3}
\defres{mm/stop/guard/jev_stop_guard/verdict}{no saving}
\defres{mm/stop/guard/jev_stop_guard_s2lite-e2c/acc}{78.3}
\defres{mm/stop/guard/jev_stop_guard_s2lite-e2c/accepted_acc}{78.3}
\defres{mm/stop/guard/jev_stop_guard_s2lite-e2c/acted}{65.3}
\defres{mm/stop/guard/jev_stop_guard_s2lite-e2c/acted_kind}{vetoed}
\defres{mm/stop/guard/jev_stop_guard_s2lite-e2c/cost_k}{12.0}
\defres{mm/stop/guard/jev_stop_guard_s2lite-e2c/cost_ref_k}{9.7}
\defres{mm/stop/guard/jev_stop_guard_s2lite-e2c/delta}{+3.0}
\defres{mm/stop/guard/jev_stop_guard_s2lite-e2c/delta_ci/hi}{+6.5}
\defres{mm/stop/guard/jev_stop_guard_s2lite-e2c/delta_ci/lo}{+0.0}
\defres{mm/stop/guard/jev_stop_guard_s2lite-e2c/fig_delta}{+3.0}
\defres{mm/stop/guard/jev_stop_guard_s2lite-e2c/fig_saving}{-24}
\defres{mm/stop/guard/jev_stop_guard_s2lite-e2c/n}{200}
\defres{mm/stop/guard/jev_stop_guard_s2lite-e2c/n_dropped}{0}
\defres{mm/stop/guard/jev_stop_guard_s2lite-e2c/s1_acc}{78.3}
\defres{mm/stop/guard/jev_stop_guard_s2lite-e2c/saving}{-23.8}
\defres{mm/stop/guard/jev_stop_guard_s2lite-e2c/saving_ci/hi}{-14.1}
\defres{mm/stop/guard/jev_stop_guard_s2lite-e2c/saving_ci/lo}{-34.6}
\defres{mm/stop/guard/jev_stop_guard_s2lite-e2c/status}{replicate}
\defres{mm/stop/guard/jev_stop_guard_s2lite-e2c/success}{84.5}
\defres{mm/stop/guard/jev_stop_guard_s2lite-e2c/success_ref}{81.5}
\defres{mm/stop/guard/jev_stop_guard_s2lite-e2c/vcode}{3}
\defres{mm/stop/guard/jev_stop_guard_s2lite-e2c/verdict}{no saving}
\defres{mm/stop/guard/jev_stop_guard_s2lite/acc}{75.4}
\defres{mm/stop/guard/jev_stop_guard_s2lite/accepted_acc}{75.4}
\defres{mm/stop/guard/jev_stop_guard_s2lite/acted}{72.6}
\defres{mm/stop/guard/jev_stop_guard_s2lite/acted_kind}{vetoed}
\defres{mm/stop/guard/jev_stop_guard_s2lite/cost_k}{13.0}
\defres{mm/stop/guard/jev_stop_guard_s2lite/cost_ref_k}{9.8}
\defres{mm/stop/guard/jev_stop_guard_s2lite/delta}{+1.6}
\defres{mm/stop/guard/jev_stop_guard_s2lite/delta_ci/hi}{+4.0}
\defres{mm/stop/guard/jev_stop_guard_s2lite/delta_ci/lo}{-0.8}
\defres{mm/stop/guard/jev_stop_guard_s2lite/fig_delta}{+1.6}
\defres{mm/stop/guard/jev_stop_guard_s2lite/fig_saving}{-32}
\defres{mm/stop/guard/jev_stop_guard_s2lite/n}{500}
\defres{mm/stop/guard/jev_stop_guard_s2lite/n_dropped}{0}
\defres{mm/stop/guard/jev_stop_guard_s2lite/reg}{C6L}
\defres{mm/stop/guard/jev_stop_guard_s2lite/s1_acc}{75.4}
\defres{mm/stop/guard/jev_stop_guard_s2lite/saving}{-32.1}
\defres{mm/stop/guard/jev_stop_guard_s2lite/saving_ci/hi}{-25.0}
\defres{mm/stop/guard/jev_stop_guard_s2lite/saving_ci/lo}{-39.4}
\defres{mm/stop/guard/jev_stop_guard_s2lite/status}{registered}
\defres{mm/stop/guard/jev_stop_guard_s2lite/success}{82.0}
\defres{mm/stop/guard/jev_stop_guard_s2lite/success_ref}{80.4}
\defres{mm/stop/guard/jev_stop_guard_s2lite/vcode}{3}
\defres{mm/stop/guard/jev_stop_guard_s2lite/verdict}{no saving}
\defres{mm/stop/guard/lite_stop_guard/acc}{79.3}
\defres{mm/stop/guard/lite_stop_guard/accepted_acc}{79.3}
\defres{mm/stop/guard/lite_stop_guard/acted}{20.7}
\defres{mm/stop/guard/lite_stop_guard/acted_kind}{vetoed}
\defres{mm/stop/guard/lite_stop_guard/cost_k}{42.4}
\defres{mm/stop/guard/lite_stop_guard/cost_ref_k}{40.6}
\defres{mm/stop/guard/lite_stop_guard/delta}{-0.5}
\defres{mm/stop/guard/lite_stop_guard/delta_ci/hi}{+0.0}
\defres{mm/stop/guard/lite_stop_guard/delta_ci/lo}{-1.5}
\defres{mm/stop/guard/lite_stop_guard/fig_delta}{-0.5}
\defres{mm/stop/guard/lite_stop_guard/fig_saving}{-4}
\defres{mm/stop/guard/lite_stop_guard/n}{200}
\defres{mm/stop/guard/lite_stop_guard/n_dropped}{0}
\defres{mm/stop/guard/lite_stop_guard/s1_acc}{79.3}
\defres{mm/stop/guard/lite_stop_guard/saving}{-4.5}
\defres{mm/stop/guard/lite_stop_guard/saving_ci/hi}{-0.6}
\defres{mm/stop/guard/lite_stop_guard/saving_ci/lo}{-9.8}
\defres{mm/stop/guard/lite_stop_guard/status}{descriptive}
\defres{mm/stop/guard/lite_stop_guard/success}{99.5}
\defres{mm/stop/guard/lite_stop_guard/success_ref}{100.0}
\defres{mm/stop/guard/lite_stop_guard/vcode}{3}
\defres{mm/stop/guard/lite_stop_guard/verdict}{no saving}
\defres{mm/stop/guard/rate50_stop_guard/acc}{51.9}
\defres{mm/stop/guard/rate50_stop_guard/accepted_acc}{51.9}
\defres{mm/stop/guard/rate50_stop_guard/acted}{48.1}
\defres{mm/stop/guard/rate50_stop_guard/acted_kind}{vetoed}
\defres{mm/stop/guard/rate50_stop_guard/cost_k}{46.4}
\defres{mm/stop/guard/rate50_stop_guard/cost_ref_k}{40.9}
\defres{mm/stop/guard/rate50_stop_guard/delta}{+0.0}
\defres{mm/stop/guard/rate50_stop_guard/delta_ci/hi}{+0.0}
\defres{mm/stop/guard/rate50_stop_guard/delta_ci/lo}{+0.0}
\defres{mm/stop/guard/rate50_stop_guard/fig_delta}{+0.0}
\defres{mm/stop/guard/rate50_stop_guard/fig_saving}{-13}
\defres{mm/stop/guard/rate50_stop_guard/n}{200}
\defres{mm/stop/guard/rate50_stop_guard/n_dropped}{0}
\defres{mm/stop/guard/rate50_stop_guard/s1_acc}{51.9}
\defres{mm/stop/guard/rate50_stop_guard/saving}{-13.2}
\defres{mm/stop/guard/rate50_stop_guard/saving_ci/hi}{-10.7}
\defres{mm/stop/guard/rate50_stop_guard/saving_ci/lo}{-16.0}
\defres{mm/stop/guard/rate50_stop_guard/status}{descriptive}
\defres{mm/stop/guard/rate50_stop_guard/success}{100.0}
\defres{mm/stop/guard/rate50_stop_guard/success_ref}{100.0}
\defres{mm/stop/guard/rate50_stop_guard/vcode}{3}
\defres{mm/stop/guard/rate50_stop_guard/verdict}{no saving}
\defres{mm/stop/guard/ratem_stop_guard_s2lite/acc}{62.0}
\defres{mm/stop/guard/ratem_stop_guard_s2lite/accepted_acc}{62.0}
\defres{mm/stop/guard/ratem_stop_guard_s2lite/acted}{30.3}
\defres{mm/stop/guard/ratem_stop_guard_s2lite/acted_kind}{vetoed}
\defres{mm/stop/guard/ratem_stop_guard_s2lite/cost_k}{10.2}
\defres{mm/stop/guard/ratem_stop_guard_s2lite/cost_ref_k}{9.7}
\defres{mm/stop/guard/ratem_stop_guard_s2lite/delta}{+1.5}
\defres{mm/stop/guard/ratem_stop_guard_s2lite/delta_ci/hi}{+5.0}
\defres{mm/stop/guard/ratem_stop_guard_s2lite/delta_ci/lo}{-2.0}
\defres{mm/stop/guard/ratem_stop_guard_s2lite/fig_delta}{+1.5}
\defres{mm/stop/guard/ratem_stop_guard_s2lite/fig_saving}{-5}
\defres{mm/stop/guard/ratem_stop_guard_s2lite/n}{200}
\defres{mm/stop/guard/ratem_stop_guard_s2lite/n_dropped}{0}
\defres{mm/stop/guard/ratem_stop_guard_s2lite/s1_acc}{62.0}
\defres{mm/stop/guard/ratem_stop_guard_s2lite/saving}{-5.3}
\defres{mm/stop/guard/ratem_stop_guard_s2lite/saving_ci/hi}{-4.0}
\defres{mm/stop/guard/ratem_stop_guard_s2lite/saving_ci/lo}{-6.9}
\defres{mm/stop/guard/ratem_stop_guard_s2lite/status}{descriptive}
\defres{mm/stop/guard/ratem_stop_guard_s2lite/success}{83.0}
\defres{mm/stop/guard/ratem_stop_guard_s2lite/success_ref}{81.5}
\defres{mm/stop/guard/ratem_stop_guard_s2lite/vcode}{3}
\defres{mm/stop/guard/ratem_stop_guard_s2lite/verdict}{no saving}
\defres{mm/stop/trigger/heuristic_stop_trigger/acc}{90.1}
\defres{mm/stop/trigger/heuristic_stop_trigger/accepted_acc}{90.1}
\defres{mm/stop/trigger/heuristic_stop_trigger/acted}{9.9}
\defres{mm/stop/trigger/heuristic_stop_trigger/acted_kind}{fired}
\defres{mm/stop/trigger/heuristic_stop_trigger/cost_k}{31.1}
\defres{mm/stop/trigger/heuristic_stop_trigger/cost_ref_k}{40.9}
\defres{mm/stop/trigger/heuristic_stop_trigger/delta}{-50.0}
\defres{mm/stop/trigger/heuristic_stop_trigger/delta_ci/hi}{-43.0}
\defres{mm/stop/trigger/heuristic_stop_trigger/delta_ci/lo}{-57.0}
\defres{mm/stop/trigger/heuristic_stop_trigger/fig_delta}{-50.0}
\defres{mm/stop/trigger/heuristic_stop_trigger/fig_saving}{24}
\defres{mm/stop/trigger/heuristic_stop_trigger/n}{200}
\defres{mm/stop/trigger/heuristic_stop_trigger/n_dropped}{0}
\defres{mm/stop/trigger/heuristic_stop_trigger/s1_acc}{90.1}
\defres{mm/stop/trigger/heuristic_stop_trigger/saving}{24.1}
\defres{mm/stop/trigger/heuristic_stop_trigger/saving_ci/hi}{27.4}
\defres{mm/stop/trigger/heuristic_stop_trigger/saving_ci/lo}{20.7}
\defres{mm/stop/trigger/heuristic_stop_trigger/status}{descriptive}
\defres{mm/stop/trigger/heuristic_stop_trigger/success}{50.0}
\defres{mm/stop/trigger/heuristic_stop_trigger/success_ref}{100.0}
\defres{mm/stop/trigger/heuristic_stop_trigger/vcode}{4}
\defres{mm/stop/trigger/heuristic_stop_trigger/verdict}{costs success}
\defres{mm/stop/trigger/jev_stop_trigger-e2c/acc}{100.0}
\defres{mm/stop/trigger/jev_stop_trigger-e2c/accepted_acc}{100.0}
\defres{mm/stop/trigger/jev_stop_trigger-e2c/acted}{0.0}
\defres{mm/stop/trigger/jev_stop_trigger-e2c/acted_kind}{fired}
\defres{mm/stop/trigger/jev_stop_trigger-e2c/cost_k}{40.6}
\defres{mm/stop/trigger/jev_stop_trigger-e2c/cost_ref_k}{40.9}
\defres{mm/stop/trigger/jev_stop_trigger-e2c/delta}{+0.0}
\defres{mm/stop/trigger/jev_stop_trigger-e2c/delta_ci/hi}{+0.0}
\defres{mm/stop/trigger/jev_stop_trigger-e2c/delta_ci/lo}{+0.0}
\defres{mm/stop/trigger/jev_stop_trigger-e2c/fig_delta}{+0.0}
\defres{mm/stop/trigger/jev_stop_trigger-e2c/fig_saving}{1}
\defres{mm/stop/trigger/jev_stop_trigger-e2c/n}{200}
\defres{mm/stop/trigger/jev_stop_trigger-e2c/n_dropped}{0}
\defres{mm/stop/trigger/jev_stop_trigger-e2c/s1_acc}{100.0}
\defres{mm/stop/trigger/jev_stop_trigger-e2c/saving}{0.8}
\defres{mm/stop/trigger/jev_stop_trigger-e2c/saving_ci/hi}{1.5}
\defres{mm/stop/trigger/jev_stop_trigger-e2c/saving_ci/lo}{0.2}
\defres{mm/stop/trigger/jev_stop_trigger-e2c/status}{replicate}
\defres{mm/stop/trigger/jev_stop_trigger-e2c/success}{100.0}
\defres{mm/stop/trigger/jev_stop_trigger-e2c/success_ref}{100.0}
\defres{mm/stop/trigger/jev_stop_trigger-e2c/vcode}{2}
\defres{mm/stop/trigger/jev_stop_trigger-e2c/verdict}{mixed}
\defres{mm/stop/trigger/jev_stop_trigger/acc}{100.0}
\defres{mm/stop/trigger/jev_stop_trigger/accepted_acc}{100.0}
\defres{mm/stop/trigger/jev_stop_trigger/acted}{0.0}
\defres{mm/stop/trigger/jev_stop_trigger/acted_kind}{fired}
\defres{mm/stop/trigger/jev_stop_trigger/cost_k}{40.6}
\defres{mm/stop/trigger/jev_stop_trigger/cost_ref_k}{40.6}
\defres{mm/stop/trigger/jev_stop_trigger/delta}{+0.0}
\defres{mm/stop/trigger/jev_stop_trigger/delta_ci/hi}{+0.0}
\defres{mm/stop/trigger/jev_stop_trigger/delta_ci/lo}{+0.0}
\defres{mm/stop/trigger/jev_stop_trigger/fig_delta}{+0.0}
\defres{mm/stop/trigger/jev_stop_trigger/fig_saving}{0}
\defres{mm/stop/trigger/jev_stop_trigger/n}{200}
\defres{mm/stop/trigger/jev_stop_trigger/n_dropped}{0}
\defres{mm/stop/trigger/jev_stop_trigger/s1_acc}{100.0}
\defres{mm/stop/trigger/jev_stop_trigger/saving}{-0.1}
\defres{mm/stop/trigger/jev_stop_trigger/saving_ci/hi}{0.6}
\defres{mm/stop/trigger/jev_stop_trigger/saving_ci/lo}{-0.7}
\defres{mm/stop/trigger/jev_stop_trigger/status}{descriptive}
\defres{mm/stop/trigger/jev_stop_trigger/success}{100.0}
\defres{mm/stop/trigger/jev_stop_trigger/success_ref}{100.0}
\defres{mm/stop/trigger/jev_stop_trigger/vcode}{3}
\defres{mm/stop/trigger/jev_stop_trigger/verdict}{no saving}
\defres{mm/stop/trigger/rate10_stop_trigger/acc}{89.6}
\defres{mm/stop/trigger/rate10_stop_trigger/accepted_acc}{89.6}
\defres{mm/stop/trigger/rate10_stop_trigger/acted}{10.4}
\defres{mm/stop/trigger/rate10_stop_trigger/acted_kind}{fired}
\defres{mm/stop/trigger/rate10_stop_trigger/cost_k}{29.2}
\defres{mm/stop/trigger/rate10_stop_trigger/cost_ref_k}{40.9}
\defres{mm/stop/trigger/rate10_stop_trigger/delta}{-49.5}
\defres{mm/stop/trigger/rate10_stop_trigger/delta_ci/hi}{-42.5}
\defres{mm/stop/trigger/rate10_stop_trigger/delta_ci/lo}{-56.5}
\defres{mm/stop/trigger/rate10_stop_trigger/fig_delta}{-49.5}
\defres{mm/stop/trigger/rate10_stop_trigger/fig_saving}{29}
\defres{mm/stop/trigger/rate10_stop_trigger/n}{200}
\defres{mm/stop/trigger/rate10_stop_trigger/n_dropped}{0}
\defres{mm/stop/trigger/rate10_stop_trigger/s1_acc}{89.6}
\defres{mm/stop/trigger/rate10_stop_trigger/saving}{28.7}
\defres{mm/stop/trigger/rate10_stop_trigger/saving_ci/hi}{33.2}
\defres{mm/stop/trigger/rate10_stop_trigger/saving_ci/lo}{24.0}
\defres{mm/stop/trigger/rate10_stop_trigger/status}{descriptive}
\defres{mm/stop/trigger/rate10_stop_trigger/success}{50.5}
\defres{mm/stop/trigger/rate10_stop_trigger/success_ref}{100.0}
\defres{mm/stop/trigger/rate10_stop_trigger/vcode}{4}
\defres{mm/stop/trigger/rate10_stop_trigger/verdict}{costs success}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.5/acc}{98.9}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.5/accepted_acc}{98.9}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.5/acted}{78.1}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.5/acted_kind}{decided}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.5/cost_k}{6.6}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.5/cost_ref_k}{42.9}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.5/coverage}{78.1}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.5/delta}{-21.5}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.5/delta_ci/hi}{-16.0}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.5/delta_ci/lo}{-27.5}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.5/fig_delta}{-21.5}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.5/fig_saving}{85}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.5/n}{200}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.5/n_dropped}{0}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.5/s1_acc}{98.5}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.5/saving}{84.5}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.5/saving_ci/hi}{86.4}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.5/saving_ci/lo}{82.0}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.5/status}{descriptive}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.5/success}{78.5}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.5/success_ref}{100.0}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.5/vcode}{4}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.5/verdict}{costs success}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.7/acc}{98.9}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.7/accepted_acc}{98.9}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.7/acted}{77.3}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.7/acted_kind}{decided}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.7/cost_k}{8.2}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.7/cost_ref_k}{42.9}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.7/coverage}{77.3}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.7/delta}{-24.0}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.7/delta_ci/hi}{-18.0}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.7/delta_ci/lo}{-30.0}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.7/fig_delta}{-24.0}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.7/fig_saving}{81}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.7/n}{200}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.7/n_dropped}{0}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.7/s1_acc}{98.5}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.7/saving}{81.0}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.7/saving_ci/hi}{82.1}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.7/saving_ci/lo}{79.5}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.7/status}{descriptive}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.7/success}{76.0}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.7/success_ref}{100.0}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.7/vcode}{4}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.7/verdict}{costs success}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.8/acc}{99.1}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.8/accepted_acc}{99.1}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.8/acted}{74.6}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.8/acted_kind}{decided}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.8/cost_k}{10.1}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.8/cost_ref_k}{42.9}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.8/coverage}{74.6}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.8/delta}{-23.5}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.8/delta_ci/hi}{-18.0}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.8/delta_ci/lo}{-29.5}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.8/fig_delta}{-23.5}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.8/fig_saving}{76}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.8/n}{200}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.8/n_dropped}{0}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.8/s1_acc}{98.7}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.8/saving}{76.5}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.8/saving_ci/hi}{78.1}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.8/saving_ci/lo}{74.5}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.8/status}{descriptive}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.8/success}{76.5}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.8/success_ref}{100.0}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.8/vcode}{4}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.8/verdict}{costs success}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.9/acc}{99.9}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.9/accepted_acc}{99.9}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.9/acted}{73.1}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.9/acted_kind}{decided}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.9/cost_k}{12.0}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.9/cost_ref_k}{42.9}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.9/coverage}{73.1}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.9/delta}{-20.5}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.9/delta_ci/hi}{-15.0}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.9/delta_ci/lo}{-26.5}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.9/fig_delta}{-20.5}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.9/fig_saving}{72}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.9/n}{200}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.9/n_dropped}{0}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.9/s1_acc}{99.6}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.9/saving}{72.0}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.9/saving_ci/hi}{73.5}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.9/saving_ci/lo}{70.3}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.9/status}{descriptive}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.9/success}{79.5}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.9/success_ref}{100.0}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.9/vcode}{4}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.9/verdict}{costs success}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.95/acc}{100.0}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.95/accepted_acc}{100.0}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.95/acted}{68.7}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.95/acted_kind}{decided}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.95/cost_k}{14.3}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.95/cost_ref_k}{42.9}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.95/coverage}{68.7}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.95/delta}{-20.5}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.95/delta_ci/hi}{-15.0}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.95/delta_ci/lo}{-26.0}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.95/fig_delta}{-20.5}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.95/fig_saving}{67}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.95/n}{200}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.95/n_dropped}{0}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.95/s1_acc}{99.8}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.95/saving}{66.8}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.95/saving_ci/hi}{69.0}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.95/saving_ci/lo}{64.5}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.95/status}{descriptive}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.95/success}{79.5}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.95/success_ref}{100.0}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.95/vcode}{4}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.95/verdict}{costs success}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.99/acc}{99.3}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.99/accepted_acc}{99.3}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.99/acted}{41.1}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.99/acted_kind}{decided}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.99/cost_k}{26.1}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.99/cost_ref_k}{42.9}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.99/coverage}{41.1}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.99/delta}{-8.0}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.99/delta_ci/hi}{-4.5}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.99/delta_ci/lo}{-12.0}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.99/fig_delta}{-8.0}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.99/fig_saving}{39}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.99/n}{200}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.99/n_dropped}{0}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.99/s1_acc}{97.6}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.99/saving}{39.3}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.99/saving_ci/hi}{43.0}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.99/saving_ci/lo}{35.7}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.99/status}{descriptive}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.99/success}{92.0}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.99/success_ref}{100.0}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.99/vcode}{4}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.99/verdict}{costs success}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.9_s2lite/acted}{0.0}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.9_s2lite/acted_kind}{decided}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.9_s2lite/cost_k}{9.8}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.9_s2lite/cost_ref_k}{9.8}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.9_s2lite/coverage}{0.0}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.9_s2lite/delta}{+1.0}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.9_s2lite/delta_ci/hi}{+3.2}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.9_s2lite/delta_ci/lo}{-1.0}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.9_s2lite/fig_delta}{+1.0}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.9_s2lite/fig_saving}{0}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.9_s2lite/n}{500}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.9_s2lite/n_dropped}{0}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.9_s2lite/reg}{C1L}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.9_s2lite/saving}{0.2}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.9_s2lite/saving_ci/hi}{0.7}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.9_s2lite/saving_ci/lo}{-0.3}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.9_s2lite/status}{registered}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.9_s2lite/success}{81.2}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.9_s2lite/success_ref}{80.2}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.9_s2lite/vcode}{2}
\defres{mm/tool_params/cascade/jev_ts_cascade_tau0.9_s2lite/verdict}{mixed}
\defres{mm/tool_params/cascade/jev_ts_cascade_tauhat/acc}{100.0}
\defres{mm/tool_params/cascade/jev_ts_cascade_tauhat/accepted_acc}{100.0}
\defres{mm/tool_params/cascade/jev_ts_cascade_tauhat/acted}{20.8}
\defres{mm/tool_params/cascade/jev_ts_cascade_tauhat/acted_kind}{decided}
\defres{mm/tool_params/cascade/jev_ts_cascade_tauhat/cost_k}{36.4}
\defres{mm/tool_params/cascade/jev_ts_cascade_tauhat/cost_ref_k}{42.4}
\defres{mm/tool_params/cascade/jev_ts_cascade_tauhat/coverage}{20.8}
\defres{mm/tool_params/cascade/jev_ts_cascade_tauhat/delta}{+0.0}
\defres{mm/tool_params/cascade/jev_ts_cascade_tauhat/delta_ci/hi}{+0.0}
\defres{mm/tool_params/cascade/jev_ts_cascade_tauhat/delta_ci/lo}{+0.0}
\defres{mm/tool_params/cascade/jev_ts_cascade_tauhat/fig_delta}{+0.0}
\defres{mm/tool_params/cascade/jev_ts_cascade_tauhat/fig_saving}{14}
\defres{mm/tool_params/cascade/jev_ts_cascade_tauhat/fresh/acc}{100.0}
\defres{mm/tool_params/cascade/jev_ts_cascade_tauhat/fresh/accepted_acc}{100.0}
\defres{mm/tool_params/cascade/jev_ts_cascade_tauhat/fresh/acted}{23.1}
\defres{mm/tool_params/cascade/jev_ts_cascade_tauhat/fresh/acted_kind}{decided}
\defres{mm/tool_params/cascade/jev_ts_cascade_tauhat/fresh/cost_k}{33.5}
\defres{mm/tool_params/cascade/jev_ts_cascade_tauhat/fresh/cost_ref_k}{41.3}
\defres{mm/tool_params/cascade/jev_ts_cascade_tauhat/fresh/coverage}{23.1}
\defres{mm/tool_params/cascade/jev_ts_cascade_tauhat/fresh/delta}{+0.4}
\defres{mm/tool_params/cascade/jev_ts_cascade_tauhat/fresh/fig_delta}{+0.4}
\defres{mm/tool_params/cascade/jev_ts_cascade_tauhat/fresh/fig_saving}{19}
\defres{mm/tool_params/cascade/jev_ts_cascade_tauhat/fresh/n}{500}
\defres{mm/tool_params/cascade/jev_ts_cascade_tauhat/fresh/n_dropped}{0}
\defres{mm/tool_params/cascade/jev_ts_cascade_tauhat/fresh/s1_acc}{97.4}
\defres{mm/tool_params/cascade/jev_ts_cascade_tauhat/fresh/saving}{18.8}
\defres{mm/tool_params/cascade/jev_ts_cascade_tauhat/fresh/success}{99.8}
\defres{mm/tool_params/cascade/jev_ts_cascade_tauhat/fresh/success_ref}{99.4}
\defres{mm/tool_params/cascade/jev_ts_cascade_tauhat/fresh/verdict}{takes over safely}
\defres{mm/tool_params/cascade/jev_ts_cascade_tauhat/n}{500}
\defres{mm/tool_params/cascade/jev_ts_cascade_tauhat/n_dropped}{0}
\defres{mm/tool_params/cascade/jev_ts_cascade_tauhat/reg}{C1F}
\defres{mm/tool_params/cascade/jev_ts_cascade_tauhat/s1_acc}{96.1}
\defres{mm/tool_params/cascade/jev_ts_cascade_tauhat/saving}{14.2}
\defres{mm/tool_params/cascade/jev_ts_cascade_tauhat/saving_ci/hi}{15.7}
\defres{mm/tool_params/cascade/jev_ts_cascade_tauhat/saving_ci/lo}{12.7}
\defres{mm/tool_params/cascade/jev_ts_cascade_tauhat/status}{registered}
\defres{mm/tool_params/cascade/jev_ts_cascade_tauhat/success}{99.8}
\defres{mm/tool_params/cascade/jev_ts_cascade_tauhat/success_ref}{99.8}
\defres{mm/tool_params/cascade/jev_ts_cascade_tauhat/vcode}{1}
\defres{mm/tool_params/cascade/jev_ts_cascade_tauhat/verdict}{takes over safely}
\defres{mm/tool_params/cascade/lite_ts_cascade_tau0.7/acc}{96.0}
\defres{mm/tool_params/cascade/lite_ts_cascade_tau0.7/accepted_acc}{96.0}
\defres{mm/tool_params/cascade/lite_ts_cascade_tau0.7/acted}{84.0}
\defres{mm/tool_params/cascade/lite_ts_cascade_tau0.7/acted_kind}{decided}
\defres{mm/tool_params/cascade/lite_ts_cascade_tau0.7/cost_k}{26.7}
\defres{mm/tool_params/cascade/lite_ts_cascade_tau0.7/cost_ref_k}{42.9}
\defres{mm/tool_params/cascade/lite_ts_cascade_tau0.7/coverage}{84.0}
\defres{mm/tool_params/cascade/lite_ts_cascade_tau0.7/delta}{-57.5}
\defres{mm/tool_params/cascade/lite_ts_cascade_tau0.7/delta_ci/hi}{-50.5}
\defres{mm/tool_params/cascade/lite_ts_cascade_tau0.7/delta_ci/lo}{-64.0}
\defres{mm/tool_params/cascade/lite_ts_cascade_tau0.7/fig_delta}{-57.5}
\defres{mm/tool_params/cascade/lite_ts_cascade_tau0.7/fig_saving}{38}
\defres{mm/tool_params/cascade/lite_ts_cascade_tau0.7/n}{200}
\defres{mm/tool_params/cascade/lite_ts_cascade_tau0.7/n_dropped}{0}
\defres{mm/tool_params/cascade/lite_ts_cascade_tau0.7/s1_acc}{94.2}
\defres{mm/tool_params/cascade/lite_ts_cascade_tau0.7/saving}{37.9}
\defres{mm/tool_params/cascade/lite_ts_cascade_tau0.7/saving_ci/hi}{42.9}
\defres{mm/tool_params/cascade/lite_ts_cascade_tau0.7/saving_ci/lo}{32.6}
\defres{mm/tool_params/cascade/lite_ts_cascade_tau0.7/status}{descriptive}
\defres{mm/tool_params/cascade/lite_ts_cascade_tau0.7/success}{42.5}
\defres{mm/tool_params/cascade/lite_ts_cascade_tau0.7/success_ref}{100.0}
\defres{mm/tool_params/cascade/lite_ts_cascade_tau0.7/vcode}{4}
\defres{mm/tool_params/cascade/lite_ts_cascade_tau0.7/verdict}{costs success}
\defres{mm/tool_params/cascade/lite_ts_cascade_tau0.9/acc}{97.7}
\defres{mm/tool_params/cascade/lite_ts_cascade_tau0.9/accepted_acc}{97.7}
\defres{mm/tool_params/cascade/lite_ts_cascade_tau0.9/acted}{83.7}
\defres{mm/tool_params/cascade/lite_ts_cascade_tau0.9/acted_kind}{decided}
\defres{mm/tool_params/cascade/lite_ts_cascade_tau0.9/cost_k}{26.3}
\defres{mm/tool_params/cascade/lite_ts_cascade_tau0.9/cost_ref_k}{42.9}
\defres{mm/tool_params/cascade/lite_ts_cascade_tau0.9/coverage}{83.7}
\defres{mm/tool_params/cascade/lite_ts_cascade_tau0.9/delta}{-56.5}
\defres{mm/tool_params/cascade/lite_ts_cascade_tau0.9/delta_ci/hi}{-49.5}
\defres{mm/tool_params/cascade/lite_ts_cascade_tau0.9/delta_ci/lo}{-63.5}
\defres{mm/tool_params/cascade/lite_ts_cascade_tau0.9/fig_delta}{-56.5}
\defres{mm/tool_params/cascade/lite_ts_cascade_tau0.9/fig_saving}{39}
\defres{mm/tool_params/cascade/lite_ts_cascade_tau0.9/n}{200}
\defres{mm/tool_params/cascade/lite_ts_cascade_tau0.9/n_dropped}{0}
\defres{mm/tool_params/cascade/lite_ts_cascade_tau0.9/s1_acc}{95.7}
\defres{mm/tool_params/cascade/lite_ts_cascade_tau0.9/saving}{38.8}
\defres{mm/tool_params/cascade/lite_ts_cascade_tau0.9/saving_ci/hi}{42.9}
\defres{mm/tool_params/cascade/lite_ts_cascade_tau0.9/saving_ci/lo}{34.7}
\defres{mm/tool_params/cascade/lite_ts_cascade_tau0.9/status}{descriptive}
\defres{mm/tool_params/cascade/lite_ts_cascade_tau0.9/success}{43.5}
\defres{mm/tool_params/cascade/lite_ts_cascade_tau0.9/success_ref}{100.0}
\defres{mm/tool_params/cascade/lite_ts_cascade_tau0.9/vcode}{4}
\defres{mm/tool_params/cascade/lite_ts_cascade_tau0.9/verdict}{costs success}
\defres{mm/tool_params/cascade/lite_ts_cascade_tau0.99/acc}{94.2}
\defres{mm/tool_params/cascade/lite_ts_cascade_tau0.99/accepted_acc}{94.2}
\defres{mm/tool_params/cascade/lite_ts_cascade_tau0.99/acted}{43.7}
\defres{mm/tool_params/cascade/lite_ts_cascade_tau0.99/acted_kind}{decided}
\defres{mm/tool_params/cascade/lite_ts_cascade_tau0.99/cost_k}{43.2}
\defres{mm/tool_params/cascade/lite_ts_cascade_tau0.99/cost_ref_k}{42.9}
\defres{mm/tool_params/cascade/lite_ts_cascade_tau0.99/coverage}{43.7}
\defres{mm/tool_params/cascade/lite_ts_cascade_tau0.99/delta}{-25.0}
\defres{mm/tool_params/cascade/lite_ts_cascade_tau0.99/delta_ci/hi}{-19.0}
\defres{mm/tool_params/cascade/lite_ts_cascade_tau0.99/delta_ci/lo}{-31.0}
\defres{mm/tool_params/cascade/lite_ts_cascade_tau0.99/fig_delta}{-25.0}
\defres{mm/tool_params/cascade/lite_ts_cascade_tau0.99/fig_saving}{-1}
\defres{mm/tool_params/cascade/lite_ts_cascade_tau0.99/n}{200}
\defres{mm/tool_params/cascade/lite_ts_cascade_tau0.99/n_dropped}{0}
\defres{mm/tool_params/cascade/lite_ts_cascade_tau0.99/s1_acc}{91.6}
\defres{mm/tool_params/cascade/lite_ts_cascade_tau0.99/saving}{-0.7}
\defres{mm/tool_params/cascade/lite_ts_cascade_tau0.99/saving_ci/hi}{3.5}
\defres{mm/tool_params/cascade/lite_ts_cascade_tau0.99/saving_ci/lo}{-4.8}
\defres{mm/tool_params/cascade/lite_ts_cascade_tau0.99/status}{descriptive}
\defres{mm/tool_params/cascade/lite_ts_cascade_tau0.99/success}{75.0}
\defres{mm/tool_params/cascade/lite_ts_cascade_tau0.99/success_ref}{100.0}
\defres{mm/tool_params/cascade/lite_ts_cascade_tau0.99/vcode}{4}
\defres{mm/tool_params/cascade/lite_ts_cascade_tau0.99/verdict}{costs success}
\defres{mm/tool_params/replace/jev_ts_params_replace/acc}{98.2}
\defres{mm/tool_params/replace/jev_ts_params_replace/accepted_acc}{98.2}
\defres{mm/tool_params/replace/jev_ts_params_replace/acted}{85.7}
\defres{mm/tool_params/replace/jev_ts_params_replace/acted_kind}{decided}
\defres{mm/tool_params/replace/jev_ts_params_replace/cost_k}{5.1}
\defres{mm/tool_params/replace/jev_ts_params_replace/cost_ref_k}{42.9}
\defres{mm/tool_params/replace/jev_ts_params_replace/coverage}{85.7}
\defres{mm/tool_params/replace/jev_ts_params_replace/delta}{-20.0}
\defres{mm/tool_params/replace/jev_ts_params_replace/delta_ci/hi}{-14.5}
\defres{mm/tool_params/replace/jev_ts_params_replace/delta_ci/lo}{-25.5}
\defres{mm/tool_params/replace/jev_ts_params_replace/fig_delta}{-20.0}
\defres{mm/tool_params/replace/jev_ts_params_replace/fig_saving}{88}
\defres{mm/tool_params/replace/jev_ts_params_replace/n}{200}
\defres{mm/tool_params/replace/jev_ts_params_replace/n_dropped}{0}
\defres{mm/tool_params/replace/jev_ts_params_replace/s1_acc}{98.2}
\defres{mm/tool_params/replace/jev_ts_params_replace/saving}{88.1}
\defres{mm/tool_params/replace/jev_ts_params_replace/saving_ci/hi}{90.0}
\defres{mm/tool_params/replace/jev_ts_params_replace/saving_ci/lo}{85.6}
\defres{mm/tool_params/replace/jev_ts_params_replace/status}{descriptive}
\defres{mm/tool_params/replace/jev_ts_params_replace/success}{80.0}
\defres{mm/tool_params/replace/jev_ts_params_replace/success_ref}{100.0}
\defres{mm/tool_params/replace/jev_ts_params_replace/vcode}{4}
\defres{mm/tool_params/replace/jev_ts_params_replace/verdict}{costs success}
\defres{mm/tool_params/replace/jev_ts_params_replace_answercopy/acc}{98.2}
\defres{mm/tool_params/replace/jev_ts_params_replace_answercopy/accepted_acc}{98.1}
\defres{mm/tool_params/replace/jev_ts_params_replace_answercopy/acted}{84.9}
\defres{mm/tool_params/replace/jev_ts_params_replace_answercopy/acted_kind}{decided}
\defres{mm/tool_params/replace/jev_ts_params_replace_answercopy/cost_k}{5.5}
\defres{mm/tool_params/replace/jev_ts_params_replace_answercopy/cost_ref_k}{40.9}
\defres{mm/tool_params/replace/jev_ts_params_replace_answercopy/coverage}{84.9}
\defres{mm/tool_params/replace/jev_ts_params_replace_answercopy/delta}{-20.0}
\defres{mm/tool_params/replace/jev_ts_params_replace_answercopy/delta_ci/hi}{-14.5}
\defres{mm/tool_params/replace/jev_ts_params_replace_answercopy/delta_ci/lo}{-25.5}
\defres{mm/tool_params/replace/jev_ts_params_replace_answercopy/fig_delta}{-20.0}
\defres{mm/tool_params/replace/jev_ts_params_replace_answercopy/fig_saving}{87}
\defres{mm/tool_params/replace/jev_ts_params_replace_answercopy/n}{200}
\defres{mm/tool_params/replace/jev_ts_params_replace_answercopy/n_dropped}{0}
\defres{mm/tool_params/replace/jev_ts_params_replace_answercopy/s1_acc}{98.2}
\defres{mm/tool_params/replace/jev_ts_params_replace_answercopy/saving}{86.6}
\defres{mm/tool_params/replace/jev_ts_params_replace_answercopy/saving_ci/hi}{89.1}
\defres{mm/tool_params/replace/jev_ts_params_replace_answercopy/saving_ci/lo}{83.4}
\defres{mm/tool_params/replace/jev_ts_params_replace_answercopy/status}{descriptive}
\defres{mm/tool_params/replace/jev_ts_params_replace_answercopy/success}{80.0}
\defres{mm/tool_params/replace/jev_ts_params_replace_answercopy/success_ref}{100.0}
\defres{mm/tool_params/replace/jev_ts_params_replace_answercopy/vcode}{4}
\defres{mm/tool_params/replace/jev_ts_params_replace_answercopy/verdict}{costs success}
\defres{mm/tool_params/replace/lite_ts_params_replace/acc}{91.8}
\defres{mm/tool_params/replace/lite_ts_params_replace/accepted_acc}{91.8}
\defres{mm/tool_params/replace/lite_ts_params_replace/acted}{85.9}
\defres{mm/tool_params/replace/lite_ts_params_replace/acted_kind}{decided}
\defres{mm/tool_params/replace/lite_ts_params_replace/cost_k}{27.1}
\defres{mm/tool_params/replace/lite_ts_params_replace/cost_ref_k}{42.9}
\defres{mm/tool_params/replace/lite_ts_params_replace/coverage}{85.9}
\defres{mm/tool_params/replace/lite_ts_params_replace/delta}{-60.5}
\defres{mm/tool_params/replace/lite_ts_params_replace/delta_ci/hi}{-53.5}
\defres{mm/tool_params/replace/lite_ts_params_replace/delta_ci/lo}{-67.5}
\defres{mm/tool_params/replace/lite_ts_params_replace/fig_delta}{-60.5}
\defres{mm/tool_params/replace/lite_ts_params_replace/fig_saving}{37}
\defres{mm/tool_params/replace/lite_ts_params_replace/n}{200}
\defres{mm/tool_params/replace/lite_ts_params_replace/n_dropped}{0}
\defres{mm/tool_params/replace/lite_ts_params_replace/s1_acc}{91.8}
\defres{mm/tool_params/replace/lite_ts_params_replace/saving}{36.9}
\defres{mm/tool_params/replace/lite_ts_params_replace/saving_ci/hi}{42.7}
\defres{mm/tool_params/replace/lite_ts_params_replace/saving_ci/lo}{30.7}
\defres{mm/tool_params/replace/lite_ts_params_replace/status}{descriptive}
\defres{mm/tool_params/replace/lite_ts_params_replace/success}{39.5}
\defres{mm/tool_params/replace/lite_ts_params_replace/success_ref}{100.0}
\defres{mm/tool_params/replace/lite_ts_params_replace/vcode}{4}
\defres{mm/tool_params/replace/lite_ts_params_replace/verdict}{costs success}
\defres{mm/tool_select/assist/bm25_ts_assist_k3/acc}{16.2}
\defres{mm/tool_select/assist/bm25_ts_assist_k3/accepted_acc}{12.0}
\defres{mm/tool_select/assist/bm25_ts_assist_k3/acted}{100.0}
\defres{mm/tool_select/assist/bm25_ts_assist_k3/acted_kind}{shortlist}
\defres{mm/tool_select/assist/bm25_ts_assist_k3/cost_k}{15.3}
\defres{mm/tool_select/assist/bm25_ts_assist_k3/cost_ref_k}{40.9}
\defres{mm/tool_select/assist/bm25_ts_assist_k3/delta}{-83.0}
\defres{mm/tool_select/assist/bm25_ts_assist_k3/delta_ci/hi}{-77.5}
\defres{mm/tool_select/assist/bm25_ts_assist_k3/delta_ci/lo}{-88.0}
\defres{mm/tool_select/assist/bm25_ts_assist_k3/fig_delta}{-83.0}
\defres{mm/tool_select/assist/bm25_ts_assist_k3/fig_saving}{63}
\defres{mm/tool_select/assist/bm25_ts_assist_k3/n}{200}
\defres{mm/tool_select/assist/bm25_ts_assist_k3/n_dropped}{0}
\defres{mm/tool_select/assist/bm25_ts_assist_k3/recall_k}{16.2}
\defres{mm/tool_select/assist/bm25_ts_assist_k3/s1_acc}{12.0}
\defres{mm/tool_select/assist/bm25_ts_assist_k3/saving}{62.7}
\defres{mm/tool_select/assist/bm25_ts_assist_k3/saving_ci/hi}{70.6}
\defres{mm/tool_select/assist/bm25_ts_assist_k3/saving_ci/lo}{53.8}
\defres{mm/tool_select/assist/bm25_ts_assist_k3/status}{descriptive}
\defres{mm/tool_select/assist/bm25_ts_assist_k3/success}{17.0}
\defres{mm/tool_select/assist/bm25_ts_assist_k3/success_ref}{100.0}
\defres{mm/tool_select/assist/bm25_ts_assist_k3/vcode}{4}
\defres{mm/tool_select/assist/bm25_ts_assist_k3/verdict}{costs success}
\defres{mm/tool_select/assist/bm25_ts_assist_k3_s2lite/acc}{18.8}
\defres{mm/tool_select/assist/bm25_ts_assist_k3_s2lite/accepted_acc}{16.9}
\defres{mm/tool_select/assist/bm25_ts_assist_k3_s2lite/acted}{100.0}
\defres{mm/tool_select/assist/bm25_ts_assist_k3_s2lite/acted_kind}{shortlist}
\defres{mm/tool_select/assist/bm25_ts_assist_k3_s2lite/cost_k}{2.1}
\defres{mm/tool_select/assist/bm25_ts_assist_k3_s2lite/cost_ref_k}{9.8}
\defres{mm/tool_select/assist/bm25_ts_assist_k3_s2lite/delta}{-69.5}
\defres{mm/tool_select/assist/bm25_ts_assist_k3_s2lite/delta_ci/hi}{-63.0}
\defres{mm/tool_select/assist/bm25_ts_assist_k3_s2lite/delta_ci/lo}{-76.0}
\defres{mm/tool_select/assist/bm25_ts_assist_k3_s2lite/fig_delta}{-69.5}
\defres{mm/tool_select/assist/bm25_ts_assist_k3_s2lite/fig_saving}{79}
\defres{mm/tool_select/assist/bm25_ts_assist_k3_s2lite/n}{200}
\defres{mm/tool_select/assist/bm25_ts_assist_k3_s2lite/n_dropped}{0}
\defres{mm/tool_select/assist/bm25_ts_assist_k3_s2lite/recall_k}{18.8}
\defres{mm/tool_select/assist/bm25_ts_assist_k3_s2lite/s1_acc}{16.9}
\defres{mm/tool_select/assist/bm25_ts_assist_k3_s2lite/saving}{79.0}
\defres{mm/tool_select/assist/bm25_ts_assist_k3_s2lite/saving_ci/hi}{83.6}
\defres{mm/tool_select/assist/bm25_ts_assist_k3_s2lite/saving_ci/lo}{73.8}
\defres{mm/tool_select/assist/bm25_ts_assist_k3_s2lite/status}{descriptive}
\defres{mm/tool_select/assist/bm25_ts_assist_k3_s2lite/success}{12.5}
\defres{mm/tool_select/assist/bm25_ts_assist_k3_s2lite/success_ref}{82.0}
\defres{mm/tool_select/assist/bm25_ts_assist_k3_s2lite/vcode}{4}
\defres{mm/tool_select/assist/bm25_ts_assist_k3_s2lite/verdict}{costs success}
\defres{mm/tool_select/assist/bm25_ts_assist_k5/acc}{18.7}
\defres{mm/tool_select/assist/bm25_ts_assist_k5/accepted_acc}{11.6}
\defres{mm/tool_select/assist/bm25_ts_assist_k5/acted}{100.0}
\defres{mm/tool_select/assist/bm25_ts_assist_k5/acted_kind}{shortlist}
\defres{mm/tool_select/assist/bm25_ts_assist_k5/cost_k}{16.3}
\defres{mm/tool_select/assist/bm25_ts_assist_k5/cost_ref_k}{40.9}
\defres{mm/tool_select/assist/bm25_ts_assist_k5/delta}{-81.5}
\defres{mm/tool_select/assist/bm25_ts_assist_k5/delta_ci/hi}{-76.0}
\defres{mm/tool_select/assist/bm25_ts_assist_k5/delta_ci/lo}{-86.5}
\defres{mm/tool_select/assist/bm25_ts_assist_k5/fig_delta}{-81.5}
\defres{mm/tool_select/assist/bm25_ts_assist_k5/fig_saving}{60}
\defres{mm/tool_select/assist/bm25_ts_assist_k5/n}{200}
\defres{mm/tool_select/assist/bm25_ts_assist_k5/n_dropped}{0}
\defres{mm/tool_select/assist/bm25_ts_assist_k5/recall_k}{18.7}
\defres{mm/tool_select/assist/bm25_ts_assist_k5/s1_acc}{11.6}
\defres{mm/tool_select/assist/bm25_ts_assist_k5/saving}{60.1}
\defres{mm/tool_select/assist/bm25_ts_assist_k5/saving_ci/hi}{67.7}
\defres{mm/tool_select/assist/bm25_ts_assist_k5/saving_ci/lo}{51.7}
\defres{mm/tool_select/assist/bm25_ts_assist_k5/status}{descriptive}
\defres{mm/tool_select/assist/bm25_ts_assist_k5/success}{18.5}
\defres{mm/tool_select/assist/bm25_ts_assist_k5/success_ref}{100.0}
\defres{mm/tool_select/assist/bm25_ts_assist_k5/vcode}{4}
\defres{mm/tool_select/assist/bm25_ts_assist_k5/verdict}{costs success}
\defres{mm/tool_select/assist/bm25task_ts_assist_k3/acc}{10.7}
\defres{mm/tool_select/assist/bm25task_ts_assist_k3/accepted_acc}{8.1}
\defres{mm/tool_select/assist/bm25task_ts_assist_k3/acted}{100.0}
\defres{mm/tool_select/assist/bm25task_ts_assist_k3/acted_kind}{shortlist}
\defres{mm/tool_select/assist/bm25task_ts_assist_k3/cost_k}{15.0}
\defres{mm/tool_select/assist/bm25task_ts_assist_k3/cost_ref_k}{40.9}
\defres{mm/tool_select/assist/bm25task_ts_assist_k3/delta}{-75.5}
\defres{mm/tool_select/assist/bm25task_ts_assist_k3/delta_ci/hi}{-69.5}
\defres{mm/tool_select/assist/bm25task_ts_assist_k3/delta_ci/lo}{-81.5}
\defres{mm/tool_select/assist/bm25task_ts_assist_k3/fig_delta}{-75.5}
\defres{mm/tool_select/assist/bm25task_ts_assist_k3/fig_saving}{63}
\defres{mm/tool_select/assist/bm25task_ts_assist_k3/n}{200}
\defres{mm/tool_select/assist/bm25task_ts_assist_k3/n_dropped}{0}
\defres{mm/tool_select/assist/bm25task_ts_assist_k3/recall_k}{10.7}
\defres{mm/tool_select/assist/bm25task_ts_assist_k3/s1_acc}{8.1}
\defres{mm/tool_select/assist/bm25task_ts_assist_k3/saving}{63.5}
\defres{mm/tool_select/assist/bm25task_ts_assist_k3/saving_ci/hi}{69.4}
\defres{mm/tool_select/assist/bm25task_ts_assist_k3/saving_ci/lo}{56.9}
\defres{mm/tool_select/assist/bm25task_ts_assist_k3/status}{descriptive}
\defres{mm/tool_select/assist/bm25task_ts_assist_k3/success}{24.5}
\defres{mm/tool_select/assist/bm25task_ts_assist_k3/success_ref}{100.0}
\defres{mm/tool_select/assist/bm25task_ts_assist_k3/vcode}{4}
\defres{mm/tool_select/assist/bm25task_ts_assist_k3/verdict}{costs success}
\defres{mm/tool_select/assist/embed_ts_assist_k3-e2c/acc}{24.8}
\defres{mm/tool_select/assist/embed_ts_assist_k3-e2c/accepted_acc}{12.5}
\defres{mm/tool_select/assist/embed_ts_assist_k3-e2c/acted}{100.0}
\defres{mm/tool_select/assist/embed_ts_assist_k3-e2c/acted_kind}{shortlist}
\defres{mm/tool_select/assist/embed_ts_assist_k3-e2c/cost_k}{9.7}
\defres{mm/tool_select/assist/embed_ts_assist_k3-e2c/cost_ref_k}{40.9}
\defres{mm/tool_select/assist/embed_ts_assist_k3-e2c/delta}{-70.0}
\defres{mm/tool_select/assist/embed_ts_assist_k3-e2c/delta_ci/hi}{-63.5}
\defres{mm/tool_select/assist/embed_ts_assist_k3-e2c/delta_ci/lo}{-76.0}
\defres{mm/tool_select/assist/embed_ts_assist_k3-e2c/fig_delta}{-70.0}
\defres{mm/tool_select/assist/embed_ts_assist_k3-e2c/fig_saving}{76}
\defres{mm/tool_select/assist/embed_ts_assist_k3-e2c/n}{200}
\defres{mm/tool_select/assist/embed_ts_assist_k3-e2c/n_dropped}{0}
\defres{mm/tool_select/assist/embed_ts_assist_k3-e2c/recall_k}{24.8}
\defres{mm/tool_select/assist/embed_ts_assist_k3-e2c/s1_acc}{12.5}
\defres{mm/tool_select/assist/embed_ts_assist_k3-e2c/saving}{76.2}
\defres{mm/tool_select/assist/embed_ts_assist_k3-e2c/saving_ci/hi}{79.6}
\defres{mm/tool_select/assist/embed_ts_assist_k3-e2c/saving_ci/lo}{72.4}
\defres{mm/tool_select/assist/embed_ts_assist_k3-e2c/status}{replicate}
\defres{mm/tool_select/assist/embed_ts_assist_k3-e2c/success}{30.0}
\defres{mm/tool_select/assist/embed_ts_assist_k3-e2c/success_ref}{100.0}
\defres{mm/tool_select/assist/embed_ts_assist_k3-e2c/vcode}{4}
\defres{mm/tool_select/assist/embed_ts_assist_k3-e2c/verdict}{costs success}
\defres{mm/tool_select/assist/embed_ts_assist_k3/acc}{25.4}
\defres{mm/tool_select/assist/embed_ts_assist_k3/accepted_acc}{12.8}
\defres{mm/tool_select/assist/embed_ts_assist_k3/acted}{100.0}
\defres{mm/tool_select/assist/embed_ts_assist_k3/acted_kind}{shortlist}
\defres{mm/tool_select/assist/embed_ts_assist_k3/cost_k}{9.2}
\defres{mm/tool_select/assist/embed_ts_assist_k3/cost_ref_k}{42.9}
\defres{mm/tool_select/assist/embed_ts_assist_k3/delta}{-72.0}
\defres{mm/tool_select/assist/embed_ts_assist_k3/delta_ci/hi}{-65.5}
\defres{mm/tool_select/assist/embed_ts_assist_k3/delta_ci/lo}{-78.0}
\defres{mm/tool_select/assist/embed_ts_assist_k3/fig_delta}{-72.0}
\defres{mm/tool_select/assist/embed_ts_assist_k3/fig_saving}{78}
\defres{mm/tool_select/assist/embed_ts_assist_k3/n}{200}
\defres{mm/tool_select/assist/embed_ts_assist_k3/n_dropped}{0}
\defres{mm/tool_select/assist/embed_ts_assist_k3/recall_k}{25.4}
\defres{mm/tool_select/assist/embed_ts_assist_k3/s1_acc}{12.8}
\defres{mm/tool_select/assist/embed_ts_assist_k3/saving}{78.5}
\defres{mm/tool_select/assist/embed_ts_assist_k3/saving_ci/hi}{81.6}
\defres{mm/tool_select/assist/embed_ts_assist_k3/saving_ci/lo}{75.2}
\defres{mm/tool_select/assist/embed_ts_assist_k3/status}{descriptive}
\defres{mm/tool_select/assist/embed_ts_assist_k3/success}{28.0}
\defres{mm/tool_select/assist/embed_ts_assist_k3/success_ref}{100.0}
\defres{mm/tool_select/assist/embed_ts_assist_k3/vcode}{4}
\defres{mm/tool_select/assist/embed_ts_assist_k3/verdict}{costs success}
\defres{mm/tool_select/assist/heuristic_ts_assist_k3/acc}{13.7}
\defres{mm/tool_select/assist/heuristic_ts_assist_k3/accepted_acc}{10.6}
\defres{mm/tool_select/assist/heuristic_ts_assist_k3/acted}{100.0}
\defres{mm/tool_select/assist/heuristic_ts_assist_k3/acted_kind}{shortlist}
\defres{mm/tool_select/assist/heuristic_ts_assist_k3/cost_k}{18.1}
\defres{mm/tool_select/assist/heuristic_ts_assist_k3/cost_ref_k}{40.9}
\defres{mm/tool_select/assist/heuristic_ts_assist_k3/delta}{-69.0}
\defres{mm/tool_select/assist/heuristic_ts_assist_k3/delta_ci/hi}{-62.5}
\defres{mm/tool_select/assist/heuristic_ts_assist_k3/delta_ci/lo}{-75.5}
\defres{mm/tool_select/assist/heuristic_ts_assist_k3/fig_delta}{-69.0}
\defres{mm/tool_select/assist/heuristic_ts_assist_k3/fig_saving}{56}
\defres{mm/tool_select/assist/heuristic_ts_assist_k3/n}{200}
\defres{mm/tool_select/assist/heuristic_ts_assist_k3/n_dropped}{0}
\defres{mm/tool_select/assist/heuristic_ts_assist_k3/recall_k}{13.7}
\defres{mm/tool_select/assist/heuristic_ts_assist_k3/s1_acc}{10.6}
\defres{mm/tool_select/assist/heuristic_ts_assist_k3/saving}{55.8}
\defres{mm/tool_select/assist/heuristic_ts_assist_k3/saving_ci/hi}{63.8}
\defres{mm/tool_select/assist/heuristic_ts_assist_k3/saving_ci/lo}{46.9}
\defres{mm/tool_select/assist/heuristic_ts_assist_k3/status}{descriptive}
\defres{mm/tool_select/assist/heuristic_ts_assist_k3/success}{31.0}
\defres{mm/tool_select/assist/heuristic_ts_assist_k3/success_ref}{100.0}
\defres{mm/tool_select/assist/heuristic_ts_assist_k3/vcode}{4}
\defres{mm/tool_select/assist/heuristic_ts_assist_k3/verdict}{costs success}
\defres{mm/tool_select/assist/jev_ts_assist_k3-e2c/acc}{94.1}
\defres{mm/tool_select/assist/jev_ts_assist_k3-e2c/accepted_acc}{89.3}
\defres{mm/tool_select/assist/jev_ts_assist_k3-e2c/acted}{100.0}
\defres{mm/tool_select/assist/jev_ts_assist_k3-e2c/acted_kind}{shortlist}
\defres{mm/tool_select/assist/jev_ts_assist_k3-e2c/cost_k}{19.5}
\defres{mm/tool_select/assist/jev_ts_assist_k3-e2c/cost_ref_k}{40.9}
\defres{mm/tool_select/assist/jev_ts_assist_k3-e2c/delta}{-9.5}
\defres{mm/tool_select/assist/jev_ts_assist_k3-e2c/delta_ci/hi}{-5.5}
\defres{mm/tool_select/assist/jev_ts_assist_k3-e2c/delta_ci/lo}{-14.0}
\defres{mm/tool_select/assist/jev_ts_assist_k3-e2c/fig_delta}{-9.5}
\defres{mm/tool_select/assist/jev_ts_assist_k3-e2c/fig_saving}{52}
\defres{mm/tool_select/assist/jev_ts_assist_k3-e2c/n}{200}
\defres{mm/tool_select/assist/jev_ts_assist_k3-e2c/n_dropped}{0}
\defres{mm/tool_select/assist/jev_ts_assist_k3-e2c/recall_k}{94.1}
\defres{mm/tool_select/assist/jev_ts_assist_k3-e2c/s1_acc}{89.3}
\defres{mm/tool_select/assist/jev_ts_assist_k3-e2c/saving}{52.3}
\defres{mm/tool_select/assist/jev_ts_assist_k3-e2c/saving_ci/hi}{53.8}
\defres{mm/tool_select/assist/jev_ts_assist_k3-e2c/saving_ci/lo}{50.7}
\defres{mm/tool_select/assist/jev_ts_assist_k3-e2c/status}{replicate}
\defres{mm/tool_select/assist/jev_ts_assist_k3-e2c/success}{90.5}
\defres{mm/tool_select/assist/jev_ts_assist_k3-e2c/success_ref}{100.0}
\defres{mm/tool_select/assist/jev_ts_assist_k3-e2c/vcode}{4}
\defres{mm/tool_select/assist/jev_ts_assist_k3-e2c/verdict}{costs success}
\defres{mm/tool_select/assist/jev_ts_assist_k3/acc}{94.6}
\defres{mm/tool_select/assist/jev_ts_assist_k3/accepted_acc}{89.6}
\defres{mm/tool_select/assist/jev_ts_assist_k3/acted}{100.0}
\defres{mm/tool_select/assist/jev_ts_assist_k3/acted_kind}{shortlist}
\defres{mm/tool_select/assist/jev_ts_assist_k3/cost_k}{19.6}
\defres{mm/tool_select/assist/jev_ts_assist_k3/cost_ref_k}{42.4}
\defres{mm/tool_select/assist/jev_ts_assist_k3/delta}{-7.8}
\defres{mm/tool_select/assist/jev_ts_assist_k3/delta_ci/hi}{-5.4}
\defres{mm/tool_select/assist/jev_ts_assist_k3/delta_ci/lo}{-10.2}
\defres{mm/tool_select/assist/jev_ts_assist_k3/fig_delta}{-7.8}
\defres{mm/tool_select/assist/jev_ts_assist_k3/fig_saving}{54}
\defres{mm/tool_select/assist/jev_ts_assist_k3/n}{500}
\defres{mm/tool_select/assist/jev_ts_assist_k3/n_dropped}{0}
\defres{mm/tool_select/assist/jev_ts_assist_k3/recall_k}{94.6}
\defres{mm/tool_select/assist/jev_ts_assist_k3/reg}{C2F, C3}
\defres{mm/tool_select/assist/jev_ts_assist_k3/s1_acc}{89.6}
\defres{mm/tool_select/assist/jev_ts_assist_k3/saving}{53.7}
\defres{mm/tool_select/assist/jev_ts_assist_k3/saving_ci/hi}{54.6}
\defres{mm/tool_select/assist/jev_ts_assist_k3/saving_ci/lo}{52.8}
\defres{mm/tool_select/assist/jev_ts_assist_k3/status}{registered}
\defres{mm/tool_select/assist/jev_ts_assist_k3/success}{92.0}
\defres{mm/tool_select/assist/jev_ts_assist_k3/success_ref}{99.8}
\defres{mm/tool_select/assist/jev_ts_assist_k3/vcode}{4}
\defres{mm/tool_select/assist/jev_ts_assist_k3/verdict}{costs success}
\defres{mm/tool_select/assist/jev_ts_assist_k3_s2lite/acc}{94.8}
\defres{mm/tool_select/assist/jev_ts_assist_k3_s2lite/accepted_acc}{91.3}
\defres{mm/tool_select/assist/jev_ts_assist_k3_s2lite/acted}{100.0}
\defres{mm/tool_select/assist/jev_ts_assist_k3_s2lite/acted_kind}{shortlist}
\defres{mm/tool_select/assist/jev_ts_assist_k3_s2lite/cost_k}{4.7}
\defres{mm/tool_select/assist/jev_ts_assist_k3_s2lite/cost_ref_k}{9.8}
\defres{mm/tool_select/assist/jev_ts_assist_k3_s2lite/delta}{-3.4}
\defres{mm/tool_select/assist/jev_ts_assist_k3_s2lite/delta_ci/hi}{+0.6}
\defres{mm/tool_select/assist/jev_ts_assist_k3_s2lite/delta_ci/lo}{-7.2}
\defres{mm/tool_select/assist/jev_ts_assist_k3_s2lite/fig_delta}{-3.4}
\defres{mm/tool_select/assist/jev_ts_assist_k3_s2lite/fig_saving}{52}
\defres{mm/tool_select/assist/jev_ts_assist_k3_s2lite/n}{500}
\defres{mm/tool_select/assist/jev_ts_assist_k3_s2lite/n_dropped}{0}
\defres{mm/tool_select/assist/jev_ts_assist_k3_s2lite/recall_k}{94.8}
\defres{mm/tool_select/assist/jev_ts_assist_k3_s2lite/reg}{C2L}
\defres{mm/tool_select/assist/jev_ts_assist_k3_s2lite/s1_acc}{91.3}
\defres{mm/tool_select/assist/jev_ts_assist_k3_s2lite/saving}{52.0}
\defres{mm/tool_select/assist/jev_ts_assist_k3_s2lite/saving_ci/hi}{52.7}
\defres{mm/tool_select/assist/jev_ts_assist_k3_s2lite/saving_ci/lo}{51.2}
\defres{mm/tool_select/assist/jev_ts_assist_k3_s2lite/status}{registered}
\defres{mm/tool_select/assist/jev_ts_assist_k3_s2lite/success}{76.8}
\defres{mm/tool_select/assist/jev_ts_assist_k3_s2lite/success_ref}{80.2}
\defres{mm/tool_select/assist/jev_ts_assist_k3_s2lite/vcode}{4}
\defres{mm/tool_select/assist/jev_ts_assist_k3_s2lite/verdict}{costs success}
\defres{mm/tool_select/assist/jev_ts_assist_k5-e2c/acc}{96.4}
\defres{mm/tool_select/assist/jev_ts_assist_k5-e2c/accepted_acc}{86.7}
\defres{mm/tool_select/assist/jev_ts_assist_k5-e2c/acted}{100.0}
\defres{mm/tool_select/assist/jev_ts_assist_k5-e2c/acted_kind}{shortlist}
\defres{mm/tool_select/assist/jev_ts_assist_k5-e2c/cost_k}{22.4}
\defres{mm/tool_select/assist/jev_ts_assist_k5-e2c/cost_ref_k}{40.9}
\defres{mm/tool_select/assist/jev_ts_assist_k5-e2c/delta}{-8.0}
\defres{mm/tool_select/assist/jev_ts_assist_k5-e2c/delta_ci/hi}{-4.5}
\defres{mm/tool_select/assist/jev_ts_assist_k5-e2c/delta_ci/lo}{-12.0}
\defres{mm/tool_select/assist/jev_ts_assist_k5-e2c/fig_delta}{-8.0}
\defres{mm/tool_select/assist/jev_ts_assist_k5-e2c/fig_saving}{45}
\defres{mm/tool_select/assist/jev_ts_assist_k5-e2c/n}{200}
\defres{mm/tool_select/assist/jev_ts_assist_k5-e2c/n_dropped}{0}
\defres{mm/tool_select/assist/jev_ts_assist_k5-e2c/recall_k}{96.4}
\defres{mm/tool_select/assist/jev_ts_assist_k5-e2c/s1_acc}{86.7}
\defres{mm/tool_select/assist/jev_ts_assist_k5-e2c/saving}{45.2}
\defres{mm/tool_select/assist/jev_ts_assist_k5-e2c/saving_ci/hi}{47.3}
\defres{mm/tool_select/assist/jev_ts_assist_k5-e2c/saving_ci/lo}{42.8}
\defres{mm/tool_select/assist/jev_ts_assist_k5-e2c/status}{replicate}
\defres{mm/tool_select/assist/jev_ts_assist_k5-e2c/success}{92.0}
\defres{mm/tool_select/assist/jev_ts_assist_k5-e2c/success_ref}{100.0}
\defres{mm/tool_select/assist/jev_ts_assist_k5-e2c/vcode}{4}
\defres{mm/tool_select/assist/jev_ts_assist_k5-e2c/verdict}{costs success}
\defres{mm/tool_select/assist/jev_ts_assist_k5/acc}{96.2}
\defres{mm/tool_select/assist/jev_ts_assist_k5/accepted_acc}{87.6}
\defres{mm/tool_select/assist/jev_ts_assist_k5/acted}{100.0}
\defres{mm/tool_select/assist/jev_ts_assist_k5/acted_kind}{shortlist}
\defres{mm/tool_select/assist/jev_ts_assist_k5/cost_k}{22.2}
\defres{mm/tool_select/assist/jev_ts_assist_k5/cost_ref_k}{42.9}
\defres{mm/tool_select/assist/jev_ts_assist_k5/delta}{-10.0}
\defres{mm/tool_select/assist/jev_ts_assist_k5/delta_ci/hi}{-6.0}
\defres{mm/tool_select/assist/jev_ts_assist_k5/delta_ci/lo}{-14.5}
\defres{mm/tool_select/assist/jev_ts_assist_k5/fig_delta}{-10.0}
\defres{mm/tool_select/assist/jev_ts_assist_k5/fig_saving}{48}
\defres{mm/tool_select/assist/jev_ts_assist_k5/n}{200}
\defres{mm/tool_select/assist/jev_ts_assist_k5/n_dropped}{0}
\defres{mm/tool_select/assist/jev_ts_assist_k5/recall_k}{96.2}
\defres{mm/tool_select/assist/jev_ts_assist_k5/s1_acc}{87.6}
\defres{mm/tool_select/assist/jev_ts_assist_k5/saving}{48.3}
\defres{mm/tool_select/assist/jev_ts_assist_k5/saving_ci/hi}{50.1}
\defres{mm/tool_select/assist/jev_ts_assist_k5/saving_ci/lo}{46.3}
\defres{mm/tool_select/assist/jev_ts_assist_k5/status}{descriptive}
\defres{mm/tool_select/assist/jev_ts_assist_k5/success}{90.0}
\defres{mm/tool_select/assist/jev_ts_assist_k5/success_ref}{100.0}
\defres{mm/tool_select/assist/jev_ts_assist_k5/vcode}{4}
\defres{mm/tool_select/assist/jev_ts_assist_k5/verdict}{costs success}
\defres{mm/tool_select/assist/lite_ts_assist_k3-e2c/acc}{88.0}
\defres{mm/tool_select/assist/lite_ts_assist_k3-e2c/accepted_acc}{85.3}
\defres{mm/tool_select/assist/lite_ts_assist_k3-e2c/acted}{100.0}
\defres{mm/tool_select/assist/lite_ts_assist_k3-e2c/acted_kind}{shortlist}
\defres{mm/tool_select/assist/lite_ts_assist_k3-e2c/cost_k}{36.8}
\defres{mm/tool_select/assist/lite_ts_assist_k3-e2c/cost_ref_k}{40.9}
\defres{mm/tool_select/assist/lite_ts_assist_k3-e2c/delta}{-13.5}
\defres{mm/tool_select/assist/lite_ts_assist_k3-e2c/delta_ci/hi}{-9.0}
\defres{mm/tool_select/assist/lite_ts_assist_k3-e2c/delta_ci/lo}{-18.5}
\defres{mm/tool_select/assist/lite_ts_assist_k3-e2c/fig_delta}{-13.5}
\defres{mm/tool_select/assist/lite_ts_assist_k3-e2c/fig_saving}{10}
\defres{mm/tool_select/assist/lite_ts_assist_k3-e2c/n}{200}
\defres{mm/tool_select/assist/lite_ts_assist_k3-e2c/n_dropped}{0}
\defres{mm/tool_select/assist/lite_ts_assist_k3-e2c/recall_k}{88.0}
\defres{mm/tool_select/assist/lite_ts_assist_k3-e2c/s1_acc}{85.3}
\defres{mm/tool_select/assist/lite_ts_assist_k3-e2c/saving}{10.2}
\defres{mm/tool_select/assist/lite_ts_assist_k3-e2c/saving_ci/hi}{13.8}
\defres{mm/tool_select/assist/lite_ts_assist_k3-e2c/saving_ci/lo}{6.5}
\defres{mm/tool_select/assist/lite_ts_assist_k3-e2c/status}{replicate}
\defres{mm/tool_select/assist/lite_ts_assist_k3-e2c/success}{86.5}
\defres{mm/tool_select/assist/lite_ts_assist_k3-e2c/success_ref}{100.0}
\defres{mm/tool_select/assist/lite_ts_assist_k3-e2c/vcode}{4}
\defres{mm/tool_select/assist/lite_ts_assist_k3-e2c/verdict}{costs success}
\defres{mm/tool_select/assist/lite_ts_assist_k3/acc}{89.3}
\defres{mm/tool_select/assist/lite_ts_assist_k3/accepted_acc}{86.1}
\defres{mm/tool_select/assist/lite_ts_assist_k3/acted}{100.0}
\defres{mm/tool_select/assist/lite_ts_assist_k3/acted_kind}{shortlist}
\defres{mm/tool_select/assist/lite_ts_assist_k3/cost_k}{36.7}
\defres{mm/tool_select/assist/lite_ts_assist_k3/cost_ref_k}{42.9}
\defres{mm/tool_select/assist/lite_ts_assist_k3/delta}{-12.5}
\defres{mm/tool_select/assist/lite_ts_assist_k3/delta_ci/hi}{-8.0}
\defres{mm/tool_select/assist/lite_ts_assist_k3/delta_ci/lo}{-17.5}
\defres{mm/tool_select/assist/lite_ts_assist_k3/fig_delta}{-12.5}
\defres{mm/tool_select/assist/lite_ts_assist_k3/fig_saving}{15}
\defres{mm/tool_select/assist/lite_ts_assist_k3/n}{200}
\defres{mm/tool_select/assist/lite_ts_assist_k3/n_dropped}{0}
\defres{mm/tool_select/assist/lite_ts_assist_k3/recall_k}{89.3}
\defres{mm/tool_select/assist/lite_ts_assist_k3/s1_acc}{86.1}
\defres{mm/tool_select/assist/lite_ts_assist_k3/saving}{14.6}
\defres{mm/tool_select/assist/lite_ts_assist_k3/saving_ci/hi}{17.8}
\defres{mm/tool_select/assist/lite_ts_assist_k3/saving_ci/lo}{11.5}
\defres{mm/tool_select/assist/lite_ts_assist_k3/status}{descriptive}
\defres{mm/tool_select/assist/lite_ts_assist_k3/success}{87.5}
\defres{mm/tool_select/assist/lite_ts_assist_k3/success_ref}{100.0}
\defres{mm/tool_select/assist/lite_ts_assist_k3/vcode}{4}
\defres{mm/tool_select/assist/lite_ts_assist_k3/verdict}{costs success}
\defres{mm/tool_select/assist/random_ts_assist_k3/acc}{6.5}
\defres{mm/tool_select/assist/random_ts_assist_k3/accepted_acc}{2.2}
\defres{mm/tool_select/assist/random_ts_assist_k3/acted}{100.0}
\defres{mm/tool_select/assist/random_ts_assist_k3/acted_kind}{shortlist}
\defres{mm/tool_select/assist/random_ts_assist_k3/cost_k}{35.8}
\defres{mm/tool_select/assist/random_ts_assist_k3/cost_ref_k}{40.9}
\defres{mm/tool_select/assist/random_ts_assist_k3/delta}{-94.0}
\defres{mm/tool_select/assist/random_ts_assist_k3/delta_ci/hi}{-90.5}
\defres{mm/tool_select/assist/random_ts_assist_k3/delta_ci/lo}{-97.0}
\defres{mm/tool_select/assist/random_ts_assist_k3/fig_delta}{-94.0}
\defres{mm/tool_select/assist/random_ts_assist_k3/fig_saving}{13}
\defres{mm/tool_select/assist/random_ts_assist_k3/n}{200}
\defres{mm/tool_select/assist/random_ts_assist_k3/n_dropped}{0}
\defres{mm/tool_select/assist/random_ts_assist_k3/recall_k}{6.5}
\defres{mm/tool_select/assist/random_ts_assist_k3/s1_acc}{2.2}
\defres{mm/tool_select/assist/random_ts_assist_k3/saving}{12.5}
\defres{mm/tool_select/assist/random_ts_assist_k3/saving_ci/hi}{23.8}
\defres{mm/tool_select/assist/random_ts_assist_k3/saving_ci/lo}{0.8}
\defres{mm/tool_select/assist/random_ts_assist_k3/status}{descriptive}
\defres{mm/tool_select/assist/random_ts_assist_k3/success}{6.0}
\defres{mm/tool_select/assist/random_ts_assist_k3/success_ref}{100.0}
\defres{mm/tool_select/assist/random_ts_assist_k3/vcode}{4}
\defres{mm/tool_select/assist/random_ts_assist_k3/verdict}{costs success}
\defres{mm/tool_select/assist/s2self_ts_assist_k3/acc}{92.8}
\defres{mm/tool_select/assist/s2self_ts_assist_k3/accepted_acc}{91.5}
\defres{mm/tool_select/assist/s2self_ts_assist_k3/acted}{100.0}
\defres{mm/tool_select/assist/s2self_ts_assist_k3/acted_kind}{shortlist}
\defres{mm/tool_select/assist/s2self_ts_assist_k3/cost_k}{107.2}
\defres{mm/tool_select/assist/s2self_ts_assist_k3/cost_ref_k}{40.9}
\defres{mm/tool_select/assist/s2self_ts_assist_k3/delta}{-5.5}
\defres{mm/tool_select/assist/s2self_ts_assist_k3/delta_ci/hi}{-2.5}
\defres{mm/tool_select/assist/s2self_ts_assist_k3/delta_ci/lo}{-9.0}
\defres{mm/tool_select/assist/s2self_ts_assist_k3/fig_delta}{-5.5}
\defres{mm/tool_select/assist/s2self_ts_assist_k3/fig_saving}{-162}
\defres{mm/tool_select/assist/s2self_ts_assist_k3/n}{200}
\defres{mm/tool_select/assist/s2self_ts_assist_k3/n_dropped}{0}
\defres{mm/tool_select/assist/s2self_ts_assist_k3/recall_k}{92.8}
\defres{mm/tool_select/assist/s2self_ts_assist_k3/s1_acc}{91.5}
\defres{mm/tool_select/assist/s2self_ts_assist_k3/saving}{-161.9}
\defres{mm/tool_select/assist/s2self_ts_assist_k3/saving_ci/hi}{-153.8}
\defres{mm/tool_select/assist/s2self_ts_assist_k3/saving_ci/lo}{-170.8}
\defres{mm/tool_select/assist/s2self_ts_assist_k3/status}{descriptive}
\defres{mm/tool_select/assist/s2self_ts_assist_k3/success}{94.5}
\defres{mm/tool_select/assist/s2self_ts_assist_k3/success_ref}{100.0}
\defres{mm/tool_select/assist/s2self_ts_assist_k3/vcode}{4}
\defres{mm/tool_select/assist/s2self_ts_assist_k3/verdict}{costs success}
\defres{mm/tool_select/assist/tfidf_ts_assist_k3/acc}{28.8}
\defres{mm/tool_select/assist/tfidf_ts_assist_k3/accepted_acc}{15.6}
\defres{mm/tool_select/assist/tfidf_ts_assist_k3/acted}{100.0}
\defres{mm/tool_select/assist/tfidf_ts_assist_k3/acted_kind}{shortlist}
\defres{mm/tool_select/assist/tfidf_ts_assist_k3/cost_k}{13.4}
\defres{mm/tool_select/assist/tfidf_ts_assist_k3/cost_ref_k}{40.9}
\defres{mm/tool_select/assist/tfidf_ts_assist_k3/delta}{-67.0}
\defres{mm/tool_select/assist/tfidf_ts_assist_k3/delta_ci/hi}{-60.5}
\defres{mm/tool_select/assist/tfidf_ts_assist_k3/delta_ci/lo}{-73.5}
\defres{mm/tool_select/assist/tfidf_ts_assist_k3/fig_delta}{-67.0}
\defres{mm/tool_select/assist/tfidf_ts_assist_k3/fig_saving}{67}
\defres{mm/tool_select/assist/tfidf_ts_assist_k3/n}{200}
\defres{mm/tool_select/assist/tfidf_ts_assist_k3/n_dropped}{0}
\defres{mm/tool_select/assist/tfidf_ts_assist_k3/recall_k}{28.8}
\defres{mm/tool_select/assist/tfidf_ts_assist_k3/s1_acc}{15.6}
\defres{mm/tool_select/assist/tfidf_ts_assist_k3/saving}{67.2}
\defres{mm/tool_select/assist/tfidf_ts_assist_k3/saving_ci/hi}{72.1}
\defres{mm/tool_select/assist/tfidf_ts_assist_k3/saving_ci/lo}{61.7}
\defres{mm/tool_select/assist/tfidf_ts_assist_k3/status}{descriptive}
\defres{mm/tool_select/assist/tfidf_ts_assist_k3/success}{33.0}
\defres{mm/tool_select/assist/tfidf_ts_assist_k3/success_ref}{100.0}
\defres{mm/tool_select/assist/tfidf_ts_assist_k3/vcode}{4}
\defres{mm/tool_select/assist/tfidf_ts_assist_k3/verdict}{costs success}
\defres{mm/tool_select/assist/tfidf_ts_assist_k5/acc}{25.6}
\defres{mm/tool_select/assist/tfidf_ts_assist_k5/accepted_acc}{9.0}
\defres{mm/tool_select/assist/tfidf_ts_assist_k5/acted}{100.0}
\defres{mm/tool_select/assist/tfidf_ts_assist_k5/acted_kind}{shortlist}
\defres{mm/tool_select/assist/tfidf_ts_assist_k5/cost_k}{24.3}
\defres{mm/tool_select/assist/tfidf_ts_assist_k5/cost_ref_k}{40.9}
\defres{mm/tool_select/assist/tfidf_ts_assist_k5/delta}{-75.0}
\defres{mm/tool_select/assist/tfidf_ts_assist_k5/delta_ci/hi}{-69.0}
\defres{mm/tool_select/assist/tfidf_ts_assist_k5/delta_ci/lo}{-81.0}
\defres{mm/tool_select/assist/tfidf_ts_assist_k5/fig_delta}{-75.0}
\defres{mm/tool_select/assist/tfidf_ts_assist_k5/fig_saving}{41}
\defres{mm/tool_select/assist/tfidf_ts_assist_k5/n}{200}
\defres{mm/tool_select/assist/tfidf_ts_assist_k5/n_dropped}{0}
\defres{mm/tool_select/assist/tfidf_ts_assist_k5/recall_k}{25.6}
\defres{mm/tool_select/assist/tfidf_ts_assist_k5/s1_acc}{9.0}
\defres{mm/tool_select/assist/tfidf_ts_assist_k5/saving}{40.6}
\defres{mm/tool_select/assist/tfidf_ts_assist_k5/saving_ci/hi}{49.9}
\defres{mm/tool_select/assist/tfidf_ts_assist_k5/saving_ci/lo}{30.9}
\defres{mm/tool_select/assist/tfidf_ts_assist_k5/status}{descriptive}
\defres{mm/tool_select/assist/tfidf_ts_assist_k5/success}{25.0}
\defres{mm/tool_select/assist/tfidf_ts_assist_k5/success_ref}{100.0}
\defres{mm/tool_select/assist/tfidf_ts_assist_k5/vcode}{4}
\defres{mm/tool_select/assist/tfidf_ts_assist_k5/verdict}{costs success}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.5/acc}{93.7}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.5/accepted_acc}{93.7}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.5/acted}{97.3}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.5/acted_kind}{decided}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.5/cost_k}{6.6}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.5/cost_ref_k}{42.9}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.5/coverage}{97.3}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.5/delta}{-21.5}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.5/delta_ci/hi}{-16.0}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.5/delta_ci/lo}{-27.5}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.5/fig_delta}{-21.5}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.5/fig_saving}{85}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.5/n}{200}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.5/n_dropped}{0}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.5/s1_acc}{92.6}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.5/saving}{84.5}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.5/saving_ci/hi}{86.4}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.5/saving_ci/lo}{82.0}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.5/status}{descriptive}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.5/success}{78.5}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.5/success_ref}{100.0}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.5/vcode}{4}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.5/verdict}{costs success}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.7/acc}{96.1}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.7/accepted_acc}{96.1}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.7/acted}{91.3}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.7/acted_kind}{decided}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.7/cost_k}{8.2}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.7/cost_ref_k}{42.9}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.7/coverage}{91.3}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.7/delta}{-24.0}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.7/delta_ci/hi}{-18.0}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.7/delta_ci/lo}{-30.0}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.7/fig_delta}{-24.0}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.7/fig_saving}{81}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.7/n}{200}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.7/n_dropped}{0}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.7/s1_acc}{94.9}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.7/saving}{81.0}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.7/saving_ci/hi}{82.1}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.7/saving_ci/lo}{79.5}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.7/status}{descriptive}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.7/success}{76.0}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.7/success_ref}{100.0}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.7/vcode}{4}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.7/verdict}{costs success}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.8/acc}{96.3}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.8/accepted_acc}{96.3}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.8/acted}{86.5}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.8/acted_kind}{decided}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.8/cost_k}{10.1}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.8/cost_ref_k}{42.9}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.8/coverage}{86.5}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.8/delta}{-23.5}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.8/delta_ci/hi}{-18.0}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.8/delta_ci/lo}{-29.5}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.8/fig_delta}{-23.5}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.8/fig_saving}{76}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.8/n}{200}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.8/n_dropped}{0}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.8/s1_acc}{94.4}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.8/saving}{76.5}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.8/saving_ci/hi}{78.1}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.8/saving_ci/lo}{74.5}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.8/status}{descriptive}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.8/success}{76.5}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.8/success_ref}{100.0}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.8/vcode}{4}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.8/verdict}{costs success}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.9/acc}{96.4}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.9/accepted_acc}{96.4}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.9/acted}{81.3}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.9/acted_kind}{decided}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.9/cost_k}{12.0}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.9/cost_ref_k}{42.9}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.9/coverage}{81.3}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.9/delta}{-20.5}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.9/delta_ci/hi}{-15.0}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.9/delta_ci/lo}{-26.5}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.9/fig_delta}{-20.5}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.9/fig_saving}{72}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.9/n}{200}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.9/n_dropped}{0}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.9/s1_acc}{94.5}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.9/saving}{72.0}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.9/saving_ci/hi}{73.5}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.9/saving_ci/lo}{70.3}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.9/status}{descriptive}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.9/success}{79.5}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.9/success_ref}{100.0}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.9/vcode}{4}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.9/verdict}{costs success}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.95/acc}{96.1}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.95/accepted_acc}{96.1}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.95/acted}{74.3}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.95/acted_kind}{decided}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.95/cost_k}{14.3}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.95/cost_ref_k}{42.9}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.95/coverage}{74.3}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.95/delta}{-20.5}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.95/delta_ci/hi}{-15.0}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.95/delta_ci/lo}{-26.0}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.95/fig_delta}{-20.5}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.95/fig_saving}{67}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.95/n}{200}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.95/n_dropped}{0}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.95/s1_acc}{94.1}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.95/saving}{66.8}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.95/saving_ci/hi}{69.0}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.95/saving_ci/lo}{64.5}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.95/status}{descriptive}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.95/success}{79.5}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.95/success_ref}{100.0}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.95/vcode}{4}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.95/verdict}{costs success}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.99/acc}{97.6}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.99/accepted_acc}{97.6}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.99/acted}{45.1}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.99/acted_kind}{decided}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.99/cost_k}{26.1}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.99/cost_ref_k}{42.9}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.99/coverage}{45.1}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.99/delta}{-8.0}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.99/delta_ci/hi}{-4.5}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.99/delta_ci/lo}{-12.0}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.99/fig_delta}{-8.0}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.99/fig_saving}{39}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.99/n}{200}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.99/n_dropped}{0}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.99/s1_acc}{94.2}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.99/saving}{39.3}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.99/saving_ci/hi}{43.0}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.99/saving_ci/lo}{35.7}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.99/status}{descriptive}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.99/success}{92.0}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.99/success_ref}{100.0}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.99/vcode}{4}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.99/verdict}{costs success}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.9_s2lite/acted}{0.0}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.9_s2lite/acted_kind}{decided}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.9_s2lite/cost_k}{9.8}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.9_s2lite/cost_ref_k}{9.8}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.9_s2lite/coverage}{0.0}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.9_s2lite/delta}{+1.0}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.9_s2lite/delta_ci/hi}{+3.2}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.9_s2lite/delta_ci/lo}{-1.0}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.9_s2lite/fig_delta}{+1.0}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.9_s2lite/fig_saving}{0}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.9_s2lite/n}{500}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.9_s2lite/n_dropped}{0}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.9_s2lite/reg}{C1L}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.9_s2lite/saving}{0.2}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.9_s2lite/saving_ci/hi}{0.7}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.9_s2lite/saving_ci/lo}{-0.3}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.9_s2lite/status}{registered}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.9_s2lite/success}{81.2}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.9_s2lite/success_ref}{80.2}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.9_s2lite/vcode}{2}
\defres{mm/tool_select/cascade/jev_ts_cascade_tau0.9_s2lite/verdict}{mixed}
\defres{mm/tool_select/cascade/jev_ts_cascade_tauhat/acc}{100.0}
\defres{mm/tool_select/cascade/jev_ts_cascade_tauhat/accepted_acc}{100.0}
\defres{mm/tool_select/cascade/jev_ts_cascade_tauhat/acted}{27.2}
\defres{mm/tool_select/cascade/jev_ts_cascade_tauhat/acted_kind}{decided}
\defres{mm/tool_select/cascade/jev_ts_cascade_tauhat/cost_k}{36.4}
\defres{mm/tool_select/cascade/jev_ts_cascade_tauhat/cost_ref_k}{42.4}
\defres{mm/tool_select/cascade/jev_ts_cascade_tauhat/coverage}{27.2}
\defres{mm/tool_select/cascade/jev_ts_cascade_tauhat/delta}{+0.0}
\defres{mm/tool_select/cascade/jev_ts_cascade_tauhat/delta_ci/hi}{+0.0}
\defres{mm/tool_select/cascade/jev_ts_cascade_tauhat/delta_ci/lo}{+0.0}
\defres{mm/tool_select/cascade/jev_ts_cascade_tauhat/fig_delta}{+0.0}
\defres{mm/tool_select/cascade/jev_ts_cascade_tauhat/fig_saving}{14}
\defres{mm/tool_select/cascade/jev_ts_cascade_tauhat/fresh/acc}{100.0}
\defres{mm/tool_select/cascade/jev_ts_cascade_tauhat/fresh/accepted_acc}{100.0}
\defres{mm/tool_select/cascade/jev_ts_cascade_tauhat/fresh/acted}{28.9}
\defres{mm/tool_select/cascade/jev_ts_cascade_tauhat/fresh/acted_kind}{decided}
\defres{mm/tool_select/cascade/jev_ts_cascade_tauhat/fresh/cost_k}{33.5}
\defres{mm/tool_select/cascade/jev_ts_cascade_tauhat/fresh/cost_ref_k}{41.3}
\defres{mm/tool_select/cascade/jev_ts_cascade_tauhat/fresh/coverage}{28.9}
\defres{mm/tool_select/cascade/jev_ts_cascade_tauhat/fresh/delta}{+0.4}
\defres{mm/tool_select/cascade/jev_ts_cascade_tauhat/fresh/fig_delta}{+0.4}
\defres{mm/tool_select/cascade/jev_ts_cascade_tauhat/fresh/fig_saving}{19}
\defres{mm/tool_select/cascade/jev_ts_cascade_tauhat/fresh/n}{500}
\defres{mm/tool_select/cascade/jev_ts_cascade_tauhat/fresh/n_dropped}{0}
\defres{mm/tool_select/cascade/jev_ts_cascade_tauhat/fresh/s1_acc}{94.1}
\defres{mm/tool_select/cascade/jev_ts_cascade_tauhat/fresh/saving}{18.8}
\defres{mm/tool_select/cascade/jev_ts_cascade_tauhat/fresh/success}{99.8}
\defres{mm/tool_select/cascade/jev_ts_cascade_tauhat/fresh/success_ref}{99.4}
\defres{mm/tool_select/cascade/jev_ts_cascade_tauhat/fresh/verdict}{takes over safely}
\defres{mm/tool_select/cascade/jev_ts_cascade_tauhat/n}{500}
\defres{mm/tool_select/cascade/jev_ts_cascade_tauhat/n_dropped}{0}
\defres{mm/tool_select/cascade/jev_ts_cascade_tauhat/reg}{C1F}
\defres{mm/tool_select/cascade/jev_ts_cascade_tauhat/s1_acc}{94.2}
\defres{mm/tool_select/cascade/jev_ts_cascade_tauhat/saving}{14.2}
\defres{mm/tool_select/cascade/jev_ts_cascade_tauhat/saving_ci/hi}{15.7}
\defres{mm/tool_select/cascade/jev_ts_cascade_tauhat/saving_ci/lo}{12.7}
\defres{mm/tool_select/cascade/jev_ts_cascade_tauhat/status}{registered}
\defres{mm/tool_select/cascade/jev_ts_cascade_tauhat/success}{99.8}
\defres{mm/tool_select/cascade/jev_ts_cascade_tauhat/success_ref}{99.8}
\defres{mm/tool_select/cascade/jev_ts_cascade_tauhat/vcode}{1}
\defres{mm/tool_select/cascade/jev_ts_cascade_tauhat/verdict}{takes over safely}
\defres{mm/tool_select/cascade/lite_ts_cascade_tau0.7/acc}{80.6}
\defres{mm/tool_select/cascade/lite_ts_cascade_tau0.7/accepted_acc}{80.6}
\defres{mm/tool_select/cascade/lite_ts_cascade_tau0.7/acted}{99.9}
\defres{mm/tool_select/cascade/lite_ts_cascade_tau0.7/acted_kind}{decided}
\defres{mm/tool_select/cascade/lite_ts_cascade_tau0.7/cost_k}{26.7}
\defres{mm/tool_select/cascade/lite_ts_cascade_tau0.7/cost_ref_k}{42.9}
\defres{mm/tool_select/cascade/lite_ts_cascade_tau0.7/coverage}{99.9}
\defres{mm/tool_select/cascade/lite_ts_cascade_tau0.7/delta}{-57.5}
\defres{mm/tool_select/cascade/lite_ts_cascade_tau0.7/delta_ci/hi}{-50.5}
\defres{mm/tool_select/cascade/lite_ts_cascade_tau0.7/delta_ci/lo}{-64.0}
\defres{mm/tool_select/cascade/lite_ts_cascade_tau0.7/fig_delta}{-57.5}
\defres{mm/tool_select/cascade/lite_ts_cascade_tau0.7/fig_saving}{38}
\defres{mm/tool_select/cascade/lite_ts_cascade_tau0.7/n}{200}
\defres{mm/tool_select/cascade/lite_ts_cascade_tau0.7/n_dropped}{0}
\defres{mm/tool_select/cascade/lite_ts_cascade_tau0.7/s1_acc}{80.5}
\defres{mm/tool_select/cascade/lite_ts_cascade_tau0.7/saving}{37.9}
\defres{mm/tool_select/cascade/lite_ts_cascade_tau0.7/saving_ci/hi}{42.9}
\defres{mm/tool_select/cascade/lite_ts_cascade_tau0.7/saving_ci/lo}{32.6}
\defres{mm/tool_select/cascade/lite_ts_cascade_tau0.7/status}{descriptive}
\defres{mm/tool_select/cascade/lite_ts_cascade_tau0.7/success}{42.5}
\defres{mm/tool_select/cascade/lite_ts_cascade_tau0.7/success_ref}{100.0}
\defres{mm/tool_select/cascade/lite_ts_cascade_tau0.7/vcode}{4}
\defres{mm/tool_select/cascade/lite_ts_cascade_tau0.7/verdict}{costs success}
\defres{mm/tool_select/cascade/lite_ts_cascade_tau0.9/acc}{82.7}
\defres{mm/tool_select/cascade/lite_ts_cascade_tau0.9/accepted_acc}{82.7}
\defres{mm/tool_select/cascade/lite_ts_cascade_tau0.9/acted}{98.3}
\defres{mm/tool_select/cascade/lite_ts_cascade_tau0.9/acted_kind}{decided}
\defres{mm/tool_select/cascade/lite_ts_cascade_tau0.9/cost_k}{26.3}
\defres{mm/tool_select/cascade/lite_ts_cascade_tau0.9/cost_ref_k}{42.9}
\defres{mm/tool_select/cascade/lite_ts_cascade_tau0.9/coverage}{98.3}
\defres{mm/tool_select/cascade/lite_ts_cascade_tau0.9/delta}{-56.5}
\defres{mm/tool_select/cascade/lite_ts_cascade_tau0.9/delta_ci/hi}{-49.5}
\defres{mm/tool_select/cascade/lite_ts_cascade_tau0.9/delta_ci/lo}{-63.5}
\defres{mm/tool_select/cascade/lite_ts_cascade_tau0.9/fig_delta}{-56.5}
\defres{mm/tool_select/cascade/lite_ts_cascade_tau0.9/fig_saving}{39}
\defres{mm/tool_select/cascade/lite_ts_cascade_tau0.9/n}{200}
\defres{mm/tool_select/cascade/lite_ts_cascade_tau0.9/n_dropped}{0}
\defres{mm/tool_select/cascade/lite_ts_cascade_tau0.9/s1_acc}{82.0}
\defres{mm/tool_select/cascade/lite_ts_cascade_tau0.9/saving}{38.8}
\defres{mm/tool_select/cascade/lite_ts_cascade_tau0.9/saving_ci/hi}{42.9}
\defres{mm/tool_select/cascade/lite_ts_cascade_tau0.9/saving_ci/lo}{34.7}
\defres{mm/tool_select/cascade/lite_ts_cascade_tau0.9/status}{descriptive}
\defres{mm/tool_select/cascade/lite_ts_cascade_tau0.9/success}{43.5}
\defres{mm/tool_select/cascade/lite_ts_cascade_tau0.9/success_ref}{100.0}
\defres{mm/tool_select/cascade/lite_ts_cascade_tau0.9/vcode}{4}
\defres{mm/tool_select/cascade/lite_ts_cascade_tau0.9/verdict}{costs success}
\defres{mm/tool_select/cascade/lite_ts_cascade_tau0.99/acc}{89.7}
\defres{mm/tool_select/cascade/lite_ts_cascade_tau0.99/accepted_acc}{89.7}
\defres{mm/tool_select/cascade/lite_ts_cascade_tau0.99/acted}{50.0}
\defres{mm/tool_select/cascade/lite_ts_cascade_tau0.99/acted_kind}{decided}
\defres{mm/tool_select/cascade/lite_ts_cascade_tau0.99/cost_k}{43.2}
\defres{mm/tool_select/cascade/lite_ts_cascade_tau0.99/cost_ref_k}{42.9}
\defres{mm/tool_select/cascade/lite_ts_cascade_tau0.99/coverage}{50.0}
\defres{mm/tool_select/cascade/lite_ts_cascade_tau0.99/delta}{-25.0}
\defres{mm/tool_select/cascade/lite_ts_cascade_tau0.99/delta_ci/hi}{-19.0}
\defres{mm/tool_select/cascade/lite_ts_cascade_tau0.99/delta_ci/lo}{-31.0}
\defres{mm/tool_select/cascade/lite_ts_cascade_tau0.99/fig_delta}{-25.0}
\defres{mm/tool_select/cascade/lite_ts_cascade_tau0.99/fig_saving}{-1}
\defres{mm/tool_select/cascade/lite_ts_cascade_tau0.99/n}{200}
\defres{mm/tool_select/cascade/lite_ts_cascade_tau0.99/n_dropped}{0}
\defres{mm/tool_select/cascade/lite_ts_cascade_tau0.99/s1_acc}{84.8}
\defres{mm/tool_select/cascade/lite_ts_cascade_tau0.99/saving}{-0.7}
\defres{mm/tool_select/cascade/lite_ts_cascade_tau0.99/saving_ci/hi}{3.5}
\defres{mm/tool_select/cascade/lite_ts_cascade_tau0.99/saving_ci/lo}{-4.8}
\defres{mm/tool_select/cascade/lite_ts_cascade_tau0.99/status}{descriptive}
\defres{mm/tool_select/cascade/lite_ts_cascade_tau0.99/success}{75.0}
\defres{mm/tool_select/cascade/lite_ts_cascade_tau0.99/success_ref}{100.0}
\defres{mm/tool_select/cascade/lite_ts_cascade_tau0.99/vcode}{4}
\defres{mm/tool_select/cascade/lite_ts_cascade_tau0.99/verdict}{costs success}
\defres{mm/tool_select/guard/jev_ts_guard/acc}{98.0}
\defres{mm/tool_select/guard/jev_ts_guard/accepted_acc}{98.0}
\defres{mm/tool_select/guard/jev_ts_guard/acted}{2.1}
\defres{mm/tool_select/guard/jev_ts_guard/acted_kind}{vetoed}
\defres{mm/tool_select/guard/jev_ts_guard/cost_k}{43.0}
\defres{mm/tool_select/guard/jev_ts_guard/cost_ref_k}{42.9}
\defres{mm/tool_select/guard/jev_ts_guard/delta}{+0.0}
\defres{mm/tool_select/guard/jev_ts_guard/delta_ci/hi}{+0.0}
\defres{mm/tool_select/guard/jev_ts_guard/delta_ci/lo}{+0.0}
\defres{mm/tool_select/guard/jev_ts_guard/fig_delta}{+0.0}
\defres{mm/tool_select/guard/jev_ts_guard/fig_saving}{0}
\defres{mm/tool_select/guard/jev_ts_guard/n}{200}
\defres{mm/tool_select/guard/jev_ts_guard/n_dropped}{0}
\defres{mm/tool_select/guard/jev_ts_guard/s1_acc}{98.0}
\defres{mm/tool_select/guard/jev_ts_guard/saving}{-0.2}
\defres{mm/tool_select/guard/jev_ts_guard/saving_ci/hi}{0.9}
\defres{mm/tool_select/guard/jev_ts_guard/saving_ci/lo}{-1.3}
\defres{mm/tool_select/guard/jev_ts_guard/status}{descriptive}
\defres{mm/tool_select/guard/jev_ts_guard/success}{100.0}
\defres{mm/tool_select/guard/jev_ts_guard/success_ref}{100.0}
\defres{mm/tool_select/guard/jev_ts_guard/vcode}{3}
\defres{mm/tool_select/guard/jev_ts_guard/verdict}{no saving}
\defres{mm/tool_select/guard/jev_ts_guard_s2lite/acc}{97.8}
\defres{mm/tool_select/guard/jev_ts_guard_s2lite/accepted_acc}{97.8}
\defres{mm/tool_select/guard/jev_ts_guard_s2lite/acted}{3.0}
\defres{mm/tool_select/guard/jev_ts_guard_s2lite/acted_kind}{vetoed}
\defres{mm/tool_select/guard/jev_ts_guard_s2lite/cost_k}{10.4}
\defres{mm/tool_select/guard/jev_ts_guard_s2lite/cost_ref_k}{9.8}
\defres{mm/tool_select/guard/jev_ts_guard_s2lite/delta}{+4.5}
\defres{mm/tool_select/guard/jev_ts_guard_s2lite/delta_ci/hi}{+9.0}
\defres{mm/tool_select/guard/jev_ts_guard_s2lite/delta_ci/lo}{+0.0}
\defres{mm/tool_select/guard/jev_ts_guard_s2lite/fig_delta}{+4.5}
\defres{mm/tool_select/guard/jev_ts_guard_s2lite/fig_saving}{-7}
\defres{mm/tool_select/guard/jev_ts_guard_s2lite/n}{200}
\defres{mm/tool_select/guard/jev_ts_guard_s2lite/n_dropped}{0}
\defres{mm/tool_select/guard/jev_ts_guard_s2lite/s1_acc}{97.8}
\defres{mm/tool_select/guard/jev_ts_guard_s2lite/saving}{-6.7}
\defres{mm/tool_select/guard/jev_ts_guard_s2lite/saving_ci/hi}{-5.5}
\defres{mm/tool_select/guard/jev_ts_guard_s2lite/saving_ci/lo}{-8.1}
\defres{mm/tool_select/guard/jev_ts_guard_s2lite/status}{descriptive}
\defres{mm/tool_select/guard/jev_ts_guard_s2lite/success}{86.5}
\defres{mm/tool_select/guard/jev_ts_guard_s2lite/success_ref}{82.0}
\defres{mm/tool_select/guard/jev_ts_guard_s2lite/vcode}{3}
\defres{mm/tool_select/guard/jev_ts_guard_s2lite/verdict}{no saving}
\defres{mm/tool_select/guard/lite_ts_guard/acc}{89.6}
\defres{mm/tool_select/guard/lite_ts_guard/accepted_acc}{89.6}
\defres{mm/tool_select/guard/lite_ts_guard/acted}{11.0}
\defres{mm/tool_select/guard/lite_ts_guard/acted_kind}{vetoed}
\defres{mm/tool_select/guard/lite_ts_guard/cost_k}{53.6}
\defres{mm/tool_select/guard/lite_ts_guard/cost_ref_k}{42.9}
\defres{mm/tool_select/guard/lite_ts_guard/delta}{+0.0}
\defres{mm/tool_select/guard/lite_ts_guard/delta_ci/hi}{+0.0}
\defres{mm/tool_select/guard/lite_ts_guard/delta_ci/lo}{+0.0}
\defres{mm/tool_select/guard/lite_ts_guard/fig_delta}{+0.0}
\defres{mm/tool_select/guard/lite_ts_guard/fig_saving}{-25}
\defres{mm/tool_select/guard/lite_ts_guard/n}{200}
\defres{mm/tool_select/guard/lite_ts_guard/n_dropped}{0}
\defres{mm/tool_select/guard/lite_ts_guard/s1_acc}{89.6}
\defres{mm/tool_select/guard/lite_ts_guard/saving}{-24.9}
\defres{mm/tool_select/guard/lite_ts_guard/saving_ci/hi}{-22.0}
\defres{mm/tool_select/guard/lite_ts_guard/saving_ci/lo}{-27.9}
\defres{mm/tool_select/guard/lite_ts_guard/status}{descriptive}
\defres{mm/tool_select/guard/lite_ts_guard/success}{100.0}
\defres{mm/tool_select/guard/lite_ts_guard/success_ref}{100.0}
\defres{mm/tool_select/guard/lite_ts_guard/vcode}{3}
\defres{mm/tool_select/guard/lite_ts_guard/verdict}{no saving}
\defres{mm/tool_select/replace/bm25_ts_replace/acc}{8.4}
\defres{mm/tool_select/replace/bm25_ts_replace/accepted_acc}{8.4}
\defres{mm/tool_select/replace/bm25_ts_replace/acted}{100.0}
\defres{mm/tool_select/replace/bm25_ts_replace/acted_kind}{decided}
\defres{mm/tool_select/replace/bm25_ts_replace/cost_k}{15.0}
\defres{mm/tool_select/replace/bm25_ts_replace/cost_ref_k}{40.9}
\defres{mm/tool_select/replace/bm25_ts_replace/coverage}{100.0}
\defres{mm/tool_select/replace/bm25_ts_replace/delta}{-87.5}
\defres{mm/tool_select/replace/bm25_ts_replace/delta_ci/hi}{-83.0}
\defres{mm/tool_select/replace/bm25_ts_replace/delta_ci/lo}{-92.0}
\defres{mm/tool_select/replace/bm25_ts_replace/fig_delta}{-87.5}
\defres{mm/tool_select/replace/bm25_ts_replace/fig_saving}{63}
\defres{mm/tool_select/replace/bm25_ts_replace/n}{200}
\defres{mm/tool_select/replace/bm25_ts_replace/n_dropped}{0}
\defres{mm/tool_select/replace/bm25_ts_replace/s1_acc}{8.4}
\defres{mm/tool_select/replace/bm25_ts_replace/saving}{63.3}
\defres{mm/tool_select/replace/bm25_ts_replace/saving_ci/hi}{72.1}
\defres{mm/tool_select/replace/bm25_ts_replace/saving_ci/lo}{53.8}
\defres{mm/tool_select/replace/bm25_ts_replace/status}{descriptive}
\defres{mm/tool_select/replace/bm25_ts_replace/success}{12.5}
\defres{mm/tool_select/replace/bm25_ts_replace/success_ref}{100.0}
\defres{mm/tool_select/replace/bm25_ts_replace/vcode}{4}
\defres{mm/tool_select/replace/bm25_ts_replace/verdict}{costs success}
\defres{mm/tool_select/replace/embed_ts_replace/acc}{4.2}
\defres{mm/tool_select/replace/embed_ts_replace/accepted_acc}{4.2}
\defres{mm/tool_select/replace/embed_ts_replace/acted}{100.0}
\defres{mm/tool_select/replace/embed_ts_replace/acted_kind}{decided}
\defres{mm/tool_select/replace/embed_ts_replace/cost_k}{8.7}
\defres{mm/tool_select/replace/embed_ts_replace/cost_ref_k}{40.9}
\defres{mm/tool_select/replace/embed_ts_replace/coverage}{100.0}
\defres{mm/tool_select/replace/embed_ts_replace/delta}{-100.0}
\defres{mm/tool_select/replace/embed_ts_replace/delta_ci/hi}{-100.0}
\defres{mm/tool_select/replace/embed_ts_replace/delta_ci/lo}{-100.0}
\defres{mm/tool_select/replace/embed_ts_replace/fig_delta}{-100.0}
\defres{mm/tool_select/replace/embed_ts_replace/fig_saving}{79}
\defres{mm/tool_select/replace/embed_ts_replace/n}{200}
\defres{mm/tool_select/replace/embed_ts_replace/n_dropped}{0}
\defres{mm/tool_select/replace/embed_ts_replace/s1_acc}{4.2}
\defres{mm/tool_select/replace/embed_ts_replace/saving}{78.7}
\defres{mm/tool_select/replace/embed_ts_replace/saving_ci/hi}{86.3}
\defres{mm/tool_select/replace/embed_ts_replace/saving_ci/lo}{70.0}
\defres{mm/tool_select/replace/embed_ts_replace/status}{descriptive}
\defres{mm/tool_select/replace/embed_ts_replace/success}{0.0}
\defres{mm/tool_select/replace/embed_ts_replace/success_ref}{100.0}
\defres{mm/tool_select/replace/embed_ts_replace/vcode}{4}
\defres{mm/tool_select/replace/embed_ts_replace/verdict}{costs success}
\defres{mm/tool_select/replace/heuristic_ts_replace/acc}{35.3}
\defres{mm/tool_select/replace/heuristic_ts_replace/accepted_acc}{35.3}
\defres{mm/tool_select/replace/heuristic_ts_replace/acted}{100.0}
\defres{mm/tool_select/replace/heuristic_ts_replace/acted_kind}{decided}
\defres{mm/tool_select/replace/heuristic_ts_replace/cost_k}{1.7}
\defres{mm/tool_select/replace/heuristic_ts_replace/cost_ref_k}{40.9}
\defres{mm/tool_select/replace/heuristic_ts_replace/coverage}{100.0}
\defres{mm/tool_select/replace/heuristic_ts_replace/delta}{-87.5}
\defres{mm/tool_select/replace/heuristic_ts_replace/delta_ci/hi}{-83.0}
\defres{mm/tool_select/replace/heuristic_ts_replace/delta_ci/lo}{-92.0}
\defres{mm/tool_select/replace/heuristic_ts_replace/fig_delta}{-87.5}
\defres{mm/tool_select/replace/heuristic_ts_replace/fig_saving}{96}
\defres{mm/tool_select/replace/heuristic_ts_replace/n}{200}
\defres{mm/tool_select/replace/heuristic_ts_replace/n_dropped}{0}
\defres{mm/tool_select/replace/heuristic_ts_replace/s1_acc}{35.3}
\defres{mm/tool_select/replace/heuristic_ts_replace/saving}{95.7}
\defres{mm/tool_select/replace/heuristic_ts_replace/saving_ci/hi}{95.9}
\defres{mm/tool_select/replace/heuristic_ts_replace/saving_ci/lo}{95.5}
\defres{mm/tool_select/replace/heuristic_ts_replace/status}{descriptive}
\defres{mm/tool_select/replace/heuristic_ts_replace/success}{12.5}
\defres{mm/tool_select/replace/heuristic_ts_replace/success_ref}{100.0}
\defres{mm/tool_select/replace/heuristic_ts_replace/vcode}{4}
\defres{mm/tool_select/replace/heuristic_ts_replace/verdict}{costs success}
\defres{mm/tool_select/replace/jev_ts_params_replace/acc}{89.9}
\defres{mm/tool_select/replace/jev_ts_params_replace/accepted_acc}{89.9}
\defres{mm/tool_select/replace/jev_ts_params_replace/acted}{100.0}
\defres{mm/tool_select/replace/jev_ts_params_replace/acted_kind}{decided}
\defres{mm/tool_select/replace/jev_ts_params_replace/cost_k}{5.1}
\defres{mm/tool_select/replace/jev_ts_params_replace/cost_ref_k}{42.9}
\defres{mm/tool_select/replace/jev_ts_params_replace/coverage}{100.0}
\defres{mm/tool_select/replace/jev_ts_params_replace/delta}{-20.0}
\defres{mm/tool_select/replace/jev_ts_params_replace/delta_ci/hi}{-14.5}
\defres{mm/tool_select/replace/jev_ts_params_replace/delta_ci/lo}{-25.5}
\defres{mm/tool_select/replace/jev_ts_params_replace/fig_delta}{-20.0}
\defres{mm/tool_select/replace/jev_ts_params_replace/fig_saving}{88}
\defres{mm/tool_select/replace/jev_ts_params_replace/n}{200}
\defres{mm/tool_select/replace/jev_ts_params_replace/n_dropped}{0}
\defres{mm/tool_select/replace/jev_ts_params_replace/s1_acc}{89.9}
\defres{mm/tool_select/replace/jev_ts_params_replace/saving}{88.1}
\defres{mm/tool_select/replace/jev_ts_params_replace/saving_ci/hi}{90.0}
\defres{mm/tool_select/replace/jev_ts_params_replace/saving_ci/lo}{85.6}
\defres{mm/tool_select/replace/jev_ts_params_replace/status}{descriptive}
\defres{mm/tool_select/replace/jev_ts_params_replace/success}{80.0}
\defres{mm/tool_select/replace/jev_ts_params_replace/success_ref}{100.0}
\defres{mm/tool_select/replace/jev_ts_params_replace/vcode}{4}
\defres{mm/tool_select/replace/jev_ts_params_replace/verdict}{costs success}
\defres{mm/tool_select/replace/jev_ts_params_replace_answercopy/acc}{89.7}
\defres{mm/tool_select/replace/jev_ts_params_replace_answercopy/accepted_acc}{89.7}
\defres{mm/tool_select/replace/jev_ts_params_replace_answercopy/acted}{100.0}
\defres{mm/tool_select/replace/jev_ts_params_replace_answercopy/acted_kind}{decided}
\defres{mm/tool_select/replace/jev_ts_params_replace_answercopy/cost_k}{5.5}
\defres{mm/tool_select/replace/jev_ts_params_replace_answercopy/cost_ref_k}{40.9}
\defres{mm/tool_select/replace/jev_ts_params_replace_answercopy/coverage}{100.0}
\defres{mm/tool_select/replace/jev_ts_params_replace_answercopy/delta}{-20.0}
\defres{mm/tool_select/replace/jev_ts_params_replace_answercopy/delta_ci/hi}{-14.5}
\defres{mm/tool_select/replace/jev_ts_params_replace_answercopy/delta_ci/lo}{-25.5}
\defres{mm/tool_select/replace/jev_ts_params_replace_answercopy/fig_delta}{-20.0}
\defres{mm/tool_select/replace/jev_ts_params_replace_answercopy/fig_saving}{87}
\defres{mm/tool_select/replace/jev_ts_params_replace_answercopy/n}{200}
\defres{mm/tool_select/replace/jev_ts_params_replace_answercopy/n_dropped}{0}
\defres{mm/tool_select/replace/jev_ts_params_replace_answercopy/s1_acc}{89.7}
\defres{mm/tool_select/replace/jev_ts_params_replace_answercopy/saving}{86.6}
\defres{mm/tool_select/replace/jev_ts_params_replace_answercopy/saving_ci/hi}{89.1}
\defres{mm/tool_select/replace/jev_ts_params_replace_answercopy/saving_ci/lo}{83.4}
\defres{mm/tool_select/replace/jev_ts_params_replace_answercopy/status}{descriptive}
\defres{mm/tool_select/replace/jev_ts_params_replace_answercopy/success}{80.0}
\defres{mm/tool_select/replace/jev_ts_params_replace_answercopy/success_ref}{100.0}
\defres{mm/tool_select/replace/jev_ts_params_replace_answercopy/vcode}{4}
\defres{mm/tool_select/replace/jev_ts_params_replace_answercopy/verdict}{costs success}
\defres{mm/tool_select/replace/jev_ts_replace-e2c/acc}{95.5}
\defres{mm/tool_select/replace/jev_ts_replace-e2c/accepted_acc}{95.5}
\defres{mm/tool_select/replace/jev_ts_replace-e2c/acted}{100.0}
\defres{mm/tool_select/replace/jev_ts_replace-e2c/acted_kind}{decided}
\defres{mm/tool_select/replace/jev_ts_replace-e2c/cost_k}{14.2}
\defres{mm/tool_select/replace/jev_ts_replace-e2c/cost_ref_k}{40.9}
\defres{mm/tool_select/replace/jev_ts_replace-e2c/coverage}{100.0}
\defres{mm/tool_select/replace/jev_ts_replace-e2c/delta}{-18.5}
\defres{mm/tool_select/replace/jev_ts_replace-e2c/delta_ci/hi}{-13.0}
\defres{mm/tool_select/replace/jev_ts_replace-e2c/delta_ci/lo}{-24.0}
\defres{mm/tool_select/replace/jev_ts_replace-e2c/fig_delta}{-18.5}
\defres{mm/tool_select/replace/jev_ts_replace-e2c/fig_saving}{65}
\defres{mm/tool_select/replace/jev_ts_replace-e2c/n}{200}
\defres{mm/tool_select/replace/jev_ts_replace-e2c/n_dropped}{0}
\defres{mm/tool_select/replace/jev_ts_replace-e2c/s1_acc}{95.5}
\defres{mm/tool_select/replace/jev_ts_replace-e2c/saving}{65.4}
\defres{mm/tool_select/replace/jev_ts_replace-e2c/saving_ci/hi}{67.4}
\defres{mm/tool_select/replace/jev_ts_replace-e2c/saving_ci/lo}{63.4}
\defres{mm/tool_select/replace/jev_ts_replace-e2c/status}{replicate}
\defres{mm/tool_select/replace/jev_ts_replace-e2c/success}{81.5}
\defres{mm/tool_select/replace/jev_ts_replace-e2c/success_ref}{100.0}
\defres{mm/tool_select/replace/jev_ts_replace-e2c/vcode}{4}
\defres{mm/tool_select/replace/jev_ts_replace-e2c/verdict}{costs success}
\defres{mm/tool_select/replace/jev_ts_replace/acc}{95.4}
\defres{mm/tool_select/replace/jev_ts_replace/accepted_acc}{95.4}
\defres{mm/tool_select/replace/jev_ts_replace/acted}{100.0}
\defres{mm/tool_select/replace/jev_ts_replace/acted_kind}{decided}
\defres{mm/tool_select/replace/jev_ts_replace/cost_k}{14.2}
\defres{mm/tool_select/replace/jev_ts_replace/cost_ref_k}{42.9}
\defres{mm/tool_select/replace/jev_ts_replace/coverage}{100.0}
\defres{mm/tool_select/replace/jev_ts_replace/delta}{-19.0}
\defres{mm/tool_select/replace/jev_ts_replace/delta_ci/hi}{-13.5}
\defres{mm/tool_select/replace/jev_ts_replace/delta_ci/lo}{-24.5}
\defres{mm/tool_select/replace/jev_ts_replace/fig_delta}{-19.0}
\defres{mm/tool_select/replace/jev_ts_replace/fig_saving}{67}
\defres{mm/tool_select/replace/jev_ts_replace/n}{200}
\defres{mm/tool_select/replace/jev_ts_replace/n_dropped}{0}
\defres{mm/tool_select/replace/jev_ts_replace/s1_acc}{95.4}
\defres{mm/tool_select/replace/jev_ts_replace/saving}{67.0}
\defres{mm/tool_select/replace/jev_ts_replace/saving_ci/hi}{69.1}
\defres{mm/tool_select/replace/jev_ts_replace/saving_ci/lo}{65.1}
\defres{mm/tool_select/replace/jev_ts_replace/status}{descriptive}
\defres{mm/tool_select/replace/jev_ts_replace/success}{81.0}
\defres{mm/tool_select/replace/jev_ts_replace/success_ref}{100.0}
\defres{mm/tool_select/replace/jev_ts_replace/vcode}{4}
\defres{mm/tool_select/replace/jev_ts_replace/verdict}{costs success}
\defres{mm/tool_select/replace/lite_ts_params_replace/acc}{79.9}
\defres{mm/tool_select/replace/lite_ts_params_replace/accepted_acc}{79.9}
\defres{mm/tool_select/replace/lite_ts_params_replace/acted}{100.0}
\defres{mm/tool_select/replace/lite_ts_params_replace/acted_kind}{decided}
\defres{mm/tool_select/replace/lite_ts_params_replace/cost_k}{27.1}
\defres{mm/tool_select/replace/lite_ts_params_replace/cost_ref_k}{42.9}
\defres{mm/tool_select/replace/lite_ts_params_replace/coverage}{100.0}
\defres{mm/tool_select/replace/lite_ts_params_replace/delta}{-60.5}
\defres{mm/tool_select/replace/lite_ts_params_replace/delta_ci/hi}{-53.5}
\defres{mm/tool_select/replace/lite_ts_params_replace/delta_ci/lo}{-67.5}
\defres{mm/tool_select/replace/lite_ts_params_replace/fig_delta}{-60.5}
\defres{mm/tool_select/replace/lite_ts_params_replace/fig_saving}{37}
\defres{mm/tool_select/replace/lite_ts_params_replace/n}{200}
\defres{mm/tool_select/replace/lite_ts_params_replace/n_dropped}{0}
\defres{mm/tool_select/replace/lite_ts_params_replace/s1_acc}{79.9}
\defres{mm/tool_select/replace/lite_ts_params_replace/saving}{36.9}
\defres{mm/tool_select/replace/lite_ts_params_replace/saving_ci/hi}{42.7}
\defres{mm/tool_select/replace/lite_ts_params_replace/saving_ci/lo}{30.7}
\defres{mm/tool_select/replace/lite_ts_params_replace/status}{descriptive}
\defres{mm/tool_select/replace/lite_ts_params_replace/success}{39.5}
\defres{mm/tool_select/replace/lite_ts_params_replace/success_ref}{100.0}
\defres{mm/tool_select/replace/lite_ts_params_replace/vcode}{4}
\defres{mm/tool_select/replace/lite_ts_params_replace/verdict}{costs success}
\defres{mm/tool_select/replace/lite_ts_replace/acc}{82.7}
\defres{mm/tool_select/replace/lite_ts_replace/accepted_acc}{82.7}
\defres{mm/tool_select/replace/lite_ts_replace/acted}{100.0}
\defres{mm/tool_select/replace/lite_ts_replace/acted_kind}{decided}
\defres{mm/tool_select/replace/lite_ts_replace/cost_k}{24.2}
\defres{mm/tool_select/replace/lite_ts_replace/cost_ref_k}{40.9}
\defres{mm/tool_select/replace/lite_ts_replace/coverage}{100.0}
\defres{mm/tool_select/replace/lite_ts_replace/delta}{-58.5}
\defres{mm/tool_select/replace/lite_ts_replace/delta_ci/hi}{-51.5}
\defres{mm/tool_select/replace/lite_ts_replace/delta_ci/lo}{-65.0}
\defres{mm/tool_select/replace/lite_ts_replace/fig_delta}{-58.5}
\defres{mm/tool_select/replace/lite_ts_replace/fig_saving}{41}
\defres{mm/tool_select/replace/lite_ts_replace/n}{200}
\defres{mm/tool_select/replace/lite_ts_replace/n_dropped}{0}
\defres{mm/tool_select/replace/lite_ts_replace/s1_acc}{82.7}
\defres{mm/tool_select/replace/lite_ts_replace/saving}{40.9}
\defres{mm/tool_select/replace/lite_ts_replace/saving_ci/hi}{45.3}
\defres{mm/tool_select/replace/lite_ts_replace/saving_ci/lo}{36.5}
\defres{mm/tool_select/replace/lite_ts_replace/status}{descriptive}
\defres{mm/tool_select/replace/lite_ts_replace/success}{41.5}
\defres{mm/tool_select/replace/lite_ts_replace/success_ref}{100.0}
\defres{mm/tool_select/replace/lite_ts_replace/vcode}{4}
\defres{mm/tool_select/replace/lite_ts_replace/verdict}{costs success}
\defres{mm/tool_select/replace/prior_recent_ts_replace/acc}{0.0}
\defres{mm/tool_select/replace/prior_recent_ts_replace/accepted_acc}{0.0}
\defres{mm/tool_select/replace/prior_recent_ts_replace/acted}{100.0}
\defres{mm/tool_select/replace/prior_recent_ts_replace/acted_kind}{decided}
\defres{mm/tool_select/replace/prior_recent_ts_replace/cost_k}{40.4}
\defres{mm/tool_select/replace/prior_recent_ts_replace/cost_ref_k}{40.9}
\defres{mm/tool_select/replace/prior_recent_ts_replace/coverage}{100.0}
\defres{mm/tool_select/replace/prior_recent_ts_replace/delta}{-100.0}
\defres{mm/tool_select/replace/prior_recent_ts_replace/delta_ci/hi}{-100.0}
\defres{mm/tool_select/replace/prior_recent_ts_replace/delta_ci/lo}{-100.0}
\defres{mm/tool_select/replace/prior_recent_ts_replace/fig_delta}{-100.0}
\defres{mm/tool_select/replace/prior_recent_ts_replace/fig_saving}{1}
\defres{mm/tool_select/replace/prior_recent_ts_replace/n}{200}
\defres{mm/tool_select/replace/prior_recent_ts_replace/n_dropped}{0}
\defres{mm/tool_select/replace/prior_recent_ts_replace/s1_acc}{0.0}
\defres{mm/tool_select/replace/prior_recent_ts_replace/saving}{1.3}
\defres{mm/tool_select/replace/prior_recent_ts_replace/saving_ci/hi}{13.9}
\defres{mm/tool_select/replace/prior_recent_ts_replace/saving_ci/lo}{-11.9}
\defres{mm/tool_select/replace/prior_recent_ts_replace/status}{descriptive}
\defres{mm/tool_select/replace/prior_recent_ts_replace/success}{0.0}
\defres{mm/tool_select/replace/prior_recent_ts_replace/success_ref}{100.0}
\defres{mm/tool_select/replace/prior_recent_ts_replace/vcode}{4}
\defres{mm/tool_select/replace/prior_recent_ts_replace/verdict}{costs success}
\defres{mm/tool_select/replace/random_ts_replace/acc}{2.9}
\defres{mm/tool_select/replace/random_ts_replace/accepted_acc}{2.9}
\defres{mm/tool_select/replace/random_ts_replace/acted}{100.0}
\defres{mm/tool_select/replace/random_ts_replace/acted_kind}{decided}
\defres{mm/tool_select/replace/random_ts_replace/cost_k}{3.0}
\defres{mm/tool_select/replace/random_ts_replace/cost_ref_k}{40.9}
\defres{mm/tool_select/replace/random_ts_replace/coverage}{100.0}
\defres{mm/tool_select/replace/random_ts_replace/delta}{-100.0}
\defres{mm/tool_select/replace/random_ts_replace/delta_ci/hi}{-100.0}
\defres{mm/tool_select/replace/random_ts_replace/delta_ci/lo}{-100.0}
\defres{mm/tool_select/replace/random_ts_replace/fig_delta}{-100.0}
\defres{mm/tool_select/replace/random_ts_replace/fig_saving}{93}
\defres{mm/tool_select/replace/random_ts_replace/n}{200}
\defres{mm/tool_select/replace/random_ts_replace/n_dropped}{0}
\defres{mm/tool_select/replace/random_ts_replace/s1_acc}{2.9}
\defres{mm/tool_select/replace/random_ts_replace/saving}{92.7}
\defres{mm/tool_select/replace/random_ts_replace/saving_ci/hi}{94.0}
\defres{mm/tool_select/replace/random_ts_replace/saving_ci/lo}{91.2}
\defres{mm/tool_select/replace/random_ts_replace/status}{descriptive}
\defres{mm/tool_select/replace/random_ts_replace/success}{0.0}
\defres{mm/tool_select/replace/random_ts_replace/success_ref}{100.0}
\defres{mm/tool_select/replace/random_ts_replace/vcode}{4}
\defres{mm/tool_select/replace/random_ts_replace/verdict}{costs success}
\defres{mm/tool_select/replace/tfidf_ts_replace/acc}{10.0}
\defres{mm/tool_select/replace/tfidf_ts_replace/accepted_acc}{10.0}
\defres{mm/tool_select/replace/tfidf_ts_replace/acted}{100.0}
\defres{mm/tool_select/replace/tfidf_ts_replace/acted_kind}{decided}
\defres{mm/tool_select/replace/tfidf_ts_replace/cost_k}{18.7}
\defres{mm/tool_select/replace/tfidf_ts_replace/cost_ref_k}{40.9}
\defres{mm/tool_select/replace/tfidf_ts_replace/coverage}{100.0}
\defres{mm/tool_select/replace/tfidf_ts_replace/delta}{-87.5}
\defres{mm/tool_select/replace/tfidf_ts_replace/delta_ci/hi}{-83.0}
\defres{mm/tool_select/replace/tfidf_ts_replace/delta_ci/lo}{-92.0}
\defres{mm/tool_select/replace/tfidf_ts_replace/fig_delta}{-87.5}
\defres{mm/tool_select/replace/tfidf_ts_replace/fig_saving}{54}
\defres{mm/tool_select/replace/tfidf_ts_replace/n}{200}
\defres{mm/tool_select/replace/tfidf_ts_replace/n_dropped}{0}
\defres{mm/tool_select/replace/tfidf_ts_replace/s1_acc}{10.0}
\defres{mm/tool_select/replace/tfidf_ts_replace/saving}{54.4}
\defres{mm/tool_select/replace/tfidf_ts_replace/saving_ci/hi}{68.0}
\defres{mm/tool_select/replace/tfidf_ts_replace/saving_ci/lo}{39.1}
\defres{mm/tool_select/replace/tfidf_ts_replace/status}{descriptive}
\defres{mm/tool_select/replace/tfidf_ts_replace/success}{12.5}
\defres{mm/tool_select/replace/tfidf_ts_replace/success_ref}{100.0}
\defres{mm/tool_select/replace/tfidf_ts_replace/vcode}{4}
\defres{mm/tool_select/replace/tfidf_ts_replace/verdict}{costs success}
\defres{mm/xcell/flash/action/assist/acc}{23.6}
\defres{mm/xcell/flash/action/assist/acted}{100.0}
\defres{mm/xcell/flash/action/assist/delta}{-40.7}
\defres{mm/xcell/flash/action/assist/explore}{E6a}
\defres{mm/xcell/flash/action/assist/fig_delta}{-40.7}
\defres{mm/xcell/flash/action/assist/fig_saving}{-182}
\defres{mm/xcell/flash/action/assist/losses}{58}
\defres{mm/xcell/flash/action/assist/n}{140}
\defres{mm/xcell/flash/action/assist/row}{jev\_action\_assist\_k3}
\defres{mm/xcell/flash/action/assist/saving}{-182.0}
\defres{mm/xcell/flash/action/assist/state}{exploratory}
\defres{mm/xcell/flash/action/assist/vcode}{4}
\defres{mm/xcell/flash/action/assist/verdict}{costs success}
\defres{mm/xcell/flash/action/assist/wins}{1}
\defres{mm/xcell/flash/action/cascade/acc}{73.5}
\defres{mm/xcell/flash/action/cascade/acted}{23.3}
\defres{mm/xcell/flash/action/cascade/coverage}{23.3}
\defres{mm/xcell/flash/action/cascade/delta}{+0.0}
\defres{mm/xcell/flash/action/cascade/explore}{E6a}
\defres{mm/xcell/flash/action/cascade/fig_delta}{+0.0}
\defres{mm/xcell/flash/action/cascade/fig_saving}{14}
\defres{mm/xcell/flash/action/cascade/losses}{4}
\defres{mm/xcell/flash/action/cascade/n}{140}
\defres{mm/xcell/flash/action/cascade/row}{jev\_action\_cascade\_tauhat}
\defres{mm/xcell/flash/action/cascade/saving}{14.0}
\defres{mm/xcell/flash/action/cascade/state}{exploratory}
\defres{mm/xcell/flash/action/cascade/vcode}{1}
\defres{mm/xcell/flash/action/cascade/verdict}{takes over safely}
\defres{mm/xcell/flash/action/cascade/wins}{4}
\defres{mm/xcell/flash/action/guard/acc}{65.5}
\defres{mm/xcell/flash/action/guard/acted}{46.5}
\defres{mm/xcell/flash/action/guard/delta}{-0.7}
\defres{mm/xcell/flash/action/guard/explore}{E6c}
\defres{mm/xcell/flash/action/guard/fig_delta}{-0.7}
\defres{mm/xcell/flash/action/guard/fig_saving}{-87}
\defres{mm/xcell/flash/action/guard/losses}{4}
\defres{mm/xcell/flash/action/guard/n}{140}
\defres{mm/xcell/flash/action/guard/row}{jev\_action\_guard}
\defres{mm/xcell/flash/action/guard/saving}{-86.7}
\defres{mm/xcell/flash/action/guard/state}{exploratory}
\defres{mm/xcell/flash/action/guard/vcode}{3}
\defres{mm/xcell/flash/action/guard/verdict}{no saving}
\defres{mm/xcell/flash/action/guard/wins}{3}
\defres{mm/xcell/flash/action/replace/acc}{17.7}
\defres{mm/xcell/flash/action/replace/acted}{100.0}
\defres{mm/xcell/flash/action/replace/coverage}{100.0}
\defres{mm/xcell/flash/action/replace/delta}{-64.3}
\defres{mm/xcell/flash/action/replace/explore}{E6a}
\defres{mm/xcell/flash/action/replace/fig_delta}{-64.3}
\defres{mm/xcell/flash/action/replace/fig_saving}{91}
\defres{mm/xcell/flash/action/replace/losses}{90}
\defres{mm/xcell/flash/action/replace/n}{140}
\defres{mm/xcell/flash/action/replace/row}{jev\_action\_replace}
\defres{mm/xcell/flash/action/replace/saving}{90.7}
\defres{mm/xcell/flash/action/replace/state}{exploratory}
\defres{mm/xcell/flash/action/replace/vcode}{4}
\defres{mm/xcell/flash/action/replace/verdict}{costs success}
\defres{mm/xcell/flash/action/replace/wins}{0}
\defres{mm/xcell/flash/action/trigger/acc}{67.1}
\defres{mm/xcell/flash/action/trigger/acted}{74.9}
\defres{mm/xcell/flash/action/trigger/coverage}{100.0}
\defres{mm/xcell/flash/action/trigger/delta}{-2.1}
\defres{mm/xcell/flash/action/trigger/explore}{E6f}
\defres{mm/xcell/flash/action/trigger/fig_delta}{-2.1}
\defres{mm/xcell/flash/action/trigger/fig_saving}{-111}
\defres{mm/xcell/flash/action/trigger/losses}{6}
\defres{mm/xcell/flash/action/trigger/n}{140}
\defres{mm/xcell/flash/action/trigger/row}{jev\_action\_trigger}
\defres{mm/xcell/flash/action/trigger/saving}{-111.2}
\defres{mm/xcell/flash/action/trigger/state}{exploratory}
\defres{mm/xcell/flash/action/trigger/vcode}{3}
\defres{mm/xcell/flash/action/trigger/verdict}{no saving}
\defres{mm/xcell/flash/action/trigger/wins}{3}
\defres{mm/xcell/flash/memory_read/cascade/acc}{76.2}
\defres{mm/xcell/flash/memory_read/cascade/acted}{54.4}
\defres{mm/xcell/flash/memory_read/cascade/coverage}{54.4}
\defres{mm/xcell/flash/memory_read/cascade/delta}{+0.0}
\defres{mm/xcell/flash/memory_read/cascade/explore}{E6b}
\defres{mm/xcell/flash/memory_read/cascade/fig_delta}{+0.0}
\defres{mm/xcell/flash/memory_read/cascade/fig_saving}{-21}
\defres{mm/xcell/flash/memory_read/cascade/losses}{1}
\defres{mm/xcell/flash/memory_read/cascade/n}{200}
\defres{mm/xcell/flash/memory_read/cascade/row}{mr\_cascade}
\defres{mm/xcell/flash/memory_read/cascade/saving}{-20.5}
\defres{mm/xcell/flash/memory_read/cascade/state}{exploratory}
\defres{mm/xcell/flash/memory_read/cascade/vcode}{3}
\defres{mm/xcell/flash/memory_read/cascade/verdict}{no saving}
\defres{mm/xcell/flash/memory_read/cascade/wins}{1}
\defres{mm/xcell/flash/memory_read/guard/acc}{58.7}
\defres{mm/xcell/flash/memory_read/guard/acted}{41.2}
\defres{mm/xcell/flash/memory_read/guard/coverage}{0.0}
\defres{mm/xcell/flash/memory_read/guard/delta}{+0.0}
\defres{mm/xcell/flash/memory_read/guard/explore}{E6d}
\defres{mm/xcell/flash/memory_read/guard/fig_delta}{+0.0}
\defres{mm/xcell/flash/memory_read/guard/fig_saving}{-140}
\defres{mm/xcell/flash/memory_read/guard/losses}{0}
\defres{mm/xcell/flash/memory_read/guard/n}{200}
\defres{mm/xcell/flash/memory_read/guard/row}{mr\_guard}
\defres{mm/xcell/flash/memory_read/guard/saving}{-139.8}
\defres{mm/xcell/flash/memory_read/guard/state}{exploratory}
\defres{mm/xcell/flash/memory_read/guard/vcode}{3}
\defres{mm/xcell/flash/memory_read/guard/verdict}{no saving}
\defres{mm/xcell/flash/memory_read/guard/wins}{0}
\defres{mm/xcell/flash/memory_read/replace/acc}{57.2}
\defres{mm/xcell/flash/memory_read/replace/acted}{100.0}
\defres{mm/xcell/flash/memory_read/replace/coverage}{100.0}
\defres{mm/xcell/flash/memory_read/replace/delta}{+0.5}
\defres{mm/xcell/flash/memory_read/replace/equiv}{assist}
\defres{mm/xcell/flash/memory_read/replace/equiv_note}{with k = 1}
\defres{mm/xcell/flash/memory_read/replace/explore}{E6e}
\defres{mm/xcell/flash/memory_read/replace/fig_delta}{+0.5}
\defres{mm/xcell/flash/memory_read/replace/fig_saving}{-11}
\defres{mm/xcell/flash/memory_read/replace/losses}{0}
\defres{mm/xcell/flash/memory_read/replace/n}{200}
\defres{mm/xcell/flash/memory_read/replace/row}{mr\_replace}
\defres{mm/xcell/flash/memory_read/replace/saving}{-11.1}
\defres{mm/xcell/flash/memory_read/replace/state}{exploratory}
\defres{mm/xcell/flash/memory_read/replace/vcode}{3}
\defres{mm/xcell/flash/memory_read/replace/verdict}{no saving}
\defres{mm/xcell/flash/memory_read/replace/wins}{1}
\defres{mm/xcell/flash/memory_read/trigger/acc}{24.8}
\defres{mm/xcell/flash/memory_read/trigger/acted}{0.0}
\defres{mm/xcell/flash/memory_read/trigger/coverage}{100.0}
\defres{mm/xcell/flash/memory_read/trigger/delta}{+0.0}
\defres{mm/xcell/flash/memory_read/trigger/explore}{E6b}
\defres{mm/xcell/flash/memory_read/trigger/fig_delta}{+0.0}
\defres{mm/xcell/flash/memory_read/trigger/fig_saving}{-1}
\defres{mm/xcell/flash/memory_read/trigger/losses}{0}
\defres{mm/xcell/flash/memory_read/trigger/n}{200}
\defres{mm/xcell/flash/memory_read/trigger/row}{mr\_trigger}
\defres{mm/xcell/flash/memory_read/trigger/saving}{-0.9}
\defres{mm/xcell/flash/memory_read/trigger/state}{exploratory}
\defres{mm/xcell/flash/memory_read/trigger/vcode}{3}
\defres{mm/xcell/flash/memory_read/trigger/verdict}{no saving}
\defres{mm/xcell/flash/memory_read/trigger/wins}{0}
\defres{mm/xcell/flash/memory_write/assist/acc}{69.3}
\defres{mm/xcell/flash/memory_write/assist/acted}{100.0}
\defres{mm/xcell/flash/memory_write/assist/coverage}{0.0}
\defres{mm/xcell/flash/memory_write/assist/delta}{+0.0}
\defres{mm/xcell/flash/memory_write/assist/explore}{E6d}
\defres{mm/xcell/flash/memory_write/assist/fig_delta}{+0.0}
\defres{mm/xcell/flash/memory_write/assist/fig_saving}{-74}
\defres{mm/xcell/flash/memory_write/assist/losses}{0}
\defres{mm/xcell/flash/memory_write/assist/n}{200}
\defres{mm/xcell/flash/memory_write/assist/row}{mw\_assist}
\defres{mm/xcell/flash/memory_write/assist/saving}{-74.2}
\defres{mm/xcell/flash/memory_write/assist/state}{exploratory}
\defres{mm/xcell/flash/memory_write/assist/vcode}{3}
\defres{mm/xcell/flash/memory_write/assist/verdict}{no saving}
\defres{mm/xcell/flash/memory_write/assist/wins}{0}
\defres{mm/xcell/flash/memory_write/cascade/acc}{100.0}
\defres{mm/xcell/flash/memory_write/cascade/acted}{44.0}
\defres{mm/xcell/flash/memory_write/cascade/coverage}{44.0}
\defres{mm/xcell/flash/memory_write/cascade/delta}{-1.0}
\defres{mm/xcell/flash/memory_write/cascade/explore}{E6b}
\defres{mm/xcell/flash/memory_write/cascade/fig_delta}{-1.0}
\defres{mm/xcell/flash/memory_write/cascade/fig_saving}{-48}
\defres{mm/xcell/flash/memory_write/cascade/losses}{3}
\defres{mm/xcell/flash/memory_write/cascade/n}{200}
\defres{mm/xcell/flash/memory_write/cascade/row}{mw\_cascade}
\defres{mm/xcell/flash/memory_write/cascade/saving}{-48.1}
\defres{mm/xcell/flash/memory_write/cascade/state}{exploratory}
\defres{mm/xcell/flash/memory_write/cascade/vcode}{3}
\defres{mm/xcell/flash/memory_write/cascade/verdict}{no saving}
\defres{mm/xcell/flash/memory_write/cascade/wins}{1}
\defres{mm/xcell/flash/memory_write/guard/acc}{96.8}
\defres{mm/xcell/flash/memory_write/guard/acted}{0.0}
\defres{mm/xcell/flash/memory_write/guard/coverage}{0.0}
\defres{mm/xcell/flash/memory_write/guard/delta}{+0.0}
\defres{mm/xcell/flash/memory_write/guard/explore}{E6b}
\defres{mm/xcell/flash/memory_write/guard/fig_delta}{+0.0}
\defres{mm/xcell/flash/memory_write/guard/fig_saving}{-60}
\defres{mm/xcell/flash/memory_write/guard/losses}{0}
\defres{mm/xcell/flash/memory_write/guard/n}{200}
\defres{mm/xcell/flash/memory_write/guard/row}{mw\_guard}
\defres{mm/xcell/flash/memory_write/guard/saving}{-60.3}
\defres{mm/xcell/flash/memory_write/guard/state}{exploratory}
\defres{mm/xcell/flash/memory_write/guard/vcode}{3}
\defres{mm/xcell/flash/memory_write/guard/verdict}{no saving}
\defres{mm/xcell/flash/memory_write/guard/wins}{0}
\defres{mm/xcell/flash/memory_write/replace/acc}{69.4}
\defres{mm/xcell/flash/memory_write/replace/acted}{100.0}
\defres{mm/xcell/flash/memory_write/replace/coverage}{100.0}
\defres{mm/xcell/flash/memory_write/replace/delta}{+0.5}
\defres{mm/xcell/flash/memory_write/replace/equiv}{trigger}
\defres{mm/xcell/flash/memory_write/replace/equiv_note}{at tau = 0.5}
\defres{mm/xcell/flash/memory_write/replace/explore}{E6e}
\defres{mm/xcell/flash/memory_write/replace/fig_delta}{+0.5}
\defres{mm/xcell/flash/memory_write/replace/fig_saving}{-47}
\defres{mm/xcell/flash/memory_write/replace/losses}{0}
\defres{mm/xcell/flash/memory_write/replace/n}{200}
\defres{mm/xcell/flash/memory_write/replace/row}{mw\_replace}
\defres{mm/xcell/flash/memory_write/replace/saving}{-47.4}
\defres{mm/xcell/flash/memory_write/replace/state}{exploratory}
\defres{mm/xcell/flash/memory_write/replace/vcode}{3}
\defres{mm/xcell/flash/memory_write/replace/verdict}{no saving}
\defres{mm/xcell/flash/memory_write/replace/wins}{1}
\defres{mm/xcell/flash/reflection/assist/acc}{69.0}
\defres{mm/xcell/flash/reflection/assist/acted}{100.0}
\defres{mm/xcell/flash/reflection/assist/coverage}{0.0}
\defres{mm/xcell/flash/reflection/assist/delta}{-0.5}
\defres{mm/xcell/flash/reflection/assist/explore}{E6d}
\defres{mm/xcell/flash/reflection/assist/fig_delta}{-0.5}
\defres{mm/xcell/flash/reflection/assist/fig_saving}{-66}
\defres{mm/xcell/flash/reflection/assist/losses}{1}
\defres{mm/xcell/flash/reflection/assist/n}{200}
\defres{mm/xcell/flash/reflection/assist/row}{rf\_assist}
\defres{mm/xcell/flash/reflection/assist/saving}{-65.7}
\defres{mm/xcell/flash/reflection/assist/state}{exploratory}
\defres{mm/xcell/flash/reflection/assist/vcode}{3}
\defres{mm/xcell/flash/reflection/assist/verdict}{no saving}
\defres{mm/xcell/flash/reflection/assist/wins}{0}
\defres{mm/xcell/flash/reflection/cascade/acc}{100.0}
\defres{mm/xcell/flash/reflection/cascade/acted}{6.4}
\defres{mm/xcell/flash/reflection/cascade/coverage}{6.4}
\defres{mm/xcell/flash/reflection/cascade/delta}{+0.5}
\defres{mm/xcell/flash/reflection/cascade/explore}{E6b}
\defres{mm/xcell/flash/reflection/cascade/fig_delta}{+0.5}
\defres{mm/xcell/flash/reflection/cascade/fig_saving}{-25}
\defres{mm/xcell/flash/reflection/cascade/losses}{0}
\defres{mm/xcell/flash/reflection/cascade/n}{200}
\defres{mm/xcell/flash/reflection/cascade/row}{rf\_cascade}
\defres{mm/xcell/flash/reflection/cascade/saving}{-25.4}
\defres{mm/xcell/flash/reflection/cascade/state}{exploratory}
\defres{mm/xcell/flash/reflection/cascade/vcode}{3}
\defres{mm/xcell/flash/reflection/cascade/verdict}{no saving}
\defres{mm/xcell/flash/reflection/cascade/wins}{1}
\defres{mm/xcell/flash/reflection/guard/acc}{100.0}
\defres{mm/xcell/flash/reflection/guard/acted}{90.9}
\defres{mm/xcell/flash/reflection/guard/coverage}{0.0}
\defres{mm/xcell/flash/reflection/guard/delta}{+0.0}
\defres{mm/xcell/flash/reflection/guard/explore}{E6d}
\defres{mm/xcell/flash/reflection/guard/fig_delta}{+0.0}
\defres{mm/xcell/flash/reflection/guard/fig_saving}{-61}
\defres{mm/xcell/flash/reflection/guard/losses}{0}
\defres{mm/xcell/flash/reflection/guard/n}{200}
\defres{mm/xcell/flash/reflection/guard/row}{rf\_guard}
\defres{mm/xcell/flash/reflection/guard/saving}{-61.2}
\defres{mm/xcell/flash/reflection/guard/state}{exploratory}
\defres{mm/xcell/flash/reflection/guard/vcode}{3}
\defres{mm/xcell/flash/reflection/guard/verdict}{no saving}
\defres{mm/xcell/flash/reflection/guard/wins}{0}
\defres{mm/xcell/flash/reflection/replace/acc}{99.9}
\defres{mm/xcell/flash/reflection/replace/acted}{100.0}
\defres{mm/xcell/flash/reflection/replace/coverage}{100.0}
\defres{mm/xcell/flash/reflection/replace/delta}{-0.5}
\defres{mm/xcell/flash/reflection/replace/equiv}{trigger}
\defres{mm/xcell/flash/reflection/replace/equiv_note}{at tau = 0.5}
\defres{mm/xcell/flash/reflection/replace/explore}{E6e}
\defres{mm/xcell/flash/reflection/replace/fig_delta}{-0.5}
\defres{mm/xcell/flash/reflection/replace/fig_saving}{-7}
\defres{mm/xcell/flash/reflection/replace/losses}{1}
\defres{mm/xcell/flash/reflection/replace/n}{200}
\defres{mm/xcell/flash/reflection/replace/row}{rf\_replace}
\defres{mm/xcell/flash/reflection/replace/saving}{-7.2}
\defres{mm/xcell/flash/reflection/replace/state}{exploratory}
\defres{mm/xcell/flash/reflection/replace/vcode}{3}
\defres{mm/xcell/flash/reflection/replace/verdict}{no saving}
\defres{mm/xcell/flash/reflection/replace/wins}{0}
\defres{mm/xcell/flash/routing/assist/acc}{92.8}
\defres{mm/xcell/flash/routing/assist/acted}{100.0}
\defres{mm/xcell/flash/routing/assist/coverage}{0.0}
\defres{mm/xcell/flash/routing/assist/delta}{-2.0}
\defres{mm/xcell/flash/routing/assist/explore}{E6d}
\defres{mm/xcell/flash/routing/assist/fig_delta}{-2.0}
\defres{mm/xcell/flash/routing/assist/fig_saving}{-31}
\defres{mm/xcell/flash/routing/assist/losses}{11}
\defres{mm/xcell/flash/routing/assist/n}{200}
\defres{mm/xcell/flash/routing/assist/row}{rt\_assist}
\defres{mm/xcell/flash/routing/assist/saving}{-31.0}
\defres{mm/xcell/flash/routing/assist/state}{exploratory}
\defres{mm/xcell/flash/routing/assist/vcode}{3}
\defres{mm/xcell/flash/routing/assist/verdict}{no saving}
\defres{mm/xcell/flash/routing/assist/wins}{7}
\defres{mm/xcell/flash/routing/cascade/acc}{100.0}
\defres{mm/xcell/flash/routing/cascade/acted}{5.5}
\defres{mm/xcell/flash/routing/cascade/coverage}{5.5}
\defres{mm/xcell/flash/routing/cascade/delta}{-4.0}
\defres{mm/xcell/flash/routing/cascade/explore}{E6b}
\defres{mm/xcell/flash/routing/cascade/fig_delta}{-4.0}
\defres{mm/xcell/flash/routing/cascade/fig_saving}{-113}
\defres{mm/xcell/flash/routing/cascade/losses}{12}
\defres{mm/xcell/flash/routing/cascade/n}{200}
\defres{mm/xcell/flash/routing/cascade/row}{rt\_cascade}
\defres{mm/xcell/flash/routing/cascade/saving}{-113.1}
\defres{mm/xcell/flash/routing/cascade/state}{exploratory}
\defres{mm/xcell/flash/routing/cascade/vcode}{4}
\defres{mm/xcell/flash/routing/cascade/verdict}{costs success}
\defres{mm/xcell/flash/routing/cascade/wins}{4}
\defres{mm/xcell/flash/routing/guard/acc}{100.0}
\defres{mm/xcell/flash/routing/guard/acted}{95.8}
\defres{mm/xcell/flash/routing/guard/coverage}{0.0}
\defres{mm/xcell/flash/routing/guard/delta}{+0.0}
\defres{mm/xcell/flash/routing/guard/explore}{E6d}
\defres{mm/xcell/flash/routing/guard/fig_delta}{+0.0}
\defres{mm/xcell/flash/routing/guard/fig_saving}{-23}
\defres{mm/xcell/flash/routing/guard/losses}{8}
\defres{mm/xcell/flash/routing/guard/n}{200}
\defres{mm/xcell/flash/routing/guard/row}{rt\_guard}
\defres{mm/xcell/flash/routing/guard/saving}{-22.6}
\defres{mm/xcell/flash/routing/guard/state}{exploratory}
\defres{mm/xcell/flash/routing/guard/vcode}{3}
\defres{mm/xcell/flash/routing/guard/verdict}{no saving}
\defres{mm/xcell/flash/routing/guard/wins}{8}
\defres{mm/xcell/flash/routing/replace/acc}{97.8}
\defres{mm/xcell/flash/routing/replace/acted}{100.0}
\defres{mm/xcell/flash/routing/replace/coverage}{100.0}
\defres{mm/xcell/flash/routing/replace/delta}{+4.0}
\defres{mm/xcell/flash/routing/replace/equiv}{trigger}
\defres{mm/xcell/flash/routing/replace/equiv_note}{at tau = 0.5}
\defres{mm/xcell/flash/routing/replace/explore}{E6e}
\defres{mm/xcell/flash/routing/replace/fig_delta}{+4.0}
\defres{mm/xcell/flash/routing/replace/fig_saving}{-7}
\defres{mm/xcell/flash/routing/replace/losses}{3}
\defres{mm/xcell/flash/routing/replace/n}{200}
\defres{mm/xcell/flash/routing/replace/row}{rt\_replace}
\defres{mm/xcell/flash/routing/replace/saving}{-6.7}
\defres{mm/xcell/flash/routing/replace/state}{exploratory}
\defres{mm/xcell/flash/routing/replace/vcode}{3}
\defres{mm/xcell/flash/routing/replace/verdict}{no saving}
\defres{mm/xcell/flash/routing/replace/wins}{11}
\defres{mm/xcell/flash/stop/assist/acc}{99.3}
\defres{mm/xcell/flash/stop/assist/acted}{100.0}
\defres{mm/xcell/flash/stop/assist/coverage}{0.0}
\defres{mm/xcell/flash/stop/assist/delta}{+0.0}
\defres{mm/xcell/flash/stop/assist/explore}{E6d}
\defres{mm/xcell/flash/stop/assist/fig_delta}{+0.0}
\defres{mm/xcell/flash/stop/assist/fig_saving}{-17}
\defres{mm/xcell/flash/stop/assist/losses}{0}
\defres{mm/xcell/flash/stop/assist/n}{200}
\defres{mm/xcell/flash/stop/assist/row}{st\_assist}
\defres{mm/xcell/flash/stop/assist/saving}{-16.7}
\defres{mm/xcell/flash/stop/assist/state}{exploratory}
\defres{mm/xcell/flash/stop/assist/vcode}{3}
\defres{mm/xcell/flash/stop/assist/verdict}{no saving}
\defres{mm/xcell/flash/stop/assist/wins}{0}
\defres{mm/xcell/flash/stop/cascade/acc}{100.0}
\defres{mm/xcell/flash/stop/cascade/acted}{94.2}
\defres{mm/xcell/flash/stop/cascade/coverage}{94.2}
\defres{mm/xcell/flash/stop/cascade/delta}{+0.0}
\defres{mm/xcell/flash/stop/cascade/explore}{E6b}
\defres{mm/xcell/flash/stop/cascade/fig_delta}{+0.0}
\defres{mm/xcell/flash/stop/cascade/fig_saving}{-1}
\defres{mm/xcell/flash/stop/cascade/losses}{0}
\defres{mm/xcell/flash/stop/cascade/n}{200}
\defres{mm/xcell/flash/stop/cascade/row}{st\_cascade}
\defres{mm/xcell/flash/stop/cascade/saving}{-0.7}
\defres{mm/xcell/flash/stop/cascade/state}{exploratory}
\defres{mm/xcell/flash/stop/cascade/vcode}{3}
\defres{mm/xcell/flash/stop/cascade/verdict}{no saving}
\defres{mm/xcell/flash/stop/cascade/wins}{0}
\defres{mm/xcell/flash/stop/replace/acc}{98.1}
\defres{mm/xcell/flash/stop/replace/acted}{100.0}
\defres{mm/xcell/flash/stop/replace/coverage}{100.0}
\defres{mm/xcell/flash/stop/replace/delta}{+0.5}
\defres{mm/xcell/flash/stop/replace/equiv}{cascade}
\defres{mm/xcell/flash/stop/replace/equiv_note}{at tau = 0.5}
\defres{mm/xcell/flash/stop/replace/explore}{E6e}
\defres{mm/xcell/flash/stop/replace/fig_delta}{+0.5}
\defres{mm/xcell/flash/stop/replace/fig_saving}{-7}
\defres{mm/xcell/flash/stop/replace/losses}{0}
\defres{mm/xcell/flash/stop/replace/n}{200}
\defres{mm/xcell/flash/stop/replace/row}{st\_replace}
\defres{mm/xcell/flash/stop/replace/saving}{-6.8}
\defres{mm/xcell/flash/stop/replace/state}{exploratory}
\defres{mm/xcell/flash/stop/replace/vcode}{3}
\defres{mm/xcell/flash/stop/replace/verdict}{no saving}
\defres{mm/xcell/flash/stop/replace/wins}{1}
\defres{mm/xcell/flash/tool_params/assist/acc}{98.8}
\defres{mm/xcell/flash/tool_params/assist/acted}{100.0}
\defres{mm/xcell/flash/tool_params/assist/coverage}{0.0}
\defres{mm/xcell/flash/tool_params/assist/delta}{+0.0}
\defres{mm/xcell/flash/tool_params/assist/explore}{E6b}
\defres{mm/xcell/flash/tool_params/assist/fig_delta}{+0.0}
\defres{mm/xcell/flash/tool_params/assist/fig_saving}{9}
\defres{mm/xcell/flash/tool_params/assist/losses}{0}
\defres{mm/xcell/flash/tool_params/assist/n}{200}
\defres{mm/xcell/flash/tool_params/assist/row}{tp\_assist}
\defres{mm/xcell/flash/tool_params/assist/saving}{8.9}
\defres{mm/xcell/flash/tool_params/assist/state}{exploratory}
\defres{mm/xcell/flash/tool_params/assist/vcode}{1}
\defres{mm/xcell/flash/tool_params/assist/verdict}{takes over safely}
\defres{mm/xcell/flash/tool_params/assist/wins}{0}
\defres{mm/xcell/flash/tool_params/guard/acc}{93.8}
\defres{mm/xcell/flash/tool_params/guard/acted}{6.3}
\defres{mm/xcell/flash/tool_params/guard/coverage}{0.0}
\defres{mm/xcell/flash/tool_params/guard/delta}{+0.0}
\defres{mm/xcell/flash/tool_params/guard/explore}{E6b}
\defres{mm/xcell/flash/tool_params/guard/fig_delta}{+0.0}
\defres{mm/xcell/flash/tool_params/guard/fig_saving}{-7}
\defres{mm/xcell/flash/tool_params/guard/losses}{0}
\defres{mm/xcell/flash/tool_params/guard/n}{200}
\defres{mm/xcell/flash/tool_params/guard/row}{tp\_guard}
\defres{mm/xcell/flash/tool_params/guard/saving}{-6.7}
\defres{mm/xcell/flash/tool_params/guard/state}{exploratory}
\defres{mm/xcell/flash/tool_params/guard/vcode}{3}
\defres{mm/xcell/flash/tool_params/guard/verdict}{no saving}
\defres{mm/xcell/flash/tool_params/guard/wins}{0}
\defres{mm/xcell/flash/tool_params/trigger/acc}{100.0}
\defres{mm/xcell/flash/tool_params/trigger/acted}{0.0}
\defres{mm/xcell/flash/tool_params/trigger/coverage}{100.0}
\defres{mm/xcell/flash/tool_params/trigger/delta}{+0.0}
\defres{mm/xcell/flash/tool_params/trigger/explore}{E6f}
\defres{mm/xcell/flash/tool_params/trigger/fig_delta}{+0.0}
\defres{mm/xcell/flash/tool_params/trigger/fig_saving}{-1}
\defres{mm/xcell/flash/tool_params/trigger/losses}{0}
\defres{mm/xcell/flash/tool_params/trigger/n}{100}
\defres{mm/xcell/flash/tool_params/trigger/row}{tp\_trigger}
\defres{mm/xcell/flash/tool_params/trigger/saving}{-1.2}
\defres{mm/xcell/flash/tool_params/trigger/state}{exploratory}
\defres{mm/xcell/flash/tool_params/trigger/vcode}{3}
\defres{mm/xcell/flash/tool_params/trigger/verdict}{no saving}
\defres{mm/xcell/flash/tool_params/trigger/wins}{0}
\defres{mm/xcell/flash/tool_select/trigger/acc}{86.3}
\defres{mm/xcell/flash/tool_select/trigger/acted}{13.7}
\defres{mm/xcell/flash/tool_select/trigger/coverage}{100.0}
\defres{mm/xcell/flash/tool_select/trigger/delta}{+0.0}
\defres{mm/xcell/flash/tool_select/trigger/explore}{E6f}
\defres{mm/xcell/flash/tool_select/trigger/fig_delta}{+0.0}
\defres{mm/xcell/flash/tool_select/trigger/fig_saving}{-14}
\defres{mm/xcell/flash/tool_select/trigger/losses}{0}
\defres{mm/xcell/flash/tool_select/trigger/n}{100}
\defres{mm/xcell/flash/tool_select/trigger/row}{ts\_trigger}
\defres{mm/xcell/flash/tool_select/trigger/saving}{-14.2}
\defres{mm/xcell/flash/tool_select/trigger/state}{exploratory}
\defres{mm/xcell/flash/tool_select/trigger/vcode}{3}
\defres{mm/xcell/flash/tool_select/trigger/verdict}{no saving}
\defres{mm/xcell/flash/tool_select/trigger/wins}{0}
\defres{mm/xcell/lite/routing/assist/acc}{92.8}
\defres{mm/xcell/lite/routing/assist/acted}{100.0}
\defres{mm/xcell/lite/routing/assist/coverage}{0.0}
\defres{mm/xcell/lite/routing/assist/delta}{-2.0}
\defres{mm/xcell/lite/routing/assist/explore}{E6d}
\defres{mm/xcell/lite/routing/assist/fig_delta}{-2.0}
\defres{mm/xcell/lite/routing/assist/fig_saving}{-31}
\defres{mm/xcell/lite/routing/assist/losses}{11}
\defres{mm/xcell/lite/routing/assist/n}{200}
\defres{mm/xcell/lite/routing/assist/row}{rt\_assist}
\defres{mm/xcell/lite/routing/assist/saving}{-31.0}
\defres{mm/xcell/lite/routing/assist/state}{exploratory}
\defres{mm/xcell/lite/routing/assist/vcode}{3}
\defres{mm/xcell/lite/routing/assist/verdict}{no saving}
\defres{mm/xcell/lite/routing/assist/wins}{7}
\defres{mm/xcell/lite/routing/cascade/acc}{100.0}
\defres{mm/xcell/lite/routing/cascade/acted}{5.5}
\defres{mm/xcell/lite/routing/cascade/coverage}{5.5}
\defres{mm/xcell/lite/routing/cascade/delta}{-4.0}
\defres{mm/xcell/lite/routing/cascade/explore}{E6b}
\defres{mm/xcell/lite/routing/cascade/fig_delta}{-4.0}
\defres{mm/xcell/lite/routing/cascade/fig_saving}{-113}
\defres{mm/xcell/lite/routing/cascade/losses}{12}
\defres{mm/xcell/lite/routing/cascade/n}{200}
\defres{mm/xcell/lite/routing/cascade/row}{rt\_cascade}
\defres{mm/xcell/lite/routing/cascade/saving}{-113.1}
\defres{mm/xcell/lite/routing/cascade/state}{exploratory}
\defres{mm/xcell/lite/routing/cascade/vcode}{4}
\defres{mm/xcell/lite/routing/cascade/verdict}{costs success}
\defres{mm/xcell/lite/routing/cascade/wins}{4}
\defres{mm/xcell/lite/routing/guard/acc}{100.0}
\defres{mm/xcell/lite/routing/guard/acted}{95.8}
\defres{mm/xcell/lite/routing/guard/coverage}{0.0}
\defres{mm/xcell/lite/routing/guard/delta}{+0.0}
\defres{mm/xcell/lite/routing/guard/explore}{E6d}
\defres{mm/xcell/lite/routing/guard/fig_delta}{+0.0}
\defres{mm/xcell/lite/routing/guard/fig_saving}{-23}
\defres{mm/xcell/lite/routing/guard/losses}{8}
\defres{mm/xcell/lite/routing/guard/n}{200}
\defres{mm/xcell/lite/routing/guard/row}{rt\_guard}
\defres{mm/xcell/lite/routing/guard/saving}{-22.6}
\defres{mm/xcell/lite/routing/guard/state}{exploratory}
\defres{mm/xcell/lite/routing/guard/vcode}{3}
\defres{mm/xcell/lite/routing/guard/verdict}{no saving}
\defres{mm/xcell/lite/routing/guard/wins}{8}
\defres{mm/xcell/lite/routing/replace/acc}{97.8}
\defres{mm/xcell/lite/routing/replace/acted}{100.0}
\defres{mm/xcell/lite/routing/replace/coverage}{100.0}
\defres{mm/xcell/lite/routing/replace/delta}{+4.0}
\defres{mm/xcell/lite/routing/replace/equiv}{trigger}
\defres{mm/xcell/lite/routing/replace/equiv_note}{at tau = 0.5}
\defres{mm/xcell/lite/routing/replace/explore}{E6e}
\defres{mm/xcell/lite/routing/replace/fig_delta}{+4.0}
\defres{mm/xcell/lite/routing/replace/fig_saving}{-7}
\defres{mm/xcell/lite/routing/replace/losses}{3}
\defres{mm/xcell/lite/routing/replace/n}{200}
\defres{mm/xcell/lite/routing/replace/row}{rt\_replace}
\defres{mm/xcell/lite/routing/replace/saving}{-6.7}
\defres{mm/xcell/lite/routing/replace/state}{exploratory}
\defres{mm/xcell/lite/routing/replace/vcode}{3}
\defres{mm/xcell/lite/routing/replace/verdict}{no saving}
\defres{mm/xcell/lite/routing/replace/wins}{11}
\makeatother


==> generated/primaries.tex <==
\makeatletter
\providecommand{\res}[1]{\ifcsname jevres@#1\endcsname\csname jevres@#1\endcsname\else\tbd\fi}
\providecommand{\defres}[2]{\expandafter\def\csname jevres@#1\endcsname{#2}}
\defres{primaries/C1F/alpha_adj}{0.005}
\defres{primaries/C1F/decision}{NI: policy NI with zero coverage for Intern-Decision (A6.11 (c).4, A6.12, A6.16 (m), A6.20 (e), A6.22 (a))}
\defres{primaries/C1F/full_set_family/p_decisive}{$<$0.001}
\defres{primaries/C1F/full_set_family/p_holm}{0.001}
\defres{primaries/C1F/holm_rank}{2}
\defres{primaries/C1F/intern/arg_coverage}{0.0}
\defres{primaries/C1F/intern/coverage}{0.0}
\defres{primaries/C1F/intern/delta}{+0.2}
\defres{primaries/C1F/intern/delta_ci/hi}{+0.6}
\defres{primaries/C1F/intern/delta_ci/lo}{+0.0}
\defres{primaries/C1F/intern/discordance}{0.2}
\defres{primaries/C1F/intern/full_set/delta}{+0.2}
\defres{primaries/C1F/intern/full_set/p_decisive}{$<$0.001}
\defres{primaries/C1F/intern/loss_rate_ub}{0.6}
\defres{primaries/C1F/intern/losses}{0}
\defres{primaries/C1F/intern/mde}{-2.5}
\defres{primaries/C1F/intern/n_dropped}{0}
\defres{primaries/C1F/intern/n_expected}{500}
\defres{primaries/C1F/intern/n_pairs}{500}
\defres{primaries/C1F/intern/p_decisive}{$<$0.001}
\defres{primaries/C1F/intern/readouts/cost_arm}{0.0437}
\defres{primaries/C1F/intern/readouts/cost_ref}{0.0436}
\defres{primaries/C1F/intern/readouts/cost_savings}{-0.2}
\defres{primaries/C1F/intern/readouts/cost_savings_ci/hi}{0.4}
\defres{primaries/C1F/intern/readouts/cost_savings_ci/lo}{-0.7}
\defres{primaries/C1F/intern/readouts/token_savings}{-0.0}
\defres{primaries/C1F/intern/success_arm}{99.8}
\defres{primaries/C1F/intern/success_ref}{99.6}
\defres{primaries/C1F/intern/tango_lcb_adj}{-1.1}
\defres{primaries/C1F/intern/tool_coverage}{0.0}
\defres{primaries/C1F/intern/wins}{1}
\defres{primaries/C1F/jev/arg_coverage}{20.8}
\defres{primaries/C1F/jev/coverage}{40.6}
\defres{primaries/C1F/jev/delta}{+0.0}
\defres{primaries/C1F/jev/delta_ci/hi}{+0.0}
\defres{primaries/C1F/jev/delta_ci/lo}{+0.0}
\defres{primaries/C1F/jev/discordance}{0.0}
\defres{primaries/C1F/jev/full_set/delta}{+0.0}
\defres{primaries/C1F/jev/full_set/p_decisive}{$<$0.001}
\defres{primaries/C1F/jev/loss_rate_ub}{0.6}
\defres{primaries/C1F/jev/losses}{0}
\defres{primaries/C1F/jev/n_dropped}{0}
\defres{primaries/C1F/jev/n_expected}{500}
\defres{primaries/C1F/jev/n_pairs}{500}
\defres{primaries/C1F/jev/p_decisive}{$<$0.001}
\defres{primaries/C1F/jev/readouts/cost_arm}{0.0364}
\defres{primaries/C1F/jev/readouts/cost_ref}{0.0424}
\defres{primaries/C1F/jev/readouts/cost_savings}{14.2}
\defres{primaries/C1F/jev/readouts/cost_savings_ci/hi}{15.7}
\defres{primaries/C1F/jev/readouts/cost_savings_ci/lo}{12.7}
\defres{primaries/C1F/jev/readouts/token_savings}{25.5}
\defres{primaries/C1F/jev/success_arm}{99.8}
\defres{primaries/C1F/jev/success_ref}{99.8}
\defres{primaries/C1F/jev/tango_lcb_adj}{-1.3}
\defres{primaries/C1F/jev/tool_coverage}{27.2}
\defres{primaries/C1F/jev/wins}{0}
\defres{primaries/C1F/p_decisive}{$<$0.001}
\defres{primaries/C1F/p_holm}{0.001}
\defres{primaries/C1F/replication}{cross-backend replication of policy NI}
\defres{primaries/C1F/rule}{max(p\_Jev, p\_Intern)}
\defres{primaries/C1L/alpha_adj}{0.007}
\defres{primaries/C1L/decision}{not NI as a conjunction: Jev NI; Intern-Decision inconclusive at this n}
\defres{primaries/C1L/full_set_family/p_decisive}{0.024}
\defres{primaries/C1L/full_set_family/p_holm}{0.168}
\defres{primaries/C1L/holm_rank}{5}
\defres{primaries/C1L/intern/arg_coverage}{0.0}
\defres{primaries/C1L/intern/coverage}{0.0}
\defres{primaries/C1L/intern/delta}{-0.6}
\defres{primaries/C1L/intern/delta_ci/hi}{+1.6}
\defres{primaries/C1L/intern/delta_ci/lo}{-2.8}
\defres{primaries/C1L/intern/discordance}{6.6}
\defres{primaries/C1L/intern/full_set/delta}{-0.6}
\defres{primaries/C1L/intern/full_set/p_decisive}{0.024}
\defres{primaries/C1L/intern/losses}{18}
\defres{primaries/C1L/intern/mde}{+0.8}
\defres{primaries/C1L/intern/n_dropped}{0}
\defres{primaries/C1L/intern/n_expected}{500}
\defres{primaries/C1L/intern/n_pairs}{500}
\defres{primaries/C1L/intern/p_decisive}{0.024}
\defres{primaries/C1L/intern/readouts/cost_arm}{0.00978}
\defres{primaries/C1L/intern/readouts/cost_ref}{0.00988}
\defres{primaries/C1L/intern/readouts/cost_savings}{1.0}
\defres{primaries/C1L/intern/readouts/cost_savings_ci/hi}{1.4}
\defres{primaries/C1L/intern/readouts/cost_savings_ci/lo}{0.5}
\defres{primaries/C1L/intern/readouts/token_savings}{0.0}
\defres{primaries/C1L/intern/success_arm}{82.8}
\defres{primaries/C1L/intern/success_ref}{83.4}
\defres{primaries/C1L/intern/tango_lcb_adj}{-3.7}
\defres{primaries/C1L/intern/tool_coverage}{0.0}
\defres{primaries/C1L/intern/wins}{15}
\defres{primaries/C1L/jev/arg_coverage}{0.0}
\defres{primaries/C1L/jev/coverage}{0.0}
\defres{primaries/C1L/jev/delta}{+1.0}
\defres{primaries/C1L/jev/delta_ci/hi}{+3.2}
\defres{primaries/C1L/jev/delta_ci/lo}{-1.0}
\defres{primaries/C1L/jev/discordance}{5.8}
\defres{primaries/C1L/jev/full_set/delta}{+1.0}
\defres{primaries/C1L/jev/full_set/p_decisive}{$<$0.001}
\defres{primaries/C1L/jev/losses}{12}
\defres{primaries/C1L/jev/mde}{+0.5}
\defres{primaries/C1L/jev/n_dropped}{0}
\defres{primaries/C1L/jev/n_expected}{500}
\defres{primaries/C1L/jev/n_pairs}{500}
\defres{primaries/C1L/jev/p_decisive}{$<$0.001}
\defres{primaries/C1L/jev/readouts/cost_arm}{0.00978}
\defres{primaries/C1L/jev/readouts/cost_ref}{0.0098}
\defres{primaries/C1L/jev/readouts/cost_savings}{0.2}
\defres{primaries/C1L/jev/readouts/cost_savings_ci/hi}{0.7}
\defres{primaries/C1L/jev/readouts/cost_savings_ci/lo}{-0.3}
\defres{primaries/C1L/jev/readouts/token_savings}{0.2}
\defres{primaries/C1L/jev/success_arm}{81.2}
\defres{primaries/C1L/jev/success_ref}{80.2}
\defres{primaries/C1L/jev/tango_lcb_adj}{-1.8}
\defres{primaries/C1L/jev/tool_coverage}{0.0}
\defres{primaries/C1L/jev/wins}{17}
\defres{primaries/C1L/p_decisive}{0.024}
\defres{primaries/C1L/p_holm}{0.168}
\defres{primaries/C1L/replication}{split (Jev passes)}
\defres{primaries/C1L/rule}{max(p\_Jev, p\_Intern)}
\defres{primaries/C2F/alpha_adj}{0.025}
\defres{primaries/C2F/decision}{not NI as a conjunction: Jev not NI: loss of 7.8 pt (95 \% CI entirely below 0); Intern-Decision not NI: loss of 3.6 pt (95 \% CI entirely below 0)}
\defres{primaries/C2F/full_set_family/p_decisive}{1.000}
\defres{primaries/C2F/full_set_family/p_holm}{1.000}
\defres{primaries/C2F/holm_rank}{10}
\defres{primaries/C2F/intern/delta}{-3.6}
\defres{primaries/C2F/intern/delta_ci/hi}{-2.0}
\defres{primaries/C2F/intern/delta_ci/lo}{-5.4}
\defres{primaries/C2F/intern/discordance}{4.4}
\defres{primaries/C2F/intern/full_set/delta}{-3.6}
\defres{primaries/C2F/intern/full_set/p_decisive}{0.767}
\defres{primaries/C2F/intern/losses}{20}
\defres{primaries/C2F/intern/mde}{-0.4}
\defres{primaries/C2F/intern/n_dropped}{0}
\defres{primaries/C2F/intern/n_expected}{500}
\defres{primaries/C2F/intern/n_pairs}{500}
\defres{primaries/C2F/intern/p_decisive}{0.767}
\defres{primaries/C2F/intern/readouts/cost_arm}{0.0205}
\defres{primaries/C2F/intern/readouts/cost_ref}{0.0436}
\defres{primaries/C2F/intern/readouts/cost_savings}{53.0}
\defres{primaries/C2F/intern/readouts/cost_savings_ci/hi}{55.1}
\defres{primaries/C2F/intern/readouts/cost_savings_ci/lo}{50.5}
\defres{primaries/C2F/intern/readouts/token_savings}{73.6}
\defres{primaries/C2F/intern/success_arm}{96.0}
\defres{primaries/C2F/intern/success_ref}{99.6}
\defres{primaries/C2F/intern/tango_lcb_adj}{-5.7}
\defres{primaries/C2F/intern/wins}{2}
\defres{primaries/C2F/jev/delta}{-7.8}
\defres{primaries/C2F/jev/delta_ci/hi}{-5.4}
\defres{primaries/C2F/jev/delta_ci/lo}{-10.2}
\defres{primaries/C2F/jev/discordance}{8.2}
\defres{primaries/C2F/jev/full_set/delta}{-7.8}
\defres{primaries/C2F/jev/full_set/p_decisive}{1.000}
\defres{primaries/C2F/jev/losses}{40}
\defres{primaries/C2F/jev/mde}{+0.6}
\defres{primaries/C2F/jev/n_dropped}{0}
\defres{primaries/C2F/jev/n_expected}{500}
\defres{primaries/C2F/jev/n_pairs}{500}
\defres{primaries/C2F/jev/p_decisive}{1.000}
\defres{primaries/C2F/jev/readouts/cost_arm}{0.0196}
\defres{primaries/C2F/jev/readouts/cost_ref}{0.0424}
\defres{primaries/C2F/jev/readouts/cost_savings}{53.7}
\defres{primaries/C2F/jev/readouts/cost_savings_ci/hi}{54.6}
\defres{primaries/C2F/jev/readouts/cost_savings_ci/lo}{52.8}
\defres{primaries/C2F/jev/readouts/token_savings}{75.8}
\defres{primaries/C2F/jev/success_arm}{92.0}
\defres{primaries/C2F/jev/success_ref}{99.8}
\defres{primaries/C2F/jev/tango_lcb_adj}{-10.5}
\defres{primaries/C2F/jev/wins}{1}
\defres{primaries/C2F/p_decisive}{1.000}
\defres{primaries/C2F/p_holm}{1.000}
\defres{primaries/C2F/replication}{not reached (Holm step-down stopped at an earlier primary)}
\defres{primaries/C2F/rule}{max(p\_Jev, p\_Intern)}
\defres{primaries/C2L/alpha_adj}{0.050}
\defres{primaries/C2L/decision}{not NI as a conjunction: Jev inconclusive at this n; Intern-Decision not NI: loss of 14.8 pt (95 \% CI entirely below 0)}
\defres{primaries/C2L/full_set_family/p_decisive}{1.000}
\defres{primaries/C2L/full_set_family/p_holm}{1.000}
\defres{primaries/C2L/holm_rank}{11}
\defres{primaries/C2L/intern/delta}{-14.8}
\defres{primaries/C2L/intern/delta_ci/hi}{-10.6}
\defres{primaries/C2L/intern/delta_ci/lo}{-19.0}
\defres{primaries/C2L/intern/discordance}{25.6}
\defres{primaries/C2L/intern/full_set/delta}{-14.8}
\defres{primaries/C2L/intern/full_set/p_decisive}{1.000}
\defres{primaries/C2L/intern/losses}{101}
\defres{primaries/C2L/intern/mde}{+2.6}
\defres{primaries/C2L/intern/n_dropped}{0}
\defres{primaries/C2L/intern/n_expected}{500}
\defres{primaries/C2L/intern/n_pairs}{500}
\defres{primaries/C2L/intern/p_decisive}{1.000}
\defres{primaries/C2L/intern/readouts/cost_arm}{0.00458}
\defres{primaries/C2L/intern/readouts/cost_ref}{0.00988}
\defres{primaries/C2L/intern/readouts/cost_savings}{53.7}
\defres{primaries/C2L/intern/readouts/cost_savings_ci/hi}{56.6}
\defres{primaries/C2L/intern/readouts/cost_savings_ci/lo}{50.3}
\defres{primaries/C2L/intern/readouts/token_savings}{73.0}
\defres{primaries/C2L/intern/success_arm}{68.6}
\defres{primaries/C2L/intern/success_ref}{83.4}
\defres{primaries/C2L/intern/tango_lcb_adj}{-18.4}
\defres{primaries/C2L/intern/wins}{27}
\defres{primaries/C2L/jev/delta}{-3.4}
\defres{primaries/C2L/jev/delta_ci/hi}{+0.6}
\defres{primaries/C2L/jev/delta_ci/lo}{-7.2}
\defres{primaries/C2L/jev/discordance}{20.6}
\defres{primaries/C2L/jev/full_set/delta}{-3.4}
\defres{primaries/C2L/jev/full_set/p_decisive}{0.591}
\defres{primaries/C2L/jev/losses}{60}
\defres{primaries/C2L/jev/mde}{+2.0}
\defres{primaries/C2L/jev/n_dropped}{0}
\defres{primaries/C2L/jev/n_expected}{500}
\defres{primaries/C2L/jev/n_pairs}{500}
\defres{primaries/C2L/jev/p_decisive}{0.591}
\defres{primaries/C2L/jev/readouts/cost_arm}{0.0047}
\defres{primaries/C2L/jev/readouts/cost_ref}{0.0098}
\defres{primaries/C2L/jev/readouts/cost_savings}{52.0}
\defres{primaries/C2L/jev/readouts/cost_savings_ci/hi}{52.7}
\defres{primaries/C2L/jev/readouts/cost_savings_ci/lo}{51.2}
\defres{primaries/C2L/jev/readouts/token_savings}{76.6}
\defres{primaries/C2L/jev/success_arm}{76.8}
\defres{primaries/C2L/jev/success_ref}{80.2}
\defres{primaries/C2L/jev/tango_lcb_adj}{-6.8}
\defres{primaries/C2L/jev/wins}{43}
\defres{primaries/C2L/p_decisive}{1.000}
\defres{primaries/C2L/p_holm}{1.000}
\defres{primaries/C2L/replication}{not reached (Holm step-down stopped at an earlier primary)}
\defres{primaries/C2L/rule}{max(p\_Jev, p\_Intern)}
\defres{primaries/C3/alpha_adj}{0.005}
\defres{primaries/C3/decision}{superior}
\defres{primaries/C3/full_set_family/p_decisive}{$<$0.001}
\defres{primaries/C3/full_set_family/p_holm}{$<$0.001}
\defres{primaries/C3/holm_rank}{1}
\defres{primaries/C3/jev/delta}{+73.2}
\defres{primaries/C3/jev/delta_ci/hi}{+78.2}
\defres{primaries/C3/jev/delta_ci/lo}{+68.0}
\defres{primaries/C3/jev/discordance}{87.6}
\defres{primaries/C3/jev/full_set/delta}{+73.2}
\defres{primaries/C3/jev/full_set/p_decisive}{$<$0.001}
\defres{primaries/C3/jev/losses}{36}
\defres{primaries/C3/jev/mde}{+14.4}
\defres{primaries/C3/jev/n_dropped}{0}
\defres{primaries/C3/jev/n_expected}{500}
\defres{primaries/C3/jev/n_pairs}{500}
\defres{primaries/C3/jev/p_decisive}{$<$0.001}
\defres{primaries/C3/jev/success_arm}{92.0}
\defres{primaries/C3/jev/success_ref}{18.8}
\defres{primaries/C3/jev/wins}{402}
\defres{primaries/C3/p_decisive}{$<$0.001}
\defres{primaries/C3/p_holm}{$<$0.001}
\defres{primaries/C3/rule}{sign\_exact}
\defres{primaries/C4/alpha_adj}{0.008}
\defres{primaries/C4/decision}{superiority not established (Holm step-down stopped earlier)}
\defres{primaries/C4/full_set_family/p_decisive}{0.360}
\defres{primaries/C4/full_set_family/p_holm}{1.000}
\defres{primaries/C4/holm_rank}{6}
\defres{primaries/C4/jev/delta}{+0.6}
\defres{primaries/C4/jev/delta_ci/hi}{+2.8}
\defres{primaries/C4/jev/delta_ci/lo}{-1.6}
\defres{primaries/C4/jev/discordance}{6.2}
\defres{primaries/C4/jev/full_set/delta}{+0.6}
\defres{primaries/C4/jev/full_set/p_decisive}{0.360}
\defres{primaries/C4/jev/losses}{14}
\defres{primaries/C4/jev/mde}{+3.6}
\defres{primaries/C4/jev/n_dropped}{0}
\defres{primaries/C4/jev/n_expected}{500}
\defres{primaries/C4/jev/n_pairs}{500}
\defres{primaries/C4/jev/p_decisive}{0.360}
\defres{primaries/C4/jev/readouts/cost_arm}{0.0134}
\defres{primaries/C4/jev/readouts/cost_ref}{0.00981}
\defres{primaries/C4/jev/readouts/cost_savings}{-36.2}
\defres{primaries/C4/jev/readouts/cost_savings_ci/hi}{-33.3}
\defres{primaries/C4/jev/readouts/cost_savings_ci/lo}{-39.3}
\defres{primaries/C4/jev/readouts/token_savings}{-0.1}
\defres{primaries/C4/jev/success_arm}{81.4}
\defres{primaries/C4/jev/success_ref}{80.8}
\defres{primaries/C4/jev/wins}{17}
\defres{primaries/C4/p_decisive}{0.360}
\defres{primaries/C4/p_holm}{1.000}
\defres{primaries/C4/rule}{sign\_exact}
\defres{primaries/C5/alpha_adj}{0.013}
\defres{primaries/C5/decision}{superiority not established (Holm step-down stopped earlier)}
\defres{primaries/C5/full_set_family/p_decisive}{0.918}
\defres{primaries/C5/full_set_family/p_holm}{1.000}
\defres{primaries/C5/holm_rank}{8}
\defres{primaries/C5/jev/du_gross}{-0.0233}
\defres{primaries/C5/jev/du_gross_ci/hi}{0.0087}
\defres{primaries/C5/jev/du_gross_ci/lo}{-0.0557}
\defres{primaries/C5/jev/du_mde}{0.0516}
\defres{primaries/C5/jev/du_net}{-0.0236}
\defres{primaries/C5/jev/du_net_ci/hi}{0.00834}
\defres{primaries/C5/jev/du_net_ci/lo}{-0.0561}
\defres{primaries/C5/jev/full_set/du_gross}{-0.0233}
\defres{primaries/C5/jev/full_set/p_decisive}{0.918}
\defres{primaries/C5/jev/n_dropped}{0}
\defres{primaries/C5/jev/n_expected}{500}
\defres{primaries/C5/jev/n_pairs}{500}
\defres{primaries/C5/jev/p_decisive}{0.918}
\defres{primaries/C5/jev/success_arm}{83.0}
\defres{primaries/C5/jev/success_ref}{85.4}
\defres{primaries/C5/p_decisive}{0.918}
\defres{primaries/C5/p_holm}{1.000}
\defres{primaries/C5/rule}{paired\_t}
\defres{primaries/C6F/alpha_adj}{0.006}
\defres{primaries/C6F/decision}{NI}
\defres{primaries/C6F/full_set_family/p_decisive}{$<$0.001}
\defres{primaries/C6F/full_set_family/p_holm}{0.002}
\defres{primaries/C6F/holm_rank}{4}
\defres{primaries/C6F/intern/delta}{-0.4}
\defres{primaries/C6F/intern/delta_ci/hi}{+0.0}
\defres{primaries/C6F/intern/delta_ci/lo}{-1.0}
\defres{primaries/C6F/intern/discordance}{0.4}
\defres{primaries/C6F/intern/full_set/delta}{-0.4}
\defres{primaries/C6F/intern/full_set/p_decisive}{$<$0.001}
\defres{primaries/C6F/intern/loss_rate_ub}{1.3}
\defres{primaries/C6F/intern/losses}{2}
\defres{primaries/C6F/intern/mde}{-2.2}
\defres{primaries/C6F/intern/n_dropped}{0}
\defres{primaries/C6F/intern/n_expected}{500}
\defres{primaries/C6F/intern/n_pairs}{500}
\defres{primaries/C6F/intern/p_decisive}{$<$0.001}
\defres{primaries/C6F/intern/readouts/cost_arm}{0.0449}
\defres{primaries/C6F/intern/readouts/cost_ref}{0.0436}
\defres{primaries/C6F/intern/readouts/cost_savings}{-3.0}
\defres{primaries/C6F/intern/readouts/cost_savings_ci/hi}{-0.4}
\defres{primaries/C6F/intern/readouts/cost_savings_ci/lo}{-6.0}
\defres{primaries/C6F/intern/readouts/token_savings}{-6.4}
\defres{primaries/C6F/intern/success_arm}{99.2}
\defres{primaries/C6F/intern/success_ref}{99.6}
\defres{primaries/C6F/intern/tango_lcb_adj}{-1.9}
\defres{primaries/C6F/intern/wins}{0}
\defres{primaries/C6F/jev/delta}{-0.6}
\defres{primaries/C6F/jev/delta_ci/hi}{+0.0}
\defres{primaries/C6F/jev/delta_ci/lo}{-1.4}
\defres{primaries/C6F/jev/discordance}{0.6}
\defres{primaries/C6F/jev/full_set/delta}{-0.6}
\defres{primaries/C6F/jev/full_set/p_decisive}{$<$0.001}
\defres{primaries/C6F/jev/loss_rate_ub}{1.5}
\defres{primaries/C6F/jev/losses}{3}
\defres{primaries/C6F/jev/mde}{-1.9}
\defres{primaries/C6F/jev/n_dropped}{0}
\defres{primaries/C6F/jev/n_expected}{500}
\defres{primaries/C6F/jev/n_pairs}{500}
\defres{primaries/C6F/jev/p_decisive}{$<$0.001}
\defres{primaries/C6F/jev/readouts/cost_arm}{0.0433}
\defres{primaries/C6F/jev/readouts/cost_ref}{0.0408}
\defres{primaries/C6F/jev/readouts/cost_savings}{-6.2}
\defres{primaries/C6F/jev/readouts/cost_savings_ci/hi}{-4.0}
\defres{primaries/C6F/jev/readouts/cost_savings_ci/lo}{-9.1}
\defres{primaries/C6F/jev/readouts/token_savings}{-3.3}
\defres{primaries/C6F/jev/success_arm}{99.2}
\defres{primaries/C6F/jev/success_ref}{99.8}
\defres{primaries/C6F/jev/tango_lcb_adj}{-2.3}
\defres{primaries/C6F/jev/wins}{0}
\defres{primaries/C6F/p_decisive}{$<$0.001}
\defres{primaries/C6F/p_holm}{0.002}
\defres{primaries/C6F/replication}{cross-backend replication}
\defres{primaries/C6F/rule}{max(p\_Jev, p\_Intern)}
\defres{primaries/C6L/alpha_adj}{0.017}
\defres{primaries/C6L/decision}{not NI as a conjunction: Jev inconclusive at this n; Intern-Decision not NI: loss of 6.0 pt (95 \% CI entirely below 0)}
\defres{primaries/C6L/full_set_family/p_decisive}{0.975}
\defres{primaries/C6L/full_set_family/p_holm}{1.000}
\defres{primaries/C6L/holm_rank}{9}
\defres{primaries/C6L/intern/delta}{-6.0}
\defres{primaries/C6L/intern/delta_ci/hi}{-3.0}
\defres{primaries/C6L/intern/delta_ci/lo}{-9.2}
\defres{primaries/C6L/intern/discordance}{12.8}
\defres{primaries/C6L/intern/full_set/delta}{-6.0}
\defres{primaries/C6L/intern/full_set/p_decisive}{0.975}
\defres{primaries/C6L/intern/losses}{47}
\defres{primaries/C6L/intern/mde}{+1.7}
\defres{primaries/C6L/intern/n_dropped}{0}
\defres{primaries/C6L/intern/n_expected}{500}
\defres{primaries/C6L/intern/n_pairs}{500}
\defres{primaries/C6L/intern/p_decisive}{0.975}
\defres{primaries/C6L/intern/readouts/cost_arm}{0.0144}
\defres{primaries/C6L/intern/readouts/cost_ref}{0.00988}
\defres{primaries/C6L/intern/readouts/cost_savings}{-45.3}
\defres{primaries/C6L/intern/readouts/cost_savings_ci/hi}{-37.7}
\defres{primaries/C6L/intern/readouts/cost_savings_ci/lo}{-53.1}
\defres{primaries/C6L/intern/readouts/token_savings}{-58.3}
\defres{primaries/C6L/intern/success_arm}{77.4}
\defres{primaries/C6L/intern/success_ref}{83.4}
\defres{primaries/C6L/intern/tango_lcb_adj}{-9.6}
\defres{primaries/C6L/intern/wins}{17}
\defres{primaries/C6L/jev/delta}{+1.6}
\defres{primaries/C6L/jev/delta_ci/hi}{+4.0}
\defres{primaries/C6L/jev/delta_ci/lo}{-0.8}
\defres{primaries/C6L/jev/discordance}{7.6}
\defres{primaries/C6L/jev/full_set/delta}{+1.6}
\defres{primaries/C6L/jev/full_set/p_decisive}{$<$0.001}
\defres{primaries/C6L/jev/losses}{15}
\defres{primaries/C6L/jev/mde}{+0.6}
\defres{primaries/C6L/jev/n_dropped}{0}
\defres{primaries/C6L/jev/n_expected}{500}
\defres{primaries/C6L/jev/n_pairs}{500}
\defres{primaries/C6L/jev/p_decisive}{$<$0.001}
\defres{primaries/C6L/jev/readouts/cost_arm}{0.013}
\defres{primaries/C6L/jev/readouts/cost_ref}{0.0098}
\defres{primaries/C6L/jev/readouts/cost_savings}{-32.1}
\defres{primaries/C6L/jev/readouts/cost_savings_ci/hi}{-25.0}
\defres{primaries/C6L/jev/readouts/cost_savings_ci/lo}{-39.4}
\defres{primaries/C6L/jev/readouts/token_savings}{-38.8}
\defres{primaries/C6L/jev/success_arm}{82.0}
\defres{primaries/C6L/jev/success_ref}{80.4}
\defres{primaries/C6L/jev/tango_lcb_adj}{-1.1}
\defres{primaries/C6L/jev/wins}{23}
\defres{primaries/C6L/p_decisive}{0.975}
\defres{primaries/C6L/p_holm}{1.000}
\defres{primaries/C6L/replication}{not reached (Holm step-down stopped at an earlier primary)}
\defres{primaries/C6L/rule}{max(p\_Jev, p\_Intern)}
\defres{primaries/C7/alpha_adj}{0.010}
\defres{primaries/C7/decision}{transfer NI was not established; inconclusive at this n}
\defres{primaries/C7/full_set_family/p_decisive}{0.766}
\defres{primaries/C7/full_set_family/p_holm}{1.000}
\defres{primaries/C7/holm_rank}{7}
\defres{primaries/C7/jev/delta}{-8.1}
\defres{primaries/C7/jev/delta_ci/hi}{+0.0}
\defres{primaries/C7/jev/delta_ci/lo}{-16.1}
\defres{primaries/C7/jev/discordance}{28.2}
\defres{primaries/C7/jev/full_set/delta}{-8.1}
\defres{primaries/C7/jev/full_set/p_decisive}{0.766}
\defres{primaries/C7/jev/losses}{27}
\defres{primaries/C7/jev/mde}{+8.7}
\defres{primaries/C7/jev/n_dropped}{0}
\defres{primaries/C7/jev/n_expected}{149}
\defres{primaries/C7/jev/n_pairs}{149}
\defres{primaries/C7/jev/p_decisive}{0.766}
\defres{primaries/C7/jev/readouts/cost_arm}{0.0901}
\defres{primaries/C7/jev/readouts/cost_ref}{0.0762}
\defres{primaries/C7/jev/readouts/cost_savings}{-18.1}
\defres{primaries/C7/jev/readouts/cost_savings_ci/hi}{-12.0}
\defres{primaries/C7/jev/readouts/cost_savings_ci/lo}{-24.6}
\defres{primaries/C7/jev/readouts/token_savings}{25.1}
\defres{primaries/C7/jev/success_arm}{57.7}
\defres{primaries/C7/jev/success_ref}{65.8}
\defres{primaries/C7/jev/tango_lcb_adj}{-18.3}
\defres{primaries/C7/jev/wins}{15}
\defres{primaries/C7/p_decisive}{0.766}
\defres{primaries/C7/p_holm}{1.000}
\defres{primaries/C7/rule}{bb\_ordered}
\defres{primaries/C8/alpha_adj}{0.006}
\defres{primaries/C8/decision}{NI}
\defres{primaries/C8/full_set_family/p_decisive}{$<$0.001}
\defres{primaries/C8/full_set_family/p_holm}{0.001}
\defres{primaries/C8/holm_rank}{3}
\defres{primaries/C8/jev/delta}{-0.4}
\defres{primaries/C8/jev/delta_ci/hi}{+0.8}
\defres{primaries/C8/jev/delta_ci/lo}{-1.5}
\defres{primaries/C8/jev/discordance}{4.1}
\defres{primaries/C8/jev/full_set/delta}{-0.4}
\defres{primaries/C8/jev/full_set/p_decisive}{$<$0.001}
\defres{primaries/C8/jev/losses}{25}
\defres{primaries/C8/jev/mde}{-1.0}
\defres{primaries/C8/jev/n_dropped}{0}
\defres{primaries/C8/jev/n_expected}{1114}
\defres{primaries/C8/jev/n_pairs}{1114}
\defres{primaries/C8/jev/p_decisive}{$<$0.001}
\defres{primaries/C8/jev/readouts/cost_per_1k_arm}{0.0167}
\defres{primaries/C8/jev/readouts/cost_per_1k_ref}{0.63}
\defres{primaries/C8/jev/readouts/p50_latency_ratio}{0.0807}
\defres{primaries/C8/jev/success_arm}{89.9}
\defres{primaries/C8/jev/success_ref}{90.3}
\defres{primaries/C8/jev/tango_lcb_adj}{-2.0}
\defres{primaries/C8/jev/wins}{21}
\defres{primaries/C8/p_decisive}{$<$0.001}
\defres{primaries/C8/p_holm}{0.001}
\defres{primaries/C8/rule}{bb\_ordered}
\makeatother


==> generated/results.tex <==
\makeatletter
\providecommand{\res}[1]{\ifcsname jevres@#1\endcsname\csname jevres@#1\endcsname\else\tbd\fi}
\providecommand{\defres}[2]{\expandafter\def\csname jevres@#1\endcsname{#2}}
\defres{data_stats/bfcl_e1/in_candidates}{58.9}
\defres{data_stats/bfcl_e1/n_param_slots}{2091}
\defres{e1_bfcl_when2call/bm25/tool_params/bfcl/acc}{31.5}
\defres{e1_bfcl_when2call/bm25/tool_params/bfcl/acc_gold_in_candidates}{53.3}
\defres{e1_bfcl_when2call/bm25/tool_params/bfcl/auroc}{0.57}
\defres{e1_bfcl_when2call/bm25/tool_params/bfcl/brier}{0.267}
\defres{e1_bfcl_when2call/bm25/tool_params/bfcl/cost_per_1k_usd}{0}
\defres{e1_bfcl_when2call/bm25/tool_params/bfcl/coverage}{1}
\defres{e1_bfcl_when2call/bm25/tool_params/bfcl/defer_correct}{0.0}
\defres{e1_bfcl_when2call/bm25/tool_params/bfcl/ece}{0.182}
\defres{e1_bfcl_when2call/bm25/tool_params/bfcl/fill_precision}{31.5}
\defres{e1_bfcl_when2call/bm25/tool_params/bfcl/fill_rate}{100.0}
\defres{e1_bfcl_when2call/bm25/tool_params/bfcl/input_tokens}{0}
\defres{e1_bfcl_when2call/bm25/tool_params/bfcl/latency_p50_ms}{1}
\defres{e1_bfcl_when2call/bm25/tool_params/bfcl/latency_p95_ms}{2}
\defres{e1_bfcl_when2call/bm25/tool_params/bfcl/n}{1949}
\defres{e1_bfcl_when2call/bm25/tool_params/bfcl/n_errors}{0}
\defres{e1_bfcl_when2call/bm25/tool_params/bfcl:live_multiple/acc}{27.1}
\defres{e1_bfcl_when2call/bm25/tool_params/bfcl:live_multiple/acc_gold_in_candidates}{48.9}
\defres{e1_bfcl_when2call/bm25/tool_params/bfcl:live_multiple/auroc}{0.56}
\defres{e1_bfcl_when2call/bm25/tool_params/bfcl:live_multiple/brier}{0.262}
\defres{e1_bfcl_when2call/bm25/tool_params/bfcl:live_multiple/cost_per_1k_usd}{0}
\defres{e1_bfcl_when2call/bm25/tool_params/bfcl:live_multiple/coverage}{1}
\defres{e1_bfcl_when2call/bm25/tool_params/bfcl:live_multiple/defer_correct}{0.0}
\defres{e1_bfcl_when2call/bm25/tool_params/bfcl:live_multiple/ece}{0.208}
\defres{e1_bfcl_when2call/bm25/tool_params/bfcl:live_multiple/fill_precision}{27.1}
\defres{e1_bfcl_when2call/bm25/tool_params/bfcl:live_multiple/fill_rate}{100.0}
\defres{e1_bfcl_when2call/bm25/tool_params/bfcl:live_multiple/input_tokens}{0}
\defres{e1_bfcl_when2call/bm25/tool_params/bfcl:live_multiple/latency_p50_ms}{1}
\defres{e1_bfcl_when2call/bm25/tool_params/bfcl:live_multiple/latency_p95_ms}{4}
\defres{e1_bfcl_when2call/bm25/tool_params/bfcl:live_multiple/n}{653}
\defres{e1_bfcl_when2call/bm25/tool_params/bfcl:live_multiple/n_errors}{0}
\defres{e1_bfcl_when2call/bm25/tool_params/bfcl:live_simple/acc}{29.5}
\defres{e1_bfcl_when2call/bm25/tool_params/bfcl:live_simple/acc_gold_in_candidates}{52.3}
\defres{e1_bfcl_when2call/bm25/tool_params/bfcl:live_simple/auroc}{0.55}
\defres{e1_bfcl_when2call/bm25/tool_params/bfcl:live_simple/brier}{0.304}
\defres{e1_bfcl_when2call/bm25/tool_params/bfcl:live_simple/cost_per_1k_usd}{0}
\defres{e1_bfcl_when2call/bm25/tool_params/bfcl:live_simple/coverage}{1}
\defres{e1_bfcl_when2call/bm25/tool_params/bfcl:live_simple/defer_correct}{0.0}
\defres{e1_bfcl_when2call/bm25/tool_params/bfcl:live_simple/ece}{0.262}
\defres{e1_bfcl_when2call/bm25/tool_params/bfcl:live_simple/fill_precision}{29.5}
\defres{e1_bfcl_when2call/bm25/tool_params/bfcl:live_simple/fill_rate}{100.0}
\defres{e1_bfcl_when2call/bm25/tool_params/bfcl:live_simple/input_tokens}{0}
\defres{e1_bfcl_when2call/bm25/tool_params/bfcl:live_simple/latency_p50_ms}{1}
\defres{e1_bfcl_when2call/bm25/tool_params/bfcl:live_simple/latency_p95_ms}{2}
\defres{e1_bfcl_when2call/bm25/tool_params/bfcl:live_simple/n}{380}
\defres{e1_bfcl_when2call/bm25/tool_params/bfcl:live_simple/n_errors}{0}
\defres{e1_bfcl_when2call/bm25/tool_params/bfcl:multiple/acc}{37.3}
\defres{e1_bfcl_when2call/bm25/tool_params/bfcl:multiple/acc_gold_in_candidates}{56.4}
\defres{e1_bfcl_when2call/bm25/tool_params/bfcl:multiple/auroc}{0.56}
\defres{e1_bfcl_when2call/bm25/tool_params/bfcl:multiple/brier}{0.265}
\defres{e1_bfcl_when2call/bm25/tool_params/bfcl:multiple/cost_per_1k_usd}{0}
\defres{e1_bfcl_when2call/bm25/tool_params/bfcl:multiple/coverage}{1}
\defres{e1_bfcl_when2call/bm25/tool_params/bfcl:multiple/defer_correct}{0.0}
\defres{e1_bfcl_when2call/bm25/tool_params/bfcl:multiple/ece}{0.136}
\defres{e1_bfcl_when2call/bm25/tool_params/bfcl:multiple/fill_precision}{37.3}
\defres{e1_bfcl_when2call/bm25/tool_params/bfcl:multiple/fill_rate}{100.0}
\defres{e1_bfcl_when2call/bm25/tool_params/bfcl:multiple/input_tokens}{0}
\defres{e1_bfcl_when2call/bm25/tool_params/bfcl:multiple/latency_p50_ms}{1}
\defres{e1_bfcl_when2call/bm25/tool_params/bfcl:multiple/latency_p95_ms}{1}
\defres{e1_bfcl_when2call/bm25/tool_params/bfcl:multiple/n}{459}
\defres{e1_bfcl_when2call/bm25/tool_params/bfcl:multiple/n_errors}{0}
\defres{e1_bfcl_when2call/bm25/tool_params/bfcl:simple_python/acc}{33.5}
\defres{e1_bfcl_when2call/bm25/tool_params/bfcl:simple_python/acc_gold_in_candidates}{56.5}
\defres{e1_bfcl_when2call/bm25/tool_params/bfcl:simple_python/auroc}{0.61}
\defres{e1_bfcl_when2call/bm25/tool_params/bfcl:simple_python/brier}{0.246}
\defres{e1_bfcl_when2call/bm25/tool_params/bfcl:simple_python/cost_per_1k_usd}{0}
\defres{e1_bfcl_when2call/bm25/tool_params/bfcl:simple_python/coverage}{1}
\defres{e1_bfcl_when2call/bm25/tool_params/bfcl:simple_python/defer_correct}{0.0}
\defres{e1_bfcl_when2call/bm25/tool_params/bfcl:simple_python/ece}{0.147}
\defres{e1_bfcl_when2call/bm25/tool_params/bfcl:simple_python/fill_precision}{33.5}
\defres{e1_bfcl_when2call/bm25/tool_params/bfcl:simple_python/fill_rate}{100.0}
\defres{e1_bfcl_when2call/bm25/tool_params/bfcl:simple_python/input_tokens}{0}
\defres{e1_bfcl_when2call/bm25/tool_params/bfcl:simple_python/latency_p50_ms}{1}
\defres{e1_bfcl_when2call/bm25/tool_params/bfcl:simple_python/latency_p95_ms}{1}
\defres{e1_bfcl_when2call/bm25/tool_params/bfcl:simple_python/n}{457}
\defres{e1_bfcl_when2call/bm25/tool_params/bfcl:simple_python/n_errors}{0}
\defres{e1_bfcl_when2call/bm25/tool_select/bfcl/acc}{61.4}
\defres{e1_bfcl_when2call/bm25/tool_select/bfcl/auroc}{0.82}
\defres{e1_bfcl_when2call/bm25/tool_select/bfcl/brier}{0.189}
\defres{e1_bfcl_when2call/bm25/tool_select/bfcl/cost_per_1k_usd}{0}
\defres{e1_bfcl_when2call/bm25/tool_select/bfcl/coverage}{1}
\defres{e1_bfcl_when2call/bm25/tool_select/bfcl/ece}{0.140}
\defres{e1_bfcl_when2call/bm25/tool_select/bfcl/input_tokens}{0}
\defres{e1_bfcl_when2call/bm25/tool_select/bfcl/latency_p50_ms}{0}
\defres{e1_bfcl_when2call/bm25/tool_select/bfcl/latency_p95_ms}{1}
\defres{e1_bfcl_when2call/bm25/tool_select/bfcl/n}{1114}
\defres{e1_bfcl_when2call/bm25/tool_select/bfcl/n_errors}{0}
\defres{e1_bfcl_when2call/bm25/tool_select/bfcl:irrelevance/acc}{0.0}
\defres{e1_bfcl_when2call/bm25/tool_select/bfcl:irrelevance/brier}{0.419}
\defres{e1_bfcl_when2call/bm25/tool_select/bfcl:irrelevance/cost_per_1k_usd}{0}
\defres{e1_bfcl_when2call/bm25/tool_select/bfcl:irrelevance/coverage}{1}
\defres{e1_bfcl_when2call/bm25/tool_select/bfcl:irrelevance/ece}{0.628}
\defres{e1_bfcl_when2call/bm25/tool_select/bfcl:irrelevance/input_tokens}{0}
\defres{e1_bfcl_when2call/bm25/tool_select/bfcl:irrelevance/latency_p50_ms}{0}
\defres{e1_bfcl_when2call/bm25/tool_select/bfcl:irrelevance/latency_p95_ms}{0}
\defres{e1_bfcl_when2call/bm25/tool_select/bfcl:irrelevance/n}{185}
\defres{e1_bfcl_when2call/bm25/tool_select/bfcl:irrelevance/n_errors}{0}
\defres{e1_bfcl_when2call/bm25/tool_select/bfcl:live_irrelevance/acc}{0.0}
\defres{e1_bfcl_when2call/bm25/tool_select/bfcl:live_irrelevance/brier}{0.434}
\defres{e1_bfcl_when2call/bm25/tool_select/bfcl:live_irrelevance/cost_per_1k_usd}{0}
\defres{e1_bfcl_when2call/bm25/tool_select/bfcl:live_irrelevance/coverage}{1}
\defres{e1_bfcl_when2call/bm25/tool_select/bfcl:live_irrelevance/ece}{0.622}
\defres{e1_bfcl_when2call/bm25/tool_select/bfcl:live_irrelevance/input_tokens}{0}
\defres{e1_bfcl_when2call/bm25/tool_select/bfcl:live_irrelevance/latency_p50_ms}{0}
\defres{e1_bfcl_when2call/bm25/tool_select/bfcl:live_irrelevance/latency_p95_ms}{1}
\defres{e1_bfcl_when2call/bm25/tool_select/bfcl:live_irrelevance/n}{185}
\defres{e1_bfcl_when2call/bm25/tool_select/bfcl:live_irrelevance/n_errors}{0}
\defres{e1_bfcl_when2call/bm25/tool_select/bfcl:live_multiple/acc}{74.2}
\defres{e1_bfcl_when2call/bm25/tool_select/bfcl:live_multiple/auroc}{0.80}
\defres{e1_bfcl_when2call/bm25/tool_select/bfcl:live_multiple/brier}{0.157}
\defres{e1_bfcl_when2call/bm25/tool_select/bfcl:live_multiple/cost_per_1k_usd}{0}
\defres{e1_bfcl_when2call/bm25/tool_select/bfcl:live_multiple/coverage}{1}
\defres{e1_bfcl_when2call/bm25/tool_select/bfcl:live_multiple/ece}{0.065}
\defres{e1_bfcl_when2call/bm25/tool_select/bfcl:live_multiple/input_tokens}{0}
\defres{e1_bfcl_when2call/bm25/tool_select/bfcl:live_multiple/latency_p50_ms}{0}
\defres{e1_bfcl_when2call/bm25/tool_select/bfcl:live_multiple/latency_p95_ms}{1}
\defres{e1_bfcl_when2call/bm25/tool_select/bfcl:live_multiple/n}{186}
\defres{e1_bfcl_when2call/bm25/tool_select/bfcl:live_multiple/n_errors}{0}
\defres{e1_bfcl_when2call/bm25/tool_select/bfcl:live_simple/acc}{100.0}
\defres{e1_bfcl_when2call/bm25/tool_select/bfcl:live_simple/brier}{0.051}
\defres{e1_bfcl_when2call/bm25/tool_select/bfcl:live_simple/cost_per_1k_usd}{0}
\defres{e1_bfcl_when2call/bm25/tool_select/bfcl:live_simple/coverage}{1}
\defres{e1_bfcl_when2call/bm25/tool_select/bfcl:live_simple/ece}{0.173}
\defres{e1_bfcl_when2call/bm25/tool_select/bfcl:live_simple/input_tokens}{0}
\defres{e1_bfcl_when2call/bm25/tool_select/bfcl:live_simple/latency_p50_ms}{0}
\defres{e1_bfcl_when2call/bm25/tool_select/bfcl:live_simple/latency_p95_ms}{0}
\defres{e1_bfcl_when2call/bm25/tool_select/bfcl:live_simple/n}{186}
\defres{e1_bfcl_when2call/bm25/tool_select/bfcl:live_simple/n_errors}{0}
\defres{e1_bfcl_when2call/bm25/tool_select/bfcl:multiple/acc}{93.5}
\defres{e1_bfcl_when2call/bm25/tool_select/bfcl:multiple/auroc}{0.96}
\defres{e1_bfcl_when2call/bm25/tool_select/bfcl:multiple/brier}{0.055}
\defres{e1_bfcl_when2call/bm25/tool_select/bfcl:multiple/cost_per_1k_usd}{0}
\defres{e1_bfcl_when2call/bm25/tool_select/bfcl:multiple/coverage}{1}
\defres{e1_bfcl_when2call/bm25/tool_select/bfcl:multiple/ece}{0.104}
\defres{e1_bfcl_when2call/bm25/tool_select/bfcl:multiple/input_tokens}{0}
\defres{e1_bfcl_when2call/bm25/tool_select/bfcl:multiple/latency_p50_ms}{0}
\defres{e1_bfcl_when2call/bm25/tool_select/bfcl:multiple/latency_p95_ms}{1}
\defres{e1_bfcl_when2call/bm25/tool_select/bfcl:multiple/n}{186}
\defres{e1_bfcl_when2call/bm25/tool_select/bfcl:multiple/n_errors}{0}
\defres{e1_bfcl_when2call/bm25/tool_select/bfcl:simple_python/acc}{100.0}
\defres{e1_bfcl_when2call/bm25/tool_select/bfcl:simple_python/brier}{0.023}
\defres{e1_bfcl_when2call/bm25/tool_select/bfcl:simple_python/cost_per_1k_usd}{0}
\defres{e1_bfcl_when2call/bm25/tool_select/bfcl:simple_python/coverage}{1}
\defres{e1_bfcl_when2call/bm25/tool_select/bfcl:simple_python/ece}{0.096}
\defres{e1_bfcl_when2call/bm25/tool_select/bfcl:simple_python/input_tokens}{0}
\defres{e1_bfcl_when2call/bm25/tool_select/bfcl:simple_python/latency_p50_ms}{0}
\defres{e1_bfcl_when2call/bm25/tool_select/bfcl:simple_python/latency_p95_ms}{1}
\defres{e1_bfcl_when2call/bm25/tool_select/bfcl:simple_python/n}{186}
\defres{e1_bfcl_when2call/bm25/tool_select/bfcl:simple_python/n_errors}{0}
\defres{e1_bfcl_when2call/bm25/tool_select/when2call/acc}{29.5}
\defres{e1_bfcl_when2call/bm25/tool_select/when2call/auroc}{0.57}
\defres{e1_bfcl_when2call/bm25/tool_select/when2call/brier}{0.578}
\defres{e1_bfcl_when2call/bm25/tool_select/when2call/cost_per_1k_usd}{0}
\defres{e1_bfcl_when2call/bm25/tool_select/when2call/coverage}{1}
\defres{e1_bfcl_when2call/bm25/tool_select/when2call/ece}{0.604}
\defres{e1_bfcl_when2call/bm25/tool_select/when2call/input_tokens}{0}
\defres{e1_bfcl_when2call/bm25/tool_select/when2call/latency_p50_ms}{1}
\defres{e1_bfcl_when2call/bm25/tool_select/when2call/latency_p95_ms}{1}
\defres{e1_bfcl_when2call/bm25/tool_select/when2call/n}{928}
\defres{e1_bfcl_when2call/bm25/tool_select/when2call/n_errors}{0}
\defres{e1_bfcl_when2call/bm25/tool_select/when2call:BFCLv2LiveMultiple/acc}{29.3}
\defres{e1_bfcl_when2call/bm25/tool_select/when2call:BFCLv2LiveMultiple/auroc}{0.58}
\defres{e1_bfcl_when2call/bm25/tool_select/when2call:BFCLv2LiveMultiple/brier}{0.631}
\defres{e1_bfcl_when2call/bm25/tool_select/when2call:BFCLv2LiveMultiple/cost_per_1k_usd}{0}
\defres{e1_bfcl_when2call/bm25/tool_select/when2call:BFCLv2LiveMultiple/coverage}{1}
\defres{e1_bfcl_when2call/bm25/tool_select/when2call:BFCLv2LiveMultiple/ece}{0.647}
\defres{e1_bfcl_when2call/bm25/tool_select/when2call:BFCLv2LiveMultiple/input_tokens}{0}
\defres{e1_bfcl_when2call/bm25/tool_select/when2call:BFCLv2LiveMultiple/latency_p50_ms}{1}
\defres{e1_bfcl_when2call/bm25/tool_select/when2call:BFCLv2LiveMultiple/latency_p95_ms}{1}
\defres{e1_bfcl_when2call/bm25/tool_select/when2call:BFCLv2LiveMultiple/n}{731}
\defres{e1_bfcl_when2call/bm25/tool_select/when2call:BFCLv2LiveMultiple/n_errors}{0}
\defres{e1_bfcl_when2call/bm25/tool_select/when2call:BFCLv2LiveSimple/acc}{30.5}
\defres{e1_bfcl_when2call/bm25/tool_select/when2call:BFCLv2LiveSimple/auroc}{0.72}
\defres{e1_bfcl_when2call/bm25/tool_select/when2call:BFCLv2LiveSimple/brier}{0.381}
\defres{e1_bfcl_when2call/bm25/tool_select/when2call:BFCLv2LiveSimple/cost_per_1k_usd}{0}
\defres{e1_bfcl_when2call/bm25/tool_select/when2call:BFCLv2LiveSimple/coverage}{1}
\defres{e1_bfcl_when2call/bm25/tool_select/when2call:BFCLv2LiveSimple/ece}{0.443}
\defres{e1_bfcl_when2call/bm25/tool_select/when2call:BFCLv2LiveSimple/input_tokens}{0}
\defres{e1_bfcl_when2call/bm25/tool_select/when2call:BFCLv2LiveSimple/latency_p50_ms}{0}
\defres{e1_bfcl_when2call/bm25/tool_select/when2call:BFCLv2LiveSimple/latency_p95_ms}{1}
\defres{e1_bfcl_when2call/bm25/tool_select/when2call:BFCLv2LiveSimple/n}{197}
\defres{e1_bfcl_when2call/bm25/tool_select/when2call:BFCLv2LiveSimple/n_errors}{0}
\defres{e1_bfcl_when2call/gemini_embed/tool_params/bfcl/acc}{40.0}
\defres{e1_bfcl_when2call/gemini_embed/tool_params/bfcl/acc_gold_in_candidates}{60.4}
\defres{e1_bfcl_when2call/gemini_embed/tool_params/bfcl/auroc}{0.57}
\defres{e1_bfcl_when2call/gemini_embed/tool_params/bfcl/brier}{0.261}
\defres{e1_bfcl_when2call/gemini_embed/tool_params/bfcl/cost_per_1k_usd}{0.0109}
\defres{e1_bfcl_when2call/gemini_embed/tool_params/bfcl/coverage}{1}
\defres{e1_bfcl_when2call/gemini_embed/tool_params/bfcl/defer_correct}{10.5}
\defres{e1_bfcl_when2call/gemini_embed/tool_params/bfcl/ece}{0.110}
\defres{e1_bfcl_when2call/gemini_embed/tool_params/bfcl/fill_precision}{37.4}
\defres{e1_bfcl_when2call/gemini_embed/tool_params/bfcl/fill_rate}{95.4}
\defres{e1_bfcl_when2call/gemini_embed/tool_params/bfcl/input_tokens}{72.3}
\defres{e1_bfcl_when2call/gemini_embed/tool_params/bfcl/latency_p50_ms}{218}
\defres{e1_bfcl_when2call/gemini_embed/tool_params/bfcl/latency_p95_ms}{341}
\defres{e1_bfcl_when2call/gemini_embed/tool_params/bfcl/n}{1949}
\defres{e1_bfcl_when2call/gemini_embed/tool_params/bfcl/n_errors}{0}
\defres{e1_bfcl_when2call/gemini_embed/tool_params/bfcl:live_multiple/acc}{33.1}
\defres{e1_bfcl_when2call/gemini_embed/tool_params/bfcl:live_multiple/acc_gold_in_candidates}{50.6}
\defres{e1_bfcl_when2call/gemini_embed/tool_params/bfcl:live_multiple/auroc}{0.55}
\defres{e1_bfcl_when2call/gemini_embed/tool_params/bfcl:live_multiple/brier}{0.264}
\defres{e1_bfcl_when2call/gemini_embed/tool_params/bfcl:live_multiple/cost_per_1k_usd}{0.0127}
\defres{e1_bfcl_when2call/gemini_embed/tool_params/bfcl:live_multiple/coverage}{1}
\defres{e1_bfcl_when2call/gemini_embed/tool_params/bfcl:live_multiple/defer_correct}{11.3}
\defres{e1_bfcl_when2call/gemini_embed/tool_params/bfcl:live_multiple/ece}{0.150}
\defres{e1_bfcl_when2call/gemini_embed/tool_params/bfcl:live_multiple/fill_precision}{29.6}
\defres{e1_bfcl_when2call/gemini_embed/tool_params/bfcl:live_multiple/fill_rate}{94.8}
\defres{e1_bfcl_when2call/gemini_embed/tool_params/bfcl:live_multiple/input_tokens}{84.9}
\defres{e1_bfcl_when2call/gemini_embed/tool_params/bfcl:live_multiple/latency_p50_ms}{222}
\defres{e1_bfcl_when2call/gemini_embed/tool_params/bfcl:live_multiple/latency_p95_ms}{347}
\defres{e1_bfcl_when2call/gemini_embed/tool_params/bfcl:live_multiple/n}{653}
\defres{e1_bfcl_when2call/gemini_embed/tool_params/bfcl:live_multiple/n_errors}{0}
\defres{e1_bfcl_when2call/gemini_embed/tool_params/bfcl:live_simple/acc}{40.5}
\defres{e1_bfcl_when2call/gemini_embed/tool_params/bfcl:live_simple/acc_gold_in_candidates}{68.7}
\defres{e1_bfcl_when2call/gemini_embed/tool_params/bfcl:live_simple/auroc}{0.57}
\defres{e1_bfcl_when2call/gemini_embed/tool_params/bfcl:live_simple/brier}{0.272}
\defres{e1_bfcl_when2call/gemini_embed/tool_params/bfcl:live_simple/cost_per_1k_usd}{0.0129}
\defres{e1_bfcl_when2call/gemini_embed/tool_params/bfcl:live_simple/coverage}{1}
\defres{e1_bfcl_when2call/gemini_embed/tool_params/bfcl:live_simple/defer_correct}{4.2}
\defres{e1_bfcl_when2call/gemini_embed/tool_params/bfcl:live_simple/ece}{0.118}
\defres{e1_bfcl_when2call/gemini_embed/tool_params/bfcl:live_simple/fill_precision}{39.4}
\defres{e1_bfcl_when2call/gemini_embed/tool_params/bfcl:live_simple/fill_rate}{98.2}
\defres{e1_bfcl_when2call/gemini_embed/tool_params/bfcl:live_simple/input_tokens}{85.8}
\defres{e1_bfcl_when2call/gemini_embed/tool_params/bfcl:live_simple/latency_p50_ms}{214}
\defres{e1_bfcl_when2call/gemini_embed/tool_params/bfcl:live_simple/latency_p95_ms}{311}
\defres{e1_bfcl_when2call/gemini_embed/tool_params/bfcl:live_simple/n}{380}
\defres{e1_bfcl_when2call/gemini_embed/tool_params/bfcl:live_simple/n_errors}{0}
\defres{e1_bfcl_when2call/gemini_embed/tool_params/bfcl:multiple/acc}{47.7}
\defres{e1_bfcl_when2call/gemini_embed/tool_params/bfcl:multiple/acc_gold_in_candidates}{65.0}
\defres{e1_bfcl_when2call/gemini_embed/tool_params/bfcl:multiple/auroc}{0.56}
\defres{e1_bfcl_when2call/gemini_embed/tool_params/bfcl:multiple/brier}{0.264}
\defres{e1_bfcl_when2call/gemini_embed/tool_params/bfcl:multiple/cost_per_1k_usd}{0.00851}
\defres{e1_bfcl_when2call/gemini_embed/tool_params/bfcl:multiple/coverage}{1}
\defres{e1_bfcl_when2call/gemini_embed/tool_params/bfcl:multiple/defer_correct}{14.1}
\defres{e1_bfcl_when2call/gemini_embed/tool_params/bfcl:multiple/ece}{0.104}
\defres{e1_bfcl_when2call/gemini_embed/tool_params/bfcl:multiple/fill_precision}{45.4}
\defres{e1_bfcl_when2call/gemini_embed/tool_params/bfcl:multiple/fill_rate}{94.6}
\defres{e1_bfcl_when2call/gemini_embed/tool_params/bfcl:multiple/input_tokens}{56.7}
\defres{e1_bfcl_when2call/gemini_embed/tool_params/bfcl:multiple/latency_p50_ms}{209}
\defres{e1_bfcl_when2call/gemini_embed/tool_params/bfcl:multiple/latency_p95_ms}{304}
\defres{e1_bfcl_when2call/gemini_embed/tool_params/bfcl:multiple/n}{459}
\defres{e1_bfcl_when2call/gemini_embed/tool_params/bfcl:multiple/n_errors}{0}
\defres{e1_bfcl_when2call/gemini_embed/tool_params/bfcl:simple_python/acc}{41.6}
\defres{e1_bfcl_when2call/gemini_embed/tool_params/bfcl:simple_python/acc_gold_in_candidates}{62.0}
\defres{e1_bfcl_when2call/gemini_embed/tool_params/bfcl:simple_python/auroc}{0.61}
\defres{e1_bfcl_when2call/gemini_embed/tool_params/bfcl:simple_python/brier}{0.244}
\defres{e1_bfcl_when2call/gemini_embed/tool_params/bfcl:simple_python/cost_per_1k_usd}{0.00884}
\defres{e1_bfcl_when2call/gemini_embed/tool_params/bfcl:simple_python/coverage}{1}
\defres{e1_bfcl_when2call/gemini_embed/tool_params/bfcl:simple_python/defer_correct}{11.8}
\defres{e1_bfcl_when2call/gemini_embed/tool_params/bfcl:simple_python/ece}{0.090}
\defres{e1_bfcl_when2call/gemini_embed/tool_params/bfcl:simple_python/fill_precision}{38.8}
\defres{e1_bfcl_when2call/gemini_embed/tool_params/bfcl:simple_python/fill_rate}{94.7}
\defres{e1_bfcl_when2call/gemini_embed/tool_params/bfcl:simple_python/input_tokens}{58.9}
\defres{e1_bfcl_when2call/gemini_embed/tool_params/bfcl:simple_python/latency_p50_ms}{224}
\defres{e1_bfcl_when2call/gemini_embed/tool_params/bfcl:simple_python/latency_p95_ms}{352}
\defres{e1_bfcl_when2call/gemini_embed/tool_params/bfcl:simple_python/n}{457}
\defres{e1_bfcl_when2call/gemini_embed/tool_params/bfcl:simple_python/n_errors}{0}
\defres{e1_bfcl_when2call/gemini_embed/tool_select/bfcl/acc}{79.3}
\defres{e1_bfcl_when2call/gemini_embed/tool_select/bfcl/auroc}{0.72}
\defres{e1_bfcl_when2call/gemini_embed/tool_select/bfcl/brier}{0.153}
\defres{e1_bfcl_when2call/gemini_embed/tool_select/bfcl/cost_per_1k_usd}{0.0121}
\defres{e1_bfcl_when2call/gemini_embed/tool_select/bfcl/coverage}{1}
\defres{e1_bfcl_when2call/gemini_embed/tool_select/bfcl/ece}{0.049}
\defres{e1_bfcl_when2call/gemini_embed/tool_select/bfcl/input_tokens}{80.5}
\defres{e1_bfcl_when2call/gemini_embed/tool_select/bfcl/latency_p50_ms}{183}
\defres{e1_bfcl_when2call/gemini_embed/tool_select/bfcl/latency_p95_ms}{267}
\defres{e1_bfcl_when2call/gemini_embed/tool_select/bfcl/n}{1114}
\defres{e1_bfcl_when2call/gemini_embed/tool_select/bfcl/n_errors}{0}
\defres{e1_bfcl_when2call/gemini_embed/tool_select/bfcl:irrelevance/acc}{36.2}
\defres{e1_bfcl_when2call/gemini_embed/tool_select/bfcl:irrelevance/auroc}{0.34}
\defres{e1_bfcl_when2call/gemini_embed/tool_select/bfcl:irrelevance/brier}{0.412}
\defres{e1_bfcl_when2call/gemini_embed/tool_select/bfcl:irrelevance/cost_per_1k_usd}{0.008}
\defres{e1_bfcl_when2call/gemini_embed/tool_select/bfcl:irrelevance/coverage}{1}
\defres{e1_bfcl_when2call/gemini_embed/tool_select/bfcl:irrelevance/ece}{0.362}
\defres{e1_bfcl_when2call/gemini_embed/tool_select/bfcl:irrelevance/input_tokens}{53.3}
\defres{e1_bfcl_when2call/gemini_embed/tool_select/bfcl:irrelevance/latency_p50_ms}{177}
\defres{e1_bfcl_when2call/gemini_embed/tool_select/bfcl:irrelevance/latency_p95_ms}{237}
\defres{e1_bfcl_when2call/gemini_embed/tool_select/bfcl:irrelevance/n}{185}
\defres{e1_bfcl_when2call/gemini_embed/tool_select/bfcl:irrelevance/n_errors}{0}
\defres{e1_bfcl_when2call/gemini_embed/tool_select/bfcl:live_irrelevance/acc}{55.7}
\defres{e1_bfcl_when2call/gemini_embed/tool_select/bfcl:live_irrelevance/auroc}{0.61}
\defres{e1_bfcl_when2call/gemini_embed/tool_select/bfcl:live_irrelevance/brier}{0.260}
\defres{e1_bfcl_when2call/gemini_embed/tool_select/bfcl:live_irrelevance/cost_per_1k_usd}{0.0158}
\defres{e1_bfcl_when2call/gemini_embed/tool_select/bfcl:live_irrelevance/coverage}{1}
\defres{e1_bfcl_when2call/gemini_embed/tool_select/bfcl:live_irrelevance/ece}{0.133}
\defres{e1_bfcl_when2call/gemini_embed/tool_select/bfcl:live_irrelevance/input_tokens}{105}
\defres{e1_bfcl_when2call/gemini_embed/tool_select/bfcl:live_irrelevance/latency_p50_ms}{175}
\defres{e1_bfcl_when2call/gemini_embed/tool_select/bfcl:live_irrelevance/latency_p95_ms}{278}
\defres{e1_bfcl_when2call/gemini_embed/tool_select/bfcl:live_irrelevance/n}{185}
\defres{e1_bfcl_when2call/gemini_embed/tool_select/bfcl:live_irrelevance/n_errors}{0}
\defres{e1_bfcl_when2call/gemini_embed/tool_select/bfcl:live_multiple/acc}{93.0}
\defres{e1_bfcl_when2call/gemini_embed/tool_select/bfcl:live_multiple/auroc}{0.78}
\defres{e1_bfcl_when2call/gemini_embed/tool_select/bfcl:live_multiple/brier}{0.135}
\defres{e1_bfcl_when2call/gemini_embed/tool_select/bfcl:live_multiple/cost_per_1k_usd}{0.0179}
\defres{e1_bfcl_when2call/gemini_embed/tool_select/bfcl:live_multiple/coverage}{1}
\defres{e1_bfcl_when2call/gemini_embed/tool_select/bfcl:live_multiple/ece}{0.254}
\defres{e1_bfcl_when2call/gemini_embed/tool_select/bfcl:live_multiple/input_tokens}{119}
\defres{e1_bfcl_when2call/gemini_embed/tool_select/bfcl:live_multiple/latency_p50_ms}{183}
\defres{e1_bfcl_when2call/gemini_embed/tool_select/bfcl:live_multiple/latency_p95_ms}{252}
\defres{e1_bfcl_when2call/gemini_embed/tool_select/bfcl:live_multiple/n}{186}
\defres{e1_bfcl_when2call/gemini_embed/tool_select/bfcl:live_multiple/n_errors}{0}
\defres{e1_bfcl_when2call/gemini_embed/tool_select/bfcl:live_simple/acc}{90.3}
\defres{e1_bfcl_when2call/gemini_embed/tool_select/bfcl:live_simple/auroc}{0.92}
\defres{e1_bfcl_when2call/gemini_embed/tool_select/bfcl:live_simple/brier}{0.063}
\defres{e1_bfcl_when2call/gemini_embed/tool_select/bfcl:live_simple/cost_per_1k_usd}{0.01}
\defres{e1_bfcl_when2call/gemini_embed/tool_select/bfcl:live_simple/coverage}{1}
\defres{e1_bfcl_when2call/gemini_embed/tool_select/bfcl:live_simple/ece}{0.053}
\defres{e1_bfcl_when2call/gemini_embed/tool_select/bfcl:live_simple/input_tokens}{66.7}
\defres{e1_bfcl_when2call/gemini_embed/tool_select/bfcl:live_simple/latency_p50_ms}{176}
\defres{e1_bfcl_when2call/gemini_embed/tool_select/bfcl:live_simple/latency_p95_ms}{230}
\defres{e1_bfcl_when2call/gemini_embed/tool_select/bfcl:live_simple/n}{186}
\defres{e1_bfcl_when2call/gemini_embed/tool_select/bfcl:live_simple/n_errors}{0}
\defres{e1_bfcl_when2call/gemini_embed/tool_select/bfcl:multiple/acc}{100.0}
\defres{e1_bfcl_when2call/gemini_embed/tool_select/bfcl:multiple/brier}{0.049}
\defres{e1_bfcl_when2call/gemini_embed/tool_select/bfcl:multiple/cost_per_1k_usd}{0.0119}
\defres{e1_bfcl_when2call/gemini_embed/tool_select/bfcl:multiple/coverage}{1}
\defres{e1_bfcl_when2call/gemini_embed/tool_select/bfcl:multiple/ece}{0.172}
\defres{e1_bfcl_when2call/gemini_embed/tool_select/bfcl:multiple/input_tokens}{79}
\defres{e1_bfcl_when2call/gemini_embed/tool_select/bfcl:multiple/latency_p50_ms}{197}
\defres{e1_bfcl_when2call/gemini_embed/tool_select/bfcl:multiple/latency_p95_ms}{274}
\defres{e1_bfcl_when2call/gemini_embed/tool_select/bfcl:multiple/n}{186}
\defres{e1_bfcl_when2call/gemini_embed/tool_select/bfcl:multiple/n_errors}{0}
\defres{e1_bfcl_when2call/gemini_embed/tool_select/bfcl:simple_python/acc}{100.0}
\defres{e1_bfcl_when2call/gemini_embed/tool_select/bfcl:simple_python/brier}{0.003}
\defres{e1_bfcl_when2call/gemini_embed/tool_select/bfcl:simple_python/cost_per_1k_usd}{0.00889}
\defres{e1_bfcl_when2call/gemini_embed/tool_select/bfcl:simple_python/coverage}{1}
\defres{e1_bfcl_when2call/gemini_embed/tool_select/bfcl:simple_python/ece}{0.044}
\defres{e1_bfcl_when2call/gemini_embed/tool_select/bfcl:simple_python/input_tokens}{59.3}
\defres{e1_bfcl_when2call/gemini_embed/tool_select/bfcl:simple_python/latency_p50_ms}{196}
\defres{e1_bfcl_when2call/gemini_embed/tool_select/bfcl:simple_python/latency_p95_ms}{285}
\defres{e1_bfcl_when2call/gemini_embed/tool_select/bfcl:simple_python/n}{186}
\defres{e1_bfcl_when2call/gemini_embed/tool_select/bfcl:simple_python/n_errors}{0}
\defres{e1_bfcl_when2call/gemini_embed/tool_select/when2call/acc}{43.2}
\defres{e1_bfcl_when2call/gemini_embed/tool_select/when2call/auroc}{0.52}
\defres{e1_bfcl_when2call/gemini_embed/tool_select/when2call/brier}{0.248}
\defres{e1_bfcl_when2call/gemini_embed/tool_select/when2call/cost_per_1k_usd}{0.073}
\defres{e1_bfcl_when2call/gemini_embed/tool_select/when2call/coverage}{1}
\defres{e1_bfcl_when2call/gemini_embed/tool_select/when2call/ece}{0.049}
\defres{e1_bfcl_when2call/gemini_embed/tool_select/when2call/input_tokens}{487}
\defres{e1_bfcl_when2call/gemini_embed/tool_select/when2call/latency_p50_ms}{170}
\defres{e1_bfcl_when2call/gemini_embed/tool_select/when2call/latency_p95_ms}{221}
\defres{e1_bfcl_when2call/gemini_embed/tool_select/when2call/n}{928}
\defres{e1_bfcl_when2call/gemini_embed/tool_select/when2call/n_errors}{0}
\defres{e1_bfcl_when2call/gemini_embed/tool_select/when2call:BFCLv2LiveMultiple/acc}{43.0}
\defres{e1_bfcl_when2call/gemini_embed/tool_select/when2call:BFCLv2LiveMultiple/auroc}{0.48}
\defres{e1_bfcl_when2call/gemini_embed/tool_select/when2call:BFCLv2LiveMultiple/brier}{0.251}
\defres{e1_bfcl_when2call/gemini_embed/tool_select/when2call:BFCLv2LiveMultiple/cost_per_1k_usd}{0.0874}
\defres{e1_bfcl_when2call/gemini_embed/tool_select/when2call:BFCLv2LiveMultiple/coverage}{1}
\defres{e1_bfcl_when2call/gemini_embed/tool_select/when2call:BFCLv2LiveMultiple/ece}{0.070}
\defres{e1_bfcl_when2call/gemini_embed/tool_select/when2call:BFCLv2LiveMultiple/input_tokens}{583}
\defres{e1_bfcl_when2call/gemini_embed/tool_select/when2call:BFCLv2LiveMultiple/latency_p50_ms}{173}
\defres{e1_bfcl_when2call/gemini_embed/tool_select/when2call:BFCLv2LiveMultiple/latency_p95_ms}{224}
\defres{e1_bfcl_when2call/gemini_embed/tool_select/when2call:BFCLv2LiveMultiple/n}{731}
\defres{e1_bfcl_when2call/gemini_embed/tool_select/when2call:BFCLv2LiveMultiple/n_errors}{0}
\defres{e1_bfcl_when2call/gemini_embed/tool_select/when2call:BFCLv2LiveSimple/acc}{44.2}
\defres{e1_bfcl_when2call/gemini_embed/tool_select/when2call:BFCLv2LiveSimple/auroc}{0.62}
\defres{e1_bfcl_when2call/gemini_embed/tool_select/when2call:BFCLv2LiveSimple/brier}{0.234}
\defres{e1_bfcl_when2call/gemini_embed/tool_select/when2call:BFCLv2LiveSimple/cost_per_1k_usd}{0.0195}
\defres{e1_bfcl_when2call/gemini_embed/tool_select/when2call:BFCLv2LiveSimple/coverage}{1}
\defres{e1_bfcl_when2call/gemini_embed/tool_select/when2call:BFCLv2LiveSimple/ece}{0.052}
\defres{e1_bfcl_when2call/gemini_embed/tool_select/when2call:BFCLv2LiveSimple/input_tokens}{130}
\defres{e1_bfcl_when2call/gemini_embed/tool_select/when2call:BFCLv2LiveSimple/latency_p50_ms}{164}
\defres{e1_bfcl_when2call/gemini_embed/tool_select/when2call:BFCLv2LiveSimple/latency_p95_ms}{199}
\defres{e1_bfcl_when2call/gemini_embed/tool_select/when2call:BFCLv2LiveSimple/n}{197}
\defres{e1_bfcl_when2call/gemini_embed/tool_select/when2call:BFCLv2LiveSimple/n_errors}{0}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_params/bfcl/acc}{96.3}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_params/bfcl/acc_gold_in_candidates}{98.3}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_params/bfcl/cost_per_1k_usd}{0.214}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_params/bfcl/coverage}{1}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_params/bfcl/input_tokens}{70.4}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_params/bfcl/latency_p50_ms}{936}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_params/bfcl/latency_p95_ms}{4156}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_params/bfcl/n}{1949}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_params/bfcl/n_errors}{0}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_params/bfcl/omit_rate}{0.219}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_params/bfcl:live_multiple/acc}{93.1}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_params/bfcl:live_multiple/acc_gold_in_candidates}{97.2}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_params/bfcl:live_multiple/cost_per_1k_usd}{0.212}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_params/bfcl:live_multiple/coverage}{1}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_params/bfcl:live_multiple/input_tokens}{76.1}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_params/bfcl:live_multiple/latency_p50_ms}{943}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_params/bfcl:live_multiple/latency_p95_ms}{2447}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_params/bfcl:live_multiple/n}{653}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_params/bfcl:live_multiple/n_errors}{0}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_params/bfcl:live_multiple/omit_rate}{0.325}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_params/bfcl:live_simple/acc}{96.1}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_params/bfcl:live_simple/acc_gold_in_candidates}{97.2}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_params/bfcl:live_simple/cost_per_1k_usd}{0.248}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_params/bfcl:live_simple/coverage}{1}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_params/bfcl:live_simple/input_tokens}{86.9}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_params/bfcl:live_simple/latency_p50_ms}{899}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_params/bfcl:live_simple/latency_p95_ms}{2387}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_params/bfcl:live_simple/n}{380}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_params/bfcl:live_simple/n_errors}{0}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_params/bfcl:live_simple/omit_rate}{0.276}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_params/bfcl:multiple/acc}{98.7}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_params/bfcl:multiple/acc_gold_in_candidates}{99.3}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_params/bfcl:multiple/cost_per_1k_usd}{0.201}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_params/bfcl:multiple/coverage}{1}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_params/bfcl:multiple/input_tokens}{59.6}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_params/bfcl:multiple/latency_p50_ms}{898}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_params/bfcl:multiple/latency_p95_ms}{4800}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_params/bfcl:multiple/n}{459}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_params/bfcl:multiple/n_errors}{0}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_params/bfcl:multiple/omit_rate}{0.12}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_params/bfcl:simple_python/acc}{98.5}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_params/bfcl:simple_python/acc_gold_in_candidates}{99.3}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_params/bfcl:simple_python/cost_per_1k_usd}{0.203}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_params/bfcl:simple_python/coverage}{1}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_params/bfcl:simple_python/input_tokens}{59.5}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_params/bfcl:simple_python/latency_p50_ms}{1008}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_params/bfcl:simple_python/latency_p95_ms}{5872}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_params/bfcl:simple_python/n}{457}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_params/bfcl:simple_python/n_errors}{0}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_params/bfcl:simple_python/omit_rate}{0.12}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_select/bfcl/acc}{84.2}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_select/bfcl/cost_per_1k_usd}{1.17}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_select/bfcl/coverage}{1}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_select/bfcl/input_tokens}{411}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_select/bfcl/latency_p50_ms}{884}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_select/bfcl/latency_p95_ms}{3085}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_select/bfcl/n}{1114}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_select/bfcl/n_errors}{0}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_select/bfcl:irrelevance/acc}{56.8}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_select/bfcl:irrelevance/cost_per_1k_usd}{1.64}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_select/bfcl:irrelevance/coverage}{1}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_select/bfcl:irrelevance/input_tokens}{144}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_select/bfcl:irrelevance/latency_p50_ms}{1016}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_select/bfcl:irrelevance/latency_p95_ms}{5049}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_select/bfcl:irrelevance/n}{185}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_select/bfcl:irrelevance/n_errors}{0}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_select/bfcl:live_irrelevance/acc}{53.5}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_select/bfcl:live_irrelevance/cost_per_1k_usd}{1.63}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_select/bfcl:live_irrelevance/coverage}{1}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_select/bfcl:live_irrelevance/input_tokens}{651}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_select/bfcl:live_irrelevance/latency_p50_ms}{926}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_select/bfcl:live_irrelevance/latency_p95_ms}{2335}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_select/bfcl:live_irrelevance/n}{185}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_select/bfcl:live_irrelevance/n_errors}{0}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_select/bfcl:live_multiple/acc}{96.8}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_select/bfcl:live_multiple/cost_per_1k_usd}{1.74}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_select/bfcl:live_multiple/coverage}{1}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_select/bfcl:live_multiple/input_tokens}{932}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_select/bfcl:live_multiple/latency_p50_ms}{852}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_select/bfcl:live_multiple/latency_p95_ms}{2430}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_select/bfcl:live_multiple/n}{186}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_select/bfcl:live_multiple/n_errors}{0}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_select/bfcl:live_simple/acc}{98.9}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_select/bfcl:live_simple/cost_per_1k_usd}{0.627}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_select/bfcl:live_simple/coverage}{1}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_select/bfcl:live_simple/input_tokens}{210}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_select/bfcl:live_simple/latency_p50_ms}{841}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_select/bfcl:live_simple/latency_p95_ms}{1869}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_select/bfcl:live_simple/n}{186}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_select/bfcl:live_simple/n_errors}{0}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_select/bfcl:multiple/acc}{98.9}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_select/bfcl:multiple/cost_per_1k_usd}{0.857}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_select/bfcl:multiple/coverage}{1}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_select/bfcl:multiple/input_tokens}{376}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_select/bfcl:multiple/latency_p50_ms}{824}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_select/bfcl:multiple/latency_p95_ms}{3240}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_select/bfcl:multiple/n}{186}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_select/bfcl:multiple/n_errors}{0}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_select/bfcl:simple_python/acc}{100.0}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_select/bfcl:simple_python/cost_per_1k_usd}{0.527}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_select/bfcl:simple_python/coverage}{1}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_select/bfcl:simple_python/input_tokens}{155}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_select/bfcl:simple_python/latency_p50_ms}{904}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_select/bfcl:simple_python/latency_p95_ms}{2797}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_select/bfcl:simple_python/n}{186}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_select/bfcl:simple_python/n_errors}{0}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_select/when2call/acc}{42.1}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_select/when2call/cost_per_1k_usd}{1.52}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_select/when2call/coverage}{0.995}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_select/when2call/input_tokens}{776}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_select/when2call/latency_p50_ms}{851}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_select/when2call/latency_p95_ms}{1626}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_select/when2call/n}{776}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_select/when2call/n_errors}{4}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_select/when2call:BFCLv2LiveMultiple/acc}{39.0}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_select/when2call:BFCLv2LiveMultiple/cost_per_1k_usd}{1.68}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_select/when2call:BFCLv2LiveMultiple/coverage}{0.994}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_select/when2call:BFCLv2LiveMultiple/input_tokens}{883}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_select/when2call:BFCLv2LiveMultiple/latency_p50_ms}{851}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_select/when2call:BFCLv2LiveMultiple/latency_p95_ms}{1721}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_select/when2call:BFCLv2LiveMultiple/n}{649}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_select/when2call:BFCLv2LiveMultiple/n_errors}{4}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_select/when2call:BFCLv2LiveSimple/acc}{58.3}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_select/when2call:BFCLv2LiveSimple/cost_per_1k_usd}{0.702}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_select/when2call:BFCLv2LiveSimple/coverage}{1}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_select/when2call:BFCLv2LiveSimple/input_tokens}{230}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_select/when2call:BFCLv2LiveSimple/latency_p50_ms}{849}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_select/when2call:BFCLv2LiveSimple/latency_p95_ms}{1465}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_select/when2call:BFCLv2LiveSimple/n}{127}
\defres{e1_bfcl_when2call/gemini_flash_fc/tool_select/when2call:BFCLv2LiveSimple/n_errors}{0}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_params/bfcl/acc}{93.6}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_params/bfcl/acc_gold_in_candidates}{95.9}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_params/bfcl/auroc}{0.76}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_params/bfcl/brier}{0.053}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_params/bfcl/cost_per_1k_usd}{0.673}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_params/bfcl/coverage}{1}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_params/bfcl/defer_correct}{90.2}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_params/bfcl/ece}{0.041}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_params/bfcl/fill_precision}{91.0}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_params/bfcl/fill_rate}{62.2}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_params/bfcl/input_tokens}{162}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_params/bfcl/latency_p50_ms}{2710}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_params/bfcl/latency_p95_ms}{7624}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_params/bfcl/n}{1949}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_params/bfcl/n_errors}{0}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_params/bfcl/n_parse_fail}{2}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_params/bfcl:live_multiple/acc}{92.2}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_params/bfcl:live_multiple/acc_gold_in_candidates}{92.8}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_params/bfcl:live_multiple/auroc}{0.79}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_params/bfcl:live_multiple/brier}{0.057}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_params/bfcl:live_multiple/cost_per_1k_usd}{0.723}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_params/bfcl:live_multiple/coverage}{1}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_params/bfcl:live_multiple/defer_correct}{91.4}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_params/bfcl:live_multiple/ece}{0.045}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_params/bfcl:live_multiple/fill_precision}{88.4}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_params/bfcl:live_multiple/fill_rate}{58.2}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_params/bfcl:live_multiple/input_tokens}{166}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_params/bfcl:live_multiple/latency_p50_ms}{2875}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_params/bfcl:live_multiple/latency_p95_ms}{10965}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_params/bfcl:live_multiple/n}{653}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_params/bfcl:live_multiple/n_errors}{0}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_params/bfcl:live_multiple/n_parse_fail}{2}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_params/bfcl:live_simple/acc}{89.7}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_params/bfcl:live_simple/acc_gold_in_candidates}{94.4}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_params/bfcl:live_simple/auroc}{0.82}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_params/bfcl:live_simple/brier}{0.088}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_params/bfcl:live_simple/cost_per_1k_usd}{0.718}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_params/bfcl:live_simple/coverage}{1}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_params/bfcl:live_simple/defer_correct}{83.7}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_params/bfcl:live_simple/ece}{0.082}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_params/bfcl:live_simple/fill_precision}{84.9}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_params/bfcl:live_simple/fill_rate}{62.6}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_params/bfcl:live_simple/input_tokens}{179}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_params/bfcl:live_simple/latency_p50_ms}{2992}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_params/bfcl:live_simple/latency_p95_ms}{7104}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_params/bfcl:live_simple/n}{380}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_params/bfcl:live_simple/n_errors}{0}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_params/bfcl:multiple/acc}{97.8}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_params/bfcl:multiple/acc_gold_in_candidates}{98.3}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_params/bfcl:multiple/auroc}{0.72}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_params/bfcl:multiple/brier}{0.022}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_params/bfcl:multiple/cost_per_1k_usd}{0.606}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_params/bfcl:multiple/coverage}{1}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_params/bfcl:multiple/defer_correct}{96.8}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_params/bfcl:multiple/ece}{0.022}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_params/bfcl:multiple/fill_precision}{98.0}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_params/bfcl:multiple/fill_rate}{66.2}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_params/bfcl:multiple/input_tokens}{149}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_params/bfcl:multiple/latency_p50_ms}{2683}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_params/bfcl:multiple/latency_p95_ms}{6119}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_params/bfcl:multiple/n}{459}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_params/bfcl:multiple/n_errors}{0}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_params/bfcl:simple_python/acc}{94.5}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_params/bfcl:simple_python/acc_gold_in_candidates}{98.5}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_params/bfcl:simple_python/auroc}{0.66}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_params/bfcl:simple_python/brier}{0.051}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_params/bfcl:simple_python/cost_per_1k_usd}{0.633}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_params/bfcl:simple_python/coverage}{1}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_params/bfcl:simple_python/defer_correct}{88.7}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_params/bfcl:simple_python/ece}{0.036}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_params/bfcl:simple_python/fill_precision}{92.1}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_params/bfcl:simple_python/fill_rate}{63.5}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_params/bfcl:simple_python/input_tokens}{153}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_params/bfcl:simple_python/latency_p50_ms}{2449}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_params/bfcl:simple_python/latency_p95_ms}{5780}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_params/bfcl:simple_python/n}{457}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_params/bfcl:simple_python/n_errors}{0}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_select/bfcl/acc}{90.3}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_select/bfcl/auroc}{0.71}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_select/bfcl/brier}{0.087}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_select/bfcl/cost_per_1k_usd}{0.63}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_select/bfcl/coverage}{1}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_select/bfcl/ece}{0.075}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_select/bfcl/input_tokens}{242}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_select/bfcl/latency_p50_ms}{2551}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_select/bfcl/latency_p95_ms}{6492}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_select/bfcl/n}{1114}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_select/bfcl/n_errors}{0}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_select/bfcl:irrelevance/acc}{88.1}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_select/bfcl:irrelevance/auroc}{0.74}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_select/bfcl:irrelevance/brier}{0.108}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_select/bfcl:irrelevance/cost_per_1k_usd}{0.471}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_select/bfcl:irrelevance/coverage}{1}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_select/bfcl:irrelevance/ece}{0.096}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_select/bfcl:irrelevance/input_tokens}{191}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_select/bfcl:irrelevance/latency_p50_ms}{2048}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_select/bfcl:irrelevance/latency_p95_ms}{5724}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_select/bfcl:irrelevance/n}{185}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_select/bfcl:irrelevance/n_errors}{0}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_select/bfcl:live_irrelevance/acc}{66.5}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_select/bfcl:live_irrelevance/auroc}{0.80}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_select/bfcl:live_irrelevance/brier}{0.294}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_select/bfcl:live_irrelevance/cost_per_1k_usd}{0.753}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_select/bfcl:live_irrelevance/coverage}{1}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_select/bfcl:live_irrelevance/ece}{0.306}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_select/bfcl:live_irrelevance/input_tokens}{291}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_select/bfcl:live_irrelevance/latency_p50_ms}{2414}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_select/bfcl:live_irrelevance/latency_p95_ms}{5120}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_select/bfcl:live_irrelevance/n}{185}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_select/bfcl:live_irrelevance/n_errors}{0}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_select/bfcl:live_multiple/acc}{96.2}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_select/bfcl:live_multiple/auroc}{0.69}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_select/bfcl:live_multiple/brier}{0.034}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_select/bfcl:live_multiple/cost_per_1k_usd}{0.9}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_select/bfcl:live_multiple/coverage}{1}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_select/bfcl:live_multiple/ece}{0.019}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_select/bfcl:live_multiple/input_tokens}{329}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_select/bfcl:live_multiple/latency_p50_ms}{2857}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_select/bfcl:live_multiple/latency_p95_ms}{6541}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_select/bfcl:live_multiple/n}{186}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_select/bfcl:live_multiple/n_errors}{0}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_select/bfcl:live_simple/acc}{94.6}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_select/bfcl:live_simple/auroc}{0.37}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_select/bfcl:live_simple/brier}{0.054}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_select/bfcl:live_simple/cost_per_1k_usd}{0.51}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_select/bfcl:live_simple/coverage}{1}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_select/bfcl:live_simple/ece}{0.043}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_select/bfcl:live_simple/input_tokens}{216}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_select/bfcl:live_simple/latency_p50_ms}{2848}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_select/bfcl:live_simple/latency_p95_ms}{7819}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_select/bfcl:live_simple/n}{186}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_select/bfcl:live_simple/n_errors}{0}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_select/bfcl:multiple/acc}{97.8}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_select/bfcl:multiple/auroc}{0.81}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_select/bfcl:multiple/brier}{0.017}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_select/bfcl:multiple/cost_per_1k_usd}{0.648}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_select/bfcl:multiple/coverage}{1}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_select/bfcl:multiple/ece}{0.023}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_select/bfcl:multiple/input_tokens}{231}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_select/bfcl:multiple/latency_p50_ms}{2562}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_select/bfcl:multiple/latency_p95_ms}{7400}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_select/bfcl:multiple/n}{186}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_select/bfcl:multiple/n_errors}{0}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_select/bfcl:simple_python/acc}{98.4}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_select/bfcl:simple_python/auroc}{0.53}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_select/bfcl:simple_python/brier}{0.016}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_select/bfcl:simple_python/cost_per_1k_usd}{0.494}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_select/bfcl:simple_python/coverage}{1}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_select/bfcl:simple_python/ece}{0.009}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_select/bfcl:simple_python/input_tokens}{195}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_select/bfcl:simple_python/latency_p50_ms}{2561}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_select/bfcl:simple_python/latency_p95_ms}{5979}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_select/bfcl:simple_python/n}{186}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_select/bfcl:simple_python/n_errors}{0}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_select/when2call/acc}{74.0}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_select/when2call/auroc}{0.60}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_select/when2call/brier}{0.241}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_select/when2call/cost_per_1k_usd}{1.32}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_select/when2call/coverage}{1}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_select/when2call/ece}{0.238}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_select/when2call/input_tokens}{659}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_select/when2call/latency_p50_ms}{2289}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_select/when2call/latency_p95_ms}{5857}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_select/when2call/n}{928}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_select/when2call/n_errors}{0}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_select/when2call:BFCLv2LiveMultiple/acc}{74.3}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_select/when2call:BFCLv2LiveMultiple/auroc}{0.59}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_select/when2call:BFCLv2LiveMultiple/brier}{0.239}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_select/when2call:BFCLv2LiveMultiple/cost_per_1k_usd}{1.46}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_select/when2call:BFCLv2LiveMultiple/coverage}{1}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_select/when2call:BFCLv2LiveMultiple/ece}{0.237}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_select/when2call:BFCLv2LiveMultiple/input_tokens}{754}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_select/when2call:BFCLv2LiveMultiple/latency_p50_ms}{2264}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_select/when2call:BFCLv2LiveMultiple/latency_p95_ms}{5896}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_select/when2call:BFCLv2LiveMultiple/n}{731}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_select/when2call:BFCLv2LiveMultiple/n_errors}{0}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_select/when2call:BFCLv2LiveSimple/acc}{73.1}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_select/when2call:BFCLv2LiveSimple/auroc}{0.62}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_select/when2call:BFCLv2LiveSimple/brier}{0.250}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_select/when2call:BFCLv2LiveSimple/cost_per_1k_usd}{0.782}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_select/when2call:BFCLv2LiveSimple/coverage}{1}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_select/when2call:BFCLv2LiveSimple/ece}{0.244}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_select/when2call:BFCLv2LiveSimple/input_tokens}{303}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_select/when2call:BFCLv2LiveSimple/latency_p50_ms}{2410}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_select/when2call:BFCLv2LiveSimple/latency_p95_ms}{5749}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_select/when2call:BFCLv2LiveSimple/n}{197}
\defres{e1_bfcl_when2call/gemini_flash_typed/tool_select/when2call:BFCLv2LiveSimple/n_errors}{0}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_params/bfcl/acc}{89.0}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_params/bfcl/acc_gold_in_candidates}{93.3}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_params/bfcl/auroc}{0.68}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_params/bfcl/brier}{0.088}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_params/bfcl/cost_per_1k_usd}{0.158}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_params/bfcl/coverage}{1}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_params/bfcl/defer_correct}{82.9}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_params/bfcl/ece}{0.088}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_params/bfcl/fill_precision}{84.9}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_params/bfcl/fill_rate}{64.9}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_params/bfcl/input_tokens}{162}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_params/bfcl/latency_p50_ms}{882}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_params/bfcl/latency_p95_ms}{2571}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_params/bfcl/n}{1949}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_params/bfcl/n_errors}{0}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_params/bfcl/n_parse_fail}{1}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_params/bfcl:live_multiple/acc}{86.8}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_params/bfcl:live_multiple/acc_gold_in_candidates}{88.4}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_params/bfcl:live_multiple/auroc}{0.72}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_params/bfcl:live_multiple/brier}{0.095}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_params/bfcl:live_multiple/cost_per_1k_usd}{0.169}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_params/bfcl:live_multiple/coverage}{1}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_params/bfcl:live_multiple/defer_correct}{84.9}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_params/bfcl:live_multiple/ece}{0.097}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_params/bfcl:live_multiple/fill_precision}{80.0}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_params/bfcl:live_multiple/fill_rate}{61.3}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_params/bfcl:live_multiple/input_tokens}{166}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_params/bfcl:live_multiple/latency_p50_ms}{991}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_params/bfcl:live_multiple/latency_p95_ms}{7164}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_params/bfcl:live_multiple/n}{653}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_params/bfcl:live_multiple/n_errors}{0}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_params/bfcl:live_multiple/n_parse_fail}{1}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_params/bfcl:live_simple/acc}{88.2}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_params/bfcl:live_simple/acc_gold_in_candidates}{95.3}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_params/bfcl:live_simple/auroc}{0.75}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_params/bfcl:live_simple/brier}{0.086}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_params/bfcl:live_simple/cost_per_1k_usd}{0.168}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_params/bfcl:live_simple/coverage}{1}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_params/bfcl:live_simple/defer_correct}{78.9}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_params/bfcl:live_simple/ece}{0.088}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_params/bfcl:live_simple/fill_precision}{82.9}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_params/bfcl:live_simple/fill_rate}{64.7}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_params/bfcl:live_simple/input_tokens}{179}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_params/bfcl:live_simple/latency_p50_ms}{898}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_params/bfcl:live_simple/latency_p95_ms}{2359}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_params/bfcl:live_simple/n}{380}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_params/bfcl:live_simple/n_errors}{0}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_params/bfcl:multiple/acc}{92.8}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_params/bfcl:multiple/acc_gold_in_candidates}{95.0}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_params/bfcl:multiple/auroc}{0.67}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_params/bfcl:multiple/brier}{0.063}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_params/bfcl:multiple/cost_per_1k_usd}{0.145}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_params/bfcl:multiple/coverage}{1}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_params/bfcl:multiple/defer_correct}{88.5}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_params/bfcl:multiple/ece}{0.069}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_params/bfcl:multiple/fill_precision}{92.0}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_params/bfcl:multiple/fill_rate}{68.2}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_params/bfcl:multiple/input_tokens}{149}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_params/bfcl:multiple/latency_p50_ms}{788}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_params/bfcl:multiple/latency_p95_ms}{1567}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_params/bfcl:multiple/n}{459}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_params/bfcl:multiple/n_errors}{0}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_params/bfcl:simple_python/acc}{89.1}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_params/bfcl:simple_python/acc_gold_in_candidates}{96.3}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_params/bfcl:simple_python/auroc}{0.54}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_params/bfcl:simple_python/brier}{0.105}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_params/bfcl:simple_python/cost_per_1k_usd}{0.149}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_params/bfcl:simple_python/coverage}{1}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_params/bfcl:simple_python/defer_correct}{78.5}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_params/bfcl:simple_python/ece}{0.102}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_params/bfcl:simple_python/fill_precision}{85.6}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_params/bfcl:simple_python/fill_rate}{66.7}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_params/bfcl:simple_python/input_tokens}{153}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_params/bfcl:simple_python/latency_p50_ms}{835}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_params/bfcl:simple_python/latency_p95_ms}{1626}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_params/bfcl:simple_python/n}{457}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_params/bfcl:simple_python/n_errors}{0}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_select/bfcl/acc}{90.7}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_select/bfcl/auroc}{0.65}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_select/bfcl/brier}{0.088}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_select/bfcl/cost_per_1k_usd}{0.147}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_select/bfcl/coverage}{1}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_select/bfcl/ece}{0.080}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_select/bfcl/input_tokens}{242}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_select/bfcl/latency_p50_ms}{576}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_select/bfcl/latency_p95_ms}{1519}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_select/bfcl/n}{1114}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_select/bfcl/n_errors}{0}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_select/bfcl:irrelevance/acc}{88.1}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_select/bfcl:irrelevance/auroc}{0.52}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_select/bfcl:irrelevance/brier}{0.117}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_select/bfcl:irrelevance/cost_per_1k_usd}{0.109}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_select/bfcl:irrelevance/coverage}{1}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_select/bfcl:irrelevance/ece}{0.114}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_select/bfcl:irrelevance/input_tokens}{191}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_select/bfcl:irrelevance/latency_p50_ms}{547}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_select/bfcl:irrelevance/latency_p95_ms}{1774}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_select/bfcl:irrelevance/n}{185}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_select/bfcl:irrelevance/n_errors}{0}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_select/bfcl:live_irrelevance/acc}{71.9}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_select/bfcl:live_irrelevance/auroc}{0.66}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_select/bfcl:live_irrelevance/brier}{0.260}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_select/bfcl:live_irrelevance/cost_per_1k_usd}{0.176}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_select/bfcl:live_irrelevance/coverage}{1}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_select/bfcl:live_irrelevance/ece}{0.265}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_select/bfcl:live_irrelevance/input_tokens}{291}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_select/bfcl:live_irrelevance/latency_p50_ms}{589}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_select/bfcl:live_irrelevance/latency_p95_ms}{1477}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_select/bfcl:live_irrelevance/n}{185}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_select/bfcl:live_irrelevance/n_errors}{0}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_select/bfcl:live_multiple/acc}{93.5}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_select/bfcl:live_multiple/auroc}{0.64}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_select/bfcl:live_multiple/brier}{0.060}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_select/bfcl:live_multiple/cost_per_1k_usd}{0.214}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_select/bfcl:live_multiple/coverage}{1}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_select/bfcl:live_multiple/ece}{0.041}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_select/bfcl:live_multiple/input_tokens}{329}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_select/bfcl:live_multiple/latency_p50_ms}{627}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_select/bfcl:live_multiple/latency_p95_ms}{3209}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_select/bfcl:live_multiple/n}{186}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_select/bfcl:live_multiple/n_errors}{0}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_select/bfcl:live_simple/acc}{94.1}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_select/bfcl:live_simple/auroc}{0.79}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_select/bfcl:live_simple/brier}{0.058}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_select/bfcl:live_simple/cost_per_1k_usd}{0.115}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_select/bfcl:live_simple/coverage}{1}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_select/bfcl:live_simple/ece}{0.058}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_select/bfcl:live_simple/input_tokens}{216}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_select/bfcl:live_simple/latency_p50_ms}{542}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_select/bfcl:live_simple/latency_p95_ms}{1456}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_select/bfcl:live_simple/n}{186}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_select/bfcl:live_simple/n_errors}{0}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_select/bfcl:multiple/acc}{97.8}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_select/bfcl:multiple/auroc}{0.98}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_select/bfcl:multiple/brier}{0.014}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_select/bfcl:multiple/cost_per_1k_usd}{0.154}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_select/bfcl:multiple/coverage}{1}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_select/bfcl:multiple/ece}{0.020}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_select/bfcl:multiple/input_tokens}{231}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_select/bfcl:multiple/latency_p50_ms}{582}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_select/bfcl:multiple/latency_p95_ms}{1240}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_select/bfcl:multiple/n}{186}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_select/bfcl:multiple/n_errors}{0}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_select/bfcl:simple_python/acc}{98.4}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_select/bfcl:simple_python/auroc}{0.57}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_select/bfcl:simple_python/brier}{0.016}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_select/bfcl:simple_python/cost_per_1k_usd}{0.114}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_select/bfcl:simple_python/coverage}{1}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_select/bfcl:simple_python/ece}{0.013}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_select/bfcl:simple_python/input_tokens}{195}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_select/bfcl:simple_python/latency_p50_ms}{582}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_select/bfcl:simple_python/latency_p95_ms}{1261}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_select/bfcl:simple_python/n}{186}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_select/bfcl:simple_python/n_errors}{0}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_select/when2call/acc}{62.6}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_select/when2call/auroc}{0.56}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_select/when2call/brier}{0.355}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_select/when2call/cost_per_1k_usd}{0.291}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_select/when2call/coverage}{1}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_select/when2call/ece}{0.355}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_select/when2call/input_tokens}{659}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_select/when2call/latency_p50_ms}{570}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_select/when2call/latency_p95_ms}{1490}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_select/when2call/n}{928}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_select/when2call/n_errors}{0}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_select/when2call:BFCLv2LiveMultiple/acc}{62.2}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_select/when2call:BFCLv2LiveMultiple/auroc}{0.57}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_select/when2call:BFCLv2LiveMultiple/brier}{0.357}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_select/when2call:BFCLv2LiveMultiple/cost_per_1k_usd}{0.32}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_select/when2call:BFCLv2LiveMultiple/coverage}{1}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_select/when2call:BFCLv2LiveMultiple/ece}{0.359}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_select/when2call:BFCLv2LiveMultiple/input_tokens}{754}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_select/when2call:BFCLv2LiveMultiple/latency_p50_ms}{572}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_select/when2call:BFCLv2LiveMultiple/latency_p95_ms}{1547}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_select/when2call:BFCLv2LiveMultiple/n}{731}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_select/when2call:BFCLv2LiveMultiple/n_errors}{0}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_select/when2call:BFCLv2LiveSimple/acc}{64.0}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_select/when2call:BFCLv2LiveSimple/auroc}{0.51}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_select/when2call:BFCLv2LiveSimple/brier}{0.347}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_select/when2call:BFCLv2LiveSimple/cost_per_1k_usd}{0.184}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_select/when2call:BFCLv2LiveSimple/coverage}{1}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_select/when2call:BFCLv2LiveSimple/ece}{0.343}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_select/when2call:BFCLv2LiveSimple/input_tokens}{303}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_select/when2call:BFCLv2LiveSimple/latency_p50_ms}{560}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_select/when2call:BFCLv2LiveSimple/latency_p95_ms}{1303}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_select/when2call:BFCLv2LiveSimple/n}{197}
\defres{e1_bfcl_when2call/gemini_lite_dist/tool_select/when2call:BFCLv2LiveSimple/n_errors}{0}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_params/bfcl/acc}{89.7}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_params/bfcl/acc_gold_in_candidates}{95.2}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_params/bfcl/auroc}{0.69}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_params/bfcl/brier}{0.083}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_params/bfcl/cost_per_1k_usd}{0.0957}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_params/bfcl/coverage}{1}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_params/bfcl/defer_correct}{81.7}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_params/bfcl/ece}{0.063}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_params/bfcl/fill_precision}{85.5}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_params/bfcl/fill_rate}{65.7}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_params/bfcl/input_tokens}{160}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_params/bfcl/latency_p50_ms}{649}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_params/bfcl/latency_p95_ms}{1328}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_params/bfcl/n}{1949}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_params/bfcl/n_errors}{0}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_params/bfcl/n_parse_fail}{15}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_params/bfcl:live_multiple/acc}{89.0}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_params/bfcl:live_multiple/acc_gold_in_candidates}{92.3}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_params/bfcl:live_multiple/auroc}{0.75}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_params/bfcl:live_multiple/brier}{0.076}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_params/bfcl:live_multiple/cost_per_1k_usd}{0.0971}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_params/bfcl:live_multiple/coverage}{1}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_params/bfcl:live_multiple/defer_correct}{84.9}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_params/bfcl:live_multiple/ece}{0.065}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_params/bfcl:live_multiple/fill_precision}{82.9}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_params/bfcl:live_multiple/fill_rate}{61.7}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_params/bfcl:live_multiple/input_tokens}{164}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_params/bfcl:live_multiple/latency_p50_ms}{664}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_params/bfcl:live_multiple/latency_p95_ms}{1328}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_params/bfcl:live_multiple/n}{653}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_params/bfcl:live_multiple/n_errors}{0}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_params/bfcl:live_multiple/n_parse_fail}{7}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_params/bfcl:live_simple/acc}{87.4}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_params/bfcl:live_simple/acc_gold_in_candidates}{94.4}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_params/bfcl:live_simple/auroc}{0.73}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_params/bfcl:live_simple/brier}{0.095}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_params/bfcl:live_simple/cost_per_1k_usd}{0.1}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_params/bfcl:live_simple/coverage}{1}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_params/bfcl:live_simple/defer_correct}{78.3}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_params/bfcl:live_simple/ece}{0.076}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_params/bfcl:live_simple/fill_precision}{81.8}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_params/bfcl:live_simple/fill_rate}{65.0}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_params/bfcl:live_simple/input_tokens}{176}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_params/bfcl:live_simple/latency_p50_ms}{620}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_params/bfcl:live_simple/latency_p95_ms}{1213}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_params/bfcl:live_simple/n}{380}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_params/bfcl:live_simple/n_errors}{0}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_params/bfcl:live_simple/n_parse_fail}{4}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_params/bfcl:multiple/acc}{93.2}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_params/bfcl:multiple/acc_gold_in_candidates}{97.4}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_params/bfcl:multiple/auroc}{0.71}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_params/bfcl:multiple/brier}{0.060}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_params/bfcl:multiple/cost_per_1k_usd}{0.0924}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_params/bfcl:multiple/coverage}{1}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_params/bfcl:multiple/defer_correct}{85.3}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_params/bfcl:multiple/ece}{0.043}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_params/bfcl:multiple/fill_precision}{91.9}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_params/bfcl:multiple/fill_rate}{69.9}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_params/bfcl:multiple/input_tokens}{150}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_params/bfcl:multiple/latency_p50_ms}{653}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_params/bfcl:multiple/latency_p95_ms}{1214}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_params/bfcl:multiple/n}{459}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_params/bfcl:multiple/n_errors}{0}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_params/bfcl:multiple/n_parse_fail}{4}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_params/bfcl:simple_python/acc}{89.1}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_params/bfcl:simple_python/acc_gold_in_candidates}{97.4}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_params/bfcl:simple_python/auroc}{0.58}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_params/bfcl:simple_python/brier}{0.105}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_params/bfcl:simple_python/cost_per_1k_usd}{0.0931}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_params/bfcl:simple_python/coverage}{1}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_params/bfcl:simple_python/defer_correct}{76.9}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_params/bfcl:simple_python/ece}{0.095}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_params/bfcl:simple_python/fill_precision}{85.4}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_params/bfcl:simple_python/fill_rate}{67.6}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_params/bfcl:simple_python/input_tokens}{152}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_params/bfcl:simple_python/latency_p50_ms}{649}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_params/bfcl:simple_python/latency_p95_ms}{1437}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_params/bfcl:simple_python/n}{457}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_params/bfcl:simple_python/n_errors}{0}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_select/bfcl/acc}{90.4}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_select/bfcl/auroc}{0.77}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_select/bfcl/brier}{0.087}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_select/bfcl/cost_per_1k_usd}{0.119}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_select/bfcl/coverage}{1}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_select/bfcl/ece}{0.078}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_select/bfcl/input_tokens}{238}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_select/bfcl/latency_p50_ms}{534}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_select/bfcl/latency_p95_ms}{1101}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_select/bfcl/n}{1114}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_select/bfcl/n_errors}{0}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_select/bfcl:irrelevance/acc}{88.1}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_select/bfcl:irrelevance/auroc}{0.70}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_select/bfcl:irrelevance/brier}{0.110}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_select/bfcl:irrelevance/cost_per_1k_usd}{0.104}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_select/bfcl:irrelevance/coverage}{1}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_select/bfcl:irrelevance/ece}{0.104}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_select/bfcl:irrelevance/input_tokens}{190}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_select/bfcl:irrelevance/latency_p50_ms}{509}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_select/bfcl:irrelevance/latency_p95_ms}{1062}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_select/bfcl:irrelevance/n}{185}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_select/bfcl:irrelevance/n_errors}{0}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_select/bfcl:live_irrelevance/acc}{70.8}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_select/bfcl:live_irrelevance/auroc}{0.71}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_select/bfcl:live_irrelevance/brier}{0.260}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_select/bfcl:live_irrelevance/cost_per_1k_usd}{0.133}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_select/bfcl:live_irrelevance/coverage}{1}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_select/bfcl:live_irrelevance/ece}{0.261}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_select/bfcl:live_irrelevance/input_tokens}{285}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_select/bfcl:live_irrelevance/latency_p50_ms}{531}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_select/bfcl:live_irrelevance/latency_p95_ms}{1043}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_select/bfcl:live_irrelevance/n}{185}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_select/bfcl:live_irrelevance/n_errors}{0}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_select/bfcl:live_multiple/acc}{95.2}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_select/bfcl:live_multiple/auroc}{0.84}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_select/bfcl:live_multiple/brier}{0.043}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_select/bfcl:live_multiple/cost_per_1k_usd}{0.143}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_select/bfcl:live_multiple/coverage}{1}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_select/bfcl:live_multiple/ece}{0.030}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_select/bfcl:live_multiple/input_tokens}{319}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_select/bfcl:live_multiple/latency_p50_ms}{522}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_select/bfcl:live_multiple/latency_p95_ms}{1076}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_select/bfcl:live_multiple/n}{186}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_select/bfcl:live_multiple/n_errors}{0}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_select/bfcl:live_simple/acc}{90.9}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_select/bfcl:live_simple/auroc}{0.86}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_select/bfcl:live_simple/brier}{0.083}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_select/bfcl:live_simple/cost_per_1k_usd}{0.112}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_select/bfcl:live_simple/coverage}{1}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_select/bfcl:live_simple/ece}{0.076}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_select/bfcl:live_simple/input_tokens}{215}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_select/bfcl:live_simple/latency_p50_ms}{539}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_select/bfcl:live_simple/latency_p95_ms}{965}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_select/bfcl:live_simple/n}{186}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_select/bfcl:live_simple/n_errors}{0}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_select/bfcl:multiple/acc}{98.4}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_select/bfcl:multiple/auroc}{0.70}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_select/bfcl:multiple/brier}{0.016}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_select/bfcl:multiple/cost_per_1k_usd}{0.115}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_select/bfcl:multiple/coverage}{1}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_select/bfcl:multiple/ece}{0.007}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_select/bfcl:multiple/input_tokens}{227}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_select/bfcl:multiple/latency_p50_ms}{550}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_select/bfcl:multiple/latency_p95_ms}{1285}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_select/bfcl:multiple/n}{186}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_select/bfcl:multiple/n_errors}{0}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_select/bfcl:simple_python/acc}{98.9}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_select/bfcl:simple_python/auroc}{0.98}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_select/bfcl:simple_python/brier}{0.010}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_select/bfcl:simple_python/cost_per_1k_usd}{0.106}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_select/bfcl:simple_python/coverage}{1}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_select/bfcl:simple_python/ece}{0.000}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_select/bfcl:simple_python/input_tokens}{195}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_select/bfcl:simple_python/latency_p50_ms}{549}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_select/bfcl:simple_python/latency_p95_ms}{1153}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_select/bfcl:simple_python/n}{186}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_select/bfcl:simple_python/n_errors}{0}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_select/when2call/acc}{64.9}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_select/when2call/auroc}{0.62}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_select/when2call/brier}{0.327}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_select/when2call/cost_per_1k_usd}{0.243}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_select/when2call/coverage}{1}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_select/when2call/ece}{0.325}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_select/when2call/input_tokens}{652}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_select/when2call/latency_p50_ms}{521}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_select/when2call/latency_p95_ms}{1055}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_select/when2call/n}{928}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_select/when2call/n_errors}{0}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_select/when2call:BFCLv2LiveMultiple/acc}{65.0}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_select/when2call:BFCLv2LiveMultiple/auroc}{0.62}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_select/when2call:BFCLv2LiveMultiple/brier}{0.326}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_select/when2call:BFCLv2LiveMultiple/cost_per_1k_usd}{0.272}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_select/when2call:BFCLv2LiveMultiple/coverage}{1}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_select/when2call:BFCLv2LiveMultiple/ece}{0.324}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_select/when2call:BFCLv2LiveMultiple/input_tokens}{747}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_select/when2call:BFCLv2LiveMultiple/latency_p50_ms}{523}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_select/when2call:BFCLv2LiveMultiple/latency_p95_ms}{1066}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_select/when2call:BFCLv2LiveMultiple/n}{731}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_select/when2call:BFCLv2LiveMultiple/n_errors}{0}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_select/when2call:BFCLv2LiveSimple/acc}{64.5}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_select/when2call:BFCLv2LiveSimple/auroc}{0.61}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_select/when2call:BFCLv2LiveSimple/brier}{0.331}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_select/when2call:BFCLv2LiveSimple/cost_per_1k_usd}{0.136}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_select/when2call:BFCLv2LiveSimple/coverage}{1}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_select/when2call:BFCLv2LiveSimple/ece}{0.329}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_select/when2call:BFCLv2LiveSimple/input_tokens}{297}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_select/when2call:BFCLv2LiveSimple/latency_p50_ms}{515}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_select/when2call:BFCLv2LiveSimple/latency_p95_ms}{935}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_select/when2call:BFCLv2LiveSimple/n}{197}
\defres{e1_bfcl_when2call/gemini_lite_label/tool_select/when2call:BFCLv2LiveSimple/n_errors}{0}
\defres{e1_bfcl_when2call/gemma4_dist/tool_params/bfcl/acc}{87.4}
\defres{e1_bfcl_when2call/gemma4_dist/tool_params/bfcl/acc_gold_in_candidates}{94.3}
\defres{e1_bfcl_when2call/gemma4_dist/tool_params/bfcl/auroc}{0.71}
\defres{e1_bfcl_when2call/gemma4_dist/tool_params/bfcl/brier}{0.101}
\defres{e1_bfcl_when2call/gemma4_dist/tool_params/bfcl/cost_per_1k_usd}{0}
\defres{e1_bfcl_when2call/gemma4_dist/tool_params/bfcl/coverage}{1}
\defres{e1_bfcl_when2call/gemma4_dist/tool_params/bfcl/defer_correct}{77.6}
\defres{e1_bfcl_when2call/gemma4_dist/tool_params/bfcl/ece}{0.095}
\defres{e1_bfcl_when2call/gemma4_dist/tool_params/bfcl/fill_precision}{82.6}
\defres{e1_bfcl_when2call/gemma4_dist/tool_params/bfcl/fill_rate}{67.4}
\defres{e1_bfcl_when2call/gemma4_dist/tool_params/bfcl/input_tokens}{162}
\defres{e1_bfcl_when2call/gemma4_dist/tool_params/bfcl/latency_p50_ms}{3536}
\defres{e1_bfcl_when2call/gemma4_dist/tool_params/bfcl/latency_p95_ms}{14832}
\defres{e1_bfcl_when2call/gemma4_dist/tool_params/bfcl/n}{1949}
\defres{e1_bfcl_when2call/gemma4_dist/tool_params/bfcl/n_errors}{0}
\defres{e1_bfcl_when2call/gemma4_dist/tool_params/bfcl/n_parse_fail}{18}
\defres{e1_bfcl_when2call/gemma4_dist/tool_params/bfcl/unpriced}{1}
\defres{e1_bfcl_when2call/gemma4_dist/tool_params/bfcl:live_multiple/acc}{82.8}
\defres{e1_bfcl_when2call/gemma4_dist/tool_params/bfcl:live_multiple/acc_gold_in_candidates}{89.8}
\defres{e1_bfcl_when2call/gemma4_dist/tool_params/bfcl:live_multiple/auroc}{0.72}
\defres{e1_bfcl_when2call/gemma4_dist/tool_params/bfcl:live_multiple/brier}{0.129}
\defres{e1_bfcl_when2call/gemma4_dist/tool_params/bfcl:live_multiple/cost_per_1k_usd}{0}
\defres{e1_bfcl_when2call/gemma4_dist/tool_params/bfcl:live_multiple/coverage}{1}
\defres{e1_bfcl_when2call/gemma4_dist/tool_params/bfcl:live_multiple/defer_correct}{74.2}
\defres{e1_bfcl_when2call/gemma4_dist/tool_params/bfcl:live_multiple/ece}{0.122}
\defres{e1_bfcl_when2call/gemma4_dist/tool_params/bfcl:live_multiple/fill_precision}{75.4}
\defres{e1_bfcl_when2call/gemma4_dist/tool_params/bfcl:live_multiple/fill_rate}{66.0}
\defres{e1_bfcl_when2call/gemma4_dist/tool_params/bfcl:live_multiple/input_tokens}{166}
\defres{e1_bfcl_when2call/gemma4_dist/tool_params/bfcl:live_multiple/latency_p50_ms}{4823}
\defres{e1_bfcl_when2call/gemma4_dist/tool_params/bfcl:live_multiple/latency_p95_ms}{24216}
\defres{e1_bfcl_when2call/gemma4_dist/tool_params/bfcl:live_multiple/n}{653}
\defres{e1_bfcl_when2call/gemma4_dist/tool_params/bfcl:live_multiple/n_errors}{0}
\defres{e1_bfcl_when2call/gemma4_dist/tool_params/bfcl:live_multiple/n_parse_fail}{13}
\defres{e1_bfcl_when2call/gemma4_dist/tool_params/bfcl:live_multiple/unpriced}{1}
\defres{e1_bfcl_when2call/gemma4_dist/tool_params/bfcl:live_simple/acc}{85.8}
\defres{e1_bfcl_when2call/gemma4_dist/tool_params/bfcl:live_simple/acc_gold_in_candidates}{94.9}
\defres{e1_bfcl_when2call/gemma4_dist/tool_params/bfcl:live_simple/auroc}{0.65}
\defres{e1_bfcl_when2call/gemma4_dist/tool_params/bfcl:live_simple/brier}{0.119}
\defres{e1_bfcl_when2call/gemma4_dist/tool_params/bfcl:live_simple/cost_per_1k_usd}{0}
\defres{e1_bfcl_when2call/gemma4_dist/tool_params/bfcl:live_simple/coverage}{1}
\defres{e1_bfcl_when2call/gemma4_dist/tool_params/bfcl:live_simple/defer_correct}{74.1}
\defres{e1_bfcl_when2call/gemma4_dist/tool_params/bfcl:live_simple/ece}{0.113}
\defres{e1_bfcl_when2call/gemma4_dist/tool_params/bfcl:live_simple/fill_precision}{79.6}
\defres{e1_bfcl_when2call/gemma4_dist/tool_params/bfcl:live_simple/fill_rate}{67.1}
\defres{e1_bfcl_when2call/gemma4_dist/tool_params/bfcl:live_simple/input_tokens}{179}
\defres{e1_bfcl_when2call/gemma4_dist/tool_params/bfcl:live_simple/latency_p50_ms}{3040}
\defres{e1_bfcl_when2call/gemma4_dist/tool_params/bfcl:live_simple/latency_p95_ms}{11061}
\defres{e1_bfcl_when2call/gemma4_dist/tool_params/bfcl:live_simple/n}{380}
\defres{e1_bfcl_when2call/gemma4_dist/tool_params/bfcl:live_simple/n_errors}{0}
\defres{e1_bfcl_when2call/gemma4_dist/tool_params/bfcl:live_simple/n_parse_fail}{3}
\defres{e1_bfcl_when2call/gemma4_dist/tool_params/bfcl:live_simple/unpriced}{1}
\defres{e1_bfcl_when2call/gemma4_dist/tool_params/bfcl:multiple/acc}{93.5}
\defres{e1_bfcl_when2call/gemma4_dist/tool_params/bfcl:multiple/acc_gold_in_candidates}{96.4}
\defres{e1_bfcl_when2call/gemma4_dist/tool_params/bfcl:multiple/auroc}{0.81}
\defres{e1_bfcl_when2call/gemma4_dist/tool_params/bfcl:multiple/brier}{0.053}
\defres{e1_bfcl_when2call/gemma4_dist/tool_params/bfcl:multiple/cost_per_1k_usd}{0}
\defres{e1_bfcl_when2call/gemma4_dist/tool_params/bfcl:multiple/coverage}{1}
\defres{e1_bfcl_when2call/gemma4_dist/tool_params/bfcl:multiple/defer_correct}{87.8}
\defres{e1_bfcl_when2call/gemma4_dist/tool_params/bfcl:multiple/ece}{0.049}
\defres{e1_bfcl_when2call/gemma4_dist/tool_params/bfcl:multiple/fill_precision}{92.1}
\defres{e1_bfcl_when2call/gemma4_dist/tool_params/bfcl:multiple/fill_rate}{69.1}
\defres{e1_bfcl_when2call/gemma4_dist/tool_params/bfcl:multiple/input_tokens}{149}
\defres{e1_bfcl_when2call/gemma4_dist/tool_params/bfcl:multiple/latency_p50_ms}{3137}
\defres{e1_bfcl_when2call/gemma4_dist/tool_params/bfcl:multiple/latency_p95_ms}{7441}
\defres{e1_bfcl_when2call/gemma4_dist/tool_params/bfcl:multiple/n}{459}
\defres{e1_bfcl_when2call/gemma4_dist/tool_params/bfcl:multiple/n_errors}{0}
\defres{e1_bfcl_when2call/gemma4_dist/tool_params/bfcl:multiple/unpriced}{1}
\defres{e1_bfcl_when2call/gemma4_dist/tool_params/bfcl:simple_python/acc}{89.3}
\defres{e1_bfcl_when2call/gemma4_dist/tool_params/bfcl:simple_python/acc_gold_in_candidates}{97.4}
\defres{e1_bfcl_when2call/gemma4_dist/tool_params/bfcl:simple_python/auroc}{0.63}
\defres{e1_bfcl_when2call/gemma4_dist/tool_params/bfcl:simple_python/brier}{0.096}
\defres{e1_bfcl_when2call/gemma4_dist/tool_params/bfcl:simple_python/cost_per_1k_usd}{0}
\defres{e1_bfcl_when2call/gemma4_dist/tool_params/bfcl:simple_python/coverage}{1}
\defres{e1_bfcl_when2call/gemma4_dist/tool_params/bfcl:simple_python/defer_correct}{77.4}
\defres{e1_bfcl_when2call/gemma4_dist/tool_params/bfcl:simple_python/ece}{0.091}
\defres{e1_bfcl_when2call/gemma4_dist/tool_params/bfcl:simple_python/fill_precision}{85.2}
\defres{e1_bfcl_when2call/gemma4_dist/tool_params/bfcl:simple_python/fill_rate}{67.8}
\defres{e1_bfcl_when2call/gemma4_dist/tool_params/bfcl:simple_python/input_tokens}{153}
\defres{e1_bfcl_when2call/gemma4_dist/tool_params/bfcl:simple_python/latency_p50_ms}{3309}
\defres{e1_bfcl_when2call/gemma4_dist/tool_params/bfcl:simple_python/latency_p95_ms}{8754}
\defres{e1_bfcl_when2call/gemma4_dist/tool_params/bfcl:simple_python/n}{457}
\defres{e1_bfcl_when2call/gemma4_dist/tool_params/bfcl:simple_python/n_errors}{0}
\defres{e1_bfcl_when2call/gemma4_dist/tool_params/bfcl:simple_python/n_parse_fail}{2}
\defres{e1_bfcl_when2call/gemma4_dist/tool_params/bfcl:simple_python/unpriced}{1}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/bfcl/acc}{89.1}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/bfcl/auroc}{0.68}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/bfcl/brier}{0.097}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/bfcl/cost_per_1k_usd}{0}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/bfcl/coverage}{1}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/bfcl/ece}{0.094}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/bfcl/input_tokens}{242}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/bfcl/latency_p50_ms}{1188}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/bfcl/latency_p95_ms}{2468}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/bfcl/n}{1114}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/bfcl/n_errors}{0}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/bfcl/unpriced}{1}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/bfcl:irrelevance/acc}{85.4}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/bfcl:irrelevance/auroc}{0.63}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/bfcl:irrelevance/brier}{0.135}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/bfcl:irrelevance/cost_per_1k_usd}{0}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/bfcl:irrelevance/coverage}{1}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/bfcl:irrelevance/ece}{0.133}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/bfcl:irrelevance/input_tokens}{191}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/bfcl:irrelevance/latency_p50_ms}{880}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/bfcl:irrelevance/latency_p95_ms}{1954}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/bfcl:irrelevance/n}{185}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/bfcl:irrelevance/n_errors}{0}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/bfcl:irrelevance/unpriced}{1}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/bfcl:live_irrelevance/acc}{63.2}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/bfcl:live_irrelevance/auroc}{0.72}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/bfcl:live_irrelevance/brier}{0.320}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/bfcl:live_irrelevance/cost_per_1k_usd}{0}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/bfcl:live_irrelevance/coverage}{1}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/bfcl:live_irrelevance/ece}{0.335}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/bfcl:live_irrelevance/input_tokens}{291}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/bfcl:live_irrelevance/latency_p50_ms}{1228}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/bfcl:live_irrelevance/latency_p95_ms}{3389}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/bfcl:live_irrelevance/n}{185}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/bfcl:live_irrelevance/n_errors}{0}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/bfcl:live_irrelevance/unpriced}{1}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/bfcl:live_multiple/acc}{91.9}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/bfcl:live_multiple/auroc}{0.87}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/bfcl:live_multiple/brier}{0.065}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/bfcl:live_multiple/cost_per_1k_usd}{0}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/bfcl:live_multiple/coverage}{1}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/bfcl:live_multiple/ece}{0.051}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/bfcl:live_multiple/input_tokens}{329}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/bfcl:live_multiple/latency_p50_ms}{1521}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/bfcl:live_multiple/latency_p95_ms}{2307}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/bfcl:live_multiple/n}{186}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/bfcl:live_multiple/n_errors}{0}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/bfcl:live_multiple/unpriced}{1}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/bfcl:live_simple/acc}{96.2}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/bfcl:live_simple/auroc}{0.55}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/bfcl:live_simple/brier}{0.037}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/bfcl:live_simple/cost_per_1k_usd}{0}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/bfcl:live_simple/coverage}{1}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/bfcl:live_simple/ece}{0.039}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/bfcl:live_simple/input_tokens}{216}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/bfcl:live_simple/latency_p50_ms}{885}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/bfcl:live_simple/latency_p95_ms}{2799}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/bfcl:live_simple/n}{186}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/bfcl:live_simple/n_errors}{0}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/bfcl:live_simple/unpriced}{1}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/bfcl:multiple/acc}{99.5}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/bfcl:multiple/auroc}{0.99}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/bfcl:multiple/brier}{0.008}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/bfcl:multiple/cost_per_1k_usd}{0}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/bfcl:multiple/coverage}{1}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/bfcl:multiple/ece}{0.009}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/bfcl:multiple/input_tokens}{231}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/bfcl:multiple/latency_p50_ms}{1367}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/bfcl:multiple/latency_p95_ms}{2633}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/bfcl:multiple/n}{186}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/bfcl:multiple/n_errors}{0}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/bfcl:multiple/unpriced}{1}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/bfcl:simple_python/acc}{98.4}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/bfcl:simple_python/auroc}{0.67}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/bfcl:simple_python/brier}{0.015}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/bfcl:simple_python/cost_per_1k_usd}{0}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/bfcl:simple_python/coverage}{1}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/bfcl:simple_python/ece}{0.016}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/bfcl:simple_python/input_tokens}{195}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/bfcl:simple_python/latency_p50_ms}{948}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/bfcl:simple_python/latency_p95_ms}{2195}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/bfcl:simple_python/n}{186}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/bfcl:simple_python/n_errors}{0}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/bfcl:simple_python/unpriced}{1}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/when2call/acc}{54.4}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/when2call/auroc}{0.66}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/when2call/brier}{0.385}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/when2call/cost_per_1k_usd}{0}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/when2call/coverage}{1}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/when2call/ece}{0.392}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/when2call/input_tokens}{659}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/when2call/latency_p50_ms}{1273}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/when2call/latency_p95_ms}{2073}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/when2call/n}{928}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/when2call/n_errors}{0}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/when2call/n_parse_fail}{13}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/when2call/unpriced}{1}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/when2call:BFCLv2LiveMultiple/acc}{53.5}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/when2call:BFCLv2LiveMultiple/auroc}{0.66}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/when2call:BFCLv2LiveMultiple/brier}{0.384}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/when2call:BFCLv2LiveMultiple/cost_per_1k_usd}{0}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/when2call:BFCLv2LiveMultiple/coverage}{1}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/when2call:BFCLv2LiveMultiple/ece}{0.393}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/when2call:BFCLv2LiveMultiple/input_tokens}{754}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/when2call:BFCLv2LiveMultiple/latency_p50_ms}{1287}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/when2call:BFCLv2LiveMultiple/latency_p95_ms}{2198}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/when2call:BFCLv2LiveMultiple/n}{731}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/when2call:BFCLv2LiveMultiple/n_errors}{0}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/when2call:BFCLv2LiveMultiple/n_parse_fail}{13}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/when2call:BFCLv2LiveMultiple/unpriced}{1}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/when2call:BFCLv2LiveSimple/acc}{57.9}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/when2call:BFCLv2LiveSimple/auroc}{0.65}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/when2call:BFCLv2LiveSimple/brier}{0.387}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/when2call:BFCLv2LiveSimple/cost_per_1k_usd}{0}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/when2call:BFCLv2LiveSimple/coverage}{1}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/when2call:BFCLv2LiveSimple/ece}{0.386}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/when2call:BFCLv2LiveSimple/input_tokens}{303}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/when2call:BFCLv2LiveSimple/latency_p50_ms}{1240}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/when2call:BFCLv2LiveSimple/latency_p95_ms}{1972}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/when2call:BFCLv2LiveSimple/n}{197}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/when2call:BFCLv2LiveSimple/n_errors}{0}
\defres{e1_bfcl_when2call/gemma4_dist/tool_select/when2call:BFCLv2LiveSimple/unpriced}{1}
\defres{e1_bfcl_when2call/jev/tool_params/bfcl/acc}{89.6}
\defres{e1_bfcl_when2call/jev/tool_params/bfcl/acc_gold_in_candidates}{95.7}
\defres{e1_bfcl_when2call/jev/tool_params/bfcl/auroc}{0.86}
\defres{e1_bfcl_when2call/jev/tool_params/bfcl/brier}{0.074}
\defres{e1_bfcl_when2call/jev/tool_params/bfcl/cost_per_1k_usd}{0.00805}
\defres{e1_bfcl_when2call/jev/tool_params/bfcl/coverage}{1}
\defres{e1_bfcl_when2call/jev/tool_params/bfcl/defer_correct}{80.9}
\defres{e1_bfcl_when2call/jev/tool_params/bfcl/ece}{0.029}
\defres{e1_bfcl_when2call/jev/tool_params/bfcl/fill_precision}{85.0}
\defres{e1_bfcl_when2call/jev/tool_params/bfcl/fill_rate}{66.4}
\defres{e1_bfcl_when2call/jev/tool_params/bfcl/input_tokens}{192}
\defres{e1_bfcl_when2call/jev/tool_params/bfcl/latency_p50_ms}{209}
\defres{e1_bfcl_when2call/jev/tool_params/bfcl/latency_p95_ms}{343}
\defres{e1_bfcl_when2call/jev/tool_params/bfcl/n}{1949}
\defres{e1_bfcl_when2call/jev/tool_params/bfcl/n_errors}{0}
\defres{e1_bfcl_when2call/jev/tool_params/bfcl:live_multiple/acc}{89.1}
\defres{e1_bfcl_when2call/jev/tool_params/bfcl:live_multiple/acc_gold_in_candidates}{93.1}
\defres{e1_bfcl_when2call/jev/tool_params/bfcl:live_multiple/auroc}{0.83}
\defres{e1_bfcl_when2call/jev/tool_params/bfcl:live_multiple/brier}{0.086}
\defres{e1_bfcl_when2call/jev/tool_params/bfcl:live_multiple/cost_per_1k_usd}{0.00778}
\defres{e1_bfcl_when2call/jev/tool_params/bfcl:live_multiple/coverage}{1}
\defres{e1_bfcl_when2call/jev/tool_params/bfcl:live_multiple/defer_correct}{84.2}
\defres{e1_bfcl_when2call/jev/tool_params/bfcl:live_multiple/ece}{0.052}
\defres{e1_bfcl_when2call/jev/tool_params/bfcl:live_multiple/fill_precision}{82.6}
\defres{e1_bfcl_when2call/jev/tool_params/bfcl:live_multiple/fill_rate}{62.5}
\defres{e1_bfcl_when2call/jev/tool_params/bfcl:live_multiple/input_tokens}{185}
\defres{e1_bfcl_when2call/jev/tool_params/bfcl:live_multiple/latency_p50_ms}{209}
\defres{e1_bfcl_when2call/jev/tool_params/bfcl:live_multiple/latency_p95_ms}{317}
\defres{e1_bfcl_when2call/jev/tool_params/bfcl:live_multiple/n}{653}
\defres{e1_bfcl_when2call/jev/tool_params/bfcl:live_multiple/n_errors}{0}
\defres{e1_bfcl_when2call/jev/tool_params/bfcl:live_simple/acc}{88.7}
\defres{e1_bfcl_when2call/jev/tool_params/bfcl:live_simple/acc_gold_in_candidates}{94.9}
\defres{e1_bfcl_when2call/jev/tool_params/bfcl:live_simple/auroc}{0.94}
\defres{e1_bfcl_when2call/jev/tool_params/bfcl:live_simple/brier}{0.063}
\defres{e1_bfcl_when2call/jev/tool_params/bfcl:live_simple/cost_per_1k_usd}{0.00934}
\defres{e1_bfcl_when2call/jev/tool_params/bfcl:live_simple/coverage}{1}
\defres{e1_bfcl_when2call/jev/tool_params/bfcl:live_simple/defer_correct}{80.7}
\defres{e1_bfcl_when2call/jev/tool_params/bfcl:live_simple/ece}{0.037}
\defres{e1_bfcl_when2call/jev/tool_params/bfcl:live_simple/fill_precision}{82.9}
\defres{e1_bfcl_when2call/jev/tool_params/bfcl:live_simple/fill_rate}{64.5}
\defres{e1_bfcl_when2call/jev/tool_params/bfcl:live_simple/input_tokens}{222}
\defres{e1_bfcl_when2call/jev/tool_params/bfcl:live_simple/latency_p50_ms}{202}
\defres{e1_bfcl_when2call/jev/tool_params/bfcl:live_simple/latency_p95_ms}{322}
\defres{e1_bfcl_when2call/jev/tool_params/bfcl:live_simple/n}{380}
\defres{e1_bfcl_when2call/jev/tool_params/bfcl:live_simple/n_errors}{0}
\defres{e1_bfcl_when2call/jev/tool_params/bfcl:multiple/acc}{92.8}
\defres{e1_bfcl_when2call/jev/tool_params/bfcl:multiple/acc_gold_in_candidates}{96.7}
\defres{e1_bfcl_when2call/jev/tool_params/bfcl:multiple/auroc}{0.91}
\defres{e1_bfcl_when2call/jev/tool_params/bfcl:multiple/brier}{0.050}
\defres{e1_bfcl_when2call/jev/tool_params/bfcl:multiple/cost_per_1k_usd}{0.00766}
\defres{e1_bfcl_when2call/jev/tool_params/bfcl:multiple/coverage}{1}
\defres{e1_bfcl_when2call/jev/tool_params/bfcl:multiple/defer_correct}{85.3}
\defres{e1_bfcl_when2call/jev/tool_params/bfcl:multiple/ece}{0.024}
\defres{e1_bfcl_when2call/jev/tool_params/bfcl:multiple/fill_precision}{91.6}
\defres{e1_bfcl_when2call/jev/tool_params/bfcl:multiple/fill_rate}{69.7}
\defres{e1_bfcl_when2call/jev/tool_params/bfcl:multiple/input_tokens}{182}
\defres{e1_bfcl_when2call/jev/tool_params/bfcl:multiple/latency_p50_ms}{206}
\defres{e1_bfcl_when2call/jev/tool_params/bfcl:multiple/latency_p95_ms}{321}
\defres{e1_bfcl_when2call/jev/tool_params/bfcl:multiple/n}{459}
\defres{e1_bfcl_when2call/jev/tool_params/bfcl:multiple/n_errors}{0}
\defres{e1_bfcl_when2call/jev/tool_params/bfcl:simple_python/acc}{87.7}
\defres{e1_bfcl_when2call/jev/tool_params/bfcl:simple_python/acc_gold_in_candidates}{98.5}
\defres{e1_bfcl_when2call/jev/tool_params/bfcl:simple_python/auroc}{0.81}
\defres{e1_bfcl_when2call/jev/tool_params/bfcl:simple_python/brier}{0.091}
\defres{e1_bfcl_when2call/jev/tool_params/bfcl:simple_python/cost_per_1k_usd}{0.00775}
\defres{e1_bfcl_when2call/jev/tool_params/bfcl:simple_python/coverage}{1}
\defres{e1_bfcl_when2call/jev/tool_params/bfcl:simple_python/defer_correct}{72.0}
\defres{e1_bfcl_when2call/jev/tool_params/bfcl:simple_python/ece}{0.061}
\defres{e1_bfcl_when2call/jev/tool_params/bfcl:simple_python/fill_precision}{83.2}
\defres{e1_bfcl_when2call/jev/tool_params/bfcl:simple_python/fill_rate}{70.2}
\defres{e1_bfcl_when2call/jev/tool_params/bfcl:simple_python/input_tokens}{185}
\defres{e1_bfcl_when2call/jev/tool_params/bfcl:simple_python/latency_p50_ms}{218}
\defres{e1_bfcl_when2call/jev/tool_params/bfcl:simple_python/latency_p95_ms}{424}
\defres{e1_bfcl_when2call/jev/tool_params/bfcl:simple_python/n}{457}
\defres{e1_bfcl_when2call/jev/tool_params/bfcl:simple_python/n_errors}{0}
\defres{e1_bfcl_when2call/jev/tool_select/bfcl/acc}{89.9}
\defres{e1_bfcl_when2call/jev/tool_select/bfcl/auroc}{0.87}
\defres{e1_bfcl_when2call/jev/tool_select/bfcl/brier}{0.072}
\defres{e1_bfcl_when2call/jev/tool_select/bfcl/cost_per_1k_usd}{0.0167}
\defres{e1_bfcl_when2call/jev/tool_select/bfcl/coverage}{1}
\defres{e1_bfcl_when2call/jev/tool_select/bfcl/ece}{0.045}
\defres{e1_bfcl_when2call/jev/tool_select/bfcl/input_tokens}{398}
\defres{e1_bfcl_when2call/jev/tool_select/bfcl/latency_p50_ms}{206}
\defres{e1_bfcl_when2call/jev/tool_select/bfcl/latency_p95_ms}{327}
\defres{e1_bfcl_when2call/jev/tool_select/bfcl/n}{1114}
\defres{e1_bfcl_when2call/jev/tool_select/bfcl/n_errors}{0}
\defres{e1_bfcl_when2call/jev/tool_select/bfcl:irrelevance/acc}{85.4}
\defres{e1_bfcl_when2call/jev/tool_select/bfcl:irrelevance/auroc}{0.85}
\defres{e1_bfcl_when2call/jev/tool_select/bfcl:irrelevance/brier}{0.103}
\defres{e1_bfcl_when2call/jev/tool_select/bfcl:irrelevance/cost_per_1k_usd}{0.0148}
\defres{e1_bfcl_when2call/jev/tool_select/bfcl:irrelevance/coverage}{1}
\defres{e1_bfcl_when2call/jev/tool_select/bfcl:irrelevance/ece}{0.087}
\defres{e1_bfcl_when2call/jev/tool_select/bfcl:irrelevance/input_tokens}{353}
\defres{e1_bfcl_when2call/jev/tool_select/bfcl:irrelevance/latency_p50_ms}{207}
\defres{e1_bfcl_when2call/jev/tool_select/bfcl:irrelevance/latency_p95_ms}{315}
\defres{e1_bfcl_when2call/jev/tool_select/bfcl:irrelevance/n}{185}
\defres{e1_bfcl_when2call/jev/tool_select/bfcl:irrelevance/n_errors}{0}
\defres{e1_bfcl_when2call/jev/tool_select/bfcl:live_irrelevance/acc}{62.7}
\defres{e1_bfcl_when2call/jev/tool_select/bfcl:live_irrelevance/auroc}{0.84}
\defres{e1_bfcl_when2call/jev/tool_select/bfcl:live_irrelevance/brier}{0.239}
\defres{e1_bfcl_when2call/jev/tool_select/bfcl:live_irrelevance/cost_per_1k_usd}{0.0187}
\defres{e1_bfcl_when2call/jev/tool_select/bfcl:live_irrelevance/coverage}{1}
\defres{e1_bfcl_when2call/jev/tool_select/bfcl:live_irrelevance/ece}{0.237}
\defres{e1_bfcl_when2call/jev/tool_select/bfcl:live_irrelevance/input_tokens}{446}
\defres{e1_bfcl_when2call/jev/tool_select/bfcl:live_irrelevance/latency_p50_ms}{207}
\defres{e1_bfcl_when2call/jev/tool_select/bfcl:live_irrelevance/latency_p95_ms}{289}
\defres{e1_bfcl_when2call/jev/tool_select/bfcl:live_irrelevance/n}{185}
\defres{e1_bfcl_when2call/jev/tool_select/bfcl:live_irrelevance/n_errors}{0}
\defres{e1_bfcl_when2call/jev/tool_select/bfcl:live_multiple/acc}{94.6}
\defres{e1_bfcl_when2call/jev/tool_select/bfcl:live_multiple/auroc}{0.96}
\defres{e1_bfcl_when2call/jev/tool_select/bfcl:live_multiple/brier}{0.029}
\defres{e1_bfcl_when2call/jev/tool_select/bfcl:live_multiple/cost_per_1k_usd}{0.0208}
\defres{e1_bfcl_when2call/jev/tool_select/bfcl:live_multiple/coverage}{1}
\defres{e1_bfcl_when2call/jev/tool_select/bfcl:live_multiple/ece}{0.032}
\defres{e1_bfcl_when2call/jev/tool_select/bfcl:live_multiple/input_tokens}{496}
\defres{e1_bfcl_when2call/jev/tool_select/bfcl:live_multiple/latency_p50_ms}{207}
\defres{e1_bfcl_when2call/jev/tool_select/bfcl:live_multiple/latency_p95_ms}{307}
\defres{e1_bfcl_when2call/jev/tool_select/bfcl:live_multiple/n}{186}
\defres{e1_bfcl_when2call/jev/tool_select/bfcl:live_multiple/n_errors}{0}
\defres{e1_bfcl_when2call/jev/tool_select/bfcl:live_simple/acc}{97.8}
\defres{e1_bfcl_when2call/jev/tool_select/bfcl:live_simple/auroc}{0.98}
\defres{e1_bfcl_when2call/jev/tool_select/bfcl:live_simple/brier}{0.045}
\defres{e1_bfcl_when2call/jev/tool_select/bfcl:live_simple/cost_per_1k_usd}{0.0158}
\defres{e1_bfcl_when2call/jev/tool_select/bfcl:live_simple/coverage}{1}
\defres{e1_bfcl_when2call/jev/tool_select/bfcl:live_simple/ece}{0.100}
\defres{e1_bfcl_when2call/jev/tool_select/bfcl:live_simple/input_tokens}{377}
\defres{e1_bfcl_when2call/jev/tool_select/bfcl:live_simple/latency_p50_ms}{201}
\defres{e1_bfcl_when2call/jev/tool_select/bfcl:live_simple/latency_p95_ms}{351}
\defres{e1_bfcl_when2call/jev/tool_select/bfcl:live_simple/n}{186}
\defres{e1_bfcl_when2call/jev/tool_select/bfcl:live_simple/n_errors}{0}
\defres{e1_bfcl_when2call/jev/tool_select/bfcl:multiple/acc}{98.9}
\defres{e1_bfcl_when2call/jev/tool_select/bfcl:multiple/auroc}{0.99}
\defres{e1_bfcl_when2call/jev/tool_select/bfcl:multiple/brier}{0.006}
\defres{e1_bfcl_when2call/jev/tool_select/bfcl:multiple/cost_per_1k_usd}{0.0157}
\defres{e1_bfcl_when2call/jev/tool_select/bfcl:multiple/coverage}{1}
\defres{e1_bfcl_when2call/jev/tool_select/bfcl:multiple/ece}{0.019}
\defres{e1_bfcl_when2call/jev/tool_select/bfcl:multiple/input_tokens}{375}
\defres{e1_bfcl_when2call/jev/tool_select/bfcl:multiple/latency_p50_ms}{202}
\defres{e1_bfcl_when2call/jev/tool_select/bfcl:multiple/latency_p95_ms}{300}
\defres{e1_bfcl_when2call/jev/tool_select/bfcl:multiple/n}{186}
\defres{e1_bfcl_when2call/jev/tool_select/bfcl:multiple/n_errors}{0}
\defres{e1_bfcl_when2call/jev/tool_select/bfcl:simple_python/acc}{100.0}
\defres{e1_bfcl_when2call/jev/tool_select/bfcl:simple_python/brier}{0.008}
\defres{e1_bfcl_when2call/jev/tool_select/bfcl:simple_python/cost_per_1k_usd}{0.0143}
\defres{e1_bfcl_when2call/jev/tool_select/bfcl:simple_python/coverage}{1}
\defres{e1_bfcl_when2call/jev/tool_select/bfcl:simple_python/ece}{0.025}
\defres{e1_bfcl_when2call/jev/tool_select/bfcl:simple_python/input_tokens}{341}
\defres{e1_bfcl_when2call/jev/tool_select/bfcl:simple_python/latency_p50_ms}{212}
\defres{e1_bfcl_when2call/jev/tool_select/bfcl:simple_python/latency_p95_ms}{367}
\defres{e1_bfcl_when2call/jev/tool_select/bfcl:simple_python/n}{186}
\defres{e1_bfcl_when2call/jev/tool_select/bfcl:simple_python/n_errors}{0}
\defres{e1_bfcl_when2call/jev/tool_select/when2call/acc}{75.4}
\defres{e1_bfcl_when2call/jev/tool_select/when2call/auroc}{0.72}
\defres{e1_bfcl_when2call/jev/tool_select/when2call/brier}{0.170}
\defres{e1_bfcl_when2call/jev/tool_select/when2call/cost_per_1k_usd}{0.0332}
\defres{e1_bfcl_when2call/jev/tool_select/when2call/coverage}{1}
\defres{e1_bfcl_when2call/jev/tool_select/when2call/ece}{0.080}
\defres{e1_bfcl_when2call/jev/tool_select/when2call/input_tokens}{790}
\defres{e1_bfcl_when2call/jev/tool_select/when2call/latency_p50_ms}{203}
\defres{e1_bfcl_when2call/jev/tool_select/when2call/latency_p95_ms}{292}
\defres{e1_bfcl_when2call/jev/tool_select/when2call/n}{928}
\defres{e1_bfcl_when2call/jev/tool_select/when2call/n_errors}{0}
\defres{e1_bfcl_when2call/jev/tool_select/when2call:BFCLv2LiveMultiple/acc}{75.2}
\defres{e1_bfcl_when2call/jev/tool_select/when2call:BFCLv2LiveMultiple/auroc}{0.73}
\defres{e1_bfcl_when2call/jev/tool_select/when2call:BFCLv2LiveMultiple/brier}{0.170}
\defres{e1_bfcl_when2call/jev/tool_select/when2call:BFCLv2LiveMultiple/cost_per_1k_usd}{0.0371}
\defres{e1_bfcl_when2call/jev/tool_select/when2call:BFCLv2LiveMultiple/coverage}{1}
\defres{e1_bfcl_when2call/jev/tool_select/when2call:BFCLv2LiveMultiple/ece}{0.082}
\defres{e1_bfcl_when2call/jev/tool_select/when2call:BFCLv2LiveMultiple/input_tokens}{883}
\defres{e1_bfcl_when2call/jev/tool_select/when2call:BFCLv2LiveMultiple/latency_p50_ms}{204}
\defres{e1_bfcl_when2call/jev/tool_select/when2call:BFCLv2LiveMultiple/latency_p95_ms}{286}
\defres{e1_bfcl_when2call/jev/tool_select/when2call:BFCLv2LiveMultiple/n}{731}
\defres{e1_bfcl_when2call/jev/tool_select/when2call:BFCLv2LiveMultiple/n_errors}{0}
\defres{e1_bfcl_when2call/jev/tool_select/when2call:BFCLv2LiveSimple/acc}{76.1}
\defres{e1_bfcl_when2call/jev/tool_select/when2call:BFCLv2LiveSimple/auroc}{0.71}
\defres{e1_bfcl_when2call/jev/tool_select/when2call:BFCLv2LiveSimple/brier}{0.173}
\defres{e1_bfcl_when2call/jev/tool_select/when2call:BFCLv2LiveSimple/cost_per_1k_usd}{0.0187}
\defres{e1_bfcl_when2call/jev/tool_select/when2call:BFCLv2LiveSimple/coverage}{1}
\defres{e1_bfcl_when2call/jev/tool_select/when2call:BFCLv2LiveSimple/ece}{0.115}
\defres{e1_bfcl_when2call/jev/tool_select/when2call:BFCLv2LiveSimple/input_tokens}{444}
\defres{e1_bfcl_when2call/jev/tool_select/when2call:BFCLv2LiveSimple/latency_p50_ms}{200}
\defres{e1_bfcl_when2call/jev/tool_select/when2call:BFCLv2LiveSimple/latency_p95_ms}{306}
\defres{e1_bfcl_when2call/jev/tool_select/when2call:BFCLv2LiveSimple/n}{197}
\defres{e1_bfcl_when2call/jev/tool_select/when2call:BFCLv2LiveSimple/n_errors}{0}
\defres{e1_bfcl_when2call/tfidf/tool_params/bfcl/acc}{31.6}
\defres{e1_bfcl_when2call/tfidf/tool_params/bfcl/acc_gold_in_candidates}{53.6}
\defres{e1_bfcl_when2call/tfidf/tool_params/bfcl/auroc}{0.59}
\defres{e1_bfcl_when2call/tfidf/tool_params/bfcl/brier}{0.453}
\defres{e1_bfcl_when2call/tfidf/tool_params/bfcl/cost_per_1k_usd}{0}
\defres{e1_bfcl_when2call/tfidf/tool_params/bfcl/coverage}{1}
\defres{e1_bfcl_when2call/tfidf/tool_params/bfcl/defer_correct}{0.0}
\defres{e1_bfcl_when2call/tfidf/tool_params/bfcl/ece}{0.440}
\defres{e1_bfcl_when2call/tfidf/tool_params/bfcl/fill_precision}{31.6}
\defres{e1_bfcl_when2call/tfidf/tool_params/bfcl/fill_rate}{100.0}
\defres{e1_bfcl_when2call/tfidf/tool_params/bfcl/input_tokens}{0}
\defres{e1_bfcl_when2call/tfidf/tool_params/bfcl/latency_p50_ms}{1}
\defres{e1_bfcl_when2call/tfidf/tool_params/bfcl/latency_p95_ms}{5}
\defres{e1_bfcl_when2call/tfidf/tool_params/bfcl/n}{1949}
\defres{e1_bfcl_when2call/tfidf/tool_params/bfcl/n_errors}{0}
\defres{e1_bfcl_when2call/tfidf/tool_params/bfcl:live_multiple/acc}{28.6}
\defres{e1_bfcl_when2call/tfidf/tool_params/bfcl:live_multiple/acc_gold_in_candidates}{51.7}
\defres{e1_bfcl_when2call/tfidf/tool_params/bfcl:live_multiple/auroc}{0.54}
\defres{e1_bfcl_when2call/tfidf/tool_params/bfcl:live_multiple/brier}{0.467}
\defres{e1_bfcl_when2call/tfidf/tool_params/bfcl:live_multiple/cost_per_1k_usd}{0}
\defres{e1_bfcl_when2call/tfidf/tool_params/bfcl:live_multiple/coverage}{1}
\defres{e1_bfcl_when2call/tfidf/tool_params/bfcl:live_multiple/defer_correct}{0.0}
\defres{e1_bfcl_when2call/tfidf/tool_params/bfcl:live_multiple/ece}{0.461}
\defres{e1_bfcl_when2call/tfidf/tool_params/bfcl:live_multiple/fill_precision}{28.6}
\defres{e1_bfcl_when2call/tfidf/tool_params/bfcl:live_multiple/fill_rate}{100.0}
\defres{e1_bfcl_when2call/tfidf/tool_params/bfcl:live_multiple/input_tokens}{0}
\defres{e1_bfcl_when2call/tfidf/tool_params/bfcl:live_multiple/latency_p50_ms}{1}
\defres{e1_bfcl_when2call/tfidf/tool_params/bfcl:live_multiple/latency_p95_ms}{9}
\defres{e1_bfcl_when2call/tfidf/tool_params/bfcl:live_multiple/n}{653}
\defres{e1_bfcl_when2call/tfidf/tool_params/bfcl:live_multiple/n_errors}{0}
\defres{e1_bfcl_when2call/tfidf/tool_params/bfcl:live_simple/acc}{30.3}
\defres{e1_bfcl_when2call/tfidf/tool_params/bfcl:live_simple/acc_gold_in_candidates}{53.7}
\defres{e1_bfcl_when2call/tfidf/tool_params/bfcl:live_simple/auroc}{0.63}
\defres{e1_bfcl_when2call/tfidf/tool_params/bfcl:live_simple/brier}{0.495}
\defres{e1_bfcl_when2call/tfidf/tool_params/bfcl:live_simple/cost_per_1k_usd}{0}
\defres{e1_bfcl_when2call/tfidf/tool_params/bfcl:live_simple/coverage}{1}
\defres{e1_bfcl_when2call/tfidf/tool_params/bfcl:live_simple/defer_correct}{0.0}
\defres{e1_bfcl_when2call/tfidf/tool_params/bfcl:live_simple/ece}{0.509}
\defres{e1_bfcl_when2call/tfidf/tool_params/bfcl:live_simple/fill_precision}{30.3}
\defres{e1_bfcl_when2call/tfidf/tool_params/bfcl:live_simple/fill_rate}{100.0}
\defres{e1_bfcl_when2call/tfidf/tool_params/bfcl:live_simple/input_tokens}{0}
\defres{e1_bfcl_when2call/tfidf/tool_params/bfcl:live_simple/latency_p50_ms}{1}
\defres{e1_bfcl_when2call/tfidf/tool_params/bfcl:live_simple/latency_p95_ms}{4}
\defres{e1_bfcl_when2call/tfidf/tool_params/bfcl:live_simple/n}{380}
\defres{e1_bfcl_when2call/tfidf/tool_params/bfcl:live_simple/n_errors}{0}
\defres{e1_bfcl_when2call/tfidf/tool_params/bfcl:multiple/acc}{36.2}
\defres{e1_bfcl_when2call/tfidf/tool_params/bfcl:multiple/acc_gold_in_candidates}{54.8}
\defres{e1_bfcl_when2call/tfidf/tool_params/bfcl:multiple/auroc}{0.58}
\defres{e1_bfcl_when2call/tfidf/tool_params/bfcl:multiple/brier}{0.432}
\defres{e1_bfcl_when2call/tfidf/tool_params/bfcl:multiple/cost_per_1k_usd}{0}
\defres{e1_bfcl_when2call/tfidf/tool_params/bfcl:multiple/coverage}{1}
\defres{e1_bfcl_when2call/tfidf/tool_params/bfcl:multiple/defer_correct}{0.0}
\defres{e1_bfcl_when2call/tfidf/tool_params/bfcl:multiple/ece}{0.394}
\defres{e1_bfcl_when2call/tfidf/tool_params/bfcl:multiple/fill_precision}{36.2}
\defres{e1_bfcl_when2call/tfidf/tool_params/bfcl:multiple/fill_rate}{100.0}
\defres{e1_bfcl_when2call/tfidf/tool_params/bfcl:multiple/input_tokens}{0}
\defres{e1_bfcl_when2call/tfidf/tool_params/bfcl:multiple/latency_p50_ms}{1}
\defres{e1_bfcl_when2call/tfidf/tool_params/bfcl:multiple/latency_p95_ms}{2}
\defres{e1_bfcl_when2call/tfidf/tool_params/bfcl:multiple/n}{459}
\defres{e1_bfcl_when2call/tfidf/tool_params/bfcl:multiple/n_errors}{0}
\defres{e1_bfcl_when2call/tfidf/tool_params/bfcl:simple_python/acc}{32.4}
\defres{e1_bfcl_when2call/tfidf/tool_params/bfcl:simple_python/acc_gold_in_candidates}{54.6}
\defres{e1_bfcl_when2call/tfidf/tool_params/bfcl:simple_python/auroc}{0.63}
\defres{e1_bfcl_when2call/tfidf/tool_params/bfcl:simple_python/brier}{0.419}
\defres{e1_bfcl_when2call/tfidf/tool_params/bfcl:simple_python/cost_per_1k_usd}{0}
\defres{e1_bfcl_when2call/tfidf/tool_params/bfcl:simple_python/coverage}{1}
\defres{e1_bfcl_when2call/tfidf/tool_params/bfcl:simple_python/defer_correct}{0.0}
\defres{e1_bfcl_when2call/tfidf/tool_params/bfcl:simple_python/ece}{0.423}
\defres{e1_bfcl_when2call/tfidf/tool_params/bfcl:simple_python/fill_precision}{32.4}
\defres{e1_bfcl_when2call/tfidf/tool_params/bfcl:simple_python/fill_rate}{100.0}
\defres{e1_bfcl_when2call/tfidf/tool_params/bfcl:simple_python/input_tokens}{0}
\defres{e1_bfcl_when2call/tfidf/tool_params/bfcl:simple_python/latency_p50_ms}{1}
\defres{e1_bfcl_when2call/tfidf/tool_params/bfcl:simple_python/latency_p95_ms}{2}
\defres{e1_bfcl_when2call/tfidf/tool_params/bfcl:simple_python/n}{457}
\defres{e1_bfcl_when2call/tfidf/tool_params/bfcl:simple_python/n_errors}{0}
\defres{e1_bfcl_when2call/tfidf/tool_select/bfcl/acc}{62.3}
\defres{e1_bfcl_when2call/tfidf/tool_select/bfcl/auroc}{0.82}
\defres{e1_bfcl_when2call/tfidf/tool_select/bfcl/brier}{0.243}
\defres{e1_bfcl_when2call/tfidf/tool_select/bfcl/cost_per_1k_usd}{0}
\defres{e1_bfcl_when2call/tfidf/tool_select/bfcl/coverage}{1}
\defres{e1_bfcl_when2call/tfidf/tool_select/bfcl/ece}{0.251}
\defres{e1_bfcl_when2call/tfidf/tool_select/bfcl/input_tokens}{0}
\defres{e1_bfcl_when2call/tfidf/tool_select/bfcl/latency_p50_ms}{0}
\defres{e1_bfcl_when2call/tfidf/tool_select/bfcl/latency_p95_ms}{1}
\defres{e1_bfcl_when2call/tfidf/tool_select/bfcl/n}{1114}
\defres{e1_bfcl_when2call/tfidf/tool_select/bfcl/n_errors}{0}
\defres{e1_bfcl_when2call/tfidf/tool_select/bfcl:irrelevance/acc}{0.0}
\defres{e1_bfcl_when2call/tfidf/tool_select/bfcl:irrelevance/brier}{0.583}
\defres{e1_bfcl_when2call/tfidf/tool_select/bfcl:irrelevance/cost_per_1k_usd}{0}
\defres{e1_bfcl_when2call/tfidf/tool_select/bfcl:irrelevance/coverage}{1}
\defres{e1_bfcl_when2call/tfidf/tool_select/bfcl:irrelevance/ece}{0.724}
\defres{e1_bfcl_when2call/tfidf/tool_select/bfcl:irrelevance/input_tokens}{0}
\defres{e1_bfcl_when2call/tfidf/tool_select/bfcl:irrelevance/latency_p50_ms}{0}
\defres{e1_bfcl_when2call/tfidf/tool_select/bfcl:irrelevance/latency_p95_ms}{0}
\defres{e1_bfcl_when2call/tfidf/tool_select/bfcl:irrelevance/n}{185}
\defres{e1_bfcl_when2call/tfidf/tool_select/bfcl:irrelevance/n_errors}{0}
\defres{e1_bfcl_when2call/tfidf/tool_select/bfcl:live_irrelevance/acc}{0.0}
\defres{e1_bfcl_when2call/tfidf/tool_select/bfcl:live_irrelevance/brier}{0.673}
\defres{e1_bfcl_when2call/tfidf/tool_select/bfcl:live_irrelevance/cost_per_1k_usd}{0}
\defres{e1_bfcl_when2call/tfidf/tool_select/bfcl:live_irrelevance/coverage}{1}
\defres{e1_bfcl_when2call/tfidf/tool_select/bfcl:live_irrelevance/ece}{0.779}
\defres{e1_bfcl_when2call/tfidf/tool_select/bfcl:live_irrelevance/input_tokens}{0}
\defres{e1_bfcl_when2call/tfidf/tool_select/bfcl:live_irrelevance/latency_p50_ms}{0}
\defres{e1_bfcl_when2call/tfidf/tool_select/bfcl:live_irrelevance/latency_p95_ms}{1}
\defres{e1_bfcl_when2call/tfidf/tool_select/bfcl:live_irrelevance/n}{185}
\defres{e1_bfcl_when2call/tfidf/tool_select/bfcl:live_irrelevance/n_errors}{0}
\defres{e1_bfcl_when2call/tfidf/tool_select/bfcl:live_multiple/acc}{77.4}
\defres{e1_bfcl_when2call/tfidf/tool_select/bfcl:live_multiple/auroc}{0.82}
\defres{e1_bfcl_when2call/tfidf/tool_select/bfcl:live_multiple/brier}{0.145}
\defres{e1_bfcl_when2call/tfidf/tool_select/bfcl:live_multiple/cost_per_1k_usd}{0}
\defres{e1_bfcl_when2call/tfidf/tool_select/bfcl:live_multiple/coverage}{1}
\defres{e1_bfcl_when2call/tfidf/tool_select/bfcl:live_multiple/ece}{0.082}
\defres{e1_bfcl_when2call/tfidf/tool_select/bfcl:live_multiple/input_tokens}{0}
\defres{e1_bfcl_when2call/tfidf/tool_select/bfcl:live_multiple/latency_p50_ms}{1}
\defres{e1_bfcl_when2call/tfidf/tool_select/bfcl:live_multiple/latency_p95_ms}{1}
\defres{e1_bfcl_when2call/tfidf/tool_select/bfcl:live_multiple/n}{186}
\defres{e1_bfcl_when2call/tfidf/tool_select/bfcl:live_multiple/n_errors}{0}
\defres{e1_bfcl_when2call/tfidf/tool_select/bfcl:live_simple/acc}{100.0}
\defres{e1_bfcl_when2call/tfidf/tool_select/bfcl:live_simple/brier}{0.018}
\defres{e1_bfcl_when2call/tfidf/tool_select/bfcl:live_simple/cost_per_1k_usd}{0}
\defres{e1_bfcl_when2call/tfidf/tool_select/bfcl:live_simple/coverage}{1}
\defres{e1_bfcl_when2call/tfidf/tool_select/bfcl:live_simple/ece}{0.042}
\defres{e1_bfcl_when2call/tfidf/tool_select/bfcl:live_simple/input_tokens}{0}
\defres{e1_bfcl_when2call/tfidf/tool_select/bfcl:live_simple/latency_p50_ms}{0}
\defres{e1_bfcl_when2call/tfidf/tool_select/bfcl:live_simple/latency_p95_ms}{1}
\defres{e1_bfcl_when2call/tfidf/tool_select/bfcl:live_simple/n}{186}
\defres{e1_bfcl_when2call/tfidf/tool_select/bfcl:live_simple/n_errors}{0}
\defres{e1_bfcl_when2call/tfidf/tool_select/bfcl:multiple/acc}{95.7}
\defres{e1_bfcl_when2call/tfidf/tool_select/bfcl:multiple/auroc}{0.96}
\defres{e1_bfcl_when2call/tfidf/tool_select/bfcl:multiple/brier}{0.033}
\defres{e1_bfcl_when2call/tfidf/tool_select/bfcl:multiple/cost_per_1k_usd}{0}
\defres{e1_bfcl_when2call/tfidf/tool_select/bfcl:multiple/coverage}{1}
\defres{e1_bfcl_when2call/tfidf/tool_select/bfcl:multiple/ece}{0.037}
\defres{e1_bfcl_when2call/tfidf/tool_select/bfcl:multiple/input_tokens}{0}
\defres{e1_bfcl_when2call/tfidf/tool_select/bfcl:multiple/latency_p50_ms}{0}
\defres{e1_bfcl_when2call/tfidf/tool_select/bfcl:multiple/latency_p95_ms}{1}
\defres{e1_bfcl_when2call/tfidf/tool_select/bfcl:multiple/n}{186}
\defres{e1_bfcl_when2call/tfidf/tool_select/bfcl:multiple/n_errors}{0}
\defres{e1_bfcl_when2call/tfidf/tool_select/bfcl:simple_python/acc}{100.0}
\defres{e1_bfcl_when2call/tfidf/tool_select/bfcl:simple_python/brier}{0.011}
\defres{e1_bfcl_when2call/tfidf/tool_select/bfcl:simple_python/cost_per_1k_usd}{0}
\defres{e1_bfcl_when2call/tfidf/tool_select/bfcl:simple_python/coverage}{1}
\defres{e1_bfcl_when2call/tfidf/tool_select/bfcl:simple_python/ece}{0.022}
\defres{e1_bfcl_when2call/tfidf/tool_select/bfcl:simple_python/input_tokens}{0}
\defres{e1_bfcl_when2call/tfidf/tool_select/bfcl:simple_python/latency_p50_ms}{0}
\defres{e1_bfcl_when2call/tfidf/tool_select/bfcl:simple_python/latency_p95_ms}{1}
\defres{e1_bfcl_when2call/tfidf/tool_select/bfcl:simple_python/n}{186}
\defres{e1_bfcl_when2call/tfidf/tool_select/bfcl:simple_python/n_errors}{0}
\defres{e1_bfcl_when2call/tfidf/tool_select/when2call/acc}{30.4}
\defres{e1_bfcl_when2call/tfidf/tool_select/when2call/auroc}{0.53}
\defres{e1_bfcl_when2call/tfidf/tool_select/when2call/brier}{0.575}
\defres{e1_bfcl_when2call/tfidf/tool_select/when2call/cost_per_1k_usd}{0}
\defres{e1_bfcl_when2call/tfidf/tool_select/when2call/coverage}{1}
\defres{e1_bfcl_when2call/tfidf/tool_select/when2call/ece}{0.590}
\defres{e1_bfcl_when2call/tfidf/tool_select/when2call/input_tokens}{0}
\defres{e1_bfcl_when2call/tfidf/tool_select/when2call/latency_p50_ms}{1}
\defres{e1_bfcl_when2call/tfidf/tool_select/when2call/latency_p95_ms}{1}
\defres{e1_bfcl_when2call/tfidf/tool_select/when2call/n}{928}
\defres{e1_bfcl_when2call/tfidf/tool_select/when2call/n_errors}{0}
\defres{e1_bfcl_when2call/tfidf/tool_select/when2call:BFCLv2LiveMultiple/acc}{29.8}
\defres{e1_bfcl_when2call/tfidf/tool_select/when2call:BFCLv2LiveMultiple/auroc}{0.49}
\defres{e1_bfcl_when2call/tfidf/tool_select/when2call:BFCLv2LiveMultiple/brier}{0.596}
\defres{e1_bfcl_when2call/tfidf/tool_select/when2call:BFCLv2LiveMultiple/cost_per_1k_usd}{0}
\defres{e1_bfcl_when2call/tfidf/tool_select/when2call:BFCLv2LiveMultiple/coverage}{1}
\defres{e1_bfcl_when2call/tfidf/tool_select/when2call:BFCLv2LiveMultiple/ece}{0.605}
\defres{e1_bfcl_when2call/tfidf/tool_select/when2call:BFCLv2LiveMultiple/input_tokens}{0}
\defres{e1_bfcl_when2call/tfidf/tool_select/when2call:BFCLv2LiveMultiple/latency_p50_ms}{1}
\defres{e1_bfcl_when2call/tfidf/tool_select/when2call:BFCLv2LiveMultiple/latency_p95_ms}{2}
\defres{e1_bfcl_when2call/tfidf/tool_select/when2call:BFCLv2LiveMultiple/n}{731}
\defres{e1_bfcl_when2call/tfidf/tool_select/when2call:BFCLv2LiveMultiple/n_errors}{0}
\defres{e1_bfcl_when2call/tfidf/tool_select/when2call:BFCLv2LiveSimple/acc}{32.5}
\defres{e1_bfcl_when2call/tfidf/tool_select/when2call:BFCLv2LiveSimple/auroc}{0.67}
\defres{e1_bfcl_when2call/tfidf/tool_select/when2call:BFCLv2LiveSimple/brier}{0.494}
\defres{e1_bfcl_when2call/tfidf/tool_select/when2call:BFCLv2LiveSimple/cost_per_1k_usd}{0}
\defres{e1_bfcl_when2call/tfidf/tool_select/when2call:BFCLv2LiveSimple/coverage}{1}
\defres{e1_bfcl_when2call/tfidf/tool_select/when2call:BFCLv2LiveSimple/ece}{0.543}
\defres{e1_bfcl_when2call/tfidf/tool_select/when2call:BFCLv2LiveSimple/input_tokens}{0}
\defres{e1_bfcl_when2call/tfidf/tool_select/when2call:BFCLv2LiveSimple/latency_p50_ms}{0}
\defres{e1_bfcl_when2call/tfidf/tool_select/when2call:BFCLv2LiveSimple/latency_p95_ms}{1}
\defres{e1_bfcl_when2call/tfidf/tool_select/when2call:BFCLv2LiveSimple/n}{197}
\defres{e1_bfcl_when2call/tfidf/tool_select/when2call:BFCLv2LiveSimple/n_errors}{0}
\defres{e1_bfcl_when2call_rl/jevagent_rl/tool_params/bfcl/acc}{85.0}
\defres{e1_bfcl_when2call_rl/jevagent_rl/tool_params/bfcl/acc_gold_in_candidates}{95.0}
\defres{e1_bfcl_when2call_rl/jevagent_rl/tool_params/bfcl/ece}{0.132}
\defres{e1_bfcl_when2call_rl/jevagent_rl/tool_select/bfcl/acc}{88.4}
\defres{e1_bfcl_when2call_rl/jevagent_rl/tool_select/bfcl/auroc}{0.71}
\defres{e1_bfcl_when2call_rl/jevagent_rl/tool_select/bfcl/cost_per_1k_usd}{0}
\defres{e1_bfcl_when2call_rl/jevagent_rl/tool_select/bfcl/ece}{0.098}
\defres{e1_bfcl_when2call_rl/jevagent_rl/tool_select/bfcl/latency_p50_ms}{228}
\defres{e1_bfcl_when2call_rl/jevagent_rl/tool_select/when2call/acc}{54.0}
\defres{e1_bfcl_when2call_rl/jevagent_rl/tool_select/when2call/ece}{0.458}
\defres{e2a_jevgym_shadow_cal/jev_shadow_cal/cost_usd}{0.0428}
\defres{e2a_jevgym_shadow_cal/jev_shadow_cal/decisions/ece}{0.046}
\defres{e2a_jevgym_shadow_cal/jev_shadow_cal/decisions/gold/gates/stop_guard-shadow/ece}{0.154}
\defres{e2a_jevgym_shadow_cal/jev_shadow_cal/decisions/gold/gates/stop_trigger-shadow/ece}{0.028}
\defres{e2a_jevgym_shadow_cal/jev_shadow_cal/decisions/noul/ece}{0.045}
\defres{e2a_jevgym_shadow_cal/jev_shadow_cal/llm_calls}{7.50}
\defres{e2a_jevgym_shadow_cal/jev_shadow_cal/steps}{7.50}
\defres{e2a_jevgym_shadow_cal/jev_shadow_cal/success}{100.0}
\defres{e2a_jevgym_shadow_cal/jev_shadow_cal/success_ci/hi}{100.0}
\defres{e2a_jevgym_shadow_cal/jev_shadow_cal/success_ci/lo}{100.0}
\defres{e2a_jevgym_shadow_cal/jev_shadow_cal_s2lite/cost_usd}{0.00977}
\defres{e2a_jevgym_shadow_cal/jev_shadow_cal_s2lite/decisions/ece}{0.030}
\defres{e2a_jevgym_shadow_cal/jev_shadow_cal_s2lite/decisions/gold/gates/stop_guard-shadow/ece}{0.079}
\defres{e2a_jevgym_shadow_cal/jev_shadow_cal_s2lite/decisions/gold/gates/stop_trigger-shadow/ece}{0.027}
\defres{e2a_jevgym_shadow_cal/jev_shadow_cal_s2lite/decisions/noul/ece}{0.034}
\defres{e2a_jevgym_shadow_cal/jev_shadow_cal_s2lite/llm_calls}{7.59}
\defres{e2a_jevgym_shadow_cal/jev_shadow_cal_s2lite/steps}{7.59}
\defres{e2a_jevgym_shadow_cal/jev_shadow_cal_s2lite/success}{86.0}
\defres{e2a_jevgym_shadow_cal/jev_shadow_cal_s2lite/success_ci/hi}{91.3}
\defres{e2a_jevgym_shadow_cal/jev_shadow_cal_s2lite/success_ci/lo}{80.7}
\defres{e2a_jevgym_shadow_cal_intern/intern_shadow_cal/cost_usd}{0.0436}
\defres{e2a_jevgym_shadow_cal_intern/intern_shadow_cal/decisions/ece}{0.069}
\defres{e2a_jevgym_shadow_cal_intern/intern_shadow_cal/decisions/gold/gates/stop_guard-shadow/ece}{0.207}
\defres{e2a_jevgym_shadow_cal_intern/intern_shadow_cal/decisions/gold/gates/stop_trigger-shadow/ece}{0.238}
\defres{e2a_jevgym_shadow_cal_intern/intern_shadow_cal/decisions/noul/ece}{0.205}
\defres{e2a_jevgym_shadow_cal_intern/intern_shadow_cal/llm_calls}{7.50}
\defres{e2a_jevgym_shadow_cal_intern/intern_shadow_cal/steps}{7.50}
\defres{e2a_jevgym_shadow_cal_intern/intern_shadow_cal/success}{100.0}
\defres{e2a_jevgym_shadow_cal_intern/intern_shadow_cal/success_ci/hi}{100.0}
\defres{e2a_jevgym_shadow_cal_intern/intern_shadow_cal/success_ci/lo}{100.0}
\defres{e2a_jevgym_shadow_cal_intern/intern_shadow_cal_s2lite/cost_usd}{0.00979}
\defres{e2a_jevgym_shadow_cal_intern/intern_shadow_cal_s2lite/decisions/ece}{0.107}
\defres{e2a_jevgym_shadow_cal_intern/intern_shadow_cal_s2lite/decisions/gold/gates/stop_guard-shadow/ece}{0.130}
\defres{e2a_jevgym_shadow_cal_intern/intern_shadow_cal_s2lite/decisions/gold/gates/stop_trigger-shadow/ece}{0.240}
\defres{e2a_jevgym_shadow_cal_intern/intern_shadow_cal_s2lite/decisions/noul/ece}{0.205}
\defres{e2a_jevgym_shadow_cal_intern/intern_shadow_cal_s2lite/llm_calls}{7.59}
\defres{e2a_jevgym_shadow_cal_intern/intern_shadow_cal_s2lite/steps}{7.59}
\defres{e2a_jevgym_shadow_cal_intern/intern_shadow_cal_s2lite/success}{86.0}
\defres{e2a_jevgym_shadow_cal_intern/intern_shadow_cal_s2lite/success_ci/hi}{91.3}
\defres{e2a_jevgym_shadow_cal_intern/intern_shadow_cal_s2lite/success_ci/lo}{80.7}
\defres{e2a_jevgym_tool_decisions/bm25_ts_assist_k3_s2lite/cost_usd}{0.00205}
\defres{e2a_jevgym_tool_decisions/bm25_ts_assist_k3_s2lite/decisions/ece}{0.780}
\defres{e2a_jevgym_tool_decisions/bm25_ts_assist_k3_s2lite/llm_calls}{5.75}
\defres{e2a_jevgym_tool_decisions/bm25_ts_assist_k3_s2lite/steps}{5.75}
\defres{e2a_jevgym_tool_decisions/bm25_ts_assist_k3_s2lite/success}{12.5}
\defres{e2a_jevgym_tool_decisions/bm25_ts_assist_k3_s2lite/success_ci/hi}{17.0}
\defres{e2a_jevgym_tool_decisions/bm25_ts_assist_k3_s2lite/success_ci/lo}{8.0}
\defres{e2a_jevgym_tool_decisions/bm25_ts_assist_k3_s2lite/vs_baseline/cost_savings}{79.0}
\defres{e2a_jevgym_tool_decisions/bm25_ts_assist_k3_s2lite/vs_baseline/delta}{-69.5}
\defres{e2a_jevgym_tool_decisions/bm25_ts_assist_k3_s2lite/vs_baseline/delta_ci/hi}{-63.0}
\defres{e2a_jevgym_tool_decisions/bm25_ts_assist_k3_s2lite/vs_baseline/delta_ci/lo}{-76.0}
\defres{e2a_jevgym_tool_decisions/bm25_ts_assist_k3_s2lite/vs_baseline/ni/p_decisive}{1.000}
\defres{e2a_jevgym_tool_decisions/embed_ts_assist_k3/cost_usd}{0.00924}
\defres{e2a_jevgym_tool_decisions/embed_ts_assist_k3/decisions/ece}{0.153}
\defres{e2a_jevgym_tool_decisions/embed_ts_assist_k3/llm_calls}{4.82}
\defres{e2a_jevgym_tool_decisions/embed_ts_assist_k3/steps}{4.82}
\defres{e2a_jevgym_tool_decisions/embed_ts_assist_k3/success}{28.0}
\defres{e2a_jevgym_tool_decisions/embed_ts_assist_k3/success_ci/hi}{34.0}
\defres{e2a_jevgym_tool_decisions/embed_ts_assist_k3/success_ci/lo}{21.5}
\defres{e2a_jevgym_tool_decisions/embed_ts_assist_k3/vs_baseline/cost_savings}{78.5}
\defres{e2a_jevgym_tool_decisions/embed_ts_assist_k3/vs_baseline/delta}{-72.0}
\defres{e2a_jevgym_tool_decisions/embed_ts_assist_k3/vs_baseline/delta_ci/hi}{-65.5}
\defres{e2a_jevgym_tool_decisions/embed_ts_assist_k3/vs_baseline/delta_ci/lo}{-78.0}
\defres{e2a_jevgym_tool_decisions/embed_ts_assist_k3/vs_baseline/ni/p_decisive}{1.000}
\defres{e2a_jevgym_tool_decisions/headline/iso_cost/delta_ci/hi}{+0.0}
\defres{e2a_jevgym_tool_decisions/headline/iso_cost/delta_ci/lo}{+0.0}
\defres{e2a_jevgym_tool_decisions/headline/iso_cost/success}{99.8}
\defres{e2a_jevgym_tool_decisions/headline/iso_cost_by_reference/llm_only_s2lite/delta_ci/hi}{+3.2}
\defres{e2a_jevgym_tool_decisions/headline/iso_cost_by_reference/llm_only_s2lite/delta_ci/lo}{-1.0}
\defres{e2a_jevgym_tool_decisions/headline/iso_cost_by_reference/llm_only_s2lite/success}{81.2}
\defres{e2a_jevgym_tool_decisions/headline/iso_quality/cost_savings_ci/hi}{15.6}
\defres{e2a_jevgym_tool_decisions/headline/iso_quality/cost_savings_ci/lo}{12.7}
\defres{e2a_jevgym_tool_decisions/headline/iso_quality/delta_ci/hi}{+0.0}
\defres{e2a_jevgym_tool_decisions/headline/iso_quality/delta_ci/lo}{+0.0}
\defres{e2a_jevgym_tool_decisions/headline/iso_quality_by_reference/llm_only_s2lite/cost_savings_ci/hi}{0.7}
\defres{e2a_jevgym_tool_decisions/headline/iso_quality_by_reference/llm_only_s2lite/cost_savings_ci/lo}{-0.2}
\defres{e2a_jevgym_tool_decisions/headline/iso_quality_by_reference/llm_only_s2lite/delta_ci/hi}{+3.2}
\defres{e2a_jevgym_tool_decisions/headline/iso_quality_by_reference/llm_only_s2lite/delta_ci/lo}{-1.0}
\defres{e2a_jevgym_tool_decisions/jev_shadow/cost_usd}{0.0408}
\defres{e2a_jevgym_tool_decisions/jev_shadow/decisions/ece}{0.049}
\defres{e2a_jevgym_tool_decisions/jev_shadow/decisions/gold/gates/stop_guard-shadow/ece}{0.171}
\defres{e2a_jevgym_tool_decisions/jev_shadow/decisions/gold/gates/stop_trigger-shadow/ece}{0.029}
\defres{e2a_jevgym_tool_decisions/jev_shadow/decisions/noul/ece}{0.048}
\defres{e2a_jevgym_tool_decisions/jev_shadow/llm_calls}{7.51}
\defres{e2a_jevgym_tool_decisions/jev_shadow/steps}{7.51}
\defres{e2a_jevgym_tool_decisions/jev_shadow/success}{99.8}
\defres{e2a_jevgym_tool_decisions/jev_shadow/success_ci/hi}{100.0}
\defres{e2a_jevgym_tool_decisions/jev_shadow/success_ci/lo}{99.4}
\defres{e2a_jevgym_tool_decisions/jev_shadow/vs_baseline/cost_savings}{3.7}
\defres{e2a_jevgym_tool_decisions/jev_shadow/vs_baseline/delta}{+0.0}
\defres{e2a_jevgym_tool_decisions/jev_shadow/vs_baseline/delta_ci/hi}{+0.0}
\defres{e2a_jevgym_tool_decisions/jev_shadow/vs_baseline/delta_ci/lo}{+0.0}
\defres{e2a_jevgym_tool_decisions/jev_shadow/vs_baseline/ni/p_decisive}{$<$0.001}
\defres{e2a_jevgym_tool_decisions/jev_shadow_s2lite/cost_usd}{0.00976}
\defres{e2a_jevgym_tool_decisions/jev_shadow_s2lite/decisions/ece}{0.029}
\defres{e2a_jevgym_tool_decisions/jev_shadow_s2lite/decisions/gold/gates/stop_guard-shadow/ece}{0.077}
\defres{e2a_jevgym_tool_decisions/jev_shadow_s2lite/decisions/gold/gates/stop_trigger-shadow/ece}{0.028}
\defres{e2a_jevgym_tool_decisions/jev_shadow_s2lite/decisions/noul/ece}{0.034}
\defres{e2a_jevgym_tool_decisions/jev_shadow_s2lite/llm_calls}{7.57}
\defres{e2a_jevgym_tool_decisions/jev_shadow_s2lite/steps}{7.57}
\defres{e2a_jevgym_tool_decisions/jev_shadow_s2lite/success}{81.2}
\defres{e2a_jevgym_tool_decisions/jev_shadow_s2lite/success_ci/hi}{84.4}
\defres{e2a_jevgym_tool_decisions/jev_shadow_s2lite/success_ci/lo}{78.0}
\defres{e2a_jevgym_tool_decisions/jev_shadow_s2lite/vs_baseline/cost_savings}{0.4}
\defres{e2a_jevgym_tool_decisions/jev_shadow_s2lite/vs_baseline/delta}{+1.0}
\defres{e2a_jevgym_tool_decisions/jev_shadow_s2lite/vs_baseline/delta_ci/hi}{+3.2}
\defres{e2a_jevgym_tool_decisions/jev_shadow_s2lite/vs_baseline/delta_ci/lo}{-1.2}
\defres{e2a_jevgym_tool_decisions/jev_shadow_s2lite/vs_baseline/ni/p_decisive}{$<$0.001}
\defres{e2a_jevgym_tool_decisions/jev_ts_assist_k3/cost_usd}{0.0196}
\defres{e2a_jevgym_tool_decisions/jev_ts_assist_k3/decisions/ece}{0.051}
\defres{e2a_jevgym_tool_decisions/jev_ts_assist_k3/llm_calls}{8.10}
\defres{e2a_jevgym_tool_decisions/jev_ts_assist_k3/steps}{8.10}
\defres{e2a_jevgym_tool_decisions/jev_ts_assist_k3/success}{92.0}
\defres{e2a_jevgym_tool_decisions/jev_ts_assist_k3/success_ci/hi}{94.2}
\defres{e2a_jevgym_tool_decisions/jev_ts_assist_k3/success_ci/lo}{89.4}
\defres{e2a_jevgym_tool_decisions/jev_ts_assist_k3/vs_baseline/cost_savings}{53.7}
\defres{e2a_jevgym_tool_decisions/jev_ts_assist_k3/vs_baseline/delta}{-7.8}
\defres{e2a_jevgym_tool_decisions/jev_ts_assist_k3/vs_baseline/delta_ci/hi}{-5.4}
\defres{e2a_jevgym_tool_decisions/jev_ts_assist_k3/vs_baseline/delta_ci/lo}{-10.2}
\defres{e2a_jevgym_tool_decisions/jev_ts_assist_k3/vs_baseline/ni/p_decisive}{1.000}
\defres{e2a_jevgym_tool_decisions/jev_ts_assist_k3_s2lite/cost_usd}{0.0047}
\defres{e2a_jevgym_tool_decisions/jev_ts_assist_k3_s2lite/decisions/ece}{0.065}
\defres{e2a_jevgym_tool_decisions/jev_ts_assist_k3_s2lite/llm_calls}{8.04}
\defres{e2a_jevgym_tool_decisions/jev_ts_assist_k3_s2lite/steps}{8.04}
\defres{e2a_jevgym_tool_decisions/jev_ts_assist_k3_s2lite/success}{76.8}
\defres{e2a_jevgym_tool_decisions/jev_ts_assist_k3_s2lite/success_ci/hi}{80.6}
\defres{e2a_jevgym_tool_decisions/jev_ts_assist_k3_s2lite/success_ci/lo}{73.2}
\defres{e2a_jevgym_tool_decisions/jev_ts_assist_k3_s2lite/vs_baseline/cost_savings}{52.0}
\defres{e2a_jevgym_tool_decisions/jev_ts_assist_k3_s2lite/vs_baseline/delta}{-3.4}
\defres{e2a_jevgym_tool_decisions/jev_ts_assist_k3_s2lite/vs_baseline/delta_ci/hi}{+0.6}
\defres{e2a_jevgym_tool_decisions/jev_ts_assist_k3_s2lite/vs_baseline/delta_ci/lo}{-7.2}
\defres{e2a_jevgym_tool_decisions/jev_ts_assist_k3_s2lite/vs_baseline/ni/p_decisive}{0.591}
\defres{e2a_jevgym_tool_decisions/jev_ts_assist_k5/cost_usd}{0.0222}
\defres{e2a_jevgym_tool_decisions/jev_ts_assist_k5/decisions/ece}{0.044}
\defres{e2a_jevgym_tool_decisions/jev_ts_assist_k5/llm_calls}{8.37}
\defres{e2a_jevgym_tool_decisions/jev_ts_assist_k5/steps}{8.37}
\defres{e2a_jevgym_tool_decisions/jev_ts_assist_k5/success}{90.0}
\defres{e2a_jevgym_tool_decisions/jev_ts_assist_k5/success_ci/hi}{94.0}
\defres{e2a_jevgym_tool_decisions/jev_ts_assist_k5/success_ci/lo}{85.5}
\defres{e2a_jevgym_tool_decisions/jev_ts_assist_k5/vs_baseline/cost_savings}{48.3}
\defres{e2a_jevgym_tool_decisions/jev_ts_assist_k5/vs_baseline/delta}{-10.0}
\defres{e2a_jevgym_tool_decisions/jev_ts_assist_k5/vs_baseline/delta_ci/hi}{-6.0}
\defres{e2a_jevgym_tool_decisions/jev_ts_assist_k5/vs_baseline/delta_ci/lo}{-14.5}
\defres{e2a_jevgym_tool_decisions/jev_ts_assist_k5/vs_baseline/ni/p_decisive}{1.000}
\defres{e2a_jevgym_tool_decisions/jev_ts_cascade_tau0.5/cost_usd}{0.00664}
\defres{e2a_jevgym_tool_decisions/jev_ts_cascade_tau0.5/decisions/ece}{0.025}
\defres{e2a_jevgym_tool_decisions/jev_ts_cascade_tau0.5/llm_calls}{2.31}
\defres{e2a_jevgym_tool_decisions/jev_ts_cascade_tau0.5/n_tasks}{200}
\defres{e2a_jevgym_tool_decisions/jev_ts_cascade_tau0.5/steps}{7.11}
\defres{e2a_jevgym_tool_decisions/jev_ts_cascade_tau0.5/success}{78.5}
\defres{e2a_jevgym_tool_decisions/jev_ts_cascade_tau0.5/success_ci/hi}{84.0}
\defres{e2a_jevgym_tool_decisions/jev_ts_cascade_tau0.5/success_ci/lo}{73.0}
\defres{e2a_jevgym_tool_decisions/jev_ts_cascade_tau0.5/vs_baseline/cost_savings}{84.5}
\defres{e2a_jevgym_tool_decisions/jev_ts_cascade_tau0.5/vs_baseline/delta}{-21.5}
\defres{e2a_jevgym_tool_decisions/jev_ts_cascade_tau0.5/vs_baseline/delta_ci/hi}{-16.0}
\defres{e2a_jevgym_tool_decisions/jev_ts_cascade_tau0.5/vs_baseline/delta_ci/lo}{-27.5}
\defres{e2a_jevgym_tool_decisions/jev_ts_cascade_tau0.5/vs_baseline/ni/p_decisive}{1.000}
\defres{e2a_jevgym_tool_decisions/jev_ts_cascade_tau0.7/cost_usd}{0.00818}
\defres{e2a_jevgym_tool_decisions/jev_ts_cascade_tau0.7/decisions/ece}{0.034}
\defres{e2a_jevgym_tool_decisions/jev_ts_cascade_tau0.7/llm_calls}{2.35}
\defres{e2a_jevgym_tool_decisions/jev_ts_cascade_tau0.7/n_tasks}{200}
\defres{e2a_jevgym_tool_decisions/jev_ts_cascade_tau0.7/steps}{6.89}
\defres{e2a_jevgym_tool_decisions/jev_ts_cascade_tau0.7/success}{76.0}
\defres{e2a_jevgym_tool_decisions/jev_ts_cascade_tau0.7/success_ci/hi}{81.5}
\defres{e2a_jevgym_tool_decisions/jev_ts_cascade_tau0.7/success_ci/lo}{70.0}
\defres{e2a_jevgym_tool_decisions/jev_ts_cascade_tau0.7/vs_baseline/cost_savings}{81.0}
\defres{e2a_jevgym_tool_decisions/jev_ts_cascade_tau0.7/vs_baseline/delta}{-24.0}
\defres{e2a_jevgym_tool_decisions/jev_ts_cascade_tau0.7/vs_baseline/delta_ci/hi}{-18.5}
\defres{e2a_jevgym_tool_decisions/jev_ts_cascade_tau0.7/vs_baseline/delta_ci/lo}{-30.5}
\defres{e2a_jevgym_tool_decisions/jev_ts_cascade_tau0.7/vs_baseline/ni/p_decisive}{1.000}
\defres{e2a_jevgym_tool_decisions/jev_ts_cascade_tau0.8/cost_usd}{0.0101}
\defres{e2a_jevgym_tool_decisions/jev_ts_cascade_tau0.8/decisions/ece}{0.033}
\defres{e2a_jevgym_tool_decisions/jev_ts_cascade_tau0.8/llm_calls}{2.61}
\defres{e2a_jevgym_tool_decisions/jev_ts_cascade_tau0.8/n_tasks}{200}
\defres{e2a_jevgym_tool_decisions/jev_ts_cascade_tau0.8/steps}{6.98}
\defres{e2a_jevgym_tool_decisions/jev_ts_cascade_tau0.8/success}{76.5}
\defres{e2a_jevgym_tool_decisions/jev_ts_cascade_tau0.8/success_ci/hi}{82.0}
\defres{e2a_jevgym_tool_decisions/jev_ts_cascade_tau0.8/success_ci/lo}{70.5}
\defres{e2a_jevgym_tool_decisions/jev_ts_cascade_tau0.8/vs_baseline/cost_savings}{76.5}
\defres{e2a_jevgym_tool_decisions/jev_ts_cascade_tau0.8/vs_baseline/delta}{-23.5}
\defres{e2a_jevgym_tool_decisions/jev_ts_cascade_tau0.8/vs_baseline/delta_ci/hi}{-18.0}
\defres{e2a_jevgym_tool_decisions/jev_ts_cascade_tau0.8/vs_baseline/delta_ci/lo}{-30.0}
\defres{e2a_jevgym_tool_decisions/jev_ts_cascade_tau0.8/vs_baseline/ni/p_decisive}{1.000}
\defres{e2a_jevgym_tool_decisions/jev_ts_cascade_tau0.9/cost_usd}{0.012}
\defres{e2a_jevgym_tool_decisions/jev_ts_cascade_tau0.9/decisions/ece}{0.027}
\defres{e2a_jevgym_tool_decisions/jev_ts_cascade_tau0.9/llm_calls}{2.67}
\defres{e2a_jevgym_tool_decisions/jev_ts_cascade_tau0.9/n_tasks}{200}
\defres{e2a_jevgym_tool_decisions/jev_ts_cascade_tau0.9/steps}{7.02}
\defres{e2a_jevgym_tool_decisions/jev_ts_cascade_tau0.9/success}{79.5}
\defres{e2a_jevgym_tool_decisions/jev_ts_cascade_tau0.9/success_ci/hi}{85.0}
\defres{e2a_jevgym_tool_decisions/jev_ts_cascade_tau0.9/success_ci/lo}{73.5}
\defres{e2a_jevgym_tool_decisions/jev_ts_cascade_tau0.9/vs_baseline/cost_savings}{72.0}
\defres{e2a_jevgym_tool_decisions/jev_ts_cascade_tau0.9/vs_baseline/delta}{-20.5}
\defres{e2a_jevgym_tool_decisions/jev_ts_cascade_tau0.9/vs_baseline/delta_ci/hi}{-15.0}
\defres{e2a_jevgym_tool_decisions/jev_ts_cascade_tau0.9/vs_baseline/delta_ci/lo}{-26.5}
\defres{e2a_jevgym_tool_decisions/jev_ts_cascade_tau0.9/vs_baseline/ni/p_decisive}{1.000}
\defres{e2a_jevgym_tool_decisions/jev_ts_cascade_tau0.95/cost_usd}{0.0143}
\defres{e2a_jevgym_tool_decisions/jev_ts_cascade_tau0.95/decisions/ece}{0.029}
\defres{e2a_jevgym_tool_decisions/jev_ts_cascade_tau0.95/llm_calls}{2.96}
\defres{e2a_jevgym_tool_decisions/jev_ts_cascade_tau0.95/n_tasks}{200}
\defres{e2a_jevgym_tool_decisions/jev_ts_cascade_tau0.95/steps}{7.09}
\defres{e2a_jevgym_tool_decisions/jev_ts_cascade_tau0.95/success}{79.5}
\defres{e2a_jevgym_tool_decisions/jev_ts_cascade_tau0.95/success_ci/hi}{85.0}
\defres{e2a_jevgym_tool_decisions/jev_ts_cascade_tau0.95/success_ci/lo}{74.0}
\defres{e2a_jevgym_tool_decisions/jev_ts_cascade_tau0.95/vs_baseline/cost_savings}{66.8}
\defres{e2a_jevgym_tool_decisions/jev_ts_cascade_tau0.95/vs_baseline/delta}{-20.5}
\defres{e2a_jevgym_tool_decisions/jev_ts_cascade_tau0.95/vs_baseline/delta_ci/hi}{-15.5}
\defres{e2a_jevgym_tool_decisions/jev_ts_cascade_tau0.95/vs_baseline/delta_ci/lo}{-26.5}
\defres{e2a_jevgym_tool_decisions/jev_ts_cascade_tau0.95/vs_baseline/ni/p_decisive}{1.000}
\defres{e2a_jevgym_tool_decisions/jev_ts_cascade_tau0.99/cost_usd}{0.0261}
\defres{e2a_jevgym_tool_decisions/jev_ts_cascade_tau0.99/decisions/ece}{0.045}
\defres{e2a_jevgym_tool_decisions/jev_ts_cascade_tau0.99/llm_calls}{4.89}
\defres{e2a_jevgym_tool_decisions/jev_ts_cascade_tau0.99/n_tasks}{200}
\defres{e2a_jevgym_tool_decisions/jev_ts_cascade_tau0.99/steps}{7.36}
\defres{e2a_jevgym_tool_decisions/jev_ts_cascade_tau0.99/success}{92.0}
\defres{e2a_jevgym_tool_decisions/jev_ts_cascade_tau0.99/success_ci/hi}{95.5}
\defres{e2a_jevgym_tool_decisions/jev_ts_cascade_tau0.99/success_ci/lo}{88.0}
\defres{e2a_jevgym_tool_decisions/jev_ts_cascade_tau0.99/vs_baseline/cost_savings}{39.3}
\defres{e2a_jevgym_tool_decisions/jev_ts_cascade_tau0.99/vs_baseline/delta}{-8.0}
\defres{e2a_jevgym_tool_decisions/jev_ts_cascade_tau0.99/vs_baseline/delta_ci/hi}{-4.5}
\defres{e2a_jevgym_tool_decisions/jev_ts_cascade_tau0.99/vs_baseline/delta_ci/lo}{-12.0}
\defres{e2a_jevgym_tool_decisions/jev_ts_cascade_tau0.99/vs_baseline/ni/p_decisive}{1.000}
\defres{e2a_jevgym_tool_decisions/jev_ts_cascade_tau0.9_s2lite/cost_usd}{0.00978}
\defres{e2a_jevgym_tool_decisions/jev_ts_cascade_tau0.9_s2lite/llm_calls}{7.57}
\defres{e2a_jevgym_tool_decisions/jev_ts_cascade_tau0.9_s2lite/steps}{7.57}
\defres{e2a_jevgym_tool_decisions/jev_ts_cascade_tau0.9_s2lite/success}{81.2}
\defres{e2a_jevgym_tool_decisions/jev_ts_cascade_tau0.9_s2lite/success_ci/hi}{84.6}
\defres{e2a_jevgym_tool_decisions/jev_ts_cascade_tau0.9_s2lite/success_ci/lo}{77.8}
\defres{e2a_jevgym_tool_decisions/jev_ts_cascade_tau0.9_s2lite/vs_baseline/cost_savings}{0.2}
\defres{e2a_jevgym_tool_decisions/jev_ts_cascade_tau0.9_s2lite/vs_baseline/delta}{+1.0}
\defres{e2a_jevgym_tool_decisions/jev_ts_cascade_tau0.9_s2lite/vs_baseline/delta_ci/hi}{+3.2}
\defres{e2a_jevgym_tool_decisions/jev_ts_cascade_tau0.9_s2lite/vs_baseline/delta_ci/lo}{-1.0}
\defres{e2a_jevgym_tool_decisions/jev_ts_cascade_tau0.9_s2lite/vs_baseline/ni/p_decisive}{$<$0.001}
\defres{e2a_jevgym_tool_decisions/jev_ts_cascade_tauhat/cost_usd}{0.0364}
\defres{e2a_jevgym_tool_decisions/jev_ts_cascade_tauhat/decisions/ece}{0.054}
\defres{e2a_jevgym_tool_decisions/jev_ts_cascade_tauhat/llm_calls}{6.42}
\defres{e2a_jevgym_tool_decisions/jev_ts_cascade_tauhat/n_tasks}{500}
\defres{e2a_jevgym_tool_decisions/jev_ts_cascade_tauhat/steps}{7.51}
\defres{e2a_jevgym_tool_decisions/jev_ts_cascade_tauhat/success}{99.8}
\defres{e2a_jevgym_tool_decisions/jev_ts_cascade_tauhat/success_ci/hi}{100.0}
\defres{e2a_jevgym_tool_decisions/jev_ts_cascade_tauhat/success_ci/lo}{99.4}
\defres{e2a_jevgym_tool_decisions/jev_ts_cascade_tauhat/vs_baseline/cost_savings}{14.2}
\defres{e2a_jevgym_tool_decisions/jev_ts_cascade_tauhat/vs_baseline/delta}{+0.0}
\defres{e2a_jevgym_tool_decisions/jev_ts_cascade_tauhat/vs_baseline/delta_ci/hi}{+0.0}
\defres{e2a_jevgym_tool_decisions/jev_ts_cascade_tauhat/vs_baseline/delta_ci/lo}{+0.0}
\defres{e2a_jevgym_tool_decisions/jev_ts_cascade_tauhat/vs_baseline/ni/p_decisive}{$<$0.001}
\defres{e2a_jevgym_tool_decisions/jev_ts_guard/cost_usd}{0.043}
\defres{e2a_jevgym_tool_decisions/jev_ts_guard/decisions/noul/ece}{0.129}
\defres{e2a_jevgym_tool_decisions/jev_ts_guard/llm_calls}{7.66}
\defres{e2a_jevgym_tool_decisions/jev_ts_guard/steps}{7.50}
\defres{e2a_jevgym_tool_decisions/jev_ts_guard/success}{100.0}
\defres{e2a_jevgym_tool_decisions/jev_ts_guard/success_ci/hi}{100.0}
\defres{e2a_jevgym_tool_decisions/jev_ts_guard/success_ci/lo}{100.0}
\defres{e2a_jevgym_tool_decisions/jev_ts_guard/vs_baseline/cost_savings}{-0.2}
\defres{e2a_jevgym_tool_decisions/jev_ts_guard/vs_baseline/delta}{+0.0}
\defres{e2a_jevgym_tool_decisions/jev_ts_guard/vs_baseline/delta_ci/hi}{+0.0}
\defres{e2a_jevgym_tool_decisions/jev_ts_guard/vs_baseline/delta_ci/lo}{+0.0}
\defres{e2a_jevgym_tool_decisions/jev_ts_guard/vs_baseline/ni/p_decisive}{0.002}
\defres{e2a_jevgym_tool_decisions/jev_ts_guard_s2lite/cost_usd}{0.0104}
\defres{e2a_jevgym_tool_decisions/jev_ts_guard_s2lite/decisions/noul/ece}{0.094}
\defres{e2a_jevgym_tool_decisions/jev_ts_guard_s2lite/llm_calls}{7.80}
\defres{e2a_jevgym_tool_decisions/jev_ts_guard_s2lite/steps}{7.57}
\defres{e2a_jevgym_tool_decisions/jev_ts_guard_s2lite/success}{86.5}
\defres{e2a_jevgym_tool_decisions/jev_ts_guard_s2lite/success_ci/hi}{91.0}
\defres{e2a_jevgym_tool_decisions/jev_ts_guard_s2lite/success_ci/lo}{81.5}
\defres{e2a_jevgym_tool_decisions/jev_ts_guard_s2lite/vs_baseline/cost_savings}{-6.7}
\defres{e2a_jevgym_tool_decisions/jev_ts_guard_s2lite/vs_baseline/delta}{+4.5}
\defres{e2a_jevgym_tool_decisions/jev_ts_guard_s2lite/vs_baseline/delta_ci/hi}{+9.0}
\defres{e2a_jevgym_tool_decisions/jev_ts_guard_s2lite/vs_baseline/delta_ci/lo}{+0.0}
\defres{e2a_jevgym_tool_decisions/jev_ts_guard_s2lite/vs_baseline/ni/p_decisive}{0.001}
\defres{e2a_jevgym_tool_decisions/jev_ts_params_replace/cost_usd}{0.00509}
\defres{e2a_jevgym_tool_decisions/jev_ts_params_replace/decisions/ece}{0.024}
\defres{e2a_jevgym_tool_decisions/jev_ts_params_replace/llm_calls}{1.80}
\defres{e2a_jevgym_tool_decisions/jev_ts_params_replace/steps}{7.58}
\defres{e2a_jevgym_tool_decisions/jev_ts_params_replace/success}{80.0}
\defres{e2a_jevgym_tool_decisions/jev_ts_params_replace/success_ci/hi}{85.5}
\defres{e2a_jevgym_tool_decisions/jev_ts_params_replace/success_ci/lo}{74.5}
\defres{e2a_jevgym_tool_decisions/jev_ts_params_replace/vs_baseline/cost_savings}{88.1}
\defres{e2a_jevgym_tool_decisions/jev_ts_params_replace/vs_baseline/delta}{-20.0}
\defres{e2a_jevgym_tool_decisions/jev_ts_params_replace/vs_baseline/delta_ci/hi}{-15.0}
\defres{e2a_jevgym_tool_decisions/jev_ts_params_replace/vs_baseline/delta_ci/lo}{-25.5}
\defres{e2a_jevgym_tool_decisions/jev_ts_params_replace/vs_baseline/ni/p_decisive}{1.000}
\defres{e2a_jevgym_tool_decisions/jev_ts_replace/cost_usd}{0.0142}
\defres{e2a_jevgym_tool_decisions/jev_ts_replace/decisions/ece}{0.030}
\defres{e2a_jevgym_tool_decisions/jev_ts_replace/llm_calls}{6.87}
\defres{e2a_jevgym_tool_decisions/jev_ts_replace/steps}{6.87}
\defres{e2a_jevgym_tool_decisions/jev_ts_replace/success}{81.0}
\defres{e2a_jevgym_tool_decisions/jev_ts_replace/success_ci/hi}{86.0}
\defres{e2a_jevgym_tool_decisions/jev_ts_replace/success_ci/lo}{75.5}
\defres{e2a_jevgym_tool_decisions/jev_ts_replace/vs_baseline/cost_savings}{67.0}
\defres{e2a_jevgym_tool_decisions/jev_ts_replace/vs_baseline/delta}{-19.0}
\defres{e2a_jevgym_tool_decisions/jev_ts_replace/vs_baseline/delta_ci/hi}{-13.5}
\defres{e2a_jevgym_tool_decisions/jev_ts_replace/vs_baseline/delta_ci/lo}{-24.5}
\defres{e2a_jevgym_tool_decisions/jev_ts_replace/vs_baseline/ni/p_decisive}{1.000}
\defres{e2a_jevgym_tool_decisions/lite_ts_assist_k3/cost_usd}{0.0367}
\defres{e2a_jevgym_tool_decisions/lite_ts_assist_k3/decisions/ece}{0.126}
\defres{e2a_jevgym_tool_decisions/lite_ts_assist_k3/llm_calls}{7.54}
\defres{e2a_jevgym_tool_decisions/lite_ts_assist_k3/steps}{7.54}
\defres{e2a_jevgym_tool_decisions/lite_ts_assist_k3/success}{87.5}
\defres{e2a_jevgym_tool_decisions/lite_ts_assist_k3/success_ci/hi}{92.0}
\defres{e2a_jevgym_tool_decisions/lite_ts_assist_k3/success_ci/lo}{83.0}
\defres{e2a_jevgym_tool_decisions/lite_ts_assist_k3/vs_baseline/cost_savings}{14.6}
\defres{e2a_jevgym_tool_decisions/lite_ts_assist_k3/vs_baseline/delta}{-12.5}
\defres{e2a_jevgym_tool_decisions/lite_ts_assist_k3/vs_baseline/delta_ci/hi}{-8.0}
\defres{e2a_jevgym_tool_decisions/lite_ts_assist_k3/vs_baseline/delta_ci/lo}{-17.0}
\defres{e2a_jevgym_tool_decisions/lite_ts_assist_k3/vs_baseline/ni/p_decisive}{1.000}
\defres{e2a_jevgym_tool_decisions/lite_ts_cascade_tau0.7/cost_usd}{0.0267}
\defres{e2a_jevgym_tool_decisions/lite_ts_cascade_tau0.7/decisions/ece}{0.110}
\defres{e2a_jevgym_tool_decisions/lite_ts_cascade_tau0.7/llm_calls}{1.45}
\defres{e2a_jevgym_tool_decisions/lite_ts_cascade_tau0.7/steps}{6.18}
\defres{e2a_jevgym_tool_decisions/lite_ts_cascade_tau0.7/success}{42.5}
\defres{e2a_jevgym_tool_decisions/lite_ts_cascade_tau0.7/success_ci/hi}{49.0}
\defres{e2a_jevgym_tool_decisions/lite_ts_cascade_tau0.7/success_ci/lo}{36.0}
\defres{e2a_jevgym_tool_decisions/lite_ts_cascade_tau0.7/vs_baseline/cost_savings}{37.9}
\defres{e2a_jevgym_tool_decisions/lite_ts_cascade_tau0.7/vs_baseline/delta}{-57.5}
\defres{e2a_jevgym_tool_decisions/lite_ts_cascade_tau0.7/vs_baseline/delta_ci/hi}{-51.0}
\defres{e2a_jevgym_tool_decisions/lite_ts_cascade_tau0.7/vs_baseline/delta_ci/lo}{-64.5}
\defres{e2a_jevgym_tool_decisions/lite_ts_cascade_tau0.7/vs_baseline/ni/p_decisive}{1.000}
\defres{e2a_jevgym_tool_decisions/lite_ts_cascade_tau0.9/cost_usd}{0.0263}
\defres{e2a_jevgym_tool_decisions/lite_ts_cascade_tau0.9/decisions/ece}{0.095}
\defres{e2a_jevgym_tool_decisions/lite_ts_cascade_tau0.9/llm_calls}{1.42}
\defres{e2a_jevgym_tool_decisions/lite_ts_cascade_tau0.9/steps}{6.01}
\defres{e2a_jevgym_tool_decisions/lite_ts_cascade_tau0.9/success}{43.5}
\defres{e2a_jevgym_tool_decisions/lite_ts_cascade_tau0.9/success_ci/hi}{50.5}
\defres{e2a_jevgym_tool_decisions/lite_ts_cascade_tau0.9/success_ci/lo}{37.0}
\defres{e2a_jevgym_tool_decisions/lite_ts_cascade_tau0.9/vs_baseline/cost_savings}{38.8}
\defres{e2a_jevgym_tool_decisions/lite_ts_cascade_tau0.9/vs_baseline/delta}{-56.5}
\defres{e2a_jevgym_tool_decisions/lite_ts_cascade_tau0.9/vs_baseline/delta_ci/hi}{-50.0}
\defres{e2a_jevgym_tool_decisions/lite_ts_cascade_tau0.9/vs_baseline/delta_ci/lo}{-63.5}
\defres{e2a_jevgym_tool_decisions/lite_ts_cascade_tau0.9/vs_baseline/ni/p_decisive}{1.000}
\defres{e2a_jevgym_tool_decisions/lite_ts_cascade_tau0.99/cost_usd}{0.0432}
\defres{e2a_jevgym_tool_decisions/lite_ts_cascade_tau0.99/decisions/ece}{0.113}
\defres{e2a_jevgym_tool_decisions/lite_ts_cascade_tau0.99/llm_calls}{4.31}
\defres{e2a_jevgym_tool_decisions/lite_ts_cascade_tau0.99/steps}{6.96}
\defres{e2a_jevgym_tool_decisions/lite_ts_cascade_tau0.99/success}{75.0}
\defres{e2a_jevgym_tool_decisions/lite_ts_cascade_tau0.99/success_ci/hi}{81.0}
\defres{e2a_jevgym_tool_decisions/lite_ts_cascade_tau0.99/success_ci/lo}{69.0}
\defres{e2a_jevgym_tool_decisions/lite_ts_cascade_tau0.99/vs_baseline/cost_savings}{-0.7}
\defres{e2a_jevgym_tool_decisions/lite_ts_cascade_tau0.99/vs_baseline/delta}{-25.0}
\defres{e2a_jevgym_tool_decisions/lite_ts_cascade_tau0.99/vs_baseline/delta_ci/hi}{-19.0}
\defres{e2a_jevgym_tool_decisions/lite_ts_cascade_tau0.99/vs_baseline/delta_ci/lo}{-31.0}
\defres{e2a_jevgym_tool_decisions/lite_ts_cascade_tau0.99/vs_baseline/ni/p_decisive}{1.000}
\defres{e2a_jevgym_tool_decisions/lite_ts_guard/cost_usd}{0.0536}
\defres{e2a_jevgym_tool_decisions/lite_ts_guard/decisions/noul/ece}{0.105}
\defres{e2a_jevgym_tool_decisions/lite_ts_guard/llm_calls}{8.90}
\defres{e2a_jevgym_tool_decisions/lite_ts_guard/steps}{8.02}
\defres{e2a_jevgym_tool_decisions/lite_ts_guard/success}{100.0}
\defres{e2a_jevgym_tool_decisions/lite_ts_guard/success_ci/hi}{100.0}
\defres{e2a_jevgym_tool_decisions/lite_ts_guard/success_ci/lo}{100.0}
\defres{e2a_jevgym_tool_decisions/lite_ts_guard/vs_baseline/cost_savings}{-24.9}
\defres{e2a_jevgym_tool_decisions/lite_ts_guard/vs_baseline/delta}{+0.0}
\defres{e2a_jevgym_tool_decisions/lite_ts_guard/vs_baseline/delta_ci/hi}{+0.0}
\defres{e2a_jevgym_tool_decisions/lite_ts_guard/vs_baseline/delta_ci/lo}{+0.0}
\defres{e2a_jevgym_tool_decisions/lite_ts_guard/vs_baseline/ni/p_decisive}{0.002}
\defres{e2a_jevgym_tool_decisions/lite_ts_params_replace/cost_usd}{0.0271}
\defres{e2a_jevgym_tool_decisions/lite_ts_params_replace/decisions/ece}{0.127}
\defres{e2a_jevgym_tool_decisions/lite_ts_params_replace/llm_calls}{1.46}
\defres{e2a_jevgym_tool_decisions/lite_ts_params_replace/steps}{6.37}
\defres{e2a_jevgym_tool_decisions/lite_ts_params_replace/success}{39.5}
\defres{e2a_jevgym_tool_decisions/lite_ts_params_replace/success_ci/hi}{46.5}
\defres{e2a_jevgym_tool_decisions/lite_ts_params_replace/success_ci/lo}{33.0}
\defres{e2a_jevgym_tool_decisions/lite_ts_params_replace/vs_baseline/cost_savings}{36.9}
\defres{e2a_jevgym_tool_decisions/lite_ts_params_replace/vs_baseline/delta}{-60.5}
\defres{e2a_jevgym_tool_decisions/lite_ts_params_replace/vs_baseline/delta_ci/hi}{-54.0}
\defres{e2a_jevgym_tool_decisions/lite_ts_params_replace/vs_baseline/delta_ci/lo}{-67.5}
\defres{e2a_jevgym_tool_decisions/lite_ts_params_replace/vs_baseline/ni/p_decisive}{1.000}
\defres{e2a_jevgym_tool_decisions/llm_only/cost_usd}{0.0424}
\defres{e2a_jevgym_tool_decisions/llm_only/llm_calls}{7.51}
\defres{e2a_jevgym_tool_decisions/llm_only/n_tasks}{500}
\defres{e2a_jevgym_tool_decisions/llm_only/steps}{7.51}
\defres{e2a_jevgym_tool_decisions/llm_only/success}{99.8}
\defres{e2a_jevgym_tool_decisions/llm_only/success_ci/hi}{100.0}
\defres{e2a_jevgym_tool_decisions/llm_only/success_ci/lo}{99.4}
\defres{e2a_jevgym_tool_decisions/llm_only_s2lite/cost_usd}{0.0098}
\defres{e2a_jevgym_tool_decisions/llm_only_s2lite/llm_calls}{7.58}
\defres{e2a_jevgym_tool_decisions/llm_only_s2lite/steps}{7.58}
\defres{e2a_jevgym_tool_decisions/llm_only_s2lite/success}{80.2}
\defres{e2a_jevgym_tool_decisions/llm_only_s2lite/success_ci/hi}{83.8}
\defres{e2a_jevgym_tool_decisions/llm_only_s2lite/success_ci/lo}{76.6}
\defres{e2a_jevgym_tool_decisions/llm_only_s2lite/vs_baseline/cost_savings}{76.9}
\defres{e2a_jevgym_tool_decisions/llm_only_s2lite/vs_baseline/delta}{-19.6}
\defres{e2a_jevgym_tool_decisions/llm_only_s2lite/vs_baseline/delta_ci/hi}{-16.0}
\defres{e2a_jevgym_tool_decisions/llm_only_s2lite/vs_baseline/delta_ci/lo}{-23.2}
\defres{e2a_jevgym_tool_decisions/llm_only_s2lite/vs_baseline/ni/p_decisive}{1.000}
\defres{e2a_jevgym_tool_decisions_intern/headline/iso_cost/delta_ci/hi}{+0.0}
\defres{e2a_jevgym_tool_decisions_intern/headline/iso_cost/delta_ci/lo}{+0.0}
\defres{e2a_jevgym_tool_decisions_intern/headline/iso_cost/success}{100.0}
\defres{e2a_jevgym_tool_decisions_intern/headline/iso_cost_by_reference/llm_only_s2lite/success}{83.4}
\defres{e2a_jevgym_tool_decisions_intern/headline/iso_quality/cost_savings_ci/hi}{6.3}
\defres{e2a_jevgym_tool_decisions_intern/headline/iso_quality/cost_savings_ci/lo}{4.3}
\defres{e2a_jevgym_tool_decisions_intern/headline/iso_quality/delta_ci/hi}{+0.0}
\defres{e2a_jevgym_tool_decisions_intern/headline/iso_quality/delta_ci/lo}{+0.0}
\defres{e2a_jevgym_tool_decisions_intern/headline/iso_quality_by_reference/llm_only_s2lite/cost_savings_ci/hi}{1.4}
\defres{e2a_jevgym_tool_decisions_intern/headline/iso_quality_by_reference/llm_only_s2lite/cost_savings_ci/lo}{0.5}
\defres{e2a_jevgym_tool_decisions_intern/headline/iso_quality_by_reference/llm_only_s2lite/delta_ci/hi}{+1.6}
\defres{e2a_jevgym_tool_decisions_intern/headline/iso_quality_by_reference/llm_only_s2lite/delta_ci/lo}{-2.8}
\defres{e2a_jevgym_tool_decisions_intern/intern08_ts_assist_k3/cost_usd}{0.0311}
\defres{e2a_jevgym_tool_decisions_intern/intern08_ts_assist_k3/decisions/ece}{0.326}
\defres{e2a_jevgym_tool_decisions_intern/intern08_ts_assist_k3/llm_calls}{11.19}
\defres{e2a_jevgym_tool_decisions_intern/intern08_ts_assist_k3/steps}{11.19}
\defres{e2a_jevgym_tool_decisions_intern/intern08_ts_assist_k3/success}{17.0}
\defres{e2a_jevgym_tool_decisions_intern/intern08_ts_assist_k3/success_ci/hi}{22.5}
\defres{e2a_jevgym_tool_decisions_intern/intern08_ts_assist_k3/success_ci/lo}{12.0}
\defres{e2a_jevgym_tool_decisions_intern/intern08_ts_assist_k3/vs_baseline/cost_savings}{28.5}
\defres{e2a_jevgym_tool_decisions_intern/intern08_ts_assist_k3/vs_baseline/delta}{-83.0}
\defres{e2a_jevgym_tool_decisions_intern/intern08_ts_assist_k3/vs_baseline/delta_ci/hi}{-77.5}
\defres{e2a_jevgym_tool_decisions_intern/intern08_ts_assist_k3/vs_baseline/delta_ci/lo}{-88.0}
\defres{e2a_jevgym_tool_decisions_intern/intern08_ts_assist_k3/vs_baseline/ni/p_decisive}{1.000}
\defres{e2a_jevgym_tool_decisions_intern/intern08_ts_replace/cost_usd}{0.0402}
\defres{e2a_jevgym_tool_decisions_intern/intern08_ts_replace/decisions/ece}{0.496}
\defres{e2a_jevgym_tool_decisions_intern/intern08_ts_replace/llm_calls}{14.37}
\defres{e2a_jevgym_tool_decisions_intern/intern08_ts_replace/steps}{14.37}
\defres{e2a_jevgym_tool_decisions_intern/intern08_ts_replace/success}{3.5}
\defres{e2a_jevgym_tool_decisions_intern/intern08_ts_replace/success_ci/hi}{6.0}
\defres{e2a_jevgym_tool_decisions_intern/intern08_ts_replace/success_ci/lo}{1.5}
\defres{e2a_jevgym_tool_decisions_intern/intern08_ts_replace/vs_baseline/cost_savings}{7.6}
\defres{e2a_jevgym_tool_decisions_intern/intern08_ts_replace/vs_baseline/delta}{-96.5}
\defres{e2a_jevgym_tool_decisions_intern/intern08_ts_replace/vs_baseline/delta_ci/hi}{-94.0}
\defres{e2a_jevgym_tool_decisions_intern/intern08_ts_replace/vs_baseline/delta_ci/lo}{-99.0}
\defres{e2a_jevgym_tool_decisions_intern/intern08_ts_replace/vs_baseline/ni/p_decisive}{1.000}
\defres{e2a_jevgym_tool_decisions_intern/intern2b_ts_assist_k3/cost_usd}{0.0278}
\defres{e2a_jevgym_tool_decisions_intern/intern2b_ts_assist_k3/decisions/ece}{0.395}
\defres{e2a_jevgym_tool_decisions_intern/intern2b_ts_assist_k3/llm_calls}{10.99}
\defres{e2a_jevgym_tool_decisions_intern/intern2b_ts_assist_k3/steps}{10.99}
\defres{e2a_jevgym_tool_decisions_intern/intern2b_ts_assist_k3/success}{25.5}
\defres{e2a_jevgym_tool_decisions_intern/intern2b_ts_assist_k3/success_ci/hi}{31.5}
\defres{e2a_jevgym_tool_decisions_intern/intern2b_ts_assist_k3/success_ci/lo}{19.5}
\defres{e2a_jevgym_tool_decisions_intern/intern2b_ts_assist_k3/vs_baseline/cost_savings}{36.1}
\defres{e2a_jevgym_tool_decisions_intern/intern2b_ts_assist_k3/vs_baseline/delta}{-74.5}
\defres{e2a_jevgym_tool_decisions_intern/intern2b_ts_assist_k3/vs_baseline/delta_ci/hi}{-68.5}
\defres{e2a_jevgym_tool_decisions_intern/intern2b_ts_assist_k3/vs_baseline/delta_ci/lo}{-80.0}
\defres{e2a_jevgym_tool_decisions_intern/intern2b_ts_assist_k3/vs_baseline/ni/p_decisive}{1.000}
\defres{e2a_jevgym_tool_decisions_intern/intern2b_ts_replace/cost_usd}{0.0246}
\defres{e2a_jevgym_tool_decisions_intern/intern2b_ts_replace/decisions/ece}{0.464}
\defres{e2a_jevgym_tool_decisions_intern/intern2b_ts_replace/llm_calls}{9.19}
\defres{e2a_jevgym_tool_decisions_intern/intern2b_ts_replace/steps}{9.19}
\defres{e2a_jevgym_tool_decisions_intern/intern2b_ts_replace/success}{3.0}
\defres{e2a_jevgym_tool_decisions_intern/intern2b_ts_replace/success_ci/hi}{5.5}
\defres{e2a_jevgym_tool_decisions_intern/intern2b_ts_replace/success_ci/lo}{1.0}
\defres{e2a_jevgym_tool_decisions_intern/intern2b_ts_replace/vs_baseline/cost_savings}{43.6}
\defres{e2a_jevgym_tool_decisions_intern/intern2b_ts_replace/vs_baseline/delta}{-97.0}
\defres{e2a_jevgym_tool_decisions_intern/intern2b_ts_replace/vs_baseline/delta_ci/hi}{-94.5}
\defres{e2a_jevgym_tool_decisions_intern/intern2b_ts_replace/vs_baseline/delta_ci/lo}{-99.0}
\defres{e2a_jevgym_tool_decisions_intern/intern2b_ts_replace/vs_baseline/ni/p_decisive}{1.000}
\defres{e2a_jevgym_tool_decisions_intern/intern4b_uncal_ts_guard/cost_usd}{0.0446}
\defres{e2a_jevgym_tool_decisions_intern/intern4b_uncal_ts_guard/decisions/noul/ece}{0.060}
\defres{e2a_jevgym_tool_decisions_intern/intern4b_uncal_ts_guard/llm_calls}{7.96}
\defres{e2a_jevgym_tool_decisions_intern/intern4b_uncal_ts_guard/steps}{7.63}
\defres{e2a_jevgym_tool_decisions_intern/intern4b_uncal_ts_guard/success}{100.0}
\defres{e2a_jevgym_tool_decisions_intern/intern4b_uncal_ts_guard/success_ci/hi}{100.0}
\defres{e2a_jevgym_tool_decisions_intern/intern4b_uncal_ts_guard/success_ci/lo}{100.0}
\defres{e2a_jevgym_tool_decisions_intern/intern4b_uncal_ts_guard/vs_baseline/cost_savings}{-2.4}
\defres{e2a_jevgym_tool_decisions_intern/intern4b_uncal_ts_guard/vs_baseline/delta}{+0.0}
\defres{e2a_jevgym_tool_decisions_intern/intern4b_uncal_ts_guard/vs_baseline/delta_ci/hi}{+0.0}
\defres{e2a_jevgym_tool_decisions_intern/intern4b_uncal_ts_guard/vs_baseline/delta_ci/lo}{+0.0}
\defres{e2a_jevgym_tool_decisions_intern/intern4b_uncal_ts_guard/vs_baseline/ni/p_decisive}{0.002}
\defres{e2a_jevgym_tool_decisions_intern/intern_shadow/cost_usd}{0.0425}
\defres{e2a_jevgym_tool_decisions_intern/intern_shadow/decisions/ece}{0.054}
\defres{e2a_jevgym_tool_decisions_intern/intern_shadow/decisions/gold/gates/stop_guard-shadow/ece}{0.215}
\defres{e2a_jevgym_tool_decisions_intern/intern_shadow/decisions/gold/gates/stop_trigger-shadow/ece}{0.239}
\defres{e2a_jevgym_tool_decisions_intern/intern_shadow/decisions/noul/ece}{0.202}
\defres{e2a_jevgym_tool_decisions_intern/intern_shadow/llm_calls}{7.51}
\defres{e2a_jevgym_tool_decisions_intern/intern_shadow/steps}{7.51}
\defres{e2a_jevgym_tool_decisions_intern/intern_shadow/success}{99.8}
\defres{e2a_jevgym_tool_decisions_intern/intern_shadow/success_ci/hi}{100.0}
\defres{e2a_jevgym_tool_decisions_intern/intern_shadow/success_ci/lo}{99.4}
\defres{e2a_jevgym_tool_decisions_intern/intern_shadow/vs_baseline/cost_savings}{2.6}
\defres{e2a_jevgym_tool_decisions_intern/intern_shadow/vs_baseline/delta}{+0.2}
\defres{e2a_jevgym_tool_decisions_intern/intern_shadow/vs_baseline/delta_ci/hi}{+0.8}
\defres{e2a_jevgym_tool_decisions_intern/intern_shadow/vs_baseline/delta_ci/lo}{+0.0}
\defres{e2a_jevgym_tool_decisions_intern/intern_shadow/vs_baseline/ni/p_decisive}{$<$0.001}
\defres{e2a_jevgym_tool_decisions_intern/intern_shadow_s2lite/cost_usd}{0.00981}
\defres{e2a_jevgym_tool_decisions_intern/intern_shadow_s2lite/decisions/ece}{0.100}
\defres{e2a_jevgym_tool_decisions_intern/intern_shadow_s2lite/decisions/gold/gates/stop_guard-shadow/ece}{0.130}
\defres{e2a_jevgym_tool_decisions_intern/intern_shadow_s2lite/decisions/gold/gates/stop_trigger-shadow/ece}{0.241}
\defres{e2a_jevgym_tool_decisions_intern/intern_shadow_s2lite/decisions/noul/ece}{0.208}
\defres{e2a_jevgym_tool_decisions_intern/intern_shadow_s2lite/llm_calls}{7.57}
\defres{e2a_jevgym_tool_decisions_intern/intern_shadow_s2lite/steps}{7.57}
\defres{e2a_jevgym_tool_decisions_intern/intern_shadow_s2lite/success}{81.6}
\defres{e2a_jevgym_tool_decisions_intern/intern_shadow_s2lite/success_ci/hi}{85.0}
\defres{e2a_jevgym_tool_decisions_intern/intern_shadow_s2lite/success_ci/lo}{78.2}
\defres{e2a_jevgym_tool_decisions_intern/intern_shadow_s2lite/vs_baseline/cost_savings}{0.7}
\defres{e2a_jevgym_tool_decisions_intern/intern_shadow_s2lite/vs_baseline/delta}{-1.8}
\defres{e2a_jevgym_tool_decisions_intern/intern_shadow_s2lite/vs_baseline/delta_ci/hi}{+0.4}
\defres{e2a_jevgym_tool_decisions_intern/intern_shadow_s2lite/vs_baseline/delta_ci/lo}{-3.8}
\defres{e2a_jevgym_tool_decisions_intern/intern_shadow_s2lite/vs_baseline/ni/p_decisive}{0.153}
\defres{e2a_jevgym_tool_decisions_intern/intern_stop_guard/cost_usd}{0.0449}
\defres{e2a_jevgym_tool_decisions_intern/intern_stop_guard/decisions/noul/ece}{0.343}
\defres{e2a_jevgym_tool_decisions_intern/intern_stop_guard/llm_calls}{7.91}
\defres{e2a_jevgym_tool_decisions_intern/intern_stop_guard/steps}{7.91}
\defres{e2a_jevgym_tool_decisions_intern/intern_stop_guard/success}{99.2}
\defres{e2a_jevgym_tool_decisions_intern/intern_stop_guard/success_ci/hi}{99.8}
\defres{e2a_jevgym_tool_decisions_intern/intern_stop_guard/success_ci/lo}{98.4}
\defres{e2a_jevgym_tool_decisions_intern/intern_stop_guard/vs_baseline/cost_savings}{-3.0}
\defres{e2a_jevgym_tool_decisions_intern/intern_stop_guard/vs_baseline/delta}{-0.4}
\defres{e2a_jevgym_tool_decisions_intern/intern_stop_guard/vs_baseline/delta_ci/hi}{+0.0}
\defres{e2a_jevgym_tool_decisions_intern/intern_stop_guard/vs_baseline/delta_ci/lo}{-1.0}
\defres{e2a_jevgym_tool_decisions_intern/intern_stop_guard/vs_baseline/ni/p_decisive}{$<$0.001}
\defres{e2a_jevgym_tool_decisions_intern/intern_stop_guard_s2lite/cost_usd}{0.0144}
\defres{e2a_jevgym_tool_decisions_intern/intern_stop_guard_s2lite/decisions/noul/ece}{0.259}
\defres{e2a_jevgym_tool_decisions_intern/intern_stop_guard_s2lite/llm_calls}{11.07}
\defres{e2a_jevgym_tool_decisions_intern/intern_stop_guard_s2lite/steps}{11.07}
\defres{e2a_jevgym_tool_decisions_intern/intern_stop_guard_s2lite/success}{77.4}
\defres{e2a_jevgym_tool_decisions_intern/intern_stop_guard_s2lite/success_ci/hi}{81.0}
\defres{e2a_jevgym_tool_decisions_intern/intern_stop_guard_s2lite/success_ci/lo}{73.6}
\defres{e2a_jevgym_tool_decisions_intern/intern_stop_guard_s2lite/vs_baseline/cost_savings}{-45.3}
\defres{e2a_jevgym_tool_decisions_intern/intern_stop_guard_s2lite/vs_baseline/delta}{-6.0}
\defres{e2a_jevgym_tool_decisions_intern/intern_stop_guard_s2lite/vs_baseline/delta_ci/hi}{-3.0}
\defres{e2a_jevgym_tool_decisions_intern/intern_stop_guard_s2lite/vs_baseline/delta_ci/lo}{-9.2}
\defres{e2a_jevgym_tool_decisions_intern/intern_stop_guard_s2lite/vs_baseline/ni/p_decisive}{0.975}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_assist_k3/cost_usd}{0.0205}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_assist_k3/decisions/ece}{0.031}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_assist_k3/llm_calls}{8.56}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_assist_k3/steps}{8.56}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_assist_k3/success}{96.0}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_assist_k3/success_ci/hi}{97.6}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_assist_k3/success_ci/lo}{94.0}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_assist_k3/vs_baseline/cost_savings}{53.0}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_assist_k3/vs_baseline/delta}{-3.6}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_assist_k3/vs_baseline/delta_ci/hi}{-2.0}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_assist_k3/vs_baseline/delta_ci/lo}{-5.4}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_assist_k3/vs_baseline/ni/p_decisive}{0.767}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_assist_k3_s2lite/cost_usd}{0.00458}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_assist_k3_s2lite/decisions/ece}{0.066}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_assist_k3_s2lite/llm_calls}{8.60}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_assist_k3_s2lite/steps}{8.60}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_assist_k3_s2lite/success}{68.6}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_assist_k3_s2lite/success_ci/hi}{72.6}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_assist_k3_s2lite/success_ci/lo}{64.2}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_assist_k3_s2lite/vs_baseline/cost_savings}{53.7}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_assist_k3_s2lite/vs_baseline/delta}{-14.8}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_assist_k3_s2lite/vs_baseline/delta_ci/hi}{-10.8}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_assist_k3_s2lite/vs_baseline/delta_ci/lo}{-19.2}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_assist_k3_s2lite/vs_baseline/ni/p_decisive}{1.000}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_assist_k5/cost_usd}{0.0205}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_assist_k5/decisions/ece}{0.051}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_assist_k5/llm_calls}{8.06}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_assist_k5/steps}{8.06}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_assist_k5/success}{97.5}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_assist_k5/success_ci/hi}{99.5}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_assist_k5/success_ci/lo}{95.0}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_assist_k5/vs_baseline/cost_savings}{53.0}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_assist_k5/vs_baseline/delta}{-2.5}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_assist_k5/vs_baseline/delta_ci/hi}{-0.5}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_assist_k5/vs_baseline/delta_ci/lo}{-5.0}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_assist_k5/vs_baseline/ni/p_decisive}{0.459}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_cascade_tau0.5/cost_usd}{0.00836}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_cascade_tau0.5/decisions/ece}{0.088}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_cascade_tau0.5/llm_calls}{4.30}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_cascade_tau0.5/steps}{4.53}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_cascade_tau0.5/success}{28.5}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_cascade_tau0.5/success_ci/hi}{34.5}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_cascade_tau0.5/success_ci/lo}{22.5}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_cascade_tau0.5/vs_baseline/cost_savings}{80.8}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_cascade_tau0.5/vs_baseline/delta}{-71.5}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_cascade_tau0.5/vs_baseline/delta_ci/hi}{-65.0}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_cascade_tau0.5/vs_baseline/delta_ci/lo}{-77.5}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_cascade_tau0.5/vs_baseline/ni/p_decisive}{1.000}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_cascade_tau0.7/cost_usd}{0.0161}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_cascade_tau0.7/decisions/ece}{0.087}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_cascade_tau0.7/llm_calls}{4.79}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_cascade_tau0.7/steps}{4.97}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_cascade_tau0.7/success}{36.0}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_cascade_tau0.7/success_ci/hi}{42.5}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_cascade_tau0.7/success_ci/lo}{29.5}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_cascade_tau0.7/vs_baseline/cost_savings}{63.0}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_cascade_tau0.7/vs_baseline/delta}{-64.0}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_cascade_tau0.7/vs_baseline/delta_ci/hi}{-57.5}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_cascade_tau0.7/vs_baseline/delta_ci/lo}{-70.5}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_cascade_tau0.7/vs_baseline/ni/p_decisive}{1.000}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_cascade_tau0.8/cost_usd}{0.0216}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_cascade_tau0.8/decisions/ece}{0.079}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_cascade_tau0.8/llm_calls}{5.46}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_cascade_tau0.8/steps}{5.62}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_cascade_tau0.8/success}{49.5}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_cascade_tau0.8/success_ci/hi}{56.5}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_cascade_tau0.8/success_ci/lo}{42.5}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_cascade_tau0.8/vs_baseline/cost_savings}{50.4}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_cascade_tau0.8/vs_baseline/delta}{-50.5}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_cascade_tau0.8/vs_baseline/delta_ci/hi}{-43.5}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_cascade_tau0.8/vs_baseline/delta_ci/lo}{-57.0}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_cascade_tau0.8/vs_baseline/ni/p_decisive}{1.000}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_cascade_tau0.9/cost_usd}{0.0281}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_cascade_tau0.9/decisions/ece}{0.069}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_cascade_tau0.9/llm_calls}{6.36}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_cascade_tau0.9/steps}{6.46}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_cascade_tau0.9/success}{68.0}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_cascade_tau0.9/success_ci/hi}{74.5}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_cascade_tau0.9/success_ci/lo}{61.5}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_cascade_tau0.9/vs_baseline/cost_savings}{35.4}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_cascade_tau0.9/vs_baseline/delta}{-32.0}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_cascade_tau0.9/vs_baseline/delta_ci/hi}{-25.5}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_cascade_tau0.9/vs_baseline/delta_ci/lo}{-38.5}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_cascade_tau0.9/vs_baseline/ni/p_decisive}{1.000}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_cascade_tau0.95/cost_usd}{0.0352}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_cascade_tau0.95/decisions/ece}{0.041}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_cascade_tau0.95/llm_calls}{6.96}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_cascade_tau0.95/steps}{7.06}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_cascade_tau0.95/success}{86.0}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_cascade_tau0.95/success_ci/hi}{91.0}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_cascade_tau0.95/success_ci/lo}{81.0}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_cascade_tau0.95/vs_baseline/cost_savings}{19.2}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_cascade_tau0.95/vs_baseline/delta}{-14.0}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_cascade_tau0.95/vs_baseline/delta_ci/hi}{-9.5}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_cascade_tau0.95/vs_baseline/delta_ci/lo}{-19.0}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_cascade_tau0.95/vs_baseline/ni/p_decisive}{1.000}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_cascade_tau0.99/cost_usd}{0.0412}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_cascade_tau0.99/decisions/ece}{0.053}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_cascade_tau0.99/llm_calls}{7.50}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_cascade_tau0.99/steps}{7.50}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_cascade_tau0.99/success}{100.0}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_cascade_tau0.99/success_ci/hi}{100.0}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_cascade_tau0.99/success_ci/lo}{100.0}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_cascade_tau0.99/vs_baseline/cost_savings}{5.3}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_cascade_tau0.99/vs_baseline/delta}{+0.0}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_cascade_tau0.99/vs_baseline/delta_ci/hi}{+0.0}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_cascade_tau0.99/vs_baseline/delta_ci/lo}{+0.0}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_cascade_tau0.99/vs_baseline/ni/p_decisive}{0.002}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_cascade_tau0.9_s2lite/cost_usd}{0.00978}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_cascade_tau0.9_s2lite/llm_calls}{7.57}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_cascade_tau0.9_s2lite/steps}{7.57}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_cascade_tau0.9_s2lite/success}{82.8}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_cascade_tau0.9_s2lite/success_ci/hi}{86.2}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_cascade_tau0.9_s2lite/success_ci/lo}{79.4}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_cascade_tau0.9_s2lite/vs_baseline/cost_savings}{1.0}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_cascade_tau0.9_s2lite/vs_baseline/delta}{-0.6}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_cascade_tau0.9_s2lite/vs_baseline/delta_ci/hi}{+1.6}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_cascade_tau0.9_s2lite/vs_baseline/delta_ci/lo}{-2.8}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_cascade_tau0.9_s2lite/vs_baseline/ni/p_decisive}{0.024}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_cascade_tauhat/cost_usd}{0.0437}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_cascade_tauhat/llm_calls}{7.52}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_cascade_tauhat/steps}{7.52}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_cascade_tauhat/success}{99.8}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_cascade_tauhat/success_ci/hi}{100.0}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_cascade_tauhat/success_ci/lo}{99.4}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_cascade_tauhat/vs_baseline/cost_savings}{-0.2}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_cascade_tauhat/vs_baseline/delta}{+0.2}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_cascade_tauhat/vs_baseline/delta_ci/hi}{+0.8}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_cascade_tauhat/vs_baseline/delta_ci/lo}{+0.0}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_cascade_tauhat/vs_baseline/ni/p_decisive}{$<$0.001}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_guard/cost_usd}{0.0432}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_guard/decisions/noul/ece}{0.138}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_guard/llm_calls}{8.02}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_guard/steps}{7.66}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_guard/success}{100.0}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_guard/success_ci/hi}{100.0}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_guard/success_ci/lo}{100.0}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_guard/vs_baseline/cost_savings}{0.7}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_guard/vs_baseline/delta}{+0.0}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_guard/vs_baseline/delta_ci/hi}{+0.0}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_guard/vs_baseline/delta_ci/lo}{+0.0}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_guard/vs_baseline/ni/p_decisive}{0.002}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_guard_s2lite/cost_usd}{0.0103}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_guard_s2lite/decisions/noul/ece}{0.101}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_guard_s2lite/llm_calls}{7.89}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_guard_s2lite/steps}{7.55}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_guard_s2lite/success}{84.5}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_guard_s2lite/success_ci/hi}{89.0}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_guard_s2lite/success_ci/lo}{79.5}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_guard_s2lite/vs_baseline/cost_savings}{-4.4}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_guard_s2lite/vs_baseline/delta}{-0.5}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_guard_s2lite/vs_baseline/delta_ci/hi}{+3.5}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_guard_s2lite/vs_baseline/delta_ci/lo}{-4.5}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_guard_s2lite/vs_baseline/ni/p_decisive}{0.139}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_params_replace/cost_usd}{0.00213}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_params_replace/decisions/ece}{0.085}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_params_replace/llm_calls}{1.09}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_params_replace/steps}{4.39}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_params_replace/success}{14.0}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_params_replace/success_ci/hi}{19.0}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_params_replace/success_ci/lo}{9.0}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_params_replace/vs_baseline/cost_savings}{95.1}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_params_replace/vs_baseline/delta}{-86.0}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_params_replace/vs_baseline/delta_ci/hi}{-81.0}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_params_replace/vs_baseline/delta_ci/lo}{-90.5}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_params_replace/vs_baseline/ni/p_decisive}{1.000}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_replace/cost_usd}{0.00792}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_replace/decisions/ece}{0.083}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_replace/llm_calls}{4.55}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_replace/steps}{4.55}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_replace/success}{26.5}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_replace/success_ci/hi}{32.5}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_replace/success_ci/lo}{20.5}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_replace/vs_baseline/cost_savings}{81.8}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_replace/vs_baseline/delta}{-73.5}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_replace/vs_baseline/delta_ci/hi}{-67.0}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_replace/vs_baseline/delta_ci/lo}{-79.5}
\defres{e2a_jevgym_tool_decisions_intern/intern_ts_replace/vs_baseline/ni/p_decisive}{1.000}
\defres{e2a_jevgym_tool_decisions_intern/jev_shadow/cost_usd}{0.0411}
\defres{e2a_jevgym_tool_decisions_intern/jev_shadow/decisions/ece}{0.046}
\defres{e2a_jevgym_tool_decisions_intern/jev_shadow/decisions/gold/gates/stop_guard-shadow/ece}{0.170}
\defres{e2a_jevgym_tool_decisions_intern/jev_shadow/decisions/gold/gates/stop_trigger-shadow/ece}{0.029}
\defres{e2a_jevgym_tool_decisions_intern/jev_shadow/decisions/noul/ece}{0.048}
\defres{e2a_jevgym_tool_decisions_intern/jev_shadow/llm_calls}{7.50}
\defres{e2a_jevgym_tool_decisions_intern/jev_shadow/steps}{7.50}
\defres{e2a_jevgym_tool_decisions_intern/jev_shadow/success}{100.0}
\defres{e2a_jevgym_tool_decisions_intern/jev_shadow/success_ci/hi}{100.0}
\defres{e2a_jevgym_tool_decisions_intern/jev_shadow/success_ci/lo}{100.0}
\defres{e2a_jevgym_tool_decisions_intern/jev_shadow/vs_baseline/cost_savings}{5.5}
\defres{e2a_jevgym_tool_decisions_intern/jev_shadow/vs_baseline/delta}{+0.0}
\defres{e2a_jevgym_tool_decisions_intern/jev_shadow/vs_baseline/delta_ci/hi}{+0.0}
\defres{e2a_jevgym_tool_decisions_intern/jev_shadow/vs_baseline/delta_ci/lo}{+0.0}
\defres{e2a_jevgym_tool_decisions_intern/jev_shadow/vs_baseline/ni/p_decisive}{0.002}
\defres{e2a_jevgym_tool_decisions_intern/jev_ts_assist_k3/cost_usd}{0.0195}
\defres{e2a_jevgym_tool_decisions_intern/jev_ts_assist_k3/decisions/ece}{0.048}
\defres{e2a_jevgym_tool_decisions_intern/jev_ts_assist_k3/llm_calls}{8.05}
\defres{e2a_jevgym_tool_decisions_intern/jev_ts_assist_k3/steps}{8.05}
\defres{e2a_jevgym_tool_decisions_intern/jev_ts_assist_k3/success}{91.5}
\defres{e2a_jevgym_tool_decisions_intern/jev_ts_assist_k3/success_ci/hi}{95.0}
\defres{e2a_jevgym_tool_decisions_intern/jev_ts_assist_k3/success_ci/lo}{87.5}
\defres{e2a_jevgym_tool_decisions_intern/jev_ts_assist_k3/vs_baseline/cost_savings}{55.2}
\defres{e2a_jevgym_tool_decisions_intern/jev_ts_assist_k3/vs_baseline/delta}{-8.5}
\defres{e2a_jevgym_tool_decisions_intern/jev_ts_assist_k3/vs_baseline/delta_ci/hi}{-4.5}
\defres{e2a_jevgym_tool_decisions_intern/jev_ts_assist_k3/vs_baseline/delta_ci/lo}{-12.5}
\defres{e2a_jevgym_tool_decisions_intern/jev_ts_assist_k3/vs_baseline/ni/p_decisive}{1.000}
\defres{e2a_jevgym_tool_decisions_intern/jev_ts_guard/cost_usd}{0.0421}
\defres{e2a_jevgym_tool_decisions_intern/jev_ts_guard/decisions/noul/ece}{0.131}
\defres{e2a_jevgym_tool_decisions_intern/jev_ts_guard/llm_calls}{7.66}
\defres{e2a_jevgym_tool_decisions_intern/jev_ts_guard/steps}{7.50}
\defres{e2a_jevgym_tool_decisions_intern/jev_ts_guard/success}{100.0}
\defres{e2a_jevgym_tool_decisions_intern/jev_ts_guard/success_ci/hi}{100.0}
\defres{e2a_jevgym_tool_decisions_intern/jev_ts_guard/success_ci/lo}{100.0}
\defres{e2a_jevgym_tool_decisions_intern/jev_ts_guard/vs_baseline/cost_savings}{3.1}
\defres{e2a_jevgym_tool_decisions_intern/jev_ts_guard/vs_baseline/delta}{+0.0}
\defres{e2a_jevgym_tool_decisions_intern/jev_ts_guard/vs_baseline/delta_ci/hi}{+0.0}
\defres{e2a_jevgym_tool_decisions_intern/jev_ts_guard/vs_baseline/delta_ci/lo}{+0.0}
\defres{e2a_jevgym_tool_decisions_intern/jev_ts_guard/vs_baseline/ni/p_decisive}{0.002}
\defres{e2a_jevgym_tool_decisions_intern/jev_ts_replace/cost_usd}{0.014}
\defres{e2a_jevgym_tool_decisions_intern/jev_ts_replace/decisions/ece}{0.027}
\defres{e2a_jevgym_tool_decisions_intern/jev_ts_replace/llm_calls}{6.80}
\defres{e2a_jevgym_tool_decisions_intern/jev_ts_replace/steps}{6.80}
\defres{e2a_jevgym_tool_decisions_intern/jev_ts_replace/success}{79.0}
\defres{e2a_jevgym_tool_decisions_intern/jev_ts_replace/success_ci/hi}{84.5}
\defres{e2a_jevgym_tool_decisions_intern/jev_ts_replace/success_ci/lo}{73.0}
\defres{e2a_jevgym_tool_decisions_intern/jev_ts_replace/vs_baseline/cost_savings}{67.8}
\defres{e2a_jevgym_tool_decisions_intern/jev_ts_replace/vs_baseline/delta}{-21.0}
\defres{e2a_jevgym_tool_decisions_intern/jev_ts_replace/vs_baseline/delta_ci/hi}{-15.5}
\defres{e2a_jevgym_tool_decisions_intern/jev_ts_replace/vs_baseline/delta_ci/lo}{-26.5}
\defres{e2a_jevgym_tool_decisions_intern/jev_ts_replace/vs_baseline/ni/p_decisive}{1.000}
\defres{e2a_jevgym_tool_decisions_intern/llm_only/cost_usd}{0.0436}
\defres{e2a_jevgym_tool_decisions_intern/llm_only/llm_calls}{7.52}
\defres{e2a_jevgym_tool_decisions_intern/llm_only/steps}{7.52}
\defres{e2a_jevgym_tool_decisions_intern/llm_only/success}{99.6}
\defres{e2a_jevgym_tool_decisions_intern/llm_only/success_ci/hi}{100.0}
\defres{e2a_jevgym_tool_decisions_intern/llm_only/success_ci/lo}{99.0}
\defres{e2a_jevgym_tool_decisions_intern/llm_only_s2lite/cost_usd}{0.00988}
\defres{e2a_jevgym_tool_decisions_intern/llm_only_s2lite/llm_calls}{7.57}
\defres{e2a_jevgym_tool_decisions_intern/llm_only_s2lite/steps}{7.57}
\defres{e2a_jevgym_tool_decisions_intern/llm_only_s2lite/success}{83.4}
\defres{e2a_jevgym_tool_decisions_intern/llm_only_s2lite/success_ci/hi}{86.6}
\defres{e2a_jevgym_tool_decisions_intern/llm_only_s2lite/success_ci/lo}{80.0}
\defres{e2a_jevgym_tool_decisions_intern/llm_only_s2lite/vs_baseline/cost_savings}{77.4}
\defres{e2a_jevgym_tool_decisions_intern/llm_only_s2lite/vs_baseline/delta}{-16.2}
\defres{e2a_jevgym_tool_decisions_intern/llm_only_s2lite/vs_baseline/delta_ci/hi}{-12.8}
\defres{e2a_jevgym_tool_decisions_intern/llm_only_s2lite/vs_baseline/delta_ci/lo}{-19.6}
\defres{e2a_jevgym_tool_decisions_intern/llm_only_s2lite/vs_baseline/ni/p_decisive}{1.000}
\defres{e2b_jevgym_meta_control/headline/iso_cost/delta_ci/hi}{+0.0}
\defres{e2b_jevgym_meta_control/headline/iso_cost/delta_ci/lo}{+0.0}
\defres{e2b_jevgym_meta_control/headline/iso_cost/success}{100.0}
\defres{e2b_jevgym_meta_control/headline/iso_cost_by_reference/llm_only_s2lite/delta_ci/hi}{+7.5}
\defres{e2b_jevgym_meta_control/headline/iso_cost_by_reference/llm_only_s2lite/delta_ci/lo}{-0.5}
\defres{e2b_jevgym_meta_control/headline/iso_cost_by_reference/llm_only_s2lite/success}{84.5}
\defres{e2b_jevgym_meta_control/headline/iso_quality/cost_savings_ci/hi}{1.7}
\defres{e2b_jevgym_meta_control/headline/iso_quality/cost_savings_ci/lo}{0.1}
\defres{e2b_jevgym_meta_control/headline/iso_quality/delta_ci/hi}{+0.0}
\defres{e2b_jevgym_meta_control/headline/iso_quality/delta_ci/lo}{+0.0}
\defres{e2b_jevgym_meta_control/headline/iso_quality_by_reference/llm_only_s2lite/cost_savings_ci/hi}{0.7}
\defres{e2b_jevgym_meta_control/headline/iso_quality_by_reference/llm_only_s2lite/cost_savings_ci/lo}{-1.0}
\defres{e2b_jevgym_meta_control/headline/iso_quality_by_reference/llm_only_s2lite/delta_ci/hi}{+7.5}
\defres{e2b_jevgym_meta_control/headline/iso_quality_by_reference/llm_only_s2lite/delta_ci/lo}{-0.5}
\defres{e2b_jevgym_meta_control/jev_mem/cost_usd}{0.0426}
\defres{e2b_jevgym_meta_control/jev_mem/decisions/ece}{0.269}
\defres{e2b_jevgym_meta_control/jev_mem/decisions/noul/ece}{0.253}
\defres{e2b_jevgym_meta_control/jev_mem/llm_calls}{7.50}
\defres{e2b_jevgym_meta_control/jev_mem/steps}{7.50}
\defres{e2b_jevgym_meta_control/jev_mem/success}{100.0}
\defres{e2b_jevgym_meta_control/jev_mem/success_ci/hi}{100.0}
\defres{e2b_jevgym_meta_control/jev_mem/success_ci/lo}{100.0}
\defres{e2b_jevgym_meta_control/jev_mem/vs_baseline/cost_savings}{-4.8}
\defres{e2b_jevgym_meta_control/jev_mem/vs_baseline/delta}{+0.0}
\defres{e2b_jevgym_meta_control/jev_mem/vs_baseline/delta_ci/hi}{+0.0}
\defres{e2b_jevgym_meta_control/jev_mem/vs_baseline/delta_ci/lo}{+0.0}
\defres{e2b_jevgym_meta_control/jev_mem/vs_baseline/ni/p_decisive}{0.002}
\defres{e2b_jevgym_meta_control/jev_reflect_trigger/cost_usd}{0.0403}
\defres{e2b_jevgym_meta_control/jev_reflect_trigger/decisions/noul/ece}{0.159}
\defres{e2b_jevgym_meta_control/jev_reflect_trigger/llm_calls}{8.43}
\defres{e2b_jevgym_meta_control/jev_reflect_trigger/steps}{7.52}
\defres{e2b_jevgym_meta_control/jev_reflect_trigger/success}{100.0}
\defres{e2b_jevgym_meta_control/jev_reflect_trigger/success_ci/hi}{100.0}
\defres{e2b_jevgym_meta_control/jev_reflect_trigger/success_ci/lo}{100.0}
\defres{e2b_jevgym_meta_control/jev_reflect_trigger/vs_baseline/cost_savings}{0.9}
\defres{e2b_jevgym_meta_control/jev_reflect_trigger/vs_baseline/delta}{+0.0}
\defres{e2b_jevgym_meta_control/jev_reflect_trigger/vs_baseline/delta_ci/hi}{+0.0}
\defres{e2b_jevgym_meta_control/jev_reflect_trigger/vs_baseline/delta_ci/lo}{+0.0}
\defres{e2b_jevgym_meta_control/jev_reflect_trigger/vs_baseline/ni/p_decisive}{0.002}
\defres{e2b_jevgym_meta_control/jev_reflect_trigger_s2lite_e2b/cost_usd}{0.00977}
\defres{e2b_jevgym_meta_control/jev_reflect_trigger_s2lite_e2b/decisions/noul/ece}{0.137}
\defres{e2b_jevgym_meta_control/jev_reflect_trigger_s2lite_e2b/llm_calls}{8.49}
\defres{e2b_jevgym_meta_control/jev_reflect_trigger_s2lite_e2b/steps}{7.57}
\defres{e2b_jevgym_meta_control/jev_reflect_trigger_s2lite_e2b/success}{84.5}
\defres{e2b_jevgym_meta_control/jev_reflect_trigger_s2lite_e2b/success_ci/hi}{89.5}
\defres{e2b_jevgym_meta_control/jev_reflect_trigger_s2lite_e2b/success_ci/lo}{79.5}
\defres{e2b_jevgym_meta_control/jev_reflect_trigger_s2lite_e2b/vs_baseline/cost_savings}{-0.2}
\defres{e2b_jevgym_meta_control/jev_reflect_trigger_s2lite_e2b/vs_baseline/delta}{+3.5}
\defres{e2b_jevgym_meta_control/jev_reflect_trigger_s2lite_e2b/vs_baseline/delta_ci/hi}{+7.5}
\defres{e2b_jevgym_meta_control/jev_reflect_trigger_s2lite_e2b/vs_baseline/delta_ci/lo}{-0.5}
\defres{e2b_jevgym_meta_control/jev_reflect_trigger_s2lite_e2b/vs_baseline/ni/p_decisive}{0.002}
\defres{e2b_jevgym_meta_control/jev_route_tau0.2/cost_usd}{0.0291}
\defres{e2b_jevgym_meta_control/jev_route_tau0.2/decisions/noul/ece}{0.142}
\defres{e2b_jevgym_meta_control/jev_route_tau0.2/llm_calls}{7.54}
\defres{e2b_jevgym_meta_control/jev_route_tau0.2/steps}{7.54}
\defres{e2b_jevgym_meta_control/jev_route_tau0.2/success}{97.0}
\defres{e2b_jevgym_meta_control/jev_route_tau0.2/success_ci/hi}{99.0}
\defres{e2b_jevgym_meta_control/jev_route_tau0.2/success_ci/lo}{94.5}
\defres{e2b_jevgym_meta_control/jev_route_tau0.2/vs_baseline/cost_savings}{28.4}
\defres{e2b_jevgym_meta_control/jev_route_tau0.2/vs_baseline/delta}{-3.0}
\defres{e2b_jevgym_meta_control/jev_route_tau0.2/vs_baseline/delta_ci/hi}{-1.0}
\defres{e2b_jevgym_meta_control/jev_route_tau0.2/vs_baseline/delta_ci/lo}{-5.5}
\defres{e2b_jevgym_meta_control/jev_route_tau0.2/vs_baseline/ni/p_decisive}{0.631}
\defres{e2b_jevgym_meta_control/jev_route_tau0.4/cost_usd}{0.0134}
\defres{e2b_jevgym_meta_control/jev_route_tau0.4/decisions/noul/ece}{0.174}
\defres{e2b_jevgym_meta_control/jev_route_tau0.4/llm_calls}{7.57}
\defres{e2b_jevgym_meta_control/jev_route_tau0.4/steps}{7.57}
\defres{e2b_jevgym_meta_control/jev_route_tau0.4/success}{81.4}
\defres{e2b_jevgym_meta_control/jev_route_tau0.4/success_ci/hi}{85.0}
\defres{e2b_jevgym_meta_control/jev_route_tau0.4/success_ci/lo}{77.8}
\defres{e2b_jevgym_meta_control/jev_route_tau0.4/vs_baseline/cost_savings}{67.3}
\defres{e2b_jevgym_meta_control/jev_route_tau0.4/vs_baseline/delta}{-18.4}
\defres{e2b_jevgym_meta_control/jev_route_tau0.4/vs_baseline/delta_ci/hi}{-15.0}
\defres{e2b_jevgym_meta_control/jev_route_tau0.4/vs_baseline/delta_ci/lo}{-22.0}
\defres{e2b_jevgym_meta_control/jev_route_tau0.4/vs_baseline/ni/p_decisive}{1.000}
\defres{e2b_jevgym_meta_control/jev_route_tau0.6/cost_usd}{0.0101}
\defres{e2b_jevgym_meta_control/jev_route_tau0.6/decisions/noul/ece}{0.201}
\defres{e2b_jevgym_meta_control/jev_route_tau0.6/llm_calls}{7.54}
\defres{e2b_jevgym_meta_control/jev_route_tau0.6/steps}{7.54}
\defres{e2b_jevgym_meta_control/jev_route_tau0.6/success}{83.0}
\defres{e2b_jevgym_meta_control/jev_route_tau0.6/success_ci/hi}{88.0}
\defres{e2b_jevgym_meta_control/jev_route_tau0.6/success_ci/lo}{77.5}
\defres{e2b_jevgym_meta_control/jev_route_tau0.6/vs_baseline/cost_savings}{75.2}
\defres{e2b_jevgym_meta_control/jev_route_tau0.6/vs_baseline/delta}{-17.0}
\defres{e2b_jevgym_meta_control/jev_route_tau0.6/vs_baseline/delta_ci/hi}{-12.0}
\defres{e2b_jevgym_meta_control/jev_route_tau0.6/vs_baseline/delta_ci/lo}{-22.0}
\defres{e2b_jevgym_meta_control/jev_route_tau0.6/vs_baseline/ni/p_decisive}{1.000}
\defres{e2b_jevgym_meta_control/jev_route_tau0.8/cost_usd}{0.0101}
\defres{e2b_jevgym_meta_control/jev_route_tau0.8/decisions/noul/ece}{0.204}
\defres{e2b_jevgym_meta_control/jev_route_tau0.8/llm_calls}{7.54}
\defres{e2b_jevgym_meta_control/jev_route_tau0.8/steps}{7.54}
\defres{e2b_jevgym_meta_control/jev_route_tau0.8/success}{84.0}
\defres{e2b_jevgym_meta_control/jev_route_tau0.8/success_ci/hi}{89.0}
\defres{e2b_jevgym_meta_control/jev_route_tau0.8/success_ci/lo}{78.5}
\defres{e2b_jevgym_meta_control/jev_route_tau0.8/vs_baseline/cost_savings}{75.2}
\defres{e2b_jevgym_meta_control/jev_route_tau0.8/vs_baseline/delta}{-16.0}
\defres{e2b_jevgym_meta_control/jev_route_tau0.8/vs_baseline/delta_ci/hi}{-11.0}
\defres{e2b_jevgym_meta_control/jev_route_tau0.8/vs_baseline/delta_ci/lo}{-21.0}
\defres{e2b_jevgym_meta_control/jev_route_tau0.8/vs_baseline/ni/p_decisive}{1.000}
\defres{e2b_jevgym_meta_control/jev_stop_guard/cost_usd}{0.0433}
\defres{e2b_jevgym_meta_control/jev_stop_guard/decisions/noul/ece}{0.243}
\defres{e2b_jevgym_meta_control/jev_stop_guard/llm_calls}{7.72}
\defres{e2b_jevgym_meta_control/jev_stop_guard/steps}{7.72}
\defres{e2b_jevgym_meta_control/jev_stop_guard/success}{99.2}
\defres{e2b_jevgym_meta_control/jev_stop_guard/success_ci/hi}{99.8}
\defres{e2b_jevgym_meta_control/jev_stop_guard/success_ci/lo}{98.4}
\defres{e2b_jevgym_meta_control/jev_stop_guard/vs_baseline/cost_savings}{-6.2}
\defres{e2b_jevgym_meta_control/jev_stop_guard/vs_baseline/delta}{-0.6}
\defres{e2b_jevgym_meta_control/jev_stop_guard/vs_baseline/delta_ci/hi}{+0.0}
\defres{e2b_jevgym_meta_control/jev_stop_guard/vs_baseline/delta_ci/lo}{-1.4}
\defres{e2b_jevgym_meta_control/jev_stop_guard/vs_baseline/ni/p_decisive}{$<$0.001}
\defres{e2b_jevgym_meta_control/jev_stop_guard_s2lite/cost_usd}{0.013}
\defres{e2b_jevgym_meta_control/jev_stop_guard_s2lite/decisions/noul/ece}{0.128}
\defres{e2b_jevgym_meta_control/jev_stop_guard_s2lite/llm_calls}{9.91}
\defres{e2b_jevgym_meta_control/jev_stop_guard_s2lite/steps}{9.91}
\defres{e2b_jevgym_meta_control/jev_stop_guard_s2lite/success}{82.0}
\defres{e2b_jevgym_meta_control/jev_stop_guard_s2lite/success_ci/hi}{85.4}
\defres{e2b_jevgym_meta_control/jev_stop_guard_s2lite/success_ci/lo}{78.6}
\defres{e2b_jevgym_meta_control/jev_stop_guard_s2lite/vs_baseline/cost_savings}{-32.1}
\defres{e2b_jevgym_meta_control/jev_stop_guard_s2lite/vs_baseline/delta}{+1.6}
\defres{e2b_jevgym_meta_control/jev_stop_guard_s2lite/vs_baseline/delta_ci/hi}{+4.0}
\defres{e2b_jevgym_meta_control/jev_stop_guard_s2lite/vs_baseline/delta_ci/lo}{-0.8}
\defres{e2b_jevgym_meta_control/jev_stop_guard_s2lite/vs_baseline/ni/p_decisive}{$<$0.001}
\defres{e2b_jevgym_meta_control/jev_stop_trigger/cost_usd}{0.0406}
\defres{e2b_jevgym_meta_control/jev_stop_trigger/decisions/noul/ece}{0.029}
\defres{e2b_jevgym_meta_control/jev_stop_trigger/llm_calls}{7.50}
\defres{e2b_jevgym_meta_control/jev_stop_trigger/steps}{7.50}
\defres{e2b_jevgym_meta_control/jev_stop_trigger/success}{100.0}
\defres{e2b_jevgym_meta_control/jev_stop_trigger/success_ci/hi}{100.0}
\defres{e2b_jevgym_meta_control/jev_stop_trigger/success_ci/lo}{100.0}
\defres{e2b_jevgym_meta_control/jev_stop_trigger/vs_baseline/cost_savings}{-0.1}
\defres{e2b_jevgym_meta_control/jev_stop_trigger/vs_baseline/delta}{+0.0}
\defres{e2b_jevgym_meta_control/jev_stop_trigger/vs_baseline/delta_ci/hi}{+0.0}
\defres{e2b_jevgym_meta_control/jev_stop_trigger/vs_baseline/delta_ci/lo}{+0.0}
\defres{e2b_jevgym_meta_control/jev_stop_trigger/vs_baseline/ni/p_decisive}{0.002}
\defres{e2b_jevgym_meta_control/lite_route/cost_usd}{0.0144}
\defres{e2b_jevgym_meta_control/lite_route/decisions/noul/ece}{0.027}
\defres{e2b_jevgym_meta_control/lite_route/llm_calls}{7.55}
\defres{e2b_jevgym_meta_control/lite_route/steps}{7.55}
\defres{e2b_jevgym_meta_control/lite_route/success}{85.0}
\defres{e2b_jevgym_meta_control/lite_route/success_ci/hi}{90.0}
\defres{e2b_jevgym_meta_control/lite_route/success_ci/lo}{80.0}
\defres{e2b_jevgym_meta_control/lite_route/vs_baseline/cost_savings}{64.5}
\defres{e2b_jevgym_meta_control/lite_route/vs_baseline/delta}{-15.0}
\defres{e2b_jevgym_meta_control/lite_route/vs_baseline/delta_ci/hi}{-10.0}
\defres{e2b_jevgym_meta_control/lite_route/vs_baseline/delta_ci/lo}{-20.0}
\defres{e2b_jevgym_meta_control/lite_route/vs_baseline/ni/p_decisive}{1.000}
\defres{e2b_jevgym_meta_control/lite_stop_guard/cost_usd}{0.0424}
\defres{e2b_jevgym_meta_control/lite_stop_guard/decisions/noul/ece}{0.209}
\defres{e2b_jevgym_meta_control/lite_stop_guard/llm_calls}{7.75}
\defres{e2b_jevgym_meta_control/lite_stop_guard/steps}{7.75}
\defres{e2b_jevgym_meta_control/lite_stop_guard/success}{99.5}
\defres{e2b_jevgym_meta_control/lite_stop_guard/success_ci/hi}{100.0}
\defres{e2b_jevgym_meta_control/lite_stop_guard/success_ci/lo}{98.5}
\defres{e2b_jevgym_meta_control/lite_stop_guard/vs_baseline/cost_savings}{-4.5}
\defres{e2b_jevgym_meta_control/lite_stop_guard/vs_baseline/delta}{-0.5}
\defres{e2b_jevgym_meta_control/lite_stop_guard/vs_baseline/delta_ci/hi}{+0.0}
\defres{e2b_jevgym_meta_control/lite_stop_guard/vs_baseline/delta_ci/lo}{-1.5}
\defres{e2b_jevgym_meta_control/lite_stop_guard/vs_baseline/ni/p_decisive}{0.016}
\defres{e2b_jevgym_meta_control/llm_only/cost_usd}{0.0408}
\defres{e2b_jevgym_meta_control/llm_only/llm_calls}{7.52}
\defres{e2b_jevgym_meta_control/llm_only/steps}{7.52}
\defres{e2b_jevgym_meta_control/llm_only/success}{99.8}
\defres{e2b_jevgym_meta_control/llm_only/success_ci/hi}{100.0}
\defres{e2b_jevgym_meta_control/llm_only/success_ci/lo}{99.4}
\defres{e2b_jevgym_meta_control/llm_only_s2lite/cost_usd}{0.0098}
\defres{e2b_jevgym_meta_control/llm_only_s2lite/llm_calls}{7.58}
\defres{e2b_jevgym_meta_control/llm_only_s2lite/steps}{7.58}
\defres{e2b_jevgym_meta_control/llm_only_s2lite/success}{80.4}
\defres{e2b_jevgym_meta_control/llm_only_s2lite/success_ci/hi}{83.6}
\defres{e2b_jevgym_meta_control/llm_only_s2lite/success_ci/lo}{76.6}
\defres{e2b_jevgym_meta_control/llm_only_s2lite/vs_baseline/cost_savings}{76.0}
\defres{e2b_jevgym_meta_control/llm_only_s2lite/vs_baseline/delta}{-19.4}
\defres{e2b_jevgym_meta_control/llm_only_s2lite/vs_baseline/delta_ci/hi}{-15.8}
\defres{e2b_jevgym_meta_control/llm_only_s2lite/vs_baseline/delta_ci/lo}{-23.0}
\defres{e2b_jevgym_meta_control/llm_only_s2lite/vs_baseline/ni/p_decisive}{1.000}
\defres{e2b_jevgym_meta_control/mem_always/cost_usd}{0.0554}
\defres{e2b_jevgym_meta_control/mem_always/llm_calls}{7.82}
\defres{e2b_jevgym_meta_control/mem_always/steps}{7.82}
\defres{e2b_jevgym_meta_control/mem_always/success}{98.0}
\defres{e2b_jevgym_meta_control/mem_always/success_ci/hi}{99.5}
\defres{e2b_jevgym_meta_control/mem_always/success_ci/lo}{96.0}
\defres{e2b_jevgym_meta_control/mem_always/vs_baseline/cost_savings}{-36.3}
\defres{e2b_jevgym_meta_control/mem_always/vs_baseline/delta}{-2.0}
\defres{e2b_jevgym_meta_control/mem_always/vs_baseline/delta_ci/hi}{-0.5}
\defres{e2b_jevgym_meta_control/mem_always/vs_baseline/delta_ci/lo}{-4.0}
\defres{e2b_jevgym_meta_control/mem_always/vs_baseline/ni/p_decisive}{0.306}
\defres{e2b_jevgym_meta_control/mem_llm_gate/cost_usd}{0.0648}
\defres{e2b_jevgym_meta_control/mem_llm_gate/llm_calls}{14.00}
\defres{e2b_jevgym_meta_control/mem_llm_gate/steps}{7.50}
\defres{e2b_jevgym_meta_control/mem_llm_gate/success}{100.0}
\defres{e2b_jevgym_meta_control/mem_llm_gate/success_ci/hi}{100.0}
\defres{e2b_jevgym_meta_control/mem_llm_gate/success_ci/lo}{100.0}
\defres{e2b_jevgym_meta_control/mem_llm_gate/vs_baseline/cost_savings}{-59.6}
\defres{e2b_jevgym_meta_control/mem_llm_gate/vs_baseline/delta}{+0.0}
\defres{e2b_jevgym_meta_control/mem_llm_gate/vs_baseline/delta_ci/hi}{+0.0}
\defres{e2b_jevgym_meta_control/mem_llm_gate/vs_baseline/delta_ci/lo}{+0.0}
\defres{e2b_jevgym_meta_control/mem_llm_gate/vs_baseline/ni/p_decisive}{0.002}
\defres{e2b_jevgym_meta_control/meta_shadow/cost_usd}{0.0421}
\defres{e2b_jevgym_meta_control/meta_shadow/decisions/gold/gates/memory_write-shadow/ece}{0.229}
\defres{e2b_jevgym_meta_control/meta_shadow/decisions/gold/gates/reflection-shadow/ece}{0.314}
\defres{e2b_jevgym_meta_control/meta_shadow/decisions/gold/gates/stop_guard-shadow/ece}{0.169}
\defres{e2b_jevgym_meta_control/meta_shadow/decisions/gold/gates/stop_trigger-shadow/ece}{0.029}
\defres{e2b_jevgym_meta_control/meta_shadow/decisions/gold/probes/stop/by_d/1/far_ci/hi}{0.526}
\defres{e2b_jevgym_meta_control/meta_shadow/decisions/gold/probes/stop/by_d/1/far_ci/lo}{0.352}
\defres{e2b_jevgym_meta_control/meta_shadow/decisions/gold/probes/stop/by_d/2/far_ci/hi}{0}
\defres{e2b_jevgym_meta_control/meta_shadow/decisions/gold/probes/stop/by_d/2/far_ci/lo}{0}
\defres{e2b_jevgym_meta_control/meta_shadow/decisions/gold/probes/stop/by_d/3-4/far_ci/hi}{0}
\defres{e2b_jevgym_meta_control/meta_shadow/decisions/gold/probes/stop/by_d/3-4/far_ci/lo}{0}
\defres{e2b_jevgym_meta_control/meta_shadow/decisions/gold/probes/stop/by_d/5+/far_ci/hi}{0}
\defres{e2b_jevgym_meta_control/meta_shadow/decisions/gold/probes/stop/by_d/5+/far_ci/lo}{0}
\defres{e2b_jevgym_meta_control/meta_shadow/decisions/gold/probes/stop/by_kind/ok/frr_ci/hi}{0.105}
\defres{e2b_jevgym_meta_control/meta_shadow/decisions/gold/probes/stop/by_kind/ok/frr_ci/lo}{0.047}
\defres{e2b_jevgym_meta_control/meta_shadow/decisions/gold/probes/stop/by_kind/premature/far_ci/hi}{0}
\defres{e2b_jevgym_meta_control/meta_shadow/decisions/gold/probes/stop/by_kind/premature/far_ci/lo}{0}
\defres{e2b_jevgym_meta_control/meta_shadow/decisions/gold/probes/stop/by_kind/wrong_answer/far_ci/hi}{0.526}
\defres{e2b_jevgym_meta_control/meta_shadow/decisions/gold/probes/stop/by_kind/wrong_answer/far_ci/lo}{0.352}
\defres{e2b_jevgym_meta_control/meta_shadow/decisions/gold/probes/stop/by_operator/T5/far_ci/hi}{0}
\defres{e2b_jevgym_meta_control/meta_shadow/decisions/gold/probes/stop/by_operator/T5/far_ci/lo}{0}
\defres{e2b_jevgym_meta_control/meta_shadow/decisions/gold/probes/stop/by_operator/T6/far_ci/hi}{0.625}
\defres{e2b_jevgym_meta_control/meta_shadow/decisions/gold/probes/stop/by_operator/T6/far_ci/lo}{0.427}
\defres{e2b_jevgym_meta_control/meta_shadow/decisions/gold/probes/stop/by_source/edit/far_ci/hi}{0.149}
\defres{e2b_jevgym_meta_control/meta_shadow/decisions/gold/probes/stop/by_source/edit/far_ci/lo}{0.0978}
\defres{e2b_jevgym_meta_control/meta_shadow/decisions/gold/probes/stop/by_source/forced_premature/far_ci/hi}{0}
\defres{e2b_jevgym_meta_control/meta_shadow/decisions/gold/probes/stop/by_source/forced_premature/far_ci/lo}{0}
\defres{e2b_jevgym_meta_control/meta_shadow/decisions/gold/probes/stop/by_source/natural/frr_ci/hi}{0.12}
\defres{e2b_jevgym_meta_control/meta_shadow/decisions/gold/probes/stop/by_source/natural/frr_ci/lo}{0.045}
\defres{e2b_jevgym_meta_control/meta_shadow/decisions/gold/probes/stop/by_source/transplant/far_ci/hi}{0.366}
\defres{e2b_jevgym_meta_control/meta_shadow/decisions/gold/probes/stop/by_source/transplant/far_ci/lo}{0.0976}
\defres{e2b_jevgym_meta_control/meta_shadow/decisions/gold/probes/stop/by_source/transplant/frr_ci/hi}{0.107}
\defres{e2b_jevgym_meta_control/meta_shadow/decisions/gold/probes/stop/by_source/transplant/frr_ci/lo}{0.0252}
\defres{e2b_jevgym_meta_control/meta_shadow/decisions/gold/probes/stop/far_edit/T5/far_ci/hi}{0}
\defres{e2b_jevgym_meta_control/meta_shadow/decisions/gold/probes/stop/far_edit/T5/far_ci/lo}{0}
\defres{e2b_jevgym_meta_control/meta_shadow/decisions/gold/probes/stop/far_edit/T6/far_ci/hi}{0.625}
\defres{e2b_jevgym_meta_control/meta_shadow/decisions/gold/probes/stop/far_edit/T6/far_ci/lo}{0.427}
\defres{e2b_jevgym_meta_control/meta_shadow/decisions/gold/probes/stop/far_model/far}{3.7}
\defres{e2b_jevgym_meta_control/meta_shadow/decisions/gold/probes/stop/far_model/far_ci/hi}{0.061}
\defres{e2b_jevgym_meta_control/meta_shadow/decisions/gold/probes/stop/far_model/far_ci/lo}{0.0166}
\defres{e2b_jevgym_meta_control/meta_shadow/decisions/gold/probes/stop/far_model/n}{241}
\defres{e2b_jevgym_meta_control/meta_shadow/decisions/gold/probes/stop/frr/frr}{8.0}
\defres{e2b_jevgym_meta_control/meta_shadow/decisions/gold/probes/stop/frr/frr_ci/hi}{0.12}
\defres{e2b_jevgym_meta_control/meta_shadow/decisions/gold/probes/stop/frr/frr_ci/lo}{0.045}
\defres{e2b_jevgym_meta_control/meta_shadow/decisions/gold/probes/stop/frr/n}{200}
\defres{e2b_jevgym_meta_control/meta_shadow/decisions/gold/probes/tool_select/by_d/2/far_ci/hi}{0.128}
\defres{e2b_jevgym_meta_control/meta_shadow/decisions/gold/probes/tool_select/by_d/2/far_ci/lo}{0.0213}
\defres{e2b_jevgym_meta_control/meta_shadow/decisions/gold/probes/tool_select/by_d/3-4/far_ci/hi}{0.188}
\defres{e2b_jevgym_meta_control/meta_shadow/decisions/gold/probes/tool_select/by_d/3-4/far_ci/lo}{0.0899}
\defres{e2b_jevgym_meta_control/meta_shadow/decisions/gold/probes/tool_select/by_d/5+/far_ci/hi}{0.145}
\defres{e2b_jevgym_meta_control/meta_shadow/decisions/gold/probes/tool_select/by_d/5+/far_ci/lo}{0.0737}
\defres{e2b_jevgym_meta_control/meta_shadow/decisions/gold/probes/tool_select/by_kind/detour/far_ci/hi}{0.163}
\defres{e2b_jevgym_meta_control/meta_shadow/decisions/gold/probes/tool_select/by_kind/detour/far_ci/lo}{0.0954}
\defres{e2b_jevgym_meta_control/meta_shadow/decisions/gold/probes/tool_select/by_kind/fatal/far_ci/hi}{0.117}
\defres{e2b_jevgym_meta_control/meta_shadow/decisions/gold/probes/tool_select/by_kind/fatal/far_ci/lo}{0.0415}
\defres{e2b_jevgym_meta_control/meta_shadow/decisions/gold/probes/tool_select/by_kind/progress/frr_ci/hi}{0.0204}
\defres{e2b_jevgym_meta_control/meta_shadow/decisions/gold/probes/tool_select/by_kind/progress/frr_ci/lo}{0.00742}
\defres{e2b_jevgym_meta_control/meta_shadow/decisions/gold/probes/tool_select/by_operator/T1/far_ci/hi}{0.201}
\defres{e2b_jevgym_meta_control/meta_shadow/decisions/gold/probes/tool_select/by_operator/T1/far_ci/lo}{0.115}
\defres{e2b_jevgym_meta_control/meta_shadow/decisions/gold/probes/tool_select/by_operator/T2/far_ci/hi}{0.104}
\defres{e2b_jevgym_meta_control/meta_shadow/decisions/gold/probes/tool_select/by_operator/T2/far_ci/lo}{0.012}
\defres{e2b_jevgym_meta_control/meta_shadow/decisions/gold/probes/tool_select/by_operator/T3/far_ci/hi}{0.0974}
\defres{e2b_jevgym_meta_control/meta_shadow/decisions/gold/probes/tool_select/by_operator/T3/far_ci/lo}{0.0258}
\defres{e2b_jevgym_meta_control/meta_shadow/decisions/gold/probes/tool_select/by_operator/T4/far_ci/hi}{0.3}
\defres{e2b_jevgym_meta_control/meta_shadow/decisions/gold/probes/tool_select/by_operator/T4/far_ci/lo}{0}
\defres{e2b_jevgym_meta_control/meta_shadow/decisions/gold/probes/tool_select/by_source/edit/far_ci/hi}{0.14}
\defres{e2b_jevgym_meta_control/meta_shadow/decisions/gold/probes/tool_select/by_source/edit/far_ci/lo}{0.0852}
\defres{e2b_jevgym_meta_control/meta_shadow/decisions/gold/probes/tool_select/by_source/natural/frr_ci/hi}{0.0218}
\defres{e2b_jevgym_meta_control/meta_shadow/decisions/gold/probes/tool_select/by_source/natural/frr_ci/lo}{0.0084}
\defres{e2b_jevgym_meta_control/meta_shadow/decisions/gold/probes/tool_select/by_source/transplant/frr_ci/hi}{0.0207}
\defres{e2b_jevgym_meta_control/meta_shadow/decisions/gold/probes/tool_select/by_source/transplant/frr_ci/lo}{0}
\defres{e2b_jevgym_meta_control/meta_shadow/decisions/gold/probes/tool_select/far_fatal/far}{7.7}
\defres{e2b_jevgym_meta_control/meta_shadow/decisions/gold/probes/tool_select/far_fatal/far_ci/hi}{0.117}
\defres{e2b_jevgym_meta_control/meta_shadow/decisions/gold/probes/tool_select/far_fatal/far_ci/lo}{0.0415}
\defres{e2b_jevgym_meta_control/meta_shadow/decisions/gold/probes/tool_select/far_fatal/n}{181}
\defres{e2b_jevgym_meta_control/meta_shadow/decisions/gold/probes/tool_select/headline/far}{0.0}
\defres{e2b_jevgym_meta_control/meta_shadow/decisions/gold/probes/tool_select/headline/far_ci/hi}{0}
\defres{e2b_jevgym_meta_control/meta_shadow/decisions/gold/probes/tool_select/headline/far_ci/lo}{0}
\defres{e2b_jevgym_meta_control/meta_shadow/decisions/gold/probes/tool_select/headline/frr}{1.3}
\defres{e2b_jevgym_meta_control/meta_shadow/decisions/gold/probes/tool_select/headline/frr_ci/hi}{0.0204}
\defres{e2b_jevgym_meta_control/meta_shadow/decisions/gold/probes/tool_select/headline/frr_ci/lo}{0.00742}
\defres{e2b_jevgym_meta_control/meta_shadow/decisions/gold/probes/tool_select/headline/n_right}{1631}
\defres{e2b_jevgym_meta_control/meta_shadow/decisions/gold/probes/tool_select/headline/n_wrong}{2}
\defres{e2b_jevgym_meta_control/meta_shadow/decisions/noul/ece}{0.176}
\defres{e2b_jevgym_meta_control/meta_shadow/llm_calls}{7.50}
\defres{e2b_jevgym_meta_control/meta_shadow/steps}{7.50}
\defres{e2b_jevgym_meta_control/meta_shadow/success}{100.0}
\defres{e2b_jevgym_meta_control/meta_shadow/success_ci/hi}{100.0}
\defres{e2b_jevgym_meta_control/meta_shadow/success_ci/lo}{100.0}
\defres{e2b_jevgym_meta_control/meta_shadow/vs_baseline/cost_savings}{-3.6}
\defres{e2b_jevgym_meta_control/meta_shadow/vs_baseline/delta}{+0.0}
\defres{e2b_jevgym_meta_control/meta_shadow/vs_baseline/delta_ci/hi}{+0.0}
\defres{e2b_jevgym_meta_control/meta_shadow/vs_baseline/delta_ci/lo}{+0.0}
\defres{e2b_jevgym_meta_control/meta_shadow/vs_baseline/ni/p_decisive}{0.002}
\defres{e2b_jevgym_meta_control/meta_shadow_s2lite/cost_usd}{0.00979}
\defres{e2b_jevgym_meta_control/meta_shadow_s2lite/decisions/gold/gates/memory_write-shadow/ece}{0.229}
\defres{e2b_jevgym_meta_control/meta_shadow_s2lite/decisions/gold/gates/reflection-shadow/ece}{0.239}
\defres{e2b_jevgym_meta_control/meta_shadow_s2lite/decisions/gold/gates/routing-shadow/ece}{0.204}
\defres{e2b_jevgym_meta_control/meta_shadow_s2lite/decisions/gold/gates/stop_guard-shadow/ece}{0.092}
\defres{e2b_jevgym_meta_control/meta_shadow_s2lite/decisions/gold/gates/stop_trigger-shadow/ece}{0.028}
\defres{e2b_jevgym_meta_control/meta_shadow_s2lite/decisions/gold/probes/stop/by_d/1/far_ci/hi}{0.47}
\defres{e2b_jevgym_meta_control/meta_shadow_s2lite/decisions/gold/probes/stop/by_d/1/far_ci/lo}{0.358}
\defres{e2b_jevgym_meta_control/meta_shadow_s2lite/decisions/gold/probes/stop/by_d/2/far_ci/hi}{0.0189}
\defres{e2b_jevgym_meta_control/meta_shadow_s2lite/decisions/gold/probes/stop/by_d/2/far_ci/lo}{0.00226}
\defres{e2b_jevgym_meta_control/meta_shadow_s2lite/decisions/gold/probes/stop/by_d/3-4/far_ci/hi}{0}
\defres{e2b_jevgym_meta_control/meta_shadow_s2lite/decisions/gold/probes/stop/by_d/3-4/far_ci/lo}{0}
\defres{e2b_jevgym_meta_control/meta_shadow_s2lite/decisions/gold/probes/stop/by_d/5+/far_ci/hi}{0}
\defres{e2b_jevgym_meta_control/meta_shadow_s2lite/decisions/gold/probes/stop/by_d/5+/far_ci/lo}{0}
\defres{e2b_jevgym_meta_control/meta_shadow_s2lite/decisions/gold/probes/stop/by_kind/ok/frr_ci/hi}{0.0235}
\defres{e2b_jevgym_meta_control/meta_shadow_s2lite/decisions/gold/probes/stop/by_kind/ok/frr_ci/lo}{0.00367}
\defres{e2b_jevgym_meta_control/meta_shadow_s2lite/decisions/gold/probes/stop/by_kind/premature/far_ci/hi}{0.00665}
\defres{e2b_jevgym_meta_control/meta_shadow_s2lite/decisions/gold/probes/stop/by_kind/premature/far_ci/lo}{0.000733}
\defres{e2b_jevgym_meta_control/meta_shadow_s2lite/decisions/gold/probes/stop/by_kind/wrong_answer/far_ci/hi}{0.47}
\defres{e2b_jevgym_meta_control/meta_shadow_s2lite/decisions/gold/probes/stop/by_kind/wrong_answer/far_ci/lo}{0.358}
\defres{e2b_jevgym_meta_control/meta_shadow_s2lite/decisions/gold/probes/stop/by_operator/T5/far_ci/hi}{0}
\defres{e2b_jevgym_meta_control/meta_shadow_s2lite/decisions/gold/probes/stop/by_operator/T5/far_ci/lo}{0}
\defres{e2b_jevgym_meta_control/meta_shadow_s2lite/decisions/gold/probes/stop/by_operator/T6/far_ci/hi}{0.465}
\defres{e2b_jevgym_meta_control/meta_shadow_s2lite/decisions/gold/probes/stop/by_operator/T6/far_ci/lo}{0.339}
\defres{e2b_jevgym_meta_control/meta_shadow_s2lite/decisions/gold/probes/stop/by_source/edit/far_ci/hi}{0.107}
\defres{e2b_jevgym_meta_control/meta_shadow_s2lite/decisions/gold/probes/stop/by_source/edit/far_ci/lo}{0.0764}
\defres{e2b_jevgym_meta_control/meta_shadow_s2lite/decisions/gold/probes/stop/by_source/forced_premature/far_ci/hi}{0.018}
\defres{e2b_jevgym_meta_control/meta_shadow_s2lite/decisions/gold/probes/stop/by_source/forced_premature/far_ci/lo}{0.002}
\defres{e2b_jevgym_meta_control/meta_shadow_s2lite/decisions/gold/probes/stop/by_source/natural/far_ci/hi}{0.505}
\defres{e2b_jevgym_meta_control/meta_shadow_s2lite/decisions/gold/probes/stop/by_source/natural/far_ci/lo}{0.308}
\defres{e2b_jevgym_meta_control/meta_shadow_s2lite/decisions/gold/probes/stop/by_source/natural/frr_ci/hi}{0.0221}
\defres{e2b_jevgym_meta_control/meta_shadow_s2lite/decisions/gold/probes/stop/by_source/natural/frr_ci/lo}{0.00244}
\defres{e2b_jevgym_meta_control/meta_shadow_s2lite/decisions/gold/probes/stop/by_source/transplant/far_ci/hi}{0.541}
\defres{e2b_jevgym_meta_control/meta_shadow_s2lite/decisions/gold/probes/stop/by_source/transplant/far_ci/lo}{0.347}
\defres{e2b_jevgym_meta_control/meta_shadow_s2lite/decisions/gold/probes/stop/by_source/transplant/frr_ci/hi}{0.0249}
\defres{e2b_jevgym_meta_control/meta_shadow_s2lite/decisions/gold/probes/stop/by_source/transplant/frr_ci/lo}{0.00249}
\defres{e2b_jevgym_meta_control/meta_shadow_s2lite/decisions/gold/probes/stop/far_edit/T5/far_ci/hi}{0}
\defres{e2b_jevgym_meta_control/meta_shadow_s2lite/decisions/gold/probes/stop/far_edit/T5/far_ci/lo}{0}
\defres{e2b_jevgym_meta_control/meta_shadow_s2lite/decisions/gold/probes/stop/far_edit/T6/far_ci/hi}{0.465}
\defres{e2b_jevgym_meta_control/meta_shadow_s2lite/decisions/gold/probes/stop/far_edit/T6/far_ci/lo}{0.339}
\defres{e2b_jevgym_meta_control/meta_shadow_s2lite/decisions/gold/probes/stop/far_model/far}{12.3}
\defres{e2b_jevgym_meta_control/meta_shadow_s2lite/decisions/gold/probes/stop/far_model/far_ci/hi}{0.152}
\defres{e2b_jevgym_meta_control/meta_shadow_s2lite/decisions/gold/probes/stop/far_model/far_ci/lo}{0.0937}
\defres{e2b_jevgym_meta_control/meta_shadow_s2lite/decisions/gold/probes/stop/far_model/n}{689}
\defres{e2b_jevgym_meta_control/meta_shadow_s2lite/decisions/gold/probes/stop/far_nat/far}{40.7}
\defres{e2b_jevgym_meta_control/meta_shadow_s2lite/decisions/gold/probes/stop/far_nat/far_ci/hi}{0.505}
\defres{e2b_jevgym_meta_control/meta_shadow_s2lite/decisions/gold/probes/stop/far_nat/far_ci/lo}{0.308}
\defres{e2b_jevgym_meta_control/meta_shadow_s2lite/decisions/gold/probes/stop/far_nat/n}{91}
\defres{e2b_jevgym_meta_control/meta_shadow_s2lite/decisions/gold/probes/stop/frr/frr}{1.2}
\defres{e2b_jevgym_meta_control/meta_shadow_s2lite/decisions/gold/probes/stop/frr/frr_ci/hi}{0.0221}
\defres{e2b_jevgym_meta_control/meta_shadow_s2lite/decisions/gold/probes/stop/frr/frr_ci/lo}{0.00244}
\defres{e2b_jevgym_meta_control/meta_shadow_s2lite/decisions/gold/probes/stop/frr/n}{409}
\defres{e2b_jevgym_meta_control/meta_shadow_s2lite/decisions/gold/probes/tool_select/by_d/2/far_ci/hi}{0.0854}
\defres{e2b_jevgym_meta_control/meta_shadow_s2lite/decisions/gold/probes/tool_select/by_d/2/far_ci/lo}{0.0285}
\defres{e2b_jevgym_meta_control/meta_shadow_s2lite/decisions/gold/probes/tool_select/by_d/3-4/far_ci/hi}{0.172}
\defres{e2b_jevgym_meta_control/meta_shadow_s2lite/decisions/gold/probes/tool_select/by_d/3-4/far_ci/lo}{0.11}
\defres{e2b_jevgym_meta_control/meta_shadow_s2lite/decisions/gold/probes/tool_select/by_d/5+/far_ci/hi}{0.127}
\defres{e2b_jevgym_meta_control/meta_shadow_s2lite/decisions/gold/probes/tool_select/by_d/5+/far_ci/lo}{0.0836}
\defres{e2b_jevgym_meta_control/meta_shadow_s2lite/decisions/gold/probes/tool_select/by_kind/detour/far_ci/hi}{0.157}
\defres{e2b_jevgym_meta_control/meta_shadow_s2lite/decisions/gold/probes/tool_select/by_kind/detour/far_ci/lo}{0.113}
\defres{e2b_jevgym_meta_control/meta_shadow_s2lite/decisions/gold/probes/tool_select/by_kind/fatal/far_ci/hi}{0.0796}
\defres{e2b_jevgym_meta_control/meta_shadow_s2lite/decisions/gold/probes/tool_select/by_kind/fatal/far_ci/lo}{0.0371}
\defres{e2b_jevgym_meta_control/meta_shadow_s2lite/decisions/gold/probes/tool_select/by_kind/progress/frr_ci/hi}{0.0166}
\defres{e2b_jevgym_meta_control/meta_shadow_s2lite/decisions/gold/probes/tool_select/by_kind/progress/frr_ci/lo}{0.00886}
\defres{e2b_jevgym_meta_control/meta_shadow_s2lite/decisions/gold/probes/tool_select/by_operator/T1/far_ci/hi}{0.153}
\defres{e2b_jevgym_meta_control/meta_shadow_s2lite/decisions/gold/probes/tool_select/by_operator/T1/far_ci/lo}{0.106}
\defres{e2b_jevgym_meta_control/meta_shadow_s2lite/decisions/gold/probes/tool_select/by_operator/T2/far_ci/hi}{0}
\defres{e2b_jevgym_meta_control/meta_shadow_s2lite/decisions/gold/probes/tool_select/by_operator/T2/far_ci/lo}{0}
\defres{e2b_jevgym_meta_control/meta_shadow_s2lite/decisions/gold/probes/tool_select/by_operator/T3/far_ci/hi}{0.092}
\defres{e2b_jevgym_meta_control/meta_shadow_s2lite/decisions/gold/probes/tool_select/by_operator/T3/far_ci/lo}{0.0438}
\defres{e2b_jevgym_meta_control/meta_shadow_s2lite/decisions/gold/probes/tool_select/by_operator/T4/far_ci/hi}{0.203}
\defres{e2b_jevgym_meta_control/meta_shadow_s2lite/decisions/gold/probes/tool_select/by_operator/T4/far_ci/lo}{0.0345}
\defres{e2b_jevgym_meta_control/meta_shadow_s2lite/decisions/gold/probes/tool_select/by_source/edit/far_ci/hi}{0.108}
\defres{e2b_jevgym_meta_control/meta_shadow_s2lite/decisions/gold/probes/tool_select/by_source/edit/far_ci/lo}{0.0762}
\defres{e2b_jevgym_meta_control/meta_shadow_s2lite/decisions/gold/probes/tool_select/by_source/natural/far_ci/hi}{0.821}
\defres{e2b_jevgym_meta_control/meta_shadow_s2lite/decisions/gold/probes/tool_select/by_source/natural/far_ci/lo}{0.514}
\defres{e2b_jevgym_meta_control/meta_shadow_s2lite/decisions/gold/probes/tool_select/by_source/natural/frr_ci/hi}{0.0177}
\defres{e2b_jevgym_meta_control/meta_shadow_s2lite/decisions/gold/probes/tool_select/by_source/natural/frr_ci/lo}{0.00954}
\defres{e2b_jevgym_meta_control/meta_shadow_s2lite/decisions/gold/probes/tool_select/by_source/transplant/far_ci/hi}{1}
\defres{e2b_jevgym_meta_control/meta_shadow_s2lite/decisions/gold/probes/tool_select/by_source/transplant/far_ci/lo}{0.429}
\defres{e2b_jevgym_meta_control/meta_shadow_s2lite/decisions/gold/probes/tool_select/by_source/transplant/frr_ci/hi}{0.0167}
\defres{e2b_jevgym_meta_control/meta_shadow_s2lite/decisions/gold/probes/tool_select/by_source/transplant/frr_ci/lo}{0.00359}
\defres{e2b_jevgym_meta_control/meta_shadow_s2lite/decisions/gold/probes/tool_select/far_fatal/far}{5.7}
\defres{e2b_jevgym_meta_control/meta_shadow_s2lite/decisions/gold/probes/tool_select/far_fatal/far_ci/hi}{0.0796}
\defres{e2b_jevgym_meta_control/meta_shadow_s2lite/decisions/gold/probes/tool_select/far_fatal/far_ci/lo}{0.0371}
\defres{e2b_jevgym_meta_control/meta_shadow_s2lite/decisions/gold/probes/tool_select/far_fatal/n}{470}
\defres{e2b_jevgym_meta_control/meta_shadow_s2lite/decisions/gold/probes/tool_select/headline/far}{67.4}
\defres{e2b_jevgym_meta_control/meta_shadow_s2lite/decisions/gold/probes/tool_select/headline/far_ci/hi}{0.826}
\defres{e2b_jevgym_meta_control/meta_shadow_s2lite/decisions/gold/probes/tool_select/headline/far_ci/lo}{0.513}
\defres{e2b_jevgym_meta_control/meta_shadow_s2lite/decisions/gold/probes/tool_select/headline/frr}{1.3}
\defres{e2b_jevgym_meta_control/meta_shadow_s2lite/decisions/gold/probes/tool_select/headline/frr_ci/hi}{0.0166}
\defres{e2b_jevgym_meta_control/meta_shadow_s2lite/decisions/gold/probes/tool_select/headline/frr_ci/lo}{0.00886}
\defres{e2b_jevgym_meta_control/meta_shadow_s2lite/decisions/gold/probes/tool_select/headline/n_right}{4078}
\defres{e2b_jevgym_meta_control/meta_shadow_s2lite/decisions/gold/probes/tool_select/headline/n_wrong}{43}
\defres{e2b_jevgym_meta_control/meta_shadow_s2lite/decisions/noul/ece}{0.171}
\defres{e2b_jevgym_meta_control/meta_shadow_s2lite/llm_calls}{7.57}
\defres{e2b_jevgym_meta_control/meta_shadow_s2lite/steps}{7.57}
\defres{e2b_jevgym_meta_control/meta_shadow_s2lite/success}{81.8}
\defres{e2b_jevgym_meta_control/meta_shadow_s2lite/success_ci/hi}{85.2}
\defres{e2b_jevgym_meta_control/meta_shadow_s2lite/success_ci/lo}{78.4}
\defres{e2b_jevgym_meta_control/meta_shadow_s2lite/vs_baseline/cost_savings}{0.1}
\defres{e2b_jevgym_meta_control/meta_shadow_s2lite/vs_baseline/delta}{+1.4}
\defres{e2b_jevgym_meta_control/meta_shadow_s2lite/vs_baseline/delta_ci/hi}{+3.4}
\defres{e2b_jevgym_meta_control/meta_shadow_s2lite/vs_baseline/delta_ci/lo}{-0.6}
\defres{e2b_jevgym_meta_control/meta_shadow_s2lite/vs_baseline/ni/p_decisive}{$<$0.001}
\defres{e2b_jevgym_meta_control/reflect_always/cost_usd}{0.0731}
\defres{e2b_jevgym_meta_control/reflect_always/llm_calls}{14.98}
\defres{e2b_jevgym_meta_control/reflect_always/steps}{7.99}
\defres{e2b_jevgym_meta_control/reflect_always/success}{96.0}
\defres{e2b_jevgym_meta_control/reflect_always/success_ci/hi}{98.5}
\defres{e2b_jevgym_meta_control/reflect_always/success_ci/lo}{93.0}
\defres{e2b_jevgym_meta_control/reflect_always/vs_baseline/cost_savings}{-80.0}
\defres{e2b_jevgym_meta_control/reflect_always/vs_baseline/delta}{-4.0}
\defres{e2b_jevgym_meta_control/reflect_always/vs_baseline/delta_ci/hi}{-1.5}
\defres{e2b_jevgym_meta_control/reflect_always/vs_baseline/delta_ci/lo}{-7.0}
\defres{e2b_jevgym_meta_control/reflect_always/vs_baseline/ni/p_decisive}{0.856}
\defres{e2b_jevgym_meta_control/reflect_always_s2lite/cost_usd}{0.0143}
\defres{e2b_jevgym_meta_control/reflect_always_s2lite/llm_calls}{14.12}
\defres{e2b_jevgym_meta_control/reflect_always_s2lite/steps}{7.56}
\defres{e2b_jevgym_meta_control/reflect_always_s2lite/success}{89.5}
\defres{e2b_jevgym_meta_control/reflect_always_s2lite/success_ci/hi}{93.5}
\defres{e2b_jevgym_meta_control/reflect_always_s2lite/success_ci/lo}{85.0}
\defres{e2b_jevgym_meta_control/reflect_always_s2lite/vs_baseline/cost_savings}{-46.4}
\defres{e2b_jevgym_meta_control/reflect_always_s2lite/vs_baseline/delta}{+8.5}
\defres{e2b_jevgym_meta_control/reflect_always_s2lite/vs_baseline/delta_ci/hi}{+13.0}
\defres{e2b_jevgym_meta_control/reflect_always_s2lite/vs_baseline/delta_ci/lo}{+4.0}
\defres{e2b_jevgym_meta_control/reflect_always_s2lite/vs_baseline/ni/p_decisive}{$<$0.001}
\defres{e2b_jevgym_meta_control/small_only/cost_usd}{0.00981}
\defres{e2b_jevgym_meta_control/small_only/llm_calls}{7.57}
\defres{e2b_jevgym_meta_control/small_only/steps}{7.57}
\defres{e2b_jevgym_meta_control/small_only/success}{80.8}
\defres{e2b_jevgym_meta_control/small_only/success_ci/hi}{84.2}
\defres{e2b_jevgym_meta_control/small_only/success_ci/lo}{77.4}
\defres{e2b_jevgym_meta_control/small_only/vs_baseline/cost_savings}{-0.0}
\defres{e2b_jevgym_meta_control/small_only/vs_baseline/delta}{+0.4}
\defres{e2b_jevgym_meta_control/small_only/vs_baseline/delta_ci/hi}{+2.2}
\defres{e2b_jevgym_meta_control/small_only/vs_baseline/delta_ci/lo}{-1.6}
\defres{e2b_jevgym_meta_control/small_only/vs_baseline/ni/p_decisive}{0.001}
\defres{e2c_jevgym_baselines/bm25_ts_assist_k3/cost_usd}{0.0161}
\defres{e2c_jevgym_baselines/bm25_ts_assist_k3/decisions/ece}{0.808}
\defres{e2c_jevgym_baselines/bm25_ts_assist_k3/llm_calls}{7.82}
\defres{e2c_jevgym_baselines/bm25_ts_assist_k3/steps}{7.82}
\defres{e2c_jevgym_baselines/bm25_ts_assist_k3/success}{18.8}
\defres{e2c_jevgym_baselines/bm25_ts_assist_k3/success_ci/hi}{22.2}
\defres{e2c_jevgym_baselines/bm25_ts_assist_k3/success_ci/lo}{15.4}
\defres{e2c_jevgym_baselines/bm25_ts_assist_k3/vs_baseline/cost_savings}{62.7}
\defres{e2c_jevgym_baselines/bm25_ts_assist_k3/vs_baseline/delta}{-83.0}
\defres{e2c_jevgym_baselines/bm25_ts_assist_k3/vs_baseline/delta_ci/hi}{-77.5}
\defres{e2c_jevgym_baselines/bm25_ts_assist_k3/vs_baseline/delta_ci/lo}{-88.0}
\defres{e2c_jevgym_baselines/bm25_ts_assist_k3/vs_baseline/ni/p_decisive}{1.000}
\defres{e2c_jevgym_baselines/bm25_ts_assist_k5/cost_usd}{0.0163}
\defres{e2c_jevgym_baselines/bm25_ts_assist_k5/decisions/ece}{0.811}
\defres{e2c_jevgym_baselines/bm25_ts_assist_k5/llm_calls}{7.48}
\defres{e2c_jevgym_baselines/bm25_ts_assist_k5/steps}{7.48}
\defres{e2c_jevgym_baselines/bm25_ts_assist_k5/success}{18.5}
\defres{e2c_jevgym_baselines/bm25_ts_assist_k5/success_ci/hi}{24.0}
\defres{e2c_jevgym_baselines/bm25_ts_assist_k5/success_ci/lo}{13.5}
\defres{e2c_jevgym_baselines/bm25_ts_assist_k5/vs_baseline/cost_savings}{60.1}
\defres{e2c_jevgym_baselines/bm25_ts_assist_k5/vs_baseline/delta}{-81.5}
\defres{e2c_jevgym_baselines/bm25_ts_assist_k5/vs_baseline/delta_ci/hi}{-76.0}
\defres{e2c_jevgym_baselines/bm25_ts_assist_k5/vs_baseline/delta_ci/lo}{-86.5}
\defres{e2c_jevgym_baselines/bm25_ts_assist_k5/vs_baseline/ni/p_decisive}{1.000}
\defres{e2c_jevgym_baselines/bm25_ts_replace/cost_usd}{0.015}
\defres{e2c_jevgym_baselines/bm25_ts_replace/decisions/ece}{0.801}
\defres{e2c_jevgym_baselines/bm25_ts_replace/llm_calls}{8.73}
\defres{e2c_jevgym_baselines/bm25_ts_replace/steps}{8.73}
\defres{e2c_jevgym_baselines/bm25_ts_replace/success}{12.5}
\defres{e2c_jevgym_baselines/bm25_ts_replace/success_ci/hi}{17.5}
\defres{e2c_jevgym_baselines/bm25_ts_replace/success_ci/lo}{8.0}
\defres{e2c_jevgym_baselines/bm25_ts_replace/vs_baseline/cost_savings}{63.3}
\defres{e2c_jevgym_baselines/bm25_ts_replace/vs_baseline/delta}{-87.5}
\defres{e2c_jevgym_baselines/bm25_ts_replace/vs_baseline/delta_ci/hi}{-82.5}
\defres{e2c_jevgym_baselines/bm25_ts_replace/vs_baseline/delta_ci/lo}{-92.0}
\defres{e2c_jevgym_baselines/bm25_ts_replace/vs_baseline/ni/p_decisive}{1.000}
\defres{e2c_jevgym_baselines/bm25task_ts_assist_k3/cost_usd}{0.015}
\defres{e2c_jevgym_baselines/bm25task_ts_assist_k3/decisions/ece}{0.722}
\defres{e2c_jevgym_baselines/bm25task_ts_assist_k3/llm_calls}{8.79}
\defres{e2c_jevgym_baselines/bm25task_ts_assist_k3/steps}{8.79}
\defres{e2c_jevgym_baselines/bm25task_ts_assist_k3/success}{24.5}
\defres{e2c_jevgym_baselines/bm25task_ts_assist_k3/success_ci/hi}{30.5}
\defres{e2c_jevgym_baselines/bm25task_ts_assist_k3/success_ci/lo}{18.5}
\defres{e2c_jevgym_baselines/bm25task_ts_assist_k3/vs_baseline/cost_savings}{63.5}
\defres{e2c_jevgym_baselines/bm25task_ts_assist_k3/vs_baseline/delta}{-75.5}
\defres{e2c_jevgym_baselines/bm25task_ts_assist_k3/vs_baseline/delta_ci/hi}{-69.5}
\defres{e2c_jevgym_baselines/bm25task_ts_assist_k3/vs_baseline/delta_ci/lo}{-81.0}
\defres{e2c_jevgym_baselines/bm25task_ts_assist_k3/vs_baseline/ni/p_decisive}{1.000}
\defres{e2c_jevgym_baselines/embed_ts_assist_k3/cost_usd}{0.00975}
\defres{e2c_jevgym_baselines/embed_ts_assist_k3/decisions/ece}{0.153}
\defres{e2c_jevgym_baselines/embed_ts_assist_k3/llm_calls}{5.03}
\defres{e2c_jevgym_baselines/embed_ts_assist_k3/steps}{5.03}
\defres{e2c_jevgym_baselines/embed_ts_assist_k3/success}{30.0}
\defres{e2c_jevgym_baselines/embed_ts_assist_k3/success_ci/hi}{36.5}
\defres{e2c_jevgym_baselines/embed_ts_assist_k3/success_ci/lo}{23.5}
\defres{e2c_jevgym_baselines/embed_ts_assist_k3/vs_baseline/cost_savings}{76.2}
\defres{e2c_jevgym_baselines/embed_ts_assist_k3/vs_baseline/delta}{-70.0}
\defres{e2c_jevgym_baselines/embed_ts_assist_k3/vs_baseline/delta_ci/hi}{-63.5}
\defres{e2c_jevgym_baselines/embed_ts_assist_k3/vs_baseline/delta_ci/lo}{-76.0}
\defres{e2c_jevgym_baselines/embed_ts_assist_k3/vs_baseline/ni/p_decisive}{1.000}
\defres{e2c_jevgym_baselines/embed_ts_replace/cost_usd}{0.00871}
\defres{e2c_jevgym_baselines/embed_ts_replace/decisions/ece}{0.432}
\defres{e2c_jevgym_baselines/embed_ts_replace/llm_calls}{4.29}
\defres{e2c_jevgym_baselines/embed_ts_replace/steps}{4.29}
\defres{e2c_jevgym_baselines/embed_ts_replace/success}{0.0}
\defres{e2c_jevgym_baselines/embed_ts_replace/success_ci/hi}{0.0}
\defres{e2c_jevgym_baselines/embed_ts_replace/success_ci/lo}{0.0}
\defres{e2c_jevgym_baselines/embed_ts_replace/vs_baseline/cost_savings}{78.7}
\defres{e2c_jevgym_baselines/embed_ts_replace/vs_baseline/delta}{-100.0}
\defres{e2c_jevgym_baselines/embed_ts_replace/vs_baseline/delta_ci/hi}{-100.0}
\defres{e2c_jevgym_baselines/embed_ts_replace/vs_baseline/delta_ci/lo}{-100.0}
\defres{e2c_jevgym_baselines/embed_ts_replace/vs_baseline/ni/p_decisive}{1.000}
\defres{e2c_jevgym_baselines/headline/iso_cost/delta_ci/hi}{+0.0}
\defres{e2c_jevgym_baselines/headline/iso_cost/delta_ci/lo}{+0.0}
\defres{e2c_jevgym_baselines/headline/iso_cost/success}{100.0}
\defres{e2c_jevgym_baselines/headline/iso_cost_by_reference/llm_only_s2lite/delta_ci/hi}{+9.0}
\defres{e2c_jevgym_baselines/headline/iso_cost_by_reference/llm_only_s2lite/delta_ci/lo}{+1.5}
\defres{e2c_jevgym_baselines/headline/iso_cost_by_reference/llm_only_s2lite/success}{86.5}
\defres{e2c_jevgym_baselines/headline/iso_quality/cost_savings_ci/hi}{1.8}
\defres{e2c_jevgym_baselines/headline/iso_quality/cost_savings_ci/lo}{0.4}
\defres{e2c_jevgym_baselines/headline/iso_quality/delta_ci/hi}{+0.0}
\defres{e2c_jevgym_baselines/headline/iso_quality/delta_ci/lo}{+0.0}
\defres{e2c_jevgym_baselines/headline/iso_quality_by_reference/llm_only_s2lite/cost_savings_ci/hi}{0.3}
\defres{e2c_jevgym_baselines/headline/iso_quality_by_reference/llm_only_s2lite/cost_savings_ci/lo}{-0.5}
\defres{e2c_jevgym_baselines/headline/iso_quality_by_reference/llm_only_s2lite/delta_ci/hi}{+9.0}
\defres{e2c_jevgym_baselines/headline/iso_quality_by_reference/llm_only_s2lite/delta_ci/lo}{+1.5}
\defres{e2c_jevgym_baselines/heuristic_memw/cost_usd}{0.0517}
\defres{e2c_jevgym_baselines/heuristic_memw/decisions/noul/ece}{0.351}
\defres{e2c_jevgym_baselines/heuristic_memw/llm_calls}{7.64}
\defres{e2c_jevgym_baselines/heuristic_memw/steps}{7.64}
\defres{e2c_jevgym_baselines/heuristic_memw/success}{97.5}
\defres{e2c_jevgym_baselines/heuristic_memw/success_ci/hi}{99.5}
\defres{e2c_jevgym_baselines/heuristic_memw/success_ci/lo}{95.0}
\defres{e2c_jevgym_baselines/heuristic_memw/vs_baseline/cost_savings}{-26.3}
\defres{e2c_jevgym_baselines/heuristic_memw/vs_baseline/delta}{-2.5}
\defres{e2c_jevgym_baselines/heuristic_memw/vs_baseline/delta_ci/hi}{-0.5}
\defres{e2c_jevgym_baselines/heuristic_memw/vs_baseline/delta_ci/lo}{-5.0}
\defres{e2c_jevgym_baselines/heuristic_memw/vs_baseline/ni/p_decisive}{0.459}
\defres{e2c_jevgym_baselines/heuristic_reflect_trigger/cost_usd}{0.0407}
\defres{e2c_jevgym_baselines/heuristic_reflect_trigger/decisions/noul/ece}{0.010}
\defres{e2c_jevgym_baselines/heuristic_reflect_trigger/llm_calls}{7.51}
\defres{e2c_jevgym_baselines/heuristic_reflect_trigger/steps}{7.50}
\defres{e2c_jevgym_baselines/heuristic_reflect_trigger/success}{100.0}
\defres{e2c_jevgym_baselines/heuristic_reflect_trigger/success_ci/hi}{100.0}
\defres{e2c_jevgym_baselines/heuristic_reflect_trigger/success_ci/lo}{100.0}
\defres{e2c_jevgym_baselines/heuristic_reflect_trigger/vs_baseline/cost_savings}{0.6}
\defres{e2c_jevgym_baselines/heuristic_reflect_trigger/vs_baseline/delta}{+0.0}
\defres{e2c_jevgym_baselines/heuristic_reflect_trigger/vs_baseline/delta_ci/hi}{+0.0}
\defres{e2c_jevgym_baselines/heuristic_reflect_trigger/vs_baseline/delta_ci/lo}{+0.0}
\defres{e2c_jevgym_baselines/heuristic_reflect_trigger/vs_baseline/ni/p_decisive}{0.002}
\defres{e2c_jevgym_baselines/heuristic_reflect_trigger_s2lite/cost_usd}{0.00974}
\defres{e2c_jevgym_baselines/heuristic_reflect_trigger_s2lite/decisions/noul/ece}{0.017}
\defres{e2c_jevgym_baselines/heuristic_reflect_trigger_s2lite/llm_calls}{7.56}
\defres{e2c_jevgym_baselines/heuristic_reflect_trigger_s2lite/steps}{7.55}
\defres{e2c_jevgym_baselines/heuristic_reflect_trigger_s2lite/success}{83.0}
\defres{e2c_jevgym_baselines/heuristic_reflect_trigger_s2lite/success_ci/hi}{88.0}
\defres{e2c_jevgym_baselines/heuristic_reflect_trigger_s2lite/success_ci/lo}{77.5}
\defres{e2c_jevgym_baselines/heuristic_reflect_trigger_s2lite/vs_baseline/cost_savings}{-0.3}
\defres{e2c_jevgym_baselines/heuristic_reflect_trigger_s2lite/vs_baseline/delta}{+1.5}
\defres{e2c_jevgym_baselines/heuristic_reflect_trigger_s2lite/vs_baseline/delta_ci/hi}{+4.5}
\defres{e2c_jevgym_baselines/heuristic_reflect_trigger_s2lite/vs_baseline/delta_ci/lo}{-1.5}
\defres{e2c_jevgym_baselines/heuristic_reflect_trigger_s2lite/vs_baseline/ni/p_decisive}{0.005}
\defres{e2c_jevgym_baselines/heuristic_route/cost_usd}{0.00983}
\defres{e2c_jevgym_baselines/heuristic_route/decisions/noul/ece}{0.012}
\defres{e2c_jevgym_baselines/heuristic_route/llm_calls}{7.57}
\defres{e2c_jevgym_baselines/heuristic_route/steps}{7.57}
\defres{e2c_jevgym_baselines/heuristic_route/success}{83.5}
\defres{e2c_jevgym_baselines/heuristic_route/success_ci/hi}{88.5}
\defres{e2c_jevgym_baselines/heuristic_route/success_ci/lo}{78.5}
\defres{e2c_jevgym_baselines/heuristic_route/vs_baseline/cost_savings}{76.0}
\defres{e2c_jevgym_baselines/heuristic_route/vs_baseline/delta}{-16.5}
\defres{e2c_jevgym_baselines/heuristic_route/vs_baseline/delta_ci/hi}{-11.5}
\defres{e2c_jevgym_baselines/heuristic_route/vs_baseline/delta_ci/lo}{-21.5}
\defres{e2c_jevgym_baselines/heuristic_route/vs_baseline/ni/p_decisive}{1.000}
\defres{e2c_jevgym_baselines/heuristic_stop_guard/cost_usd}{0.0405}
\defres{e2c_jevgym_baselines/heuristic_stop_guard/decisions/noul/ece}{0.010}
\defres{e2c_jevgym_baselines/heuristic_stop_guard/llm_calls}{7.50}
\defres{e2c_jevgym_baselines/heuristic_stop_guard/steps}{7.50}
\defres{e2c_jevgym_baselines/heuristic_stop_guard/success}{100.0}
\defres{e2c_jevgym_baselines/heuristic_stop_guard/success_ci/hi}{100.0}
\defres{e2c_jevgym_baselines/heuristic_stop_guard/success_ci/lo}{100.0}
\defres{e2c_jevgym_baselines/heuristic_stop_guard/vs_baseline/cost_savings}{1.1}
\defres{e2c_jevgym_baselines/heuristic_stop_guard/vs_baseline/delta}{+0.0}
\defres{e2c_jevgym_baselines/heuristic_stop_guard/vs_baseline/delta_ci/hi}{+0.0}
\defres{e2c_jevgym_baselines/heuristic_stop_guard/vs_baseline/delta_ci/lo}{+0.0}
\defres{e2c_jevgym_baselines/heuristic_stop_guard/vs_baseline/ni/p_decisive}{0.002}
\defres{e2c_jevgym_baselines/heuristic_stop_guard_s2lite/cost_usd}{0.00972}
\defres{e2c_jevgym_baselines/heuristic_stop_guard_s2lite/decisions/noul/ece}{0.125}
\defres{e2c_jevgym_baselines/heuristic_stop_guard_s2lite/llm_calls}{7.55}
\defres{e2c_jevgym_baselines/heuristic_stop_guard_s2lite/steps}{7.55}
\defres{e2c_jevgym_baselines/heuristic_stop_guard_s2lite/success}{86.5}
\defres{e2c_jevgym_baselines/heuristic_stop_guard_s2lite/success_ci/hi}{91.0}
\defres{e2c_jevgym_baselines/heuristic_stop_guard_s2lite/success_ci/lo}{81.5}
\defres{e2c_jevgym_baselines/heuristic_stop_guard_s2lite/vs_baseline/cost_savings}{-0.1}
\defres{e2c_jevgym_baselines/heuristic_stop_guard_s2lite/vs_baseline/delta}{+5.0}
\defres{e2c_jevgym_baselines/heuristic_stop_guard_s2lite/vs_baseline/delta_ci/hi}{+9.0}
\defres{e2c_jevgym_baselines/heuristic_stop_guard_s2lite/vs_baseline/delta_ci/lo}{+1.5}
\defres{e2c_jevgym_baselines/heuristic_stop_guard_s2lite/vs_baseline/ni/p_decisive}{$<$0.001}
\defres{e2c_jevgym_baselines/heuristic_stop_trigger/cost_usd}{0.0311}
\defres{e2c_jevgym_baselines/heuristic_stop_trigger/decisions/noul/ece}{0.107}
\defres{e2c_jevgym_baselines/heuristic_stop_trigger/llm_calls}{6.04}
\defres{e2c_jevgym_baselines/heuristic_stop_trigger/steps}{5.54}
\defres{e2c_jevgym_baselines/heuristic_stop_trigger/success}{50.0}
\defres{e2c_jevgym_baselines/heuristic_stop_trigger/success_ci/hi}{56.5}
\defres{e2c_jevgym_baselines/heuristic_stop_trigger/success_ci/lo}{43.0}
\defres{e2c_jevgym_baselines/heuristic_stop_trigger/vs_baseline/cost_savings}{24.1}
\defres{e2c_jevgym_baselines/heuristic_stop_trigger/vs_baseline/delta}{-50.0}
\defres{e2c_jevgym_baselines/heuristic_stop_trigger/vs_baseline/delta_ci/hi}{-43.0}
\defres{e2c_jevgym_baselines/heuristic_stop_trigger/vs_baseline/delta_ci/lo}{-56.5}
\defres{e2c_jevgym_baselines/heuristic_stop_trigger/vs_baseline/ni/p_decisive}{1.000}
\defres{e2c_jevgym_baselines/heuristic_ts_assist_k3/cost_usd}{0.0181}
\defres{e2c_jevgym_baselines/heuristic_ts_assist_k3/decisions/ece}{0.884}
\defres{e2c_jevgym_baselines/heuristic_ts_assist_k3/llm_calls}{9.35}
\defres{e2c_jevgym_baselines/heuristic_ts_assist_k3/steps}{9.35}
\defres{e2c_jevgym_baselines/heuristic_ts_assist_k3/success}{31.0}
\defres{e2c_jevgym_baselines/heuristic_ts_assist_k3/success_ci/hi}{38.0}
\defres{e2c_jevgym_baselines/heuristic_ts_assist_k3/success_ci/lo}{24.5}
\defres{e2c_jevgym_baselines/heuristic_ts_assist_k3/vs_baseline/cost_savings}{55.8}
\defres{e2c_jevgym_baselines/heuristic_ts_assist_k3/vs_baseline/delta}{-69.0}
\defres{e2c_jevgym_baselines/heuristic_ts_assist_k3/vs_baseline/delta_ci/hi}{-62.5}
\defres{e2c_jevgym_baselines/heuristic_ts_assist_k3/vs_baseline/delta_ci/lo}{-75.0}
\defres{e2c_jevgym_baselines/heuristic_ts_assist_k3/vs_baseline/ni/p_decisive}{1.000}
\defres{e2c_jevgym_baselines/heuristic_ts_replace/cost_usd}{0.00175}
\defres{e2c_jevgym_baselines/heuristic_ts_replace/decisions/ece}{0.637}
\defres{e2c_jevgym_baselines/heuristic_ts_replace/llm_calls}{2.12}
\defres{e2c_jevgym_baselines/heuristic_ts_replace/steps}{2.12}
\defres{e2c_jevgym_baselines/heuristic_ts_replace/success}{12.5}
\defres{e2c_jevgym_baselines/heuristic_ts_replace/success_ci/hi}{17.5}
\defres{e2c_jevgym_baselines/heuristic_ts_replace/success_ci/lo}{8.0}
\defres{e2c_jevgym_baselines/heuristic_ts_replace/vs_baseline/cost_savings}{95.7}
\defres{e2c_jevgym_baselines/heuristic_ts_replace/vs_baseline/delta}{-87.5}
\defres{e2c_jevgym_baselines/heuristic_ts_replace/vs_baseline/delta_ci/hi}{-82.5}
\defres{e2c_jevgym_baselines/heuristic_ts_replace/vs_baseline/delta_ci/lo}{-92.0}
\defres{e2c_jevgym_baselines/heuristic_ts_replace/vs_baseline/ni/p_decisive}{1.000}
\defres{e2c_jevgym_baselines/jev_memw/cost_usd}{0.0569}
\defres{e2c_jevgym_baselines/jev_memw/decisions/noul/ece}{0.267}
\defres{e2c_jevgym_baselines/jev_memw/llm_calls}{7.55}
\defres{e2c_jevgym_baselines/jev_memw/steps}{7.55}
\defres{e2c_jevgym_baselines/jev_memw/success}{99.0}
\defres{e2c_jevgym_baselines/jev_memw/success_ci/hi}{100.0}
\defres{e2c_jevgym_baselines/jev_memw/success_ci/lo}{97.5}
\defres{e2c_jevgym_baselines/jev_memw/vs_baseline/cost_savings}{-38.9}
\defres{e2c_jevgym_baselines/jev_memw/vs_baseline/delta}{-1.0}
\defres{e2c_jevgym_baselines/jev_memw/vs_baseline/delta_ci/hi}{+0.0}
\defres{e2c_jevgym_baselines/jev_memw/vs_baseline/delta_ci/lo}{-2.5}
\defres{e2c_jevgym_baselines/jev_memw/vs_baseline/ni/p_decisive}{0.059}
\defres{e2c_jevgym_baselines/jev_reflect_trigger/cost_usd}{0.0429}
\defres{e2c_jevgym_baselines/jev_reflect_trigger/decisions/noul/ece}{0.159}
\defres{e2c_jevgym_baselines/jev_reflect_trigger/llm_calls}{8.45}
\defres{e2c_jevgym_baselines/jev_reflect_trigger/steps}{7.53}
\defres{e2c_jevgym_baselines/jev_reflect_trigger/success}{100.0}
\defres{e2c_jevgym_baselines/jev_reflect_trigger/success_ci/hi}{100.0}
\defres{e2c_jevgym_baselines/jev_reflect_trigger/success_ci/lo}{100.0}
\defres{e2c_jevgym_baselines/jev_reflect_trigger/vs_baseline/cost_savings}{-4.8}
\defres{e2c_jevgym_baselines/jev_reflect_trigger/vs_baseline/delta}{+0.0}
\defres{e2c_jevgym_baselines/jev_reflect_trigger/vs_baseline/delta_ci/hi}{+0.0}
\defres{e2c_jevgym_baselines/jev_reflect_trigger/vs_baseline/delta_ci/lo}{+0.0}
\defres{e2c_jevgym_baselines/jev_reflect_trigger/vs_baseline/ni/p_decisive}{0.002}
\defres{e2c_jevgym_baselines/jev_reflect_trigger_s2lite/cost_usd}{0.00991}
\defres{e2c_jevgym_baselines/jev_reflect_trigger_s2lite/decisions/noul/ece}{0.206}
\defres{e2c_jevgym_baselines/jev_reflect_trigger_s2lite/llm_calls}{8.60}
\defres{e2c_jevgym_baselines/jev_reflect_trigger_s2lite/steps}{7.62}
\defres{e2c_jevgym_baselines/jev_reflect_trigger_s2lite/success}{83.0}
\defres{e2c_jevgym_baselines/jev_reflect_trigger_s2lite/success_ci/hi}{86.2}
\defres{e2c_jevgym_baselines/jev_reflect_trigger_s2lite/success_ci/lo}{79.8}
\defres{e2c_jevgym_baselines/jev_reflect_trigger_s2lite/vs_baseline/cost_savings}{-1.9}
\defres{e2c_jevgym_baselines/jev_reflect_trigger_s2lite/vs_baseline/delta}{+1.8}
\defres{e2c_jevgym_baselines/jev_reflect_trigger_s2lite/vs_baseline/delta_ci/hi}{+4.8}
\defres{e2c_jevgym_baselines/jev_reflect_trigger_s2lite/vs_baseline/delta_ci/lo}{-1.6}
\defres{e2c_jevgym_baselines/jev_reflect_trigger_s2lite/vs_baseline/ni/p_decisive}{0.002}
\defres{e2c_jevgym_baselines/jev_route_tau0.2/cost_usd}{0.0309}
\defres{e2c_jevgym_baselines/jev_route_tau0.2/decisions/noul/ece}{0.138}
\defres{e2c_jevgym_baselines/jev_route_tau0.2/llm_calls}{7.54}
\defres{e2c_jevgym_baselines/jev_route_tau0.2/steps}{7.54}
\defres{e2c_jevgym_baselines/jev_route_tau0.2/success}{96.0}
\defres{e2c_jevgym_baselines/jev_route_tau0.2/success_ci/hi}{98.5}
\defres{e2c_jevgym_baselines/jev_route_tau0.2/success_ci/lo}{93.0}
\defres{e2c_jevgym_baselines/jev_route_tau0.2/vs_baseline/cost_savings}{24.6}
\defres{e2c_jevgym_baselines/jev_route_tau0.2/vs_baseline/delta}{-4.0}
\defres{e2c_jevgym_baselines/jev_route_tau0.2/vs_baseline/delta_ci/hi}{-1.5}
\defres{e2c_jevgym_baselines/jev_route_tau0.2/vs_baseline/delta_ci/lo}{-7.0}
\defres{e2c_jevgym_baselines/jev_route_tau0.2/vs_baseline/ni/p_decisive}{0.856}
\defres{e2c_jevgym_baselines/jev_route_tau0.4/cost_usd}{0.0129}
\defres{e2c_jevgym_baselines/jev_route_tau0.4/decisions/noul/ece}{0.174}
\defres{e2c_jevgym_baselines/jev_route_tau0.4/llm_calls}{7.54}
\defres{e2c_jevgym_baselines/jev_route_tau0.4/steps}{7.54}
\defres{e2c_jevgym_baselines/jev_route_tau0.4/success}{83.0}
\defres{e2c_jevgym_baselines/jev_route_tau0.4/success_ci/hi}{88.0}
\defres{e2c_jevgym_baselines/jev_route_tau0.4/success_ci/lo}{77.5}
\defres{e2c_jevgym_baselines/jev_route_tau0.4/vs_baseline/cost_savings}{68.4}
\defres{e2c_jevgym_baselines/jev_route_tau0.4/vs_baseline/delta}{-17.0}
\defres{e2c_jevgym_baselines/jev_route_tau0.4/vs_baseline/delta_ci/hi}{-12.0}
\defres{e2c_jevgym_baselines/jev_route_tau0.4/vs_baseline/delta_ci/lo}{-22.0}
\defres{e2c_jevgym_baselines/jev_route_tau0.4/vs_baseline/ni/p_decisive}{1.000}
\defres{e2c_jevgym_baselines/jev_route_tau0.5/cost_usd}{0.0115}
\defres{e2c_jevgym_baselines/jev_route_tau0.5/decisions/noul/ece}{0.187}
\defres{e2c_jevgym_baselines/jev_route_tau0.5/llm_calls}{7.55}
\defres{e2c_jevgym_baselines/jev_route_tau0.5/steps}{7.55}
\defres{e2c_jevgym_baselines/jev_route_tau0.5/success}{84.5}
\defres{e2c_jevgym_baselines/jev_route_tau0.5/success_ci/hi}{89.5}
\defres{e2c_jevgym_baselines/jev_route_tau0.5/success_ci/lo}{79.5}
\defres{e2c_jevgym_baselines/jev_route_tau0.5/vs_baseline/cost_savings}{71.8}
\defres{e2c_jevgym_baselines/jev_route_tau0.5/vs_baseline/delta}{-15.5}
\defres{e2c_jevgym_baselines/jev_route_tau0.5/vs_baseline/delta_ci/hi}{-10.5}
\defres{e2c_jevgym_baselines/jev_route_tau0.5/vs_baseline/delta_ci/lo}{-20.5}
\defres{e2c_jevgym_baselines/jev_route_tau0.5/vs_baseline/ni/p_decisive}{1.000}
\defres{e2c_jevgym_baselines/jev_route_tau0.6/cost_usd}{0.0101}
\defres{e2c_jevgym_baselines/jev_route_tau0.6/decisions/noul/ece}{0.200}
\defres{e2c_jevgym_baselines/jev_route_tau0.6/llm_calls}{7.55}
\defres{e2c_jevgym_baselines/jev_route_tau0.6/steps}{7.55}
\defres{e2c_jevgym_baselines/jev_route_tau0.6/success}{82.0}
\defres{e2c_jevgym_baselines/jev_route_tau0.6/success_ci/hi}{87.0}
\defres{e2c_jevgym_baselines/jev_route_tau0.6/success_ci/lo}{76.5}
\defres{e2c_jevgym_baselines/jev_route_tau0.6/vs_baseline/cost_savings}{75.4}
\defres{e2c_jevgym_baselines/jev_route_tau0.6/vs_baseline/delta}{-18.0}
\defres{e2c_jevgym_baselines/jev_route_tau0.6/vs_baseline/delta_ci/hi}{-13.0}
\defres{e2c_jevgym_baselines/jev_route_tau0.6/vs_baseline/delta_ci/lo}{-23.0}
\defres{e2c_jevgym_baselines/jev_route_tau0.6/vs_baseline/ni/p_decisive}{1.000}
\defres{e2c_jevgym_baselines/jev_route_tau0.8/cost_usd}{0.0101}
\defres{e2c_jevgym_baselines/jev_route_tau0.8/decisions/noul/ece}{0.203}
\defres{e2c_jevgym_baselines/jev_route_tau0.8/llm_calls}{7.55}
\defres{e2c_jevgym_baselines/jev_route_tau0.8/steps}{7.55}
\defres{e2c_jevgym_baselines/jev_route_tau0.8/success}{84.0}
\defres{e2c_jevgym_baselines/jev_route_tau0.8/success_ci/hi}{89.0}
\defres{e2c_jevgym_baselines/jev_route_tau0.8/success_ci/lo}{79.0}
\defres{e2c_jevgym_baselines/jev_route_tau0.8/vs_baseline/cost_savings}{75.4}
\defres{e2c_jevgym_baselines/jev_route_tau0.8/vs_baseline/delta}{-16.0}
\defres{e2c_jevgym_baselines/jev_route_tau0.8/vs_baseline/delta_ci/hi}{-11.0}
\defres{e2c_jevgym_baselines/jev_route_tau0.8/vs_baseline/delta_ci/lo}{-21.0}
\defres{e2c_jevgym_baselines/jev_route_tau0.8/vs_baseline/ni/p_decisive}{1.000}
\defres{e2c_jevgym_baselines/jev_stop_guard/cost_usd}{0.0421}
\defres{e2c_jevgym_baselines/jev_stop_guard/decisions/noul/ece}{0.203}
\defres{e2c_jevgym_baselines/jev_stop_guard/llm_calls}{7.62}
\defres{e2c_jevgym_baselines/jev_stop_guard/steps}{7.62}
\defres{e2c_jevgym_baselines/jev_stop_guard/success}{100.0}
\defres{e2c_jevgym_baselines/jev_stop_guard/success_ci/hi}{100.0}
\defres{e2c_jevgym_baselines/jev_stop_guard/success_ci/lo}{100.0}
\defres{e2c_jevgym_baselines/jev_stop_guard/vs_baseline/cost_savings}{-2.9}
\defres{e2c_jevgym_baselines/jev_stop_guard/vs_baseline/delta}{+0.0}
\defres{e2c_jevgym_baselines/jev_stop_guard/vs_baseline/delta_ci/hi}{+0.0}
\defres{e2c_jevgym_baselines/jev_stop_guard/vs_baseline/delta_ci/lo}{+0.0}
\defres{e2c_jevgym_baselines/jev_stop_guard/vs_baseline/ni/p_decisive}{0.002}
\defres{e2c_jevgym_baselines/jev_stop_guard_s2lite/cost_usd}{0.012}
\defres{e2c_jevgym_baselines/jev_stop_guard_s2lite/decisions/noul/ece}{0.128}
\defres{e2c_jevgym_baselines/jev_stop_guard_s2lite/llm_calls}{9.23}
\defres{e2c_jevgym_baselines/jev_stop_guard_s2lite/steps}{9.23}
\defres{e2c_jevgym_baselines/jev_stop_guard_s2lite/success}{84.5}
\defres{e2c_jevgym_baselines/jev_stop_guard_s2lite/success_ci/hi}{89.0}
\defres{e2c_jevgym_baselines/jev_stop_guard_s2lite/success_ci/lo}{79.5}
\defres{e2c_jevgym_baselines/jev_stop_guard_s2lite/vs_baseline/cost_savings}{-23.8}
\defres{e2c_jevgym_baselines/jev_stop_guard_s2lite/vs_baseline/delta}{+3.0}
\defres{e2c_jevgym_baselines/jev_stop_guard_s2lite/vs_baseline/delta_ci/hi}{+7.0}
\defres{e2c_jevgym_baselines/jev_stop_guard_s2lite/vs_baseline/delta_ci/lo}{-0.5}
\defres{e2c_jevgym_baselines/jev_stop_guard_s2lite/vs_baseline/ni/p_decisive}{0.001}
\defres{e2c_jevgym_baselines/jev_stop_trigger/cost_usd}{0.0406}
\defres{e2c_jevgym_baselines/jev_stop_trigger/decisions/noul/ece}{0.029}
\defres{e2c_jevgym_baselines/jev_stop_trigger/llm_calls}{7.50}
\defres{e2c_jevgym_baselines/jev_stop_trigger/steps}{7.50}
\defres{e2c_jevgym_baselines/jev_stop_trigger/success}{100.0}
\defres{e2c_jevgym_baselines/jev_stop_trigger/success_ci/hi}{100.0}
\defres{e2c_jevgym_baselines/jev_stop_trigger/success_ci/lo}{100.0}
\defres{e2c_jevgym_baselines/jev_stop_trigger/vs_baseline/cost_savings}{0.8}
\defres{e2c_jevgym_baselines/jev_stop_trigger/vs_baseline/delta}{+0.0}
\defres{e2c_jevgym_baselines/jev_stop_trigger/vs_baseline/delta_ci/hi}{+0.0}
\defres{e2c_jevgym_baselines/jev_stop_trigger/vs_baseline/delta_ci/lo}{+0.0}
\defres{e2c_jevgym_baselines/jev_stop_trigger/vs_baseline/ni/p_decisive}{0.002}
\defres{e2c_jevgym_baselines/jev_ts_assist_k3/cost_usd}{0.0195}
\defres{e2c_jevgym_baselines/jev_ts_assist_k3/decisions/ece}{0.045}
\defres{e2c_jevgym_baselines/jev_ts_assist_k3/llm_calls}{8.10}
\defres{e2c_jevgym_baselines/jev_ts_assist_k3/steps}{8.10}
\defres{e2c_jevgym_baselines/jev_ts_assist_k3/success}{90.5}
\defres{e2c_jevgym_baselines/jev_ts_assist_k3/success_ci/hi}{94.5}
\defres{e2c_jevgym_baselines/jev_ts_assist_k3/success_ci/lo}{86.0}
\defres{e2c_jevgym_baselines/jev_ts_assist_k3/vs_baseline/cost_savings}{52.3}
\defres{e2c_jevgym_baselines/jev_ts_assist_k3/vs_baseline/delta}{-9.5}
\defres{e2c_jevgym_baselines/jev_ts_assist_k3/vs_baseline/delta_ci/hi}{-5.5}
\defres{e2c_jevgym_baselines/jev_ts_assist_k3/vs_baseline/delta_ci/lo}{-14.0}
\defres{e2c_jevgym_baselines/jev_ts_assist_k3/vs_baseline/ni/p_decisive}{1.000}
\defres{e2c_jevgym_baselines/jev_ts_assist_k5/cost_usd}{0.0224}
\defres{e2c_jevgym_baselines/jev_ts_assist_k5/decisions/ece}{0.047}
\defres{e2c_jevgym_baselines/jev_ts_assist_k5/llm_calls}{8.44}
\defres{e2c_jevgym_baselines/jev_ts_assist_k5/steps}{8.44}
\defres{e2c_jevgym_baselines/jev_ts_assist_k5/success}{92.0}
\defres{e2c_jevgym_baselines/jev_ts_assist_k5/success_ci/hi}{95.5}
\defres{e2c_jevgym_baselines/jev_ts_assist_k5/success_ci/lo}{88.0}
\defres{e2c_jevgym_baselines/jev_ts_assist_k5/vs_baseline/cost_savings}{45.2}
\defres{e2c_jevgym_baselines/jev_ts_assist_k5/vs_baseline/delta}{-8.0}
\defres{e2c_jevgym_baselines/jev_ts_assist_k5/vs_baseline/delta_ci/hi}{-4.5}
\defres{e2c_jevgym_baselines/jev_ts_assist_k5/vs_baseline/delta_ci/lo}{-12.0}
\defres{e2c_jevgym_baselines/jev_ts_assist_k5/vs_baseline/ni/p_decisive}{1.000}
\defres{e2c_jevgym_baselines/jev_ts_params_replace_answercopy/cost_usd}{0.00548}
\defres{e2c_jevgym_baselines/jev_ts_params_replace_answercopy/decisions/ece}{0.033}
\defres{e2c_jevgym_baselines/jev_ts_params_replace_answercopy/llm_calls}{1.91}
\defres{e2c_jevgym_baselines/jev_ts_params_replace_answercopy/steps}{7.61}
\defres{e2c_jevgym_baselines/jev_ts_params_replace_answercopy/success}{80.0}
\defres{e2c_jevgym_baselines/jev_ts_params_replace_answercopy/success_ci/hi}{85.5}
\defres{e2c_jevgym_baselines/jev_ts_params_replace_answercopy/success_ci/lo}{74.5}
\defres{e2c_jevgym_baselines/jev_ts_params_replace_answercopy/vs_baseline/cost_savings}{86.6}
\defres{e2c_jevgym_baselines/jev_ts_params_replace_answercopy/vs_baseline/delta}{-20.0}
\defres{e2c_jevgym_baselines/jev_ts_params_replace_answercopy/vs_baseline/delta_ci/hi}{-15.0}
\defres{e2c_jevgym_baselines/jev_ts_params_replace_answercopy/vs_baseline/delta_ci/lo}{-25.5}
\defres{e2c_jevgym_baselines/jev_ts_params_replace_answercopy/vs_baseline/ni/p_decisive}{1.000}
\defres{e2c_jevgym_baselines/jev_ts_replace/cost_usd}{0.0142}
\defres{e2c_jevgym_baselines/jev_ts_replace/decisions/ece}{0.031}
\defres{e2c_jevgym_baselines/jev_ts_replace/llm_calls}{6.88}
\defres{e2c_jevgym_baselines/jev_ts_replace/steps}{6.88}
\defres{e2c_jevgym_baselines/jev_ts_replace/success}{81.5}
\defres{e2c_jevgym_baselines/jev_ts_replace/success_ci/hi}{86.5}
\defres{e2c_jevgym_baselines/jev_ts_replace/success_ci/lo}{76.0}
\defres{e2c_jevgym_baselines/jev_ts_replace/vs_baseline/cost_savings}{65.4}
\defres{e2c_jevgym_baselines/jev_ts_replace/vs_baseline/delta}{-18.5}
\defres{e2c_jevgym_baselines/jev_ts_replace/vs_baseline/delta_ci/hi}{-13.0}
\defres{e2c_jevgym_baselines/jev_ts_replace/vs_baseline/delta_ci/lo}{-24.0}
\defres{e2c_jevgym_baselines/jev_ts_replace/vs_baseline/ni/p_decisive}{1.000}
\defres{e2c_jevgym_baselines/lite_route/cost_usd}{0.0142}
\defres{e2c_jevgym_baselines/lite_route/decisions/noul/ece}{0.027}
\defres{e2c_jevgym_baselines/lite_route/llm_calls}{7.55}
\defres{e2c_jevgym_baselines/lite_route/steps}{7.55}
\defres{e2c_jevgym_baselines/lite_route/success}{84.0}
\defres{e2c_jevgym_baselines/lite_route/success_ci/hi}{89.0}
\defres{e2c_jevgym_baselines/lite_route/success_ci/lo}{78.5}
\defres{e2c_jevgym_baselines/lite_route/vs_baseline/cost_savings}{65.2}
\defres{e2c_jevgym_baselines/lite_route/vs_baseline/delta}{-16.0}
\defres{e2c_jevgym_baselines/lite_route/vs_baseline/delta_ci/hi}{-11.0}
\defres{e2c_jevgym_baselines/lite_route/vs_baseline/delta_ci/lo}{-21.0}
\defres{e2c_jevgym_baselines/lite_route/vs_baseline/ni/p_decisive}{1.000}
\defres{e2c_jevgym_baselines/lite_ts_assist_k3/cost_usd}{0.0368}
\defres{e2c_jevgym_baselines/lite_ts_assist_k3/decisions/ece}{0.135}
\defres{e2c_jevgym_baselines/lite_ts_assist_k3/llm_calls}{7.57}
\defres{e2c_jevgym_baselines/lite_ts_assist_k3/steps}{7.57}
\defres{e2c_jevgym_baselines/lite_ts_assist_k3/success}{86.5}
\defres{e2c_jevgym_baselines/lite_ts_assist_k3/success_ci/hi}{91.0}
\defres{e2c_jevgym_baselines/lite_ts_assist_k3/success_ci/lo}{81.5}
\defres{e2c_jevgym_baselines/lite_ts_assist_k3/vs_baseline/cost_savings}{10.2}
\defres{e2c_jevgym_baselines/lite_ts_assist_k3/vs_baseline/delta}{-13.5}
\defres{e2c_jevgym_baselines/lite_ts_assist_k3/vs_baseline/delta_ci/hi}{-9.0}
\defres{e2c_jevgym_baselines/lite_ts_assist_k3/vs_baseline/delta_ci/lo}{-18.5}
\defres{e2c_jevgym_baselines/lite_ts_assist_k3/vs_baseline/ni/p_decisive}{1.000}
\defres{e2c_jevgym_baselines/lite_ts_replace/cost_usd}{0.0242}
\defres{e2c_jevgym_baselines/lite_ts_replace/decisions/ece}{0.163}
\defres{e2c_jevgym_baselines/lite_ts_replace/llm_calls}{5.67}
\defres{e2c_jevgym_baselines/lite_ts_replace/steps}{5.67}
\defres{e2c_jevgym_baselines/lite_ts_replace/success}{41.5}
\defres{e2c_jevgym_baselines/lite_ts_replace/success_ci/hi}{49.0}
\defres{e2c_jevgym_baselines/lite_ts_replace/success_ci/lo}{35.0}
\defres{e2c_jevgym_baselines/lite_ts_replace/vs_baseline/cost_savings}{40.9}
\defres{e2c_jevgym_baselines/lite_ts_replace/vs_baseline/delta}{-58.5}
\defres{e2c_jevgym_baselines/lite_ts_replace/vs_baseline/delta_ci/hi}{-52.0}
\defres{e2c_jevgym_baselines/lite_ts_replace/vs_baseline/delta_ci/lo}{-65.5}
\defres{e2c_jevgym_baselines/lite_ts_replace/vs_baseline/ni/p_decisive}{1.000}
\defres{e2c_jevgym_baselines/llm_only/cost_usd}{0.0409}
\defres{e2c_jevgym_baselines/llm_only/llm_calls}{7.50}
\defres{e2c_jevgym_baselines/llm_only/steps}{7.50}
\defres{e2c_jevgym_baselines/llm_only/success}{100.0}
\defres{e2c_jevgym_baselines/llm_only/success_ci/hi}{100.0}
\defres{e2c_jevgym_baselines/llm_only/success_ci/lo}{100.0}
\defres{e2c_jevgym_baselines/llm_only_s2lite/cost_usd}{0.00973}
\defres{e2c_jevgym_baselines/llm_only_s2lite/llm_calls}{7.57}
\defres{e2c_jevgym_baselines/llm_only_s2lite/steps}{7.57}
\defres{e2c_jevgym_baselines/llm_only_s2lite/success}{81.2}
\defres{e2c_jevgym_baselines/llm_only_s2lite/success_ci/hi}{84.6}
\defres{e2c_jevgym_baselines/llm_only_s2lite/success_ci/lo}{77.8}
\defres{e2c_jevgym_baselines/llm_only_s2lite/vs_baseline/cost_savings}{76.3}
\defres{e2c_jevgym_baselines/llm_only_s2lite/vs_baseline/delta}{-18.5}
\defres{e2c_jevgym_baselines/llm_only_s2lite/vs_baseline/delta_ci/hi}{-13.0}
\defres{e2c_jevgym_baselines/llm_only_s2lite/vs_baseline/delta_ci/lo}{-24.0}
\defres{e2c_jevgym_baselines/llm_only_s2lite/vs_baseline/ni/p_decisive}{1.000}
\defres{e2c_jevgym_baselines/prior_recent_ts_replace/cost_usd}{0.0404}
\defres{e2c_jevgym_baselines/prior_recent_ts_replace/decisions/ece}{0.990}
\defres{e2c_jevgym_baselines/prior_recent_ts_replace/llm_calls}{21.59}
\defres{e2c_jevgym_baselines/prior_recent_ts_replace/steps}{21.59}
\defres{e2c_jevgym_baselines/prior_recent_ts_replace/success}{0.0}
\defres{e2c_jevgym_baselines/prior_recent_ts_replace/success_ci/hi}{0.0}
\defres{e2c_jevgym_baselines/prior_recent_ts_replace/success_ci/lo}{0.0}
\defres{e2c_jevgym_baselines/prior_recent_ts_replace/vs_baseline/cost_savings}{1.3}
\defres{e2c_jevgym_baselines/prior_recent_ts_replace/vs_baseline/delta}{-100.0}
\defres{e2c_jevgym_baselines/prior_recent_ts_replace/vs_baseline/delta_ci/hi}{-100.0}
\defres{e2c_jevgym_baselines/prior_recent_ts_replace/vs_baseline/delta_ci/lo}{-100.0}
\defres{e2c_jevgym_baselines/prior_recent_ts_replace/vs_baseline/ni/p_decisive}{1.000}
\defres{e2c_jevgym_baselines/random_ts_assist_k3/cost_usd}{0.0358}
\defres{e2c_jevgym_baselines/random_ts_assist_k3/decisions/ece}{0.007}
\defres{e2c_jevgym_baselines/random_ts_assist_k3/llm_calls}{14.85}
\defres{e2c_jevgym_baselines/random_ts_assist_k3/steps}{14.85}
\defres{e2c_jevgym_baselines/random_ts_assist_k3/success}{6.0}
\defres{e2c_jevgym_baselines/random_ts_assist_k3/success_ci/hi}{9.5}
\defres{e2c_jevgym_baselines/random_ts_assist_k3/success_ci/lo}{3.0}
\defres{e2c_jevgym_baselines/random_ts_assist_k3/vs_baseline/cost_savings}{12.5}
\defres{e2c_jevgym_baselines/random_ts_assist_k3/vs_baseline/delta}{-94.0}
\defres{e2c_jevgym_baselines/random_ts_assist_k3/vs_baseline/delta_ci/hi}{-90.5}
\defres{e2c_jevgym_baselines/random_ts_assist_k3/vs_baseline/delta_ci/lo}{-97.0}
\defres{e2c_jevgym_baselines/random_ts_assist_k3/vs_baseline/ni/p_decisive}{1.000}
\defres{e2c_jevgym_baselines/random_ts_replace/cost_usd}{0.003}
\defres{e2c_jevgym_baselines/random_ts_replace/decisions/ece}{0.014}
\defres{e2c_jevgym_baselines/random_ts_replace/llm_calls}{3.33}
\defres{e2c_jevgym_baselines/random_ts_replace/steps}{3.33}
\defres{e2c_jevgym_baselines/random_ts_replace/success}{0.0}
\defres{e2c_jevgym_baselines/random_ts_replace/success_ci/hi}{0.0}
\defres{e2c_jevgym_baselines/random_ts_replace/success_ci/lo}{0.0}
\defres{e2c_jevgym_baselines/random_ts_replace/vs_baseline/cost_savings}{92.7}
\defres{e2c_jevgym_baselines/random_ts_replace/vs_baseline/delta}{-100.0}
\defres{e2c_jevgym_baselines/random_ts_replace/vs_baseline/delta_ci/hi}{-100.0}
\defres{e2c_jevgym_baselines/random_ts_replace/vs_baseline/delta_ci/lo}{-100.0}
\defres{e2c_jevgym_baselines/random_ts_replace/vs_baseline/ni/p_decisive}{1.000}
\defres{e2c_jevgym_baselines/randscore_route_tau0.2/cost_usd}{0.0338}
\defres{e2c_jevgym_baselines/randscore_route_tau0.2/decisions/noul/ece}{0.077}
\defres{e2c_jevgym_baselines/randscore_route_tau0.2/llm_calls}{7.53}
\defres{e2c_jevgym_baselines/randscore_route_tau0.2/steps}{7.53}
\defres{e2c_jevgym_baselines/randscore_route_tau0.2/success}{96.5}
\defres{e2c_jevgym_baselines/randscore_route_tau0.2/success_ci/hi}{99.0}
\defres{e2c_jevgym_baselines/randscore_route_tau0.2/success_ci/lo}{93.5}
\defres{e2c_jevgym_baselines/randscore_route_tau0.2/vs_baseline/cost_savings}{17.5}
\defres{e2c_jevgym_baselines/randscore_route_tau0.2/vs_baseline/delta}{-3.5}
\defres{e2c_jevgym_baselines/randscore_route_tau0.2/vs_baseline/delta_ci/hi}{-1.0}
\defres{e2c_jevgym_baselines/randscore_route_tau0.2/vs_baseline/delta_ci/lo}{-6.0}
\defres{e2c_jevgym_baselines/randscore_route_tau0.2/vs_baseline/ni/p_decisive}{0.747}
\defres{e2c_jevgym_baselines/randscore_route_tau0.4/cost_usd}{0.0289}
\defres{e2c_jevgym_baselines/randscore_route_tau0.4/decisions/noul/ece}{0.180}
\defres{e2c_jevgym_baselines/randscore_route_tau0.4/llm_calls}{7.53}
\defres{e2c_jevgym_baselines/randscore_route_tau0.4/steps}{7.53}
\defres{e2c_jevgym_baselines/randscore_route_tau0.4/success}{94.0}
\defres{e2c_jevgym_baselines/randscore_route_tau0.4/success_ci/hi}{97.0}
\defres{e2c_jevgym_baselines/randscore_route_tau0.4/success_ci/lo}{90.5}
\defres{e2c_jevgym_baselines/randscore_route_tau0.4/vs_baseline/cost_savings}{29.5}
\defres{e2c_jevgym_baselines/randscore_route_tau0.4/vs_baseline/delta}{-6.0}
\defres{e2c_jevgym_baselines/randscore_route_tau0.4/vs_baseline/delta_ci/hi}{-3.0}
\defres{e2c_jevgym_baselines/randscore_route_tau0.4/vs_baseline/delta_ci/lo}{-9.5}
\defres{e2c_jevgym_baselines/randscore_route_tau0.4/vs_baseline/ni/p_decisive}{0.993}
\defres{e2c_jevgym_baselines/randscore_route_tau0.6/cost_usd}{0.0216}
\defres{e2c_jevgym_baselines/randscore_route_tau0.6/decisions/noul/ece}{0.268}
\defres{e2c_jevgym_baselines/randscore_route_tau0.6/llm_calls}{7.54}
\defres{e2c_jevgym_baselines/randscore_route_tau0.6/steps}{7.54}
\defres{e2c_jevgym_baselines/randscore_route_tau0.6/success}{88.0}
\defres{e2c_jevgym_baselines/randscore_route_tau0.6/success_ci/hi}{92.0}
\defres{e2c_jevgym_baselines/randscore_route_tau0.6/success_ci/lo}{83.5}
\defres{e2c_jevgym_baselines/randscore_route_tau0.6/vs_baseline/cost_savings}{47.3}
\defres{e2c_jevgym_baselines/randscore_route_tau0.6/vs_baseline/delta}{-12.0}
\defres{e2c_jevgym_baselines/randscore_route_tau0.6/vs_baseline/delta_ci/hi}{-7.5}
\defres{e2c_jevgym_baselines/randscore_route_tau0.6/vs_baseline/delta_ci/lo}{-16.5}
\defres{e2c_jevgym_baselines/randscore_route_tau0.6/vs_baseline/ni/p_decisive}{1.000}
\defres{e2c_jevgym_baselines/randscore_route_tau0.8/cost_usd}{0.0159}
\defres{e2c_jevgym_baselines/randscore_route_tau0.8/decisions/noul/ece}{0.384}
\defres{e2c_jevgym_baselines/randscore_route_tau0.8/llm_calls}{7.54}
\defres{e2c_jevgym_baselines/randscore_route_tau0.8/steps}{7.54}
\defres{e2c_jevgym_baselines/randscore_route_tau0.8/success}{87.0}
\defres{e2c_jevgym_baselines/randscore_route_tau0.8/success_ci/hi}{91.0}
\defres{e2c_jevgym_baselines/randscore_route_tau0.8/success_ci/lo}{82.0}
\defres{e2c_jevgym_baselines/randscore_route_tau0.8/vs_baseline/cost_savings}{61.1}
\defres{e2c_jevgym_baselines/randscore_route_tau0.8/vs_baseline/delta}{-13.0}
\defres{e2c_jevgym_baselines/randscore_route_tau0.8/vs_baseline/delta_ci/hi}{-8.5}
\defres{e2c_jevgym_baselines/randscore_route_tau0.8/vs_baseline/delta_ci/lo}{-17.5}
\defres{e2c_jevgym_baselines/randscore_route_tau0.8/vs_baseline/ni/p_decisive}{1.000}
\defres{e2c_jevgym_baselines/rate10_reflect_trigger/cost_usd}{0.0423}
\defres{e2c_jevgym_baselines/rate10_reflect_trigger/decisions/noul/ece}{0.001}
\defres{e2c_jevgym_baselines/rate10_reflect_trigger/llm_calls}{8.10}
\defres{e2c_jevgym_baselines/rate10_reflect_trigger/steps}{7.53}
\defres{e2c_jevgym_baselines/rate10_reflect_trigger/success}{100.0}
\defres{e2c_jevgym_baselines/rate10_reflect_trigger/success_ci/hi}{100.0}
\defres{e2c_jevgym_baselines/rate10_reflect_trigger/success_ci/lo}{100.0}
\defres{e2c_jevgym_baselines/rate10_reflect_trigger/vs_baseline/cost_savings}{-3.4}
\defres{e2c_jevgym_baselines/rate10_reflect_trigger/vs_baseline/delta}{+0.0}
\defres{e2c_jevgym_baselines/rate10_reflect_trigger/vs_baseline/delta_ci/hi}{+0.0}
\defres{e2c_jevgym_baselines/rate10_reflect_trigger/vs_baseline/delta_ci/lo}{+0.0}
\defres{e2c_jevgym_baselines/rate10_reflect_trigger/vs_baseline/ni/p_decisive}{0.002}
\defres{e2c_jevgym_baselines/rate10_reflect_trigger_s2lite/cost_usd}{0.01}
\defres{e2c_jevgym_baselines/rate10_reflect_trigger_s2lite/decisions/noul/ece}{0.106}
\defres{e2c_jevgym_baselines/rate10_reflect_trigger_s2lite/llm_calls}{8.17}
\defres{e2c_jevgym_baselines/rate10_reflect_trigger_s2lite/steps}{7.55}
\defres{e2c_jevgym_baselines/rate10_reflect_trigger_s2lite/success}{87.0}
\defres{e2c_jevgym_baselines/rate10_reflect_trigger_s2lite/success_ci/hi}{91.5}
\defres{e2c_jevgym_baselines/rate10_reflect_trigger_s2lite/success_ci/lo}{82.5}
\defres{e2c_jevgym_baselines/rate10_reflect_trigger_s2lite/vs_baseline/cost_savings}{-3.3}
\defres{e2c_jevgym_baselines/rate10_reflect_trigger_s2lite/vs_baseline/delta}{+5.5}
\defres{e2c_jevgym_baselines/rate10_reflect_trigger_s2lite/vs_baseline/delta_ci/hi}{+10.0}
\defres{e2c_jevgym_baselines/rate10_reflect_trigger_s2lite/vs_baseline/delta_ci/lo}{+1.5}
\defres{e2c_jevgym_baselines/rate10_reflect_trigger_s2lite/vs_baseline/ni/p_decisive}{$<$0.001}
\defres{e2c_jevgym_baselines/rate10_route/cost_usd}{0.0132}
\defres{e2c_jevgym_baselines/rate10_route/decisions/noul/ece}{0.024}
\defres{e2c_jevgym_baselines/rate10_route/llm_calls}{7.55}
\defres{e2c_jevgym_baselines/rate10_route/steps}{7.55}
\defres{e2c_jevgym_baselines/rate10_route/success}{83.0}
\defres{e2c_jevgym_baselines/rate10_route/success_ci/hi}{88.0}
\defres{e2c_jevgym_baselines/rate10_route/success_ci/lo}{77.5}
\defres{e2c_jevgym_baselines/rate10_route/vs_baseline/cost_savings}{67.9}
\defres{e2c_jevgym_baselines/rate10_route/vs_baseline/delta}{-17.0}
\defres{e2c_jevgym_baselines/rate10_route/vs_baseline/delta_ci/hi}{-12.0}
\defres{e2c_jevgym_baselines/rate10_route/vs_baseline/delta_ci/lo}{-22.0}
\defres{e2c_jevgym_baselines/rate10_route/vs_baseline/ni/p_decisive}{1.000}
\defres{e2c_jevgym_baselines/rate10_stop_trigger/cost_usd}{0.0292}
\defres{e2c_jevgym_baselines/rate10_stop_trigger/decisions/noul/ece}{0.104}
\defres{e2c_jevgym_baselines/rate10_stop_trigger/llm_calls}{5.78}
\defres{e2c_jevgym_baselines/rate10_stop_trigger/steps}{5.28}
\defres{e2c_jevgym_baselines/rate10_stop_trigger/success}{50.5}
\defres{e2c_jevgym_baselines/rate10_stop_trigger/success_ci/hi}{57.5}
\defres{e2c_jevgym_baselines/rate10_stop_trigger/success_ci/lo}{43.5}
\defres{e2c_jevgym_baselines/rate10_stop_trigger/vs_baseline/cost_savings}{28.7}
\defres{e2c_jevgym_baselines/rate10_stop_trigger/vs_baseline/delta}{-49.5}
\defres{e2c_jevgym_baselines/rate10_stop_trigger/vs_baseline/delta_ci/hi}{-42.5}
\defres{e2c_jevgym_baselines/rate10_stop_trigger/vs_baseline/delta_ci/lo}{-56.0}
\defres{e2c_jevgym_baselines/rate10_stop_trigger/vs_baseline/ni/p_decisive}{1.000}
\defres{e2c_jevgym_baselines/rate30_reflect_trigger/cost_usd}{0.0461}
\defres{e2c_jevgym_baselines/rate30_reflect_trigger/decisions/noul/ece}{0.001}
\defres{e2c_jevgym_baselines/rate30_reflect_trigger/llm_calls}{9.57}
\defres{e2c_jevgym_baselines/rate30_reflect_trigger/steps}{7.58}
\defres{e2c_jevgym_baselines/rate30_reflect_trigger/success}{99.0}
\defres{e2c_jevgym_baselines/rate30_reflect_trigger/success_ci/hi}{100.0}
\defres{e2c_jevgym_baselines/rate30_reflect_trigger/success_ci/lo}{97.5}
\defres{e2c_jevgym_baselines/rate30_reflect_trigger/vs_baseline/cost_savings}{-12.5}
\defres{e2c_jevgym_baselines/rate30_reflect_trigger/vs_baseline/delta}{-1.0}
\defres{e2c_jevgym_baselines/rate30_reflect_trigger/vs_baseline/delta_ci/hi}{+0.0}
\defres{e2c_jevgym_baselines/rate30_reflect_trigger/vs_baseline/delta_ci/lo}{-2.5}
\defres{e2c_jevgym_baselines/rate30_reflect_trigger/vs_baseline/ni/p_decisive}{0.059}
\defres{e2c_jevgym_baselines/rate30_reflect_trigger_s2lite/cost_usd}{0.0106}
\defres{e2c_jevgym_baselines/rate30_reflect_trigger_s2lite/decisions/noul/ece}{0.298}
\defres{e2c_jevgym_baselines/rate30_reflect_trigger_s2lite/llm_calls}{9.46}
\defres{e2c_jevgym_baselines/rate30_reflect_trigger_s2lite/steps}{7.54}
\defres{e2c_jevgym_baselines/rate30_reflect_trigger_s2lite/success}{88.0}
\defres{e2c_jevgym_baselines/rate30_reflect_trigger_s2lite/success_ci/hi}{92.5}
\defres{e2c_jevgym_baselines/rate30_reflect_trigger_s2lite/success_ci/lo}{83.5}
\defres{e2c_jevgym_baselines/rate30_reflect_trigger_s2lite/vs_baseline/cost_savings}{-9.7}
\defres{e2c_jevgym_baselines/rate30_reflect_trigger_s2lite/vs_baseline/delta}{+6.5}
\defres{e2c_jevgym_baselines/rate30_reflect_trigger_s2lite/vs_baseline/delta_ci/hi}{+11.5}
\defres{e2c_jevgym_baselines/rate30_reflect_trigger_s2lite/vs_baseline/delta_ci/lo}{+1.5}
\defres{e2c_jevgym_baselines/rate30_reflect_trigger_s2lite/vs_baseline/ni/p_decisive}{$<$0.001}
\defres{e2c_jevgym_baselines/rate30_route/cost_usd}{0.0193}
\defres{e2c_jevgym_baselines/rate30_route/decisions/noul/ece}{0.025}
\defres{e2c_jevgym_baselines/rate30_route/llm_calls}{7.54}
\defres{e2c_jevgym_baselines/rate30_route/steps}{7.54}
\defres{e2c_jevgym_baselines/rate30_route/success}{86.5}
\defres{e2c_jevgym_baselines/rate30_route/success_ci/hi}{90.5}
\defres{e2c_jevgym_baselines/rate30_route/success_ci/lo}{82.0}
\defres{e2c_jevgym_baselines/rate30_route/vs_baseline/cost_savings}{52.8}
\defres{e2c_jevgym_baselines/rate30_route/vs_baseline/delta}{-13.5}
\defres{e2c_jevgym_baselines/rate30_route/vs_baseline/delta_ci/hi}{-9.0}
\defres{e2c_jevgym_baselines/rate30_route/vs_baseline/delta_ci/lo}{-18.5}
\defres{e2c_jevgym_baselines/rate30_route/vs_baseline/ni/p_decisive}{1.000}
\defres{e2c_jevgym_baselines/rate50_reflect_trigger/cost_usd}{0.0507}
\defres{e2c_jevgym_baselines/rate50_reflect_trigger/decisions/noul/ece}{0.002}
\defres{e2c_jevgym_baselines/rate50_reflect_trigger/llm_calls}{10.91}
\defres{e2c_jevgym_baselines/rate50_reflect_trigger/steps}{7.63}
\defres{e2c_jevgym_baselines/rate50_reflect_trigger/success}{98.5}
\defres{e2c_jevgym_baselines/rate50_reflect_trigger/success_ci/hi}{100.0}
\defres{e2c_jevgym_baselines/rate50_reflect_trigger/success_ci/lo}{96.5}
\defres{e2c_jevgym_baselines/rate50_reflect_trigger/vs_baseline/cost_savings}{-24.0}
\defres{e2c_jevgym_baselines/rate50_reflect_trigger/vs_baseline/delta}{-1.5}
\defres{e2c_jevgym_baselines/rate50_reflect_trigger/vs_baseline/delta_ci/hi}{+0.0}
\defres{e2c_jevgym_baselines/rate50_reflect_trigger/vs_baseline/delta_ci/lo}{-3.5}
\defres{e2c_jevgym_baselines/rate50_reflect_trigger/vs_baseline/ni/p_decisive}{0.155}
\defres{e2c_jevgym_baselines/rate50_reflect_trigger_s2lite/cost_usd}{0.0116}
\defres{e2c_jevgym_baselines/rate50_reflect_trigger_s2lite/decisions/noul/ece}{0.496}
\defres{e2c_jevgym_baselines/rate50_reflect_trigger_s2lite/llm_calls}{10.84}
\defres{e2c_jevgym_baselines/rate50_reflect_trigger_s2lite/steps}{7.55}
\defres{e2c_jevgym_baselines/rate50_reflect_trigger_s2lite/success}{90.0}
\defres{e2c_jevgym_baselines/rate50_reflect_trigger_s2lite/success_ci/hi}{94.0}
\defres{e2c_jevgym_baselines/rate50_reflect_trigger_s2lite/success_ci/lo}{85.5}
\defres{e2c_jevgym_baselines/rate50_reflect_trigger_s2lite/vs_baseline/cost_savings}{-19.5}
\defres{e2c_jevgym_baselines/rate50_reflect_trigger_s2lite/vs_baseline/delta}{+8.5}
\defres{e2c_jevgym_baselines/rate50_reflect_trigger_s2lite/vs_baseline/delta_ci/hi}{+13.5}
\defres{e2c_jevgym_baselines/rate50_reflect_trigger_s2lite/vs_baseline/delta_ci/lo}{+4.0}
\defres{e2c_jevgym_baselines/rate50_reflect_trigger_s2lite/vs_baseline/ni/p_decisive}{$<$0.001}
\defres{e2c_jevgym_baselines/rate50_route/cost_usd}{0.0255}
\defres{e2c_jevgym_baselines/rate50_route/decisions/noul/ece}{0.029}
\defres{e2c_jevgym_baselines/rate50_route/llm_calls}{7.52}
\defres{e2c_jevgym_baselines/rate50_route/steps}{7.52}
\defres{e2c_jevgym_baselines/rate50_route/success}{89.0}
\defres{e2c_jevgym_baselines/rate50_route/success_ci/hi}{93.5}
\defres{e2c_jevgym_baselines/rate50_route/success_ci/lo}{84.5}
\defres{e2c_jevgym_baselines/rate50_route/vs_baseline/cost_savings}{37.6}
\defres{e2c_jevgym_baselines/rate50_route/vs_baseline/delta}{-11.0}
\defres{e2c_jevgym_baselines/rate50_route/vs_baseline/delta_ci/hi}{-7.0}
\defres{e2c_jevgym_baselines/rate50_route/vs_baseline/delta_ci/lo}{-15.5}
\defres{e2c_jevgym_baselines/rate50_route/vs_baseline/ni/p_decisive}{1.000}
\defres{e2c_jevgym_baselines/rate50_stop_guard/cost_usd}{0.0464}
\defres{e2c_jevgym_baselines/rate50_stop_guard/decisions/noul/ece}{0.481}
\defres{e2c_jevgym_baselines/rate50_stop_guard/llm_calls}{8.43}
\defres{e2c_jevgym_baselines/rate50_stop_guard/steps}{8.43}
\defres{e2c_jevgym_baselines/rate50_stop_guard/success}{100.0}
\defres{e2c_jevgym_baselines/rate50_stop_guard/success_ci/hi}{100.0}
\defres{e2c_jevgym_baselines/rate50_stop_guard/success_ci/lo}{100.0}
\defres{e2c_jevgym_baselines/rate50_stop_guard/vs_baseline/cost_savings}{-13.2}
\defres{e2c_jevgym_baselines/rate50_stop_guard/vs_baseline/delta}{+0.0}
\defres{e2c_jevgym_baselines/rate50_stop_guard/vs_baseline/delta_ci/hi}{+0.0}
\defres{e2c_jevgym_baselines/rate50_stop_guard/vs_baseline/delta_ci/lo}{+0.0}
\defres{e2c_jevgym_baselines/rate50_stop_guard/vs_baseline/ni/p_decisive}{0.002}
\defres{e2c_jevgym_baselines/ratem_memw/cost_usd}{0.0556}
\defres{e2c_jevgym_baselines/ratem_memw/decisions/noul/ece}{0.325}
\defres{e2c_jevgym_baselines/ratem_memw/llm_calls}{7.63}
\defres{e2c_jevgym_baselines/ratem_memw/steps}{7.63}
\defres{e2c_jevgym_baselines/ratem_memw/success}{98.5}
\defres{e2c_jevgym_baselines/ratem_memw/success_ci/hi}{100.0}
\defres{e2c_jevgym_baselines/ratem_memw/success_ci/lo}{96.5}
\defres{e2c_jevgym_baselines/ratem_memw/vs_baseline/cost_savings}{-35.8}
\defres{e2c_jevgym_baselines/ratem_memw/vs_baseline/delta}{-1.5}
\defres{e2c_jevgym_baselines/ratem_memw/vs_baseline/delta_ci/hi}{+0.0}
\defres{e2c_jevgym_baselines/ratem_memw/vs_baseline/delta_ci/lo}{-3.5}
\defres{e2c_jevgym_baselines/ratem_memw/vs_baseline/ni/p_decisive}{0.155}
\defres{e2c_jevgym_baselines/ratem_reflect_trigger_s2lite/cost_usd}{0.0103}
\defres{e2c_jevgym_baselines/ratem_reflect_trigger_s2lite/decisions/noul/ece}{0.163}
\defres{e2c_jevgym_baselines/ratem_reflect_trigger_s2lite/llm_calls}{8.56}
\defres{e2c_jevgym_baselines/ratem_reflect_trigger_s2lite/steps}{7.59}
\defres{e2c_jevgym_baselines/ratem_reflect_trigger_s2lite/success}{85.4}
\defres{e2c_jevgym_baselines/ratem_reflect_trigger_s2lite/success_ci/hi}{88.6}
\defres{e2c_jevgym_baselines/ratem_reflect_trigger_s2lite/success_ci/lo}{82.4}
\defres{e2c_jevgym_baselines/ratem_reflect_trigger_s2lite/vs_baseline/cost_savings}{-5.9}
\defres{e2c_jevgym_baselines/ratem_reflect_trigger_s2lite/vs_baseline/delta}{+4.2}
\defres{e2c_jevgym_baselines/ratem_reflect_trigger_s2lite/vs_baseline/delta_ci/hi}{+7.2}
\defres{e2c_jevgym_baselines/ratem_reflect_trigger_s2lite/vs_baseline/delta_ci/lo}{+0.8}
\defres{e2c_jevgym_baselines/ratem_reflect_trigger_s2lite/vs_baseline/ni/p_decisive}{$<$0.001}
\defres{e2c_jevgym_baselines/ratem_route/cost_usd}{0.0114}
\defres{e2c_jevgym_baselines/ratem_route/decisions/noul/ece}{0.022}
\defres{e2c_jevgym_baselines/ratem_route/llm_calls}{7.55}
\defres{e2c_jevgym_baselines/ratem_route/steps}{7.55}
\defres{e2c_jevgym_baselines/ratem_route/success}{83.5}
\defres{e2c_jevgym_baselines/ratem_route/success_ci/hi}{88.5}
\defres{e2c_jevgym_baselines/ratem_route/success_ci/lo}{78.0}
\defres{e2c_jevgym_baselines/ratem_route/vs_baseline/cost_savings}{72.3}
\defres{e2c_jevgym_baselines/ratem_route/vs_baseline/delta}{-16.5}
\defres{e2c_jevgym_baselines/ratem_route/vs_baseline/delta_ci/hi}{-11.5}
\defres{e2c_jevgym_baselines/ratem_route/vs_baseline/delta_ci/lo}{-21.5}
\defres{e2c_jevgym_baselines/ratem_route/vs_baseline/ni/p_decisive}{1.000}
\defres{e2c_jevgym_baselines/ratem_stop_guard_s2lite/cost_usd}{0.0102}
\defres{e2c_jevgym_baselines/ratem_stop_guard_s2lite/decisions/noul/ece}{0.379}
\defres{e2c_jevgym_baselines/ratem_stop_guard_s2lite/llm_calls}{8.02}
\defres{e2c_jevgym_baselines/ratem_stop_guard_s2lite/steps}{8.02}
\defres{e2c_jevgym_baselines/ratem_stop_guard_s2lite/success}{83.0}
\defres{e2c_jevgym_baselines/ratem_stop_guard_s2lite/success_ci/hi}{88.0}
\defres{e2c_jevgym_baselines/ratem_stop_guard_s2lite/success_ci/lo}{77.5}
\defres{e2c_jevgym_baselines/ratem_stop_guard_s2lite/vs_baseline/cost_savings}{-5.3}
\defres{e2c_jevgym_baselines/ratem_stop_guard_s2lite/vs_baseline/delta}{+1.5}
\defres{e2c_jevgym_baselines/ratem_stop_guard_s2lite/vs_baseline/delta_ci/hi}{+5.0}
\defres{e2c_jevgym_baselines/ratem_stop_guard_s2lite/vs_baseline/delta_ci/lo}{-2.0}
\defres{e2c_jevgym_baselines/ratem_stop_guard_s2lite/vs_baseline/ni/p_decisive}{0.012}
\defres{e2c_jevgym_baselines/reflect_always/cost_usd}{0.0677}
\defres{e2c_jevgym_baselines/reflect_always/llm_calls}{14.62}
\defres{e2c_jevgym_baselines/reflect_always/steps}{7.81}
\defres{e2c_jevgym_baselines/reflect_always/success}{97.5}
\defres{e2c_jevgym_baselines/reflect_always/success_ci/hi}{99.5}
\defres{e2c_jevgym_baselines/reflect_always/success_ci/lo}{95.0}
\defres{e2c_jevgym_baselines/reflect_always/vs_baseline/cost_savings}{-65.3}
\defres{e2c_jevgym_baselines/reflect_always/vs_baseline/delta}{-2.5}
\defres{e2c_jevgym_baselines/reflect_always/vs_baseline/delta_ci/hi}{-0.5}
\defres{e2c_jevgym_baselines/reflect_always/vs_baseline/delta_ci/lo}{-5.0}
\defres{e2c_jevgym_baselines/reflect_always/vs_baseline/ni/p_decisive}{0.459}
\defres{e2c_jevgym_baselines/s2self_reflect_trigger/cost_usd}{0.0528}
\defres{e2c_jevgym_baselines/s2self_reflect_trigger/decisions/noul/ece}{0.050}
\defres{e2c_jevgym_baselines/s2self_reflect_trigger/llm_calls}{7.67}
\defres{e2c_jevgym_baselines/s2self_reflect_trigger/steps}{7.51}
\defres{e2c_jevgym_baselines/s2self_reflect_trigger/success}{100.0}
\defres{e2c_jevgym_baselines/s2self_reflect_trigger/success_ci/hi}{100.0}
\defres{e2c_jevgym_baselines/s2self_reflect_trigger/success_ci/lo}{100.0}
\defres{e2c_jevgym_baselines/s2self_reflect_trigger/vs_baseline/cost_savings}{-29.0}
\defres{e2c_jevgym_baselines/s2self_reflect_trigger/vs_baseline/delta}{+0.0}
\defres{e2c_jevgym_baselines/s2self_reflect_trigger/vs_baseline/delta_ci/hi}{+0.0}
\defres{e2c_jevgym_baselines/s2self_reflect_trigger/vs_baseline/delta_ci/lo}{+0.0}
\defres{e2c_jevgym_baselines/s2self_reflect_trigger/vs_baseline/ni/p_decisive}{0.002}
\defres{e2c_jevgym_baselines/s2self_reflect_trigger_s2lite/cost_usd}{0.0122}
\defres{e2c_jevgym_baselines/s2self_reflect_trigger_s2lite/decisions/noul/ece}{0.016}
\defres{e2c_jevgym_baselines/s2self_reflect_trigger_s2lite/llm_calls}{7.56}
\defres{e2c_jevgym_baselines/s2self_reflect_trigger_s2lite/steps}{7.55}
\defres{e2c_jevgym_baselines/s2self_reflect_trigger_s2lite/success}{84.0}
\defres{e2c_jevgym_baselines/s2self_reflect_trigger_s2lite/success_ci/hi}{89.0}
\defres{e2c_jevgym_baselines/s2self_reflect_trigger_s2lite/success_ci/lo}{78.5}
\defres{e2c_jevgym_baselines/s2self_reflect_trigger_s2lite/vs_baseline/cost_savings}{-25.8}
\defres{e2c_jevgym_baselines/s2self_reflect_trigger_s2lite/vs_baseline/delta}{+2.5}
\defres{e2c_jevgym_baselines/s2self_reflect_trigger_s2lite/vs_baseline/delta_ci/hi}{+6.0}
\defres{e2c_jevgym_baselines/s2self_reflect_trigger_s2lite/vs_baseline/delta_ci/lo}{-0.5}
\defres{e2c_jevgym_baselines/s2self_reflect_trigger_s2lite/vs_baseline/ni/p_decisive}{0.002}
\defres{e2c_jevgym_baselines/s2self_route/cost_usd}{0.0226}
\defres{e2c_jevgym_baselines/s2self_route/decisions/noul/ece}{0.029}
\defres{e2c_jevgym_baselines/s2self_route/llm_calls}{7.54}
\defres{e2c_jevgym_baselines/s2self_route/steps}{7.54}
\defres{e2c_jevgym_baselines/s2self_route/success}{82.5}
\defres{e2c_jevgym_baselines/s2self_route/success_ci/hi}{87.5}
\defres{e2c_jevgym_baselines/s2self_route/success_ci/lo}{77.0}
\defres{e2c_jevgym_baselines/s2self_route/vs_baseline/cost_savings}{44.7}
\defres{e2c_jevgym_baselines/s2self_route/vs_baseline/delta}{-17.5}
\defres{e2c_jevgym_baselines/s2self_route/vs_baseline/delta_ci/hi}{-12.5}
\defres{e2c_jevgym_baselines/s2self_route/vs_baseline/delta_ci/lo}{-22.5}
\defres{e2c_jevgym_baselines/s2self_route/vs_baseline/ni/p_decisive}{1.000}
\defres{e2c_jevgym_baselines/s2self_ts_assist_k3/cost_usd}{0.107}
\defres{e2c_jevgym_baselines/s2self_ts_assist_k3/decisions/ece}{0.075}
\defres{e2c_jevgym_baselines/s2self_ts_assist_k3/llm_calls}{7.87}
\defres{e2c_jevgym_baselines/s2self_ts_assist_k3/steps}{7.87}
\defres{e2c_jevgym_baselines/s2self_ts_assist_k3/success}{94.5}
\defres{e2c_jevgym_baselines/s2self_ts_assist_k3/success_ci/hi}{97.5}
\defres{e2c_jevgym_baselines/s2self_ts_assist_k3/success_ci/lo}{91.0}
\defres{e2c_jevgym_baselines/s2self_ts_assist_k3/vs_baseline/cost_savings}{-161.9}
\defres{e2c_jevgym_baselines/s2self_ts_assist_k3/vs_baseline/delta}{-5.5}
\defres{e2c_jevgym_baselines/s2self_ts_assist_k3/vs_baseline/delta_ci/hi}{-2.5}
\defres{e2c_jevgym_baselines/s2self_ts_assist_k3/vs_baseline/delta_ci/lo}{-8.5}
\defres{e2c_jevgym_baselines/s2self_ts_assist_k3/vs_baseline/ni/p_decisive}{0.983}
\defres{e2c_jevgym_baselines/tfidf_ts_assist_k3/cost_usd}{0.0134}
\defres{e2c_jevgym_baselines/tfidf_ts_assist_k3/decisions/ece}{0.579}
\defres{e2c_jevgym_baselines/tfidf_ts_assist_k3/llm_calls}{7.31}
\defres{e2c_jevgym_baselines/tfidf_ts_assist_k3/steps}{7.31}
\defres{e2c_jevgym_baselines/tfidf_ts_assist_k3/success}{33.0}
\defres{e2c_jevgym_baselines/tfidf_ts_assist_k3/success_ci/hi}{39.5}
\defres{e2c_jevgym_baselines/tfidf_ts_assist_k3/success_ci/lo}{26.5}
\defres{e2c_jevgym_baselines/tfidf_ts_assist_k3/vs_baseline/cost_savings}{67.2}
\defres{e2c_jevgym_baselines/tfidf_ts_assist_k3/vs_baseline/delta}{-67.0}
\defres{e2c_jevgym_baselines/tfidf_ts_assist_k3/vs_baseline/delta_ci/hi}{-60.5}
\defres{e2c_jevgym_baselines/tfidf_ts_assist_k3/vs_baseline/delta_ci/lo}{-73.0}
\defres{e2c_jevgym_baselines/tfidf_ts_assist_k3/vs_baseline/ni/p_decisive}{1.000}
\defres{e2c_jevgym_baselines/tfidf_ts_assist_k5/cost_usd}{0.0243}
\defres{e2c_jevgym_baselines/tfidf_ts_assist_k5/decisions/ece}{0.764}
\defres{e2c_jevgym_baselines/tfidf_ts_assist_k5/llm_calls}{10.96}
\defres{e2c_jevgym_baselines/tfidf_ts_assist_k5/steps}{10.96}
\defres{e2c_jevgym_baselines/tfidf_ts_assist_k5/success}{25.0}
\defres{e2c_jevgym_baselines/tfidf_ts_assist_k5/success_ci/hi}{31.0}
\defres{e2c_jevgym_baselines/tfidf_ts_assist_k5/success_ci/lo}{19.0}
\defres{e2c_jevgym_baselines/tfidf_ts_assist_k5/vs_baseline/cost_savings}{40.6}
\defres{e2c_jevgym_baselines/tfidf_ts_assist_k5/vs_baseline/delta}{-75.0}
\defres{e2c_jevgym_baselines/tfidf_ts_assist_k5/vs_baseline/delta_ci/hi}{-69.0}
\defres{e2c_jevgym_baselines/tfidf_ts_assist_k5/vs_baseline/delta_ci/lo}{-81.0}
\defres{e2c_jevgym_baselines/tfidf_ts_assist_k5/vs_baseline/ni/p_decisive}{1.000}
\defres{e2c_jevgym_baselines/tfidf_ts_replace/cost_usd}{0.0187}
\defres{e2c_jevgym_baselines/tfidf_ts_replace/decisions/ece}{0.760}
\defres{e2c_jevgym_baselines/tfidf_ts_replace/llm_calls}{7.24}
\defres{e2c_jevgym_baselines/tfidf_ts_replace/steps}{7.24}
\defres{e2c_jevgym_baselines/tfidf_ts_replace/success}{12.5}
\defres{e2c_jevgym_baselines/tfidf_ts_replace/success_ci/hi}{17.0}
\defres{e2c_jevgym_baselines/tfidf_ts_replace/success_ci/lo}{8.0}
\defres{e2c_jevgym_baselines/tfidf_ts_replace/vs_baseline/cost_savings}{54.4}
\defres{e2c_jevgym_baselines/tfidf_ts_replace/vs_baseline/delta}{-87.5}
\defres{e2c_jevgym_baselines/tfidf_ts_replace/vs_baseline/delta_ci/hi}{-82.5}
\defres{e2c_jevgym_baselines/tfidf_ts_replace/vs_baseline/delta_ci/lo}{-92.0}
\defres{e2c_jevgym_baselines/tfidf_ts_replace/vs_baseline/ni/p_decisive}{1.000}
\defres{tau2/airline/headline/iso_cost/delta_ci/hi}{+12.0}
\defres{tau2/airline/headline/iso_cost/delta_ci/lo}{-8.0}
\defres{tau2/airline/headline/iso_cost/success}{72.0}
\defres{tau2/airline/jev_guard/cost_usd}{0.0787}
\defres{tau2/airline/jev_guard/llm_calls}{12.26}
\defres{tau2/airline/jev_guard/steps}{12.09}
\defres{tau2/airline/jev_guard/success}{73.3}
\defres{tau2/airline/jev_guard/success_ci/hi}{82.7}
\defres{tau2/airline/jev_guard/success_ci/lo}{63.3}
\defres{tau2/airline/jev_guard/vs_baseline/cost_savings}{-2.3}
\defres{tau2/airline/jev_guard/vs_baseline/delta}{+5.3}
\defres{tau2/airline/jev_guard/vs_baseline/delta_ci/hi}{+12.7}
\defres{tau2/airline/jev_guard/vs_baseline/delta_ci/lo}{-2.7}
\defres{tau2/airline/jev_guard/vs_baseline/ni/p_decisive}{0.170}
\defres{tau2/airline/jev_shadow/cost_usd}{0.0664}
\defres{tau2/airline/jev_shadow/decisions/ece}{0.146}
\defres{tau2/airline/jev_shadow/decisions/gold/gates/stop_trigger-shadow/ece}{0.673}
\defres{tau2/airline/jev_shadow/decisions/noul/ece}{0.673}
\defres{tau2/airline/jev_shadow/llm_calls}{10.84}
\defres{tau2/airline/jev_shadow/steps}{10.84}
\defres{tau2/airline/jev_shadow/success}{64.4}
\defres{tau2/airline/jev_shadow/success_ci/hi}{86.7}
\defres{tau2/airline/jev_shadow/success_ci/lo}{40.0}
\defres{tau2/airline/jev_shadow/vs_baseline/cost_savings}{3.2}
\defres{tau2/airline/jev_shadow/vs_baseline/delta}{-2.2}
\defres{tau2/airline/jev_shadow/vs_baseline/delta_ci/hi}{+4.4}
\defres{tau2/airline/jev_shadow/vs_baseline/delta_ci/lo}{-8.9}
\defres{tau2/airline/jev_shadow/vs_baseline/ni/p_decisive}{0.464}
\defres{tau2/airline/jev_ts_assist_k3/cost_usd}{0.0871}
\defres{tau2/airline/jev_ts_assist_k3/decisions/ece}{0.137}
\defres{tau2/airline/jev_ts_assist_k3/llm_calls}{12.82}
\defres{tau2/airline/jev_ts_assist_k3/steps}{12.82}
\defres{tau2/airline/jev_ts_assist_k3/success}{68.0}
\defres{tau2/airline/jev_ts_assist_k3/success_ci/hi}{79.3}
\defres{tau2/airline/jev_ts_assist_k3/success_ci/lo}{57.3}
\defres{tau2/airline/jev_ts_assist_k3/vs_baseline/cost_savings}{-13.3}
\defres{tau2/airline/jev_ts_assist_k3/vs_baseline/delta}{+0.0}
\defres{tau2/airline/jev_ts_assist_k3/vs_baseline/delta_ci/hi}{+8.0}
\defres{tau2/airline/jev_ts_assist_k3/vs_baseline/delta_ci/lo}{-8.0}
\defres{tau2/airline/jev_ts_assist_k3/vs_baseline/ni/p_decisive}{0.466}
\defres{tau2/airline/jev_ts_cascade_tau0.5/cost_usd}{0.117}
\defres{tau2/airline/jev_ts_cascade_tau0.5/decisions/ece}{0.167}
\defres{tau2/airline/jev_ts_cascade_tau0.5/llm_calls}{12.75}
\defres{tau2/airline/jev_ts_cascade_tau0.5/steps}{16.69}
\defres{tau2/airline/jev_ts_cascade_tau0.5/success}{54.7}
\defres{tau2/airline/jev_ts_cascade_tau0.5/success_ci/hi}{66.0}
\defres{tau2/airline/jev_ts_cascade_tau0.5/success_ci/lo}{44.0}
\defres{tau2/airline/jev_ts_cascade_tau0.5/vs_baseline/cost_savings}{-52.2}
\defres{tau2/airline/jev_ts_cascade_tau0.5/vs_baseline/delta}{-13.3}
\defres{tau2/airline/jev_ts_cascade_tau0.5/vs_baseline/delta_ci/hi}{-5.3}
\defres{tau2/airline/jev_ts_cascade_tau0.5/vs_baseline/delta_ci/lo}{-22.0}
\defres{tau2/airline/jev_ts_cascade_tau0.5/vs_baseline/ni/p_decisive}{0.985}
\defres{tau2/airline/jev_ts_cascade_tau0.7/cost_usd}{0.0815}
\defres{tau2/airline/jev_ts_cascade_tau0.7/decisions/ece}{0.128}
\defres{tau2/airline/jev_ts_cascade_tau0.7/llm_calls}{9.85}
\defres{tau2/airline/jev_ts_cascade_tau0.7/steps}{11.78}
\defres{tau2/airline/jev_ts_cascade_tau0.7/success}{61.3}
\defres{tau2/airline/jev_ts_cascade_tau0.7/success_ci/hi}{72.7}
\defres{tau2/airline/jev_ts_cascade_tau0.7/success_ci/lo}{49.3}
\defres{tau2/airline/jev_ts_cascade_tau0.7/vs_baseline/cost_savings}{-6.0}
\defres{tau2/airline/jev_ts_cascade_tau0.7/vs_baseline/delta}{-6.7}
\defres{tau2/airline/jev_ts_cascade_tau0.7/vs_baseline/delta_ci/hi}{+0.7}
\defres{tau2/airline/jev_ts_cascade_tau0.7/vs_baseline/delta_ci/lo}{-14.7}
\defres{tau2/airline/jev_ts_cascade_tau0.7/vs_baseline/ni/p_decisive}{0.816}
\defres{tau2/airline/jev_ts_cascade_tau0.8/cost_usd}{0.0826}
\defres{tau2/airline/jev_ts_cascade_tau0.8/decisions/ece}{0.157}
\defres{tau2/airline/jev_ts_cascade_tau0.8/llm_calls}{10.26}
\defres{tau2/airline/jev_ts_cascade_tau0.8/steps}{11.71}
\defres{tau2/airline/jev_ts_cascade_tau0.8/success}{61.3}
\defres{tau2/airline/jev_ts_cascade_tau0.8/success_ci/hi}{72.0}
\defres{tau2/airline/jev_ts_cascade_tau0.8/success_ci/lo}{50.0}
\defres{tau2/airline/jev_ts_cascade_tau0.8/vs_baseline/cost_savings}{-7.3}
\defres{tau2/airline/jev_ts_cascade_tau0.8/vs_baseline/delta}{-6.7}
\defres{tau2/airline/jev_ts_cascade_tau0.8/vs_baseline/delta_ci/hi}{+0.7}
\defres{tau2/airline/jev_ts_cascade_tau0.8/vs_baseline/delta_ci/lo}{-14.0}
\defres{tau2/airline/jev_ts_cascade_tau0.8/vs_baseline/ni/p_decisive}{0.706}
\defres{tau2/airline/jev_ts_cascade_tau0.9/cost_usd}{0.0885}
\defres{tau2/airline/jev_ts_cascade_tau0.9/decisions/ece}{0.141}
\defres{tau2/airline/jev_ts_cascade_tau0.9/llm_calls}{10.95}
\defres{tau2/airline/jev_ts_cascade_tau0.9/steps}{11.81}
\defres{tau2/airline/jev_ts_cascade_tau0.9/success}{65.3}
\defres{tau2/airline/jev_ts_cascade_tau0.9/success_ci/hi}{76.0}
\defres{tau2/airline/jev_ts_cascade_tau0.9/success_ci/lo}{54.0}
\defres{tau2/airline/jev_ts_cascade_tau0.9/vs_baseline/cost_savings}{-15.0}
\defres{tau2/airline/jev_ts_cascade_tau0.9/vs_baseline/delta}{-2.7}
\defres{tau2/airline/jev_ts_cascade_tau0.9/vs_baseline/delta_ci/hi}{+3.3}
\defres{tau2/airline/jev_ts_cascade_tau0.9/vs_baseline/delta_ci/lo}{-8.7}
\defres{tau2/airline/jev_ts_cascade_tau0.9/vs_baseline/ni/p_decisive}{0.541}
\defres{tau2/airline/jev_ts_cascade_tau0.95/cost_usd}{0.0958}
\defres{tau2/airline/jev_ts_cascade_tau0.95/decisions/ece}{0.192}
\defres{tau2/airline/jev_ts_cascade_tau0.95/llm_calls}{11.53}
\defres{tau2/airline/jev_ts_cascade_tau0.95/steps}{12.02}
\defres{tau2/airline/jev_ts_cascade_tau0.95/success}{69.3}
\defres{tau2/airline/jev_ts_cascade_tau0.95/success_ci/hi}{79.3}
\defres{tau2/airline/jev_ts_cascade_tau0.95/success_ci/lo}{58.7}
\defres{tau2/airline/jev_ts_cascade_tau0.95/vs_baseline/cost_savings}{-24.5}
\defres{tau2/airline/jev_ts_cascade_tau0.95/vs_baseline/delta}{+1.3}
\defres{tau2/airline/jev_ts_cascade_tau0.95/vs_baseline/delta_ci/hi}{+7.3}
\defres{tau2/airline/jev_ts_cascade_tau0.95/vs_baseline/delta_ci/lo}{-5.3}
\defres{tau2/airline/jev_ts_cascade_tau0.95/vs_baseline/ni/p_decisive}{0.170}
\defres{tau2/airline/jev_ts_cascade_tau0.99/cost_usd}{0.0778}
\defres{tau2/airline/jev_ts_cascade_tau0.99/decisions/ece}{0.169}
\defres{tau2/airline/jev_ts_cascade_tau0.99/llm_calls}{11.53}
\defres{tau2/airline/jev_ts_cascade_tau0.99/steps}{11.80}
\defres{tau2/airline/jev_ts_cascade_tau0.99/success}{66.7}
\defres{tau2/airline/jev_ts_cascade_tau0.99/success_ci/hi}{77.3}
\defres{tau2/airline/jev_ts_cascade_tau0.99/success_ci/lo}{55.3}
\defres{tau2/airline/jev_ts_cascade_tau0.99/vs_baseline/cost_savings}{-1.1}
\defres{tau2/airline/jev_ts_cascade_tau0.99/vs_baseline/delta}{-1.3}
\defres{tau2/airline/jev_ts_cascade_tau0.99/vs_baseline/delta_ci/hi}{+5.3}
\defres{tau2/airline/jev_ts_cascade_tau0.99/vs_baseline/delta_ci/lo}{-8.0}
\defres{tau2/airline/jev_ts_cascade_tau0.99/vs_baseline/ni/p_decisive}{0.273}
\defres{tau2/airline/jev_ts_cascade_tauhat_e2/cost_usd}{0.0728}
\defres{tau2/airline/jev_ts_cascade_tauhat_e2/decisions/ece}{0.149}
\defres{tau2/airline/jev_ts_cascade_tauhat_e2/llm_calls}{11.11}
\defres{tau2/airline/jev_ts_cascade_tauhat_e2/steps}{11.25}
\defres{tau2/airline/jev_ts_cascade_tauhat_e2/success}{70.7}
\defres{tau2/airline/jev_ts_cascade_tauhat_e2/success_ci/hi}{80.7}
\defres{tau2/airline/jev_ts_cascade_tauhat_e2/success_ci/lo}{60.0}
\defres{tau2/airline/jev_ts_cascade_tauhat_e2/vs_baseline/cost_savings}{5.3}
\defres{tau2/airline/jev_ts_cascade_tauhat_e2/vs_baseline/delta}{+2.7}
\defres{tau2/airline/jev_ts_cascade_tauhat_e2/vs_baseline/delta_ci/hi}{+9.3}
\defres{tau2/airline/jev_ts_cascade_tauhat_e2/vs_baseline/delta_ci/lo}{-4.0}
\defres{tau2/airline/jev_ts_cascade_tauhat_e2/vs_baseline/ni/p_decisive}{0.116}
\defres{tau2/airline/jev_ts_cascade_tauhat_refit/cost_usd}{0.0975}
\defres{tau2/airline/jev_ts_cascade_tauhat_refit/decisions/ece}{0.115}
\defres{tau2/airline/jev_ts_cascade_tauhat_refit/llm_calls}{11.76}
\defres{tau2/airline/jev_ts_cascade_tauhat_refit/steps}{12.99}
\defres{tau2/airline/jev_ts_cascade_tauhat_refit/success}{60.7}
\defres{tau2/airline/jev_ts_cascade_tauhat_refit/success_ci/hi}{72.0}
\defres{tau2/airline/jev_ts_cascade_tauhat_refit/success_ci/lo}{48.7}
\defres{tau2/airline/jev_ts_cascade_tauhat_refit/vs_baseline/cost_savings}{-26.8}
\defres{tau2/airline/jev_ts_cascade_tauhat_refit/vs_baseline/delta}{-7.3}
\defres{tau2/airline/jev_ts_cascade_tauhat_refit/vs_baseline/delta_ci/hi}{+2.7}
\defres{tau2/airline/jev_ts_cascade_tauhat_refit/vs_baseline/delta_ci/lo}{-18.0}
\defres{tau2/airline/jev_ts_cascade_tauhat_refit/vs_baseline/ni/p_decisive}{0.881}
\defres{tau2/airline/llm_only/cost_usd}{0.0769}
\defres{tau2/airline/llm_only/llm_calls}{12.19}
\defres{tau2/airline/llm_only/steps}{12.19}
\defres{tau2/airline/llm_only/success}{68.0}
\defres{tau2/airline/llm_only/success_ci/hi}{78.0}
\defres{tau2/airline/llm_only/success_ci/lo}{56.0}
\defres{tau2/airline_shadow/headline/iso_cost/delta_ci/hi}{+0.0}
\defres{tau2/airline_shadow/headline/iso_cost/delta_ci/lo}{+0.0}
\defres{tau2/airline_shadow/headline/iso_cost/success}{66.7}
\defres{tau2/airline_shadow/jev_guard/cost_usd}{0.0672}
\defres{tau2/airline_shadow/jev_guard/llm_calls}{10.98}
\defres{tau2/airline_shadow/jev_guard/steps}{10.87}
\defres{tau2/airline_shadow/jev_guard/success}{68.9}
\defres{tau2/airline_shadow/jev_guard/success_ci/hi}{88.9}
\defres{tau2/airline_shadow/jev_guard/success_ci/lo}{46.7}
\defres{tau2/airline_shadow/jev_guard/vs_baseline/cost_savings}{2.0}
\defres{tau2/airline_shadow/jev_guard/vs_baseline/delta}{+2.2}
\defres{tau2/airline_shadow/jev_guard/vs_baseline/delta_ci/hi}{+13.3}
\defres{tau2/airline_shadow/jev_guard/vs_baseline/delta_ci/lo}{-8.9}
\defres{tau2/airline_shadow/jev_guard/vs_baseline/ni/p_decisive}{0.830}
\defres{tau2/airline_shadow/jev_shadow/cost_usd}{0.0664}
\defres{tau2/airline_shadow/jev_shadow/decisions/ece}{0.146}
\defres{tau2/airline_shadow/jev_shadow/decisions/gold/gates/stop_trigger-shadow/ece}{0.673}
\defres{tau2/airline_shadow/jev_shadow/decisions/noul/ece}{0.673}
\defres{tau2/airline_shadow/jev_shadow/llm_calls}{10.84}
\defres{tau2/airline_shadow/jev_shadow/steps}{10.84}
\defres{tau2/airline_shadow/jev_shadow/success}{64.4}
\defres{tau2/airline_shadow/jev_shadow/success_ci/hi}{86.7}
\defres{tau2/airline_shadow/jev_shadow/success_ci/lo}{40.0}
\defres{tau2/airline_shadow/jev_shadow/vs_baseline/cost_savings}{3.2}
\defres{tau2/airline_shadow/jev_shadow/vs_baseline/delta}{-2.2}
\defres{tau2/airline_shadow/jev_shadow/vs_baseline/delta_ci/hi}{+4.4}
\defres{tau2/airline_shadow/jev_shadow/vs_baseline/delta_ci/lo}{-8.9}
\defres{tau2/airline_shadow/jev_shadow/vs_baseline/ni/p_decisive}{0.464}
\defres{tau2/airline_shadow/jev_ts_assist_k3/cost_usd}{0.0855}
\defres{tau2/airline_shadow/jev_ts_assist_k3/decisions/ece}{0.113}
\defres{tau2/airline_shadow/jev_ts_assist_k3/llm_calls}{12.87}
\defres{tau2/airline_shadow/jev_ts_assist_k3/steps}{12.87}
\defres{tau2/airline_shadow/jev_ts_assist_k3/success}{75.6}
\defres{tau2/airline_shadow/jev_ts_assist_k3/success_ci/hi}{93.3}
\defres{tau2/airline_shadow/jev_ts_assist_k3/success_ci/lo}{55.6}
\defres{tau2/airline_shadow/jev_ts_assist_k3/vs_baseline/cost_savings}{-24.5}
\defres{tau2/airline_shadow/jev_ts_assist_k3/vs_baseline/delta}{+8.9}
\defres{tau2/airline_shadow/jev_ts_assist_k3/vs_baseline/delta_ci/hi}{+20.0}
\defres{tau2/airline_shadow/jev_ts_assist_k3/vs_baseline/delta_ci/lo}{-2.2}
\defres{tau2/airline_shadow/jev_ts_assist_k3/vs_baseline/ni/p_decisive}{0.600}
\defres{tau2/airline_shadow/jev_ts_cascade_tau0.5/cost_usd}{0.157}
\defres{tau2/airline_shadow/jev_ts_cascade_tau0.5/decisions/ece}{0.164}
\defres{tau2/airline_shadow/jev_ts_cascade_tau0.5/llm_calls}{16.58}
\defres{tau2/airline_shadow/jev_ts_cascade_tau0.5/steps}{20.11}
\defres{tau2/airline_shadow/jev_ts_cascade_tau0.5/success}{51.1}
\defres{tau2/airline_shadow/jev_ts_cascade_tau0.5/success_ci/hi}{71.1}
\defres{tau2/airline_shadow/jev_ts_cascade_tau0.5/success_ci/lo}{31.1}
\defres{tau2/airline_shadow/jev_ts_cascade_tau0.5/vs_baseline/cost_savings}{-128.5}
\defres{tau2/airline_shadow/jev_ts_cascade_tau0.5/vs_baseline/delta}{-15.6}
\defres{tau2/airline_shadow/jev_ts_cascade_tau0.5/vs_baseline/delta_ci/hi}{-4.4}
\defres{tau2/airline_shadow/jev_ts_cascade_tau0.5/vs_baseline/delta_ci/lo}{-28.9}
\defres{tau2/airline_shadow/jev_ts_cascade_tau0.5/vs_baseline/ni/p_decisive}{0.997}
\defres{tau2/airline_shadow/jev_ts_cascade_tau0.7/cost_usd}{0.073}
\defres{tau2/airline_shadow/jev_ts_cascade_tau0.7/decisions/ece}{0.131}
\defres{tau2/airline_shadow/jev_ts_cascade_tau0.7/llm_calls}{8.98}
\defres{tau2/airline_shadow/jev_ts_cascade_tau0.7/steps}{10.53}
\defres{tau2/airline_shadow/jev_ts_cascade_tau0.7/success}{64.4}
\defres{tau2/airline_shadow/jev_ts_cascade_tau0.7/success_ci/hi}{86.7}
\defres{tau2/airline_shadow/jev_ts_cascade_tau0.7/success_ci/lo}{42.2}
\defres{tau2/airline_shadow/jev_ts_cascade_tau0.7/vs_baseline/cost_savings}{-6.4}
\defres{tau2/airline_shadow/jev_ts_cascade_tau0.7/vs_baseline/delta}{-2.2}
\defres{tau2/airline_shadow/jev_ts_cascade_tau0.7/vs_baseline/delta_ci/hi}{+4.4}
\defres{tau2/airline_shadow/jev_ts_cascade_tau0.7/vs_baseline/delta_ci/lo}{-11.1}
\defres{tau2/airline_shadow/jev_ts_cascade_tau0.7/vs_baseline/ni/p_decisive}{0.464}
\defres{tau2/airline_shadow/jev_ts_cascade_tau0.8/cost_usd}{0.0738}
\defres{tau2/airline_shadow/jev_ts_cascade_tau0.8/decisions/ece}{0.125}
\defres{tau2/airline_shadow/jev_ts_cascade_tau0.8/llm_calls}{9.62}
\defres{tau2/airline_shadow/jev_ts_cascade_tau0.8/steps}{10.89}
\defres{tau2/airline_shadow/jev_ts_cascade_tau0.8/success}{64.4}
\defres{tau2/airline_shadow/jev_ts_cascade_tau0.8/success_ci/hi}{84.4}
\defres{tau2/airline_shadow/jev_ts_cascade_tau0.8/success_ci/lo}{44.4}
\defres{tau2/airline_shadow/jev_ts_cascade_tau0.8/vs_baseline/cost_savings}{-7.6}
\defres{tau2/airline_shadow/jev_ts_cascade_tau0.8/vs_baseline/delta}{-2.2}
\defres{tau2/airline_shadow/jev_ts_cascade_tau0.8/vs_baseline/delta_ci/hi}{+4.4}
\defres{tau2/airline_shadow/jev_ts_cascade_tau0.8/vs_baseline/delta_ci/lo}{-8.9}
\defres{tau2/airline_shadow/jev_ts_cascade_tau0.8/vs_baseline/ni/p_decisive}{0.830}
\defres{tau2/airline_shadow/jev_ts_cascade_tau0.9/cost_usd}{0.0731}
\defres{tau2/airline_shadow/jev_ts_cascade_tau0.9/decisions/ece}{0.146}
\defres{tau2/airline_shadow/jev_ts_cascade_tau0.9/llm_calls}{10.04}
\defres{tau2/airline_shadow/jev_ts_cascade_tau0.9/steps}{10.87}
\defres{tau2/airline_shadow/jev_ts_cascade_tau0.9/success}{64.4}
\defres{tau2/airline_shadow/jev_ts_cascade_tau0.9/success_ci/hi}{86.7}
\defres{tau2/airline_shadow/jev_ts_cascade_tau0.9/success_ci/lo}{40.0}
\defres{tau2/airline_shadow/jev_ts_cascade_tau0.9/vs_baseline/cost_savings}{-6.5}
\defres{tau2/airline_shadow/jev_ts_cascade_tau0.9/vs_baseline/delta}{-2.2}
\defres{tau2/airline_shadow/jev_ts_cascade_tau0.9/vs_baseline/delta_ci/hi}{+4.4}
\defres{tau2/airline_shadow/jev_ts_cascade_tau0.9/vs_baseline/delta_ci/lo}{-8.9}
\defres{tau2/airline_shadow/jev_ts_cascade_tau0.9/vs_baseline/ni/p_decisive}{0.464}
\defres{tau2/airline_shadow/jev_ts_cascade_tau0.95/cost_usd}{0.0955}
\defres{tau2/airline_shadow/jev_ts_cascade_tau0.95/decisions/ece}{0.149}
\defres{tau2/airline_shadow/jev_ts_cascade_tau0.95/llm_calls}{10.47}
\defres{tau2/airline_shadow/jev_ts_cascade_tau0.95/steps}{10.93}
\defres{tau2/airline_shadow/jev_ts_cascade_tau0.95/success}{71.1}
\defres{tau2/airline_shadow/jev_ts_cascade_tau0.95/success_ci/hi}{88.9}
\defres{tau2/airline_shadow/jev_ts_cascade_tau0.95/success_ci/lo}{51.1}
\defres{tau2/airline_shadow/jev_ts_cascade_tau0.95/vs_baseline/cost_savings}{-39.2}
\defres{tau2/airline_shadow/jev_ts_cascade_tau0.95/vs_baseline/delta}{+4.4}
\defres{tau2/airline_shadow/jev_ts_cascade_tau0.95/vs_baseline/delta_ci/hi}{+11.1}
\defres{tau2/airline_shadow/jev_ts_cascade_tau0.95/vs_baseline/delta_ci/lo}{+0.0}
\defres{tau2/airline_shadow/jev_ts_cascade_tau0.95/vs_baseline/ni/p_decisive}{0.466}
\defres{tau2/airline_shadow/jev_ts_cascade_tau0.99/cost_usd}{0.0612}
\defres{tau2/airline_shadow/jev_ts_cascade_tau0.99/decisions/ece}{0.142}
\defres{tau2/airline_shadow/jev_ts_cascade_tau0.99/llm_calls}{9.64}
\defres{tau2/airline_shadow/jev_ts_cascade_tau0.99/steps}{9.84}
\defres{tau2/airline_shadow/jev_ts_cascade_tau0.99/success}{68.9}
\defres{tau2/airline_shadow/jev_ts_cascade_tau0.99/success_ci/hi}{86.7}
\defres{tau2/airline_shadow/jev_ts_cascade_tau0.99/success_ci/lo}{48.9}
\defres{tau2/airline_shadow/jev_ts_cascade_tau0.99/vs_baseline/cost_savings}{10.8}
\defres{tau2/airline_shadow/jev_ts_cascade_tau0.99/vs_baseline/delta}{+2.2}
\defres{tau2/airline_shadow/jev_ts_cascade_tau0.99/vs_baseline/delta_ci/hi}{+8.9}
\defres{tau2/airline_shadow/jev_ts_cascade_tau0.99/vs_baseline/delta_ci/lo}{-4.4}
\defres{tau2/airline_shadow/jev_ts_cascade_tau0.99/vs_baseline/ni/p_decisive}{0.464}
\defres{tau2/airline_shadow/jev_ts_cascade_tauhat_e2/cost_usd}{0.0658}
\defres{tau2/airline_shadow/jev_ts_cascade_tauhat_e2/decisions/ece}{0.142}
\defres{tau2/airline_shadow/jev_ts_cascade_tauhat_e2/llm_calls}{10.31}
\defres{tau2/airline_shadow/jev_ts_cascade_tauhat_e2/steps}{10.44}
\defres{tau2/airline_shadow/jev_ts_cascade_tauhat_e2/success}{64.4}
\defres{tau2/airline_shadow/jev_ts_cascade_tauhat_e2/success_ci/hi}{86.7}
\defres{tau2/airline_shadow/jev_ts_cascade_tauhat_e2/success_ci/lo}{42.2}
\defres{tau2/airline_shadow/jev_ts_cascade_tauhat_e2/vs_baseline/cost_savings}{4.2}
\defres{tau2/airline_shadow/jev_ts_cascade_tauhat_e2/vs_baseline/delta}{-2.2}
\defres{tau2/airline_shadow/jev_ts_cascade_tauhat_e2/vs_baseline/delta_ci/hi}{+4.4}
\defres{tau2/airline_shadow/jev_ts_cascade_tauhat_e2/vs_baseline/delta_ci/lo}{-8.9}
\defres{tau2/airline_shadow/jev_ts_cascade_tauhat_e2/vs_baseline/ni/p_decisive}{0.830}
\defres{tau2/airline_shadow/jev_ts_cascade_tauhat_refit/cost_usd}{0.101}
\defres{tau2/airline_shadow/jev_ts_cascade_tauhat_refit/decisions/ece}{0.095}
\defres{tau2/airline_shadow/jev_ts_cascade_tauhat_refit/llm_calls}{12.13}
\defres{tau2/airline_shadow/jev_ts_cascade_tauhat_refit/steps}{13.31}
\defres{tau2/airline_shadow/jev_ts_cascade_tauhat_refit/success}{60.0}
\defres{tau2/airline_shadow/jev_ts_cascade_tauhat_refit/success_ci/hi}{80.0}
\defres{tau2/airline_shadow/jev_ts_cascade_tauhat_refit/success_ci/lo}{37.8}
\defres{tau2/airline_shadow/jev_ts_cascade_tauhat_refit/vs_baseline/cost_savings}{-46.8}
\defres{tau2/airline_shadow/jev_ts_cascade_tauhat_refit/vs_baseline/delta}{-6.7}
\defres{tau2/airline_shadow/jev_ts_cascade_tauhat_refit/vs_baseline/delta_ci/hi}{+6.7}
\defres{tau2/airline_shadow/jev_ts_cascade_tauhat_refit/vs_baseline/delta_ci/lo}{-24.4}
\defres{tau2/airline_shadow/jev_ts_cascade_tauhat_refit/vs_baseline/ni/p_decisive}{0.830}
\defres{tau2/airline_shadow/llm_only/cost_usd}{0.0686}
\defres{tau2/airline_shadow/llm_only/llm_calls}{11.29}
\defres{tau2/airline_shadow/llm_only/steps}{11.29}
\defres{tau2/airline_shadow/llm_only/success}{66.7}
\defres{tau2/airline_shadow/llm_only/success_ci/hi}{86.7}
\defres{tau2/airline_shadow/llm_only/success_ci/lo}{44.4}
\defres{tau2/airline_test/headline/iso_cost/delta_ci/hi}{+20.0}
\defres{tau2/airline_test/headline/iso_cost/delta_ci/lo}{-8.6}
\defres{tau2/airline_test/headline/iso_cost/success}{77.1}
\defres{tau2/airline_test/jev_guard/cost_usd}{0.0836}
\defres{tau2/airline_test/jev_guard/llm_calls}{12.81}
\defres{tau2/airline_test/jev_guard/steps}{12.61}
\defres{tau2/airline_test/jev_guard/success}{75.2}
\defres{tau2/airline_test/jev_guard/success_ci/hi}{85.7}
\defres{tau2/airline_test/jev_guard/success_ci/lo}{63.8}
\defres{tau2/airline_test/jev_guard/vs_baseline/cost_savings}{-3.9}
\defres{tau2/airline_test/jev_guard/vs_baseline/delta}{+6.7}
\defres{tau2/airline_test/jev_guard/vs_baseline/delta_ci/hi}{+17.1}
\defres{tau2/airline_test/jev_guard/vs_baseline/delta_ci/lo}{-3.8}
\defres{tau2/airline_test/jev_guard/vs_baseline/ni/p_decisive}{0.374}
\defres{tau2/airline_test/jev_ts_assist_k3/cost_usd}{0.0878}
\defres{tau2/airline_test/jev_ts_assist_k3/decisions/ece}{0.168}
\defres{tau2/airline_test/jev_ts_assist_k3/llm_calls}{12.80}
\defres{tau2/airline_test/jev_ts_assist_k3/steps}{12.80}
\defres{tau2/airline_test/jev_ts_assist_k3/success}{64.8}
\defres{tau2/airline_test/jev_ts_assist_k3/success_ci/hi}{78.1}
\defres{tau2/airline_test/jev_ts_assist_k3/success_ci/lo}{50.5}
\defres{tau2/airline_test/jev_ts_assist_k3/vs_baseline/cost_savings}{-9.2}
\defres{tau2/airline_test/jev_ts_assist_k3/vs_baseline/delta}{-3.8}
\defres{tau2/airline_test/jev_ts_assist_k3/vs_baseline/delta_ci/hi}{+5.7}
\defres{tau2/airline_test/jev_ts_assist_k3/vs_baseline/delta_ci/lo}{-13.3}
\defres{tau2/airline_test/jev_ts_assist_k3/vs_baseline/ni/p_decisive}{0.701}
\defres{tau2/airline_test/jev_ts_cascade_tau0.5/cost_usd}{0.1}
\defres{tau2/airline_test/jev_ts_cascade_tau0.5/decisions/ece}{0.191}
\defres{tau2/airline_test/jev_ts_cascade_tau0.5/llm_calls}{11.11}
\defres{tau2/airline_test/jev_ts_cascade_tau0.5/steps}{15.23}
\defres{tau2/airline_test/jev_ts_cascade_tau0.5/success}{56.2}
\defres{tau2/airline_test/jev_ts_cascade_tau0.5/success_ci/hi}{69.5}
\defres{tau2/airline_test/jev_ts_cascade_tau0.5/success_ci/lo}{41.9}
\defres{tau2/airline_test/jev_ts_cascade_tau0.5/vs_baseline/cost_savings}{-24.4}
\defres{tau2/airline_test/jev_ts_cascade_tau0.5/vs_baseline/delta}{-12.4}
\defres{tau2/airline_test/jev_ts_cascade_tau0.5/vs_baseline/delta_ci/hi}{-1.0}
\defres{tau2/airline_test/jev_ts_cascade_tau0.5/vs_baseline/delta_ci/lo}{-24.8}
\defres{tau2/airline_test/jev_ts_cascade_tau0.5/vs_baseline/ni/p_decisive}{0.950}
\defres{tau2/airline_test/jev_ts_cascade_tau0.7/cost_usd}{0.0852}
\defres{tau2/airline_test/jev_ts_cascade_tau0.7/decisions/ece}{0.131}
\defres{tau2/airline_test/jev_ts_cascade_tau0.7/llm_calls}{10.22}
\defres{tau2/airline_test/jev_ts_cascade_tau0.7/steps}{12.31}
\defres{tau2/airline_test/jev_ts_cascade_tau0.7/success}{60.0}
\defres{tau2/airline_test/jev_ts_cascade_tau0.7/success_ci/hi}{72.4}
\defres{tau2/airline_test/jev_ts_cascade_tau0.7/success_ci/lo}{46.7}
\defres{tau2/airline_test/jev_ts_cascade_tau0.7/vs_baseline/cost_savings}{-5.8}
\defres{tau2/airline_test/jev_ts_cascade_tau0.7/vs_baseline/delta}{-8.6}
\defres{tau2/airline_test/jev_ts_cascade_tau0.7/vs_baseline/delta_ci/hi}{+2.9}
\defres{tau2/airline_test/jev_ts_cascade_tau0.7/vs_baseline/delta_ci/lo}{-19.0}
\defres{tau2/airline_test/jev_ts_cascade_tau0.7/vs_baseline/ni/p_decisive}{0.875}
\defres{tau2/airline_test/jev_ts_cascade_tau0.8/cost_usd}{0.0863}
\defres{tau2/airline_test/jev_ts_cascade_tau0.8/decisions/ece}{0.171}
\defres{tau2/airline_test/jev_ts_cascade_tau0.8/llm_calls}{10.53}
\defres{tau2/airline_test/jev_ts_cascade_tau0.8/steps}{12.07}
\defres{tau2/airline_test/jev_ts_cascade_tau0.8/success}{60.0}
\defres{tau2/airline_test/jev_ts_cascade_tau0.8/success_ci/hi}{72.4}
\defres{tau2/airline_test/jev_ts_cascade_tau0.8/success_ci/lo}{46.7}
\defres{tau2/airline_test/jev_ts_cascade_tau0.8/vs_baseline/cost_savings}{-7.2}
\defres{tau2/airline_test/jev_ts_cascade_tau0.8/vs_baseline/delta}{-8.6}
\defres{tau2/airline_test/jev_ts_cascade_tau0.8/vs_baseline/delta_ci/hi}{+1.9}
\defres{tau2/airline_test/jev_ts_cascade_tau0.8/vs_baseline/delta_ci/lo}{-18.1}
\defres{tau2/airline_test/jev_ts_cascade_tau0.8/vs_baseline/ni/p_decisive}{0.687}
\defres{tau2/airline_test/jev_ts_cascade_tau0.9/cost_usd}{0.095}
\defres{tau2/airline_test/jev_ts_cascade_tau0.9/decisions/ece}{0.142}
\defres{tau2/airline_test/jev_ts_cascade_tau0.9/llm_calls}{11.33}
\defres{tau2/airline_test/jev_ts_cascade_tau0.9/steps}{12.22}
\defres{tau2/airline_test/jev_ts_cascade_tau0.9/success}{65.7}
\defres{tau2/airline_test/jev_ts_cascade_tau0.9/success_ci/hi}{78.1}
\defres{tau2/airline_test/jev_ts_cascade_tau0.9/success_ci/lo}{53.3}
\defres{tau2/airline_test/jev_ts_cascade_tau0.9/vs_baseline/cost_savings}{-18.1}
\defres{tau2/airline_test/jev_ts_cascade_tau0.9/vs_baseline/delta}{-2.9}
\defres{tau2/airline_test/jev_ts_cascade_tau0.9/vs_baseline/delta_ci/hi}{+5.7}
\defres{tau2/airline_test/jev_ts_cascade_tau0.9/vs_baseline/delta_ci/lo}{-10.5}
\defres{tau2/airline_test/jev_ts_cascade_tau0.9/vs_baseline/ni/p_decisive}{0.736}
\defres{tau2/airline_test/jev_ts_cascade_tau0.95/cost_usd}{0.0959}
\defres{tau2/airline_test/jev_ts_cascade_tau0.95/decisions/ece}{0.209}
\defres{tau2/airline_test/jev_ts_cascade_tau0.95/llm_calls}{11.98}
\defres{tau2/airline_test/jev_ts_cascade_tau0.95/steps}{12.49}
\defres{tau2/airline_test/jev_ts_cascade_tau0.95/success}{68.6}
\defres{tau2/airline_test/jev_ts_cascade_tau0.95/success_ci/hi}{80.0}
\defres{tau2/airline_test/jev_ts_cascade_tau0.95/success_ci/lo}{56.2}
\defres{tau2/airline_test/jev_ts_cascade_tau0.95/vs_baseline/cost_savings}{-19.2}
\defres{tau2/airline_test/jev_ts_cascade_tau0.95/vs_baseline/delta}{+0.0}
\defres{tau2/airline_test/jev_ts_cascade_tau0.95/vs_baseline/delta_ci/hi}{+8.6}
\defres{tau2/airline_test/jev_ts_cascade_tau0.95/vs_baseline/delta_ci/lo}{-8.6}
\defres{tau2/airline_test/jev_ts_cascade_tau0.95/vs_baseline/ni/p_decisive}{0.736}
\defres{tau2/airline_test/jev_ts_cascade_tau0.99/cost_usd}{0.0849}
\defres{tau2/airline_test/jev_ts_cascade_tau0.99/decisions/ece}{0.182}
\defres{tau2/airline_test/jev_ts_cascade_tau0.99/llm_calls}{12.33}
\defres{tau2/airline_test/jev_ts_cascade_tau0.99/steps}{12.64}
\defres{tau2/airline_test/jev_ts_cascade_tau0.99/success}{65.7}
\defres{tau2/airline_test/jev_ts_cascade_tau0.99/success_ci/hi}{79.0}
\defres{tau2/airline_test/jev_ts_cascade_tau0.99/success_ci/lo}{51.4}
\defres{tau2/airline_test/jev_ts_cascade_tau0.99/vs_baseline/cost_savings}{-5.5}
\defres{tau2/airline_test/jev_ts_cascade_tau0.99/vs_baseline/delta}{-2.9}
\defres{tau2/airline_test/jev_ts_cascade_tau0.99/vs_baseline/delta_ci/hi}{+6.7}
\defres{tau2/airline_test/jev_ts_cascade_tau0.99/vs_baseline/delta_ci/lo}{-11.4}
\defres{tau2/airline_test/jev_ts_cascade_tau0.99/vs_baseline/ni/p_decisive}{0.378}
\defres{tau2/airline_test/jev_ts_cascade_tauhat_e2/cost_usd}{0.0759}
\defres{tau2/airline_test/jev_ts_cascade_tauhat_e2/decisions/ece}{0.160}
\defres{tau2/airline_test/jev_ts_cascade_tauhat_e2/llm_calls}{11.45}
\defres{tau2/airline_test/jev_ts_cascade_tauhat_e2/steps}{11.60}
\defres{tau2/airline_test/jev_ts_cascade_tauhat_e2/success}{73.3}
\defres{tau2/airline_test/jev_ts_cascade_tauhat_e2/success_ci/hi}{84.8}
\defres{tau2/airline_test/jev_ts_cascade_tauhat_e2/success_ci/lo}{61.9}
\defres{tau2/airline_test/jev_ts_cascade_tauhat_e2/vs_baseline/cost_savings}{5.7}
\defres{tau2/airline_test/jev_ts_cascade_tauhat_e2/vs_baseline/delta}{+4.8}
\defres{tau2/airline_test/jev_ts_cascade_tauhat_e2/vs_baseline/delta_ci/hi}{+14.3}
\defres{tau2/airline_test/jev_ts_cascade_tauhat_e2/vs_baseline/delta_ci/lo}{-4.8}
\defres{tau2/airline_test/jev_ts_cascade_tauhat_e2/vs_baseline/ni/p_decisive}{0.075}
\defres{tau2/airline_test/jev_ts_cascade_tauhat_refit/cost_usd}{0.0962}
\defres{tau2/airline_test/jev_ts_cascade_tauhat_refit/decisions/ece}{0.125}
\defres{tau2/airline_test/jev_ts_cascade_tauhat_refit/llm_calls}{11.60}
\defres{tau2/airline_test/jev_ts_cascade_tauhat_refit/steps}{12.86}
\defres{tau2/airline_test/jev_ts_cascade_tauhat_refit/success}{61.0}
\defres{tau2/airline_test/jev_ts_cascade_tauhat_refit/success_ci/hi}{74.3}
\defres{tau2/airline_test/jev_ts_cascade_tauhat_refit/success_ci/lo}{47.6}
\defres{tau2/airline_test/jev_ts_cascade_tauhat_refit/vs_baseline/cost_savings}{-19.5}
\defres{tau2/airline_test/jev_ts_cascade_tauhat_refit/vs_baseline/delta}{-7.6}
\defres{tau2/airline_test/jev_ts_cascade_tauhat_refit/vs_baseline/delta_ci/hi}{+4.8}
\defres{tau2/airline_test/jev_ts_cascade_tauhat_refit/vs_baseline/delta_ci/lo}{-21.0}
\defres{tau2/airline_test/jev_ts_cascade_tauhat_refit/vs_baseline/ni/p_decisive}{0.875}
\defres{tau2/airline_test/llm_only/cost_usd}{0.0805}
\defres{tau2/airline_test/llm_only/llm_calls}{12.57}
\defres{tau2/airline_test/llm_only/steps}{12.57}
\defres{tau2/airline_test/llm_only/success}{68.6}
\defres{tau2/airline_test/llm_only/success_ci/hi}{81.9}
\defres{tau2/airline_test/llm_only/success_ci/lo}{54.3}
\defres{tau2/retail/headline/iso_cost/success}{64.0}
\defres{tau2/retail/jev_ts_cascade_tauhat_e2/cost_usd}{0.0816}
\defres{tau2/retail/jev_ts_cascade_tauhat_e2/decisions/ece}{0.175}
\defres{tau2/retail/jev_ts_cascade_tauhat_e2/llm_calls}{11.56}
\defres{tau2/retail/jev_ts_cascade_tauhat_e2/steps}{11.67}
\defres{tau2/retail/jev_ts_cascade_tauhat_e2/success}{63.5}
\defres{tau2/retail/jev_ts_cascade_tauhat_e2/success_ci/hi}{69.6}
\defres{tau2/retail/jev_ts_cascade_tauhat_e2/success_ci/lo}{56.7}
\defres{tau2/retail/jev_ts_cascade_tauhat_e2/vs_baseline/cost_savings}{-9.0}
\defres{tau2/retail/jev_ts_cascade_tauhat_e2/vs_baseline/delta}{+0.9}
\defres{tau2/retail/jev_ts_cascade_tauhat_e2/vs_baseline/delta_ci/hi}{+6.7}
\defres{tau2/retail/jev_ts_cascade_tauhat_e2/vs_baseline/delta_ci/lo}{-4.7}
\defres{tau2/retail/jev_ts_cascade_tauhat_e2/vs_baseline/ni/p_decisive}{0.347}
\defres{tau2/retail/jev_ts_cascade_tauhat_refit/cost_usd}{0.0882}
\defres{tau2/retail/jev_ts_cascade_tauhat_refit/decisions/ece}{0.147}
\defres{tau2/retail/jev_ts_cascade_tauhat_refit/llm_calls}{10.75}
\defres{tau2/retail/jev_ts_cascade_tauhat_refit/steps}{11.55}
\defres{tau2/retail/jev_ts_cascade_tauhat_refit/success}{58.5}
\defres{tau2/retail/jev_ts_cascade_tauhat_refit/success_ci/hi}{64.9}
\defres{tau2/retail/jev_ts_cascade_tauhat_refit/success_ci/lo}{52.0}
\defres{tau2/retail/jev_ts_cascade_tauhat_refit/vs_baseline/cost_savings}{-17.7}
\defres{tau2/retail/jev_ts_cascade_tauhat_refit/vs_baseline/delta}{-4.1}
\defres{tau2/retail/jev_ts_cascade_tauhat_refit/vs_baseline/delta_ci/hi}{+2.0}
\defres{tau2/retail/jev_ts_cascade_tauhat_refit/vs_baseline/delta_ci/lo}{-9.9}
\defres{tau2/retail/jev_ts_cascade_tauhat_refit/vs_baseline/ni/p_decisive}{0.610}
\defres{tau2/retail/llm_only/cost_usd}{0.0749}
\defres{tau2/retail/llm_only/llm_calls}{11.63}
\defres{tau2/retail/llm_only/steps}{11.63}
\defres{tau2/retail/llm_only/success}{62.6}
\defres{tau2/retail/llm_only/success_ci/hi}{68.7}
\defres{tau2/retail/llm_only/success_ci/lo}{56.4}
\makeatother


==> generated/secondary.tex <==
\makeatletter
\providecommand{\res}[1]{\ifcsname jevres@#1\endcsname\csname jevres@#1\endcsname\else\tbd\fi}
\providecommand{\defres}[2]{\expandafter\def\csname jevres@#1\endcsname{#2}}
\defres{calibration/c1/intern/flash/tool_params/tauhat}{0.6309}
\defres{calibration/c1/intern/flash/tool_select/tauhat}{always defer}
\defres{calibration/c1/intern/lite/tool_params/tauhat}{0.8518}
\defres{calibration/c1/intern/lite/tool_select/tauhat}{always defer}
\defres{calibration/c1/jev/flash/tool_params/tauhat}{0.99}
\defres{calibration/c1/jev/flash/tool_select/tauhat}{1.00}
\defres{calibration/c1/jev/lite/tool_params/tauhat}{0.13}
\defres{calibration/c1/jev/lite/tool_select/tauhat}{always defer}
\defres{secondary/h1/ci_above_0}{66}
\defres{secondary/h1/ci_below_0}{0}
\defres{secondary/h1/clause1}{holds}
\defres{secondary/h1/clause2}{does not hold}
\defres{secondary/h1/clause2/n_cells}{8}
\defres{secondary/h1/clause2/n_over_confident}{3}
\defres{secondary/h1/clause2/n_return}{0}
\defres{secondary/h1/clause2/over_confident_cells}{\jev{} arguments (Flash); Intern-Decision tool selection (Flash); Intern-Decision tool selection (Flash-Lite)}
\defres{secondary/h1/losses}{2}
\defres{secondary/h1/n_absent}{0}
\defres{secondary/h1/n_cells}{72}
\defres{secondary/h1/n_estimable}{72}
\defres{secondary/h1/n_v_w}{72}
\defres{secondary/h1/projection/losses}{8}
\defres{secondary/h1/projection/ties}{0}
\defres{secondary/h1/projection/wins}{64}
\defres{secondary/h1/ties}{0}
\defres{secondary/h1/verdict}{falsified}
\defres{secondary/h1/wins}{70}
\defres{secondary/h3/absent}{ALFWorld (E6 not run)}
\defres{secondary/h3/counterexample/copy_share}{9.7}
\defres{secondary/h3/counterexample/cost_savings}{14.2}
\defres{secondary/h3/counterexample/credited}{irreversible, copy-dependent, bounded-recoverable}
\defres{secondary/h3/counterexample/delta}{+0.0}
\defres{secondary/h3/counterexample/irreversible_share}{14.1}
\defres{secondary/h3/counterexample/n}{500}
\defres{secondary/h3/n_counterexamples}{1}
\defres{secondary/h3/n_credited/l2_flash}{48}
\defres{secondary/h3/n_credited/l2_lite}{9}
\defres{secondary/h3/n_credited/l3_flash}{8}
\defres{secondary/h3/n_negligible}{4}
\defres{secondary/h3/n_qualifying/l2_flash}{13}
\defres{secondary/h3/n_qualifying/l2_lite}{5}
\defres{secondary/h3/n_qualifying/l3_flash}{0}
\defres{secondary/h3/n_universe}{69}
\defres{secondary/h3/tau_b/flash_vs_lite/p}{0.500}
\defres{secondary/h3/tau_b/flash_vs_lite/value}{+0.55}
\defres{secondary/h3/tau_b/l2_vs_l3/p}{--}
\defres{secondary/h3/tau_b/l2_vs_l3/value}{undefined}
\defres{secondary/h3/verdict}{falsified}
\defres{secondary/h4/verdict}{not tested at matched accuracy}
\defres{secondary/proxy/delta_success/p}{0.008}
\defres{secondary/proxy/delta_success/p_two}{0.016}
\defres{secondary/proxy/delta_success/tau_b}{+0.66}
\defres{secondary/proxy/delta_success_pass1/p}{0.015}
\defres{secondary/proxy/delta_success_pass1/p_two}{0.030}
\defres{secondary/proxy/delta_success_pass1/tau_b}{+0.61}
\defres{secondary/proxy/delta_success_pass1_sens/p}{0.005}
\defres{secondary/proxy/delta_success_pass1_sens/p_two}{0.009}
\defres{secondary/proxy/delta_success_pass1_sens/tau_b}{+0.66}
\defres{secondary/proxy/delta_success_sens/p}{0.003}
\defres{secondary/proxy/delta_success_sens/p_two}{0.005}
\defres{secondary/proxy/delta_success_sens/tau_b}{+0.70}
\defres{secondary/proxy/iso_quality_savings/p}{0.111}
\defres{secondary/proxy/iso_quality_savings/p_two}{0.111}
\defres{secondary/proxy/iso_quality_savings/tau_b}{+0.73}
\defres{secondary/proxy/iso_quality_savings_sens/p}{0.200}
\defres{secondary/proxy/iso_quality_savings_sens/p_two}{0.200}
\defres{secondary/proxy/iso_quality_savings_sens/tau_b}{+0.48}
\defres{secondary/proxy/n}{9}
\defres{secondary/proxy/n_qualifying_e2}{1}
\defres{secondary/proxy/n_qualifying_tau2}{0}
\defres{secondary/proxy/n_sens}{10}
\defres{secondary/proxy/net_cost_savings/p}{0.978}
\defres{secondary/proxy/net_cost_savings/p_two}{0.075}
\defres{secondary/proxy/net_cost_savings/tau_b}{-0.50}
\defres{secondary/proxy/net_cost_savings_sens/p}{0.986}
\defres{secondary/proxy/net_cost_savings_sens/p_two}{0.047}
\defres{secondary/proxy/net_cost_savings_sens/tau_b}{-0.51}
\defres{tau2/refit/tool_params/n_paired}{115}
\defres{tau2/refit/tool_params/tauhat}{1.00}
\defres{tau2/refit/tool_select/n_paired}{488}
\defres{tau2/refit/tool_select/tauhat}{0.28}
\makeatother


==> generated/stage2.tex <==
\makeatletter
\providecommand{\res}[1]{\ifcsname jevres@#1\endcsname\csname jevres@#1\endcsname\else\tbd\fi}
\providecommand{\defres}[2]{\expandafter\def\csname jevres@#1\endcsname{#2}}
\defres{stage2/S2-1/alpha_adj}{0.025}
\defres{stage2/S2-1/cost/boundary}{0}
\defres{stage2/S2-1/cost/decision}{cost saving established}
\defres{stage2/S2-1/cost/est}{0.0168}
\defres{stage2/S2-1/cost/est_ci/hi}{0.0179}
\defres{stage2/S2-1/cost/est_ci/lo}{0.0157}
\defres{stage2/S2-1/cost/p}{$<$0.001}
\defres{stage2/S2-1/cost_arm}{0.0245}
\defres{stage2/S2-1/cost_ref}{0.0413}
\defres{stage2/S2-1/cost_savings}{40.7}
\defres{stage2/S2-1/cost_savings_ci/hi}{42.5}
\defres{stage2/S2-1/cost_savings_ci/lo}{38.9}
\defres{stage2/S2-1/coverage/arg_coverage}{51.4}
\defres{stage2/S2-1/coverage/tool_coverage}{52.5}
\defres{stage2/S2-1/decision}{not rejected: the registered joint claim was not established}
\defres{stage2/S2-1/delta}{-2.2}
\defres{stage2/S2-1/delta_ci/hi}{-0.8}
\defres{stage2/S2-1/delta_ci/lo}{-3.8}
\defres{stage2/S2-1/holm_rank}{3}
\defres{stage2/S2-1/n_dropped}{0}
\defres{stage2/S2-1/n_expected}{500}
\defres{stage2/S2-1/n_pairs}{500}
\defres{stage2/S2-1/ni/boundary}{-3.0}
\defres{stage2/S2-1/ni/decision}{not NI: loss of 2.2 pt (95 \% CI entirely below 0)}
\defres{stage2/S2-1/ni/discordance}{3.0}
\defres{stage2/S2-1/ni/est}{-2.2}
\defres{stage2/S2-1/ni/est_ci/hi}{-0.8}
\defres{stage2/S2-1/ni/est_ci/lo}{-3.8}
\defres{stage2/S2-1/ni/est_ci_newcombe/hi}{-0.6}
\defres{stage2/S2-1/ni/est_ci_newcombe/lo}{-4.1}
\defres{stage2/S2-1/ni/losses}{13}
\defres{stage2/S2-1/ni/p}{0.178}
\defres{stage2/S2-1/ni/success_arm}{97.2}
\defres{stage2/S2-1/ni/success_ref}{99.4}
\defres{stage2/S2-1/ni/wins}{2}
\defres{stage2/S2-1/p_decisive}{0.178}
\defres{stage2/S2-1/p_holm}{0.356}
\defres{stage2/S2-1L/alpha_adj}{0.013}
\defres{stage2/S2-1L/decision}{not tested (no decision point qualified in Stage 1; the best-practice profile is LLM-only) -- A7.1 (g) 5}
\defres{stage2/S2-1L/holm_rank}{3}
\defres{stage2/S2-1L/p_decisive}{1.000}
\defres{stage2/S2-1L/p_holm}{1.000}
\defres{stage2/S2-1T/alpha_adj}{0.017}
\defres{stage2/S2-1T/decision}{not rejected: the registered joint claim was not established}
\defres{stage2/S2-1T/delta}{-2.54}
\defres{stage2/S2-1T/delta_ci/hi}{-2.21}
\defres{stage2/S2-1T/delta_ci/lo}{-2.87}
\defres{stage2/S2-1T/holm_rank}{4}
\defres{stage2/S2-1T/latency/boundary}{0}
\defres{stage2/S2-1T/latency/decision}{the wrong direction: latency saving reversed (95 \% CI entirely below 0)}
\defres{stage2/S2-1T/latency/est}{-2.54}
\defres{stage2/S2-1T/latency/est_ci/hi}{-2.21}
\defres{stage2/S2-1T/latency/est_ci/lo}{-2.87}
\defres{stage2/S2-1T/latency/p}{1.000}
\defres{stage2/S2-1T/latency_arm_s}{9.35}
\defres{stage2/S2-1T/latency_ref_s}{6.8}
\defres{stage2/S2-1T/latency_savings}{-37.4}
\defres{stage2/S2-1T/n_dropped}{0}
\defres{stage2/S2-1T/n_expected}{500}
\defres{stage2/S2-1T/n_pairs}{500}
\defres{stage2/S2-1T/p_decisive}{1.000}
\defres{stage2/S2-1T/p_holm}{1.000}
\defres{stage2/S2-1X/alpha_adj}{0.025}
\defres{stage2/S2-1X/cost/boundary}{0}
\defres{stage2/S2-1X/cost/decision}{the wrong direction: cost saving reversed (95 \% CI entirely below 0)}
\defres{stage2/S2-1X/cost/est}{-0.000423}
\defres{stage2/S2-1X/cost/est_ci/hi}{-0.000394}
\defres{stage2/S2-1X/cost/est_ci/lo}{-0.000452}
\defres{stage2/S2-1X/cost/p}{1.000}
\defres{stage2/S2-1X/cost_arm}{0.00246}
\defres{stage2/S2-1X/cost_ref}{0.00203}
\defres{stage2/S2-1X/cost_savings}{-20.8}
\defres{stage2/S2-1X/cost_savings_ci/hi}{-19.6}
\defres{stage2/S2-1X/cost_savings_ci/lo}{-22.0}
\defres{stage2/S2-1X/coverage/arg_coverage}{0.0}
\defres{stage2/S2-1X/coverage/tool_coverage}{0.0}
\defres{stage2/S2-1X/decision}{not rejected: the registered joint claim was not established}
\defres{stage2/S2-1X/delta}{+7.2}
\defres{stage2/S2-1X/delta_ci/hi}{+10.6}
\defres{stage2/S2-1X/delta_ci/lo}{+3.8}
\defres{stage2/S2-1X/holm_rank}{5}
\defres{stage2/S2-1X/n_dropped}{0}
\defres{stage2/S2-1X/n_expected}{500}
\defres{stage2/S2-1X/n_pairs}{500}
\defres{stage2/S2-1X/ni/boundary}{-3.0}
\defres{stage2/S2-1X/ni/decision}{NI}
\defres{stage2/S2-1X/ni/discordance}{15.2}
\defres{stage2/S2-1X/ni/est}{+7.2}
\defres{stage2/S2-1X/ni/est_ci/hi}{+10.6}
\defres{stage2/S2-1X/ni/est_ci/lo}{+3.8}
\defres{stage2/S2-1X/ni/est_ci_newcombe/hi}{+10.6}
\defres{stage2/S2-1X/ni/est_ci_newcombe/lo}{+3.8}
\defres{stage2/S2-1X/ni/losses}{20}
\defres{stage2/S2-1X/ni/p}{$<$0.001}
\defres{stage2/S2-1X/ni/success_arm}{85.4}
\defres{stage2/S2-1X/ni/success_ref}{78.2}
\defres{stage2/S2-1X/ni/wins}{56}
\defres{stage2/S2-1X/p_decisive}{1.000}
\defres{stage2/S2-1X/p_holm}{1.000}
\defres{stage2/S2-2/alpha_adj}{0.050}
\defres{stage2/S2-2/cost/boundary}{0}
\defres{stage2/S2-2/cost/decision}{cost saving established}
\defres{stage2/S2-2/cost/est}{0.00907}
\defres{stage2/S2-2/cost/est_ci/hi}{0.0101}
\defres{stage2/S2-2/cost/est_ci/lo}{0.00805}
\defres{stage2/S2-2/cost/p}{$<$0.001}
\defres{stage2/S2-2/cost_arm}{0.0245}
\defres{stage2/S2-2/cost_ref}{0.0335}
\defres{stage2/S2-2/cost_savings}{27.0}
\defres{stage2/S2-2/cost_savings_ci/hi}{29.4}
\defres{stage2/S2-2/cost_savings_ci/lo}{24.6}
\defres{stage2/S2-2/coverage/arg_coverage}{51.4}
\defres{stage2/S2-2/coverage/tool_coverage}{52.5}
\defres{stage2/S2-2/decision}{not rejected: the registered joint claim was not established}
\defres{stage2/S2-2/delta}{-2.6}
\defres{stage2/S2-2/delta_ci/hi}{-1.2}
\defres{stage2/S2-2/delta_ci/lo}{-4.2}
\defres{stage2/S2-2/holm_rank}{4}
\defres{stage2/S2-2/n_dropped}{0}
\defres{stage2/S2-2/n_expected}{500}
\defres{stage2/S2-2/n_pairs}{500}
\defres{stage2/S2-2/ni/boundary}{-3.0}
\defres{stage2/S2-2/ni/decision}{not NI: loss of 2.6 pt (95 \% CI entirely below 0)}
\defres{stage2/S2-2/ni/discordance}{3.0}
\defres{stage2/S2-2/ni/est}{-2.6}
\defres{stage2/S2-2/ni/est_ci/hi}{-1.2}
\defres{stage2/S2-2/ni/est_ci/lo}{-4.2}
\defres{stage2/S2-2/ni/est_ci_newcombe/hi}{-1.1}
\defres{stage2/S2-2/ni/est_ci_newcombe/lo}{-4.5}
\defres{stage2/S2-2/ni/losses}{14}
\defres{stage2/S2-2/ni/p}{0.326}
\defres{stage2/S2-2/ni/success_arm}{97.2}
\defres{stage2/S2-2/ni/success_ref}{99.8}
\defres{stage2/S2-2/ni/wins}{1}
\defres{stage2/S2-2/p_decisive}{0.326}
\defres{stage2/S2-2/p_holm}{0.356}
\defres{stage2/S2-3/accuracy/intern}{75.2}
\defres{stage2/S2-3/accuracy/jev}{91.5}
\defres{stage2/S2-3/accuracy/rl}{99.2}
\defres{stage2/S2-3/alpha_adj}{0.013}
\defres{stage2/S2-3/corpus/eligible_tasks}{200}
\defres{stage2/S2-3/corpus/excluded}{0}
\defres{stage2/S2-3/corpus/occurrences}{5314}
\defres{stage2/S2-3/corpus/tasks}{200}
\defres{stage2/S2-3/corpus/unique_questions}{3939}
\defres{stage2/S2-3/decision}{rejects: the claim holds}
\defres{stage2/S2-3/delta}{+24.0}
\defres{stage2/S2-3/delta_ci/hi}{+25.9}
\defres{stage2/S2-3/delta_ci/lo}{+22.1}
\defres{stage2/S2-3/delta_jev}{+7.7}
\defres{stage2/S2-3/delta_jev_ci/hi}{+9.1}
\defres{stage2/S2-3/delta_jev_ci/lo}{+6.3}
\defres{stage2/S2-3/holm_rank}{1}
\defres{stage2/S2-3/intern/boundary}{+0.0}
\defres{stage2/S2-3/intern/decision}{accuracy gain over Intern-Decision-4B established}
\defres{stage2/S2-3/intern/est}{+24.0}
\defres{stage2/S2-3/intern/est_ci/hi}{+25.9}
\defres{stage2/S2-3/intern/est_ci/lo}{+22.1}
\defres{stage2/S2-3/intern/est_ci_boot/hi}{+25.9}
\defres{stage2/S2-3/intern/est_ci_boot/lo}{+22.1}
\defres{stage2/S2-3/intern/p}{$<$0.001}
\defres{stage2/S2-3/jev/boundary}{-5.0}
\defres{stage2/S2-3/jev/decision}{non-inferiority to Jev (no more than 5 pt less accurate) established}
\defres{stage2/S2-3/jev/est}{+7.7}
\defres{stage2/S2-3/jev/est_ci/hi}{+9.1}
\defres{stage2/S2-3/jev/est_ci/lo}{+6.3}
\defres{stage2/S2-3/jev/est_ci_boot/hi}{+9.2}
\defres{stage2/S2-3/jev/est_ci_boot/lo}{+6.3}
\defres{stage2/S2-3/jev/p}{$<$0.001}
\defres{stage2/S2-3/n_eligible}{200}
\defres{stage2/S2-3/n_excluded}{0}
\defres{stage2/S2-3/n_pairs}{200}
\defres{stage2/S2-3/p_decisive}{$<$0.001}
\defres{stage2/S2-3/p_holm}{$<$0.001}
\defres{stage2/S2-3/strata/after_off_plan/intern}{47.6}
\defres{stage2/S2-3/strata/after_off_plan/jev}{81.5}
\defres{stage2/S2-3/strata/after_off_plan/occurrences}{386}
\defres{stage2/S2-3/strata/after_off_plan/rl}{94.7}
\defres{stage2/S2-3/strata/after_off_plan/tasks}{57}
\defres{stage2/S2-3/strata/llm_only_source/intern}{76.3}
\defres{stage2/S2-3/strata/llm_only_source/jev}{92.0}
\defres{stage2/S2-3/strata/llm_only_source/occurrences}{1{,}498}
\defres{stage2/S2-3/strata/llm_only_source/rl}{100.0}
\defres{stage2/S2-3/strata/llm_only_source/tasks}{200}
\defres{stage2/S2-3/strata/on_plan/intern}{76.1}
\defres{stage2/S2-3/strata/on_plan/jev}{92.0}
\defres{stage2/S2-3/strata/on_plan/occurrences}{4{,}928}
\defres{stage2/S2-3/strata/on_plan/rl}{99.9}
\defres{stage2/S2-3/strata/on_plan/tasks}{200}
\defres{stage2/S2-4/alpha_adj}{0.017}
\defres{stage2/S2-4/cost/boundary}{0}
\defres{stage2/S2-4/cost/decision}{cost saving established}
\defres{stage2/S2-4/cost/est}{0.0335}
\defres{stage2/S2-4/cost/est_ci/hi}{0.0345}
\defres{stage2/S2-4/cost/est_ci/lo}{0.0325}
\defres{stage2/S2-4/cost/p}{$<$0.001}
\defres{stage2/S2-4/cost_arm}{0.00779}
\defres{stage2/S2-4/cost_ref}{0.0413}
\defres{stage2/S2-4/cost_savings}{81.1}
\defres{stage2/S2-4/cost_savings_ci/hi}{81.6}
\defres{stage2/S2-4/cost_savings_ci/lo}{80.7}
\defres{stage2/S2-4/coverage/arg_coverage}{75.0}
\defres{stage2/S2-4/coverage/tool_coverage}{99.9}
\defres{stage2/S2-4/decision}{rejects: the claim holds}
\defres{stage2/S2-4/delta}{+0.6}
\defres{stage2/S2-4/delta_ci/hi}{+1.4}
\defres{stage2/S2-4/delta_ci/lo}{+0.0}
\defres{stage2/S2-4/holm_rank}{2}
\defres{stage2/S2-4/n_dropped}{0}
\defres{stage2/S2-4/n_expected}{500}
\defres{stage2/S2-4/n_pairs}{500}
\defres{stage2/S2-4/ni/boundary}{-3.0}
\defres{stage2/S2-4/ni/decision}{NI}
\defres{stage2/S2-4/ni/discordance}{0.6}
\defres{stage2/S2-4/ni/est}{+0.6}
\defres{stage2/S2-4/ni/est_ci/hi}{+1.4}
\defres{stage2/S2-4/ni/est_ci/lo}{+0.0}
\defres{stage2/S2-4/ni/est_ci_newcombe/hi}{+1.7}
\defres{stage2/S2-4/ni/est_ci_newcombe/lo}{-0.3}
\defres{stage2/S2-4/ni/loss_rate_ub}{0.6}
\defres{stage2/S2-4/ni/losses}{0}
\defres{stage2/S2-4/ni/p}{$<$0.001}
\defres{stage2/S2-4/ni/success_arm}{100.0}
\defres{stage2/S2-4/ni/success_ref}{99.4}
\defres{stage2/S2-4/ni/wins}{3}
\defres{stage2/S2-4/p_decisive}{$<$0.001}
\defres{stage2/S2-4/p_holm}{$<$0.001}
\defres{stage2/S2-4/tariff/busy_throughput/cost_savings}{82.1}
\defres{stage2/S2-4/tariff/busy_throughput/p_cost}{$<$0.001}
\defres{stage2/S2-4/tariff/busy_throughput/q}{0.00155}
\defres{stage2/S2-4/tariff/jev_api_price/cost_savings}{83.8}
\defres{stage2/S2-4/tariff/jev_api_price/p_cost}{$<$0.001}
\defres{stage2/S2-4/tariff/jev_api_price/q}{0.000875}
\defres{stage2/S2-4/tariff/q}{0.00196}
\defres{stage2/S2-4/tariff/zero/cost_savings}{85.9}
\defres{stage2/S2-4/tariff/zero/p_cost}{$<$0.001}
\defres{stage2/S2-4/tariff/zero/q}{0}
\defres{stage2/S2-4S/alpha_adj}{0.010}
\defres{stage2/S2-4S/cost/boundary}{0}
\defres{stage2/S2-4S/cost/decision}{the wrong direction: cost saving reversed (95 \% CI entirely below 0)}
\defres{stage2/S2-4S/cost/est}{-0.000594}
\defres{stage2/S2-4S/cost/est_ci/hi}{-0.00018}
\defres{stage2/S2-4S/cost/est_ci/lo}{-0.00101}
\defres{stage2/S2-4S/cost/p}{0.997}
\defres{stage2/S2-4S/cost_arm}{0.0419}
\defres{stage2/S2-4S/cost_ref}{0.0413}
\defres{stage2/S2-4S/cost_savings}{-1.4}
\defres{stage2/S2-4S/cost_savings_ci/hi}{-0.4}
\defres{stage2/S2-4S/cost_savings_ci/lo}{-2.5}
\defres{stage2/S2-4S/coverage/arg_coverage}{6.8}
\defres{stage2/S2-4S/coverage/tool_coverage}{17.3}
\defres{stage2/S2-4S/decision}{not rejected: the registered joint claim was not established}
\defres{stage2/S2-4S/delta}{+0.0}
\defres{stage2/S2-4S/delta_ci/hi}{+0.6}
\defres{stage2/S2-4S/delta_ci/lo}{-0.6}
\defres{stage2/S2-4S/holm_rank}{2}
\defres{stage2/S2-4S/n_dropped}{0}
\defres{stage2/S2-4S/n_expected}{500}
\defres{stage2/S2-4S/n_pairs}{500}
\defres{stage2/S2-4S/ni/boundary}{-3.0}
\defres{stage2/S2-4S/ni/decision}{NI}
\defres{stage2/S2-4S/ni/discordance}{0.4}
\defres{stage2/S2-4S/ni/est}{+0.0}
\defres{stage2/S2-4S/ni/est_ci/hi}{+0.6}
\defres{stage2/S2-4S/ni/est_ci/lo}{-0.6}
\defres{stage2/S2-4S/ni/est_ci_newcombe/hi}{+1.0}
\defres{stage2/S2-4S/ni/est_ci_newcombe/lo}{-1.0}
\defres{stage2/S2-4S/ni/loss_rate_ub}{0.9}
\defres{stage2/S2-4S/ni/losses}{1}
\defres{stage2/S2-4S/ni/p}{$<$0.001}
\defres{stage2/S2-4S/ni/success_arm}{99.4}
\defres{stage2/S2-4S/ni/success_ref}{99.4}
\defres{stage2/S2-4S/ni/wins}{1}
\defres{stage2/S2-4S/p_decisive}{0.997}
\defres{stage2/S2-4S/p_holm}{1.000}
\defres{stage2/S2-4S/tariff/busy_throughput/cost_savings}{-1.1}
\defres{stage2/S2-4S/tariff/busy_throughput/p_cost}{0.983}
\defres{stage2/S2-4S/tariff/busy_throughput/q}{0.00202}
\defres{stage2/S2-4S/tariff/jev_api_price/cost_savings}{-1.3}
\defres{stage2/S2-4S/tariff/jev_api_price/p_cost}{0.995}
\defres{stage2/S2-4S/tariff/jev_api_price/q}{0.00212}
\defres{stage2/S2-4S/tariff/q}{0.00217}
\defres{stage2/S2-4S/tariff/zero/cost_savings}{3.8}
\defres{stage2/S2-4S/tariff/zero/p_cost}{$<$0.001}
\defres{stage2/S2-4S/tariff/zero/q}{0}
\defres{stage2/S2-L3a/alpha_adj}{0.008}
\defres{stage2/S2-L3a/cost/boundary}{0}
\defres{stage2/S2-L3a/cost/decision}{no cost saving established at this n}
\defres{stage2/S2-L3a/cost/est}{-0.00336}
\defres{stage2/S2-L3a/cost/est_ci/hi}{0.0000569}
\defres{stage2/S2-L3a/cost/est_ci/lo}{-0.00677}
\defres{stage2/S2-L3a/cost/p}{0.973}
\defres{stage2/S2-L3a/cost_arm}{0.134}
\defres{stage2/S2-L3a/cost_ref}{0.13}
\defres{stage2/S2-L3a/cost_savings}{-2.6}
\defres{stage2/S2-L3a/cost_savings_ci/hi}{0.1}
\defres{stage2/S2-L3a/cost_savings_ci/lo}{-5.2}
\defres{stage2/S2-L3a/coverage/arg_coverage}{0.7}
\defres{stage2/S2-L3a/coverage/tool_coverage}{8.1}
\defres{stage2/S2-L3a/decision}{not rejected: the registered joint claim was not established}
\defres{stage2/S2-L3a/delta}{-1.6}
\defres{stage2/S2-L3a/delta_ci/hi}{+1.8}
\defres{stage2/S2-L3a/delta_ci/lo}{-5.0}
\defres{stage2/S2-L3a/holm_rank}{1}
\defres{stage2/S2-L3a/n_dropped}{0}
\defres{stage2/S2-L3a/n_expected}{560}
\defres{stage2/S2-L3a/n_pairs}{560}
\defres{stage2/S2-L3a/ni/boundary}{-5.0}
\defres{stage2/S2-L3a/ni/decision}{NI}
\defres{stage2/S2-L3a/ni/discordance}{17.0}
\defres{stage2/S2-L3a/ni/est}{-1.6}
\defres{stage2/S2-L3a/ni/est_ci/hi}{+1.8}
\defres{stage2/S2-L3a/ni/est_ci/lo}{-5.0}
\defres{stage2/S2-L3a/ni/est_ci_newcombe/hi}{+1.8}
\defres{stage2/S2-L3a/ni/est_ci_newcombe/lo}{-5.0}
\defres{stage2/S2-L3a/ni/losses}{52}
\defres{stage2/S2-L3a/ni/p}{0.027}
\defres{stage2/S2-L3a/ni/success_arm}{22.7}
\defres{stage2/S2-L3a/ni/success_ref}{24.3}
\defres{stage2/S2-L3a/ni/wins}{43}
\defres{stage2/S2-L3a/p_decisive}{0.973}
\defres{stage2/S2-L3a/p_holm}{1.000}
\defres{stage2/S2-L3b/alpha_adj}{0.050}
\defres{stage2/S2-L3b/decision}{not run (A7.1 (h): E6 not run in Stage 1)}
\defres{stage2/S2-L3b/holm_rank}{6}
\defres{stage2/S2-L3b/p_decisive}{1.000}
\defres{stage2/S2-L3b/p_holm}{1.000}
\defres{stage2/descriptive/jevagent_default/cost_savings}{18.1}
\defres{stage2/descriptive/jevagent_default/cost_savings_ci/hi}{19.6}
\defres{stage2/descriptive/jevagent_default/cost_savings_ci/lo}{16.6}
\defres{stage2/descriptive/jevagent_default/delta}{+0.4}
\defres{stage2/descriptive/jevagent_default/delta_ci/hi}{+1.0}
\defres{stage2/descriptive/jevagent_default/delta_ci/lo}{+0.0}
\defres{stage2/descriptive/llm_only_xsmall/cost_savings}{75.3}
\defres{stage2/descriptive/llm_only_xsmall/cost_savings_ci/hi}{75.7}
\defres{stage2/descriptive/llm_only_xsmall/cost_savings_ci/lo}{74.8}
\defres{stage2/descriptive/llm_only_xsmall/delta}{+20.4}
\defres{stage2/descriptive/llm_only_xsmall/delta_ci/hi}{+24.2}
\defres{stage2/descriptive/llm_only_xsmall/delta_ci/lo}{+16.9}
\defres{stage2/descriptive/llm_only_xsmall/delta_ci_tango/hi}{+24.2}
\defres{stage2/descriptive/llm_only_xsmall/delta_ci_tango/lo}{+17.0}
\defres{stage2/descriptive/llm_only_xsmall/latency_diff_s}{-10.15}
\defres{stage2/descriptive/llm_only_xsmall/latency_diff_s_ci/hi}{-8.54}
\defres{stage2/descriptive/llm_only_xsmall/latency_diff_s_ci/lo}{-11.79}
\defres{stage2/descriptive/llm_only_xsmall/n_pairs}{500}
\defres{stage2/descriptive/llm_only_xsmall/success_arm}{98.6}
\defres{stage2/descriptive/llm_only_xsmall/success_ref}{78.2}
\defres{stage2/descriptive/logo-reflection/cost_savings}{-35.2}
\defres{stage2/descriptive/logo-reflection/cost_savings_ci/hi}{-28.5}
\defres{stage2/descriptive/logo-reflection/cost_savings_ci/lo}{-42.0}
\defres{stage2/descriptive/logo-reflection/delta}{+3.5}
\defres{stage2/descriptive/logo-reflection/delta_ci/hi}{+7.0}
\defres{stage2/descriptive/logo-reflection/delta_ci/lo}{+0.9}
\defres{stage2/descriptive/logo-reflection/delta_ci_tango/hi}{+7.0}
\defres{stage2/descriptive/logo-reflection/delta_ci_tango/lo}{+1.5}
\defres{stage2/descriptive/logo-reflection/latency_diff_s}{-1.76}
\defres{stage2/descriptive/logo-reflection/latency_diff_s_ci/hi}{-1.48}
\defres{stage2/descriptive/logo-reflection/latency_diff_s_ci/lo}{-2.08}
\defres{stage2/descriptive/logo-reflection/n_pairs}{200}
\defres{stage2/descriptive/logo-reflection/success_arm}{100.0}
\defres{stage2/descriptive/logo-reflection/success_ref}{96.5}
\defres{stage2/descriptive/logo-tool/cost_savings}{-69.2}
\defres{stage2/descriptive/logo-tool/cost_savings_ci/hi}{-61.6}
\defres{stage2/descriptive/logo-tool/cost_savings_ci/lo}{-76.7}
\defres{stage2/descriptive/logo-tool/delta}{+2.0}
\defres{stage2/descriptive/logo-tool/delta_ci/hi}{+5.4}
\defres{stage2/descriptive/logo-tool/delta_ci/lo}{-0.8}
\defres{stage2/descriptive/logo-tool/delta_ci_tango/hi}{+5.3}
\defres{stage2/descriptive/logo-tool/delta_ci_tango/lo}{-0.6}
\defres{stage2/descriptive/logo-tool/latency_diff_s}{-0.71}
\defres{stage2/descriptive/logo-tool/latency_diff_s_ci/hi}{-0.42}
\defres{stage2/descriptive/logo-tool/latency_diff_s_ci/lo}{-1.04}
\defres{stage2/descriptive/logo-tool/n_pairs}{200}
\defres{stage2/descriptive/logo-tool/success_arm}{98.5}
\defres{stage2/descriptive/logo-tool/success_ref}{96.5}
\defres{stage2/intervention/best_single/arg_coverage}{23.1}
\defres{stage2/intervention/best_single/llm_calls}{6.23}
\defres{stage2/intervention/best_single/llm_calls_avoided}{+1.29}
\defres{stage2/intervention/best_single/n}{500}
\defres{stage2/intervention/best_single/success}{99.8}
\defres{stage2/intervention/best_single/tool_coverage}{28.9}
\defres{stage2/intervention/best_single/tool_decisions}{3{,}755}
\defres{stage2/intervention/best_single/trigger_fires}{0}
\defres{stage2/intervention/best_single/trigger_questions}{0}
\defres{stage2/intervention/best_single/trigger_tasks}{0}
\defres{stage2/intervention/first200/interaction}{-2.5}
\defres{stage2/intervention/first200/interaction_ci/hi}{+0.0}
\defres{stage2/intervention/first200/interaction_ci/lo}{-5.0}
\defres{stage2/intervention/first200/n}{200}
\defres{stage2/intervention/first200/successes/best_single}{200}
\defres{stage2/intervention/first200/successes/jevagent_best}{193}
\defres{stage2/intervention/first200/successes/jevagent_minus_tool}{197}
\defres{stage2/intervention/first200/successes/llm_only}{199}
\defres{stage2/intervention/jevagent_best/arg_coverage}{51.4}
\defres{stage2/intervention/jevagent_best/failures}{14}
\defres{stage2/intervention/jevagent_best/failures_fired}{14}
\defres{stage2/intervention/jevagent_best/llm_calls}{5.37}
\defres{stage2/intervention/jevagent_best/llm_calls_avoided}{+2.15}
\defres{stage2/intervention/jevagent_best/n}{500}
\defres{stage2/intervention/jevagent_best/success}{97.2}
\defres{stage2/intervention/jevagent_best/tool_coverage}{52.5}
\defres{stage2/intervention/jevagent_best/tool_decisions}{3{,}770}
\defres{stage2/intervention/jevagent_best/trigger_fire_rate}{14.3}
\defres{stage2/intervention/jevagent_best/trigger_fires}{469}
\defres{stage2/intervention/jevagent_best/trigger_questions}{3{,}270}
\defres{stage2/intervention/jevagent_best/trigger_tasks}{416}
\defres{stage2/intervention/jevagent_best_rl/arg_coverage}{75.0}
\defres{stage2/intervention/jevagent_best_rl/llm_calls}{3.03}
\defres{stage2/intervention/jevagent_best_rl/llm_calls_avoided}{+4.49}
\defres{stage2/intervention/jevagent_best_rl/n}{500}
\defres{stage2/intervention/jevagent_best_rl/success}{100.0}
\defres{stage2/intervention/jevagent_best_rl/tool_coverage}{99.9}
\defres{stage2/intervention/jevagent_best_rl/tool_decisions}{3{,}750}
\defres{stage2/intervention/jevagent_best_rl/trigger_fire_rate}{0.0}
\defres{stage2/intervention/jevagent_best_rl/trigger_fires}{0}
\defres{stage2/intervention/jevagent_best_rl/trigger_questions}{3{,}250}
\defres{stage2/intervention/jevagent_best_rl/trigger_tasks}{0}
\defres{stage2/intervention/jevagent_best_sl4b/arg_coverage}{6.8}
\defres{stage2/intervention/jevagent_best_sl4b/llm_calls}{7.48}
\defres{stage2/intervention/jevagent_best_sl4b/llm_calls_avoided}{+0.04}
\defres{stage2/intervention/jevagent_best_sl4b/n}{500}
\defres{stage2/intervention/jevagent_best_sl4b/success}{99.4}
\defres{stage2/intervention/jevagent_best_sl4b/tool_coverage}{17.3}
\defres{stage2/intervention/jevagent_best_sl4b/tool_decisions}{3{,}754}
\defres{stage2/intervention/jevagent_best_sl4b/trigger_fire_rate}{0.0}
\defres{stage2/intervention/jevagent_best_sl4b/trigger_fires}{1}
\defres{stage2/intervention/jevagent_best_sl4b/trigger_questions}{3{,}254}
\defres{stage2/intervention/jevagent_best_sl4b/trigger_tasks}{1}
\defres{stage2/intervention/jevagent_best_x/arg_coverage}{0.0}
\defres{stage2/intervention/jevagent_best_x/llm_calls}{8.37}
\defres{stage2/intervention/jevagent_best_x/llm_calls_avoided}{-0.96}
\defres{stage2/intervention/jevagent_best_x/n}{500}
\defres{stage2/intervention/jevagent_best_x/success}{85.4}
\defres{stage2/intervention/jevagent_best_x/tool_coverage}{0.0}
\defres{stage2/intervention/jevagent_best_x/tool_decisions}{3{,}738}
\defres{stage2/intervention/jevagent_best_x/trigger_fire_rate}{13.9}
\defres{stage2/intervention/jevagent_best_x/trigger_fires}{449}
\defres{stage2/intervention/jevagent_best_x/trigger_questions}{3{,}238}
\defres{stage2/intervention/jevagent_best_x/trigger_tasks}{424}
\defres{stage2/intervention/jevagent_default/arg_coverage}{22.7}
\defres{stage2/intervention/jevagent_default/llm_calls}{6.26}
\defres{stage2/intervention/jevagent_default/llm_calls_avoided}{+1.26}
\defres{stage2/intervention/jevagent_default/n}{500}
\defres{stage2/intervention/jevagent_default/success}{99.8}
\defres{stage2/intervention/jevagent_default/tool_coverage}{28.2}
\defres{stage2/intervention/jevagent_default/tool_decisions}{3{,}755}
\defres{stage2/intervention/jevagent_default/trigger_fires}{0}
\defres{stage2/intervention/jevagent_default/trigger_questions}{0}
\defres{stage2/intervention/jevagent_default/trigger_tasks}{0}
\defres{stage2/intervention/jevagent_minus_tool/arg_coverage}{0.0}
\defres{stage2/intervention/jevagent_minus_tool/llm_calls}{8.51}
\defres{stage2/intervention/jevagent_minus_tool/llm_calls_avoided}{-0.99}
\defres{stage2/intervention/jevagent_minus_tool/n}{200}
\defres{stage2/intervention/jevagent_minus_tool/success}{98.5}
\defres{stage2/intervention/jevagent_minus_tool/tool_coverage}{0.0}
\defres{stage2/intervention/jevagent_minus_tool/tool_decisions}{1{,}513}
\defres{stage2/intervention/jevagent_minus_tool/trigger_fire_rate}{14.3}
\defres{stage2/intervention/jevagent_minus_tool/trigger_fires}{188}
\defres{stage2/intervention/jevagent_minus_tool/trigger_questions}{1{,}313}
\defres{stage2/intervention/jevagent_minus_tool/trigger_tasks}{167}
\defres{stage2/intervention/llm_only/arg_coverage}{0.0}
\defres{stage2/intervention/llm_only/llm_calls}{7.52}
\defres{stage2/intervention/llm_only/n}{500}
\defres{stage2/intervention/llm_only/success}{99.4}
\defres{stage2/intervention/llm_only/tool_coverage}{0.0}
\defres{stage2/intervention/llm_only/tool_decisions}{3{,}759}
\defres{stage2/intervention/llm_only/trigger_fires}{0}
\defres{stage2/intervention/llm_only/trigger_questions}{0}
\defres{stage2/intervention/llm_only/trigger_tasks}{0}
\defres{stage2/intervention/llm_only_x/arg_coverage}{0.0}
\defres{stage2/intervention/llm_only_x/llm_calls}{7.41}
\defres{stage2/intervention/llm_only_x/n}{500}
\defres{stage2/intervention/llm_only_x/success}{78.2}
\defres{stage2/intervention/llm_only_x/tool_coverage}{0.0}
\defres{stage2/intervention/llm_only_x/tool_decisions}{3{,}706}
\defres{stage2/intervention/llm_only_x/trigger_fires}{0}
\defres{stage2/intervention/llm_only_x/trigger_questions}{0}
\defres{stage2/intervention/llm_only_x/trigger_tasks}{0}
\defres{stage2/intervention/llm_only_xsmall/arg_coverage}{0.0}
\defres{stage2/intervention/llm_only_xsmall/llm_calls}{7.63}
\defres{stage2/intervention/llm_only_xsmall/llm_calls_avoided}{-0.22}
\defres{stage2/intervention/llm_only_xsmall/n}{500}
\defres{stage2/intervention/llm_only_xsmall/success}{98.6}
\defres{stage2/intervention/llm_only_xsmall/tool_coverage}{0.0}
\defres{stage2/intervention/llm_only_xsmall/tool_decisions}{3{,}817}
\defres{stage2/intervention/llm_only_xsmall/trigger_fires}{0}
\defres{stage2/intervention/llm_only_xsmall/trigger_questions}{0}
\defres{stage2/intervention/llm_only_xsmall/trigger_tasks}{0}
\defres{stage2/intervention/telecom_jevagent_best/arg_coverage}{0.7}
\defres{stage2/intervention/telecom_jevagent_best/llm_calls}{16.81}
\defres{stage2/intervention/telecom_jevagent_best/llm_calls_avoided}{-0.09}
\defres{stage2/intervention/telecom_jevagent_best/n}{560}
\defres{stage2/intervention/telecom_jevagent_best/success}{22.7}
\defres{stage2/intervention/telecom_jevagent_best/tool_coverage}{8.1}
\defres{stage2/intervention/telecom_jevagent_best/tool_decisions}{9{,}430}
\defres{stage2/intervention/telecom_jevagent_best/trigger_fires}{0}
\defres{stage2/intervention/telecom_jevagent_best/trigger_questions}{0}
\defres{stage2/intervention/telecom_jevagent_best/trigger_tasks}{0}
\defres{stage2/intervention/telecom_llm_only/arg_coverage}{0.0}
\defres{stage2/intervention/telecom_llm_only/llm_calls}{16.72}
\defres{stage2/intervention/telecom_llm_only/n}{560}
\defres{stage2/intervention/telecom_llm_only/success}{24.3}
\defres{stage2/intervention/telecom_llm_only/tool_coverage}{0.0}
\defres{stage2/intervention/telecom_llm_only/tool_decisions}{9{,}365}
\defres{stage2/intervention/telecom_llm_only/trigger_fires}{0}
\defres{stage2/intervention/telecom_llm_only/trigger_questions}{0}
\defres{stage2/intervention/telecom_llm_only/trigger_tasks}{0}
\defres{stage2/scorecard/best_single/cost_usd}{0.0335}
\defres{stage2/scorecard/best_single/latency_s}{7.92}
\defres{stage2/scorecard/best_single/llm_calls}{6.23}
\defres{stage2/scorecard/best_single/n}{500}
\defres{stage2/scorecard/best_single/s1_calls}{11.3}
\defres{stage2/scorecard/best_single/success}{99.8}
\defres{stage2/scorecard/best_single/success_ci/hi}{100.0}
\defres{stage2/scorecard/best_single/success_ci/lo}{98.9}
\defres{stage2/scorecard/best_single/vs_baseline/cost_savings}{18.8}
\defres{stage2/scorecard/best_single/vs_baseline/cost_savings_ci/hi}{20.3}
\defres{stage2/scorecard/best_single/vs_baseline/cost_savings_ci/lo}{17.2}
\defres{stage2/scorecard/best_single/vs_baseline/delta}{+0.4}
\defres{stage2/scorecard/best_single/vs_baseline/delta_ci/hi}{+1.5}
\defres{stage2/scorecard/best_single/vs_baseline/delta_ci/lo}{-0.5}
\defres{stage2/scorecard/jevagent_best/cost_usd}{0.0245}
\defres{stage2/scorecard/jevagent_best/latency_s}{9.35}
\defres{stage2/scorecard/jevagent_best/llm_calls}{5.37}
\defres{stage2/scorecard/jevagent_best/n}{500}
\defres{stage2/scorecard/jevagent_best/s1_calls}{21.2}
\defres{stage2/scorecard/jevagent_best/success}{97.2}
\defres{stage2/scorecard/jevagent_best/success_ci/hi}{98.3}
\defres{stage2/scorecard/jevagent_best/success_ci/lo}{95.4}
\defres{stage2/scorecard/jevagent_best/vs_baseline/cost_savings}{40.7}
\defres{stage2/scorecard/jevagent_best/vs_baseline/cost_savings_ci/hi}{42.5}
\defres{stage2/scorecard/jevagent_best/vs_baseline/cost_savings_ci/lo}{38.9}
\defres{stage2/scorecard/jevagent_best/vs_baseline/delta}{-2.2}
\defres{stage2/scorecard/jevagent_best/vs_baseline/delta_ci/hi}{-0.6}
\defres{stage2/scorecard/jevagent_best/vs_baseline/delta_ci/lo}{-4.1}
\defres{stage2/scorecard/jevagent_best_rl/cost_usd}{0.00583}
\defres{stage2/scorecard/jevagent_best_rl/latency_s}{9.77}
\defres{stage2/scorecard/jevagent_best_rl/llm_calls}{3.03}
\defres{stage2/scorecard/jevagent_best_rl/n}{500}
\defres{stage2/scorecard/jevagent_best_rl/s1_calls}{24.6}
\defres{stage2/scorecard/jevagent_best_rl/success}{100.0}
\defres{stage2/scorecard/jevagent_best_rl/success_ci/hi}{100.0}
\defres{stage2/scorecard/jevagent_best_rl/success_ci/lo}{99.2}
\defres{stage2/scorecard/jevagent_best_rl/vs_baseline/cost_savings}{85.9}
\defres{stage2/scorecard/jevagent_best_rl/vs_baseline/cost_savings_ci/hi}{86.3}
\defres{stage2/scorecard/jevagent_best_rl/vs_baseline/cost_savings_ci/lo}{85.4}
\defres{stage2/scorecard/jevagent_best_rl/vs_baseline/delta}{+0.6}
\defres{stage2/scorecard/jevagent_best_rl/vs_baseline/delta_ci/hi}{+1.7}
\defres{stage2/scorecard/jevagent_best_rl/vs_baseline/delta_ci/lo}{-0.3}
\defres{stage2/scorecard/jevagent_best_sl4b/cost_usd}{0.0397}
\defres{stage2/scorecard/jevagent_best_sl4b/latency_s}{13.8}
\defres{stage2/scorecard/jevagent_best_sl4b/llm_calls}{7.48}
\defres{stage2/scorecard/jevagent_best_sl4b/n}{500}
\defres{stage2/scorecard/jevagent_best_sl4b/s1_calls}{15.9}
\defres{stage2/scorecard/jevagent_best_sl4b/success}{99.4}
\defres{stage2/scorecard/jevagent_best_sl4b/success_ci/hi}{99.8}
\defres{stage2/scorecard/jevagent_best_sl4b/success_ci/lo}{98.3}
\defres{stage2/scorecard/jevagent_best_sl4b/vs_baseline/cost_savings}{3.8}
\defres{stage2/scorecard/jevagent_best_sl4b/vs_baseline/cost_savings_ci/hi}{4.7}
\defres{stage2/scorecard/jevagent_best_sl4b/vs_baseline/cost_savings_ci/lo}{2.9}
\defres{stage2/scorecard/jevagent_best_sl4b/vs_baseline/delta}{+0.0}
\defres{stage2/scorecard/jevagent_best_sl4b/vs_baseline/delta_ci/hi}{+1.0}
\defres{stage2/scorecard/jevagent_best_sl4b/vs_baseline/delta_ci/lo}{-1.0}
\defres{stage2/scorecard/jevagent_best_x/cost_usd}{0.00246}
\defres{stage2/scorecard/jevagent_best_x/latency_s}{37.5}
\defres{stage2/scorecard/jevagent_best_x/llm_calls}{8.37}
\defres{stage2/scorecard/jevagent_best_x/n}{500}
\defres{stage2/scorecard/jevagent_best_x/s1_calls}{6.48}
\defres{stage2/scorecard/jevagent_best_x/success}{85.4}
\defres{stage2/scorecard/jevagent_best_x/success_ci/hi}{88.2}
\defres{stage2/scorecard/jevagent_best_x/success_ci/lo}{82.0}
\defres{stage2/scorecard/jevagent_best_x/vs_baseline/cost_savings}{-20.8}
\defres{stage2/scorecard/jevagent_best_x/vs_baseline/cost_savings_ci/hi}{-19.6}
\defres{stage2/scorecard/jevagent_best_x/vs_baseline/cost_savings_ci/lo}{-22.0}
\defres{stage2/scorecard/jevagent_best_x/vs_baseline/delta}{+7.2}
\defres{stage2/scorecard/jevagent_best_x/vs_baseline/delta_ci/hi}{+10.6}
\defres{stage2/scorecard/jevagent_best_x/vs_baseline/delta_ci/lo}{+3.8}
\defres{stage2/scorecard/jevagent_default/cost_usd}{0.0338}
\defres{stage2/scorecard/jevagent_default/latency_s}{7.96}
\defres{stage2/scorecard/jevagent_default/llm_calls}{6.26}
\defres{stage2/scorecard/jevagent_default/n}{500}
\defres{stage2/scorecard/jevagent_default/s1_calls}{11.2}
\defres{stage2/scorecard/jevagent_default/success}{99.8}
\defres{stage2/scorecard/jevagent_default/success_ci/hi}{100.0}
\defres{stage2/scorecard/jevagent_default/success_ci/lo}{98.9}
\defres{stage2/scorecard/jevagent_default/vs_baseline/cost_savings}{18.1}
\defres{stage2/scorecard/jevagent_default/vs_baseline/cost_savings_ci/hi}{19.6}
\defres{stage2/scorecard/jevagent_default/vs_baseline/cost_savings_ci/lo}{16.6}
\defres{stage2/scorecard/jevagent_default/vs_baseline/delta}{+0.4}
\defres{stage2/scorecard/jevagent_default/vs_baseline/delta_ci/hi}{+1.5}
\defres{stage2/scorecard/jevagent_default/vs_baseline/delta_ci/lo}{-0.5}
\defres{stage2/scorecard/llm_only/cost_usd}{0.0413}
\defres{stage2/scorecard/llm_only/latency_s}{6.8}
\defres{stage2/scorecard/llm_only/llm_calls}{7.52}
\defres{stage2/scorecard/llm_only/n}{500}
\defres{stage2/scorecard/llm_only/s1_calls}{0}
\defres{stage2/scorecard/llm_only/success}{99.4}
\defres{stage2/scorecard/llm_only/success_ci/hi}{99.8}
\defres{stage2/scorecard/llm_only/success_ci/lo}{98.3}
\defres{stage2/scorecard/llm_only_x/cost_usd}{0.00203}
\defres{stage2/scorecard/llm_only_x/latency_s}{33.5}
\defres{stage2/scorecard/llm_only_x/llm_calls}{7.41}
\defres{stage2/scorecard/llm_only_x/n}{500}
\defres{stage2/scorecard/llm_only_x/s1_calls}{0}
\defres{stage2/scorecard/llm_only_x/success}{78.2}
\defres{stage2/scorecard/llm_only_x/success_ci/hi}{81.6}
\defres{stage2/scorecard/llm_only_x/success_ci/lo}{74.4}
\defres{stage2/scorecard/llm_only_xsmall/cost_usd}{0.000503}
\defres{stage2/scorecard/llm_only_xsmall/latency_s}{23.4}
\defres{stage2/scorecard/llm_only_xsmall/llm_calls}{7.63}
\defres{stage2/scorecard/llm_only_xsmall/n}{500}
\defres{stage2/scorecard/llm_only_xsmall/s1_calls}{0}
\defres{stage2/scorecard/llm_only_xsmall/success}{98.6}
\defres{stage2/scorecard/llm_only_xsmall/success_ci/hi}{99.3}
\defres{stage2/scorecard/llm_only_xsmall/success_ci/lo}{97.1}
\defres{stage2/scorecard/llm_only_xsmall/vs_baseline/cost_savings}{75.3}
\defres{stage2/scorecard/llm_only_xsmall/vs_baseline/cost_savings_ci/hi}{75.7}
\defres{stage2/scorecard/llm_only_xsmall/vs_baseline/cost_savings_ci/lo}{74.8}
\defres{stage2/scorecard/llm_only_xsmall/vs_baseline/delta}{+20.4}
\defres{stage2/scorecard/llm_only_xsmall/vs_baseline/delta_ci/hi}{+24.2}
\defres{stage2/scorecard/llm_only_xsmall/vs_baseline/delta_ci/lo}{+16.9}
\defres{stage2/selection/reflection/arm}{jev\_reflect\_trigger}
\defres{stage2/selection/reflection/losses}{0}
\defres{stage2/selection/reflection/n}{200}
\defres{stage2/selection/reflection/savings}{0.9}
\defres{stage2/selection/reflection/savings_ci/hi}{1.8}
\defres{stage2/selection/reflection/savings_ci/lo}{0.0}
\defres{stage2/selection/reflection/wins}{0}
\defres{stage2/selection/tool/arm}{jev\_ts\_cascade\_tauhat}
\defres{stage2/selection/tool/losses}{0}
\defres{stage2/selection/tool/n}{500}
\defres{stage2/selection/tool/savings}{14.2}
\defres{stage2/selection/tool/savings_ci/hi}{15.7}
\defres{stage2/selection/tool/savings_ci/lo}{12.8}
\defres{stage2/selection/tool/wins}{0}
\defres{stage2_ladder/sl0.8b/corpus_acc}{48.3}
\defres{stage2_ladder/sl0.8b/corpus_acc_offplan}{31.5}
\defres{stage2_ladder/sl0.8b/corpus_tasks}{200}
\defres{stage2_ladder/sl0.8b/ece}{0.056}
\defres{stage2_ladder/sl0.8b/vs_jev/corpus_delta}{-43.1}
\defres{stage2_ladder/sl0.8b/vs_jev/corpus_delta_ci/hi}{-39.9}
\defres{stage2_ladder/sl0.8b/vs_jev/corpus_delta_ci/lo}{-46.3}
\defres{stage2_ladder/sl2b/corpus_acc}{68.4}
\defres{stage2_ladder/sl2b/corpus_acc_offplan}{47.2}
\defres{stage2_ladder/sl2b/corpus_tasks}{200}
\defres{stage2_ladder/sl2b/ece}{0.177}
\defres{stage2_ladder/sl2b/vs_jev/corpus_delta}{-23.0}
\defres{stage2_ladder/sl2b/vs_jev/corpus_delta_ci/hi}{-20.9}
\defres{stage2_ladder/sl2b/vs_jev/corpus_delta_ci/lo}{-25.2}
\defres{stage2_ladder/sl9b/corpus_acc}{91.8}
\defres{stage2_ladder/sl9b/corpus_acc_offplan}{74.3}
\defres{stage2_ladder/sl9b/corpus_tasks}{200}
\defres{stage2_ladder/sl9b/ece}{0.071}
\defres{stage2_ladder/sl9b/vs_jev/corpus_delta}{+0.3}
\defres{stage2_ladder/sl9b/vs_jev/corpus_delta_ci/hi}{+1.4}
\defres{stage2_ladder/sl9b/vs_jev/corpus_delta_ci/lo}{-0.7}
\defres{stage2_rl/base/corpus_acc}{50.1}
\defres{stage2_rl/base/corpus_acc_offplan}{26.7}
\defres{stage2_rl/base/corpus_tasks}{200}
\defres{stage2_rl/base/ece}{0.160}
\defres{stage2_rl/base/l1_acc}{87.5}
\defres{stage2_rl/base/l1_n}{1114}
\defres{stage2_rl/base/live_n}{100}
\defres{stage2_rl/base/live_success}{13.0}
\defres{stage2_rl/base/own_acc}{38.4}
\defres{stage2_rl/frozen/corpus_acc}{99.2}
\defres{stage2_rl/frozen/corpus_acc_offplan}{94.7}
\defres{stage2_rl/frozen/corpus_tasks}{200}
\defres{stage2_rl/frozen/ece}{0.010}
\defres{stage2_rl/frozen/l1_acc}{88.4}
\defres{stage2_rl/frozen/l1_n}{1114}
\defres{stage2_rl/frozen/live_n}{100}
\defres{stage2_rl/frozen/live_success}{100.0}
\defres{stage2_rl/frozen/own_acc}{100.0}
\defres{stage2_rl/intern/corpus_acc}{75.2}
\defres{stage2_rl/intern/corpus_acc_offplan}{47.6}
\defres{stage2_rl/intern/corpus_tasks}{200}
\defres{stage2_rl/intern/ece}{0.049}
\defres{stage2_rl/intern/l1_acc}{88.2}
\defres{stage2_rl/intern/l1_n}{1114}
\defres{stage2_rl/intern/live_n}{100}
\defres{stage2_rl/intern/live_success}{30.0}
\defres{stage2_rl/intern/own_acc}{63.8}
\defres{stage2_rl/jev/corpus_acc}{91.5}
\defres{stage2_rl/jev/corpus_acc_offplan}{81.5}
\defres{stage2_rl/jev/corpus_tasks}{200}
\defres{stage2_rl/jev/ece}{0.043}
\defres{stage2_rl/jev/l1_acc}{89.9}
\defres{stage2_rl/jev/l1_n}{1114}
\defres{stage2_rl/jev/live_n}{100}
\defres{stage2_rl/jev/live_success}{84.0}
\defres{stage2_rl/jev/own_acc}{90.9}
\defres{stage2_rl/sft_v1/corpus_acc}{99.2}
\defres{stage2_rl/sft_v1/corpus_acc_offplan}{93.8}
\defres{stage2_rl/sft_v1/corpus_tasks}{200}
\defres{stage2_rl/sft_v1/ece}{0.011}
\defres{stage2_rl/sft_v1/l1_acc}{86.9}
\defres{stage2_rl/sft_v1/l1_n}{1114}
\defres{stage2_rl/sft_v1/live_n}{100}
\defres{stage2_rl/sft_v1/live_success}{100.0}
\defres{stage2_rl/sft_v1/own_acc}{100.0}
\defres{stage2_s1/frozen/corpus_acc}{99.2}
\defres{stage2_s1/frozen/corpus_acc_offplan}{94.7}
\defres{stage2_s1/frozen/corpus_tasks}{200}
\defres{stage2_s1/frozen/ece}{0.010}
\defres{stage2_s1/frozen/l1_acc}{88.4}
\defres{stage2_s1/frozen/l1_n}{1114}
\defres{stage2_s1/frozen/live_n}{200}
\defres{stage2_s1/frozen/live_success}{100.0}
\defres{stage2_s1/frozen/own_acc}{100.0}
\defres{stage2_s1/frozen/vs_jev/corpus_delta}{+7.7}
\defres{stage2_s1/frozen/vs_jev/corpus_delta_ci/hi}{+9.1}
\defres{stage2_s1/frozen/vs_jev/corpus_delta_ci/lo}{+6.4}
\defres{stage2_s1/frozen/vs_jev/corpus_n}{200}
\defres{stage2_s1/frozen/vs_jev/e1_delta}{-1.5}
\defres{stage2_s1/frozen/vs_jev/e1_delta_ci/hi}{+0.3}
\defres{stage2_s1/frozen/vs_jev/e1_delta_ci/lo}{-3.4}
\defres{stage2_s1/frozen/vs_jev/e1_n}{1114}
\defres{stage2_s1/frozen/vs_jev/live_delta}{+17.0}
\defres{stage2_s1/frozen/vs_jev/live_delta_ci/hi}{+22.8}
\defres{stage2_s1/frozen/vs_jev/live_delta_ci/lo}{+12.1}
\defres{stage2_s1/frozen/vs_jev/live_n}{200}
\defres{stage2_s1/intern/corpus_acc}{75.2}
\defres{stage2_s1/intern/corpus_acc_offplan}{47.6}
\defres{stage2_s1/intern/corpus_tasks}{200}
\defres{stage2_s1/intern/ece}{0.049}
\defres{stage2_s1/intern/l1_acc}{88.2}
\defres{stage2_s1/intern/l1_n}{1114}
\defres{stage2_s1/intern/live_n}{200}
\defres{stage2_s1/intern/live_success}{26.5}
\defres{stage2_s1/intern/own_acc}{62.2}
\defres{stage2_s1/intern/vs_jev/corpus_delta}{-16.3}
\defres{stage2_s1/intern/vs_jev/corpus_delta_ci/hi}{-14.5}
\defres{stage2_s1/intern/vs_jev/corpus_delta_ci/lo}{-18.1}
\defres{stage2_s1/intern/vs_jev/corpus_n}{200}
\defres{stage2_s1/intern/vs_jev/e1_delta}{-1.7}
\defres{stage2_s1/intern/vs_jev/e1_delta_ci/hi}{-0.5}
\defres{stage2_s1/intern/vs_jev/e1_delta_ci/lo}{-2.9}
\defres{stage2_s1/intern/vs_jev/e1_n}{1114}
\defres{stage2_s1/intern/vs_jev/live_delta}{-56.5}
\defres{stage2_s1/intern/vs_jev/live_delta_ci/hi}{-49.0}
\defres{stage2_s1/intern/vs_jev/live_delta_ci/lo}{-62.8}
\defres{stage2_s1/intern/vs_jev/live_n}{200}
\defres{stage2_s1/jev/corpus_acc}{91.5}
\defres{stage2_s1/jev/corpus_acc_offplan}{81.5}
\defres{stage2_s1/jev/corpus_tasks}{200}
\defres{stage2_s1/jev/ece}{0.043}
\defres{stage2_s1/jev/l1_acc}{89.9}
\defres{stage2_s1/jev/l1_n}{1114}
\defres{stage2_s1/jev/live_n}{200}
\defres{stage2_s1/jev/live_success}{83.0}
\defres{stage2_s1/jev/own_acc}{91.0}
\defres{stage2_s1/kendall/e1_vs_corpus}{0.000}
\defres{stage2_s1/kendall/e1_vs_live}{-0.200}
\defres{stage2_s1/sl27b/corpus_acc}{93.9}
\defres{stage2_s1/sl27b/corpus_acc_offplan}{85.1}
\defres{stage2_s1/sl27b/corpus_tasks}{200}
\defres{stage2_s1/sl27b/ece}{0.012}
\defres{stage2_s1/sl27b/l1_acc}{90.8}
\defres{stage2_s1/sl27b/l1_n}{1114}
\defres{stage2_s1/sl27b/live_n}{200}
\defres{stage2_s1/sl27b/live_success}{63.0}
\defres{stage2_s1/sl27b/own_acc}{87.7}
\defres{stage2_s1/sl27b/vs_jev/corpus_delta}{+2.5}
\defres{stage2_s1/sl27b/vs_jev/corpus_delta_ci/hi}{+3.3}
\defres{stage2_s1/sl27b/vs_jev/corpus_delta_ci/lo}{+1.6}
\defres{stage2_s1/sl27b/vs_jev/corpus_n}{200}
\defres{stage2_s1/sl27b/vs_jev/e1_delta}{+0.8}
\defres{stage2_s1/sl27b/vs_jev/e1_delta_ci/hi}{+2.1}
\defres{stage2_s1/sl27b/vs_jev/e1_delta_ci/lo}{-0.5}
\defres{stage2_s1/sl27b/vs_jev/e1_n}{1114}
\defres{stage2_s1/sl27b/vs_jev/live_delta}{-20.0}
\defres{stage2_s1/sl27b/vs_jev/live_delta_ci/hi}{-14.4}
\defres{stage2_s1/sl27b/vs_jev/live_delta_ci/lo}{-25.7}
\defres{stage2_s1/sl27b/vs_jev/live_n}{200}
\defres{stage2_s1/sl4b/corpus_acc}{89.1}
\defres{stage2_s1/sl4b/corpus_acc_offplan}{76.8}
\defres{stage2_s1/sl4b/corpus_tasks}{200}
\defres{stage2_s1/sl4b/ece}{0.078}
\defres{stage2_s1/sl4b/l1_acc}{91.3}
\defres{stage2_s1/sl4b/l1_n}{1114}
\defres{stage2_s1/sl4b/live_n}{200}
\defres{stage2_s1/sl4b/live_success}{60.0}
\defres{stage2_s1/sl4b/own_acc}{81.6}
\defres{stage2_s1/sl4b/vs_jev/corpus_delta}{-2.4}
\defres{stage2_s1/sl4b/vs_jev/corpus_delta_ci/hi}{-1.3}
\defres{stage2_s1/sl4b/vs_jev/corpus_delta_ci/lo}{-3.5}
\defres{stage2_s1/sl4b/vs_jev/corpus_n}{200}
\defres{stage2_s1/sl4b/vs_jev/e1_delta}{+1.3}
\defres{stage2_s1/sl4b/vs_jev/e1_delta_ci/hi}{+2.6}
\defres{stage2_s1/sl4b/vs_jev/e1_delta_ci/lo}{+0.1}
\defres{stage2_s1/sl4b/vs_jev/e1_n}{1114}
\defres{stage2_s1/sl4b/vs_jev/live_delta}{-23.0}
\defres{stage2_s1/sl4b/vs_jev/live_delta_ci/hi}{-17.0}
\defres{stage2_s1/sl4b/vs_jev/live_delta_ci/lo}{-28.9}
\defres{stage2_s1/sl4b/vs_jev/live_n}{200}
\defres{stage2_v2/corpus_acc}{99.4}
\defres{stage2_v2/corpus_acc_offplan}{95.0}
\defres{stage2_v2/corpus_tasks}{200}
\defres{stage2_v2/ece}{0.010}
\defres{stage2_v2/label}{exploratory (A7.19)}
\defres{stage2_v2/live_n}{200}
\defres{stage2_v2/live_success}{100.0}
\defres{stage2_v2/own_acc}{100.0}
\defres{stage2_v2/profile/arg_coverage}{74.5}
\defres{stage2_v2/profile/cost_arm}{0.0187}
\defres{stage2_v2/profile/cost_ref}{0.0413}
\defres{stage2_v2/profile/cost_savings}{54.8}
\defres{stage2_v2/profile/cost_savings_ci/hi}{55.8}
\defres{stage2_v2/profile/cost_savings_ci/lo}{53.8}
\defres{stage2_v2/profile/delta}{+0.6}
\defres{stage2_v2/profile/delta_ci/hi}{+1.7}
\defres{stage2_v2/profile/delta_ci/lo}{-0.3}
\defres{stage2_v2/profile/delta_ci_tango/hi}{+1.7}
\defres{stage2_v2/profile/delta_ci_tango/lo}{-0.2}
\defres{stage2_v2/profile/latency_diff_s}{+15.78}
\defres{stage2_v2/profile/latency_diff_s_ci/hi}{+16.46}
\defres{stage2_v2/profile/latency_diff_s_ci/lo}{+15.11}
\defres{stage2_v2/profile/llm_calls}{3.09}
\defres{stage2_v2/profile/n_dropped}{0}
\defres{stage2_v2/profile/n_expected}{500}
\defres{stage2_v2/profile/n_pairs}{500}
\defres{stage2_v2/profile/success_arm}{100.0}
\defres{stage2_v2/profile/success_ref}{99.4}
\defres{stage2_v2/profile/tariff/busy_throughput/cost_savings}{55.6}
\defres{stage2_v2/profile/tariff/busy_throughput/cost_savings_ci/hi}{56.6}
\defres{stage2_v2/profile/tariff/busy_throughput/cost_savings_ci/lo}{54.6}
\defres{stage2_v2/profile/tariff/busy_throughput/q}{0.012}
\defres{stage2_v2/profile/tariff/jev_api_price/cost_savings}{82.6}
\defres{stage2_v2/profile/tariff/jev_api_price/cost_savings_ci/hi}{83.0}
\defres{stage2_v2/profile/tariff/jev_api_price/cost_savings_ci/lo}{82.1}
\defres{stage2_v2/profile/tariff/jev_api_price/q}{0.000884}
\defres{stage2_v2/profile/tariff/q}{0.0124}
\defres{stage2_v2/profile/tariff/reference_host/cost_savings}{75.9}
\defres{stage2_v2/profile/tariff/reference_host/cost_savings_ci/hi}{76.4}
\defres{stage2_v2/profile/tariff/reference_host/cost_savings_ci/lo}{75.4}
\defres{stage2_v2/profile/tariff/reference_host/q}{0.00366}
\defres{stage2_v2/profile/tariff/zero/cost_savings}{84.7}
\defres{stage2_v2/profile/tariff/zero/cost_savings_ci/hi}{85.2}
\defres{stage2_v2/profile/tariff/zero/cost_savings_ci/lo}{84.3}
\defres{stage2_v2/profile/tariff/zero/q}{0}
\defres{stage2_v2/profile/tool_coverage}{98.9}
\defres{stage2_v2/steps}{7.50}
\defres{stage2_v2/vs_jev/corpus_delta}{+7.9}
\defres{stage2_v2/vs_jev/corpus_delta_ci/hi}{+9.3}
\defres{stage2_v2/vs_jev/corpus_delta_ci/lo}{+6.5}
\defres{stage2_v2/vs_jev/corpus_n}{200}
\defres{stage2_v2/vs_jev/live_delta}{+17.0}
\defres{stage2_v2/vs_jev/live_delta_ci/hi}{+22.8}
\defres{stage2_v2/vs_jev/live_delta_ci/lo}{+12.1}
\defres{stage2_v2/vs_jev/live_n}{200}
\makeatother


==> generated/stage2_sol.tex <==
\makeatletter
\providecommand{\res}[1]{\ifcsname jevres@#1\endcsname\csname jevres@#1\endcsname\else\tbd\fi}
\providecommand{\defres}[2]{\expandafter\def\csname jevres@#1\endcsname{#2}}
\defres{stage2_sol/arm/jevagent_best_sol/cached_share}{89.5}
\defres{stage2_sol/arm/jevagent_best_sol/cost_usd}{0.0111}
\defres{stage2_sol/arm/jevagent_best_sol/cost_usd_cw}{0.0123}
\defres{stage2_sol/arm/jevagent_best_sol/latency_s}{23.27}
\defres{stage2_sol/arm/jevagent_best_sol/llm_calls}{8.43}
\defres{stage2_sol/arm/jevagent_best_sol/n}{500}
\defres{stage2_sol/arm/jevagent_best_sol/reasoning_tokens}{0}
\defres{stage2_sol/arm/jevagent_best_sol/s1_calls}{6.50}
\defres{stage2_sol/arm/jevagent_best_sol/success}{98.4}
\defres{stage2_sol/arm/jevagent_best_sol/success_ci/hi}{99.2}
\defres{stage2_sol/arm/jevagent_best_sol/success_ci/lo}{96.9}
\defres{stage2_sol/arm/jevagent_best_sol/wall_s}{23.37}
\defres{stage2_sol/arm/llm_only_sol/cached_share}{90.5}
\defres{stage2_sol/arm/llm_only_sol/cost_usd}{0.00927}
\defres{stage2_sol/arm/llm_only_sol/cost_usd_cw}{0.0105}
\defres{stage2_sol/arm/llm_only_sol/latency_s}{19.12}
\defres{stage2_sol/arm/llm_only_sol/llm_calls}{7.50}
\defres{stage2_sol/arm/llm_only_sol/n}{500}
\defres{stage2_sol/arm/llm_only_sol/reasoning_tokens}{0}
\defres{stage2_sol/arm/llm_only_sol/s1_calls}{0.00}
\defres{stage2_sol/arm/llm_only_sol/success}{99.0}
\defres{stage2_sol/arm/llm_only_sol/success_ci/hi}{99.6}
\defres{stage2_sol/arm/llm_only_sol/success_ci/lo}{97.7}
\defres{stage2_sol/arm/llm_only_sol/wall_s}{19.16}
\defres{stage2_sol/arm/llm_only_solsmall/cached_share}{85.1}
\defres{stage2_sol/arm/llm_only_solsmall/cost_usd}{0.000717}
\defres{stage2_sol/arm/llm_only_solsmall/cost_usd_cw}{0.000813}
\defres{stage2_sol/arm/llm_only_solsmall/latency_s}{12.77}
\defres{stage2_sol/arm/llm_only_solsmall/llm_calls}{7.50}
\defres{stage2_sol/arm/llm_only_solsmall/n}{500}
\defres{stage2_sol/arm/llm_only_solsmall/reasoning_tokens}{0}
\defres{stage2_sol/arm/llm_only_solsmall/s1_calls}{0.00}
\defres{stage2_sol/arm/llm_only_solsmall/success}{99.8}
\defres{stage2_sol/arm/llm_only_solsmall/success_ci/hi}{100.0}
\defres{stage2_sol/arm/llm_only_solsmall/success_ci/lo}{98.9}
\defres{stage2_sol/arm/llm_only_solsmall/wall_s}{12.81}
\defres{stage2_sol/envelope}{80}
\defres{stage2_sol/fit/tool_params/always_defer}{no}
\defres{stage2_sol/fit/tool_params/tau}{0.57}
\defres{stage2_sol/fit/tool_select/always_defer}{yes}
\defres{stage2_sol/intervention/jevagent_best_sol/arg_coverage}{0.0}
\defres{stage2_sol/intervention/jevagent_best_sol/llm_calls}{8.43}
\defres{stage2_sol/intervention/jevagent_best_sol/llm_calls_avoided}{-0.93}
\defres{stage2_sol/intervention/jevagent_best_sol/tool_coverage}{0.0}
\defres{stage2_sol/intervention/jevagent_best_sol/trigger_fire_rate}{14.2}
\defres{stage2_sol/intervention/jevagent_best_sol/trigger_fires}{463}
\defres{stage2_sol/intervention/jevagent_best_sol/trigger_questions}{3{,}250}
\defres{stage2_sol/intervention/jevagent_best_sol/trigger_tasks}{413}
\defres{stage2_sol/intervention/llm_only_sol/arg_coverage}{0.0}
\defres{stage2_sol/intervention/llm_only_sol/llm_calls}{7.50}
\defres{stage2_sol/intervention/llm_only_sol/tool_coverage}{0.0}
\defres{stage2_sol/intervention/llm_only_sol/trigger_fires}{0}
\defres{stage2_sol/intervention/llm_only_sol/trigger_questions}{0}
\defres{stage2_sol/intervention/llm_only_sol/trigger_tasks}{0}
\defres{stage2_sol/intervention/llm_only_solsmall/arg_coverage}{0.0}
\defres{stage2_sol/intervention/llm_only_solsmall/llm_calls}{7.50}
\defres{stage2_sol/intervention/llm_only_solsmall/llm_calls_avoided}{-0.00}
\defres{stage2_sol/intervention/llm_only_solsmall/tool_coverage}{0.0}
\defres{stage2_sol/intervention/llm_only_solsmall/trigger_fires}{0}
\defres{stage2_sol/intervention/llm_only_solsmall/trigger_questions}{0}
\defres{stage2_sol/intervention/llm_only_solsmall/trigger_tasks}{0}
\defres{stage2_sol/jevagent_best_sol/cost_arm}{0.0111}
\defres{stage2_sol/jevagent_best_sol/cost_ref}{0.00927}
\defres{stage2_sol/jevagent_best_sol/cost_savings}{-19.8}
\defres{stage2_sol/jevagent_best_sol/cost_savings_ci/hi}{-14.2}
\defres{stage2_sol/jevagent_best_sol/cost_savings_ci/lo}{-25.6}
\defres{stage2_sol/jevagent_best_sol/cost_savings_cw}{-17.3}
\defres{stage2_sol/jevagent_best_sol/cost_savings_cw_ci/hi}{-11.2}
\defres{stage2_sol/jevagent_best_sol/cost_savings_cw_ci/lo}{-23.7}
\defres{stage2_sol/jevagent_best_sol/delta}{-0.6}
\defres{stage2_sol/jevagent_best_sol/delta_ci/hi}{+0.6}
\defres{stage2_sol/jevagent_best_sol/delta_ci/lo}{-2.0}
\defres{stage2_sol/jevagent_best_sol/delta_ci_newcombe/hi}{+0.9}
\defres{stage2_sol/jevagent_best_sol/delta_ci_newcombe/lo}{-2.2}
\defres{stage2_sol/jevagent_best_sol/latency_diff_s}{+4.15}
\defres{stage2_sol/jevagent_best_sol/latency_diff_s_ci/hi}{+4.46}
\defres{stage2_sol/jevagent_best_sol/latency_diff_s_ci/lo}{+3.84}
\defres{stage2_sol/jevagent_best_sol/losses}{7}
\defres{stage2_sol/jevagent_best_sol/n_dropped}{0}
\defres{stage2_sol/jevagent_best_sol/n_pairs}{500}
\defres{stage2_sol/jevagent_best_sol/success_arm}{98.4}
\defres{stage2_sol/jevagent_best_sol/success_ref}{99.0}
\defres{stage2_sol/jevagent_best_sol/wall_diff_s}{+4.21}
\defres{stage2_sol/jevagent_best_sol/wins}{4}
\defres{stage2_sol/label}{descriptive (A7.12 (i)): no test, outside every Holm table}
\defres{stage2_sol/llm_only_solsmall/cost_arm}{0.000717}
\defres{stage2_sol/llm_only_solsmall/cost_ref}{0.00927}
\defres{stage2_sol/llm_only_solsmall/cost_savings}{92.3}
\defres{stage2_sol/llm_only_solsmall/cost_savings_ci/hi}{92.5}
\defres{stage2_sol/llm_only_solsmall/cost_savings_ci/lo}{92.1}
\defres{stage2_sol/llm_only_solsmall/cost_savings_cw}{92.3}
\defres{stage2_sol/llm_only_solsmall/cost_savings_cw_ci/hi}{92.5}
\defres{stage2_sol/llm_only_solsmall/cost_savings_cw_ci/lo}{92.0}
\defres{stage2_sol/llm_only_solsmall/delta}{+0.8}
\defres{stage2_sol/llm_only_solsmall/delta_ci/hi}{+1.8}
\defres{stage2_sol/llm_only_solsmall/delta_ci/lo}{-0.2}
\defres{stage2_sol/llm_only_solsmall/delta_ci_newcombe/hi}{+2.1}
\defres{stage2_sol/llm_only_solsmall/delta_ci_newcombe/lo}{-0.3}
\defres{stage2_sol/llm_only_solsmall/latency_diff_s}{-6.35}
\defres{stage2_sol/llm_only_solsmall/latency_diff_s_ci/hi}{-5.62}
\defres{stage2_sol/llm_only_solsmall/latency_diff_s_ci/lo}{-7.14}
\defres{stage2_sol/llm_only_solsmall/losses}{1}
\defres{stage2_sol/llm_only_solsmall/n_dropped}{0}
\defres{stage2_sol/llm_only_solsmall/n_pairs}{500}
\defres{stage2_sol/llm_only_solsmall/success_arm}{99.8}
\defres{stage2_sol/llm_only_solsmall/success_ref}{99.0}
\defres{stage2_sol/llm_only_solsmall/wall_diff_s}{-6.35}
\defres{stage2_sol/llm_only_solsmall/wins}{5}
\defres{stage2_sol/n}{500}
\defres{stage2_sol/predicted_500}{23.33}
\defres{stage2_sol/spend}{14.89}
\defres{stage2_sol/status}{complete}
\makeatother

